Interpretable Neural Networks with Frank-Wolfe: Sparse Relevance Maps and Relevance Orderings

We study the effects of constrained optimization formulations and Frank-Wolfe algorithms for obtaining interpretable neural network predictions. Reformulating the Rate-Distortion Explanations (RDE) method for relevance attribution as a constrained optimization problem provides precise control over the sparsity of relevance maps. This enables a novel multi-rate as well as a relevance-ordering variant of RDE that both empirically outperform standard RDE and other baseline methods in a well-established comparison test. We showcase several deterministic and stochastic variants of the Frank-Wolfe algorithm and their effectiveness for RDE.

==> img/mnist/mnist_rate_accuracy_afw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.0800390625
0.636942675159236 0.08
1.27388535031847 0.08
1.91082802547771 0.0800390625
2.54777070063694 0.0801953125
3.18471337579618 0.0801953125
3.82165605095541 0.08015625
4.45859872611465 0.0807421875
5.09554140127389 0.0812890625
5.73248407643312 0.081484375
6.36942675159236 0.0828125
7.00636942675159 0.08421875
7.64331210191083 0.0865625
8.28025477707006 0.0915234375
8.9171974522293 0.09453125
9.55414012738853 0.099375
10.1910828025478 0.105859375
10.828025477707 0.1126171875
11.4649681528662 0.12890625
12.1019108280255 0.141796875
12.7388535031847 0.163046875
13.3757961783439 0.1765625
14.0127388535032 0.194453125
14.6496815286624 0.210703125
15.2866242038217 0.229765625
15.9235668789809 0.2376171875
16.5605095541401 0.2627734375
17.1974522292994 0.2853515625
17.8343949044586 0.2970703125
18.4713375796178 0.3216796875
19.1082802547771 0.343203125
19.7452229299363 0.3616015625
20.3821656050955 0.3821875
21.0191082802548 0.402265625
21.656050955414 0.4203125
22.2929936305732 0.439921875
22.9299363057325 0.462734375
23.5668789808917 0.4715625
24.203821656051 0.494453125
24.8407643312102 0.5161328125
25.4777070063694 0.5325390625
26.1146496815287 0.538984375
26.7515923566879 0.562578125
27.3885350318471 0.5776171875
28.0254777070064 0.5883984375
28.6624203821656 0.6056640625
29.2993630573248 0.6172265625
29.9363057324841 0.631015625
30.5732484076433 0.651484375
31.2101910828025 0.6636328125
31.8471337579618 0.671171875
32.484076433121 0.6841796875
33.1210191082803 0.700390625
33.7579617834395 0.726796875
34.3949044585987 0.7437890625
35.031847133758 0.76453125
35.6687898089172 0.771796875
36.3057324840764 0.7730859375
36.9426751592357 0.7831640625
37.5796178343949 0.790625
38.2165605095541 0.80390625
38.8535031847134 0.812109375
39.4904458598726 0.8151953125
40.1273885350318 0.824765625
40.7643312101911 0.83484375
41.4012738853503 0.8398828125
42.0382165605096 0.8394140625
42.6751592356688 0.8509765625
43.312101910828 0.8517578125
43.9490445859873 0.856328125
44.5859872611465 0.8596484375
45.2229299363057 0.8577734375
45.859872611465 0.8601171875
46.4968152866242 0.86328125
47.1337579617834 0.8659375
47.7707006369427 0.868828125
48.4076433121019 0.8691015625
49.0445859872611 0.8758984375
49.6815286624204 0.88140625
50.3184713375796 0.87953125
50.9554140127388 0.8826953125
51.5923566878981 0.8790234375
52.2292993630573 0.885859375
52.8662420382166 0.8878125
53.5031847133758 0.888125
54.140127388535 0.89453125
54.7770700636943 0.894375
55.4140127388535 0.901640625
56.0509554140127 0.896875
56.687898089172 0.8993359375
57.3248407643312 0.9051953125
57.9617834394904 0.90640625
58.5987261146497 0.9101953125
59.2356687898089 0.9244921875
59.8726114649682 0.92578125
60.5095541401274 0.9262109375
61.1464968152866 0.92515625
61.7834394904459 0.9359765625
62.4203821656051 0.941328125
63.0573248407643 0.946015625
63.6942675159236 0.953984375
64.3312101910828 0.9560546875
64.968152866242 0.957265625
65.6050955414013 0.9564453125
66.2420382165605 0.9552734375
66.8789808917197 0.95390625
67.515923566879 0.955703125
68.1528662420382 0.9573828125
68.7898089171974 0.9566015625
69.4267515923567 0.9549609375
70.0636942675159 0.95125
70.7006369426752 0.9532421875
71.3375796178344 0.9562890625
71.9745222929936 0.9584375
72.6114649681529 0.9615234375
73.2484076433121 0.961015625
73.8853503184713 0.9623046875
74.5222929936306 0.96109375
75.1592356687898 0.9608984375
75.796178343949 0.9598828125
76.4331210191083 0.9595703125
77.0700636942675 0.9593359375
77.7070063694268 0.9601171875
78.343949044586 0.958125
78.9808917197452 0.9589453125
79.6178343949044 0.9578125
80.2547770700637 0.959609375
80.8917197452229 0.9621875
81.5286624203822 0.9621875
82.1656050955414 0.9640234375
82.8025477707006 0.964765625
83.4394904458599 0.9632421875
84.0764331210191 0.96734375
84.7133757961783 0.9653125
85.3503184713376 0.9737109375
85.9872611464968 0.9730859375
86.6242038216561 0.9792578125
87.2611464968153 0.9849609375
87.8980891719745 0.9846875
88.5350318471338 0.983515625
89.171974522293 0.98796875
89.8089171974522 0.9884375
90.4458598726115 0.99109375
91.0828025477707 0.99375
91.7197452229299 0.99046875
92.3566878980892 0.9995703125
92.9936305732484 0.999921875
93.6305732484076 1
94.2675159235669 1
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color3, fill opacity=0.25]
(axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.08)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0794660509262088)
--(axis cs:3.18471337579618,0.0794660509262088)
--(axis cs:3.82165605095541,0.0792858621352551)
--(axis cs:4.45859872611465,0.0795442180368752)
--(axis cs:5.09554140127389,0.0797168177256575)
--(axis cs:5.73248407643312,0.0797961818564482)
--(axis cs:6.36942675159236,0.0805070186624383)
--(axis cs:7.00636942675159,0.0813066118063968)
--(axis cs:7.64331210191083,0.0830907207347702)
--(axis cs:8.28025477707006,0.0869226820767843)
--(axis cs:8.9171974522293,0.0894843253028884)
--(axis cs:9.55414012738853,0.0936485620696956)
--(axis cs:10.1910828025478,0.0992842595694344)
--(axis cs:10.828025477707,0.105418132864576)
--(axis cs:11.4649681528662,0.120510705070937)
--(axis cs:12.1019108280255,0.132704824416344)
--(axis cs:12.7388535031847,0.153413121822403)
--(axis cs:13.3757961783439,0.166304816079056)
--(axis cs:14.0127388535032,0.183683243816362)
--(axis cs:14.6496815286624,0.199849131428738)
--(axis cs:15.2866242038217,0.218719145246398)
--(axis cs:15.9235668789809,0.226304535745616)
--(axis cs:16.5605095541401,0.250943161458296)
--(axis cs:17.1974522292994,0.272807194058734)
--(axis cs:17.8343949044586,0.284152683452854)
--(axis cs:18.4713375796178,0.308812683245743)
--(axis cs:19.1082802547771,0.330126824582584)
--(axis cs:19.7452229299363,0.348539109307697)
--(axis cs:20.3821656050955,0.369335959762082)
--(axis cs:21.0191082802548,0.389525518946378)
--(axis cs:21.656050955414,0.407553214817517)
--(axis cs:22.2929936305732,0.427399555106244)
--(axis cs:22.9299363057325,0.449953898931305)
--(axis cs:23.5668789808917,0.458404894411604)
--(axis cs:24.203821656051,0.481440990810791)
--(axis cs:24.8407643312102,0.503584964063124)
--(axis cs:25.4777070063694,0.520173243441115)
--(axis cs:26.1146496815287,0.526538817231511)
--(axis cs:26.7515923566879,0.550021592660891)
--(axis cs:27.3885350318471,0.565117479566172)
--(axis cs:28.0254777070064,0.57570999918494)
--(axis cs:28.6624203821656,0.593118613137638)
--(axis cs:29.2993630573248,0.604989910206138)
--(axis cs:29.9363057324841,0.618902731145406)
--(axis cs:30.5732484076433,0.639544787624371)
--(axis cs:31.2101910828025,0.651693930291512)
--(axis cs:31.8471337579618,0.659355645299291)
--(axis cs:32.484076433121,0.672074183190525)
--(axis cs:33.1210191082803,0.688129003898861)
--(axis cs:33.7579617834395,0.714405577765633)
--(axis cs:34.3949044585987,0.731367527948402)
--(axis cs:35.031847133758,0.752604611889572)
--(axis cs:35.6687898089172,0.760084509999535)
--(axis cs:36.3057324840764,0.761820487723476)
--(axis cs:36.9426751592357,0.772142235357844)
--(axis cs:37.5796178343949,0.779851162459378)
--(axis cs:38.2165605095541,0.793509456199823)
--(axis cs:38.8535031847134,0.801982820347649)
--(axis cs:39.4904458598726,0.805031707199258)
--(axis cs:40.1273885350318,0.81512041709681)
--(axis cs:40.7643312101911,0.825476907464431)
--(axis cs:41.4012738853503,0.830680726775478)
--(axis cs:42.0382165605096,0.829946291895489)
--(axis cs:42.6751592356688,0.841698777058726)
--(axis cs:43.312101910828,0.84246805319099)
--(axis cs:43.9490445859873,0.847497453634829)
--(axis cs:44.5859872611465,0.851031613548664)
--(axis cs:45.2229299363057,0.849168519427741)
--(axis cs:45.859872611465,0.851846448623402)
--(axis cs:46.4968152866242,0.854855073120181)
--(axis cs:47.1337579617834,0.857337388745739)
--(axis cs:47.7707006369427,0.86077731256616)
--(axis cs:48.4076433121019,0.860564674884759)
--(axis cs:49.0445859872611,0.867560052217532)
--(axis cs:49.6815286624204,0.873462370244928)
--(axis cs:50.3184713375796,0.87199080168658)
--(axis cs:50.9554140127388,0.875060412142916)
--(axis cs:51.5923566878981,0.871096091404715)
--(axis cs:52.2292993630573,0.878002445669722)
--(axis cs:52.8662420382166,0.880022175790631)
--(axis cs:53.5031847133758,0.880010693324263)
--(axis cs:54.140127388535,0.886300361024842)
--(axis cs:54.7770700636943,0.885798954560863)
--(axis cs:55.4140127388535,0.892980874091288)
--(axis cs:56.0509554140127,0.888175351054599)
--(axis cs:56.687898089172,0.890808777877971)
--(axis cs:57.3248407643312,0.896988764069428)
--(axis cs:57.9617834394904,0.897890727892456)
--(axis cs:58.5987261146497,0.901721355293647)
--(axis cs:59.2356687898089,0.916598276879019)
--(axis cs:59.8726114649682,0.91803146741003)
--(axis cs:60.5095541401274,0.918570847340836)
--(axis cs:61.1464968152866,0.917654336537628)
--(axis cs:61.7834394904459,0.928880265495694)
--(axis cs:62.4203821656051,0.934437215313553)
--(axis cs:63.0573248407643,0.939506724216192)
--(axis cs:63.6942675159236,0.948088391542942)
--(axis cs:64.3312101910828,0.95043957254288)
--(axis cs:64.968152866242,0.95170417336903)
--(axis cs:65.6050955414013,0.95123253852686)
--(axis cs:66.2420382165605,0.949931260703031)
--(axis cs:66.8789808917197,0.948322096889573)
--(axis cs:67.515923566879,0.950520467467579)
--(axis cs:68.1528662420382,0.952619707742676)
--(axis cs:68.7898089171974,0.951824213285285)
--(axis cs:69.4267515923567,0.950060836879634)
--(axis cs:70.0636942675159,0.945950461098198)
--(axis cs:70.7006369426752,0.947917780475769)
--(axis cs:71.3375796178344,0.95121823468351)
--(axis cs:71.9745222929936,0.953437532186612)
--(axis cs:72.6114649681529,0.957373280251276)
--(axis cs:73.2484076433121,0.957757285035019)
--(axis cs:73.8853503184713,0.959338831052978)
--(axis cs:74.5222929936306,0.95844164779482)
--(axis cs:75.1592356687898,0.958474888303516)
--(axis cs:75.796178343949,0.957427924188563)
--(axis cs:76.4331210191083,0.95703603755711)
--(axis cs:77.0700636942675,0.956823630821492)
--(axis cs:77.7070063694268,0.956952928148907)
--(axis cs:78.343949044586,0.95456787025593)
--(axis cs:78.9808917197452,0.95609693836109)
--(axis cs:79.6178343949044,0.954725544771386)
--(axis cs:80.2547770700637,0.95681367167715)
--(axis cs:80.8917197452229,0.958989211221117)
--(axis cs:81.5286624203822,0.959148856302204)
--(axis cs:82.1656050955414,0.961092554971918)
--(axis cs:82.8025477707006,0.961378443273315)
--(axis cs:83.4394904458599,0.960236108461986)
--(axis cs:84.0764331210191,0.963498748300798)
--(axis cs:84.7133757961783,0.961095222447535)
--(axis cs:85.3503184713376,0.970085860253203)
--(axis cs:85.9872611464968,0.969433015267392)
--(axis cs:86.6242038216561,0.976299854620281)
--(axis cs:87.2611464968153,0.981587310681834)
--(axis cs:87.8980891719745,0.981717601797391)
--(axis cs:88.5350318471338,0.98113666282682)
--(axis cs:89.171974522293,0.984893983223308)
--(axis cs:89.8089171974522,0.98533667377592)
--(axis cs:90.4458598726115,0.987987498256139)
--(axis cs:91.0828025477707,0.990853047465978)
--(axis cs:91.7197452229299,0.987347185115542)
--(axis cs:92.3566878980892,0.998664109987648)
--(axis cs:92.9936305732484,0.99953201368597)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1.00031173631403)
--(axis cs:92.3566878980892,1.00047651501235)
--(axis cs:91.7197452229299,0.993590314884458)
--(axis cs:91.0828025477707,0.996646952534022)
--(axis cs:90.4458598726115,0.994200001743861)
--(axis cs:89.8089171974522,0.99153832622408)
--(axis cs:89.171974522293,0.991043516776692)
--(axis cs:88.5350318471338,0.98589458717318)
--(axis cs:87.8980891719745,0.987657398202609)
--(axis cs:87.2611464968153,0.988334564318166)
--(axis cs:86.6242038216561,0.982215770379719)
--(axis cs:85.9872611464968,0.976738859732608)
--(axis cs:85.3503184713376,0.977336014746797)
--(axis cs:84.7133757961783,0.969529777552465)
--(axis cs:84.0764331210191,0.971188751699202)
--(axis cs:83.4394904458599,0.966248266538014)
--(axis cs:82.8025477707006,0.968152806726685)
--(axis cs:82.1656050955414,0.966954320028082)
--(axis cs:81.5286624203822,0.965226143697796)
--(axis cs:80.8917197452229,0.965385788778883)
--(axis cs:80.2547770700637,0.96240507832285)
--(axis cs:79.6178343949044,0.960899455228614)
--(axis cs:78.9808917197452,0.961793686638911)
--(axis cs:78.343949044586,0.96168212974407)
--(axis cs:77.7070063694268,0.963281446851093)
--(axis cs:77.0700636942675,0.961848244178508)
--(axis cs:76.4331210191083,0.96210458744289)
--(axis cs:75.796178343949,0.962337700811437)
--(axis cs:75.1592356687898,0.963321986696484)
--(axis cs:74.5222929936306,0.96374585220518)
--(axis cs:73.8853503184713,0.965270543947022)
--(axis cs:73.2484076433121,0.964273964964981)
--(axis cs:72.6114649681529,0.965673594748724)
--(axis cs:71.9745222929936,0.963437467813388)
--(axis cs:71.3375796178344,0.96135989031649)
--(axis cs:70.7006369426752,0.958566594524231)
--(axis cs:70.0636942675159,0.956549538901802)
--(axis cs:69.4267515923567,0.959861038120365)
--(axis cs:68.7898089171974,0.961378911714714)
--(axis cs:68.1528662420382,0.962145917257324)
--(axis cs:67.515923566879,0.960885782532421)
--(axis cs:66.8789808917197,0.959490403110427)
--(axis cs:66.2420382165605,0.960615614296969)
--(axis cs:65.6050955414013,0.96165808647314)
--(axis cs:64.968152866242,0.96282707663097)
--(axis cs:64.3312101910828,0.96166980245712)
--(axis cs:63.6942675159236,0.959880358457058)
--(axis cs:63.0573248407643,0.952524525783808)
--(axis cs:62.4203821656051,0.948219034686447)
--(axis cs:61.7834394904459,0.943072859504306)
--(axis cs:61.1464968152866,0.932658163462372)
--(axis cs:60.5095541401274,0.933851027659164)
--(axis cs:59.8726114649682,0.93353103258997)
--(axis cs:59.2356687898089,0.932386098120981)
--(axis cs:58.5987261146497,0.918669269706352)
--(axis cs:57.9617834394904,0.914921772107544)
--(axis cs:57.3248407643312,0.913401860930572)
--(axis cs:56.687898089172,0.907863097122029)
--(axis cs:56.0509554140127,0.905574648945401)
--(axis cs:55.4140127388535,0.910300375908712)
--(axis cs:54.7770700636943,0.902951045439137)
--(axis cs:54.140127388535,0.902762138975158)
--(axis cs:53.5031847133758,0.896239306675737)
--(axis cs:52.8662420382166,0.895602824209369)
--(axis cs:52.2292993630573,0.893716304330278)
--(axis cs:51.5923566878981,0.886950783595285)
--(axis cs:50.9554140127388,0.890330212857084)
--(axis cs:50.3184713375796,0.88707169831342)
--(axis cs:49.6815286624204,0.889350129755072)
--(axis cs:49.0445859872611,0.884236822782468)
--(axis cs:48.4076433121019,0.877638450115241)
--(axis cs:47.7707006369427,0.87687893743384)
--(axis cs:47.1337579617834,0.874537611254261)
--(axis cs:46.4968152866242,0.871707426879819)
--(axis cs:45.859872611465,0.868387926376598)
--(axis cs:45.2229299363057,0.866378355572259)
--(axis cs:44.5859872611465,0.868265261451336)
--(axis cs:43.9490445859873,0.865158796365171)
--(axis cs:43.312101910828,0.86104757180901)
--(axis cs:42.6751592356688,0.860254347941274)
--(axis cs:42.0382165605096,0.848881833104511)
--(axis cs:41.4012738853503,0.849084898224521)
--(axis cs:40.7643312101911,0.844210592535569)
--(axis cs:40.1273885350318,0.83441083290319)
--(axis cs:39.4904458598726,0.825358917800742)
--(axis cs:38.8535031847134,0.822235929652351)
--(axis cs:38.2165605095541,0.814303043800177)
--(axis cs:37.5796178343949,0.801398837540622)
--(axis cs:36.9426751592357,0.794185889642156)
--(axis cs:36.3057324840764,0.784351387276524)
--(axis cs:35.6687898089172,0.783509240000465)
--(axis cs:35.031847133758,0.776457888110428)
--(axis cs:34.3949044585987,0.756210597051598)
--(axis cs:33.7579617834395,0.739188172234367)
--(axis cs:33.1210191082803,0.712652246101139)
--(axis cs:32.484076433121,0.696285191809475)
--(axis cs:31.8471337579618,0.682988104700708)
--(axis cs:31.2101910828025,0.675571694708487)
--(axis cs:30.5732484076433,0.663423962375629)
--(axis cs:29.9363057324841,0.643128518854594)
--(axis cs:29.2993630573248,0.629463214793862)
--(axis cs:28.6624203821656,0.618209511862362)
--(axis cs:28.0254777070064,0.60108687581506)
--(axis cs:27.3885350318471,0.590116895433829)
--(axis cs:26.7515923566879,0.575134657339109)
--(axis cs:26.1146496815287,0.551429932768489)
--(axis cs:25.4777070063694,0.544904881558885)
--(axis cs:24.8407643312102,0.528680660936876)
--(axis cs:24.203821656051,0.507465259189209)
--(axis cs:23.5668789808917,0.484720105588396)
--(axis cs:22.9299363057325,0.475514851068695)
--(axis cs:22.2929936305732,0.452444194893756)
--(axis cs:21.656050955414,0.433071785182483)
--(axis cs:21.0191082802548,0.415005731053622)
--(axis cs:20.3821656050955,0.395039040237918)
--(axis cs:19.7452229299363,0.374664015692303)
--(axis cs:19.1082802547771,0.356279425417416)
--(axis cs:18.4713375796178,0.334546691754257)
--(axis cs:17.8343949044586,0.309987941547146)
--(axis cs:17.1974522292994,0.297895930941266)
--(axis cs:16.5605095541401,0.274603713541704)
--(axis cs:15.9235668789809,0.248929839254384)
--(axis cs:15.2866242038217,0.240812104753602)
--(axis cs:14.6496815286624,0.221557118571262)
--(axis cs:14.0127388535032,0.205223006183638)
--(axis cs:13.3757961783439,0.186820183920944)
--(axis cs:12.7388535031847,0.172680628177597)
--(axis cs:12.1019108280255,0.150888925583656)
--(axis cs:11.4649681528662,0.137301794929063)
--(axis cs:10.828025477707,0.119816242135424)
--(axis cs:10.1910828025478,0.112434490430566)
--(axis cs:9.55414012738853,0.105101437930304)
--(axis cs:8.9171974522293,0.0995781746971116)
--(axis cs:8.28025477707006,0.0961241929232157)
--(axis cs:7.64331210191083,0.0900342792652298)
--(axis cs:7.00636942675159,0.0871308881936032)
--(axis cs:6.36942675159236,0.0851179813375617)
--(axis cs:5.73248407643312,0.0831725681435518)
--(axis cs:5.09554140127389,0.0828613072743425)
--(axis cs:4.45859872611465,0.0819401569631248)
--(axis cs:3.82165605095541,0.0810266378647449)
--(axis cs:3.18471337579618,0.0809245740737912)
--(axis cs:2.54777070063694,0.0809245740737912)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.08)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_afw_order.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.080078125
0.636942675159236 0.08
1.27388535031847 0.08
1.91082802547771 0.0800390625
2.54777070063694 0.08015625
3.18471337579618 0.080078125
3.82165605095541 0.080390625
4.45859872611465 0.0807421875
5.09554140127389 0.08078125
5.73248407643312 0.082421875
6.36942675159236 0.0844921875
7.00636942675159 0.0888671875
7.64331210191083 0.095546875
8.28025477707006 0.1023828125
8.9171974522293 0.1132421875
9.55414012738853 0.123359375
10.1910828025478 0.1333984375
10.828025477707 0.14484375
11.4649681528662 0.162578125
12.1019108280255 0.17828125
12.7388535031847 0.1987109375
13.3757961783439 0.210625
14.0127388535032 0.225234375
14.6496815286624 0.240703125
15.2866242038217 0.255703125
15.9235668789809 0.2651171875
16.5605095541401 0.2774609375
17.1974522292994 0.2872265625
17.8343949044586 0.303515625
18.4713375796178 0.32265625
19.1082802547771 0.3329296875
19.7452229299363 0.350390625
20.3821656050955 0.3656640625
21.0191082802548 0.378671875
21.656050955414 0.39859375
22.2929936305732 0.4127734375
22.9299363057325 0.42828125
23.5668789808917 0.447734375
24.203821656051 0.46296875
24.8407643312102 0.472109375
25.4777070063694 0.48265625
26.1146496815287 0.4969140625
26.7515923566879 0.5059765625
27.3885350318471 0.51609375
28.0254777070064 0.5414453125
28.6624203821656 0.5482421875
29.2993630573248 0.55046875
29.9363057324841 0.5585546875
30.5732484076433 0.56578125
31.2101910828025 0.579140625
31.8471337579618 0.5837109375
32.484076433121 0.5946484375
33.1210191082803 0.6078515625
33.7579617834395 0.6116015625
34.3949044585987 0.617890625
35.031847133758 0.6356640625
35.6687898089172 0.646640625
36.3057324840764 0.6619140625
36.9426751592357 0.6625
37.5796178343949 0.6726953125
38.2165605095541 0.6791796875
38.8535031847134 0.688984375
39.4904458598726 0.6912109375
40.1273885350318 0.7026171875
40.7643312101911 0.70609375
41.4012738853503 0.714140625
42.0382165605096 0.715
42.6751592356688 0.7162890625
43.312101910828 0.7175
43.9490445859873 0.72609375
44.5859872611465 0.7310546875
45.2229299363057 0.730859375
45.859872611465 0.73625
46.4968152866242 0.7418359375
47.1337579617834 0.7388671875
47.7707006369427 0.73828125
48.4076433121019 0.740859375
49.0445859872611 0.7486328125
49.6815286624204 0.7526171875
50.3184713375796 0.7546484375
50.9554140127388 0.76
51.5923566878981 0.7592578125
52.2292993630573 0.7627734375
52.8662420382166 0.772578125
53.5031847133758 0.773203125
54.140127388535 0.7803125
54.7770700636943 0.7884765625
55.4140127388535 0.795234375
56.0509554140127 0.803671875
56.687898089172 0.814140625
57.3248407643312 0.81875
57.9617834394904 0.82375
58.5987261146497 0.828203125
59.2356687898089 0.8357421875
59.8726114649682 0.845390625
60.5095541401274 0.847734375
61.1464968152866 0.85578125
61.7834394904459 0.8598828125
62.4203821656051 0.865703125
63.0573248407643 0.8733203125
63.6942675159236 0.876640625
64.3312101910828 0.8865234375
64.968152866242 0.8777734375
65.6050955414013 0.8751953125
66.2420382165605 0.8828515625
66.8789808917197 0.8903515625
67.515923566879 0.8953515625
68.1528662420382 0.903046875
68.7898089171974 0.9078125
69.4267515923567 0.9165234375
70.0636942675159 0.92609375
70.7006369426752 0.93203125
71.3375796178344 0.9358203125
71.9745222929936 0.94328125
72.6114649681529 0.9456640625
73.2484076433121 0.9449609375
73.8853503184713 0.9501171875
74.5222929936306 0.954921875
75.1592356687898 0.9556640625
75.796178343949 0.95515625
76.4331210191083 0.9551171875
77.0700636942675 0.95765625
77.7070063694268 0.9564453125
78.343949044586 0.9586328125
78.9808917197452 0.9601171875
79.6178343949044 0.960859375
80.2547770700637 0.9608984375
80.8917197452229 0.960625
81.5286624203822 0.964453125
82.1656050955414 0.9650390625
82.8025477707006 0.964609375
83.4394904458599 0.96515625
84.0764331210191 0.970546875
84.7133757961783 0.9699609375
85.3503184713376 0.9689453125
85.9872611464968 0.9711328125
86.6242038216561 0.9735546875
87.2611464968153 0.9748828125
87.8980891719745 0.9790234375
88.5350318471338 0.9782421875
89.171974522293 0.9783203125
89.8089171974522 0.98125
90.4458598726115 0.9833203125
91.0828025477707 0.9871484375
91.7197452229299 0.9825
92.3566878980892 0.9825
92.9936305732484 0.989375
93.6305732484076 0.995625
94.2675159235669 0.9931640625
94.9044585987261 0.99515625
95.5414012738853 0.998203125
96.1783439490446 0.9999609375
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color3, fill opacity=0.25]
(axis cs:0,0.0804683683438268)
--(axis cs:0,0.0796878816561732)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.08)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0794816527402516)
--(axis cs:3.18471337579618,0.079298593503853)
--(axis cs:3.82165605095541,0.0792895534879121)
--(axis cs:4.45859872611465,0.0794233195967747)
--(axis cs:5.09554140127389,0.0793248739207086)
--(axis cs:5.73248407643312,0.0801411520116587)
--(axis cs:6.36942675159236,0.0815978852026673)
--(axis cs:7.00636942675159,0.0848423273324081)
--(axis cs:7.64331210191083,0.0903657990672381)
--(axis cs:8.28025477707006,0.0963792982260419)
--(axis cs:8.9171974522293,0.106164309087)
--(axis cs:9.55414012738853,0.115517936895271)
--(axis cs:10.1910828025478,0.124853472028571)
--(axis cs:10.828025477707,0.135786544109953)
--(axis cs:11.4649681528662,0.152879471585253)
--(axis cs:12.1019108280255,0.168392092965877)
--(axis cs:12.7388535031847,0.188626828750234)
--(axis cs:13.3757961783439,0.200542524227112)
--(axis cs:14.0127388535032,0.214863512289606)
--(axis cs:14.6496815286624,0.230195175228519)
--(axis cs:15.2866242038217,0.244884967674301)
--(axis cs:15.9235668789809,0.254045881220399)
--(axis cs:16.5605095541401,0.266158538301255)
--(axis cs:17.1974522292994,0.275686655983254)
--(axis cs:17.8343949044586,0.291553843024107)
--(axis cs:18.4713375796178,0.310646218519165)
--(axis cs:19.1082802547771,0.320707547192294)
--(axis cs:19.7452229299363,0.337975048006325)
--(axis cs:20.3821656050955,0.353249703767925)
--(axis cs:21.0191082802548,0.366087355254906)
--(axis cs:21.656050955414,0.38613441884221)
--(axis cs:22.2929936305732,0.400082721074971)
--(axis cs:22.9299363057325,0.415896809200642)
--(axis cs:23.5668789808917,0.435051063928444)
--(axis cs:24.203821656051,0.450404328412559)
--(axis cs:24.8407643312102,0.459865108060431)
--(axis cs:25.4777070063694,0.47064886155688)
--(axis cs:26.1146496815287,0.485099667807049)
--(axis cs:26.7515923566879,0.49419705564205)
--(axis cs:27.3885350318471,0.504184541283925)
--(axis cs:28.0254777070064,0.530117180922938)
--(axis cs:28.6624203821656,0.536759172636895)
--(axis cs:29.2993630573248,0.538865531756968)
--(axis cs:29.9363057324841,0.546846133535118)
--(axis cs:30.5732484076433,0.554188670029775)
--(axis cs:31.2101910828025,0.567407248406147)
--(axis cs:31.8471337579618,0.571719202056359)
--(axis cs:32.484076433121,0.582702979508482)
--(axis cs:33.1210191082803,0.596006596298057)
--(axis cs:33.7579617834395,0.599528166785102)
--(axis cs:34.3949044585987,0.606077220446792)
--(axis cs:35.031847133758,0.623562448589121)
--(axis cs:35.6687898089172,0.634626326179025)
--(axis cs:36.3057324840764,0.65043905705263)
--(axis cs:36.9426751592357,0.65102902733827)
--(axis cs:37.5796178343949,0.661459623803559)
--(axis cs:38.2165605095541,0.668144308446922)
--(axis cs:38.8535031847134,0.678060684747882)
--(axis cs:39.4904458598726,0.680737382937993)
--(axis cs:40.1273885350318,0.692643041952776)
--(axis cs:40.7643312101911,0.696373794532297)
--(axis cs:41.4012738853503,0.704642079916483)
--(axis cs:42.0382165605096,0.705917870306733)
--(axis cs:42.6751592356688,0.707001565165154)
--(axis cs:43.312101910828,0.708244155899901)
--(axis cs:43.9490445859873,0.716856277210859)
--(axis cs:44.5859872611465,0.721725536243144)
--(axis cs:45.2229299363057,0.721649430811427)
--(axis cs:45.859872611465,0.727124658303584)
--(axis cs:46.4968152866242,0.732987894230901)
--(axis cs:47.1337579617834,0.72989501953125)
--(axis cs:47.7707006369427,0.72916133128512)
--(axis cs:48.4076433121019,0.731877372059697)
--(axis cs:49.0445859872611,0.739483375884031)
--(axis cs:49.6815286624204,0.743321655434544)
--(axis cs:50.3184713375796,0.745394179306185)
--(axis cs:50.9554140127388,0.750735852441327)
--(axis cs:51.5923566878981,0.750116408617649)
--(axis cs:52.2292993630573,0.753641737706311)
--(axis cs:52.8662420382166,0.763521083634164)
--(axis cs:53.5031847133758,0.763946009151096)
--(axis cs:54.140127388535,0.77103143064116)
--(axis cs:54.7770700636943,0.779115011006566)
--(axis cs:55.4140127388535,0.785649142315325)
--(axis cs:56.0509554140127,0.794054221640992)
--(axis cs:56.687898089172,0.804607160231467)
--(axis cs:57.3248407643312,0.809108423363467)
--(axis cs:57.9617834394904,0.814426512780058)
--(axis cs:58.5987261146497,0.818974803139435)
--(axis cs:59.2356687898089,0.826616364098166)
--(axis cs:59.8726114649682,0.83680803156156)
--(axis cs:60.5095541401274,0.838962571878052)
--(axis cs:61.1464968152866,0.847115616166085)
--(axis cs:61.7834394904459,0.85158378170743)
--(axis cs:62.4203821656051,0.858147199446179)
--(axis cs:63.0573248407643,0.866063286321919)
--(axis cs:63.6942675159236,0.869582427060744)
--(axis cs:64.3312101910828,0.879848468059795)
--(axis cs:64.968152866242,0.870823175826985)
--(axis cs:65.6050955414013,0.867968286065225)
--(axis cs:66.2420382165605,0.875641566527099)
--(axis cs:66.8789808917197,0.882959229890373)
--(axis cs:67.515923566879,0.887852718521837)
--(axis cs:68.1528662420382,0.895874581874827)
--(axis cs:68.7898089171974,0.900153232312808)
--(axis cs:69.4267515923567,0.908925474903625)
--(axis cs:70.0636942675159,0.918893422502443)
--(axis cs:70.7006369426752,0.925212248938101)
--(axis cs:71.3375796178344,0.929437459079682)
--(axis cs:71.9745222929936,0.937430095080729)
--(axis cs:72.6114649681529,0.940298478611796)
--(axis cs:73.2484076433121,0.939598853993084)
--(axis cs:73.8853503184713,0.945416909785055)
--(axis cs:74.5222929936306,0.951051610764153)
--(axis cs:75.1592356687898,0.951778140509145)
--(axis cs:75.796178343949,0.95153497703362)
--(axis cs:76.4331210191083,0.951704519840489)
--(axis cs:77.0700636942675,0.954375032697568)
--(axis cs:77.7070063694268,0.952894954593325)
--(axis cs:78.343949044586,0.955647825174087)
--(axis cs:78.9808917197452,0.957159834200256)
--(axis cs:79.6178343949044,0.95821633425728)
--(axis cs:80.2547770700637,0.9587209617871)
--(axis cs:80.8917197452229,0.958220307792485)
--(axis cs:81.5286624203822,0.961477863025179)
--(axis cs:82.1656050955414,0.961843826891791)
--(axis cs:82.8025477707006,0.961521502751231)
--(axis cs:83.4394904458599,0.962019874296978)
--(axis cs:84.0764331210191,0.967107003769734)
--(axis cs:84.7133757961783,0.966374624733209)
--(axis cs:85.3503184713376,0.965340722717102)
--(axis cs:85.9872611464968,0.967596837765514)
--(axis cs:86.6242038216561,0.969956883767963)
--(axis cs:87.2611464968153,0.971832202364241)
--(axis cs:87.8980891719745,0.976493929720801)
--(axis cs:88.5350318471338,0.975991686294007)
--(axis cs:89.171974522293,0.975705869604997)
--(axis cs:89.8089171974522,0.978788171354306)
--(axis cs:90.4458598726115,0.980862997389848)
--(axis cs:91.0828025477707,0.983941285408615)
--(axis cs:91.7197452229299,0.979257843753092)
--(axis cs:92.3566878980892,0.9797112343142)
--(axis cs:92.9936305732484,0.98625610948776)
--(axis cs:93.6305732484076,0.993034864715368)
--(axis cs:94.2675159235669,0.99019961317271)
--(axis cs:94.9044585987261,0.992478705103349)
--(axis cs:95.5414012738853,0.99641214092453)
--(axis cs:96.1783439490446,0.999684993785267)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1.00023688121473)
--(axis cs:95.5414012738853,0.99999410907547)
--(axis cs:94.9044585987261,0.997833794896651)
--(axis cs:94.2675159235669,0.99612851182729)
--(axis cs:93.6305732484076,0.998215135284632)
--(axis cs:92.9936305732484,0.99249389051224)
--(axis cs:92.3566878980892,0.9852887656858)
--(axis cs:91.7197452229299,0.985742156246908)
--(axis cs:91.0828025477707,0.990355589591385)
--(axis cs:90.4458598726115,0.985777627610152)
--(axis cs:89.8089171974522,0.983711828645694)
--(axis cs:89.171974522293,0.980934755395003)
--(axis cs:88.5350318471338,0.980492688705993)
--(axis cs:87.8980891719745,0.981552945279199)
--(axis cs:87.2611464968153,0.977933422635759)
--(axis cs:86.6242038216561,0.977152491232037)
--(axis cs:85.9872611464968,0.974668787234486)
--(axis cs:85.3503184713376,0.972549902282898)
--(axis cs:84.7133757961783,0.973547250266791)
--(axis cs:84.0764331210191,0.973986746230266)
--(axis cs:83.4394904458599,0.968292625703022)
--(axis cs:82.8025477707006,0.967697247248769)
--(axis cs:82.1656050955414,0.968234298108209)
--(axis cs:81.5286624203822,0.967428386974821)
--(axis cs:80.8917197452229,0.963029692207515)
--(axis cs:80.2547770700637,0.9630759132129)
--(axis cs:79.6178343949044,0.96350241574272)
--(axis cs:78.9808917197452,0.963074540799744)
--(axis cs:78.343949044586,0.961617799825913)
--(axis cs:77.7070063694268,0.959995670406675)
--(axis cs:77.0700636942675,0.960937467302432)
--(axis cs:76.4331210191083,0.958529855159511)
--(axis cs:75.796178343949,0.95877752296638)
--(axis cs:75.1592356687898,0.959549984490855)
--(axis cs:74.5222929936306,0.958792139235847)
--(axis cs:73.8853503184713,0.954817465214945)
--(axis cs:73.2484076433121,0.950323021006916)
--(axis cs:72.6114649681529,0.951029646388204)
--(axis cs:71.9745222929936,0.949132404919271)
--(axis cs:71.3375796178344,0.942203165920318)
--(axis cs:70.7006369426752,0.938850251061899)
--(axis cs:70.0636942675159,0.933294077497558)
--(axis cs:69.4267515923567,0.924121400096375)
--(axis cs:68.7898089171974,0.915471767687192)
--(axis cs:68.1528662420382,0.910219168125173)
--(axis cs:67.515923566879,0.902850406478163)
--(axis cs:66.8789808917197,0.897743895109627)
--(axis cs:66.2420382165605,0.890061558472901)
--(axis cs:65.6050955414013,0.882422338934776)
--(axis cs:64.968152866242,0.884723699173015)
--(axis cs:64.3312101910828,0.893198406940204)
--(axis cs:63.6942675159236,0.883698822939256)
--(axis cs:63.0573248407643,0.880577338678081)
--(axis cs:62.4203821656051,0.873259050553821)
--(axis cs:61.7834394904459,0.86818184329257)
--(axis cs:61.1464968152866,0.864446883833915)
--(axis cs:60.5095541401274,0.856506178121948)
--(axis cs:59.8726114649682,0.85397321843844)
--(axis cs:59.2356687898089,0.844868010901834)
--(axis cs:58.5987261146497,0.837431446860565)
--(axis cs:57.9617834394904,0.833073487219942)
--(axis cs:57.3248407643312,0.828391576636533)
--(axis cs:56.687898089172,0.823674089768533)
--(axis cs:56.0509554140127,0.813289528359008)
--(axis cs:55.4140127388535,0.804819607684675)
--(axis cs:54.7770700636943,0.797838113993434)
--(axis cs:54.140127388535,0.78959356935884)
--(axis cs:53.5031847133758,0.782460240848904)
--(axis cs:52.8662420382166,0.781635166365836)
--(axis cs:52.2292993630573,0.771905137293689)
--(axis cs:51.5923566878981,0.768399216382351)
--(axis cs:50.9554140127388,0.769264147558673)
--(axis cs:50.3184713375796,0.763902695693815)
--(axis cs:49.6815286624204,0.761912719565456)
--(axis cs:49.0445859872611,0.757782249115969)
--(axis cs:48.4076433121019,0.749841377940303)
--(axis cs:47.7707006369427,0.74740116871488)
--(axis cs:47.1337579617834,0.74783935546875)
--(axis cs:46.4968152866242,0.750683980769099)
--(axis cs:45.859872611465,0.745375341696416)
--(axis cs:45.2229299363057,0.740069319188573)
--(axis cs:44.5859872611465,0.740383838756856)
--(axis cs:43.9490445859873,0.735331222789141)
--(axis cs:43.312101910828,0.726755844100099)
--(axis cs:42.6751592356688,0.725576559834846)
--(axis cs:42.0382165605096,0.724082129693267)
--(axis cs:41.4012738853503,0.723639170083517)
--(axis cs:40.7643312101911,0.715813705467703)
--(axis cs:40.1273885350318,0.712591333047224)
--(axis cs:39.4904458598726,0.701684492062007)
--(axis cs:38.8535031847134,0.699908065252118)
--(axis cs:38.2165605095541,0.690215066553078)
--(axis cs:37.5796178343949,0.683931001196441)
--(axis cs:36.9426751592357,0.67397097266173)
--(axis cs:36.3057324840764,0.67338906794737)
--(axis cs:35.6687898089172,0.658654923820974)
--(axis cs:35.031847133758,0.647765676410879)
--(axis cs:34.3949044585987,0.629704029553208)
--(axis cs:33.7579617834395,0.623674958214898)
--(axis cs:33.1210191082803,0.619696528701943)
--(axis cs:32.484076433121,0.606593895491518)
--(axis cs:31.8471337579618,0.595702672943641)
--(axis cs:31.2101910828025,0.590874001593853)
--(axis cs:30.5732484076433,0.577373829970225)
--(axis cs:29.9363057324841,0.570263241464882)
--(axis cs:29.2993630573248,0.562071968243032)
--(axis cs:28.6624203821656,0.559725202363105)
--(axis cs:28.0254777070064,0.552773444077062)
--(axis cs:27.3885350318471,0.528002958716075)
--(axis cs:26.7515923566879,0.51775606935795)
--(axis cs:26.1146496815287,0.508728457192951)
--(axis cs:25.4777070063694,0.49466363844312)
--(axis cs:24.8407643312102,0.484353641939569)
--(axis cs:24.203821656051,0.475533171587441)
--(axis cs:23.5668789808917,0.460417686071556)
--(axis cs:22.9299363057325,0.440665690799358)
--(axis cs:22.2929936305732,0.425464153925029)
--(axis cs:21.656050955414,0.41105308115779)
--(axis cs:21.0191082802548,0.391256394745094)
--(axis cs:20.3821656050955,0.378078421232075)
--(axis cs:19.7452229299363,0.362806201993675)
--(axis cs:19.1082802547771,0.345151827807706)
--(axis cs:18.4713375796178,0.334666281480835)
--(axis cs:17.8343949044586,0.315477406975893)
--(axis cs:17.1974522292994,0.298766469016746)
--(axis cs:16.5605095541401,0.288763336698745)
--(axis cs:15.9235668789809,0.276188493779601)
--(axis cs:15.2866242038217,0.266521282325699)
--(axis cs:14.6496815286624,0.251211074771481)
--(axis cs:14.0127388535032,0.235605237710394)
--(axis cs:13.3757961783439,0.220707475772888)
--(axis cs:12.7388535031847,0.208795046249766)
--(axis cs:12.1019108280255,0.188170407034123)
--(axis cs:11.4649681528662,0.172276778414747)
--(axis cs:10.828025477707,0.153900955890047)
--(axis cs:10.1910828025478,0.141943402971429)
--(axis cs:9.55414012738853,0.131200813104729)
--(axis cs:8.9171974522293,0.120320065913)
--(axis cs:8.28025477707006,0.108386326773958)
--(axis cs:7.64331210191083,0.100727950932762)
--(axis cs:7.00636942675159,0.0928920476675919)
--(axis cs:6.36942675159236,0.0873864897973327)
--(axis cs:5.73248407643312,0.0847025979883413)
--(axis cs:5.09554140127389,0.0822376260792914)
--(axis cs:4.45859872611465,0.0820610554032253)
--(axis cs:3.82165605095541,0.0814916965120878)
--(axis cs:3.18471337579618,0.080857656496147)
--(axis cs:2.54777070063694,0.0808308472597484)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.08)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0804683683438268)
--cycle;


==> img/mnist/mnist_rate_accuracy_deeptaylor.tex <==
% deep taylor
\addplot [line width=0.5, opacity=0.8, color5, mark=x, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color5, thin}]
table [row sep=\\]{%
0	0.08 \\
0.636942675159236	0.08 \\
1.27388535031847	0.080078125 \\
1.91082802547771	0.080078125 \\
2.54777070063694	0.0800390625 \\
3.18471337579618	0.08 \\
3.82165605095541	0.0800390625 \\
4.45859872611465	0.0801953125 \\
5.09554140127389	0.0805078125 \\
5.73248407643312	0.080234375 \\
6.36942675159236	0.080234375 \\
7.00636942675159	0.080390625 \\
7.64331210191083	0.0801953125 \\
8.28025477707006	0.08046875 \\
8.9171974522293	0.0810546875 \\
9.55414012738853	0.0816796875 \\
10.1910828025478	0.0823046875 \\
10.828025477707	0.0834375 \\
11.4649681528662	0.08390625 \\
12.1019108280255	0.0842578125 \\
12.7388535031847	0.0857421875 \\
13.3757961783439	0.0879296875 \\
14.0127388535032	0.0893359375 \\
14.6496815286624	0.09140625 \\
15.2866242038217	0.0944921875 \\
15.9235668789809	0.0969921875 \\
16.5605095541401	0.1040234375 \\
17.1974522292994	0.1086328125 \\
17.8343949044586	0.1147265625 \\
18.4713375796178	0.1140625 \\
19.1082802547771	0.1217578125 \\
19.7452229299363	0.1259375 \\
20.3821656050955	0.1351171875 \\
21.0191082802548	0.140078125 \\
21.656050955414	0.1512109375 \\
22.2929936305732	0.1575 \\
22.9299363057325	0.168359375 \\
23.5668789808917	0.178984375 \\
24.203821656051	0.1796875 \\
24.8407643312102	0.191796875 \\
25.4777070063694	0.1969921875 \\
26.1146496815287	0.202421875 \\
26.7515923566879	0.22109375 \\
27.3885350318471	0.235390625 \\
28.0254777070064	0.24015625 \\
28.6624203821656	0.252265625 \\
29.2993630573248	0.2621875 \\
29.9363057324841	0.2730859375 \\
30.5732484076433	0.285234375 \\
31.2101910828025	0.2965625 \\
31.8471337579618	0.309609375 \\
32.484076433121	0.32734375 \\
33.1210191082803	0.344453125 \\
33.7579617834395	0.367890625 \\
34.3949044585987	0.3899609375 \\
35.031847133758	0.4094140625 \\
35.6687898089172	0.42265625 \\
36.3057324840764	0.4469140625 \\
36.9426751592357	0.464921875 \\
37.5796178343949	0.475703125 \\
38.2165605095541	0.4910546875 \\
38.8535031847134	0.5129296875 \\
39.4904458598726	0.51109375 \\
40.1273885350318	0.5275 \\
40.7643312101911	0.541796875 \\
41.4012738853503	0.5603515625 \\
42.0382165605096	0.581875 \\
42.6751592356688	0.590546875 \\
43.312101910828	0.6025 \\
43.9490445859873	0.6203515625 \\
44.5859872611465	0.640859375 \\
45.2229299363057	0.6558203125 \\
45.859872611465	0.671953125 \\
46.4968152866242	0.6831640625 \\
47.1337579617834	0.6869140625 \\
47.7707006369427	0.6935546875 \\
48.4076433121019	0.7011328125 \\
49.0445859872611	0.7162109375 \\
49.6815286624204	0.7234375 \\
50.3184713375796	0.7299609375 \\
50.9554140127388	0.740234375 \\
51.5923566878981	0.7484375 \\
52.2292993630573	0.7481640625 \\
52.8662420382166	0.7487109375 \\
53.5031847133758	0.7566015625 \\
54.140127388535	0.768984375 \\
54.7770700636943	0.77703125 \\
55.4140127388535	0.7890234375 \\
56.0509554140127	0.8006640625 \\
56.687898089172	0.8053125 \\
57.3248407643312	0.8116796875 \\
57.9617834394904	0.819375 \\
58.5987261146497	0.8206640625 \\
59.2356687898089	0.8255859375 \\
59.8726114649682	0.8333984375 \\
60.5095541401274	0.8325 \\
61.1464968152866	0.8385546875 \\
61.7834394904459	0.8424609375 \\
62.4203821656051	0.847109375 \\
63.0573248407643	0.8498828125 \\
63.6942675159236	0.8482421875 \\
64.3312101910828	0.8525390625 \\
64.968152866242	0.858984375 \\
65.6050955414013	0.8675390625 \\
66.2420382165605	0.87453125 \\
66.8789808917197	0.88625 \\
67.515923566879	0.8924609375 \\
68.1528662420382	0.901640625 \\
68.7898089171974	0.901328125 \\
69.4267515923567	0.91296875 \\
70.0636942675159	0.9131640625 \\
70.7006369426752	0.9121875 \\
71.3375796178344	0.916484375 \\
71.9745222929936	0.9211328125 \\
72.6114649681529	0.9248828125 \\
73.2484076433121	0.9249609375 \\
73.8853503184713	0.9296875 \\
74.5222929936306	0.935 \\
75.1592356687898	0.9383984375 \\
75.796178343949	0.9398046875 \\
76.4331210191083	0.947578125 \\
77.0700636942675	0.955078125 \\
77.7070063694268	0.9603125 \\
78.343949044586	0.9666015625 \\
78.9808917197452	0.9708984375 \\
79.6178343949044	0.9715234375 \\
80.2547770700637	0.9753125 \\
80.8917197452229	0.9758203125 \\
81.5286624203822	0.9783203125 \\
82.1656050955414	0.979609375 \\
82.8025477707006	0.97875 \\
83.4394904458599	0.9805859375 \\
84.0764331210191	0.98265625 \\
84.7133757961783	0.9827734375 \\
85.3503184713376	0.983046875 \\
85.9872611464968	0.9906640625 \\
86.6242038216561	0.9940234375 \\
87.2611464968153	0.99546875 \\
87.8980891719745	0.998828125 \\
88.5350318471338	0.999453125 \\
89.171974522293	0.999609375 \\
89.8089171974522	0.9996484375 \\
90.4458598726115	0.9999609375 \\
91.0828025477707	1 \\
91.7197452229299	1 \\
92.3566878980892	1 \\
92.9936305732484	1 \\
93.6305732484076	1 \\
94.2675159235669	1 \\
94.9044585987261	1 \\
95.5414012738853	1 \\
96.1783439490446	1 \\
96.8152866242038	1 \\
97.4522292993631	1 \\
98.0891719745223	1 \\
98.7261146496815	1 \\
99.3630573248408	1 \\
100	1 \\
};
\path [fill=color5, fill opacity=0.5] (axis cs:0,0.0803902433438268)
--(axis cs:0,0.0796097566561732)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0796882636859699)
--(axis cs:1.91082802547771,0.0795262375705343)
--(axis cs:2.54777070063694,0.0795611139660534)
--(axis cs:3.18471337579618,0.0796097566561732)
--(axis cs:3.82165605095541,0.0795611139660534)
--(axis cs:4.45859872611465,0.0795790085175115)
--(axis cs:5.09554140127389,0.0795148322201369)
--(axis cs:5.73248407643312,0.079559336105337)
--(axis cs:6.36942675159236,0.079559336105337)
--(axis cs:7.00636942675159,0.0793591489172716)
--(axis cs:7.64331210191083,0.07946645970515)
--(axis cs:8.28025477707006,0.0795173843863087)
--(axis cs:8.9171974522293,0.0795755196602696)
--(axis cs:9.55414012738853,0.0798806096187187)
--(axis cs:10.1910828025478,0.080167689869894)
--(axis cs:10.828025477707,0.0808852085535734)
--(axis cs:11.4649681528662,0.0811793511278462)
--(axis cs:12.1019108280255,0.0813877060699924)
--(axis cs:12.7388535031847,0.0824896836389188)
--(axis cs:13.3757961783439,0.0841795452462793)
--(axis cs:14.0127388535032,0.0853381953353229)
--(axis cs:14.6496815286624,0.0871445447885255)
--(axis cs:15.2866242038217,0.0898315468054298)
--(axis cs:15.9235668789809,0.0921185541601414)
--(axis cs:16.5605095541401,0.0985227509190205)
--(axis cs:17.1974522292994,0.102858602841281)
--(axis cs:17.8343949044586,0.108809651888024)
--(axis cs:18.4713375796178,0.107835789202418)
--(axis cs:19.1082802547771,0.115104577312961)
--(axis cs:19.7452229299363,0.119011819546525)
--(axis cs:20.3821656050955,0.128320896129892)
--(axis cs:21.0191082802548,0.13289402005312)
--(axis cs:21.656050955414,0.143486587007909)
--(axis cs:22.2929936305732,0.149716890304533)
--(axis cs:22.9299363057325,0.159867895217247)
--(axis cs:23.5668789808917,0.17025954938806)
--(axis cs:24.203821656051,0.170973150126227)
--(axis cs:24.8407643312102,0.182809365860648)
--(axis cs:25.4777070063694,0.187733985168681)
--(axis cs:26.1146496815287,0.192988279986332)
--(axis cs:26.7515923566879,0.211659586353022)
--(axis cs:27.3885350318471,0.225894747223009)
--(axis cs:28.0254777070064,0.230410114663008)
--(axis cs:28.6624203821656,0.242427424223872)
--(axis cs:29.2993630573248,0.252663824871421)
--(axis cs:29.9363057324841,0.263066492806078)
--(axis cs:30.5732484076433,0.274859906474478)
--(axis cs:31.2101910828025,0.285987138013069)
--(axis cs:31.8471337579618,0.298519100679947)
--(axis cs:32.484076433121,0.316215368784699)
--(axis cs:33.1210191082803,0.332362912481013)
--(axis cs:33.7579617834395,0.35579449793793)
--(axis cs:34.3949044585987,0.377691668669001)
--(axis cs:35.031847133758,0.396902736787898)
--(axis cs:35.6687898089172,0.409980013580736)
--(axis cs:36.3057324840764,0.434271673327979)
--(axis cs:36.9426751592357,0.452163220481837)
--(axis cs:37.5796178343949,0.46306063564172)
--(axis cs:38.2165605095541,0.478402472067692)
--(axis cs:38.8535031847134,0.500968148444096)
--(axis cs:39.4904458598726,0.499047865417266)
--(axis cs:40.1273885350318,0.51583786973139)
--(axis cs:40.7643312101911,0.530225716816901)
--(axis cs:41.4012738853503,0.548956333154322)
--(axis cs:42.0382165605096,0.570719215937068)
--(axis cs:42.6751592356688,0.579802523744197)
--(axis cs:43.312101910828,0.591700950609647)
--(axis cs:43.9490445859873,0.609627986037199)
--(axis cs:44.5859872611465,0.630417517286842)
--(axis cs:45.2229299363057,0.646146958434955)
--(axis cs:45.859872611465,0.662721687254752)
--(axis cs:46.4968152866242,0.674029964266679)
--(axis cs:47.1337579617834,0.677738377246409)
--(axis cs:47.7707006369427,0.684363084774926)
--(axis cs:48.4076433121019,0.69123555963224)
--(axis cs:49.0445859872611,0.706498611942223)
--(axis cs:49.6815286624204,0.71413601452683)
--(axis cs:50.3184713375796,0.720925862274335)
--(axis cs:50.9554140127388,0.731090648557807)
--(axis cs:51.5923566878981,0.73928043637294)
--(axis cs:52.2292993630573,0.739287301077148)
--(axis cs:52.8662420382166,0.739869970361852)
--(axis cs:53.5031847133758,0.748097676310039)
--(axis cs:54.140127388535,0.760408763955092)
--(axis cs:54.7770700636943,0.768932880615191)
--(axis cs:55.4140127388535,0.781182883089094)
--(axis cs:56.0509554140127,0.793341176472163)
--(axis cs:56.687898089172,0.79823254815576)
--(axis cs:57.3248407643312,0.804732513831583)
--(axis cs:57.9617834394904,0.812434833042603)
--(axis cs:58.5987261146497,0.813681992759781)
--(axis cs:59.2356687898089,0.819267705007704)
--(axis cs:59.8726114649682,0.827548415973898)
--(axis cs:60.5095541401274,0.827009115056138)
--(axis cs:61.1464968152866,0.832299027621484)
--(axis cs:61.7834394904459,0.836096553834758)
--(axis cs:62.4203821656051,0.840462133674332)
--(axis cs:63.0573248407643,0.843209964171033)
--(axis cs:63.6942675159236,0.84178799172111)
--(axis cs:64.3312101910828,0.845767856265824)
--(axis cs:64.968152866242,0.852095692984208)
--(axis cs:65.6050955414013,0.860761851111394)
--(axis cs:66.2420382165605,0.867679679218154)
--(axis cs:66.8789808917197,0.879287175289857)
--(axis cs:67.515923566879,0.885544008752127)
--(axis cs:68.1528662420382,0.894855645603163)
--(axis cs:68.7898089171974,0.894690821861413)
--(axis cs:69.4267515923567,0.906897841002954)
--(axis cs:70.0636942675159,0.907123703221118)
--(axis cs:70.7006369426752,0.906515025104899)
--(axis cs:71.3375796178344,0.911230527743419)
--(axis cs:71.9745222929936,0.916085961616503)
--(axis cs:72.6114649681529,0.920102781588323)
--(axis cs:73.2484076433121,0.920148842791494)
--(axis cs:73.8853503184713,0.924931705796455)
--(axis cs:74.5222929936306,0.930557948713751)
--(axis cs:75.1592356687898,0.933837236537094)
--(axis cs:75.796178343949,0.935613940601003)
--(axis cs:76.4331210191083,0.942898642721202)
--(axis cs:77.0700636942675,0.950270135045095)
--(axis cs:77.7070063694268,0.955861869305932)
--(axis cs:78.343949044586,0.962378794146675)
--(axis cs:78.9808917197452,0.967420076128414)
--(axis cs:79.6178343949044,0.967796412754537)
--(axis cs:80.2547770700637,0.972376766086428)
--(axis cs:80.8917197452229,0.973124050362959)
--(axis cs:81.5286624203822,0.975959932200394)
--(axis cs:82.1656050955414,0.977407705693233)
--(axis cs:82.8025477707006,0.976593877492057)
--(axis cs:83.4394904458599,0.978433100263671)
--(axis cs:84.0764331210191,0.980414938004389)
--(axis cs:84.7133757961783,0.980386377586861)
--(axis cs:85.3503184713376,0.980716706526302)
--(axis cs:85.9872611464968,0.987545960409922)
--(axis cs:86.6242038216561,0.991162535402943)
--(axis cs:87.2611464968153,0.992852455405348)
--(axis cs:87.8980891719745,0.997360232664496)
--(axis cs:88.5350318471338,0.998433856164788)
--(axis cs:89.171974522293,0.998744482930473)
--(axis cs:89.8089171974522,0.998827112005908)
--(axis cs:90.4458598726115,0.999684993785267)
--(axis cs:91.0828025477707,1)
--(axis cs:91.7197452229299,1)
--(axis cs:92.3566878980892,1)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1)
--(axis cs:91.7197452229299,1)
--(axis cs:91.0828025477707,1)
--(axis cs:90.4458598726115,1.00023688121473)
--(axis cs:89.8089171974522,1.00046976299409)
--(axis cs:89.171974522293,1.00047426706953)
--(axis cs:88.5350318471338,1.00047239383521)
--(axis cs:87.8980891719745,1.0002960173355)
--(axis cs:87.2611464968153,0.998085044594652)
--(axis cs:86.6242038216561,0.996884339597057)
--(axis cs:85.9872611464968,0.993782164590078)
--(axis cs:85.3503184713376,0.985377043473698)
--(axis cs:84.7133757961783,0.985160497413139)
--(axis cs:84.0764331210191,0.984897561995611)
--(axis cs:83.4394904458599,0.982738774736329)
--(axis cs:82.8025477707006,0.980906122507943)
--(axis cs:82.1656050955414,0.981811044306767)
--(axis cs:81.5286624203822,0.980680692799606)
--(axis cs:80.8917197452229,0.978516574637041)
--(axis cs:80.2547770700637,0.978248233913572)
--(axis cs:79.6178343949044,0.975250462245463)
--(axis cs:78.9808917197452,0.974376798871586)
--(axis cs:78.343949044586,0.970824330853325)
--(axis cs:77.7070063694268,0.964763130694068)
--(axis cs:77.0700636942675,0.959886114954905)
--(axis cs:76.4331210191083,0.952257607278798)
--(axis cs:75.796178343949,0.943995434398997)
--(axis cs:75.1592356687898,0.942959638462906)
--(axis cs:74.5222929936306,0.939442051286249)
--(axis cs:73.8853503184713,0.934443294203545)
--(axis cs:73.2484076433121,0.929773032208505)
--(axis cs:72.6114649681529,0.929662843411677)
--(axis cs:71.9745222929936,0.926179663383497)
--(axis cs:71.3375796178344,0.921738222256581)
--(axis cs:70.7006369426752,0.917859974895101)
--(axis cs:70.0636942675159,0.919204421778882)
--(axis cs:69.4267515923567,0.919039658997046)
--(axis cs:68.7898089171974,0.907965428138587)
--(axis cs:68.1528662420382,0.908425604396837)
--(axis cs:67.515923566879,0.899377866247873)
--(axis cs:66.8789808917197,0.893212824710143)
--(axis cs:66.2420382165605,0.881382820781846)
--(axis cs:65.6050955414013,0.874316273888606)
--(axis cs:64.968152866242,0.865873057015793)
--(axis cs:64.3312101910828,0.859310268734176)
--(axis cs:63.6942675159236,0.85469638327889)
--(axis cs:63.0573248407643,0.856555660828967)
--(axis cs:62.4203821656051,0.853756616325668)
--(axis cs:61.7834394904459,0.848825321165242)
--(axis cs:61.1464968152866,0.844810347378516)
--(axis cs:60.5095541401274,0.837990884943863)
--(axis cs:59.8726114649682,0.839248459026101)
--(axis cs:59.2356687898089,0.831904169992296)
--(axis cs:58.5987261146497,0.827646132240219)
--(axis cs:57.9617834394904,0.826315166957397)
--(axis cs:57.3248407643312,0.818626861168417)
--(axis cs:56.687898089172,0.81239245184424)
--(axis cs:56.0509554140127,0.807986948527837)
--(axis cs:55.4140127388535,0.796863991910906)
--(axis cs:54.7770700636943,0.785129619384809)
--(axis cs:54.140127388535,0.777559986044908)
--(axis cs:53.5031847133758,0.765105448689961)
--(axis cs:52.8662420382166,0.757551904638148)
--(axis cs:52.2292993630573,0.757040823922852)
--(axis cs:51.5923566878981,0.75759456362706)
--(axis cs:50.9554140127388,0.749378101442193)
--(axis cs:50.3184713375796,0.738996012725665)
--(axis cs:49.6815286624204,0.73273898547317)
--(axis cs:49.0445859872611,0.725923263057777)
--(axis cs:48.4076433121019,0.71103006536776)
--(axis cs:47.7707006369427,0.702746290225074)
--(axis cs:47.1337579617834,0.696089747753591)
--(axis cs:46.4968152866242,0.692298160733321)
--(axis cs:45.859872611465,0.681184562745248)
--(axis cs:45.2229299363057,0.665493666565045)
--(axis cs:44.5859872611465,0.651301232713158)
--(axis cs:43.9490445859873,0.631075138962801)
--(axis cs:43.312101910828,0.613299049390353)
--(axis cs:42.6751592356688,0.601291226255803)
--(axis cs:42.0382165605096,0.593030784062932)
--(axis cs:41.4012738853503,0.571746791845678)
--(axis cs:40.7643312101911,0.553368033183099)
--(axis cs:40.1273885350318,0.53916213026861)
--(axis cs:39.4904458598726,0.523139634582734)
--(axis cs:38.8535031847134,0.524891226555904)
--(axis cs:38.2165605095541,0.503706902932308)
--(axis cs:37.5796178343949,0.48834561435828)
--(axis cs:36.9426751592357,0.477680529518163)
--(axis cs:36.3057324840764,0.459556451672021)
--(axis cs:35.6687898089172,0.435332486419264)
--(axis cs:35.031847133758,0.421925388212102)
--(axis cs:34.3949044585987,0.402230206330999)
--(axis cs:33.7579617834395,0.37998675206207)
--(axis cs:33.1210191082803,0.356543337518987)
--(axis cs:32.484076433121,0.338472131215301)
--(axis cs:31.8471337579618,0.320699649320053)
--(axis cs:31.2101910828025,0.307137861986931)
--(axis cs:30.5732484076433,0.295608843525522)
--(axis cs:29.9363057324841,0.283105382193922)
--(axis cs:29.2993630573248,0.271711175128579)
--(axis cs:28.6624203821656,0.262103825776128)
--(axis cs:28.0254777070064,0.249902385336992)
--(axis cs:27.3885350318471,0.244886502776991)
--(axis cs:26.7515923566879,0.230527913646978)
--(axis cs:26.1146496815287,0.211855470013668)
--(axis cs:25.4777070063694,0.206250389831319)
--(axis cs:24.8407643312102,0.200784384139352)
--(axis cs:24.203821656051,0.188401849873773)
--(axis cs:23.5668789808917,0.18770920061194)
--(axis cs:22.9299363057325,0.176850854782753)
--(axis cs:22.2929936305732,0.165283109695467)
--(axis cs:21.656050955414,0.158935287992091)
--(axis cs:21.0191082802548,0.14726222994688)
--(axis cs:20.3821656050955,0.141913478870108)
--(axis cs:19.7452229299363,0.132863180453475)
--(axis cs:19.1082802547771,0.128411047687039)
--(axis cs:18.4713375796178,0.120289210797582)
--(axis cs:17.8343949044586,0.120643473111976)
--(axis cs:17.1974522292994,0.114407022158719)
--(axis cs:16.5605095541401,0.109524124080979)
--(axis cs:15.9235668789809,0.101865820839859)
--(axis cs:15.2866242038217,0.0991528281945702)
--(axis cs:14.6496815286624,0.0956679552114745)
--(axis cs:14.0127388535032,0.0933336796646771)
--(axis cs:13.3757961783439,0.0916798297537207)
--(axis cs:12.7388535031847,0.0889946913610812)
--(axis cs:12.1019108280255,0.0871279189300076)
--(axis cs:11.4649681528662,0.0866331488721538)
--(axis cs:10.828025477707,0.0859897914464266)
--(axis cs:10.1910828025478,0.084441685130106)
--(axis cs:9.55414012738853,0.0834787653812813)
--(axis cs:8.9171974522293,0.0825338553397304)
--(axis cs:8.28025477707006,0.0814201156136913)
--(axis cs:7.64331210191083,0.08092416529485)
--(axis cs:7.00636942675159,0.0814221010827284)
--(axis cs:6.36942675159236,0.080909413894663)
--(axis cs:5.73248407643312,0.080909413894663)
--(axis cs:5.09554140127389,0.0815007927798631)
--(axis cs:4.45859872611465,0.0808116164824885)
--(axis cs:3.82165605095541,0.0805170110339466)
--(axis cs:3.18471337579618,0.0803902433438268)
--(axis cs:2.54777070063694,0.0805170110339466)
--(axis cs:1.91082802547771,0.0806300124294657)
--(axis cs:1.27388535031847,0.0804679863140301)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0803902433438268)
--cycle;


==> img/mnist/mnist_rate_accuracy_fw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.0800390625
0.636942675159236 0.08
1.27388535031847 0.08
1.91082802547771 0.0800390625
2.54777070063694 0.08
3.18471337579618 0.080078125
3.82165605095541 0.0801953125
4.45859872611465 0.080625
5.09554140127389 0.081015625
5.73248407643312 0.0818359375
6.36942675159236 0.0821484375
7.00636942675159 0.0859765625
7.64331210191083 0.0873828125
8.28025477707006 0.0924609375
8.9171974522293 0.098984375
9.55414012738853 0.109609375
10.1910828025478 0.1248828125
10.828025477707 0.139453125
11.4649681528662 0.1509375
12.1019108280255 0.172578125
12.7388535031847 0.1900390625
13.3757961783439 0.2115234375
14.0127388535032 0.227890625
14.6496815286624 0.2530859375
15.2866242038217 0.2666015625
15.9235668789809 0.288046875
16.5605095541401 0.30328125
17.1974522292994 0.316328125
17.8343949044586 0.343125
18.4713375796178 0.369296875
19.1082802547771 0.3937109375
19.7452229299363 0.4153125
20.3821656050955 0.446328125
21.0191082802548 0.46859375
21.656050955414 0.4751953125
22.2929936305732 0.5003125
22.9299363057325 0.5219921875
23.5668789808917 0.5436328125
24.203821656051 0.5658984375
24.8407643312102 0.5801171875
25.4777070063694 0.6015625
26.1146496815287 0.620078125
26.7515923566879 0.6311328125
27.3885350318471 0.642734375
28.0254777070064 0.66234375
28.6624203821656 0.679765625
29.2993630573248 0.68390625
29.9363057324841 0.6958203125
30.5732484076433 0.710703125
31.2101910828025 0.725390625
31.8471337579618 0.7366796875
32.484076433121 0.7477734375
33.1210191082803 0.758359375
33.7579617834395 0.7767578125
34.3949044585987 0.7871484375
35.031847133758 0.7953125
35.6687898089172 0.8084375
36.3057324840764 0.8101953125
36.9426751592357 0.8144140625
37.5796178343949 0.8180859375
38.2165605095541 0.8233203125
38.8535031847134 0.828125
39.4904458598726 0.8280859375
40.1273885350318 0.8321875
40.7643312101911 0.8333203125
41.4012738853503 0.831171875
42.0382165605096 0.8290234375
42.6751592356688 0.828671875
43.312101910828 0.83390625
43.9490445859873 0.838125
44.5859872611465 0.843984375
45.2229299363057 0.850859375
45.859872611465 0.8586328125
46.4968152866242 0.8633203125
47.1337579617834 0.869453125
47.7707006369427 0.8673046875
48.4076433121019 0.8725390625
49.0445859872611 0.8726171875
49.6815286624204 0.86640625
50.3184713375796 0.863828125
50.9554140127388 0.859765625
51.5923566878981 0.8703125
52.2292993630573 0.8749609375
52.8662420382166 0.8748828125
53.5031847133758 0.8732421875
54.140127388535 0.8762109375
54.7770700636943 0.8793359375
55.4140127388535 0.8803125
56.0509554140127 0.869453125
56.687898089172 0.8704296875
57.3248407643312 0.8753515625
57.9617834394904 0.877109375
58.5987261146497 0.8824609375
59.2356687898089 0.8941015625
59.8726114649682 0.8941796875
60.5095541401274 0.9065234375
61.1464968152866 0.9157421875
61.7834394904459 0.9120703125
62.4203821656051 0.913359375
63.0573248407643 0.9152734375
63.6942675159236 0.91953125
64.3312101910828 0.916640625
64.968152866242 0.920078125
65.6050955414013 0.9205078125
66.2420382165605 0.9178125
66.8789808917197 0.920390625
67.515923566879 0.9240625
68.1528662420382 0.9263671875
68.7898089171974 0.93609375
69.4267515923567 0.934375
70.0636942675159 0.937734375
70.7006369426752 0.947109375
71.3375796178344 0.948359375
71.9745222929936 0.9494921875
72.6114649681529 0.9526953125
73.2484076433121 0.95484375
73.8853503184713 0.9574609375
74.5222929936306 0.956484375
75.1592356687898 0.9568359375
75.796178343949 0.957109375
76.4331210191083 0.9567578125
77.0700636942675 0.9554296875
77.7070063694268 0.9569921875
78.343949044586 0.958125
78.9808917197452 0.9584765625
79.6178343949044 0.958984375
80.2547770700637 0.9603125
80.8917197452229 0.958515625
81.5286624203822 0.9597265625
82.1656050955414 0.9623046875
82.8025477707006 0.9663671875
83.4394904458599 0.967578125
84.0764331210191 0.96828125
84.7133757961783 0.96671875
85.3503184713376 0.968671875
85.9872611464968 0.9715625
86.6242038216561 0.9772265625
87.2611464968153 0.980234375
87.8980891719745 0.9818359375
88.5350318471338 0.983984375
89.171974522293 0.9840234375
89.8089171974522 0.9857421875
90.4458598726115 0.985078125
91.0828025477707 0.98890625
91.7197452229299 0.99234375
92.3566878980892 0.998046875
92.9936305732484 0.999375
93.6305732484076 0.99953125
94.2675159235669 0.9996875
94.9044585987261 0.9998828125
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color0, fill opacity=0.25]
(axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.0796097566561732)
--(axis cs:1.27388535031847,0.08)
--(axis cs:1.91082802547771,0.0795611139660534)
--(axis cs:2.54777070063694,0.0796097566561732)
--(axis cs:3.18471337579618,0.0795262375705343)
--(axis cs:3.82165605095541,0.0792812511737538)
--(axis cs:4.45859872611465,0.0795235225629169)
--(axis cs:5.09554140127389,0.0795082666952702)
--(axis cs:5.73248407643312,0.0799132235117579)
--(axis cs:6.36942675159236,0.0800770154363518)
--(axis cs:7.00636942675159,0.0825388795727938)
--(axis cs:7.64331210191083,0.0835859155537804)
--(axis cs:8.28025477707006,0.0876749561009193)
--(axis cs:8.9171974522293,0.093216090952472)
--(axis cs:9.55414012738853,0.102621705220055)
--(axis cs:10.1910828025478,0.11676486137685)
--(axis cs:10.828025477707,0.130499069954544)
--(axis cs:11.4649681528662,0.141477483943888)
--(axis cs:12.1019108280255,0.162433002405433)
--(axis cs:12.7388535031847,0.179525222238255)
--(axis cs:13.3757961783439,0.200512323153203)
--(axis cs:14.0127388535032,0.216521035150026)
--(axis cs:14.6496815286624,0.241310175658734)
--(axis cs:15.2866242038217,0.254799067591689)
--(axis cs:15.9235668789809,0.276168360979107)
--(axis cs:16.5605095541401,0.290735474003982)
--(axis cs:17.1974522292994,0.30328699295441)
--(axis cs:17.8343949044586,0.329686583173225)
--(axis cs:18.4713375796178,0.35547655314979)
--(axis cs:19.1082802547771,0.379972830844282)
--(axis cs:19.7452229299363,0.401955865616856)
--(axis cs:20.3821656050955,0.433015776747015)
--(axis cs:21.0191082802548,0.455389770445179)
--(axis cs:21.656050955414,0.46204188088457)
--(axis cs:22.2929936305732,0.486896300675454)
--(axis cs:22.9299363057325,0.509120655906611)
--(axis cs:23.5668789808917,0.530649367924686)
--(axis cs:24.203821656051,0.553003449455894)
--(axis cs:24.8407643312102,0.567248689395133)
--(axis cs:25.4777070063694,0.588529597471809)
--(axis cs:26.1146496815287,0.607015894258345)
--(axis cs:26.7515923566879,0.618174239555399)
--(axis cs:27.3885350318471,0.629782985219083)
--(axis cs:28.0254777070064,0.649468751611062)
--(axis cs:28.6624203821656,0.666847390352073)
--(axis cs:29.2993630573248,0.67098533951324)
--(axis cs:29.9363057324841,0.682829949108461)
--(axis cs:30.5732484076433,0.697991601583507)
--(axis cs:31.2101910828025,0.712557394469867)
--(axis cs:31.8471337579618,0.724105479453436)
--(axis cs:32.484076433121,0.735366174667153)
--(axis cs:33.1210191082803,0.746176390873199)
--(axis cs:33.7579617834395,0.764682220082964)
--(axis cs:34.3949044585987,0.775432949520169)
--(axis cs:35.031847133758,0.783636603827227)
--(axis cs:35.6687898089172,0.797177626915524)
--(axis cs:36.3057324840764,0.798623684285009)
--(axis cs:36.9426751592357,0.803340118519258)
--(axis cs:37.5796178343949,0.80716297707337)
--(axis cs:38.2165605095541,0.812857918177675)
--(axis cs:38.8535031847134,0.817609310337396)
--(axis cs:39.4904458598726,0.817334813453978)
--(axis cs:40.1273885350318,0.821703202135623)
--(axis cs:40.7643312101911,0.823233677221157)
--(axis cs:41.4012738853503,0.82126752584024)
--(axis cs:42.0382165605096,0.819362754098827)
--(axis cs:42.6751592356688,0.819329786850328)
--(axis cs:43.312101910828,0.824792166224046)
--(axis cs:43.9490445859873,0.828631539135854)
--(axis cs:44.5859872611465,0.83471051733363)
--(axis cs:45.2229299363057,0.841707471323275)
--(axis cs:45.859872611465,0.849463267958729)
--(axis cs:46.4968152866242,0.854232827460237)
--(axis cs:47.1337579617834,0.860538263970184)
--(axis cs:47.7707006369427,0.858600252465818)
--(axis cs:48.4076433121019,0.863856292901)
--(axis cs:49.0445859872611,0.864400277593949)
--(axis cs:49.6815286624204,0.858420686694519)
--(axis cs:50.3184713375796,0.855696482805801)
--(axis cs:50.9554140127388,0.851477796899953)
--(axis cs:51.5923566878981,0.862017555044632)
--(axis cs:52.2292993630573,0.86633220682802)
--(axis cs:52.8662420382166,0.866420962184787)
--(axis cs:53.5031847133758,0.864765259007915)
--(axis cs:54.140127388535,0.867552176072084)
--(axis cs:54.7770700636943,0.870644779851804)
--(axis cs:55.4140127388535,0.871427810397571)
--(axis cs:56.0509554140127,0.860773711173649)
--(axis cs:56.687898089172,0.862005694922733)
--(axis cs:57.3248407643312,0.866833809584758)
--(axis cs:57.9617834394904,0.868757695683296)
--(axis cs:58.5987261146497,0.874146282346356)
--(axis cs:59.2356687898089,0.885770328508008)
--(axis cs:59.8726114649682,0.885980314477025)
--(axis cs:60.5095541401274,0.898541504414036)
--(axis cs:61.1464968152866,0.908250361366753)
--(axis cs:61.7834394904459,0.904653930689178)
--(axis cs:62.4203821656051,0.906250332850608)
--(axis cs:63.0573248407643,0.908194359159356)
--(axis cs:63.6942675159236,0.912453782135266)
--(axis cs:64.3312101910828,0.909519080213475)
--(axis cs:64.968152866242,0.913268351899397)
--(axis cs:65.6050955414013,0.914075378800492)
--(axis cs:66.2420382165605,0.911168061397779)
--(axis cs:66.8789808917197,0.914244412040582)
--(axis cs:67.515923566879,0.917698362179796)
--(axis cs:68.1528662420382,0.92026485607191)
--(axis cs:68.7898089171974,0.93016412253027)
--(axis cs:69.4267515923567,0.928295751366613)
--(axis cs:70.0636942675159,0.931683010890361)
--(axis cs:70.7006369426752,0.942072617222491)
--(axis cs:71.3375796178344,0.943408644957384)
--(axis cs:71.9745222929936,0.944632700366366)
--(axis cs:72.6114649681529,0.948210478457243)
--(axis cs:73.2484076433121,0.950813950318992)
--(axis cs:73.8853503184713,0.953758582955847)
--(axis cs:74.5222929936306,0.952428185889844)
--(axis cs:75.1592356687898,0.953342870392091)
--(axis cs:75.796178343949,0.954326011260802)
--(axis cs:76.4331210191083,0.954235501898247)
--(axis cs:77.0700636942675,0.952473140499203)
--(axis cs:77.7070063694268,0.954398573959447)
--(axis cs:78.343949044586,0.955917720302286)
--(axis cs:78.9808917197452,0.955802386688925)
--(axis cs:79.6178343949044,0.9564988723531)
--(axis cs:80.2547770700637,0.957273513049597)
--(axis cs:80.8917197452229,0.955230867353348)
--(axis cs:81.5286624203822,0.956794256744509)
--(axis cs:82.1656050955414,0.958659524070887)
--(axis cs:82.8025477707006,0.962996830814175)
--(axis cs:83.4394904458599,0.963572469953655)
--(axis cs:84.0764331210191,0.964223922207315)
--(axis cs:84.7133757961783,0.962592881785354)
--(axis cs:85.3503184713376,0.964637788218208)
--(axis cs:85.9872611464968,0.967796556668263)
--(axis cs:86.6242038216561,0.974721145538114)
--(axis cs:87.2611464968153,0.978360446600369)
--(axis cs:87.8980891719745,0.979850014456885)
--(axis cs:88.5350318471338,0.981439801840912)
--(axis cs:89.171974522293,0.981517961063046)
--(axis cs:89.8089171974522,0.982914605840956)
--(axis cs:90.4458598726115,0.982357846218539)
--(axis cs:91.0828025477707,0.985799998256139)
--(axis cs:91.7197452229299,0.989305792923769)
--(axis cs:92.3566878980892,0.996191566875785)
--(axis cs:92.9936305732484,0.998287546022885)
--(axis cs:93.6305732484076,0.998585697425242)
--(axis cs:94.2675159235669,0.998912377545586)
--(axis cs:94.9044585987261,0.999405800203062)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1.00035982479694)
--(axis cs:94.2675159235669,1.00046262245441)
--(axis cs:93.6305732484076,1.00047680257476)
--(axis cs:92.9936305732484,1.00046245397712)
--(axis cs:92.3566878980892,0.999902183124215)
--(axis cs:91.7197452229299,0.995381707076231)
--(axis cs:91.0828025477707,0.992012501743861)
--(axis cs:90.4458598726115,0.987798403781461)
--(axis cs:89.8089171974522,0.988569769159043)
--(axis cs:89.171974522293,0.986528913936954)
--(axis cs:88.5350318471338,0.986528948159088)
--(axis cs:87.8980891719745,0.983821860543115)
--(axis cs:87.2611464968153,0.982108303399631)
--(axis cs:86.6242038216561,0.979731979461886)
--(axis cs:85.9872611464968,0.975328443331737)
--(axis cs:85.3503184713376,0.972705961781791)
--(axis cs:84.7133757961783,0.970844618214646)
--(axis cs:84.0764331210191,0.972338577792685)
--(axis cs:83.4394904458599,0.971583780046345)
--(axis cs:82.8025477707006,0.969737544185824)
--(axis cs:82.1656050955414,0.965949850929113)
--(axis cs:81.5286624203822,0.962658868255491)
--(axis cs:80.8917197452229,0.961800382646652)
--(axis cs:80.2547770700637,0.963351486950404)
--(axis cs:79.6178343949044,0.9614698776469)
--(axis cs:78.9808917197452,0.961150738311075)
--(axis cs:78.343949044586,0.960332279697714)
--(axis cs:77.7070063694268,0.959585801040553)
--(axis cs:77.0700636942675,0.958386234500797)
--(axis cs:76.4331210191083,0.959280123101753)
--(axis cs:75.796178343949,0.959892738739198)
--(axis cs:75.1592356687898,0.960329004607909)
--(axis cs:74.5222929936306,0.960540564110156)
--(axis cs:73.8853503184713,0.961163292044153)
--(axis cs:73.2484076433121,0.958873549681008)
--(axis cs:72.6114649681529,0.957180146542756)
--(axis cs:71.9745222929936,0.954351674633634)
--(axis cs:71.3375796178344,0.953310105042616)
--(axis cs:70.7006369426752,0.952146132777509)
--(axis cs:70.0636942675159,0.943785739109639)
--(axis cs:69.4267515923567,0.940454248633387)
--(axis cs:68.7898089171974,0.94202337746973)
--(axis cs:68.1528662420382,0.93246951892809)
--(axis cs:67.515923566879,0.930426637820204)
--(axis cs:66.8789808917197,0.926536837959418)
--(axis cs:66.2420382165605,0.924456938602221)
--(axis cs:65.6050955414013,0.926940246199508)
--(axis cs:64.968152866242,0.926887898100603)
--(axis cs:64.3312101910828,0.923762169786525)
--(axis cs:63.6942675159236,0.926608717864734)
--(axis cs:63.0573248407643,0.922352515840644)
--(axis cs:62.4203821656051,0.920468417149392)
--(axis cs:61.7834394904459,0.919486694310822)
--(axis cs:61.1464968152866,0.923234013633247)
--(axis cs:60.5095541401274,0.914505370585964)
--(axis cs:59.8726114649682,0.902379060522975)
--(axis cs:59.2356687898089,0.902432796491992)
--(axis cs:58.5987261146497,0.890775592653644)
--(axis cs:57.9617834394904,0.885461054316704)
--(axis cs:57.3248407643312,0.883869315415242)
--(axis cs:56.687898089172,0.878853680077267)
--(axis cs:56.0509554140127,0.878132538826351)
--(axis cs:55.4140127388535,0.889197189602429)
--(axis cs:54.7770700636943,0.888027095148196)
--(axis cs:54.140127388535,0.884869698927916)
--(axis cs:53.5031847133758,0.881719115992085)
--(axis cs:52.8662420382166,0.883344662815213)
--(axis cs:52.2292993630573,0.88358966817198)
--(axis cs:51.5923566878981,0.878607444955368)
--(axis cs:50.9554140127388,0.868053453100047)
--(axis cs:50.3184713375796,0.871959767194199)
--(axis cs:49.6815286624204,0.874391813305481)
--(axis cs:49.0445859872611,0.880834097406051)
--(axis cs:48.4076433121019,0.881221832099)
--(axis cs:47.7707006369427,0.876009122534182)
--(axis cs:47.1337579617834,0.878367986029816)
--(axis cs:46.4968152866242,0.872407797539763)
--(axis cs:45.859872611465,0.867802357041271)
--(axis cs:45.2229299363057,0.860011278676725)
--(axis cs:44.5859872611465,0.85325823266637)
--(axis cs:43.9490445859873,0.847618460864146)
--(axis cs:43.312101910828,0.843020333775954)
--(axis cs:42.6751592356688,0.838013963149672)
--(axis cs:42.0382165605096,0.838684120901173)
--(axis cs:41.4012738853503,0.84107622415976)
--(axis cs:40.7643312101911,0.843406947778843)
--(axis cs:40.1273885350318,0.842671797864377)
--(axis cs:39.4904458598726,0.838837061546022)
--(axis cs:38.8535031847134,0.838640689662604)
--(axis cs:38.2165605095541,0.833782706822325)
--(axis cs:37.5796178343949,0.82900889792663)
--(axis cs:36.9426751592357,0.825488006480742)
--(axis cs:36.3057324840764,0.821766940714991)
--(axis cs:35.6687898089172,0.819697373084476)
--(axis cs:35.031847133758,0.806988396172773)
--(axis cs:34.3949044585987,0.798863925479831)
--(axis cs:33.7579617834395,0.788833404917036)
--(axis cs:33.1210191082803,0.770542359126801)
--(axis cs:32.484076433121,0.760180700332847)
--(axis cs:31.8471337579618,0.749253895546564)
--(axis cs:31.2101910828025,0.738223855530133)
--(axis cs:30.5732484076433,0.723414648416493)
--(axis cs:29.9363057324841,0.708810675891539)
--(axis cs:29.2993630573248,0.69682716048676)
--(axis cs:28.6624203821656,0.692683859647928)
--(axis cs:28.0254777070064,0.675218748388938)
--(axis cs:27.3885350318471,0.655685764780917)
--(axis cs:26.7515923566879,0.644091385444601)
--(axis cs:26.1146496815287,0.633140355741655)
--(axis cs:25.4777070063694,0.614595402528191)
--(axis cs:24.8407643312102,0.592985685604867)
--(axis cs:24.203821656051,0.578793425544106)
--(axis cs:23.5668789808917,0.556616257075313)
--(axis cs:22.9299363057325,0.534863719093389)
--(axis cs:22.2929936305732,0.513728699324546)
--(axis cs:21.656050955414,0.48834874411543)
--(axis cs:21.0191082802548,0.481797729554821)
--(axis cs:20.3821656050955,0.459640473252985)
--(axis cs:19.7452229299363,0.428669134383144)
--(axis cs:19.1082802547771,0.407449044155718)
--(axis cs:18.4713375796178,0.38311719685021)
--(axis cs:17.8343949044586,0.356563416826775)
--(axis cs:17.1974522292994,0.32936925704559)
--(axis cs:16.5605095541401,0.315827025996018)
--(axis cs:15.9235668789809,0.299925389020893)
--(axis cs:15.2866242038217,0.278404057408311)
--(axis cs:14.6496815286624,0.264861699341266)
--(axis cs:14.0127388535032,0.239260214849974)
--(axis cs:13.3757961783439,0.222534551846797)
--(axis cs:12.7388535031847,0.200552902761745)
--(axis cs:12.1019108280255,0.182723247594567)
--(axis cs:11.4649681528662,0.160397516056112)
--(axis cs:10.828025477707,0.148407180045456)
--(axis cs:10.1910828025478,0.13300076362315)
--(axis cs:9.55414012738853,0.116597044779945)
--(axis cs:8.9171974522293,0.104752659047528)
--(axis cs:8.28025477707006,0.0972469188990807)
--(axis cs:7.64331210191083,0.0911797094462196)
--(axis cs:7.00636942675159,0.0894142454272062)
--(axis cs:6.36942675159236,0.0842198595636482)
--(axis cs:5.73248407643312,0.083758651488242)
--(axis cs:5.09554140127389,0.0825229833047298)
--(axis cs:4.45859872611465,0.0817264774370831)
--(axis cs:3.82165605095541,0.0811093738262463)
--(axis cs:3.18471337579618,0.0806300124294657)
--(axis cs:2.54777070063694,0.0803902433438268)
--(axis cs:1.91082802547771,0.0805170110339466)
--(axis cs:1.27388535031847,0.08)
--(axis cs:0.636942675159236,0.0803902433438268)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_fw_order.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.0800390625
0.636942675159236 0.08
1.27388535031847 0.0800390625
1.91082802547771 0.0800390625
2.54777070063694 0.0799609375
3.18471337579618 0.0801953125
3.82165605095541 0.0803515625
4.45859872611465 0.0809375
5.09554140127389 0.0809375
5.73248407643312 0.082265625
6.36942675159236 0.08546875
7.00636942675159 0.091015625
7.64331210191083 0.095859375
8.28025477707006 0.0998046875
8.9171974522293 0.1091796875
9.55414012738853 0.12125
10.1910828025478 0.1325
10.828025477707 0.14734375
11.4649681528662 0.169453125
12.1019108280255 0.18578125
12.7388535031847 0.2037109375
13.3757961783439 0.219921875
14.0127388535032 0.23984375
14.6496815286624 0.256796875
15.2866242038217 0.273046875
15.9235668789809 0.2884375
16.5605095541401 0.30234375
17.1974522292994 0.3141796875
17.8343949044586 0.3366796875
18.4713375796178 0.3555859375
19.1082802547771 0.3763671875
19.7452229299363 0.3896875
20.3821656050955 0.3981640625
21.0191082802548 0.4199609375
21.656050955414 0.437421875
22.2929936305732 0.4596875
22.9299363057325 0.467421875
23.5668789808917 0.4846484375
24.203821656051 0.4980859375
24.8407643312102 0.5116015625
25.4777070063694 0.53109375
26.1146496815287 0.5558203125
26.7515923566879 0.566484375
27.3885350318471 0.57671875
28.0254777070064 0.601015625
28.6624203821656 0.6041015625
29.2993630573248 0.6183203125
29.9363057324841 0.6313671875
30.5732484076433 0.6427734375
31.2101910828025 0.648828125
31.8471337579618 0.6585546875
32.484076433121 0.672109375
33.1210191082803 0.68296875
33.7579617834395 0.694140625
34.3949044585987 0.7011328125
35.031847133758 0.7081640625
35.6687898089172 0.72046875
36.3057324840764 0.7315234375
36.9426751592357 0.7415625
37.5796178343949 0.739765625
38.2165605095541 0.748984375
38.8535031847134 0.755
39.4904458598726 0.765859375
40.1273885350318 0.7626953125
40.7643312101911 0.7603515625
41.4012738853503 0.760859375
42.0382165605096 0.76125
42.6751592356688 0.7628125
43.312101910828 0.773203125
43.9490445859873 0.78390625
44.5859872611465 0.793515625
45.2229299363057 0.8048046875
45.859872611465 0.8090625
46.4968152866242 0.8153515625
47.1337579617834 0.824140625
47.7707006369427 0.83015625
48.4076433121019 0.8375390625
49.0445859872611 0.8391015625
49.6815286624204 0.8429296875
50.3184713375796 0.8412109375
50.9554140127388 0.8465234375
51.5923566878981 0.85359375
52.2292993630573 0.8501953125
52.8662420382166 0.8553125
53.5031847133758 0.856796875
54.140127388535 0.8598828125
54.7770700636943 0.865
55.4140127388535 0.8683984375
56.0509554140127 0.8672265625
56.687898089172 0.8709375
57.3248407643312 0.8803125
57.9617834394904 0.881953125
58.5987261146497 0.8895703125
59.2356687898089 0.898984375
59.8726114649682 0.8963671875
60.5095541401274 0.91203125
61.1464968152866 0.9032421875
61.7834394904459 0.90390625
62.4203821656051 0.9164453125
63.0573248407643 0.91390625
63.6942675159236 0.9164453125
64.3312101910828 0.9164453125
64.968152866242 0.9203125
65.6050955414013 0.92125
66.2420382165605 0.9290625
66.8789808917197 0.9299609375
67.515923566879 0.9327734375
68.1528662420382 0.92921875
68.7898089171974 0.9398046875
69.4267515923567 0.9427734375
70.0636942675159 0.9451953125
70.7006369426752 0.9473828125
71.3375796178344 0.953203125
71.9745222929936 0.9632421875
72.6114649681529 0.9615234375
73.2484076433121 0.9633984375
73.8853503184713 0.9642578125
74.5222929936306 0.967265625
75.1592356687898 0.9673828125
75.796178343949 0.9714453125
76.4331210191083 0.9732421875
77.0700636942675 0.9742578125
77.7070063694268 0.975078125
78.343949044586 0.9734375
78.9808917197452 0.9742578125
79.6178343949044 0.976484375
80.2547770700637 0.97765625
80.8917197452229 0.98015625
81.5286624203822 0.9818359375
82.1656050955414 0.98
82.8025477707006 0.980625
83.4394904458599 0.9833203125
84.0764331210191 0.9848046875
84.7133757961783 0.9844140625
85.3503184713376 0.9823046875
85.9872611464968 0.9834765625
86.6242038216561 0.9819140625
87.2611464968153 0.983671875
87.8980891719745 0.9839453125
88.5350318471338 0.9850390625
89.171974522293 0.985546875
89.8089171974522 0.985625
90.4458598726115 0.9908203125
91.0828025477707 0.9923828125
91.7197452229299 0.992734375
92.3566878980892 0.9927734375
92.9936305732484 0.9990234375
93.6305732484076 0.99921875
94.2675159235669 0.9998828125
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color0, fill opacity=0.25]
(axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0796849937852672)
--(axis cs:3.18471337579618,0.0795785251417647)
--(axis cs:3.82165605095541,0.0793593328289674)
--(axis cs:4.45859872611465,0.0795900737571732)
--(axis cs:5.09554140127389,0.0794828643447494)
--(axis cs:5.73248407643312,0.0800781467983787)
--(axis cs:6.36942675159236,0.0822962837206601)
--(axis cs:7.00636942675159,0.08658792088691)
--(axis cs:7.64331210191083,0.0906375899774072)
--(axis cs:8.28025477707006,0.0940352540021227)
--(axis cs:8.9171974522293,0.102344327678566)
--(axis cs:9.55414012738853,0.113387326183936)
--(axis cs:10.1910828025478,0.123872037843378)
--(axis cs:10.828025477707,0.137901092523823)
--(axis cs:11.4649681528662,0.159376873220016)
--(axis cs:12.1019108280255,0.175271882239647)
--(axis cs:12.7388535031847,0.192920798773168)
--(axis cs:13.3757961783439,0.208846013697238)
--(axis cs:14.0127388535032,0.228593462311926)
--(axis cs:14.6496815286624,0.245668252763124)
--(axis cs:15.2866242038217,0.261460749560162)
--(axis cs:15.9235668789809,0.27672991967049)
--(axis cs:16.5605095541401,0.290476569190162)
--(axis cs:17.1974522292994,0.301820823409926)
--(axis cs:17.8343949044586,0.323916367971297)
--(axis cs:18.4713375796178,0.342597558731789)
--(axis cs:19.1082802547771,0.363313680952195)
--(axis cs:19.7452229299363,0.376333498780734)
--(axis cs:20.3821656050955,0.384842611456612)
--(axis cs:21.0191082802548,0.406538136781724)
--(axis cs:21.656050955414,0.423843617113981)
--(axis cs:22.2929936305732,0.446080333709379)
--(axis cs:22.9299363057325,0.453802547620782)
--(axis cs:23.5668789808917,0.471156100231443)
--(axis cs:24.203821656051,0.484593014903344)
--(axis cs:24.8407643312102,0.497932134574814)
--(axis cs:25.4777070063694,0.517766735163389)
--(axis cs:26.1146496815287,0.542543960801386)
--(axis cs:26.7515923566879,0.553168053651623)
--(axis cs:27.3885350318471,0.563308805285688)
--(axis cs:28.0254777070064,0.587597060126563)
--(axis cs:28.6624203821656,0.590812769395261)
--(axis cs:29.2993630573248,0.605445412488048)
--(axis cs:29.9363057324841,0.618639081614148)
--(axis cs:30.5732484076433,0.629918320750185)
--(axis cs:31.2101910828025,0.636320605155752)
--(axis cs:31.8471337579618,0.646054919960276)
--(axis cs:32.484076433121,0.659889447729917)
--(axis cs:33.1210191082803,0.670979294979496)
--(axis cs:33.7579617834395,0.68259287666867)
--(axis cs:34.3949044585987,0.689775634400876)
--(axis cs:35.031847133758,0.696876689944981)
--(axis cs:35.6687898089172,0.709612326714422)
--(axis cs:36.3057324840764,0.720802862928775)
--(axis cs:36.9426751592357,0.730335693956653)
--(axis cs:37.5796178343949,0.728596211417795)
--(axis cs:38.2165605095541,0.737883477700047)
--(axis cs:38.8535031847134,0.744024799472147)
--(axis cs:39.4904458598726,0.755021249718318)
--(axis cs:40.1273885350318,0.752130982044077)
--(axis cs:40.7643312101911,0.749757568215905)
--(axis cs:41.4012738853503,0.749975206425379)
--(axis cs:42.0382165605096,0.750338170339367)
--(axis cs:42.6751592356688,0.75202238198816)
--(axis cs:43.312101910828,0.762888421958653)
--(axis cs:43.9490445859873,0.773726215336265)
--(axis cs:44.5859872611465,0.783241930482547)
--(axis cs:45.2229299363057,0.794754118926441)
--(axis cs:45.859872611465,0.798844945038378)
--(axis cs:46.4968152866242,0.805324015709704)
--(axis cs:47.1337579617834,0.814687368850987)
--(axis cs:47.7707006369427,0.82134211407959)
--(axis cs:48.4076433121019,0.829014839173623)
--(axis cs:49.0445859872611,0.830316476661893)
--(axis cs:49.6815286624204,0.834287859415822)
--(axis cs:50.3184713375796,0.832547651196671)
--(axis cs:50.9554140127388,0.838488048491931)
--(axis cs:51.5923566878981,0.845453774241969)
--(axis cs:52.2292993630573,0.841732300016857)
--(axis cs:52.8662420382166,0.846720900371134)
--(axis cs:53.5031847133758,0.848170139155707)
--(axis cs:54.140127388535,0.851133896009228)
--(axis cs:54.7770700636943,0.856416035067393)
--(axis cs:55.4140127388535,0.859880019829586)
--(axis cs:56.0509554140127,0.858706413211004)
--(axis cs:56.687898089172,0.862569475459802)
--(axis cs:57.3248407643312,0.871580350555458)
--(axis cs:57.9617834394904,0.873314427099196)
--(axis cs:58.5987261146497,0.881085635434745)
--(axis cs:59.2356687898089,0.890933821694808)
--(axis cs:59.8726114649682,0.887791307128078)
--(axis cs:60.5095541401274,0.903851883188612)
--(axis cs:61.1464968152866,0.894824954815184)
--(axis cs:61.7834394904459,0.89563575435274)
--(axis cs:62.4203821656051,0.908554479394012)
--(axis cs:63.0573248407643,0.905947097124819)
--(axis cs:63.6942675159236,0.908673075476329)
--(axis cs:64.3312101910828,0.908793762637666)
--(axis cs:64.968152866242,0.912793186735861)
--(axis cs:65.6050955414013,0.913445686815167)
--(axis cs:66.2420382165605,0.921284561310268)
--(axis cs:66.8789808917197,0.922151747451048)
--(axis cs:67.515923566879,0.925208002470842)
--(axis cs:68.1528662420382,0.921818892360459)
--(axis cs:68.7898089171974,0.932627461769324)
--(axis cs:69.4267515923567,0.936029596825362)
--(axis cs:70.0636942675159,0.93865827915041)
--(axis cs:70.7006369426752,0.940979075575839)
--(axis cs:71.3375796178344,0.946959470155084)
--(axis cs:71.9745222929936,0.957318984228452)
--(axis cs:72.6114649681529,0.955915970576941)
--(axis cs:73.2484076433121,0.958436087861886)
--(axis cs:73.8853503184713,0.95935999315381)
--(axis cs:74.5222929936306,0.962978505892754)
--(axis cs:75.1592356687898,0.963004876849221)
--(axis cs:75.796178343949,0.967715370255322)
--(axis cs:76.4331210191083,0.96977911060746)
--(axis cs:77.0700636942675,0.971040223377279)
--(axis cs:77.7070063694268,0.972078968961536)
--(axis cs:78.343949044586,0.970229627824048)
--(axis cs:78.9808917197452,0.971163697273928)
--(axis cs:79.6178343949044,0.973633255666393)
--(axis cs:80.2547770700637,0.974591725920994)
--(axis cs:80.8917197452229,0.977980314578685)
--(axis cs:81.5286624203822,0.979207000913979)
--(axis cs:82.1656050955414,0.97805942754402)
--(axis cs:82.8025477707006,0.978799405928851)
--(axis cs:83.4394904458599,0.980863239961859)
--(axis cs:84.0764331210191,0.982134526718994)
--(axis cs:84.7133757961783,0.981799277654057)
--(axis cs:85.3503184713376,0.980275564573839)
--(axis cs:85.9872611464968,0.981108052387155)
--(axis cs:86.6242038216561,0.979966782733506)
--(axis cs:87.2611464968153,0.981252171659446)
--(axis cs:87.8980891719745,0.981458221624463)
--(axis cs:88.5350318471338,0.982325721992241)
--(axis cs:89.171974522293,0.982748827450145)
--(axis cs:89.8089171974522,0.982814942466809)
--(axis cs:90.4458598726115,0.987705844507046)
--(axis cs:91.0828025477707,0.989347824395909)
--(axis cs:91.7197452229299,0.989728469462312)
--(axis cs:92.3566878980892,0.989771028889531)
--(axis cs:92.9936305732484,0.997676509003252)
--(axis cs:93.6305732484076,0.99800785187816)
--(axis cs:94.2675159235669,0.999405800203062)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1.00035982479694)
--(axis cs:93.6305732484076,1.00042964812184)
--(axis cs:92.9936305732484,1.00037036599675)
--(axis cs:92.3566878980892,0.995775846110469)
--(axis cs:91.7197452229299,0.995740280537688)
--(axis cs:91.0828025477707,0.995417800604092)
--(axis cs:90.4458598726115,0.993934780492954)
--(axis cs:89.8089171974522,0.988435057533191)
--(axis cs:89.171974522293,0.988344922549855)
--(axis cs:88.5350318471338,0.987752403007759)
--(axis cs:87.8980891719745,0.986432403375537)
--(axis cs:87.2611464968153,0.986091578340554)
--(axis cs:86.6242038216561,0.983861342266494)
--(axis cs:85.9872611464968,0.985845072612845)
--(axis cs:85.3503184713376,0.984333810426161)
--(axis cs:84.7133757961783,0.987028847345943)
--(axis cs:84.0764331210191,0.987474848281006)
--(axis cs:83.4394904458599,0.985777385038141)
--(axis cs:82.8025477707006,0.982450594071149)
--(axis cs:82.1656050955414,0.98194057245598)
--(axis cs:81.5286624203822,0.984464874086021)
--(axis cs:80.8917197452229,0.982332185421315)
--(axis cs:80.2547770700637,0.980720774079006)
--(axis cs:79.6178343949044,0.979335494333607)
--(axis cs:78.9808917197452,0.977351927726072)
--(axis cs:78.343949044586,0.976645372175952)
--(axis cs:77.7070063694268,0.978077281038464)
--(axis cs:77.0700636942675,0.977475401622721)
--(axis cs:76.4331210191083,0.97670526439254)
--(axis cs:75.796178343949,0.975175254744678)
--(axis cs:75.1592356687898,0.971760748150779)
--(axis cs:74.5222929936306,0.971552744107246)
--(axis cs:73.8853503184713,0.96915563184619)
--(axis cs:73.2484076433121,0.968360787138114)
--(axis cs:72.6114649681529,0.967130904423059)
--(axis cs:71.9745222929936,0.969165390771548)
--(axis cs:71.3375796178344,0.959446779844916)
--(axis cs:70.7006369426752,0.953786549424161)
--(axis cs:70.0636942675159,0.95173234584959)
--(axis cs:69.4267515923567,0.949517278174638)
--(axis cs:68.7898089171974,0.946981913230676)
--(axis cs:68.1528662420382,0.936618607639541)
--(axis cs:67.515923566879,0.940338872529158)
--(axis cs:66.8789808917197,0.937770127548952)
--(axis cs:66.2420382165605,0.936840438689732)
--(axis cs:65.6050955414013,0.929054313184833)
--(axis cs:64.968152866242,0.927831813264139)
--(axis cs:64.3312101910828,0.924096862362335)
--(axis cs:63.6942675159236,0.924217549523671)
--(axis cs:63.0573248407643,0.921865402875181)
--(axis cs:62.4203821656051,0.924336145605988)
--(axis cs:61.7834394904459,0.91217674564726)
--(axis cs:61.1464968152866,0.911659420184815)
--(axis cs:60.5095541401274,0.920210616811388)
--(axis cs:59.8726114649682,0.904943067871922)
--(axis cs:59.2356687898089,0.907034928305192)
--(axis cs:58.5987261146497,0.898054989565255)
--(axis cs:57.9617834394904,0.890591822900804)
--(axis cs:57.3248407643312,0.889044649444542)
--(axis cs:56.687898089172,0.879305524540198)
--(axis cs:56.0509554140127,0.875746711788996)
--(axis cs:55.4140127388535,0.876916855170414)
--(axis cs:54.7770700636943,0.873583964932607)
--(axis cs:54.140127388535,0.868631728990772)
--(axis cs:53.5031847133758,0.865423610844293)
--(axis cs:52.8662420382166,0.863904099628866)
--(axis cs:52.2292993630573,0.858658324983143)
--(axis cs:51.5923566878981,0.861733725758031)
--(axis cs:50.9554140127388,0.854558826508069)
--(axis cs:50.3184713375796,0.849874223803329)
--(axis cs:49.6815286624204,0.851571515584178)
--(axis cs:49.0445859872611,0.847886648338107)
--(axis cs:48.4076433121019,0.846063285826377)
--(axis cs:47.7707006369427,0.83897038592041)
--(axis cs:47.1337579617834,0.833593881149013)
--(axis cs:46.4968152866242,0.825379109290296)
--(axis cs:45.859872611465,0.819280054961622)
--(axis cs:45.2229299363057,0.814855256073559)
--(axis cs:44.5859872611465,0.803789319517452)
--(axis cs:43.9490445859873,0.794086284663735)
--(axis cs:43.312101910828,0.783517828041347)
--(axis cs:42.6751592356688,0.77360261801184)
--(axis cs:42.0382165605096,0.772161829660633)
--(axis cs:41.4012738853503,0.771743543574621)
--(axis cs:40.7643312101911,0.770945556784095)
--(axis cs:40.1273885350318,0.773259642955923)
--(axis cs:39.4904458598726,0.776697500281682)
--(axis cs:38.8535031847134,0.765975200527853)
--(axis cs:38.2165605095541,0.760085272299953)
--(axis cs:37.5796178343949,0.750935038582205)
--(axis cs:36.9426751592357,0.752789306043347)
--(axis cs:36.3057324840764,0.742244012071225)
--(axis cs:35.6687898089172,0.731325173285578)
--(axis cs:35.031847133758,0.719451435055019)
--(axis cs:34.3949044585987,0.712489990599124)
--(axis cs:33.7579617834395,0.70568837333133)
--(axis cs:33.1210191082803,0.694958205020504)
--(axis cs:32.484076433121,0.684329302270083)
--(axis cs:31.8471337579618,0.671054455039724)
--(axis cs:31.2101910828025,0.661335644844248)
--(axis cs:30.5732484076433,0.655628554249815)
--(axis cs:29.9363057324841,0.644095293385852)
--(axis cs:29.2993630573248,0.631195212511952)
--(axis cs:28.6624203821656,0.617390355604739)
--(axis cs:28.0254777070064,0.614434189873437)
--(axis cs:27.3885350318471,0.590128694714312)
--(axis cs:26.7515923566879,0.579800696348377)
--(axis cs:26.1146496815287,0.569096664198613)
--(axis cs:25.4777070063694,0.544420764836612)
--(axis cs:24.8407643312102,0.525270990425186)
--(axis cs:24.203821656051,0.511578860096656)
--(axis cs:23.5668789808917,0.498140774768557)
--(axis cs:22.9299363057325,0.481041202379218)
--(axis cs:22.2929936305732,0.473294666290621)
--(axis cs:21.656050955414,0.451000132886019)
--(axis cs:21.0191082802548,0.433383738218276)
--(axis cs:20.3821656050955,0.411485513543388)
--(axis cs:19.7452229299363,0.403041501219266)
--(axis cs:19.1082802547771,0.389420694047805)
--(axis cs:18.4713375796178,0.368574316268211)
--(axis cs:17.8343949044586,0.349443007028703)
--(axis cs:17.1974522292994,0.326538551590074)
--(axis cs:16.5605095541401,0.314210930809838)
--(axis cs:15.9235668789809,0.30014508032951)
--(axis cs:15.2866242038217,0.284633000439838)
--(axis cs:14.6496815286624,0.267925497236876)
--(axis cs:14.0127388535032,0.251094037688074)
--(axis cs:13.3757961783439,0.230997736302762)
--(axis cs:12.7388535031847,0.214501076226832)
--(axis cs:12.1019108280255,0.196290617760353)
--(axis cs:11.4649681528662,0.179529376779984)
--(axis cs:10.828025477707,0.156786407476177)
--(axis cs:10.1910828025478,0.141127962156622)
--(axis cs:9.55414012738853,0.129112673816064)
--(axis cs:8.9171974522293,0.116015047321434)
--(axis cs:8.28025477707006,0.105574120997877)
--(axis cs:7.64331210191083,0.101081160022593)
--(axis cs:7.00636942675159,0.09544332911309)
--(axis cs:6.36942675159236,0.0886412162793399)
--(axis cs:5.73248407643312,0.0844531032016213)
--(axis cs:5.09554140127389,0.0823921356552506)
--(axis cs:4.45859872611465,0.0822849262428268)
--(axis cs:3.82165605095541,0.0813437921710326)
--(axis cs:3.18471337579618,0.0808120998582353)
--(axis cs:2.54777070063694,0.0802368812147328)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_guidedbackprop.tex <==
% guided backprop
\addplot [line width=0.5, opacity=0.8, color8, mark=oplus*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table [row sep=\\]{%
0	0.0799609375 \\
0.636942675159236	0.08 \\
1.27388535031847	0.0800390625 \\
1.91082802547771	0.08 \\
2.54777070063694	0.0801953125 \\
3.18471337579618	0.08 \\
3.82165605095541	0.079921875 \\
4.45859872611465	0.0805078125 \\
5.09554140127389	0.0804296875 \\
5.73248407643312	0.0802734375 \\
6.36942675159236	0.0805078125 \\
7.00636942675159	0.0805859375 \\
7.64331210191083	0.08109375 \\
8.28025477707006	0.080703125 \\
8.9171974522293	0.0808984375 \\
9.55414012738853	0.0816015625 \\
10.1910828025478	0.0821484375 \\
10.828025477707	0.0839453125 \\
11.4649681528662	0.0845703125 \\
12.1019108280255	0.0861328125 \\
12.7388535031847	0.0871484375 \\
13.3757961783439	0.0870703125 \\
14.0127388535032	0.08828125 \\
14.6496815286624	0.0893359375 \\
15.2866242038217	0.08953125 \\
15.9235668789809	0.0893359375 \\
16.5605095541401	0.08890625 \\
17.1974522292994	0.0895703125 \\
17.8343949044586	0.0887109375 \\
18.4713375796178	0.0886328125 \\
19.1082802547771	0.08671875 \\
19.7452229299363	0.0871484375 \\
20.3821656050955	0.0882421875 \\
21.0191082802548	0.0875390625 \\
21.656050955414	0.0876953125 \\
22.2929936305732	0.0860546875 \\
22.9299363057325	0.084921875 \\
23.5668789808917	0.08453125 \\
24.203821656051	0.0842578125 \\
24.8407643312102	0.0830078125 \\
25.4777070063694	0.0834765625 \\
26.1146496815287	0.0834375 \\
26.7515923566879	0.0824609375 \\
27.3885350318471	0.0820703125 \\
28.0254777070064	0.0823046875 \\
28.6624203821656	0.081875 \\
29.2993630573248	0.0824609375 \\
29.9363057324841	0.08234375 \\
30.5732484076433	0.081875 \\
31.2101910828025	0.081875 \\
31.8471337579618	0.081953125 \\
32.484076433121	0.0813671875 \\
33.1210191082803	0.0816796875 \\
33.7579617834395	0.0822265625 \\
34.3949044585987	0.08203125 \\
35.031847133758	0.081171875 \\
35.6687898089172	0.0815625 \\
36.3057324840764	0.081171875 \\
36.9426751592357	0.0812109375 \\
37.5796178343949	0.08171875 \\
38.2165605095541	0.0815625 \\
38.8535031847134	0.081328125 \\
39.4904458598726	0.08140625 \\
40.1273885350318	0.081484375 \\
40.7643312101911	0.081640625 \\
41.4012738853503	0.081796875 \\
42.0382165605096	0.0813671875 \\
42.6751592356688	0.0810546875 \\
43.312101910828	0.0809375 \\
43.9490445859873	0.08140625 \\
44.5859872611465	0.080625 \\
45.2229299363057	0.0808984375 \\
45.859872611465	0.081015625 \\
46.4968152866242	0.0804296875 \\
47.1337579617834	0.0805859375 \\
47.7707006369427	0.080390625 \\
48.4076433121019	0.0803125 \\
49.0445859872611	0.080859375 \\
49.6815286624204	0.0805078125 \\
50.3184713375796	0.0805859375 \\
50.9554140127388	0.080390625 \\
51.5923566878981	0.080390625 \\
52.2292993630573	0.0803515625 \\
52.8662420382166	0.080078125 \\
53.5031847133758	0.0800390625 \\
54.140127388535	0.0801171875 \\
54.7770700636943	0.0801953125 \\
55.4140127388535	0.08 \\
56.0509554140127	0.0801171875 \\
56.687898089172	0.080234375 \\
57.3248407643312	0.0801953125 \\
57.9617834394904	0.0801171875 \\
58.5987261146497	0.080078125 \\
59.2356687898089	0.0801171875 \\
59.8726114649682	0.08015625 \\
60.5095541401274	0.0800390625 \\
61.1464968152866	0.0799609375 \\
61.7834394904459	0.0800390625 \\
62.4203821656051	0.080078125 \\
63.0573248407643	0.0800390625 \\
63.6942675159236	0.0800390625 \\
64.3312101910828	0.08015625 \\
64.968152866242	0.08015625 \\
65.6050955414013	0.08015625 \\
66.2420382165605	0.08015625 \\
66.8789808917197	0.080078125 \\
67.515923566879	0.0802734375 \\
68.1528662420382	0.0807421875 \\
68.7898089171974	0.0803515625 \\
69.4267515923567	0.08078125 \\
70.0636942675159	0.080703125 \\
70.7006369426752	0.08109375 \\
71.3375796178344	0.0808203125 \\
71.9745222929936	0.0810546875 \\
72.6114649681529	0.081796875 \\
73.2484076433121	0.08140625 \\
73.8853503184713	0.081875 \\
74.5222929936306	0.08328125 \\
75.1592356687898	0.08234375 \\
75.796178343949	0.0831640625 \\
76.4331210191083	0.0860546875 \\
77.0700636942675	0.0855859375 \\
77.7070063694268	0.0874609375 \\
78.343949044586	0.0884765625 \\
78.9808917197452	0.090390625 \\
79.6178343949044	0.0998046875 \\
80.2547770700637	0.106875 \\
80.8917197452229	0.115859375 \\
81.5286624203822	0.1257421875 \\
82.1656050955414	0.1361328125 \\
82.8025477707006	0.156953125 \\
83.4394904458599	0.16796875 \\
84.0764331210191	0.176640625 \\
84.7133757961783	0.197109375 \\
85.3503184713376	0.2005859375 \\
85.9872611464968	0.215859375 \\
86.6242038216561	0.2296484375 \\
87.2611464968153	0.2609375 \\
87.8980891719745	0.2815234375 \\
88.5350318471338	0.292265625 \\
89.171974522293	0.3206640625 \\
89.8089171974522	0.35171875 \\
90.4458598726115	0.39890625 \\
91.0828025477707	0.42109375 \\
91.7197452229299	0.47140625 \\
92.3566878980892	0.511484375 \\
92.9936305732484	0.5566796875 \\
93.6305732484076	0.6012890625 \\
94.2675159235669	0.6421484375 \\
94.9044585987261	0.6933984375 \\
95.5414012738853	0.751875 \\
96.1783439490446	0.8236328125 \\
96.8152866242038	0.8816015625 \\
97.4522292993631	0.9396484375 \\
98.0891719745223	0.9582421875 \\
98.7261146496815	0.981171875 \\
99.3630573248408	0.99171875 \\
100	1 \\
};
\path [fill=color8, fill opacity=0.5] (axis cs:0,0.0802368812147328)
--(axis cs:0,0.0796849937852672)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0794483826402493)
--(axis cs:2.54777070063694,0.0794658466226402)
--(axis cs:3.18471337579618,0.0796097566561732)
--(axis cs:3.82165605095541,0.0795320136859699)
--(axis cs:4.45859872611465,0.0795151323955609)
--(axis cs:5.09554140127389,0.0793634747691256)
--(axis cs:5.73248407643312,0.0794468673331431)
--(axis cs:6.36942675159236,0.0794411805779433)
--(axis cs:7.00636942675159,0.0793242358512974)
--(axis cs:7.64331210191083,0.0795424481168043)
--(axis cs:8.28025477707006,0.0791476024014316)
--(axis cs:8.9171974522293,0.0793664186033662)
--(axis cs:9.55414012738853,0.0798024846187187)
--(axis cs:10.1910828025478,0.0799776099555934)
--(axis cs:10.828025477707,0.0811413863851592)
--(axis cs:11.4649681528662,0.0815954261753419)
--(axis cs:12.1019108280255,0.0826168696229322)
--(axis cs:12.7388535031847,0.0835214287962932)
--(axis cs:13.3757961783439,0.0834238003045823)
--(axis cs:14.0127388535032,0.084531246821087)
--(axis cs:14.6496815286624,0.085298509201592)
--(axis cs:15.2866242038217,0.0854106943201532)
--(axis cs:15.9235668789809,0.0852716926507086)
--(axis cs:16.5605095541401,0.0849724785429137)
--(axis cs:17.1974522292994,0.0856177783246586)
--(axis cs:17.8343949044586,0.0849644128691229)
--(axis cs:18.4713375796178,0.0848373286594136)
--(axis cs:19.1082802547771,0.083249160387083)
--(axis cs:19.7452229299363,0.0834973513886621)
--(axis cs:20.3821656050955,0.0846599905536999)
--(axis cs:21.0191082802548,0.0842020745245122)
--(axis cs:21.656050955414,0.0842637902998366)
--(axis cs:22.2929936305732,0.0827994359337181)
--(axis cs:22.9299363057325,0.081980056447104)
--(axis cs:23.5668789808917,0.0816534957809791)
--(axis cs:24.203821656051,0.0814102231885198)
--(axis cs:24.8407643312102,0.0805973333392693)
--(axis cs:25.4777070063694,0.0808008269153788)
--(axis cs:26.1146496815287,0.0808673473280304)
--(axis cs:26.7515923566879,0.0802971228455717)
--(axis cs:27.3885350318471,0.0800534168670263)
--(axis cs:28.0254777070064,0.0802039783607906)
--(axis cs:28.6624203821656,0.0799823195856138)
--(axis cs:29.2993630573248,0.0802967785467717)
--(axis cs:29.9363057324841,0.0801972554062174)
--(axis cs:30.5732484076433,0.079984446503281)
--(axis cs:31.2101910828025,0.0799458255600451)
--(axis cs:31.8471337579618,0.0799132720024117)
--(axis cs:32.484076433121,0.0796193639802044)
--(axis cs:33.1210191082803,0.079847778519601)
--(axis cs:33.7579617834395,0.0801065768331437)
--(axis cs:34.3949044585987,0.0800728677931587)
--(axis cs:35.031847133758,0.0795304945005887)
--(axis cs:35.6687898089172,0.0798007923473361)
--(axis cs:36.3057324840764,0.0796741364359903)
--(axis cs:36.9426751592357,0.0795934713115423)
--(axis cs:37.5796178343949,0.0798352244607436)
--(axis cs:38.2165605095541,0.0798033316860692)
--(axis cs:38.8535031847134,0.0796866537187795)
--(axis cs:39.4904458598726,0.0797219450786497)
--(axis cs:40.1273885350318,0.0796923096383298)
--(axis cs:40.7643312101911,0.0798267406620111)
--(axis cs:41.4012738853503,0.0798471098234276)
--(axis cs:42.0382165605096,0.0797582192796155)
--(axis cs:42.6751592356688,0.0796387244924916)
--(axis cs:43.312101910828,0.0795423692981873)
--(axis cs:43.9490445859873,0.0797756172383304)
--(axis cs:44.5859872611465,0.0794614195317585)
--(axis cs:45.2229299363057,0.0795876160410428)
--(axis cs:45.859872611465,0.0796291727671386)
--(axis cs:46.4968152866242,0.0795188924387148)
--(axis cs:47.1337579617834,0.0795218232020411)
--(axis cs:47.7707006369427,0.0795210935635494)
--(axis cs:48.4076433121019,0.0795373775455865)
--(axis cs:49.0445859872611,0.0795768812680165)
--(axis cs:49.6815286624204,0.0795187416064964)
--(axis cs:50.3184713375796,0.079524066101224)
--(axis cs:50.9554140127388,0.0795207508910488)
--(axis cs:51.5923566878981,0.0795200659506994)
--(axis cs:52.2292993630573,0.07952661642193)
--(axis cs:52.8662420382166,0.0796882636859699)
--(axis cs:53.5031847133758,0.0797631187852672)
--(axis cs:54.140127388535,0.0796392389660534)
--(axis cs:54.7770700636943,0.0795790085175115)
--(axis cs:55.4140127388535,0.08)
--(axis cs:56.0509554140127,0.0796392389660534)
--(axis cs:56.687898089172,0.079561768685842)
--(axis cs:57.3248407643312,0.0795790085175115)
--(axis cs:57.9617834394904,0.079640175203062)
--(axis cs:58.5987261146497,0.0796882636859699)
--(axis cs:59.2356687898089,0.079640175203062)
--(axis cs:59.8726114649682,0.0796043625705343)
--(axis cs:60.5095541401274,0.0797631187852672)
--(axis cs:61.1464968152866,0.0796849937852672)
--(axis cs:61.7834394904459,0.0797631187852672)
--(axis cs:62.4203821656051,0.0796882636859699)
--(axis cs:63.0573248407643,0.0797631187852672)
--(axis cs:63.6942675159236,0.0797631187852672)
--(axis cs:64.3312101910828,0.0796051731767434)
--(axis cs:64.968152866242,0.0796051731767434)
--(axis cs:65.6050955414013,0.0796051731767434)
--(axis cs:66.2420382165605,0.0796046326402493)
--(axis cs:66.8789808917197,0.0796882636859699)
--(axis cs:67.515923566879,0.0795441759262088)
--(axis cs:68.1528662420382,0.0795477059453869)
--(axis cs:68.7898089171974,0.0795249923331431)
--(axis cs:69.4267515923567,0.0795533658484639)
--(axis cs:70.0636942675159,0.0795376251696992)
--(axis cs:70.7006369426752,0.0796439369782609)
--(axis cs:71.3375796178344,0.0795614485307938)
--(axis cs:71.9745222929936,0.0796292846345682)
--(axis cs:72.6114649681529,0.0799479227558648)
--(axis cs:73.2484076433121,0.0797669588697554)
--(axis cs:73.8853503184713,0.0799872861212841)
--(axis cs:74.5222929936306,0.0808061408327077)
--(axis cs:75.1592356687898,0.0802417998830905)
--(axis cs:75.796178343949,0.0807316755957397)
--(axis cs:76.4331210191083,0.0827482040271373)
--(axis cs:77.0700636942675,0.0823936412842862)
--(axis cs:77.7070063694268,0.0838019015175232)
--(axis cs:78.343949044586,0.0845820603596542)
--(axis cs:78.9808917197452,0.0860881010255035)
--(axis cs:79.6178343949044,0.0942139071670029)
--(axis cs:80.2547770700637,0.101139617592641)
--(axis cs:80.8917197452229,0.109231035714239)
--(axis cs:81.5286624203822,0.118191657609777)
--(axis cs:82.1656050955414,0.128127317066001)
--(axis cs:82.8025477707006,0.148734846034331)
--(axis cs:83.4394904458599,0.159721348680507)
--(axis cs:84.0764331210191,0.168454174458445)
--(axis cs:84.7133757961783,0.189139408129686)
--(axis cs:85.3503184713376,0.192262165269516)
--(axis cs:85.9872611464968,0.207402042808337)
--(axis cs:86.6242038216561,0.221084937536894)
--(axis cs:87.2611464968153,0.251639699901799)
--(axis cs:87.8980891719745,0.27224719405425)
--(axis cs:88.5350318471338,0.283312734956479)
--(axis cs:89.171974522293,0.311395066654124)
--(axis cs:89.8089171974522,0.342578381272999)
--(axis cs:90.4458598726115,0.389366847538738)
--(axis cs:91.0828025477707,0.411182858396273)
--(axis cs:91.7197452229299,0.460691563522931)
--(axis cs:92.3566878980892,0.50048202665427)
--(axis cs:92.9936305732484,0.546009240856223)
--(axis cs:93.6305732484076,0.590671071232448)
--(axis cs:94.2675159235669,0.631304408700883)
--(axis cs:94.9044585987261,0.682841274898987)
--(axis cs:95.5414012738853,0.741938821484603)
--(axis cs:96.1783439490446,0.814823690629031)
--(axis cs:96.8152866242038,0.873261354619634)
--(axis cs:97.4522292993631,0.933091579773798)
--(axis cs:98.0891719745223,0.953671750453462)
--(axis cs:98.7261146496815,0.978425374350164)
--(axis cs:99.3630573248408,0.988640253854268)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,0.994797246145732)
--(axis cs:98.7261146496815,0.983918375649836)
--(axis cs:98.0891719745223,0.962812624546538)
--(axis cs:97.4522292993631,0.946205295226202)
--(axis cs:96.8152866242038,0.889941770380366)
--(axis cs:96.1783439490446,0.832441934370969)
--(axis cs:95.5414012738853,0.761811178515397)
--(axis cs:94.9044585987261,0.703955600101013)
--(axis cs:94.2675159235669,0.652992466299117)
--(axis cs:93.6305732484076,0.611907053767552)
--(axis cs:92.9936305732484,0.567350134143777)
--(axis cs:92.3566878980892,0.52248672334573)
--(axis cs:91.7197452229299,0.482120936477069)
--(axis cs:91.0828025477707,0.431004641603727)
--(axis cs:90.4458598726115,0.408445652461262)
--(axis cs:89.8089171974522,0.360859118727001)
--(axis cs:89.171974522293,0.329933058345876)
--(axis cs:88.5350318471338,0.301218515043521)
--(axis cs:87.8980891719745,0.29079968094575)
--(axis cs:87.2611464968153,0.270235300098201)
--(axis cs:86.6242038216561,0.238211937463106)
--(axis cs:85.9872611464968,0.224316707191663)
--(axis cs:85.3503184713376,0.208909709730484)
--(axis cs:84.7133757961783,0.205079341870314)
--(axis cs:84.0764331210191,0.184827075541555)
--(axis cs:83.4394904458599,0.176216151319493)
--(axis cs:82.8025477707006,0.165171403965669)
--(axis cs:82.1656050955414,0.144138307933999)
--(axis cs:81.5286624203822,0.133292717390223)
--(axis cs:80.8917197452229,0.122487714285761)
--(axis cs:80.2547770700637,0.112610382407359)
--(axis cs:79.6178343949044,0.105395467832997)
--(axis cs:78.9808917197452,0.0946931489744965)
--(axis cs:78.343949044586,0.0923710646403458)
--(axis cs:77.7070063694268,0.0911199734824768)
--(axis cs:77.0700636942675,0.0887782337157138)
--(axis cs:76.4331210191083,0.0893611709728627)
--(axis cs:75.796178343949,0.0855964494042603)
--(axis cs:75.1592356687898,0.0844457001169095)
--(axis cs:74.5222929936306,0.0857563591672924)
--(axis cs:73.8853503184713,0.0837627138787159)
--(axis cs:73.2484076433121,0.0830455411302446)
--(axis cs:72.6114649681529,0.0836458272441352)
--(axis cs:71.9745222929936,0.0824800903654318)
--(axis cs:71.3375796178344,0.0820791764692062)
--(axis cs:70.7006369426752,0.0825435630217391)
--(axis cs:70.0636942675159,0.0818686248303008)
--(axis cs:69.4267515923567,0.0820091341515361)
--(axis cs:68.7898089171974,0.0811781326668569)
--(axis cs:68.1528662420382,0.0819366690546131)
--(axis cs:67.515923566879,0.0810026990737912)
--(axis cs:66.8789808917197,0.0804679863140301)
--(axis cs:66.2420382165605,0.0807078673597507)
--(axis cs:65.6050955414013,0.0807073268232566)
--(axis cs:64.968152866242,0.0807073268232566)
--(axis cs:64.3312101910828,0.0807073268232566)
--(axis cs:63.6942675159236,0.0803150062147328)
--(axis cs:63.0573248407643,0.0803150062147328)
--(axis cs:62.4203821656051,0.0804679863140301)
--(axis cs:61.7834394904459,0.0803150062147328)
--(axis cs:61.1464968152866,0.0802368812147328)
--(axis cs:60.5095541401274,0.0803150062147328)
--(axis cs:59.8726114649682,0.0807081374294657)
--(axis cs:59.2356687898089,0.080594199796938)
--(axis cs:58.5987261146497,0.0804679863140301)
--(axis cs:57.9617834394904,0.080594199796938)
--(axis cs:57.3248407643312,0.0808116164824885)
--(axis cs:56.687898089172,0.080906981314158)
--(axis cs:56.0509554140127,0.0805951360339466)
--(axis cs:55.4140127388535,0.08)
--(axis cs:54.7770700636943,0.0808116164824885)
--(axis cs:54.140127388535,0.0805951360339466)
--(axis cs:53.5031847133758,0.0803150062147328)
--(axis cs:52.8662420382166,0.0804679863140301)
--(axis cs:52.2292993630573,0.08117650857807)
--(axis cs:51.5923566878981,0.0812611840493005)
--(axis cs:50.9554140127388,0.0812604991089512)
--(axis cs:50.3184713375796,0.081647808898776)
--(axis cs:49.6815286624204,0.0814968833935036)
--(axis cs:49.0445859872611,0.0821418687319835)
--(axis cs:48.4076433121019,0.0810876224544134)
--(axis cs:47.7707006369427,0.0812601564364506)
--(axis cs:47.1337579617834,0.0816500517979589)
--(axis cs:46.4968152866242,0.0813404825612852)
--(axis cs:45.859872611465,0.0824020772328614)
--(axis cs:45.2229299363057,0.0822092589589572)
--(axis cs:44.5859872611465,0.0817885804682415)
--(axis cs:43.9490445859873,0.0830368827616696)
--(axis cs:43.312101910828,0.0823326307018127)
--(axis cs:42.6751592356688,0.0824706505075084)
--(axis cs:42.0382165605096,0.0829761557203845)
--(axis cs:41.4012738853503,0.0837466401765724)
--(axis cs:40.7643312101911,0.0834545093379889)
--(axis cs:40.1273885350318,0.0832764403616702)
--(axis cs:39.4904458598726,0.0830905549213503)
--(axis cs:38.8535031847134,0.0829695962812205)
--(axis cs:38.2165605095541,0.0833216683139308)
--(axis cs:37.5796178343949,0.0836022755392564)
--(axis cs:36.9426751592357,0.0828284036884577)
--(axis cs:36.3057324840764,0.0826696135640097)
--(axis cs:35.6687898089172,0.0833242076526639)
--(axis cs:35.031847133758,0.0828132554994113)
--(axis cs:34.3949044585987,0.0839896322068413)
--(axis cs:33.7579617834395,0.0843465481668564)
--(axis cs:33.1210191082803,0.083511596480399)
--(axis cs:32.484076433121,0.0831150110197956)
--(axis cs:31.8471337579618,0.0839929779975883)
--(axis cs:31.2101910828025,0.0838041744399549)
--(axis cs:30.5732484076433,0.083765553496719)
--(axis cs:29.9363057324841,0.0844902445937825)
--(axis cs:29.2993630573248,0.0846250964532283)
--(axis cs:28.6624203821656,0.0837676804143862)
--(axis cs:28.0254777070064,0.0844053966392094)
--(axis cs:27.3885350318471,0.0840872081329737)
--(axis cs:26.7515923566879,0.0846247521544283)
--(axis cs:26.1146496815287,0.0860076526719696)
--(axis cs:25.4777070063694,0.0861522980846212)
--(axis cs:24.8407643312102,0.0854182916607307)
--(axis cs:24.203821656051,0.0871054018114802)
--(axis cs:23.5668789808917,0.0874090042190209)
--(axis cs:22.9299363057325,0.0878636935528959)
--(axis cs:22.2929936305732,0.0893099390662819)
--(axis cs:21.656050955414,0.0911268347001634)
--(axis cs:21.0191082802548,0.0908760504754878)
--(axis cs:20.3821656050955,0.0918243844463001)
--(axis cs:19.7452229299363,0.0907995236113378)
--(axis cs:19.1082802547771,0.090188339612917)
--(axis cs:18.4713375796178,0.0924282963405864)
--(axis cs:17.8343949044586,0.0924574621308771)
--(axis cs:17.1974522292994,0.0935228466753414)
--(axis cs:16.5605095541401,0.0928400214570863)
--(axis cs:15.9235668789809,0.0934001823492915)
--(axis cs:15.2866242038217,0.0936518056798468)
--(axis cs:14.6496815286624,0.093373365798408)
--(axis cs:14.0127388535032,0.092031253178913)
--(axis cs:13.3757961783439,0.0907168246954177)
--(axis cs:12.7388535031847,0.0907754462037067)
--(axis cs:12.1019108280255,0.0896487553770678)
--(axis cs:11.4649681528662,0.0875451988246581)
--(axis cs:10.828025477707,0.0867492386148408)
--(axis cs:10.1910828025478,0.0843192650444066)
--(axis cs:9.55414012738853,0.0834006403812813)
--(axis cs:8.9171974522293,0.0824304563966338)
--(axis cs:8.28025477707006,0.0822586475985684)
--(axis cs:7.64331210191083,0.0826450518831957)
--(axis cs:7.00636942675159,0.0818476391487026)
--(axis cs:6.36942675159236,0.0815744444220566)
--(axis cs:5.73248407643312,0.0811000076668569)
--(axis cs:5.09554140127389,0.0814959002308744)
--(axis cs:4.45859872611465,0.0815004926044391)
--(axis cs:3.82165605095541,0.0803117363140301)
--(axis cs:3.18471337579618,0.0803902433438268)
--(axis cs:2.54777070063694,0.0809247783773598)
--(axis cs:1.91082802547771,0.0805516173597507)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0802368812147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_lafw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.08
0.636942675159236 0.08
1.27388535031847 0.0800390625
1.91082802547771 0.0800390625
2.54777070063694 0.08015625
3.18471337579618 0.0801171875
3.82165605095541 0.0803125
4.45859872611465 0.080546875
5.09554140127389 0.080859375
5.73248407643312 0.0810546875
6.36942675159236 0.0828125
7.00636942675159 0.084765625
7.64331210191083 0.0883203125
8.28025477707006 0.0920703125
8.9171974522293 0.095703125
9.55414012738853 0.1003515625
10.1910828025478 0.1066015625
10.828025477707 0.1152734375
11.4649681528662 0.1259765625
12.1019108280255 0.1396484375
12.7388535031847 0.151484375
13.3757961783439 0.17125
14.0127388535032 0.186015625
14.6496815286624 0.2056640625
15.2866242038217 0.227109375
15.9235668789809 0.24390625
16.5605095541401 0.26046875
17.1974522292994 0.2869921875
17.8343949044586 0.3034765625
18.4713375796178 0.31984375
19.1082802547771 0.3401171875
19.7452229299363 0.3516015625
20.3821656050955 0.36328125
21.0191082802548 0.37921875
21.656050955414 0.4034765625
22.2929936305732 0.419921875
22.9299363057325 0.4337109375
23.5668789808917 0.4560546875
24.203821656051 0.4736328125
24.8407643312102 0.490625
25.4777070063694 0.501953125
26.1146496815287 0.523359375
26.7515923566879 0.5391015625
27.3885350318471 0.56453125
28.0254777070064 0.5744921875
28.6624203821656 0.597890625
29.2993630573248 0.6148828125
29.9363057324841 0.6244921875
30.5732484076433 0.6401953125
31.2101910828025 0.6640625
31.8471337579618 0.675234375
32.484076433121 0.6897265625
33.1210191082803 0.7035546875
33.7579617834395 0.720390625
34.3949044585987 0.734140625
35.031847133758 0.75234375
35.6687898089172 0.76375
36.3057324840764 0.775234375
36.9426751592357 0.783046875
37.5796178343949 0.7903515625
38.2165605095541 0.796953125
38.8535031847134 0.81078125
39.4904458598726 0.8148046875
40.1273885350318 0.8205078125
40.7643312101911 0.8306640625
41.4012738853503 0.8358203125
42.0382165605096 0.841953125
42.6751592356688 0.846328125
43.312101910828 0.85640625
43.9490445859873 0.8589453125
44.5859872611465 0.8601171875
45.2229299363057 0.8609375
45.859872611465 0.8634765625
46.4968152866242 0.8663671875
47.1337579617834 0.8647265625
47.7707006369427 0.8683203125
48.4076433121019 0.870859375
49.0445859872611 0.8741796875
49.6815286624204 0.8783984375
50.3184713375796 0.883359375
50.9554140127388 0.887734375
51.5923566878981 0.8889453125
52.2292993630573 0.8841796875
52.8662420382166 0.886875
53.5031847133758 0.88375
54.140127388535 0.88703125
54.7770700636943 0.8908203125
55.4140127388535 0.8974609375
56.0509554140127 0.8969921875
56.687898089172 0.8975390625
57.3248407643312 0.8943359375
57.9617834394904 0.8993359375
58.5987261146497 0.8996484375
59.2356687898089 0.8966796875
59.8726114649682 0.8934375
60.5095541401274 0.898125
61.1464968152866 0.8962109375
61.7834394904459 0.8993359375
62.4203821656051 0.9054296875
63.0573248407643 0.912421875
63.6942675159236 0.9190625
64.3312101910828 0.9252734375
64.968152866242 0.9311328125
65.6050955414013 0.934921875
66.2420382165605 0.9299609375
66.8789808917197 0.93375
67.515923566879 0.9374609375
68.1528662420382 0.941171875
68.7898089171974 0.9348828125
69.4267515923567 0.9376171875
70.0636942675159 0.9404296875
70.7006369426752 0.9365234375
71.3375796178344 0.9413671875
71.9745222929936 0.947421875
72.6114649681529 0.9553515625
73.2484076433121 0.9565234375
73.8853503184713 0.95515625
74.5222929936306 0.959609375
75.1592356687898 0.96234375
75.796178343949 0.9617578125
76.4331210191083 0.960703125
77.0700636942675 0.9570703125
77.7070063694268 0.9578515625
78.343949044586 0.955859375
78.9808917197452 0.952890625
79.6178343949044 0.9557421875
80.2547770700637 0.959140625
80.8917197452229 0.960390625
81.5286624203822 0.9609765625
82.1656050955414 0.957890625
82.8025477707006 0.9573828125
83.4394904458599 0.9591796875
84.0764331210191 0.9624609375
84.7133757961783 0.9653125
85.3503184713376 0.969609375
85.9872611464968 0.9709375
86.6242038216561 0.9736328125
87.2611464968153 0.9765234375
87.8980891719745 0.980078125
88.5350318471338 0.98046875
89.171974522293 0.9826171875
89.8089171974522 0.9841015625
90.4458598726115 0.9830859375
91.0828025477707 0.983984375
91.7197452229299 0.986875
92.3566878980892 0.990859375
92.9936305732484 0.9944921875
93.6305732484076 0.9995703125
94.2675159235669 0.9999609375
94.9044585987261 1
95.5414012738853 1
96.1783439490446 0.9999609375
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color1, fill opacity=0.25]
(axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.0796097566561732)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0794805491941847)
--(axis cs:3.18471337579618,0.0795016092928163)
--(axis cs:3.82165605095541,0.0794412565488254)
--(axis cs:4.45859872611465,0.0793160817407698)
--(axis cs:5.09554140127389,0.0794596590739039)
--(axis cs:5.73248407643312,0.079340522987529)
--(axis cs:6.36942675159236,0.0803751865360526)
--(axis cs:7.00636942675159,0.0816277768088909)
--(axis cs:7.64331210191083,0.0843443229503481)
--(axis cs:8.28025477707006,0.0873588886417152)
--(axis cs:8.9171974522293,0.0904788008437958)
--(axis cs:9.55414012738853,0.0944683179672034)
--(axis cs:10.1910828025478,0.0999885166883834)
--(axis cs:10.828025477707,0.10782017768326)
--(axis cs:11.4649681528662,0.117688473700241)
--(axis cs:12.1019108280255,0.130522973333694)
--(axis cs:12.7388535031847,0.141857135909294)
--(axis cs:13.3757961783439,0.16110246885851)
--(axis cs:14.0127388535032,0.175520346363344)
--(axis cs:14.6496815286624,0.194677510581706)
--(axis cs:15.2866242038217,0.215601102818737)
--(axis cs:15.9235668789809,0.232115812226383)
--(axis cs:16.5605095541401,0.248626646131103)
--(axis cs:17.1974522292994,0.274922174006835)
--(axis cs:17.8343949044586,0.291501663940716)
--(axis cs:18.4713375796178,0.307882715485989)
--(axis cs:19.1082802547771,0.327816999743507)
--(axis cs:19.7452229299363,0.339561920368105)
--(axis cs:20.3821656050955,0.351109719591036)
--(axis cs:21.0191082802548,0.366683834678562)
--(axis cs:21.656050955414,0.390763579708404)
--(axis cs:22.2929936305732,0.407301859035955)
--(axis cs:22.9299363057325,0.420958982795135)
--(axis cs:23.5668789808917,0.443517258177069)
--(axis cs:24.203821656051,0.461351052709779)
--(axis cs:24.8407643312102,0.478340249849127)
--(axis cs:25.4777070063694,0.489848771675048)
--(axis cs:26.1146496815287,0.511325025090848)
--(axis cs:26.7515923566879,0.526929940271615)
--(axis cs:27.3885350318471,0.552272108297164)
--(axis cs:28.0254777070064,0.562301750781455)
--(axis cs:28.6624203821656,0.585591981949487)
--(axis cs:29.2993630573248,0.602421262989305)
--(axis cs:29.9363057324841,0.612120790418436)
--(axis cs:30.5732484076433,0.627637801150252)
--(axis cs:31.2101910828025,0.651499667727182)
--(axis cs:31.8471337579618,0.662728987900946)
--(axis cs:32.484076433121,0.677150541445965)
--(axis cs:33.1210191082803,0.691319545307074)
--(axis cs:33.7579617834395,0.708564878009897)
--(axis cs:34.3949044585987,0.722279560837651)
--(axis cs:35.031847133758,0.741114820502904)
--(axis cs:35.6687898089172,0.752879064661838)
--(axis cs:36.3057324840764,0.764369541140623)
--(axis cs:36.9426751592357,0.772368938821258)
--(axis cs:37.5796178343949,0.77931024369002)
--(axis cs:38.2165605095541,0.786288412484218)
--(axis cs:38.8535031847134,0.800462676016393)
--(axis cs:39.4904458598726,0.804788440848613)
--(axis cs:40.1273885350318,0.810493500044203)
--(axis cs:40.7643312101911,0.820931521188886)
--(axis cs:41.4012738853503,0.826330486010398)
--(axis cs:42.0382165605096,0.832483111878095)
--(axis cs:42.6751592356688,0.836973603680827)
--(axis cs:43.312101910828,0.847634939531391)
--(axis cs:43.9490445859873,0.850431094154556)
--(axis cs:44.5859872611465,0.851309605083456)
--(axis cs:45.2229299363057,0.852255974717794)
--(axis cs:45.859872611465,0.854810885676949)
--(axis cs:46.4968152866242,0.858158623818017)
--(axis cs:47.1337579617834,0.856716247577429)
--(axis cs:47.7707006369427,0.860558262640572)
--(axis cs:48.4076433121019,0.862985792529818)
--(axis cs:49.0445859872611,0.866309067430385)
--(axis cs:49.6815286624204,0.870673431136618)
--(axis cs:50.3184713375796,0.87564302483309)
--(axis cs:50.9554140127388,0.88023343489499)
--(axis cs:51.5923566878981,0.881736308628833)
--(axis cs:52.2292993630573,0.876842489933742)
--(axis cs:52.8662420382166,0.879908153058214)
--(axis cs:53.5031847133758,0.8769020186663)
--(axis cs:54.140127388535,0.879778033772606)
--(axis cs:54.7770700636943,0.883522110416434)
--(axis cs:55.4140127388535,0.889840024245389)
--(axis cs:56.0509554140127,0.889174472641953)
--(axis cs:56.687898089172,0.889887629486737)
--(axis cs:57.3248407643312,0.886535377089141)
--(axis cs:57.9617834394904,0.891740446423729)
--(axis cs:58.5987261146497,0.892104995892499)
--(axis cs:59.2356687898089,0.889539116774083)
--(axis cs:59.8726114649682,0.886526314854601)
--(axis cs:60.5095541401274,0.890834570944321)
--(axis cs:61.1464968152866,0.889306320780564)
--(axis cs:61.7834394904459,0.892313816911131)
--(axis cs:62.4203821656051,0.89828751009531)
--(axis cs:63.0573248407643,0.905299995436425)
--(axis cs:63.6942675159236,0.912434273120129)
--(axis cs:64.3312101910828,0.918588541288219)
--(axis cs:64.968152866242,0.924509949596984)
--(axis cs:65.6050955414013,0.928373533718094)
--(axis cs:66.2420382165605,0.923261901591046)
--(axis cs:66.8789808917197,0.927325180728649)
--(axis cs:67.515923566879,0.931142304085921)
--(axis cs:68.1528662420382,0.934944326672644)
--(axis cs:68.7898089171974,0.928862914079877)
--(axis cs:69.4267515923567,0.93170428250351)
--(axis cs:70.0636942675159,0.934897235225154)
--(axis cs:70.7006369426752,0.930818938851851)
--(axis cs:71.3375796178344,0.9354173522387)
--(axis cs:71.9745222929936,0.941518566803672)
--(axis cs:72.6114649681529,0.950195583581825)
--(axis cs:73.2484076433121,0.951631067093863)
--(axis cs:73.8853503184713,0.950184255591579)
--(axis cs:74.5222929936306,0.954895943209136)
--(axis cs:75.1592356687898,0.957760859135109)
--(axis cs:75.796178343949,0.957122788106536)
--(axis cs:76.4331210191083,0.956086284411662)
--(axis cs:77.0700636942675,0.952489161505214)
--(axis cs:77.7070063694268,0.953623398581809)
--(axis cs:78.343949044586,0.951829982091187)
--(axis cs:78.9808917197452,0.948704129353734)
--(axis cs:79.6178343949044,0.95179965655492)
--(axis cs:80.2547770700637,0.955950967210093)
--(axis cs:80.8917197452229,0.957669360391974)
--(axis cs:81.5286624203822,0.957988581454328)
--(axis cs:82.1656050955414,0.954498871107856)
--(axis cs:82.8025477707006,0.953620214167007)
--(axis cs:83.4394904458599,0.956135972512386)
--(axis cs:84.0764331210191,0.959653453000758)
--(axis cs:84.7133757961783,0.962202652473508)
--(axis cs:85.3503184713376,0.96606239735756)
--(axis cs:85.9872611464968,0.967347553441438)
--(axis cs:86.6242038216561,0.969696901399793)
--(axis cs:87.2611464968153,0.972488630489015)
--(axis cs:87.8980891719745,0.976901903321424)
--(axis cs:88.5350318471338,0.978461741805218)
--(axis cs:89.171974522293,0.980221528460443)
--(axis cs:89.8089171974522,0.981439785816497)
--(axis cs:90.4458598726115,0.980799895890078)
--(axis cs:91.0828025477707,0.981488044570897)
--(axis cs:91.7197452229299,0.983906507001256)
--(axis cs:92.3566878980892,0.987745935843726)
--(axis cs:92.9936305732484,0.991700244371619)
--(axis cs:93.6305732484076,0.998664109987648)
--(axis cs:94.2675159235669,0.999684993785267)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,0.999684993785267)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1.00023688121473)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1.00023688121473)
--(axis cs:93.6305732484076,1.00047651501235)
--(axis cs:92.9936305732484,0.997284130628381)
--(axis cs:92.3566878980892,0.993972814156274)
--(axis cs:91.7197452229299,0.989843492998744)
--(axis cs:91.0828025477707,0.986480705429103)
--(axis cs:90.4458598726115,0.985371979109922)
--(axis cs:89.8089171974522,0.986763339183503)
--(axis cs:89.171974522293,0.985012846539557)
--(axis cs:88.5350318471338,0.982475758194782)
--(axis cs:87.8980891719745,0.983254346678576)
--(axis cs:87.2611464968153,0.980558244510985)
--(axis cs:86.6242038216561,0.977568723600207)
--(axis cs:85.9872611464968,0.974527446558562)
--(axis cs:85.3503184713376,0.973156352642439)
--(axis cs:84.7133757961783,0.968422347526492)
--(axis cs:84.0764331210191,0.965268421999242)
--(axis cs:83.4394904458599,0.962223402487614)
--(axis cs:82.8025477707006,0.961145410832993)
--(axis cs:82.1656050955414,0.961282378892144)
--(axis cs:81.5286624203822,0.963964543545672)
--(axis cs:80.8917197452229,0.963111889608026)
--(axis cs:80.2547770700637,0.962330282789907)
--(axis cs:79.6178343949044,0.95968471844508)
--(axis cs:78.9808917197452,0.957077120646266)
--(axis cs:78.343949044586,0.959888767908813)
--(axis cs:77.7070063694268,0.962079726418191)
--(axis cs:77.0700636942675,0.961651463494786)
--(axis cs:76.4331210191083,0.965319965588338)
--(axis cs:75.796178343949,0.966392836893464)
--(axis cs:75.1592356687898,0.966926640864891)
--(axis cs:74.5222929936306,0.964322806790864)
--(axis cs:73.8853503184713,0.960128244408421)
--(axis cs:73.2484076433121,0.961415807906137)
--(axis cs:72.6114649681529,0.960507541418175)
--(axis cs:71.9745222929936,0.953325183196328)
--(axis cs:71.3375796178344,0.9473170227613)
--(axis cs:70.7006369426752,0.942227936148149)
--(axis cs:70.0636942675159,0.945962139774846)
--(axis cs:69.4267515923567,0.94353009249649)
--(axis cs:68.7898089171974,0.940902710920123)
--(axis cs:68.1528662420382,0.947399423327356)
--(axis cs:67.515923566879,0.943779570914079)
--(axis cs:66.8789808917197,0.940174819271351)
--(axis cs:66.2420382165605,0.936659973408954)
--(axis cs:65.6050955414013,0.941470216281906)
--(axis cs:64.968152866242,0.937755675403016)
--(axis cs:64.3312101910828,0.931958333711781)
--(axis cs:63.6942675159236,0.925690726879871)
--(axis cs:63.0573248407643,0.919543754563575)
--(axis cs:62.4203821656051,0.91257186490469)
--(axis cs:61.7834394904459,0.906358058088869)
--(axis cs:61.1464968152866,0.903115554219436)
--(axis cs:60.5095541401274,0.905415429055679)
--(axis cs:59.8726114649682,0.900348685145399)
--(axis cs:59.2356687898089,0.903820258225917)
--(axis cs:58.5987261146497,0.907191879107501)
--(axis cs:57.9617834394904,0.906931428576271)
--(axis cs:57.3248407643312,0.902136497910859)
--(axis cs:56.687898089172,0.905190495513263)
--(axis cs:56.0509554140127,0.904809902358047)
--(axis cs:55.4140127388535,0.905081850754611)
--(axis cs:54.7770700636943,0.898118514583566)
--(axis cs:54.140127388535,0.894284466227394)
--(axis cs:53.5031847133758,0.8905979813337)
--(axis cs:52.8662420382166,0.893841846941786)
--(axis cs:52.2292993630573,0.891516885066258)
--(axis cs:51.5923566878981,0.896154316371167)
--(axis cs:50.9554140127388,0.89523531510501)
--(axis cs:50.3184713375796,0.89107572516691)
--(axis cs:49.6815286624204,0.886123443863382)
--(axis cs:49.0445859872611,0.882050307569615)
--(axis cs:48.4076433121019,0.878732957470182)
--(axis cs:47.7707006369427,0.876082362359428)
--(axis cs:47.1337579617834,0.872736877422571)
--(axis cs:46.4968152866242,0.874575751181983)
--(axis cs:45.859872611465,0.872142239323051)
--(axis cs:45.2229299363057,0.869619025282206)
--(axis cs:44.5859872611465,0.868924769916544)
--(axis cs:43.9490445859873,0.867459530845444)
--(axis cs:43.312101910828,0.865177560468609)
--(axis cs:42.6751592356688,0.855682646319173)
--(axis cs:42.0382165605096,0.851423138121905)
--(axis cs:41.4012738853503,0.845310138989602)
--(axis cs:40.7643312101911,0.840396603811114)
--(axis cs:40.1273885350318,0.830522124955797)
--(axis cs:39.4904458598726,0.824820934151387)
--(axis cs:38.8535031847134,0.821099823983607)
--(axis cs:38.2165605095541,0.807617837515782)
--(axis cs:37.5796178343949,0.80139288130998)
--(axis cs:36.9426751592357,0.793724811178742)
--(axis cs:36.3057324840764,0.786099208859377)
--(axis cs:35.6687898089172,0.774620935338162)
--(axis cs:35.031847133758,0.763572679497096)
--(axis cs:34.3949044585987,0.746001689162349)
--(axis cs:33.7579617834395,0.732216371990103)
--(axis cs:33.1210191082803,0.715789829692926)
--(axis cs:32.484076433121,0.702302583554035)
--(axis cs:31.8471337579618,0.687739762099054)
--(axis cs:31.2101910828025,0.676625332272818)
--(axis cs:30.5732484076433,0.652752823849748)
--(axis cs:29.9363057324841,0.636863584581564)
--(axis cs:29.2993630573248,0.627344362010695)
--(axis cs:28.6624203821656,0.610189268050513)
--(axis cs:28.0254777070064,0.586682624218545)
--(axis cs:27.3885350318471,0.576790391702836)
--(axis cs:26.7515923566879,0.551273184728385)
--(axis cs:26.1146496815287,0.535393724909152)
--(axis cs:25.4777070063694,0.514057478324952)
--(axis cs:24.8407643312102,0.502909750150873)
--(axis cs:24.203821656051,0.485914572290221)
--(axis cs:23.5668789808917,0.468592116822931)
--(axis cs:22.9299363057325,0.446462892204865)
--(axis cs:22.2929936305732,0.432541890964045)
--(axis cs:21.656050955414,0.416189545291596)
--(axis cs:21.0191082802548,0.391753665321438)
--(axis cs:20.3821656050955,0.375452780408964)
--(axis cs:19.7452229299363,0.363641204631895)
--(axis cs:19.1082802547771,0.352417375256493)
--(axis cs:18.4713375796178,0.331804784514011)
--(axis cs:17.8343949044586,0.315451461059284)
--(axis cs:17.1974522292994,0.299062200993165)
--(axis cs:16.5605095541401,0.272310853868897)
--(axis cs:15.9235668789809,0.255696687773617)
--(axis cs:15.2866242038217,0.238617647181263)
--(axis cs:14.6496815286624,0.216650614418294)
--(axis cs:14.0127388535032,0.196510903636656)
--(axis cs:13.3757961783439,0.18139753114149)
--(axis cs:12.7388535031847,0.161111614090706)
--(axis cs:12.1019108280255,0.148773901666306)
--(axis cs:11.4649681528662,0.134264651299759)
--(axis cs:10.828025477707,0.12272669731674)
--(axis cs:10.1910828025478,0.113214608311617)
--(axis cs:9.55414012738853,0.106234807032797)
--(axis cs:8.9171974522293,0.100927449156204)
--(axis cs:8.28025477707006,0.0967817363582848)
--(axis cs:7.64331210191083,0.0922963020496519)
--(axis cs:7.00636942675159,0.0879034731911091)
--(axis cs:6.36942675159236,0.0852498134639474)
--(axis cs:5.73248407643312,0.082768852012471)
--(axis cs:5.09554140127389,0.0822590909260961)
--(axis cs:4.45859872611465,0.0817776682592302)
--(axis cs:3.82165605095541,0.0811837434511746)
--(axis cs:3.18471337579618,0.0807327657071837)
--(axis cs:2.54777070063694,0.0808319508058153)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.0803902433438268)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_accuracy_lafw_order.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.079921875
0.636942675159236 0.0800390625
1.27388535031847 0.08
1.91082802547771 0.08
2.54777070063694 0.080078125
3.18471337579618 0.08015625
3.82165605095541 0.0802734375
4.45859872611465 0.081015625
5.09554140127389 0.0812890625
5.73248407643312 0.0822265625
6.36942675159236 0.0837109375
7.00636942675159 0.086640625
7.64331210191083 0.0912109375
8.28025477707006 0.0957421875
8.9171974522293 0.106171875
9.55414012738853 0.115234375
10.1910828025478 0.12578125
10.828025477707 0.1425
11.4649681528662 0.1602734375
12.1019108280255 0.175859375
12.7388535031847 0.2025
13.3757961783439 0.2134375
14.0127388535032 0.2261328125
14.6496815286624 0.241640625
15.2866242038217 0.2561328125
15.9235668789809 0.2757421875
16.5605095541401 0.2904296875
17.1974522292994 0.31296875
17.8343949044586 0.3249609375
18.4713375796178 0.3384765625
19.1082802547771 0.350234375
19.7452229299363 0.3718359375
20.3821656050955 0.3866796875
21.0191082802548 0.4027734375
21.656050955414 0.4189453125
22.2929936305732 0.4330859375
22.9299363057325 0.452421875
23.5668789808917 0.4672265625
24.203821656051 0.48
24.8407643312102 0.48734375
25.4777070063694 0.490859375
26.1146496815287 0.5021875
26.7515923566879 0.50875
27.3885350318471 0.520390625
28.0254777070064 0.526640625
28.6624203821656 0.5353125
29.2993630573248 0.5410546875
29.9363057324841 0.55015625
30.5732484076433 0.556875
31.2101910828025 0.5643359375
31.8471337579618 0.5728515625
32.484076433121 0.5845703125
33.1210191082803 0.5908984375
33.7579617834395 0.6091796875
34.3949044585987 0.6269140625
35.031847133758 0.633046875
35.6687898089172 0.6430859375
36.3057324840764 0.657734375
36.9426751592357 0.6650390625
37.5796178343949 0.66875
38.2165605095541 0.675625
38.8535031847134 0.68328125
39.4904458598726 0.688515625
40.1273885350318 0.6856640625
40.7643312101911 0.69015625
41.4012738853503 0.6965625
42.0382165605096 0.7001953125
42.6751592356688 0.7043359375
43.312101910828 0.70953125
43.9490445859873 0.707890625
44.5859872611465 0.7056640625
45.2229299363057 0.7137890625
45.859872611465 0.718125
46.4968152866242 0.724453125
47.1337579617834 0.7230859375
47.7707006369427 0.72875
48.4076433121019 0.735546875
49.0445859872611 0.7353515625
49.6815286624204 0.73984375
50.3184713375796 0.744140625
50.9554140127388 0.7398828125
51.5923566878981 0.7471875
52.2292993630573 0.75640625
52.8662420382166 0.7571875
53.5031847133758 0.7697265625
54.140127388535 0.775859375
54.7770700636943 0.7762109375
55.4140127388535 0.78484375
56.0509554140127 0.795390625
56.687898089172 0.798828125
57.3248407643312 0.813046875
57.9617834394904 0.810703125
58.5987261146497 0.8111328125
59.2356687898089 0.8180078125
59.8726114649682 0.8255078125
60.5095541401274 0.8258203125
61.1464968152866 0.8333203125
61.7834394904459 0.836875
62.4203821656051 0.8340625
63.0573248407643 0.8396875
63.6942675159236 0.8449609375
64.3312101910828 0.8521484375
64.968152866242 0.855859375
65.6050955414013 0.8641015625
66.2420382165605 0.86515625
66.8789808917197 0.869453125
67.515923566879 0.8758203125
68.1528662420382 0.880625
68.7898089171974 0.8897265625
69.4267515923567 0.9083203125
70.0636942675159 0.9128125
70.7006369426752 0.9250390625
71.3375796178344 0.929921875
71.9745222929936 0.9343359375
72.6114649681529 0.945546875
73.2484076433121 0.949375
73.8853503184713 0.954140625
74.5222929936306 0.9571875
75.1592356687898 0.954375
75.796178343949 0.9569921875
76.4331210191083 0.9580859375
77.0700636942675 0.9584375
77.7070063694268 0.960625
78.343949044586 0.9598046875
78.9808917197452 0.9659765625
79.6178343949044 0.9691015625
80.2547770700637 0.97171875
80.8917197452229 0.9726171875
81.5286624203822 0.969765625
82.1656050955414 0.968203125
82.8025477707006 0.967890625
83.4394904458599 0.9661328125
84.0764331210191 0.9640234375
84.7133757961783 0.959296875
85.3503184713376 0.9594140625
85.9872611464968 0.9653125
86.6242038216561 0.9721875
87.2611464968153 0.9746875
87.8980891719745 0.9808984375
88.5350318471338 0.980625
89.171974522293 0.9821875
89.8089171974522 0.9803125
90.4458598726115 0.981640625
91.0828025477707 0.986875
91.7197452229299 0.9839453125
92.3566878980892 0.985859375
92.9936305732484 0.989453125
93.6305732484076 0.9858203125
94.2675159235669 0.9877734375
94.9044585987261 0.98921875
95.5414012738853 0.996953125
96.1783439490446 0.999921875
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};

\path [fill=color1, fill opacity=0.25]
(axis cs:0,0.0803121183438268)
--(axis cs:0,0.0795316316561732)
--(axis cs:0.636942675159236,0.0797631187852672)
--(axis cs:1.27388535031847,0.0794481125705343)
--(axis cs:1.91082802547771,0.08)
--(axis cs:2.54777070063694,0.0796878816561732)
--(axis cs:3.18471337579618,0.0794807697591671)
--(axis cs:3.82165605095541,0.0794466870757716)
--(axis cs:4.45859872611465,0.0794137573532886)
--(axis cs:5.09554140127389,0.0794893221274166)
--(axis cs:5.73248407643312,0.0800212076528019)
--(axis cs:6.36942675159236,0.08091846070254)
--(axis cs:7.00636942675159,0.0830604877383157)
--(axis cs:7.64331210191083,0.086621109982783)
--(axis cs:8.28025477707006,0.0904755784906051)
--(axis cs:8.9171974522293,0.0996829451047511)
--(axis cs:9.55414012738853,0.1078857421875)
--(axis cs:10.1910828025478,0.117827116215199)
--(axis cs:10.828025477707,0.133762203961586)
--(axis cs:11.4649681528662,0.151006451415632)
--(axis cs:12.1019108280255,0.166223100923763)
--(axis cs:12.7388535031847,0.192466414346203)
--(axis cs:13.3757961783439,0.203416709458515)
--(axis cs:14.0127388535032,0.215564801237545)
--(axis cs:14.6496815286624,0.230530160949263)
--(axis cs:15.2866242038217,0.244673517585412)
--(axis cs:15.9235668789809,0.264137550273371)
--(axis cs:16.5605095541401,0.278666016526898)
--(axis cs:17.1974522292994,0.300850063335551)
--(axis cs:17.8343949044586,0.312600108264775)
--(axis cs:18.4713375796178,0.326158421922543)
--(axis cs:19.1082802547771,0.33777389575043)
--(axis cs:19.7452229299363,0.359277109056355)
--(axis cs:20.3821656050955,0.374087538629277)
--(axis cs:21.0191082802548,0.390249683776774)
--(axis cs:21.656050955414,0.406441552012565)
--(axis cs:22.2929936305732,0.420571979924286)
--(axis cs:22.9299363057325,0.440296673196329)
--(axis cs:23.5668789808917,0.455362690819394)
--(axis cs:24.203821656051,0.468355247154156)
--(axis cs:24.8407643312102,0.475766823978702)
--(axis cs:25.4777070063694,0.479689974758844)
--(axis cs:26.1146496815287,0.49108771689687)
--(axis cs:26.7515923566879,0.497555147338855)
--(axis cs:27.3885350318471,0.509111473447737)
--(axis cs:28.0254777070064,0.515342504841689)
--(axis cs:28.6624203821656,0.524109916476642)
--(axis cs:29.2993630573248,0.530118270655178)
--(axis cs:29.9363057324841,0.538781392695725)
--(axis cs:30.5732484076433,0.545431964566984)
--(axis cs:31.2101910828025,0.552531144986471)
--(axis cs:31.8471337579618,0.561553765478339)
--(axis cs:32.484076433121,0.573032846745948)
--(axis cs:33.1210191082803,0.579091145901763)
--(axis cs:33.7579617834395,0.59712803353822)
--(axis cs:34.3949044585987,0.614790833307564)
--(axis cs:35.031847133758,0.621300412203183)
--(axis cs:35.6687898089172,0.631389403738871)
--(axis cs:36.3057324840764,0.645871727993975)
--(axis cs:36.9426751592357,0.653120767063354)
--(axis cs:37.5796178343949,0.65727468939144)
--(axis cs:38.2165605095541,0.664361951236355)
--(axis cs:38.8535031847134,0.6722537663219)
--(axis cs:39.4904458598726,0.677669858059211)
--(axis cs:40.1273885350318,0.67508803123786)
--(axis cs:40.7643312101911,0.679815446218709)
--(axis cs:41.4012738853503,0.686297482652228)
--(axis cs:42.0382165605096,0.690209819169806)
--(axis cs:42.6751592356688,0.694534481930811)
--(axis cs:43.312101910828,0.699843957349474)
--(axis cs:43.9490445859873,0.698264175326045)
--(axis cs:44.5859872611465,0.696258554823755)
--(axis cs:45.2229299363057,0.704637378633381)
--(axis cs:45.859872611465,0.709364705011379)
--(axis cs:46.4968152866242,0.715893845767125)
--(axis cs:47.1337579617834,0.714303990171162)
--(axis cs:47.7707006369427,0.719979776864275)
--(axis cs:48.4076433121019,0.726849333110668)
--(axis cs:49.0445859872611,0.726541645631544)
--(axis cs:49.6815286624204,0.731007343227122)
--(axis cs:50.3184713375796,0.735117093701871)
--(axis cs:50.9554140127388,0.73110327495018)
--(axis cs:51.5923566878981,0.738521161171193)
--(axis cs:52.2292993630573,0.74771162114256)
--(axis cs:52.8662420382166,0.748435322487525)
--(axis cs:53.5031847133758,0.760371380135414)
--(axis cs:54.140127388535,0.766482658543362)
--(axis cs:54.7770700636943,0.76644792973304)
--(axis cs:55.4140127388535,0.774800189243051)
--(axis cs:56.0509554140127,0.785324404746706)
--(axis cs:56.687898089172,0.788811127088738)
--(axis cs:57.3248407643312,0.803115736712441)
--(axis cs:57.9617834394904,0.800800340650982)
--(axis cs:58.5987261146497,0.801434412597119)
--(axis cs:59.2356687898089,0.808759175594344)
--(axis cs:59.8726114649682,0.816410248615608)
--(axis cs:60.5095541401274,0.817101030796636)
--(axis cs:61.1464968152866,0.824600090903049)
--(axis cs:61.7834394904459,0.828110912627856)
--(axis cs:62.4203821656051,0.825220749154283)
--(axis cs:63.0573248407643,0.830649299972653)
--(axis cs:63.6942675159236,0.835913649533857)
--(axis cs:64.3312101910828,0.842903603746394)
--(axis cs:64.968152866242,0.846776572639632)
--(axis cs:65.6050955414013,0.855195690296891)
--(axis cs:66.2420382165605,0.855965936196364)
--(axis cs:66.8789808917197,0.860168989559402)
--(axis cs:67.515923566879,0.866587301067714)
--(axis cs:68.1528662420382,0.871353601051469)
--(axis cs:68.7898089171974,0.880839902437844)
--(axis cs:69.4267515923567,0.899729450017355)
--(axis cs:70.0636942675159,0.904318651517944)
--(axis cs:70.7006369426752,0.917186771635371)
--(axis cs:71.3375796178344,0.922467305769186)
--(axis cs:71.9745222929936,0.927199165816313)
--(axis cs:72.6114649681529,0.939034083481649)
--(axis cs:73.2484076433121,0.943153676014597)
--(axis cs:73.8853503184713,0.948250988585355)
--(axis cs:74.5222929936306,0.951411858263208)
--(axis cs:75.1592356687898,0.948456767374514)
--(axis cs:75.796178343949,0.951848998572913)
--(axis cs:76.4331210191083,0.952545599154913)
--(axis cs:77.0700636942675,0.953222511093503)
--(axis cs:77.7070063694268,0.955521818502614)
--(axis cs:78.343949044586,0.954362254111681)
--(axis cs:78.9808917197452,0.960263398005863)
--(axis cs:79.6178343949044,0.963539186564768)
--(axis cs:80.2547770700637,0.966330482888016)
--(axis cs:80.8917197452229,0.967595080728425)
--(axis cs:81.5286624203822,0.96497290761001)
--(axis cs:82.1656050955414,0.963324464656042)
--(axis cs:82.8025477707006,0.962748174927564)
--(axis cs:83.4394904458599,0.961175510206486)
--(axis cs:84.0764331210191,0.959200269682292)
--(axis cs:84.7133757961783,0.954342053195605)
--(axis cs:85.3503184713376,0.954542049907599)
--(axis cs:85.9872611464968,0.960295662619453)
--(axis cs:86.6242038216561,0.967509960584781)
--(axis cs:87.2611464968153,0.970047190102123)
--(axis cs:87.8980891719745,0.976941306564517)
--(axis cs:88.5350318471338,0.977696991447883)
--(axis cs:89.171974522293,0.978608153639106)
--(axis cs:89.8089171974522,0.977097065086533)
--(axis cs:90.4458598726115,0.977910103523667)
--(axis cs:91.0828025477707,0.982785699189964)
--(axis cs:91.7197452229299,0.979687752687445)
--(axis cs:92.3566878980892,0.981750045138415)
--(axis cs:92.9936305732484,0.986062557519794)
--(axis cs:93.6305732484076,0.982703548794827)
--(axis cs:94.2675159235669,0.984595879032664)
--(axis cs:94.9044585987261,0.986064371871814)
--(axis cs:95.5414012738853,0.994707163939042)
--(axis cs:96.1783439490446,0.99953201368597)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1.00031173631403)
--(axis cs:95.5414012738853,0.999199086060958)
--(axis cs:94.9044585987261,0.992373128128186)
--(axis cs:94.2675159235669,0.990950995967336)
--(axis cs:93.6305732484076,0.988937076205173)
--(axis cs:92.9936305732484,0.992843692480206)
--(axis cs:92.3566878980892,0.989968704861585)
--(axis cs:91.7197452229299,0.988202872312555)
--(axis cs:91.0828025477707,0.990964300810036)
--(axis cs:90.4458598726115,0.985371146476333)
--(axis cs:89.8089171974522,0.983527934913467)
--(axis cs:89.171974522293,0.985766846360894)
--(axis cs:88.5350318471338,0.983553008552117)
--(axis cs:87.8980891719745,0.984855568435483)
--(axis cs:87.2611464968153,0.979327809897877)
--(axis cs:86.6242038216561,0.976865039415219)
--(axis cs:85.9872611464968,0.970329337380547)
--(axis cs:85.3503184713376,0.964286075092401)
--(axis cs:84.7133757961783,0.964251696804395)
--(axis cs:84.0764331210191,0.968846605317708)
--(axis cs:83.4394904458599,0.971090114793514)
--(axis cs:82.8025477707006,0.973033075072436)
--(axis cs:82.1656050955414,0.973081785343958)
--(axis cs:81.5286624203822,0.97455834238999)
--(axis cs:80.8917197452229,0.977639294271575)
--(axis cs:80.2547770700637,0.977107017111984)
--(axis cs:79.6178343949044,0.974663938435232)
--(axis cs:78.9808917197452,0.971689726994137)
--(axis cs:78.343949044586,0.96524712088832)
--(axis cs:77.7070063694268,0.965728181497386)
--(axis cs:77.0700636942675,0.963652488906497)
--(axis cs:76.4331210191083,0.963626275845087)
--(axis cs:75.796178343949,0.962135376427087)
--(axis cs:75.1592356687898,0.960293232625486)
--(axis cs:74.5222929936306,0.962963141736792)
--(axis cs:73.8853503184713,0.960030261414645)
--(axis cs:73.2484076433121,0.955596323985403)
--(axis cs:72.6114649681529,0.952059666518351)
--(axis cs:71.9745222929936,0.941472709183687)
--(axis cs:71.3375796178344,0.937376444230814)
--(axis cs:70.7006369426752,0.932891353364629)
--(axis cs:70.0636942675159,0.921306348482057)
--(axis cs:69.4267515923567,0.916911174982645)
--(axis cs:68.7898089171974,0.898613222562156)
--(axis cs:68.1528662420382,0.889896398948531)
--(axis cs:67.515923566879,0.885053323932286)
--(axis cs:66.8789808917197,0.878737260440598)
--(axis cs:66.2420382165605,0.874346563803636)
--(axis cs:65.6050955414013,0.873007434703109)
--(axis cs:64.968152866242,0.864942177360368)
--(axis cs:64.3312101910828,0.861393271253606)
--(axis cs:63.6942675159236,0.854008225466143)
--(axis cs:63.0573248407643,0.848725700027347)
--(axis cs:62.4203821656051,0.842904250845717)
--(axis cs:61.7834394904459,0.845639087372145)
--(axis cs:61.1464968152866,0.842040534096951)
--(axis cs:60.5095541401274,0.834539594203364)
--(axis cs:59.8726114649682,0.834605376384392)
--(axis cs:59.2356687898089,0.827256449405656)
--(axis cs:58.5987261146497,0.820831212402881)
--(axis cs:57.9617834394904,0.820605909349018)
--(axis cs:57.3248407643312,0.822978013287559)
--(axis cs:56.687898089172,0.808845122911262)
--(axis cs:56.0509554140127,0.805456845253295)
--(axis cs:55.4140127388535,0.794887310756949)
--(axis cs:54.7770700636943,0.785973945266961)
--(axis cs:54.140127388535,0.785236091456638)
--(axis cs:53.5031847133758,0.779081744864586)
--(axis cs:52.8662420382166,0.765939677512475)
--(axis cs:52.2292993630573,0.76510087885744)
--(axis cs:51.5923566878981,0.755853838828807)
--(axis cs:50.9554140127388,0.74866235004982)
--(axis cs:50.3184713375796,0.753164156298129)
--(axis cs:49.6815286624204,0.748680156772878)
--(axis cs:49.0445859872611,0.744161479368456)
--(axis cs:48.4076433121019,0.744244416889332)
--(axis cs:47.7707006369427,0.737520223135725)
--(axis cs:47.1337579617834,0.731867884828838)
--(axis cs:46.4968152866242,0.733012404232875)
--(axis cs:45.859872611465,0.726885294988621)
--(axis cs:45.2229299363057,0.722940746366619)
--(axis cs:44.5859872611465,0.715069570176245)
--(axis cs:43.9490445859873,0.717517074673955)
--(axis cs:43.312101910828,0.719218542650526)
--(axis cs:42.6751592356688,0.714137393069189)
--(axis cs:42.0382165605096,0.710180805830194)
--(axis cs:41.4012738853503,0.706827517347772)
--(axis cs:40.7643312101911,0.700497053781291)
--(axis cs:40.1273885350318,0.69624009376214)
--(axis cs:39.4904458598726,0.699361391940789)
--(axis cs:38.8535031847134,0.6943087336781)
--(axis cs:38.2165605095541,0.686888048763645)
--(axis cs:37.5796178343949,0.68022531060856)
--(axis cs:36.9426751592357,0.676957357936646)
--(axis cs:36.3057324840764,0.669597022006025)
--(axis cs:35.6687898089172,0.654782471261129)
--(axis cs:35.031847133758,0.644793337796817)
--(axis cs:34.3949044585987,0.639037291692436)
--(axis cs:33.7579617834395,0.62123134146178)
--(axis cs:33.1210191082803,0.602705729098237)
--(axis cs:32.484076433121,0.596107778254052)
--(axis cs:31.8471337579618,0.584149359521661)
--(axis cs:31.2101910828025,0.576140730013529)
--(axis cs:30.5732484076433,0.568318035433016)
--(axis cs:29.9363057324841,0.561531107304275)
--(axis cs:29.2993630573248,0.551991104344822)
--(axis cs:28.6624203821656,0.546515083523358)
--(axis cs:28.0254777070064,0.537938745158311)
--(axis cs:27.3885350318471,0.531669776552263)
--(axis cs:26.7515923566879,0.519944852661145)
--(axis cs:26.1146496815287,0.51328728310313)
--(axis cs:25.4777070063694,0.502028775241156)
--(axis cs:24.8407643312102,0.498920676021298)
--(axis cs:24.203821656051,0.491644752845844)
--(axis cs:23.5668789808917,0.479090434180606)
--(axis cs:22.9299363057325,0.464547076803671)
--(axis cs:22.2929936305732,0.445599895075714)
--(axis cs:21.656050955414,0.431449072987435)
--(axis cs:21.0191082802548,0.415297191223226)
--(axis cs:20.3821656050955,0.399271836370723)
--(axis cs:19.7452229299363,0.384394765943645)
--(axis cs:19.1082802547771,0.36269485424957)
--(axis cs:18.4713375796178,0.350794703077457)
--(axis cs:17.8343949044586,0.337321766735225)
--(axis cs:17.1974522292994,0.325087436664449)
--(axis cs:16.5605095541401,0.302193358473102)
--(axis cs:15.9235668789809,0.287346824726629)
--(axis cs:15.2866242038217,0.267592107414588)
--(axis cs:14.6496815286624,0.252751089050737)
--(axis cs:14.0127388535032,0.236700823762455)
--(axis cs:13.3757961783439,0.223458290541485)
--(axis cs:12.7388535031847,0.212533585653797)
--(axis cs:12.1019108280255,0.185495649076237)
--(axis cs:11.4649681528662,0.169540423584368)
--(axis cs:10.828025477707,0.151237796038414)
--(axis cs:10.1910828025478,0.133735383784801)
--(axis cs:9.55414012738853,0.1225830078125)
--(axis cs:8.9171974522293,0.112660804895249)
--(axis cs:8.28025477707006,0.101008796509395)
--(axis cs:7.64331210191083,0.095800765017217)
--(axis cs:7.00636942675159,0.0902207622616843)
--(axis cs:6.36942675159236,0.08650341429746)
--(axis cs:5.73248407643312,0.0844319173471981)
--(axis cs:5.09554140127389,0.0830888028725834)
--(axis cs:4.45859872611465,0.0826174926467114)
--(axis cs:3.82165605095541,0.0811001879242284)
--(axis cs:3.18471337579618,0.0808317302408329)
--(axis cs:2.54777070063694,0.0804683683438268)
--(axis cs:1.91082802547771,0.08)
--(axis cs:1.27388535031847,0.0805518874294657)
--(axis cs:0.636942675159236,0.0803150062147328)
--(axis cs:0,0.0803121183438268)
--cycle;


==> img/mnist/mnist_rate_accuracy_lagrange.tex <==
\addplot [line width=0.5, opacity=0.7, color4, mark=o, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color4, thin}]
table [row sep=\\]{%
0	0.08 \\
0.636942675159236	0.08 \\
1.27388535031847	0.0800390625 \\
1.91082802547771	0.0799609375 \\
2.54777070063694	0.0800390625 \\
3.18471337579618	0.0800390625 \\
3.82165605095541	0.0800390625 \\
4.45859872611465	0.0801171875 \\
5.09554140127389	0.0803125 \\
5.73248407643312	0.0805078125 \\
6.36942675159236	0.081328125 \\
7.00636942675159	0.0816015625 \\
7.64331210191083	0.08328125 \\
8.28025477707006	0.0857421875 \\
8.9171974522293	0.0907421875 \\
9.55414012738853	0.09859375 \\
10.1910828025478	0.1140234375 \\
10.828025477707	0.1346484375 \\
11.4649681528662	0.15765625 \\
12.1019108280255	0.191484375 \\
12.7388535031847	0.2190625 \\
13.3757961783439	0.2421484375 \\
14.0127388535032	0.263203125 \\
14.6496815286624	0.28765625 \\
15.2866242038217	0.309140625 \\
15.9235668789809	0.330859375 \\
16.5605095541401	0.3490234375 \\
17.1974522292994	0.36984375 \\
17.8343949044586	0.386640625 \\
18.4713375796178	0.4015625 \\
19.1082802547771	0.4303125 \\
19.7452229299363	0.4480859375 \\
20.3821656050955	0.4655078125 \\
21.0191082802548	0.4794921875 \\
21.656050955414	0.4915234375 \\
22.2929936305732	0.509765625 \\
22.9299363057325	0.53421875 \\
23.5668789808917	0.549765625 \\
24.203821656051	0.5680078125 \\
24.8407643312102	0.5748828125 \\
25.4777070063694	0.5937109375 \\
26.1146496815287	0.6023046875 \\
26.7515923566879	0.6076171875 \\
27.3885350318471	0.615 \\
28.0254777070064	0.6351171875 \\
28.6624203821656	0.6504296875 \\
29.2993630573248	0.67484375 \\
29.9363057324841	0.6940234375 \\
30.5732484076433	0.71 \\
31.2101910828025	0.7122265625 \\
31.8471337579618	0.7258984375 \\
32.484076433121	0.7394921875 \\
33.1210191082803	0.7513671875 \\
33.7579617834395	0.759296875 \\
34.3949044585987	0.7668359375 \\
35.031847133758	0.7794921875 \\
35.6687898089172	0.787890625 \\
36.3057324840764	0.7988671875 \\
36.9426751592357	0.8019921875 \\
37.5796178343949	0.810078125 \\
38.2165605095541	0.815078125 \\
38.8535031847134	0.8271484375 \\
39.4904458598726	0.8295703125 \\
40.1273885350318	0.836640625 \\
40.7643312101911	0.839453125 \\
41.4012738853503	0.8462109375 \\
42.0382165605096	0.857109375 \\
42.6751592356688	0.8490234375 \\
43.312101910828	0.8490625 \\
43.9490445859873	0.8480859375 \\
44.5859872611465	0.8484375 \\
45.2229299363057	0.8474609375 \\
45.859872611465	0.8484765625 \\
46.4968152866242	0.8554296875 \\
47.1337579617834	0.8575 \\
47.7707006369427	0.855390625 \\
48.4076433121019	0.8573828125 \\
49.0445859872611	0.8551171875 \\
49.6815286624204	0.86 \\
50.3184713375796	0.861171875 \\
50.9554140127388	0.86234375 \\
51.5923566878981	0.8639453125 \\
52.2292993630573	0.8646875 \\
52.8662420382166	0.86609375 \\
53.5031847133758	0.8706640625 \\
54.140127388535	0.8705078125 \\
54.7770700636943	0.8721484375 \\
55.4140127388535	0.87765625 \\
56.0509554140127	0.880390625 \\
56.687898089172	0.87953125 \\
57.3248407643312	0.8821875 \\
57.9617834394904	0.8842578125 \\
58.5987261146497	0.8803125 \\
59.2356687898089	0.888125 \\
59.8726114649682	0.888671875 \\
60.5095541401274	0.8902734375 \\
61.1464968152866	0.8959375 \\
61.7834394904459	0.8925 \\
62.4203821656051	0.8982421875 \\
63.0573248407643	0.899921875 \\
63.6942675159236	0.901875 \\
64.3312101910828	0.9077734375 \\
64.968152866242	0.908359375 \\
65.6050955414013	0.91296875 \\
66.2420382165605	0.915859375 \\
66.8789808917197	0.92078125 \\
67.515923566879	0.923984375 \\
68.1528662420382	0.931796875 \\
68.7898089171974	0.92875 \\
69.4267515923567	0.9334375 \\
70.0636942675159	0.93890625 \\
70.7006369426752	0.938046875 \\
71.3375796178344	0.938828125 \\
71.9745222929936	0.936328125 \\
72.6114649681529	0.942890625 \\
73.2484076433121	0.9452734375 \\
73.8853503184713	0.9469140625 \\
74.5222929936306	0.948046875 \\
75.1592356687898	0.950625 \\
75.796178343949	0.9546875 \\
76.4331210191083	0.9609375 \\
77.0700636942675	0.9627734375 \\
77.7070063694268	0.961328125 \\
78.343949044586	0.961953125 \\
78.9808917197452	0.9636328125 \\
79.6178343949044	0.9691796875 \\
80.2547770700637	0.9703515625 \\
80.8917197452229	0.9738671875 \\
81.5286624203822	0.9771875 \\
82.1656050955414	0.978515625 \\
82.8025477707006	0.9783984375 \\
83.4394904458599	0.978125 \\
84.0764331210191	0.9786328125 \\
84.7133757961783	0.981015625 \\
85.3503184713376	0.984453125 \\
85.9872611464968	0.987734375 \\
86.6242038216561	0.988671875 \\
87.2611464968153	0.9868359375 \\
87.8980891719745	0.9888671875 \\
88.5350318471338	0.9898046875 \\
89.171974522293	0.9916015625 \\
89.8089171974522	0.9908984375 \\
90.4458598726115	0.99328125 \\
91.0828025477707	0.9982421875 \\
91.7197452229299	0.9996484375 \\
92.3566878980892	0.9997265625 \\
92.9936305732484	1 \\
93.6305732484076	1 \\
94.2675159235669	1 \\
94.9044585987261	0.9999609375 \\
95.5414012738853	0.999921875 \\
96.1783439490446	1 \\
96.8152866242038	1 \\
97.4522292993631	1 \\
98.0891719745223	1 \\
98.7261146496815	1 \\
99.3630573248408	1 \\
100	1 \\
};
\path [fill=color4, fill opacity=0.25]
(axis cs:0,0.0803902433438268)
--(axis cs:0,0.0796097566561732)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0796849937852672)
--(axis cs:2.54777070063694,0.0795614258411496)
--(axis cs:3.18471337579618,0.0794220335958935)
--(axis cs:3.82165605095541,0.0795611139660534)
--(axis cs:4.45859872611465,0.0793881302870293)
--(axis cs:5.09554140127389,0.0793575387101754)
--(axis cs:5.73248407643312,0.0792471742325641)
--(axis cs:6.36942675159236,0.0795530194972056)
--(axis cs:7.00636942675159,0.0795708246143049)
--(axis cs:7.64331210191083,0.0806489996449017)
--(axis cs:8.28025477707006,0.082261128279813)
--(axis cs:8.9171974522293,0.0862921762477288)
--(axis cs:9.55414012738853,0.0928741077639684)
--(axis cs:10.1910828025478,0.106704479835518)
--(axis cs:10.828025477707,0.126218167683065)
--(axis cs:11.4649681528662,0.148138068356265)
--(axis cs:12.1019108280255,0.181169108559577)
--(axis cs:12.7388535031847,0.208457041366329)
--(axis cs:13.3757961783439,0.231164381474097)
--(axis cs:14.0127388535032,0.25219898904181)
--(axis cs:14.6496815286624,0.276657559039238)
--(axis cs:15.2866242038217,0.297907622250045)
--(axis cs:15.9235668789809,0.319498477854123)
--(axis cs:16.5605095541401,0.337385718433135)
--(axis cs:17.1974522292994,0.358178119251284)
--(axis cs:17.8343949044586,0.374872337774218)
--(axis cs:18.4713375796178,0.389653328820889)
--(axis cs:19.1082802547771,0.4183935856927)
--(axis cs:19.7452229299363,0.436075552417392)
--(axis cs:20.3821656050955,0.453580006256245)
--(axis cs:21.0191082802548,0.46743157267107)
--(axis cs:21.656050955414,0.47950956658516)
--(axis cs:22.2929936305732,0.497516369414079)
--(axis cs:22.9299363057325,0.521780450031953)
--(axis cs:23.5668789808917,0.537430626796851)
--(axis cs:24.203821656051,0.55562295659797)
--(axis cs:24.8407643312102,0.562709745737227)
--(axis cs:25.4777070063694,0.581590867612257)
--(axis cs:26.1146496815287,0.589995840866377)
--(axis cs:26.7515923566879,0.595415730032272)
--(axis cs:27.3885350318471,0.602494052871185)
--(axis cs:28.0254777070064,0.622354136498863)
--(axis cs:28.6624203821656,0.637657568063408)
--(axis cs:29.2993630573248,0.662067145410667)
--(axis cs:29.9363057324841,0.681324633564914)
--(axis cs:30.5732484076433,0.697455162356269)
--(axis cs:31.2101910828025,0.699681362572701)
--(axis cs:31.8471337579618,0.713147370915987)
--(axis cs:32.484076433121,0.726791975526626)
--(axis cs:33.1210191082803,0.738813711351819)
--(axis cs:33.7579617834395,0.746568564238243)
--(axis cs:34.3949044585987,0.754238665682722)
--(axis cs:35.031847133758,0.76729130403833)
--(axis cs:35.6687898089172,0.775916404639599)
--(axis cs:36.3057324840764,0.787139076157295)
--(axis cs:36.9426751592357,0.790562487891015)
--(axis cs:37.5796178343949,0.798855952134204)
--(axis cs:38.2165605095541,0.804078079310425)
--(axis cs:38.8535031847134,0.816510494766304)
--(axis cs:39.4904458598726,0.819251326953104)
--(axis cs:40.1273885350318,0.82662277919973)
--(axis cs:40.7643312101911,0.82981083745469)
--(axis cs:41.4012738853503,0.83674982676204)
--(axis cs:42.0382165605096,0.848297014386353)
--(axis cs:42.6751592356688,0.839810605736525)
--(axis cs:43.312101910828,0.840270657449225)
--(axis cs:43.9490445859873,0.83942698677136)
--(axis cs:44.5859872611465,0.83964255635677)
--(axis cs:45.2229299363057,0.838618689499472)
--(axis cs:45.859872611465,0.839722895368908)
--(axis cs:46.4968152866242,0.84667678642682)
--(axis cs:47.1337579617834,0.849003941327748)
--(axis cs:47.7707006369427,0.84671613990267)
--(axis cs:48.4076433121019,0.849023847857414)
--(axis cs:49.0445859872611,0.846713455449671)
--(axis cs:49.6815286624204,0.851709870834022)
--(axis cs:50.3184713375796,0.853073984034509)
--(axis cs:50.9554140127388,0.85457512779433)
--(axis cs:51.5923566878981,0.856330795756299)
--(axis cs:52.2292993630573,0.857190156453421)
--(axis cs:52.8662420382166,0.858646220326196)
--(axis cs:53.5031847133758,0.863310919336681)
--(axis cs:54.140127388535,0.863057612211244)
--(axis cs:54.7770700636943,0.864656233468338)
--(axis cs:55.4140127388535,0.870082753601996)
--(axis cs:56.0509554140127,0.872835271381446)
--(axis cs:56.687898089172,0.871609686140945)
--(axis cs:57.3248407643312,0.874519385363994)
--(axis cs:57.9617834394904,0.876528120206145)
--(axis cs:58.5987261146497,0.872826474015471)
--(axis cs:59.2356687898089,0.880739271951558)
--(axis cs:59.8726114649682,0.880897193893152)
--(axis cs:60.5095541401274,0.882717699299516)
--(axis cs:61.1464968152866,0.888706958938045)
--(axis cs:61.7834394904459,0.885176493361441)
--(axis cs:62.4203821656051,0.890808285870415)
--(axis cs:63.0573248407643,0.892532778391894)
--(axis cs:63.6942675159236,0.89477241672848)
--(axis cs:64.3312101910828,0.900875622285978)
--(axis cs:64.968152866242,0.901100737126926)
--(axis cs:65.6050955414013,0.905822745148221)
--(axis cs:66.2420382165605,0.908475927148133)
--(axis cs:66.8789808917197,0.913537243426492)
--(axis cs:67.515923566879,0.916878016346711)
--(axis cs:68.1528662420382,0.924840880568162)
--(axis cs:68.7898089171974,0.921863654568167)
--(axis cs:69.4267515923567,0.926722145938792)
--(axis cs:70.0636942675159,0.9321234451881)
--(axis cs:70.7006369426752,0.931642312062663)
--(axis cs:71.3375796178344,0.932367087386883)
--(axis cs:71.9745222929936,0.930046068385659)
--(axis cs:72.6114649681529,0.936613100577903)
--(axis cs:73.2484076433121,0.938947332728225)
--(axis cs:73.8853503184713,0.941088059410215)
--(axis cs:74.5222929936306,0.942164656346115)
--(axis cs:75.1592356687898,0.945014278732808)
--(axis cs:75.796178343949,0.949431355892708)
--(axis cs:76.4331210191083,0.956335303513787)
--(axis cs:77.0700636942675,0.958369540551997)
--(axis cs:77.7070063694268,0.95692458334756)
--(axis cs:78.343949044586,0.957518527106846)
--(axis cs:78.9808917197452,0.959142599124966)
--(axis cs:79.6178343949044,0.96511738630928)
--(axis cs:80.2547770700637,0.966356766062063)
--(axis cs:80.8917197452229,0.970483857333211)
--(axis cs:81.5286624203822,0.974631591342128)
--(axis cs:82.1656050955414,0.976148216132012)
--(axis cs:82.8025477707006,0.975922395345677)
--(axis cs:83.4394904458599,0.975251235646951)
--(axis cs:84.0764331210191,0.975775245821405)
--(axis cs:84.7133757961783,0.978138336843406)
--(axis cs:85.3503184713376,0.981560547946515)
--(axis cs:85.9872611464968,0.984645296560511)
--(axis cs:86.6242038216561,0.98550674456499)
--(axis cs:87.2611464968153,0.983821542190092)
--(axis cs:87.8980891719745,0.985748703119738)
--(axis cs:88.5350318471338,0.986680283603302)
--(axis cs:89.171974522293,0.988506580521015)
--(axis cs:89.8089171974522,0.987786075397467)
--(axis cs:90.4458598726115,0.9903292677734)
--(axis cs:91.0828025477707,0.996472588950925)
--(axis cs:91.7197452229299,0.998827112005908)
--(axis cs:92.3566878980892,0.999000782885928)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,0.999684993785267)
--(axis cs:95.5414012738853,0.99953201368597)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1.00031173631403)
--(axis cs:94.9044585987261,1.00023688121473)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1.00045234211407)
--(axis cs:91.7197452229299,1.00046976299409)
--(axis cs:91.0828025477707,1.00001178604907)
--(axis cs:90.4458598726115,0.9962332322266)
--(axis cs:89.8089171974522,0.994010799602533)
--(axis cs:89.171974522293,0.994696544478985)
--(axis cs:88.5350318471338,0.992929091396698)
--(axis cs:87.8980891719745,0.991985671880262)
--(axis cs:87.2611464968153,0.989850332809908)
--(axis cs:86.6242038216561,0.99183700543501)
--(axis cs:85.9872611464968,0.990823453439489)
--(axis cs:85.3503184713376,0.987345702053485)
--(axis cs:84.7133757961783,0.983892913156594)
--(axis cs:84.0764331210191,0.981490379178595)
--(axis cs:83.4394904458599,0.980998764353049)
--(axis cs:82.8025477707006,0.980874479654323)
--(axis cs:82.1656050955414,0.980883033867988)
--(axis cs:81.5286624203822,0.979743408657872)
--(axis cs:80.8917197452229,0.977250517666789)
--(axis cs:80.2547770700637,0.974346358937937)
--(axis cs:79.6178343949044,0.97324198869072)
--(axis cs:78.9808917197452,0.968123025875034)
--(axis cs:78.343949044586,0.966387722893154)
--(axis cs:77.7070063694268,0.96573166665244)
--(axis cs:77.0700636942675,0.967177334448003)
--(axis cs:76.4331210191083,0.965539696486213)
--(axis cs:75.796178343949,0.959943644107292)
--(axis cs:75.1592356687898,0.956235721267192)
--(axis cs:74.5222929936306,0.953929093653885)
--(axis cs:73.8853503184713,0.952740065589785)
--(axis cs:73.2484076433121,0.951599542271776)
--(axis cs:72.6114649681529,0.949168149422097)
--(axis cs:71.9745222929936,0.942610181614341)
--(axis cs:71.3375796178344,0.945289162613117)
--(axis cs:70.7006369426752,0.944451437937336)
--(axis cs:70.0636942675159,0.9456890548119)
--(axis cs:69.4267515923567,0.940152854061209)
--(axis cs:68.7898089171974,0.935636345431833)
--(axis cs:68.1528662420382,0.938752869431838)
--(axis cs:67.515923566879,0.931090733653289)
--(axis cs:66.8789808917197,0.928025256573508)
--(axis cs:66.2420382165605,0.923242822851867)
--(axis cs:65.6050955414013,0.920114754851779)
--(axis cs:64.968152866242,0.915618012873074)
--(axis cs:64.3312101910828,0.914671252714022)
--(axis cs:63.6942675159236,0.90897758327152)
--(axis cs:63.0573248407643,0.907310971608106)
--(axis cs:62.4203821656051,0.905676089129584)
--(axis cs:61.7834394904459,0.899823506638559)
--(axis cs:61.1464968152866,0.903168041061955)
--(axis cs:60.5095541401274,0.897829175700484)
--(axis cs:59.8726114649682,0.896446556106848)
--(axis cs:59.2356687898089,0.895510728048442)
--(axis cs:58.5987261146497,0.887798525984529)
--(axis cs:57.9617834394904,0.891987504793855)
--(axis cs:57.3248407643312,0.889855614636006)
--(axis cs:56.687898089172,0.887452813859055)
--(axis cs:56.0509554140127,0.887945978618554)
--(axis cs:55.4140127388535,0.885229746398004)
--(axis cs:54.7770700636943,0.879640641531663)
--(axis cs:54.140127388535,0.877958012788756)
--(axis cs:53.5031847133758,0.878017205663319)
--(axis cs:52.8662420382166,0.873541279673804)
--(axis cs:52.2292993630573,0.872184843546579)
--(axis cs:51.5923566878981,0.871559829243701)
--(axis cs:50.9554140127388,0.87011237220567)
--(axis cs:50.3184713375796,0.869269765965492)
--(axis cs:49.6815286624204,0.868290129165978)
--(axis cs:49.0445859872611,0.863520919550329)
--(axis cs:48.4076433121019,0.865741777142586)
--(axis cs:47.7707006369427,0.86406511009733)
--(axis cs:47.1337579617834,0.865996058672252)
--(axis cs:46.4968152866242,0.864182588573181)
--(axis cs:45.859872611465,0.857230229631092)
--(axis cs:45.2229299363057,0.856303185500528)
--(axis cs:44.5859872611465,0.85723244364323)
--(axis cs:43.9490445859873,0.856744888228641)
--(axis cs:43.312101910828,0.857854342550775)
--(axis cs:42.6751592356688,0.858236269263475)
--(axis cs:42.0382165605096,0.865921735613647)
--(axis cs:41.4012738853503,0.85567204823796)
--(axis cs:40.7643312101911,0.84909541254531)
--(axis cs:40.1273885350318,0.84665847080027)
--(axis cs:39.4904458598726,0.839889298046896)
--(axis cs:38.8535031847134,0.837786380233696)
--(axis cs:38.2165605095541,0.826078170689575)
--(axis cs:37.5796178343949,0.821300297865796)
--(axis cs:36.9426751592357,0.813421887108985)
--(axis cs:36.3057324840764,0.810595298842705)
--(axis cs:35.6687898089172,0.799864845360401)
--(axis cs:35.031847133758,0.79169307096167)
--(axis cs:34.3949044585987,0.779433209317278)
--(axis cs:33.7579617834395,0.772025185761757)
--(axis cs:33.1210191082803,0.763920663648181)
--(axis cs:32.484076433121,0.752192399473374)
--(axis cs:31.8471337579618,0.738649504084013)
--(axis cs:31.2101910828025,0.724771762427299)
--(axis cs:30.5732484076433,0.722544837643731)
--(axis cs:29.9363057324841,0.706722241435086)
--(axis cs:29.2993630573248,0.687620354589332)
--(axis cs:28.6624203821656,0.663201806936592)
--(axis cs:28.0254777070064,0.647880238501137)
--(axis cs:27.3885350318471,0.627505947128815)
--(axis cs:26.7515923566879,0.619818644967728)
--(axis cs:26.1146496815287,0.614613534133623)
--(axis cs:25.4777070063694,0.605831007387744)
--(axis cs:24.8407643312102,0.587055879262773)
--(axis cs:24.203821656051,0.58039266840203)
--(axis cs:23.5668789808917,0.562100623203149)
--(axis cs:22.9299363057325,0.546657049968047)
--(axis cs:22.2929936305732,0.522014880585921)
--(axis cs:21.656050955414,0.50353730841484)
--(axis cs:21.0191082802548,0.49155280232893)
--(axis cs:20.3821656050955,0.477435618743755)
--(axis cs:19.7452229299363,0.460096322582608)
--(axis cs:19.1082802547771,0.4422314143073)
--(axis cs:18.4713375796178,0.413471671179111)
--(axis cs:17.8343949044586,0.398408912225783)
--(axis cs:17.1974522292994,0.381509380748716)
--(axis cs:16.5605095541401,0.360661156566865)
--(axis cs:15.9235668789809,0.342220272145877)
--(axis cs:15.2866242038217,0.320373627749955)
--(axis cs:14.6496815286624,0.298654940960762)
--(axis cs:14.0127388535032,0.27420726095819)
--(axis cs:13.3757961783439,0.253132493525903)
--(axis cs:12.7388535031847,0.229667958633671)
--(axis cs:12.1019108280255,0.201799641440423)
--(axis cs:11.4649681528662,0.167174431643735)
--(axis cs:10.828025477707,0.143078707316935)
--(axis cs:10.1910828025478,0.121342395164482)
--(axis cs:9.55414012738853,0.104313392236032)
--(axis cs:8.9171974522293,0.0951921987522712)
--(axis cs:8.28025477707006,0.089223246720187)
--(axis cs:7.64331210191083,0.0859135003550983)
--(axis cs:7.00636942675159,0.0836323003856951)
--(axis cs:6.36942675159236,0.0831032305027944)
--(axis cs:5.73248407643312,0.0817684507674359)
--(axis cs:5.09554140127389,0.0812674612898246)
--(axis cs:4.45859872611465,0.0808462447129707)
--(axis cs:3.82165605095541,0.0805170110339466)
--(axis cs:3.18471337579618,0.0806560914041064)
--(axis cs:2.54777070063694,0.0805166991588504)
--(axis cs:1.91082802547771,0.0802368812147328)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0803902433438268)
--cycle;


==> img/mnist/mnist_rate_accuracy_lcg_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color8, mark=oplus*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table {%
0 0.0799609375
0.636942675159236 0.0799609375
1.27388535031847 0.08
1.91082802547771 0.0800390625
2.54777070063694 0.08015625
3.18471337579618 0.08
3.82165605095541 0.0803515625
4.45859872611465 0.080546875
5.09554140127389 0.08125
5.73248407643312 0.081953125
6.36942675159236 0.0826953125
7.00636942675159 0.0853125
7.64331210191083 0.08578125
8.28025477707006 0.091953125
8.9171974522293 0.0987109375
9.55414012738853 0.1055859375
10.1910828025478 0.1188671875
10.828025477707 0.140703125
11.4649681528662 0.14921875
12.1019108280255 0.1662890625
12.7388535031847 0.1837890625
13.3757961783439 0.206328125
14.0127388535032 0.2279296875
14.6496815286624 0.24484375
15.2866242038217 0.2573046875
15.9235668789809 0.278359375
16.5605095541401 0.29390625
17.1974522292994 0.3228515625
17.8343949044586 0.34375
18.4713375796178 0.35796875
19.1082802547771 0.393515625
19.7452229299363 0.4217578125
20.3821656050955 0.4382421875
21.0191082802548 0.4574609375
21.656050955414 0.475078125
22.2929936305732 0.4904296875
22.9299363057325 0.5173046875
23.5668789808917 0.5340234375
24.203821656051 0.5559765625
24.8407643312102 0.57671875
25.4777070063694 0.592890625
26.1146496815287 0.613671875
26.7515923566879 0.631484375
27.3885350318471 0.6451171875
28.0254777070064 0.6648828125
28.6624203821656 0.6794140625
29.2993630573248 0.689140625
29.9363057324841 0.7107421875
30.5732484076433 0.7176953125
31.2101910828025 0.7325390625
31.8471337579618 0.7430859375
32.484076433121 0.7507421875
33.1210191082803 0.759453125
33.7579617834395 0.7755078125
34.3949044585987 0.7809375
35.031847133758 0.786796875
35.6687898089172 0.8016015625
36.3057324840764 0.814296875
36.9426751592357 0.816328125
37.5796178343949 0.820390625
38.2165605095541 0.8190234375
38.8535031847134 0.8282421875
39.4904458598726 0.8351171875
40.1273885350318 0.845859375
40.7643312101911 0.8425390625
41.4012738853503 0.8415625
42.0382165605096 0.847734375
42.6751592356688 0.84671875
43.312101910828 0.849140625
43.9490445859873 0.8514453125
44.5859872611465 0.85734375
45.2229299363057 0.863984375
45.859872611465 0.8741015625
46.4968152866242 0.8788671875
47.1337579617834 0.88640625
47.7707006369427 0.8823828125
48.4076433121019 0.8880859375
49.0445859872611 0.8860546875
49.6815286624204 0.8934375
50.3184713375796 0.8901171875
50.9554140127388 0.894609375
51.5923566878981 0.893203125
52.2292993630573 0.8962890625
52.8662420382166 0.8956640625
53.5031847133758 0.8921875
54.140127388535 0.893984375
54.7770700636943 0.8955078125
55.4140127388535 0.8962890625
56.0509554140127 0.8969140625
56.687898089172 0.8994921875
57.3248407643312 0.901953125
57.9617834394904 0.9055078125
58.5987261146497 0.9125390625
59.2356687898089 0.911484375
59.8726114649682 0.9105078125
60.5095541401274 0.9175
61.1464968152866 0.9216796875
61.7834394904459 0.9223828125
62.4203821656051 0.926953125
63.0573248407643 0.926484375
63.6942675159236 0.9321875
64.3312101910828 0.9305078125
64.968152866242 0.9327734375
65.6050955414013 0.935390625
66.2420382165605 0.9344140625
66.8789808917197 0.934140625
67.515923566879 0.9355078125
68.1528662420382 0.9405078125
68.7898089171974 0.9439453125
69.4267515923567 0.9456640625
70.0636942675159 0.9476953125
70.7006369426752 0.952734375
71.3375796178344 0.9557421875
71.9745222929936 0.955703125
72.6114649681529 0.9594921875
73.2484076433121 0.9576953125
73.8853503184713 0.9555078125
74.5222929936306 0.95578125
75.1592356687898 0.9547265625
75.796178343949 0.9547265625
76.4331210191083 0.9540625
77.0700636942675 0.956953125
77.7070063694268 0.958828125
78.343949044586 0.959609375
78.9808917197452 0.960625
79.6178343949044 0.95890625
80.2547770700637 0.959140625
80.8917197452229 0.9610546875
81.5286624203822 0.961015625
82.1656050955414 0.9657421875
82.8025477707006 0.9632421875
83.4394904458599 0.962421875
84.0764331210191 0.964921875
84.7133757961783 0.9693359375
85.3503184713376 0.9771875
85.9872611464968 0.97671875
86.6242038216561 0.9812109375
87.2611464968153 0.983046875
87.8980891719745 0.9883203125
88.5350318471338 0.987890625
89.171974522293 0.9840625
89.8089171974522 0.9891015625
90.4458598726115 0.98796875
91.0828025477707 0.991953125
91.7197452229299 0.9894140625
92.3566878980892 0.996640625
92.9936305732484 0.9983984375
93.6305732484076 0.9988671875
94.2675159235669 0.9983984375
94.9044585987261 0.9966015625
95.5414012738853 0.9979296875
96.1783439490446 0.9997265625
96.8152866242038 0.9999609375
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color8, fill opacity=0.25]
(axis cs:0,0.0802368812147328)
--(axis cs:0,0.0796849937852672)
--(axis cs:0.636942675159236,0.0796849937852672)
--(axis cs:1.27388535031847,0.0794481125705343)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0794807697591671)
--(axis cs:3.18471337579618,0.0796097566561732)
--(axis cs:3.82165605095541,0.0794378272748438)
--(axis cs:4.45859872611465,0.0793790760993065)
--(axis cs:5.09554140127389,0.0795573992641118)
--(axis cs:5.73248407643312,0.0797963114935755)
--(axis cs:6.36942675159236,0.0803558579706517)
--(axis cs:7.00636942675159,0.0820970187442681)
--(axis cs:7.64331210191083,0.0823660289364563)
--(axis cs:8.28025477707006,0.0872526412218591)
--(axis cs:8.9171974522293,0.0930171326800074)
--(axis cs:9.55414012738853,0.0990448706814846)
--(axis cs:10.1910828025478,0.111101606112014)
--(axis cs:10.828025477707,0.131751250296078)
--(axis cs:11.4649681528662,0.139648655485183)
--(axis cs:12.1019108280255,0.156256063488999)
--(axis cs:12.7388535031847,0.173226579982163)
--(axis cs:13.3757961783439,0.195315826593657)
--(axis cs:14.0127388535032,0.216840226102395)
--(axis cs:14.6496815286624,0.233381965174465)
--(axis cs:15.2866242038217,0.245627968186112)
--(axis cs:15.9235668789809,0.266362465163587)
--(axis cs:16.5605095541401,0.281364798134735)
--(axis cs:17.1974522292994,0.309784193544828)
--(axis cs:17.8343949044586,0.330069855057692)
--(axis cs:18.4713375796178,0.344161696459218)
--(axis cs:19.1082802547771,0.379505494462185)
--(axis cs:19.7452229299363,0.407797883371694)
--(axis cs:20.3821656050955,0.424571484207226)
--(axis cs:21.0191082802548,0.443661078986257)
--(axis cs:21.656050955414,0.461448866643449)
--(axis cs:22.2929936305732,0.47656144159622)
--(axis cs:22.9299363057325,0.503760366088711)
--(axis cs:23.5668789808917,0.520579782387515)
--(axis cs:24.203821656051,0.542436785585264)
--(axis cs:24.8407643312102,0.563334699074524)
--(axis cs:25.4777070063694,0.579278422197236)
--(axis cs:26.1146496815287,0.600216780360345)
--(axis cs:26.7515923566879,0.617930117127469)
--(axis cs:27.3885350318471,0.63186319005735)
--(axis cs:28.0254777070064,0.651282738808172)
--(axis cs:28.6624203821656,0.666079619846198)
--(axis cs:29.2993630573248,0.675573565497997)
--(axis cs:29.9363057324841,0.697283089938963)
--(axis cs:30.5732484076433,0.704407999637159)
--(axis cs:31.2101910828025,0.719319467603121)
--(axis cs:31.8471337579618,0.730307309566552)
--(axis cs:32.484076433121,0.73825643516948)
--(axis cs:33.1210191082803,0.746864189386646)
--(axis cs:33.7579617834395,0.763282393000103)
--(axis cs:34.3949044585987,0.768877793314311)
--(axis cs:35.031847133758,0.774818760185535)
--(axis cs:35.6687898089172,0.789950010320815)
--(axis cs:36.3057324840764,0.802743127888225)
--(axis cs:36.9426751592357,0.805091488085699)
--(axis cs:37.5796178343949,0.80933259077824)
--(axis cs:38.2165605095541,0.808224546794552)
--(axis cs:38.8535031847134,0.817889898073781)
--(axis cs:39.4904458598726,0.825141114906385)
--(axis cs:40.1273885350318,0.836294747308817)
--(axis cs:40.7643312101911,0.832938133477917)
--(axis cs:41.4012738853503,0.831871008926019)
--(axis cs:42.0382165605096,0.838212108155148)
--(axis cs:42.6751592356688,0.837135258620639)
--(axis cs:43.312101910828,0.840200443323347)
--(axis cs:43.9490445859873,0.842410600118164)
--(axis cs:44.5859872611465,0.84854150700761)
--(axis cs:45.2229299363057,0.855439610073986)
--(axis cs:45.859872611465,0.865646759044714)
--(axis cs:46.4968152866242,0.870658714584466)
--(axis cs:47.1337579617834,0.878140782694888)
--(axis cs:47.7707006369427,0.874256422088456)
--(axis cs:48.4076433121019,0.880024812963548)
--(axis cs:49.0445859872611,0.878126965470381)
--(axis cs:49.6815286624204,0.885588236523818)
--(axis cs:50.3184713375796,0.882139549350315)
--(axis cs:50.9554140127388,0.88663051349171)
--(axis cs:51.5923566878981,0.88526262240994)
--(axis cs:52.2292993630573,0.888356079260286)
--(axis cs:52.8662420382166,0.887465307400579)
--(axis cs:53.5031847133758,0.884070237249112)
--(axis cs:54.140127388535,0.885752236946989)
--(axis cs:54.7770700636943,0.887111974719343)
--(axis cs:55.4140127388535,0.88788811477206)
--(axis cs:56.0509554140127,0.888634464140719)
--(axis cs:56.687898089172,0.891184829624484)
--(axis cs:57.3248407643312,0.893625155824326)
--(axis cs:57.9617834394904,0.897793693093612)
--(axis cs:58.5987261146497,0.904944140379516)
--(axis cs:59.2356687898089,0.904236748952498)
--(axis cs:59.8726114649682,0.903448041903168)
--(axis cs:60.5095541401274,0.910973563512439)
--(axis cs:61.1464968152866,0.915101569911934)
--(axis cs:61.7834394904459,0.915619687531276)
--(axis cs:62.4203821656051,0.920593765483753)
--(axis cs:63.0573248407643,0.920135709402665)
--(axis cs:63.6942675159236,0.926029588100691)
--(axis cs:64.3312101910828,0.924259899010849)
--(axis cs:64.968152866242,0.926679952089234)
--(axis cs:65.6050955414013,0.929552191965307)
--(axis cs:66.2420382165605,0.928137190888172)
--(axis cs:66.8789808917197,0.928109684413486)
--(axis cs:67.515923566879,0.929509040858917)
--(axis cs:68.1528662420382,0.934760193052898)
--(axis cs:68.7898089171974,0.938306628553287)
--(axis cs:69.4267515923567,0.94076384024151)
--(axis cs:70.0636942675159,0.942370681588334)
--(axis cs:70.7006369426752,0.947464725300598)
--(axis cs:71.3375796178344,0.950713201736147)
--(axis cs:71.9745222929936,0.950662522662143)
--(axis cs:72.6114649681529,0.954975140567778)
--(axis cs:73.2484076433121,0.953479466201336)
--(axis cs:73.8853503184713,0.951526280089473)
--(axis cs:74.5222929936306,0.952103184176575)
--(axis cs:75.1592356687898,0.951089748002769)
--(axis cs:75.796178343949,0.951310534346938)
--(axis cs:76.4331210191083,0.950632606599423)
--(axis cs:77.0700636942675,0.95383868092962)
--(axis cs:77.7070063694268,0.956210065389153)
--(axis cs:78.343949044586,0.957010853846848)
--(axis cs:78.9808917197452,0.957638889677457)
--(axis cs:79.6178343949044,0.955613608379933)
--(axis cs:80.2547770700637,0.956176401879254)
--(axis cs:80.8917197452229,0.958330823118275)
--(axis cs:81.5286624203822,0.957861435835938)
--(axis cs:82.1656050955414,0.96196271635551)
--(axis cs:82.8025477707006,0.960211031453124)
--(axis cs:83.4394904458599,0.959453532598268)
--(axis cs:84.0764331210191,0.961967521236876)
--(axis cs:84.7133757961783,0.965290508189733)
--(axis cs:85.3503184713376,0.97385647873796)
--(axis cs:85.9872611464968,0.972528589837397)
--(axis cs:86.6242038216561,0.97758097196175)
--(axis cs:87.2611464968153,0.979651564359424)
--(axis cs:87.8980891719745,0.985115019438777)
--(axis cs:88.5350318471338,0.984776802981064)
--(axis cs:89.171974522293,0.981547970080159)
--(axis cs:89.8089171974522,0.985989200397467)
--(axis cs:90.4458598726115,0.984908897454318)
--(axis cs:91.0828025477707,0.988888309186586)
--(axis cs:91.7197452229299,0.986294431530268)
--(axis cs:92.3566878980892,0.994304134166511)
--(axis cs:92.9936305732484,0.996702099314925)
--(axis cs:93.6305732484076,0.997422471040475)
--(axis cs:94.2675159235669,0.996702099314925)
--(axis cs:94.9044585987261,0.994254286557247)
--(axis cs:95.5414012738853,0.996025742783463)
--(axis cs:96.1783439490446,0.999000782885928)
--(axis cs:96.8152866242038,0.999684993785267)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1.00023688121473)
--(axis cs:96.1783439490446,1.00045234211407)
--(axis cs:95.5414012738853,0.999833632216537)
--(axis cs:94.9044585987261,0.998948838442753)
--(axis cs:94.2675159235669,1.00009477568508)
--(axis cs:93.6305732484076,1.00031190395952)
--(axis cs:92.9936305732484,1.00009477568508)
--(axis cs:92.3566878980892,0.998977115833489)
--(axis cs:91.7197452229299,0.992533693469732)
--(axis cs:91.0828025477707,0.995017940813414)
--(axis cs:90.4458598726115,0.991028602545682)
--(axis cs:89.8089171974522,0.992213924602533)
--(axis cs:89.171974522293,0.986577029919841)
--(axis cs:88.5350318471338,0.991004447018936)
--(axis cs:87.8980891719745,0.991525605561223)
--(axis cs:87.2611464968153,0.986442185640576)
--(axis cs:86.6242038216561,0.98484090303825)
--(axis cs:85.9872611464968,0.980908910162603)
--(axis cs:85.3503184713376,0.98051852126204)
--(axis cs:84.7133757961783,0.973381366810267)
--(axis cs:84.0764331210191,0.967876228763124)
--(axis cs:83.4394904458599,0.965390217401732)
--(axis cs:82.8025477707006,0.966273343546876)
--(axis cs:82.1656050955414,0.96952165864449)
--(axis cs:81.5286624203822,0.964169814164062)
--(axis cs:80.8917197452229,0.963778551881725)
--(axis cs:80.2547770700637,0.962104848120746)
--(axis cs:79.6178343949044,0.962198891620067)
--(axis cs:78.9808917197452,0.963611110322543)
--(axis cs:78.343949044586,0.962207896153152)
--(axis cs:77.7070063694268,0.961446184610847)
--(axis cs:77.0700636942675,0.96006756907038)
--(axis cs:76.4331210191083,0.957492393400577)
--(axis cs:75.796178343949,0.958142590653062)
--(axis cs:75.1592356687898,0.958363376997231)
--(axis cs:74.5222929936306,0.959459315823425)
--(axis cs:73.8853503184713,0.959489344910527)
--(axis cs:73.2484076433121,0.961911158798664)
--(axis cs:72.6114649681529,0.964009234432222)
--(axis cs:71.9745222929936,0.960743727337857)
--(axis cs:71.3375796178344,0.960771173263853)
--(axis cs:70.7006369426752,0.958004024699402)
--(axis cs:70.0636942675159,0.953019943411667)
--(axis cs:69.4267515923567,0.95056428475849)
--(axis cs:68.7898089171974,0.949583996446714)
--(axis cs:68.1528662420382,0.946255431947102)
--(axis cs:67.515923566879,0.941506584141083)
--(axis cs:66.8789808917197,0.940171565586514)
--(axis cs:66.2420382165605,0.940690934111828)
--(axis cs:65.6050955414013,0.941229058034693)
--(axis cs:64.968152866242,0.938866922910766)
--(axis cs:64.3312101910828,0.936755725989151)
--(axis cs:63.6942675159236,0.938345411899309)
--(axis cs:63.0573248407643,0.932833040597336)
--(axis cs:62.4203821656051,0.933312484516247)
--(axis cs:61.7834394904459,0.929145937468724)
--(axis cs:61.1464968152866,0.928257805088066)
--(axis cs:60.5095541401274,0.924026436487561)
--(axis cs:59.8726114649682,0.917567583096832)
--(axis cs:59.2356687898089,0.918732001047502)
--(axis cs:58.5987261146497,0.920133984620484)
--(axis cs:57.9617834394904,0.913221931906388)
--(axis cs:57.3248407643312,0.910281094175674)
--(axis cs:56.687898089172,0.907799545375516)
--(axis cs:56.0509554140127,0.905193660859281)
--(axis cs:55.4140127388535,0.90469001022794)
--(axis cs:54.7770700636943,0.903903650280657)
--(axis cs:54.140127388535,0.902216513053011)
--(axis cs:53.5031847133758,0.900304762750888)
--(axis cs:52.8662420382166,0.903862817599421)
--(axis cs:52.2292993630573,0.904222045739714)
--(axis cs:51.5923566878981,0.90114362759006)
--(axis cs:50.9554140127388,0.90258823650829)
--(axis cs:50.3184713375796,0.898094825649685)
--(axis cs:49.6815286624204,0.901286763476182)
--(axis cs:49.0445859872611,0.893982409529619)
--(axis cs:48.4076433121019,0.896147062036452)
--(axis cs:47.7707006369427,0.890509202911544)
--(axis cs:47.1337579617834,0.894671717305112)
--(axis cs:46.4968152866242,0.887075660415534)
--(axis cs:45.859872611465,0.882556365955286)
--(axis cs:45.2229299363057,0.872529139926014)
--(axis cs:44.5859872611465,0.86614599299239)
--(axis cs:43.9490445859873,0.860480024881836)
--(axis cs:43.312101910828,0.858080806676653)
--(axis cs:42.6751592356688,0.856302241379361)
--(axis cs:42.0382165605096,0.857256641844852)
--(axis cs:41.4012738853503,0.851253991073981)
--(axis cs:40.7643312101911,0.852139991522083)
--(axis cs:40.1273885350318,0.855424002691183)
--(axis cs:39.4904458598726,0.845093260093615)
--(axis cs:38.8535031847134,0.838594476926219)
--(axis cs:38.2165605095541,0.829822328205448)
--(axis cs:37.5796178343949,0.83144865922176)
--(axis cs:36.9426751592357,0.827564761914301)
--(axis cs:36.3057324840764,0.825850622111775)
--(axis cs:35.6687898089172,0.813253114679185)
--(axis cs:35.031847133758,0.798774989814465)
--(axis cs:34.3949044585987,0.792997206685689)
--(axis cs:33.7579617834395,0.787733231999897)
--(axis cs:33.1210191082803,0.772042060613354)
--(axis cs:32.484076433121,0.76322793983052)
--(axis cs:31.8471337579618,0.755864565433448)
--(axis cs:31.2101910828025,0.745758657396879)
--(axis cs:30.5732484076433,0.73098262536284)
--(axis cs:29.9363057324841,0.724201285061037)
--(axis cs:29.2993630573248,0.702707684502003)
--(axis cs:28.6624203821656,0.692748505153802)
--(axis cs:28.0254777070064,0.678482886191828)
--(axis cs:27.3885350318471,0.65837118494265)
--(axis cs:26.7515923566879,0.645038632872531)
--(axis cs:26.1146496815287,0.627126969639655)
--(axis cs:25.4777070063694,0.606502827802764)
--(axis cs:24.8407643312102,0.590102800925475)
--(axis cs:24.203821656051,0.569516339414737)
--(axis cs:23.5668789808917,0.547467092612485)
--(axis cs:22.9299363057325,0.530849008911289)
--(axis cs:22.2929936305732,0.50429793340378)
--(axis cs:21.656050955414,0.488707383356551)
--(axis cs:21.0191082802548,0.471260796013743)
--(axis cs:20.3821656050955,0.451912890792774)
--(axis cs:19.7452229299363,0.435717741628306)
--(axis cs:19.1082802547771,0.407525755537815)
--(axis cs:18.4713375796178,0.371775803540782)
--(axis cs:17.8343949044586,0.357430144942308)
--(axis cs:17.1974522292994,0.335918931455172)
--(axis cs:16.5605095541401,0.306447701865265)
--(axis cs:15.9235668789809,0.290356284836413)
--(axis cs:15.2866242038217,0.268981406813888)
--(axis cs:14.6496815286624,0.256305534825535)
--(axis cs:14.0127388535032,0.239019148897605)
--(axis cs:13.3757961783439,0.217340423406343)
--(axis cs:12.7388535031847,0.194351545017837)
--(axis cs:12.1019108280255,0.176322061511001)
--(axis cs:11.4649681528662,0.158788844514817)
--(axis cs:10.828025477707,0.149654999703922)
--(axis cs:10.1910828025478,0.126632768887986)
--(axis cs:9.55414012738853,0.112127004318515)
--(axis cs:8.9171974522293,0.104404742319993)
--(axis cs:8.28025477707006,0.0966536087781409)
--(axis cs:7.64331210191083,0.0891964710635437)
--(axis cs:7.00636942675159,0.0885279812557319)
--(axis cs:6.36942675159236,0.0850347670293483)
--(axis cs:5.73248407643312,0.0841099385064246)
--(axis cs:5.09554140127389,0.0829426007358882)
--(axis cs:4.45859872611465,0.0817146739006935)
--(axis cs:3.82165605095541,0.0812652977251562)
--(axis cs:3.18471337579618,0.0803902433438268)
--(axis cs:2.54777070063694,0.0808317302408329)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.0805518874294657)
--(axis cs:0.636942675159236,0.0802368812147328)
--(axis cs:0,0.0802368812147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_lcg_order.tex <==
\addplot [line width=0.5, opacity=0.7, color8, mark=oplus*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table {%
0 0.08
0.636942675159236 0.0799609375
1.27388535031847 0.08
1.91082802547771 0.0800390625
2.54777070063694 0.080078125
3.18471337579618 0.0803515625
3.82165605095541 0.080234375
4.45859872611465 0.080859375
5.09554140127389 0.0810546875
5.73248407643312 0.0821484375
6.36942675159236 0.085390625
7.00636942675159 0.0894921875
7.64331210191083 0.095703125
8.28025477707006 0.104453125
8.9171974522293 0.1091015625
9.55414012738853 0.1206640625
10.1910828025478 0.13328125
10.828025477707 0.1519140625
11.4649681528662 0.1701953125
12.1019108280255 0.1838671875
12.7388535031847 0.2053125
13.3757961783439 0.224375
14.0127388535032 0.2458203125
14.6496815286624 0.2567578125
15.2866242038217 0.27609375
15.9235668789809 0.2988671875
16.5605095541401 0.315078125
17.1974522292994 0.3291796875
17.8343949044586 0.341015625
18.4713375796178 0.3602734375
19.1082802547771 0.3791796875
19.7452229299363 0.399765625
20.3821656050955 0.4155078125
21.0191082802548 0.4405078125
21.656050955414 0.4607421875
22.2929936305732 0.468515625
22.9299363057325 0.479453125
23.5668789808917 0.494140625
24.203821656051 0.504296875
24.8407643312102 0.528515625
25.4777070063694 0.5462109375
26.1146496815287 0.5663671875
26.7515923566879 0.5859765625
27.3885350318471 0.5997265625
28.0254777070064 0.604609375
28.6624203821656 0.6154296875
29.2993630573248 0.6237890625
29.9363057324841 0.6383203125
30.5732484076433 0.6487109375
31.2101910828025 0.6672265625
31.8471337579618 0.664296875
32.484076433121 0.6725
33.1210191082803 0.6812890625
33.7579617834395 0.68875
34.3949044585987 0.6931640625
35.031847133758 0.6996484375
35.6687898089172 0.710703125
36.3057324840764 0.714609375
36.9426751592357 0.71671875
37.5796178343949 0.7253515625
38.2165605095541 0.728984375
38.8535031847134 0.7330078125
39.4904458598726 0.733984375
40.1273885350318 0.7424609375
40.7643312101911 0.75828125
41.4012738853503 0.7583984375
42.0382165605096 0.75984375
42.6751592356688 0.7751171875
43.312101910828 0.77015625
43.9490445859873 0.782734375
44.5859872611465 0.781484375
45.2229299363057 0.791015625
45.859872611465 0.8008203125
46.4968152866242 0.802734375
47.1337579617834 0.811796875
47.7707006369427 0.815234375
48.4076433121019 0.8195703125
49.0445859872611 0.82328125
49.6815286624204 0.8204296875
50.3184713375796 0.8235546875
50.9554140127388 0.8337109375
51.5923566878981 0.8398046875
52.2292993630573 0.8379296875
52.8662420382166 0.833671875
53.5031847133758 0.8408984375
54.140127388535 0.836953125
54.7770700636943 0.8427734375
55.4140127388535 0.8451171875
56.0509554140127 0.853828125
56.687898089172 0.8530859375
57.3248407643312 0.86234375
57.9617834394904 0.8716796875
58.5987261146497 0.87453125
59.2356687898089 0.8850390625
59.8726114649682 0.89125
60.5095541401274 0.89265625
61.1464968152866 0.89875
61.7834394904459 0.9051953125
62.4203821656051 0.9036328125
63.0573248407643 0.90234375
63.6942675159236 0.9035546875
64.3312101910828 0.9146875
64.968152866242 0.91578125
65.6050955414013 0.9182421875
66.2420382165605 0.92078125
66.8789808917197 0.9362109375
67.515923566879 0.9426953125
68.1528662420382 0.9471484375
68.7898089171974 0.9446484375
69.4267515923567 0.950234375
70.0636942675159 0.9547265625
70.7006369426752 0.960625
71.3375796178344 0.9622265625
71.9745222929936 0.961796875
72.6114649681529 0.9601171875
73.2484076433121 0.966171875
73.8853503184713 0.96859375
74.5222929936306 0.9694140625
75.1592356687898 0.97609375
75.796178343949 0.975390625
76.4331210191083 0.976796875
77.0700636942675 0.9784765625
77.7070063694268 0.9796484375
78.343949044586 0.98140625
78.9808917197452 0.9837109375
79.6178343949044 0.9837890625
80.2547770700637 0.9865234375
80.8917197452229 0.9894921875
81.5286624203822 0.9879296875
82.1656050955414 0.9934765625
82.8025477707006 0.9916796875
83.4394904458599 0.993828125
84.0764331210191 0.99015625
84.7133757961783 0.9882421875
85.3503184713376 0.992265625
85.9872611464968 0.98734375
86.6242038216561 0.987421875
87.2611464968153 0.9900390625
87.8980891719745 0.991015625
88.5350318471338 0.994609375
89.171974522293 0.9958984375
89.8089171974522 0.9944921875
90.4458598726115 0.995390625
91.0828025477707 0.99375
91.7197452229299 0.9981640625
92.3566878980892 0.99875
92.9936305732484 0.9980859375
93.6305732484076 0.998671875
94.2675159235669 0.99984375
94.9044585987261 0.9999609375
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color8, fill opacity=0.25]
(axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.0796849937852672)
--(axis cs:1.27388535031847,0.08)
--(axis cs:1.91082802547771,0.0795611139660534)
--(axis cs:2.54777070063694,0.0796882636859699)
--(axis cs:3.18471337579618,0.0795244516788826)
--(axis cs:3.82165605095541,0.079455034682641)
--(axis cs:4.45859872611465,0.0795708536070001)
--(axis cs:5.09554140127389,0.079575016045179)
--(axis cs:5.73248407643312,0.0800793186965949)
--(axis cs:6.36942675159236,0.0821851227440611)
--(axis cs:7.00636942675159,0.0853611037583557)
--(axis cs:7.64331210191083,0.0904988622677835)
--(axis cs:8.28025477707006,0.0980813587012777)
--(axis cs:8.9171974522293,0.102276871259219)
--(axis cs:9.55414012738853,0.112822158833206)
--(axis cs:10.1910828025478,0.124578809563047)
--(axis cs:10.828025477707,0.142428209511095)
--(axis cs:11.4649681528662,0.160200094233783)
--(axis cs:12.1019108280255,0.173456135514597)
--(axis cs:12.7388535031847,0.194764607796448)
--(axis cs:13.3757961783439,0.213456194368885)
--(axis cs:14.0127388535032,0.234611100120225)
--(axis cs:14.6496815286624,0.245575152447791)
--(axis cs:15.2866242038217,0.264809552881443)
--(axis cs:15.9235668789809,0.287079966623854)
--(axis cs:16.5605095541401,0.303049583739984)
--(axis cs:17.1974522292994,0.316735369006602)
--(axis cs:17.8343949044586,0.328254366273183)
--(axis cs:18.4713375796178,0.347404441483465)
--(axis cs:19.1082802547771,0.366104714731351)
--(axis cs:19.7452229299363,0.386431847271775)
--(axis cs:20.3821656050955,0.402051394494552)
--(axis cs:21.0191082802548,0.427068491992515)
--(axis cs:21.656050955414,0.447083337721387)
--(axis cs:22.2929936305732,0.454844480261551)
--(axis cs:22.9299363057325,0.465816029781401)
--(axis cs:23.5668789808917,0.480514362673659)
--(axis cs:24.203821656051,0.490569830896948)
--(axis cs:24.8407643312102,0.514986599195356)
--(axis cs:25.4777070063694,0.532676510300668)
--(axis cs:26.1146496815287,0.553046799153742)
--(axis cs:26.7515923566879,0.573013574662371)
--(axis cs:27.3885350318471,0.587036198333287)
--(axis cs:28.0254777070064,0.591959992376323)
--(axis cs:28.6624203821656,0.602839136279056)
--(axis cs:29.2993630573248,0.611173835410666)
--(axis cs:29.9363057324841,0.625624430742555)
--(axis cs:30.5732484076433,0.636162495303615)
--(axis cs:31.2101910828025,0.654830810616598)
--(axis cs:31.8471337579618,0.651966117743444)
--(axis cs:32.484076433121,0.660305695110454)
--(axis cs:33.1210191082803,0.669121468735008)
--(axis cs:33.7579617834395,0.676887466047233)
--(axis cs:34.3949044585987,0.681430171575258)
--(axis cs:35.031847133758,0.688043196776379)
--(axis cs:35.6687898089172,0.699235491336614)
--(axis cs:36.3057324840764,0.703361087505558)
--(axis cs:36.9426751592357,0.705592846253489)
--(axis cs:37.5796178343949,0.714267746174612)
--(axis cs:38.2165605095541,0.717768856545883)
--(axis cs:38.8535031847134,0.721673066331301)
--(axis cs:39.4904458598726,0.723216735474671)
--(axis cs:40.1273885350318,0.731819633483145)
--(axis cs:40.7643312101911,0.747124971726397)
--(axis cs:41.4012738853503,0.747162762065915)
--(axis cs:42.0382165605096,0.748802586393)
--(axis cs:42.6751592356688,0.764280691577913)
--(axis cs:43.312101910828,0.759278723429259)
--(axis cs:43.9490445859873,0.77197714731425)
--(axis cs:44.5859872611465,0.770630573632743)
--(axis cs:45.2229299363057,0.780655803016881)
--(axis cs:45.859872611465,0.790788115537188)
--(axis cs:46.4968152866242,0.792522771995651)
--(axis cs:47.1337579617834,0.801600853955566)
--(axis cs:47.7707006369427,0.805647867631635)
--(axis cs:48.4076433121019,0.810027138398764)
--(axis cs:49.0445859872611,0.813661969955603)
--(axis cs:49.6815286624204,0.810804824594756)
--(axis cs:50.3184713375796,0.81405481688688)
--(axis cs:50.9554140127388,0.824631868250673)
--(axis cs:51.5923566878981,0.83080737672028)
--(axis cs:52.2292993630573,0.828659325265174)
--(axis cs:52.8662420382166,0.824384947256105)
--(axis cs:53.5031847133758,0.831636324887262)
--(axis cs:54.140127388535,0.827327573172795)
--(axis cs:54.7770700636943,0.833221242498332)
--(axis cs:55.4140127388535,0.835661023525975)
--(axis cs:56.0509554140127,0.844554508355577)
--(axis cs:56.687898089172,0.843733845724935)
--(axis cs:57.3248407643312,0.853252748386897)
--(axis cs:57.9617834394904,0.862625813807935)
--(axis cs:58.5987261146497,0.865525422208201)
--(axis cs:59.2356687898089,0.876176345876804)
--(axis cs:59.8726114649682,0.882511419527336)
--(axis cs:60.5095541401274,0.884231558738049)
--(axis cs:61.1464968152866,0.890318872951219)
--(axis cs:61.7834394904459,0.897005722676605)
--(axis cs:62.4203821656051,0.895057053758585)
--(axis cs:63.0573248407643,0.894134215179826)
--(axis cs:63.6942675159236,0.895092185646745)
--(axis cs:64.3312101910828,0.906798999430284)
--(axis cs:64.968152866242,0.90773125199857)
--(axis cs:65.6050955414013,0.910488435376832)
--(axis cs:66.2420382165605,0.913270482798524)
--(axis cs:66.8789808917197,0.929282299254505)
--(axis cs:67.515923566879,0.936388646943067)
--(axis cs:68.1528662420382,0.940872563038543)
--(axis cs:68.7898089171974,0.93823795597918)
--(axis cs:69.4267515923567,0.944142320330792)
--(axis cs:70.0636942675159,0.948919696851998)
--(axis cs:70.7006369426752,0.955248305033525)
--(axis cs:71.3375796178344,0.957126082694427)
--(axis cs:71.9745222929936,0.956494553162269)
--(axis cs:72.6114649681529,0.95484336854407)
--(axis cs:73.2484076433121,0.961376360213195)
--(axis cs:73.8853503184713,0.963809559199355)
--(axis cs:74.5222929936306,0.965167787417131)
--(axis cs:75.1592356687898,0.972665986063941)
--(axis cs:75.796178343949,0.97201755034652)
--(axis cs:76.4331210191083,0.973364245657583)
--(axis cs:77.0700636942675,0.97596176592328)
--(axis cs:77.7070063694268,0.976882716423022)
--(axis cs:78.343949044586,0.978283682816482)
--(axis cs:78.9808917197452,0.980100606112012)
--(axis cs:79.6178343949044,0.980046198800482)
--(axis cs:80.2547770700637,0.983134298659077)
--(axis cs:80.8917197452229,0.986172974712505)
--(axis cs:81.5286624203822,0.98456703257439)
--(axis cs:82.1656050955414,0.990400608615425)
--(axis cs:82.8025477707006,0.988433741714049)
--(axis cs:83.4394904458599,0.990796305365847)
--(axis cs:84.0764331210191,0.986897178399226)
--(axis cs:84.7133757961783,0.985041081204018)
--(axis cs:85.3503184713376,0.989193379319165)
--(axis cs:85.9872611464968,0.984238073967708)
--(axis cs:86.6242038216561,0.984355649528244)
--(axis cs:87.2611464968153,0.986914086341949)
--(axis cs:87.8980891719745,0.987895826854511)
--(axis cs:88.5350318471338,0.991836148122269)
--(axis cs:89.171974522293,0.993374945626387)
--(axis cs:89.8089171974522,0.991700244371619)
--(axis cs:90.4458598726115,0.992758544480289)
--(axis cs:91.0828025477707,0.990853047465978)
--(axis cs:91.7197452229299,0.996359443764944)
--(axis cs:92.3566878980892,0.997237115880388)
--(axis cs:92.9936305732484,0.996247289507575)
--(axis cs:93.6305732484076,0.997115681979445)
--(axis cs:94.2675159235669,0.999293484977071)
--(axis cs:94.9044585987261,0.999684993785267)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1.00023688121473)
--(axis cs:94.2675159235669,1.00039401502293)
--(axis cs:93.6305732484076,1.00022806802056)
--(axis cs:92.9936305732484,0.999924585492425)
--(axis cs:92.3566878980892,1.00026288411961)
--(axis cs:91.7197452229299,0.999968681235056)
--(axis cs:91.0828025477707,0.996646952534022)
--(axis cs:90.4458598726115,0.998022705519711)
--(axis cs:89.8089171974522,0.997284130628381)
--(axis cs:89.171974522293,0.998421929373613)
--(axis cs:88.5350318471338,0.997382601877731)
--(axis cs:87.8980891719745,0.994135423145489)
--(axis cs:87.2611464968153,0.993164038658051)
--(axis cs:86.6242038216561,0.990488100471756)
--(axis cs:85.9872611464968,0.990449426032292)
--(axis cs:85.3503184713376,0.995337870680835)
--(axis cs:84.7133757961783,0.991443293795982)
--(axis cs:84.0764331210191,0.993415321600774)
--(axis cs:83.4394904458599,0.996859944634153)
--(axis cs:82.8025477707006,0.994925633285951)
--(axis cs:82.1656050955414,0.996552516384575)
--(axis cs:81.5286624203822,0.99129234242561)
--(axis cs:80.8917197452229,0.992811400287495)
--(axis cs:80.2547770700637,0.989912576340923)
--(axis cs:79.6178343949044,0.987531926199518)
--(axis cs:78.9808917197452,0.987321268887988)
--(axis cs:78.343949044586,0.984528817183518)
--(axis cs:77.7070063694268,0.982414158576978)
--(axis cs:77.0700636942675,0.98099135907672)
--(axis cs:76.4331210191083,0.980229504342417)
--(axis cs:75.796178343949,0.97876369965348)
--(axis cs:75.1592356687898,0.979521513936059)
--(axis cs:74.5222929936306,0.973660337582869)
--(axis cs:73.8853503184713,0.973377940800645)
--(axis cs:73.2484076433121,0.970967389786805)
--(axis cs:72.6114649681529,0.96539100645593)
--(axis cs:71.9745222929936,0.967099196837731)
--(axis cs:71.3375796178344,0.967327042305573)
--(axis cs:70.7006369426752,0.966001694966474)
--(axis cs:70.0636942675159,0.960533428148002)
--(axis cs:69.4267515923567,0.956326429669208)
--(axis cs:68.7898089171974,0.951058919020821)
--(axis cs:68.1528662420382,0.953424311961457)
--(axis cs:67.515923566879,0.949001978056933)
--(axis cs:66.8789808917197,0.943139575745495)
--(axis cs:66.2420382165605,0.928292017201476)
--(axis cs:65.6050955414013,0.925995939623168)
--(axis cs:64.968152866242,0.92383124800143)
--(axis cs:64.3312101910828,0.922576000569716)
--(axis cs:63.6942675159236,0.912017189353255)
--(axis cs:63.0573248407643,0.910553284820174)
--(axis cs:62.4203821656051,0.912208571241415)
--(axis cs:61.7834394904459,0.913384902323395)
--(axis cs:61.1464968152866,0.907181127048781)
--(axis cs:60.5095541401274,0.901080941261951)
--(axis cs:59.8726114649682,0.899988580472664)
--(axis cs:59.2356687898089,0.893901779123196)
--(axis cs:58.5987261146497,0.883537077791799)
--(axis cs:57.9617834394904,0.880733561192065)
--(axis cs:57.3248407643312,0.871434751613103)
--(axis cs:56.687898089172,0.862438029275064)
--(axis cs:56.0509554140127,0.863101741644423)
--(axis cs:55.4140127388535,0.854573351474025)
--(axis cs:54.7770700636943,0.852325632501668)
--(axis cs:54.140127388535,0.846578676827205)
--(axis cs:53.5031847133758,0.850160550112738)
--(axis cs:52.8662420382166,0.842958802743895)
--(axis cs:52.2292993630573,0.847200049734826)
--(axis cs:51.5923566878981,0.84880199827972)
--(axis cs:50.9554140127388,0.842790006749327)
--(axis cs:50.3184713375796,0.833054558113121)
--(axis cs:49.6815286624204,0.830054550405244)
--(axis cs:49.0445859872611,0.832900530044397)
--(axis cs:48.4076433121019,0.829113486601236)
--(axis cs:47.7707006369427,0.824820882368365)
--(axis cs:47.1337579617834,0.821992896044434)
--(axis cs:46.4968152866242,0.812945978004349)
--(axis cs:45.859872611465,0.810852509462812)
--(axis cs:45.2229299363057,0.801375446983119)
--(axis cs:44.5859872611465,0.792338176367257)
--(axis cs:43.9490445859873,0.79349160268575)
--(axis cs:43.312101910828,0.781033776570741)
--(axis cs:42.6751592356688,0.785953683422087)
--(axis cs:42.0382165605096,0.770884913607)
--(axis cs:41.4012738853503,0.769634112934085)
--(axis cs:40.7643312101911,0.769437528273603)
--(axis cs:40.1273885350318,0.753102241516854)
--(axis cs:39.4904458598726,0.744752014525329)
--(axis cs:38.8535031847134,0.744342558668699)
--(axis cs:38.2165605095541,0.740199893454117)
--(axis cs:37.5796178343949,0.736435378825388)
--(axis cs:36.9426751592357,0.727844653746511)
--(axis cs:36.3057324840764,0.725857662494442)
--(axis cs:35.6687898089172,0.722170758663386)
--(axis cs:35.031847133758,0.711253678223621)
--(axis cs:34.3949044585987,0.704897953424742)
--(axis cs:33.7579617834395,0.700612533952767)
--(axis cs:33.1210191082803,0.693456656264992)
--(axis cs:32.484076433121,0.684694304889546)
--(axis cs:31.8471337579618,0.676627632256556)
--(axis cs:31.2101910828025,0.679622314383402)
--(axis cs:30.5732484076433,0.661259379696385)
--(axis cs:29.9363057324841,0.651016194257445)
--(axis cs:29.2993630573248,0.636404289589334)
--(axis cs:28.6624203821656,0.628020238720944)
--(axis cs:28.0254777070064,0.617258757623677)
--(axis cs:27.3885350318471,0.612416926666713)
--(axis cs:26.7515923566879,0.598939550337629)
--(axis cs:26.1146496815287,0.579687575846258)
--(axis cs:25.4777070063694,0.559745364699332)
--(axis cs:24.8407643312102,0.542044650804644)
--(axis cs:24.203821656051,0.518023919103052)
--(axis cs:23.5668789808917,0.507766887326341)
--(axis cs:22.9299363057325,0.493090220218599)
--(axis cs:22.2929936305732,0.482186769738449)
--(axis cs:21.656050955414,0.474401037278613)
--(axis cs:21.0191082802548,0.453947133007485)
--(axis cs:20.3821656050955,0.428964230505448)
--(axis cs:19.7452229299363,0.413099402728225)
--(axis cs:19.1082802547771,0.392254660268649)
--(axis cs:18.4713375796178,0.373142433516535)
--(axis cs:17.8343949044586,0.353776883726817)
--(axis cs:17.1974522292994,0.341624005993398)
--(axis cs:16.5605095541401,0.327106666260016)
--(axis cs:15.9235668789809,0.310654408376146)
--(axis cs:15.2866242038217,0.287377947118557)
--(axis cs:14.6496815286624,0.267940472552209)
--(axis cs:14.0127388535032,0.257029524879775)
--(axis cs:13.3757961783439,0.235293805631115)
--(axis cs:12.7388535031847,0.215860392203552)
--(axis cs:12.1019108280255,0.194278239485403)
--(axis cs:11.4649681528662,0.180190530766217)
--(axis cs:10.828025477707,0.161399915488905)
--(axis cs:10.1910828025478,0.141983690436953)
--(axis cs:9.55414012738853,0.128505966166794)
--(axis cs:8.9171974522293,0.115926253740781)
--(axis cs:8.28025477707006,0.110824891298722)
--(axis cs:7.64331210191083,0.100907387732216)
--(axis cs:7.00636942675159,0.0936232712416443)
--(axis cs:6.36942675159236,0.0885961272559389)
--(axis cs:5.73248407643312,0.0842175563034051)
--(axis cs:5.09554140127389,0.082534358954821)
--(axis cs:4.45859872611465,0.0821478963929999)
--(axis cs:3.82165605095541,0.081013715317359)
--(axis cs:3.18471337579618,0.0811786733211174)
--(axis cs:2.54777070063694,0.0804679863140301)
--(axis cs:1.91082802547771,0.0805170110339466)
--(axis cs:1.27388535031847,0.08)
--(axis cs:0.636942675159236,0.0802368812147328)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_accuracy_lime.tex <==
% lime
\addplot [line width=0.5, opacity=0.8, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table [row sep=\\]{%
0	0.0800390625 \\
0.636942675159236	0.08 \\
1.27388535031847	0.0800390625 \\
1.91082802547771	0.0800390625 \\
2.54777070063694	0.08 \\
3.18471337579618	0.08 \\
3.82165605095541	0.08 \\
4.45859872611465	0.0799609375 \\
5.09554140127389	0.0800390625 \\
5.73248407643312	0.0800390625 \\
6.36942675159236	0.0799609375 \\
7.00636942675159	0.08 \\
7.64331210191083	0.0800390625 \\
8.28025477707006	0.0801953125 \\
8.9171974522293	0.080390625 \\
9.55414012738853	0.080234375 \\
10.1910828025478	0.080390625 \\
10.828025477707	0.0811328125 \\
11.4649681528662	0.08171875 \\
12.1019108280255	0.0821875 \\
12.7388535031847	0.0814453125 \\
13.3757961783439	0.081953125 \\
14.0127388535032	0.0825 \\
14.6496815286624	0.0816796875 \\
15.2866242038217	0.0815625 \\
15.9235668789809	0.0812890625 \\
16.5605095541401	0.0811328125 \\
17.1974522292994	0.080859375 \\
17.8343949044586	0.08109375 \\
18.4713375796178	0.0808984375 \\
19.1082802547771	0.0814453125 \\
19.7452229299363	0.0815234375 \\
20.3821656050955	0.0815625 \\
21.0191082802548	0.0815234375 \\
21.656050955414	0.0808984375 \\
22.2929936305732	0.0819921875 \\
22.9299363057325	0.0817578125 \\
23.5668789808917	0.08171875 \\
24.203821656051	0.0815234375 \\
24.8407643312102	0.0807421875 \\
25.4777070063694	0.0812890625 \\
26.1146496815287	0.0812109375 \\
26.7515923566879	0.0815234375 \\
27.3885350318471	0.081640625 \\
28.0254777070064	0.0814453125 \\
28.6624203821656	0.0816796875 \\
29.2993630573248	0.08375 \\
29.9363057324841	0.0850390625 \\
30.5732484076433	0.0852734375 \\
31.2101910828025	0.0834765625 \\
31.8471337579618	0.08640625 \\
32.484076433121	0.0891796875 \\
33.1210191082803	0.093515625 \\
33.7579617834395	0.0984765625 \\
34.3949044585987	0.10734375 \\
35.031847133758	0.108671875 \\
35.6687898089172	0.111484375 \\
36.3057324840764	0.114453125 \\
36.9426751592357	0.1160546875 \\
37.5796178343949	0.114140625 \\
38.2165605095541	0.12 \\
38.8535031847134	0.12171875 \\
39.4904458598726	0.122890625 \\
40.1273885350318	0.1270703125 \\
40.7643312101911	0.13078125 \\
41.4012738853503	0.14125 \\
42.0382165605096	0.146484375 \\
42.6751592356688	0.152421875 \\
43.312101910828	0.156796875 \\
43.9490445859873	0.1628125 \\
44.5859872611465	0.1676171875 \\
45.2229299363057	0.1726953125 \\
45.859872611465	0.1781640625 \\
46.4968152866242	0.1842578125 \\
47.1337579617834	0.195625 \\
47.7707006369427	0.1987109375 \\
48.4076433121019	0.2015625 \\
49.0445859872611	0.209140625 \\
49.6815286624204	0.2283984375 \\
50.3184713375796	0.243203125 \\
50.9554140127388	0.2562890625 \\
51.5923566878981	0.2737109375 \\
52.2292993630573	0.2824609375 \\
52.8662420382166	0.2899609375 \\
53.5031847133758	0.306796875 \\
54.140127388535	0.3201953125 \\
54.7770700636943	0.33078125 \\
55.4140127388535	0.3380859375 \\
56.0509554140127	0.340390625 \\
56.687898089172	0.3444921875 \\
57.3248407643312	0.3573046875 \\
57.9617834394904	0.3652734375 \\
58.5987261146497	0.37140625 \\
59.2356687898089	0.388046875 \\
59.8726114649682	0.3884765625 \\
60.5095541401274	0.3950390625 \\
61.1464968152866	0.401640625 \\
61.7834394904459	0.410625 \\
62.4203821656051	0.4158984375 \\
63.0573248407643	0.4243359375 \\
63.6942675159236	0.4247265625 \\
64.3312101910828	0.426015625 \\
64.968152866242	0.431875 \\
65.6050955414013	0.4403125 \\
66.2420382165605	0.4420703125 \\
66.8789808917197	0.457421875 \\
67.515923566879	0.4637109375 \\
68.1528662420382	0.4755078125 \\
68.7898089171974	0.4841015625 \\
69.4267515923567	0.49484375 \\
70.0636942675159	0.502421875 \\
70.7006369426752	0.5149609375 \\
71.3375796178344	0.5283984375 \\
71.9745222929936	0.5463671875 \\
72.6114649681529	0.55765625 \\
73.2484076433121	0.566796875 \\
73.8853503184713	0.5813671875 \\
74.5222929936306	0.598046875 \\
75.1592356687898	0.6250390625 \\
75.796178343949	0.637265625 \\
76.4331210191083	0.66359375 \\
77.0700636942675	0.6820703125 \\
77.7070063694268	0.697578125 \\
78.343949044586	0.723515625 \\
78.9808917197452	0.7337109375 \\
79.6178343949044	0.7446484375 \\
80.2547770700637	0.7585546875 \\
80.8917197452229	0.7666015625 \\
81.5286624203822	0.7715625 \\
82.1656050955414	0.779296875 \\
82.8025477707006	0.7849609375 \\
83.4394904458599	0.7917578125 \\
84.0764331210191	0.796328125 \\
84.7133757961783	0.79875 \\
85.3503184713376	0.8020703125 \\
85.9872611464968	0.8098828125 \\
86.6242038216561	0.81375 \\
87.2611464968153	0.8262890625 \\
87.8980891719745	0.837734375 \\
88.5350318471338	0.8431640625 \\
89.171974522293	0.853125 \\
89.8089171974522	0.8718359375 \\
90.4458598726115	0.8872265625 \\
91.0828025477707	0.9026171875 \\
91.7197452229299	0.913125 \\
92.3566878980892	0.9168359375 \\
92.9936305732484	0.925546875 \\
93.6305732484076	0.94078125 \\
94.2675159235669	0.95484375 \\
94.9044585987261	0.9703125 \\
95.5414012738853	0.9823046875 \\
96.1783439490446	0.9898828125 \\
96.8152866242038	0.997734375 \\
97.4522292993631	1 \\
98.0891719745223	1 \\
98.7261146496815	1 \\
99.3630573248408	1 \\
100	1 \\
};
\path [fill=color3, fill opacity=0.5] (axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0796097566561732)
--(axis cs:3.18471337579618,0.0796097566561732)
--(axis cs:3.82165605095541,0.08)
--(axis cs:4.45859872611465,0.0796849937852672)
--(axis cs:5.09554140127389,0.0797631187852672)
--(axis cs:5.73248407643312,0.0797631187852672)
--(axis cs:6.36942675159236,0.0796849937852672)
--(axis cs:7.00636942675159,0.08)
--(axis cs:7.64331210191083,0.0795611139660534)
--(axis cs:8.28025477707006,0.0795785251417647)
--(axis cs:8.9171974522293,0.0795216078256564)
--(axis cs:9.55414012738853,0.0795588947591671)
--(axis cs:10.1910828025478,0.0794362880719877)
--(axis cs:10.828025477707,0.0793053012802322)
--(axis cs:11.4649681528662,0.0798535092338951)
--(axis cs:12.1019108280255,0.080148012285977)
--(axis cs:12.7388535031847,0.0796833934009735)
--(axis cs:13.3757961783439,0.0798590586886991)
--(axis cs:14.0127388535032,0.0801538987827071)
--(axis cs:14.6496815286624,0.07974338143742)
--(axis cs:15.2866242038217,0.0796825379227344)
--(axis cs:15.9235668789809,0.0795842248271232)
--(axis cs:16.5605095541401,0.0794254419589772)
--(axis cs:17.1974522292994,0.0790837658973554)
--(axis cs:17.8343949044586,0.0792402900728288)
--(axis cs:18.4713375796178,0.0790249465021004)
--(axis cs:19.1082802547771,0.0796977447654961)
--(axis cs:19.7452229299363,0.0797336602451883)
--(axis cs:20.3821656050955,0.0796371914900252)
--(axis cs:21.0191082802548,0.079514017770651)
--(axis cs:21.656050955414,0.0793712895901861)
--(axis cs:22.2929936305732,0.0799781753132004)
--(axis cs:22.9299363057325,0.0796595875180874)
--(axis cs:23.5668789808917,0.0797300151750243)
--(axis cs:24.203821656051,0.0795417960063351)
--(axis cs:24.8407643312102,0.0793145909826035)
--(axis cs:25.4777070063694,0.0793000654448602)
--(axis cs:26.1146496815287,0.0793895518965139)
--(axis cs:26.7515923566879,0.0794403227284955)
--(axis cs:27.3885350318471,0.0793853284869206)
--(axis cs:28.0254777070064,0.07932167495199)
--(axis cs:28.6624203821656,0.0792227362568453)
--(axis cs:29.2993630573248,0.0805382282384869)
--(axis cs:29.9363057324841,0.0814695336932773)
--(axis cs:30.5732484076433,0.0814112863679683)
--(axis cs:31.2101910828025,0.079229340030381)
--(axis cs:31.8471337579618,0.0818952275272626)
--(axis cs:32.484076433121,0.0843566123680843)
--(axis cs:33.1210191082803,0.0883914046531665)
--(axis cs:33.7579617834395,0.09305723176348)
--(axis cs:34.3949044585987,0.102278905775502)
--(axis cs:35.031847133758,0.103553532155711)
--(axis cs:35.6687898089172,0.106862760081461)
--(axis cs:36.3057324840764,0.110103617415401)
--(axis cs:36.9426751592357,0.112042509110882)
--(axis cs:37.5796178343949,0.110027598099997)
--(axis cs:38.2165605095541,0.115805752170054)
--(axis cs:38.8535031847134,0.117481239494404)
--(axis cs:39.4904458598726,0.118232622770727)
--(axis cs:40.1273885350318,0.122057620302874)
--(axis cs:40.7643312101911,0.125455989455387)
--(axis cs:41.4012738853503,0.135543842860431)
--(axis cs:42.0382165605096,0.140533775925542)
--(axis cs:42.6751592356688,0.146639116844797)
--(axis cs:43.312101910828,0.151027376933054)
--(axis cs:43.9490445859873,0.157165009637362)
--(axis cs:44.5859872611465,0.161976099239363)
--(axis cs:45.2229299363057,0.166986348776344)
--(axis cs:45.859872611465,0.172327505673099)
--(axis cs:46.4968152866242,0.178038321093565)
--(axis cs:47.1337579617834,0.189295233480231)
--(axis cs:47.7707006369427,0.192384173221654)
--(axis cs:48.4076433121019,0.194907954725329)
--(axis cs:49.0445859872611,0.201879770347784)
--(axis cs:49.6815286624204,0.220371119366986)
--(axis cs:50.3184713375796,0.234649697313797)
--(axis cs:50.9554140127388,0.247373173558946)
--(axis cs:51.5923566878981,0.264854359861524)
--(axis cs:52.2292993630573,0.273369059004776)
--(axis cs:52.8662420382166,0.28055555656874)
--(axis cs:53.5031847133758,0.297518390926373)
--(axis cs:54.140127388535,0.311015892844354)
--(axis cs:54.7770700636943,0.32191107980756)
--(axis cs:55.4140127388535,0.329123108202973)
--(axis cs:56.0509554140127,0.331524319461538)
--(axis cs:56.687898089172,0.335075374704274)
--(axis cs:57.3248407643312,0.347830985215515)
--(axis cs:57.9617834394904,0.355694277435024)
--(axis cs:58.5987261146497,0.36165673631267)
--(axis cs:59.2356687898089,0.378820491007594)
--(axis cs:59.8726114649682,0.379536689179761)
--(axis cs:60.5095541401274,0.386110697646487)
--(axis cs:61.1464968152866,0.393038954483419)
--(axis cs:61.7834394904459,0.402084212076992)
--(axis cs:62.4203821656051,0.407118832060027)
--(axis cs:63.0573248407643,0.415441517237106)
--(axis cs:63.6942675159236,0.415636355890518)
--(axis cs:64.3312101910828,0.416908410644278)
--(axis cs:64.968152866242,0.422498537813408)
--(axis cs:65.6050955414013,0.430368661035232)
--(axis cs:66.2420382165605,0.432145906005367)
--(axis cs:66.8789808917197,0.447570914230149)
--(axis cs:67.515923566879,0.453654588375734)
--(axis cs:68.1528662420382,0.465402108306148)
--(axis cs:68.7898089171974,0.474205137738953)
--(axis cs:69.4267515923567,0.48479720754269)
--(axis cs:70.0636942675159,0.49216644298461)
--(axis cs:70.7006369426752,0.504488635025394)
--(axis cs:71.3375796178344,0.517915255402664)
--(axis cs:71.9745222929936,0.535650755807665)
--(axis cs:72.6114649681529,0.546954922792267)
--(axis cs:73.2484076433121,0.555639474815868)
--(axis cs:73.8853503184713,0.569734168521416)
--(axis cs:74.5222929936306,0.586590226615178)
--(axis cs:75.1592356687898,0.613577999237896)
--(axis cs:75.796178343949,0.625945039824827)
--(axis cs:76.4331210191083,0.652620993625857)
--(axis cs:77.0700636942675,0.671503993403147)
--(axis cs:77.7070063694268,0.687477737884575)
--(axis cs:78.343949044586,0.713799594928576)
--(axis cs:78.9808917197452,0.724878570428051)
--(axis cs:79.6178343949044,0.736697498479555)
--(axis cs:80.2547770700637,0.751366259178735)
--(axis cs:80.8917197452229,0.760038866772619)
--(axis cs:81.5286624203822,0.765454737805417)
--(axis cs:82.1656050955414,0.773694685456325)
--(axis cs:82.8025477707006,0.779689068497693)
--(axis cs:83.4394904458599,0.786536983538602)
--(axis cs:84.0764331210191,0.791237807605499)
--(axis cs:84.7133757961783,0.793388791945504)
--(axis cs:85.3503184713376,0.796433372983015)
--(axis cs:85.9872611464968,0.804473995553544)
--(axis cs:86.6242038216561,0.808585430268283)
--(axis cs:87.2611464968153,0.820685503284708)
--(axis cs:87.8980891719745,0.831361556407681)
--(axis cs:88.5350318471338,0.836697042779548)
--(axis cs:89.171974522293,0.846478924463713)
--(axis cs:89.8089171974522,0.865311019517237)
--(axis cs:90.4458598726115,0.880667659746353)
--(axis cs:91.0828025477707,0.897317044099013)
--(axis cs:91.7197452229299,0.907966117374987)
--(axis cs:92.3566878980892,0.911430868619604)
--(axis cs:92.9936305732484,0.920462620839416)
--(axis cs:93.6305732484076,0.935577960867506)
--(axis cs:94.2675159235669,0.948955960822272)
--(axis cs:94.9044585987261,0.964915362988124)
--(axis cs:95.5414012738853,0.977305092231919)
--(axis cs:96.1783439490446,0.985881568118775)
--(axis cs:96.8152866242038,0.995670772846973)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,0.999797977153027)
--(axis cs:96.1783439490446,0.993884056881225)
--(axis cs:95.5414012738853,0.987304282768081)
--(axis cs:94.9044585987261,0.975709637011876)
--(axis cs:94.2675159235669,0.960731539177728)
--(axis cs:93.6305732484076,0.945984539132494)
--(axis cs:92.9936305732484,0.930631129160584)
--(axis cs:92.3566878980892,0.922241006380396)
--(axis cs:91.7197452229299,0.918283882625013)
--(axis cs:91.0828025477707,0.907917330900987)
--(axis cs:90.4458598726115,0.893785465253647)
--(axis cs:89.8089171974522,0.878360855482763)
--(axis cs:89.171974522293,0.859771075536287)
--(axis cs:88.5350318471338,0.849631082220452)
--(axis cs:87.8980891719745,0.844107193592319)
--(axis cs:87.2611464968153,0.831892621715292)
--(axis cs:86.6242038216561,0.818914569731717)
--(axis cs:85.9872611464968,0.815291629446456)
--(axis cs:85.3503184713376,0.807707252016985)
--(axis cs:84.7133757961783,0.804111208054496)
--(axis cs:84.0764331210191,0.801418442394501)
--(axis cs:83.4394904458599,0.796978641461398)
--(axis cs:82.8025477707006,0.790232806502307)
--(axis cs:82.1656050955414,0.784899064543675)
--(axis cs:81.5286624203822,0.777670262194583)
--(axis cs:80.8917197452229,0.773164258227381)
--(axis cs:80.2547770700637,0.765743115821265)
--(axis cs:79.6178343949044,0.752599376520445)
--(axis cs:78.9808917197452,0.742543304571949)
--(axis cs:78.343949044586,0.733231655071424)
--(axis cs:77.7070063694268,0.707678512115425)
--(axis cs:77.0700636942675,0.692636631596853)
--(axis cs:76.4331210191083,0.674566506374143)
--(axis cs:75.796178343949,0.648586210175173)
--(axis cs:75.1592356687898,0.636500125762104)
--(axis cs:74.5222929936306,0.609503523384822)
--(axis cs:73.8853503184713,0.593000206478585)
--(axis cs:73.2484076433121,0.577954275184132)
--(axis cs:72.6114649681529,0.568357577207733)
--(axis cs:71.9745222929936,0.557083619192335)
--(axis cs:71.3375796178344,0.538881619597336)
--(axis cs:70.7006369426752,0.525433239974606)
--(axis cs:70.0636942675159,0.51267730701539)
--(axis cs:69.4267515923567,0.50489029245731)
--(axis cs:68.7898089171974,0.493997987261047)
--(axis cs:68.1528662420382,0.485613516693852)
--(axis cs:67.515923566879,0.473767286624266)
--(axis cs:66.8789808917197,0.467272835769851)
--(axis cs:66.2420382165605,0.451994718994633)
--(axis cs:65.6050955414013,0.450256338964768)
--(axis cs:64.968152866242,0.441251462186592)
--(axis cs:64.3312101910828,0.435122839355722)
--(axis cs:63.6942675159236,0.433816769109483)
--(axis cs:63.0573248407643,0.433230357762894)
--(axis cs:62.4203821656051,0.424678042939973)
--(axis cs:61.7834394904459,0.419165787923008)
--(axis cs:61.1464968152866,0.410242295516581)
--(axis cs:60.5095541401274,0.403967427353513)
--(axis cs:59.8726114649682,0.397416435820239)
--(axis cs:59.2356687898089,0.397273258992406)
--(axis cs:58.5987261146497,0.38115576368733)
--(axis cs:57.9617834394904,0.374852597564976)
--(axis cs:57.3248407643312,0.366778389784485)
--(axis cs:56.687898089172,0.353909000295726)
--(axis cs:56.0509554140127,0.349256930538462)
--(axis cs:55.4140127388535,0.347048766797027)
--(axis cs:54.7770700636943,0.33965142019244)
--(axis cs:54.140127388535,0.329374732155646)
--(axis cs:53.5031847133758,0.316075359073628)
--(axis cs:52.8662420382166,0.29936631843126)
--(axis cs:52.2292993630573,0.291552815995224)
--(axis cs:51.5923566878981,0.282567515138476)
--(axis cs:50.9554140127388,0.265204951441054)
--(axis cs:50.3184713375796,0.251756552686203)
--(axis cs:49.6815286624204,0.236425755633014)
--(axis cs:49.0445859872611,0.216401479652216)
--(axis cs:48.4076433121019,0.208217045274671)
--(axis cs:47.7707006369427,0.205037701778346)
--(axis cs:47.1337579617834,0.201954766519769)
--(axis cs:46.4968152866242,0.190477303906435)
--(axis cs:45.859872611465,0.184000619326901)
--(axis cs:45.2229299363057,0.178404276223656)
--(axis cs:44.5859872611465,0.173258275760637)
--(axis cs:43.9490445859873,0.168459990362638)
--(axis cs:43.312101910828,0.162566373066946)
--(axis cs:42.6751592356688,0.158204633155203)
--(axis cs:42.0382165605096,0.152434974074458)
--(axis cs:41.4012738853503,0.146956157139569)
--(axis cs:40.7643312101911,0.136106510544613)
--(axis cs:40.1273885350318,0.132083004697126)
--(axis cs:39.4904458598726,0.127548627229273)
--(axis cs:38.8535031847134,0.125956260505596)
--(axis cs:38.2165605095541,0.124194247829946)
--(axis cs:37.5796178343949,0.118253651900003)
--(axis cs:36.9426751592357,0.120066865889118)
--(axis cs:36.3057324840764,0.118802632584599)
--(axis cs:35.6687898089172,0.116105989918539)
--(axis cs:35.031847133758,0.113790217844289)
--(axis cs:34.3949044585987,0.112408594224498)
--(axis cs:33.7579617834395,0.10389589323652)
--(axis cs:33.1210191082803,0.0986398453468335)
--(axis cs:32.484076433121,0.0940027626319157)
--(axis cs:31.8471337579618,0.0909172724727375)
--(axis cs:31.2101910828025,0.087723784969619)
--(axis cs:30.5732484076433,0.0891355886320317)
--(axis cs:29.9363057324841,0.0886085913067227)
--(axis cs:29.2993630573248,0.0869617717615131)
--(axis cs:28.6624203821656,0.0841366387431547)
--(axis cs:28.0254777070064,0.08356895004801)
--(axis cs:27.3885350318471,0.0838959215130794)
--(axis cs:26.7515923566879,0.0836065522715045)
--(axis cs:26.1146496815287,0.0830323231034861)
--(axis cs:25.4777070063694,0.0832780595551398)
--(axis cs:24.8407643312102,0.0821697840173965)
--(axis cs:24.203821656051,0.083505078993665)
--(axis cs:23.5668789808917,0.0837074848249757)
--(axis cs:22.9299363057325,0.0838560374819126)
--(axis cs:22.2929936305732,0.0840061996867996)
--(axis cs:21.656050955414,0.0824255854098139)
--(axis cs:21.0191082802548,0.083532857229349)
--(axis cs:20.3821656050955,0.0834878085099748)
--(axis cs:19.7452229299363,0.0833132147548117)
--(axis cs:19.1082802547771,0.0831928802345039)
--(axis cs:18.4713375796178,0.0827719284978996)
--(axis cs:17.8343949044586,0.0829472099271713)
--(axis cs:17.1974522292994,0.0826349841026446)
--(axis cs:16.5605095541401,0.0828401830410228)
--(axis cs:15.9235668789809,0.0829939001728768)
--(axis cs:15.2866242038217,0.0834424620772656)
--(axis cs:14.6496815286624,0.08361599356258)
--(axis cs:14.0127388535032,0.084846101217293)
--(axis cs:13.3757961783439,0.0840471913113009)
--(axis cs:12.7388535031847,0.0832072315990265)
--(axis cs:12.1019108280255,0.084226987714023)
--(axis cs:11.4649681528662,0.0835839907661049)
--(axis cs:10.828025477707,0.0829603237197678)
--(axis cs:10.1910828025478,0.0813449619280123)
--(axis cs:9.55414012738853,0.0809098552408329)
--(axis cs:8.9171974522293,0.0812596421743436)
--(axis cs:8.28025477707006,0.0808120998582353)
--(axis cs:7.64331210191083,0.0805170110339466)
--(axis cs:7.00636942675159,0.08)
--(axis cs:6.36942675159236,0.0802368812147328)
--(axis cs:5.73248407643312,0.0803150062147328)
--(axis cs:5.09554140127389,0.0803150062147328)
--(axis cs:4.45859872611465,0.0802368812147328)
--(axis cs:3.82165605095541,0.08)
--(axis cs:3.18471337579618,0.0803902433438268)
--(axis cs:2.54777070063694,0.0803902433438268)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_lrp.tex <==
% lrp-a-flat
\addplot [line width=0.5, opacity=0.8, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table [row sep=\\]{%
0	0.08 \\
0.636942675159236	0.07984375 \\
1.27388535031847	0.079921875 \\
1.91082802547771	0.080078125 \\
2.54777070063694	0.0800390625 \\
3.18471337579618	0.0801171875 \\
3.82165605095541	0.080078125 \\
4.45859872611465	0.0800390625 \\
5.09554140127389	0.0802734375 \\
5.73248407643312	0.0802734375 \\
6.36942675159236	0.08015625 \\
7.00636942675159	0.0803125 \\
7.64331210191083	0.08046875 \\
8.28025477707006	0.0805859375 \\
8.9171974522293	0.080390625 \\
9.55414012738853	0.0807421875 \\
10.1910828025478	0.0806640625 \\
10.828025477707	0.0812109375 \\
11.4649681528662	0.0812109375 \\
12.1019108280255	0.081328125 \\
12.7388535031847	0.081328125 \\
13.3757961783439	0.081796875 \\
14.0127388535032	0.083125 \\
14.6496815286624	0.0828125 \\
15.2866242038217	0.0829296875 \\
15.9235668789809	0.0844140625 \\
16.5605095541401	0.086328125 \\
17.1974522292994	0.0868359375 \\
17.8343949044586	0.0914453125 \\
18.4713375796178	0.0944140625 \\
19.1082802547771	0.0954296875 \\
19.7452229299363	0.098203125 \\
20.3821656050955	0.1030859375 \\
21.0191082802548	0.1054296875 \\
21.656050955414	0.1156640625 \\
22.2929936305732	0.1228125 \\
22.9299363057325	0.1241015625 \\
23.5668789808917	0.1341015625 \\
24.203821656051	0.1484375 \\
24.8407643312102	0.16046875 \\
25.4777070063694	0.18125 \\
26.1146496815287	0.1919921875 \\
26.7515923566879	0.2077734375 \\
27.3885350318471	0.22953125 \\
28.0254777070064	0.2441796875 \\
28.6624203821656	0.261640625 \\
29.2993630573248	0.280234375 \\
29.9363057324841	0.294453125 \\
30.5732484076433	0.3178125 \\
31.2101910828025	0.33484375 \\
31.8471337579618	0.3520703125 \\
32.484076433121	0.3730859375 \\
33.1210191082803	0.3878125 \\
33.7579617834395	0.4065625 \\
34.3949044585987	0.42328125 \\
35.031847133758	0.44859375 \\
35.6687898089172	0.468828125 \\
36.3057324840764	0.4930078125 \\
36.9426751592357	0.5148046875 \\
37.5796178343949	0.5403515625 \\
38.2165605095541	0.555390625 \\
38.8535031847134	0.5657421875 \\
39.4904458598726	0.591484375 \\
40.1273885350318	0.6108203125 \\
40.7643312101911	0.621171875 \\
41.4012738853503	0.6344140625 \\
42.0382165605096	0.6478125 \\
42.6751592356688	0.6598828125 \\
43.312101910828	0.6691796875 \\
43.9490445859873	0.6828125 \\
44.5859872611465	0.69625 \\
45.2229299363057	0.701796875 \\
45.859872611465	0.70796875 \\
46.4968152866242	0.7101953125 \\
47.1337579617834	0.7165234375 \\
47.7707006369427	0.723984375 \\
48.4076433121019	0.72765625 \\
49.0445859872611	0.747109375 \\
49.6815286624204	0.754609375 \\
50.3184713375796	0.7774609375 \\
50.9554140127388	0.781484375 \\
51.5923566878981	0.7977734375 \\
52.2292993630573	0.8065234375 \\
52.8662420382166	0.820703125 \\
53.5031847133758	0.82953125 \\
54.140127388535	0.844140625 \\
54.7770700636943	0.84578125 \\
55.4140127388535	0.8477734375 \\
56.0509554140127	0.8587890625 \\
56.687898089172	0.861640625 \\
57.3248407643312	0.868671875 \\
57.9617834394904	0.8716015625 \\
58.5987261146497	0.8783203125 \\
59.2356687898089	0.8762890625 \\
59.8726114649682	0.88921875 \\
60.5095541401274	0.89875 \\
61.1464968152866	0.903125 \\
61.7834394904459	0.9048046875 \\
62.4203821656051	0.9107421875 \\
63.0573248407643	0.91109375 \\
63.6942675159236	0.9135546875 \\
64.3312101910828	0.918203125 \\
64.968152866242	0.9240234375 \\
65.6050955414013	0.9271875 \\
66.2420382165605	0.9301953125 \\
66.8789808917197	0.92828125 \\
67.515923566879	0.930390625 \\
68.1528662420382	0.934609375 \\
68.7898089171974	0.9344921875 \\
69.4267515923567	0.9385546875 \\
70.0636942675159	0.9396875 \\
70.7006369426752	0.9416796875 \\
71.3375796178344	0.944140625 \\
71.9745222929936	0.9468359375 \\
72.6114649681529	0.9493359375 \\
73.2484076433121	0.9537109375 \\
73.8853503184713	0.95296875 \\
74.5222929936306	0.94671875 \\
75.1592356687898	0.9453515625 \\
75.796178343949	0.940390625 \\
76.4331210191083	0.9435546875 \\
77.0700636942675	0.9450390625 \\
77.7070063694268	0.949765625 \\
78.343949044586	0.954296875 \\
78.9808917197452	0.955 \\
79.6178343949044	0.9584765625 \\
80.2547770700637	0.9587109375 \\
80.8917197452229	0.96015625 \\
81.5286624203822	0.9580078125 \\
82.1656050955414	0.960078125 \\
82.8025477707006	0.95984375 \\
83.4394904458599	0.962421875 \\
84.0764331210191	0.9619140625 \\
84.7133757961783	0.9617578125 \\
85.3503184713376	0.963359375 \\
85.9872611464968	0.9645703125 \\
86.6242038216561	0.9699609375 \\
87.2611464968153	0.9690234375 \\
87.8980891719745	0.9721484375 \\
88.5350318471338	0.9766796875 \\
89.171974522293	0.98125 \\
89.8089171974522	0.9880078125 \\
90.4458598726115	0.9953515625 \\
91.0828025477707	0.998828125 \\
91.7197452229299	0.9997265625 \\
92.3566878980892	1 \\
92.9936305732484	1 \\
93.6305732484076	1 \\
94.2675159235669	1 \\
94.9044585987261	1 \\
95.5414012738853	1 \\
96.1783439490446	1 \\
96.8152866242038	1 \\
97.4522292993631	1 \\
98.0891719745223	1 \\
98.7261146496815	1 \\
99.3630573248408	1 \\
100	1 \\
};
\path [fill=color1, fill opacity=0.5] (axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.0792921326402493)
--(axis cs:1.27388535031847,0.0795320136859699)
--(axis cs:1.91082802547771,0.0796878816561732)
--(axis cs:2.54777070063694,0.0797631187852672)
--(axis cs:3.18471337579618,0.0795008835175115)
--(axis cs:3.82165605095541,0.0796878816561732)
--(axis cs:4.45859872611465,0.0795611139660534)
--(axis cs:5.09554140127389,0.0795439716226402)
--(axis cs:5.73248407643312,0.0793588872401396)
--(axis cs:6.36942675159236,0.0794807697591671)
--(axis cs:7.00636942675159,0.0794405726841588)
--(axis cs:7.64331210191083,0.0794385749176835)
--(axis cs:8.28025477707006,0.079386352098084)
--(axis cs:8.9171974522293,0.0793597269369767)
--(axis cs:9.55414012738853,0.0793143822391432)
--(axis cs:10.1910828025478,0.0794047251401709)
--(axis cs:10.828025477707,0.0796337720558918)
--(axis cs:11.4649681528662,0.0796810599268858)
--(axis cs:12.1019108280255,0.0797298893941367)
--(axis cs:12.7388535031847,0.0796820304852502)
--(axis cs:13.3757961783439,0.0798592226642076)
--(axis cs:14.0127388535032,0.0806405167513265)
--(axis cs:14.6496815286624,0.0804173697245437)
--(axis cs:15.2866242038217,0.0804907544265082)
--(axis cs:15.9235668789809,0.081561192851301)
--(axis cs:16.5605095541401,0.0829480776205506)
--(axis cs:17.1974522292994,0.0832850759785979)
--(axis cs:17.8343949044586,0.0869882079388749)
--(axis cs:18.4713375796178,0.0896137493166177)
--(axis cs:19.1082802547771,0.0903589772290817)
--(axis cs:19.7452229299363,0.092665194348619)
--(axis cs:20.3821656050955,0.0969583360980303)
--(axis cs:21.0191082802548,0.0990761065622773)
--(axis cs:21.656050955414,0.108343435532394)
--(axis cs:22.2929936305732,0.114920127986511)
--(axis cs:22.9299363057325,0.116127511460012)
--(axis cs:23.5668789808917,0.125496869552057)
--(axis cs:24.203821656051,0.13911880873066)
--(axis cs:24.8407643312102,0.150610636941507)
--(axis cs:25.4777070063694,0.170924597633018)
--(axis cs:26.1146496815287,0.181327062806431)
--(axis cs:26.7515923566879,0.196402071904634)
--(axis cs:27.3885350318471,0.217834544252708)
--(axis cs:28.0254777070064,0.232353278996435)
--(axis cs:28.6624203821656,0.249762198791871)
--(axis cs:29.2993630573248,0.268572781394209)
--(axis cs:29.9363057324841,0.282733726519407)
--(axis cs:30.5732484076433,0.306100300394366)
--(axis cs:31.2101910828025,0.322930738151475)
--(axis cs:31.8471337579618,0.340073893296518)
--(axis cs:32.484076433121,0.361147167622868)
--(axis cs:33.1210191082803,0.375888698368586)
--(axis cs:33.7579617834395,0.394229845615551)
--(axis cs:34.3949044585987,0.410844651317188)
--(axis cs:35.031847133758,0.43571497913139)
--(axis cs:35.6687898089172,0.455936968265288)
--(axis cs:36.3057324840764,0.480308586137035)
--(axis cs:36.9426751592357,0.502219321161464)
--(axis cs:37.5796178343949,0.528062561588236)
--(axis cs:38.2165605095541,0.543237129111541)
--(axis cs:38.8535031847134,0.553837978497924)
--(axis cs:39.4904458598726,0.580065977738206)
--(axis cs:40.1273885350318,0.600119410000742)
--(axis cs:40.7643312101911,0.611156959927824)
--(axis cs:41.4012738853503,0.624642770504143)
--(axis cs:42.0382165605096,0.638413450570181)
--(axis cs:42.6751592356688,0.65091606044095)
--(axis cs:43.312101910828,0.660358986051365)
--(axis cs:43.9490445859873,0.67447430236052)
--(axis cs:44.5859872611465,0.688155127408027)
--(axis cs:45.2229299363057,0.693644643348401)
--(axis cs:45.859872611465,0.699890092819301)
--(axis cs:46.4968152866242,0.702124045961092)
--(axis cs:47.1337579617834,0.70774281377073)
--(axis cs:47.7707006369427,0.715389567353569)
--(axis cs:48.4076433121019,0.718820062453674)
--(axis cs:49.0445859872611,0.73770444561163)
--(axis cs:49.6815286624204,0.745192332759121)
--(axis cs:50.3184713375796,0.767915359073159)
--(axis cs:50.9554140127388,0.772284240768209)
--(axis cs:51.5923566878981,0.788458864724337)
--(axis cs:52.2292993630573,0.797079288866743)
--(axis cs:52.8662420382166,0.811266529252887)
--(axis cs:53.5031847133758,0.820186466593142)
--(axis cs:54.140127388535,0.835087401435185)
--(axis cs:54.7770700636943,0.837113587311367)
--(axis cs:55.4140127388535,0.839437965627731)
--(axis cs:56.0509554140127,0.850959424696124)
--(axis cs:56.687898089172,0.853630096151925)
--(axis cs:57.3248407643312,0.861076001373973)
--(axis cs:57.9617834394904,0.864194951947454)
--(axis cs:58.5987261146497,0.871036457658681)
--(axis cs:59.2356687898089,0.868911661587369)
--(axis cs:59.8726114649682,0.882155381551478)
--(axis cs:60.5095541401274,0.892046572391965)
--(axis cs:61.1464968152866,0.896547120268766)
--(axis cs:61.7834394904459,0.898603888094817)
--(axis cs:62.4203821656051,0.904765215619713)
--(axis cs:63.0573248407643,0.904953843835871)
--(axis cs:63.6942675159236,0.907679452109487)
--(axis cs:64.3312101910828,0.912155332491988)
--(axis cs:64.968152866242,0.918375722865434)
--(axis cs:65.6050955414013,0.921909995058207)
--(axis cs:66.2420382165605,0.924792890878881)
--(axis cs:66.8789808917197,0.922859871175202)
--(axis cs:67.515923566879,0.925258675239874)
--(axis cs:68.1528662420382,0.929367851469926)
--(axis cs:68.7898089171974,0.929975206545706)
--(axis cs:69.4267515923567,0.934055324149133)
--(axis cs:70.0636942675159,0.935103471259652)
--(axis cs:70.7006369426752,0.936968548299828)
--(axis cs:71.3375796178344,0.939575554356949)
--(axis cs:71.9745222929936,0.942288085177346)
--(axis cs:72.6114649681529,0.944529047904636)
--(axis cs:73.2484076433121,0.948869668303788)
--(axis cs:73.8853503184713,0.948308061347159)
--(axis cs:74.5222929936306,0.941885474671241)
--(axis cs:75.1592356687898,0.940453773577977)
--(axis cs:75.796178343949,0.93554967899882)
--(axis cs:76.4331210191083,0.938545623293004)
--(axis cs:77.0700636942675,0.939786335676898)
--(axis cs:77.7070063694268,0.944477457908344)
--(axis cs:78.343949044586,0.949089778411199)
--(axis cs:78.9808917197452,0.950133664274581)
--(axis cs:79.6178343949044,0.954235589666724)
--(axis cs:80.2547770700637,0.955345757642624)
--(axis cs:80.8917197452229,0.957627125160442)
--(axis cs:81.5286624203822,0.955274391340682)
--(axis cs:82.1656050955414,0.957527293557724)
--(axis cs:82.8025477707006,0.956739753736356)
--(axis cs:83.4394904458599,0.959465403601003)
--(axis cs:84.0764331210191,0.958724147776306)
--(axis cs:84.7133757961783,0.958813538306838)
--(axis cs:85.3503184713376,0.960200559469042)
--(axis cs:85.9872611464968,0.961207834833779)
--(axis cs:86.6242038216561,0.96620503810164)
--(axis cs:87.2611464968153,0.965160669096609)
--(axis cs:87.8980891719745,0.96803231417024)
--(axis cs:88.5350318471338,0.972387444652113)
--(axis cs:89.171974522293,0.977324229378027)
--(axis cs:89.8089171974522,0.983992478466556)
--(axis cs:90.4458598726115,0.992518926224717)
--(axis cs:91.0828025477707,0.99734759779268)
--(axis cs:91.7197452229299,0.999000782885928)
--(axis cs:92.3566878980892,1)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1)
--(axis cs:91.7197452229299,1.00045234211407)
--(axis cs:91.0828025477707,1.00030865220732)
--(axis cs:90.4458598726115,0.998184198775283)
--(axis cs:89.8089171974522,0.992023146533444)
--(axis cs:89.171974522293,0.985175770621973)
--(axis cs:88.5350318471338,0.980971930347887)
--(axis cs:87.8980891719745,0.97626456082976)
--(axis cs:87.2611464968153,0.972886205903391)
--(axis cs:86.6242038216561,0.97371683689836)
--(axis cs:85.9872611464968,0.967932790166221)
--(axis cs:85.3503184713376,0.966518190530958)
--(axis cs:84.7133757961783,0.964702086693162)
--(axis cs:84.0764331210191,0.965103977223694)
--(axis cs:83.4394904458599,0.965378346398997)
--(axis cs:82.8025477707006,0.962947746263644)
--(axis cs:82.1656050955414,0.962628956442276)
--(axis cs:81.5286624203822,0.960741233659318)
--(axis cs:80.8917197452229,0.962685374839558)
--(axis cs:80.2547770700637,0.962076117357376)
--(axis cs:79.6178343949044,0.962717535333276)
--(axis cs:78.9808917197452,0.959866335725419)
--(axis cs:78.343949044586,0.959503971588801)
--(axis cs:77.7070063694268,0.955053792091656)
--(axis cs:77.0700636942675,0.950291789323103)
--(axis cs:76.4331210191083,0.948563751706996)
--(axis cs:75.796178343949,0.94523157100118)
--(axis cs:75.1592356687898,0.950249351422023)
--(axis cs:74.5222929936306,0.951552025328759)
--(axis cs:73.8853503184713,0.957629438652841)
--(axis cs:73.2484076433121,0.958552206696212)
--(axis cs:72.6114649681529,0.954142827095364)
--(axis cs:71.9745222929936,0.951383789822654)
--(axis cs:71.3375796178344,0.948705695643051)
--(axis cs:70.7006369426752,0.946390826700172)
--(axis cs:70.0636942675159,0.944271528740348)
--(axis cs:69.4267515923567,0.943054050850867)
--(axis cs:68.7898089171974,0.939009168454294)
--(axis cs:68.1528662420382,0.939850898530074)
--(axis cs:67.515923566879,0.935522574760126)
--(axis cs:66.8789808917197,0.933702628824798)
--(axis cs:66.2420382165605,0.935597734121119)
--(axis cs:65.6050955414013,0.932465004941793)
--(axis cs:64.968152866242,0.929671152134566)
--(axis cs:64.3312101910828,0.924250917508012)
--(axis cs:63.6942675159236,0.919429922890513)
--(axis cs:63.0573248407643,0.91723365616413)
--(axis cs:62.4203821656051,0.916719159380287)
--(axis cs:61.7834394904459,0.911005486905183)
--(axis cs:61.1464968152866,0.909702879731234)
--(axis cs:60.5095541401274,0.905453427608035)
--(axis cs:59.8726114649682,0.896282118448521)
--(axis cs:59.2356687898089,0.883666463412631)
--(axis cs:58.5987261146497,0.885604167341319)
--(axis cs:57.9617834394904,0.879008173052546)
--(axis cs:57.3248407643312,0.876267748626027)
--(axis cs:56.687898089172,0.869651153848075)
--(axis cs:56.0509554140127,0.866618700303876)
--(axis cs:55.4140127388535,0.856108909372269)
--(axis cs:54.7770700636943,0.854448912688633)
--(axis cs:54.140127388535,0.853193848564815)
--(axis cs:53.5031847133758,0.838876033406858)
--(axis cs:52.8662420382166,0.830139720747113)
--(axis cs:52.2292993630573,0.815967586133257)
--(axis cs:51.5923566878981,0.807088010275663)
--(axis cs:50.9554140127388,0.790684509231791)
--(axis cs:50.3184713375796,0.787006515926841)
--(axis cs:49.6815286624204,0.764026417240879)
--(axis cs:49.0445859872611,0.75651430438837)
--(axis cs:48.4076433121019,0.736492437546326)
--(axis cs:47.7707006369427,0.732579182646432)
--(axis cs:47.1337579617834,0.72530406122927)
--(axis cs:46.4968152866242,0.718266579038908)
--(axis cs:45.859872611465,0.716047407180699)
--(axis cs:45.2229299363057,0.709949106651599)
--(axis cs:44.5859872611465,0.704344872591973)
--(axis cs:43.9490445859873,0.69115069763948)
--(axis cs:43.312101910828,0.678000388948635)
--(axis cs:42.6751592356688,0.66884956455905)
--(axis cs:42.0382165605096,0.657211549429819)
--(axis cs:41.4012738853503,0.644185354495857)
--(axis cs:40.7643312101911,0.631186790072176)
--(axis cs:40.1273885350318,0.621521214999258)
--(axis cs:39.4904458598726,0.602902772261794)
--(axis cs:38.8535031847134,0.577646396502076)
--(axis cs:38.2165605095541,0.567544120888459)
--(axis cs:37.5796178343949,0.552640563411764)
--(axis cs:36.9426751592357,0.527390053838536)
--(axis cs:36.3057324840764,0.505707038862965)
--(axis cs:35.6687898089172,0.481719281734712)
--(axis cs:35.031847133758,0.46147252086861)
--(axis cs:34.3949044585987,0.435717848682812)
--(axis cs:33.7579617834395,0.418895154384449)
--(axis cs:33.1210191082803,0.399736301631414)
--(axis cs:32.484076433121,0.385024707377132)
--(axis cs:31.8471337579618,0.364066731703482)
--(axis cs:31.2101910828025,0.346756761848525)
--(axis cs:30.5732484076433,0.329524699605634)
--(axis cs:29.9363057324841,0.306172523480593)
--(axis cs:29.2993630573248,0.291895968605791)
--(axis cs:28.6624203821656,0.273519051208129)
--(axis cs:28.0254777070064,0.256006096003565)
--(axis cs:27.3885350318471,0.241227955747292)
--(axis cs:26.7515923566879,0.219144803095366)
--(axis cs:26.1146496815287,0.202657312193569)
--(axis cs:25.4777070063694,0.191575402366982)
--(axis cs:24.8407643312102,0.170326863058493)
--(axis cs:24.203821656051,0.15775619126934)
--(axis cs:23.5668789808917,0.142706255447943)
--(axis cs:22.9299363057325,0.132075613539988)
--(axis cs:22.2929936305732,0.130704872013489)
--(axis cs:21.656050955414,0.122984689467606)
--(axis cs:21.0191082802548,0.111783268437723)
--(axis cs:20.3821656050955,0.10921353890197)
--(axis cs:19.7452229299363,0.103741055651381)
--(axis cs:19.1082802547771,0.100500397770918)
--(axis cs:18.4713375796178,0.0992143756833823)
--(axis cs:17.8343949044586,0.0959024170611251)
--(axis cs:17.1974522292994,0.0903867990214021)
--(axis cs:16.5605095541401,0.0897081723794494)
--(axis cs:15.9235668789809,0.0872669321486989)
--(axis cs:15.2866242038217,0.0853686205734918)
--(axis cs:14.6496815286624,0.0852076302754563)
--(axis cs:14.0127388535032,0.0856094832486736)
--(axis cs:13.3757961783439,0.0837345273357924)
--(axis cs:12.7388535031847,0.0829742195147498)
--(axis cs:12.1019108280255,0.0829263606058634)
--(axis cs:11.4649681528662,0.0827408150731141)
--(axis cs:10.828025477707,0.0827881029441082)
--(axis cs:10.1910828025478,0.081923399859829)
--(axis cs:9.55414012738853,0.0821699927608568)
--(axis cs:8.9171974522293,0.0814215230630233)
--(axis cs:8.28025477707006,0.081785522901916)
--(axis cs:7.64331210191083,0.0814989250823165)
--(axis cs:7.00636942675159,0.0811844273158412)
--(axis cs:6.36942675159236,0.0808317302408329)
--(axis cs:5.73248407643312,0.0811879877598604)
--(axis cs:5.09554140127389,0.0810029033773598)
--(axis cs:4.45859872611465,0.0805170110339466)
--(axis cs:3.82165605095541,0.0804683683438268)
--(axis cs:3.18471337579618,0.0807334914824885)
--(axis cs:2.54777070063694,0.0803150062147328)
--(axis cs:1.91082802547771,0.0804683683438268)
--(axis cs:1.27388535031847,0.0803117363140301)
--(axis cs:0.636942675159236,0.0803953673597507)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_accuracy_pgd_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color9, mark=square*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color9, thin}]
table {%
0 0.079921875
0.636942675159236 0.0799609375
1.27388535031847 0.08
1.91082802547771 0.08
2.54777070063694 0.080078125
3.18471337579618 0.0800390625
3.82165605095541 0.0803515625
4.45859872611465 0.0804296875
5.09554140127389 0.0810546875
5.73248407643312 0.082421875
6.36942675159236 0.084453125
7.00636942675159 0.0856640625
7.64331210191083 0.0906640625
8.28025477707006 0.0956640625
8.9171974522293 0.1069921875
9.55414012738853 0.11671875
10.1910828025478 0.126171875
10.828025477707 0.1449609375
11.4649681528662 0.162734375
12.1019108280255 0.1814453125
12.7388535031847 0.196953125
13.3757961783439 0.212421875
14.0127388535032 0.234375
14.6496815286624 0.2507421875
15.2866242038217 0.2637109375
15.9235668789809 0.2838671875
16.5605095541401 0.30375
17.1974522292994 0.320625
17.8343949044586 0.332890625
18.4713375796178 0.364296875
19.1082802547771 0.3875
19.7452229299363 0.4048828125
20.3821656050955 0.418203125
21.0191082802548 0.44078125
21.656050955414 0.4596875
22.2929936305732 0.4780859375
22.9299363057325 0.489140625
23.5668789808917 0.4988671875
24.203821656051 0.5178125
24.8407643312102 0.53765625
25.4777070063694 0.5587890625
26.1146496815287 0.5755078125
26.7515923566879 0.5809765625
27.3885350318471 0.598046875
28.0254777070064 0.61046875
28.6624203821656 0.6233984375
29.2993630573248 0.6448828125
29.9363057324841 0.6564453125
30.5732484076433 0.660625
31.2101910828025 0.665078125
31.8471337579618 0.67015625
32.484076433121 0.688671875
33.1210191082803 0.6914453125
33.7579617834395 0.6928515625
34.3949044585987 0.6930078125
35.031847133758 0.6943359375
35.6687898089172 0.69375
36.3057324840764 0.6974609375
36.9426751592357 0.691875
37.5796178343949 0.7003125
38.2165605095541 0.6920703125
38.8535031847134 0.6966796875
39.4904458598726 0.694921875
40.1273885350318 0.70015625
40.7643312101911 0.705234375
41.4012738853503 0.7151953125
42.0382165605096 0.720859375
42.6751592356688 0.7348828125
43.312101910828 0.736171875
43.9490445859873 0.740234375
44.5859872611465 0.7441015625
45.2229299363057 0.7558984375
45.859872611465 0.768125
46.4968152866242 0.77546875
47.1337579617834 0.78203125
47.7707006369427 0.7884765625
48.4076433121019 0.7893359375
49.0445859872611 0.79265625
49.6815286624204 0.8004296875
50.3184713375796 0.808828125
50.9554140127388 0.814609375
51.5923566878981 0.81921875
52.2292993630573 0.8281640625
52.8662420382166 0.832421875
53.5031847133758 0.8253125
54.140127388535 0.8363671875
54.7770700636943 0.841796875
55.4140127388535 0.8487890625
56.0509554140127 0.852890625
56.687898089172 0.858125
57.3248407643312 0.862421875
57.9617834394904 0.8640234375
58.5987261146497 0.8722265625
59.2356687898089 0.87984375
59.8726114649682 0.878203125
60.5095541401274 0.8771875
61.1464968152866 0.87734375
61.7834394904459 0.8791796875
62.4203821656051 0.88515625
63.0573248407643 0.88703125
63.6942675159236 0.8944140625
64.3312101910828 0.9019921875
64.968152866242 0.904296875
65.6050955414013 0.910625
66.2420382165605 0.9175390625
66.8789808917197 0.9183203125
67.515923566879 0.916640625
68.1528662420382 0.9269921875
68.7898089171974 0.927734375
69.4267515923567 0.930859375
70.0636942675159 0.9351953125
70.7006369426752 0.936875
71.3375796178344 0.93375
71.9745222929936 0.9308984375
72.6114649681529 0.9323828125
73.2484076433121 0.92828125
73.8853503184713 0.9319140625
74.5222929936306 0.934140625
75.1592356687898 0.9342578125
75.796178343949 0.93609375
76.4331210191083 0.937421875
77.0700636942675 0.9398046875
77.7070063694268 0.9415625
78.343949044586 0.948125
78.9808917197452 0.9503125
79.6178343949044 0.955859375
80.2547770700637 0.9532421875
80.8917197452229 0.9549609375
81.5286624203822 0.9548046875
82.1656050955414 0.9544921875
82.8025477707006 0.9592578125
83.4394904458599 0.9643359375
84.0764331210191 0.96359375
84.7133757961783 0.9689453125
85.3503184713376 0.97203125
85.9872611464968 0.971328125
86.6242038216561 0.9762109375
87.2611464968153 0.9801171875
87.8980891719745 0.9819921875
88.5350318471338 0.9848046875
89.171974522293 0.9923828125
89.8089171974522 0.99234375
90.4458598726115 0.989609375
91.0828025477707 0.99109375
91.7197452229299 0.9931640625
92.3566878980892 0.9955078125
92.9936305732484 0.994921875
93.6305732484076 0.9998828125
94.2675159235669 0.9998046875
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color9, fill opacity=0.25]
(axis cs:0,0.0803121183438268)
--(axis cs:0,0.0795316316561732)
--(axis cs:0.636942675159236,0.0796849937852672)
--(axis cs:1.27388535031847,0.08)
--(axis cs:1.91082802547771,0.08)
--(axis cs:2.54777070063694,0.0795262375705343)
--(axis cs:3.18471337579618,0.0795611139660534)
--(axis cs:3.82165605095541,0.0795257137560751)
--(axis cs:4.45859872611465,0.0792289846452084)
--(axis cs:5.09554140127389,0.0793842856221431)
--(axis cs:5.73248407643312,0.0802083931725306)
--(axis cs:6.36942675159236,0.0816179385168195)
--(axis cs:7.00636942675159,0.0823405875512544)
--(axis cs:7.64331210191083,0.0861548076272893)
--(axis cs:8.28025477707006,0.0903566985554823)
--(axis cs:8.9171974522293,0.100402052347038)
--(axis cs:9.55414012738853,0.109256389014742)
--(axis cs:10.1910828025478,0.118050060896828)
--(axis cs:10.828025477707,0.135992955775719)
--(axis cs:11.4649681528662,0.153014296889207)
--(axis cs:12.1019108280255,0.171359962569139)
--(axis cs:12.7388535031847,0.186594410613858)
--(axis cs:13.3757961783439,0.201947914964501)
--(axis cs:14.0127388535032,0.223397152253049)
--(axis cs:14.6496815286624,0.239432565739107)
--(axis cs:15.2866242038217,0.251857746726474)
--(axis cs:15.9235668789809,0.271803780713341)
--(axis cs:16.5605095541401,0.291388369123502)
--(axis cs:17.1974522292994,0.307945519562424)
--(axis cs:17.8343949044586,0.319978505340151)
--(axis cs:18.4713375796178,0.350992969314151)
--(axis cs:19.1082802547771,0.374149603486681)
--(axis cs:19.7452229299363,0.391466352167196)
--(axis cs:20.3821656050955,0.4049796587292)
--(axis cs:21.0191082802548,0.427542016913132)
--(axis cs:21.656050955414,0.44633644496929)
--(axis cs:22.2929936305732,0.464845730865008)
--(axis cs:22.9299363057325,0.475693850058738)
--(axis cs:23.5668789808917,0.485496130133992)
--(axis cs:24.203821656051,0.504430909808874)
--(axis cs:24.8407643312102,0.524361341431334)
--(axis cs:25.4777070063694,0.545661508490783)
--(axis cs:26.1146496815287,0.562259021481303)
--(axis cs:26.7515923566879,0.567845444742657)
--(axis cs:27.3885350318471,0.584922210152682)
--(axis cs:28.0254777070064,0.596969981037743)
--(axis cs:28.6624203821656,0.610021942801525)
--(axis cs:29.2993630573248,0.631711335275305)
--(axis cs:29.9363057324841,0.64333214816639)
--(axis cs:30.5732484076433,0.64722620528005)
--(axis cs:31.2101910828025,0.651744246692669)
--(axis cs:31.8471337579618,0.656947948860986)
--(axis cs:32.484076433121,0.67531329954878)
--(axis cs:33.1210191082803,0.677739447203267)
--(axis cs:33.7579617834395,0.679215773112294)
--(axis cs:34.3949044585987,0.679749599689869)
--(axis cs:35.031847133758,0.681456825311217)
--(axis cs:35.6687898089172,0.680739320263393)
--(axis cs:36.3057324840764,0.684788151699677)
--(axis cs:36.9426751592357,0.679891076963112)
--(axis cs:37.5796178343949,0.68835825707172)
--(axis cs:38.2165605095541,0.679929727964334)
--(axis cs:38.8535031847134,0.684684038444372)
--(axis cs:39.4904458598726,0.682950927955945)
--(axis cs:40.1273885350318,0.688678225761625)
--(axis cs:40.7643312101911,0.693995855148987)
--(axis cs:41.4012738853503,0.704261225824268)
--(axis cs:42.0382165605096,0.710159356783945)
--(axis cs:42.6751592356688,0.724136069136813)
--(axis cs:43.312101910828,0.725725950956593)
--(axis cs:43.9490445859873,0.729991708285138)
--(axis cs:44.5859872611465,0.734518794166248)
--(axis cs:45.2229299363057,0.746305691290071)
--(axis cs:45.859872611465,0.758778430815419)
--(axis cs:46.4968152866242,0.766140517217853)
--(axis cs:47.1337579617834,0.772779512104704)
--(axis cs:47.7707006369427,0.779291495418243)
--(axis cs:48.4076433121019,0.780067713351)
--(axis cs:49.0445859872611,0.783503515977181)
--(axis cs:49.6815286624204,0.791075795412023)
--(axis cs:50.3184713375796,0.799457131288147)
--(axis cs:50.9554140127388,0.805459132241515)
--(axis cs:51.5923566878981,0.810620960838031)
--(axis cs:52.2292993630573,0.81976091561283)
--(axis cs:52.8662420382166,0.824003341233525)
--(axis cs:53.5031847133758,0.816691760050986)
--(axis cs:54.140127388535,0.828058412698226)
--(axis cs:54.7770700636943,0.833282245379185)
--(axis cs:55.4140127388535,0.84087279567557)
--(axis cs:56.0509554140127,0.844671258202552)
--(axis cs:56.687898089172,0.849969643301938)
--(axis cs:57.3248407643312,0.854429466362486)
--(axis cs:57.9617834394904,0.856556155919733)
--(axis cs:58.5987261146497,0.864865682168696)
--(axis cs:59.2356687898089,0.873202967926088)
--(axis cs:59.8726114649682,0.87153437567499)
--(axis cs:60.5095541401274,0.870487363116396)
--(axis cs:61.1464968152866,0.870965392192957)
--(axis cs:61.7834394904459,0.872660092783255)
--(axis cs:62.4203821656051,0.878558171757246)
--(axis cs:63.0573248407643,0.87983491776824)
--(axis cs:63.6942675159236,0.887224887960039)
--(axis cs:64.3312101910828,0.894982215440101)
--(axis cs:64.968152866242,0.897298146329252)
--(axis cs:65.6050955414013,0.903350613042437)
--(axis cs:66.2420382165605,0.910219677294794)
--(axis cs:66.8789808917197,0.910632877024479)
--(axis cs:67.515923566879,0.909282953998195)
--(axis cs:68.1528662420382,0.920263610308615)
--(axis cs:68.7898089171974,0.921450919049968)
--(axis cs:69.4267515923567,0.924722260447251)
--(axis cs:70.0636942675159,0.929538502568092)
--(axis cs:70.7006369426752,0.931340164570761)
--(axis cs:71.3375796178344,0.92826962752369)
--(axis cs:71.9745222929936,0.92575979928608)
--(axis cs:72.6114649681529,0.927246987888427)
--(axis cs:73.2484076433121,0.923962685964699)
--(axis cs:73.8853503184713,0.927358255173952)
--(axis cs:74.5222929936306,0.929548995994219)
--(axis cs:75.1592356687898,0.929739940924966)
--(axis cs:75.796178343949,0.931672781885627)
--(axis cs:76.4331210191083,0.933059299946204)
--(axis cs:77.0700636942675,0.935547582702656)
--(axis cs:77.7070063694268,0.937033806568386)
--(axis cs:78.343949044586,0.943632547137593)
--(axis cs:78.9808917197452,0.946280925793341)
--(axis cs:79.6178343949044,0.951933452551805)
--(axis cs:80.2547770700637,0.949463583839769)
--(axis cs:80.8917197452229,0.950678217534616)
--(axis cs:81.5286624203822,0.950878366535905)
--(axis cs:82.1656050955414,0.950304428478679)
--(axis cs:82.8025477707006,0.95506020865332)
--(axis cs:83.4394904458599,0.960314188450412)
--(axis cs:84.0764331210191,0.959162782615129)
--(axis cs:84.7133757961783,0.965159380918374)
--(axis cs:85.3503184713376,0.967845074706586)
--(axis cs:85.9872611464968,0.966593968210748)
--(axis cs:86.6242038216561,0.972084545630415)
--(axis cs:87.2611464968153,0.97597976016313)
--(axis cs:87.8980891719745,0.978419612574632)
--(axis cs:88.5350318471338,0.981586588990303)
--(axis cs:89.171974522293,0.98913925475615)
--(axis cs:89.8089171974522,0.989286820787884)
--(axis cs:90.4458598726115,0.986461664705037)
--(axis cs:91.0828025477707,0.987987498256139)
--(axis cs:91.7197452229299,0.99019961317271)
--(axis cs:92.3566878980892,0.992899532387924)
--(axis cs:92.9936305732484,0.992201596218539)
--(axis cs:93.6305732484076,0.999405800203062)
--(axis cs:94.2675159235669,0.999190078326407)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1.00041929667359)
--(axis cs:93.6305732484076,1.00035982479694)
--(axis cs:92.9936305732484,0.997642153781461)
--(axis cs:92.3566878980892,0.998116092612076)
--(axis cs:91.7197452229299,0.99612851182729)
--(axis cs:91.0828025477707,0.994200001743861)
--(axis cs:90.4458598726115,0.992757085294963)
--(axis cs:89.8089171974522,0.995400679212116)
--(axis cs:89.171974522293,0.99562637024385)
--(axis cs:88.5350318471338,0.988022786009697)
--(axis cs:87.8980891719745,0.985564762425368)
--(axis cs:87.2611464968153,0.98425461483687)
--(axis cs:86.6242038216561,0.980337329369585)
--(axis cs:85.9872611464968,0.976062281789252)
--(axis cs:85.3503184713376,0.976217425293414)
--(axis cs:84.7133757961783,0.972731244081626)
--(axis cs:84.0764331210191,0.968024717384871)
--(axis cs:83.4394904458599,0.968357686549588)
--(axis cs:82.8025477707006,0.96345541634668)
--(axis cs:82.1656050955414,0.95867994652132)
--(axis cs:81.5286624203822,0.958731008464095)
--(axis cs:80.8917197452229,0.959243657465384)
--(axis cs:80.2547770700637,0.957020791160231)
--(axis cs:79.6178343949044,0.959785297448195)
--(axis cs:78.9808917197452,0.954344074206659)
--(axis cs:78.343949044586,0.952617452862407)
--(axis cs:77.7070063694268,0.946091193431614)
--(axis cs:77.0700636942675,0.944061792297344)
--(axis cs:76.4331210191083,0.941784450053796)
--(axis cs:75.796178343949,0.940514718114372)
--(axis cs:75.1592356687898,0.938775684075034)
--(axis cs:74.5222929936306,0.938732254005781)
--(axis cs:73.8853503184713,0.936469869826048)
--(axis cs:73.2484076433121,0.932599814035301)
--(axis cs:72.6114649681529,0.937518637111573)
--(axis cs:71.9745222929936,0.93603707571392)
--(axis cs:71.3375796178344,0.93923037247631)
--(axis cs:70.7006369426752,0.942409835429239)
--(axis cs:70.0636942675159,0.940852122431908)
--(axis cs:69.4267515923567,0.93699648955275)
--(axis cs:68.7898089171974,0.934017830950032)
--(axis cs:68.1528662420382,0.933720764691385)
--(axis cs:67.515923566879,0.923998296001805)
--(axis cs:66.8789808917197,0.926007747975521)
--(axis cs:66.2420382165605,0.924858447705205)
--(axis cs:65.6050955414013,0.917899386957563)
--(axis cs:64.968152866242,0.911295603670748)
--(axis cs:64.3312101910828,0.909002159559899)
--(axis cs:63.6942675159236,0.901603237039961)
--(axis cs:63.0573248407643,0.89422758223176)
--(axis cs:62.4203821656051,0.891754328242753)
--(axis cs:61.7834394904459,0.885699282216745)
--(axis cs:61.1464968152866,0.883722107807043)
--(axis cs:60.5095541401274,0.883887636883604)
--(axis cs:59.8726114649682,0.884871874325009)
--(axis cs:59.2356687898089,0.886484532073912)
--(axis cs:58.5987261146497,0.879587442831304)
--(axis cs:57.9617834394904,0.871490719080267)
--(axis cs:57.3248407643312,0.870414283637514)
--(axis cs:56.687898089172,0.866280356698062)
--(axis cs:56.0509554140127,0.861109991797448)
--(axis cs:55.4140127388535,0.856705329324429)
--(axis cs:54.7770700636943,0.850311504620815)
--(axis cs:54.140127388535,0.844675962301774)
--(axis cs:53.5031847133758,0.833933239949014)
--(axis cs:52.8662420382166,0.840840408766475)
--(axis cs:52.2292993630573,0.836567209387169)
--(axis cs:51.5923566878981,0.827816539161969)
--(axis cs:50.9554140127388,0.823759617758485)
--(axis cs:50.3184713375796,0.818199118711853)
--(axis cs:49.6815286624204,0.809783579587977)
--(axis cs:49.0445859872611,0.801808984022819)
--(axis cs:48.4076433121019,0.798604161649)
--(axis cs:47.7707006369427,0.797661629581757)
--(axis cs:47.1337579617834,0.791282987895296)
--(axis cs:46.4968152866242,0.784796982782147)
--(axis cs:45.859872611465,0.777471569184581)
--(axis cs:45.2229299363057,0.765491183709929)
--(axis cs:44.5859872611465,0.753684330833753)
--(axis cs:43.9490445859873,0.750477041714862)
--(axis cs:43.312101910828,0.746617799043407)
--(axis cs:42.6751592356688,0.745629555863187)
--(axis cs:42.0382165605096,0.731559393216055)
--(axis cs:41.4012738853503,0.726129399175732)
--(axis cs:40.7643312101911,0.716472894851013)
--(axis cs:40.1273885350318,0.711634274238375)
--(axis cs:39.4904458598726,0.706892822044055)
--(axis cs:38.8535031847134,0.708675336555628)
--(axis cs:38.2165605095541,0.704210897035666)
--(axis cs:37.5796178343949,0.71226674292828)
--(axis cs:36.9426751592357,0.703858923036888)
--(axis cs:36.3057324840764,0.710133723300323)
--(axis cs:35.6687898089172,0.706760679736607)
--(axis cs:35.031847133758,0.707215049688783)
--(axis cs:34.3949044585987,0.706266025310131)
--(axis cs:33.7579617834395,0.706487351887706)
--(axis cs:33.1210191082803,0.705151177796733)
--(axis cs:32.484076433121,0.70203045045122)
--(axis cs:31.8471337579618,0.683364551139014)
--(axis cs:31.2101910828025,0.678412003307331)
--(axis cs:30.5732484076433,0.67402379471995)
--(axis cs:29.9363057324841,0.66955847683361)
--(axis cs:29.2993630573248,0.658054289724695)
--(axis cs:28.6624203821656,0.636774932198475)
--(axis cs:28.0254777070064,0.623967518962257)
--(axis cs:27.3885350318471,0.611171539847318)
--(axis cs:26.7515923566879,0.594107680257343)
--(axis cs:26.1146496815287,0.588756603518697)
--(axis cs:25.4777070063694,0.571916616509217)
--(axis cs:24.8407643312102,0.550951158568666)
--(axis cs:24.203821656051,0.531194090191126)
--(axis cs:23.5668789808917,0.512238244866008)
--(axis cs:22.9299363057325,0.502587399941262)
--(axis cs:22.2929936305732,0.491326144134992)
--(axis cs:21.656050955414,0.47303855503071)
--(axis cs:21.0191082802548,0.454020483086868)
--(axis cs:20.3821656050955,0.4314265912708)
--(axis cs:19.7452229299363,0.418299272832804)
--(axis cs:19.1082802547771,0.400850396513319)
--(axis cs:18.4713375796178,0.377600780685849)
--(axis cs:17.8343949044586,0.345802744659849)
--(axis cs:17.1974522292994,0.333304480437576)
--(axis cs:16.5605095541401,0.316111630876498)
--(axis cs:15.9235668789809,0.295930594286659)
--(axis cs:15.2866242038217,0.275564128273526)
--(axis cs:14.6496815286624,0.262051809260893)
--(axis cs:14.0127388535032,0.245352847746951)
--(axis cs:13.3757961783439,0.222895835035499)
--(axis cs:12.7388535031847,0.207311839386142)
--(axis cs:12.1019108280255,0.191530662430861)
--(axis cs:11.4649681528662,0.172454453110793)
--(axis cs:10.828025477707,0.153928919224281)
--(axis cs:10.1910828025478,0.134293689103172)
--(axis cs:9.55414012738853,0.124181110985258)
--(axis cs:8.9171974522293,0.113582322652962)
--(axis cs:8.28025477707006,0.100971426444518)
--(axis cs:7.64331210191083,0.0951733173727107)
--(axis cs:7.00636942675159,0.0889875374487456)
--(axis cs:6.36942675159236,0.0872883114831805)
--(axis cs:5.73248407643312,0.0846353568274694)
--(axis cs:5.09554140127389,0.0827250893778569)
--(axis cs:4.45859872611465,0.0816303903547916)
--(axis cs:3.82165605095541,0.0811774112439249)
--(axis cs:3.18471337579618,0.0805170110339466)
--(axis cs:2.54777070063694,0.0806300124294657)
--(axis cs:1.91082802547771,0.08)
--(axis cs:1.27388535031847,0.08)
--(axis cs:0.636942675159236,0.0802368812147328)
--(axis cs:0,0.0803121183438268)
--cycle;


==> img/mnist/mnist_rate_accuracy_sensitivity.tex <==
\addplot [line width=0.5, opacity=0.7, color6, mark=square, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color6, thin}]
table [row sep=\\]{%
0	0.0800390625 \\
0.636942675159236	0.079921875 \\
1.27388535031847	0.08 \\
1.91082802547771	0.0799609375 \\
2.54777070063694	0.080078125 \\
3.18471337579618	0.0799609375 \\
3.82165605095541	0.080078125 \\
4.45859872611465	0.080078125 \\
5.09554140127389	0.08 \\
5.73248407643312	0.0800390625 \\
6.36942675159236	0.080078125 \\
7.00636942675159	0.0800390625 \\
7.64331210191083	0.08015625 \\
8.28025477707006	0.0801171875 \\
8.9171974522293	0.0801953125 \\
9.55414012738853	0.080078125 \\
10.1910828025478	0.0805078125 \\
10.828025477707	0.0801953125 \\
11.4649681528662	0.0805078125 \\
12.1019108280255	0.08046875 \\
12.7388535031847	0.0803125 \\
13.3757961783439	0.08046875 \\
14.0127388535032	0.0812890625 \\
14.6496815286624	0.08109375 \\
15.2866242038217	0.0815234375 \\
15.9235668789809	0.081484375 \\
16.5605095541401	0.0822265625 \\
17.1974522292994	0.082421875 \\
17.8343949044586	0.0837890625 \\
18.4713375796178	0.0825 \\
19.1082802547771	0.083203125 \\
19.7452229299363	0.0834765625 \\
20.3821656050955	0.0845703125 \\
21.0191082802548	0.08546875 \\
21.656050955414	0.0867578125 \\
22.2929936305732	0.08796875 \\
22.9299363057325	0.0896484375 \\
23.5668789808917	0.08875 \\
24.203821656051	0.0895703125 \\
24.8407643312102	0.089140625 \\
25.4777070063694	0.088984375 \\
26.1146496815287	0.0896484375 \\
26.7515923566879	0.0922265625 \\
27.3885350318471	0.0958203125 \\
28.0254777070064	0.096640625 \\
28.6624203821656	0.0991796875 \\
29.2993630573248	0.0999609375 \\
29.9363057324841	0.102578125 \\
30.5732484076433	0.107109375 \\
31.2101910828025	0.1094921875 \\
31.8471337579618	0.114765625 \\
32.484076433121	0.116171875 \\
33.1210191082803	0.12109375 \\
33.7579617834395	0.1256640625 \\
34.3949044585987	0.1294140625 \\
35.031847133758	0.134140625 \\
35.6687898089172	0.1401171875 \\
36.3057324840764	0.1440234375 \\
36.9426751592357	0.1427734375 \\
37.5796178343949	0.1469140625 \\
38.2165605095541	0.152421875 \\
38.8535031847134	0.1559375 \\
39.4904458598726	0.165078125 \\
40.1273885350318	0.17171875 \\
40.7643312101911	0.1757421875 \\
41.4012738853503	0.1807421875 \\
42.0382165605096	0.18828125 \\
42.6751592356688	0.1955078125 \\
43.312101910828	0.2020703125 \\
43.9490445859873	0.2083203125 \\
44.5859872611465	0.2128515625 \\
45.2229299363057	0.2216796875 \\
45.859872611465	0.23375 \\
46.4968152866242	0.2341015625 \\
47.1337579617834	0.238671875 \\
47.7707006369427	0.246953125 \\
48.4076433121019	0.251953125 \\
49.0445859872611	0.2569921875 \\
49.6815286624204	0.272890625 \\
50.3184713375796	0.2794140625 \\
50.9554140127388	0.2872265625 \\
51.5923566878981	0.2959765625 \\
52.2292993630573	0.3000390625 \\
52.8662420382166	0.3098046875 \\
53.5031847133758	0.3173046875 \\
54.140127388535	0.32875 \\
54.7770700636943	0.332265625 \\
55.4140127388535	0.3379296875 \\
56.0509554140127	0.3518359375 \\
56.687898089172	0.357734375 \\
57.3248407643312	0.3718359375 \\
57.9617834394904	0.373359375 \\
58.5987261146497	0.3844140625 \\
59.2356687898089	0.393359375 \\
59.8726114649682	0.409375 \\
60.5095541401274	0.4223828125 \\
61.1464968152866	0.4371484375 \\
61.7834394904459	0.4365625 \\
62.4203821656051	0.4478125 \\
63.0573248407643	0.459921875 \\
63.6942675159236	0.4777734375 \\
64.3312101910828	0.478671875 \\
64.968152866242	0.4875390625 \\
65.6050955414013	0.5021484375 \\
66.2420382165605	0.51375 \\
66.8789808917197	0.5248046875 \\
67.515923566879	0.535859375 \\
68.1528662420382	0.544375 \\
68.7898089171974	0.552578125 \\
69.4267515923567	0.56984375 \\
70.0636942675159	0.57734375 \\
70.7006369426752	0.601640625 \\
71.3375796178344	0.6110546875 \\
71.9745222929936	0.6245703125 \\
72.6114649681529	0.64234375 \\
73.2484076433121	0.6474609375 \\
73.8853503184713	0.6596484375 \\
74.5222929936306	0.666484375 \\
75.1592356687898	0.6815234375 \\
75.796178343949	0.6938671875 \\
76.4331210191083	0.7019921875 \\
77.0700636942675	0.716484375 \\
77.7070063694268	0.7287890625 \\
78.343949044586	0.7366796875 \\
78.9808917197452	0.746484375 \\
79.6178343949044	0.75484375 \\
80.2547770700637	0.7687109375 \\
80.8917197452229	0.7834765625 \\
81.5286624203822	0.7952734375 \\
82.1656050955414	0.80984375 \\
82.8025477707006	0.815625 \\
83.4394904458599	0.82484375 \\
84.0764331210191	0.8334765625 \\
84.7133757961783	0.842421875 \\
85.3503184713376	0.852734375 \\
85.9872611464968	0.861328125 \\
86.6242038216561	0.8676171875 \\
87.2611464968153	0.8786328125 \\
87.8980891719745	0.8890234375 \\
88.5350318471338	0.900859375 \\
89.171974522293	0.9056640625 \\
89.8089171974522	0.9189453125 \\
90.4458598726115	0.923046875 \\
91.0828025477707	0.9359765625 \\
91.7197452229299	0.94171875 \\
92.3566878980892	0.94296875 \\
92.9936305732484	0.955546875 \\
93.6305732484076	0.954921875 \\
94.2675159235669	0.9679296875 \\
94.9044585987261	0.9703125 \\
95.5414012738853	0.9772265625 \\
96.1783439490446	0.9834375 \\
96.8152866242038	0.990625 \\
97.4522292993631	0.9991796875 \\
98.0891719745223	0.9997265625 \\
98.7261146496815	1 \\
99.3630573248408	1 \\
100	1 \\
};
\path [fill=color6, fill opacity=0.25]
(axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.0795316316561732)
--(axis cs:1.27388535031847,0.0796097566561732)
--(axis cs:1.91082802547771,0.0796849937852672)
--(axis cs:2.54777070063694,0.0795262375705343)
--(axis cs:3.18471337579618,0.0796849937852672)
--(axis cs:3.82165605095541,0.0796878816561732)
--(axis cs:4.45859872611465,0.0796878816561732)
--(axis cs:5.09554140127389,0.08)
--(axis cs:5.73248407643312,0.0795611139660534)
--(axis cs:6.36942675159236,0.0795270481767434)
--(axis cs:7.00636942675159,0.0795611139660534)
--(axis cs:7.64331210191083,0.0793772921809793)
--(axis cs:8.28025477707006,0.0793891529515992)
--(axis cs:8.9171974522293,0.0794658466226402)
--(axis cs:9.55414012738853,0.0792980202486001)
--(axis cs:10.1910828025478,0.0794410408841543)
--(axis cs:10.828025477707,0.0794660509262088)
--(axis cs:11.4649681528662,0.0794417395361487)
--(axis cs:12.1019108280255,0.0794375628866239)
--(axis cs:12.7388535031847,0.0794412565488254)
--(axis cs:13.3757961783439,0.07944089187329)
--(axis cs:14.0127388535032,0.0796713199554412)
--(axis cs:14.6496815286624,0.079644553788764)
--(axis cs:15.2866242038217,0.079816241518894)
--(axis cs:15.9235668789809,0.0798000700786497)
--(axis cs:16.5605095541401,0.0801668271763479)
--(axis cs:17.1974522292994,0.0802937164219664)
--(axis cs:17.8343949044586,0.0811322168008414)
--(axis cs:18.4713375796178,0.0802917078969714)
--(axis cs:19.1082802547771,0.0806963701904014)
--(axis cs:19.7452229299363,0.0809098037659862)
--(axis cs:20.3821656050955,0.0816463016829554)
--(axis cs:21.0191082802548,0.0822819432283154)
--(axis cs:21.656050955414,0.0833018857489706)
--(axis cs:22.2929936305732,0.0842341165671928)
--(axis cs:22.9299363057325,0.085602271565582)
--(axis cs:23.5668789808917,0.0848402039410833)
--(axis cs:24.203821656051,0.0854477864083398)
--(axis cs:24.8407643312102,0.085101148851573)
--(axis cs:25.4777070063694,0.0849316038570004)
--(axis cs:26.1146496815287,0.0855044605219479)
--(axis cs:26.7515923566879,0.0876113521206866)
--(axis cs:27.3885350318471,0.0907106965148081)
--(axis cs:28.0254777070064,0.0914621957319257)
--(axis cs:28.6624203821656,0.0938343039215452)
--(axis cs:29.2993630573248,0.0943998207997928)
--(axis cs:29.9363057324841,0.0967855831825735)
--(axis cs:30.5732484076433,0.100890782113838)
--(axis cs:31.2101910828025,0.102970421828276)
--(axis cs:31.8471337579618,0.108076706510872)
--(axis cs:32.484076433121,0.109540838544511)
--(axis cs:33.1210191082803,0.11445858001369)
--(axis cs:33.7579617834395,0.118751917959595)
--(axis cs:34.3949044585987,0.122325854529565)
--(axis cs:35.031847133758,0.127033448611665)
--(axis cs:35.6687898089172,0.133008407366142)
--(axis cs:36.3057324840764,0.137114894073991)
--(axis cs:36.9426751592357,0.135523951006034)
--(axis cs:37.5796178343949,0.139251128409082)
--(axis cs:38.2165605095541,0.144885637091025)
--(axis cs:38.8535031847134,0.148223834550277)
--(axis cs:39.4904458598726,0.156880487733567)
--(axis cs:40.1273885350318,0.163196336145095)
--(axis cs:40.7643312101911,0.166900815858948)
--(axis cs:41.4012738853503,0.171824694251407)
--(axis cs:42.0382165605096,0.1790771484375)
--(axis cs:42.6751592356688,0.186220411431594)
--(axis cs:43.312101910828,0.192502250157404)
--(axis cs:43.9490445859873,0.19874423298111)
--(axis cs:44.5859872611465,0.203000821068392)
--(axis cs:45.2229299363057,0.211450173462229)
--(axis cs:45.859872611465,0.22330199346711)
--(axis cs:46.4968152866242,0.22338661874226)
--(axis cs:47.1337579617834,0.22799059012359)
--(axis cs:47.7707006369427,0.236272551633995)
--(axis cs:48.4076433121019,0.24118743692757)
--(axis cs:49.0445859872611,0.245932974242191)
--(axis cs:49.6815286624204,0.261725788332831)
--(axis cs:50.3184713375796,0.268044610265491)
--(axis cs:50.9554140127388,0.275935890022164)
--(axis cs:51.5923566878981,0.284893687299526)
--(axis cs:52.2292993630573,0.288859867546647)
--(axis cs:52.8662420382166,0.298867453169643)
--(axis cs:53.5031847133758,0.306277494349817)
--(axis cs:54.140127388535,0.317579799324069)
--(axis cs:54.7770700636943,0.321160406211422)
--(axis cs:55.4140127388535,0.326591799766416)
--(axis cs:56.0509554140127,0.340684929708942)
--(axis cs:56.687898089172,0.346643509501047)
--(axis cs:57.3248407643312,0.360826582562532)
--(axis cs:57.9617834394904,0.362532130509764)
--(axis cs:58.5987261146497,0.373285902225729)
--(axis cs:59.2356687898089,0.382117448100658)
--(axis cs:59.8726114649682,0.398172496286166)
--(axis cs:60.5095541401274,0.41118957720885)
--(axis cs:61.1464968152866,0.425831795296908)
--(axis cs:61.7834394904459,0.425338335562796)
--(axis cs:62.4203821656051,0.436442831513365)
--(axis cs:63.0573248407643,0.448439385705177)
--(axis cs:63.6942675159236,0.466386187714647)
--(axis cs:64.3312101910828,0.467327069691546)
--(axis cs:64.968152866242,0.476340330434516)
--(axis cs:65.6050955414013,0.491009168656594)
--(axis cs:66.2420382165605,0.502716666853272)
--(axis cs:66.8789808917197,0.513583716386587)
--(axis cs:67.515923566879,0.524982711502674)
--(axis cs:68.1528662420382,0.533486724997598)
--(axis cs:68.7898089171974,0.541777888996442)
--(axis cs:69.4267515923567,0.558930623099385)
--(axis cs:70.0636942675159,0.566249472402304)
--(axis cs:70.7006369426752,0.590465649588183)
--(axis cs:71.3375796178344,0.600176551339304)
--(axis cs:71.9745222929936,0.614253218835856)
--(axis cs:72.6114649681529,0.632174889983507)
--(axis cs:73.2484076433121,0.637303037043942)
--(axis cs:73.8853503184713,0.649451459238784)
--(axis cs:74.5222929936306,0.65656635930184)
--(axis cs:75.1592356687898,0.671704726502261)
--(axis cs:75.796178343949,0.684567536520073)
--(axis cs:76.4331210191083,0.693399781418893)
--(axis cs:77.0700636942675,0.70741176642829)
--(axis cs:77.7070063694268,0.720234877021923)
--(axis cs:78.343949044586,0.728083362964988)
--(axis cs:78.9808917197452,0.737665608057462)
--(axis cs:79.6178343949044,0.74626027114152)
--(axis cs:80.2547770700637,0.760125905036899)
--(axis cs:80.8917197452229,0.775075667984657)
--(axis cs:81.5286624203822,0.786881611787408)
--(axis cs:82.1656050955414,0.801991070119932)
--(axis cs:82.8025477707006,0.808361970278022)
--(axis cs:83.4394904458599,0.817888119752426)
--(axis cs:84.0764331210191,0.826985348091568)
--(axis cs:84.7133757961783,0.836012660456619)
--(axis cs:85.3503184713376,0.846713672155367)
--(axis cs:85.9872611464968,0.855669010613648)
--(axis cs:86.6242038216561,0.862313643318877)
--(axis cs:87.2611464968153,0.87274387189425)
--(axis cs:87.8980891719745,0.882722350532962)
--(axis cs:88.5350318471338,0.894186135889357)
--(axis cs:89.171974522293,0.899026613433947)
--(axis cs:89.8089171974522,0.912835659823667)
--(axis cs:90.4458598726115,0.917216129309249)
--(axis cs:91.0828025477707,0.930380267695474)
--(axis cs:91.7197452229299,0.936661531495382)
--(axis cs:92.3566878980892,0.938234278462705)
--(axis cs:92.9936305732484,0.950964309294277)
--(axis cs:93.6305732484076,0.950663142872303)
--(axis cs:94.2675159235669,0.963707624958852)
--(axis cs:94.9044585987261,0.966015451608168)
--(axis cs:95.5414012738853,0.972878442643336)
--(axis cs:96.1783439490446,0.979976596737723)
--(axis cs:96.8152866242038,0.987063934681982)
--(axis cs:97.4522292993631,0.997927231816602)
--(axis cs:98.0891719745223,0.999000782885928)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1.00045234211407)
--(axis cs:97.4522292993631,1.0004321431834)
--(axis cs:96.8152866242038,0.994186065318018)
--(axis cs:96.1783439490446,0.986898403262277)
--(axis cs:95.5414012738853,0.981574682356664)
--(axis cs:94.9044585987261,0.974609548391832)
--(axis cs:94.2675159235669,0.972151750041148)
--(axis cs:93.6305732484076,0.959180607127697)
--(axis cs:92.9936305732484,0.960129440705723)
--(axis cs:92.3566878980892,0.947703221537295)
--(axis cs:91.7197452229299,0.946775968504618)
--(axis cs:91.0828025477707,0.941572857304526)
--(axis cs:90.4458598726115,0.928877620690751)
--(axis cs:89.8089171974522,0.925054965176333)
--(axis cs:89.171974522293,0.912301511566053)
--(axis cs:88.5350318471338,0.907532614110643)
--(axis cs:87.8980891719745,0.895324524467038)
--(axis cs:87.2611464968153,0.88452175310575)
--(axis cs:86.6242038216561,0.872920731681123)
--(axis cs:85.9872611464968,0.866987239386352)
--(axis cs:85.3503184713376,0.858755077844634)
--(axis cs:84.7133757961783,0.84883108954338)
--(axis cs:84.0764331210191,0.839967776908432)
--(axis cs:83.4394904458599,0.831799380247574)
--(axis cs:82.8025477707006,0.822888029721978)
--(axis cs:82.1656050955414,0.817696429880068)
--(axis cs:81.5286624203822,0.803665263212592)
--(axis cs:80.8917197452229,0.791877457015343)
--(axis cs:80.2547770700637,0.777295969963101)
--(axis cs:79.6178343949044,0.76342722885848)
--(axis cs:78.9808917197452,0.755303141942538)
--(axis cs:78.343949044586,0.745276012035012)
--(axis cs:77.7070063694268,0.737343247978077)
--(axis cs:77.0700636942675,0.72555698357171)
--(axis cs:76.4331210191083,0.710584593581107)
--(axis cs:75.796178343949,0.703166838479927)
--(axis cs:75.1592356687898,0.691342148497739)
--(axis cs:74.5222929936306,0.67640239069816)
--(axis cs:73.8853503184713,0.669845415761216)
--(axis cs:73.2484076433121,0.657618837956058)
--(axis cs:72.6114649681529,0.652512610016493)
--(axis cs:71.9745222929936,0.634887406164144)
--(axis cs:71.3375796178344,0.621932823660696)
--(axis cs:70.7006369426752,0.612815600411817)
--(axis cs:70.0636942675159,0.588438027597696)
--(axis cs:69.4267515923567,0.580756876900615)
--(axis cs:68.7898089171974,0.563378361003558)
--(axis cs:68.1528662420382,0.555263275002402)
--(axis cs:67.515923566879,0.546736038497327)
--(axis cs:66.8789808917197,0.536025658613413)
--(axis cs:66.2420382165605,0.524783333146728)
--(axis cs:65.6050955414013,0.513287706343406)
--(axis cs:64.968152866242,0.498737794565484)
--(axis cs:64.3312101910828,0.490016680308454)
--(axis cs:63.6942675159236,0.489160687285353)
--(axis cs:63.0573248407643,0.471404364294823)
--(axis cs:62.4203821656051,0.459182168486635)
--(axis cs:61.7834394904459,0.447786664437204)
--(axis cs:61.1464968152866,0.448465079703092)
--(axis cs:60.5095541401274,0.433576047791149)
--(axis cs:59.8726114649682,0.420577503713834)
--(axis cs:59.2356687898089,0.404601301899342)
--(axis cs:58.5987261146497,0.395542222774271)
--(axis cs:57.9617834394904,0.384186619490236)
--(axis cs:57.3248407643312,0.382845292437468)
--(axis cs:56.687898089172,0.368825240498953)
--(axis cs:56.0509554140127,0.362986945291058)
--(axis cs:55.4140127388535,0.349267575233584)
--(axis cs:54.7770700636943,0.343370843788578)
--(axis cs:54.140127388535,0.339920200675931)
--(axis cs:53.5031847133758,0.328331880650183)
--(axis cs:52.8662420382166,0.320741921830357)
--(axis cs:52.2292993630573,0.311218257453353)
--(axis cs:51.5923566878981,0.307059437700474)
--(axis cs:50.9554140127388,0.298517234977836)
--(axis cs:50.3184713375796,0.290783514734509)
--(axis cs:49.6815286624204,0.284055461667169)
--(axis cs:49.0445859872611,0.268051400757809)
--(axis cs:48.4076433121019,0.26271881307243)
--(axis cs:47.7707006369427,0.257633698366005)
--(axis cs:47.1337579617834,0.24935315987641)
--(axis cs:46.4968152866242,0.24481650625774)
--(axis cs:45.859872611465,0.24419800653289)
--(axis cs:45.2229299363057,0.231909201537771)
--(axis cs:44.5859872611465,0.222702303931608)
--(axis cs:43.9490445859873,0.21789639201889)
--(axis cs:43.312101910828,0.211638374842596)
--(axis cs:42.6751592356688,0.204795213568406)
--(axis cs:42.0382165605096,0.1974853515625)
--(axis cs:41.4012738853503,0.189659680748593)
--(axis cs:40.7643312101911,0.184583559141052)
--(axis cs:40.1273885350318,0.180241163854905)
--(axis cs:39.4904458598726,0.173275762266433)
--(axis cs:38.8535031847134,0.163651165449723)
--(axis cs:38.2165605095541,0.159958112908975)
--(axis cs:37.5796178343949,0.154576996590918)
--(axis cs:36.9426751592357,0.150022923993966)
--(axis cs:36.3057324840764,0.150931980926009)
--(axis cs:35.6687898089172,0.147225967633858)
--(axis cs:35.031847133758,0.141247801388335)
--(axis cs:34.3949044585987,0.136502270470435)
--(axis cs:33.7579617834395,0.132576207040405)
--(axis cs:33.1210191082803,0.12772891998631)
--(axis cs:32.484076433121,0.122802911455489)
--(axis cs:31.8471337579618,0.121454543489128)
--(axis cs:31.2101910828025,0.116013953171724)
--(axis cs:30.5732484076433,0.113327967886162)
--(axis cs:29.9363057324841,0.108370666817426)
--(axis cs:29.2993630573248,0.105522054200207)
--(axis cs:28.6624203821656,0.104525071078455)
--(axis cs:28.0254777070064,0.101819054268074)
--(axis cs:27.3885350318471,0.100929928485192)
--(axis cs:26.7515923566879,0.0968417728793134)
--(axis cs:26.1146496815287,0.0937924144780521)
--(axis cs:25.4777070063694,0.0930371461429996)
--(axis cs:24.8407643312102,0.093180101148427)
--(axis cs:24.203821656051,0.0936928385916602)
--(axis cs:23.5668789808917,0.0926597960589167)
--(axis cs:22.9299363057325,0.093694603434418)
--(axis cs:22.2929936305732,0.0917033834328072)
--(axis cs:21.656050955414,0.0902137392510294)
--(axis cs:21.0191082802548,0.0886555567716846)
--(axis cs:20.3821656050955,0.0874943233170446)
--(axis cs:19.7452229299363,0.0860433212340138)
--(axis cs:19.1082802547771,0.0857098798095986)
--(axis cs:18.4713375796178,0.0847082921030286)
--(axis cs:17.8343949044586,0.0864459081991586)
--(axis cs:17.1974522292994,0.0845500335780336)
--(axis cs:16.5605095541401,0.0842862978236521)
--(axis cs:15.9235668789809,0.0831686799213503)
--(axis cs:15.2866242038217,0.0832306334811061)
--(axis cs:14.6496815286624,0.082542946211236)
--(axis cs:14.0127388535032,0.0829068050445588)
--(axis cs:13.3757961783439,0.08149660812671)
--(axis cs:12.7388535031847,0.0811837434511746)
--(axis cs:12.1019108280255,0.0814999371133761)
--(axis cs:11.4649681528662,0.0815738854638513)
--(axis cs:10.828025477707,0.0809245740737912)
--(axis cs:10.1910828025478,0.0815745841158457)
--(axis cs:9.55414012738853,0.0808582297513999)
--(axis cs:8.9171974522293,0.0809247783773598)
--(axis cs:8.28025477707006,0.0808452220484008)
--(axis cs:7.64331210191083,0.0809352078190207)
--(axis cs:7.00636942675159,0.0805170110339466)
--(axis cs:6.36942675159236,0.0806292018232566)
--(axis cs:5.73248407643312,0.0805170110339466)
--(axis cs:5.09554140127389,0.08)
--(axis cs:4.45859872611465,0.0804683683438268)
--(axis cs:3.82165605095541,0.0804683683438268)
--(axis cs:3.18471337579618,0.0802368812147328)
--(axis cs:2.54777070063694,0.0806300124294657)
--(axis cs:1.91082802547771,0.0802368812147328)
--(axis cs:1.27388535031847,0.0803902433438268)
--(axis cs:0.636942675159236,0.0803121183438268)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_sfw_order_var_a.tex <==
\addplot [line width=0.5, opacity=0.7, color10, mark=triangle*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color10, thin}]
table {%
0 0.0800390625
0.636942675159236 0.08
1.27388535031847 0.0800390625
1.91082802547771 0.0800390625
2.54777070063694 0.0801171875
3.18471337579618 0.080234375
3.82165605095541 0.0801171875
4.45859872611465 0.0805078125
5.09554140127389 0.0812890625
5.73248407643312 0.081796875
6.36942675159236 0.08390625
7.00636942675159 0.0873828125
7.64331210191083 0.09125
8.28025477707006 0.0973046875
8.9171974522293 0.101484375
9.55414012738853 0.1116015625
10.1910828025478 0.1262109375
10.828025477707 0.136328125
11.4649681528662 0.1544140625
12.1019108280255 0.1704296875
12.7388535031847 0.1921484375
13.3757961783439 0.2051171875
14.0127388535032 0.222578125
14.6496815286624 0.2370703125
15.2866242038217 0.2469140625
15.9235668789809 0.2660546875
16.5605095541401 0.2782421875
17.1974522292994 0.3029296875
17.8343949044586 0.337109375
18.4713375796178 0.3601953125
19.1082802547771 0.3798828125
19.7452229299363 0.394921875
20.3821656050955 0.4217578125
21.0191082802548 0.4547265625
21.656050955414 0.4796875
22.2929936305732 0.504609375
22.9299363057325 0.522734375
23.5668789808917 0.5443359375
24.203821656051 0.5629296875
24.8407643312102 0.5874609375
25.4777070063694 0.6048828125
26.1146496815287 0.621171875
26.7515923566879 0.6255859375
27.3885350318471 0.644921875
28.0254777070064 0.6496875
28.6624203821656 0.6685546875
29.2993630573248 0.68
29.9363057324841 0.6951171875
30.5732484076433 0.7008203125
31.2101910828025 0.710390625
31.8471337579618 0.73171875
32.484076433121 0.7454296875
33.1210191082803 0.7548046875
33.7579617834395 0.7605078125
34.3949044585987 0.7631640625
35.031847133758 0.7760546875
35.6687898089172 0.776328125
36.3057324840764 0.7887890625
36.9426751592357 0.7993359375
37.5796178343949 0.809375
38.2165605095541 0.81734375
38.8535031847134 0.826640625
39.4904458598726 0.828984375
40.1273885350318 0.82890625
40.7643312101911 0.8366796875
41.4012738853503 0.841328125
42.0382165605096 0.8502734375
42.6751592356688 0.85546875
43.312101910828 0.8550390625
43.9490445859873 0.8566015625
44.5859872611465 0.858359375
45.2229299363057 0.861328125
45.859872611465 0.870703125
46.4968152866242 0.8695703125
47.1337579617834 0.87640625
47.7707006369427 0.883515625
48.4076433121019 0.89078125
49.0445859872611 0.8902734375
49.6815286624204 0.89984375
50.3184713375796 0.90375
50.9554140127388 0.9055859375
51.5923566878981 0.9077734375
52.2292993630573 0.90671875
52.8662420382166 0.9133984375
53.5031847133758 0.9173828125
54.140127388535 0.92390625
54.7770700636943 0.9258984375
55.4140127388535 0.9340625
56.0509554140127 0.9387109375
56.687898089172 0.938984375
57.3248407643312 0.943984375
57.9617834394904 0.9461328125
58.5987261146497 0.950546875
59.2356687898089 0.955546875
59.8726114649682 0.9559375
60.5095541401274 0.960859375
61.1464968152866 0.9644140625
61.7834394904459 0.962734375
62.4203821656051 0.962265625
63.0573248407643 0.9675
63.6942675159236 0.970078125
64.3312101910828 0.9730078125
64.968152866242 0.9722265625
65.6050955414013 0.978125
66.2420382165605 0.9799609375
66.8789808917197 0.9841796875
67.515923566879 0.9855859375
68.1528662420382 0.9891015625
68.7898089171974 0.9890234375
69.4267515923567 0.9905078125
70.0636942675159 0.9939453125
70.7006369426752 0.994140625
71.3375796178344 0.993125
71.9745222929936 0.9930859375
72.6114649681529 0.993828125
73.2484076433121 0.9940234375
73.8853503184713 0.9956640625
74.5222929936306 0.9969921875
75.1592356687898 0.997265625
75.796178343949 0.9980078125
76.4331210191083 0.9966015625
77.0700636942675 0.9989453125
77.7070063694268 0.99875
78.343949044586 0.9976953125
78.9808917197452 0.9991015625
79.6178343949044 0.9990625
80.2547770700637 0.999609375
80.8917197452229 0.9998828125
81.5286624203822 0.9997265625
82.1656050955414 0.999921875
82.8025477707006 1
83.4394904458599 0.9999609375
84.0764331210191 0.9998046875
84.7133757961783 0.9999609375
85.3503184713376 1
85.9872611464968 0.9999609375
86.6242038216561 1
87.2611464968153 0.9999609375
87.8980891719745 1
88.5350318471338 1
89.171974522293 1
89.8089171974522 1
90.4458598726115 1
91.0828025477707 1
91.7197452229299 1
92.3566878980892 1
92.9936305732484 1
93.6305732484076 1
94.2675159235669 1
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color10, fill opacity=0.25]
(axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.0796097566561732)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0795001585958936)
--(axis cs:3.18471337579618,0.0795588947591671)
--(axis cs:3.82165605095541,0.0792034522748438)
--(axis cs:4.45859872611465,0.0794404822918312)
--(axis cs:5.09554140127389,0.0797105748810358)
--(axis cs:5.73248407643312,0.0799451041680858)
--(axis cs:6.36942675159236,0.0811189808346655)
--(axis cs:7.00636942675159,0.0837759910798206)
--(axis cs:7.64331210191083,0.0868552653041885)
--(axis cs:8.28025477707006,0.0919681481495552)
--(axis cs:8.9171974522293,0.0956602009519761)
--(axis cs:9.55414012738853,0.104653316452231)
--(axis cs:10.1910828025478,0.118371694560281)
--(axis cs:10.828025477707,0.12788267651296)
--(axis cs:11.4649681528662,0.145462995156473)
--(axis cs:12.1019108280255,0.160668908367828)
--(axis cs:12.7388535031847,0.182012609326156)
--(axis cs:13.3757961783439,0.194847330057211)
--(axis cs:14.0127388535032,0.212163917513896)
--(axis cs:14.6496815286624,0.226851481528413)
--(axis cs:15.2866242038217,0.236326118180862)
--(axis cs:15.9235668789809,0.254969688159511)
--(axis cs:16.5605095541401,0.26673867477287)
--(axis cs:17.1974522292994,0.290871902349586)
--(axis cs:17.8343949044586,0.324579822189079)
--(axis cs:18.4713375796178,0.347235244761765)
--(axis cs:19.1082802547771,0.366681276450882)
--(axis cs:19.7452229299363,0.381288375215995)
--(axis cs:20.3821656050955,0.408009492153108)
--(axis cs:21.0191082802548,0.440990321584474)
--(axis cs:21.656050955414,0.465839990958282)
--(axis cs:22.2929936305732,0.49077123110511)
--(axis cs:22.9299363057325,0.509081663210349)
--(axis cs:23.5668789808917,0.53068097206588)
--(axis cs:24.203821656051,0.549540154438183)
--(axis cs:24.8407643312102,0.574152087671735)
--(axis cs:25.4777070063694,0.591874692765848)
--(axis cs:26.1146496815287,0.608316590172812)
--(axis cs:26.7515923566879,0.612693075894272)
--(axis cs:27.3885350318471,0.632271926941809)
--(axis cs:28.0254777070064,0.637233432283749)
--(axis cs:28.6624203821656,0.65636280847627)
--(axis cs:29.2993630573248,0.667951530294915)
--(axis cs:29.9363057324841,0.683122209258598)
--(axis cs:30.5732484076433,0.688906794075804)
--(axis cs:31.2101910828025,0.698674532873838)
--(axis cs:31.8471337579618,0.720147501672319)
--(axis cs:32.484076433121,0.733909606129202)
--(axis cs:33.1210191082803,0.743303947171945)
--(axis cs:33.7579617834395,0.749091209772619)
--(axis cs:34.3949044585987,0.751950876016272)
--(axis cs:35.031847133758,0.765146989552337)
--(axis cs:35.6687898089172,0.765146351111261)
--(axis cs:36.3057324840764,0.777671928068115)
--(axis cs:36.9426751592357,0.788341819981423)
--(axis cs:37.5796178343949,0.798390448819918)
--(axis cs:38.2165605095541,0.806337894416004)
--(axis cs:38.8535031847134,0.815998977911879)
--(axis cs:39.4904458598726,0.818632999637784)
--(axis cs:40.1273885350318,0.818631743280042)
--(axis cs:40.7643312101911,0.826966165298877)
--(axis cs:41.4012738853503,0.831786973186985)
--(axis cs:42.0382165605096,0.841310159325432)
--(axis cs:42.6751592356688,0.846732847125593)
--(axis cs:43.312101910828,0.846378253402161)
--(axis cs:43.9490445859873,0.847936814289725)
--(axis cs:44.5859872611465,0.849758761285901)
--(axis cs:45.2229299363057,0.852301621730815)
--(axis cs:45.859872611465,0.861854264970696)
--(axis cs:46.4968152866242,0.86060959489156)
--(axis cs:47.1337579617834,0.867646057071285)
--(axis cs:47.7707006369427,0.874938432865804)
--(axis cs:48.4076433121019,0.882311804458634)
--(axis cs:49.0445859872611,0.881640684033073)
--(axis cs:49.6815286624204,0.891802456763971)
--(axis cs:50.3184713375796,0.895712246926407)
--(axis cs:50.9554140127388,0.897123611733161)
--(axis cs:51.5923566878981,0.899263770761773)
--(axis cs:52.2292993630573,0.898523803428186)
--(axis cs:52.8662420382166,0.905321265286054)
--(axis cs:53.5031847133758,0.909460336365644)
--(axis cs:54.140127388535,0.916295912472544)
--(axis cs:54.7770700636943,0.918240658270521)
--(axis cs:55.4140127388535,0.926867617376621)
--(axis cs:56.0509554140127,0.931215273600584)
--(axis cs:56.687898089172,0.931734302718424)
--(axis cs:57.3248407643312,0.936851038806833)
--(axis cs:57.9617834394904,0.938805654479751)
--(axis cs:58.5987261146497,0.943532004891889)
--(axis cs:59.2356687898089,0.949044364643684)
--(axis cs:59.8726114649682,0.949484123881425)
--(axis cs:60.5095541401274,0.954263487778042)
--(axis cs:61.1464968152866,0.958107255178831)
--(axis cs:61.7834394904459,0.956323626167308)
--(axis cs:62.4203821656051,0.95594412691464)
--(axis cs:63.0573248407643,0.961120497554461)
--(axis cs:63.6942675159236,0.963761791335826)
--(axis cs:64.3312101910828,0.967009413475802)
--(axis cs:64.968152866242,0.96617326567839)
--(axis cs:65.6050955414013,0.972558941768349)
--(axis cs:66.2420382165605,0.974735059090125)
--(axis cs:66.8789808917197,0.979259587562576)
--(axis cs:67.515923566879,0.980916385041429)
--(axis cs:68.1528662420382,0.984967017408945)
--(axis cs:68.7898089171974,0.984888676170816)
--(axis cs:69.4267515923567,0.986631527436977)
--(axis cs:70.0636942675159,0.99071487441533)
--(axis cs:70.7006369426752,0.991014147154254)
--(axis cs:71.3375796178344,0.98983109145718)
--(axis cs:71.9745222929936,0.989899855573859)
--(axis cs:72.6114649681529,0.990822368184848)
--(axis cs:73.2484076433121,0.991026891033849)
--(axis cs:73.8853503184713,0.993051729291555)
--(axis cs:74.5222929936306,0.994743209700192)
--(axis cs:75.1592356687898,0.995083808106907)
--(axis cs:75.796178343949,0.996117534890052)
--(axis cs:76.4331210191083,0.994179920084647)
--(axis cs:77.0700636942675,0.997529139034255)
--(axis cs:77.7070063694268,0.997215599964603)
--(axis cs:78.343949044586,0.995642243707459)
--(axis cs:78.9808917197452,0.997794725829093)
--(axis cs:79.6178343949044,0.997728075493831)
--(axis cs:80.2547770700637,0.998739500891049)
--(axis cs:80.8917197452229,0.99940517584115)
--(axis cs:81.5286624203822,0.99899955205472)
--(axis cs:82.1656050955414,0.99953201368597)
--(axis cs:82.8025477707006,1)
--(axis cs:83.4394904458599,0.999684993785267)
--(axis cs:84.0764331210191,0.99918862534761)
--(axis cs:84.7133757961783,0.999684993785267)
--(axis cs:85.3503184713376,1)
--(axis cs:85.9872611464968,0.999684993785267)
--(axis cs:86.6242038216561,1)
--(axis cs:87.2611464968153,0.999684993785267)
--(axis cs:87.8980891719745,1)
--(axis cs:88.5350318471338,1)
--(axis cs:89.171974522293,1)
--(axis cs:89.8089171974522,1)
--(axis cs:90.4458598726115,1)
--(axis cs:91.0828025477707,1)
--(axis cs:91.7197452229299,1)
--(axis cs:92.3566878980892,1)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1)
--(axis cs:91.7197452229299,1)
--(axis cs:91.0828025477707,1)
--(axis cs:90.4458598726115,1)
--(axis cs:89.8089171974522,1)
--(axis cs:89.171974522293,1)
--(axis cs:88.5350318471338,1)
--(axis cs:87.8980891719745,1)
--(axis cs:87.2611464968153,1.00023688121473)
--(axis cs:86.6242038216561,1)
--(axis cs:85.9872611464968,1.00023688121473)
--(axis cs:85.3503184713376,1)
--(axis cs:84.7133757961783,1.00023688121473)
--(axis cs:84.0764331210191,1.00042074965239)
--(axis cs:83.4394904458599,1.00023688121473)
--(axis cs:82.8025477707006,1)
--(axis cs:82.1656050955414,1.00031173631403)
--(axis cs:81.5286624203822,1.00045357294528)
--(axis cs:80.8917197452229,1.00036044915885)
--(axis cs:80.2547770700637,1.00047924910895)
--(axis cs:79.6178343949044,1.00039692450617)
--(axis cs:78.9808917197452,1.00040839917091)
--(axis cs:78.343949044586,0.999748381292541)
--(axis cs:77.7070063694268,1.0002844000354)
--(axis cs:77.0700636942675,1.00036148596574)
--(axis cs:76.4331210191083,0.999023204915353)
--(axis cs:75.796178343949,0.999898090109949)
--(axis cs:75.1592356687898,0.999447441893093)
--(axis cs:74.5222929936306,0.999241165299808)
--(axis cs:73.8853503184713,0.998276395708445)
--(axis cs:73.2484076433121,0.997019983966151)
--(axis cs:72.6114649681529,0.996833881815151)
--(axis cs:71.9745222929936,0.996272019426141)
--(axis cs:71.3375796178344,0.99641890854282)
--(axis cs:70.7006369426752,0.997267102845746)
--(axis cs:70.0636942675159,0.99717575058467)
--(axis cs:69.4267515923567,0.994384097563023)
--(axis cs:68.7898089171974,0.993158198829184)
--(axis cs:68.1528662420382,0.993236107591055)
--(axis cs:67.515923566879,0.990255489958571)
--(axis cs:66.8789808917197,0.989099787437424)
--(axis cs:66.2420382165605,0.985186815909875)
--(axis cs:65.6050955414013,0.983691058231651)
--(axis cs:64.968152866242,0.978279859321609)
--(axis cs:64.3312101910828,0.979006211524198)
--(axis cs:63.6942675159236,0.976394458664175)
--(axis cs:63.0573248407643,0.973879502445539)
--(axis cs:62.4203821656051,0.96858712308536)
--(axis cs:61.7834394904459,0.969145123832692)
--(axis cs:61.1464968152866,0.970720869821169)
--(axis cs:60.5095541401274,0.967455262221957)
--(axis cs:59.8726114649682,0.962390876118575)
--(axis cs:59.2356687898089,0.962049385356316)
--(axis cs:58.5987261146497,0.957561745108111)
--(axis cs:57.9617834394904,0.953459970520249)
--(axis cs:57.3248407643312,0.951117711193167)
--(axis cs:56.687898089172,0.946234447281576)
--(axis cs:56.0509554140127,0.946206601399416)
--(axis cs:55.4140127388535,0.941257382623379)
--(axis cs:54.7770700636943,0.933556216729479)
--(axis cs:54.140127388535,0.931516587527456)
--(axis cs:53.5031847133758,0.925305288634356)
--(axis cs:52.8662420382166,0.921475609713946)
--(axis cs:52.2292993630573,0.914913696571814)
--(axis cs:51.5923566878981,0.916283104238227)
--(axis cs:50.9554140127388,0.914048263266839)
--(axis cs:50.3184713375796,0.911787753073593)
--(axis cs:49.6815286624204,0.907885043236029)
--(axis cs:49.0445859872611,0.898906190966926)
--(axis cs:48.4076433121019,0.899250695541366)
--(axis cs:47.7707006369427,0.892092817134197)
--(axis cs:47.1337579617834,0.885166442928715)
--(axis cs:46.4968152866242,0.87853103010844)
--(axis cs:45.859872611465,0.879551985029304)
--(axis cs:45.2229299363057,0.870354628269185)
--(axis cs:44.5859872611465,0.8669599887141)
--(axis cs:43.9490445859873,0.865266310710275)
--(axis cs:43.312101910828,0.863699871597838)
--(axis cs:42.6751592356688,0.864204652874407)
--(axis cs:42.0382165605096,0.859236715674568)
--(axis cs:41.4012738853503,0.850869276813015)
--(axis cs:40.7643312101911,0.846393209701123)
--(axis cs:40.1273885350318,0.839180756719958)
--(axis cs:39.4904458598726,0.839335750362216)
--(axis cs:38.8535031847134,0.837282272088121)
--(axis cs:38.2165605095541,0.828349605583996)
--(axis cs:37.5796178343949,0.820359551180082)
--(axis cs:36.9426751592357,0.810330055018577)
--(axis cs:36.3057324840764,0.799906196931885)
--(axis cs:35.6687898089172,0.787509898888739)
--(axis cs:35.031847133758,0.786962385447663)
--(axis cs:34.3949044585987,0.774377248983728)
--(axis cs:33.7579617834395,0.771924415227381)
--(axis cs:33.1210191082803,0.766305427828054)
--(axis cs:32.484076433121,0.756949768870798)
--(axis cs:31.8471337579618,0.743289998327681)
--(axis cs:31.2101910828025,0.722106717126162)
--(axis cs:30.5732484076433,0.712733830924196)
--(axis cs:29.9363057324841,0.707112165741402)
--(axis cs:29.2993630573248,0.692048469705085)
--(axis cs:28.6624203821656,0.68074656652373)
--(axis cs:28.0254777070064,0.662141567716251)
--(axis cs:27.3885350318471,0.657571823058191)
--(axis cs:26.7515923566879,0.638478799105728)
--(axis cs:26.1146496815287,0.634027159827188)
--(axis cs:25.4777070063694,0.617890932234151)
--(axis cs:24.8407643312102,0.600769787328264)
--(axis cs:24.203821656051,0.576319220561817)
--(axis cs:23.5668789808917,0.55799090293412)
--(axis cs:22.9299363057325,0.536387086789651)
--(axis cs:22.2929936305732,0.51844751889489)
--(axis cs:21.656050955414,0.493535009041718)
--(axis cs:21.0191082802548,0.468462803415526)
--(axis cs:20.3821656050955,0.435506132846892)
--(axis cs:19.7452229299363,0.408555374784005)
--(axis cs:19.1082802547771,0.393084348549118)
--(axis cs:18.4713375796178,0.373155380238235)
--(axis cs:17.8343949044586,0.349638927810921)
--(axis cs:17.1974522292994,0.314987472650414)
--(axis cs:16.5605095541401,0.28974570022713)
--(axis cs:15.9235668789809,0.277139686840489)
--(axis cs:15.2866242038217,0.257502006819138)
--(axis cs:14.6496815286624,0.247289143471587)
--(axis cs:14.0127388535032,0.232992332486104)
--(axis cs:13.3757961783439,0.215387044942789)
--(axis cs:12.7388535031847,0.202284265673844)
--(axis cs:12.1019108280255,0.180190466632172)
--(axis cs:11.4649681528662,0.163365129843527)
--(axis cs:10.828025477707,0.14477357348704)
--(axis cs:10.1910828025478,0.134050180439719)
--(axis cs:9.55414012738853,0.118549808547769)
--(axis cs:8.9171974522293,0.107308549048024)
--(axis cs:8.28025477707006,0.102641226850445)
--(axis cs:7.64331210191083,0.0956447346958115)
--(axis cs:7.00636942675159,0.0909896339201794)
--(axis cs:6.36942675159236,0.0866935191653345)
--(axis cs:5.73248407643312,0.0836486458319142)
--(axis cs:5.09554140127389,0.0828675501189642)
--(axis cs:4.45859872611465,0.0815751427081688)
--(axis cs:3.82165605095541,0.0810309227251562)
--(axis cs:3.18471337579618,0.0809098552408329)
--(axis cs:2.54777070063694,0.0807342164041065)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.0803902433438268)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_sfw_order_var_b.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.0800390625
0.636942675159236 0.08
1.27388535031847 0.080078125
1.91082802547771 0.0800390625
2.54777070063694 0.0799609375
3.18471337579618 0.080234375
3.82165605095541 0.0802734375
4.45859872611465 0.0805078125
5.09554140127389 0.0809765625
5.73248407643312 0.0825390625
6.36942675159236 0.08375
7.00636942675159 0.0871484375
7.64331210191083 0.0912109375
8.28025477707006 0.098046875
8.9171974522293 0.104453125
9.55414012738853 0.1112109375
10.1910828025478 0.126640625
10.828025477707 0.1417578125
11.4649681528662 0.1584765625
12.1019108280255 0.1668359375
12.7388535031847 0.1885546875
13.3757961783439 0.2091015625
14.0127388535032 0.219453125
14.6496815286624 0.2365234375
15.2866242038217 0.258359375
15.9235668789809 0.2702734375
16.5605095541401 0.2937109375
17.1974522292994 0.3139453125
17.8343949044586 0.3361328125
18.4713375796178 0.35453125
19.1082802547771 0.3823046875
19.7452229299363 0.3978515625
20.3821656050955 0.4262109375
21.0191082802548 0.45515625
21.656050955414 0.4782421875
22.2929936305732 0.5038671875
22.9299363057325 0.51828125
23.5668789808917 0.5405078125
24.203821656051 0.550703125
24.8407643312102 0.566328125
25.4777070063694 0.5890234375
26.1146496815287 0.61109375
26.7515923566879 0.62703125
27.3885350318471 0.63296875
28.0254777070064 0.650234375
28.6624203821656 0.6649609375
29.2993630573248 0.6782421875
29.9363057324841 0.6955078125
30.5732484076433 0.708515625
31.2101910828025 0.717421875
31.8471337579618 0.7241796875
32.484076433121 0.7416796875
33.1210191082803 0.7571484375
33.7579617834395 0.761484375
34.3949044585987 0.7780078125
35.031847133758 0.7852734375
35.6687898089172 0.7891015625
36.3057324840764 0.8025
36.9426751592357 0.81234375
37.5796178343949 0.8245703125
38.2165605095541 0.8232421875
38.8535031847134 0.828203125
39.4904458598726 0.838125
40.1273885350318 0.8419140625
40.7643312101911 0.8450390625
41.4012738853503 0.842578125
42.0382165605096 0.8481640625
42.6751592356688 0.8516015625
43.312101910828 0.8555078125
43.9490445859873 0.857109375
44.5859872611465 0.8616015625
45.2229299363057 0.863203125
45.859872611465 0.8712890625
46.4968152866242 0.880703125
47.1337579617834 0.89046875
47.7707006369427 0.88890625
48.4076433121019 0.8871484375
49.0445859872611 0.89125
49.6815286624204 0.902578125
50.3184713375796 0.902578125
50.9554140127388 0.9072265625
51.5923566878981 0.915703125
52.2292993630573 0.9085546875
52.8662420382166 0.9127734375
53.5031847133758 0.918671875
54.140127388535 0.9177734375
54.7770700636943 0.91953125
55.4140127388535 0.9237890625
56.0509554140127 0.922265625
56.687898089172 0.930546875
57.3248407643312 0.9349609375
57.9617834394904 0.9406640625
58.5987261146497 0.945546875
59.2356687898089 0.947890625
59.8726114649682 0.9508984375
60.5095541401274 0.9555078125
61.1464968152866 0.9595703125
61.7834394904459 0.9587109375
62.4203821656051 0.963203125
63.0573248407643 0.9654296875
63.6942675159236 0.9671875
64.3312101910828 0.9717578125
64.968152866242 0.973828125
65.6050955414013 0.976015625
66.2420382165605 0.9804296875
66.8789808917197 0.9808203125
67.515923566879 0.9802734375
68.1528662420382 0.9784765625
68.7898089171974 0.9824609375
69.4267515923567 0.983125
70.0636942675159 0.9808984375
70.7006369426752 0.9855078125
71.3375796178344 0.9868359375
71.9745222929936 0.9847265625
72.6114649681529 0.9862109375
73.2484076433121 0.984765625
73.8853503184713 0.9871875
74.5222929936306 0.985546875
75.1592356687898 0.9869140625
75.796178343949 0.989453125
76.4331210191083 0.9929296875
77.0700636942675 0.9964453125
77.7070063694268 0.99640625
78.343949044586 0.99953125
78.9808917197452 0.9997265625
79.6178343949044 0.9997265625
80.2547770700637 0.999609375
80.8917197452229 0.9996484375
81.5286624203822 0.999921875
82.1656050955414 0.9999609375
82.8025477707006 0.9996875
83.4394904458599 0.9992578125
84.0764331210191 0.9998046875
84.7133757961783 0.9996484375
85.3503184713376 0.999609375
85.9872611464968 0.9996875
86.6242038216561 0.9998046875
87.2611464968153 0.999921875
87.8980891719745 1
88.5350318471338 0.9999609375
89.171974522293 1
89.8089171974522 1
90.4458598726115 1
91.0828025477707 1
91.7197452229299 1
92.3566878980892 1
92.9936305732484 1
93.6305732484076 1
94.2675159235669 1
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color0, fill opacity=0.25]
(axis cs:0,0.0803150062147328)
--(axis cs:0,0.0797631187852672)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0796882636859699)
--(axis cs:1.91082802547771,0.0795611139660534)
--(axis cs:2.54777070063694,0.0794833008411496)
--(axis cs:3.18471337579618,0.079561768685842)
--(axis cs:3.82165605095541,0.0792806072965044)
--(axis cs:4.45859872611465,0.0793067373919504)
--(axis cs:5.09554140127389,0.079358267384819)
--(axis cs:5.73248407643312,0.0802560212883711)
--(axis cs:6.36942675159236,0.0810375657928992)
--(axis cs:7.00636942675159,0.0835403768777569)
--(axis cs:7.64331210191083,0.0867723931211778)
--(axis cs:8.28025477707006,0.0925925308322478)
--(axis cs:8.9171974522293,0.0983837134441934)
--(axis cs:9.55414012738853,0.104417409295805)
--(axis cs:10.1910828025478,0.118745421425495)
--(axis cs:10.828025477707,0.133197950073283)
--(axis cs:11.4649681528662,0.14953538915455)
--(axis cs:12.1019108280255,0.157519221281014)
--(axis cs:12.7388535031847,0.178606690977993)
--(axis cs:13.3757961783439,0.199308502587224)
--(axis cs:14.0127388535032,0.209479315603653)
--(axis cs:14.6496815286624,0.226295657062128)
--(axis cs:15.2866242038217,0.247876470086139)
--(axis cs:15.9235668789809,0.259514139104889)
--(axis cs:16.5605095541401,0.282232660108789)
--(axis cs:17.1974522292994,0.301906054053394)
--(axis cs:17.8343949044586,0.323777771090319)
--(axis cs:18.4713375796178,0.341581620673105)
--(axis cs:19.1082802547771,0.369167068961449)
--(axis cs:19.7452229299363,0.384762954984305)
--(axis cs:20.3821656050955,0.412687921284891)
--(axis cs:21.0191082802548,0.441139686165127)
--(axis cs:21.656050955414,0.4642879489006)
--(axis cs:22.2929936305732,0.490207683165357)
--(axis cs:22.9299363057325,0.504510842209166)
--(axis cs:23.5668789808917,0.526942548892765)
--(axis cs:24.203821656051,0.537226153393749)
--(axis cs:24.8407643312102,0.553270058777487)
--(axis cs:25.4777070063694,0.576084980553161)
--(axis cs:26.1146496815287,0.59845985597464)
--(axis cs:26.7515923566879,0.614697616956675)
--(axis cs:27.3885350318471,0.620507732618821)
--(axis cs:28.0254777070064,0.638085355128666)
--(axis cs:28.6624203821656,0.653013521198838)
--(axis cs:29.2993630573248,0.666564268673498)
--(axis cs:29.9363057324841,0.683781175088836)
--(axis cs:30.5732484076433,0.6970008028846)
--(axis cs:31.2101910828025,0.705679231207114)
--(axis cs:31.8471337579618,0.712517078089026)
--(axis cs:32.484076433121,0.730392407356705)
--(axis cs:33.1210191082803,0.745885196901088)
--(axis cs:33.7579617834395,0.750288284509808)
--(axis cs:34.3949044585987,0.767029157138934)
--(axis cs:35.031847133758,0.774317662656199)
--(axis cs:35.6687898089172,0.778295926293617)
--(axis cs:36.3057324840764,0.791991100154823)
--(axis cs:36.9426751592357,0.801889669533278)
--(axis cs:37.5796178343949,0.814510659579146)
--(axis cs:38.2165605095541,0.813215101387293)
--(axis cs:38.8535031847134,0.818123309846408)
--(axis cs:39.4904458598726,0.828247904866994)
--(axis cs:40.1273885350318,0.832270237407371)
--(axis cs:40.7643312101911,0.835642050517465)
--(axis cs:41.4012738853503,0.833122142246389)
--(axis cs:42.0382165605096,0.839091462140464)
--(axis cs:42.6751592356688,0.842628099184706)
--(axis cs:43.312101910828,0.846740707699165)
--(axis cs:43.9490445859873,0.848496693742331)
--(axis cs:44.5859872611465,0.852650162215528)
--(axis cs:45.2229299363057,0.854478231072182)
--(axis cs:45.859872611465,0.862615651103536)
--(axis cs:46.4968152866242,0.872255577136218)
--(axis cs:47.1337579617834,0.882304919670522)
--(axis cs:47.7707006369427,0.880494551371728)
--(axis cs:48.4076433121019,0.87838665427284)
--(axis cs:49.0445859872611,0.882417152115228)
--(axis cs:49.6815286624204,0.893992910288861)
--(axis cs:50.3184713375796,0.893839015926579)
--(axis cs:50.9554140127388,0.898488246339707)
--(axis cs:51.5923566878981,0.90731230260417)
--(axis cs:52.2292993630573,0.899798467326572)
--(axis cs:52.8662420382166,0.904313718240652)
--(axis cs:53.5031847133758,0.910306201348715)
--(axis cs:54.140127388535,0.909693959554197)
--(axis cs:54.7770700636943,0.911297700174117)
--(axis cs:55.4140127388535,0.915783622907191)
--(axis cs:56.0509554140127,0.914255040346211)
--(axis cs:56.687898089172,0.922799226994705)
--(axis cs:57.3248407643312,0.927479620600643)
--(axis cs:57.9617834394904,0.933267095097554)
--(axis cs:58.5987261146497,0.938289510028294)
--(axis cs:59.2356687898089,0.940570333898162)
--(axis cs:59.8726114649682,0.943609081589041)
--(axis cs:60.5095541401274,0.948321934343962)
--(axis cs:61.1464968152866,0.952368008890046)
--(axis cs:61.7834394904459,0.951677685069072)
--(axis cs:62.4203821656051,0.956166049403627)
--(axis cs:63.0573248407643,0.958580433328537)
--(axis cs:63.6942675159236,0.960448179463357)
--(axis cs:64.3312101910828,0.965651794946384)
--(axis cs:64.968152866242,0.967876474277693)
--(axis cs:65.6050955414013,0.970182835172814)
--(axis cs:66.2420382165605,0.975032895616421)
--(axis cs:66.8789808917197,0.975505990172639)
--(axis cs:67.515923566879,0.974899112632924)
--(axis cs:68.1528662420382,0.973153526991785)
--(axis cs:68.7898089171974,0.97743470813265)
--(axis cs:69.4267515923567,0.978254776972056)
--(axis cs:70.0636942675159,0.9762572445944)
--(axis cs:70.7006369426752,0.981457192846301)
--(axis cs:71.3375796178344,0.982945837983225)
--(axis cs:71.9745222929936,0.980656492244146)
--(axis cs:72.6114649681529,0.982408981238272)
--(axis cs:73.2484076433121,0.980716458707837)
--(axis cs:73.8853503184713,0.983462414856418)
--(axis cs:74.5222929936306,0.98202870778765)
--(axis cs:75.1592356687898,0.983721486225546)
--(axis cs:75.796178343949,0.986307308862325)
--(axis cs:76.4331210191083,0.989872343979018)
--(axis cs:77.0700636942675,0.994028967741778)
--(axis cs:77.7070063694268,0.993990059417176)
--(axis cs:78.343949044586,0.998583965498336)
--(axis cs:78.9808917197452,0.998997914180619)
--(axis cs:79.6178343949044,0.99899770970515)
--(axis cs:80.2547770700637,0.998742933714657)
--(axis cs:80.8917197452229,0.99882566186045)
--(axis cs:81.5286624203822,0.999531631656173)
--(axis cs:82.1656050955414,0.999684993785267)
--(axis cs:82.8025477707006,0.998912377545586)
--(axis cs:83.4394904458599,0.998076376183888)
--(axis cs:84.0764331210191,0.999190078326407)
--(axis cs:84.7133757961783,0.998827112005908)
--(axis cs:85.3503184713376,0.998744482930473)
--(axis cs:85.9872611464968,0.998911033012999)
--(axis cs:86.6242038216561,0.999190078326407)
--(axis cs:87.2611464968153,0.99953201368597)
--(axis cs:87.8980891719745,1)
--(axis cs:88.5350318471338,0.999684993785267)
--(axis cs:89.171974522293,1)
--(axis cs:89.8089171974522,1)
--(axis cs:90.4458598726115,1)
--(axis cs:91.0828025477707,1)
--(axis cs:91.7197452229299,1)
--(axis cs:92.3566878980892,1)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1)
--(axis cs:91.7197452229299,1)
--(axis cs:91.0828025477707,1)
--(axis cs:90.4458598726115,1)
--(axis cs:89.8089171974522,1)
--(axis cs:89.171974522293,1)
--(axis cs:88.5350318471338,1.00023688121473)
--(axis cs:87.8980891719745,1)
--(axis cs:87.2611464968153,1.00031173631403)
--(axis cs:86.6242038216561,1.00041929667359)
--(axis cs:85.9872611464968,1.000463966987)
--(axis cs:85.3503184713376,1.00047426706953)
--(axis cs:84.7133757961783,1.00046976299409)
--(axis cs:84.0764331210191,1.00041929667359)
--(axis cs:83.4394904458599,1.00043924881611)
--(axis cs:82.8025477707006,1.00046262245441)
--(axis cs:82.1656050955414,1.00023688121473)
--(axis cs:81.5286624203822,1.00031211834383)
--(axis cs:80.8917197452229,1.00047121313955)
--(axis cs:80.2547770700637,1.00047581628534)
--(axis cs:79.6178343949044,1.00045541529485)
--(axis cs:78.9808917197452,1.00045521081938)
--(axis cs:78.343949044586,1.00047853450166)
--(axis cs:77.7070063694268,0.998822440582824)
--(axis cs:77.0700636942675,0.998861657258222)
--(axis cs:76.4331210191083,0.995987031020982)
--(axis cs:75.796178343949,0.992598941137675)
--(axis cs:75.1592356687898,0.990106638774454)
--(axis cs:74.5222929936306,0.98906504221235)
--(axis cs:73.8853503184713,0.990912585143582)
--(axis cs:73.2484076433121,0.988814791292163)
--(axis cs:72.6114649681529,0.990012893761728)
--(axis cs:71.9745222929936,0.988796632755854)
--(axis cs:71.3375796178344,0.990726037016775)
--(axis cs:70.7006369426752,0.989558432153699)
--(axis cs:70.0636942675159,0.9855396304056)
--(axis cs:69.4267515923567,0.987995223027944)
--(axis cs:68.7898089171974,0.98748716686735)
--(axis cs:68.1528662420382,0.983799598008215)
--(axis cs:67.515923566879,0.985647762367076)
--(axis cs:66.8789808917197,0.986134634827361)
--(axis cs:66.2420382165605,0.985826479383579)
--(axis cs:65.6050955414013,0.981848414827186)
--(axis cs:64.968152866242,0.979779775722308)
--(axis cs:64.3312101910828,0.977863830053616)
--(axis cs:63.6942675159236,0.973926820536643)
--(axis cs:63.0573248407643,0.972278941671463)
--(axis cs:62.4203821656051,0.970240200596373)
--(axis cs:61.7834394904459,0.965744189930928)
--(axis cs:61.1464968152866,0.966772616109954)
--(axis cs:60.5095541401274,0.962693690656038)
--(axis cs:59.8726114649682,0.958187793410959)
--(axis cs:59.2356687898089,0.955210916101838)
--(axis cs:58.5987261146497,0.952804239971706)
--(axis cs:57.9617834394904,0.948061029902446)
--(axis cs:57.3248407643312,0.942442254399357)
--(axis cs:56.687898089172,0.938294523005295)
--(axis cs:56.0509554140127,0.930276209653789)
--(axis cs:55.4140127388535,0.931794502092809)
--(axis cs:54.7770700636943,0.927764799825883)
--(axis cs:54.140127388535,0.925852915445803)
--(axis cs:53.5031847133758,0.927037548651285)
--(axis cs:52.8662420382166,0.921233156759347)
--(axis cs:52.2292993630573,0.917310907673428)
--(axis cs:51.5923566878981,0.92409394739583)
--(axis cs:50.9554140127388,0.915964878660293)
--(axis cs:50.3184713375796,0.911317234073421)
--(axis cs:49.6815286624204,0.911163339711139)
--(axis cs:49.0445859872611,0.900082847884772)
--(axis cs:48.4076433121019,0.89591022072716)
--(axis cs:47.7707006369427,0.897317948628272)
--(axis cs:47.1337579617834,0.898632580329478)
--(axis cs:46.4968152866242,0.889150672863782)
--(axis cs:45.859872611465,0.879962473896464)
--(axis cs:45.2229299363057,0.871928018927817)
--(axis cs:44.5859872611465,0.870552962784472)
--(axis cs:43.9490445859873,0.865722056257669)
--(axis cs:43.312101910828,0.864274917300835)
--(axis cs:42.6751592356688,0.860575025815294)
--(axis cs:42.0382165605096,0.857236662859536)
--(axis cs:41.4012738853503,0.85203410775361)
--(axis cs:40.7643312101911,0.854436074482535)
--(axis cs:40.1273885350318,0.851557887592629)
--(axis cs:39.4904458598726,0.848002095133006)
--(axis cs:38.8535031847134,0.838282940153592)
--(axis cs:38.2165605095541,0.833269273612707)
--(axis cs:37.5796178343949,0.834629965420854)
--(axis cs:36.9426751592357,0.822797830466722)
--(axis cs:36.3057324840764,0.813008899845177)
--(axis cs:35.6687898089172,0.799907198706383)
--(axis cs:35.031847133758,0.796229212343801)
--(axis cs:34.3949044585987,0.788986467861066)
--(axis cs:33.7579617834395,0.772680465490192)
--(axis cs:33.1210191082803,0.768411678098912)
--(axis cs:32.484076433121,0.752966967643295)
--(axis cs:31.8471337579618,0.735842296910974)
--(axis cs:31.2101910828025,0.729164518792886)
--(axis cs:30.5732484076433,0.7200304471154)
--(axis cs:29.9363057324841,0.707234449911164)
--(axis cs:29.2993630573248,0.689920106326502)
--(axis cs:28.6624203821656,0.676908353801162)
--(axis cs:28.0254777070064,0.662383394871334)
--(axis cs:27.3885350318471,0.645429767381179)
--(axis cs:26.7515923566879,0.639364883043325)
--(axis cs:26.1146496815287,0.62372764402536)
--(axis cs:25.4777070063694,0.601961894446839)
--(axis cs:24.8407643312102,0.579386191222513)
--(axis cs:24.203821656051,0.564180096606251)
--(axis cs:23.5668789808917,0.554073076107235)
--(axis cs:22.9299363057325,0.532051657790834)
--(axis cs:22.2929936305732,0.517526691834643)
--(axis cs:21.656050955414,0.4921964260994)
--(axis cs:21.0191082802548,0.469172813834873)
--(axis cs:20.3821656050955,0.439733953715109)
--(axis cs:19.7452229299363,0.410940170015695)
--(axis cs:19.1082802547771,0.395442306038551)
--(axis cs:18.4713375796178,0.367480879326895)
--(axis cs:17.8343949044586,0.348487853909681)
--(axis cs:17.1974522292994,0.325984570946606)
--(axis cs:16.5605095541401,0.305189214891211)
--(axis cs:15.9235668789809,0.281032735895111)
--(axis cs:15.2866242038217,0.268842279913861)
--(axis cs:14.6496815286624,0.246751217937872)
--(axis cs:14.0127388535032,0.229426934396347)
--(axis cs:13.3757961783439,0.218894622412776)
--(axis cs:12.7388535031847,0.198502684022007)
--(axis cs:12.1019108280255,0.176152653718986)
--(axis cs:11.4649681528662,0.16741773584545)
--(axis cs:10.828025477707,0.150317674926717)
--(axis cs:10.1910828025478,0.134535828574505)
--(axis cs:9.55414012738853,0.118004465704195)
--(axis cs:8.9171974522293,0.110522536555807)
--(axis cs:8.28025477707006,0.103501219167752)
--(axis cs:7.64331210191083,0.0956494818788222)
--(axis cs:7.00636942675159,0.0907564981222431)
--(axis cs:6.36942675159236,0.0864624342071008)
--(axis cs:5.73248407643312,0.0848221037116289)
--(axis cs:5.09554140127389,0.082594857615181)
--(axis cs:4.45859872611465,0.0817088876080496)
--(axis cs:3.82165605095541,0.0812662677034956)
--(axis cs:3.18471337579618,0.080906981314158)
--(axis cs:2.54777070063694,0.0804385741588504)
--(axis cs:1.91082802547771,0.0805170110339466)
--(axis cs:1.27388535031847,0.0804679863140301)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0803150062147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_sfw_order_var_c.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.08
0.636942675159236 0.08
1.27388535031847 0.0799609375
1.91082802547771 0.08
2.54777070063694 0.0799609375
3.18471337579618 0.0804296875
3.82165605095541 0.08046875
4.45859872611465 0.08046875
5.09554140127389 0.0814453125
5.73248407643312 0.0828515625
6.36942675159236 0.0833984375
7.00636942675159 0.0859375
7.64331210191083 0.0898046875
8.28025477707006 0.096484375
8.9171974522293 0.1074609375
9.55414012738853 0.118359375
10.1910828025478 0.129375
10.828025477707 0.1430078125
11.4649681528662 0.16171875
12.1019108280255 0.18296875
12.7388535031847 0.198984375
13.3757961783439 0.217734375
14.0127388535032 0.2308203125
14.6496815286624 0.24546875
15.2866242038217 0.2624609375
15.9235668789809 0.2835546875
16.5605095541401 0.2955859375
17.1974522292994 0.30921875
17.8343949044586 0.332734375
18.4713375796178 0.3530859375
19.1082802547771 0.370234375
19.7452229299363 0.3903515625
20.3821656050955 0.4110546875
21.0191082802548 0.4383984375
21.656050955414 0.46578125
22.2929936305732 0.4708203125
22.9299363057325 0.4982421875
23.5668789808917 0.5135546875
24.203821656051 0.5355078125
24.8407643312102 0.546953125
25.4777070063694 0.5540234375
26.1146496815287 0.5684765625
26.7515923566879 0.5794140625
27.3885350318471 0.59171875
28.0254777070064 0.6025390625
28.6624203821656 0.6171875
29.2993630573248 0.625078125
29.9363057324841 0.635859375
30.5732484076433 0.642421875
31.2101910828025 0.6652734375
31.8471337579618 0.6716015625
32.484076433121 0.6771484375
33.1210191082803 0.6846484375
33.7579617834395 0.697578125
34.3949044585987 0.7102734375
35.031847133758 0.71234375
35.6687898089172 0.725234375
36.3057324840764 0.739921875
36.9426751592357 0.7434765625
37.5796178343949 0.7584375
38.2165605095541 0.77046875
38.8535031847134 0.7728125
39.4904458598726 0.780234375
40.1273885350318 0.7862890625
40.7643312101911 0.79484375
41.4012738853503 0.7983984375
42.0382165605096 0.8009765625
42.6751592356688 0.803046875
43.312101910828 0.82421875
43.9490445859873 0.8218359375
44.5859872611465 0.8254296875
45.2229299363057 0.8249609375
45.859872611465 0.8253125
46.4968152866242 0.826875
47.1337579617834 0.843515625
47.7707006369427 0.8503125
48.4076433121019 0.853046875
49.0445859872611 0.86046875
49.6815286624204 0.8665234375
50.3184713375796 0.8725
50.9554140127388 0.8775
51.5923566878981 0.8832421875
52.2292993630573 0.881328125
52.8662420382166 0.886640625
53.5031847133758 0.883359375
54.140127388535 0.88140625
54.7770700636943 0.8888671875
55.4140127388535 0.8841796875
56.0509554140127 0.893046875
56.687898089172 0.889921875
57.3248407643312 0.888359375
57.9617834394904 0.892265625
58.5987261146497 0.9006640625
59.2356687898089 0.9010546875
59.8726114649682 0.9091015625
60.5095541401274 0.9185546875
61.1464968152866 0.918984375
61.7834394904459 0.924140625
62.4203821656051 0.922734375
63.0573248407643 0.923828125
63.6942675159236 0.9266796875
64.3312101910828 0.93359375
64.968152866242 0.9336328125
65.6050955414013 0.938984375
66.2420382165605 0.94109375
66.8789808917197 0.9464453125
67.515923566879 0.9475390625
68.1528662420382 0.94453125
68.7898089171974 0.9534375
69.4267515923567 0.958984375
70.0636942675159 0.962734375
70.7006369426752 0.972421875
71.3375796178344 0.9779296875
71.9745222929936 0.9807421875
72.6114649681529 0.98203125
73.2484076433121 0.98015625
73.8853503184713 0.9826953125
74.5222929936306 0.9863671875
75.1592356687898 0.9862109375
75.796178343949 0.982890625
76.4331210191083 0.97734375
77.0700636942675 0.9821875
77.7070063694268 0.98046875
78.343949044586 0.9759765625
78.9808917197452 0.97484375
79.6178343949044 0.9764453125
80.2547770700637 0.9805078125
80.8917197452229 0.9780859375
81.5286624203822 0.97984375
82.1656050955414 0.9778515625
82.8025477707006 0.98265625
83.4394904458599 0.9856640625
84.0764331210191 0.982890625
84.7133757961783 0.9794921875
85.3503184713376 0.9791796875
85.9872611464968 0.9825
86.6242038216561 0.985234375
87.2611464968153 0.9934765625
87.8980891719745 0.9877734375
88.5350318471338 0.9898046875
89.171974522293 0.9910546875
89.8089171974522 0.9932421875
90.4458598726115 0.9925
91.0828025477707 0.99515625
91.7197452229299 0.996953125
92.3566878980892 0.9998046875
92.9936305732484 0.99984375
93.6305732484076 0.999921875
94.2675159235669 1
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color1, fill opacity=0.25]
(axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0796849937852672)
--(axis cs:1.91082802547771,0.0796097566561732)
--(axis cs:2.54777070063694,0.0796849937852672)
--(axis cs:3.18471337579618,0.0795156261737538)
--(axis cs:3.82165605095541,0.0795145692262762)
--(axis cs:4.45859872611465,0.0795150378425476)
--(axis cs:5.09554140127389,0.0797321914601642)
--(axis cs:5.73248407643312,0.0805299468954206)
--(axis cs:6.36942675159236,0.0807875307204789)
--(axis cs:7.00636942675159,0.0826053605628276)
--(axis cs:7.64331210191083,0.0856024003704458)
--(axis cs:8.28025477707006,0.0911277828045435)
--(axis cs:8.9171974522293,0.100899536133948)
--(axis cs:9.55414012738853,0.110851306486972)
--(axis cs:10.1910828025478,0.121114113130358)
--(axis cs:10.828025477707,0.134177183320741)
--(axis cs:11.4649681528662,0.152259301023139)
--(axis cs:12.1019108280255,0.173219969972495)
--(axis cs:12.7388535031847,0.189093033320884)
--(axis cs:13.3757961783439,0.207523355707614)
--(axis cs:14.0127388535032,0.220395757959584)
--(axis cs:14.6496815286624,0.234779042209876)
--(axis cs:15.2866242038217,0.251465315617172)
--(axis cs:15.9235668789809,0.272597797415108)
--(axis cs:16.5605095541401,0.284114334825024)
--(axis cs:17.1974522292994,0.297738817516286)
--(axis cs:17.8343949044586,0.320932845976857)
--(axis cs:18.4713375796178,0.340876520008623)
--(axis cs:19.1082802547771,0.357867935367142)
--(axis cs:19.7452229299363,0.377381461110493)
--(axis cs:20.3821656050955,0.397882927448236)
--(axis cs:21.0191082802548,0.424931680680764)
--(axis cs:21.656050955414,0.45249814887886)
--(axis cs:22.2929936305732,0.457503314164854)
--(axis cs:22.9299363057325,0.484762501732997)
--(axis cs:23.5668789808917,0.500208694959128)
--(axis cs:24.203821656051,0.522598953427661)
--(axis cs:24.8407643312102,0.534230540298321)
--(axis cs:25.4777070063694,0.541360261951704)
--(axis cs:26.1146496815287,0.555911126939996)
--(axis cs:26.7515923566879,0.566771190083931)
--(axis cs:27.3885350318471,0.579085693418352)
--(axis cs:28.0254777070064,0.590034408243727)
--(axis cs:28.6624203821656,0.60489800801091)
--(axis cs:29.2993630573248,0.612799077180476)
--(axis cs:29.9363057324841,0.623294312999315)
--(axis cs:30.5732484076433,0.629795708795155)
--(axis cs:31.2101910828025,0.652942190829015)
--(axis cs:31.8471337579618,0.659620207419779)
--(axis cs:32.484076433121,0.665165813917196)
--(axis cs:33.1210191082803,0.672603672484493)
--(axis cs:33.7579617834395,0.685733014127059)
--(axis cs:34.3949044585987,0.698431126010053)
--(axis cs:35.031847133758,0.700733907039006)
--(axis cs:35.6687898089172,0.713752300986018)
--(axis cs:36.3057324840764,0.728661896045122)
--(axis cs:36.9426751592357,0.732337668222945)
--(axis cs:37.5796178343949,0.747386542636175)
--(axis cs:38.2165605095541,0.759151258526589)
--(axis cs:38.8535031847134,0.76139719603891)
--(axis cs:39.4904458598726,0.769000510024399)
--(axis cs:40.1273885350318,0.775235887233254)
--(axis cs:40.7643312101911,0.783783047967672)
--(axis cs:41.4012738853503,0.787487625256519)
--(axis cs:42.0382165605096,0.79002247433401)
--(axis cs:42.6751592356688,0.79218876358907)
--(axis cs:43.312101910828,0.813806417095156)
--(axis cs:43.9490445859873,0.811700815021463)
--(axis cs:44.5859872611465,0.815241656510319)
--(axis cs:45.2229299363057,0.814811534255052)
--(axis cs:45.859872611465,0.815596653970439)
--(axis cs:46.4968152866242,0.817332302152003)
--(axis cs:47.1337579617834,0.834335418066558)
--(axis cs:47.7707006369427,0.841186701091048)
--(axis cs:48.4076433121019,0.843952366365701)
--(axis cs:49.0445859872611,0.85163431646193)
--(axis cs:49.6815286624204,0.857760871985948)
--(axis cs:50.3184713375796,0.864340624534814)
--(axis cs:50.9554140127388,0.869493378518449)
--(axis cs:51.5923566878981,0.875273015276557)
--(axis cs:52.2292993630573,0.873313690690402)
--(axis cs:52.8662420382166,0.878392699733712)
--(axis cs:53.5031847133758,0.874760875280523)
--(axis cs:54.140127388535,0.873237328765959)
--(axis cs:54.7770700636943,0.880572215598455)
--(axis cs:55.4140127388535,0.875743427720974)
--(axis cs:56.0509554140127,0.88479600541045)
--(axis cs:56.687898089172,0.881433940727771)
--(axis cs:57.3248407643312,0.880105814892742)
--(axis cs:57.9617834394904,0.883884860158194)
--(axis cs:58.5987261146497,0.892270621078039)
--(axis cs:59.2356687898089,0.89286049557211)
--(axis cs:59.8726114649682,0.900929513484554)
--(axis cs:60.5095541401274,0.910583047455916)
--(axis cs:61.1464968152866,0.911154385116896)
--(axis cs:61.7834394904459,0.916259324701819)
--(axis cs:62.4203821656051,0.914964717077767)
--(axis cs:63.0573248407643,0.916305304912101)
--(axis cs:63.6942675159236,0.919237772240613)
--(axis cs:64.3312101910828,0.926448746135278)
--(axis cs:64.968152866242,0.926399500107173)
--(axis cs:65.6050955414013,0.932040194145543)
--(axis cs:66.2420382165605,0.934184527178249)
--(axis cs:66.8789808917197,0.93959969252611)
--(axis cs:67.515923566879,0.940918067325212)
--(axis cs:68.1528662420382,0.938078058607983)
--(axis cs:68.7898089171974,0.94697630094714)
--(axis cs:69.4267515923567,0.95283084456974)
--(axis cs:70.0636942675159,0.956726704692167)
--(axis cs:70.7006369426752,0.966636386054086)
--(axis cs:71.3375796178344,0.972454769343287)
--(axis cs:71.9745222929936,0.975949516747123)
--(axis cs:72.6114649681529,0.977311152315908)
--(axis cs:73.2484076433121,0.975613134726003)
--(axis cs:73.8853503184713,0.978416212607895)
--(axis cs:74.5222929936306,0.982068700225907)
--(axis cs:75.1592356687898,0.981882981093623)
--(axis cs:75.796178343949,0.978600552481528)
--(axis cs:76.4331210191083,0.972969032024209)
--(axis cs:77.0700636942675,0.977835594916688)
--(axis cs:77.7070063694268,0.976027000635093)
--(axis cs:78.343949044586,0.971674887130783)
--(axis cs:78.9808917197452,0.970572021547165)
--(axis cs:79.6178343949044,0.972088154662714)
--(axis cs:80.2547770700637,0.97614009987264)
--(axis cs:80.8917197452229,0.973900741214456)
--(axis cs:81.5286624203822,0.975733187422818)
--(axis cs:82.1656050955414,0.974068977938259)
--(axis cs:82.8025477707006,0.978709016266828)
--(axis cs:83.4394904458599,0.981530310378858)
--(axis cs:84.0764331210191,0.978818413531254)
--(axis cs:84.7133757961783,0.975407389433166)
--(axis cs:85.3503184713376,0.975030392062006)
--(axis cs:85.9872611464968,0.978573090824444)
--(axis cs:86.6242038216561,0.98138147546789)
--(axis cs:87.2611464968153,0.990315742741513)
--(axis cs:87.8980891719745,0.984502704763643)
--(axis cs:88.5350318471338,0.986619821814251)
--(axis cs:89.171974522293,0.987893867741513)
--(axis cs:89.8089171974522,0.990235910188161)
--(axis cs:90.4458598726115,0.989474231760776)
--(axis cs:91.0828025477707,0.992471868594514)
--(axis cs:91.7197452229299,0.994707163939042)
--(axis cs:92.3566878980892,0.999190078326407)
--(axis cs:92.9936305732484,0.999293484977071)
--(axis cs:93.6305732484076,0.99953201368597)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1.00031173631403)
--(axis cs:92.9936305732484,1.00039401502293)
--(axis cs:92.3566878980892,1.00041929667359)
--(axis cs:91.7197452229299,0.999199086060958)
--(axis cs:91.0828025477707,0.997840631405486)
--(axis cs:90.4458598726115,0.995525768239225)
--(axis cs:89.8089171974522,0.996248464811839)
--(axis cs:89.171974522293,0.994215507258487)
--(axis cs:88.5350318471338,0.992989553185749)
--(axis cs:87.8980891719745,0.991044170236357)
--(axis cs:87.2611464968153,0.996637382258487)
--(axis cs:86.6242038216561,0.98908727453211)
--(axis cs:85.9872611464968,0.986426909175556)
--(axis cs:85.3503184713376,0.983328982937994)
--(axis cs:84.7133757961783,0.983576985566834)
--(axis cs:84.0764331210191,0.986962836468746)
--(axis cs:83.4394904458599,0.989797814621142)
--(axis cs:82.8025477707006,0.986603483733172)
--(axis cs:82.1656050955414,0.981634147061741)
--(axis cs:81.5286624203822,0.983954312577182)
--(axis cs:80.8917197452229,0.982271133785544)
--(axis cs:80.2547770700637,0.98487552512736)
--(axis cs:79.6178343949044,0.980802470337286)
--(axis cs:78.9808917197452,0.979115478452835)
--(axis cs:78.343949044586,0.980278237869217)
--(axis cs:77.7070063694268,0.984910499364907)
--(axis cs:77.0700636942675,0.986539405083312)
--(axis cs:76.4331210191083,0.981718467975791)
--(axis cs:75.796178343949,0.987180697518472)
--(axis cs:75.1592356687898,0.990538893906377)
--(axis cs:74.5222929936306,0.990665674774093)
--(axis cs:73.8853503184713,0.986974412392105)
--(axis cs:73.2484076433121,0.984699365273997)
--(axis cs:72.6114649681529,0.986751347684092)
--(axis cs:71.9745222929936,0.985534858252877)
--(axis cs:71.3375796178344,0.983404605656713)
--(axis cs:70.7006369426752,0.978207363945914)
--(axis cs:70.0636942675159,0.968742045307833)
--(axis cs:69.4267515923567,0.96513790543026)
--(axis cs:68.7898089171974,0.95989869905286)
--(axis cs:68.1528662420382,0.950984441392017)
--(axis cs:67.515923566879,0.954160057674788)
--(axis cs:66.8789808917197,0.95329093247389)
--(axis cs:66.2420382165605,0.948002972821751)
--(axis cs:65.6050955414013,0.945928555854457)
--(axis cs:64.968152866242,0.940866124892827)
--(axis cs:64.3312101910828,0.940738753864722)
--(axis cs:63.6942675159236,0.934121602759386)
--(axis cs:63.0573248407643,0.931350945087899)
--(axis cs:62.4203821656051,0.930504032922233)
--(axis cs:61.7834394904459,0.932021925298181)
--(axis cs:61.1464968152866,0.926814364883104)
--(axis cs:60.5095541401274,0.926526327544084)
--(axis cs:59.8726114649682,0.917273611515446)
--(axis cs:59.2356687898089,0.909248879427889)
--(axis cs:58.5987261146497,0.909057503921961)
--(axis cs:57.9617834394904,0.900646389841806)
--(axis cs:57.3248407643312,0.896612935107258)
--(axis cs:56.687898089172,0.898409809272229)
--(axis cs:56.0509554140127,0.90129774458955)
--(axis cs:55.4140127388535,0.892615947279026)
--(axis cs:54.7770700636943,0.897162159401545)
--(axis cs:54.140127388535,0.889575171234041)
--(axis cs:53.5031847133758,0.891957874719477)
--(axis cs:52.8662420382166,0.894888550266288)
--(axis cs:52.2292993630573,0.889342559309598)
--(axis cs:51.5923566878981,0.891211359723443)
--(axis cs:50.9554140127388,0.885506621481551)
--(axis cs:50.3184713375796,0.880659375465186)
--(axis cs:49.6815286624204,0.875286003014052)
--(axis cs:49.0445859872611,0.86930318353807)
--(axis cs:48.4076433121019,0.862141383634299)
--(axis cs:47.7707006369427,0.859438298908952)
--(axis cs:47.1337579617834,0.852695831933442)
--(axis cs:46.4968152866242,0.836417697847997)
--(axis cs:45.859872611465,0.835028346029561)
--(axis cs:45.2229299363057,0.835110340744948)
--(axis cs:44.5859872611465,0.835617718489681)
--(axis cs:43.9490445859873,0.831971059978537)
--(axis cs:43.312101910828,0.834631082904844)
--(axis cs:42.6751592356688,0.81390498641093)
--(axis cs:42.0382165605096,0.811930650665991)
--(axis cs:41.4012738853503,0.809309249743481)
--(axis cs:40.7643312101911,0.805904452032328)
--(axis cs:40.1273885350318,0.797342237766746)
--(axis cs:39.4904458598726,0.791468239975601)
--(axis cs:38.8535031847134,0.78422780396109)
--(axis cs:38.2165605095541,0.781786241473411)
--(axis cs:37.5796178343949,0.769488457363825)
--(axis cs:36.9426751592357,0.754615456777055)
--(axis cs:36.3057324840764,0.751181853954878)
--(axis cs:35.6687898089172,0.736716449013982)
--(axis cs:35.031847133758,0.723953592960994)
--(axis cs:34.3949044585987,0.722115748989948)
--(axis cs:33.7579617834395,0.709423235872941)
--(axis cs:33.1210191082803,0.696693202515507)
--(axis cs:32.484076433121,0.689131061082804)
--(axis cs:31.8471337579618,0.683582917580221)
--(axis cs:31.2101910828025,0.677604684170985)
--(axis cs:30.5732484076433,0.655048041204845)
--(axis cs:29.9363057324841,0.648424437000685)
--(axis cs:29.2993630573248,0.637357172819524)
--(axis cs:28.6624203821656,0.62947699198909)
--(axis cs:28.0254777070064,0.615043716756273)
--(axis cs:27.3885350318471,0.604351806581648)
--(axis cs:26.7515923566879,0.592056934916069)
--(axis cs:26.1146496815287,0.581041998060004)
--(axis cs:25.4777070063694,0.566686613048296)
--(axis cs:24.8407643312102,0.559675709701679)
--(axis cs:24.203821656051,0.548416671572339)
--(axis cs:23.5668789808917,0.526900680040872)
--(axis cs:22.9299363057325,0.511721873267003)
--(axis cs:22.2929936305732,0.484137310835146)
--(axis cs:21.656050955414,0.47906435112114)
--(axis cs:21.0191082802548,0.451865194319236)
--(axis cs:20.3821656050955,0.424226447551764)
--(axis cs:19.7452229299363,0.403321663889507)
--(axis cs:19.1082802547771,0.382600814632858)
--(axis cs:18.4713375796178,0.365295354991377)
--(axis cs:17.8343949044586,0.344535904023143)
--(axis cs:17.1974522292994,0.320698682483714)
--(axis cs:16.5605095541401,0.307057540174976)
--(axis cs:15.9235668789809,0.294511577584892)
--(axis cs:15.2866242038217,0.273456559382828)
--(axis cs:14.6496815286624,0.256158457790124)
--(axis cs:14.0127388535032,0.241244867040416)
--(axis cs:13.3757961783439,0.227945394292386)
--(axis cs:12.7388535031847,0.208875716679116)
--(axis cs:12.1019108280255,0.192717530027505)
--(axis cs:11.4649681528662,0.171178198976861)
--(axis cs:10.828025477707,0.151838441679259)
--(axis cs:10.1910828025478,0.137635886869642)
--(axis cs:9.55414012738853,0.125867443513028)
--(axis cs:8.9171974522293,0.114022338866052)
--(axis cs:8.28025477707006,0.101840967195456)
--(axis cs:7.64331210191083,0.0940069746295542)
--(axis cs:7.00636942675159,0.0892696394371724)
--(axis cs:6.36942675159236,0.0860093442795212)
--(axis cs:5.73248407643312,0.0851731781045794)
--(axis cs:5.09554140127389,0.0831584335398359)
--(axis cs:4.45859872611465,0.0814224621574524)
--(axis cs:3.82165605095541,0.0814229307737238)
--(axis cs:3.18471337579618,0.0813437488262462)
--(axis cs:2.54777070063694,0.0802368812147328)
--(axis cs:1.91082802547771,0.0803902433438268)
--(axis cs:1.27388535031847,0.0802368812147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_accuracy_sfw_order_var_d.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.08
0.636942675159236 0.08
1.27388535031847 0.0800390625
1.91082802547771 0.0799609375
2.54777070063694 0.0800390625
3.18471337579618 0.0801171875
3.82165605095541 0.08015625
4.45859872611465 0.080703125
5.09554140127389 0.081328125
5.73248407643312 0.082734375
6.36942675159236 0.0848046875
7.00636942675159 0.08828125
7.64331210191083 0.0914453125
8.28025477707006 0.099375
8.9171974522293 0.1054296875
9.55414012738853 0.115625
10.1910828025478 0.12671875
10.828025477707 0.14796875
11.4649681528662 0.161484375
12.1019108280255 0.179453125
12.7388535031847 0.1940234375
13.3757961783439 0.2108203125
14.0127388535032 0.2296875
14.6496815286624 0.25328125
15.2866242038217 0.2611328125
15.9235668789809 0.2809375
16.5605095541401 0.2941015625
17.1974522292994 0.311875
17.8343949044586 0.3259375
18.4713375796178 0.346640625
19.1082802547771 0.366953125
19.7452229299363 0.3956640625
20.3821656050955 0.4137109375
21.0191082802548 0.441015625
21.656050955414 0.4603125
22.2929936305732 0.4801171875
22.9299363057325 0.494453125
23.5668789808917 0.5178125
24.203821656051 0.533515625
24.8407643312102 0.543125
25.4777070063694 0.5569140625
26.1146496815287 0.577265625
26.7515923566879 0.5880859375
27.3885350318471 0.603671875
28.0254777070064 0.6134765625
28.6624203821656 0.6195703125
29.2993630573248 0.6334375
29.9363057324841 0.6452734375
30.5732484076433 0.6605078125
31.2101910828025 0.6669921875
31.8471337579618 0.693515625
32.484076433121 0.6972265625
33.1210191082803 0.70953125
33.7579617834395 0.71546875
34.3949044585987 0.7267578125
35.031847133758 0.740390625
35.6687898089172 0.7501953125
36.3057324840764 0.755078125
36.9426751592357 0.7619921875
37.5796178343949 0.7715234375
38.2165605095541 0.7710546875
38.8535031847134 0.77421875
39.4904458598726 0.7849609375
40.1273885350318 0.800625
40.7643312101911 0.8073828125
41.4012738853503 0.8062890625
42.0382165605096 0.8063671875
42.6751592356688 0.809453125
43.312101910828 0.8196875
43.9490445859873 0.826640625
44.5859872611465 0.83234375
45.2229299363057 0.8448828125
45.859872611465 0.8451171875
46.4968152866242 0.853515625
47.1337579617834 0.8577734375
47.7707006369427 0.8620703125
48.4076433121019 0.8695703125
49.0445859872611 0.8809375
49.6815286624204 0.889609375
50.3184713375796 0.8891015625
50.9554140127388 0.893984375
51.5923566878981 0.88828125
52.2292993630573 0.88296875
52.8662420382166 0.88234375
53.5031847133758 0.891640625
54.140127388535 0.886640625
54.7770700636943 0.8831640625
55.4140127388535 0.8852734375
56.0509554140127 0.88828125
56.687898089172 0.8858203125
57.3248407643312 0.8951171875
57.9617834394904 0.8983203125
58.5987261146497 0.903125
59.2356687898089 0.906171875
59.8726114649682 0.9059375
60.5095541401274 0.9121484375
61.1464968152866 0.9191796875
61.7834394904459 0.9195703125
62.4203821656051 0.926640625
63.0573248407643 0.93609375
63.6942675159236 0.9351953125
64.3312101910828 0.939296875
64.968152866242 0.9453125
65.6050955414013 0.947421875
66.2420382165605 0.955390625
66.8789808917197 0.954296875
67.515923566879 0.9533984375
68.1528662420382 0.9609375
68.7898089171974 0.9644921875
69.4267515923567 0.9653515625
70.0636942675159 0.9683984375
70.7006369426752 0.9669140625
71.3375796178344 0.9662109375
71.9745222929936 0.9673046875
72.6114649681529 0.9687890625
73.2484076433121 0.9706640625
73.8853503184713 0.970234375
74.5222929936306 0.9722265625
75.1592356687898 0.972890625
75.796178343949 0.9755078125
76.4331210191083 0.9728125
77.0700636942675 0.971875
77.7070063694268 0.97671875
78.343949044586 0.980703125
78.9808917197452 0.9799609375
79.6178343949044 0.9834375
80.2547770700637 0.981484375
80.8917197452229 0.9838671875
81.5286624203822 0.9840625
82.1656050955414 0.982421875
82.8025477707006 0.986640625
83.4394904458599 0.985234375
84.0764331210191 0.9833203125
84.7133757961783 0.98609375
85.3503184713376 0.9858203125
85.9872611464968 0.989140625
86.6242038216561 0.9928515625
87.2611464968153 0.993515625
87.8980891719745 0.9955859375
88.5350318471338 0.996328125
89.171974522293 0.9972265625
89.8089171974522 0.9973828125
90.4458598726115 0.996484375
91.0828025477707 0.99546875
91.7197452229299 0.995703125
92.3566878980892 0.994609375
92.9936305732484 0.99734375
93.6305732484076 0.998828125
94.2675159235669 0.999765625
94.9044585987261 0.999921875
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color3, fill opacity=0.25]
(axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0794833008411496)
--(axis cs:2.54777070063694,0.0795611139660534)
--(axis cs:3.18471337579618,0.0795016092928163)
--(axis cs:3.82165605095541,0.079376909682641)
--(axis cs:4.45859872611465,0.0795358366125115)
--(axis cs:5.09554140127389,0.079640638139564)
--(axis cs:5.73248407643312,0.0804128556740863)
--(axis cs:6.36942675159236,0.0818113750849239)
--(axis cs:7.00636942675159,0.0844209319737852)
--(axis cs:7.64331210191083,0.086933315665488)
--(axis cs:8.28025477707006,0.0936582764010211)
--(axis cs:8.9171974522293,0.0989918353167827)
--(axis cs:9.55414012738853,0.108349138313541)
--(axis cs:10.1910828025478,0.118772788375319)
--(axis cs:10.828025477707,0.138854143051905)
--(axis cs:11.4649681528662,0.152030314972516)
--(axis cs:12.1019108280255,0.169604191404065)
--(axis cs:12.7388535031847,0.183875311652924)
--(axis cs:13.3757961783439,0.200724935290756)
--(axis cs:14.0127388535032,0.219419579772669)
--(axis cs:14.6496815286624,0.242645037340541)
--(axis cs:15.2866242038217,0.25028551375223)
--(axis cs:15.9235668789809,0.269744550934462)
--(axis cs:16.5605095541401,0.282893626385558)
--(axis cs:17.1974522292994,0.300143223690891)
--(axis cs:17.8343949044586,0.31373670813754)
--(axis cs:18.4713375796178,0.334165098783931)
--(axis cs:19.1082802547771,0.354138765237454)
--(axis cs:19.7452229299363,0.382370885706581)
--(axis cs:20.3821656050955,0.400409423355375)
--(axis cs:21.0191082802548,0.427741546323028)
--(axis cs:21.656050955414,0.446773212837547)
--(axis cs:22.2929936305732,0.466760302100794)
--(axis cs:22.9299363057325,0.481454258693097)
--(axis cs:23.5668789808917,0.505189532490785)
--(axis cs:24.203821656051,0.520934089506975)
--(axis cs:24.8407643312102,0.530708654902822)
--(axis cs:25.4777070063694,0.544319913894108)
--(axis cs:26.1146496815287,0.564730341164539)
--(axis cs:26.7515923566879,0.575254315247805)
--(axis cs:27.3885350318471,0.590998013352268)
--(axis cs:28.0254777070064,0.600754803547162)
--(axis cs:28.6624203821656,0.606681762631146)
--(axis cs:29.2993630573248,0.620475023707059)
--(axis cs:29.9363057324841,0.632443348234625)
--(axis cs:30.5732484076433,0.647620233837926)
--(axis cs:31.2101910828025,0.65437823617588)
--(axis cs:31.8471337579618,0.681040337672513)
--(axis cs:32.484076433121,0.684777754465731)
--(axis cs:33.1210191082803,0.697458206041386)
--(axis cs:33.7579617834395,0.703323839705804)
--(axis cs:34.3949044585987,0.714802703274133)
--(axis cs:35.031847133758,0.728872115332161)
--(axis cs:35.6687898089172,0.738843830116802)
--(axis cs:36.3057324840764,0.743798616749816)
--(axis cs:36.9426751592357,0.750522780278715)
--(axis cs:37.5796178343949,0.760190702915814)
--(axis cs:38.2165605095541,0.759574229330955)
--(axis cs:38.8535031847134,0.762974954302607)
--(axis cs:39.4904458598726,0.773890411885118)
--(axis cs:40.1273885350318,0.789554938772142)
--(axis cs:40.7643312101911,0.796436685150004)
--(axis cs:41.4012738853503,0.795265991617158)
--(axis cs:42.0382165605096,0.795272688286519)
--(axis cs:42.6751592356688,0.798358054978367)
--(axis cs:43.312101910828,0.80873650701923)
--(axis cs:43.9490445859873,0.815853573245524)
--(axis cs:44.5859872611465,0.821668744793431)
--(axis cs:45.2229299363057,0.834493065491104)
--(axis cs:45.859872611465,0.834735561338163)
--(axis cs:46.4968152866242,0.843300870527435)
--(axis cs:47.1337579617834,0.847737186395092)
--(axis cs:47.7707006369427,0.852150681817081)
--(axis cs:48.4076433121019,0.859783340896605)
--(axis cs:49.0445859872611,0.871689596207466)
--(axis cs:49.6815286624204,0.880756205072594)
--(axis cs:50.3184713375796,0.880343981008318)
--(axis cs:50.9554140127388,0.885664371979787)
--(axis cs:51.5923566878981,0.879720438880134)
--(axis cs:52.2292993630573,0.874450533500019)
--(axis cs:52.8662420382166,0.873944886684123)
--(axis cs:53.5031847133758,0.883276287375417)
--(axis cs:54.140127388535,0.878351340682457)
--(axis cs:54.7770700636943,0.875077155351037)
--(axis cs:55.4140127388535,0.877260314097383)
--(axis cs:56.0509554140127,0.880563548170825)
--(axis cs:56.687898089172,0.878243344188756)
--(axis cs:57.3248407643312,0.887072068563431)
--(axis cs:57.9617834394904,0.890604223038048)
--(axis cs:58.5987261146497,0.895286736054973)
--(axis cs:59.2356687898089,0.898454791044199)
--(axis cs:59.8726114649682,0.898365184218342)
--(axis cs:60.5095541401274,0.904193619958775)
--(axis cs:61.1464968152866,0.911085910266937)
--(axis cs:61.7834394904459,0.911515863890171)
--(axis cs:62.4203821656051,0.918469496868704)
--(axis cs:63.0573248407643,0.928132968473605)
--(axis cs:63.6942675159236,0.927687869189207)
--(axis cs:64.3312101910828,0.931984078731181)
--(axis cs:64.968152866242,0.938270280705455)
--(axis cs:65.6050955414013,0.940718269560987)
--(axis cs:66.2420382165605,0.948936948712046)
--(axis cs:66.8789808917197,0.947452572082838)
--(axis cs:67.515923566879,0.946778342623368)
--(axis cs:68.1528662420382,0.955015894430447)
--(axis cs:68.7898089171974,0.958856305475934)
--(axis cs:69.4267515923567,0.959942139492766)
--(axis cs:70.0636942675159,0.963266676477749)
--(axis cs:70.7006369426752,0.961672723762104)
--(axis cs:71.3375796178344,0.961134235875001)
--(axis cs:71.9745222929936,0.962247689988702)
--(axis cs:72.6114649681529,0.96389227768154)
--(axis cs:73.2484076433121,0.966393118991567)
--(axis cs:73.8853503184713,0.966038564246301)
--(axis cs:74.5222929936306,0.967961065245365)
--(axis cs:75.1592356687898,0.968934831095345)
--(axis cs:75.796178343949,0.971361714507328)
--(axis cs:76.4331210191083,0.968405609556168)
--(axis cs:77.0700636942675,0.967509624986973)
--(axis cs:77.7070063694268,0.972211924642821)
--(axis cs:78.343949044586,0.976134595648253)
--(axis cs:78.9808917197452,0.975458462097938)
--(axis cs:79.6178343949044,0.978987338064761)
--(axis cs:80.2547770700637,0.977126242592546)
--(axis cs:80.8917197452229,0.97954229645067)
--(axis cs:81.5286624203822,0.979735215031034)
--(axis cs:82.1656050955414,0.978053087831145)
--(axis cs:82.8025477707006,0.982471964041819)
--(axis cs:83.4394904458599,0.980969139759697)
--(axis cs:84.0764331210191,0.97896599412723)
--(axis cs:84.7133757961783,0.981893537771955)
--(axis cs:85.3503184713376,0.981627290551836)
--(axis cs:85.9872611464968,0.985210377970007)
--(axis cs:86.6242038216561,0.989478819188722)
--(axis cs:87.2611464968153,0.990305245403856)
--(axis cs:87.8980891719745,0.99284636310632)
--(axis cs:88.5350318471338,0.993836514722171)
--(axis cs:89.171974522293,0.995006660921457)
--(axis cs:89.8089171974522,0.99526149176307)
--(axis cs:90.4458598726115,0.99405581995625)
--(axis cs:91.0828025477707,0.992845913734285)
--(axis cs:91.7197452229299,0.993117596246576)
--(axis cs:92.3566878980892,0.991836148122269)
--(axis cs:92.9936305732484,0.995222675133889)
--(axis cs:93.6305732484076,0.997360232664496)
--(axis cs:94.2675159235669,0.999093018685842)
--(axis cs:94.9044585987261,0.99953201368597)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1.00031173631403)
--(axis cs:94.2675159235669,1.00043823131416)
--(axis cs:93.6305732484076,1.0002960173355)
--(axis cs:92.9936305732484,0.999464824866111)
--(axis cs:92.3566878980892,0.997382601877731)
--(axis cs:91.7197452229299,0.998288653753424)
--(axis cs:91.0828025477707,0.998091586265715)
--(axis cs:90.4458598726115,0.99891293004375)
--(axis cs:89.8089171974522,0.99950413323693)
--(axis cs:89.171974522293,0.999446464078543)
--(axis cs:88.5350318471338,0.998819735277829)
--(axis cs:87.8980891719745,0.99832551189368)
--(axis cs:87.2611464968153,0.996726004596144)
--(axis cs:86.6242038216561,0.996224305811278)
--(axis cs:85.9872611464968,0.993070872029993)
--(axis cs:85.3503184713376,0.990013334448164)
--(axis cs:84.7133757961783,0.990293962228045)
--(axis cs:84.0764331210191,0.98767463087277)
--(axis cs:83.4394904458599,0.989499610240303)
--(axis cs:82.8025477707006,0.990809285958181)
--(axis cs:82.1656050955414,0.986790662168855)
--(axis cs:81.5286624203822,0.988389784968966)
--(axis cs:80.8917197452229,0.98819207854933)
--(axis cs:80.2547770700637,0.985842507407454)
--(axis cs:79.6178343949044,0.987887661935239)
--(axis cs:78.9808917197452,0.984463412902062)
--(axis cs:78.343949044586,0.985271654351747)
--(axis cs:77.7070063694268,0.981225575357179)
--(axis cs:77.0700636942675,0.976240375013027)
--(axis cs:76.4331210191083,0.977219390443832)
--(axis cs:75.796178343949,0.979653910492671)
--(axis cs:75.1592356687898,0.976846418904655)
--(axis cs:74.5222929936306,0.976492059754635)
--(axis cs:73.8853503184713,0.974430185753699)
--(axis cs:73.2484076433121,0.974935006008433)
--(axis cs:72.6114649681529,0.97368584731846)
--(axis cs:71.9745222929936,0.972361685011297)
--(axis cs:71.3375796178344,0.971287639124999)
--(axis cs:70.7006369426752,0.972155401237896)
--(axis cs:70.0636942675159,0.973530198522251)
--(axis cs:69.4267515923567,0.970760985507234)
--(axis cs:68.7898089171974,0.970128069524066)
--(axis cs:68.1528662420382,0.966859105569553)
--(axis cs:67.515923566879,0.960018532376632)
--(axis cs:66.8789808917197,0.961141177917162)
--(axis cs:66.2420382165605,0.961844301287954)
--(axis cs:65.6050955414013,0.954125480439012)
--(axis cs:64.968152866242,0.952354719294545)
--(axis cs:64.3312101910828,0.946609671268819)
--(axis cs:63.6942675159236,0.942702755810793)
--(axis cs:63.0573248407643,0.944054531526395)
--(axis cs:62.4203821656051,0.934811753131295)
--(axis cs:61.7834394904459,0.927624761109829)
--(axis cs:61.1464968152866,0.927273464733063)
--(axis cs:60.5095541401274,0.920103255041225)
--(axis cs:59.8726114649682,0.913509815781658)
--(axis cs:59.2356687898089,0.913888958955801)
--(axis cs:58.5987261146497,0.910963263945027)
--(axis cs:57.9617834394904,0.906036401961952)
--(axis cs:57.3248407643312,0.903162306436569)
--(axis cs:56.687898089172,0.893397280811244)
--(axis cs:56.0509554140127,0.895998951829175)
--(axis cs:55.4140127388535,0.893286560902617)
--(axis cs:54.7770700636943,0.891250969648963)
--(axis cs:54.140127388535,0.894929909317543)
--(axis cs:53.5031847133758,0.900004962624583)
--(axis cs:52.8662420382166,0.890742613315877)
--(axis cs:52.2292993630573,0.891486966499981)
--(axis cs:51.5923566878981,0.896842061119867)
--(axis cs:50.9554140127388,0.902304378020213)
--(axis cs:50.3184713375796,0.897859143991682)
--(axis cs:49.6815286624204,0.898462544927406)
--(axis cs:49.0445859872611,0.890185403792534)
--(axis cs:48.4076433121019,0.879357284103395)
--(axis cs:47.7707006369427,0.871989943182919)
--(axis cs:47.1337579617834,0.867809688604908)
--(axis cs:46.4968152866242,0.863730379472565)
--(axis cs:45.859872611465,0.855498813661837)
--(axis cs:45.2229299363057,0.855272559508896)
--(axis cs:44.5859872611465,0.843018755206569)
--(axis cs:43.9490445859873,0.837427676754476)
--(axis cs:43.312101910828,0.83063849298077)
--(axis cs:42.6751592356688,0.820548195021633)
--(axis cs:42.0382165605096,0.817461686713481)
--(axis cs:41.4012738853503,0.817312133382842)
--(axis cs:40.7643312101911,0.818328939849996)
--(axis cs:40.1273885350318,0.811695061227858)
--(axis cs:39.4904458598726,0.796031463114882)
--(axis cs:38.8535031847134,0.785462545697393)
--(axis cs:38.2165605095541,0.782535145669045)
--(axis cs:37.5796178343949,0.782856172084185)
--(axis cs:36.9426751592357,0.773461594721285)
--(axis cs:36.3057324840764,0.766357633250184)
--(axis cs:35.6687898089172,0.761546794883199)
--(axis cs:35.031847133758,0.751909134667839)
--(axis cs:34.3949044585987,0.738712921725867)
--(axis cs:33.7579617834395,0.727613660294196)
--(axis cs:33.1210191082803,0.721604293958614)
--(axis cs:32.484076433121,0.709675370534269)
--(axis cs:31.8471337579618,0.705990912327487)
--(axis cs:31.2101910828025,0.67960613882412)
--(axis cs:30.5732484076433,0.673395391162074)
--(axis cs:29.9363057324841,0.658103526765375)
--(axis cs:29.2993630573248,0.646399976292941)
--(axis cs:28.6624203821656,0.632458862368854)
--(axis cs:28.0254777070064,0.626198321452838)
--(axis cs:27.3885350318471,0.616345736647732)
--(axis cs:26.7515923566879,0.600917559752195)
--(axis cs:26.1146496815287,0.589800908835461)
--(axis cs:25.4777070063694,0.569508211105892)
--(axis cs:24.8407643312102,0.555541345097177)
--(axis cs:24.203821656051,0.546097160493025)
--(axis cs:23.5668789808917,0.530435467509215)
--(axis cs:22.9299363057325,0.507451991306903)
--(axis cs:22.2929936305732,0.493474072899206)
--(axis cs:21.656050955414,0.473851787162453)
--(axis cs:21.0191082802548,0.454289703676972)
--(axis cs:20.3821656050955,0.427012451644625)
--(axis cs:19.7452229299363,0.408957239293419)
--(axis cs:19.1082802547771,0.379767484762546)
--(axis cs:18.4713375796178,0.359116151216069)
--(axis cs:17.8343949044586,0.33813829186246)
--(axis cs:17.1974522292994,0.323606776309109)
--(axis cs:16.5605095541401,0.305309498614442)
--(axis cs:15.9235668789809,0.292130449065538)
--(axis cs:15.2866242038217,0.27198011124777)
--(axis cs:14.6496815286624,0.263917462659459)
--(axis cs:14.0127388535032,0.239955420227331)
--(axis cs:13.3757961783439,0.220915689709244)
--(axis cs:12.7388535031847,0.204171563347076)
--(axis cs:12.1019108280255,0.189302058595935)
--(axis cs:11.4649681528662,0.170938435027484)
--(axis cs:10.828025477707,0.157083356948095)
--(axis cs:10.1910828025478,0.134664711624681)
--(axis cs:9.55414012738853,0.122900861686459)
--(axis cs:8.9171974522293,0.111867539683217)
--(axis cs:8.28025477707006,0.105091723598979)
--(axis cs:7.64331210191083,0.095957309334512)
--(axis cs:7.00636942675159,0.0921415680262149)
--(axis cs:6.36942675159236,0.0877979999150761)
--(axis cs:5.73248407643312,0.0850558943259137)
--(axis cs:5.09554140127389,0.083015611860436)
--(axis cs:4.45859872611465,0.0818704133874885)
--(axis cs:3.82165605095541,0.080935590317359)
--(axis cs:3.18471337579618,0.0807327657071837)
--(axis cs:2.54777070063694,0.0805170110339466)
--(axis cs:1.91082802547771,0.0804385741588504)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_accuracy_sfw_order_var_e.tex <==
\addplot [line width=0.5, opacity=0.7, color4, mark=o, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color4, thin}]
table {%
0 0.0799609375
0.636942675159236 0.0800390625
1.27388535031847 0.0800390625
1.91082802547771 0.0800390625
2.54777070063694 0.0800390625
3.18471337579618 0.0801171875
3.82165605095541 0.0801953125
4.45859872611465 0.0808984375
5.09554140127389 0.0816796875
5.73248407643312 0.0828125
6.36942675159236 0.0859765625
7.00636942675159 0.0881640625
7.64331210191083 0.0953515625
8.28025477707006 0.09953125
8.9171974522293 0.1084765625
9.55414012738853 0.1198828125
10.1910828025478 0.1335546875
10.828025477707 0.1514453125
11.4649681528662 0.1705859375
12.1019108280255 0.1964453125
12.7388535031847 0.211484375
13.3757961783439 0.2276171875
14.0127388535032 0.2440234375
14.6496815286624 0.258046875
15.2866242038217 0.2720703125
15.9235668789809 0.2869921875
16.5605095541401 0.3020703125
17.1974522292994 0.31046875
17.8343949044586 0.32875
18.4713375796178 0.3461328125
19.1082802547771 0.364609375
19.7452229299363 0.38078125
20.3821656050955 0.4068359375
21.0191082802548 0.4226171875
21.656050955414 0.4362109375
22.2929936305732 0.4584375
22.9299363057325 0.4667578125
23.5668789808917 0.4787890625
24.203821656051 0.50234375
24.8407643312102 0.507578125
25.4777070063694 0.525390625
26.1146496815287 0.5352734375
26.7515923566879 0.5453125
27.3885350318471 0.560859375
28.0254777070064 0.576796875
28.6624203821656 0.5828515625
29.2993630573248 0.5905078125
29.9363057324841 0.6035546875
30.5732484076433 0.613046875
31.2101910828025 0.6294921875
31.8471337579618 0.653203125
32.484076433121 0.656328125
33.1210191082803 0.6709375
33.7579617834395 0.6746875
34.3949044585987 0.6898046875
35.031847133758 0.6998828125
35.6687898089172 0.71296875
36.3057324840764 0.7205078125
36.9426751592357 0.7328515625
37.5796178343949 0.740703125
38.2165605095541 0.7425390625
38.8535031847134 0.7456640625
39.4904458598726 0.74859375
40.1273885350318 0.7438671875
40.7643312101911 0.7415625
41.4012738853503 0.73421875
42.0382165605096 0.74515625
42.6751592356688 0.754296875
43.312101910828 0.7609375
43.9490445859873 0.7700390625
44.5859872611465 0.778046875
45.2229299363057 0.780859375
45.859872611465 0.7921484375
46.4968152866242 0.7973046875
47.1337579617834 0.8033203125
47.7707006369427 0.8125390625
48.4076433121019 0.81265625
49.0445859872611 0.81765625
49.6815286624204 0.8245703125
50.3184713375796 0.8246875
50.9554140127388 0.82703125
51.5923566878981 0.8265234375
52.2292993630573 0.828828125
52.8662420382166 0.83671875
53.5031847133758 0.83734375
54.140127388535 0.841875
54.7770700636943 0.843984375
55.4140127388535 0.8479296875
56.0509554140127 0.8532421875
56.687898089172 0.8636328125
57.3248407643312 0.869375
57.9617834394904 0.8824609375
58.5987261146497 0.8903515625
59.2356687898089 0.885546875
59.8726114649682 0.8821484375
60.5095541401274 0.88609375
61.1464968152866 0.9005859375
61.7834394904459 0.904921875
62.4203821656051 0.9098828125
63.0573248407643 0.913671875
63.6942675159236 0.9126171875
64.3312101910828 0.9199609375
64.968152866242 0.924375
65.6050955414013 0.931953125
66.2420382165605 0.9333984375
66.8789808917197 0.93890625
67.515923566879 0.9402734375
68.1528662420382 0.93796875
68.7898089171974 0.9430859375
69.4267515923567 0.94375
70.0636942675159 0.9508203125
70.7006369426752 0.9521484375
71.3375796178344 0.9566796875
71.9745222929936 0.9615234375
72.6114649681529 0.9679296875
73.2484076433121 0.9696875
73.8853503184713 0.9671484375
74.5222929936306 0.974140625
75.1592356687898 0.9758203125
75.796178343949 0.975625
76.4331210191083 0.973984375
77.0700636942675 0.97546875
77.7070063694268 0.975703125
78.343949044586 0.976953125
78.9808917197452 0.979296875
79.6178343949044 0.9796484375
80.2547770700637 0.9799609375
80.8917197452229 0.98046875
81.5286624203822 0.98
82.1656050955414 0.97984375
82.8025477707006 0.979765625
83.4394904458599 0.9806640625
84.0764331210191 0.98109375
84.7133757961783 0.9812109375
85.3503184713376 0.9836328125
85.9872611464968 0.9852734375
86.6242038216561 0.9856640625
87.2611464968153 0.9847265625
87.8980891719745 0.9880859375
88.5350318471338 0.9894140625
89.171974522293 0.992265625
89.8089171974522 0.9955859375
90.4458598726115 0.998203125
91.0828025477707 0.9988671875
91.7197452229299 0.9996484375
92.3566878980892 0.999296875
92.9936305732484 0.998671875
93.6305732484076 0.998671875
94.2675159235669 1
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color4, fill opacity=0.25]
(axis cs:0,0.0802368812147328)
--(axis cs:0,0.0796849937852672)
--(axis cs:0.636942675159236,0.0795611139660534)
--(axis cs:1.27388535031847,0.0795611139660534)
--(axis cs:1.91082802547771,0.0797631187852672)
--(axis cs:2.54777070063694,0.0795611139660534)
--(axis cs:3.18471337579618,0.0793879259262088)
--(axis cs:3.82165605095541,0.0795785251417647)
--(axis cs:4.45859872611465,0.0795799085937995)
--(axis cs:5.09554140127389,0.079853318168993)
--(axis cs:5.73248407643312,0.0804644306565343)
--(axis cs:6.36942675159236,0.0826344877856837)
--(axis cs:7.00636942675159,0.0843362870667915)
--(axis cs:7.64331210191083,0.090307015143815)
--(axis cs:8.28025477707006,0.0939571126450598)
--(axis cs:8.9171974522293,0.101878111630236)
--(axis cs:9.55414012738853,0.112354755033588)
--(axis cs:10.1910828025478,0.125229483238068)
--(axis cs:10.828025477707,0.142538904894165)
--(axis cs:11.4649681528662,0.161200699039109)
--(axis cs:12.1019108280255,0.186644115385362)
--(axis cs:12.7388535031847,0.201835846071252)
--(axis cs:13.3757961783439,0.217389275939259)
--(axis cs:14.0127388535032,0.23409176656752)
--(axis cs:14.6496815286624,0.247576216117328)
--(axis cs:15.2866242038217,0.261680465096336)
--(axis cs:15.9235668789809,0.276020836760797)
--(axis cs:16.5605095541401,0.291108935396903)
--(axis cs:17.1974522292994,0.299188184933308)
--(axis cs:17.8343949044586,0.317049052727565)
--(axis cs:18.4713375796178,0.333881227547163)
--(axis cs:19.1082802547771,0.351889730442773)
--(axis cs:19.7452229299363,0.367759442683726)
--(axis cs:20.3821656050955,0.393812499624709)
--(axis cs:21.0191082802548,0.409678626900991)
--(axis cs:21.656050955414,0.423230190311081)
--(axis cs:22.2929936305732,0.445317752163304)
--(axis cs:22.9299363057325,0.453485636725622)
--(axis cs:23.5668789808917,0.465336465444966)
--(axis cs:24.203821656051,0.489319082188953)
--(axis cs:24.8407643312102,0.494303754456495)
--(axis cs:25.4777070063694,0.51219400554871)
--(axis cs:26.1146496815287,0.521999151148106)
--(axis cs:26.7515923566879,0.532009434385031)
--(axis cs:27.3885350318471,0.547443853209951)
--(axis cs:28.0254777070064,0.56385320768065)
--(axis cs:28.6624203821656,0.569938536946965)
--(axis cs:29.2993630573248,0.577642429675236)
--(axis cs:29.9363057324841,0.590620953366216)
--(axis cs:30.5732484076433,0.60005834135143)
--(axis cs:31.2101910828025,0.616839595192939)
--(axis cs:31.8471337579618,0.640456400581458)
--(axis cs:32.484076433121,0.643504628504195)
--(axis cs:33.1210191082803,0.658285043131011)
--(axis cs:33.7579617834395,0.661977465435978)
--(axis cs:34.3949044585987,0.676995125386324)
--(axis cs:35.031847133758,0.687279722217671)
--(axis cs:35.6687898089172,0.700656846966184)
--(axis cs:36.3057324840764,0.708157608415769)
--(axis cs:36.9426751592357,0.720614094342048)
--(axis cs:37.5796178343949,0.728501453813511)
--(axis cs:38.2165605095541,0.73060814595636)
--(axis cs:38.8535031847134,0.733733770449505)
--(axis cs:39.4904458598726,0.736922257660751)
--(axis cs:40.1273885350318,0.732524582481896)
--(axis cs:40.7643312101911,0.730477735908138)
--(axis cs:41.4012738853503,0.72360152360644)
--(axis cs:42.0382165605096,0.734942808521016)
--(axis cs:42.6751592356688,0.743997409851109)
--(axis cs:43.312101910828,0.750789675172383)
--(axis cs:43.9490445859873,0.760049555740676)
--(axis cs:44.5859872611465,0.767701806720021)
--(axis cs:45.2229299363057,0.770745939854879)
--(axis cs:45.859872611465,0.782801971944979)
--(axis cs:46.4968152866242,0.788220138078546)
--(axis cs:47.1337579617834,0.794469069982456)
--(axis cs:47.7707006369427,0.804373160756505)
--(axis cs:48.4076433121019,0.804490558111536)
--(axis cs:49.0445859872611,0.809963088747761)
--(axis cs:49.6815286624204,0.816764576979427)
--(axis cs:50.3184713375796,0.816590952439858)
--(axis cs:50.9554140127388,0.819114239683415)
--(axis cs:51.5923566878981,0.818707781475484)
--(axis cs:52.2292993630573,0.820589400743338)
--(axis cs:52.8662420382166,0.828137667194837)
--(axis cs:53.5031847133758,0.828873794247361)
--(axis cs:54.140127388535,0.833101141622962)
--(axis cs:54.7770700636943,0.834889047163108)
--(axis cs:55.4140127388535,0.838536735873669)
--(axis cs:56.0509554140127,0.844097279630951)
--(axis cs:56.687898089172,0.854645842222139)
--(axis cs:57.3248407643312,0.86035004863805)
--(axis cs:57.9617834394904,0.873700531947823)
--(axis cs:58.5987261146497,0.881799781282707)
--(axis cs:59.2356687898089,0.876954130751769)
--(axis cs:59.8726114649682,0.873459903462975)
--(axis cs:60.5095541401274,0.877776613080331)
--(axis cs:61.1464968152866,0.892393309633812)
--(axis cs:61.7834394904459,0.897014469577946)
--(axis cs:62.4203821656051,0.902065021399272)
--(axis cs:63.0573248407643,0.905541735587289)
--(axis cs:63.6942675159236,0.904362517132724)
--(axis cs:64.3312101910828,0.911816340750905)
--(axis cs:64.968152866242,0.916155578814742)
--(axis cs:65.6050955414013,0.923795448135717)
--(axis cs:66.2420382165605,0.925388215590299)
--(axis cs:66.8789808917197,0.931030283275783)
--(axis cs:67.515923566879,0.932631377700066)
--(axis cs:68.1528662420382,0.930415724012955)
--(axis cs:68.7898089171974,0.935869124519666)
--(axis cs:69.4267515923567,0.936562494195028)
--(axis cs:70.0636942675159,0.944243169046813)
--(axis cs:70.7006369426752,0.945843237026809)
--(axis cs:71.3375796178344,0.950435782066195)
--(axis cs:71.9745222929936,0.95578656137322)
--(axis cs:72.6114649681529,0.963184008832331)
--(axis cs:73.2484076433121,0.965388960727134)
--(axis cs:73.8853503184713,0.962527709330479)
--(axis cs:74.5222929936306,0.970741717491643)
--(axis cs:75.1592356687898,0.972912398824756)
--(axis cs:75.796178343949,0.972632160546634)
--(axis cs:76.4331210191083,0.970670396451021)
--(axis cs:77.0700636942675,0.972478151907887)
--(axis cs:77.7070063694268,0.972952829116786)
--(axis cs:78.343949044586,0.974446132425551)
--(axis cs:78.9808917197452,0.978016008946331)
--(axis cs:79.6178343949044,0.978393485817035)
--(axis cs:80.2547770700637,0.978595549541593)
--(axis cs:80.8917197452229,0.978842326274419)
--(axis cs:81.5286624203822,0.978462107837107)
--(axis cs:82.1656050955414,0.978011312371206)
--(axis cs:82.8025477707006,0.97837616667235)
--(axis cs:83.4394904458599,0.979307872864972)
--(axis cs:84.0764331210191,0.979133086447835)
--(axis cs:84.7133757961783,0.979103995419339)
--(axis cs:85.3503184713376,0.980959974362146)
--(axis cs:85.9872611464968,0.982459485111135)
--(axis cs:86.6242038216561,0.982772284041962)
--(axis cs:87.2611464968153,0.982071399911302)
--(axis cs:87.8980891719745,0.985018715936478)
--(axis cs:88.5350318471338,0.986294431530268)
--(axis cs:89.171974522293,0.989221885533909)
--(axis cs:89.8089171974522,0.992993933150569)
--(axis cs:90.4458598726115,0.996415888889825)
--(axis cs:91.0828025477707,0.997422471040475)
--(axis cs:91.7197452229299,0.998827112005908)
--(axis cs:92.3566878980892,0.998145783668542)
--(axis cs:92.9936305732484,0.997115681979445)
--(axis cs:93.6305732484076,0.997115681979445)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1.00022806802056)
--(axis cs:92.9936305732484,1.00022806802056)
--(axis cs:92.3566878980892,1.00044796633146)
--(axis cs:91.7197452229299,1.00046976299409)
--(axis cs:91.0828025477707,1.00031190395952)
--(axis cs:90.4458598726115,0.999990361110175)
--(axis cs:89.8089171974522,0.998177941849431)
--(axis cs:89.171974522293,0.995309364466091)
--(axis cs:88.5350318471338,0.992533693469732)
--(axis cs:87.8980891719745,0.991153159063522)
--(axis cs:87.2611464968153,0.987381725088698)
--(axis cs:86.6242038216561,0.988555840958039)
--(axis cs:85.9872611464968,0.988087389888865)
--(axis cs:85.3503184713376,0.986305650637854)
--(axis cs:84.7133757961783,0.983317879580661)
--(axis cs:84.0764331210191,0.983054413552165)
--(axis cs:83.4394904458599,0.982020252135028)
--(axis cs:82.8025477707006,0.98115508332765)
--(axis cs:82.1656050955414,0.981676187628794)
--(axis cs:81.5286624203822,0.981537892162893)
--(axis cs:80.8917197452229,0.982095173725581)
--(axis cs:80.2547770700637,0.981326325458407)
--(axis cs:79.6178343949044,0.980903389182965)
--(axis cs:78.9808917197452,0.980577741053669)
--(axis cs:78.343949044586,0.979460117574449)
--(axis cs:77.7070063694268,0.978453420883214)
--(axis cs:77.0700636942675,0.978459348092113)
--(axis cs:76.4331210191083,0.977298353548979)
--(axis cs:75.796178343949,0.978617839453366)
--(axis cs:75.1592356687898,0.978728226175244)
--(axis cs:74.5222929936306,0.977539532508357)
--(axis cs:73.8853503184713,0.971769165669521)
--(axis cs:73.2484076433121,0.973986039272866)
--(axis cs:72.6114649681529,0.972675366167669)
--(axis cs:71.9745222929936,0.96726031362678)
--(axis cs:71.3375796178344,0.962923592933805)
--(axis cs:70.7006369426752,0.958453637973191)
--(axis cs:70.0636942675159,0.957397455953187)
--(axis cs:69.4267515923567,0.950937505804972)
--(axis cs:68.7898089171974,0.950302750480335)
--(axis cs:68.1528662420382,0.945521775987045)
--(axis cs:67.515923566879,0.947915497299934)
--(axis cs:66.8789808917197,0.946782216724217)
--(axis cs:66.2420382165605,0.941408659409701)
--(axis cs:65.6050955414013,0.940110801864283)
--(axis cs:64.968152866242,0.932594421185258)
--(axis cs:64.3312101910828,0.928105534249095)
--(axis cs:63.6942675159236,0.920871857867276)
--(axis cs:63.0573248407643,0.921802014412711)
--(axis cs:62.4203821656051,0.917700603600728)
--(axis cs:61.7834394904459,0.912829280422054)
--(axis cs:61.1464968152866,0.908778565366188)
--(axis cs:60.5095541401274,0.894410886919669)
--(axis cs:59.8726114649682,0.890836971537025)
--(axis cs:59.2356687898089,0.894139619248231)
--(axis cs:58.5987261146497,0.898903343717293)
--(axis cs:57.9617834394904,0.891221343052177)
--(axis cs:57.3248407643312,0.87839995136195)
--(axis cs:56.687898089172,0.872619782777861)
--(axis cs:56.0509554140127,0.862387095369049)
--(axis cs:55.4140127388535,0.857322639126331)
--(axis cs:54.7770700636943,0.853079702836892)
--(axis cs:54.140127388535,0.850648858377038)
--(axis cs:53.5031847133758,0.845813705752639)
--(axis cs:52.8662420382166,0.845299832805163)
--(axis cs:52.2292993630573,0.837066849256663)
--(axis cs:51.5923566878981,0.834339093524516)
--(axis cs:50.9554140127388,0.834948260316585)
--(axis cs:50.3184713375796,0.832784047560142)
--(axis cs:49.6815286624204,0.832376048020573)
--(axis cs:49.0445859872611,0.825349411252239)
--(axis cs:48.4076433121019,0.820821941888464)
--(axis cs:47.7707006369427,0.820704964243495)
--(axis cs:47.1337579617834,0.812171555017544)
--(axis cs:46.4968152866242,0.806389236921454)
--(axis cs:45.859872611465,0.801494903055021)
--(axis cs:45.2229299363057,0.790972810145121)
--(axis cs:44.5859872611465,0.78839194327998)
--(axis cs:43.9490445859873,0.780028569259324)
--(axis cs:43.312101910828,0.771085324827617)
--(axis cs:42.6751592356688,0.764596340148891)
--(axis cs:42.0382165605096,0.755369691478984)
--(axis cs:41.4012738853503,0.74483597639356)
--(axis cs:40.7643312101911,0.752647264091862)
--(axis cs:40.1273885350318,0.755209792518104)
--(axis cs:39.4904458598726,0.760265242339249)
--(axis cs:38.8535031847134,0.757594354550495)
--(axis cs:38.2165605095541,0.75446997904364)
--(axis cs:37.5796178343949,0.752904796186489)
--(axis cs:36.9426751592357,0.745089030657952)
--(axis cs:36.3057324840764,0.732858016584231)
--(axis cs:35.6687898089172,0.725280653033816)
--(axis cs:35.031847133758,0.712485902782329)
--(axis cs:34.3949044585987,0.702614249613676)
--(axis cs:33.7579617834395,0.687397534564022)
--(axis cs:33.1210191082803,0.683589956868989)
--(axis cs:32.484076433121,0.669151621495805)
--(axis cs:31.8471337579618,0.665949849418542)
--(axis cs:31.2101910828025,0.642144779807061)
--(axis cs:30.5732484076433,0.62603540864857)
--(axis cs:29.9363057324841,0.616488421633784)
--(axis cs:29.2993630573248,0.603373195324764)
--(axis cs:28.6624203821656,0.595764588053035)
--(axis cs:28.0254777070064,0.58974054231935)
--(axis cs:27.3885350318471,0.57427489679005)
--(axis cs:26.7515923566879,0.558615565614969)
--(axis cs:26.1146496815287,0.548547723851894)
--(axis cs:25.4777070063694,0.53858724445129)
--(axis cs:24.8407643312102,0.520852495543505)
--(axis cs:24.203821656051,0.515368417811047)
--(axis cs:23.5668789808917,0.492241659555034)
--(axis cs:22.9299363057325,0.480029988274378)
--(axis cs:22.2929936305732,0.471557247836696)
--(axis cs:21.656050955414,0.449191684688919)
--(axis cs:21.0191082802548,0.435555748099009)
--(axis cs:20.3821656050955,0.419859375375291)
--(axis cs:19.7452229299363,0.393803057316274)
--(axis cs:19.1082802547771,0.377329019557227)
--(axis cs:18.4713375796178,0.358384397452837)
--(axis cs:17.8343949044586,0.340450947272435)
--(axis cs:17.1974522292994,0.321749315066692)
--(axis cs:16.5605095541401,0.313031689603097)
--(axis cs:15.9235668789809,0.297963538239203)
--(axis cs:15.2866242038217,0.282460159903664)
--(axis cs:14.6496815286624,0.268517533882672)
--(axis cs:14.0127388535032,0.25395510843248)
--(axis cs:13.3757961783439,0.237845099060741)
--(axis cs:12.7388535031847,0.221132903928748)
--(axis cs:12.1019108280255,0.206246509614638)
--(axis cs:11.4649681528662,0.179971175960891)
--(axis cs:10.828025477707,0.160351720105835)
--(axis cs:10.1910828025478,0.141879891761932)
--(axis cs:9.55414012738853,0.127410869966412)
--(axis cs:8.9171974522293,0.115075013369764)
--(axis cs:8.28025477707006,0.10510538735494)
--(axis cs:7.64331210191083,0.100396109856185)
--(axis cs:7.00636942675159,0.0919918379332085)
--(axis cs:6.36942675159236,0.0893186372143163)
--(axis cs:5.73248407643312,0.0851605693434657)
--(axis cs:5.09554140127389,0.083506056831007)
--(axis cs:4.45859872611465,0.0822169664062005)
--(axis cs:3.82165605095541,0.0808120998582353)
--(axis cs:3.18471337579618,0.0808464490737912)
--(axis cs:2.54777070063694,0.0805170110339466)
--(axis cs:1.91082802547771,0.0803150062147328)
--(axis cs:1.27388535031847,0.0805170110339466)
--(axis cs:0.636942675159236,0.0805170110339466)
--(axis cs:0,0.0802368812147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_sfw_order_var_f.tex <==
\addplot [line width=0.5, opacity=0.7, color5, mark=x, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color5, thin}]
table {%
0 0.08
0.636942675159236 0.0800390625
1.27388535031847 0.0799609375
1.91082802547771 0.08
2.54777070063694 0.0801953125
3.18471337579618 0.0803515625
3.82165605095541 0.0800390625
4.45859872611465 0.0812109375
5.09554140127389 0.0813671875
5.73248407643312 0.0828125
6.36942675159236 0.086171875
7.00636942675159 0.0884765625
7.64331210191083 0.0931640625
8.28025477707006 0.1029296875
8.9171974522293 0.1057421875
9.55414012738853 0.117890625
10.1910828025478 0.13390625
10.828025477707 0.1451953125
11.4649681528662 0.1664453125
12.1019108280255 0.181875
12.7388535031847 0.2067578125
13.3757961783439 0.222109375
14.0127388535032 0.2398046875
14.6496815286624 0.256171875
15.2866242038217 0.2666796875
15.9235668789809 0.2846875
16.5605095541401 0.2953515625
17.1974522292994 0.311015625
17.8343949044586 0.3244140625
18.4713375796178 0.3478125
19.1082802547771 0.3651171875
19.7452229299363 0.3845703125
20.3821656050955 0.4
21.0191082802548 0.4234765625
21.656050955414 0.4451171875
22.2929936305732 0.46109375
22.9299363057325 0.488125
23.5668789808917 0.5029296875
24.203821656051 0.51546875
24.8407643312102 0.51703125
25.4777070063694 0.5380859375
26.1146496815287 0.547578125
26.7515923566879 0.5542578125
27.3885350318471 0.571640625
28.0254777070064 0.5790625
28.6624203821656 0.5898046875
29.2993630573248 0.5971484375
29.9363057324841 0.61640625
30.5732484076433 0.6216015625
31.2101910828025 0.6305859375
31.8471337579618 0.6396875
32.484076433121 0.662109375
33.1210191082803 0.677265625
33.7579617834395 0.689296875
34.3949044585987 0.6965625
35.031847133758 0.7121875
35.6687898089172 0.7183203125
36.3057324840764 0.7199609375
36.9426751592357 0.72640625
37.5796178343949 0.7416796875
38.2165605095541 0.7411328125
38.8535031847134 0.7457421875
39.4904458598726 0.74921875
40.1273885350318 0.7547265625
40.7643312101911 0.7481640625
41.4012738853503 0.7528515625
42.0382165605096 0.761796875
42.6751592356688 0.768671875
43.312101910828 0.7834375
43.9490445859873 0.7899609375
44.5859872611465 0.7898828125
45.2229299363057 0.7900390625
45.859872611465 0.796171875
46.4968152866242 0.8054296875
47.1337579617834 0.81078125
47.7707006369427 0.8062109375
48.4076433121019 0.8041015625
49.0445859872611 0.81015625
49.6815286624204 0.8116015625
50.3184713375796 0.81984375
50.9554140127388 0.8226171875
51.5923566878981 0.83015625
52.2292993630573 0.83390625
52.8662420382166 0.8371875
53.5031847133758 0.847734375
54.140127388535 0.854140625
54.7770700636943 0.852109375
55.4140127388535 0.8553125
56.0509554140127 0.85390625
56.687898089172 0.8603125
57.3248407643312 0.8644140625
57.9617834394904 0.862890625
58.5987261146497 0.8758203125
59.2356687898089 0.88296875
59.8726114649682 0.8877734375
60.5095541401274 0.8903515625
61.1464968152866 0.901484375
61.7834394904459 0.9043359375
62.4203821656051 0.9051953125
63.0573248407643 0.91703125
63.6942675159236 0.9107421875
64.3312101910828 0.9275
64.968152866242 0.9279296875
65.6050955414013 0.9336328125
66.2420382165605 0.938828125
66.8789808917197 0.93625
67.515923566879 0.9459765625
68.1528662420382 0.9480859375
68.7898089171974 0.9500390625
69.4267515923567 0.956796875
70.0636942675159 0.963046875
70.7006369426752 0.9594140625
71.3375796178344 0.95828125
71.9745222929936 0.9630859375
72.6114649681529 0.9675
73.2484076433121 0.9685546875
73.8853503184713 0.970078125
74.5222929936306 0.97484375
75.1592356687898 0.977734375
75.796178343949 0.9793359375
76.4331210191083 0.979453125
77.0700636942675 0.9798046875
77.7070063694268 0.9824609375
78.343949044586 0.9815625
78.9808917197452 0.981171875
79.6178343949044 0.9838671875
80.2547770700637 0.9827734375
80.8917197452229 0.9840234375
81.5286624203822 0.9862890625
82.1656050955414 0.986875
82.8025477707006 0.9888671875
83.4394904458599 0.9852734375
84.0764331210191 0.984296875
84.7133757961783 0.9857421875
85.3503184713376 0.9909765625
85.9872611464968 0.99515625
86.6242038216561 0.9966796875
87.2611464968153 0.995703125
87.8980891719745 0.995625
88.5350318471338 0.996796875
89.171974522293 0.9973046875
89.8089171974522 0.99875
90.4458598726115 0.998828125
91.0828025477707 0.9987109375
91.7197452229299 0.9995703125
92.3566878980892 0.9999609375
92.9936305732484 1
93.6305732484076 1
94.2675159235669 1
94.9044585987261 1
95.5414012738853 1
96.1783439490446 1
96.8152866242038 1
97.4522292993631 1
98.0891719745223 1
98.7261146496815 1
99.3630573248408 1
100 1
};
\path [fill=color5, fill opacity=0.25]
(axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.0797631187852672)
--(axis cs:1.27388535031847,0.0796849937852672)
--(axis cs:1.91082802547771,0.0796097566561732)
--(axis cs:2.54777070063694,0.0795785251417647)
--(axis cs:3.18471337579618,0.0795249923331431)
--(axis cs:3.82165605095541,0.0794222751417647)
--(axis cs:4.45859872611465,0.0796807677517729)
--(axis cs:5.09554140127389,0.0797434687897464)
--(axis cs:5.73248407643312,0.08046875)
--(axis cs:6.36942675159236,0.0827719592974398)
--(axis cs:7.00636942675159,0.0845574970658264)
--(axis cs:7.64331210191083,0.0884602037412883)
--(axis cs:8.28025477707006,0.0969210871306533)
--(axis cs:8.9171974522293,0.0993843395182582)
--(axis cs:9.55414012738853,0.110404957319491)
--(axis cs:10.1910828025478,0.125403178657721)
--(axis cs:10.828025477707,0.136110713870423)
--(axis cs:11.4649681528662,0.156614801438753)
--(axis cs:12.1019108280255,0.171838058517622)
--(axis cs:12.7388535031847,0.196587772927582)
--(axis cs:13.3757961783439,0.21157822262048)
--(axis cs:14.0127388535032,0.229335971376844)
--(axis cs:14.6496815286624,0.245735155968559)
--(axis cs:15.2866242038217,0.256196803908249)
--(axis cs:15.9235668789809,0.274063146274251)
--(axis cs:16.5605095541401,0.284462760618156)
--(axis cs:17.1974522292994,0.299498564334751)
--(axis cs:17.8343949044586,0.312783182882459)
--(axis cs:18.4713375796178,0.335705524805429)
--(axis cs:19.1082802547771,0.352446436065174)
--(axis cs:19.7452229299363,0.371723370440562)
--(axis cs:20.3821656050955,0.387184465814116)
--(axis cs:21.0191082802548,0.410767600721254)
--(axis cs:21.656050955414,0.43219722848726)
--(axis cs:22.2929936305732,0.448079657710129)
--(axis cs:22.9299363057325,0.47542883068922)
--(axis cs:23.5668789808917,0.490158816487512)
--(axis cs:24.203821656051,0.502571918941099)
--(axis cs:24.8407643312102,0.50402292980005)
--(axis cs:25.4777070063694,0.52525418750717)
--(axis cs:26.1146496815287,0.534702385914359)
--(axis cs:26.7515923566879,0.541281841633761)
--(axis cs:27.3885350318471,0.558529511940906)
--(axis cs:28.0254777070064,0.565741490804596)
--(axis cs:28.6624203821656,0.576433072928593)
--(axis cs:29.2993630573248,0.583636279468117)
--(axis cs:29.9363057324841,0.603086851716301)
--(axis cs:30.5732484076433,0.608404474453542)
--(axis cs:31.2101910828025,0.617270024598304)
--(axis cs:31.8471337579618,0.626222674186946)
--(axis cs:32.484076433121,0.648760719807813)
--(axis cs:33.1210191082803,0.664179425598032)
--(axis cs:33.7579617834395,0.676569114483855)
--(axis cs:34.3949044585987,0.68398855859423)
--(axis cs:35.031847133758,0.699818096501602)
--(axis cs:35.6687898089172,0.706047655651266)
--(axis cs:36.3057324840764,0.707791078325536)
--(axis cs:36.9426751592357,0.71427992991132)
--(axis cs:37.5796178343949,0.729765993968236)
--(axis cs:38.2165605095541,0.729409797173126)
--(axis cs:38.8535031847134,0.733722327285523)
--(axis cs:39.4904458598726,0.737294336031872)
--(axis cs:40.1273885350318,0.743110874696111)
--(axis cs:40.7643312101911,0.73660250873829)
--(axis cs:41.4012738853503,0.741849248013369)
--(axis cs:42.0382165605096,0.750941851822374)
--(axis cs:42.6751592356688,0.757966997610275)
--(axis cs:43.312101910828,0.773131728778067)
--(axis cs:43.9490445859873,0.780024121637922)
--(axis cs:44.5859872611465,0.779902737619666)
--(axis cs:45.2229299363057,0.780521890687681)
--(axis cs:45.859872611465,0.786437978789959)
--(axis cs:46.4968152866242,0.796039909248634)
--(axis cs:47.1337579617834,0.801808907646784)
--(axis cs:47.7707006369427,0.797442388100992)
--(axis cs:48.4076433121019,0.795265821855412)
--(axis cs:49.0445859872611,0.801575201925165)
--(axis cs:49.6815286624204,0.802843385498119)
--(axis cs:50.3184713375796,0.811105203631709)
--(axis cs:50.9554140127388,0.813874387638106)
--(axis cs:51.5923566878981,0.821125274107978)
--(axis cs:52.2292993630573,0.824840624460341)
--(axis cs:52.8662420382166,0.828327230051291)
--(axis cs:53.5031847133758,0.838852201513295)
--(axis cs:54.140127388535,0.845510348869533)
--(axis cs:54.7770700636943,0.843553526099322)
--(axis cs:55.4140127388535,0.846732928094095)
--(axis cs:56.0509554140127,0.845737985478579)
--(axis cs:56.687898089172,0.852157490470186)
--(axis cs:57.3248407643312,0.856189195291379)
--(axis cs:57.9617834394904,0.8542599517573)
--(axis cs:58.5987261146497,0.866795286838536)
--(axis cs:59.2356687898089,0.873995012693051)
--(axis cs:59.8726114649682,0.878634658412987)
--(axis cs:60.5095541401274,0.881151452563259)
--(axis cs:61.1464968152866,0.892425639177904)
--(axis cs:61.7834394904459,0.895829545923496)
--(axis cs:62.4203821656051,0.896830324649101)
--(axis cs:63.0573248407643,0.908537313801025)
--(axis cs:63.6942675159236,0.902018275664344)
--(axis cs:64.3312101910828,0.919087575096023)
--(axis cs:64.968152866242,0.919464051921368)
--(axis cs:65.6050955414013,0.925454201770087)
--(axis cs:66.2420382165605,0.930866613496729)
--(axis cs:66.8789808917197,0.928396504198928)
--(axis cs:67.515923566879,0.93859023929487)
--(axis cs:68.1528662420382,0.941314709259203)
--(axis cs:68.7898089171974,0.943608992132599)
--(axis cs:69.4267515923567,0.950777533552128)
--(axis cs:70.0636942675159,0.957592148368405)
--(axis cs:70.7006369426752,0.954457391485944)
--(axis cs:71.3375796178344,0.953368287662976)
--(axis cs:71.9745222929936,0.958217382265003)
--(axis cs:72.6114649681529,0.962776020850606)
--(axis cs:73.2484076433121,0.96423324326616)
--(axis cs:73.8853503184713,0.965967671176971)
--(axis cs:74.5222929936306,0.971386939449135)
--(axis cs:75.1592356687898,0.975404462335774)
--(axis cs:75.796178343949,0.977641708861129)
--(axis cs:76.4331210191083,0.977654337035388)
--(axis cs:77.0700636942675,0.977619424328711)
--(axis cs:77.7070063694268,0.979834212415872)
--(axis cs:78.343949044586,0.979055745190401)
--(axis cs:78.9808917197452,0.978956374492834)
--(axis cs:79.6178343949044,0.981102059144901)
--(axis cs:80.2547770700637,0.980050776915369)
--(axis cs:80.8917197452229,0.98114881770948)
--(axis cs:81.5286624203822,0.983282785188161)
--(axis cs:82.1656050955414,0.983824560831764)
--(axis cs:82.8025477707006,0.985670273452356)
--(axis cs:83.4394904458599,0.982420672317581)
--(axis cs:84.0764331210191,0.981729913083664)
--(axis cs:84.7133757961783,0.982857942146413)
--(axis cs:85.3503184713376,0.987855498885776)
--(axis cs:85.9872611464968,0.992471868594514)
--(axis cs:86.6242038216561,0.994348719802645)
--(axis cs:87.2611464968153,0.993136163083664)
--(axis cs:87.8980891719745,0.993041258485288)
--(axis cs:88.5350318471338,0.994504681849991)
--(axis cs:89.171974522293,0.995170480869394)
--(axis cs:89.8089171974522,0.997237115880388)
--(axis cs:90.4458598726115,0.997360232664496)
--(axis cs:91.0828025477707,0.997176197603499)
--(axis cs:91.7197452229299,0.998664109987648)
--(axis cs:92.3566878980892,0.999684993785267)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1.00023688121473)
--(axis cs:91.7197452229299,1.00047651501235)
--(axis cs:91.0828025477707,1.0002456773965)
--(axis cs:90.4458598726115,1.0002960173355)
--(axis cs:89.8089171974522,1.00026288411961)
--(axis cs:89.171974522293,0.999438894130606)
--(axis cs:88.5350318471338,0.99908906815001)
--(axis cs:87.8980891719745,0.998208741514712)
--(axis cs:87.2611464968153,0.998270086916336)
--(axis cs:86.6242038216561,0.999010655197355)
--(axis cs:85.9872611464968,0.997840631405486)
--(axis cs:85.3503184713376,0.994097626114224)
--(axis cs:84.7133757961783,0.988626432853587)
--(axis cs:84.0764331210191,0.986863836916336)
--(axis cs:83.4394904458599,0.988126202682419)
--(axis cs:82.8025477707006,0.992064101547644)
--(axis cs:82.1656050955414,0.989925439168236)
--(axis cs:81.5286624203822,0.989295339811839)
--(axis cs:80.8917197452229,0.98689805729052)
--(axis cs:80.2547770700637,0.985496098084631)
--(axis cs:79.6178343949044,0.986632315855099)
--(axis cs:78.9808917197452,0.983387375507166)
--(axis cs:78.343949044586,0.984069254809599)
--(axis cs:77.7070063694268,0.985087662584128)
--(axis cs:77.0700636942675,0.981989950671289)
--(axis cs:76.4331210191083,0.981251912964612)
--(axis cs:75.796178343949,0.981030166138871)
--(axis cs:75.1592356687898,0.980064287664226)
--(axis cs:74.5222929936306,0.978300560550865)
--(axis cs:73.8853503184713,0.974188578823029)
--(axis cs:73.2484076433121,0.97287613173384)
--(axis cs:72.6114649681529,0.972223979149394)
--(axis cs:71.9745222929936,0.967954492734997)
--(axis cs:71.3375796178344,0.963194212337024)
--(axis cs:70.7006369426752,0.964370733514056)
--(axis cs:70.0636942675159,0.968501601631595)
--(axis cs:69.4267515923567,0.962816216447872)
--(axis cs:68.7898089171974,0.956469132867401)
--(axis cs:68.1528662420382,0.954857165740797)
--(axis cs:67.515923566879,0.95336288570513)
--(axis cs:66.8789808917197,0.944103495801072)
--(axis cs:66.2420382165605,0.946789636503271)
--(axis cs:65.6050955414013,0.941811423229913)
--(axis cs:64.968152866242,0.936395323078632)
--(axis cs:64.3312101910828,0.935912424903977)
--(axis cs:63.6942675159236,0.919466099335656)
--(axis cs:63.0573248407643,0.925525186198975)
--(axis cs:62.4203821656051,0.913560300350899)
--(axis cs:61.7834394904459,0.912842329076504)
--(axis cs:61.1464968152866,0.910543110822096)
--(axis cs:60.5095541401274,0.899551672436742)
--(axis cs:59.8726114649682,0.896912216587013)
--(axis cs:59.2356687898089,0.891942487306948)
--(axis cs:58.5987261146497,0.884845338161464)
--(axis cs:57.9617834394904,0.8715212982427)
--(axis cs:57.3248407643312,0.872638929708621)
--(axis cs:56.687898089172,0.868467509529815)
--(axis cs:56.0509554140127,0.862074514521421)
--(axis cs:55.4140127388535,0.863892071905905)
--(axis cs:54.7770700636943,0.860665223900677)
--(axis cs:54.140127388535,0.862770901130467)
--(axis cs:53.5031847133758,0.856616548486705)
--(axis cs:52.8662420382166,0.846047769948709)
--(axis cs:52.2292993630573,0.842971875539659)
--(axis cs:51.5923566878981,0.839187225892022)
--(axis cs:50.9554140127388,0.831359987361894)
--(axis cs:50.3184713375796,0.828582296368291)
--(axis cs:49.6815286624204,0.820359739501882)
--(axis cs:49.0445859872611,0.818737298074835)
--(axis cs:48.4076433121019,0.812937303144588)
--(axis cs:47.7707006369427,0.814979486899008)
--(axis cs:47.1337579617834,0.819753592353216)
--(axis cs:46.4968152866242,0.814819465751366)
--(axis cs:45.859872611465,0.805905771210041)
--(axis cs:45.2229299363057,0.799556234312319)
--(axis cs:44.5859872611465,0.799862887380334)
--(axis cs:43.9490445859873,0.799897753362078)
--(axis cs:43.312101910828,0.793743271221933)
--(axis cs:42.6751592356688,0.779376752389725)
--(axis cs:42.0382165605096,0.772651898177626)
--(axis cs:41.4012738853503,0.763853876986631)
--(axis cs:40.7643312101911,0.75972561626171)
--(axis cs:40.1273885350318,0.766342250303889)
--(axis cs:39.4904458598726,0.761143163968128)
--(axis cs:38.8535031847134,0.757762047714477)
--(axis cs:38.2165605095541,0.752855827826873)
--(axis cs:37.5796178343949,0.753593381031764)
--(axis cs:36.9426751592357,0.73853257008868)
--(axis cs:36.3057324840764,0.732130796674464)
--(axis cs:35.6687898089172,0.730592969348734)
--(axis cs:35.031847133758,0.724556903498398)
--(axis cs:34.3949044585987,0.70913644140577)
--(axis cs:33.7579617834395,0.702024635516145)
--(axis cs:33.1210191082803,0.690351824401968)
--(axis cs:32.484076433121,0.675458030192187)
--(axis cs:31.8471337579618,0.653152325813053)
--(axis cs:31.2101910828025,0.643901850401696)
--(axis cs:30.5732484076433,0.634798650546458)
--(axis cs:29.9363057324841,0.629725648283699)
--(axis cs:29.2993630573248,0.610660595531883)
--(axis cs:28.6624203821656,0.603176302071407)
--(axis cs:28.0254777070064,0.592383509195404)
--(axis cs:27.3885350318471,0.584751738059094)
--(axis cs:26.7515923566879,0.567233783366239)
--(axis cs:26.1146496815287,0.560453864085641)
--(axis cs:25.4777070063694,0.55091768749283)
--(axis cs:24.8407643312102,0.530039570199951)
--(axis cs:24.203821656051,0.528365581058902)
--(axis cs:23.5668789808917,0.515700558512488)
--(axis cs:22.9299363057325,0.50082116931078)
--(axis cs:22.2929936305732,0.474107842289871)
--(axis cs:21.656050955414,0.45803714651274)
--(axis cs:21.0191082802548,0.436185524278746)
--(axis cs:20.3821656050955,0.412815534185885)
--(axis cs:19.7452229299363,0.397417254559438)
--(axis cs:19.1082802547771,0.377787938934826)
--(axis cs:18.4713375796178,0.359919475194572)
--(axis cs:17.8343949044586,0.33604494211754)
--(axis cs:17.1974522292994,0.322532685665249)
--(axis cs:16.5605095541401,0.306240364381844)
--(axis cs:15.9235668789809,0.295311853725749)
--(axis cs:15.2866242038217,0.277162571091751)
--(axis cs:14.6496815286624,0.266608594031441)
--(axis cs:14.0127388535032,0.250273403623156)
--(axis cs:13.3757961783439,0.23264052737952)
--(axis cs:12.7388535031847,0.216927852072418)
--(axis cs:12.1019108280255,0.191911941482378)
--(axis cs:11.4649681528662,0.176275823561247)
--(axis cs:10.828025477707,0.154279911129577)
--(axis cs:10.1910828025478,0.142409321342279)
--(axis cs:9.55414012738853,0.125376292680509)
--(axis cs:8.9171974522293,0.112100035481742)
--(axis cs:8.28025477707006,0.108938287869347)
--(axis cs:7.64331210191083,0.0978679212587117)
--(axis cs:7.00636942675159,0.0923956279341736)
--(axis cs:6.36942675159236,0.0895717907025602)
--(axis cs:5.73248407643312,0.08515625)
--(axis cs:5.09554140127389,0.0829909062102536)
--(axis cs:4.45859872611465,0.0827411072482271)
--(axis cs:3.82165605095541,0.0806558498582353)
--(axis cs:3.18471337579618,0.0811781326668569)
--(axis cs:2.54777070063694,0.0808120998582353)
--(axis cs:1.91082802547771,0.0803902433438268)
--(axis cs:1.27388535031847,0.0802368812147328)
--(axis cs:0.636942675159236,0.0803150062147328)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_accuracy_shap.tex <==
% shap
\addplot [line width=0.5, opacity=0.8, color2, mark=diamond*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color2, thin}]
table [row sep=\\]{%
0	0.0799609375 \\
0.636942675159236	0.08 \\
1.27388535031847	0.0800390625 \\
1.91082802547771	0.0799609375 \\
2.54777070063694	0.08 \\
3.18471337579618	0.0800390625 \\
3.82165605095541	0.0800390625 \\
4.45859872611465	0.0800390625 \\
5.09554140127389	0.079921875 \\
5.73248407643312	0.0798828125 \\
6.36942675159236	0.079921875 \\
7.00636942675159	0.0798828125 \\
7.64331210191083	0.0801953125 \\
8.28025477707006	0.08015625 \\
8.9171974522293	0.080234375 \\
9.55414012738853	0.0801953125 \\
10.1910828025478	0.0804296875 \\
10.828025477707	0.08125 \\
11.4649681528662	0.081875 \\
12.1019108280255	0.081875 \\
12.7388535031847	0.082734375 \\
13.3757961783439	0.0825390625 \\
14.0127388535032	0.08359375 \\
14.6496815286624	0.0866796875 \\
15.2866242038217	0.0901171875 \\
15.9235668789809	0.0934375 \\
16.5605095541401	0.097109375 \\
17.1974522292994	0.0998046875 \\
17.8343949044586	0.1030078125 \\
18.4713375796178	0.1071484375 \\
19.1082802547771	0.109765625 \\
19.7452229299363	0.111015625 \\
20.3821656050955	0.118515625 \\
21.0191082802548	0.1223828125 \\
21.656050955414	0.134609375 \\
22.2929936305732	0.142109375 \\
22.9299363057325	0.1465625 \\
23.5668789808917	0.1548046875 \\
24.203821656051	0.163671875 \\
24.8407643312102	0.17078125 \\
25.4777070063694	0.1712890625 \\
26.1146496815287	0.1767578125 \\
26.7515923566879	0.17828125 \\
27.3885350318471	0.1824609375 \\
28.0254777070064	0.190859375 \\
28.6624203821656	0.198203125 \\
29.2993630573248	0.20109375 \\
29.9363057324841	0.2105859375 \\
30.5732484076433	0.2141796875 \\
31.2101910828025	0.2244140625 \\
31.8471337579618	0.226640625 \\
32.484076433121	0.22734375 \\
33.1210191082803	0.2294921875 \\
33.7579617834395	0.2321875 \\
34.3949044585987	0.2384765625 \\
35.031847133758	0.2369921875 \\
35.6687898089172	0.23890625 \\
36.3057324840764	0.246484375 \\
36.9426751592357	0.253359375 \\
37.5796178343949	0.2477734375 \\
38.2165605095541	0.250390625 \\
38.8535031847134	0.2563671875 \\
39.4904458598726	0.2541015625 \\
40.1273885350318	0.2562109375 \\
40.7643312101911	0.26546875 \\
41.4012738853503	0.276796875 \\
42.0382165605096	0.2735546875 \\
42.6751592356688	0.271953125 \\
43.312101910828	0.2741796875 \\
43.9490445859873	0.2795703125 \\
44.5859872611465	0.275859375 \\
45.2229299363057	0.2789453125 \\
45.859872611465	0.278984375 \\
46.4968152866242	0.2884765625 \\
47.1337579617834	0.2875390625 \\
47.7707006369427	0.292109375 \\
48.4076433121019	0.2999609375 \\
49.0445859872611	0.3053125 \\
49.6815286624204	0.305703125 \\
50.3184713375796	0.30265625 \\
50.9554140127388	0.307734375 \\
51.5923566878981	0.3126953125 \\
52.2292993630573	0.3212109375 \\
52.8662420382166	0.31859375 \\
53.5031847133758	0.3240234375 \\
54.140127388535	0.3266796875 \\
54.7770700636943	0.3299609375 \\
55.4140127388535	0.3390625 \\
56.0509554140127	0.3416015625 \\
56.687898089172	0.3458203125 \\
57.3248407643312	0.347109375 \\
57.9617834394904	0.344296875 \\
58.5987261146497	0.35 \\
59.2356687898089	0.350859375 \\
59.8726114649682	0.3592578125 \\
60.5095541401274	0.3615234375 \\
61.1464968152866	0.370546875 \\
61.7834394904459	0.371328125 \\
62.4203821656051	0.37375 \\
63.0573248407643	0.373359375 \\
63.6942675159236	0.375 \\
64.3312101910828	0.3764453125 \\
64.968152866242	0.3694921875 \\
65.6050955414013	0.3724609375 \\
66.2420382165605	0.3704296875 \\
66.8789808917197	0.3716015625 \\
67.515923566879	0.37296875 \\
68.1528662420382	0.373984375 \\
68.7898089171974	0.3775 \\
69.4267515923567	0.371875 \\
70.0636942675159	0.3691796875 \\
70.7006369426752	0.374453125 \\
71.3375796178344	0.3768359375 \\
71.9745222929936	0.3812109375 \\
72.6114649681529	0.3894921875 \\
73.2484076433121	0.4028515625 \\
73.8853503184713	0.406796875 \\
74.5222929936306	0.40625 \\
75.1592356687898	0.4094140625 \\
75.796178343949	0.419453125 \\
76.4331210191083	0.42171875 \\
77.0700636942675	0.42859375 \\
77.7070063694268	0.4373828125 \\
78.343949044586	0.4352734375 \\
78.9808917197452	0.4344140625 \\
79.6178343949044	0.4351171875 \\
80.2547770700637	0.445234375 \\
80.8917197452229	0.4516796875 \\
81.5286624203822	0.4493359375 \\
82.1656050955414	0.44421875 \\
82.8025477707006	0.465859375 \\
83.4394904458599	0.480859375 \\
84.0764331210191	0.495390625 \\
84.7133757961783	0.5052734375 \\
85.3503184713376	0.5125 \\
85.9872611464968	0.5283984375 \\
86.6242038216561	0.5492578125 \\
87.2611464968153	0.5767578125 \\
87.8980891719745	0.582109375 \\
88.5350318471338	0.5861328125 \\
89.171974522293	0.6012109375 \\
89.8089171974522	0.60734375 \\
90.4458598726115	0.622734375 \\
91.0828025477707	0.6478125 \\
91.7197452229299	0.6740625 \\
92.3566878980892	0.7039453125 \\
92.9936305732484	0.7343359375 \\
93.6305732484076	0.7827734375 \\
94.2675159235669	0.8284765625 \\
94.9044585987261	0.857421875 \\
95.5414012738853	0.8803125 \\
96.1783439490446	0.9137109375 \\
96.8152866242038	0.931953125 \\
97.4522292993631	0.95296875 \\
98.0891719745223	0.972890625 \\
98.7261146496815	0.988828125 \\
99.3630573248408	0.999921875 \\
100	1 \\
};
\path [fill=color2, fill opacity=0.5] (axis cs:0,0.0802368812147328)
--(axis cs:0,0.0796849937852672)
--(axis cs:0.636942675159236,0.08)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0794829889660534)
--(axis cs:2.54777070063694,0.0794486528422541)
--(axis cs:3.18471337579618,0.0797631187852672)
--(axis cs:3.82165605095541,0.0795614258411496)
--(axis cs:4.45859872611465,0.0794227585175115)
--(axis cs:5.09554140127389,0.0792461741941847)
--(axis cs:5.73248407643312,0.0794051758411496)
--(axis cs:6.36942675159236,0.0793707981767434)
--(axis cs:7.00636942675159,0.0791549826569451)
--(axis cs:7.64331210191083,0.0792812511737538)
--(axis cs:8.28025477707006,0.0792836393554364)
--(axis cs:8.9171974522293,0.0790044295197451)
--(axis cs:9.55414012738853,0.078820787772042)
--(axis cs:10.1910828025478,0.0789474000049327)
--(axis cs:10.828025477707,0.0793537014424676)
--(axis cs:11.4649681528662,0.0794145639112929)
--(axis cs:12.1019108280255,0.0792088882407729)
--(axis cs:12.7388535031847,0.0797633731748933)
--(axis cs:13.3757961783439,0.0795462977316318)
--(axis cs:14.0127388535032,0.0800036374131539)
--(axis cs:14.6496815286624,0.0822820208396635)
--(axis cs:15.2866242038217,0.0851857432791662)
--(axis cs:15.9235668789809,0.0879829099595563)
--(axis cs:16.5605095541401,0.0910793980968658)
--(axis cs:17.1974522292994,0.0932762991681215)
--(axis cs:17.8343949044586,0.0959042327522946)
--(axis cs:18.4713375796178,0.0995851496799443)
--(axis cs:19.1082802547771,0.101899578491641)
--(axis cs:19.7452229299363,0.102680930805061)
--(axis cs:20.3821656050955,0.109980264836353)
--(axis cs:21.0191082802548,0.113346698302153)
--(axis cs:21.656050955414,0.125235901003103)
--(axis cs:22.2929936305732,0.132536447064971)
--(axis cs:22.9299363057325,0.136743553772574)
--(axis cs:23.5668789808917,0.144948380925081)
--(axis cs:24.203821656051,0.153508174401289)
--(axis cs:24.8407643312102,0.16065813922847)
--(axis cs:25.4777070063694,0.161253776518464)
--(axis cs:26.1146496815287,0.166598151853007)
--(axis cs:26.7515923566879,0.168178605918637)
--(axis cs:27.3885350318471,0.172404158672631)
--(axis cs:28.0254777070064,0.180475301872185)
--(axis cs:28.6624203821656,0.187719011904126)
--(axis cs:29.2993630573248,0.190513584260562)
--(axis cs:29.9363057324841,0.199608286575576)
--(axis cs:30.5732484076433,0.203329435654236)
--(axis cs:31.2101910828025,0.213460722540381)
--(axis cs:31.8471337579618,0.215599515377157)
--(axis cs:32.484076433121,0.216304597481071)
--(axis cs:33.1210191082803,0.218243588693776)
--(axis cs:33.7579617834395,0.220905627259934)
--(axis cs:34.3949044585987,0.227103467293812)
--(axis cs:35.031847133758,0.22549804402289)
--(axis cs:35.6687898089172,0.227721957725198)
--(axis cs:36.3057324840764,0.235033529011358)
--(axis cs:36.9426751592357,0.241903962305244)
--(axis cs:37.5796178343949,0.23627508145141)
--(axis cs:38.2165605095541,0.238762788564874)
--(axis cs:38.8535031847134,0.244829101820795)
--(axis cs:39.4904458598726,0.242714849246306)
--(axis cs:40.1273885350318,0.244949760955515)
--(axis cs:40.7643312101911,0.254079661803969)
--(axis cs:41.4012738853503,0.265238331105455)
--(axis cs:42.0382165605096,0.26194060336674)
--(axis cs:42.6751592356688,0.260377524812081)
--(axis cs:43.312101910828,0.262807404654013)
--(axis cs:43.9490445859873,0.268007753475443)
--(axis cs:44.5859872611465,0.264562151733533)
--(axis cs:45.2229299363057,0.267591546237785)
--(axis cs:45.859872611465,0.267689724097747)
--(axis cs:46.4968152866242,0.277281317179336)
--(axis cs:47.1337579617834,0.276426311968183)
--(axis cs:47.7707006369427,0.280767262642691)
--(axis cs:48.4076433121019,0.288408447938935)
--(axis cs:49.0445859872611,0.293759681527838)
--(axis cs:49.6815286624204,0.294246021394539)
--(axis cs:50.3184713375796,0.291122833951611)
--(axis cs:50.9554140127388,0.296236504938582)
--(axis cs:51.5923566878981,0.301232182177503)
--(axis cs:52.2292993630573,0.309784901939679)
--(axis cs:52.8662420382166,0.30731877397341)
--(axis cs:53.5031847133758,0.312750569644127)
--(axis cs:54.140127388535,0.315244096581782)
--(axis cs:54.7770700636943,0.318530286212914)
--(axis cs:55.4140127388535,0.327756759133739)
--(axis cs:56.0509554140127,0.330547497500635)
--(axis cs:56.687898089172,0.334731281102001)
--(axis cs:57.3248407643312,0.336049104085381)
--(axis cs:57.9617834394904,0.333588323367769)
--(axis cs:58.5987261146497,0.339342275973157)
--(axis cs:59.2356687898089,0.340346137103782)
--(axis cs:59.8726114649682,0.348658024744593)
--(axis cs:60.5095541401274,0.350768225502834)
--(axis cs:61.1464968152866,0.359735152145707)
--(axis cs:61.7834394904459,0.360748367705975)
--(axis cs:62.4203821656051,0.363365453332465)
--(axis cs:63.0573248407643,0.363262603031119)
--(axis cs:63.6942675159236,0.365029582626447)
--(axis cs:64.3312101910828,0.366182407513059)
--(axis cs:64.968152866242,0.359125973975047)
--(axis cs:65.6050955414013,0.361930711960178)
--(axis cs:66.2420382165605,0.36046056298508)
--(axis cs:66.8789808917197,0.361637521367113)
--(axis cs:67.515923566879,0.362961887687628)
--(axis cs:68.1528662420382,0.364075964504422)
--(axis cs:68.7898089171974,0.367857866995617)
--(axis cs:69.4267515923567,0.362434773062266)
--(axis cs:70.0636942675159,0.359840399094535)
--(axis cs:70.7006369426752,0.364846431827282)
--(axis cs:71.3375796178344,0.367603991303453)
--(axis cs:71.9745222929936,0.372071359482433)
--(axis cs:72.6114649681529,0.379836148001981)
--(axis cs:73.2484076433121,0.392862712102045)
--(axis cs:73.8853503184713,0.396800531221262)
--(axis cs:74.5222929936306,0.396347862712296)
--(axis cs:75.1592356687898,0.399712390498593)
--(axis cs:75.796178343949,0.409132168509097)
--(axis cs:76.4331210191083,0.411701841344387)
--(axis cs:77.0700636942675,0.418393812972618)
--(axis cs:77.7070063694268,0.427383465490203)
--(axis cs:78.343949044586,0.425123843393314)
--(axis cs:78.9808917197452,0.424263925191089)
--(axis cs:79.6178343949044,0.425151008040504)
--(axis cs:80.2547770700637,0.435333471760387)
--(axis cs:80.8917197452229,0.441975589020891)
--(axis cs:81.5286624203822,0.439300755460363)
--(axis cs:82.1656050955414,0.434474220172017)
--(axis cs:82.8025477707006,0.455703961333451)
--(axis cs:83.4394904458599,0.470979368585596)
--(axis cs:84.0764331210191,0.485879302924123)
--(axis cs:84.7133757961783,0.495726001599895)
--(axis cs:85.3503184713376,0.502954054732572)
--(axis cs:85.9872611464968,0.518938791616769)
--(axis cs:86.6242038216561,0.539760640201283)
--(axis cs:87.2611464968153,0.567390357510502)
--(axis cs:87.8980891719745,0.572534843907496)
--(axis cs:88.5350318471338,0.576542614168402)
--(axis cs:89.171974522293,0.59236400581952)
--(axis cs:89.8089171974522,0.598399519007066)
--(axis cs:90.4458598726115,0.614462167890793)
--(axis cs:91.0828025477707,0.638749455435441)
--(axis cs:91.7197452229299,0.664621120845911)
--(axis cs:92.3566878980892,0.694076994114289)
--(axis cs:92.9936305732484,0.724052609465254)
--(axis cs:93.6305732484076,0.772938804306932)
--(axis cs:94.2675159235669,0.82003304625354)
--(axis cs:94.9044585987261,0.850830756328292)
--(axis cs:95.5414012738853,0.873741306432045)
--(axis cs:96.1783439490446,0.907995061105925)
--(axis cs:96.8152866242038,0.927153199858057)
--(axis cs:97.4522292993631,0.94777695739209)
--(axis cs:98.0891719745223,0.968090948221042)
--(axis cs:98.7261146496815,0.985375541487812)
--(axis cs:99.3630573248408,0.99953201368597)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1.00031173631403)
--(axis cs:98.7261146496815,0.992280708512188)
--(axis cs:98.0891719745223,0.977690301778958)
--(axis cs:97.4522292993631,0.95816054260791)
--(axis cs:96.8152866242038,0.936753050141943)
--(axis cs:96.1783439490446,0.919426813894075)
--(axis cs:95.5414012738853,0.886883693567955)
--(axis cs:94.9044585987261,0.864012993671708)
--(axis cs:94.2675159235669,0.83692007874646)
--(axis cs:93.6305732484076,0.792608070693068)
--(axis cs:92.9936305732484,0.744619265534746)
--(axis cs:92.3566878980892,0.713813630885711)
--(axis cs:91.7197452229299,0.683503879154089)
--(axis cs:91.0828025477707,0.656875544564559)
--(axis cs:90.4458598726115,0.631006582109207)
--(axis cs:89.8089171974522,0.616287980992934)
--(axis cs:89.171974522293,0.61005786918048)
--(axis cs:88.5350318471338,0.595723010831598)
--(axis cs:87.8980891719745,0.591683906092504)
--(axis cs:87.2611464968153,0.586125267489498)
--(axis cs:86.6242038216561,0.558754984798717)
--(axis cs:85.9872611464968,0.537858083383231)
--(axis cs:85.3503184713376,0.522045945267428)
--(axis cs:84.7133757961783,0.514820873400105)
--(axis cs:84.0764331210191,0.504901947075877)
--(axis cs:83.4394904458599,0.490739381414404)
--(axis cs:82.8025477707006,0.476014788666549)
--(axis cs:82.1656050955414,0.453963279827983)
--(axis cs:81.5286624203822,0.459371119539637)
--(axis cs:80.8917197452229,0.461383785979109)
--(axis cs:80.2547770700637,0.455135278239613)
--(axis cs:79.6178343949044,0.445083366959496)
--(axis cs:78.9808917197452,0.444564199808911)
--(axis cs:78.343949044586,0.445423031606686)
--(axis cs:77.7070063694268,0.447382159509797)
--(axis cs:77.0700636942675,0.438793687027382)
--(axis cs:76.4331210191083,0.431735658655613)
--(axis cs:75.796178343949,0.429774081490903)
--(axis cs:75.1592356687898,0.419115734501407)
--(axis cs:74.5222929936306,0.416152137287704)
--(axis cs:73.8853503184713,0.416793218778738)
--(axis cs:73.2484076433121,0.412840412897955)
--(axis cs:72.6114649681529,0.399148226998019)
--(axis cs:71.9745222929936,0.390350515517567)
--(axis cs:71.3375796178344,0.386067883696547)
--(axis cs:70.7006369426752,0.384059818172718)
--(axis cs:70.0636942675159,0.378518975905465)
--(axis cs:69.4267515923567,0.381315226937734)
--(axis cs:68.7898089171974,0.387142133004383)
--(axis cs:68.1528662420382,0.383892785495578)
--(axis cs:67.515923566879,0.382975612312372)
--(axis cs:66.8789808917197,0.381565603632887)
--(axis cs:66.2420382165605,0.38039881201492)
--(axis cs:65.6050955414013,0.382991163039822)
--(axis cs:64.968152866242,0.379858401024953)
--(axis cs:64.3312101910828,0.386708217486941)
--(axis cs:63.6942675159236,0.384970417373553)
--(axis cs:63.0573248407643,0.383456146968881)
--(axis cs:62.4203821656051,0.384134546667535)
--(axis cs:61.7834394904459,0.381907882294025)
--(axis cs:61.1464968152866,0.381358597854293)
--(axis cs:60.5095541401274,0.372278649497166)
--(axis cs:59.8726114649682,0.369857600255407)
--(axis cs:59.2356687898089,0.361372612896218)
--(axis cs:58.5987261146497,0.360657724026843)
--(axis cs:57.9617834394904,0.355005426632231)
--(axis cs:57.3248407643312,0.358169645914619)
--(axis cs:56.687898089172,0.356909343897999)
--(axis cs:56.0509554140127,0.352655627499365)
--(axis cs:55.4140127388535,0.350368240866261)
--(axis cs:54.7770700636943,0.341391588787086)
--(axis cs:54.140127388535,0.338115278418217)
--(axis cs:53.5031847133758,0.335296305355873)
--(axis cs:52.8662420382166,0.32986872602659)
--(axis cs:52.2292993630573,0.332636973060321)
--(axis cs:51.5923566878981,0.324158442822497)
--(axis cs:50.9554140127388,0.319232245061418)
--(axis cs:50.3184713375796,0.314189666048389)
--(axis cs:49.6815286624204,0.317160228605461)
--(axis cs:49.0445859872611,0.316865318472162)
--(axis cs:48.4076433121019,0.311513427061065)
--(axis cs:47.7707006369427,0.303451487357309)
--(axis cs:47.1337579617834,0.298651813031817)
--(axis cs:46.4968152866242,0.299671807820664)
--(axis cs:45.859872611465,0.290279025902253)
--(axis cs:45.2229299363057,0.290299078762215)
--(axis cs:44.5859872611465,0.287156598266467)
--(axis cs:43.9490445859873,0.291132871524557)
--(axis cs:43.312101910828,0.285551970345987)
--(axis cs:42.6751592356688,0.283528725187919)
--(axis cs:42.0382165605096,0.28516877163326)
--(axis cs:41.4012738853503,0.288355418894545)
--(axis cs:40.7643312101911,0.276857838196031)
--(axis cs:40.1273885350318,0.267472114044485)
--(axis cs:39.4904458598726,0.265488275753694)
--(axis cs:38.8535031847134,0.267905273179205)
--(axis cs:38.2165605095541,0.262018461435126)
--(axis cs:37.5796178343949,0.25927179354859)
--(axis cs:36.9426751592357,0.264814787694756)
--(axis cs:36.3057324840764,0.257935220988642)
--(axis cs:35.6687898089172,0.250090542274802)
--(axis cs:35.031847133758,0.24848633097711)
--(axis cs:34.3949044585987,0.249849657706188)
--(axis cs:33.7579617834395,0.243469372740066)
--(axis cs:33.1210191082803,0.240740786306224)
--(axis cs:32.484076433121,0.238382902518929)
--(axis cs:31.8471337579618,0.237681734622843)
--(axis cs:31.2101910828025,0.235367402459619)
--(axis cs:30.5732484076433,0.225029939345764)
--(axis cs:29.9363057324841,0.221563588424424)
--(axis cs:29.2993630573248,0.211673915739438)
--(axis cs:28.6624203821656,0.208687238095874)
--(axis cs:28.0254777070064,0.201243448127815)
--(axis cs:27.3885350318471,0.192517716327369)
--(axis cs:26.7515923566879,0.188383894081363)
--(axis cs:26.1146496815287,0.186917473146993)
--(axis cs:25.4777070063694,0.181324348481536)
--(axis cs:24.8407643312102,0.18090436077153)
--(axis cs:24.203821656051,0.173835575598711)
--(axis cs:23.5668789808917,0.164660994074919)
--(axis cs:22.9299363057325,0.156381446227426)
--(axis cs:22.2929936305732,0.151682302935029)
--(axis cs:21.656050955414,0.143982848996897)
--(axis cs:21.0191082802548,0.131418926697847)
--(axis cs:20.3821656050955,0.127050985163647)
--(axis cs:19.7452229299363,0.119350319194939)
--(axis cs:19.1082802547771,0.117631671508359)
--(axis cs:18.4713375796178,0.114711725320056)
--(axis cs:17.8343949044586,0.110111392247705)
--(axis cs:17.1974522292994,0.106333075831878)
--(axis cs:16.5605095541401,0.103139351903134)
--(axis cs:15.9235668789809,0.0988920900404437)
--(axis cs:15.2866242038217,0.0950486317208338)
--(axis cs:14.6496815286624,0.0910773541603365)
--(axis cs:14.0127388535032,0.087183862586846)
--(axis cs:13.3757961783439,0.0855318272683682)
--(axis cs:12.7388535031847,0.0857053768251067)
--(axis cs:12.1019108280255,0.0845411117592271)
--(axis cs:11.4649681528662,0.0843354360887072)
--(axis cs:10.828025477707,0.0831462985575324)
--(axis cs:10.1910828025478,0.0819119749950673)
--(axis cs:9.55414012738853,0.081569837227958)
--(axis cs:8.9171974522293,0.0814643204802549)
--(axis cs:8.28025477707006,0.0810288606445635)
--(axis cs:7.64331210191083,0.0811093738262463)
--(axis cs:7.00636942675159,0.0806106423430549)
--(axis cs:6.36942675159236,0.0804729518232566)
--(axis cs:5.73248407643312,0.0803604491588504)
--(axis cs:5.09554140127389,0.0805975758058153)
--(axis cs:4.45859872611465,0.0806553664824885)
--(axis cs:3.82165605095541,0.0805166991588504)
--(axis cs:3.18471337579618,0.0803150062147328)
--(axis cs:2.54777070063694,0.0805513471577459)
--(axis cs:1.91082802547771,0.0804388860339466)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.08)
--(axis cs:0,0.0802368812147328)
--cycle;


==> img/mnist/mnist_rate_accuracy_smoothgrad.tex <==
% smoothgrad
\addplot [line width=0.5, opacity=0.8, color7, mark=triangle, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color7, thin}]
table [row sep=\\]{%
0	0.08 \\
0.636942675159236	0.0800390625 \\
1.27388535031847	0.0800390625 \\
1.91082802547771	0.08 \\
2.54777070063694	0.0800390625 \\
3.18471337579618	0.08 \\
3.82165605095541	0.080078125 \\
4.45859872611465	0.0801953125 \\
5.09554140127389	0.080234375 \\
5.73248407643312	0.0801953125 \\
6.36942675159236	0.0807421875 \\
7.00636942675159	0.0810546875 \\
7.64331210191083	0.0811328125 \\
8.28025477707006	0.0812890625 \\
8.9171974522293	0.0828515625 \\
9.55414012738853	0.08578125 \\
10.1910828025478	0.0891796875 \\
10.828025477707	0.0910546875 \\
11.4649681528662	0.095078125 \\
12.1019108280255	0.0996875 \\
12.7388535031847	0.1067578125 \\
13.3757961783439	0.1098828125 \\
14.0127388535032	0.111328125 \\
14.6496815286624	0.1173828125 \\
15.2866242038217	0.1266796875 \\
15.9235668789809	0.133515625 \\
16.5605095541401	0.1392578125 \\
17.1974522292994	0.1427734375 \\
17.8343949044586	0.155078125 \\
18.4713375796178	0.1612890625 \\
19.1082802547771	0.1689453125 \\
19.7452229299363	0.1729296875 \\
20.3821656050955	0.1893359375 \\
21.0191082802548	0.204296875 \\
21.656050955414	0.2208984375 \\
22.2929936305732	0.2308984375 \\
22.9299363057325	0.230859375 \\
23.5668789808917	0.241484375 \\
24.203821656051	0.259921875 \\
24.8407643312102	0.263828125 \\
25.4777070063694	0.2740625 \\
26.1146496815287	0.2900390625 \\
26.7515923566879	0.30984375 \\
27.3885350318471	0.3312890625 \\
28.0254777070064	0.34984375 \\
28.6624203821656	0.3744140625 \\
29.2993630573248	0.3883203125 \\
29.9363057324841	0.4085546875 \\
30.5732484076433	0.423515625 \\
31.2101910828025	0.436640625 \\
31.8471337579618	0.453515625 \\
32.484076433121	0.4634375 \\
33.1210191082803	0.4792578125 \\
33.7579617834395	0.4959375 \\
34.3949044585987	0.512265625 \\
35.031847133758	0.523046875 \\
35.6687898089172	0.5348828125 \\
36.3057324840764	0.53796875 \\
36.9426751592357	0.5521484375 \\
37.5796178343949	0.569609375 \\
38.2165605095541	0.580390625 \\
38.8535031847134	0.5925 \\
39.4904458598726	0.601875 \\
40.1273885350318	0.610390625 \\
40.7643312101911	0.6201171875 \\
41.4012738853503	0.63328125 \\
42.0382165605096	0.6413671875 \\
42.6751592356688	0.65375 \\
43.312101910828	0.658515625 \\
43.9490445859873	0.6578515625 \\
44.5859872611465	0.6705859375 \\
45.2229299363057	0.6808203125 \\
45.859872611465	0.696171875 \\
46.4968152866242	0.7019921875 \\
47.1337579617834	0.70765625 \\
47.7707006369427	0.7117578125 \\
48.4076433121019	0.7136328125 \\
49.0445859872611	0.7172265625 \\
49.6815286624204	0.729296875 \\
50.3184713375796	0.7337109375 \\
50.9554140127388	0.736953125 \\
51.5923566878981	0.74078125 \\
52.2292993630573	0.7394140625 \\
52.8662420382166	0.7533984375 \\
53.5031847133758	0.758515625 \\
54.140127388535	0.7633984375 \\
54.7770700636943	0.770234375 \\
55.4140127388535	0.7777734375 \\
56.0509554140127	0.7839453125 \\
56.687898089172	0.793828125 \\
57.3248407643312	0.791015625 \\
57.9617834394904	0.801328125 \\
58.5987261146497	0.8028125 \\
59.2356687898089	0.805234375 \\
59.8726114649682	0.813203125 \\
60.5095541401274	0.8179296875 \\
61.1464968152866	0.826875 \\
61.7834394904459	0.8444921875 \\
62.4203821656051	0.8516015625 \\
63.0573248407643	0.8650390625 \\
63.6942675159236	0.8690625 \\
64.3312101910828	0.8765234375 \\
64.968152866242	0.8809765625 \\
65.6050955414013	0.885859375 \\
66.2420382165605	0.8903515625 \\
66.8789808917197	0.9049609375 \\
67.515923566879	0.918515625 \\
68.1528662420382	0.9232421875 \\
68.7898089171974	0.92640625 \\
69.4267515923567	0.9371484375 \\
70.0636942675159	0.9426171875 \\
70.7006369426752	0.949609375 \\
71.3375796178344	0.9525 \\
71.9745222929936	0.955546875 \\
72.6114649681529	0.959609375 \\
73.2484076433121	0.9621875 \\
73.8853503184713	0.961953125 \\
74.5222929936306	0.9664453125 \\
75.1592356687898	0.9642578125 \\
75.796178343949	0.9662890625 \\
76.4331210191083	0.970859375 \\
77.0700636942675	0.97015625 \\
77.7070063694268	0.975546875 \\
78.343949044586	0.97609375 \\
78.9808917197452	0.9777734375 \\
79.6178343949044	0.979140625 \\
80.2547770700637	0.979375 \\
80.8917197452229	0.98015625 \\
81.5286624203822	0.980078125 \\
82.1656050955414	0.980390625 \\
82.8025477707006	0.9809375 \\
83.4394904458599	0.9821484375 \\
84.0764331210191	0.983828125 \\
84.7133757961783	0.9846875 \\
85.3503184713376	0.9841796875 \\
85.9872611464968	0.9852734375 \\
86.6242038216561	0.9862109375 \\
87.2611464968153	0.9880078125 \\
87.8980891719745	0.987890625 \\
88.5350318471338	0.9881640625 \\
89.171974522293	0.9954296875 \\
89.8089171974522	0.998671875 \\
90.4458598726115	0.999140625 \\
91.0828025477707	0.9997265625 \\
91.7197452229299	1 \\
92.3566878980892	1 \\
92.9936305732484	1 \\
93.6305732484076	1 \\
94.2675159235669	1 \\
94.9044585987261	1 \\
95.5414012738853	1 \\
96.1783439490446	1 \\
96.8152866242038	1 \\
97.4522292993631	1 \\
98.0891719745223	1 \\
98.7261146496815	1 \\
99.3630573248408	1 \\
100	1 \\
};
\path [fill=color7, fill opacity=0.5] (axis cs:0,0.08)
--(axis cs:0,0.08)
--(axis cs:0.636942675159236,0.0795611139660534)
--(axis cs:1.27388535031847,0.0797631187852672)
--(axis cs:1.91082802547771,0.0796097566561732)
--(axis cs:2.54777070063694,0.0794220335958935)
--(axis cs:3.18471337579618,0.08)
--(axis cs:3.82165605095541,0.0796878816561732)
--(axis cs:4.45859872611465,0.0795790085175115)
--(axis cs:5.09554140127389,0.079362960532345)
--(axis cs:5.73248407643312,0.0795790085175115)
--(axis cs:6.36942675159236,0.0795413605479671)
--(axis cs:7.00636942675159,0.0795733050345246)
--(axis cs:7.64331210191083,0.0796016692373926)
--(axis cs:8.28025477707006,0.0796620433587214)
--(axis cs:8.9171974522293,0.0805339940431206)
--(axis cs:9.55414012738853,0.0825070338481093)
--(axis cs:10.1910828025478,0.0851219373740847)
--(axis cs:10.828025477707,0.0866450421314145)
--(axis cs:11.4649681528662,0.0900588229339316)
--(axis cs:12.1019108280255,0.0940079368384537)
--(axis cs:12.7388535031847,0.100554322203047)
--(axis cs:13.3757961783439,0.103270352571749)
--(axis cs:14.0127388535032,0.104544705083276)
--(axis cs:14.6496815286624,0.110238111044365)
--(axis cs:15.2866242038217,0.118866300633224)
--(axis cs:15.9235668789809,0.125279216170622)
--(axis cs:16.5605095541401,0.130827277550503)
--(axis cs:17.1974522292994,0.134145777587272)
--(axis cs:17.8343949044586,0.145829544485598)
--(axis cs:18.4713375796178,0.151971178791751)
--(axis cs:19.1082802547771,0.159365405785153)
--(axis cs:19.7452229299363,0.16319186544449)
--(axis cs:20.3821656050955,0.179508049135373)
--(axis cs:21.0191082802548,0.194200575309102)
--(axis cs:21.656050955414,0.210224179122117)
--(axis cs:22.2929936305732,0.220031608285784)
--(axis cs:22.9299363057325,0.220043394219035)
--(axis cs:23.5668789808917,0.230405231474228)
--(axis cs:24.203821656051,0.248504182467179)
--(axis cs:24.8407643312102,0.252469654607259)
--(axis cs:25.4777070063694,0.262693303341488)
--(axis cs:26.1146496815287,0.278225891303911)
--(axis cs:26.7515923566879,0.297897100769149)
--(axis cs:27.3885350318471,0.319010457631918)
--(axis cs:28.0254777070064,0.337797927269093)
--(axis cs:28.6624203821656,0.362253818912985)
--(axis cs:29.2993630573248,0.376209750079876)
--(axis cs:29.9363057324841,0.396519316103493)
--(axis cs:30.5732484076433,0.411713919207649)
--(axis cs:31.2101910828025,0.425037958987535)
--(axis cs:31.8471337579618,0.442013271676236)
--(axis cs:32.484076433121,0.451778155535613)
--(axis cs:33.1210191082803,0.467614691317098)
--(axis cs:33.7579617834395,0.484418990332161)
--(axis cs:34.3949044585987,0.500832073538871)
--(axis cs:35.031847133758,0.511602407232738)
--(axis cs:35.6687898089172,0.523579503637095)
--(axis cs:36.3057324840764,0.526956668097891)
--(axis cs:36.9426751592357,0.540846592045722)
--(axis cs:37.5796178343949,0.558110597779142)
--(axis cs:38.2165605095541,0.569248487128514)
--(axis cs:38.8535031847134,0.581538276249216)
--(axis cs:39.4904458598726,0.591118949818403)
--(axis cs:40.1273885350318,0.600007211993887)
--(axis cs:40.7643312101911,0.609650991096502)
--(axis cs:41.4012738853503,0.622775952381317)
--(axis cs:42.0382165605096,0.630928234258617)
--(axis cs:42.6751592356688,0.643437565312448)
--(axis cs:43.312101910828,0.648692536618172)
--(axis cs:43.9490445859873,0.648243512190658)
--(axis cs:44.5859872611465,0.66149058508817)
--(axis cs:45.2229299363057,0.671518386481897)
--(axis cs:45.859872611465,0.687380320584379)
--(axis cs:46.4968152866242,0.693220936491424)
--(axis cs:47.1337579617834,0.699152740557864)
--(axis cs:47.7707006369427,0.703314949256707)
--(axis cs:48.4076433121019,0.705646549470476)
--(axis cs:49.0445859872611,0.708813296257441)
--(axis cs:49.6815286624204,0.720957140599416)
--(axis cs:50.3184713375796,0.725831140450341)
--(axis cs:50.9554140127388,0.728770734561356)
--(axis cs:51.5923566878981,0.732611197884631)
--(axis cs:52.2292993630573,0.731481436160613)
--(axis cs:52.8662420382166,0.745209539125192)
--(axis cs:53.5031847133758,0.750036666435277)
--(axis cs:54.140127388535,0.755399943866096)
--(axis cs:54.7770700636943,0.761911059281324)
--(axis cs:55.4140127388535,0.769099596607241)
--(axis cs:56.0509554140127,0.775779848720946)
--(axis cs:56.687898089172,0.785387318164195)
--(axis cs:57.3248407643312,0.782300779252884)
--(axis cs:57.9617834394904,0.792801131391527)
--(axis cs:58.5987261146497,0.794321862580691)
--(axis cs:59.2356687898089,0.796556695354874)
--(axis cs:59.8726114649682,0.804142645699419)
--(axis cs:60.5095541401274,0.809128570346326)
--(axis cs:61.1464968152866,0.817925206269878)
--(axis cs:61.7834394904459,0.835422051128353)
--(axis cs:62.4203821656051,0.842373587810889)
--(axis cs:63.0573248407643,0.855922044443432)
--(axis cs:63.6942675159236,0.860666635596977)
--(axis cs:64.3312101910828,0.86861555155615)
--(axis cs:64.968152866242,0.87298373438027)
--(axis cs:65.6050955414013,0.87753707981003)
--(axis cs:66.2420382165605,0.882177416808761)
--(axis cs:66.8789808917197,0.8965143334091)
--(axis cs:67.515923566879,0.910245832055457)
--(axis cs:68.1528662420382,0.915185149231522)
--(axis cs:68.7898089171974,0.918502180769654)
--(axis cs:69.4267515923567,0.929656511917953)
--(axis cs:70.0636942675159,0.935622537290063)
--(axis cs:70.7006369426752,0.942928258145323)
--(axis cs:71.3375796178344,0.946356381745456)
--(axis cs:71.9745222929936,0.949788778117977)
--(axis cs:72.6114649681529,0.954631509900457)
--(axis cs:73.2484076433121,0.957092150044279)
--(axis cs:73.8853503184713,0.956920747681856)
--(axis cs:74.5222929936306,0.96194197669751)
--(axis cs:75.1592356687898,0.959666134815149)
--(axis cs:75.796178343949,0.962353832929733)
--(axis cs:76.4331210191083,0.96719482503201)
--(axis cs:77.0700636942675,0.966623458388608)
--(axis cs:77.7070063694268,0.972702505745035)
--(axis cs:78.343949044586,0.973235375167584)
--(axis cs:78.9808917197452,0.975243988630819)
--(axis cs:79.6178343949044,0.97750780052664)
--(axis cs:80.2547770700637,0.978152832909103)
--(axis cs:80.8917197452229,0.979205667854788)
--(axis cs:81.5286624203822,0.97885267038023)
--(axis cs:82.1656050955414,0.979297567314183)
--(axis cs:82.8025477707006,0.979616430736478)
--(axis cs:83.4394904458599,0.980213132132345)
--(axis cs:84.0764331210191,0.981369324658458)
--(axis cs:84.7133757961783,0.982039952790679)
--(axis cs:85.3503184713376,0.981638542442481)
--(axis cs:85.9872611464968,0.98251954098967)
--(axis cs:86.6242038216561,0.983318952931702)
--(axis cs:87.2611464968153,0.984945452985288)
--(axis cs:87.8980891719745,0.984835938904902)
--(axis cs:88.5350318471338,0.985092180609493)
--(axis cs:89.171974522293,0.992805459681053)
--(axis cs:89.8089171974522,0.997115681979445)
--(axis cs:90.4458598726115,0.997873208266365)
--(axis cs:91.0828025477707,0.999000782885928)
--(axis cs:91.7197452229299,1)
--(axis cs:92.3566878980892,1)
--(axis cs:92.9936305732484,1)
--(axis cs:93.6305732484076,1)
--(axis cs:94.2675159235669,1)
--(axis cs:94.9044585987261,1)
--(axis cs:95.5414012738853,1)
--(axis cs:96.1783439490446,1)
--(axis cs:96.8152866242038,1)
--(axis cs:97.4522292993631,1)
--(axis cs:98.0891719745223,1)
--(axis cs:98.7261146496815,1)
--(axis cs:99.3630573248408,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.3630573248408,1)
--(axis cs:98.7261146496815,1)
--(axis cs:98.0891719745223,1)
--(axis cs:97.4522292993631,1)
--(axis cs:96.8152866242038,1)
--(axis cs:96.1783439490446,1)
--(axis cs:95.5414012738853,1)
--(axis cs:94.9044585987261,1)
--(axis cs:94.2675159235669,1)
--(axis cs:93.6305732484076,1)
--(axis cs:92.9936305732484,1)
--(axis cs:92.3566878980892,1)
--(axis cs:91.7197452229299,1)
--(axis cs:91.0828025477707,1.00045234211407)
--(axis cs:90.4458598726115,1.00040804173363)
--(axis cs:89.8089171974522,1.00022806802056)
--(axis cs:89.171974522293,0.998053915318947)
--(axis cs:88.5350318471338,0.991235944390507)
--(axis cs:87.8980891719745,0.990945311095098)
--(axis cs:87.2611464968153,0.991070172014712)
--(axis cs:86.6242038216561,0.989102922068298)
--(axis cs:85.9872611464968,0.98802733401033)
--(axis cs:85.3503184713376,0.986720832557519)
--(axis cs:84.7133757961783,0.987335047209322)
--(axis cs:84.0764331210191,0.986286925341542)
--(axis cs:83.4394904458599,0.984083742867655)
--(axis cs:82.8025477707006,0.982258569263522)
--(axis cs:82.1656050955414,0.981483682685817)
--(axis cs:81.5286624203822,0.98130357961977)
--(axis cs:80.8917197452229,0.981106832145211)
--(axis cs:80.2547770700637,0.980597167090897)
--(axis cs:79.6178343949044,0.98077344947336)
--(axis cs:78.9808917197452,0.980302886369181)
--(axis cs:78.343949044586,0.978952124832416)
--(axis cs:77.7070063694268,0.978391244254965)
--(axis cs:77.0700636942675,0.973689041611392)
--(axis cs:76.4331210191083,0.97452392496799)
--(axis cs:75.796178343949,0.970224292070267)
--(axis cs:75.1592356687898,0.968849490184851)
--(axis cs:74.5222929936306,0.97094864830249)
--(axis cs:73.8853503184713,0.966985502318144)
--(axis cs:73.2484076433121,0.967282849955721)
--(axis cs:72.6114649681529,0.964587240099543)
--(axis cs:71.9745222929936,0.961304971882023)
--(axis cs:71.3375796178344,0.958643618254544)
--(axis cs:70.7006369426752,0.956290491854677)
--(axis cs:70.0636942675159,0.949611837709937)
--(axis cs:69.4267515923567,0.944640363082047)
--(axis cs:68.7898089171974,0.934310319230346)
--(axis cs:68.1528662420382,0.931299225768478)
--(axis cs:67.515923566879,0.926785417944543)
--(axis cs:66.8789808917197,0.9134075415909)
--(axis cs:66.2420382165605,0.898525708191239)
--(axis cs:65.6050955414013,0.89418167018997)
--(axis cs:64.968152866242,0.88896939061973)
--(axis cs:64.3312101910828,0.88443132344385)
--(axis cs:63.6942675159236,0.877458364403023)
--(axis cs:63.0573248407643,0.874156080556568)
--(axis cs:62.4203821656051,0.860829537189111)
--(axis cs:61.7834394904459,0.853562323871647)
--(axis cs:61.1464968152866,0.835824793730122)
--(axis cs:60.5095541401274,0.826730804653674)
--(axis cs:59.8726114649682,0.822263604300581)
--(axis cs:59.2356687898089,0.813912054645126)
--(axis cs:58.5987261146497,0.811303137419309)
--(axis cs:57.9617834394904,0.809855118608472)
--(axis cs:57.3248407643312,0.799730470747116)
--(axis cs:56.687898089172,0.802268931835805)
--(axis cs:56.0509554140127,0.792110776279054)
--(axis cs:55.4140127388535,0.786447278392759)
--(axis cs:54.7770700636943,0.778557690718676)
--(axis cs:54.140127388535,0.771396931133904)
--(axis cs:53.5031847133758,0.766994583564723)
--(axis cs:52.8662420382166,0.761587335874809)
--(axis cs:52.2292993630573,0.747346688839387)
--(axis cs:51.5923566878981,0.748951302115369)
--(axis cs:50.9554140127388,0.745135515438644)
--(axis cs:50.3184713375796,0.741590734549659)
--(axis cs:49.6815286624204,0.737636609400584)
--(axis cs:49.0445859872611,0.725639828742559)
--(axis cs:48.4076433121019,0.721619075529524)
--(axis cs:47.7707006369427,0.720200675743293)
--(axis cs:47.1337579617834,0.716159759442136)
--(axis cs:46.4968152866242,0.710763438508576)
--(axis cs:45.859872611465,0.704963429415621)
--(axis cs:45.2229299363057,0.690122238518103)
--(axis cs:44.5859872611465,0.67968128991183)
--(axis cs:43.9490445859873,0.667459612809342)
--(axis cs:43.312101910828,0.668338713381828)
--(axis cs:42.6751592356688,0.664062434687552)
--(axis cs:42.0382165605096,0.651806140741383)
--(axis cs:41.4012738853503,0.643786547618683)
--(axis cs:40.7643312101911,0.630583383903498)
--(axis cs:40.1273885350318,0.620774038006113)
--(axis cs:39.4904458598726,0.612631050181597)
--(axis cs:38.8535031847134,0.603461723750784)
--(axis cs:38.2165605095541,0.591532762871486)
--(axis cs:37.5796178343949,0.581108152220858)
--(axis cs:36.9426751592357,0.563450282954278)
--(axis cs:36.3057324840764,0.548980831902109)
--(axis cs:35.6687898089172,0.546186121362905)
--(axis cs:35.031847133758,0.534491342767262)
--(axis cs:34.3949044585987,0.523699176461129)
--(axis cs:33.7579617834395,0.507456009667839)
--(axis cs:33.1210191082803,0.490900933682902)
--(axis cs:32.484076433121,0.475096844464387)
--(axis cs:31.8471337579618,0.465017978323764)
--(axis cs:31.2101910828025,0.448243291012465)
--(axis cs:30.5732484076433,0.435317330792351)
--(axis cs:29.9363057324841,0.420590058896508)
--(axis cs:29.2993630573248,0.400430874920124)
--(axis cs:28.6624203821656,0.386574306087015)
--(axis cs:28.0254777070064,0.361889572730907)
--(axis cs:27.3885350318471,0.343567667368082)
--(axis cs:26.7515923566879,0.321790399230851)
--(axis cs:26.1146496815287,0.301852233696089)
--(axis cs:25.4777070063694,0.285431696658512)
--(axis cs:24.8407643312102,0.275186595392741)
--(axis cs:24.203821656051,0.271339567532822)
--(axis cs:23.5668789808917,0.252563518525772)
--(axis cs:22.9299363057325,0.241675355780965)
--(axis cs:22.2929936305732,0.241765266714216)
--(axis cs:21.656050955414,0.231572695877883)
--(axis cs:21.0191082802548,0.214393174690898)
--(axis cs:20.3821656050955,0.199163825864627)
--(axis cs:19.7452229299363,0.18266750955551)
--(axis cs:19.1082802547771,0.178525219214847)
--(axis cs:18.4713375796178,0.170606946208249)
--(axis cs:17.8343949044586,0.164326705514402)
--(axis cs:17.1974522292994,0.151401097412728)
--(axis cs:16.5605095541401,0.147688347449497)
--(axis cs:15.9235668789809,0.141752033829378)
--(axis cs:15.2866242038217,0.134493074366776)
--(axis cs:14.6496815286624,0.124527513955635)
--(axis cs:14.0127388535032,0.118111544916724)
--(axis cs:13.3757961783439,0.116495272428251)
--(axis cs:12.7388535031847,0.112961302796953)
--(axis cs:12.1019108280255,0.105367063161546)
--(axis cs:11.4649681528662,0.100097427066068)
--(axis cs:10.828025477707,0.0954643328685855)
--(axis cs:10.1910828025478,0.0932374376259153)
--(axis cs:9.55414012738853,0.0890554661518907)
--(axis cs:8.9171974522293,0.0851691309568794)
--(axis cs:8.28025477707006,0.0829160816412786)
--(axis cs:7.64331210191083,0.0826639557626074)
--(axis cs:7.00636942675159,0.0825360699654754)
--(axis cs:6.36942675159236,0.0819430144520329)
--(axis cs:5.73248407643312,0.0808116164824885)
--(axis cs:5.09554140127389,0.081105789467655)
--(axis cs:4.45859872611465,0.0808116164824885)
--(axis cs:3.82165605095541,0.0804683683438268)
--(axis cs:3.18471337579618,0.08)
--(axis cs:2.54777070063694,0.0806560914041064)
--(axis cs:1.91082802547771,0.0803902433438268)
--(axis cs:1.27388535031847,0.0803150062147328)
--(axis cs:0.636942675159236,0.0805170110339466)
--(axis cs:0,0.08)
--cycle;


==> img/mnist/mnist_rate_distortion_afw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.915308913197368
0.636942675159236 0.91498578858329
1.27388535031847 0.914803649657988
1.91082802547771 0.91429841532663
2.54777070063694 0.913349317791872
3.18471337579618 0.911782277775346
3.82165605095541 0.90999083981791
4.45859872611465 0.906729748411453
5.09554140127389 0.903434916795813
5.73248407643312 0.900417812841479
6.36942675159236 0.894694215945201
7.00636942675159 0.889387569336686
7.64331210191083 0.881135048517026
8.28025477707006 0.870597072388046
8.9171974522293 0.862170889591798
9.55414012738853 0.85230350275524
10.1910828025478 0.840676349768182
10.828025477707 0.828587219595211
11.4649681528662 0.807895362398122
12.1019108280255 0.789963478374993
12.7388535031847 0.767780665192404
13.3757961783439 0.749061008774443
14.0127388535032 0.730703182289144
14.6496815286624 0.713336920237052
15.2866242038217 0.696164538563462
15.9235668789809 0.683129127197899
16.5605095541401 0.658982684985967
17.1974522292994 0.63746536101331
17.8343949044586 0.62156630456564
18.4713375796178 0.602626420897432
19.1082802547771 0.581555189123901
19.7452229299363 0.564984035582747
20.3821656050955 0.547818349190056
21.0191082802548 0.529938468687469
21.656050955414 0.511734374875086
22.2929936305732 0.493588492475683
22.9299363057325 0.473130440205568
23.5668789808917 0.465168025311723
24.203821656051 0.446810163522896
24.8407643312102 0.429586995257996
25.4777070063694 0.415208179622859
26.1146496815287 0.409691939741315
26.7515923566879 0.389581539589071
27.3885350318471 0.37617235991529
28.0254777070064 0.363623746802114
28.6624203821656 0.349309691839958
29.2993630573248 0.340808440262088
29.9363057324841 0.326540367218339
30.5732484076433 0.310484055424059
31.2101910828025 0.297559144405648
31.8471337579618 0.288554245882148
32.484076433121 0.276814407421629
33.1210191082803 0.260441710492412
33.7579617834395 0.239503364487885
34.3949044585987 0.223892736624241
35.031847133758 0.208092435071621
35.6687898089172 0.199500241871114
36.3057324840764 0.199177971198602
36.9426751592357 0.192788027510274
37.5796178343949 0.182338008433853
38.2165605095541 0.173344060034282
38.8535031847134 0.167367156744529
39.4904458598726 0.163300909428057
40.1273885350318 0.155602260212242
40.7643312101911 0.147643365041569
41.4012738853503 0.141839284734661
42.0382165605096 0.140232510635381
42.6751592356688 0.131736061524647
43.312101910828 0.1309209059506
43.9490445859873 0.127560166964806
44.5859872611465 0.123653554806991
45.2229299363057 0.126107670677563
45.859872611465 0.123102828502457
46.4968152866242 0.117748405108897
47.1337579617834 0.113989861230556
47.7707006369427 0.111677241985415
48.4076433121019 0.110788570758626
49.0445859872611 0.105613527766562
49.6815286624204 0.101314956081109
50.3184713375796 0.102023665100053
50.9554140127388 0.0999990273438885
51.5923566878981 0.100727519283364
52.2292993630573 0.0949924396523501
52.8662420382166 0.0927452091517416
53.5031847133758 0.0922377672049942
54.140127388535 0.0851084906651881
54.7770700636943 0.0837469956894334
55.4140127388535 0.078427087780479
56.0509554140127 0.0797018606169486
56.687898089172 0.0793509296562956
57.3248407643312 0.0757756765212982
57.9617834394904 0.0752050229689933
58.5987261146497 0.0716852389397595
59.2356687898089 0.0628523041503133
59.8726114649682 0.0615398484853986
60.5095541401274 0.0611553090224075
61.1464968152866 0.0619647382889473
61.7834394904459 0.055138935790715
62.4203821656051 0.0502990004399896
63.0573248407643 0.0470753443205705
63.6942675159236 0.0416126549717548
64.3312101910828 0.0394816218915754
64.968152866242 0.0393197855195147
65.6050955414013 0.0387365379024327
66.2420382165605 0.0390844600207929
66.8789808917197 0.0396572335913621
67.515923566879 0.0377639616260559
68.1528662420382 0.0377280032498968
68.7898089171974 0.0395276733375752
69.4267515923567 0.0394997425241782
70.0636942675159 0.0427467601134725
70.7006369426752 0.0394899606114757
71.3375796178344 0.0374553818497457
71.9745222929936 0.0358056666121862
72.6114649681529 0.0334067461780986
73.2484076433121 0.0331948279444905
73.8853503184713 0.032380459395142
74.5222929936306 0.0328791390081746
75.1592356687898 0.0332096249877149
75.796178343949 0.0342253369041694
76.4331210191083 0.0358222094300706
77.0700636942675 0.0361075645645014
77.7070063694268 0.034004829120647
78.343949044586 0.0353470029449728
78.9808917197452 0.0342256855899006
79.6178343949044 0.0339347103397715
80.2547770700637 0.0326905883020687
80.8917197452229 0.0306129866252253
81.5286624203822 0.0296275314839503
82.1656050955414 0.0280038943563311
82.8025477707006 0.0264179706975986
83.4394904458599 0.0276883253888662
84.0764331210191 0.0260155800190638
84.7133757961783 0.0264116047519734
85.3503184713376 0.0213916225164454
85.9872611464968 0.02041544202656
86.6242038216561 0.0166938163055948
87.2611464968153 0.0128769057175062
87.8980891719745 0.0123734042796175
88.5350318471338 0.0126212907249015
89.171974522293 0.00969877341185198
89.8089171974522 0.00876710197577609
90.4458598726115 0.00696005512227369
91.0828025477707 0.00507000357963955
91.7197452229299 0.00696469820454721
92.3566878980892 0.00190246118680842
92.9936305732484 0.000988494555994952
93.6305732484076 0.000251121589025419
94.2675159235669 0.000195274382585146
94.9044585987261 0.000114736001178383
95.5414012738853 9.5787042428237e-05
96.1783439490446 6.30034600218193e-05
96.8152866242038 2.95668716804437e-05
97.4522292993631 1.87533630696501e-05
98.0891719745223 6.36457348043851e-06
98.7261146496815 7.27922142111315e-06
99.3630573248408 3.3665755955381e-06
100 9.06140229517405e-11
};
\path [fill=color3, fill opacity=0.25] 
(axis cs:0,0.915962856066278)
--(axis cs:0,0.914654970328459)
--(axis cs:0.636942675159236,0.914283158835167)
--(axis cs:1.27388535031847,0.914087640524544)
--(axis cs:1.91082802547771,0.913430924960129)
--(axis cs:2.54777070063694,0.912256293648111)
--(axis cs:3.18471337579618,0.910473707980546)
--(axis cs:3.82165605095541,0.908483094041475)
--(axis cs:4.45859872611465,0.904802791038485)
--(axis cs:5.09554140127389,0.901113661500498)
--(axis cs:5.73248407643312,0.897886537667884)
--(axis cs:6.36942675159236,0.891595945371538)
--(axis cs:7.00636942675159,0.885878942636869)
--(axis cs:7.64331210191083,0.87709698716482)
--(axis cs:8.28025477707006,0.865846406006198)
--(axis cs:8.9171974522293,0.857139386622702)
--(axis cs:9.55414012738853,0.846801216676324)
--(axis cs:10.1910828025478,0.834609386948895)
--(axis cs:10.828025477707,0.822230101187516)
--(axis cs:11.4649681528662,0.801092589129152)
--(axis cs:12.1019108280255,0.782811738216031)
--(axis cs:12.7388535031847,0.760416063034622)
--(axis cs:13.3757961783439,0.741206803270781)
--(axis cs:14.0127388535032,0.722636994380957)
--(axis cs:14.6496815286624,0.705328397046499)
--(axis cs:15.2866242038217,0.688158177183164)
--(axis cs:15.9235668789809,0.674995355974663)
--(axis cs:16.5605095541401,0.650715356903853)
--(axis cs:17.1974522292994,0.62895599186688)
--(axis cs:17.8343949044586,0.612910020211655)
--(axis cs:18.4713375796178,0.594058173926197)
--(axis cs:19.1082802547771,0.572950136571611)
--(axis cs:19.7452229299363,0.556443908493746)
--(axis cs:20.3821656050955,0.539425043525434)
--(axis cs:21.0191082802548,0.521639580357484)
--(axis cs:21.656050955414,0.503355756809136)
--(axis cs:22.2929936305732,0.485421525422749)
--(axis cs:22.9299363057325,0.464921456049647)
--(axis cs:23.5668789808917,0.456905893899011)
--(axis cs:24.203821656051,0.438668149888967)
--(axis cs:24.8407643312102,0.421741411154246)
--(axis cs:25.4777070063694,0.407433021649569)
--(axis cs:26.1146496815287,0.401974215842691)
--(axis cs:26.7515923566879,0.381907880427448)
--(axis cs:27.3885350318471,0.368582455665489)
--(axis cs:28.0254777070064,0.35608170597633)
--(axis cs:28.6624203821656,0.341796851561976)
--(axis cs:29.2993630573248,0.333496038122755)
--(axis cs:29.9363057324841,0.31931917348407)
--(axis cs:30.5732484076433,0.303284805848884)
--(axis cs:31.2101910828025,0.290365955495132)
--(axis cs:31.8471337579618,0.281462862894929)
--(axis cs:32.484076433121,0.269428924767399)
--(axis cs:33.1210191082803,0.253110279428647)
--(axis cs:33.7579617834395,0.232188533970148)
--(axis cs:34.3949044585987,0.216685875437488)
--(axis cs:35.031847133758,0.201197332384349)
--(axis cs:35.6687898089172,0.192781042886167)
--(axis cs:36.3057324840764,0.192526533364479)
--(axis cs:36.9426751592357,0.186388885057522)
--(axis cs:37.5796178343949,0.176103783526238)
--(axis cs:38.2165605095541,0.167329284862912)
--(axis cs:38.8535031847134,0.161445641477199)
--(axis cs:39.4904458598726,0.157428622417217)
--(axis cs:40.1273885350318,0.150019971281917)
--(axis cs:40.7643312101911,0.142216754052287)
--(axis cs:41.4012738853503,0.136601148086713)
--(axis cs:42.0382165605096,0.134866913374383)
--(axis cs:42.6751592356688,0.126568410488518)
--(axis cs:43.312101910828,0.125673159955329)
--(axis cs:43.9490445859873,0.122592857330917)
--(axis cs:44.5859872611465,0.118849449073965)
--(axis cs:45.2229299363057,0.121121519854608)
--(axis cs:45.859872611465,0.118247195560217)
--(axis cs:46.4968152866242,0.11287470134053)
--(axis cs:47.1337579617834,0.108913165370472)
--(axis cs:47.7707006369427,0.106831128120115)
--(axis cs:48.4076433121019,0.105790324544332)
--(axis cs:49.0445859872611,0.100746786374478)
--(axis cs:49.6815286624204,0.0966117334919571)
--(axis cs:50.3184713375796,0.097474203452653)
--(axis cs:50.9554140127388,0.0953494543237822)
--(axis cs:51.5923566878981,0.0959879980044644)
--(axis cs:52.2292993630573,0.0902978002923303)
--(axis cs:52.8662420382166,0.0881144078293979)
--(axis cs:53.5031847133758,0.0874623943979949)
--(axis cs:54.140127388535,0.0803364477074269)
--(axis cs:54.7770700636943,0.0788695777581021)
--(axis cs:55.4140127388535,0.0735147618697633)
--(axis cs:56.0509554140127,0.0748851854662789)
--(axis cs:56.687898089172,0.0745169375011221)
--(axis cs:57.3248407643312,0.071104479662638)
--(axis cs:57.9617834394904,0.0704820571502817)
--(axis cs:58.5987261146497,0.0669889407971262)
--(axis cs:59.2356687898089,0.0585569928980944)
--(axis cs:59.8726114649682,0.0572470323119881)
--(axis cs:60.5095541401274,0.0569892238049506)
--(axis cs:61.1464968152866,0.0577879922073184)
--(axis cs:61.7834394904459,0.0512134085294839)
--(axis cs:62.4203821656051,0.0466112802679885)
--(axis cs:63.0573248407643,0.0436501527120883)
--(axis cs:63.6942675159236,0.0385250896034701)
--(axis cs:64.3312101910828,0.036492593545603)
--(axis cs:64.968152866242,0.0364839185978082)
--(axis cs:65.6050955414013,0.0359613727468918)
--(axis cs:66.2420382165605,0.0362052023345376)
--(axis cs:66.8789808917197,0.0367366516960766)
--(axis cs:67.515923566879,0.0350472848801591)
--(axis cs:68.1528662420382,0.0350319704476256)
--(axis cs:68.7898089171974,0.0368828395381013)
--(axis cs:69.4267515923567,0.0368030155373932)
--(axis cs:70.0636942675159,0.0398247265410934)
--(axis cs:70.7006369426752,0.0367411021605245)
--(axis cs:71.3375796178344,0.034803550525222)
--(axis cs:71.9745222929936,0.0331988405315916)
--(axis cs:72.6114649681529,0.0310653486877943)
--(axis cs:73.2484076433121,0.0310858652568207)
--(axis cs:73.8853503184713,0.0304393404965827)
--(axis cs:74.5222929936306,0.031007649038833)
--(axis cs:75.1592356687898,0.0313912537715017)
--(axis cs:75.796178343949,0.0323680204554549)
--(axis cs:76.4331210191083,0.0339531961576537)
--(axis cs:77.0700636942675,0.03425748697782)
--(axis cs:77.7070063694268,0.0320204860842728)
--(axis cs:78.343949044586,0.0332484682592898)
--(axis cs:78.9808917197452,0.0323035185151428)
--(axis cs:79.6178343949044,0.0319689105459692)
--(axis cs:80.2547770700637,0.0308564479458649)
--(axis cs:80.8917197452229,0.0287535899759082)
--(axis cs:81.5286624203822,0.0278096436494208)
--(axis cs:82.1656050955414,0.0262248204316652)
--(axis cs:82.8025477707006,0.0245133799419482)
--(axis cs:83.4394904458599,0.0258154339405192)
--(axis cs:84.0764331210191,0.0242649198781676)
--(axis cs:84.7133757961783,0.0244796527482878)
--(axis cs:85.3503184713376,0.0198492448867634)
--(axis cs:85.9872611464968,0.018759611331952)
--(axis cs:86.6242038216561,0.0152787888286266)
--(axis cs:87.2611464968153,0.0113468268075743)
--(axis cs:87.8980891719745,0.0110146644471982)
--(axis cs:88.5350318471338,0.0113305803536859)
--(axis cs:89.171974522293,0.00828942240036821)
--(axis cs:89.8089171974522,0.00743729412141854)
--(axis cs:90.4458598726115,0.00563444189845453)
--(axis cs:91.0828025477707,0.00387020980536392)
--(axis cs:91.7197452229299,0.00569052586892747)
--(axis cs:92.3566878980892,0.00136312043439152)
--(axis cs:92.9936305732484,0.000640345245243148)
--(axis cs:93.6305732484076,0.000145513728010467)
--(axis cs:94.2675159235669,0.00012748986101016)
--(axis cs:94.9044585987261,6.43759440300245e-05)
--(axis cs:95.5414012738853,5.62242169536731e-05)
--(axis cs:96.1783439490446,3.00745939604038e-05)
--(axis cs:96.8152866242038,1.79082837451201e-05)
--(axis cs:97.4522292993631,1.13741535329673e-05)
--(axis cs:98.0891719745223,4.06020099247534e-06)
--(axis cs:98.7261146496815,4.22082662474201e-06)
--(axis cs:99.3630573248408,3.14501508737969e-06)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:99.3630573248408,3.58813610369652e-06)
--(axis cs:98.7261146496815,1.03376162174843e-05)
--(axis cs:98.0891719745223,8.66894596840168e-06)
--(axis cs:97.4522292993631,2.61325726063329e-05)
--(axis cs:96.8152866242038,4.12254596157673e-05)
--(axis cs:96.1783439490446,9.59323260832348e-05)
--(axis cs:95.5414012738853,0.000135349867902801)
--(axis cs:94.9044585987261,0.000165096058326741)
--(axis cs:94.2675159235669,0.000263058904160131)
--(axis cs:93.6305732484076,0.000356729450040371)
--(axis cs:92.9936305732484,0.00133664386674676)
--(axis cs:92.3566878980892,0.00244180193922533)
--(axis cs:91.7197452229299,0.00823887054016695)
--(axis cs:91.0828025477707,0.00626979735391519)
--(axis cs:90.4458598726115,0.00828566834609285)
--(axis cs:89.8089171974522,0.0100969098301336)
--(axis cs:89.171974522293,0.0111081244233357)
--(axis cs:88.5350318471338,0.0139120010961171)
--(axis cs:87.8980891719745,0.0137321441120367)
--(axis cs:87.2611464968153,0.014406984627438)
--(axis cs:86.6242038216561,0.018108843782563)
--(axis cs:85.9872611464968,0.022071272721168)
--(axis cs:85.3503184713376,0.0229340001461274)
--(axis cs:84.7133757961783,0.0283435567556589)
--(axis cs:84.0764331210191,0.02776624015996)
--(axis cs:83.4394904458599,0.0295612168372132)
--(axis cs:82.8025477707006,0.0283225614532489)
--(axis cs:82.1656050955414,0.029782968280997)
--(axis cs:81.5286624203822,0.0314454193184798)
--(axis cs:80.8917197452229,0.0324723832745424)
--(axis cs:80.2547770700637,0.0345247286582725)
--(axis cs:79.6178343949044,0.0359005101335738)
--(axis cs:78.9808917197452,0.0361478526646583)
--(axis cs:78.343949044586,0.0374455376306558)
--(axis cs:77.7070063694268,0.0359891721570213)
--(axis cs:77.0700636942675,0.0379576421511828)
--(axis cs:76.4331210191083,0.0376912227024875)
--(axis cs:75.796178343949,0.0360826533528839)
--(axis cs:75.1592356687898,0.0350279962039281)
--(axis cs:74.5222929936306,0.0347506289775162)
--(axis cs:73.8853503184713,0.0343215782937012)
--(axis cs:73.2484076433121,0.0353037906321602)
--(axis cs:72.6114649681529,0.0357481436684028)
--(axis cs:71.9745222929936,0.0384124926927808)
--(axis cs:71.3375796178344,0.0401072131742694)
--(axis cs:70.7006369426752,0.0422388190624268)
--(axis cs:70.0636942675159,0.0456687936858516)
--(axis cs:69.4267515923567,0.0421964695109633)
--(axis cs:68.7898089171974,0.0421725071370491)
--(axis cs:68.1528662420382,0.0404240360521681)
--(axis cs:67.515923566879,0.0404806383719527)
--(axis cs:66.8789808917197,0.0425778154866476)
--(axis cs:66.2420382165605,0.0419637177070481)
--(axis cs:65.6050955414013,0.0415117030579737)
--(axis cs:64.968152866242,0.0421556524412211)
--(axis cs:64.3312101910828,0.0424706502375479)
--(axis cs:63.6942675159236,0.0447002203400395)
--(axis cs:63.0573248407643,0.0505005359290527)
--(axis cs:62.4203821656051,0.0539867206119906)
--(axis cs:61.7834394904459,0.059064463051946)
--(axis cs:61.1464968152866,0.0661414843705762)
--(axis cs:60.5095541401274,0.0653213942398645)
--(axis cs:59.8726114649682,0.0658326646588091)
--(axis cs:59.2356687898089,0.0671476154025323)
--(axis cs:58.5987261146497,0.0763815370823928)
--(axis cs:57.9617834394904,0.0799279887877048)
--(axis cs:57.3248407643312,0.0804468733799584)
--(axis cs:56.687898089172,0.0841849218114691)
--(axis cs:56.0509554140127,0.0845185357676184)
--(axis cs:55.4140127388535,0.0833394136911946)
--(axis cs:54.7770700636943,0.0886244136207648)
--(axis cs:54.140127388535,0.0898805336229493)
--(axis cs:53.5031847133758,0.0970131400119934)
--(axis cs:52.8662420382166,0.0973760104740854)
--(axis cs:52.2292993630573,0.0996870790123699)
--(axis cs:51.5923566878981,0.105467040562264)
--(axis cs:50.9554140127388,0.104648600363995)
--(axis cs:50.3184713375796,0.106573126747452)
--(axis cs:49.6815286624204,0.10601817867026)
--(axis cs:49.0445859872611,0.110480269158645)
--(axis cs:48.4076433121019,0.11578681697292)
--(axis cs:47.7707006369427,0.116523355850715)
--(axis cs:47.1337579617834,0.119066557090639)
--(axis cs:46.4968152866242,0.122622108877264)
--(axis cs:45.859872611465,0.127958461444698)
--(axis cs:45.2229299363057,0.131093821500518)
--(axis cs:44.5859872611465,0.128457660540016)
--(axis cs:43.9490445859873,0.132527476598694)
--(axis cs:43.312101910828,0.13616865194587)
--(axis cs:42.6751592356688,0.136903712560775)
--(axis cs:42.0382165605096,0.145598107896378)
--(axis cs:41.4012738853503,0.14707742138261)
--(axis cs:40.7643312101911,0.15306997603085)
--(axis cs:40.1273885350318,0.161184549142568)
--(axis cs:39.4904458598726,0.169173196438896)
--(axis cs:38.8535031847134,0.173288672011859)
--(axis cs:38.2165605095541,0.179358835205653)
--(axis cs:37.5796178343949,0.188572233341467)
--(axis cs:36.9426751592357,0.199187169963026)
--(axis cs:36.3057324840764,0.205829409032726)
--(axis cs:35.6687898089172,0.206219440856061)
--(axis cs:35.031847133758,0.214987537758892)
--(axis cs:34.3949044585987,0.231099597810995)
--(axis cs:33.7579617834395,0.246818195005623)
--(axis cs:33.1210191082803,0.267773141556178)
--(axis cs:32.484076433121,0.28419989007586)
--(axis cs:31.8471337579618,0.295645628869366)
--(axis cs:31.2101910828025,0.304752333316163)
--(axis cs:30.5732484076433,0.317683304999235)
--(axis cs:29.9363057324841,0.333761560952609)
--(axis cs:29.2993630573248,0.34812084240142)
--(axis cs:28.6624203821656,0.35682253211794)
--(axis cs:28.0254777070064,0.371165787627898)
--(axis cs:27.3885350318471,0.383762264165091)
--(axis cs:26.7515923566879,0.397255198750694)
--(axis cs:26.1146496815287,0.417409663639939)
--(axis cs:25.4777070063694,0.42298333759615)
--(axis cs:24.8407643312102,0.437432579361746)
--(axis cs:24.203821656051,0.454952177156825)
--(axis cs:23.5668789808917,0.473430156724435)
--(axis cs:22.9299363057325,0.48133942436149)
--(axis cs:22.2929936305732,0.501755459528617)
--(axis cs:21.656050955414,0.520112992941037)
--(axis cs:21.0191082802548,0.538237357017454)
--(axis cs:20.3821656050955,0.556211654854679)
--(axis cs:19.7452229299363,0.573524162671748)
--(axis cs:19.1082802547771,0.590160241676191)
--(axis cs:18.4713375796178,0.611194667868666)
--(axis cs:17.8343949044586,0.630222588919626)
--(axis cs:17.1974522292994,0.64597473015974)
--(axis cs:16.5605095541401,0.667250013068082)
--(axis cs:15.9235668789809,0.691262898421135)
--(axis cs:15.2866242038217,0.704170899943759)
--(axis cs:14.6496815286624,0.721345443427606)
--(axis cs:14.0127388535032,0.738769370197331)
--(axis cs:13.3757961783439,0.756915214278104)
--(axis cs:12.7388535031847,0.775145267350186)
--(axis cs:12.1019108280255,0.797115218533956)
--(axis cs:11.4649681528662,0.814698135667091)
--(axis cs:10.828025477707,0.834944338002905)
--(axis cs:10.1910828025478,0.84674331258747)
--(axis cs:9.55414012738853,0.857805788834155)
--(axis cs:8.9171974522293,0.867202392560895)
--(axis cs:8.28025477707006,0.875347738769893)
--(axis cs:7.64331210191083,0.885173109869232)
--(axis cs:7.00636942675159,0.892896196036503)
--(axis cs:6.36942675159236,0.897792486518864)
--(axis cs:5.73248407643312,0.902949088015073)
--(axis cs:5.09554140127389,0.905756172091129)
--(axis cs:4.45859872611465,0.908656705784422)
--(axis cs:3.82165605095541,0.911498585594345)
--(axis cs:3.18471337579618,0.913090847570147)
--(axis cs:2.54777070063694,0.914442341935632)
--(axis cs:1.91082802547771,0.91516590569313)
--(axis cs:1.27388535031847,0.915519658791432)
--(axis cs:0.636942675159236,0.915688418331412)
--(axis cs:0,0.915962856066278)
--cycle;


==> img/mnist/mnist_rate_distortion_afw_order.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.915449607248884
0.636942675159236 0.915176242744783
1.27388535031847 0.914682190249441
1.91082802547771 0.913772084489465
2.54777070063694 0.912173861322226
3.18471337579618 0.910990953030996
3.82165605095541 0.9074313430232
4.45859872611465 0.905204732693965
5.09554140127389 0.901777107832022
5.73248407643312 0.895493241799995
6.36942675159236 0.88805815255444
7.00636942675159 0.877421235116199
7.64331210191083 0.864793919131625
8.28025477707006 0.852589611630538
8.9171974522293 0.834678023834713
9.55414012738853 0.819809553235536
10.1910828025478 0.80509034646675
10.828025477707 0.790608705825871
11.4649681528662 0.772265400879551
12.1019108280255 0.75434909294825
12.7388535031847 0.734012602339499
13.3757961783439 0.718511458622525
14.0127388535032 0.703755589096108
14.6496815286624 0.690141361809801
15.2866242038217 0.673056019884534
15.9235668789809 0.659813078345032
16.5605095541401 0.649995894150343
17.1974522292994 0.637939739092253
17.8343949044586 0.621604246696224
18.4713375796178 0.60646905751375
19.1082802547771 0.593761361292563
19.7452229299363 0.580051149979408
20.3821656050955 0.563744657270145
21.0191082802548 0.548838441655971
21.656050955414 0.535300515475683
22.2929936305732 0.520726968953386
22.9299363057325 0.507369204768911
23.5668789808917 0.492367494242499
24.203821656051 0.481063198219345
24.8407643312102 0.47168433748564
25.4777070063694 0.463345173564157
26.1146496815287 0.452284361578677
26.7515923566879 0.442940475196228
27.3885350318471 0.43469707702985
28.0254777070064 0.415112930587584
28.6624203821656 0.407199297381994
29.2993630573248 0.403820028458031
29.9363057324841 0.396398271305725
30.5732484076433 0.389305908980041
31.2101910828025 0.378208639705772
31.8471337579618 0.370675102811056
32.484076433121 0.359846099165152
33.1210191082803 0.349542754055246
33.7579617834395 0.343098358662428
34.3949044585987 0.338143938376079
35.031847133758 0.322799271103195
35.6687898089172 0.315694307117246
36.3057324840764 0.303595712457718
36.9426751592357 0.300399883686296
37.5796178343949 0.293241256148347
38.2165605095541 0.287027113325744
38.8535031847134 0.278958844833786
39.4904458598726 0.277073725192752
40.1273885350318 0.268812488240079
40.7643312101911 0.266607511731944
41.4012738853503 0.258668769515669
42.0382165605096 0.258010650986588
42.6751592356688 0.254900897610409
43.312101910828 0.253573402525566
43.9490445859873 0.247112171638185
44.5859872611465 0.240690336797288
45.2229299363057 0.23978678337632
45.859872611465 0.234712186209549
46.4968152866242 0.229987169685205
47.1337579617834 0.22874216144927
47.7707006369427 0.228457732840846
48.4076433121019 0.227250038668571
49.0445859872611 0.221186982416271
49.6815286624204 0.21483827214584
50.3184713375796 0.211598783273905
50.9554140127388 0.205075571776857
51.5923566878981 0.205897579031599
52.2292993630573 0.200805963663697
52.8662420382166 0.194983098000608
53.5031847133758 0.190809230764723
54.140127388535 0.184874071660524
54.7770700636943 0.1771122625476
55.4140127388535 0.17240637197842
56.0509554140127 0.165200380136583
56.687898089172 0.157491108269344
57.3248407643312 0.151529809821642
57.9617834394904 0.149267996911286
58.5987261146497 0.145027304818455
59.2356687898089 0.140628235728703
59.8726114649682 0.132469974098498
60.5095541401274 0.131098563166065
61.1464968152866 0.123721846177063
61.7834394904459 0.120744107663856
62.4203821656051 0.116864246263923
63.0573248407643 0.110749371266425
63.6942675159236 0.105273577061602
64.3312101910828 0.0960006307258152
64.968152866242 0.100983730787933
65.6050955414013 0.101390607937153
66.2420382165605 0.0939536112970662
66.8789808917197 0.0885800787087014
67.515923566879 0.0850155579613191
68.1528662420382 0.0788848415607737
68.7898089171974 0.0745756374440814
69.4267515923567 0.0696631720866071
70.0636942675159 0.0640817408512897
70.7006369426752 0.0602443675237897
71.3375796178344 0.0561739089658933
71.9745222929936 0.0509331065852
72.6114649681529 0.0492042323331654
73.2484076433121 0.050598666790472
73.8853503184713 0.04586500811707
74.5222929936306 0.0419371488101242
75.1592356687898 0.0414111933382495
75.796178343949 0.0417806435334162
76.4331210191083 0.0414685407774015
77.0700636942675 0.0385736747149201
77.7070063694268 0.0389752724232503
78.343949044586 0.0364640797912909
78.9808917197452 0.0327410827951941
79.6178343949044 0.0327145868579718
80.2547770700637 0.0339808353346013
80.8917197452229 0.0333913020668634
81.5286624203822 0.0288722903141072
82.1656050955414 0.0282286631423352
82.8025477707006 0.0291276570003001
83.4394904458599 0.0285177660731197
84.0764331210191 0.0251389465236501
84.7133757961783 0.0240374115064332
85.3503184713376 0.0233220998378755
85.9872611464968 0.0229896859760115
86.6242038216561 0.0208383656413107
87.2611464968153 0.0212872103013934
87.8980891719745 0.0172719513569735
88.5350318471338 0.0184389122767285
89.171974522293 0.016884448133088
89.8089171974522 0.0139736285222496
90.4458598726115 0.0119679526339027
91.0828025477707 0.00893425690942674
91.7197452229299 0.011475912259665
92.3566878980892 0.0117489096601493
92.9936305732484 0.00675207172632791
93.6305732484076 0.00338955711443526
94.2675159235669 0.00461352166712146
94.9044585987261 0.00359489072526176
95.5414012738853 0.00193951262532931
96.1783439490446 0.000525704719506183
96.8152866242038 0.000343168234368439
97.4522292993631 0.000129898815571139
98.0891719745223 6.34323071804838e-05
98.7261146496815 2.44773475854354e-05
99.3630573248408 2.41404765820658e-05
100 0
};
\path [fill=color3, fill opacity=0.25] 
(axis cs:0,0.916117258812997)
--(axis cs:0,0.91478195568477)
--(axis cs:0.636942675159236,0.91454414546724)
--(axis cs:1.27388535031847,0.913926383031491)
--(axis cs:1.91082802547771,0.912834186809725)
--(axis cs:2.54777070063694,0.910913333482035)
--(axis cs:3.18471337579618,0.909620104792217)
--(axis cs:3.82165605095541,0.905600900393421)
--(axis cs:4.45859872611465,0.903051625853103)
--(axis cs:5.09554140127389,0.899376860954999)
--(axis cs:5.73248407643312,0.892455673312763)
--(axis cs:6.36942675159236,0.884500574980764)
--(axis cs:7.00636942675159,0.873117499816478)
--(axis cs:7.64331210191083,0.859828586400719)
--(axis cs:8.28025477707006,0.847165287570014)
--(axis cs:8.9171974522293,0.828669763282533)
--(axis cs:9.55414012738853,0.813432959826887)
--(axis cs:10.1910828025478,0.798365869404592)
--(axis cs:10.828025477707,0.783656148778883)
--(axis cs:11.4649681528662,0.765055817841512)
--(axis cs:12.1019108280255,0.747034015348012)
--(axis cs:12.7388535031847,0.726575208104242)
--(axis cs:13.3757961783439,0.711091830675261)
--(axis cs:14.0127388535032,0.696146756272173)
--(axis cs:14.6496815286624,0.682434599092279)
--(axis cs:15.2866242038217,0.665261525014909)
--(axis cs:15.9235668789809,0.651803519076339)
--(axis cs:16.5605095541401,0.641764035615661)
--(axis cs:17.1974522292994,0.629751689586574)
--(axis cs:17.8343949044586,0.613320414791751)
--(axis cs:18.4713375796178,0.598273312634415)
--(axis cs:19.1082802547771,0.585448762439432)
--(axis cs:19.7452229299363,0.571684340965889)
--(axis cs:20.3821656050955,0.555517680696033)
--(axis cs:21.0191082802548,0.540586839119791)
--(axis cs:21.656050955414,0.527133275351177)
--(axis cs:22.2929936305732,0.512534663389954)
--(axis cs:22.9299363057325,0.499431555229536)
--(axis cs:23.5668789808917,0.484504050017688)
--(axis cs:24.203821656051,0.473315348954023)
--(axis cs:24.8407643312102,0.464113757315054)
--(axis cs:25.4777070063694,0.45594714158458)
--(axis cs:26.1146496815287,0.444914882779834)
--(axis cs:26.7515923566879,0.435706979149635)
--(axis cs:27.3885350318471,0.427332458550806)
--(axis cs:28.0254777070064,0.408162748590086)
--(axis cs:28.6624203821656,0.400177861729343)
--(axis cs:29.2993630573248,0.396816493450706)
--(axis cs:29.9363057324841,0.389400277217329)
--(axis cs:30.5732484076433,0.382275427654163)
--(axis cs:31.2101910828025,0.371128098094798)
--(axis cs:31.8471337579618,0.363399900739337)
--(axis cs:32.484076433121,0.352604597488983)
--(axis cs:33.1210191082803,0.342453058999115)
--(axis cs:33.7579617834395,0.335822890911787)
--(axis cs:34.3949044585987,0.33102254615738)
--(axis cs:35.031847133758,0.315639203333951)
--(axis cs:35.6687898089172,0.308641479046395)
--(axis cs:36.3057324840764,0.296841316876521)
--(axis cs:36.9426751592357,0.29370947993452)
--(axis cs:37.5796178343949,0.286541417225661)
--(axis cs:38.2165605095541,0.280494713855257)
--(axis cs:38.8535031847134,0.272592082734563)
--(axis cs:39.4904458598726,0.270873669289539)
--(axis cs:40.1273885350318,0.262857133975522)
--(axis cs:40.7643312101911,0.260813109717703)
--(axis cs:41.4012738853503,0.253033074707087)
--(axis cs:42.0382165605096,0.252552132217807)
--(axis cs:42.6751592356688,0.249377876478105)
--(axis cs:43.312101910828,0.248041203554927)
--(axis cs:43.9490445859873,0.241609434274948)
--(axis cs:44.5859872611465,0.235116830144133)
--(axis cs:45.2229299363057,0.234207805623067)
--(axis cs:45.859872611465,0.229170664668496)
--(axis cs:46.4968152866242,0.224633678267529)
--(axis cs:47.1337579617834,0.223280852310602)
--(axis cs:47.7707006369427,0.222825767228994)
--(axis cs:48.4076433121019,0.221681220972545)
--(axis cs:49.0445859872611,0.215533512482399)
--(axis cs:49.6815286624204,0.209061013328002)
--(axis cs:50.3184713375796,0.205896283936269)
--(axis cs:50.9554140127388,0.199331238884632)
--(axis cs:51.5923566878981,0.200283988143619)
--(axis cs:52.2292993630573,0.195168675946904)
--(axis cs:52.8662420382166,0.189446289621054)
--(axis cs:53.5031847133758,0.185131691095327)
--(axis cs:54.140127388535,0.179260624808546)
--(axis cs:54.7770700636943,0.171481508356589)
--(axis cs:55.4140127388535,0.166680611107485)
--(axis cs:56.0509554140127,0.159538087601854)
--(axis cs:56.687898089172,0.151874165858567)
--(axis cs:57.3248407643312,0.145979351334581)
--(axis cs:57.9617834394904,0.14387868135705)
--(axis cs:58.5987261146497,0.13977415241983)
--(axis cs:59.2356687898089,0.135433238024684)
--(axis cs:59.8726114649682,0.127607245113964)
--(axis cs:60.5095541401274,0.126188227988103)
--(axis cs:61.1464968152866,0.118947260158331)
--(axis cs:61.7834394904459,0.11610762646771)
--(axis cs:62.4203821656051,0.112476541132883)
--(axis cs:63.0573248407643,0.10652487249615)
--(axis cs:63.6942675159236,0.101084523208621)
--(axis cs:64.3312101910828,0.0919961514200156)
--(axis cs:64.968152866242,0.0967749750774603)
--(axis cs:65.6050955414013,0.0969736658917849)
--(axis cs:66.2420382165605,0.0895707370184554)
--(axis cs:66.8789808917197,0.0841456078177805)
--(axis cs:67.515923566879,0.0808226167201151)
--(axis cs:68.1528662420382,0.0748263547494303)
--(axis cs:68.7898089171974,0.0704189603337535)
--(axis cs:69.4267515923567,0.0656488052388504)
--(axis cs:70.0636942675159,0.0603500289658386)
--(axis cs:70.7006369426752,0.0565740100480617)
--(axis cs:71.3375796178344,0.0526984590480881)
--(axis cs:71.9745222929936,0.0476937306623578)
--(axis cs:72.6114649681529,0.0460892667555079)
--(axis cs:73.2484076433121,0.0474279448404006)
--(axis cs:73.8853503184713,0.0429786409884854)
--(axis cs:74.5222929936306,0.0393588847976135)
--(axis cs:75.1592356687898,0.0387989128717339)
--(axis cs:75.796178343949,0.0392940805961441)
--(axis cs:76.4331210191083,0.03908784023219)
--(axis cs:77.0700636942675,0.0362147146572071)
--(axis cs:77.7070063694268,0.0365042109114913)
--(axis cs:78.343949044586,0.0342464045765542)
--(axis cs:78.9808917197452,0.0304428162074151)
--(axis cs:79.6178343949044,0.0305763913941715)
--(axis cs:80.2547770700637,0.0321756541311439)
--(axis cs:80.8917197452229,0.0314974410199046)
--(axis cs:81.5286624203822,0.0268227506785574)
--(axis cs:82.1656050955414,0.0261211382754189)
--(axis cs:82.8025477707006,0.0272042649456411)
--(axis cs:83.4394904458599,0.0265778247661281)
--(axis cs:84.0764331210191,0.0232905116017004)
--(axis cs:84.7133757961783,0.0219452536803857)
--(axis cs:85.3503184713376,0.0210941363230377)
--(axis cs:85.9872611464968,0.02086952674366)
--(axis cs:86.6242038216561,0.0187087895625336)
--(axis cs:87.2611464968153,0.0195889221269187)
--(axis cs:87.8980891719745,0.0155041994623819)
--(axis cs:88.5350318471338,0.0168763898596504)
--(axis cs:89.171974522293,0.0151436069977306)
--(axis cs:89.8089171974522,0.0122822582192337)
--(axis cs:90.4458598726115,0.0102352341674148)
--(axis cs:91.0828025477707,0.00724757849112153)
--(axis cs:91.7197452229299,0.00974375637600676)
--(axis cs:92.3566878980892,0.0100757028220196)
--(axis cs:92.9936305732484,0.00534300566990997)
--(axis cs:93.6305732484076,0.00244376891650126)
--(axis cs:94.2675159235669,0.00340200358095985)
--(axis cs:94.9044585987261,0.00252875084956916)
--(axis cs:95.5414012738853,0.00126316601069293)
--(axis cs:96.1783439490446,0.000326681505220971)
--(axis cs:96.8152866242038,0.000220066686577607)
--(axis cs:97.4522292993631,7.76966830609685e-05)
--(axis cs:98.0891719745223,3.97214872649405e-05)
--(axis cs:98.7261146496815,1.73312941764505e-05)
--(axis cs:99.3630573248408,1.64672960656239e-05)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,3.18136570985076e-05)
--(axis cs:98.7261146496815,3.16234009944203e-05)
--(axis cs:98.0891719745223,8.71431270960271e-05)
--(axis cs:97.4522292993631,0.000182100948081309)
--(axis cs:96.8152866242038,0.000466269782159272)
--(axis cs:96.1783439490446,0.000724727933791395)
--(axis cs:95.5414012738853,0.00261585923996569)
--(axis cs:94.9044585987261,0.00466103060095436)
--(axis cs:94.2675159235669,0.00582503975328307)
--(axis cs:93.6305732484076,0.00433534531236925)
--(axis cs:92.9936305732484,0.00816113778274585)
--(axis cs:92.3566878980892,0.0134221164982789)
--(axis cs:91.7197452229299,0.0132080681433231)
--(axis cs:91.0828025477707,0.0106209353277319)
--(axis cs:90.4458598726115,0.0137006711003906)
--(axis cs:89.8089171974522,0.0156649988252655)
--(axis cs:89.171974522293,0.0186252892684453)
--(axis cs:88.5350318471338,0.0200014346938066)
--(axis cs:87.8980891719745,0.0190397032515651)
--(axis cs:87.2611464968153,0.0229854984758681)
--(axis cs:86.6242038216561,0.0229679417200877)
--(axis cs:85.9872611464968,0.025109845208363)
--(axis cs:85.3503184713376,0.0255500633527134)
--(axis cs:84.7133757961783,0.0261295693324808)
--(axis cs:84.0764331210191,0.0269873814455999)
--(axis cs:83.4394904458599,0.0304577073801113)
--(axis cs:82.8025477707006,0.0310510490549591)
--(axis cs:82.1656050955414,0.0303361880092515)
--(axis cs:81.5286624203822,0.030921829949657)
--(axis cs:80.8917197452229,0.0352851631138222)
--(axis cs:80.2547770700637,0.0357860165380587)
--(axis cs:79.6178343949044,0.034852782321772)
--(axis cs:78.9808917197452,0.0350393493829731)
--(axis cs:78.343949044586,0.0386817550060277)
--(axis cs:77.7070063694268,0.0414463339350094)
--(axis cs:77.0700636942675,0.0409326347726331)
--(axis cs:76.4331210191083,0.0438492413226131)
--(axis cs:75.796178343949,0.0442672064706883)
--(axis cs:75.1592356687898,0.0440234738047651)
--(axis cs:74.5222929936306,0.0445154128226349)
--(axis cs:73.8853503184713,0.0487513752456545)
--(axis cs:73.2484076433121,0.0537693887405434)
--(axis cs:72.6114649681529,0.0523191979108228)
--(axis cs:71.9745222929936,0.0541724825080422)
--(axis cs:71.3375796178344,0.0596493588836985)
--(axis cs:70.7006369426752,0.0639147249995178)
--(axis cs:70.0636942675159,0.0678134527367409)
--(axis cs:69.4267515923567,0.0736775389343638)
--(axis cs:68.7898089171974,0.0787323145544092)
--(axis cs:68.1528662420382,0.0829433283721172)
--(axis cs:67.515923566879,0.0892084992025232)
--(axis cs:66.8789808917197,0.0930145495996222)
--(axis cs:66.2420382165605,0.0983364855756769)
--(axis cs:65.6050955414013,0.105807549982521)
--(axis cs:64.968152866242,0.105192486498406)
--(axis cs:64.3312101910828,0.100005110031615)
--(axis cs:63.6942675159236,0.109462630914583)
--(axis cs:63.0573248407643,0.1149738700367)
--(axis cs:62.4203821656051,0.121251951394963)
--(axis cs:61.7834394904459,0.125380588860001)
--(axis cs:61.1464968152866,0.128496432195795)
--(axis cs:60.5095541401274,0.136008898344027)
--(axis cs:59.8726114649682,0.137332703083033)
--(axis cs:59.2356687898089,0.145823233432723)
--(axis cs:58.5987261146497,0.15028045721708)
--(axis cs:57.9617834394904,0.154657312465523)
--(axis cs:57.3248407643312,0.157080268308702)
--(axis cs:56.687898089172,0.163108050680121)
--(axis cs:56.0509554140127,0.170862672671312)
--(axis cs:55.4140127388535,0.178132132849355)
--(axis cs:54.7770700636943,0.182743016738611)
--(axis cs:54.140127388535,0.190487518512501)
--(axis cs:53.5031847133758,0.19648677043412)
--(axis cs:52.8662420382166,0.200519906380163)
--(axis cs:52.2292993630573,0.20644325138049)
--(axis cs:51.5923566878981,0.21151116991958)
--(axis cs:50.9554140127388,0.210819904669081)
--(axis cs:50.3184713375796,0.21730128261154)
--(axis cs:49.6815286624204,0.220615530963679)
--(axis cs:49.0445859872611,0.226840452350143)
--(axis cs:48.4076433121019,0.232818856364598)
--(axis cs:47.7707006369427,0.234089698452697)
--(axis cs:47.1337579617834,0.234203470587938)
--(axis cs:46.4968152866242,0.23534066110288)
--(axis cs:45.859872611465,0.240253707750601)
--(axis cs:45.2229299363057,0.245365761129574)
--(axis cs:44.5859872611465,0.246263843450444)
--(axis cs:43.9490445859873,0.252614909001422)
--(axis cs:43.312101910828,0.259105601496204)
--(axis cs:42.6751592356688,0.260423918742713)
--(axis cs:42.0382165605096,0.263469169755369)
--(axis cs:41.4012738853503,0.264304464324251)
--(axis cs:40.7643312101911,0.272401913746184)
--(axis cs:40.1273885350318,0.274767842504635)
--(axis cs:39.4904458598726,0.283273781095965)
--(axis cs:38.8535031847134,0.285325606933009)
--(axis cs:38.2165605095541,0.29355951279623)
--(axis cs:37.5796178343949,0.299941095071033)
--(axis cs:36.9426751592357,0.307090287438071)
--(axis cs:36.3057324840764,0.310350108038915)
--(axis cs:35.6687898089172,0.322747135188097)
--(axis cs:35.031847133758,0.329959338872438)
--(axis cs:34.3949044585987,0.345265330594778)
--(axis cs:33.7579617834395,0.350373826413069)
--(axis cs:33.1210191082803,0.356632449111378)
--(axis cs:32.484076433121,0.36708760084132)
--(axis cs:31.8471337579618,0.377950304882774)
--(axis cs:31.2101910828025,0.385289181316746)
--(axis cs:30.5732484076433,0.396336390305919)
--(axis cs:29.9363057324841,0.403396265394121)
--(axis cs:29.2993630573248,0.410823563465355)
--(axis cs:28.6624203821656,0.414220733034646)
--(axis cs:28.0254777070064,0.422063112585082)
--(axis cs:27.3885350318471,0.442061695508895)
--(axis cs:26.7515923566879,0.450173971242822)
--(axis cs:26.1146496815287,0.459653840377519)
--(axis cs:25.4777070063694,0.470743205543735)
--(axis cs:24.8407643312102,0.479254917656226)
--(axis cs:24.203821656051,0.488811047484666)
--(axis cs:23.5668789808917,0.500230938467309)
--(axis cs:22.9299363057325,0.515306854308286)
--(axis cs:22.2929936305732,0.528919274516818)
--(axis cs:21.656050955414,0.543467755600189)
--(axis cs:21.0191082802548,0.557090044192151)
--(axis cs:20.3821656050955,0.571971633844257)
--(axis cs:19.7452229299363,0.588417958992928)
--(axis cs:19.1082802547771,0.602073960145695)
--(axis cs:18.4713375796178,0.614664802393085)
--(axis cs:17.8343949044586,0.629888078600698)
--(axis cs:17.1974522292994,0.646127788597933)
--(axis cs:16.5605095541401,0.658227752685025)
--(axis cs:15.9235668789809,0.667822637613726)
--(axis cs:15.2866242038217,0.68085051475416)
--(axis cs:14.6496815286624,0.697848124527323)
--(axis cs:14.0127388535032,0.711364421920044)
--(axis cs:13.3757961783439,0.725931086569788)
--(axis cs:12.7388535031847,0.741449996574756)
--(axis cs:12.1019108280255,0.761664170548489)
--(axis cs:11.4649681528662,0.77947498391759)
--(axis cs:10.828025477707,0.797561262872858)
--(axis cs:10.1910828025478,0.811814823528908)
--(axis cs:9.55414012738853,0.826186146644186)
--(axis cs:8.9171974522293,0.840686284386893)
--(axis cs:8.28025477707006,0.858013935691061)
--(axis cs:7.64331210191083,0.869759251862531)
--(axis cs:7.00636942675159,0.881724970415919)
--(axis cs:6.36942675159236,0.891615730128117)
--(axis cs:5.73248407643312,0.898530810287228)
--(axis cs:5.09554140127389,0.904177354709045)
--(axis cs:4.45859872611465,0.907357839534826)
--(axis cs:3.82165605095541,0.909261785652978)
--(axis cs:3.18471337579618,0.912361801269775)
--(axis cs:2.54777070063694,0.913434389162417)
--(axis cs:1.91082802547771,0.914709982169205)
--(axis cs:1.27388535031847,0.915437997467392)
--(axis cs:0.636942675159236,0.915808340022326)
--(axis cs:0,0.916117258812997)
--cycle;


==> img/mnist/mnist_rate_distortion_deeptaylor.tex <==
% deep taylor
\addplot [line width=0.5, opacity=0.8, color5, mark=x, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color5, thin}]
table [row sep=\\]{%
0	0.915335376235889 \\
0.636942675159236	0.915082271771971 \\
1.27388535031847	0.91424479879206 \\
1.91082802547771	0.913276129188016 \\
2.54777070063694	0.912218541947659 \\
3.18471337579618	0.911604257620638 \\
3.82165605095541	0.911175284003839 \\
4.45859872611465	0.909826359604485 \\
5.09554140127389	0.908974135591998 \\
5.73248407643312	0.908293774900958 \\
6.36942675159236	0.907473447154043 \\
7.00636942675159	0.906393431440229 \\
7.64331210191083	0.905951815156732 \\
8.28025477707006	0.904218470147462 \\
8.9171974522293	0.902101472882787 \\
9.55414012738853	0.900477692038985 \\
10.1910828025478	0.896723845738452 \\
10.828025477707	0.894179565098602 \\
11.4649681528662	0.893477294528857 \\
12.1019108280255	0.891566888187081 \\
12.7388535031847	0.888240271894028 \\
13.3757961783439	0.884488954576664 \\
14.0127388535032	0.88137079553504 \\
14.6496815286624	0.87777009712474 \\
15.2866242038217	0.873902822576929 \\
15.9235668789809	0.870108815355343 \\
16.5605095541401	0.861390735440655 \\
17.1974522292994	0.85494457275141 \\
17.8343949044586	0.847920649025473 \\
18.4713375796178	0.846121272355085 \\
19.1082802547771	0.836740155869629 \\
19.7452229299363	0.829698255549884 \\
20.3821656050955	0.820394819197172 \\
21.0191082802548	0.812082640085137 \\
21.656050955414	0.799473875238182 \\
22.2929936305732	0.791589870400203 \\
22.9299363057325	0.778498222459457 \\
23.5668789808917	0.766522562517712 \\
24.203821656051	0.76520902318447 \\
24.8407643312102	0.752617460273141 \\
25.4777070063694	0.748444118048137 \\
26.1146496815287	0.740331748355602 \\
26.7515923566879	0.725367310572619 \\
27.3885350318471	0.712151789902455 \\
28.0254777070064	0.703062452985068 \\
28.6624203821656	0.688369376331329 \\
29.2993630573248	0.676181674337513 \\
29.9363057324841	0.662932274734794 \\
30.5732484076433	0.646393780686358 \\
31.2101910828025	0.634384400523268 \\
31.8471337579618	0.617722280023099 \\
32.484076433121	0.599440590733793 \\
33.1210191082803	0.578493899753557 \\
33.7579617834395	0.556832779435354 \\
34.3949044585987	0.537908585225814 \\
35.031847133758	0.519443027112684 \\
35.6687898089172	0.503113867990323 \\
36.3057324840764	0.485386038355573 \\
36.9426751592357	0.471084762980317 \\
37.5796178343949	0.460503489380935 \\
38.2165605095541	0.444755957785783 \\
38.8535031847134	0.430286577688239 \\
39.4904458598726	0.425061081860185 \\
40.1273885350318	0.411164293277543 \\
40.7643312101911	0.398323827192544 \\
41.4012738853503	0.383630396099834 \\
42.0382165605096	0.362204089077468 \\
42.6751592356688	0.358201481853939 \\
43.312101910828	0.34662386829601 \\
43.9490445859873	0.333649465448025 \\
44.5859872611465	0.316832648819122 \\
45.2229299363057	0.304369997558201 \\
45.859872611465	0.294156126481212 \\
46.4968152866242	0.283184137022172 \\
47.1337579617834	0.275893569799897 \\
47.7707006369427	0.269129668579349 \\
48.4076433121019	0.258328677880018 \\
49.0445859872611	0.245116090051974 \\
49.6815286624204	0.237828217854067 \\
50.3184713375796	0.232163215197779 \\
50.9554140127388	0.223623458546948 \\
51.5923566878981	0.215036611587729 \\
52.2292993630573	0.213941707106927 \\
52.8662420382166	0.212799439891251 \\
53.5031847133758	0.20902592931753 \\
54.140127388535	0.198152841277115 \\
54.7770700636943	0.191852750817344 \\
55.4140127388535	0.183482652336719 \\
56.0509554140127	0.173879028802739 \\
56.687898089172	0.168464015958081 \\
57.3248407643312	0.159030446431185 \\
57.9617834394904	0.153045665059655 \\
58.5987261146497	0.150660966173305 \\
59.2356687898089	0.146985746209787 \\
59.8726114649682	0.13985838308793 \\
60.5095541401274	0.140220696715751 \\
61.1464968152866	0.135010139764054 \\
61.7834394904459	0.130481808492278 \\
62.4203821656051	0.125712885549938 \\
63.0573248407643	0.122397152133093 \\
63.6942675159236	0.122679275813362 \\
64.3312101910828	0.118041163558235 \\
64.968152866242	0.111010581968147 \\
65.6050955414013	0.106294593535604 \\
66.2420382165605	0.101823681166136 \\
66.8789808917197	0.0933961188872105 \\
67.515923566879	0.0883725285779767 \\
68.1528662420382	0.0837263520104337 \\
68.7898089171974	0.0811125841472621 \\
69.4267515923567	0.0743566789265608 \\
70.0636942675159	0.0746451852490201 \\
70.7006369426752	0.0733451048690658 \\
71.3375796178344	0.0690517881304975 \\
71.9745222929936	0.0663359004989786 \\
72.6114649681529	0.0641551511966765 \\
73.2484076433121	0.0616767963303121 \\
73.8853503184713	0.0578916561530298 \\
74.5222929936306	0.0546039811183501 \\
75.1592356687898	0.0510533706056953 \\
75.796178343949	0.0495216800049498 \\
76.4331210191083	0.0425652334779535 \\
77.0700636942675	0.036594186633338 \\
77.7070063694268	0.0327828051734647 \\
78.343949044586	0.0276230524384916 \\
78.9808917197452	0.0239834507749792 \\
79.6178343949044	0.0229497186878451 \\
80.2547770700637	0.0212276731323047 \\
80.8917197452229	0.0199170329672204 \\
81.5286624203822	0.0179383316669042 \\
82.1656050955414	0.0164051098042667 \\
82.8025477707006	0.0170719480847925 \\
83.4394904458599	0.0147021411153197 \\
84.0764331210191	0.012857970531874 \\
84.7133757961783	0.0127103532984725 \\
85.3503184713376	0.0122149122128733 \\
85.9872611464968	0.00804846793834438 \\
86.6242038216561	0.00718069574533588 \\
87.2611464968153	0.00599217281395305 \\
87.8980891719745	0.00426957931629923 \\
88.5350318471338	0.00360950384916672 \\
89.171974522293	0.00317594151343276 \\
89.8089171974522	0.00295626385952611 \\
90.4458598726115	0.00193610677373997 \\
91.0828025477707	0.000935269013459631 \\
91.7197452229299	0.000774872739007692 \\
92.3566878980892	0.000319370610022754 \\
92.9936305732484	5.08209960001954e-05 \\
93.6305732484076	9.61155259573321e-05 \\
94.2675159235669	8.0595065199538e-05 \\
94.9044585987261	4.66511258882862e-05 \\
95.5414012738853	1.83808406096986e-05 \\
96.1783439490446	6.53133978890275e-06 \\
96.8152866242038	5.30783175842764e-06 \\
97.4522292993631	2.33772143734545e-06 \\
98.0891719745223	1.4166253585185e-06 \\
98.7261146496815	8.46785898073743e-07 \\
99.3630573248408	7.34801553038955e-07 \\
100	9.07070329958515e-11 \\
};
\path [fill=color5, fill opacity=0.5] (axis cs:0,0.916021299259543)
--(axis cs:0,0.914649453212235)
--(axis cs:0.636942675159236,0.914426658049458)
--(axis cs:1.27388535031847,0.913340460753742)
--(axis cs:1.91082802547771,0.912228594968197)
--(axis cs:2.54777070063694,0.911078717220677)
--(axis cs:3.18471337579618,0.910488320391409)
--(axis cs:3.82165605095541,0.909973447525006)
--(axis cs:4.45859872611465,0.908468332925069)
--(axis cs:5.09554140127389,0.907493596505085)
--(axis cs:5.73248407643312,0.906798738013292)
--(axis cs:6.36942675159236,0.905908482284917)
--(axis cs:7.00636942675159,0.90469825465297)
--(axis cs:7.64331210191083,0.904226545581215)
--(axis cs:8.28025477707006,0.90226751384504)
--(axis cs:8.9171974522293,0.8998761060433)
--(axis cs:9.55414012738853,0.898076688611686)
--(axis cs:10.1910828025478,0.893921168489465)
--(axis cs:10.828025477707,0.89112748883518)
--(axis cs:11.4649681528662,0.89042600317386)
--(axis cs:12.1019108280255,0.888335515509553)
--(axis cs:12.7388535031847,0.884787405231616)
--(axis cs:13.3757961783439,0.880746859515919)
--(axis cs:14.0127388535032,0.877464236562605)
--(axis cs:14.6496815286624,0.87370878666027)
--(axis cs:15.2866242038217,0.869688751243828)
--(axis cs:15.9235668789809,0.865737839594113)
--(axis cs:16.5605095541401,0.856708284618609)
--(axis cs:17.1974522292994,0.850061597273688)
--(axis cs:17.8343949044586,0.843049569785489)
--(axis cs:18.4713375796178,0.840964767116838)
--(axis cs:19.1082802547771,0.831248132519379)
--(axis cs:19.7452229299363,0.824076640157659)
--(axis cs:20.3821656050955,0.814871579429015)
--(axis cs:21.0191082802548,0.806306006019857)
--(axis cs:21.656050955414,0.793570017168326)
--(axis cs:22.2929936305732,0.785557032139688)
--(axis cs:22.9299363057325,0.772176391143076)
--(axis cs:23.5668789808917,0.760217599310231)
--(axis cs:24.203821656051,0.758830773826371)
--(axis cs:24.8407643312102,0.746332373959403)
--(axis cs:25.4777070063694,0.742044061536137)
--(axis cs:26.1146496815287,0.733886743050002)
--(axis cs:26.7515923566879,0.71909247733459)
--(axis cs:27.3885350318471,0.705901804619099)
--(axis cs:28.0254777070064,0.69667733050008)
--(axis cs:28.6624203821656,0.681753932199374)
--(axis cs:29.2993630573248,0.669745053118736)
--(axis cs:29.9363057324841,0.656223472524494)
--(axis cs:30.5732484076433,0.639425701759606)
--(axis cs:31.2101910828025,0.627260073696116)
--(axis cs:31.8471337579618,0.610313532625873)
--(axis cs:32.484076433121,0.592060113204829)
--(axis cs:33.1210191082803,0.57061501272589)
--(axis cs:33.7579617834395,0.549168029191661)
--(axis cs:34.3949044585987,0.53022124529073)
--(axis cs:35.031847133758,0.511620001369217)
--(axis cs:35.6687898089172,0.495377482881874)
--(axis cs:36.3057324840764,0.47773081510971)
--(axis cs:36.9426751592357,0.463508796902034)
--(axis cs:37.5796178343949,0.452996534645691)
--(axis cs:38.2165605095541,0.43723803005064)
--(axis cs:38.8535031847134,0.423163167180769)
--(axis cs:39.4904458598726,0.417776448859819)
--(axis cs:40.1273885350318,0.404048113451446)
--(axis cs:40.7643312101911,0.391367155617844)
--(axis cs:41.4012738853503,0.376937069151164)
--(axis cs:42.0382165605096,0.355670962028971)
--(axis cs:42.6751592356688,0.351953672377583)
--(axis cs:43.312101910828,0.340315151159343)
--(axis cs:43.9490445859873,0.327499263264687)
--(axis cs:44.5859872611465,0.31090083284428)
--(axis cs:45.2229299363057,0.298667196717956)
--(axis cs:45.859872611465,0.288630159091401)
--(axis cs:46.4968152866242,0.277685112285271)
--(axis cs:47.1337579617834,0.270309959087347)
--(axis cs:47.7707006369427,0.263508471488395)
--(axis cs:48.4076433121019,0.252411178081347)
--(axis cs:49.0445859872611,0.239499686628589)
--(axis cs:49.6815286624204,0.232280069046046)
--(axis cs:50.3184713375796,0.226705755050254)
--(axis cs:50.9554140127388,0.218173003968158)
--(axis cs:51.5923566878981,0.209582907143424)
--(axis cs:52.2292993630573,0.208691092209578)
--(axis cs:52.8662420382166,0.207586038844706)
--(axis cs:53.5031847133758,0.203920387580204)
--(axis cs:54.140127388535,0.193235645999905)
--(axis cs:54.7770700636943,0.187238012165122)
--(axis cs:55.4140127388535,0.178883256756235)
--(axis cs:56.0509554140127,0.169714853703421)
--(axis cs:56.687898089172,0.164322258614614)
--(axis cs:57.3248407643312,0.154927202375599)
--(axis cs:57.9617834394904,0.148988114001428)
--(axis cs:58.5987261146497,0.146566929926113)
--(axis cs:59.2356687898089,0.143112264689868)
--(axis cs:59.8726114649682,0.136147633503749)
--(axis cs:60.5095541401274,0.136623161885763)
--(axis cs:61.1464968152866,0.131295218324259)
--(axis cs:61.7834394904459,0.126745681747613)
--(axis cs:62.4203821656051,0.121836388272709)
--(axis cs:63.0573248407643,0.118538446608972)
--(axis cs:63.6942675159236,0.118841782319147)
--(axis cs:64.3312101910828,0.114028580852933)
--(axis cs:64.968152866242,0.107054523945805)
--(axis cs:65.6050955414013,0.102441590879262)
--(axis cs:66.2420382165605,0.0979553986014958)
--(axis cs:66.8789808917197,0.0897084368142423)
--(axis cs:67.515923566879,0.0848049132176562)
--(axis cs:68.1528662420382,0.0804300869628646)
--(axis cs:68.7898089171974,0.0778935974751738)
--(axis cs:69.4267515923567,0.0714114252111716)
--(axis cs:70.0636942675159,0.0717928037381778)
--(axis cs:70.7006369426752,0.0705540190651649)
--(axis cs:71.3375796178344,0.066314371228596)
--(axis cs:71.9745222929936,0.0636789282937857)
--(axis cs:72.6114649681529,0.0616823030040923)
--(axis cs:73.2484076433121,0.0591467697825785)
--(axis cs:73.8853503184713,0.055336183557839)
--(axis cs:74.5222929936306,0.052134409475169)
--(axis cs:75.1592356687898,0.0485886096172626)
--(axis cs:75.796178343949,0.047065710676491)
--(axis cs:76.4331210191083,0.0401671068021513)
--(axis cs:77.0700636942675,0.034323703082471)
--(axis cs:77.7070063694268,0.0307541314386301)
--(axis cs:78.343949044586,0.0257823633493505)
--(axis cs:78.9808917197452,0.0223226272333411)
--(axis cs:79.6178343949044,0.021274574731983)
--(axis cs:80.2547770700637,0.0198065202505799)
--(axis cs:80.8917197452229,0.018612549846464)
--(axis cs:81.5286624203822,0.0166794891081551)
--(axis cs:82.1656050955414,0.0152014858254594)
--(axis cs:82.8025477707006,0.0159934836220462)
--(axis cs:83.4394904458599,0.0136077057896169)
--(axis cs:84.0764331210191,0.0119025554703071)
--(axis cs:84.7133757961783,0.0116941108817966)
--(axis cs:85.3503184713376,0.0112342271850805)
--(axis cs:85.9872611464968,0.00713876287489572)
--(axis cs:86.6242038216561,0.00630217322658959)
--(axis cs:87.2611464968153,0.00515317372825132)
--(axis cs:87.8980891719745,0.00352507174314945)
--(axis cs:88.5350318471338,0.00299553755074547)
--(axis cs:89.171974522293,0.00260228536439404)
--(axis cs:89.8089171974522,0.00235964951733478)
--(axis cs:90.4458598726115,0.00147974338013581)
--(axis cs:91.0828025477707,0.000685565781715712)
--(axis cs:91.7197452229299,0.000540056200638833)
--(axis cs:92.3566878980892,0.000196335600954368)
--(axis cs:92.9936305732484,3.04311749426412e-05)
--(axis cs:93.6305732484076,6.56040640905955e-05)
--(axis cs:94.2675159235669,5.32720897549295e-05)
--(axis cs:94.9044585987261,3.19703803252107e-05)
--(axis cs:95.5414012738853,1.2931140273768e-05)
--(axis cs:96.1783439490446,4.55064348021909e-06)
--(axis cs:96.8152866242038,3.7612717788439e-06)
--(axis cs:97.4522292993631,1.71390618844022e-06)
--(axis cs:98.0891719745223,1.05556421268572e-06)
--(axis cs:98.7261146496815,6.69137553531809e-07)
--(axis cs:99.3630573248408,4.8205285993947e-07)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,9.8755024613844e-07)
--(axis cs:98.7261146496815,1.02443424261568e-06)
--(axis cs:98.0891719745223,1.77768650435127e-06)
--(axis cs:97.4522292993631,2.96153668625068e-06)
--(axis cs:96.8152866242038,6.85439173801138e-06)
--(axis cs:96.1783439490446,8.5120360975864e-06)
--(axis cs:95.5414012738853,2.38305409456291e-05)
--(axis cs:94.9044585987261,6.13318714513618e-05)
--(axis cs:94.2675159235669,0.000107918040644146)
--(axis cs:93.6305732484076,0.000126626987824069)
--(axis cs:92.9936305732484,7.12108170577496e-05)
--(axis cs:92.3566878980892,0.00044240561909114)
--(axis cs:91.7197452229299,0.00100968927737655)
--(axis cs:91.0828025477707,0.00118497224520355)
--(axis cs:90.4458598726115,0.00239247016734412)
--(axis cs:89.8089171974522,0.00355287820171743)
--(axis cs:89.171974522293,0.00374959766247148)
--(axis cs:88.5350318471338,0.00422347014758797)
--(axis cs:87.8980891719745,0.00501408688944902)
--(axis cs:87.2611464968153,0.00683117189965477)
--(axis cs:86.6242038216561,0.00805921826408217)
--(axis cs:85.9872611464968,0.00895817300179303)
--(axis cs:85.3503184713376,0.013195597240666)
--(axis cs:84.7133757961783,0.0137265957151484)
--(axis cs:84.0764331210191,0.013813385593441)
--(axis cs:83.4394904458599,0.0157965764410225)
--(axis cs:82.8025477707006,0.0181504125475387)
--(axis cs:82.1656050955414,0.017608733783074)
--(axis cs:81.5286624203822,0.0191971742256533)
--(axis cs:80.8917197452229,0.0212215160879768)
--(axis cs:80.2547770700637,0.0226488260140296)
--(axis cs:79.6178343949044,0.0246248626437071)
--(axis cs:78.9808917197452,0.0256442743166173)
--(axis cs:78.343949044586,0.0294637415276326)
--(axis cs:77.7070063694268,0.0348114789082993)
--(axis cs:77.0700636942675,0.0388646701842049)
--(axis cs:76.4331210191083,0.0449633601537558)
--(axis cs:75.796178343949,0.0519776493334086)
--(axis cs:75.1592356687898,0.053518131594128)
--(axis cs:74.5222929936306,0.0570735527615311)
--(axis cs:73.8853503184713,0.0604471287482206)
--(axis cs:73.2484076433121,0.0642068228780458)
--(axis cs:72.6114649681529,0.0666279993892607)
--(axis cs:71.9745222929936,0.0689928727041715)
--(axis cs:71.3375796178344,0.071789205032399)
--(axis cs:70.7006369426752,0.0761361906729668)
--(axis cs:70.0636942675159,0.0774975667598624)
--(axis cs:69.4267515923567,0.07730193264195)
--(axis cs:68.7898089171974,0.0843315708193504)
--(axis cs:68.1528662420382,0.0870226170580027)
--(axis cs:67.515923566879,0.0919401439382973)
--(axis cs:66.8789808917197,0.0970838009601787)
--(axis cs:66.2420382165605,0.105691963730777)
--(axis cs:65.6050955414013,0.110147596191946)
--(axis cs:64.968152866242,0.11496663999049)
--(axis cs:64.3312101910828,0.122053746263537)
--(axis cs:63.6942675159236,0.126516769307577)
--(axis cs:63.0573248407643,0.126255857657214)
--(axis cs:62.4203821656051,0.129589382827167)
--(axis cs:61.7834394904459,0.134217935236943)
--(axis cs:61.1464968152866,0.138725061203848)
--(axis cs:60.5095541401274,0.143818231545738)
--(axis cs:59.8726114649682,0.143569132672111)
--(axis cs:59.2356687898089,0.150859227729706)
--(axis cs:58.5987261146497,0.154755002420498)
--(axis cs:57.9617834394904,0.157103216117882)
--(axis cs:57.3248407643312,0.16313369048677)
--(axis cs:56.687898089172,0.172605773301548)
--(axis cs:56.0509554140127,0.178043203902058)
--(axis cs:55.4140127388535,0.188082047917202)
--(axis cs:54.7770700636943,0.196467489469566)
--(axis cs:54.140127388535,0.203070036554325)
--(axis cs:53.5031847133758,0.214131471054856)
--(axis cs:52.8662420382166,0.218012840937795)
--(axis cs:52.2292993630573,0.219192322004277)
--(axis cs:51.5923566878981,0.220490316032033)
--(axis cs:50.9554140127388,0.229073913125738)
--(axis cs:50.3184713375796,0.237620675345304)
--(axis cs:49.6815286624204,0.243376366662088)
--(axis cs:49.0445859872611,0.25073249347536)
--(axis cs:48.4076433121019,0.264246177678688)
--(axis cs:47.7707006369427,0.274750865670302)
--(axis cs:47.1337579617834,0.281477180512447)
--(axis cs:46.4968152866242,0.288683161759072)
--(axis cs:45.859872611465,0.299682093871022)
--(axis cs:45.2229299363057,0.310072798398446)
--(axis cs:44.5859872611465,0.322764464793965)
--(axis cs:43.9490445859873,0.339799667631363)
--(axis cs:43.312101910828,0.352932585432677)
--(axis cs:42.6751592356688,0.364449291330295)
--(axis cs:42.0382165605096,0.368737216125964)
--(axis cs:41.4012738853503,0.390323723048503)
--(axis cs:40.7643312101911,0.405280498767243)
--(axis cs:40.1273885350318,0.418280473103641)
--(axis cs:39.4904458598726,0.432345714860552)
--(axis cs:38.8535031847134,0.437409988195709)
--(axis cs:38.2165605095541,0.452273885520925)
--(axis cs:37.5796178343949,0.46801044411618)
--(axis cs:36.9426751592357,0.478660729058601)
--(axis cs:36.3057324840764,0.493041261601436)
--(axis cs:35.6687898089172,0.510850253098773)
--(axis cs:35.031847133758,0.527266052856151)
--(axis cs:34.3949044585987,0.545595925160898)
--(axis cs:33.7579617834395,0.564497529679046)
--(axis cs:33.1210191082803,0.586372786781225)
--(axis cs:32.484076433121,0.606821068262758)
--(axis cs:31.8471337579618,0.625131027420325)
--(axis cs:31.2101910828025,0.641508727350419)
--(axis cs:30.5732484076433,0.65336185961311)
--(axis cs:29.9363057324841,0.669641076945094)
--(axis cs:29.2993630573248,0.68261829555629)
--(axis cs:28.6624203821656,0.694984820463285)
--(axis cs:28.0254777070064,0.709447575470057)
--(axis cs:27.3885350318471,0.71840177518581)
--(axis cs:26.7515923566879,0.731642143810648)
--(axis cs:26.1146496815287,0.746776753661202)
--(axis cs:25.4777070063694,0.754844174560137)
--(axis cs:24.8407643312102,0.758902546586878)
--(axis cs:24.203821656051,0.77158727254257)
--(axis cs:23.5668789808917,0.772827525725192)
--(axis cs:22.9299363057325,0.784820053775838)
--(axis cs:22.2929936305732,0.797622708660718)
--(axis cs:21.656050955414,0.805377733308038)
--(axis cs:21.0191082802548,0.817859274150416)
--(axis cs:20.3821656050955,0.825918058965329)
--(axis cs:19.7452229299363,0.835319870942108)
--(axis cs:19.1082802547771,0.842232179219879)
--(axis cs:18.4713375796178,0.851277777593333)
--(axis cs:17.8343949044586,0.852791728265457)
--(axis cs:17.1974522292994,0.859827548229132)
--(axis cs:16.5605095541401,0.866073186262701)
--(axis cs:15.9235668789809,0.874479791116572)
--(axis cs:15.2866242038217,0.878116893910029)
--(axis cs:14.6496815286624,0.881831407589209)
--(axis cs:14.0127388535032,0.885277354507475)
--(axis cs:13.3757961783439,0.888231049637408)
--(axis cs:12.7388535031847,0.891693138556441)
--(axis cs:12.1019108280255,0.894798260864608)
--(axis cs:11.4649681528662,0.896528585883854)
--(axis cs:10.828025477707,0.897231641362025)
--(axis cs:10.1910828025478,0.899526522987438)
--(axis cs:9.55414012738853,0.902878695466284)
--(axis cs:8.9171974522293,0.904326839722274)
--(axis cs:8.28025477707006,0.906169426449883)
--(axis cs:7.64331210191083,0.907677084732248)
--(axis cs:7.00636942675159,0.908088608227487)
--(axis cs:6.36942675159236,0.909038412023169)
--(axis cs:5.73248407643312,0.909788811788624)
--(axis cs:5.09554140127389,0.91045467467891)
--(axis cs:4.45859872611465,0.911184386283901)
--(axis cs:3.82165605095541,0.912377120482672)
--(axis cs:3.18471337579618,0.912720194849868)
--(axis cs:2.54777070063694,0.913358366674641)
--(axis cs:1.91082802547771,0.914323663407836)
--(axis cs:1.27388535031847,0.915149136830379)
--(axis cs:0.636942675159236,0.915737885494484)
--(axis cs:0,0.916021299259543)
--cycle;


==> img/mnist/mnist_rate_distortion_fw_100.tex <==
\addplot [line width=0.5, opacity=0.85, color0!75, dashed]
table {%
0 0.915487912946846
0.636942675159236 0.915045215713326
1.27388535031847 0.914808969512233
1.91082802547771 0.914160967329517
2.54777070063694 0.913274240126775
3.18471337579618 0.91224905250856
3.82165605095541 0.909995935870102
4.45859872611465 0.908584474861273
5.09554140127389 0.905135669106676
5.73248407643312 0.900724823622732
6.36942675159236 0.897408374529332
7.00636942675159 0.886561981342384
7.64331210191083 0.876209146613255
8.28025477707006 0.862910994400736
8.9171974522293 0.845788857490988
9.55414012738853 0.827745667689014
10.1910828025478 0.801304175640689
10.828025477707 0.776828190918895
11.4649681528662 0.748110875227721
12.1019108280255 0.722220326532843
12.7388535031847 0.689316953531816
13.3757961783439 0.66092664871423
14.0127388535032 0.644755379562266
14.6496815286624 0.624345513693988
15.2866242038217 0.609514210412744
15.9235668789809 0.59667048692645
16.5605095541401 0.58678101996542
17.1974522292994 0.57392227139906
17.8343949044586 0.574910194058903
18.4713375796178 0.565798004193348
19.1082802547771 0.550701014916413
19.7452229299363 0.547017785874195
20.3821656050955 0.543857995915459
21.0191082802548 0.539690981333843
21.656050955414 0.530637295987981
22.2929936305732 0.518486681077629
22.9299363057325 0.51685139047695
23.5668789808917 0.512695964996237
24.203821656051 0.502532421579526
24.8407643312102 0.495492132731597
25.4777070063694 0.488740926379396
26.1146496815287 0.480532125472091
26.7515923566879 0.468397729222779
27.3885350318471 0.469592037241673
28.0254777070064 0.456921698814549
28.6624203821656 0.455652996570861
29.2993630573248 0.44927287230792
29.9363057324841 0.448201455245144
30.5732484076433 0.446189503316273
31.2101910828025 0.440346710883314
31.8471337579618 0.441676955879884
32.484076433121 0.439313166164502
33.1210191082803 0.437840370963095
33.7579617834395 0.439855155192781
34.3949044585987 0.43907687817642
35.031847133758 0.439000624468317
35.6687898089172 0.438318436256959
36.3057324840764 0.437173990154697
36.9426751592357 0.439481477018271
37.5796178343949 0.435720274871273
38.2165605095541 0.433582558508351
38.8535031847134 0.430633279304093
39.4904458598726 0.427283731668322
40.1273885350318 0.425780333384646
40.7643312101911 0.423021936537443
41.4012738853503 0.418138740129616
42.0382165605096 0.41636556436777
42.6751592356688 0.418617419245311
43.312101910828 0.410180865028965
43.9490445859873 0.406431758638864
44.5859872611465 0.403000004598789
45.2229299363057 0.401433277169954
45.859872611465 0.400584516244653
46.4968152866242 0.394134248958376
47.1337579617834 0.384231924560988
47.7707006369427 0.375393046112924
48.4076433121019 0.372378783069532
49.0445859872611 0.372069841177581
49.6815286624204 0.36669386171674
50.3184713375796 0.362563002578461
50.9554140127388 0.35369223761239
51.5923566878981 0.346850260819174
52.2292993630573 0.342756030819018
52.8662420382166 0.335043088114805
53.5031847133758 0.332560255349365
54.140127388535 0.326880315289727
54.7770700636943 0.323970807665065
55.4140127388535 0.321916305263355
56.0509554140127 0.314863515489685
56.687898089172 0.311729112166436
57.3248407643312 0.311786099209924
57.9617834394904 0.299430003755649
58.5987261146497 0.294049352043485
59.2356687898089 0.28541363573823
59.8726114649682 0.280087417288131
60.5095541401274 0.274453076994502
61.1464968152866 0.274434064543803
61.7834394904459 0.270418758168151
62.4203821656051 0.268167800138718
63.0573248407643 0.264244182156545
63.6942675159236 0.259627410089309
64.3312101910828 0.25381481592965
64.968152866242 0.2526150216978
65.6050955414013 0.248970227147186
66.2420382165605 0.242059832861079
66.8789808917197 0.236714206641247
67.515923566879 0.22837265070405
68.1528662420382 0.222923177523497
68.7898089171974 0.220957456366695
69.4267515923567 0.21323090492377
70.0636942675159 0.2028080147928
70.7006369426752 0.201078995957851
71.3375796178344 0.19382991302163
71.9745222929936 0.189082478945663
72.6114649681529 0.184802072454382
73.2484076433121 0.176266051350757
73.8853503184713 0.172931844177619
74.5222929936306 0.167468048932136
75.1592356687898 0.155941097870849
75.796178343949 0.150145966028367
76.4331210191083 0.148559956045773
77.0700636942675 0.140051259906882
77.7070063694268 0.129169815261059
78.343949044586 0.127867416734567
78.9808917197452 0.119187052478432
79.6178343949044 0.110565376541174
80.2547770700637 0.100530619990495
80.8917197452229 0.0926962652005831
81.5286624203822 0.0846468743942944
82.1656050955414 0.0792691973006282
82.8025477707006 0.0754500101935587
83.4394904458599 0.0642093999012338
84.0764331210191 0.0602670641208163
84.7133757961783 0.0472253422937344
85.3503184713376 0.0449191394249386
85.9872611464968 0.0402940586146567
86.6242038216561 0.0323728216507335
87.2611464968153 0.0318905982152344
87.8980891719745 0.024689018439343
88.5350318471338 0.0166232136154585
89.171974522293 0.0156602484305796
89.8089171974522 0.00732581169836142
90.4458598726115 0.00696251184483735
91.0828025477707 0.00574095702907589
91.7197452229299 0.00809136063847779
92.3566878980892 0.00687904179741175
92.9936305732484 0.00742113188034254
93.6305732484076 0.00452158950446364
94.2675159235669 0.00307185785616563
94.9044585987261 0.00347818617224813
95.5414012738853 0.00267674682660046
96.1783439490446 0.0018786415995054
96.8152866242038 0.00229561074700407
97.4522292993631 0.00148672711680094
98.0891719745223 0.00109085303321688
98.7261146496815 9.31185712888533e-05
99.3630573248408 1.04747400924221e-05
100 0
};
\path [fill=color0!75, fill opacity=0.25] 
(axis cs:0,0.916086952117701)
--(axis cs:0,0.914888873775991)
--(axis cs:0.636942675159236,0.914337465473328)
--(axis cs:1.27388535031847,0.913958765908914)
--(axis cs:1.91082802547771,0.913312734621079)
--(axis cs:2.54777070063694,0.912278394469918)
--(axis cs:3.18471337579618,0.911062516721773)
--(axis cs:3.82165605095541,0.9084758839548)
--(axis cs:4.45859872611465,0.906880470645069)
--(axis cs:5.09554140127389,0.902986831506152)
--(axis cs:5.73248407643312,0.898136313152726)
--(axis cs:6.36942675159236,0.894630869623374)
--(axis cs:7.00636942675159,0.882899467488451)
--(axis cs:7.64331210191083,0.871890568772574)
--(axis cs:8.28025477707006,0.857845294833184)
--(axis cs:8.9171974522293,0.840125858982062)
--(axis cs:9.55414012738853,0.821524541204184)
--(axis cs:10.1910828025478,0.794371058425494)
--(axis cs:10.828025477707,0.769459268394174)
--(axis cs:11.4649681528662,0.740372311404687)
--(axis cs:12.1019108280255,0.714314769569063)
--(axis cs:12.7388535031847,0.681259392518394)
--(axis cs:13.3757961783439,0.652756236783807)
--(axis cs:14.0127388535032,0.636509541945767)
--(axis cs:14.6496815286624,0.616166407157267)
--(axis cs:15.2866242038217,0.601261210017815)
--(axis cs:15.9235668789809,0.588494886687923)
--(axis cs:16.5605095541401,0.578641261772328)
--(axis cs:17.1974522292994,0.565902578659415)
--(axis cs:17.8343949044586,0.567149866477971)
--(axis cs:18.4713375796178,0.557790600790407)
--(axis cs:19.1082802547771,0.542702326030256)
--(axis cs:19.7452229299363,0.539205800086945)
--(axis cs:20.3821656050955,0.536073480845672)
--(axis cs:21.0191082802548,0.531889356196538)
--(axis cs:21.656050955414,0.522733661934436)
--(axis cs:22.2929936305732,0.510665141984609)
--(axis cs:22.9299363057325,0.508980383762923)
--(axis cs:23.5668789808917,0.504892918736746)
--(axis cs:24.203821656051,0.494689792534744)
--(axis cs:24.8407643312102,0.487692567050021)
--(axis cs:25.4777070063694,0.480844190517302)
--(axis cs:26.1146496815287,0.472641088722325)
--(axis cs:26.7515923566879,0.460495611275398)
--(axis cs:27.3885350318471,0.461895636068399)
--(axis cs:28.0254777070064,0.449160571278783)
--(axis cs:28.6624203821656,0.448069930654321)
--(axis cs:29.2993630573248,0.44170282728191)
--(axis cs:29.9363057324841,0.440700271816389)
--(axis cs:30.5732484076433,0.438757980816018)
--(axis cs:31.2101910828025,0.432976795807309)
--(axis cs:31.8471337579618,0.434392615054719)
--(axis cs:32.484076433121,0.432027912853967)
--(axis cs:33.1210191082803,0.430530760484473)
--(axis cs:33.7579617834395,0.432686650769187)
--(axis cs:34.3949044585987,0.432034922127073)
--(axis cs:35.031847133758,0.431818217575523)
--(axis cs:35.6687898089172,0.431155116981455)
--(axis cs:36.3057324840764,0.430019217420831)
--(axis cs:36.9426751592357,0.43241254411612)
--(axis cs:37.5796178343949,0.428752936439005)
--(axis cs:38.2165605095541,0.426652655341073)
--(axis cs:38.8535031847134,0.42367520011537)
--(axis cs:39.4904458598726,0.420272258874566)
--(axis cs:40.1273885350318,0.41882667715162)
--(axis cs:40.7643312101911,0.416108829601807)
--(axis cs:41.4012738853503,0.411149889454028)
--(axis cs:42.0382165605096,0.409525286799995)
--(axis cs:42.6751592356688,0.411611325557168)
--(axis cs:43.312101910828,0.403290432458246)
--(axis cs:43.9490445859873,0.39949879545609)
--(axis cs:44.5859872611465,0.396083252054939)
--(axis cs:45.2229299363057,0.394624810943501)
--(axis cs:45.859872611465,0.393705565720332)
--(axis cs:46.4968152866242,0.387192200159632)
--(axis cs:47.1337579617834,0.37740793102866)
--(axis cs:47.7707006369427,0.368561979145001)
--(axis cs:48.4076433121019,0.365428566580027)
--(axis cs:49.0445859872611,0.365337513948355)
--(axis cs:49.6815286624204,0.359830589021392)
--(axis cs:50.3184713375796,0.35577204815489)
--(axis cs:50.9554140127388,0.346918012664807)
--(axis cs:51.5923566878981,0.340140969392754)
--(axis cs:52.2292993630573,0.336197296769861)
--(axis cs:52.8662420382166,0.32861559780386)
--(axis cs:53.5031847133758,0.326329935956806)
--(axis cs:54.140127388535,0.320671277314927)
--(axis cs:54.7770700636943,0.317953254730623)
--(axis cs:55.4140127388535,0.316031183238292)
--(axis cs:56.0509554140127,0.309112235186929)
--(axis cs:56.687898089172,0.305893024670464)
--(axis cs:57.3248407643312,0.305967448724889)
--(axis cs:57.9617834394904,0.293725963041625)
--(axis cs:58.5987261146497,0.288410134637039)
--(axis cs:59.2356687898089,0.279950552276677)
--(axis cs:59.8726114649682,0.274673589946648)
--(axis cs:60.5095541401274,0.269068687255219)
--(axis cs:61.1464968152866,0.268881098295147)
--(axis cs:61.7834394904459,0.264714475217566)
--(axis cs:62.4203821656051,0.262357884320272)
--(axis cs:63.0573248407643,0.258641166024244)
--(axis cs:63.6942675159236,0.254036980702677)
--(axis cs:64.3312101910828,0.248277004534856)
--(axis cs:64.968152866242,0.247205418790768)
--(axis cs:65.6050955414013,0.243522394012414)
--(axis cs:66.2420382165605,0.236513240069969)
--(axis cs:66.8789808917197,0.231052301460698)
--(axis cs:67.515923566879,0.222734635827819)
--(axis cs:68.1528662420382,0.217231117351856)
--(axis cs:68.7898089171974,0.215302028939503)
--(axis cs:69.4267515923567,0.207668107135497)
--(axis cs:70.0636942675159,0.197330508301924)
--(axis cs:70.7006369426752,0.195409096225146)
--(axis cs:71.3375796178344,0.188225594741322)
--(axis cs:71.9745222929936,0.183463127767615)
--(axis cs:72.6114649681529,0.179265336186722)
--(axis cs:73.2484076433121,0.170787256992192)
--(axis cs:73.8853503184713,0.167487010153424)
--(axis cs:74.5222929936306,0.162022680711326)
--(axis cs:75.1592356687898,0.150675801618299)
--(axis cs:75.796178343949,0.144824825827524)
--(axis cs:76.4331210191083,0.143447537823456)
--(axis cs:77.0700636942675,0.135184397908111)
--(axis cs:77.7070063694268,0.124591052487844)
--(axis cs:78.343949044586,0.123142092675422)
--(axis cs:78.9808917197452,0.114543908641043)
--(axis cs:79.6178343949044,0.105913506577274)
--(axis cs:80.2547770700637,0.0958007990100344)
--(axis cs:80.8917197452229,0.0882467377772278)
--(axis cs:81.5286624203822,0.0804053236544626)
--(axis cs:82.1656050955414,0.0748176773744633)
--(axis cs:82.8025477707006,0.0711583328809787)
--(axis cs:83.4394904458599,0.0601046148468988)
--(axis cs:84.0764331210191,0.0562867552772199)
--(axis cs:84.7133757961783,0.0433516485384557)
--(axis cs:85.3503184713376,0.0411609804237049)
--(axis cs:85.9872611464968,0.0367099910600922)
--(axis cs:86.6242038216561,0.0288121982870272)
--(axis cs:87.2611464968153,0.0284563750216775)
--(axis cs:87.8980891719745,0.0215171028855058)
--(axis cs:88.5350318471338,0.0140050844845083)
--(axis cs:89.171974522293,0.0131840611832843)
--(axis cs:89.8089171974522,0.00561356333726215)
--(axis cs:90.4458598726115,0.00538461781706244)
--(axis cs:91.0828025477707,0.00423388567760647)
--(axis cs:91.7197452229299,0.00626324063408438)
--(axis cs:92.3566878980892,0.0052027308319496)
--(axis cs:92.9936305732484,0.00564875053775834)
--(axis cs:93.6305732484076,0.00332908195541535)
--(axis cs:94.2675159235669,0.00218596809545872)
--(axis cs:94.9044585987261,0.00238566440884101)
--(axis cs:95.5414012738853,0.00161261678781711)
--(axis cs:96.1783439490446,0.00101171349297559)
--(axis cs:96.8152866242038,0.00138234766085642)
--(axis cs:97.4522292993631,0.000875815240832553)
--(axis cs:98.0891719745223,0.000594931222369835)
--(axis cs:98.7261146496815,5.3690763217585e-05)
--(axis cs:99.3630573248408,5.32164659810616e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,1.56278335867381e-05)
--(axis cs:98.7261146496815,0.000132546379360121)
--(axis cs:98.0891719745223,0.00158677484406393)
--(axis cs:97.4522292993631,0.00209763899276933)
--(axis cs:96.8152866242038,0.00320887383315172)
--(axis cs:96.1783439490446,0.0027455697060352)
--(axis cs:95.5414012738853,0.0037408768653838)
--(axis cs:94.9044585987261,0.00457070793565525)
--(axis cs:94.2675159235669,0.00395774761687254)
--(axis cs:93.6305732484076,0.00571409705351194)
--(axis cs:92.9936305732484,0.00919351322292675)
--(axis cs:92.3566878980892,0.0085553527628739)
--(axis cs:91.7197452229299,0.00991948064287119)
--(axis cs:91.0828025477707,0.00724802838054531)
--(axis cs:90.4458598726115,0.00854040587261225)
--(axis cs:89.8089171974522,0.00903806005946068)
--(axis cs:89.171974522293,0.0181364356778748)
--(axis cs:88.5350318471338,0.0192413427464087)
--(axis cs:87.8980891719745,0.0278609339931801)
--(axis cs:87.2611464968153,0.0353248214087913)
--(axis cs:86.6242038216561,0.0359334450144398)
--(axis cs:85.9872611464968,0.0438781261692211)
--(axis cs:85.3503184713376,0.0486772984261724)
--(axis cs:84.7133757961783,0.0510990360490131)
--(axis cs:84.0764331210191,0.0642473729644128)
--(axis cs:83.4394904458599,0.0683141849555689)
--(axis cs:82.8025477707006,0.0797416875061387)
--(axis cs:82.1656050955414,0.0837207172267931)
--(axis cs:81.5286624203822,0.0888884251341262)
--(axis cs:80.8917197452229,0.0971457926239384)
--(axis cs:80.2547770700637,0.105260440970955)
--(axis cs:79.6178343949044,0.115217246505074)
--(axis cs:78.9808917197452,0.12383019631582)
--(axis cs:78.343949044586,0.132592740793713)
--(axis cs:77.7070063694268,0.133748578034274)
--(axis cs:77.0700636942675,0.144918121905652)
--(axis cs:76.4331210191083,0.153672374268089)
--(axis cs:75.796178343949,0.15546710622921)
--(axis cs:75.1592356687898,0.161206394123399)
--(axis cs:74.5222929936306,0.172913417152946)
--(axis cs:73.8853503184713,0.178376678201815)
--(axis cs:73.2484076433121,0.181744845709321)
--(axis cs:72.6114649681529,0.190338808722043)
--(axis cs:71.9745222929936,0.194701830123711)
--(axis cs:71.3375796178344,0.199434231301938)
--(axis cs:70.7006369426752,0.206748895690556)
--(axis cs:70.0636942675159,0.208285521283675)
--(axis cs:69.4267515923567,0.218793702712043)
--(axis cs:68.7898089171974,0.226612883793886)
--(axis cs:68.1528662420382,0.228615237695138)
--(axis cs:67.515923566879,0.234010665580281)
--(axis cs:66.8789808917197,0.242376111821796)
--(axis cs:66.2420382165605,0.247606425652188)
--(axis cs:65.6050955414013,0.254418060281957)
--(axis cs:64.968152866242,0.258024624604831)
--(axis cs:64.3312101910828,0.259352627324444)
--(axis cs:63.6942675159236,0.265217839475942)
--(axis cs:63.0573248407643,0.269847198288845)
--(axis cs:62.4203821656051,0.273977715957164)
--(axis cs:61.7834394904459,0.276123041118736)
--(axis cs:61.1464968152866,0.279987030792459)
--(axis cs:60.5095541401274,0.279837466733786)
--(axis cs:59.8726114649682,0.285501244629614)
--(axis cs:59.2356687898089,0.290876719199783)
--(axis cs:58.5987261146497,0.299688569449931)
--(axis cs:57.9617834394904,0.305134044469673)
--(axis cs:57.3248407643312,0.317604749694958)
--(axis cs:56.687898089172,0.317565199662408)
--(axis cs:56.0509554140127,0.320614795792442)
--(axis cs:55.4140127388535,0.327801427288419)
--(axis cs:54.7770700636943,0.329988360599508)
--(axis cs:54.140127388535,0.333089353264528)
--(axis cs:53.5031847133758,0.338790574741924)
--(axis cs:52.8662420382166,0.341470578425751)
--(axis cs:52.2292993630573,0.349314764868174)
--(axis cs:51.5923566878981,0.353559552245593)
--(axis cs:50.9554140127388,0.360466462559973)
--(axis cs:50.3184713375796,0.369353957002031)
--(axis cs:49.6815286624204,0.373557134412088)
--(axis cs:49.0445859872611,0.378802168406807)
--(axis cs:48.4076433121019,0.379328999559037)
--(axis cs:47.7707006369427,0.382224113080847)
--(axis cs:47.1337579617834,0.391055918093317)
--(axis cs:46.4968152866242,0.40107629775712)
--(axis cs:45.859872611465,0.407463466768974)
--(axis cs:45.2229299363057,0.408241743396406)
--(axis cs:44.5859872611465,0.409916757142639)
--(axis cs:43.9490445859873,0.413364721821638)
--(axis cs:43.312101910828,0.417071297599684)
--(axis cs:42.6751592356688,0.425623512933453)
--(axis cs:42.0382165605096,0.423205841935545)
--(axis cs:41.4012738853503,0.425127590805204)
--(axis cs:40.7643312101911,0.42993504347308)
--(axis cs:40.1273885350318,0.432733989617672)
--(axis cs:39.4904458598726,0.434295204462078)
--(axis cs:38.8535031847134,0.437591358492816)
--(axis cs:38.2165605095541,0.44051246167563)
--(axis cs:37.5796178343949,0.442687613303542)
--(axis cs:36.9426751592357,0.446550409920422)
--(axis cs:36.3057324840764,0.444328762888563)
--(axis cs:35.6687898089172,0.445481755532464)
--(axis cs:35.031847133758,0.446183031361111)
--(axis cs:34.3949044585987,0.446118834225767)
--(axis cs:33.7579617834395,0.447023659616375)
--(axis cs:33.1210191082803,0.445149981441716)
--(axis cs:32.484076433121,0.446598419475037)
--(axis cs:31.8471337579618,0.448961296705049)
--(axis cs:31.2101910828025,0.447716625959319)
--(axis cs:30.5732484076433,0.453621025816527)
--(axis cs:29.9363057324841,0.455702638673899)
--(axis cs:29.2993630573248,0.45684291733393)
--(axis cs:28.6624203821656,0.463236062487402)
--(axis cs:28.0254777070064,0.464682826350315)
--(axis cs:27.3885350318471,0.477288438414948)
--(axis cs:26.7515923566879,0.476299847170161)
--(axis cs:26.1146496815287,0.488423162221857)
--(axis cs:25.4777070063694,0.496637662241491)
--(axis cs:24.8407643312102,0.503291698413173)
--(axis cs:24.203821656051,0.510375050624308)
--(axis cs:23.5668789808917,0.520499011255728)
--(axis cs:22.9299363057325,0.524722397190977)
--(axis cs:22.2929936305732,0.52630822017065)
--(axis cs:21.656050955414,0.538540930041526)
--(axis cs:21.0191082802548,0.547492606471147)
--(axis cs:20.3821656050955,0.551642510985247)
--(axis cs:19.7452229299363,0.554829771661446)
--(axis cs:19.1082802547771,0.558699703802569)
--(axis cs:18.4713375796178,0.573805407596289)
--(axis cs:17.8343949044586,0.582670521639834)
--(axis cs:17.1974522292994,0.581941964138706)
--(axis cs:16.5605095541401,0.594920778158511)
--(axis cs:15.9235668789809,0.604846087164978)
--(axis cs:15.2866242038217,0.617767210807674)
--(axis cs:14.6496815286624,0.63252462023071)
--(axis cs:14.0127388535032,0.653001217178766)
--(axis cs:13.3757961783439,0.669097060644654)
--(axis cs:12.7388535031847,0.697374514545237)
--(axis cs:12.1019108280255,0.730125883496622)
--(axis cs:11.4649681528662,0.755849439050756)
--(axis cs:10.828025477707,0.784197113443617)
--(axis cs:10.1910828025478,0.808237292855884)
--(axis cs:9.55414012738853,0.833966794173845)
--(axis cs:8.9171974522293,0.851451855999915)
--(axis cs:8.28025477707006,0.867976693968288)
--(axis cs:7.64331210191083,0.880527724453936)
--(axis cs:7.00636942675159,0.890224495196317)
--(axis cs:6.36942675159236,0.90018587943529)
--(axis cs:5.73248407643312,0.903313334092737)
--(axis cs:5.09554140127389,0.9072845067072)
--(axis cs:4.45859872611465,0.910288479077476)
--(axis cs:3.82165605095541,0.911515987785404)
--(axis cs:3.18471337579618,0.913435588295346)
--(axis cs:2.54777070063694,0.914270085783633)
--(axis cs:1.91082802547771,0.915009200037955)
--(axis cs:1.27388535031847,0.915659173115551)
--(axis cs:0.636942675159236,0.915752965953324)
--(axis cs:0,0.916086952117701)
--cycle;



==> img/mnist/mnist_rate_distortion_fw_150.tex <==
\addplot [line width=0.5, opacity=0.85, color0!75, dashed]
table {%
0 0.915382305146195
0.636942675159236 0.914970141542144
1.27388535031847 0.915084841647185
1.91082802547771 0.914672657441115
2.54777070063694 0.914212327475834
3.18471337579618 0.913220960170729
3.82165605095541 0.912011397884344
4.45859872611465 0.910271116498625
5.09554140127389 0.907805146887258
5.73248407643312 0.904242863203981
6.36942675159236 0.89887599907117
7.00636942675159 0.89520422441361
7.64331210191083 0.888951888805023
8.28025477707006 0.880638122228265
8.9171974522293 0.868310159634566
9.55414012738853 0.856295518966799
10.1910828025478 0.843578426159511
10.828025477707 0.830565461530932
11.4649681528662 0.817466486475096
12.1019108280255 0.799214179835908
12.7388535031847 0.77525200923119
13.3757961783439 0.749825204581139
14.0127388535032 0.719238875922674
14.6496815286624 0.69274621568351
15.2866242038217 0.677618468827859
15.9235668789809 0.644177168639726
16.5605095541401 0.620817931527854
17.1974522292994 0.586886936489318
17.8343949044586 0.560112419125071
18.4713375796178 0.540784668644192
19.1082802547771 0.52021298267442
19.7452229299363 0.503483692744339
20.3821656050955 0.47776432078419
21.0191082802548 0.458168963023927
21.656050955414 0.439330615072395
22.2929936305732 0.42919959536157
22.9299363057325 0.4209430413878
23.5668789808917 0.409909074380994
24.203821656051 0.395285281649558
24.8407643312102 0.382534810423094
25.4777070063694 0.377687550341943
26.1146496815287 0.373940942378395
26.7515923566879 0.368957289527043
27.3885350318471 0.362701479212919
28.0254777070064 0.354345399810209
28.6624203821656 0.344498394426482
29.2993630573248 0.341376342242293
29.9363057324841 0.333345307742711
30.5732484076433 0.332573357403162
31.2101910828025 0.324663926471039
31.8471337579618 0.326913683710081
32.484076433121 0.32659120678898
33.1210191082803 0.320155314767326
33.7579617834395 0.317981679320292
34.3949044585987 0.315988857782431
35.031847133758 0.314326251147104
35.6687898089172 0.315648991679991
36.3057324840764 0.311074124215957
36.9426751592357 0.303930646362633
37.5796178343949 0.310005887124553
38.2165605095541 0.305655508492077
38.8535031847134 0.304070272144517
39.4904458598726 0.301894533724235
40.1273885350318 0.306610746241213
40.7643312101911 0.308196723168026
41.4012738853503 0.315928344662145
42.0382165605096 0.317472639679961
42.6751592356688 0.320852260890761
43.312101910828 0.323383592734087
43.9490445859873 0.324084095048613
44.5859872611465 0.315025142884061
45.2229299363057 0.319152277886892
45.859872611465 0.324026450677074
46.4968152866242 0.329477253943492
47.1337579617834 0.322470641571378
47.7707006369427 0.320690496918135
48.4076433121019 0.315171141381502
49.0445859872611 0.31862039341583
49.6815286624204 0.316848230494065
50.3184713375796 0.311734824253609
50.9554140127388 0.307614620967853
51.5923566878981 0.302967415096702
52.2292993630573 0.295015874015523
52.8662420382166 0.292977945240106
53.5031847133758 0.282742553655186
54.140127388535 0.277017320803066
54.7770700636943 0.269432973751833
55.4140127388535 0.262960019403353
56.0509554140127 0.257977526048065
56.687898089172 0.256306366770026
57.3248407643312 0.249049860456254
57.9617834394904 0.248890964365477
58.5987261146497 0.248453443934136
59.2356687898089 0.246631741499524
59.8726114649682 0.242286956354595
60.5095541401274 0.240139586187467
61.1464968152866 0.230602680317573
61.7834394904459 0.222113800427896
62.4203821656051 0.218848561496974
63.0573248407643 0.218071100309203
63.6942675159236 0.213467243852745
64.3312101910828 0.207500600491375
64.968152866242 0.203095637814268
65.6050955414013 0.202275497348756
66.2420382165605 0.199034020901091
66.8789808917197 0.192352390481352
67.515923566879 0.186327852235178
68.1528662420382 0.183989462302427
68.7898089171974 0.179007989608661
69.4267515923567 0.17743092305233
70.0636942675159 0.174943202085094
70.7006369426752 0.160567141411056
71.3375796178344 0.155472088311443
71.9745222929936 0.148253648234799
72.6114649681529 0.141445912245308
73.2484076433121 0.135317587630301
73.8853503184713 0.128854640219673
74.5222929936306 0.127138316027557
75.1592356687898 0.116780574601628
75.796178343949 0.107932230540745
76.4331210191083 0.0987263976872696
77.0700636942675 0.0924917247439161
77.7070063694268 0.0787820686785256
78.343949044586 0.0704263659529526
78.9808917197452 0.0630980075020162
79.6178343949044 0.0592255251418106
80.2547770700637 0.0540459863126339
80.8917197452229 0.0504102434204068
81.5286624203822 0.0437424893928825
82.1656050955414 0.0402900011166711
82.8025477707006 0.033727828346471
83.4394904458599 0.027088080277011
84.0764331210191 0.0249623583670002
84.7133757961783 0.0214747706534522
85.3503184713376 0.0184794908326025
85.9872611464968 0.0141901189234948
86.6242038216561 0.0126375796409723
87.2611464968153 0.0118995866918935
87.8980891719745 0.00913080077917866
88.5350318471338 0.00738376554214972
89.171974522293 0.0081047640300825
89.8089171974522 0.00785381233154981
90.4458598726115 0.00744030028023375
91.0828025477707 0.00587845486523499
91.7197452229299 0.00305998882238
92.3566878980892 0.0024072016837481
92.9936305732484 0.00127585490933401
93.6305732484076 0.00118067963018619
94.2675159235669 0.000759041461724014
94.9044585987261 0.000429880337973345
95.5414012738853 0.000407883802483096
96.1783439490446 0.00019565841453562
96.8152866242038 0.000245576986824416
97.4522292993631 0.000565680595081441
98.0891719745223 0.00018464280216457
98.7261146496815 9.90368968772942e-05
99.3630573248408 6.23001946863433e-05
100 9.06140229517405e-11
};
\path [fill=color0!75, fill opacity=0.25] 
(axis cs:0,0.916065648687973)
--(axis cs:0,0.914698961604417)
--(axis cs:0.636942675159236,0.914178742193177)
--(axis cs:1.27388535031847,0.914312330621269)
--(axis cs:1.91082802547771,0.913823487536003)
--(axis cs:2.54777070063694,0.91332557810632)
--(axis cs:3.18471337579618,0.912120937017481)
--(axis cs:3.82165605095541,0.910748600635137)
--(axis cs:4.45859872611465,0.908801905995734)
--(axis cs:5.09554140127389,0.906028755456662)
--(axis cs:5.73248407643312,0.902038257130997)
--(axis cs:6.36942675159236,0.896189362701323)
--(axis cs:7.00636942675159,0.892154767658431)
--(axis cs:7.64331210191083,0.885486753772303)
--(axis cs:8.28025477707006,0.876615375473625)
--(axis cs:8.9171974522293,0.863555640177709)
--(axis cs:9.55414012738853,0.85107799730596)
--(axis cs:10.1910828025478,0.837979714940761)
--(axis cs:10.828025477707,0.824565820495591)
--(axis cs:11.4649681528662,0.811126920587564)
--(axis cs:12.1019108280255,0.792491081849883)
--(axis cs:12.7388535031847,0.767967146369385)
--(axis cs:13.3757961783439,0.742198216105419)
--(axis cs:14.0127388535032,0.711138357843287)
--(axis cs:14.6496815286624,0.68463600807267)
--(axis cs:15.2866242038217,0.669359784074849)
--(axis cs:15.9235668789809,0.635616283602039)
--(axis cs:16.5605095541401,0.612441618212129)
--(axis cs:17.1974522292994,0.578488549188169)
--(axis cs:17.8343949044586,0.551724153648689)
--(axis cs:18.4713375796178,0.532486051277059)
--(axis cs:19.1082802547771,0.511909136075548)
--(axis cs:19.7452229299363,0.495083114526696)
--(axis cs:20.3821656050955,0.469644484536083)
--(axis cs:21.0191082802548,0.450174978601461)
--(axis cs:21.656050955414,0.431517887336996)
--(axis cs:22.2929936305732,0.421502943666594)
--(axis cs:22.9299363057325,0.413338736112135)
--(axis cs:23.5668789808917,0.402444126453773)
--(axis cs:24.203821656051,0.387808407225253)
--(axis cs:24.8407643312102,0.37499415032605)
--(axis cs:25.4777070063694,0.370247277324942)
--(axis cs:26.1146496815287,0.366298608904458)
--(axis cs:26.7515923566879,0.361315300388226)
--(axis cs:27.3885350318471,0.355016795813694)
--(axis cs:28.0254777070064,0.346710123875161)
--(axis cs:28.6624203821656,0.336777887401041)
--(axis cs:29.2993630573248,0.333629604019209)
--(axis cs:29.9363057324841,0.325548381981876)
--(axis cs:30.5732484076433,0.324813189627526)
--(axis cs:31.2101910828025,0.316915915485578)
--(axis cs:31.8471337579618,0.319230139046358)
--(axis cs:32.484076433121,0.318715301438513)
--(axis cs:33.1210191082803,0.312277894345818)
--(axis cs:33.7579617834395,0.31011489719962)
--(axis cs:34.3949044585987,0.308266600321594)
--(axis cs:35.031847133758,0.306628402501033)
--(axis cs:35.6687898089172,0.3078844124758)
--(axis cs:36.3057324840764,0.3033783062925)
--(axis cs:36.9426751592357,0.296210123575467)
--(axis cs:37.5796178343949,0.302474501921534)
--(axis cs:38.2165605095541,0.298161148422004)
--(axis cs:38.8535031847134,0.296463163852753)
--(axis cs:39.4904458598726,0.294411314261466)
--(axis cs:40.1273885350318,0.299219873935756)
--(axis cs:40.7643312101911,0.30080569731079)
--(axis cs:41.4012738853503,0.308716723298311)
--(axis cs:42.0382165605096,0.310391143397295)
--(axis cs:42.6751592356688,0.313726464527346)
--(axis cs:43.312101910828,0.316323816036633)
--(axis cs:43.9490445859873,0.316911267483717)
--(axis cs:44.5859872611465,0.307968605298238)
--(axis cs:45.2229299363057,0.312103661206152)
--(axis cs:45.859872611465,0.316830513439785)
--(axis cs:46.4968152866242,0.322550267266227)
--(axis cs:47.1337579617834,0.315668783927383)
--(axis cs:47.7707006369427,0.313926091299527)
--(axis cs:48.4076433121019,0.308472776521296)
--(axis cs:49.0445859872611,0.311859251739822)
--(axis cs:49.6815286624204,0.310142171435545)
--(axis cs:50.3184713375796,0.304836170036508)
--(axis cs:50.9554140127388,0.300810661278206)
--(axis cs:51.5923566878981,0.296238259656308)
--(axis cs:52.2292993630573,0.288283121295588)
--(axis cs:52.8662420382166,0.286308876806651)
--(axis cs:53.5031847133758,0.276253163502774)
--(axis cs:54.140127388535,0.270625147455924)
--(axis cs:54.7770700636943,0.263314261527398)
--(axis cs:55.4140127388535,0.256913027074536)
--(axis cs:56.0509554140127,0.251967754590008)
--(axis cs:56.687898089172,0.250441784110785)
--(axis cs:57.3248407643312,0.243310636544162)
--(axis cs:57.9617834394904,0.243131485471999)
--(axis cs:58.5987261146497,0.242690552724205)
--(axis cs:59.2356687898089,0.241067846827318)
--(axis cs:59.8726114649682,0.236830265391084)
--(axis cs:60.5095541401274,0.234677824695837)
--(axis cs:61.1464968152866,0.22515794047986)
--(axis cs:61.7834394904459,0.216564799871511)
--(axis cs:62.4203821656051,0.21336533473886)
--(axis cs:63.0573248407643,0.212607254742435)
--(axis cs:63.6942675159236,0.207969434447172)
--(axis cs:64.3312101910828,0.201987425640208)
--(axis cs:64.968152866242,0.197703828613316)
--(axis cs:65.6050955414013,0.196811309262465)
--(axis cs:66.2420382165605,0.193436216666272)
--(axis cs:66.8789808917197,0.186900579360765)
--(axis cs:67.515923566879,0.180828256584497)
--(axis cs:68.1528662420382,0.178477676919975)
--(axis cs:68.7898089171974,0.173586078220833)
--(axis cs:69.4267515923567,0.172032386324866)
--(axis cs:70.0636942675159,0.169391036762798)
--(axis cs:70.7006369426752,0.154792648041904)
--(axis cs:71.3375796178344,0.149649948078517)
--(axis cs:71.9745222929936,0.142426430518202)
--(axis cs:72.6114649681529,0.135680825787101)
--(axis cs:73.2484076433121,0.129740063063384)
--(axis cs:73.8853503184713,0.123223271169249)
--(axis cs:74.5222929936306,0.121614016831066)
--(axis cs:75.1592356687898,0.111462377664042)
--(axis cs:75.796178343949,0.102794126073818)
--(axis cs:76.4331210191083,0.0937238572814889)
--(axis cs:77.0700636942675,0.0876335408298713)
--(axis cs:77.7070063694268,0.0742214997192665)
--(axis cs:78.343949044586,0.0663163087465938)
--(axis cs:78.9808917197452,0.0592316424397984)
--(axis cs:79.6178343949044,0.055680068563668)
--(axis cs:80.2547770700637,0.050559789978431)
--(axis cs:80.8917197452229,0.0470644651073618)
--(axis cs:81.5286624203822,0.0407055799530025)
--(axis cs:82.1656050955414,0.0374622752069727)
--(axis cs:82.8025477707006,0.0309137909846686)
--(axis cs:83.4394904458599,0.0245868413235545)
--(axis cs:84.0764331210191,0.0223595881545069)
--(axis cs:84.7133757961783,0.0190594931323819)
--(axis cs:85.3503184713376,0.0161062051503495)
--(axis cs:85.9872611464968,0.0120442067036494)
--(axis cs:86.6242038216561,0.0105592409643877)
--(axis cs:87.2611464968153,0.0098986716458805)
--(axis cs:87.8980891719745,0.00734246573397169)
--(axis cs:88.5350318471338,0.00568431364337512)
--(axis cs:89.171974522293,0.00637427738420478)
--(axis cs:89.8089171974522,0.00615307406314854)
--(axis cs:90.4458598726115,0.00574431157852929)
--(axis cs:91.0828025477707,0.00439489317048214)
--(axis cs:91.7197452229299,0.00210894498102751)
--(axis cs:92.3566878980892,0.00145509022827269)
--(axis cs:92.9936305732484,0.000706793805509834)
--(axis cs:93.6305732484076,0.000557843299028199)
--(axis cs:94.2675159235669,0.000297784437512988)
--(axis cs:94.9044585987261,0.000175013717891369)
--(axis cs:95.5414012738853,0.000110465842467018)
--(axis cs:96.1783439490446,3.43298167830343e-05)
--(axis cs:96.8152866242038,0.000109909609385617)
--(axis cs:97.4522292993631,0.000241712061962342)
--(axis cs:98.0891719745223,8.11361284313837e-05)
--(axis cs:98.7261146496815,4.03713184043205e-05)
--(axis cs:99.3630573248408,3.54949883657508e-05)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:99.3630573248408,8.91054010069358e-05)
--(axis cs:98.7261146496815,0.000157702475350268)
--(axis cs:98.0891719745223,0.000288149475897756)
--(axis cs:97.4522292993631,0.000889649128200541)
--(axis cs:96.8152866242038,0.000381244364263214)
--(axis cs:96.1783439490446,0.000356987012288206)
--(axis cs:95.5414012738853,0.000705301762499174)
--(axis cs:94.9044585987261,0.000684746958055321)
--(axis cs:94.2675159235669,0.00122029848593504)
--(axis cs:93.6305732484076,0.00180351596134417)
--(axis cs:92.9936305732484,0.00184491601315818)
--(axis cs:92.3566878980892,0.00335931313922352)
--(axis cs:91.7197452229299,0.0040110326637325)
--(axis cs:91.0828025477707,0.00736201655998785)
--(axis cs:90.4458598726115,0.00913628898193821)
--(axis cs:89.8089171974522,0.00955455059995109)
--(axis cs:89.171974522293,0.00983525067596021)
--(axis cs:88.5350318471338,0.00908321744092431)
--(axis cs:87.8980891719745,0.0109191358243856)
--(axis cs:87.2611464968153,0.0139005017379065)
--(axis cs:86.6242038216561,0.014715918317557)
--(axis cs:85.9872611464968,0.0163360311433402)
--(axis cs:85.3503184713376,0.0208527765148555)
--(axis cs:84.7133757961783,0.0238900481745224)
--(axis cs:84.0764331210191,0.0275651285794934)
--(axis cs:83.4394904458599,0.0295893192304675)
--(axis cs:82.8025477707006,0.0365418657082734)
--(axis cs:82.1656050955414,0.0431177270263696)
--(axis cs:81.5286624203822,0.0467793988327625)
--(axis cs:80.8917197452229,0.0537560217334518)
--(axis cs:80.2547770700637,0.0575321826468368)
--(axis cs:79.6178343949044,0.0627709817199531)
--(axis cs:78.9808917197452,0.066964372564234)
--(axis cs:78.343949044586,0.0745364231593114)
--(axis cs:77.7070063694268,0.0833426376377847)
--(axis cs:77.0700636942675,0.0973499086579609)
--(axis cs:76.4331210191083,0.10372893809305)
--(axis cs:75.796178343949,0.113070335007671)
--(axis cs:75.1592356687898,0.122098771539215)
--(axis cs:74.5222929936306,0.132662615224047)
--(axis cs:73.8853503184713,0.134486009270097)
--(axis cs:73.2484076433121,0.140895112197219)
--(axis cs:72.6114649681529,0.147210998703515)
--(axis cs:71.9745222929936,0.154080865951397)
--(axis cs:71.3375796178344,0.161294228544369)
--(axis cs:70.7006369426752,0.166341634780208)
--(axis cs:70.0636942675159,0.180495367407391)
--(axis cs:69.4267515923567,0.182829459779794)
--(axis cs:68.7898089171974,0.184429900996488)
--(axis cs:68.1528662420382,0.189501247684879)
--(axis cs:67.515923566879,0.19182744788586)
--(axis cs:66.8789808917197,0.197804201601939)
--(axis cs:66.2420382165605,0.204631825135911)
--(axis cs:65.6050955414013,0.207739685435046)
--(axis cs:64.968152866242,0.208487447015219)
--(axis cs:64.3312101910828,0.213013775342542)
--(axis cs:63.6942675159236,0.218965053258318)
--(axis cs:63.0573248407643,0.223534945875971)
--(axis cs:62.4203821656051,0.224331788255087)
--(axis cs:61.7834394904459,0.227662800984281)
--(axis cs:61.1464968152866,0.236047420155286)
--(axis cs:60.5095541401274,0.245601347679096)
--(axis cs:59.8726114649682,0.247743647318106)
--(axis cs:59.2356687898089,0.252195636171729)
--(axis cs:58.5987261146497,0.254216335144067)
--(axis cs:57.9617834394904,0.254650443258954)
--(axis cs:57.3248407643312,0.254789084368345)
--(axis cs:56.687898089172,0.262170949429267)
--(axis cs:56.0509554140127,0.263987297506122)
--(axis cs:55.4140127388535,0.269007011732171)
--(axis cs:54.7770700636943,0.275551685976269)
--(axis cs:54.140127388535,0.283409494150209)
--(axis cs:53.5031847133758,0.289231943807598)
--(axis cs:52.8662420382166,0.299647013673561)
--(axis cs:52.2292993630573,0.301748626735458)
--(axis cs:51.5923566878981,0.309696570537096)
--(axis cs:50.9554140127388,0.3144185806575)
--(axis cs:50.3184713375796,0.31863347847071)
--(axis cs:49.6815286624204,0.323554289552584)
--(axis cs:49.0445859872611,0.325381535091837)
--(axis cs:48.4076433121019,0.321869506241707)
--(axis cs:47.7707006369427,0.327454902536743)
--(axis cs:47.1337579617834,0.329272499215373)
--(axis cs:46.4968152866242,0.336404240620757)
--(axis cs:45.859872611465,0.331222387914363)
--(axis cs:45.2229299363057,0.326200894567632)
--(axis cs:44.5859872611465,0.322081680469885)
--(axis cs:43.9490445859873,0.331256922613508)
--(axis cs:43.312101910828,0.330443369431542)
--(axis cs:42.6751592356688,0.327978057254176)
--(axis cs:42.0382165605096,0.324554135962627)
--(axis cs:41.4012738853503,0.323139966025979)
--(axis cs:40.7643312101911,0.315587749025262)
--(axis cs:40.1273885350318,0.31400161854667)
--(axis cs:39.4904458598726,0.309377753187004)
--(axis cs:38.8535031847134,0.31167738043628)
--(axis cs:38.2165605095541,0.313149868562151)
--(axis cs:37.5796178343949,0.317537272327572)
--(axis cs:36.9426751592357,0.311651169149798)
--(axis cs:36.3057324840764,0.318769942139413)
--(axis cs:35.6687898089172,0.323413570884182)
--(axis cs:35.031847133758,0.322024099793175)
--(axis cs:34.3949044585987,0.323711115243268)
--(axis cs:33.7579617834395,0.325848461440964)
--(axis cs:33.1210191082803,0.328032735188834)
--(axis cs:32.484076433121,0.334467112139448)
--(axis cs:31.8471337579618,0.334597228373805)
--(axis cs:31.2101910828025,0.332411937456501)
--(axis cs:30.5732484076433,0.340333525178798)
--(axis cs:29.9363057324841,0.341142233503546)
--(axis cs:29.2993630573248,0.349123080465376)
--(axis cs:28.6624203821656,0.352218901451924)
--(axis cs:28.0254777070064,0.361980675745256)
--(axis cs:27.3885350318471,0.370386162612144)
--(axis cs:26.7515923566879,0.37659927866586)
--(axis cs:26.1146496815287,0.381583275852331)
--(axis cs:25.4777070063694,0.385127823358945)
--(axis cs:24.8407643312102,0.390075470520139)
--(axis cs:24.203821656051,0.402762156073863)
--(axis cs:23.5668789808917,0.417374022308215)
--(axis cs:22.9299363057325,0.428547346663465)
--(axis cs:22.2929936305732,0.436896247056545)
--(axis cs:21.656050955414,0.447143342807794)
--(axis cs:21.0191082802548,0.466162947446393)
--(axis cs:20.3821656050955,0.485884157032297)
--(axis cs:19.7452229299363,0.511884270961983)
--(axis cs:19.1082802547771,0.528516829273293)
--(axis cs:18.4713375796178,0.549083286011324)
--(axis cs:17.8343949044586,0.568500684601453)
--(axis cs:17.1974522292994,0.595285323790467)
--(axis cs:16.5605095541401,0.629194244843579)
--(axis cs:15.9235668789809,0.652738053677413)
--(axis cs:15.2866242038217,0.685877153580869)
--(axis cs:14.6496815286624,0.70085642329435)
--(axis cs:14.0127388535032,0.727339394002062)
--(axis cs:13.3757961783439,0.757452193056858)
--(axis cs:12.7388535031847,0.782536872092995)
--(axis cs:12.1019108280255,0.805937277821933)
--(axis cs:11.4649681528662,0.823806052362627)
--(axis cs:10.828025477707,0.836565102566273)
--(axis cs:10.1910828025478,0.849177137378261)
--(axis cs:9.55414012738853,0.861513040627638)
--(axis cs:8.9171974522293,0.873064679091422)
--(axis cs:8.28025477707006,0.884660868982906)
--(axis cs:7.64331210191083,0.892417023837742)
--(axis cs:7.00636942675159,0.898253681168789)
--(axis cs:6.36942675159236,0.901562635441016)
--(axis cs:5.73248407643312,0.906447469276965)
--(axis cs:5.09554140127389,0.909581538317855)
--(axis cs:4.45859872611465,0.911740327001516)
--(axis cs:3.82165605095541,0.91327419513355)
--(axis cs:3.18471337579618,0.914320983323977)
--(axis cs:2.54777070063694,0.915099076845348)
--(axis cs:1.91082802547771,0.915521827346228)
--(axis cs:1.27388535031847,0.915857352673102)
--(axis cs:0.636942675159236,0.915761540891111)
--(axis cs:0,0.916065648687973)
--cycle;


==> img/mnist/mnist_rate_distortion_fw_200.tex <==
\addplot [line width=0.5, opacity=0.85, color0!75, dashed]
table {%
0 0.915336998354178
0.636942675159236 0.91527969366929
1.27388535031847 0.915424975655624
1.91082802547771 0.914980346090742
2.54777070063694 0.914191121368785
3.18471337579618 0.913857269308064
3.82165605095541 0.912954539865605
4.45859872611465 0.911590013286332
5.09554140127389 0.910129435591516
5.73248407643312 0.907884511603625
6.36942675159236 0.903981410004199
7.00636942675159 0.899894725492341
7.64331210191083 0.894269491572631
8.28025477707006 0.887334489763889
8.9171974522293 0.879755109753169
9.55414012738853 0.865521906107024
10.1910828025478 0.857944057137356
10.828025477707 0.849059872928337
11.4649681528662 0.839037938176116
12.1019108280255 0.826899032744841
12.7388535031847 0.812808692029721
13.3757961783439 0.791551930957648
14.0127388535032 0.773633865622687
14.6496815286624 0.749404071915778
15.2866242038217 0.725291715928761
15.9235668789809 0.705095244854747
16.5605095541401 0.684912407622178
17.1974522292994 0.667099782184232
17.8343949044586 0.645325416859851
18.4713375796178 0.61533122525725
19.1082802547771 0.593032807420532
19.7452229299363 0.562717344262346
20.3821656050955 0.533577852824674
21.0191082802548 0.512306244846113
21.656050955414 0.490131680357008
22.2929936305732 0.468395432107718
22.9299363057325 0.449262050886464
23.5668789808917 0.428997575010289
24.203821656051 0.413518730478245
24.8407643312102 0.397034638482146
25.4777070063694 0.381514865817844
26.1146496815287 0.352923213185304
26.7515923566879 0.334114688837908
27.3885350318471 0.312353535615348
28.0254777070064 0.29982803375864
28.6624203821656 0.282132011487774
29.2993630573248 0.267311416240402
29.9363057324841 0.262278393500208
30.5732484076433 0.251373370497524
31.2101910828025 0.239368919042212
31.8471337579618 0.236331141119901
32.484076433121 0.225785426257954
33.1210191082803 0.216698216451191
33.7579617834395 0.213377448141437
34.3949044585987 0.215369425948024
35.031847133758 0.219543166866946
35.6687898089172 0.211077684837879
36.3057324840764 0.210096727543437
36.9426751592357 0.200605016596218
37.5796178343949 0.199153514450253
38.2165605095541 0.193720261009594
38.8535031847134 0.189281908830815
39.4904458598726 0.186300442287629
40.1273885350318 0.185666617064987
40.7643312101911 0.181769082941995
41.4012738853503 0.179014565436585
42.0382165605096 0.171164093773073
42.6751592356688 0.177085024226765
43.312101910828 0.172788143362433
43.9490445859873 0.172375999580338
44.5859872611465 0.178134488899382
45.2229299363057 0.177858380607846
45.859872611465 0.189362123835042
46.4968152866242 0.191314521515797
47.1337579617834 0.189467437456386
47.7707006369427 0.181427372500093
48.4076433121019 0.177252764651539
49.0445859872611 0.179996869832778
49.6815286624204 0.178178518025788
50.3184713375796 0.172918597627581
50.9554140127388 0.167952613768944
51.5923566878981 0.167160619347237
52.2292993630573 0.167040993747515
52.8662420382166 0.160383777669716
53.5031847133758 0.161861901380567
54.140127388535 0.165598488068045
54.7770700636943 0.164171006220101
55.4140127388535 0.161012829266463
56.0509554140127 0.16024769152069
56.687898089172 0.161139763459579
57.3248407643312 0.160719817747532
57.9617834394904 0.163845860580979
58.5987261146497 0.157976482447469
59.2356687898089 0.151689394723265
59.8726114649682 0.143248847313807
60.5095541401274 0.138398800110802
61.1464968152866 0.139034481840827
61.7834394904459 0.139816634096209
62.4203821656051 0.1352382834098
63.0573248407643 0.136441580585409
63.6942675159236 0.128465162533377
64.3312101910828 0.127649235514688
64.968152866242 0.1306642813212
65.6050955414013 0.122002492357379
66.2420382165605 0.112865219990293
66.8789808917197 0.100983891253821
67.515923566879 0.0963928275010844
68.1528662420382 0.0881251486991415
68.7898089171974 0.0901750602982459
69.4267515923567 0.0877991904655302
70.0636942675159 0.0891461021971327
70.7006369426752 0.0833836160948399
71.3375796178344 0.0829093757293814
71.9745222929936 0.0793818205335489
72.6114649681529 0.0797828547676361
73.2484076433121 0.0753242612097613
73.8853503184713 0.0703508535537887
74.5222929936306 0.0674488634540804
75.1592356687898 0.065087613519274
75.796178343949 0.0616689455168052
76.4331210191083 0.0547234052113347
77.0700636942675 0.0513111368798877
77.7070063694268 0.0481177876826315
78.343949044586 0.042830142404885
78.9808917197452 0.0391912810553212
79.6178343949044 0.0368622138908306
80.2547770700637 0.0313557576973151
80.8917197452229 0.0281116643202067
81.5286624203822 0.0250639856809307
82.1656050955414 0.0222087528368606
82.8025477707006 0.0216949959132656
83.4394904458599 0.0217054664667826
84.0764331210191 0.0204697811400261
84.7133757961783 0.0190991979956269
85.3503184713376 0.0164809116780654
85.9872611464968 0.0111475273382571
86.6242038216561 0.00919895314330458
87.2611464968153 0.00853665513772888
87.8980891719745 0.00737760097173887
88.5350318471338 0.00633601746684641
89.171974522293 0.00507944542504771
89.8089171974522 0.00432475832600435
90.4458598726115 0.00762210627747234
91.0828025477707 0.00381887025379746
91.7197452229299 0.00344830983026665
92.3566878980892 0.00216063900413306
92.9936305732484 0.00212456099440563
93.6305732484076 0.00184567115964462
94.2675159235669 0.00158848398049769
94.9044585987261 0.000727119561105481
95.5414012738853 0.000409845907038312
96.1783439490446 0.000385222704407486
96.8152866242038 0.000325040071403012
97.4522292993631 0.000229255270954046
98.0891719745223 0.000240667420584363
98.7261146496815 2.60579792355303e-05
99.3630573248408 1.29596769179774e-05
100 9.06140229517405e-11
};
\path [fill=color0!75, fill opacity=0.25] 
(axis cs:0,0.916028047168889)
--(axis cs:0,0.914645949539467)
--(axis cs:0.636942675159236,0.914553862602438)
--(axis cs:1.27388535031847,0.914809954016748)
--(axis cs:1.91082802547771,0.914231191292449)
--(axis cs:2.54777070063694,0.913309571716946)
--(axis cs:3.18471337579618,0.912963051694721)
--(axis cs:3.82165605095541,0.911927598571337)
--(axis cs:4.45859872611465,0.910242526096413)
--(axis cs:5.09554140127389,0.908677788687288)
--(axis cs:5.73248407643312,0.906088270503529)
--(axis cs:6.36942675159236,0.901766241683449)
--(axis cs:7.00636942675159,0.897298120275921)
--(axis cs:7.64331210191083,0.891158968775485)
--(axis cs:8.28025477707006,0.883751312135102)
--(axis cs:8.9171974522293,0.875664762399157)
--(axis cs:9.55414012738853,0.860617567919947)
--(axis cs:10.1910828025478,0.852776065417512)
--(axis cs:10.828025477707,0.843619687060235)
--(axis cs:11.4649681528662,0.833179488669314)
--(axis cs:12.1019108280255,0.820618440768605)
--(axis cs:12.7388535031847,0.806144983310874)
--(axis cs:13.3757961783439,0.78440102457766)
--(axis cs:14.0127388535032,0.766106628936085)
--(axis cs:14.6496815286624,0.74176006807102)
--(axis cs:15.2866242038217,0.717350410843549)
--(axis cs:15.9235668789809,0.696904512731689)
--(axis cs:16.5605095541401,0.676645790447651)
--(axis cs:17.1974522292994,0.65859074486282)
--(axis cs:17.8343949044586,0.63650139066753)
--(axis cs:18.4713375796178,0.606285578788079)
--(axis cs:19.1082802547771,0.583814347192083)
--(axis cs:19.7452229299363,0.553467694904245)
--(axis cs:20.3821656050955,0.524542677312382)
--(axis cs:21.0191082802548,0.503533723254122)
--(axis cs:21.656050955414,0.481219796704006)
--(axis cs:22.2929936305732,0.459616944875645)
--(axis cs:22.9299363057325,0.440560850189949)
--(axis cs:23.5668789808917,0.420306906589006)
--(axis cs:24.203821656051,0.404641952524779)
--(axis cs:24.8407643312102,0.388095863203821)
--(axis cs:25.4777070063694,0.372631646333615)
--(axis cs:26.1146496815287,0.344275508659895)
--(axis cs:26.7515923566879,0.32551476650928)
--(axis cs:27.3885350318471,0.304070617434083)
--(axis cs:28.0254777070064,0.291549323875439)
--(axis cs:28.6624203821656,0.274074363530599)
--(axis cs:29.2993630573248,0.259283121667893)
--(axis cs:29.9363057324841,0.254541792250576)
--(axis cs:30.5732484076433,0.243713387954952)
--(axis cs:31.2101910828025,0.231989135194483)
--(axis cs:31.8471337579618,0.229113795822212)
--(axis cs:32.484076433121,0.218574013959576)
--(axis cs:33.1210191082803,0.209624948847585)
--(axis cs:33.7579617834395,0.206407765440098)
--(axis cs:34.3949044585987,0.208410959424762)
--(axis cs:35.031847133758,0.212643138871969)
--(axis cs:35.6687898089172,0.204367578928953)
--(axis cs:36.3057324840764,0.203337533085796)
--(axis cs:36.9426751592357,0.194001054583566)
--(axis cs:37.5796178343949,0.19269266206461)
--(axis cs:38.2165605095541,0.187467017835692)
--(axis cs:38.8535031847134,0.18305712618489)
--(axis cs:39.4904458598726,0.180255492350585)
--(axis cs:40.1273885350318,0.179457964794283)
--(axis cs:40.7643312101911,0.175702623508494)
--(axis cs:41.4012738853503,0.172869015497743)
--(axis cs:42.0382165605096,0.1651993299639)
--(axis cs:42.6751592356688,0.171031271814982)
--(axis cs:43.312101910828,0.1667344880605)
--(axis cs:43.9490445859873,0.16638119748207)
--(axis cs:44.5859872611465,0.172222359604464)
--(axis cs:45.2229299363057,0.172011284171101)
--(axis cs:45.859872611465,0.183449762284082)
--(axis cs:46.4968152866242,0.185489439206882)
--(axis cs:47.1337579617834,0.183667901388204)
--(axis cs:47.7707006369427,0.175651554091129)
--(axis cs:48.4076433121019,0.17135307863189)
--(axis cs:49.0445859872611,0.174253004871743)
--(axis cs:49.6815286624204,0.172516291121175)
--(axis cs:50.3184713375796,0.167319104831668)
--(axis cs:50.9554140127388,0.16244996908118)
--(axis cs:51.5923566878981,0.161674257321904)
--(axis cs:52.2292993630573,0.16134550780624)
--(axis cs:52.8662420382166,0.154685883519845)
--(axis cs:53.5031847133758,0.156068060028681)
--(axis cs:54.140127388535,0.159790425769249)
--(axis cs:54.7770700636943,0.158567244275527)
--(axis cs:55.4140127388535,0.15553431395548)
--(axis cs:56.0509554140127,0.154799689867062)
--(axis cs:56.687898089172,0.155652577459207)
--(axis cs:57.3248407643312,0.155209517740009)
--(axis cs:57.9617834394904,0.158474182356609)
--(axis cs:58.5987261146497,0.15245659752212)
--(axis cs:59.2356687898089,0.146217992895622)
--(axis cs:59.8726114649682,0.137680973831866)
--(axis cs:60.5095541401274,0.132742072196376)
--(axis cs:61.1464968152866,0.133541671853761)
--(axis cs:61.7834394904459,0.134409051364712)
--(axis cs:62.4203821656051,0.129934673226699)
--(axis cs:63.0573248407643,0.131125893180125)
--(axis cs:63.6942675159236,0.123160118205009)
--(axis cs:64.3312101910828,0.122184775558156)
--(axis cs:64.968152866242,0.125150356743206)
--(axis cs:65.6050955414013,0.11665469038585)
--(axis cs:66.2420382165605,0.107683182723911)
--(axis cs:66.8789808917197,0.0960686437606275)
--(axis cs:67.515923566879,0.0916122271364423)
--(axis cs:68.1528662420382,0.0837394615139028)
--(axis cs:68.7898089171974,0.0858284732540841)
--(axis cs:69.4267515923567,0.0836283173658112)
--(axis cs:70.0636942675159,0.0849252136327837)
--(axis cs:70.7006369426752,0.0792290651634985)
--(axis cs:71.3375796178344,0.0789068756459381)
--(axis cs:71.9745222929936,0.0756760297199086)
--(axis cs:72.6114649681529,0.075992929347153)
--(axis cs:73.2484076433121,0.0715370875757836)
--(axis cs:73.8853503184713,0.0666151227136488)
--(axis cs:74.5222929936306,0.0637379336324312)
--(axis cs:75.1592356687898,0.0614349738383262)
--(axis cs:75.796178343949,0.0581241812445907)
--(axis cs:76.4331210191083,0.0514047854976002)
--(axis cs:77.0700636942675,0.0481830462176767)
--(axis cs:77.7070063694268,0.045218304247203)
--(axis cs:78.343949044586,0.0400781280178797)
--(axis cs:78.9808917197452,0.0365617999345159)
--(axis cs:79.6178343949044,0.0344359584365918)
--(axis cs:80.2547770700637,0.029274688284973)
--(axis cs:80.8917197452229,0.0261806779465479)
--(axis cs:81.5286624203822,0.0229781728895224)
--(axis cs:82.1656050955414,0.0202133645463148)
--(axis cs:82.8025477707006,0.0196279213417114)
--(axis cs:83.4394904458599,0.019861549932895)
--(axis cs:84.0764331210191,0.0184682694934263)
--(axis cs:84.7133757961783,0.0172444326215873)
--(axis cs:85.3503184713376,0.0147908645015905)
--(axis cs:85.9872611464968,0.0094045396852071)
--(axis cs:86.6242038216561,0.00753368793033128)
--(axis cs:87.2611464968153,0.00693430258709639)
--(axis cs:87.8980891719745,0.00583892421456684)
--(axis cs:88.5350318471338,0.00486163792875743)
--(axis cs:89.171974522293,0.0036809755943896)
--(axis cs:89.8089171974522,0.00307145528456702)
--(axis cs:90.4458598726115,0.005988961053796)
--(axis cs:91.0828025477707,0.00259168201354727)
--(axis cs:91.7197452229299,0.00231983210885854)
--(axis cs:92.3566878980892,0.00127478043679841)
--(axis cs:92.9936305732484,0.00133707592238649)
--(axis cs:93.6305732484076,0.00109466797372785)
--(axis cs:94.2675159235669,0.000918908117239581)
--(axis cs:94.9044585987261,0.000360607897215902)
--(axis cs:95.5414012738853,0.000153720167489084)
--(axis cs:96.1783439490446,0.000167856799766486)
--(axis cs:96.8152866242038,0.000122522875146366)
--(axis cs:97.4522292993631,0.000103316244247964)
--(axis cs:98.0891719745223,0.000110626553341494)
--(axis cs:98.7261146496815,8.81943984442484e-06)
--(axis cs:99.3630573248408,5.65552082235478e-06)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:99.3630573248408,2.02638330136e-05)
--(axis cs:98.7261146496815,4.32965186266358e-05)
--(axis cs:98.0891719745223,0.000370708287827231)
--(axis cs:97.4522292993631,0.000355194297660128)
--(axis cs:96.8152866242038,0.000527557267659658)
--(axis cs:96.1783439490446,0.000602588609048487)
--(axis cs:95.5414012738853,0.00066597164658754)
--(axis cs:94.9044585987261,0.00109363122499506)
--(axis cs:94.2675159235669,0.00225805984375581)
--(axis cs:93.6305732484076,0.00259667434556139)
--(axis cs:92.9936305732484,0.00291204606642476)
--(axis cs:92.3566878980892,0.00304649757146771)
--(axis cs:91.7197452229299,0.00457678755167476)
--(axis cs:91.0828025477707,0.00504605849404766)
--(axis cs:90.4458598726115,0.00925525150114867)
--(axis cs:89.8089171974522,0.00557806136744168)
--(axis cs:89.171974522293,0.00647791525570582)
--(axis cs:88.5350318471338,0.00781039700493538)
--(axis cs:87.8980891719745,0.0089162777289109)
--(axis cs:87.2611464968153,0.0101390076883614)
--(axis cs:86.6242038216561,0.0108642183562779)
--(axis cs:85.9872611464968,0.0128905149913071)
--(axis cs:85.3503184713376,0.0181709588545402)
--(axis cs:84.7133757961783,0.0209539633696665)
--(axis cs:84.0764331210191,0.0224712927866259)
--(axis cs:83.4394904458599,0.0235493830006703)
--(axis cs:82.8025477707006,0.0237620704848198)
--(axis cs:82.1656050955414,0.0242041411274063)
--(axis cs:81.5286624203822,0.027149798472339)
--(axis cs:80.8917197452229,0.0300426506938656)
--(axis cs:80.2547770700637,0.0334368271096571)
--(axis cs:79.6178343949044,0.0392884693450695)
--(axis cs:78.9808917197452,0.0418207621761265)
--(axis cs:78.343949044586,0.0455821567918902)
--(axis cs:77.7070063694268,0.05101727111806)
--(axis cs:77.0700636942675,0.0544392275420987)
--(axis cs:76.4331210191083,0.0580420249250691)
--(axis cs:75.796178343949,0.0652137097890197)
--(axis cs:75.1592356687898,0.0687402532002218)
--(axis cs:74.5222929936306,0.0711597932757295)
--(axis cs:73.8853503184713,0.0740865843939285)
--(axis cs:73.2484076433121,0.079111434843739)
--(axis cs:72.6114649681529,0.0835727801881192)
--(axis cs:71.9745222929936,0.0830876113471893)
--(axis cs:71.3375796178344,0.0869118758128247)
--(axis cs:70.7006369426752,0.0875381670261813)
--(axis cs:70.0636942675159,0.0933669907614817)
--(axis cs:69.4267515923567,0.0919700635652492)
--(axis cs:68.7898089171974,0.0945216473424077)
--(axis cs:68.1528662420382,0.0925108358843802)
--(axis cs:67.515923566879,0.101173427865726)
--(axis cs:66.8789808917197,0.105899138747014)
--(axis cs:66.2420382165605,0.118047257256675)
--(axis cs:65.6050955414013,0.127350294328908)
--(axis cs:64.968152866242,0.136178205899194)
--(axis cs:64.3312101910828,0.13311369547122)
--(axis cs:63.6942675159236,0.133770206861746)
--(axis cs:63.0573248407643,0.141757267990693)
--(axis cs:62.4203821656051,0.140541893592901)
--(axis cs:61.7834394904459,0.145224216827706)
--(axis cs:61.1464968152866,0.144527291827894)
--(axis cs:60.5095541401274,0.144055528025228)
--(axis cs:59.8726114649682,0.148816720795748)
--(axis cs:59.2356687898089,0.157160796550907)
--(axis cs:58.5987261146497,0.163496367372819)
--(axis cs:57.9617834394904,0.169217538805348)
--(axis cs:57.3248407643312,0.166230117755055)
--(axis cs:56.687898089172,0.16662694945995)
--(axis cs:56.0509554140127,0.165695693174318)
--(axis cs:55.4140127388535,0.166491344577446)
--(axis cs:54.7770700636943,0.169774768164675)
--(axis cs:54.140127388535,0.171406550366842)
--(axis cs:53.5031847133758,0.167655742732453)
--(axis cs:52.8662420382166,0.166081671819587)
--(axis cs:52.2292993630573,0.172736479688791)
--(axis cs:51.5923566878981,0.17264698137257)
--(axis cs:50.9554140127388,0.173455258456708)
--(axis cs:50.3184713375796,0.178518090423495)
--(axis cs:49.6815286624204,0.183840744930401)
--(axis cs:49.0445859872611,0.185740734793814)
--(axis cs:48.4076433121019,0.183152450671187)
--(axis cs:47.7707006369427,0.187203190909056)
--(axis cs:47.1337579617834,0.195266973524568)
--(axis cs:46.4968152866242,0.197139603824712)
--(axis cs:45.859872611465,0.195274485386002)
--(axis cs:45.2229299363057,0.183705477044592)
--(axis cs:44.5859872611465,0.184046618194299)
--(axis cs:43.9490445859873,0.178370801678607)
--(axis cs:43.312101910828,0.178841798664367)
--(axis cs:42.6751592356688,0.183138776638548)
--(axis cs:42.0382165605096,0.177128857582246)
--(axis cs:41.4012738853503,0.185160115375428)
--(axis cs:40.7643312101911,0.187835542375495)
--(axis cs:40.1273885350318,0.191875269335692)
--(axis cs:39.4904458598726,0.192345392224672)
--(axis cs:38.8535031847134,0.195506691476739)
--(axis cs:38.2165605095541,0.199973504183497)
--(axis cs:37.5796178343949,0.205614366835895)
--(axis cs:36.9426751592357,0.207208978608871)
--(axis cs:36.3057324840764,0.216855922001078)
--(axis cs:35.6687898089172,0.217787790746806)
--(axis cs:35.031847133758,0.226443194861923)
--(axis cs:34.3949044585987,0.222327892471286)
--(axis cs:33.7579617834395,0.220347130842775)
--(axis cs:33.1210191082803,0.223771484054797)
--(axis cs:32.484076433121,0.232996838556332)
--(axis cs:31.8471337579618,0.24354848641759)
--(axis cs:31.2101910828025,0.24674870288994)
--(axis cs:30.5732484076433,0.259033353040097)
--(axis cs:29.9363057324841,0.270014994749839)
--(axis cs:29.2993630573248,0.275339710812911)
--(axis cs:28.6624203821656,0.29018965944495)
--(axis cs:28.0254777070064,0.308106743641842)
--(axis cs:27.3885350318471,0.320636453796613)
--(axis cs:26.7515923566879,0.342714611166536)
--(axis cs:26.1146496815287,0.361570917710713)
--(axis cs:25.4777070063694,0.390398085302073)
--(axis cs:24.8407643312102,0.405973413760471)
--(axis cs:24.203821656051,0.422395508431711)
--(axis cs:23.5668789808917,0.437688243431572)
--(axis cs:22.9299363057325,0.457963251582979)
--(axis cs:22.2929936305732,0.477173919339792)
--(axis cs:21.656050955414,0.49904356401001)
--(axis cs:21.0191082802548,0.521078766438105)
--(axis cs:20.3821656050955,0.542613028336965)
--(axis cs:19.7452229299363,0.571966993620448)
--(axis cs:19.1082802547771,0.602251267648981)
--(axis cs:18.4713375796178,0.624376871726422)
--(axis cs:17.8343949044586,0.654149443052172)
--(axis cs:17.1974522292994,0.675608819505644)
--(axis cs:16.5605095541401,0.693179024796705)
--(axis cs:15.9235668789809,0.713285976977805)
--(axis cs:15.2866242038217,0.733233021013973)
--(axis cs:14.6496815286624,0.757048075760537)
--(axis cs:14.0127388535032,0.78116110230929)
--(axis cs:13.3757961783439,0.798702837337637)
--(axis cs:12.7388535031847,0.819472400748568)
--(axis cs:12.1019108280255,0.833179624721077)
--(axis cs:11.4649681528662,0.844896387682918)
--(axis cs:10.828025477707,0.854500058796439)
--(axis cs:10.1910828025478,0.8631120488572)
--(axis cs:9.55414012738853,0.8704262442941)
--(axis cs:8.9171974522293,0.88384545710718)
--(axis cs:8.28025477707006,0.890917667392676)
--(axis cs:7.64331210191083,0.897380014369778)
--(axis cs:7.00636942675159,0.90249133070876)
--(axis cs:6.36942675159236,0.906196578324948)
--(axis cs:5.73248407643312,0.909680752703721)
--(axis cs:5.09554140127389,0.911581082495744)
--(axis cs:4.45859872611465,0.91293750047625)
--(axis cs:3.82165605095541,0.913981481159873)
--(axis cs:3.18471337579618,0.914751486921407)
--(axis cs:2.54777070063694,0.915072671020625)
--(axis cs:1.91082802547771,0.915729500889036)
--(axis cs:1.27388535031847,0.916039997294499)
--(axis cs:0.636942675159236,0.916005524736142)
--(axis cs:0,0.916028047168889)
--cycle;


==> img/mnist/mnist_rate_distortion_fw_50.tex <==
\addplot [line width=0.5, opacity=0.85, color0!75, dashed]
table {%
0 0.915380861792946
0.636942675159236 0.915383144932566
1.27388535031847 0.914919858657522
1.91082802547771 0.914280837429687
2.54777070063694 0.913544164212944
3.18471337579618 0.912178813585779
3.82165605095541 0.910032978840172
4.45859872611465 0.905526603945182
5.09554140127389 0.90007177780848
5.73248407643312 0.892066826615919
6.36942675159236 0.880715677368571
7.00636942675159 0.867029773636023
7.64331210191083 0.855574743761681
8.28025477707006 0.841512999671977
8.9171974522293 0.831088222434046
9.55414012738853 0.814187564589665
10.1910828025478 0.798903066735947
10.828025477707 0.794066570041468
11.4649681528662 0.781502872162964
12.1019108280255 0.778166551473551
12.7388535031847 0.773229060251033
13.3757961783439 0.769108220571652
14.0127388535032 0.768405302316532
14.6496815286624 0.766448674754938
15.2866242038217 0.767113893361529
15.9235668789809 0.763725705401157
16.5605095541401 0.756456615184434
17.1974522292994 0.754767013814999
17.8343949044586 0.752548242188059
18.4713375796178 0.751807743742829
19.1082802547771 0.74942809819011
19.7452229299363 0.747575880927616
20.3821656050955 0.746411322871572
21.0191082802548 0.743186100354651
21.656050955414 0.743151986643206
22.2929936305732 0.74444408996671
22.9299363057325 0.742639331145911
23.5668789808917 0.738875757586211
24.203821656051 0.735007813404081
24.8407643312102 0.733304467372363
25.4777070063694 0.724095071689226
26.1146496815287 0.723792790789157
26.7515923566879 0.71460275573656
27.3885350318471 0.711621074043214
28.0254777070064 0.709554236326367
28.6624203821656 0.707948961472139
29.2993630573248 0.704595447601751
29.9363057324841 0.701846497480292
30.5732484076433 0.695644948906265
31.2101910828025 0.688934610560536
31.8471337579618 0.67919592494145
32.484076433121 0.680134236409795
33.1210191082803 0.673602279330371
33.7579617834395 0.674781162769068
34.3949044585987 0.669141111187055
35.031847133758 0.671450736996776
35.6687898089172 0.662726397861261
36.3057324840764 0.656265364653955
36.9426751592357 0.648929495347838
37.5796178343949 0.644436174313887
38.2165605095541 0.63827491648568
38.8535031847134 0.638293261194776
39.4904458598726 0.635302574991365
40.1273885350318 0.637807475826921
40.7643312101911 0.63435931269647
41.4012738853503 0.625509815027472
42.0382165605096 0.626782346446998
42.6751592356688 0.627572398126649
43.312101910828 0.625795063751866
43.9490445859873 0.618265629940724
44.5859872611465 0.613765510787489
45.2229299363057 0.606820747975726
45.859872611465 0.60180580629094
46.4968152866242 0.601324466702063
47.1337579617834 0.596612098855257
47.7707006369427 0.588396707669308
48.4076433121019 0.582080046553092
49.0445859872611 0.574375226083066
49.6815286624204 0.57518158784238
50.3184713375796 0.565726327245575
50.9554140127388 0.55927963308226
51.5923566878981 0.546239251552106
52.2292993630573 0.537682796185618
52.8662420382166 0.535396090564172
53.5031847133758 0.526927952942278
54.140127388535 0.519786018567574
54.7770700636943 0.515069774357289
55.4140127388535 0.50911460462522
56.0509554140127 0.499464796350094
56.687898089172 0.499009115548943
57.3248407643312 0.491450643263815
57.9617834394904 0.484509788887672
58.5987261146497 0.48063935753539
59.2356687898089 0.466229292955416
59.8726114649682 0.464684948758092
60.5095541401274 0.446894955912414
61.1464968152866 0.439164029247293
61.7834394904459 0.429370089986149
62.4203821656051 0.414892915179639
63.0573248407643 0.413094888798761
63.6942675159236 0.40127942673547
64.3312101910828 0.385271411459698
64.968152866242 0.379625207064989
65.6050955414013 0.36862303715532
66.2420382165605 0.35553412767896
66.8789808917197 0.34761859329148
67.515923566879 0.341347721350823
68.1528662420382 0.328659165874991
68.7898089171974 0.324885606488744
69.4267515923567 0.321978579994407
70.0636942675159 0.313819732119249
70.7006369426752 0.307274763966584
71.3375796178344 0.299424847439759
71.9745222929936 0.295225819116385
72.6114649681529 0.287742456039062
73.2484076433121 0.277565886083923
73.8853503184713 0.271040468111206
74.5222929936306 0.264334875759487
75.1592356687898 0.248862441328147
75.796178343949 0.241167243745765
76.4331210191083 0.235121310871958
77.0700636942675 0.231337513201096
77.7070063694268 0.222287233149365
78.343949044586 0.213205160398002
78.9808917197452 0.200070181025299
79.6178343949044 0.190310491075903
80.2547770700637 0.178458065770987
80.8917197452229 0.162783655520549
81.5286624203822 0.150260628012632
82.1656050955414 0.141530563537244
82.8025477707006 0.134021995457825
83.4394904458599 0.126547389049455
84.0764331210191 0.113567120818507
84.7133757961783 0.0971116496110432
85.3503184713376 0.08660414281823
85.9872611464968 0.0806303146294543
86.6242038216561 0.0714755518174441
87.2611464968153 0.0577687125653483
87.8980891719745 0.0470014068399661
88.5350318471338 0.0444161970450934
89.171974522293 0.0384261916646872
89.8089171974522 0.030004619981411
90.4458598726115 0.0245583753052139
91.0828025477707 0.0199148580256999
91.7197452229299 0.0123629242054686
92.3566878980892 0.00950510617295552
92.9936305732484 0.00678342152621233
93.6305732484076 0.0056255260977753
94.2675159235669 0.0041941598396825
94.9044585987261 0.00186462034595482
95.5414012738853 0.00133572206063176
96.1783439490446 0.000615898099505877
96.8152866242038 8.57106127047763e-05
97.4522292993631 4.0607320389337e-05
98.0891719745223 1.95488815672229e-05
98.7261146496815 2.75160538606989e-06
99.3630573248408 4.95475949494117e-06
100 0
};
\path [fill=color0!75, fill opacity=0.25] 
(axis cs:0,0.916045299834684)
--(axis cs:0,0.914716423751209)
--(axis cs:0.636942675159236,0.914708641073291)
--(axis cs:1.27388535031847,0.914127170448076)
--(axis cs:1.91082802547771,0.913454916699763)
--(axis cs:2.54777070063694,0.912596107570005)
--(axis cs:3.18471337579618,0.911009927332423)
--(axis cs:3.82165605095541,0.908537295428659)
--(axis cs:4.45859872611465,0.903445308695412)
--(axis cs:5.09554140127389,0.897518327579922)
--(axis cs:5.73248407643312,0.888804253965546)
--(axis cs:6.36942675159236,0.876560128246939)
--(axis cs:7.00636942675159,0.862121456827771)
--(axis cs:7.64331210191083,0.850138207000612)
--(axis cs:8.28025477707006,0.835632335761134)
--(axis cs:8.9171974522293,0.824927446897541)
--(axis cs:9.55414012738853,0.807754032678343)
--(axis cs:10.1910828025478,0.792190455031009)
--(axis cs:10.828025477707,0.787404129263711)
--(axis cs:11.4649681528662,0.774944492705579)
--(axis cs:12.1019108280255,0.771490100595666)
--(axis cs:12.7388535031847,0.766533469173909)
--(axis cs:13.3757961783439,0.762263082105431)
--(axis cs:14.0127388535032,0.761503096235894)
--(axis cs:14.6496815286624,0.759639557525655)
--(axis cs:15.2866242038217,0.760325278012443)
--(axis cs:15.9235668789809,0.756833354135848)
--(axis cs:16.5605095541401,0.749559054720291)
--(axis cs:17.1974522292994,0.747856205603404)
--(axis cs:17.8343949044586,0.745626381891025)
--(axis cs:18.4713375796178,0.744854241661343)
--(axis cs:19.1082802547771,0.742455972279433)
--(axis cs:19.7452229299363,0.740591248573932)
--(axis cs:20.3821656050955,0.739456039127778)
--(axis cs:21.0191082802548,0.736285590757111)
--(axis cs:21.656050955414,0.736144130753529)
--(axis cs:22.2929936305732,0.737459467030394)
--(axis cs:22.9299363057325,0.735723581093848)
--(axis cs:23.5668789808917,0.731924210512366)
--(axis cs:24.203821656051,0.727926915223218)
--(axis cs:24.8407643312102,0.726149799112428)
--(axis cs:25.4777070063694,0.716848749833739)
--(axis cs:26.1146496815287,0.716492048509606)
--(axis cs:26.7515923566879,0.707408252720213)
--(axis cs:27.3885350318471,0.704311150309109)
--(axis cs:28.0254777070064,0.702145322895017)
--(axis cs:28.6624203821656,0.700694769871717)
--(axis cs:29.2993630573248,0.697364972757536)
--(axis cs:29.9363057324841,0.694561422969982)
--(axis cs:30.5732484076433,0.688383654455324)
--(axis cs:31.2101910828025,0.681671671311142)
--(axis cs:31.8471337579618,0.671956506505268)
--(axis cs:32.484076433121,0.67286071586697)
--(axis cs:33.1210191082803,0.666295710069935)
--(axis cs:33.7579617834395,0.66740995691112)
--(axis cs:34.3949044585987,0.66183662507888)
--(axis cs:35.031847133758,0.664017792625854)
--(axis cs:35.6687898089172,0.655314204320356)
--(axis cs:36.3057324840764,0.648842851826411)
--(axis cs:36.9426751592357,0.641431933541164)
--(axis cs:37.5796178343949,0.636832262148897)
--(axis cs:38.2165605095541,0.630580799475608)
--(axis cs:38.8535031847134,0.630767986872681)
--(axis cs:39.4904458598726,0.62780579363142)
--(axis cs:40.1273885350318,0.630398554688617)
--(axis cs:40.7643312101911,0.62707476186141)
--(axis cs:41.4012738853503,0.618105305077585)
--(axis cs:42.0382165605096,0.619485247826747)
--(axis cs:42.6751592356688,0.62013284116695)
--(axis cs:43.312101910828,0.618450203806418)
--(axis cs:43.9490445859873,0.610862637219663)
--(axis cs:44.5859872611465,0.606544237730878)
--(axis cs:45.2229299363057,0.599517223112032)
--(axis cs:45.859872611465,0.594429996819101)
--(axis cs:46.4968152866242,0.594084795747848)
--(axis cs:47.1337579617834,0.589312464246975)
--(axis cs:47.7707006369427,0.580946739304946)
--(axis cs:48.4076433121019,0.574725245985554)
--(axis cs:49.0445859872611,0.566995978702684)
--(axis cs:49.6815286624204,0.567843434105363)
--(axis cs:50.3184713375796,0.558490437199575)
--(axis cs:50.9554140127388,0.551911165456391)
--(axis cs:51.5923566878981,0.538660273128939)
--(axis cs:52.2292993630573,0.530088465354935)
--(axis cs:52.8662420382166,0.527764830080567)
--(axis cs:53.5031847133758,0.5194406578414)
--(axis cs:54.140127388535,0.512355293147343)
--(axis cs:54.7770700636943,0.507564950793317)
--(axis cs:55.4140127388535,0.50167007750366)
--(axis cs:56.0509554140127,0.492121493330354)
--(axis cs:56.687898089172,0.49159361211541)
--(axis cs:57.3248407643312,0.484011747727756)
--(axis cs:57.9617834394904,0.477083994530595)
--(axis cs:58.5987261146497,0.473331736007309)
--(axis cs:59.2356687898089,0.458951789602763)
--(axis cs:59.8726114649682,0.457438301349939)
--(axis cs:60.5095541401274,0.439620408658167)
--(axis cs:61.1464968152866,0.43201014490282)
--(axis cs:61.7834394904459,0.422197028969521)
--(axis cs:62.4203821656051,0.407663795586173)
--(axis cs:63.0573248407643,0.405863246966414)
--(axis cs:63.6942675159236,0.394274910380747)
--(axis cs:64.3312101910828,0.378532413315916)
--(axis cs:64.968152866242,0.37302306527126)
--(axis cs:65.6050955414013,0.362163399053641)
--(axis cs:66.2420382165605,0.349288548424411)
--(axis cs:66.8789808917197,0.341554883476498)
--(axis cs:67.515923566879,0.33552522870704)
--(axis cs:68.1528662420382,0.323019544619755)
--(axis cs:68.7898089171974,0.319461703343315)
--(axis cs:69.4267515923567,0.316595160968095)
--(axis cs:70.0636942675159,0.308605177985191)
--(axis cs:70.7006369426752,0.302157114088966)
--(axis cs:71.3375796178344,0.29443173087848)
--(axis cs:71.9745222929936,0.290301275213935)
--(axis cs:72.6114649681529,0.282756054532647)
--(axis cs:73.2484076433121,0.272418595323918)
--(axis cs:73.8853503184713,0.265959000377081)
--(axis cs:74.5222929936306,0.259207718569371)
--(axis cs:75.1592356687898,0.243648383420116)
--(axis cs:75.796178343949,0.23575352768191)
--(axis cs:76.4331210191083,0.229645325894605)
--(axis cs:77.0700636942675,0.22587465974916)
--(axis cs:77.7070063694268,0.216558774694706)
--(axis cs:78.343949044586,0.207233449720199)
--(axis cs:78.9808917197452,0.194199779651482)
--(axis cs:79.6178343949044,0.184343580775643)
--(axis cs:80.2547770700637,0.172437273218309)
--(axis cs:80.8917197452229,0.156864239680846)
--(axis cs:81.5286624203822,0.144402593083685)
--(axis cs:82.1656050955414,0.135674594484728)
--(axis cs:82.8025477707006,0.128460828627507)
--(axis cs:83.4394904458599,0.121109431642069)
--(axis cs:84.0764331210191,0.108320186673337)
--(axis cs:84.7133757961783,0.0921375241548929)
--(axis cs:85.3503184713376,0.0817954270804245)
--(axis cs:85.9872611464968,0.0757169133760597)
--(axis cs:86.6242038216561,0.0670481044828792)
--(axis cs:87.2611464968153,0.0534464996562018)
--(axis cs:87.8980891719745,0.0429728766483307)
--(axis cs:88.5350318471338,0.0402546922730733)
--(axis cs:89.171974522293,0.0345425632848585)
--(axis cs:89.8089171974522,0.0266295825786621)
--(axis cs:90.4458598726115,0.0216697031957492)
--(axis cs:91.0828025477707,0.0175929706743253)
--(axis cs:91.7197452229299,0.0103180549096261)
--(axis cs:92.3566878980892,0.00760498324686373)
--(axis cs:92.9936305732484,0.00516629239373029)
--(axis cs:93.6305732484076,0.00412477510416096)
--(axis cs:94.2675159235669,0.00296497618317996)
--(axis cs:94.9044585987261,0.00114581374838161)
--(axis cs:95.5414012738853,0.000785723311903519)
--(axis cs:96.1783439490446,0.000305367932488156)
--(axis cs:96.8152866242038,3.23581158772247e-05)
--(axis cs:97.4522292993631,-6.50595760899227e-06)
--(axis cs:98.0891719745223,-6.47406708591682e-06)
--(axis cs:98.7261146496815,1.88411292000426e-06)
--(axis cs:99.3630573248408,1.83557453615015e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,8.0739444537322e-06)
--(axis cs:98.7261146496815,3.61909785213552e-06)
--(axis cs:98.0891719745223,4.55718302203626e-05)
--(axis cs:97.4522292993631,8.77205983876663e-05)
--(axis cs:96.8152866242038,0.000139063109532328)
--(axis cs:96.1783439490446,0.000926428266523598)
--(axis cs:95.5414012738853,0.00188572080935999)
--(axis cs:94.9044585987261,0.00258342694352802)
--(axis cs:94.2675159235669,0.00542334349618504)
--(axis cs:93.6305732484076,0.00712627709138964)
--(axis cs:92.9936305732484,0.00840055065869437)
--(axis cs:92.3566878980892,0.0114052290990473)
--(axis cs:91.7197452229299,0.0144077935013111)
--(axis cs:91.0828025477707,0.0222367453770744)
--(axis cs:90.4458598726115,0.0274470474146786)
--(axis cs:89.8089171974522,0.0333796573841598)
--(axis cs:89.171974522293,0.0423098200445159)
--(axis cs:88.5350318471338,0.0485777018171134)
--(axis cs:87.8980891719745,0.0510299370316015)
--(axis cs:87.2611464968153,0.0620909254744949)
--(axis cs:86.6242038216561,0.075902999152009)
--(axis cs:85.9872611464968,0.0855437158828488)
--(axis cs:85.3503184713376,0.0914128585560354)
--(axis cs:84.7133757961783,0.102085775067193)
--(axis cs:84.0764331210191,0.118814054963677)
--(axis cs:83.4394904458599,0.131985346456841)
--(axis cs:82.8025477707006,0.139583162288143)
--(axis cs:82.1656050955414,0.14738653258976)
--(axis cs:81.5286624203822,0.156118662941579)
--(axis cs:80.8917197452229,0.168703071360253)
--(axis cs:80.2547770700637,0.184478858323665)
--(axis cs:79.6178343949044,0.196277401376164)
--(axis cs:78.9808917197452,0.205940582399117)
--(axis cs:78.343949044586,0.219176871075804)
--(axis cs:77.7070063694268,0.228015691604025)
--(axis cs:77.0700636942675,0.236800366653032)
--(axis cs:76.4331210191083,0.24059729584931)
--(axis cs:75.796178343949,0.246580959809621)
--(axis cs:75.1592356687898,0.254076499236177)
--(axis cs:74.5222929936306,0.269462032949604)
--(axis cs:73.8853503184713,0.276121935845332)
--(axis cs:73.2484076433121,0.282713176843927)
--(axis cs:72.6114649681529,0.292728857545477)
--(axis cs:71.9745222929936,0.300150363018834)
--(axis cs:71.3375796178344,0.304417964001039)
--(axis cs:70.7006369426752,0.312392413844202)
--(axis cs:70.0636942675159,0.319034286253308)
--(axis cs:69.4267515923567,0.327361999020719)
--(axis cs:68.7898089171974,0.330309509634172)
--(axis cs:68.1528662420382,0.334298787130228)
--(axis cs:67.515923566879,0.347170213994607)
--(axis cs:66.8789808917197,0.353682303106461)
--(axis cs:66.2420382165605,0.361779706933508)
--(axis cs:65.6050955414013,0.375082675256998)
--(axis cs:64.968152866242,0.386227348858717)
--(axis cs:64.3312101910828,0.392010409603479)
--(axis cs:63.6942675159236,0.408283943090192)
--(axis cs:63.0573248407643,0.420326530631108)
--(axis cs:62.4203821656051,0.422122034773105)
--(axis cs:61.7834394904459,0.436543151002777)
--(axis cs:61.1464968152866,0.446317913591766)
--(axis cs:60.5095541401274,0.45416950316666)
--(axis cs:59.8726114649682,0.471931596166245)
--(axis cs:59.2356687898089,0.473506796308068)
--(axis cs:58.5987261146497,0.487946979063471)
--(axis cs:57.9617834394904,0.491935583244749)
--(axis cs:57.3248407643312,0.498889538799875)
--(axis cs:56.687898089172,0.506424618982476)
--(axis cs:56.0509554140127,0.506808099369833)
--(axis cs:55.4140127388535,0.516559131746779)
--(axis cs:54.7770700636943,0.522574597921262)
--(axis cs:54.140127388535,0.527216743987806)
--(axis cs:53.5031847133758,0.534415248043157)
--(axis cs:52.8662420382166,0.543027351047778)
--(axis cs:52.2292993630573,0.5452771270163)
--(axis cs:51.5923566878981,0.553818229975273)
--(axis cs:50.9554140127388,0.56664810070813)
--(axis cs:50.3184713375796,0.572962217291575)
--(axis cs:49.6815286624204,0.582519741579398)
--(axis cs:49.0445859872611,0.581754473463449)
--(axis cs:48.4076433121019,0.58943484712063)
--(axis cs:47.7707006369427,0.59584667603367)
--(axis cs:47.1337579617834,0.60391173346354)
--(axis cs:46.4968152866242,0.608564137656277)
--(axis cs:45.859872611465,0.60918161576278)
--(axis cs:45.2229299363057,0.614124272839419)
--(axis cs:44.5859872611465,0.620986783844099)
--(axis cs:43.9490445859873,0.625668622661785)
--(axis cs:43.312101910828,0.633139923697314)
--(axis cs:42.6751592356688,0.635011955086348)
--(axis cs:42.0382165605096,0.63407944506725)
--(axis cs:41.4012738853503,0.632914324977358)
--(axis cs:40.7643312101911,0.64164386353153)
--(axis cs:40.1273885350318,0.645216396965225)
--(axis cs:39.4904458598726,0.64279935635131)
--(axis cs:38.8535031847134,0.645818535516871)
--(axis cs:38.2165605095541,0.645969033495751)
--(axis cs:37.5796178343949,0.652040086478877)
--(axis cs:36.9426751592357,0.656427057154513)
--(axis cs:36.3057324840764,0.663687877481499)
--(axis cs:35.6687898089172,0.670138591402166)
--(axis cs:35.031847133758,0.678883681367698)
--(axis cs:34.3949044585987,0.67644559729523)
--(axis cs:33.7579617834395,0.682152368627016)
--(axis cs:33.1210191082803,0.680908848590807)
--(axis cs:32.484076433121,0.687407756952619)
--(axis cs:31.8471337579618,0.686435343377633)
--(axis cs:31.2101910828025,0.696197549809931)
--(axis cs:30.5732484076433,0.702906243357206)
--(axis cs:29.9363057324841,0.709131571990602)
--(axis cs:29.2993630573248,0.711825922445965)
--(axis cs:28.6624203821656,0.71520315307256)
--(axis cs:28.0254777070064,0.716963149757716)
--(axis cs:27.3885350318471,0.718930997777319)
--(axis cs:26.7515923566879,0.721797258752907)
--(axis cs:26.1146496815287,0.731093533068708)
--(axis cs:25.4777070063694,0.731341393544712)
--(axis cs:24.8407643312102,0.740459135632299)
--(axis cs:24.203821656051,0.742088711584945)
--(axis cs:23.5668789808917,0.745827304660056)
--(axis cs:22.9299363057325,0.749555081197973)
--(axis cs:22.2929936305732,0.751428712903025)
--(axis cs:21.656050955414,0.750159842532883)
--(axis cs:21.0191082802548,0.750086609952191)
--(axis cs:20.3821656050955,0.753366606615367)
--(axis cs:19.7452229299363,0.7545605132813)
--(axis cs:19.1082802547771,0.756400224100787)
--(axis cs:18.4713375796178,0.758761245824315)
--(axis cs:17.8343949044586,0.759470102485092)
--(axis cs:17.1974522292994,0.761677822026593)
--(axis cs:16.5605095541401,0.763354175648576)
--(axis cs:15.9235668789809,0.770618056666466)
--(axis cs:15.2866242038217,0.773902508710616)
--(axis cs:14.6496815286624,0.773257791984222)
--(axis cs:14.0127388535032,0.775307508397171)
--(axis cs:13.3757961783439,0.775953359037873)
--(axis cs:12.7388535031847,0.779924651328157)
--(axis cs:12.1019108280255,0.784843002351435)
--(axis cs:11.4649681528662,0.78806125162035)
--(axis cs:10.828025477707,0.800729010819226)
--(axis cs:10.1910828025478,0.805615678440886)
--(axis cs:9.55414012738853,0.820621096500988)
--(axis cs:8.9171974522293,0.83724899797055)
--(axis cs:8.28025477707006,0.84739366358282)
--(axis cs:7.64331210191083,0.86101128052275)
--(axis cs:7.00636942675159,0.871938090444274)
--(axis cs:6.36942675159236,0.884871226490203)
--(axis cs:5.73248407643312,0.895329399266292)
--(axis cs:5.09554140127389,0.902625228037038)
--(axis cs:4.45859872611465,0.907607899194952)
--(axis cs:3.82165605095541,0.911528662251686)
--(axis cs:3.18471337579618,0.913347699839135)
--(axis cs:2.54777070063694,0.914492220855884)
--(axis cs:1.91082802547771,0.915106758159611)
--(axis cs:1.27388535031847,0.915712546866968)
--(axis cs:0.636942675159236,0.916057648791841)
--(axis cs:0,0.916045299834684)
--cycle;


==> img/mnist/mnist_rate_distortion_fw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.915408829675289
0.636942675159236 0.915382273662835
1.27388535031847 0.915096716852859
1.91082802547771 0.914692572912318
2.54777070063694 0.913862062830594
3.18471337579618 0.912135634987499
3.82165605095541 0.909847007238422
4.45859872611465 0.906684231007821
5.09554140127389 0.901666516910191
5.73248407643312 0.897687930468237
6.36942675159236 0.891821020462085
7.00636942675159 0.882395655786677
7.64331210191083 0.87498702386627
8.28025477707006 0.863144064748485
8.9171974522293 0.852229911468457
9.55414012738853 0.833246941481484
10.1910828025478 0.812610879683634
10.828025477707 0.792825166148832
11.4649681528662 0.775601980706851
12.1019108280255 0.754392843041569
12.7388535031847 0.734276171533856
13.3757961783439 0.709338013472443
14.0127388535032 0.6908908565616
14.6496815286624 0.665962172550644
15.2866242038217 0.65109059715789
15.9235668789809 0.63025334887905
16.5605095541401 0.611842870320252
17.1974522292994 0.599454988868092
17.8343949044586 0.573712249294622
18.4713375796178 0.549860144949635
19.1082802547771 0.52797399037634
19.7452229299363 0.511082286236342
20.3821656050955 0.48277777820942
21.0191082802548 0.464084515760769
21.656050955414 0.457098011275812
22.2929936305732 0.43569115015518
22.9299363057325 0.41689562018284
23.5668789808917 0.396277005168085
24.203821656051 0.377319218446792
24.8407643312102 0.367335590948132
25.4777070063694 0.348365006815948
26.1146496815287 0.333453813923734
26.7515923566879 0.32227280900117
27.3885350318471 0.311638022393417
28.0254777070064 0.294828007709493
28.6624203821656 0.280404937018156
29.2993630573248 0.27610515875454
29.9363057324841 0.264157310609116
30.5732484076433 0.253143067016294
31.2101910828025 0.239077157805257
31.8471337579618 0.229905061221345
32.484076433121 0.220284622668961
33.1210191082803 0.209879552711753
33.7579617834395 0.195899192405875
34.3949044585987 0.186291122548258
35.031847133758 0.180055678856907
35.6687898089172 0.168096910978574
36.3057324840764 0.164841537991507
36.9426751592357 0.160624155317777
37.5796178343949 0.157887313298977
38.2165605095541 0.154267737419665
38.8535031847134 0.149298551698007
39.4904458598726 0.148078675652336
40.1273885350318 0.145562303348656
40.7643312101911 0.14278459742922
41.4012738853503 0.143186102443022
42.0382165605096 0.145163542037156
42.6751592356688 0.144787398323333
43.312101910828 0.140348344975882
43.9490445859873 0.136248876780294
44.5859872611465 0.129739171930641
45.2229299363057 0.125223531424405
45.859872611465 0.117969579966437
46.4968152866242 0.11452360991743
47.1337579617834 0.110260872808379
47.7707006369427 0.111834452871629
48.4076433121019 0.106263380254686
49.0445859872611 0.10574532869924
49.6815286624204 0.10945046766122
50.3184713375796 0.110568706254168
50.9554140127388 0.111466150305739
51.5923566878981 0.103554940218896
52.2292993630573 0.0993581257647757
52.8662420382166 0.0989718502349765
53.5031847133758 0.100940247271179
54.140127388535 0.0975202009991361
54.7770700636943 0.0942375160085634
55.4140127388535 0.0946136234188508
56.0509554140127 0.101208402883192
56.687898089172 0.102575054375311
57.3248407643312 0.0975976766885219
57.9617834394904 0.0980750429620181
58.5987261146497 0.0937486159518336
59.2356687898089 0.0855829494186959
59.8726114649682 0.0856079226566187
60.5095541401274 0.0769698398435431
61.1464968152866 0.0710596391034464
61.7834394904459 0.0741075598484932
62.4203821656051 0.0728888746724271
63.0573248407643 0.0709565187197391
63.6942675159236 0.0666711332657636
64.3312101910828 0.0677817963684673
64.968152866242 0.0652890624020528
65.6050955414013 0.0649960667064047
66.2420382165605 0.0659710155876101
66.8789808917197 0.0629344602092929
67.515923566879 0.0596610833853472
68.1528662420382 0.0593300504704785
68.7898089171974 0.0529158416896006
69.4267515923567 0.0530788265476271
70.0636942675159 0.0504660058111919
70.7006369426752 0.04584325387265
71.3375796178344 0.0454424565584947
71.9745222929936 0.0439342650054907
72.6114649681529 0.0414550790936585
73.2484076433121 0.0393416239747551
73.8853503184713 0.0374506893893551
74.5222929936306 0.0378209570602172
75.1592356687898 0.0379107980088606
75.796178343949 0.0387693894238152
76.4331210191083 0.0404712585807834
77.0700636942675 0.0407964303150209
77.7070063694268 0.0385946275263931
78.343949044586 0.0383558567575824
78.9808917197452 0.0358113866591839
79.6178343949044 0.0352170386562531
80.2547770700637 0.0326357289196444
80.8917197452229 0.0333434887203322
81.5286624203822 0.0327794245189457
82.1656050955414 0.030925364627635
82.8025477707006 0.0260984672632294
83.4394904458599 0.0252757583062409
84.0764331210191 0.025232290484774
84.7133757961783 0.0254289273362259
85.3503184713376 0.0245441769334865
85.9872611464968 0.0235596044504842
86.6242038216561 0.0199210327242437
87.2611464968153 0.0161681138614545
87.8980891719745 0.0141949105019622
88.5350318471338 0.0119463086903251
89.171974522293 0.0119163774524236
89.8089171974522 0.0107255865565207
90.4458598726115 0.0110226444160015
91.0828025477707 0.0086978640916785
91.7197452229299 0.00638393845839051
92.3566878980892 0.00308879387423672
92.9936305732484 0.00161427338025528
93.6305732484076 0.00157834846004424
94.2675159235669 0.000866445819476157
94.9044585987261 0.000890618483785353
95.5414012738853 7.19723169072889e-05
96.1783439490446 2.74922238068126e-05
96.8152866242038 2.4619714830198e-05
97.4522292993631 6.76046705217925e-06
98.0891719745223 4.47163104689896e-06
98.7261146496815 4.03964714622729e-06
99.3630573248408 2.36091867617694e-06
100 0
};
\path [fill=color0, fill opacity=0.25] 
(axis cs:0,0.916046968073714)
--(axis cs:0,0.914770691276864)
--(axis cs:0.636942675159236,0.914758498028928)
--(axis cs:1.27388535031847,0.91445456941585)
--(axis cs:1.91082802547771,0.913916606574993)
--(axis cs:2.54777070063694,0.913012854863054)
--(axis cs:3.18471337579618,0.91100982917224)
--(axis cs:3.82165605095541,0.908308622978042)
--(axis cs:4.45859872611465,0.904766221794161)
--(axis cs:5.09554140127389,0.899280301402026)
--(axis cs:5.73248407643312,0.894875589698842)
--(axis cs:6.36942675159236,0.888593014187804)
--(axis cs:7.00636942675159,0.878377980858574)
--(axis cs:7.64331210191083,0.870607827449441)
--(axis cs:8.28025477707006,0.858113282497584)
--(axis cs:8.9171974522293,0.846656619138755)
--(axis cs:9.55414012738853,0.827061495842175)
--(axis cs:10.1910828025478,0.805942976063722)
--(axis cs:10.828025477707,0.785697958783154)
--(axis cs:11.4649681528662,0.768194377714324)
--(axis cs:12.1019108280255,0.746724962142788)
--(axis cs:12.7388535031847,0.726447854647021)
--(axis cs:13.3757961783439,0.701219321654128)
--(axis cs:14.0127388535032,0.682670575812019)
--(axis cs:14.6496815286624,0.657590720777947)
--(axis cs:15.2866242038217,0.642613827937105)
--(axis cs:15.9235668789809,0.621836947504961)
--(axis cs:16.5605095541401,0.603132502767645)
--(axis cs:17.1974522292994,0.590474055784236)
--(axis cs:17.8343949044586,0.564762736234623)
--(axis cs:18.4713375796178,0.540866720015686)
--(axis cs:19.1082802547771,0.519077983416912)
--(axis cs:19.7452229299363,0.502409307523281)
--(axis cs:20.3821656050955,0.47417742439667)
--(axis cs:21.0191082802548,0.455643514458078)
--(axis cs:21.656050955414,0.448645870696096)
--(axis cs:22.2929936305732,0.427220025296796)
--(axis cs:22.9299363057325,0.408705403334601)
--(axis cs:23.5668789808917,0.388132939619431)
--(axis cs:24.203821656051,0.369288116863546)
--(axis cs:24.8407643312102,0.359360165543182)
--(axis cs:25.4777070063694,0.340297034304513)
--(axis cs:26.1146496815287,0.325466067054886)
--(axis cs:26.7515923566879,0.314344619606846)
--(axis cs:27.3885350318471,0.303688695996481)
--(axis cs:28.0254777070064,0.287025677472669)
--(axis cs:28.6624203821656,0.272588616439909)
--(axis cs:29.2993630573248,0.268253033455642)
--(axis cs:29.9363057324841,0.256369523872842)
--(axis cs:30.5732484076433,0.245520882229554)
--(axis cs:31.2101910828025,0.231518265077687)
--(axis cs:31.8471337579618,0.222522838244016)
--(axis cs:32.484076433121,0.212968015567766)
--(axis cs:33.1210191082803,0.202673434998279)
--(axis cs:33.7579617834395,0.188889867650648)
--(axis cs:34.3949044585987,0.179549614606825)
--(axis cs:35.031847133758,0.173504320245402)
--(axis cs:35.6687898089172,0.161686070302905)
--(axis cs:36.3057324840764,0.15838298428487)
--(axis cs:36.9426751592357,0.15444648632692)
--(axis cs:37.5796178343949,0.151742542154941)
--(axis cs:38.2165605095541,0.14829732492445)
--(axis cs:38.8535031847134,0.1432834149902)
--(axis cs:39.4904458598726,0.142020646158634)
--(axis cs:40.1273885350318,0.139599877573298)
--(axis cs:40.7643312101911,0.137045218035725)
--(axis cs:41.4012738853503,0.137550907686294)
--(axis cs:42.0382165605096,0.139605381560305)
--(axis cs:42.6751592356688,0.139229058298589)
--(axis cs:43.312101910828,0.135069925588695)
--(axis cs:43.9490445859873,0.130813242756685)
--(axis cs:44.5859872611465,0.124534683969521)
--(axis cs:45.2229299363057,0.119996745300002)
--(axis cs:45.859872611465,0.112769642833669)
--(axis cs:46.4968152866242,0.10946637417906)
--(axis cs:47.1337579617834,0.105335490534174)
--(axis cs:47.7707006369427,0.106893279375812)
--(axis cs:48.4076433121019,0.101294486330835)
--(axis cs:49.0445859872611,0.1008432175359)
--(axis cs:49.6815286624204,0.104622132668475)
--(axis cs:50.3184713375796,0.105596671142931)
--(axis cs:50.9554140127388,0.106479978827102)
--(axis cs:51.5923566878981,0.0985837157432871)
--(axis cs:52.2292993630573,0.0943923235684435)
--(axis cs:52.8662420382166,0.0940320536383234)
--(axis cs:53.5031847133758,0.095970904668254)
--(axis cs:54.140127388535,0.0926124873107951)
--(axis cs:54.7770700636943,0.0893665146532989)
--(axis cs:55.4140127388535,0.08968834081241)
--(axis cs:56.0509554140127,0.0962687417988696)
--(axis cs:56.687898089172,0.0977252103916324)
--(axis cs:57.3248407643312,0.0928192913215886)
--(axis cs:57.9617834394904,0.0933948705964049)
--(axis cs:58.5987261146497,0.0891630359608729)
--(axis cs:59.2356687898089,0.0811194412125356)
--(axis cs:59.8726114649682,0.0811911986786866)
--(axis cs:60.5095541401274,0.0727172455556102)
--(axis cs:61.1464968152866,0.0669823908726992)
--(axis cs:61.7834394904459,0.0701219403897007)
--(axis cs:62.4203821656051,0.0690022409433317)
--(axis cs:63.0573248407643,0.0671117171992203)
--(axis cs:63.6942675159236,0.0628302338262023)
--(axis cs:64.3312101910828,0.063918071841569)
--(axis cs:64.968152866242,0.0615700846981986)
--(axis cs:65.6050955414013,0.0613472164774861)
--(axis cs:66.2420382165605,0.0623286795931275)
--(axis cs:66.8789808917197,0.0594069979330209)
--(axis cs:67.515923566879,0.0561213113737372)
--(axis cs:68.1528662420382,0.0558278604533091)
--(axis cs:68.7898089171974,0.049626694600727)
--(axis cs:69.4267515923567,0.0498805006926798)
--(axis cs:70.0636942675159,0.0472871559567338)
--(axis cs:70.7006369426752,0.0431280313493462)
--(axis cs:71.3375796178344,0.0427650837760479)
--(axis cs:71.9745222929936,0.041273352376369)
--(axis cs:72.6114649681529,0.0389389197804142)
--(axis cs:73.2484076433121,0.0369884025937297)
--(axis cs:73.8853503184713,0.0352295385177088)
--(axis cs:74.5222929936306,0.0355107271548963)
--(axis cs:75.1592356687898,0.0357369934880207)
--(axis cs:75.796178343949,0.0369032424356471)
--(axis cs:76.4331210191083,0.0387632501271824)
--(axis cs:77.0700636942675,0.0389615797559466)
--(axis cs:77.7070063694268,0.036867514980996)
--(axis cs:78.343949044586,0.0367625989679835)
--(axis cs:78.9808917197452,0.0340216594034645)
--(axis cs:79.6178343949044,0.033468805765597)
--(axis cs:80.2547770700637,0.0307967537621799)
--(axis cs:80.8917197452229,0.031437428253213)
--(axis cs:81.5286624203822,0.0309884691277693)
--(axis cs:82.1656050955414,0.0289881509381444)
--(axis cs:82.8025477707006,0.0243594471735647)
--(axis cs:83.4394904458599,0.0233958379601799)
--(axis cs:84.0764331210191,0.023360811656067)
--(axis cs:84.7133757961783,0.0236349782732255)
--(axis cs:85.3503184713376,0.0228755526422535)
--(axis cs:85.9872611464968,0.0218937718287899)
--(axis cs:86.6242038216561,0.0186064654773654)
--(axis cs:87.2611464968153,0.0150264173303497)
--(axis cs:87.8980891719745,0.0130315296408964)
--(axis cs:88.5350318471338,0.0106272034435599)
--(axis cs:89.171974522293,0.0107280692483413)
--(axis cs:89.8089171974522,0.00945065306082912)
--(axis cs:90.4458598726115,0.0097430173143508)
--(axis cs:91.0828025477707,0.00742394150640178)
--(axis cs:91.7197452229299,0.00516138962103678)
--(axis cs:92.3566878980892,0.00225390964791465)
--(axis cs:92.9936305732484,0.00101118625840771)
--(axis cs:93.6305732484076,0.000989369778582739)
--(axis cs:94.2675159235669,0.000466921350769647)
--(axis cs:94.9044585987261,0.000494729316102132)
--(axis cs:95.5414012738853,3.69873910191497e-05)
--(axis cs:96.1783439490446,2.66853071952282e-07)
--(axis cs:96.8152866242038,1.28613316776119e-05)
--(axis cs:97.4522292993631,4.80411163867161e-06)
--(axis cs:98.0891719745223,3.79659651900197e-06)
--(axis cs:98.7261146496815,3.74252852109559e-06)
--(axis cs:99.3630573248408,2.086317169157e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,2.63552018319688e-06)
--(axis cs:98.7261146496815,4.33676577135899e-06)
--(axis cs:98.0891719745223,5.14666557479595e-06)
--(axis cs:97.4522292993631,8.71682246568689e-06)
--(axis cs:96.8152866242038,3.63780979827841e-05)
--(axis cs:96.1783439490446,5.47175945416729e-05)
--(axis cs:95.5414012738853,0.000106957242795428)
--(axis cs:94.9044585987261,0.00128650765146857)
--(axis cs:94.2675159235669,0.00126597028818267)
--(axis cs:93.6305732484076,0.00216732714150574)
--(axis cs:92.9936305732484,0.00221736050210285)
--(axis cs:92.3566878980892,0.00392367810055879)
--(axis cs:91.7197452229299,0.00760648729574424)
--(axis cs:91.0828025477707,0.00997178667695522)
--(axis cs:90.4458598726115,0.0123022715176523)
--(axis cs:89.8089171974522,0.0120005200522123)
--(axis cs:89.171974522293,0.0131046856565059)
--(axis cs:88.5350318471338,0.0132654139370902)
--(axis cs:87.8980891719745,0.015358291363028)
--(axis cs:87.2611464968153,0.0173098103925593)
--(axis cs:86.6242038216561,0.021235599971122)
--(axis cs:85.9872611464968,0.0252254370721784)
--(axis cs:85.3503184713376,0.0262128012247194)
--(axis cs:84.7133757961783,0.0272228763992262)
--(axis cs:84.0764331210191,0.027103769313481)
--(axis cs:83.4394904458599,0.0271556786523018)
--(axis cs:82.8025477707006,0.0278374873528942)
--(axis cs:82.1656050955414,0.0328625783171255)
--(axis cs:81.5286624203822,0.0345703799101222)
--(axis cs:80.8917197452229,0.0352495491874513)
--(axis cs:80.2547770700637,0.0344747040771088)
--(axis cs:79.6178343949044,0.0369652715469092)
--(axis cs:78.9808917197452,0.0376011139149033)
--(axis cs:78.343949044586,0.0399491145471813)
--(axis cs:77.7070063694268,0.0403217400717902)
--(axis cs:77.0700636942675,0.0426312808740951)
--(axis cs:76.4331210191083,0.0421792670343843)
--(axis cs:75.796178343949,0.0406355364119834)
--(axis cs:75.1592356687898,0.0400846025297005)
--(axis cs:74.5222929936306,0.040131186965538)
--(axis cs:73.8853503184713,0.0396718402610015)
--(axis cs:73.2484076433121,0.0416948453557805)
--(axis cs:72.6114649681529,0.0439712384069027)
--(axis cs:71.9745222929936,0.0465951776346124)
--(axis cs:71.3375796178344,0.0481198293409416)
--(axis cs:70.7006369426752,0.0485584763959539)
--(axis cs:70.0636942675159,0.0536448556656499)
--(axis cs:69.4267515923567,0.0562771524025745)
--(axis cs:68.7898089171974,0.0562049887784742)
--(axis cs:68.1528662420382,0.062832240487648)
--(axis cs:67.515923566879,0.0632008553969571)
--(axis cs:66.8789808917197,0.066461922485565)
--(axis cs:66.2420382165605,0.0696133515820928)
--(axis cs:65.6050955414013,0.0686449169353234)
--(axis cs:64.968152866242,0.0690080401059069)
--(axis cs:64.3312101910828,0.0716455208953657)
--(axis cs:63.6942675159236,0.0705120327053249)
--(axis cs:63.0573248407643,0.074801320240258)
--(axis cs:62.4203821656051,0.0767755084015226)
--(axis cs:61.7834394904459,0.0780931793072857)
--(axis cs:61.1464968152866,0.0751368873341936)
--(axis cs:60.5095541401274,0.0812224341314759)
--(axis cs:59.8726114649682,0.0900246466345508)
--(axis cs:59.2356687898089,0.0900464576248561)
--(axis cs:58.5987261146497,0.0983341959427942)
--(axis cs:57.9617834394904,0.102755215327631)
--(axis cs:57.3248407643312,0.102376062055455)
--(axis cs:56.687898089172,0.10742489835899)
--(axis cs:56.0509554140127,0.106148063967514)
--(axis cs:55.4140127388535,0.0995389060252915)
--(axis cs:54.7770700636943,0.099108517363828)
--(axis cs:54.140127388535,0.102427914687477)
--(axis cs:53.5031847133758,0.105909589874104)
--(axis cs:52.8662420382166,0.10391164683163)
--(axis cs:52.2292993630573,0.104323927961108)
--(axis cs:51.5923566878981,0.108526164694506)
--(axis cs:50.9554140127388,0.116452321784375)
--(axis cs:50.3184713375796,0.115540741365406)
--(axis cs:49.6815286624204,0.114278802653965)
--(axis cs:49.0445859872611,0.110647439862581)
--(axis cs:48.4076433121019,0.111232274178538)
--(axis cs:47.7707006369427,0.116775626367446)
--(axis cs:47.1337579617834,0.115186255082584)
--(axis cs:46.4968152866242,0.1195808456558)
--(axis cs:45.859872611465,0.123169517099205)
--(axis cs:45.2229299363057,0.130450317548808)
--(axis cs:44.5859872611465,0.134943659891762)
--(axis cs:43.9490445859873,0.141684510803902)
--(axis cs:43.312101910828,0.145626764363068)
--(axis cs:42.6751592356688,0.150345738348076)
--(axis cs:42.0382165605096,0.150721702514007)
--(axis cs:41.4012738853503,0.14882129719975)
--(axis cs:40.7643312101911,0.148523976822716)
--(axis cs:40.1273885350318,0.151524729124013)
--(axis cs:39.4904458598726,0.154136705146038)
--(axis cs:38.8535031847134,0.155313688405815)
--(axis cs:38.2165605095541,0.16023814991488)
--(axis cs:37.5796178343949,0.164032084443014)
--(axis cs:36.9426751592357,0.166801824308634)
--(axis cs:36.3057324840764,0.171300091698144)
--(axis cs:35.6687898089172,0.174507751654244)
--(axis cs:35.031847133758,0.186607037468412)
--(axis cs:34.3949044585987,0.193032630489691)
--(axis cs:33.7579617834395,0.202908517161102)
--(axis cs:33.1210191082803,0.217085670425228)
--(axis cs:32.484076433121,0.227601229770155)
--(axis cs:31.8471337579618,0.237287284198674)
--(axis cs:31.2101910828025,0.246636050532827)
--(axis cs:30.5732484076433,0.260765251803034)
--(axis cs:29.9363057324841,0.271945097345391)
--(axis cs:29.2993630573248,0.283957284053438)
--(axis cs:28.6624203821656,0.288221257596404)
--(axis cs:28.0254777070064,0.302630337946317)
--(axis cs:27.3885350318471,0.319587348790354)
--(axis cs:26.7515923566879,0.330200998395493)
--(axis cs:26.1146496815287,0.341441560792582)
--(axis cs:25.4777070063694,0.356432979327382)
--(axis cs:24.8407643312102,0.375311016353083)
--(axis cs:24.203821656051,0.385350320030038)
--(axis cs:23.5668789808917,0.40442107071674)
--(axis cs:22.9299363057325,0.42508583703108)
--(axis cs:22.2929936305732,0.444162275013564)
--(axis cs:21.656050955414,0.465550151855527)
--(axis cs:21.0191082802548,0.47252551706346)
--(axis cs:20.3821656050955,0.49137813202217)
--(axis cs:19.7452229299363,0.519755264949403)
--(axis cs:19.1082802547771,0.536869997335769)
--(axis cs:18.4713375796178,0.558853569883583)
--(axis cs:17.8343949044586,0.582661762354621)
--(axis cs:17.1974522292994,0.608435921951948)
--(axis cs:16.5605095541401,0.620553237872858)
--(axis cs:15.9235668789809,0.63866975025314)
--(axis cs:15.2866242038217,0.659567366378676)
--(axis cs:14.6496815286624,0.674333624323341)
--(axis cs:14.0127388535032,0.699111137311181)
--(axis cs:13.3757961783439,0.717456705290758)
--(axis cs:12.7388535031847,0.742104488420692)
--(axis cs:12.1019108280255,0.76206072394035)
--(axis cs:11.4649681528662,0.783009583699379)
--(axis cs:10.828025477707,0.799952373514511)
--(axis cs:10.1910828025478,0.819278783303547)
--(axis cs:9.55414012738853,0.839432387120794)
--(axis cs:8.9171974522293,0.85780320379816)
--(axis cs:8.28025477707006,0.868174846999387)
--(axis cs:7.64331210191083,0.879366220283099)
--(axis cs:7.00636942675159,0.88641333071478)
--(axis cs:6.36942675159236,0.895049026736365)
--(axis cs:5.73248407643312,0.900500271237632)
--(axis cs:5.09554140127389,0.904052732418355)
--(axis cs:4.45859872611465,0.908602240221481)
--(axis cs:3.82165605095541,0.911385391498803)
--(axis cs:3.18471337579618,0.913261440802757)
--(axis cs:2.54777070063694,0.914711270798135)
--(axis cs:1.91082802547771,0.915468539249643)
--(axis cs:1.27388535031847,0.915738864289868)
--(axis cs:0.636942675159236,0.916006049296742)
--(axis cs:0,0.916046968073714)
--cycle;


==> img/mnist/mnist_rate_distortion_fw_multi_no_marker.tex <==
\addplot [line width=0.5, opacity=0.7, color0]
table {%
0 0.915408829675289
0.636942675159236 0.915382273662835
1.27388535031847 0.915096716852859
1.91082802547771 0.914692572912318
2.54777070063694 0.913862062830594
3.18471337579618 0.912135634987499
3.82165605095541 0.909847007238422
4.45859872611465 0.906684231007821
5.09554140127389 0.901666516910191
5.73248407643312 0.897687930468237
6.36942675159236 0.891821020462085
7.00636942675159 0.882395655786677
7.64331210191083 0.87498702386627
8.28025477707006 0.863144064748485
8.9171974522293 0.852229911468457
9.55414012738853 0.833246941481484
10.1910828025478 0.812610879683634
10.828025477707 0.792825166148832
11.4649681528662 0.775601980706851
12.1019108280255 0.754392843041569
12.7388535031847 0.734276171533856
13.3757961783439 0.709338013472443
14.0127388535032 0.6908908565616
14.6496815286624 0.665962172550644
15.2866242038217 0.65109059715789
15.9235668789809 0.63025334887905
16.5605095541401 0.611842870320252
17.1974522292994 0.599454988868092
17.8343949044586 0.573712249294622
18.4713375796178 0.549860144949635
19.1082802547771 0.52797399037634
19.7452229299363 0.511082286236342
20.3821656050955 0.48277777820942
21.0191082802548 0.464084515760769
21.656050955414 0.457098011275812
22.2929936305732 0.43569115015518
22.9299363057325 0.41689562018284
23.5668789808917 0.396277005168085
24.203821656051 0.377319218446792
24.8407643312102 0.367335590948132
25.4777070063694 0.348365006815948
26.1146496815287 0.333453813923734
26.7515923566879 0.32227280900117
27.3885350318471 0.311638022393417
28.0254777070064 0.294828007709493
28.6624203821656 0.280404937018156
29.2993630573248 0.27610515875454
29.9363057324841 0.264157310609116
30.5732484076433 0.253143067016294
31.2101910828025 0.239077157805257
31.8471337579618 0.229905061221345
32.484076433121 0.220284622668961
33.1210191082803 0.209879552711753
33.7579617834395 0.195899192405875
34.3949044585987 0.186291122548258
35.031847133758 0.180055678856907
35.6687898089172 0.168096910978574
36.3057324840764 0.164841537991507
36.9426751592357 0.160624155317777
37.5796178343949 0.157887313298977
38.2165605095541 0.154267737419665
38.8535031847134 0.149298551698007
39.4904458598726 0.148078675652336
40.1273885350318 0.145562303348656
40.7643312101911 0.14278459742922
41.4012738853503 0.143186102443022
42.0382165605096 0.145163542037156
42.6751592356688 0.144787398323333
43.312101910828 0.140348344975882
43.9490445859873 0.136248876780294
44.5859872611465 0.129739171930641
45.2229299363057 0.125223531424405
45.859872611465 0.117969579966437
46.4968152866242 0.11452360991743
47.1337579617834 0.110260872808379
47.7707006369427 0.111834452871629
48.4076433121019 0.106263380254686
49.0445859872611 0.10574532869924
49.6815286624204 0.10945046766122
50.3184713375796 0.110568706254168
50.9554140127388 0.111466150305739
51.5923566878981 0.103554940218896
52.2292993630573 0.0993581257647757
52.8662420382166 0.0989718502349765
53.5031847133758 0.100940247271179
54.140127388535 0.0975202009991361
54.7770700636943 0.0942375160085634
55.4140127388535 0.0946136234188508
56.0509554140127 0.101208402883192
56.687898089172 0.102575054375311
57.3248407643312 0.0975976766885219
57.9617834394904 0.0980750429620181
58.5987261146497 0.0937486159518336
59.2356687898089 0.0855829494186959
59.8726114649682 0.0856079226566187
60.5095541401274 0.0769698398435431
61.1464968152866 0.0710596391034464
61.7834394904459 0.0741075598484932
62.4203821656051 0.0728888746724271
63.0573248407643 0.0709565187197391
63.6942675159236 0.0666711332657636
64.3312101910828 0.0677817963684673
64.968152866242 0.0652890624020528
65.6050955414013 0.0649960667064047
66.2420382165605 0.0659710155876101
66.8789808917197 0.0629344602092929
67.515923566879 0.0596610833853472
68.1528662420382 0.0593300504704785
68.7898089171974 0.0529158416896006
69.4267515923567 0.0530788265476271
70.0636942675159 0.0504660058111919
70.7006369426752 0.04584325387265
71.3375796178344 0.0454424565584947
71.9745222929936 0.0439342650054907
72.6114649681529 0.0414550790936585
73.2484076433121 0.0393416239747551
73.8853503184713 0.0374506893893551
74.5222929936306 0.0378209570602172
75.1592356687898 0.0379107980088606
75.796178343949 0.0387693894238152
76.4331210191083 0.0404712585807834
77.0700636942675 0.0407964303150209
77.7070063694268 0.0385946275263931
78.343949044586 0.0383558567575824
78.9808917197452 0.0358113866591839
79.6178343949044 0.0352170386562531
80.2547770700637 0.0326357289196444
80.8917197452229 0.0333434887203322
81.5286624203822 0.0327794245189457
82.1656050955414 0.030925364627635
82.8025477707006 0.0260984672632294
83.4394904458599 0.0252757583062409
84.0764331210191 0.025232290484774
84.7133757961783 0.0254289273362259
85.3503184713376 0.0245441769334865
85.9872611464968 0.0235596044504842
86.6242038216561 0.0199210327242437
87.2611464968153 0.0161681138614545
87.8980891719745 0.0141949105019622
88.5350318471338 0.0119463086903251
89.171974522293 0.0119163774524236
89.8089171974522 0.0107255865565207
90.4458598726115 0.0110226444160015
91.0828025477707 0.0086978640916785
91.7197452229299 0.00638393845839051
92.3566878980892 0.00308879387423672
92.9936305732484 0.00161427338025528
93.6305732484076 0.00157834846004424
94.2675159235669 0.000866445819476157
94.9044585987261 0.000890618483785353
95.5414012738853 7.19723169072889e-05
96.1783439490446 2.74922238068126e-05
96.8152866242038 2.4619714830198e-05
97.4522292993631 6.76046705217925e-06
98.0891719745223 4.47163104689896e-06
98.7261146496815 4.03964714622729e-06
99.3630573248408 2.36091867617694e-06
100 0
};
\path [fill=color0, fill opacity=0.25] 
(axis cs:0,0.916046968073714)
--(axis cs:0,0.914770691276864)
--(axis cs:0.636942675159236,0.914758498028928)
--(axis cs:1.27388535031847,0.91445456941585)
--(axis cs:1.91082802547771,0.913916606574993)
--(axis cs:2.54777070063694,0.913012854863054)
--(axis cs:3.18471337579618,0.91100982917224)
--(axis cs:3.82165605095541,0.908308622978042)
--(axis cs:4.45859872611465,0.904766221794161)
--(axis cs:5.09554140127389,0.899280301402026)
--(axis cs:5.73248407643312,0.894875589698842)
--(axis cs:6.36942675159236,0.888593014187804)
--(axis cs:7.00636942675159,0.878377980858574)
--(axis cs:7.64331210191083,0.870607827449441)
--(axis cs:8.28025477707006,0.858113282497584)
--(axis cs:8.9171974522293,0.846656619138755)
--(axis cs:9.55414012738853,0.827061495842175)
--(axis cs:10.1910828025478,0.805942976063722)
--(axis cs:10.828025477707,0.785697958783154)
--(axis cs:11.4649681528662,0.768194377714324)
--(axis cs:12.1019108280255,0.746724962142788)
--(axis cs:12.7388535031847,0.726447854647021)
--(axis cs:13.3757961783439,0.701219321654128)
--(axis cs:14.0127388535032,0.682670575812019)
--(axis cs:14.6496815286624,0.657590720777947)
--(axis cs:15.2866242038217,0.642613827937105)
--(axis cs:15.9235668789809,0.621836947504961)
--(axis cs:16.5605095541401,0.603132502767645)
--(axis cs:17.1974522292994,0.590474055784236)
--(axis cs:17.8343949044586,0.564762736234623)
--(axis cs:18.4713375796178,0.540866720015686)
--(axis cs:19.1082802547771,0.519077983416912)
--(axis cs:19.7452229299363,0.502409307523281)
--(axis cs:20.3821656050955,0.47417742439667)
--(axis cs:21.0191082802548,0.455643514458078)
--(axis cs:21.656050955414,0.448645870696096)
--(axis cs:22.2929936305732,0.427220025296796)
--(axis cs:22.9299363057325,0.408705403334601)
--(axis cs:23.5668789808917,0.388132939619431)
--(axis cs:24.203821656051,0.369288116863546)
--(axis cs:24.8407643312102,0.359360165543182)
--(axis cs:25.4777070063694,0.340297034304513)
--(axis cs:26.1146496815287,0.325466067054886)
--(axis cs:26.7515923566879,0.314344619606846)
--(axis cs:27.3885350318471,0.303688695996481)
--(axis cs:28.0254777070064,0.287025677472669)
--(axis cs:28.6624203821656,0.272588616439909)
--(axis cs:29.2993630573248,0.268253033455642)
--(axis cs:29.9363057324841,0.256369523872842)
--(axis cs:30.5732484076433,0.245520882229554)
--(axis cs:31.2101910828025,0.231518265077687)
--(axis cs:31.8471337579618,0.222522838244016)
--(axis cs:32.484076433121,0.212968015567766)
--(axis cs:33.1210191082803,0.202673434998279)
--(axis cs:33.7579617834395,0.188889867650648)
--(axis cs:34.3949044585987,0.179549614606825)
--(axis cs:35.031847133758,0.173504320245402)
--(axis cs:35.6687898089172,0.161686070302905)
--(axis cs:36.3057324840764,0.15838298428487)
--(axis cs:36.9426751592357,0.15444648632692)
--(axis cs:37.5796178343949,0.151742542154941)
--(axis cs:38.2165605095541,0.14829732492445)
--(axis cs:38.8535031847134,0.1432834149902)
--(axis cs:39.4904458598726,0.142020646158634)
--(axis cs:40.1273885350318,0.139599877573298)
--(axis cs:40.7643312101911,0.137045218035725)
--(axis cs:41.4012738853503,0.137550907686294)
--(axis cs:42.0382165605096,0.139605381560305)
--(axis cs:42.6751592356688,0.139229058298589)
--(axis cs:43.312101910828,0.135069925588695)
--(axis cs:43.9490445859873,0.130813242756685)
--(axis cs:44.5859872611465,0.124534683969521)
--(axis cs:45.2229299363057,0.119996745300002)
--(axis cs:45.859872611465,0.112769642833669)
--(axis cs:46.4968152866242,0.10946637417906)
--(axis cs:47.1337579617834,0.105335490534174)
--(axis cs:47.7707006369427,0.106893279375812)
--(axis cs:48.4076433121019,0.101294486330835)
--(axis cs:49.0445859872611,0.1008432175359)
--(axis cs:49.6815286624204,0.104622132668475)
--(axis cs:50.3184713375796,0.105596671142931)
--(axis cs:50.9554140127388,0.106479978827102)
--(axis cs:51.5923566878981,0.0985837157432871)
--(axis cs:52.2292993630573,0.0943923235684435)
--(axis cs:52.8662420382166,0.0940320536383234)
--(axis cs:53.5031847133758,0.095970904668254)
--(axis cs:54.140127388535,0.0926124873107951)
--(axis cs:54.7770700636943,0.0893665146532989)
--(axis cs:55.4140127388535,0.08968834081241)
--(axis cs:56.0509554140127,0.0962687417988696)
--(axis cs:56.687898089172,0.0977252103916324)
--(axis cs:57.3248407643312,0.0928192913215886)
--(axis cs:57.9617834394904,0.0933948705964049)
--(axis cs:58.5987261146497,0.0891630359608729)
--(axis cs:59.2356687898089,0.0811194412125356)
--(axis cs:59.8726114649682,0.0811911986786866)
--(axis cs:60.5095541401274,0.0727172455556102)
--(axis cs:61.1464968152866,0.0669823908726992)
--(axis cs:61.7834394904459,0.0701219403897007)
--(axis cs:62.4203821656051,0.0690022409433317)
--(axis cs:63.0573248407643,0.0671117171992203)
--(axis cs:63.6942675159236,0.0628302338262023)
--(axis cs:64.3312101910828,0.063918071841569)
--(axis cs:64.968152866242,0.0615700846981986)
--(axis cs:65.6050955414013,0.0613472164774861)
--(axis cs:66.2420382165605,0.0623286795931275)
--(axis cs:66.8789808917197,0.0594069979330209)
--(axis cs:67.515923566879,0.0561213113737372)
--(axis cs:68.1528662420382,0.0558278604533091)
--(axis cs:68.7898089171974,0.049626694600727)
--(axis cs:69.4267515923567,0.0498805006926798)
--(axis cs:70.0636942675159,0.0472871559567338)
--(axis cs:70.7006369426752,0.0431280313493462)
--(axis cs:71.3375796178344,0.0427650837760479)
--(axis cs:71.9745222929936,0.041273352376369)
--(axis cs:72.6114649681529,0.0389389197804142)
--(axis cs:73.2484076433121,0.0369884025937297)
--(axis cs:73.8853503184713,0.0352295385177088)
--(axis cs:74.5222929936306,0.0355107271548963)
--(axis cs:75.1592356687898,0.0357369934880207)
--(axis cs:75.796178343949,0.0369032424356471)
--(axis cs:76.4331210191083,0.0387632501271824)
--(axis cs:77.0700636942675,0.0389615797559466)
--(axis cs:77.7070063694268,0.036867514980996)
--(axis cs:78.343949044586,0.0367625989679835)
--(axis cs:78.9808917197452,0.0340216594034645)
--(axis cs:79.6178343949044,0.033468805765597)
--(axis cs:80.2547770700637,0.0307967537621799)
--(axis cs:80.8917197452229,0.031437428253213)
--(axis cs:81.5286624203822,0.0309884691277693)
--(axis cs:82.1656050955414,0.0289881509381444)
--(axis cs:82.8025477707006,0.0243594471735647)
--(axis cs:83.4394904458599,0.0233958379601799)
--(axis cs:84.0764331210191,0.023360811656067)
--(axis cs:84.7133757961783,0.0236349782732255)
--(axis cs:85.3503184713376,0.0228755526422535)
--(axis cs:85.9872611464968,0.0218937718287899)
--(axis cs:86.6242038216561,0.0186064654773654)
--(axis cs:87.2611464968153,0.0150264173303497)
--(axis cs:87.8980891719745,0.0130315296408964)
--(axis cs:88.5350318471338,0.0106272034435599)
--(axis cs:89.171974522293,0.0107280692483413)
--(axis cs:89.8089171974522,0.00945065306082912)
--(axis cs:90.4458598726115,0.0097430173143508)
--(axis cs:91.0828025477707,0.00742394150640178)
--(axis cs:91.7197452229299,0.00516138962103678)
--(axis cs:92.3566878980892,0.00225390964791465)
--(axis cs:92.9936305732484,0.00101118625840771)
--(axis cs:93.6305732484076,0.000989369778582739)
--(axis cs:94.2675159235669,0.000466921350769647)
--(axis cs:94.9044585987261,0.000494729316102132)
--(axis cs:95.5414012738853,3.69873910191497e-05)
--(axis cs:96.1783439490446,2.66853071952282e-07)
--(axis cs:96.8152866242038,1.28613316776119e-05)
--(axis cs:97.4522292993631,4.80411163867161e-06)
--(axis cs:98.0891719745223,3.79659651900197e-06)
--(axis cs:98.7261146496815,3.74252852109559e-06)
--(axis cs:99.3630573248408,2.086317169157e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,2.63552018319688e-06)
--(axis cs:98.7261146496815,4.33676577135899e-06)
--(axis cs:98.0891719745223,5.14666557479595e-06)
--(axis cs:97.4522292993631,8.71682246568689e-06)
--(axis cs:96.8152866242038,3.63780979827841e-05)
--(axis cs:96.1783439490446,5.47175945416729e-05)
--(axis cs:95.5414012738853,0.000106957242795428)
--(axis cs:94.9044585987261,0.00128650765146857)
--(axis cs:94.2675159235669,0.00126597028818267)
--(axis cs:93.6305732484076,0.00216732714150574)
--(axis cs:92.9936305732484,0.00221736050210285)
--(axis cs:92.3566878980892,0.00392367810055879)
--(axis cs:91.7197452229299,0.00760648729574424)
--(axis cs:91.0828025477707,0.00997178667695522)
--(axis cs:90.4458598726115,0.0123022715176523)
--(axis cs:89.8089171974522,0.0120005200522123)
--(axis cs:89.171974522293,0.0131046856565059)
--(axis cs:88.5350318471338,0.0132654139370902)
--(axis cs:87.8980891719745,0.015358291363028)
--(axis cs:87.2611464968153,0.0173098103925593)
--(axis cs:86.6242038216561,0.021235599971122)
--(axis cs:85.9872611464968,0.0252254370721784)
--(axis cs:85.3503184713376,0.0262128012247194)
--(axis cs:84.7133757961783,0.0272228763992262)
--(axis cs:84.0764331210191,0.027103769313481)
--(axis cs:83.4394904458599,0.0271556786523018)
--(axis cs:82.8025477707006,0.0278374873528942)
--(axis cs:82.1656050955414,0.0328625783171255)
--(axis cs:81.5286624203822,0.0345703799101222)
--(axis cs:80.8917197452229,0.0352495491874513)
--(axis cs:80.2547770700637,0.0344747040771088)
--(axis cs:79.6178343949044,0.0369652715469092)
--(axis cs:78.9808917197452,0.0376011139149033)
--(axis cs:78.343949044586,0.0399491145471813)
--(axis cs:77.7070063694268,0.0403217400717902)
--(axis cs:77.0700636942675,0.0426312808740951)
--(axis cs:76.4331210191083,0.0421792670343843)
--(axis cs:75.796178343949,0.0406355364119834)
--(axis cs:75.1592356687898,0.0400846025297005)
--(axis cs:74.5222929936306,0.040131186965538)
--(axis cs:73.8853503184713,0.0396718402610015)
--(axis cs:73.2484076433121,0.0416948453557805)
--(axis cs:72.6114649681529,0.0439712384069027)
--(axis cs:71.9745222929936,0.0465951776346124)
--(axis cs:71.3375796178344,0.0481198293409416)
--(axis cs:70.7006369426752,0.0485584763959539)
--(axis cs:70.0636942675159,0.0536448556656499)
--(axis cs:69.4267515923567,0.0562771524025745)
--(axis cs:68.7898089171974,0.0562049887784742)
--(axis cs:68.1528662420382,0.062832240487648)
--(axis cs:67.515923566879,0.0632008553969571)
--(axis cs:66.8789808917197,0.066461922485565)
--(axis cs:66.2420382165605,0.0696133515820928)
--(axis cs:65.6050955414013,0.0686449169353234)
--(axis cs:64.968152866242,0.0690080401059069)
--(axis cs:64.3312101910828,0.0716455208953657)
--(axis cs:63.6942675159236,0.0705120327053249)
--(axis cs:63.0573248407643,0.074801320240258)
--(axis cs:62.4203821656051,0.0767755084015226)
--(axis cs:61.7834394904459,0.0780931793072857)
--(axis cs:61.1464968152866,0.0751368873341936)
--(axis cs:60.5095541401274,0.0812224341314759)
--(axis cs:59.8726114649682,0.0900246466345508)
--(axis cs:59.2356687898089,0.0900464576248561)
--(axis cs:58.5987261146497,0.0983341959427942)
--(axis cs:57.9617834394904,0.102755215327631)
--(axis cs:57.3248407643312,0.102376062055455)
--(axis cs:56.687898089172,0.10742489835899)
--(axis cs:56.0509554140127,0.106148063967514)
--(axis cs:55.4140127388535,0.0995389060252915)
--(axis cs:54.7770700636943,0.099108517363828)
--(axis cs:54.140127388535,0.102427914687477)
--(axis cs:53.5031847133758,0.105909589874104)
--(axis cs:52.8662420382166,0.10391164683163)
--(axis cs:52.2292993630573,0.104323927961108)
--(axis cs:51.5923566878981,0.108526164694506)
--(axis cs:50.9554140127388,0.116452321784375)
--(axis cs:50.3184713375796,0.115540741365406)
--(axis cs:49.6815286624204,0.114278802653965)
--(axis cs:49.0445859872611,0.110647439862581)
--(axis cs:48.4076433121019,0.111232274178538)
--(axis cs:47.7707006369427,0.116775626367446)
--(axis cs:47.1337579617834,0.115186255082584)
--(axis cs:46.4968152866242,0.1195808456558)
--(axis cs:45.859872611465,0.123169517099205)
--(axis cs:45.2229299363057,0.130450317548808)
--(axis cs:44.5859872611465,0.134943659891762)
--(axis cs:43.9490445859873,0.141684510803902)
--(axis cs:43.312101910828,0.145626764363068)
--(axis cs:42.6751592356688,0.150345738348076)
--(axis cs:42.0382165605096,0.150721702514007)
--(axis cs:41.4012738853503,0.14882129719975)
--(axis cs:40.7643312101911,0.148523976822716)
--(axis cs:40.1273885350318,0.151524729124013)
--(axis cs:39.4904458598726,0.154136705146038)
--(axis cs:38.8535031847134,0.155313688405815)
--(axis cs:38.2165605095541,0.16023814991488)
--(axis cs:37.5796178343949,0.164032084443014)
--(axis cs:36.9426751592357,0.166801824308634)
--(axis cs:36.3057324840764,0.171300091698144)
--(axis cs:35.6687898089172,0.174507751654244)
--(axis cs:35.031847133758,0.186607037468412)
--(axis cs:34.3949044585987,0.193032630489691)
--(axis cs:33.7579617834395,0.202908517161102)
--(axis cs:33.1210191082803,0.217085670425228)
--(axis cs:32.484076433121,0.227601229770155)
--(axis cs:31.8471337579618,0.237287284198674)
--(axis cs:31.2101910828025,0.246636050532827)
--(axis cs:30.5732484076433,0.260765251803034)
--(axis cs:29.9363057324841,0.271945097345391)
--(axis cs:29.2993630573248,0.283957284053438)
--(axis cs:28.6624203821656,0.288221257596404)
--(axis cs:28.0254777070064,0.302630337946317)
--(axis cs:27.3885350318471,0.319587348790354)
--(axis cs:26.7515923566879,0.330200998395493)
--(axis cs:26.1146496815287,0.341441560792582)
--(axis cs:25.4777070063694,0.356432979327382)
--(axis cs:24.8407643312102,0.375311016353083)
--(axis cs:24.203821656051,0.385350320030038)
--(axis cs:23.5668789808917,0.40442107071674)
--(axis cs:22.9299363057325,0.42508583703108)
--(axis cs:22.2929936305732,0.444162275013564)
--(axis cs:21.656050955414,0.465550151855527)
--(axis cs:21.0191082802548,0.47252551706346)
--(axis cs:20.3821656050955,0.49137813202217)
--(axis cs:19.7452229299363,0.519755264949403)
--(axis cs:19.1082802547771,0.536869997335769)
--(axis cs:18.4713375796178,0.558853569883583)
--(axis cs:17.8343949044586,0.582661762354621)
--(axis cs:17.1974522292994,0.608435921951948)
--(axis cs:16.5605095541401,0.620553237872858)
--(axis cs:15.9235668789809,0.63866975025314)
--(axis cs:15.2866242038217,0.659567366378676)
--(axis cs:14.6496815286624,0.674333624323341)
--(axis cs:14.0127388535032,0.699111137311181)
--(axis cs:13.3757961783439,0.717456705290758)
--(axis cs:12.7388535031847,0.742104488420692)
--(axis cs:12.1019108280255,0.76206072394035)
--(axis cs:11.4649681528662,0.783009583699379)
--(axis cs:10.828025477707,0.799952373514511)
--(axis cs:10.1910828025478,0.819278783303547)
--(axis cs:9.55414012738853,0.839432387120794)
--(axis cs:8.9171974522293,0.85780320379816)
--(axis cs:8.28025477707006,0.868174846999387)
--(axis cs:7.64331210191083,0.879366220283099)
--(axis cs:7.00636942675159,0.88641333071478)
--(axis cs:6.36942675159236,0.895049026736365)
--(axis cs:5.73248407643312,0.900500271237632)
--(axis cs:5.09554140127389,0.904052732418355)
--(axis cs:4.45859872611465,0.908602240221481)
--(axis cs:3.82165605095541,0.911385391498803)
--(axis cs:3.18471337579618,0.913261440802757)
--(axis cs:2.54777070063694,0.914711270798135)
--(axis cs:1.91082802547771,0.915468539249643)
--(axis cs:1.27388535031847,0.915738864289868)
--(axis cs:0.636942675159236,0.916006049296742)
--(axis cs:0,0.916046968073714)
--cycle;


==> img/mnist/mnist_rate_distortion_fw_order.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.915490757476073
0.636942675159236 0.915010578921065
1.27388535031847 0.91474760026671
1.91082802547771 0.913731540681329
2.54777070063694 0.912833051431808
3.18471337579618 0.910338926757395
3.82165605095541 0.908131302742404
4.45859872611465 0.904314485385548
5.09554140127389 0.900703856719192
5.73248407643312 0.894997748746537
6.36942675159236 0.884814730351791
7.00636942675159 0.872288584357593
7.64331210191083 0.861574653004063
8.28025477707006 0.8512276030879
8.9171974522293 0.835432431065128
9.55414012738853 0.81848026470514
10.1910828025478 0.801492734531057
10.828025477707 0.783014331809245
11.4649681528662 0.760755784951616
12.1019108280255 0.741032668385888
12.7388535031847 0.722253538860241
13.3757961783439 0.704743739494588
14.0127388535032 0.682183756221784
14.6496815286624 0.666005319076357
15.2866242038217 0.647023542562674
15.9235668789809 0.633797323008184
16.5605095541401 0.619108323656255
17.1974522292994 0.604681816396769
17.8343949044586 0.583126717983978
18.4713375796178 0.56537146605202
19.1082802547771 0.547962441461859
19.7452229299363 0.533551940793404
20.3821656050955 0.523774644096848
21.0191082802548 0.505692585278884
21.656050955414 0.491664368996862
22.2929936305732 0.469802147391601
22.9299363057325 0.465561343732406
23.5668789808917 0.45033424034249
24.203821656051 0.43870364689501
24.8407643312102 0.426704705747543
25.4777070063694 0.410277907369018
26.1146496815287 0.391110377481818
26.7515923566879 0.380626496158075
27.3885350318471 0.371288379465404
28.0254777070064 0.355947949805995
28.6624203821656 0.348856199535803
29.2993630573248 0.337521006990064
29.9363057324841 0.327405258433628
30.5732484076433 0.314921620041805
31.2101910828025 0.309278398844508
31.8471337579618 0.299502296792489
32.484076433121 0.290515115989401
33.1210191082803 0.282258794739405
33.7579617834395 0.272443165287013
34.3949044585987 0.2654104744151
35.031847133758 0.258167278593064
35.6687898089172 0.24716870286853
36.3057324840764 0.23517200814216
36.9426751592357 0.224006512443573
37.5796178343949 0.223529008037713
38.2165605095541 0.214265693090365
38.8535031847134 0.210125706997982
39.4904458598726 0.202261028173446
40.1273885350318 0.203957116486441
40.7643312101911 0.204287050673341
41.4012738853503 0.201972470336243
42.0382165605096 0.201477336334298
42.6751592356688 0.201999550199111
43.312101910828 0.194133163585774
43.9490445859873 0.187755093145822
44.5859872611465 0.178515542072111
45.2229299363057 0.169968437557602
45.859872611465 0.165917585048876
46.4968152866242 0.160812498745648
47.1337579617834 0.151848262350501
47.7707006369427 0.146728808936859
48.4076433121019 0.140738722643295
49.0445859872611 0.137266037870776
49.6815286624204 0.132999625906015
50.3184713375796 0.133878470637639
50.9554140127388 0.129242176802186
51.5923566878981 0.122025740680056
52.2292993630573 0.123652576529417
52.8662420382166 0.118790074312728
53.5031847133758 0.117015596803597
54.140127388535 0.114726295740873
54.7770700636943 0.112152223481626
55.4140127388535 0.108101919763113
56.0509554140127 0.107083826029764
56.687898089172 0.103681851645894
57.3248407643312 0.0945738534637306
57.9617834394904 0.0929616215668218
58.5987261146497 0.0875148893231253
59.2356687898089 0.0803962954585116
59.8726114649682 0.0815594425908866
60.5095541401274 0.0716300295249747
61.1464968152866 0.0769246710650455
61.7834394904459 0.0760485162789313
62.4203821656051 0.0663571526837927
63.0573248407643 0.0689823783303061
63.6942675159236 0.0680411840005914
64.3312101910828 0.0670130108743147
64.968152866242 0.0626997709592758
65.6050955414013 0.0609093250881482
66.2420382165605 0.0557579271406364
66.8789808917197 0.0556030822238488
67.515923566879 0.0538660674944618
68.1528662420382 0.054423102090598
68.7898089171974 0.0481867490460544
69.4267515923567 0.0453662193938075
70.0636942675159 0.0438505820632875
70.7006369426752 0.0410007922745191
71.3375796178344 0.036494375214986
71.9745222929936 0.0306591349412725
72.6114649681529 0.0309642506185686
73.2484076433121 0.0309972415875784
73.8853503184713 0.0309658658669362
74.5222929936306 0.0279121405922089
75.1592356687898 0.0285008299376513
75.796178343949 0.0261668233992469
76.4331210191083 0.0256680856005212
77.0700636942675 0.0256736535101499
77.7070063694268 0.0242302013705633
78.343949044586 0.0237935097687121
78.9808917197452 0.0219264485699415
79.6178343949044 0.019340282296364
80.2547770700637 0.0172226791757759
80.8917197452229 0.0164835267576751
81.5286624203822 0.0139280988254476
82.1656050955414 0.0154918600868149
82.8025477707006 0.0143571076261909
83.4394904458599 0.0116984653044452
84.0764331210191 0.0112247785074742
84.7133757961783 0.0107605307436082
85.3503184713376 0.0122233772917573
85.9872611464968 0.0117261204794443
86.6242038216561 0.012617092321366
87.2611464968153 0.0115146347852646
87.8980891719745 0.0107801469898101
88.5350318471338 0.00993264867604242
89.171974522293 0.00968955186020458
89.8089171974522 0.0100993693598469
90.4458598726115 0.0080032420835381
91.0828025477707 0.00689530079517576
91.7197452229299 0.00642026233892175
92.3566878980892 0.00622262683679131
92.9936305732484 0.00270834194648978
93.6305732484076 0.00246532910370482
94.2675159235669 0.00122089033765662
94.9044585987261 0.000516502282106331
95.5414012738853 0.000369256059101039
96.1783439490446 0.000165554465234062
96.8152866242038 3.22102742854613e-05
97.4522292993631 9.50395738726462e-06
98.0891719745223 1.45919854073745e-05
98.7261146496815 5.03299618816344e-06
99.3630573248408 3.42381275547921e-06
100 0
};
\path [fill=color0, fill opacity=0.25] 
(axis cs:0,0.916100062167314)
--(axis cs:0,0.914881452784832)
--(axis cs:0.636942675159236,0.914313470814677)
--(axis cs:1.27388535031847,0.913973501996698)
--(axis cs:1.91082802547771,0.912790047561995)
--(axis cs:2.54777070063694,0.911803908594342)
--(axis cs:3.18471337579618,0.908949312724014)
--(axis cs:3.82165605095541,0.906420631841596)
--(axis cs:4.45859872611465,0.90217596296448)
--(axis cs:5.09554140127389,0.898221813561444)
--(axis cs:5.73248407643312,0.89196893655229)
--(axis cs:6.36942675159236,0.881033604149817)
--(axis cs:7.00636942675159,0.867699842986039)
--(axis cs:7.64331210191083,0.856492348194026)
--(axis cs:8.28025477707006,0.845751708922243)
--(axis cs:8.9171974522293,0.829323574164503)
--(axis cs:9.55414012738853,0.811817471678268)
--(axis cs:10.1910828025478,0.794489477944479)
--(axis cs:10.828025477707,0.775658943879808)
--(axis cs:11.4649681528662,0.753338156681822)
--(axis cs:12.1019108280255,0.733234903401258)
--(axis cs:12.7388535031847,0.714471442987423)
--(axis cs:13.3757961783439,0.696734604956684)
--(axis cs:14.0127388535032,0.674143460176928)
--(axis cs:14.6496815286624,0.657813836346996)
--(axis cs:15.2866242038217,0.638816985535322)
--(axis cs:15.9235668789809,0.625521122223058)
--(axis cs:16.5605095541401,0.610771509975498)
--(axis cs:17.1974522292994,0.596207472946174)
--(axis cs:17.8343949044586,0.574474333746119)
--(axis cs:18.4713375796178,0.556802789728624)
--(axis cs:19.1082802547771,0.539443872060295)
--(axis cs:19.7452229299363,0.524958648376389)
--(axis cs:20.3821656050955,0.515181872472168)
--(axis cs:21.0191082802548,0.497204321368023)
--(axis cs:21.656050955414,0.483049116118195)
--(axis cs:22.2929936305732,0.46131421020468)
--(axis cs:22.9299363057325,0.457099147478552)
--(axis cs:23.5668789808917,0.441958735837767)
--(axis cs:24.203821656051,0.43037850212472)
--(axis cs:24.8407643312102,0.418266031271644)
--(axis cs:25.4777070063694,0.402088639814172)
--(axis cs:26.1146496815287,0.382997735873359)
--(axis cs:26.7515923566879,0.372511943090763)
--(axis cs:27.3885350318471,0.363149333056008)
--(axis cs:28.0254777070064,0.347825937360697)
--(axis cs:28.6624203821656,0.340886555574605)
--(axis cs:29.2993630573248,0.329863707321403)
--(axis cs:29.9363057324841,0.319759799170471)
--(axis cs:30.5732484076433,0.307311513465389)
--(axis cs:31.2101910828025,0.301848237648928)
--(axis cs:31.8471337579618,0.292142371043693)
--(axis cs:32.484076433121,0.283358083904977)
--(axis cs:33.1210191082803,0.275257659202738)
--(axis cs:33.7579617834395,0.265618024698019)
--(axis cs:34.3949044585987,0.258724345011548)
--(axis cs:35.031847133758,0.251550664905785)
--(axis cs:35.6687898089172,0.240738690999376)
--(axis cs:36.3057324840764,0.228795926505741)
--(axis cs:36.9426751592357,0.217552693814755)
--(axis cs:37.5796178343949,0.217050514252541)
--(axis cs:38.2165605095541,0.20785942503929)
--(axis cs:38.8535031847134,0.203721377321834)
--(axis cs:39.4904458598726,0.195991522173591)
--(axis cs:40.1273885350318,0.197790052310887)
--(axis cs:40.7643312101911,0.198010717572202)
--(axis cs:41.4012738853503,0.195665232032491)
--(axis cs:42.0382165605096,0.195069465696254)
--(axis cs:42.6751592356688,0.195616225211938)
--(axis cs:43.312101910828,0.188077526794096)
--(axis cs:43.9490445859873,0.181779218691024)
--(axis cs:44.5859872611465,0.172530720521934)
--(axis cs:45.2229299363057,0.164194905857222)
--(axis cs:45.859872611465,0.160160465492948)
--(axis cs:46.4968152866242,0.155106428420468)
--(axis cs:47.1337579617834,0.14641312548827)
--(axis cs:47.7707006369427,0.141570019758668)
--(axis cs:48.4076433121019,0.135610048119995)
--(axis cs:49.0445859872611,0.132049176350975)
--(axis cs:49.6815286624204,0.127868487687145)
--(axis cs:50.3184713375796,0.128744844505951)
--(axis cs:50.9554140127388,0.124385867538685)
--(axis cs:51.5923566878981,0.117342221037114)
--(axis cs:52.2292993630573,0.118716718795554)
--(axis cs:52.8662420382166,0.113909362035174)
--(axis cs:53.5031847133758,0.112179083309142)
--(axis cs:54.140127388535,0.109916183562901)
--(axis cs:54.7770700636943,0.107493845599653)
--(axis cs:55.4140127388535,0.103455378336494)
--(axis cs:56.0509554140127,0.102329834727626)
--(axis cs:56.687898089172,0.0990438745495599)
--(axis cs:57.3248407643312,0.089870913279641)
--(axis cs:57.9617834394904,0.0883235473325405)
--(axis cs:58.5987261146497,0.0829602161434079)
--(axis cs:59.2356687898089,0.0760454442173949)
--(axis cs:59.8726114649682,0.0770347474792299)
--(axis cs:60.5095541401274,0.0674510529350946)
--(axis cs:61.1464968152866,0.0726095179329717)
--(axis cs:61.7834394904459,0.0716729650015062)
--(axis cs:62.4203821656051,0.0622942871205183)
--(axis cs:63.0573248407643,0.0649495420341071)
--(axis cs:63.6942675159236,0.0641924196552681)
--(axis cs:64.3312101910828,0.0631545728888824)
--(axis cs:64.968152866242,0.0589943403491474)
--(axis cs:65.6050955414013,0.0570145340255955)
--(axis cs:66.2420382165605,0.0519828394923702)
--(axis cs:66.8789808917197,0.051829920723736)
--(axis cs:67.515923566879,0.0502344726966771)
--(axis cs:68.1528662420382,0.0508521428555006)
--(axis cs:68.7898089171974,0.0447308754219712)
--(axis cs:69.4267515923567,0.0421355391246224)
--(axis cs:70.0636942675159,0.0407054535664607)
--(axis cs:70.7006369426752,0.0378853156499804)
--(axis cs:71.3375796178344,0.0335577590720622)
--(axis cs:71.9745222929936,0.0279315919537981)
--(axis cs:72.6114649681529,0.0283790800094467)
--(axis cs:73.2484076433121,0.0286801084327589)
--(axis cs:73.8853503184713,0.0287299883868922)
--(axis cs:74.5222929936306,0.0258127243393731)
--(axis cs:75.1592356687898,0.026357739363367)
--(axis cs:75.796178343949,0.024315894581346)
--(axis cs:76.4331210191083,0.0239304430312103)
--(axis cs:77.0700636942675,0.024043555160736)
--(axis cs:77.7070063694268,0.0227185099147879)
--(axis cs:78.343949044586,0.0221744552947268)
--(axis cs:78.9808917197452,0.0203570971171407)
--(axis cs:79.6178343949044,0.0178914818319974)
--(axis cs:80.2547770700637,0.015665781905156)
--(axis cs:80.8917197452229,0.0151413120097857)
--(axis cs:81.5286624203822,0.0125031925088592)
--(axis cs:82.1656050955414,0.014213472812096)
--(axis cs:82.8025477707006,0.0131599528069635)
--(axis cs:83.4394904458599,0.0104172641456342)
--(axis cs:84.0764331210191,0.00990588454552366)
--(axis cs:84.7133757961783,0.00953143308998765)
--(axis cs:85.3503184713376,0.0111041049983678)
--(axis cs:85.9872611464968,0.0106076787270567)
--(axis cs:86.6242038216561,0.0115501270571344)
--(axis cs:87.2611464968153,0.010380503120465)
--(axis cs:87.8980891719745,0.00959682235244195)
--(axis cs:88.5350318471338,0.00877357425604173)
--(axis cs:89.171974522293,0.00860284846068601)
--(axis cs:89.8089171974522,0.0090318120844762)
--(axis cs:90.4458598726115,0.00689410928134059)
--(axis cs:91.0828025477707,0.00587141634065444)
--(axis cs:91.7197452229299,0.00544597560469419)
--(axis cs:92.3566878980892,0.00518902643164934)
--(axis cs:92.9936305732484,0.0020620009013565)
--(axis cs:93.6305732484076,0.00188170634680726)
--(axis cs:94.2675159235669,0.000886161631766069)
--(axis cs:94.9044585987261,0.000371866935616938)
--(axis cs:95.5414012738853,0.000246883260322333)
--(axis cs:96.1783439490446,0.00010203649875553)
--(axis cs:96.8152866242038,2.04452126049707e-05)
--(axis cs:97.4522292993631,6.96400221629135e-06)
--(axis cs:98.0891719745223,1.01165965984184e-05)
--(axis cs:98.7261146496815,4.18702053372285e-06)
--(axis cs:99.3630573248408,2.7295464402826e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,4.11807907067581e-06)
--(axis cs:98.7261146496815,5.87897184260404e-06)
--(axis cs:98.0891719745223,1.90673742163306e-05)
--(axis cs:97.4522292993631,1.20439125582379e-05)
--(axis cs:96.8152866242038,4.39753359659519e-05)
--(axis cs:96.1783439490446,0.000229072431712593)
--(axis cs:95.5414012738853,0.000491628857879744)
--(axis cs:94.9044585987261,0.000661137628595725)
--(axis cs:94.2675159235669,0.00155561904354718)
--(axis cs:93.6305732484076,0.00304895186060238)
--(axis cs:92.9936305732484,0.00335468299162307)
--(axis cs:92.3566878980892,0.00725622724193328)
--(axis cs:91.7197452229299,0.00739454907314932)
--(axis cs:91.0828025477707,0.00791918524969709)
--(axis cs:90.4458598726115,0.00911237488573561)
--(axis cs:89.8089171974522,0.0111669266352177)
--(axis cs:89.171974522293,0.0107762552597231)
--(axis cs:88.5350318471338,0.0110917230960431)
--(axis cs:87.8980891719745,0.0119634716271783)
--(axis cs:87.2611464968153,0.0126487664500643)
--(axis cs:86.6242038216561,0.0136840575855976)
--(axis cs:85.9872611464968,0.0128445622318318)
--(axis cs:85.3503184713376,0.0133426495851468)
--(axis cs:84.7133757961783,0.0119896283972288)
--(axis cs:84.0764331210191,0.0125436724694248)
--(axis cs:83.4394904458599,0.0129796664632561)
--(axis cs:82.8025477707006,0.0155542624454184)
--(axis cs:82.1656050955414,0.0167702473615337)
--(axis cs:81.5286624203822,0.015353005142036)
--(axis cs:80.8917197452229,0.0178257415055646)
--(axis cs:80.2547770700637,0.0187795764463958)
--(axis cs:79.6178343949044,0.0207890827607306)
--(axis cs:78.9808917197452,0.0234958000227422)
--(axis cs:78.343949044586,0.0254125642426975)
--(axis cs:77.7070063694268,0.0257418928263388)
--(axis cs:77.0700636942675,0.0273037518595637)
--(axis cs:76.4331210191083,0.0274057281698321)
--(axis cs:75.796178343949,0.0280177522171479)
--(axis cs:75.1592356687898,0.0306439205119356)
--(axis cs:74.5222929936306,0.0300115568450447)
--(axis cs:73.8853503184713,0.0332017433469802)
--(axis cs:73.2484076433121,0.033314374742398)
--(axis cs:72.6114649681529,0.0335494212276905)
--(axis cs:71.9745222929936,0.033386677928747)
--(axis cs:71.3375796178344,0.0394309913579098)
--(axis cs:70.7006369426752,0.0441162688990578)
--(axis cs:70.0636942675159,0.0469957105601143)
--(axis cs:69.4267515923567,0.0485968996629927)
--(axis cs:68.7898089171974,0.0516426226701375)
--(axis cs:68.1528662420382,0.0579940613256955)
--(axis cs:67.515923566879,0.0574976622922464)
--(axis cs:66.8789808917197,0.0593762437239615)
--(axis cs:66.2420382165605,0.0595330147889026)
--(axis cs:65.6050955414013,0.0648041161507009)
--(axis cs:64.968152866242,0.0664052015694043)
--(axis cs:64.3312101910828,0.070871448859747)
--(axis cs:63.6942675159236,0.0718899483459146)
--(axis cs:63.0573248407643,0.073015214626505)
--(axis cs:62.4203821656051,0.0704200182470672)
--(axis cs:61.7834394904459,0.0804240675563564)
--(axis cs:61.1464968152866,0.0812398241971193)
--(axis cs:60.5095541401274,0.0758090061148548)
--(axis cs:59.8726114649682,0.0860841377025433)
--(axis cs:59.2356687898089,0.0847471466996283)
--(axis cs:58.5987261146497,0.0920695625028426)
--(axis cs:57.9617834394904,0.0975996958011031)
--(axis cs:57.3248407643312,0.0992767936478202)
--(axis cs:56.687898089172,0.108319828742228)
--(axis cs:56.0509554140127,0.111837817331903)
--(axis cs:55.4140127388535,0.112748461189733)
--(axis cs:54.7770700636943,0.1168106013636)
--(axis cs:54.140127388535,0.119536407918845)
--(axis cs:53.5031847133758,0.121852110298052)
--(axis cs:52.8662420382166,0.123670786590281)
--(axis cs:52.2292993630573,0.128588434263281)
--(axis cs:51.5923566878981,0.126709260322998)
--(axis cs:50.9554140127388,0.134098486065687)
--(axis cs:50.3184713375796,0.139012096769326)
--(axis cs:49.6815286624204,0.138130764124886)
--(axis cs:49.0445859872611,0.142482899390578)
--(axis cs:48.4076433121019,0.145867397166595)
--(axis cs:47.7707006369427,0.15188759811505)
--(axis cs:47.1337579617834,0.157283399212733)
--(axis cs:46.4968152866242,0.166518569070829)
--(axis cs:45.859872611465,0.171674704604804)
--(axis cs:45.2229299363057,0.175741969257983)
--(axis cs:44.5859872611465,0.184500363622288)
--(axis cs:43.9490445859873,0.193730967600621)
--(axis cs:43.312101910828,0.200188800377451)
--(axis cs:42.6751592356688,0.208382875186285)
--(axis cs:42.0382165605096,0.207885206972343)
--(axis cs:41.4012738853503,0.208279708639995)
--(axis cs:40.7643312101911,0.21056338377448)
--(axis cs:40.1273885350318,0.210124180661995)
--(axis cs:39.4904458598726,0.208530534173301)
--(axis cs:38.8535031847134,0.216530036674129)
--(axis cs:38.2165605095541,0.22067196114144)
--(axis cs:37.5796178343949,0.230007501822884)
--(axis cs:36.9426751592357,0.230460331072391)
--(axis cs:36.3057324840764,0.24154808977858)
--(axis cs:35.6687898089172,0.253598714737684)
--(axis cs:35.031847133758,0.264783892280343)
--(axis cs:34.3949044585987,0.272096603818653)
--(axis cs:33.7579617834395,0.279268305876008)
--(axis cs:33.1210191082803,0.289259930276072)
--(axis cs:32.484076433121,0.297672148073825)
--(axis cs:31.8471337579618,0.306862222541285)
--(axis cs:31.2101910828025,0.316708560040088)
--(axis cs:30.5732484076433,0.322531726618221)
--(axis cs:29.9363057324841,0.335050717696784)
--(axis cs:29.2993630573248,0.345178306658725)
--(axis cs:28.6624203821656,0.356825843497001)
--(axis cs:28.0254777070064,0.364069962251294)
--(axis cs:27.3885350318471,0.3794274258748)
--(axis cs:26.7515923566879,0.388741049225386)
--(axis cs:26.1146496815287,0.399223019090278)
--(axis cs:25.4777070063694,0.418467174923864)
--(axis cs:24.8407643312102,0.435143380223442)
--(axis cs:24.203821656051,0.4470287916653)
--(axis cs:23.5668789808917,0.458709744847214)
--(axis cs:22.9299363057325,0.474023539986261)
--(axis cs:22.2929936305732,0.478290084578523)
--(axis cs:21.656050955414,0.500279621875529)
--(axis cs:21.0191082802548,0.514180849189746)
--(axis cs:20.3821656050955,0.532367415721527)
--(axis cs:19.7452229299363,0.54214523321042)
--(axis cs:19.1082802547771,0.556481010863423)
--(axis cs:18.4713375796178,0.573940142375416)
--(axis cs:17.8343949044586,0.591779102221836)
--(axis cs:17.1974522292994,0.613156159847364)
--(axis cs:16.5605095541401,0.627445137337013)
--(axis cs:15.9235668789809,0.642073523793311)
--(axis cs:15.2866242038217,0.655230099590027)
--(axis cs:14.6496815286624,0.674196801805719)
--(axis cs:14.0127388535032,0.69022405226664)
--(axis cs:13.3757961783439,0.712752874032493)
--(axis cs:12.7388535031847,0.730035634733059)
--(axis cs:12.1019108280255,0.748830433370517)
--(axis cs:11.4649681528662,0.76817341322141)
--(axis cs:10.828025477707,0.790369719738682)
--(axis cs:10.1910828025478,0.808495991117635)
--(axis cs:9.55414012738853,0.825143057732012)
--(axis cs:8.9171974522293,0.841541287965754)
--(axis cs:8.28025477707006,0.856703497253558)
--(axis cs:7.64331210191083,0.866656957814101)
--(axis cs:7.00636942675159,0.876877325729148)
--(axis cs:6.36942675159236,0.888595856553764)
--(axis cs:5.73248407643312,0.898026560940783)
--(axis cs:5.09554140127389,0.90318589987694)
--(axis cs:4.45859872611465,0.906453007806616)
--(axis cs:3.82165605095541,0.909841973643212)
--(axis cs:3.18471337579618,0.911728540790776)
--(axis cs:2.54777070063694,0.913862194269274)
--(axis cs:1.91082802547771,0.914673033800663)
--(axis cs:1.27388535031847,0.915521698536722)
--(axis cs:0.636942675159236,0.915707687027453)
--(axis cs:0,0.916100062167314)
--cycle;


==> img/mnist/mnist_rate_distortion_guidedbackprop.tex <==
% guided backprop
\addplot [line width=0.5, opacity=0.8, color8, mark=oplus*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table [row sep=\\]{%
0	0.915419198935851 \\
0.636942675159236	0.915273207621649 \\
1.27388535031847	0.914707823789213 \\
1.91082802547771	0.913869507904165 \\
2.54777070063694	0.913013394752052 \\
3.18471337579618	0.912257456034422 \\
3.82165605095541	0.91129580319277 \\
4.45859872611465	0.91023811561754 \\
5.09554140127389	0.907923876760178 \\
5.73248407643312	0.906716485675424 \\
6.36942675159236	0.905768771958537 \\
7.00636942675159	0.90480525678955 \\
7.64331210191083	0.902187255311292 \\
8.28025477707006	0.902356616570614 \\
8.9171974522293	0.900493733673357 \\
9.55414012738853	0.898898315732367 \\
10.1910828025478	0.895839362008264 \\
10.828025477707	0.892950358011294 \\
11.4649681528662	0.890702503644861 \\
12.1019108280255	0.888129035192542 \\
12.7388535031847	0.886136925276369 \\
13.3757961783439	0.886812495104969 \\
14.0127388535032	0.884705520117423 \\
14.6496815286624	0.884087044079788 \\
15.2866242038217	0.885340465499321 \\
15.9235668789809	0.885402383042965 \\
16.5605095541401	0.88594211502932 \\
17.1974522292994	0.885218416661955 \\
17.8343949044586	0.885506086791865 \\
18.4713375796178	0.885428715795279 \\
19.1082802547771	0.887647928376682 \\
19.7452229299363	0.886752308830619 \\
20.3821656050955	0.887071484609041 \\
21.0191082802548	0.888027990973787 \\
21.656050955414	0.888410665821284 \\
22.2929936305732	0.889415876450948 \\
22.9299363057325	0.890130610123742 \\
23.5668789808917	0.890275635094731 \\
24.203821656051	0.891631569822784 \\
24.8407643312102	0.892620583759854 \\
25.4777070063694	0.893150180816883 \\
26.1146496815287	0.892903876749333 \\
26.7515923566879	0.896001957354601 \\
27.3885350318471	0.897022292610491 \\
28.0254777070064	0.896211718654959 \\
28.6624203821656	0.897029131529853 \\
29.2993630573248	0.896236566798762 \\
29.9363057324841	0.896939584694337 \\
30.5732484076433	0.897159007566515 \\
31.2101910828025	0.89871647606953 \\
31.8471337579618	0.897706985994591 \\
32.484076433121	0.899649071070016 \\
33.1210191082803	0.899592705316027 \\
33.7579617834395	0.898588186262641 \\
34.3949044585987	0.899876231305534 \\
35.031847133758	0.900660879960051 \\
35.6687898089172	0.901549399262294 \\
36.3057324840764	0.902794446302578 \\
36.9426751592357	0.901705311951227 \\
37.5796178343949	0.901079539398197 \\
38.2165605095541	0.903000890521216 \\
38.8535031847134	0.902829546070716 \\
39.4904458598726	0.902974730804563 \\
40.1273885350318	0.903853035534412 \\
40.7643312101911	0.902761922430363 \\
41.4012738853503	0.902434755390568 \\
42.0382165605096	0.903388551373209 \\
42.6751592356688	0.904235457034374 \\
43.312101910828	0.90555129257642 \\
43.9490445859873	0.904417628276715 \\
44.5859872611465	0.905949710298446 \\
45.2229299363057	0.905550172304502 \\
45.859872611465	0.906753421065223 \\
46.4968152866242	0.907238617627299 \\
47.1337579617834	0.908411964584448 \\
47.7707006369427	0.90829963987635 \\
48.4076433121019	0.907969056126894 \\
49.0445859872611	0.907433438767912 \\
49.6815286624204	0.907998645158223 \\
50.3184713375796	0.908573042987264 \\
50.9554140127388	0.909355449231225 \\
51.5923566878981	0.910093729257933 \\
52.2292993630573	0.909912631331244 \\
52.8662420382166	0.910952123866882 \\
53.5031847133758	0.911028368291445 \\
54.140127388535	0.911160915099317 \\
54.7770700636943	0.910749427694827 \\
55.4140127388535	0.911974737456185 \\
56.0509554140127	0.912093120565987 \\
56.687898089172	0.912046862507123 \\
57.3248407643312	0.911307904627174 \\
57.9617834394904	0.911712975404516 \\
58.5987261146497	0.911601988956099 \\
59.2356687898089	0.912493897862441 \\
59.8726114649682	0.912627178532639 \\
60.5095541401274	0.912731162615528 \\
61.1464968152866	0.91267963720682 \\
61.7834394904459	0.9124151742307 \\
62.4203821656051	0.911553988787018 \\
63.0573248407643	0.912145412716709 \\
63.6942675159236	0.911560647422521 \\
64.3312101910828	0.911748248105723 \\
64.968152866242	0.911549236170104 \\
65.6050955414013	0.910642357099241 \\
66.2420382165605	0.910081443866584 \\
66.8789808917197	0.909269277454005 \\
67.515923566879	0.907969251340892 \\
68.1528662420382	0.906702297338361 \\
68.7898089171974	0.906871107854604 \\
69.4267515923567	0.903943637889915 \\
70.0636942675159	0.904058258948717 \\
70.7006369426752	0.904690812151293 \\
71.3375796178344	0.904614957048043 \\
71.9745222929936	0.902753363943284 \\
72.6114649681529	0.899972072022856 \\
73.2484076433121	0.900007548634949 \\
73.8853503184713	0.898659834172286 \\
74.5222929936306	0.89608741213362 \\
75.1592356687898	0.895624526728079 \\
75.796178343949	0.892129921766973 \\
76.4331210191083	0.886886027570376 \\
77.0700636942675	0.884574898673968 \\
77.7070063694268	0.879935202053503 \\
78.343949044586	0.87738420896423 \\
78.9808917197452	0.873301222849014 \\
79.6178343949044	0.859459846226149 \\
80.2547770700637	0.851381972051854 \\
80.8917197452229	0.838325049061837 \\
81.5286624203822	0.827744927312669 \\
82.1656050955414	0.815138128031444 \\
82.8025477707006	0.797497767517543 \\
83.4394904458599	0.785797616045541 \\
84.0764331210191	0.773354304417219 \\
84.7133757961783	0.755924524638692 \\
85.3503184713376	0.747493087391772 \\
85.9872611464968	0.731259767715378 \\
86.6242038216561	0.716875819361373 \\
87.2611464968153	0.687474156982826 \\
87.8980891719745	0.669209903899209 \\
88.5350318471338	0.654326970232914 \\
89.171974522293	0.624451483624325 \\
89.8089171974522	0.591626756299606 \\
90.4458598726115	0.541414548027634 \\
91.0828025477707	0.513947991903882 \\
91.7197452229299	0.459365951042809 \\
92.3566878980892	0.425335417305231 \\
92.9936305732484	0.387144253920967 \\
93.6305732484076	0.344922417492345 \\
94.2675159235669	0.305194139519303 \\
94.9044585987261	0.259138692801098 \\
95.5414012738853	0.209719184438875 \\
96.1783439490446	0.150443376418368 \\
96.8152866242038	0.0982789489929235 \\
97.4522292993631	0.0522033661719461 \\
98.0891719745223	0.0348123389811678 \\
98.7261146496815	0.0118751109714807 \\
99.3630573248408	0.00442778939317399 \\
100	9.07070329958515e-11 \\
};
\path [fill=color8, fill opacity=0.5] (axis cs:0,0.916035021049183)
--(axis cs:0,0.91480337682252)
--(axis cs:0.636942675159236,0.914574939061817)
--(axis cs:1.27388535031847,0.91395030150023)
--(axis cs:1.91082802547771,0.912903795069358)
--(axis cs:2.54777070063694,0.911919455509997)
--(axis cs:3.18471337579618,0.911203119681637)
--(axis cs:3.82165605095541,0.910073557409134)
--(axis cs:4.45859872611465,0.908749555579711)
--(axis cs:5.09554140127389,0.906191651784703)
--(axis cs:5.73248407643312,0.904951991410723)
--(axis cs:6.36942675159236,0.90390358402279)
--(axis cs:7.00636942675159,0.90280353958022)
--(axis cs:7.64331210191083,0.899909708877216)
--(axis cs:8.28025477707006,0.900102079769843)
--(axis cs:8.9171974522293,0.898066210007033)
--(axis cs:9.55414012738853,0.896301581340794)
--(axis cs:10.1910828025478,0.892937296836845)
--(axis cs:10.828025477707,0.889789304189118)
--(axis cs:11.4649681528662,0.887468732342508)
--(axis cs:12.1019108280255,0.884588686055474)
--(axis cs:12.7388535031847,0.88256537102568)
--(axis cs:13.3757961783439,0.883284545312952)
--(axis cs:14.0127388535032,0.881121009021941)
--(axis cs:14.6496815286624,0.880448658305063)
--(axis cs:15.2866242038217,0.881727422042192)
--(axis cs:15.9235668789809,0.881838302282583)
--(axis cs:16.5605095541401,0.882367411179965)
--(axis cs:17.1974522292994,0.881712213587257)
--(axis cs:17.8343949044586,0.882065564488454)
--(axis cs:18.4713375796178,0.88195579621557)
--(axis cs:19.1082802547771,0.884306892738707)
--(axis cs:19.7452229299363,0.883312820990874)
--(axis cs:20.3821656050955,0.883718007213268)
--(axis cs:21.0191082802548,0.884877480950524)
--(axis cs:21.656050955414,0.885239294937204)
--(axis cs:22.2929936305732,0.886235524910475)
--(axis cs:22.9299363057325,0.887028324767726)
--(axis cs:23.5668789808917,0.887190339102167)
--(axis cs:24.203821656051,0.888571931893365)
--(axis cs:24.8407643312102,0.88967909085053)
--(axis cs:25.4777070063694,0.890180358857876)
--(axis cs:26.1146496815287,0.889892687080602)
--(axis cs:26.7515923566879,0.893244492125388)
--(axis cs:27.3885350318471,0.894352129479762)
--(axis cs:28.0254777070064,0.893515724225365)
--(axis cs:28.6624203821656,0.894416419636701)
--(axis cs:29.2993630573248,0.893513873404734)
--(axis cs:29.9363057324841,0.894240677268004)
--(axis cs:30.5732484076433,0.894559114130526)
--(axis cs:31.2101910828025,0.896173296920672)
--(axis cs:31.8471337579618,0.895151391978543)
--(axis cs:32.484076433121,0.897269997246324)
--(axis cs:33.1210191082803,0.897153830098623)
--(axis cs:33.7579617834395,0.896081354569313)
--(axis cs:34.3949044585987,0.89742844924345)
--(axis cs:35.031847133758,0.898281484630624)
--(axis cs:35.6687898089172,0.899289402506868)
--(axis cs:36.3057324840764,0.900654959925163)
--(axis cs:36.9426751592357,0.899486316973866)
--(axis cs:37.5796178343949,0.898774123122895)
--(axis cs:38.2165605095541,0.900840146647951)
--(axis cs:38.8535031847134,0.900643501831146)
--(axis cs:39.4904458598726,0.900780224077139)
--(axis cs:40.1273885350318,0.90171341390146)
--(axis cs:40.7643312101911,0.900520342135274)
--(axis cs:41.4012738853503,0.900144852669687)
--(axis cs:42.0382165605096,0.901205195669052)
--(axis cs:42.6751592356688,0.902207640115684)
--(axis cs:43.312101910828,0.903670981756824)
--(axis cs:43.9490445859873,0.902374155087329)
--(axis cs:44.5859872611465,0.90407348534721)
--(axis cs:45.2229299363057,0.903607161653091)
--(axis cs:45.859872611465,0.904892554802539)
--(axis cs:46.4968152866242,0.905493502619393)
--(axis cs:47.1337579617834,0.906810825930039)
--(axis cs:47.7707006369427,0.906704715644141)
--(axis cs:48.4076433121019,0.9063333203461)
--(axis cs:49.0445859872611,0.905609564703978)
--(axis cs:49.6815286624204,0.906292477072867)
--(axis cs:50.3184713375796,0.906954583021222)
--(axis cs:50.9554140127388,0.907845706187912)
--(axis cs:51.5923566878981,0.908700568231581)
--(axis cs:52.2292993630573,0.90853024288312)
--(axis cs:52.8662420382166,0.909783743704425)
--(axis cs:53.5031847133758,0.909850225094601)
--(axis cs:54.140127388535,0.91001263983582)
--(axis cs:54.7770700636943,0.909450345601798)
--(axis cs:55.4140127388535,0.910942200031589)
--(axis cs:56.0509554140127,0.910986605885415)
--(axis cs:56.687898089172,0.910926155334955)
--(axis cs:57.3248407643312,0.910038696226495)
--(axis cs:57.9617834394904,0.910534379371099)
--(axis cs:58.5987261146497,0.910408617211474)
--(axis cs:59.2356687898089,0.911414339924033)
--(axis cs:59.8726114649682,0.911542201745592)
--(axis cs:60.5095541401274,0.911744903614338)
--(axis cs:61.1464968152866,0.911706543328523)
--(axis cs:61.7834394904459,0.911381553121376)
--(axis cs:62.4203821656051,0.910465768849364)
--(axis cs:63.0573248407643,0.911128482133892)
--(axis cs:63.6942675159236,0.910496766209379)
--(axis cs:64.3312101910828,0.910592243365318)
--(axis cs:64.968152866242,0.910434829041076)
--(axis cs:65.6050955414013,0.909432635853812)
--(axis cs:66.2420382165605,0.908782079437249)
--(axis cs:66.8789808917197,0.90791103096568)
--(axis cs:67.515923566879,0.906400755364374)
--(axis cs:68.1528662420382,0.904982867603896)
--(axis cs:68.7898089171974,0.905176477708107)
--(axis cs:69.4267515923567,0.901992297582854)
--(axis cs:70.0636942675159,0.902090594597369)
--(axis cs:70.7006369426752,0.902739425920242)
--(axis cs:71.3375796178344,0.902687494916352)
--(axis cs:71.9745222929936,0.900689570663585)
--(axis cs:72.6114649681529,0.897646793446106)
--(axis cs:73.2484076433121,0.897728223389552)
--(axis cs:73.8853503184713,0.896280159778497)
--(axis cs:74.5222929936306,0.893438559295604)
--(axis cs:75.1592356687898,0.89306218816699)
--(axis cs:75.796178343949,0.889216004304009)
--(axis cs:76.4331210191083,0.883604026438727)
--(axis cs:77.0700636942675,0.881172432417026)
--(axis cs:77.7070063694268,0.876257839517636)
--(axis cs:78.343949044586,0.873580400738687)
--(axis cs:78.9808917197452,0.869219983281995)
--(axis cs:79.6178343949044,0.854834031574241)
--(axis cs:80.2547770700637,0.846791307193924)
--(axis cs:80.8917197452229,0.833421938585553)
--(axis cs:81.5286624203822,0.822419851553171)
--(axis cs:82.1656050955414,0.809758572830361)
--(axis cs:82.8025477707006,0.792173345774678)
--(axis cs:83.4394904458599,0.780576580873091)
--(axis cs:84.0764331210191,0.768058903176737)
--(axis cs:84.7133757961783,0.750790271465086)
--(axis cs:85.3503184713376,0.741899424068624)
--(axis cs:85.9872611464968,0.72565667589609)
--(axis cs:86.6242038216561,0.711127639090135)
--(axis cs:87.2611464968153,0.68167173439194)
--(axis cs:87.8980891719745,0.663393242506111)
--(axis cs:88.5350318471338,0.648628582602646)
--(axis cs:89.171974522293,0.618565022765106)
--(axis cs:89.8089171974522,0.585472064757276)
--(axis cs:90.4458598726115,0.535060224425131)
--(axis cs:91.0828025477707,0.507234169828717)
--(axis cs:91.7197452229299,0.45258077897034)
--(axis cs:92.3566878980892,0.418709887154656)
--(axis cs:92.9936305732484,0.380770377585173)
--(axis cs:93.6305732484076,0.338701464100422)
--(axis cs:94.2675159235669,0.29896197970338)
--(axis cs:94.9044585987261,0.253229706954491)
--(axis cs:95.5414012738853,0.203950142330025)
--(axis cs:96.1783439490446,0.145192854675391)
--(axis cs:96.8152866242038,0.093394162830153)
--(axis cs:97.4522292993631,0.0486655032294177)
--(axis cs:98.0891719745223,0.0321481551639622)
--(axis cs:98.7261146496815,0.0103061608552969)
--(axis cs:99.3630573248408,0.00345230154114247)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,0.00540327724520551)
--(axis cs:98.7261146496815,0.0134440610876645)
--(axis cs:98.0891719745223,0.0374765227983734)
--(axis cs:97.4522292993631,0.0557412291144744)
--(axis cs:96.8152866242038,0.103163735155694)
--(axis cs:96.1783439490446,0.155693898161346)
--(axis cs:95.5414012738853,0.215488226547725)
--(axis cs:94.9044585987261,0.265047678647705)
--(axis cs:94.2675159235669,0.311426299335225)
--(axis cs:93.6305732484076,0.351143370884268)
--(axis cs:92.9936305732484,0.39351813025676)
--(axis cs:92.3566878980892,0.431960947455805)
--(axis cs:91.7197452229299,0.466151123115279)
--(axis cs:91.0828025477707,0.520661813979047)
--(axis cs:90.4458598726115,0.547768871630137)
--(axis cs:89.8089171974522,0.597781447841937)
--(axis cs:89.171974522293,0.630337944483545)
--(axis cs:88.5350318471338,0.660025357863183)
--(axis cs:87.8980891719745,0.675026565292307)
--(axis cs:87.2611464968153,0.693276579573711)
--(axis cs:86.6242038216561,0.722623999632612)
--(axis cs:85.9872611464968,0.736862859534666)
--(axis cs:85.3503184713376,0.75308675071492)
--(axis cs:84.7133757961783,0.761058777812298)
--(axis cs:84.0764331210191,0.778649705657701)
--(axis cs:83.4394904458599,0.79101865121799)
--(axis cs:82.8025477707006,0.802822189260408)
--(axis cs:82.1656050955414,0.820517683232528)
--(axis cs:81.5286624203822,0.833070003072168)
--(axis cs:80.8917197452229,0.84322815953812)
--(axis cs:80.2547770700637,0.855972636909785)
--(axis cs:79.6178343949044,0.864085660878057)
--(axis cs:78.9808917197452,0.877382462416034)
--(axis cs:78.343949044586,0.881188017189773)
--(axis cs:77.7070063694268,0.883612564589369)
--(axis cs:77.0700636942675,0.88797736493091)
--(axis cs:76.4331210191083,0.890168028702025)
--(axis cs:75.796178343949,0.895043839229937)
--(axis cs:75.1592356687898,0.898186865289168)
--(axis cs:74.5222929936306,0.898736264971636)
--(axis cs:73.8853503184713,0.901039508566075)
--(axis cs:73.2484076433121,0.902286873880345)
--(axis cs:72.6114649681529,0.902297350599606)
--(axis cs:71.9745222929936,0.904817157222983)
--(axis cs:71.3375796178344,0.906542419179734)
--(axis cs:70.7006369426752,0.906642198382344)
--(axis cs:70.0636942675159,0.906025923300064)
--(axis cs:69.4267515923567,0.905894978196977)
--(axis cs:68.7898089171974,0.9085657380011)
--(axis cs:68.1528662420382,0.908421727072826)
--(axis cs:67.515923566879,0.90953774731741)
--(axis cs:66.8789808917197,0.910627523942329)
--(axis cs:66.2420382165605,0.911380808295919)
--(axis cs:65.6050955414013,0.91185207834467)
--(axis cs:64.968152866242,0.912663643299131)
--(axis cs:64.3312101910828,0.912904252846129)
--(axis cs:63.6942675159236,0.912624528635662)
--(axis cs:63.0573248407643,0.913162343299526)
--(axis cs:62.4203821656051,0.912642208724673)
--(axis cs:61.7834394904459,0.913448795340025)
--(axis cs:61.1464968152866,0.913652731085118)
--(axis cs:60.5095541401274,0.913717421616718)
--(axis cs:59.8726114649682,0.913712155319686)
--(axis cs:59.2356687898089,0.91357345580085)
--(axis cs:58.5987261146497,0.912795360700725)
--(axis cs:57.9617834394904,0.912891571437934)
--(axis cs:57.3248407643312,0.912577113027854)
--(axis cs:56.687898089172,0.91316756967929)
--(axis cs:56.0509554140127,0.91319963524656)
--(axis cs:55.4140127388535,0.913007274880781)
--(axis cs:54.7770700636943,0.912048509787856)
--(axis cs:54.140127388535,0.912309190362814)
--(axis cs:53.5031847133758,0.912206511488289)
--(axis cs:52.8662420382166,0.91212050402934)
--(axis cs:52.2292993630573,0.911295019779369)
--(axis cs:51.5923566878981,0.911486890284285)
--(axis cs:50.9554140127388,0.910865192274538)
--(axis cs:50.3184713375796,0.910191502953305)
--(axis cs:49.6815286624204,0.909704813243578)
--(axis cs:49.0445859872611,0.909257312831846)
--(axis cs:48.4076433121019,0.909604791907689)
--(axis cs:47.7707006369427,0.909894564108559)
--(axis cs:47.1337579617834,0.910013103238856)
--(axis cs:46.4968152866242,0.908983732635206)
--(axis cs:45.859872611465,0.908614287327907)
--(axis cs:45.2229299363057,0.907493182955913)
--(axis cs:44.5859872611465,0.907825935249682)
--(axis cs:43.9490445859873,0.906461101466101)
--(axis cs:43.312101910828,0.907431603396016)
--(axis cs:42.6751592356688,0.906263273953065)
--(axis cs:42.0382165605096,0.905571907077367)
--(axis cs:41.4012738853503,0.904724658111449)
--(axis cs:40.7643312101911,0.905003502725452)
--(axis cs:40.1273885350318,0.905992657167364)
--(axis cs:39.4904458598726,0.905169237531986)
--(axis cs:38.8535031847134,0.905015590310286)
--(axis cs:38.2165605095541,0.905161634394481)
--(axis cs:37.5796178343949,0.9033849556735)
--(axis cs:36.9426751592357,0.903924306928589)
--(axis cs:36.3057324840764,0.904933932679993)
--(axis cs:35.6687898089172,0.90380939601772)
--(axis cs:35.031847133758,0.903040275289478)
--(axis cs:34.3949044585987,0.902324013367618)
--(axis cs:33.7579617834395,0.901095017955969)
--(axis cs:33.1210191082803,0.90203158053343)
--(axis cs:32.484076433121,0.902028144893709)
--(axis cs:31.8471337579618,0.90026258001064)
--(axis cs:31.2101910828025,0.901259655218389)
--(axis cs:30.5732484076433,0.899758901002505)
--(axis cs:29.9363057324841,0.89963849212067)
--(axis cs:29.2993630573248,0.898959260192789)
--(axis cs:28.6624203821656,0.899641843423004)
--(axis cs:28.0254777070064,0.898907713084552)
--(axis cs:27.3885350318471,0.899692455741219)
--(axis cs:26.7515923566879,0.898759422583815)
--(axis cs:26.1146496815287,0.895915066418065)
--(axis cs:25.4777070063694,0.89612000277589)
--(axis cs:24.8407643312102,0.895562076669178)
--(axis cs:24.203821656051,0.894691207752204)
--(axis cs:23.5668789808917,0.893360931087295)
--(axis cs:22.9299363057325,0.893232895479759)
--(axis cs:22.2929936305732,0.892596227991422)
--(axis cs:21.656050955414,0.891582036705364)
--(axis cs:21.0191082802548,0.891178500997051)
--(axis cs:20.3821656050955,0.890424962004815)
--(axis cs:19.7452229299363,0.890191796670364)
--(axis cs:19.1082802547771,0.890988964014657)
--(axis cs:18.4713375796178,0.888901635374988)
--(axis cs:17.8343949044586,0.888946609095277)
--(axis cs:17.1974522292994,0.888724619736654)
--(axis cs:16.5605095541401,0.889516818878675)
--(axis cs:15.9235668789809,0.888966463803347)
--(axis cs:15.2866242038217,0.88895350895645)
--(axis cs:14.6496815286624,0.887725429854513)
--(axis cs:14.0127388535032,0.888290031212904)
--(axis cs:13.3757961783439,0.890340444896985)
--(axis cs:12.7388535031847,0.889708479527058)
--(axis cs:12.1019108280255,0.89166938432961)
--(axis cs:11.4649681528662,0.893936274947215)
--(axis cs:10.828025477707,0.89611141183347)
--(axis cs:10.1910828025478,0.898741427179684)
--(axis cs:9.55414012738853,0.901495050123941)
--(axis cs:8.9171974522293,0.90292125733968)
--(axis cs:8.28025477707006,0.904611153371385)
--(axis cs:7.64331210191083,0.904464801745368)
--(axis cs:7.00636942675159,0.906806973998881)
--(axis cs:6.36942675159236,0.907633959894284)
--(axis cs:5.73248407643312,0.908480979940126)
--(axis cs:5.09554140127389,0.909656101735654)
--(axis cs:4.45859872611465,0.911726675655369)
--(axis cs:3.82165605095541,0.912518048976406)
--(axis cs:3.18471337579618,0.913311792387207)
--(axis cs:2.54777070063694,0.914107333994107)
--(axis cs:1.91082802547771,0.914835220738971)
--(axis cs:1.27388535031847,0.915465346078196)
--(axis cs:0.636942675159236,0.915971476181481)
--(axis cs:0,0.916035021049183)
--cycle;


==> img/mnist/mnist_rate_distortion_lafw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.915302741399501
0.636942675159236 0.915310381227173
1.27388535031847 0.914995475520263
1.91082802547771 0.914258227829123
2.54777070063694 0.913335402513621
3.18471337579618 0.911730133137316
3.82165605095541 0.909628701402689
4.45859872611465 0.907139022229239
5.09554140127389 0.904539750129916
5.73248407643312 0.900216026304406
6.36942675159236 0.8946224541025
7.00636942675159 0.887183553889045
7.64331210191083 0.877420054306276
8.28025477707006 0.869200505382614
8.9171974522293 0.860210375931347
9.55414012738853 0.850443429017905
10.1910828025478 0.838509337615687
10.828025477707 0.825811864908901
11.4649681528662 0.811172446832061
12.1019108280255 0.793401100249612
12.7388535031847 0.778065805467777
13.3757961783439 0.758398485861253
14.0127388535032 0.742287728892406
14.6496815286624 0.721579402065836
15.2866242038217 0.699515025246656
15.9235668789809 0.681761345964624
16.5605095541401 0.66438508697116
17.1974522292994 0.643207714605378
17.8343949044586 0.624761111205808
18.4713375796178 0.61159595217483
19.1082802547771 0.592358635399578
19.7452229299363 0.582191944230872
20.3821656050955 0.569173915994616
21.0191082802548 0.553682630308613
21.656050955414 0.531897564794781
22.2929936305732 0.518357955223764
22.9299363057325 0.50181159708678
23.5668789808917 0.482705343805719
24.203821656051 0.468997071874328
24.8407643312102 0.452915339103201
25.4777070063694 0.441655073029542
26.1146496815287 0.423738010914385
26.7515923566879 0.40788089203088
27.3885350318471 0.385594900823662
28.0254777070064 0.374407381942447
28.6624203821656 0.356342855551484
29.2993630573248 0.339385882341394
29.9363057324841 0.331995763311215
30.5732484076433 0.313401800964784
31.2101910828025 0.29595127738964
31.8471337579618 0.283791048553489
32.484076433121 0.272603282312089
33.1210191082803 0.260073655153915
33.7579617834395 0.247192350117032
34.3949044585987 0.233422921467813
35.031847133758 0.220363394010757
35.6687898089172 0.209216370017131
36.3057324840764 0.198769008579866
36.9426751592357 0.190744367688978
37.5796178343949 0.182358986148493
38.2165605095541 0.177926822417077
38.8535031847134 0.165064063901258
39.4904458598726 0.162715722917317
40.1273885350318 0.157159427321186
40.7643312101911 0.148318698766522
41.4012738853503 0.14377721714278
42.0382165605096 0.138602829720825
42.6751592356688 0.133676830207639
43.312101910828 0.12667156189534
43.9490445859873 0.122104177542646
44.5859872611465 0.120553235119989
45.2229299363057 0.119954586250583
45.859872611465 0.117626565895933
46.4968152866242 0.115699243743366
47.1337579617834 0.116081722887254
47.7707006369427 0.112906380531494
48.4076433121019 0.110358066712064
49.0445859872611 0.107790123184133
49.6815286624204 0.103160788386379
50.3184713375796 0.0991367106468021
50.9554140127388 0.0959452537299339
51.5923566878981 0.0957293207844392
52.2292993630573 0.097014575309205
52.8662420382166 0.0966155208621959
53.5031847133758 0.0979744350413884
54.140127388535 0.0942241692885781
54.7770700636943 0.0897808705648023
55.4140127388535 0.0835646400736423
56.0509554140127 0.0828402382015469
56.687898089172 0.0817461795336676
57.3248407643312 0.0822025608632317
57.9617834394904 0.0793418342936406
58.5987261146497 0.0799678236256697
59.2356687898089 0.0816462846019783
59.8726114649682 0.083007300105043
60.5095541401274 0.0817354792227205
61.1464968152866 0.0818866505536019
61.7834394904459 0.0797171378625866
62.4203821656051 0.0749345766312416
63.0573248407643 0.0693686946747946
63.6942675159236 0.0662519545634936
64.3312101910828 0.0610579397772757
64.968152866242 0.0559457059931559
65.6050955414013 0.0534416099933649
66.2420382165605 0.0555164841134013
66.8789808917197 0.0529463443787822
67.515923566879 0.0505866949939173
68.1528662420382 0.0483817963352471
68.7898089171974 0.0526165446311596
69.4267515923567 0.0506457016980531
70.0636942675159 0.0494883336267139
70.7006369426752 0.0506627223169256
71.3375796178344 0.0480068205414964
71.9745222929936 0.0428354761954838
72.6114649681529 0.0373162093825658
73.2484076433121 0.0366318995352602
73.8853503184713 0.0369652617344142
74.5222929936306 0.0332911085352468
75.1592356687898 0.0316373170472444
75.796178343949 0.0311411593177179
76.4331210191083 0.0319514091085846
77.0700636942675 0.034351564828615
77.7070063694268 0.0341304306528616
78.343949044586 0.0357902779975713
78.9808917197452 0.0361412918217949
79.6178343949044 0.0337605352886618
80.2547770700637 0.0318682243650659
80.8917197452229 0.0313662603499055
81.5286624203822 0.0305514961143423
82.1656050955414 0.0324295435369711
82.8025477707006 0.0313910534468525
83.4394904458599 0.0310492427146001
84.0764331210191 0.0282324574176481
84.7133757961783 0.0261509192411468
85.3503184713376 0.0223051150410708
85.9872611464968 0.0209885128143702
86.6242038216561 0.018819360090162
87.2611464968153 0.0173918088780029
87.8980891719745 0.0158096772692081
88.5350318471338 0.0156581499106905
89.171974522293 0.0142140759399337
89.8089171974522 0.0122568617550397
90.4458598726115 0.0125247387740789
91.0828025477707 0.0117740748946687
91.7197452229299 0.00987929971591328
92.3566878980892 0.00736544472487259
92.9936305732484 0.00575279453132417
93.6305732484076 0.00194593112268304
94.2675159235669 0.000791362244527064
94.9044585987261 0.000873640433644277
95.5414012738853 0.000935613577971987
96.1783439490446 0.000932528695697515
96.8152866242038 0.000248773859986531
97.4522292993631 0.000108560647314523
98.0891719745223 0.000151885143732265
98.7261146496815 0.000203457838766827
99.3630573248408 4.9181428615539e-05
100 0
};
\path [fill=color1, fill opacity=0.25] 
(axis cs:0,0.915988724500261)
--(axis cs:0,0.91461675829874)
--(axis cs:0.636942675159236,0.914662123156497)
--(axis cs:1.27388535031847,0.914332537947731)
--(axis cs:1.91082802547771,0.913391112500781)
--(axis cs:2.54777070063694,0.912308551862419)
--(axis cs:3.18471337579618,0.910442078038938)
--(axis cs:3.82165605095541,0.908068698529155)
--(axis cs:4.45859872611465,0.905246015434783)
--(axis cs:5.09554140127389,0.902325283029826)
--(axis cs:5.73248407643312,0.897609653074322)
--(axis cs:6.36942675159236,0.891484765643754)
--(axis cs:7.00636942675159,0.883457181769895)
--(axis cs:7.64331210191083,0.873066639873815)
--(axis cs:8.28025477707006,0.864374107947791)
--(axis cs:8.9171974522293,0.855090935852519)
--(axis cs:9.55414012738853,0.844923275352592)
--(axis cs:10.1910828025478,0.832547356777541)
--(axis cs:10.828025477707,0.819389609367937)
--(axis cs:11.4649681528662,0.804459404216889)
--(axis cs:12.1019108280255,0.786320272347928)
--(axis cs:12.7388535031847,0.770723056731778)
--(axis cs:13.3757961783439,0.750925541595417)
--(axis cs:14.0127388535032,0.734644986782093)
--(axis cs:14.6496815286624,0.713781494735699)
--(axis cs:15.2866242038217,0.69137674891423)
--(axis cs:15.9235668789809,0.673507670558028)
--(axis cs:16.5605095541401,0.656134270257697)
--(axis cs:17.1974522292994,0.635018657701201)
--(axis cs:17.8343949044586,0.616712126715357)
--(axis cs:18.4713375796178,0.603648605925796)
--(axis cs:19.1082802547771,0.584168749489813)
--(axis cs:19.7452229299363,0.574121177750051)
--(axis cs:20.3821656050955,0.561055978160986)
--(axis cs:21.0191082802548,0.545484927257676)
--(axis cs:21.656050955414,0.523688497156279)
--(axis cs:22.2929936305732,0.51013448696047)
--(axis cs:22.9299363057325,0.493641400129089)
--(axis cs:23.5668789808917,0.47470647419877)
--(axis cs:24.203821656051,0.461158174126288)
--(axis cs:24.8407643312102,0.445272154369194)
--(axis cs:25.4777070063694,0.433944808707531)
--(axis cs:26.1146496815287,0.416178421506206)
--(axis cs:26.7515923566879,0.400272956921598)
--(axis cs:27.3885350318471,0.378080779156998)
--(axis cs:28.0254777070064,0.367001828963791)
--(axis cs:28.6624203821656,0.348934628139077)
--(axis cs:29.2993630573248,0.331897558007356)
--(axis cs:29.9363057324841,0.324541965679398)
--(axis cs:30.5732484076433,0.305898369705881)
--(axis cs:31.2101910828025,0.288452585148819)
--(axis cs:31.8471337579618,0.276361972940715)
--(axis cs:32.484076433121,0.265150385958328)
--(axis cs:33.1210191082803,0.252705119210878)
--(axis cs:33.7579617834395,0.240074565267971)
--(axis cs:34.3949044585987,0.226355574588511)
--(axis cs:35.031847133758,0.213663983154795)
--(axis cs:35.6687898089172,0.202785540653121)
--(axis cs:36.3057324840764,0.192388344687232)
--(axis cs:36.9426751592357,0.184479240466039)
--(axis cs:37.5796178343949,0.175968993078181)
--(axis cs:38.2165605095541,0.171749618982099)
--(axis cs:38.8535031847134,0.159133375693263)
--(axis cs:39.4904458598726,0.15692232997653)
--(axis cs:40.1273885350318,0.151380101924353)
--(axis cs:40.7643312101911,0.14274824261678)
--(axis cs:41.4012738853503,0.138314264040479)
--(axis cs:42.0382165605096,0.133139411827506)
--(axis cs:42.6751592356688,0.128332268559484)
--(axis cs:43.312101910828,0.121601321271596)
--(axis cs:43.9490445859873,0.117217738116292)
--(axis cs:44.5859872611465,0.115636897197068)
--(axis cs:45.2229299363057,0.115035567337564)
--(axis cs:45.859872611465,0.11266499895395)
--(axis cs:46.4968152866242,0.110988698398848)
--(axis cs:47.1337579617834,0.11148843516432)
--(axis cs:47.7707006369427,0.108304082616999)
--(axis cs:48.4076433121019,0.105801675231864)
--(axis cs:49.0445859872611,0.103255834034407)
--(axis cs:49.6815286624204,0.0986216274918797)
--(axis cs:50.3184713375796,0.0945843711952757)
--(axis cs:50.9554140127388,0.0915077190454938)
--(axis cs:51.5923566878981,0.0914109906709877)
--(axis cs:52.2292993630573,0.0925867217608802)
--(axis cs:52.8662420382166,0.0923803445226764)
--(axis cs:53.5031847133758,0.0938039444266989)
--(axis cs:54.140127388535,0.0898337106743475)
--(axis cs:54.7770700636943,0.0854494505521853)
--(axis cs:55.4140127388535,0.0792180746646014)
--(axis cs:56.0509554140127,0.0784562295564508)
--(axis cs:56.687898089172,0.0773919865715051)
--(axis cs:57.3248407643312,0.0776963106481681)
--(axis cs:57.9617834394904,0.0749182402856661)
--(axis cs:58.5987261146497,0.0756692648130969)
--(axis cs:59.2356687898089,0.0774577612798574)
--(axis cs:59.8726114649682,0.0788502404166265)
--(axis cs:60.5095541401274,0.0775942690105902)
--(axis cs:61.1464968152866,0.0778019164904957)
--(axis cs:61.7834394904459,0.0756975371924186)
--(axis cs:62.4203821656051,0.0710311643066155)
--(axis cs:63.0573248407643,0.0654133594800515)
--(axis cs:63.6942675159236,0.0625440827174777)
--(axis cs:64.3312101910828,0.0574020108045484)
--(axis cs:64.968152866242,0.0524073737704042)
--(axis cs:65.6050955414013,0.0499359488492624)
--(axis cs:66.2420382165605,0.0519781388753029)
--(axis cs:66.8789808917197,0.049469837781827)
--(axis cs:67.515923566879,0.047305108187971)
--(axis cs:68.1528662420382,0.0451635632969752)
--(axis cs:68.7898089171974,0.0493417718481599)
--(axis cs:69.4267515923567,0.0474610930366144)
--(axis cs:70.0636942675159,0.0463650223878635)
--(axis cs:70.7006369426752,0.0474040756771828)
--(axis cs:71.3375796178344,0.0448073317179078)
--(axis cs:71.9745222929936,0.0397920755860949)
--(axis cs:72.6114649681529,0.034523961141581)
--(axis cs:73.2484076433121,0.0339615898445374)
--(axis cs:73.8853503184713,0.0343159637369183)
--(axis cs:74.5222929936306,0.0308059977868581)
--(axis cs:75.1592356687898,0.0292616302700323)
--(axis cs:75.796178343949,0.0287916630664444)
--(axis cs:76.4331210191083,0.0296419448209389)
--(axis cs:77.0700636942675,0.0319319722175052)
--(axis cs:77.7070063694268,0.0318224533527457)
--(axis cs:78.343949044586,0.0335131889941737)
--(axis cs:78.9808917197452,0.0338675534219228)
--(axis cs:79.6178343949044,0.0314673882436643)
--(axis cs:80.2547770700637,0.0298397778550158)
--(axis cs:80.8917197452229,0.0294791868556576)
--(axis cs:81.5286624203822,0.0286358056230229)
--(axis cs:82.1656050955414,0.0304655354965049)
--(axis cs:82.8025477707006,0.0292366155300894)
--(axis cs:83.4394904458599,0.0291147301423673)
--(axis cs:84.0764331210191,0.0263109966668074)
--(axis cs:84.7133757961783,0.0242026885414352)
--(axis cs:85.3503184713376,0.0205682425572015)
--(axis cs:85.9872611464968,0.0192028930410081)
--(axis cs:86.6242038216561,0.0169658439877609)
--(axis cs:87.2611464968153,0.0155637805531377)
--(axis cs:87.8980891719745,0.0143448645515081)
--(axis cs:88.5350318471338,0.0144609553050409)
--(axis cs:89.171974522293,0.012910462950663)
--(axis cs:89.8089171974522,0.0109444996002341)
--(axis cs:90.4458598726115,0.0113065980163803)
--(axis cs:91.0828025477707,0.0105573252577524)
--(axis cs:91.7197452229299,0.00860441400253528)
--(axis cs:92.3566878980892,0.00618313116156204)
--(axis cs:92.9936305732484,0.00468431724700028)
--(axis cs:93.6305732484076,0.00134638909434175)
--(axis cs:94.2675159235669,0.000493944652924347)
--(axis cs:94.9044585987261,0.000505838605416755)
--(axis cs:95.5414012738853,0.000613635818516275)
--(axis cs:96.1783439490446,0.000549391231892527)
--(axis cs:96.8152866242038,0.00014078532281045)
--(axis cs:97.4522292993631,5.70484474716856e-05)
--(axis cs:98.0891719745223,8.92621026376843e-05)
--(axis cs:98.7261146496815,0.000127204617753413)
--(axis cs:99.3630573248408,3.31312565209583e-05)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,6.52316007101197e-05)
--(axis cs:98.7261146496815,0.000279711059780241)
--(axis cs:98.0891719745223,0.000214508184826847)
--(axis cs:97.4522292993631,0.00016007284715736)
--(axis cs:96.8152866242038,0.000356762397162611)
--(axis cs:96.1783439490446,0.0013156661595025)
--(axis cs:95.5414012738853,0.0012575913374277)
--(axis cs:94.9044585987261,0.0012414422618718)
--(axis cs:94.2675159235669,0.00108877983612978)
--(axis cs:93.6305732484076,0.00254547315102433)
--(axis cs:92.9936305732484,0.00682127181564806)
--(axis cs:92.3566878980892,0.00854775828818315)
--(axis cs:91.7197452229299,0.0111541854292913)
--(axis cs:91.0828025477707,0.0129908245315851)
--(axis cs:90.4458598726115,0.0137428795317776)
--(axis cs:89.8089171974522,0.0135692239098453)
--(axis cs:89.171974522293,0.0155176889292043)
--(axis cs:88.5350318471338,0.0168553445163401)
--(axis cs:87.8980891719745,0.0172744899869081)
--(axis cs:87.2611464968153,0.0192198372028681)
--(axis cs:86.6242038216561,0.0206728761925631)
--(axis cs:85.9872611464968,0.0227741325877324)
--(axis cs:85.3503184713376,0.02404198752494)
--(axis cs:84.7133757961783,0.0280991499408583)
--(axis cs:84.0764331210191,0.0301539181684887)
--(axis cs:83.4394904458599,0.0329837552868329)
--(axis cs:82.8025477707006,0.0335454913636156)
--(axis cs:82.1656050955414,0.0343935515774373)
--(axis cs:81.5286624203822,0.0324671866056617)
--(axis cs:80.8917197452229,0.0332533338441534)
--(axis cs:80.2547770700637,0.0338966708751161)
--(axis cs:79.6178343949044,0.0360536823336593)
--(axis cs:78.9808917197452,0.038415030221667)
--(axis cs:78.343949044586,0.0380673670009689)
--(axis cs:77.7070063694268,0.0364384079529775)
--(axis cs:77.0700636942675,0.0367711574397249)
--(axis cs:76.4331210191083,0.0342608733962302)
--(axis cs:75.796178343949,0.0334906555689915)
--(axis cs:75.1592356687898,0.0340130038244565)
--(axis cs:74.5222929936306,0.0357762192836355)
--(axis cs:73.8853503184713,0.03961455973191)
--(axis cs:73.2484076433121,0.0393022092259831)
--(axis cs:72.6114649681529,0.0401084576235506)
--(axis cs:71.9745222929936,0.0458788768048727)
--(axis cs:71.3375796178344,0.0512063093650851)
--(axis cs:70.7006369426752,0.0539213689566685)
--(axis cs:70.0636942675159,0.0526116448655644)
--(axis cs:69.4267515923567,0.0538303103594918)
--(axis cs:68.7898089171974,0.0558913174141593)
--(axis cs:68.1528662420382,0.0516000293735189)
--(axis cs:67.515923566879,0.0538682817998636)
--(axis cs:66.8789808917197,0.0564228509757373)
--(axis cs:66.2420382165605,0.0590548293514997)
--(axis cs:65.6050955414013,0.0569472711374675)
--(axis cs:64.968152866242,0.0594840382159077)
--(axis cs:64.3312101910828,0.0647138687500029)
--(axis cs:63.6942675159236,0.0699598264095096)
--(axis cs:63.0573248407643,0.0733240298695376)
--(axis cs:62.4203821656051,0.0788379889558677)
--(axis cs:61.7834394904459,0.0837367385327546)
--(axis cs:61.1464968152866,0.0859713846167081)
--(axis cs:60.5095541401274,0.0858766894348508)
--(axis cs:59.8726114649682,0.0871643597934594)
--(axis cs:59.2356687898089,0.0858348079240992)
--(axis cs:58.5987261146497,0.0842663824382425)
--(axis cs:57.9617834394904,0.0837654283016151)
--(axis cs:57.3248407643312,0.0867088110782953)
--(axis cs:56.687898089172,0.0861003724958301)
--(axis cs:56.0509554140127,0.0872242468466431)
--(axis cs:55.4140127388535,0.0879112054826832)
--(axis cs:54.7770700636943,0.0941122905774194)
--(axis cs:54.140127388535,0.0986146279028088)
--(axis cs:53.5031847133758,0.102144925656078)
--(axis cs:52.8662420382166,0.100850697201715)
--(axis cs:52.2292993630573,0.10144242885753)
--(axis cs:51.5923566878981,0.100047650897891)
--(axis cs:50.9554140127388,0.100382788414374)
--(axis cs:50.3184713375796,0.103689050098329)
--(axis cs:49.6815286624204,0.107699949280879)
--(axis cs:49.0445859872611,0.112324412333858)
--(axis cs:48.4076433121019,0.114914458192263)
--(axis cs:47.7707006369427,0.117508678445989)
--(axis cs:47.1337579617834,0.120675010610188)
--(axis cs:46.4968152866242,0.120409789087884)
--(axis cs:45.859872611465,0.122588132837916)
--(axis cs:45.2229299363057,0.124873605163602)
--(axis cs:44.5859872611465,0.125469573042911)
--(axis cs:43.9490445859873,0.126990616969)
--(axis cs:43.312101910828,0.131741802519084)
--(axis cs:42.6751592356688,0.139021391855794)
--(axis cs:42.0382165605096,0.144066247614145)
--(axis cs:41.4012738853503,0.149240170245082)
--(axis cs:40.7643312101911,0.153889154916264)
--(axis cs:40.1273885350318,0.162938752718019)
--(axis cs:39.4904458598726,0.168509115858103)
--(axis cs:38.8535031847134,0.170994752109253)
--(axis cs:38.2165605095541,0.184104025852055)
--(axis cs:37.5796178343949,0.188748979218806)
--(axis cs:36.9426751592357,0.197009494911917)
--(axis cs:36.3057324840764,0.2051496724725)
--(axis cs:35.6687898089172,0.215647199381141)
--(axis cs:35.031847133758,0.227062804866719)
--(axis cs:34.3949044585987,0.240490268347116)
--(axis cs:33.7579617834395,0.254310134966093)
--(axis cs:33.1210191082803,0.267442191096952)
--(axis cs:32.484076433121,0.280056178665849)
--(axis cs:31.8471337579618,0.291220124166264)
--(axis cs:31.2101910828025,0.303449969630462)
--(axis cs:30.5732484076433,0.320905232223688)
--(axis cs:29.9363057324841,0.339449560943033)
--(axis cs:29.2993630573248,0.346874206675431)
--(axis cs:28.6624203821656,0.363751082963891)
--(axis cs:28.0254777070064,0.381812934921102)
--(axis cs:27.3885350318471,0.393109022490326)
--(axis cs:26.7515923566879,0.415488827140163)
--(axis cs:26.1146496815287,0.431297600322564)
--(axis cs:25.4777070063694,0.449365337351553)
--(axis cs:24.8407643312102,0.460558523837209)
--(axis cs:24.203821656051,0.476835969622368)
--(axis cs:23.5668789808917,0.490704213412668)
--(axis cs:22.9299363057325,0.509981794044472)
--(axis cs:22.2929936305732,0.526581423487059)
--(axis cs:21.656050955414,0.540106632433283)
--(axis cs:21.0191082802548,0.56188033335955)
--(axis cs:20.3821656050955,0.577291853828245)
--(axis cs:19.7452229299363,0.590262710711692)
--(axis cs:19.1082802547771,0.600548521309343)
--(axis cs:18.4713375796178,0.619543298423864)
--(axis cs:17.8343949044586,0.632810095696258)
--(axis cs:17.1974522292994,0.651396771509555)
--(axis cs:16.5605095541401,0.672635903684624)
--(axis cs:15.9235668789809,0.690015021371219)
--(axis cs:15.2866242038217,0.707653301579081)
--(axis cs:14.6496815286624,0.729377309395973)
--(axis cs:14.0127388535032,0.74993047100272)
--(axis cs:13.3757961783439,0.765871430127089)
--(axis cs:12.7388535031847,0.785408554203776)
--(axis cs:12.1019108280255,0.800481928151295)
--(axis cs:11.4649681528662,0.817885489447233)
--(axis cs:10.828025477707,0.832234120449865)
--(axis cs:10.1910828025478,0.844471318453834)
--(axis cs:9.55414012738853,0.855963582683218)
--(axis cs:8.9171974522293,0.865329816010174)
--(axis cs:8.28025477707006,0.874026902817437)
--(axis cs:7.64331210191083,0.881773468738737)
--(axis cs:7.00636942675159,0.890909926008194)
--(axis cs:6.36942675159236,0.897760142561247)
--(axis cs:5.73248407643312,0.902822399534491)
--(axis cs:5.09554140127389,0.906754217230006)
--(axis cs:4.45859872611465,0.909032029023696)
--(axis cs:3.82165605095541,0.911188704276224)
--(axis cs:3.18471337579618,0.913018188235695)
--(axis cs:2.54777070063694,0.914362253164824)
--(axis cs:1.91082802547771,0.915125343157464)
--(axis cs:1.27388535031847,0.915658413092796)
--(axis cs:0.636942675159236,0.915958639297848)
--(axis cs:0,0.915988724500261)
--cycle;


==> img/mnist/mnist_rate_distortion_lafw_order.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.915496075343108
0.636942675159236 0.915037468562368
1.27388535031847 0.914695803779177
1.91082802547771 0.913854668618878
2.54777070063694 0.912720376315992
3.18471337579618 0.911093976920238
3.82165605095541 0.908041023375699
4.45859872611465 0.905114319911227
5.09554140127389 0.901263762355084
5.73248407643312 0.896527850108105
6.36942675159236 0.889631199261639
7.00636942675159 0.882391729962546
7.64331210191083 0.869597045718692
8.28025477707006 0.860009632126894
8.9171974522293 0.842441343010869
9.55414012738853 0.828024169146083
10.1910828025478 0.813655283471453
10.828025477707 0.795740368400002
11.4649681528662 0.775455452040769
12.1019108280255 0.757706733945524
12.7388535031847 0.732517512240447
13.3757961783439 0.719687391867628
14.0127388535032 0.702739428302739
14.6496815286624 0.687212164800148
15.2866242038217 0.671052298609866
15.9235668789809 0.653054282569792
16.5605095541401 0.640255403574556
17.1974522292994 0.618060587751679
17.8343949044586 0.604605953885475
18.4713375796178 0.592263609107467
19.1082802547771 0.580923880166374
19.7452229299363 0.563136266623624
20.3821656050955 0.547760979665909
21.0191082802548 0.533536295644008
21.656050955414 0.520032935291529
22.2929936305732 0.507294183338527
22.9299363057325 0.491322980314726
23.5668789808917 0.480439007607056
24.203821656051 0.470899598619435
24.8407643312102 0.462694695593673
25.4777070063694 0.460221017333679
26.1146496815287 0.44934022749716
26.7515923566879 0.443497225757455
27.3885350318471 0.433409128503408
28.0254777070064 0.424970799793955
28.6624203821656 0.415919746879372
29.2993630573248 0.409664006619423
29.9363057324841 0.402990970210521
30.5732484076433 0.395354746565135
31.2101910828025 0.389038009244978
31.8471337579618 0.380075527676818
32.484076433121 0.36869654975013
33.1210191082803 0.361441504619033
33.7579617834395 0.346380474432253
34.3949044585987 0.331695036074525
35.031847133758 0.327098474373861
35.6687898089172 0.317932535448058
36.3057324840764 0.306189422316743
36.9426751592357 0.298529391381577
37.5796178343949 0.296180473732709
38.2165605095541 0.289921496251251
38.8535031847134 0.284523594206465
39.4904458598726 0.279880362525425
40.1273885350318 0.279521992496142
40.7643312101911 0.276064411858717
41.4012738853503 0.271667758761719
42.0382165605096 0.2688733455755
42.6751592356688 0.267266162635602
43.312101910828 0.260850109793664
43.9490445859873 0.261510165953801
44.5859872611465 0.26278001210622
45.2229299363057 0.255567587741863
45.859872611465 0.251214071747841
46.4968152866242 0.24687430464602
47.1337579617834 0.245650828957047
47.7707006369427 0.242618764627337
48.4076433121019 0.235770416212001
49.0445859872611 0.234485508545643
49.6815286624204 0.230059618224745
50.3184713375796 0.226139095695358
50.9554140127388 0.22844622935428
51.5923566878981 0.222311627220438
52.2292993630573 0.213402743726499
52.8662420382166 0.21001865237166
53.5031847133758 0.198091223373954
54.140127388535 0.194763744855599
54.7770700636943 0.189628102672366
55.4140127388535 0.182766446653122
56.0509554140127 0.175827319302081
56.687898089172 0.171715376008186
57.3248407643312 0.162449113827597
57.9617834394904 0.16082253461624
58.5987261146497 0.160631243069329
59.2356687898089 0.155200397495821
59.8726114649682 0.149388460547696
60.5095541401274 0.148945511571442
61.1464968152866 0.14094542538895
61.7834394904459 0.138778391998097
62.4203821656051 0.13645550366379
63.0573248407643 0.131913253182765
63.6942675159236 0.12662047667461
64.3312101910828 0.120886488840175
64.968152866242 0.115991146484346
65.6050955414013 0.108586883327159
66.2420382165605 0.106150709809947
66.8789808917197 0.101014789890136
67.515923566879 0.0955228072658522
68.1528662420382 0.0904312012539144
68.7898089171974 0.0848162639897113
69.4267515923567 0.0725575467738428
70.0636942675159 0.0675111646931779
70.7006369426752 0.0600680325324135
71.3375796178344 0.0554429750294952
71.9745222929936 0.0521112053376045
72.6114649681529 0.0456623977015454
73.2484076433121 0.0422768441006025
73.8853503184713 0.0404502793468882
74.5222929936306 0.038205009993156
75.1592356687898 0.038789115667826
75.796178343949 0.0370411708721356
76.4331210191083 0.034779253533919
77.0700636942675 0.0348412054645624
77.7070063694268 0.032716248835934
78.343949044586 0.0328882541739669
78.9808917197452 0.0270990886943763
79.6178343949044 0.0240564372391646
80.2547770700637 0.0232153965547953
80.8917197452229 0.0220954501831108
81.5286624203822 0.0236297634242751
82.1656050955414 0.0237430354312724
82.8025477707006 0.0230408069709954
83.4394904458599 0.0245703740363691
84.0764331210191 0.0257726915479843
84.7133757961783 0.027942885032155
85.3503184713376 0.027645851939733
85.9872611464968 0.0241966290524211
86.6242038216561 0.0205407370236326
87.2611464968153 0.0186128306896097
87.8980891719745 0.0154202931427617
88.5350318471338 0.0158743181187842
89.171974522293 0.0137691727806784
89.8089171974522 0.014852178448603
90.4458598726115 0.0133645884033282
91.0828025477707 0.00955469234543793
91.7197452229299 0.0106488247660318
92.3566878980892 0.00986327043901602
92.9936305732484 0.00739640447259323
93.6305732484076 0.00951644037837666
94.2675159235669 0.00785147015031252
94.9044585987261 0.00704834791363366
95.5414012738853 0.0023607128202081
96.1783439490446 0.00056543915953985
96.8152866242038 5.45902348327204e-05
97.4522292993631 8.58937076695265e-06
98.0891719745223 6.38108385736913e-06
98.7261146496815 4.82847913395978e-06
99.3630573248408 2.88024224241845e-06
100 0
};

\path [fill=color1, fill opacity=0.25] 
(axis cs:0,0.916095289990536)
--(axis cs:0,0.91489686069568)
--(axis cs:0.636942675159236,0.914357912079354)
--(axis cs:1.27388535031847,0.913903746823856)
--(axis cs:1.91082802547771,0.913002244546182)
--(axis cs:2.54777070063694,0.911661558540937)
--(axis cs:3.18471337579618,0.909766234764611)
--(axis cs:3.82165605095541,0.906332094586662)
--(axis cs:4.45859872611465,0.902926668532582)
--(axis cs:5.09554140127389,0.898685065109246)
--(axis cs:5.73248407643312,0.893583390058454)
--(axis cs:6.36942675159236,0.886109505794764)
--(axis cs:7.00636942675159,0.878365224758546)
--(axis cs:7.64331210191083,0.86489559247674)
--(axis cs:8.28025477707006,0.854884977225947)
--(axis cs:8.9171974522293,0.836614426830189)
--(axis cs:9.55414012738853,0.821778255991708)
--(axis cs:10.1910828025478,0.807093929058894)
--(axis cs:10.828025477707,0.788871247458612)
--(axis cs:11.4649681528662,0.768371213402888)
--(axis cs:12.1019108280255,0.750500108355856)
--(axis cs:12.7388535031847,0.725261610833071)
--(axis cs:13.3757961783439,0.712308820703435)
--(axis cs:14.0127388535032,0.695093091870197)
--(axis cs:14.6496815286624,0.679213818694148)
--(axis cs:15.2866242038217,0.662928951059269)
--(axis cs:15.9235668789809,0.645066907245581)
--(axis cs:16.5605095541401,0.632160624797174)
--(axis cs:17.1974522292994,0.609938004517559)
--(axis cs:17.8343949044586,0.596356105826008)
--(axis cs:18.4713375796178,0.584057617738943)
--(axis cs:19.1082802547771,0.572739044532587)
--(axis cs:19.7452229299363,0.554908652599783)
--(axis cs:20.3821656050955,0.539654891656151)
--(axis cs:21.0191082802548,0.525455310417421)
--(axis cs:21.656050955414,0.512005791781843)
--(axis cs:22.2929936305732,0.499459382442021)
--(axis cs:22.9299363057325,0.483735955125358)
--(axis cs:23.5668789808917,0.47294911107934)
--(axis cs:24.203821656051,0.46357770578597)
--(axis cs:24.8407643312102,0.455483492736205)
--(axis cs:25.4777070063694,0.453193030876857)
--(axis cs:26.1146496815287,0.442239248149234)
--(axis cs:26.7515923566879,0.436486563966388)
--(axis cs:27.3885350318471,0.426419646294302)
--(axis cs:28.0254777070064,0.417827813765655)
--(axis cs:28.6624203821656,0.408898093435291)
--(axis cs:29.2993630573248,0.40266006409474)
--(axis cs:29.9363057324841,0.395847430701325)
--(axis cs:30.5732484076433,0.388199583639664)
--(axis cs:31.2101910828025,0.381685611501184)
--(axis cs:31.8471337579618,0.372959037615463)
--(axis cs:32.484076433121,0.361578438378227)
--(axis cs:33.1210191082803,0.354232581101764)
--(axis cs:33.7579617834395,0.339091215763885)
--(axis cs:34.3949044585987,0.324467737797324)
--(axis cs:35.031847133758,0.320029665343838)
--(axis cs:35.6687898089172,0.310967789714297)
--(axis cs:36.3057324840764,0.299252646958809)
--(axis cs:36.9426751592357,0.291533240427998)
--(axis cs:37.5796178343949,0.289472761337483)
--(axis cs:38.2165605095541,0.283309955691295)
--(axis cs:38.8535031847134,0.278000893498587)
--(axis cs:39.4904458598726,0.273540957247656)
--(axis cs:40.1273885350318,0.273263667570368)
--(axis cs:40.7643312101911,0.269891133055494)
--(axis cs:41.4012738853503,0.265551949414261)
--(axis cs:42.0382165605096,0.262984253370974)
--(axis cs:42.6751592356688,0.261459744233102)
--(axis cs:43.312101910828,0.255081071306332)
--(axis cs:43.9490445859873,0.255780405060291)
--(axis cs:44.5859872611465,0.257096471216076)
--(axis cs:45.2229299363057,0.249996575452857)
--(axis cs:45.859872611465,0.245815551734966)
--(axis cs:46.4968152866242,0.241581104591847)
--(axis cs:47.1337579617834,0.240337892941643)
--(axis cs:47.7707006369427,0.237297220015229)
--(axis cs:48.4076433121019,0.23048692151937)
--(axis cs:49.0445859872611,0.229093216304297)
--(axis cs:49.6815286624204,0.224743137844091)
--(axis cs:50.3184713375796,0.220809708270799)
--(axis cs:50.9554140127388,0.223070216190218)
--(axis cs:51.5923566878981,0.217134129018718)
--(axis cs:52.2292993630573,0.208240153147986)
--(axis cs:52.8662420382166,0.204910894356599)
--(axis cs:53.5031847133758,0.192682881522589)
--(axis cs:54.140127388535,0.18937722715858)
--(axis cs:54.7770700636943,0.184166950177703)
--(axis cs:55.4140127388535,0.177049791770536)
--(axis cs:56.0509554140127,0.170232762460985)
--(axis cs:56.687898089172,0.16623295292199)
--(axis cs:57.3248407643312,0.157036528201192)
--(axis cs:57.9617834394904,0.155334998342107)
--(axis cs:58.5987261146497,0.155204239899567)
--(axis cs:59.2356687898089,0.149948424352486)
--(axis cs:59.8726114649682,0.144194851621692)
--(axis cs:60.5095541401274,0.14379521147287)
--(axis cs:61.1464968152866,0.135854775316727)
--(axis cs:61.7834394904459,0.133739408404281)
--(axis cs:62.4203821656051,0.131349108035803)
--(axis cs:63.0573248407643,0.126704048458976)
--(axis cs:63.6942675159236,0.121374504026625)
--(axis cs:64.3312101910828,0.115635029753884)
--(axis cs:64.968152866242,0.110838581339199)
--(axis cs:65.6050955414013,0.103540382089016)
--(axis cs:66.2420382165605,0.100943024035525)
--(axis cs:66.8789808917197,0.0958790548726424)
--(axis cs:67.515923566879,0.0904338513247596)
--(axis cs:68.1528662420382,0.0853043146354148)
--(axis cs:68.7898089171974,0.0799186937648095)
--(axis cs:69.4267515923567,0.0678048251733178)
--(axis cs:70.0636942675159,0.0628755983637798)
--(axis cs:70.7006369426752,0.0558775982101887)
--(axis cs:71.3375796178344,0.0514724927371094)
--(axis cs:71.9745222929936,0.0483649740569151)
--(axis cs:72.6114649681529,0.0421912843265068)
--(axis cs:73.2484076433121,0.0390802723591826)
--(axis cs:73.8853503184713,0.0372923793557001)
--(axis cs:74.5222929936306,0.0350849892967673)
--(axis cs:75.1592356687898,0.0355708078262127)
--(axis cs:75.796178343949,0.0341826733904736)
--(axis cs:76.4331210191083,0.0317688519648733)
--(axis cs:77.0700636942675,0.0318353789071742)
--(axis cs:77.7070063694268,0.0298752400154751)
--(axis cs:78.343949044586,0.0298967515817232)
--(axis cs:78.9808917197452,0.0241327467219663)
--(axis cs:79.6178343949044,0.0212486831748139)
--(axis cs:80.2547770700637,0.0204451627178905)
--(axis cs:80.8917197452229,0.0194675271275248)
--(axis cs:81.5286624203822,0.0211045105795529)
--(axis cs:82.1656050955414,0.0212343603246165)
--(axis cs:82.8025477707006,0.0204396014593919)
--(axis cs:83.4394904458599,0.0220522183931969)
--(axis cs:84.0764331210191,0.0233687542517135)
--(axis cs:84.7133757961783,0.02534230077476)
--(axis cs:85.3503184713376,0.0250767680269205)
--(axis cs:85.9872611464968,0.0216685695996623)
--(axis cs:86.6242038216561,0.0181909699502825)
--(axis cs:87.2611464968153,0.0163554994774733)
--(axis cs:87.8980891719745,0.0133406370239793)
--(axis cs:88.5350318471338,0.014016880729732)
--(axis cs:89.171974522293,0.0118877149028677)
--(axis cs:89.8089171974522,0.0130031252610203)
--(axis cs:90.4458598726115,0.0114220480853799)
--(axis cs:91.0828025477707,0.00782227065204935)
--(axis cs:91.7197452229299,0.00884752695509475)
--(axis cs:92.3566878980892,0.00810914958600697)
--(axis cs:92.9936305732484,0.00587584367877112)
--(axis cs:93.6305732484076,0.00789053902655611)
--(axis cs:94.2675159235669,0.00636467183707306)
--(axis cs:94.9044585987261,0.00556341224449921)
--(axis cs:95.5414012738853,0.00156274541079964)
--(axis cs:96.1783439490446,0.000293845386062389)
--(axis cs:96.8152866242038,3.03284596504186e-05)
--(axis cs:97.4522292993631,5.768813798155e-06)
--(axis cs:98.0891719745223,5.28463796967285e-06)
--(axis cs:98.7261146496815,4.05818427611626e-06)
--(axis cs:99.3630573248408,2.32882908321572e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,3.43165540162118e-06)
--(axis cs:98.7261146496815,5.59877399180331e-06)
--(axis cs:98.0891719745223,7.47752974506541e-06)
--(axis cs:97.4522292993631,1.14099277357503e-05)
--(axis cs:96.8152866242038,7.88520100150222e-05)
--(axis cs:96.1783439490446,0.000837032933017311)
--(axis cs:95.5414012738853,0.00315868022961656)
--(axis cs:94.9044585987261,0.00853328358276811)
--(axis cs:94.2675159235669,0.00933826846355198)
--(axis cs:93.6305732484076,0.0111423417301972)
--(axis cs:92.9936305732484,0.00891696526641534)
--(axis cs:92.3566878980892,0.0116173912920251)
--(axis cs:91.7197452229299,0.0124501225769688)
--(axis cs:91.0828025477707,0.0112871140388265)
--(axis cs:90.4458598726115,0.0153071287212765)
--(axis cs:89.8089171974522,0.0167012316361857)
--(axis cs:89.171974522293,0.0156506306584892)
--(axis cs:88.5350318471338,0.0177317555078363)
--(axis cs:87.8980891719745,0.0174999492615441)
--(axis cs:87.2611464968153,0.0208701619017461)
--(axis cs:86.6242038216561,0.0228905040969827)
--(axis cs:85.9872611464968,0.0267246885051799)
--(axis cs:85.3503184713376,0.0302149358525455)
--(axis cs:84.7133757961783,0.03054346928955)
--(axis cs:84.0764331210191,0.0281766288442551)
--(axis cs:83.4394904458599,0.0270885296795413)
--(axis cs:82.8025477707006,0.0256420124825989)
--(axis cs:82.1656050955414,0.0262517105379282)
--(axis cs:81.5286624203822,0.0261550162689972)
--(axis cs:80.8917197452229,0.0247233732386969)
--(axis cs:80.2547770700637,0.0259856303917001)
--(axis cs:79.6178343949044,0.0268641913035154)
--(axis cs:78.9808917197452,0.0300654306667862)
--(axis cs:78.343949044586,0.0358797567662106)
--(axis cs:77.7070063694268,0.0355572576563929)
--(axis cs:77.0700636942675,0.0378470320219506)
--(axis cs:76.4331210191083,0.0377896551029647)
--(axis cs:75.796178343949,0.0398996683537977)
--(axis cs:75.1592356687898,0.0420074235094394)
--(axis cs:74.5222929936306,0.0413250306895447)
--(axis cs:73.8853503184713,0.0436081793380764)
--(axis cs:73.2484076433121,0.0454734158420224)
--(axis cs:72.6114649681529,0.049133511076584)
--(axis cs:71.9745222929936,0.0558574366182939)
--(axis cs:71.3375796178344,0.0594134573218811)
--(axis cs:70.7006369426752,0.0642584668546383)
--(axis cs:70.0636942675159,0.0721467310225761)
--(axis cs:69.4267515923567,0.0773102683743678)
--(axis cs:68.7898089171974,0.0897138342146131)
--(axis cs:68.1528662420382,0.095558087872414)
--(axis cs:67.515923566879,0.100611763206945)
--(axis cs:66.8789808917197,0.10615052490763)
--(axis cs:66.2420382165605,0.111358395584369)
--(axis cs:65.6050955414013,0.113633384565302)
--(axis cs:64.968152866242,0.121143711629494)
--(axis cs:64.3312101910828,0.126137947926465)
--(axis cs:63.6942675159236,0.131866449322595)
--(axis cs:63.0573248407643,0.137122457906553)
--(axis cs:62.4203821656051,0.141561899291776)
--(axis cs:61.7834394904459,0.143817375591912)
--(axis cs:61.1464968152866,0.146036075461174)
--(axis cs:60.5095541401274,0.154095811670015)
--(axis cs:59.8726114649682,0.154582069473699)
--(axis cs:59.2356687898089,0.160452370639155)
--(axis cs:58.5987261146497,0.166058246239091)
--(axis cs:57.9617834394904,0.166310070890374)
--(axis cs:57.3248407643312,0.167861699454003)
--(axis cs:56.687898089172,0.177197799094382)
--(axis cs:56.0509554140127,0.181421876143177)
--(axis cs:55.4140127388535,0.188483101535708)
--(axis cs:54.7770700636943,0.195089255167028)
--(axis cs:54.140127388535,0.200150262552618)
--(axis cs:53.5031847133758,0.20349956522532)
--(axis cs:52.8662420382166,0.215126410386721)
--(axis cs:52.2292993630573,0.218565334305011)
--(axis cs:51.5923566878981,0.227489125422157)
--(axis cs:50.9554140127388,0.233822242518343)
--(axis cs:50.3184713375796,0.231468483119918)
--(axis cs:49.6815286624204,0.2353760986054)
--(axis cs:49.0445859872611,0.23987780078699)
--(axis cs:48.4076433121019,0.241053910904631)
--(axis cs:47.7707006369427,0.247940309239446)
--(axis cs:47.1337579617834,0.25096376497245)
--(axis cs:46.4968152866242,0.252167504700193)
--(axis cs:45.859872611465,0.256612591760716)
--(axis cs:45.2229299363057,0.261138600030869)
--(axis cs:44.5859872611465,0.268463552996364)
--(axis cs:43.9490445859873,0.267239926847311)
--(axis cs:43.312101910828,0.266619148280997)
--(axis cs:42.6751592356688,0.273072581038103)
--(axis cs:42.0382165605096,0.274762437780026)
--(axis cs:41.4012738853503,0.277783568109177)
--(axis cs:40.7643312101911,0.282237690661941)
--(axis cs:40.1273885350318,0.285780317421917)
--(axis cs:39.4904458598726,0.286219767803195)
--(axis cs:38.8535031847134,0.291046294914343)
--(axis cs:38.2165605095541,0.296533036811206)
--(axis cs:37.5796178343949,0.302888186127935)
--(axis cs:36.9426751592357,0.305525542335156)
--(axis cs:36.3057324840764,0.313126197674676)
--(axis cs:35.6687898089172,0.324897281181819)
--(axis cs:35.031847133758,0.334167283403883)
--(axis cs:34.3949044585987,0.338922334351726)
--(axis cs:33.7579617834395,0.353669733100622)
--(axis cs:33.1210191082803,0.368650428136303)
--(axis cs:32.484076433121,0.375814661122032)
--(axis cs:31.8471337579618,0.387192017738172)
--(axis cs:31.2101910828025,0.396390406988772)
--(axis cs:30.5732484076433,0.402509909490607)
--(axis cs:29.9363057324841,0.410134509719718)
--(axis cs:29.2993630573248,0.416667949144106)
--(axis cs:28.6624203821656,0.422941400323453)
--(axis cs:28.0254777070064,0.432113785822255)
--(axis cs:27.3885350318471,0.440398610712514)
--(axis cs:26.7515923566879,0.450507887548523)
--(axis cs:26.1146496815287,0.456441206845085)
--(axis cs:25.4777070063694,0.467249003790501)
--(axis cs:24.8407643312102,0.469905898451141)
--(axis cs:24.203821656051,0.4782214914529)
--(axis cs:23.5668789808917,0.487928904134772)
--(axis cs:22.9299363057325,0.498910005504094)
--(axis cs:22.2929936305732,0.515128984235032)
--(axis cs:21.656050955414,0.528060078801214)
--(axis cs:21.0191082802548,0.541617280870594)
--(axis cs:20.3821656050955,0.555867067675667)
--(axis cs:19.7452229299363,0.571363880647465)
--(axis cs:19.1082802547771,0.589108715800162)
--(axis cs:18.4713375796178,0.600469600475991)
--(axis cs:17.8343949044586,0.612855801944942)
--(axis cs:17.1974522292994,0.626183170985799)
--(axis cs:16.5605095541401,0.648350182351938)
--(axis cs:15.9235668789809,0.661041657894003)
--(axis cs:15.2866242038217,0.679175646160463)
--(axis cs:14.6496815286624,0.695210510906149)
--(axis cs:14.0127388535032,0.71038576473528)
--(axis cs:13.3757961783439,0.727065963031822)
--(axis cs:12.7388535031847,0.739773413647824)
--(axis cs:12.1019108280255,0.764913359535193)
--(axis cs:11.4649681528662,0.782539690678651)
--(axis cs:10.828025477707,0.802609489341392)
--(axis cs:10.1910828025478,0.820216637884012)
--(axis cs:9.55414012738853,0.834270082300459)
--(axis cs:8.9171974522293,0.848268259191549)
--(axis cs:8.28025477707006,0.865134287027841)
--(axis cs:7.64331210191083,0.874298498960644)
--(axis cs:7.00636942675159,0.886418235166546)
--(axis cs:6.36942675159236,0.893152892728514)
--(axis cs:5.73248407643312,0.899472310157756)
--(axis cs:5.09554140127389,0.903842459600922)
--(axis cs:4.45859872611465,0.907301971289871)
--(axis cs:3.82165605095541,0.909749952164736)
--(axis cs:3.18471337579618,0.912421719075865)
--(axis cs:2.54777070063694,0.913779194091047)
--(axis cs:1.91082802547771,0.914707092691575)
--(axis cs:1.27388535031847,0.915487860734499)
--(axis cs:0.636942675159236,0.915717025045383)
--(axis cs:0,0.916095289990536)
--cycle;


==> img/mnist/mnist_rate_distortion_lagrange.tex <==
\addplot [line width=0.5, opacity=0.7, color4, mark=o, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color4, thin}]
table [row sep=\\]{%
0	0.915376993999816 \\
0.636942675159236	0.915301181380637 \\
1.27388535031847	0.915095863282331 \\
1.91082802547771	0.915066309319809 \\
2.54777070063694	0.914556912089465 \\
3.18471337579618	0.914050408700714 \\
3.82165605095541	0.91334185997257 \\
4.45859872611465	0.912009420450195 \\
5.09554140127389	0.909636348626809 \\
5.73248407643312	0.907860161860008 \\
6.36942675159236	0.903459103493078 \\
7.00636942675159	0.899178821969544 \\
7.64331210191083	0.891360687852139 \\
8.28025477707006	0.882510782233439 \\
8.9171974522293	0.870575697929016 \\
9.55414012738853	0.85373014628829 \\
10.1910828025478	0.82880403704592 \\
10.828025477707	0.801728717130027 \\
11.4649681528662	0.776272539156489 \\
12.1019108280255	0.740582688538125 \\
12.7388535031847	0.712167451615096 \\
13.3757961783439	0.689746533182333 \\
14.0127388535032	0.67058839776786 \\
14.6496815286624	0.648456011002418 \\
15.2866242038217	0.627357822834165 \\
15.9235668789809	0.605342271267436 \\
16.5605095541401	0.588233971744776 \\
17.1974522292994	0.569797255949816 \\
17.8343949044586	0.552798916147731 \\
18.4713375796178	0.537970454780152 \\
19.1082802547771	0.514026714018546 \\
19.7452229299363	0.497362609300762 \\
20.3821656050955	0.481528040474514 \\
21.0191082802548	0.467333763077622 \\
21.656050955414	0.453589819747722 \\
22.2929936305732	0.437440908107092 \\
22.9299363057325	0.415787727051065 \\
23.5668789808917	0.403130438275984 \\
24.203821656051	0.386620093375677 \\
24.8407643312102	0.379051973692258 \\
25.4777070063694	0.362455915327591 \\
26.1146496815287	0.353683862529069 \\
26.7515923566879	0.346368686583301 \\
27.3885350318471	0.338230803487477 \\
28.0254777070064	0.318964023661147 \\
28.6624203821656	0.305635637273608 \\
29.2993630573248	0.285338308718492 \\
29.9363057324841	0.2674965579114 \\
30.5732484076433	0.254488006920292 \\
31.2101910828025	0.251294234729567 \\
31.8471337579618	0.239006722030422 \\
32.484076433121	0.229077972588905 \\
33.1210191082803	0.219863332013647 \\
33.7579617834395	0.211874054208092 \\
34.3949044585987	0.204652551963452 \\
35.031847133758	0.195270596032547 \\
35.6687898089172	0.188883615442244 \\
36.3057324840764	0.179306339727229 \\
36.9426751592357	0.175631168204291 \\
37.5796178343949	0.168219595950775 \\
38.2165605095541	0.163624613845365 \\
38.8535031847134	0.154828338220533 \\
39.4904458598726	0.152176310110922 \\
40.1273885350318	0.147579262298631 \\
40.7643312101911	0.14506724881721 \\
41.4012738853503	0.138636813648548 \\
42.0382165605096	0.130749375878861 \\
42.6751592356688	0.134378828826085 \\
43.312101910828	0.134919929963124 \\
43.9490445859873	0.135826237982316 \\
44.5859872611465	0.133704044538879 \\
45.2229299363057	0.134250802329975 \\
45.859872611465	0.132534329362077 \\
46.4968152866242	0.126035465310146 \\
47.1337579617834	0.125930827401472 \\
47.7707006369427	0.125592656413559 \\
48.4076433121019	0.123841459849787 \\
49.0445859872611	0.125970352424755 \\
49.6815286624204	0.121472121003961 \\
50.3184713375796	0.122011292567865 \\
50.9554140127388	0.119547219503509 \\
51.5923566878981	0.118809390134158 \\
52.2292993630573	0.118456936047541 \\
52.8662420382166	0.116434631637176 \\
53.5031847133758	0.11192956779541 \\
54.140127388535	0.112676726113182 \\
54.7770700636943	0.111587388159747 \\
55.4140127388535	0.10712318214279 \\
56.0509554140127	0.103892991368941 \\
56.687898089172	0.103612429702892 \\
57.3248407643312	0.100996080613003 \\
57.9617834394904	0.100185703409074 \\
58.5987261146497	0.101781266515068 \\
59.2356687898089	0.0962965561442138 \\
59.8726114649682	0.094066632338906 \\
60.5095541401274	0.0931186110538002 \\
61.1464968152866	0.0877881358106373 \\
61.7834394904459	0.0918114116113913 \\
62.4203821656051	0.0866632086119249 \\
63.0573248407643	0.0862218490454673 \\
63.6942675159236	0.0842291281792883 \\
64.3312101910828	0.0796134932214045 \\
64.968152866242	0.078063936564344 \\
65.6050955414013	0.0743877807903369 \\
66.2420382165605	0.0707545531840084 \\
66.8789808917197	0.0660307954837778 \\
67.515923566879	0.0639236738316642 \\
68.1528662420382	0.0575884245988545 \\
68.7898089171974	0.05897056475501 \\
69.4267515923567	0.0560765100891313 \\
70.0636942675159	0.0520019816906365 \\
70.7006369426752	0.0523784343843695 \\
71.3375796178344	0.0510249114755397 \\
71.9745222929936	0.0507747160354984 \\
72.6114649681529	0.0462995235540213 \\
73.2484076433121	0.0460993004408827 \\
73.8853503184713	0.0444998244598887 \\
74.5222929936306	0.0434273816238857 \\
75.1592356687898	0.0419976529606315 \\
75.796178343949	0.038663362633422 \\
76.4331210191083	0.0345986863221942 \\
77.0700636942675	0.0317878921663949 \\
77.7070063694268	0.0329244991902299 \\
78.343949044586	0.0320254853674587 \\
78.9808917197452	0.0304725527120379 \\
79.6178343949044	0.0269356374841107 \\
80.2547770700637	0.026080083468133 \\
80.8917197452229	0.0237057695208107 \\
81.5286624203822	0.0213079189615377 \\
82.1656050955414	0.0192221641488071 \\
82.8025477707006	0.0189524420375064 \\
83.4394904458599	0.0180378178603732 \\
84.0764331210191	0.0181575719219518 \\
84.7133757961783	0.0155713079304498 \\
85.3503184713376	0.0122893515058918 \\
85.9872611464968	0.00928628754819194 \\
86.6242038216561	0.00873957551048867 \\
87.2611464968153	0.00972122557239722 \\
87.8980891719745	0.0081805289572545 \\
88.5350318471338	0.00728756979276395 \\
89.171974522293	0.00620525575017904 \\
89.8089171974522	0.0063946382176997 \\
90.4458598726115	0.00491445782913036 \\
91.0828025477707	0.0018515725074698 \\
91.7197452229299	0.000837842977011894 \\
92.3566878980892	0.000466839651853072 \\
92.9936305732484	7.20589843713743e-05 \\
93.6305732484076	0.000113988765298558 \\
94.2675159235669	0.000153000688410248 \\
94.9044585987261	0.000232973991991264 \\
95.5414012738853	0.000403371481401363 \\
96.1783439490446	0.00023171597978036 \\
96.8152866242038	0.000110334155890928 \\
97.4522292993631	0.000208980931565671 \\
98.0891719745223	0.00045508391991532 \\
98.7261146496815	0.000128178018930375 \\
99.3630573248408	1.25084403026837e-05 \\
100	9.07070329958515e-11 \\
};
\path [fill=color4, fill opacity=0.25]
(axis cs:0,0.916038538199047)
--(axis cs:0,0.914715449800585)
--(axis cs:0.636942675159236,0.914659663914735)
--(axis cs:1.27388535031847,0.9143858121773)
--(axis cs:1.91082802547771,0.914307572576902)
--(axis cs:2.54777070063694,0.913684014053957)
--(axis cs:3.18471337579618,0.913042892153762)
--(axis cs:3.82165605095541,0.91228382551161)
--(axis cs:4.45859872611465,0.91070306753085)
--(axis cs:5.09554140127389,0.907978204541236)
--(axis cs:5.73248407643312,0.905987256810499)
--(axis cs:6.36942675159236,0.901101528783673)
--(axis cs:7.00636942675159,0.896407042279415)
--(axis cs:7.64331210191083,0.887960124403626)
--(axis cs:8.28025477707006,0.878520511619829)
--(axis cs:8.9171974522293,0.865889598034456)
--(axis cs:9.55414012738853,0.848259368919545)
--(axis cs:10.1910828025478,0.822528050650763)
--(axis cs:10.828025477707,0.794900975767244)
--(axis cs:11.4649681528662,0.769016807510565)
--(axis cs:12.1019108280255,0.733057141707579)
--(axis cs:12.7388535031847,0.704482439953163)
--(axis cs:13.3757961783439,0.681971988859815)
--(axis cs:14.0127388535032,0.662872684913177)
--(axis cs:14.6496815286624,0.640837630581652)
--(axis cs:15.2866242038217,0.619676163286693)
--(axis cs:15.9235668789809,0.597705062540668)
--(axis cs:16.5605095541401,0.580426486510586)
--(axis cs:17.1974522292994,0.562032245607319)
--(axis cs:17.8343949044586,0.545037322335732)
--(axis cs:18.4713375796178,0.530217313000576)
--(axis cs:19.1082802547771,0.506304833029578)
--(axis cs:19.7452229299363,0.489597692503503)
--(axis cs:20.3821656050955,0.473830353436234)
--(axis cs:21.0191082802548,0.459550944858484)
--(axis cs:21.656050955414,0.445866746170772)
--(axis cs:22.2929936305732,0.429754461914297)
--(axis cs:22.9299363057325,0.408007459940189)
--(axis cs:23.5668789808917,0.395421099528398)
--(axis cs:24.203821656051,0.378980090989575)
--(axis cs:24.8407643312102,0.371476023330517)
--(axis cs:25.4777070063694,0.3549229120102)
--(axis cs:26.1146496815287,0.346026643654027)
--(axis cs:26.7515923566879,0.338743370764596)
--(axis cs:27.3885350318471,0.330451807638229)
--(axis cs:28.0254777070064,0.311135436738336)
--(axis cs:28.6624203821656,0.297815906055307)
--(axis cs:29.2993630573248,0.277664162694088)
--(axis cs:29.9363057324841,0.25991343583122)
--(axis cs:30.5732484076433,0.247066673126086)
--(axis cs:31.2101910828025,0.243773105263658)
--(axis cs:31.8471337579618,0.231488593013764)
--(axis cs:32.484076433121,0.221698869087956)
--(axis cs:33.1210191082803,0.212508105850258)
--(axis cs:33.7579617834395,0.204574782607854)
--(axis cs:34.3949044585987,0.19741036134706)
--(axis cs:35.031847133758,0.188252897196229)
--(axis cs:35.6687898089172,0.182062873781886)
--(axis cs:36.3057324840764,0.17251306525346)
--(axis cs:36.9426751592357,0.169094761459971)
--(axis cs:37.5796178343949,0.161829515954908)
--(axis cs:38.2165605095541,0.157387380594273)
--(axis cs:38.8535031847134,0.148816248860053)
--(axis cs:39.4904458598726,0.146343609414709)
--(axis cs:40.1273885350318,0.141919057105706)
--(axis cs:40.7643312101911,0.139620942763226)
--(axis cs:41.4012738853503,0.13330656267878)
--(axis cs:42.0382165605096,0.12578188592564)
--(axis cs:42.6751592356688,0.129110677758208)
--(axis cs:43.312101910828,0.129936945569066)
--(axis cs:43.9490445859873,0.130812644593255)
--(axis cs:44.5859872611465,0.128714570330973)
--(axis cs:45.2229299363057,0.129207162361482)
--(axis cs:45.859872611465,0.1274272378066)
--(axis cs:46.4968152866242,0.120920003928175)
--(axis cs:47.1337579617834,0.120897818669996)
--(axis cs:47.7707006369427,0.120495876526823)
--(axis cs:48.4076433121019,0.118903938156618)
--(axis cs:49.0445859872611,0.121115365754224)
--(axis cs:49.6815286624204,0.116661412838372)
--(axis cs:50.3184713375796,0.117371797097535)
--(axis cs:50.9554140127388,0.115095065865979)
--(axis cs:51.5923566878981,0.114342833863886)
--(axis cs:52.2292993630573,0.11417938331971)
--(axis cs:52.8662420382166,0.11202616243258)
--(axis cs:53.5031847133758,0.107650928085305)
--(axis cs:54.140127388535,0.108390922569208)
--(axis cs:54.7770700636943,0.107367757970249)
--(axis cs:55.4140127388535,0.102834658001136)
--(axis cs:56.0509554140127,0.0995660672179295)
--(axis cs:56.687898089172,0.0991043734108126)
--(axis cs:57.3248407643312,0.0965695209659225)
--(axis cs:57.9617834394904,0.0957798934820149)
--(axis cs:58.5987261146497,0.0974764746029992)
--(axis cs:59.2356687898089,0.0920283147027648)
--(axis cs:59.8726114649682,0.0895581537253443)
--(axis cs:60.5095541401274,0.0886879517072651)
--(axis cs:61.1464968152866,0.0834822028012807)
--(axis cs:61.7834394904459,0.087467232699381)
--(axis cs:62.4203821656051,0.0823844044498514)
--(axis cs:63.0573248407643,0.0818407833772899)
--(axis cs:63.6942675159236,0.0800005313211937)
--(axis cs:64.3312101910828,0.0754974805899454)
--(axis cs:64.968152866242,0.0737922953077323)
--(axis cs:65.6050955414013,0.0701441665268982)
--(axis cs:66.2420382165605,0.066455262136384)
--(axis cs:66.8789808917197,0.0619093074247279)
--(axis cs:67.515923566879,0.0598761119080138)
--(axis cs:68.1528662420382,0.0537043173198118)
--(axis cs:68.7898089171974,0.0551359291309032)
--(axis cs:69.4267515923567,0.0522787134001611)
--(axis cs:70.0636942675159,0.048377042037148)
--(axis cs:70.7006369426752,0.0487798378665163)
--(axis cs:71.3375796178344,0.0473899699376159)
--(axis cs:71.9745222929936,0.0472090113961065)
--(axis cs:72.6114649681529,0.0428673479623582)
--(axis cs:73.2484076433121,0.0427347209367604)
--(axis cs:73.8853503184713,0.0412273094953588)
--(axis cs:74.5222929936306,0.0402155333624846)
--(axis cs:75.1592356687898,0.0388764906961458)
--(axis cs:75.796178343949,0.035782599618533)
--(axis cs:76.4331210191083,0.0319512906890811)
--(axis cs:77.0700636942675,0.0293799033837599)
--(axis cs:77.7070063694268,0.0304335063012626)
--(axis cs:78.343949044586,0.0295832502576611)
--(axis cs:78.9808917197452,0.0280113446009558)
--(axis cs:79.6178343949044,0.0247544090137188)
--(axis cs:80.2547770700637,0.0239266101879421)
--(axis cs:80.8917197452229,0.0218407314098937)
--(axis cs:81.5286624203822,0.0197564436282338)
--(axis cs:82.1656050955414,0.0177212148902649)
--(axis cs:82.8025477707006,0.0173608178608608)
--(axis cs:83.4394904458599,0.0162781236838918)
--(axis cs:84.0764331210191,0.0164089509264018)
--(axis cs:84.7133757961783,0.0138379426777971)
--(axis cs:85.3503184713376,0.0105439800620159)
--(axis cs:85.9872611464968,0.00757646852615718)
--(axis cs:86.6242038216561,0.00713478443112948)
--(axis cs:87.2611464968153,0.00814863243061245)
--(axis cs:87.8980891719745,0.00657823859405897)
--(axis cs:88.5350318471338,0.00570726660241111)
--(axis cs:89.171974522293,0.00468944224595398)
--(axis cs:89.8089171974522,0.00485475452591465)
--(axis cs:90.4458598726115,0.00351412580395146)
--(axis cs:91.0828025477707,0.00102820806496062)
--(axis cs:91.7197452229299,0.000427322174363339)
--(axis cs:92.3566878980892,0.000113928317430068)
--(axis cs:92.9936305732484,8.66696430421069e-06)
--(axis cs:93.6305732484076,1.17968702368299e-05)
--(axis cs:94.2675159235669,6.29081408795708e-05)
--(axis cs:94.9044585987261,8.16174990142012e-05)
--(axis cs:95.5414012738853,0.000164954139637845)
--(axis cs:96.1783439490446,9.43777100304253e-05)
--(axis cs:96.8152866242038,3.14685594576686e-05)
--(axis cs:97.4522292993631,9.65517205900334e-05)
--(axis cs:98.0891719745223,0.000287876156892615)
--(axis cs:98.7261146496815,6.61862626003341e-05)
--(axis cs:99.3630573248408,8.21966136768723e-06)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,1.67972192376802e-05)
--(axis cs:98.7261146496815,0.000190169775260416)
--(axis cs:98.0891719745223,0.000622291682938025)
--(axis cs:97.4522292993631,0.000321410142541309)
--(axis cs:96.8152866242038,0.000189199752324187)
--(axis cs:96.1783439490446,0.000369054249530294)
--(axis cs:95.5414012738853,0.00064178882316488)
--(axis cs:94.9044585987261,0.000384330484968326)
--(axis cs:94.2675159235669,0.000243093235940925)
--(axis cs:93.6305732484076,0.000216180660360286)
--(axis cs:92.9936305732484,0.000135451004438538)
--(axis cs:92.3566878980892,0.000819750986276076)
--(axis cs:91.7197452229299,0.00124836377966045)
--(axis cs:91.0828025477707,0.00267493694997898)
--(axis cs:90.4458598726115,0.00631478985430925)
--(axis cs:89.8089171974522,0.00793452190948475)
--(axis cs:89.171974522293,0.0077210692544041)
--(axis cs:88.5350318471338,0.00886787298311679)
--(axis cs:87.8980891719745,0.00978281932045003)
--(axis cs:87.2611464968153,0.011293818714182)
--(axis cs:86.6242038216561,0.0103443665898479)
--(axis cs:85.9872611464968,0.0109961065702267)
--(axis cs:85.3503184713376,0.0140347229497676)
--(axis cs:84.7133757961783,0.0173046731831024)
--(axis cs:84.0764331210191,0.0199061929175018)
--(axis cs:83.4394904458599,0.0197975120368546)
--(axis cs:82.8025477707006,0.0205440662141519)
--(axis cs:82.1656050955414,0.0207231134073493)
--(axis cs:81.5286624203822,0.0228593942948415)
--(axis cs:80.8917197452229,0.0255708076317278)
--(axis cs:80.2547770700637,0.0282335567483238)
--(axis cs:79.6178343949044,0.0291168659545026)
--(axis cs:78.9808917197452,0.0329337608231199)
--(axis cs:78.343949044586,0.0344677204772563)
--(axis cs:77.7070063694268,0.0354154920791973)
--(axis cs:77.0700636942675,0.0341958809490299)
--(axis cs:76.4331210191083,0.0372460819553074)
--(axis cs:75.796178343949,0.0415441256483111)
--(axis cs:75.1592356687898,0.0451188152251172)
--(axis cs:74.5222929936306,0.0466392298852867)
--(axis cs:73.8853503184713,0.0477723394244187)
--(axis cs:73.2484076433121,0.0494638799450051)
--(axis cs:72.6114649681529,0.0497316991456844)
--(axis cs:71.9745222929936,0.0543404206748902)
--(axis cs:71.3375796178344,0.0546598530134634)
--(axis cs:70.7006369426752,0.0559770309022227)
--(axis cs:70.0636942675159,0.055626921344125)
--(axis cs:69.4267515923567,0.0598743067781015)
--(axis cs:68.7898089171974,0.0628052003791168)
--(axis cs:68.1528662420382,0.0614725318778972)
--(axis cs:67.515923566879,0.0679712357553146)
--(axis cs:66.8789808917197,0.0701522835428277)
--(axis cs:66.2420382165605,0.0750538442316327)
--(axis cs:65.6050955414013,0.0786313950537755)
--(axis cs:64.968152866242,0.0823355778209557)
--(axis cs:64.3312101910828,0.0837295058528636)
--(axis cs:63.6942675159236,0.0884577250373828)
--(axis cs:63.0573248407643,0.0906029147136447)
--(axis cs:62.4203821656051,0.0909420127739984)
--(axis cs:61.7834394904459,0.0961555905234016)
--(axis cs:61.1464968152866,0.092094068819994)
--(axis cs:60.5095541401274,0.0975492704003353)
--(axis cs:59.8726114649682,0.0985751109524677)
--(axis cs:59.2356687898089,0.100564797585663)
--(axis cs:58.5987261146497,0.106086058427136)
--(axis cs:57.9617834394904,0.104591513336132)
--(axis cs:57.3248407643312,0.105422640260084)
--(axis cs:56.687898089172,0.108120485994971)
--(axis cs:56.0509554140127,0.108219915519953)
--(axis cs:55.4140127388535,0.111411706284445)
--(axis cs:54.7770700636943,0.115807018349245)
--(axis cs:54.140127388535,0.116962529657155)
--(axis cs:53.5031847133758,0.116208207505516)
--(axis cs:52.8662420382166,0.120843100841772)
--(axis cs:52.2292993630573,0.122734488775372)
--(axis cs:51.5923566878981,0.12327594640443)
--(axis cs:50.9554140127388,0.123999373141039)
--(axis cs:50.3184713375796,0.126650788038196)
--(axis cs:49.6815286624204,0.12628282916955)
--(axis cs:49.0445859872611,0.130825339095286)
--(axis cs:48.4076433121019,0.128778981542957)
--(axis cs:47.7707006369427,0.130689436300294)
--(axis cs:47.1337579617834,0.130963836132948)
--(axis cs:46.4968152866242,0.131150926692117)
--(axis cs:45.859872611465,0.137641420917553)
--(axis cs:45.2229299363057,0.139294442298468)
--(axis cs:44.5859872611465,0.138693518746784)
--(axis cs:43.9490445859873,0.140839831371376)
--(axis cs:43.312101910828,0.139902914357183)
--(axis cs:42.6751592356688,0.139646979893963)
--(axis cs:42.0382165605096,0.135716865832081)
--(axis cs:41.4012738853503,0.143967064618317)
--(axis cs:40.7643312101911,0.150513554871194)
--(axis cs:40.1273885350318,0.153239467491557)
--(axis cs:39.4904458598726,0.158009010807135)
--(axis cs:38.8535031847134,0.160840427581014)
--(axis cs:38.2165605095541,0.169861847096458)
--(axis cs:37.5796178343949,0.174609675946643)
--(axis cs:36.9426751592357,0.18216757494861)
--(axis cs:36.3057324840764,0.186099614200999)
--(axis cs:35.6687898089172,0.195704357102601)
--(axis cs:35.031847133758,0.202288294868864)
--(axis cs:34.3949044585987,0.211894742579844)
--(axis cs:33.7579617834395,0.219173325808331)
--(axis cs:33.1210191082803,0.227218558177035)
--(axis cs:32.484076433121,0.236457076089854)
--(axis cs:31.8471337579618,0.246524851047079)
--(axis cs:31.2101910828025,0.258815364195475)
--(axis cs:30.5732484076433,0.261909340714498)
--(axis cs:29.9363057324841,0.27507967999158)
--(axis cs:29.2993630573248,0.293012454742896)
--(axis cs:28.6624203821656,0.313455368491909)
--(axis cs:28.0254777070064,0.326792610583957)
--(axis cs:27.3885350318471,0.346009799336725)
--(axis cs:26.7515923566879,0.353994002402006)
--(axis cs:26.1146496815287,0.361341081404112)
--(axis cs:25.4777070063694,0.369988918644983)
--(axis cs:24.8407643312102,0.386627924053999)
--(axis cs:24.203821656051,0.39426009576178)
--(axis cs:23.5668789808917,0.410839777023571)
--(axis cs:22.9299363057325,0.423567994161941)
--(axis cs:22.2929936305732,0.445127354299886)
--(axis cs:21.656050955414,0.461312893324671)
--(axis cs:21.0191082802548,0.47511658129676)
--(axis cs:20.3821656050955,0.489225727512793)
--(axis cs:19.7452229299363,0.505127526098022)
--(axis cs:19.1082802547771,0.521748595007514)
--(axis cs:18.4713375796178,0.545723596559729)
--(axis cs:17.8343949044586,0.56056050995973)
--(axis cs:17.1974522292994,0.577562266292312)
--(axis cs:16.5605095541401,0.596041456978965)
--(axis cs:15.9235668789809,0.612979479994205)
--(axis cs:15.2866242038217,0.635039482381637)
--(axis cs:14.6496815286624,0.656074391423183)
--(axis cs:14.0127388535032,0.678304110622544)
--(axis cs:13.3757961783439,0.697521077504851)
--(axis cs:12.7388535031847,0.719852463277029)
--(axis cs:12.1019108280255,0.748108235368671)
--(axis cs:11.4649681528662,0.783528270802413)
--(axis cs:10.828025477707,0.808556458492809)
--(axis cs:10.1910828025478,0.835080023441078)
--(axis cs:9.55414012738853,0.859200923657034)
--(axis cs:8.9171974522293,0.875261797823577)
--(axis cs:8.28025477707006,0.88650105284705)
--(axis cs:7.64331210191083,0.894761251300651)
--(axis cs:7.00636942675159,0.901950601659674)
--(axis cs:6.36942675159236,0.905816678202483)
--(axis cs:5.73248407643312,0.909733066909516)
--(axis cs:5.09554140127389,0.911294492712383)
--(axis cs:4.45859872611465,0.91331577336954)
--(axis cs:3.82165605095541,0.91439989443353)
--(axis cs:3.18471337579618,0.915057925247666)
--(axis cs:2.54777070063694,0.915429810124973)
--(axis cs:1.91082802547771,0.915825046062716)
--(axis cs:1.27388535031847,0.915805914387362)
--(axis cs:0.636942675159236,0.915942698846539)
--(axis cs:0,0.916038538199047)
--cycle;


==> img/mnist/mnist_rate_distortion_lcg_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color8, mark=oplus*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table {%
0 0.91562617259915
0.636942675159236 0.915405259396648
1.27388535031847 0.914697878982406
1.91082802547771 0.914701296045678
2.54777070063694 0.913571858579526
3.18471337579618 0.911629447565647
3.82165605095541 0.90989635861537
4.45859872611465 0.90627062419313
5.09554140127389 0.901664929325343
5.73248407643312 0.897266827522544
6.36942675159236 0.891499678526307
7.00636942675159 0.881603214829229
7.64331210191083 0.877921930794255
8.28025477707006 0.86586775789503
8.9171974522293 0.853367286107386
9.55414012738853 0.838913783097814
10.1910828025478 0.820223395661451
10.828025477707 0.79333090819011
11.4649681528662 0.776990094874636
12.1019108280255 0.761578358899569
12.7388535031847 0.740882823167485
13.3757961783439 0.715488940068171
14.0127388535032 0.695528383202618
14.6496815286624 0.677128889777232
15.2866242038217 0.661050434735371
15.9235668789809 0.642081323552702
16.5605095541401 0.624101085852017
17.1974522292994 0.594888324804197
17.8343949044586 0.574371246710944
18.4713375796178 0.557010154459276
19.1082802547771 0.528304598090181
19.7452229299363 0.503781827134953
20.3821656050955 0.490362611907767
21.0191082802548 0.469721718709334
21.656050955414 0.454832245480393
22.2929936305732 0.440697292744844
22.9299363057325 0.419041208070339
23.5668789808917 0.402929161024658
24.203821656051 0.385090475682773
24.8407643312102 0.368392946579334
25.4777070063694 0.353629329916293
26.1146496815287 0.337779790994937
26.7515923566879 0.32173826702965
27.3885350318471 0.309841447327235
28.0254777070064 0.290576352776734
28.6624203821656 0.277879646651127
29.2993630573248 0.268964150599277
29.9363057324841 0.25208379900774
30.5732484076433 0.245005959802093
31.2101910828025 0.232167457564497
31.8471337579618 0.222486240768717
32.484076433121 0.215057907965034
33.1210191082803 0.207856576342608
33.7579617834395 0.196298881818881
34.3949044585987 0.190471225767011
35.031847133758 0.184275400826034
35.6687898089172 0.1735359198014
36.3057324840764 0.162552927783724
36.9426751592357 0.159689440077666
37.5796178343949 0.156311102175162
38.2165605095541 0.155745354447092
38.8535031847134 0.148375680120271
39.4904458598726 0.143113151906369
40.1273885350318 0.135001266004775
40.7643312101911 0.135763386278446
41.4012738853503 0.135826069718052
42.0382165605096 0.131251248693662
42.6751592356688 0.131038983016725
43.312101910828 0.128373199672666
43.9490445859873 0.12603389387296
44.5859872611465 0.120835505082097
45.2229299363057 0.114406698477418
45.859872611465 0.107326851549425
46.4968152866242 0.102625034572057
47.1337579617834 0.0959944560394054
47.7707006369427 0.0975885466013159
48.4076433121019 0.0936843994127242
49.0445859872611 0.0950707601771139
49.6815286624204 0.0903567609189989
50.3184713375796 0.0898643905874174
50.9554140127388 0.087181476823615
51.5923566878981 0.0878079591348715
52.2292993630573 0.0846728394609579
52.8662420382166 0.0838916741237384
53.5031847133758 0.0848462025984769
54.140127388535 0.0836889104843832
54.7770700636943 0.0808613423181444
55.4140127388535 0.0811343835741411
56.0509554140127 0.0805354138946323
56.687898089172 0.0799217622076686
57.3248407643312 0.0779631782470923
57.9617834394904 0.0765052533149971
58.5987261146497 0.0719223316708295
59.2356687898089 0.0718476206081769
59.8726114649682 0.0734935827149359
60.5095541401274 0.069384324901726
61.1464968152866 0.066372152488637
61.7834394904459 0.0663617578779228
62.4203821656051 0.0634486958617831
63.0573248407643 0.0607583935186289
63.6942675159236 0.0589521590104452
64.3312101910828 0.0590481552995577
64.968152866242 0.0569923461125196
65.6050955414013 0.0546438719285089
66.2420382165605 0.0533192654653279
66.8789808917197 0.0535836735275397
67.515923566879 0.0518562937022565
68.1528662420382 0.048816509817362
68.7898089171974 0.0470390447532
69.4267515923567 0.0448535284258085
70.0636942675159 0.0433319408266628
70.7006369426752 0.0395865129445465
71.3375796178344 0.0369272580400793
71.9745222929936 0.0376944927882266
72.6114649681529 0.0361830650931368
73.2484076433121 0.0368106636881806
73.8853503184713 0.0378747422565944
74.5222929936306 0.0368549884056294
75.1592356687898 0.0378474424617786
75.796178343949 0.0397264251497081
76.4331210191083 0.039409449234768
77.0700636942675 0.0363005135726592
77.7070063694268 0.0336142218318465
78.343949044586 0.0326737405635242
78.9808917197452 0.0309997590022045
79.6178343949044 0.0323163575973907
80.2547770700637 0.0317925674713019
80.8917197452229 0.0308434449154332
81.5286624203822 0.0305282584986093
82.1656050955414 0.0249494998473529
82.8025477707006 0.0274197379828
83.4394904458599 0.0275417628346281
84.0764331210191 0.0254348674192704
84.7133757961783 0.0224573345458062
85.3503184713376 0.0184699229979073
85.9872611464968 0.0182812662926367
86.6242038216561 0.0150063817118424
87.2611464968153 0.0135937780417798
87.8980891719745 0.0102108644923581
88.5350318471338 0.0100011810241028
89.171974522293 0.0112621375459561
89.8089171974522 0.00856054782170097
90.4458598726115 0.00930570078741503
91.0828025477707 0.00652474137316883
91.7197452229299 0.00748313407008733
92.3566878980892 0.00393405651190163
92.9936305732484 0.0026701517500349
93.6305732484076 0.00201469335793399
94.2675159235669 0.00216887670660217
94.9044585987261 0.00291709563583769
95.5414012738853 0.00227818308211274
96.1783439490446 0.00111090563737328
96.8152866242038 0.000656898568193852
97.4522292993631 0.000544378998582207
98.0891719745223 0.000227135140391789
98.7261146496815 5.98549367258838e-05
99.3630573248408 3.32569657389759e-06
100 0
};
\path [fill=color8, fill opacity=0.25] 
(axis cs:0,0.916183831301632)
--(axis cs:0,0.915068513896668)
--(axis cs:0.636942675159236,0.914715316133188)
--(axis cs:1.27388535031847,0.913872545495004)
--(axis cs:1.91082802547771,0.913959148435468)
--(axis cs:2.54777070063694,0.912600784221325)
--(axis cs:3.18471337579618,0.910374709036271)
--(axis cs:3.82165605095541,0.908367652125262)
--(axis cs:4.45859872611465,0.904276639345266)
--(axis cs:5.09554140127389,0.899212961046811)
--(axis cs:5.73248407643312,0.894315082183287)
--(axis cs:6.36942675159236,0.888234526664009)
--(axis cs:7.00636942675159,0.877675279406277)
--(axis cs:7.64331210191083,0.873688801799981)
--(axis cs:8.28025477707006,0.860887090439479)
--(axis cs:8.9171974522293,0.847871412436206)
--(axis cs:9.55414012738853,0.83293244673586)
--(axis cs:10.1910828025478,0.813657802747334)
--(axis cs:10.828025477707,0.786216447524043)
--(axis cs:11.4649681528662,0.769643298166583)
--(axis cs:12.1019108280255,0.753992066592937)
--(axis cs:12.7388535031847,0.733035494818551)
--(axis cs:13.3757961783439,0.70735132101841)
--(axis cs:14.0127388535032,0.687415310015463)
--(axis cs:14.6496815286624,0.668873640238633)
--(axis cs:15.2866242038217,0.652678572837654)
--(axis cs:15.9235668789809,0.63365701339487)
--(axis cs:16.5605095541401,0.615375783602715)
--(axis cs:17.1974522292994,0.586023503602249)
--(axis cs:17.8343949044586,0.565164509387315)
--(axis cs:18.4713375796178,0.547887058350396)
--(axis cs:19.1082802547771,0.519117472872721)
--(axis cs:19.7452229299363,0.494838356105665)
--(axis cs:20.3821656050955,0.481555992224512)
--(axis cs:21.0191082802548,0.46092032677355)
--(axis cs:21.656050955414,0.446130471122484)
--(axis cs:22.2929936305732,0.4319091221382)
--(axis cs:22.9299363057325,0.410482101440914)
--(axis cs:23.5668789808917,0.394550282789788)
--(axis cs:24.203821656051,0.376715273653381)
--(axis cs:24.8407643312102,0.360185108441918)
--(axis cs:25.4777070063694,0.345301236003584)
--(axis cs:26.1146496815287,0.32954380630752)
--(axis cs:26.7515923566879,0.31354710644981)
--(axis cs:27.3885350318471,0.301773522549872)
--(axis cs:28.0254777070064,0.282386200375038)
--(axis cs:28.6624203821656,0.269867608807609)
--(axis cs:29.2993630573248,0.260853836051458)
--(axis cs:29.9363057324841,0.244111486541783)
--(axis cs:30.5732484076433,0.237236697153224)
--(axis cs:31.2101910828025,0.22439064056586)
--(axis cs:31.8471337579618,0.214953386593005)
--(axis cs:32.484076433121,0.20776301705447)
--(axis cs:33.1210191082803,0.200603157433261)
--(axis cs:33.7579617834395,0.189295923166261)
--(axis cs:34.3949044585987,0.183567857302749)
--(axis cs:35.031847133758,0.177456933065402)
--(axis cs:35.6687898089172,0.166955343875469)
--(axis cs:36.3057324840764,0.156131397663569)
--(axis cs:36.9426751592357,0.15345584532574)
--(axis cs:37.5796178343949,0.150179706703752)
--(axis cs:38.2165605095541,0.149691362086483)
--(axis cs:38.8535031847134,0.142633966082965)
--(axis cs:39.4904458598726,0.13741901166121)
--(axis cs:40.1273885350318,0.12964114285122)
--(axis cs:40.7643312101911,0.130423389477178)
--(axis cs:41.4012738853503,0.130421477193469)
--(axis cs:42.0382165605096,0.125839464752479)
--(axis cs:42.6751592356688,0.125704253027441)
--(axis cs:43.312101910828,0.123238729427022)
--(axis cs:43.9490445859873,0.120862912078067)
--(axis cs:44.5859872611465,0.115763052751839)
--(axis cs:45.2229299363057,0.109440630701666)
--(axis cs:45.859872611465,0.102415811267276)
--(axis cs:46.4968152866242,0.0978593301509356)
--(axis cs:47.1337579617834,0.0912098626867094)
--(axis cs:47.7707006369427,0.09279946600209)
--(axis cs:48.4076433121019,0.0889316184785178)
--(axis cs:49.0445859872611,0.0904031578846934)
--(axis cs:49.6815286624204,0.085690565357751)
--(axis cs:50.3184713375796,0.0851983892156826)
--(axis cs:50.9554140127388,0.0825138871189255)
--(axis cs:51.5923566878981,0.0830896155509688)
--(axis cs:52.2292993630573,0.0800588419778161)
--(axis cs:52.8662420382166,0.0791715934614279)
--(axis cs:53.5031847133758,0.0801560980773014)
--(axis cs:54.140127388535,0.0790146704284251)
--(axis cs:54.7770700636943,0.0760554731820972)
--(axis cs:55.4140127388535,0.0763806108249709)
--(axis cs:56.0509554140127,0.0758376631466079)
--(axis cs:56.687898089172,0.0752982221156812)
--(axis cs:57.3248407643312,0.0734605430083829)
--(axis cs:57.9617834394904,0.0721916849365807)
--(axis cs:58.5987261146497,0.0676960847903311)
--(axis cs:59.2356687898089,0.0678295118429459)
--(axis cs:59.8726114649682,0.0695176423281828)
--(axis cs:60.5095541401274,0.0656858557069433)
--(axis cs:61.1464968152866,0.0627683989788233)
--(axis cs:61.7834394904459,0.0626269861963982)
--(axis cs:62.4203821656051,0.0598577053060259)
--(axis cs:63.0573248407643,0.0571792489405725)
--(axis cs:63.6942675159236,0.0554593372552413)
--(axis cs:64.3312101910828,0.0555314684630534)
--(axis cs:64.968152866242,0.053547722156746)
--(axis cs:65.6050955414013,0.051349976379588)
--(axis cs:66.2420382165605,0.0498819155146304)
--(axis cs:66.8789808917197,0.0501631531224354)
--(axis cs:67.515923566879,0.0485153134717134)
--(axis cs:68.1528662420382,0.0455003928583661)
--(axis cs:68.7898089171974,0.043881039304414)
--(axis cs:69.4267515923567,0.0419245985390796)
--(axis cs:70.0636942675159,0.0403674044098606)
--(axis cs:70.7006369426752,0.0366890655952935)
--(axis cs:71.3375796178344,0.0341080096651272)
--(axis cs:71.9745222929936,0.0349642804188978)
--(axis cs:72.6114649681529,0.0336448599748394)
--(axis cs:73.2484076433121,0.0343515132190243)
--(axis cs:73.8853503184713,0.0354394081657558)
--(axis cs:74.5222929936306,0.0345860060059865)
--(axis cs:75.1592356687898,0.0355850176047663)
--(axis cs:75.796178343949,0.0375862245242186)
--(axis cs:76.4331210191083,0.037271408948911)
--(axis cs:77.0700636942675,0.0341976126888977)
--(axis cs:77.7070063694268,0.0317066287469141)
--(axis cs:78.343949044586,0.0307628151498378)
--(axis cs:78.9808917197452,0.0289983477322158)
--(axis cs:79.6178343949044,0.0302836813614242)
--(axis cs:80.2547770700637,0.0298445367232684)
--(axis cs:80.8917197452229,0.0290128302621715)
--(axis cs:81.5286624203822,0.0284672195824126)
--(axis cs:82.1656050955414,0.0228880547254554)
--(axis cs:82.8025477707006,0.0254405808681943)
--(axis cs:83.4394904458599,0.0256661901208849)
--(axis cs:84.0764331210191,0.0235392701871245)
--(axis cs:84.7133757961783,0.0204628583072248)
--(axis cs:85.3503184713376,0.0168843212652896)
--(axis cs:85.9872611464968,0.0164793171289252)
--(axis cs:86.6242038216561,0.0133622210067325)
--(axis cs:87.2611464968153,0.0119798217466796)
--(axis cs:87.8980891719745,0.00879583515911497)
--(axis cs:88.5350318471338,0.00861439588500679)
--(axis cs:89.171974522293,0.00994859594389245)
--(axis cs:89.8089171974522,0.00717421833197115)
--(axis cs:90.4458598726115,0.00804687754657632)
--(axis cs:91.0828025477707,0.00529462137526139)
--(axis cs:91.7197452229299,0.00624964781579829)
--(axis cs:92.3566878980892,0.00297718320088796)
--(axis cs:92.9936305732484,0.00190320054033307)
--(axis cs:93.6305732484076,0.00132037531138625)
--(axis cs:94.2675159235669,0.00143814847772095)
--(axis cs:94.9044585987261,0.00199297152973101)
--(axis cs:95.5414012738853,0.00155948381542044)
--(axis cs:96.1783439490446,0.000728172542634179)
--(axis cs:96.8152866242038,0.000396672750202151)
--(axis cs:97.4522292993631,0.000312100661626176)
--(axis cs:98.0891719745223,0.000116994620127478)
--(axis cs:98.7261146496815,3.65944152956116e-05)
--(axis cs:99.3630573248408,2.07572917945606e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,4.57566396833911e-06)
--(axis cs:98.7261146496815,8.3115458156156e-05)
--(axis cs:98.0891719745223,0.0003372756606561)
--(axis cs:97.4522292993631,0.000776657335538238)
--(axis cs:96.8152866242038,0.000917124386185554)
--(axis cs:96.1783439490446,0.00149363873211239)
--(axis cs:95.5414012738853,0.00299688234880505)
--(axis cs:94.9044585987261,0.00384121974194436)
--(axis cs:94.2675159235669,0.0028996049354834)
--(axis cs:93.6305732484076,0.00270901140448173)
--(axis cs:92.9936305732484,0.00343710295973672)
--(axis cs:92.3566878980892,0.0048909298229153)
--(axis cs:91.7197452229299,0.00871662032437636)
--(axis cs:91.0828025477707,0.00775486137107627)
--(axis cs:90.4458598726115,0.0105645240282537)
--(axis cs:89.8089171974522,0.00994687731143079)
--(axis cs:89.171974522293,0.0125756791480198)
--(axis cs:88.5350318471338,0.0113879661631988)
--(axis cs:87.8980891719745,0.0116258938256012)
--(axis cs:87.2611464968153,0.0152077343368799)
--(axis cs:86.6242038216561,0.0166505424169523)
--(axis cs:85.9872611464968,0.0200832154563482)
--(axis cs:85.3503184713376,0.020055524730525)
--(axis cs:84.7133757961783,0.0244518107843876)
--(axis cs:84.0764331210191,0.0273304646514163)
--(axis cs:83.4394904458599,0.0294173355483713)
--(axis cs:82.8025477707006,0.0293988950974056)
--(axis cs:82.1656050955414,0.0270109449692504)
--(axis cs:81.5286624203822,0.0325892974148059)
--(axis cs:80.8917197452229,0.032674059568695)
--(axis cs:80.2547770700637,0.0337405982193353)
--(axis cs:79.6178343949044,0.0343490338333573)
--(axis cs:78.9808917197452,0.0330011702721931)
--(axis cs:78.343949044586,0.0345846659772106)
--(axis cs:77.7070063694268,0.0355218149167789)
--(axis cs:77.0700636942675,0.0384034144564207)
--(axis cs:76.4331210191083,0.041547489520625)
--(axis cs:75.796178343949,0.0418666257751975)
--(axis cs:75.1592356687898,0.0401098673187909)
--(axis cs:74.5222929936306,0.0391239708052724)
--(axis cs:73.8853503184713,0.0403100763474331)
--(axis cs:73.2484076433121,0.0392698141573368)
--(axis cs:72.6114649681529,0.0387212702114341)
--(axis cs:71.9745222929936,0.0404247051575555)
--(axis cs:71.3375796178344,0.0397465064150314)
--(axis cs:70.7006369426752,0.0424839602937994)
--(axis cs:70.0636942675159,0.0462964772434651)
--(axis cs:69.4267515923567,0.0477824583125374)
--(axis cs:68.7898089171974,0.050197050201986)
--(axis cs:68.1528662420382,0.0521326267763579)
--(axis cs:67.515923566879,0.0551972739327996)
--(axis cs:66.8789808917197,0.057004193932644)
--(axis cs:66.2420382165605,0.0567566154160255)
--(axis cs:65.6050955414013,0.0579377674774298)
--(axis cs:64.968152866242,0.0604369700682932)
--(axis cs:64.3312101910828,0.062564842136062)
--(axis cs:63.6942675159236,0.0624449807656491)
--(axis cs:63.0573248407643,0.0643375380966852)
--(axis cs:62.4203821656051,0.0670396864175403)
--(axis cs:61.7834394904459,0.0700965295594473)
--(axis cs:61.1464968152866,0.0699759059984507)
--(axis cs:60.5095541401274,0.0730827940965088)
--(axis cs:59.8726114649682,0.077469523101689)
--(axis cs:59.2356687898089,0.0758657293734079)
--(axis cs:58.5987261146497,0.076148578551328)
--(axis cs:57.9617834394904,0.0808188216934135)
--(axis cs:57.3248407643312,0.0824658134858018)
--(axis cs:56.687898089172,0.0845453022996559)
--(axis cs:56.0509554140127,0.0852331646426567)
--(axis cs:55.4140127388535,0.0858881563233112)
--(axis cs:54.7770700636943,0.0856672114541916)
--(axis cs:54.140127388535,0.0883631505403413)
--(axis cs:53.5031847133758,0.0895363071196525)
--(axis cs:52.8662420382166,0.0886117547860489)
--(axis cs:52.2292993630573,0.0892868369440997)
--(axis cs:51.5923566878981,0.0925263027187743)
--(axis cs:50.9554140127388,0.0918490665283046)
--(axis cs:50.3184713375796,0.0945303919591522)
--(axis cs:49.6815286624204,0.0950229564802468)
--(axis cs:49.0445859872611,0.0997383624695344)
--(axis cs:48.4076433121019,0.0984371803469306)
--(axis cs:47.7707006369427,0.102377627200542)
--(axis cs:47.1337579617834,0.100779049392101)
--(axis cs:46.4968152866242,0.107390738993177)
--(axis cs:45.859872611465,0.112237891831573)
--(axis cs:45.2229299363057,0.119372766253169)
--(axis cs:44.5859872611465,0.125907957412354)
--(axis cs:43.9490445859873,0.131204875667853)
--(axis cs:43.312101910828,0.13350766991831)
--(axis cs:42.6751592356688,0.13637371300601)
--(axis cs:42.0382165605096,0.136663032634845)
--(axis cs:41.4012738853503,0.141230662242636)
--(axis cs:40.7643312101911,0.141103383079715)
--(axis cs:40.1273885350318,0.140361389158331)
--(axis cs:39.4904458598726,0.148807292151527)
--(axis cs:38.8535031847134,0.154117394157577)
--(axis cs:38.2165605095541,0.161799346807702)
--(axis cs:37.5796178343949,0.162442497646571)
--(axis cs:36.9426751592357,0.165923034829591)
--(axis cs:36.3057324840764,0.168974457903878)
--(axis cs:35.6687898089172,0.180116495727332)
--(axis cs:35.031847133758,0.191093868586666)
--(axis cs:34.3949044585987,0.197374594231273)
--(axis cs:33.7579617834395,0.203301840471502)
--(axis cs:33.1210191082803,0.215109995251955)
--(axis cs:32.484076433121,0.222352798875598)
--(axis cs:31.8471337579618,0.230019094944428)
--(axis cs:31.2101910828025,0.239944274563133)
--(axis cs:30.5732484076433,0.252775222450961)
--(axis cs:29.9363057324841,0.260056111473697)
--(axis cs:29.2993630573248,0.277074465147095)
--(axis cs:28.6624203821656,0.285891684494644)
--(axis cs:28.0254777070064,0.29876650517843)
--(axis cs:27.3885350318471,0.317909372104598)
--(axis cs:26.7515923566879,0.329929427609491)
--(axis cs:26.1146496815287,0.346015775682354)
--(axis cs:25.4777070063694,0.361957423829003)
--(axis cs:24.8407643312102,0.37660078471675)
--(axis cs:24.203821656051,0.393465677712165)
--(axis cs:23.5668789808917,0.411308039259528)
--(axis cs:22.9299363057325,0.427600314699764)
--(axis cs:22.2929936305732,0.449485463351488)
--(axis cs:21.656050955414,0.463534019838302)
--(axis cs:21.0191082802548,0.478523110645117)
--(axis cs:20.3821656050955,0.499169231591022)
--(axis cs:19.7452229299363,0.512725298164242)
--(axis cs:19.1082802547771,0.537491723307641)
--(axis cs:18.4713375796178,0.566133250568157)
--(axis cs:17.8343949044586,0.583577984034572)
--(axis cs:17.1974522292994,0.603753146006144)
--(axis cs:16.5605095541401,0.632826388101318)
--(axis cs:15.9235668789809,0.650505633710534)
--(axis cs:15.2866242038217,0.669422296633087)
--(axis cs:14.6496815286624,0.685384139315831)
--(axis cs:14.0127388535032,0.703641456389773)
--(axis cs:13.3757961783439,0.723626559117932)
--(axis cs:12.7388535031847,0.748730151516419)
--(axis cs:12.1019108280255,0.769164651206201)
--(axis cs:11.4649681528662,0.784336891582689)
--(axis cs:10.828025477707,0.800445368856177)
--(axis cs:10.1910828025478,0.826788988575568)
--(axis cs:9.55414012738853,0.844895119459769)
--(axis cs:8.9171974522293,0.858863159778567)
--(axis cs:8.28025477707006,0.870848425350581)
--(axis cs:7.64331210191083,0.882155059788529)
--(axis cs:7.00636942675159,0.88553115025218)
--(axis cs:6.36942675159236,0.894764830388604)
--(axis cs:5.73248407643312,0.900218572861802)
--(axis cs:5.09554140127389,0.904116897603876)
--(axis cs:4.45859872611465,0.908264609040994)
--(axis cs:3.82165605095541,0.911425065105477)
--(axis cs:3.18471337579618,0.912884186095022)
--(axis cs:2.54777070063694,0.914542932937727)
--(axis cs:1.91082802547771,0.915443443655887)
--(axis cs:1.27388535031847,0.915523212469808)
--(axis cs:0.636942675159236,0.916095202660108)
--(axis cs:0,0.916183831301632)
--cycle;


==> img/mnist/mnist_rate_distortion_lcg_order.tex <==
\addplot [line width=0.5, opacity=0.7, color8, mark=oplus*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table {%
0 0.915305616750848
0.636942675159236 0.915104276969796
1.27388535031847 0.914680134161608
1.91082802547771 0.913732679192908
2.54777070063694 0.912928702450008
3.18471337579618 0.911009453451261
3.82165605095541 0.907519996524788
4.45859872611465 0.904955653855577
5.09554140127389 0.901123620318249
5.73248407643312 0.895228285283083
6.36942675159236 0.88576494045672
7.00636942675159 0.875322219228838
7.64331210191083 0.862452866894892
8.28025477707006 0.844486607814906
8.9171974522293 0.835854918896221
9.55414012738853 0.817785027833888
10.1910828025478 0.800744521152228
10.828025477707 0.779828755349154
11.4649681528662 0.7597269068897
12.1019108280255 0.740389641670045
12.7388535031847 0.720692339941161
13.3757961783439 0.698303838759894
14.0127388535032 0.677268241543789
14.6496815286624 0.664034822392277
15.2866242038217 0.645460215373896
15.9235668789809 0.624553532737773
16.5605095541401 0.606896843616851
17.1974522292994 0.592700633887434
17.8343949044586 0.580233032823889
18.4713375796178 0.562026490755379
19.1082802547771 0.544314436789136
19.7452229299363 0.524413102623075
20.3821656050955 0.510405367866624
21.0191082802548 0.489130800076819
21.656050955414 0.471806541383266
22.2929936305732 0.461528290438291
22.9299363057325 0.451830222462886
23.5668789808917 0.437435473502264
24.203821656051 0.428033682547393
24.8407643312102 0.411751127457828
25.4777070063694 0.398010832559085
26.1146496815287 0.381173628895776
26.7515923566879 0.366762809633801
27.3885350318471 0.355874242435093
28.0254777070064 0.349636132362357
28.6624203821656 0.340885295248227
29.2993630573248 0.333129534776963
29.9363057324841 0.318998197433102
30.5732484076433 0.308014290915453
31.2101910828025 0.293767393692542
31.8471337579618 0.294178262671639
32.484076433121 0.286418663188069
33.1210191082803 0.281383040686642
33.7579617834395 0.272967095724434
34.3949044585987 0.269149393126536
35.031847133758 0.262479724669997
35.6687898089172 0.251818292368253
36.3057324840764 0.246040375977273
36.9426751592357 0.243786908097168
37.5796178343949 0.235885485906003
38.2165605095541 0.230574836349601
38.8535031847134 0.227096365827564
39.4904458598726 0.223332323912487
40.1273885350318 0.218659932552394
40.7643312101911 0.204566770229417
41.4012738853503 0.203911160669912
42.0382165605096 0.204018718927522
42.6751592356688 0.192958972539806
43.312101910828 0.196246256418473
43.9490445859873 0.186463753462388
44.5859872611465 0.187087579347251
45.2229299363057 0.180572644604636
45.859872611465 0.172599530877746
46.4968152866242 0.169491228305871
47.1337579617834 0.161181220897314
47.7707006369427 0.158453654566223
48.4076433121019 0.155576435167772
49.0445859872611 0.149600264547539
49.6815286624204 0.150167653485435
50.3184713375796 0.147926040610933
50.9554140127388 0.139548931661472
51.5923566878981 0.134268413464665
52.2292993630573 0.13256929011452
52.8662420382166 0.133278791399743
53.5031847133758 0.129121921923518
54.140127388535 0.129980546010663
54.7770700636943 0.124767307007183
55.4140127388535 0.122938730302438
56.0509554140127 0.116714704391264
56.687898089172 0.115312782582499
57.3248407643312 0.107420743578887
57.9617834394904 0.100721172405838
58.5987261146497 0.0984785476741859
59.2356687898089 0.0899122074114456
59.8726114649682 0.0875801709360784
60.5095541401274 0.0857814822080096
61.1464968152866 0.0806642020220019
61.7834394904459 0.0763994596473613
62.4203821656051 0.077293840747907
63.0573248407643 0.0767490270792127
63.6942675159236 0.0763926208628159
64.3312101910828 0.0688636174490535
64.968152866242 0.0667906978880696
65.6050955414013 0.0636646672813179
66.2420382165605 0.0617801280164295
66.8789808917197 0.0517996280471334
67.515923566879 0.0474014175402925
68.1528662420382 0.0449291401868224
68.7898089171974 0.0459351487102397
69.4267515923567 0.0419639506681663
70.0636942675159 0.0385771276694828
70.7006369426752 0.0346394974516001
71.3375796178344 0.0317807922402114
71.9745222929936 0.0318247958306212
72.6114649681529 0.0324130030668045
73.2484076433121 0.0283146823494547
73.8853503184713 0.0261554333860205
74.5222929936306 0.0255750970663115
75.1592356687898 0.0213068059649195
75.796178343949 0.0206024405150439
76.4331210191083 0.0199714512886019
77.0700636942675 0.0185886676264736
77.7070063694268 0.016945180162019
78.343949044586 0.014397255279047
78.9808917197452 0.0124586980212139
79.6178343949044 0.011667260981322
80.2547770700637 0.0103444666385021
80.8917197452229 0.00836805422664274
81.5286624203822 0.00853468114911495
82.1656050955414 0.00601527879544094
82.8025477707006 0.00706199676280075
83.4394904458599 0.0057882289191978
84.0764331210191 0.00726199630589894
84.7133757961783 0.00782822601631099
85.3503184713376 0.00590771105196135
85.9872611464968 0.0080822242196413
86.6242038216561 0.00750134771628668
87.2611464968153 0.00666886514904909
87.8980891719745 0.00663768531925017
88.5350318471338 0.00477847432329772
89.171974522293 0.00394019001174822
89.8089171974522 0.0043365117169126
90.4458598726115 0.00434969295409785
91.0828025477707 0.00519845023239229
91.7197452229299 0.00303967578635146
92.3566878980892 0.00267934223069348
92.9936305732484 0.00320065304801931
93.6305732484076 0.0024134772993173
94.2675159235669 0.000938127126275921
94.9044585987261 0.000848125722524329
95.5414012738853 0.00010513683243651
96.1783439490446 3.07861702515388e-05
96.8152866242038 1.14759269826353e-05
97.4522292993631 6.24800687128446e-06
98.0891719745223 4.4877668951937e-06
98.7261146496815 3.63551698449316e-06
99.3630573248408 3.12689711521097e-06
100 0
};
\path [fill=color8, fill opacity=0.25] 
(axis cs:0,0.915929505617713)
--(axis cs:0,0.914681727883982)
--(axis cs:0.636942675159236,0.914371571997267)
--(axis cs:1.27388535031847,0.913953156606237)
--(axis cs:1.91082802547771,0.912731164102203)
--(axis cs:2.54777070063694,0.911927037366262)
--(axis cs:3.18471337579618,0.909654127480451)
--(axis cs:3.82165605095541,0.905765210201631)
--(axis cs:4.45859872611465,0.902854190721042)
--(axis cs:5.09554140127389,0.898690838161935)
--(axis cs:5.73248407643312,0.892234856344743)
--(axis cs:6.36942675159236,0.881990603895314)
--(axis cs:7.00636942675159,0.870935216274932)
--(axis cs:7.64331210191083,0.857480508117255)
--(axis cs:8.28025477707006,0.838760542624207)
--(axis cs:8.9171974522293,0.829869197392088)
--(axis cs:9.55414012738853,0.811189218967157)
--(axis cs:10.1910828025478,0.793689864855196)
--(axis cs:10.828025477707,0.772543864254516)
--(axis cs:11.4649681528662,0.752176620037454)
--(axis cs:12.1019108280255,0.732722465477197)
--(axis cs:12.7388535031847,0.71291630182071)
--(axis cs:13.3757961783439,0.69033964605045)
--(axis cs:14.0127388535032,0.669188813375811)
--(axis cs:14.6496815286624,0.655960296284406)
--(axis cs:15.2866242038217,0.637333567768175)
--(axis cs:15.9235668789809,0.616289908056846)
--(axis cs:16.5605095541401,0.598594610812258)
--(axis cs:17.1974522292994,0.584262972165521)
--(axis cs:17.8343949044586,0.57159549213883)
--(axis cs:18.4713375796178,0.553469937700866)
--(axis cs:19.1082802547771,0.535677774931974)
--(axis cs:19.7452229299363,0.515768298008601)
--(axis cs:20.3821656050955,0.501774168298625)
--(axis cs:21.0191082802548,0.480612928550406)
--(axis cs:21.656050955414,0.463300715418809)
--(axis cs:22.2929936305732,0.453001055307822)
--(axis cs:22.9299363057325,0.443307694143706)
--(axis cs:23.5668789808917,0.428983839268504)
--(axis cs:24.203821656051,0.419586044834194)
--(axis cs:24.8407643312102,0.403452366514599)
--(axis cs:25.4777070063694,0.389685665780836)
--(axis cs:26.1146496815287,0.373168634319801)
--(axis cs:26.7515923566879,0.358913519740003)
--(axis cs:27.3885350318471,0.348145894212185)
--(axis cs:28.0254777070064,0.341900427389433)
--(axis cs:28.6624203821656,0.333116311030727)
--(axis cs:29.2993630573248,0.325347173089263)
--(axis cs:29.9363057324841,0.311238675980047)
--(axis cs:30.5732484076433,0.300462541423733)
--(axis cs:31.2101910828025,0.286443701389717)
--(axis cs:31.8471337579618,0.286863076237773)
--(axis cs:32.484076433121,0.279239827677976)
--(axis cs:33.1210191082803,0.274279823389454)
--(axis cs:33.7579617834395,0.266006407815092)
--(axis cs:34.3949044585987,0.262274624853595)
--(axis cs:35.031847133758,0.255610941770661)
--(axis cs:35.6687898089172,0.245075634847859)
--(axis cs:36.3057324840764,0.239332628305074)
--(axis cs:36.9426751592357,0.237092101564118)
--(axis cs:37.5796178343949,0.2293021379428)
--(axis cs:38.2165605095541,0.223946347020239)
--(axis cs:38.8535031847134,0.220452758995665)
--(axis cs:39.4904458598726,0.216918247494976)
--(axis cs:40.1273885350318,0.212320149810232)
--(axis cs:40.7643312101911,0.198081217789011)
--(axis cs:41.4012738853503,0.197402302229025)
--(axis cs:42.0382165605096,0.197603890149477)
--(axis cs:42.6751592356688,0.186748110684411)
--(axis cs:43.312101910828,0.189952346651581)
--(axis cs:43.9490445859873,0.180388244984503)
--(axis cs:44.5859872611465,0.180979625862106)
--(axis cs:45.2229299363057,0.174685297383739)
--(axis cs:45.859872611465,0.166859689721796)
--(axis cs:46.4968152866242,0.163711297409296)
--(axis cs:47.1337579617834,0.155454734006878)
--(axis cs:47.7707006369427,0.153034687009257)
--(axis cs:48.4076433121019,0.150176189419569)
--(axis cs:49.0445859872611,0.144178158147451)
--(axis cs:49.6815286624204,0.144734871326295)
--(axis cs:50.3184713375796,0.142425346858795)
--(axis cs:50.9554140127388,0.134215798987233)
--(axis cs:51.5923566878981,0.129189647037886)
--(axis cs:52.2292993630573,0.127243299437796)
--(axis cs:52.8662420382166,0.128041999059225)
--(axis cs:53.5031847133758,0.12385978838426)
--(axis cs:54.140127388535,0.124650861854391)
--(axis cs:54.7770700636943,0.119479198050935)
--(axis cs:55.4140127388535,0.117746419113148)
--(axis cs:56.0509554140127,0.11157039509876)
--(axis cs:56.687898089172,0.110067474471786)
--(axis cs:57.3248407643312,0.102413413633536)
--(axis cs:57.9617834394904,0.09576378511441)
--(axis cs:58.5987261146497,0.0935605250963397)
--(axis cs:59.2356687898089,0.0851959639906918)
--(axis cs:59.8726114649682,0.0829957581189154)
--(axis cs:60.5095541401274,0.0813295603714004)
--(axis cs:61.1464968152866,0.0763682354673627)
--(axis cs:61.7834394904459,0.0722783949692629)
--(axis cs:62.4203821656051,0.073016989855764)
--(axis cs:63.0573248407643,0.072653856552441)
--(axis cs:63.6942675159236,0.0721600539146906)
--(axis cs:64.3312101910828,0.0648728438267937)
--(axis cs:64.968152866242,0.0628485148120964)
--(axis cs:65.6050955414013,0.059875918231326)
--(axis cs:66.2420382165605,0.0580352944331375)
--(axis cs:66.8789808917197,0.0484762314852226)
--(axis cs:67.515923566879,0.0443082764794573)
--(axis cs:68.1528662420382,0.0419373014460038)
--(axis cs:68.7898089171974,0.042928527729114)
--(axis cs:69.4267515923567,0.0390292899850723)
--(axis cs:70.0636942675159,0.0358708046961962)
--(axis cs:70.7006369426752,0.0320230528145442)
--(axis cs:71.3375796178344,0.0293843338637855)
--(axis cs:71.9745222929936,0.0292993501398967)
--(axis cs:72.6114649681529,0.0298495382028498)
--(axis cs:73.2484076433121,0.0260237665111195)
--(axis cs:73.8853503184713,0.0238193833616253)
--(axis cs:74.5222929936306,0.0234254916187374)
--(axis cs:75.1592356687898,0.0195077931523703)
--(axis cs:75.796178343949,0.0188193626214543)
--(axis cs:76.4331210191083,0.0181485041704609)
--(axis cs:77.0700636942675,0.0170302484434474)
--(axis cs:77.7070063694268,0.0153499658708265)
--(axis cs:78.343949044586,0.0128409459960859)
--(axis cs:78.9808917197452,0.0108600499153756)
--(axis cs:79.6178343949044,0.0101045115180179)
--(axis cs:80.2547770700637,0.0089313329704321)
--(axis cs:80.8917197452229,0.00700001793491414)
--(axis cs:81.5286624203822,0.00713889175724755)
--(axis cs:82.1656050955414,0.00481752797472671)
--(axis cs:82.8025477707006,0.00577434339322353)
--(axis cs:83.4394904458599,0.00465019815362235)
--(axis cs:84.0764331210191,0.00603709374774051)
--(axis cs:84.7133757961783,0.00653728916292378)
--(axis cs:85.3503184713376,0.00478691588812579)
--(axis cs:85.9872611464968,0.0068436096998831)
--(axis cs:86.6242038216561,0.00637956558989233)
--(axis cs:87.2611464968153,0.00557513738597384)
--(axis cs:87.8980891719745,0.00552568381578891)
--(axis cs:88.5350318471338,0.00377422834750471)
--(axis cs:89.171974522293,0.00307422276795075)
--(axis cs:89.8089171974522,0.00331876298176284)
--(axis cs:90.4458598726115,0.00341823492479152)
--(axis cs:91.0828025477707,0.00423254929040241)
--(axis cs:91.7197452229299,0.00234179905341513)
--(axis cs:92.3566878980892,0.00202015229117194)
--(axis cs:92.9936305732484,0.00241997141408065)
--(axis cs:93.6305732484076,0.00179735708639289)
--(axis cs:94.2675159235669,0.000613131361304548)
--(axis cs:94.9044585987261,0.000570721068294582)
--(axis cs:95.5414012738853,6.48441563604445e-05)
--(axis cs:96.1783439490446,2.07070170665285e-05)
--(axis cs:96.8152866242038,8.73140151302451e-06)
--(axis cs:97.4522292993631,5.31474015590676e-06)
--(axis cs:98.0891719745223,4.14529717275571e-06)
--(axis cs:98.7261146496815,3.47046233852032e-06)
--(axis cs:99.3630573248408,2.80615648815124e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,3.4476377422707e-06)
--(axis cs:98.7261146496815,3.800571630466e-06)
--(axis cs:98.0891719745223,4.83023661763169e-06)
--(axis cs:97.4522292993631,7.18127358666216e-06)
--(axis cs:96.8152866242038,1.42204524522462e-05)
--(axis cs:96.1783439490446,4.08653234365492e-05)
--(axis cs:95.5414012738853,0.000145429508512575)
--(axis cs:94.9044585987261,0.00112553037675408)
--(axis cs:94.2675159235669,0.00126312289124729)
--(axis cs:93.6305732484076,0.00302959751224171)
--(axis cs:92.9936305732484,0.00398133468195798)
--(axis cs:92.3566878980892,0.00333853217021503)
--(axis cs:91.7197452229299,0.00373755251928779)
--(axis cs:91.0828025477707,0.00616435117438217)
--(axis cs:90.4458598726115,0.00528115098340418)
--(axis cs:89.8089171974522,0.00535426045206236)
--(axis cs:89.171974522293,0.00480615725554569)
--(axis cs:88.5350318471338,0.00578272029909073)
--(axis cs:87.8980891719745,0.00774968682271143)
--(axis cs:87.2611464968153,0.00776259291212434)
--(axis cs:86.6242038216561,0.00862312984268102)
--(axis cs:85.9872611464968,0.00932083873939949)
--(axis cs:85.3503184713376,0.0070285062157969)
--(axis cs:84.7133757961783,0.00911916286969821)
--(axis cs:84.0764331210191,0.00848689886405736)
--(axis cs:83.4394904458599,0.00692625968477324)
--(axis cs:82.8025477707006,0.00834965013237797)
--(axis cs:82.1656050955414,0.00721302961615516)
--(axis cs:81.5286624203822,0.00993047054098236)
--(axis cs:80.8917197452229,0.00973609051837133)
--(axis cs:80.2547770700637,0.0117576003065721)
--(axis cs:79.6178343949044,0.0132300104446261)
--(axis cs:78.9808917197452,0.0140573461270521)
--(axis cs:78.343949044586,0.015953564562008)
--(axis cs:77.7070063694268,0.0185403944532114)
--(axis cs:77.0700636942675,0.0201470868094998)
--(axis cs:76.4331210191083,0.021794398406743)
--(axis cs:75.796178343949,0.0223855184086334)
--(axis cs:75.1592356687898,0.0231058187774688)
--(axis cs:74.5222929936306,0.0277247025138856)
--(axis cs:73.8853503184713,0.0284914834104156)
--(axis cs:73.2484076433121,0.0306055981877898)
--(axis cs:72.6114649681529,0.0349764679307592)
--(axis cs:71.9745222929936,0.0343502415213457)
--(axis cs:71.3375796178344,0.0341772506166372)
--(axis cs:70.7006369426752,0.037255942088656)
--(axis cs:70.0636942675159,0.0412834506427693)
--(axis cs:69.4267515923567,0.0448986113512603)
--(axis cs:68.7898089171974,0.0489417696913654)
--(axis cs:68.1528662420382,0.0479209789276411)
--(axis cs:67.515923566879,0.0504945586011278)
--(axis cs:66.8789808917197,0.0551230246090441)
--(axis cs:66.2420382165605,0.0655249615997215)
--(axis cs:65.6050955414013,0.0674534163313098)
--(axis cs:64.968152866242,0.0707328809640429)
--(axis cs:64.3312101910828,0.0728543910713133)
--(axis cs:63.6942675159236,0.0806251878109411)
--(axis cs:63.0573248407643,0.0808441976059845)
--(axis cs:62.4203821656051,0.0815706916400501)
--(axis cs:61.7834394904459,0.0805205243254598)
--(axis cs:61.1464968152866,0.0849601685766412)
--(axis cs:60.5095541401274,0.0902334040446188)
--(axis cs:59.8726114649682,0.0921645837532414)
--(axis cs:59.2356687898089,0.0946284508321994)
--(axis cs:58.5987261146497,0.103396570252032)
--(axis cs:57.9617834394904,0.105678559697265)
--(axis cs:57.3248407643312,0.112428073524238)
--(axis cs:56.687898089172,0.120558090693212)
--(axis cs:56.0509554140127,0.121859013683769)
--(axis cs:55.4140127388535,0.128131041491728)
--(axis cs:54.7770700636943,0.130055415963431)
--(axis cs:54.140127388535,0.135310230166935)
--(axis cs:53.5031847133758,0.134384055462777)
--(axis cs:52.8662420382166,0.138515583740262)
--(axis cs:52.2292993630573,0.137895280791244)
--(axis cs:51.5923566878981,0.139347179891445)
--(axis cs:50.9554140127388,0.144882064335711)
--(axis cs:50.3184713375796,0.153426734363072)
--(axis cs:49.6815286624204,0.155600435644575)
--(axis cs:49.0445859872611,0.155022370947626)
--(axis cs:48.4076433121019,0.160976680915976)
--(axis cs:47.7707006369427,0.163872622123189)
--(axis cs:47.1337579617834,0.16690770778775)
--(axis cs:46.4968152866242,0.175271159202445)
--(axis cs:45.859872611465,0.178339372033696)
--(axis cs:45.2229299363057,0.186459991825532)
--(axis cs:44.5859872611465,0.193195532832395)
--(axis cs:43.9490445859873,0.192539261940274)
--(axis cs:43.312101910828,0.202540166185366)
--(axis cs:42.6751592356688,0.199169834395201)
--(axis cs:42.0382165605096,0.210433547705568)
--(axis cs:41.4012738853503,0.2104200191108)
--(axis cs:40.7643312101911,0.211052322669822)
--(axis cs:40.1273885350318,0.224999715294555)
--(axis cs:39.4904458598726,0.229746400329999)
--(axis cs:38.8535031847134,0.233739972659463)
--(axis cs:38.2165605095541,0.237203325678964)
--(axis cs:37.5796178343949,0.242468833869207)
--(axis cs:36.9426751592357,0.250481714630217)
--(axis cs:36.3057324840764,0.252748123649471)
--(axis cs:35.6687898089172,0.258560949888646)
--(axis cs:35.031847133758,0.269348507569333)
--(axis cs:34.3949044585987,0.276024161399477)
--(axis cs:33.7579617834395,0.279927783633777)
--(axis cs:33.1210191082803,0.28848625798383)
--(axis cs:32.484076433121,0.293597498698163)
--(axis cs:31.8471337579618,0.301493449105506)
--(axis cs:31.2101910828025,0.301091085995368)
--(axis cs:30.5732484076433,0.315566040407172)
--(axis cs:29.9363057324841,0.326757718886158)
--(axis cs:29.2993630573248,0.340911896464663)
--(axis cs:28.6624203821656,0.348654279465726)
--(axis cs:28.0254777070064,0.357371837335281)
--(axis cs:27.3885350318471,0.363602590658001)
--(axis cs:26.7515923566879,0.3746120995276)
--(axis cs:26.1146496815287,0.389178623471752)
--(axis cs:25.4777070063694,0.406335999337333)
--(axis cs:24.8407643312102,0.420049888401058)
--(axis cs:24.203821656051,0.436481320260593)
--(axis cs:23.5668789808917,0.445887107736025)
--(axis cs:22.9299363057325,0.460352750782066)
--(axis cs:22.2929936305732,0.470055525568761)
--(axis cs:21.656050955414,0.480312367347724)
--(axis cs:21.0191082802548,0.497648671603231)
--(axis cs:20.3821656050955,0.519036567434623)
--(axis cs:19.7452229299363,0.533057907237549)
--(axis cs:19.1082802547771,0.552951098646299)
--(axis cs:18.4713375796178,0.570583043809892)
--(axis cs:17.8343949044586,0.588870573508949)
--(axis cs:17.1974522292994,0.601138295609348)
--(axis cs:16.5605095541401,0.615199076421443)
--(axis cs:15.9235668789809,0.632817157418699)
--(axis cs:15.2866242038217,0.653586862979618)
--(axis cs:14.6496815286624,0.672109348500149)
--(axis cs:14.0127388535032,0.685347669711766)
--(axis cs:13.3757961783439,0.706268031469337)
--(axis cs:12.7388535031847,0.728468378061612)
--(axis cs:12.1019108280255,0.748056817862892)
--(axis cs:11.4649681528662,0.767277193741947)
--(axis cs:10.828025477707,0.787113646443791)
--(axis cs:10.1910828025478,0.807799177449261)
--(axis cs:9.55414012738853,0.82438083670062)
--(axis cs:8.9171974522293,0.841840640400353)
--(axis cs:8.28025477707006,0.850212673005605)
--(axis cs:7.64331210191083,0.867425225672529)
--(axis cs:7.00636942675159,0.879709222182744)
--(axis cs:6.36942675159236,0.889539277018126)
--(axis cs:5.73248407643312,0.898221714221423)
--(axis cs:5.09554140127389,0.903556402474563)
--(axis cs:4.45859872611465,0.907057116990112)
--(axis cs:3.82165605095541,0.909274782847946)
--(axis cs:3.18471337579618,0.912364779422071)
--(axis cs:2.54777070063694,0.913930367533754)
--(axis cs:1.91082802547771,0.914734194283613)
--(axis cs:1.27388535031847,0.915407111716979)
--(axis cs:0.636942675159236,0.915836981942325)
--(axis cs:0,0.915929505617713)
--cycle;


==> img/mnist/mnist_rate_distortion_lime.tex <==
% lime
\addplot [line width=0.5, opacity=0.8, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table [row sep=\\]{%
0	0.91543710508151 \\
0.636942675159236	0.915585651876172 \\
1.27388535031847	0.915576787189348 \\
1.91082802547771	0.915290925527224 \\
2.54777070063694	0.915278756730258 \\
3.18471337579618	0.915194998849183 \\
3.82165605095541	0.915079104295 \\
4.45859872611465	0.915108326722402 \\
5.09554140127389	0.914925917888759 \\
5.73248407643312	0.914557560179383 \\
6.36942675159236	0.914469702224014 \\
7.00636942675159	0.913753711683676 \\
7.64331210191083	0.912770537460456 \\
8.28025477707006	0.911184100208338 \\
8.9171974522293	0.910129165528342 \\
9.55414012738853	0.910462666001404 \\
10.1910828025478	0.909021566477604 \\
10.828025477707	0.906486183296656 \\
11.4649681528662	0.906148906917078 \\
12.1019108280255	0.905034248635639 \\
12.7388535031847	0.905279969074763 \\
13.3757961783439	0.904520496027544 \\
14.0127388535032	0.903918991335668 \\
14.6496815286624	0.904630380677991 \\
15.2866242038217	0.904019502460724 \\
15.9235668789809	0.904560066797421 \\
16.5605095541401	0.904168138219975 \\
17.1974522292994	0.904118463082705 \\
17.8343949044586	0.903920323172351 \\
18.4713375796178	0.904568860696745 \\
19.1082802547771	0.90429809920257 \\
19.7452229299363	0.902930330837844 \\
20.3821656050955	0.903235273869941 \\
21.0191082802548	0.90276576078264 \\
21.656050955414	0.903808741080575 \\
22.2929936305732	0.901184812705324 \\
22.9299363057325	0.902360509728896 \\
23.5668789808917	0.902265298975399 \\
24.203821656051	0.902767610903538 \\
24.8407643312102	0.904176525258226 \\
25.4777070063694	0.902202739529603 \\
26.1146496815287	0.90197532965045 \\
26.7515923566879	0.902327218234423 \\
27.3885350318471	0.900705369827629 \\
28.0254777070064	0.900729047209607 \\
28.6624203821656	0.901854064000654 \\
29.2993630573248	0.89728143998349 \\
29.9363057324841	0.896292795101908 \\
30.5732484076433	0.895537218293175 \\
31.2101910828025	0.897187682543299 \\
31.8471337579618	0.893132498653722 \\
32.484076433121	0.890714785089222 \\
33.1210191082803	0.886948736016057 \\
33.7579617834395	0.882006104671163 \\
34.3949044585987	0.874420387322898 \\
35.031847133758	0.871506732968264 \\
35.6687898089172	0.869997108142707 \\
36.3057324840764	0.86676930236863 \\
36.9426751592357	0.866714429510757 \\
37.5796178343949	0.867598727301811 \\
38.2165605095541	0.861133744007675 \\
38.8535031847134	0.856350060402765 \\
39.4904458598726	0.854047923466715 \\
40.1273885350318	0.848774573408882 \\
40.7643312101911	0.843116762450663 \\
41.4012738853503	0.832746477593901 \\
42.0382165605096	0.827815838742536 \\
42.6751592356688	0.822545443375129 \\
43.312101910828	0.817319696072955 \\
43.9490445859873	0.812070722530189 \\
44.5859872611465	0.806220889553078 \\
45.2229299363057	0.799511544863926 \\
45.859872611465	0.79083635300165 \\
46.4968152866242	0.782250520544767 \\
47.1337579617834	0.770616082445922 \\
47.7707006369427	0.763909417154791 \\
48.4076433121019	0.757454928732841 \\
49.0445859872611	0.745065760949656 \\
49.6815286624204	0.726000538135704 \\
50.3184713375796	0.708262226450752 \\
50.9554140127388	0.690048579745016 \\
51.5923566878981	0.674957971790236 \\
52.2292993630573	0.665706434693544 \\
52.8662420382166	0.655478120227017 \\
53.5031847133758	0.641898424856785 \\
54.140127388535	0.632326287357565 \\
54.7770700636943	0.626357248171679 \\
55.4140127388535	0.618911735199541 \\
56.0509554140127	0.613652929217119 \\
56.687898089172	0.606971165511573 \\
57.3248407643312	0.595724496264173 \\
57.9617834394904	0.587842557412404 \\
58.5987261146497	0.58090381089538 \\
59.2356687898089	0.571530034506847 \\
59.8726114649682	0.569889588592858 \\
60.5095541401274	0.563713377678745 \\
61.1464968152866	0.557391809035647 \\
61.7834394904459	0.54789720345679 \\
62.4203821656051	0.540904239664709 \\
63.0573248407643	0.529531146157288 \\
63.6942675159236	0.528189634916581 \\
64.3312101910828	0.525148065391357 \\
64.968152866242	0.518556802530214 \\
65.6050955414013	0.511580020514715 \\
66.2420382165605	0.507314250837804 \\
66.8789808917197	0.495842506955974 \\
67.515923566879	0.488036864569354 \\
68.1528662420382	0.47510515473493 \\
68.7898089171974	0.466748136532561 \\
69.4267515923567	0.457501385566405 \\
70.0636942675159	0.44738789318805 \\
70.7006369426752	0.435167617488694 \\
71.3375796178344	0.424216042807932 \\
71.9745222929936	0.406287107474691 \\
72.6114649681529	0.397571671697543 \\
73.2484076433121	0.386725751078706 \\
73.8853503184713	0.370718294102253 \\
74.5222929936306	0.355811752948403 \\
75.1592356687898	0.335303474996003 \\
75.796178343949	0.322482536062966 \\
76.4331210191083	0.302120582196326 \\
77.0700636942675	0.288275971846544 \\
77.7070063694268	0.2745405902648 \\
78.343949044586	0.255703049665813 \\
78.9808917197452	0.248408459409166 \\
79.6178343949044	0.237644243857793 \\
80.2547770700637	0.227614004219275 \\
80.8917197452229	0.220557744306278 \\
81.5286624203822	0.217161481885868 \\
82.1656050955414	0.209095916539626 \\
82.8025477707006	0.202346621165075 \\
83.4394904458599	0.192132493563634 \\
84.0764331210191	0.188239111987638 \\
84.7133757961783	0.18297697579593 \\
85.3503184713376	0.178581648107238 \\
85.9872611464968	0.172628597558708 \\
86.6242038216561	0.16751207508544 \\
87.2611464968153	0.155529360796829 \\
87.8980891719745	0.143290495586884 \\
88.5350318471338	0.137104894772362 \\
89.171974522293	0.128553012790049 \\
89.8089171974522	0.111984983470454 \\
90.4458598726115	0.0976898065630177 \\
91.0828025477707	0.0866216233415621 \\
91.7197452229299	0.0767197536842056 \\
92.3566878980892	0.0719527404430334 \\
92.9936305732484	0.0638333103810626 \\
93.6305732484076	0.0469847083633453 \\
94.2675159235669	0.0352582870768727 \\
94.9044585987261	0.0241656086231636 \\
95.5414012738853	0.0153325147744087 \\
96.1783439490446	0.00965307624345632 \\
96.8152866242038	0.00279312045829225 \\
97.4522292993631	0.000523178881720593 \\
98.0891719745223	0.000149517022016274 \\
98.7261146496815	0.000100566414599238 \\
99.3630573248408	1.61897074655881e-05 \\
100	9.07070329958515e-11 \\
};
\path [fill=color3, fill opacity=0.5] (axis cs:0,0.916079383064668)
--(axis cs:0,0.914794827098351)
--(axis cs:0.636942675159236,0.915023613152902)
--(axis cs:1.27388535031847,0.914999928918593)
--(axis cs:1.91082802547771,0.914634858423652)
--(axis cs:2.54777070063694,0.914631002512073)
--(axis cs:3.18471337579618,0.91456054730964)
--(axis cs:3.82165605095541,0.914376747226435)
--(axis cs:4.45859872611465,0.914453834133619)
--(axis cs:5.09554140127389,0.91424250495676)
--(axis cs:5.73248407643312,0.913795268209331)
--(axis cs:6.36942675159236,0.913650036029944)
--(axis cs:7.00636942675159,0.912842339674016)
--(axis cs:7.64331210191083,0.911691804691341)
--(axis cs:8.28025477707006,0.909851737787421)
--(axis cs:8.9171974522293,0.908587827290145)
--(axis cs:9.55414012738853,0.909026145384707)
--(axis cs:10.1910828025478,0.907342608056764)
--(axis cs:10.828025477707,0.904350631144363)
--(axis cs:11.4649681528662,0.904014384714916)
--(axis cs:12.1019108280255,0.902744131339985)
--(axis cs:12.7388535031847,0.903111451751599)
--(axis cs:13.3757961783439,0.90221471653395)
--(axis cs:14.0127388535032,0.901516992536616)
--(axis cs:14.6496815286624,0.902311676818779)
--(axis cs:15.2866242038217,0.901615368838971)
--(axis cs:15.9235668789809,0.902310700049592)
--(axis cs:16.5605095541401,0.901824217328631)
--(axis cs:17.1974522292994,0.90180607511371)
--(axis cs:17.8343949044586,0.901585910871061)
--(axis cs:18.4713375796178,0.902228954346668)
--(axis cs:19.1082802547771,0.902013120818235)
--(axis cs:19.7452229299363,0.900462179950375)
--(axis cs:20.3821656050955,0.900832517901234)
--(axis cs:21.0191082802548,0.900390831714109)
--(axis cs:21.656050955414,0.901591465540385)
--(axis cs:22.2929936305732,0.898617751249821)
--(axis cs:22.9299363057325,0.899954123061508)
--(axis cs:23.5668789808917,0.899792083070303)
--(axis cs:24.203821656051,0.900350074461279)
--(axis cs:24.8407643312102,0.90199396661653)
--(axis cs:25.4777070063694,0.899719943074677)
--(axis cs:26.1146496815287,0.899526542183869)
--(axis cs:26.7515923566879,0.899886170066379)
--(axis cs:27.3885350318471,0.898116379796748)
--(axis cs:28.0254777070064,0.898101251314369)
--(axis cs:28.6624203821656,0.899195776986203)
--(axis cs:29.2993630573248,0.894208836607503)
--(axis cs:29.9363057324841,0.893103156119897)
--(axis cs:30.5732484076433,0.892289299185698)
--(axis cs:31.2101910828025,0.893809370535307)
--(axis cs:31.8471337579618,0.8896013022374)
--(axis cs:32.484076433121,0.887161682212609)
--(axis cs:33.1210191082803,0.883353743916881)
--(axis cs:33.7579617834395,0.878236658909588)
--(axis cs:34.3949044585987,0.870891572503504)
--(axis cs:35.031847133758,0.867880082462504)
--(axis cs:35.6687898089172,0.866582462153869)
--(axis cs:36.3057324840764,0.863532219267894)
--(axis cs:36.9426751592357,0.863580213745624)
--(axis cs:37.5796178343949,0.864426726984778)
--(axis cs:38.2165605095541,0.857843239537359)
--(axis cs:38.8535031847134,0.852938050437577)
--(axis cs:39.4904458598726,0.850395456657371)
--(axis cs:40.1273885350318,0.84494529975199)
--(axis cs:40.7643312101911,0.839052134984613)
--(axis cs:41.4012738853503,0.828580789148494)
--(axis cs:42.0382165605096,0.823572215249396)
--(axis cs:42.6751592356688,0.8184068295383)
--(axis cs:43.312101910828,0.813041176847802)
--(axis cs:43.9490445859873,0.80783341690966)
--(axis cs:44.5859872611465,0.801821961949909)
--(axis cs:45.2229299363057,0.795100542299888)
--(axis cs:45.859872611465,0.786141245253086)
--(axis cs:46.4968152866242,0.777268336630078)
--(axis cs:47.1337579617834,0.765621266486912)
--(axis cs:47.7707006369427,0.758683382422502)
--(axis cs:48.4076433121019,0.751987588028317)
--(axis cs:49.0445859872611,0.739272991921812)
--(axis cs:49.6815286624204,0.719949983300406)
--(axis cs:50.3184713375796,0.702021649890628)
--(axis cs:50.9554140127388,0.683736798763827)
--(axis cs:51.5923566878981,0.668643937958223)
--(axis cs:52.2292993630573,0.659264381780015)
--(axis cs:52.8662420382166,0.648977408287483)
--(axis cs:53.5031847133758,0.635560700183553)
--(axis cs:54.140127388535,0.62615402677108)
--(axis cs:54.7770700636943,0.620321728252971)
--(axis cs:55.4140127388535,0.612876262921337)
--(axis cs:56.0509554140127,0.607626748588334)
--(axis cs:56.687898089172,0.600733833149585)
--(axis cs:57.3248407643312,0.589488692432083)
--(axis cs:57.9617834394904,0.581705857438499)
--(axis cs:58.5987261146497,0.574717515529704)
--(axis cs:59.2356687898089,0.565641832455606)
--(axis cs:59.8726114649682,0.564207783187453)
--(axis cs:60.5095541401274,0.557906424105632)
--(axis cs:61.1464968152866,0.551781055134362)
--(axis cs:61.7834394904459,0.542171460573227)
--(axis cs:62.4203821656051,0.535038087236032)
--(axis cs:63.0573248407643,0.523559485593186)
--(axis cs:63.6942675159236,0.522006073151271)
--(axis cs:64.3312101910828,0.519015678456034)
--(axis cs:64.968152866242,0.512267967690091)
--(axis cs:65.6050955414013,0.505119040978133)
--(axis cs:66.2420382165605,0.50089733363376)
--(axis cs:66.8789808917197,0.48942875257422)
--(axis cs:67.515923566879,0.481566766909845)
--(axis cs:68.1528662420382,0.468635181802191)
--(axis cs:68.7898089171974,0.460290469982757)
--(axis cs:69.4267515923567,0.450914251058123)
--(axis cs:70.0636942675159,0.440723175881328)
--(axis cs:70.7006369426752,0.428300999795265)
--(axis cs:71.3375796178344,0.417458747676298)
--(axis cs:71.9745222929936,0.399316087044996)
--(axis cs:72.6114649681529,0.390732923407522)
--(axis cs:73.2484076433121,0.379531041873277)
--(axis cs:73.8853503184713,0.363307446563321)
--(axis cs:74.5222929936306,0.348538451113968)
--(axis cs:75.1592356687898,0.328158235523277)
--(axis cs:75.796178343949,0.315533104355908)
--(axis cs:76.4331210191083,0.295522148619647)
--(axis cs:77.0700636942675,0.281975028674368)
--(axis cs:77.7070063694268,0.268629145861522)
--(axis cs:78.343949044586,0.250318336003788)
--(axis cs:78.9808917197452,0.243500947668806)
--(axis cs:79.6178343949044,0.233251181642862)
--(axis cs:80.2547770700637,0.223663685119514)
--(axis cs:80.8917197452229,0.216969299365164)
--(axis cs:81.5286624203822,0.213750519159648)
--(axis cs:82.1656050955414,0.205791898818993)
--(axis cs:82.8025477707006,0.199021669999945)
--(axis cs:83.4394904458599,0.18860557960777)
--(axis cs:84.0764331210191,0.184688508721503)
--(axis cs:84.7133757961783,0.179201842548727)
--(axis cs:85.3503184713376,0.174663746592639)
--(axis cs:85.9872611464968,0.168820576936364)
--(axis cs:86.6242038216561,0.163722893193462)
--(axis cs:87.2611464968153,0.151558019055353)
--(axis cs:87.8980891719745,0.139056003166)
--(axis cs:88.5350318471338,0.13269350623423)
--(axis cs:89.171974522293,0.124260231927237)
--(axis cs:89.8089171974522,0.107851809812196)
--(axis cs:90.4458598726115,0.0936339056558442)
--(axis cs:91.0828025477707,0.0832201671540272)
--(axis cs:91.7197452229299,0.0734753820435903)
--(axis cs:92.3566878980892,0.0685975242716085)
--(axis cs:92.9936305732484,0.0605436936574134)
--(axis cs:93.6305732484076,0.0434976539871339)
--(axis cs:94.2675159235669,0.0316875151363747)
--(axis cs:94.9044585987261,0.0211158016435392)
--(axis cs:95.5414012738853,0.0126961389591062)
--(axis cs:96.1783439490446,0.00760482673052138)
--(axis cs:96.8152866242038,0.00180161931493723)
--(axis cs:97.4522292993631,0.000305558813412788)
--(axis cs:98.0891719745223,7.30758939431056e-05)
--(axis cs:98.7261146496815,4.83394358134159e-05)
--(axis cs:99.3630573248408,9.43494100266062e-06)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,2.29444739285156e-05)
--(axis cs:98.7261146496815,0.00015279339338506)
--(axis cs:98.0891719745223,0.000225958150089443)
--(axis cs:97.4522292993631,0.000740798950028399)
--(axis cs:96.8152866242038,0.00378462160164727)
--(axis cs:96.1783439490446,0.0117013257563913)
--(axis cs:95.5414012738853,0.0179688905897112)
--(axis cs:94.9044585987261,0.0272154156027879)
--(axis cs:94.2675159235669,0.0388290590173707)
--(axis cs:93.6305732484076,0.0504717627395568)
--(axis cs:92.9936305732484,0.0671229271047119)
--(axis cs:92.3566878980892,0.0753079566144583)
--(axis cs:91.7197452229299,0.0799641253248209)
--(axis cs:91.0828025477707,0.0900230795290969)
--(axis cs:90.4458598726115,0.101745707470191)
--(axis cs:89.8089171974522,0.116118157128713)
--(axis cs:89.171974522293,0.132845793652861)
--(axis cs:88.5350318471338,0.141516283310495)
--(axis cs:87.8980891719745,0.147524988007768)
--(axis cs:87.2611464968153,0.159500702538304)
--(axis cs:86.6242038216561,0.171301256977417)
--(axis cs:85.9872611464968,0.176436618181052)
--(axis cs:85.3503184713376,0.182499549621837)
--(axis cs:84.7133757961783,0.186752109043132)
--(axis cs:84.0764331210191,0.191789715253773)
--(axis cs:83.4394904458599,0.195659407519499)
--(axis cs:82.8025477707006,0.205671572330204)
--(axis cs:82.1656050955414,0.212399934260258)
--(axis cs:81.5286624203822,0.220572444612088)
--(axis cs:80.8917197452229,0.224146189247392)
--(axis cs:80.2547770700637,0.231564323319037)
--(axis cs:79.6178343949044,0.242037306072724)
--(axis cs:78.9808917197452,0.253315971149526)
--(axis cs:78.343949044586,0.261087763327839)
--(axis cs:77.7070063694268,0.280452034668077)
--(axis cs:77.0700636942675,0.294576915018719)
--(axis cs:76.4331210191083,0.308719015773004)
--(axis cs:75.796178343949,0.329431967770025)
--(axis cs:75.1592356687898,0.34244871446873)
--(axis cs:74.5222929936306,0.363085054782837)
--(axis cs:73.8853503184713,0.378129141641185)
--(axis cs:73.2484076433121,0.393920460284134)
--(axis cs:72.6114649681529,0.404410419987564)
--(axis cs:71.9745222929936,0.413258127904385)
--(axis cs:71.3375796178344,0.430973337939566)
--(axis cs:70.7006369426752,0.442034235182123)
--(axis cs:70.0636942675159,0.454052610494771)
--(axis cs:69.4267515923567,0.464088520074686)
--(axis cs:68.7898089171974,0.473205803082365)
--(axis cs:68.1528662420382,0.481575127667668)
--(axis cs:67.515923566879,0.494506962228863)
--(axis cs:66.8789808917197,0.502256261337728)
--(axis cs:66.2420382165605,0.513731168041848)
--(axis cs:65.6050955414013,0.518041000051298)
--(axis cs:64.968152866242,0.524845637370337)
--(axis cs:64.3312101910828,0.53128045232668)
--(axis cs:63.6942675159236,0.534373196681891)
--(axis cs:63.0573248407643,0.535502806721391)
--(axis cs:62.4203821656051,0.546770392093387)
--(axis cs:61.7834394904459,0.553622946340352)
--(axis cs:61.1464968152866,0.563002562936932)
--(axis cs:60.5095541401274,0.569520331251858)
--(axis cs:59.8726114649682,0.575571393998262)
--(axis cs:59.2356687898089,0.577418236558089)
--(axis cs:58.5987261146497,0.587090106261056)
--(axis cs:57.9617834394904,0.593979257386309)
--(axis cs:57.3248407643312,0.601960300096263)
--(axis cs:56.687898089172,0.61320849787356)
--(axis cs:56.0509554140127,0.619679109845904)
--(axis cs:55.4140127388535,0.624947207477744)
--(axis cs:54.7770700636943,0.632392768090387)
--(axis cs:54.140127388535,0.63849854794405)
--(axis cs:53.5031847133758,0.648236149530017)
--(axis cs:52.8662420382166,0.66197883216655)
--(axis cs:52.2292993630573,0.672148487607073)
--(axis cs:51.5923566878981,0.681272005622249)
--(axis cs:50.9554140127388,0.696360360726206)
--(axis cs:50.3184713375796,0.714502803010875)
--(axis cs:49.6815286624204,0.732051092971002)
--(axis cs:49.0445859872611,0.7508585299775)
--(axis cs:48.4076433121019,0.762922269437365)
--(axis cs:47.7707006369427,0.769135451887081)
--(axis cs:47.1337579617834,0.775610898404932)
--(axis cs:46.4968152866242,0.787232704459455)
--(axis cs:45.859872611465,0.795531460750215)
--(axis cs:45.2229299363057,0.803922547427965)
--(axis cs:44.5859872611465,0.810619817156248)
--(axis cs:43.9490445859873,0.816308028150717)
--(axis cs:43.312101910828,0.821598215298107)
--(axis cs:42.6751592356688,0.826684057211959)
--(axis cs:42.0382165605096,0.832059462235675)
--(axis cs:41.4012738853503,0.836912166039307)
--(axis cs:40.7643312101911,0.847181389916714)
--(axis cs:40.1273885350318,0.852603847065774)
--(axis cs:39.4904458598726,0.857700390276058)
--(axis cs:38.8535031847134,0.859762070367953)
--(axis cs:38.2165605095541,0.864424248477991)
--(axis cs:37.5796178343949,0.870770727618844)
--(axis cs:36.9426751592357,0.869848645275891)
--(axis cs:36.3057324840764,0.870006385469365)
--(axis cs:35.6687898089172,0.873411754131544)
--(axis cs:35.031847133758,0.875133383474024)
--(axis cs:34.3949044585987,0.877949202142292)
--(axis cs:33.7579617834395,0.885775550432738)
--(axis cs:33.1210191082803,0.890543728115232)
--(axis cs:32.484076433121,0.894267887965834)
--(axis cs:31.8471337579618,0.896663695070044)
--(axis cs:31.2101910828025,0.900565994551291)
--(axis cs:30.5732484076433,0.898785137400652)
--(axis cs:29.9363057324841,0.899482434083919)
--(axis cs:29.2993630573248,0.900354043359477)
--(axis cs:28.6624203821656,0.904512351015106)
--(axis cs:28.0254777070064,0.903356843104844)
--(axis cs:27.3885350318471,0.903294359858509)
--(axis cs:26.7515923566879,0.904768266402466)
--(axis cs:26.1146496815287,0.90442411711703)
--(axis cs:25.4777070063694,0.904685535984529)
--(axis cs:24.8407643312102,0.906359083899922)
--(axis cs:24.203821656051,0.905185147345798)
--(axis cs:23.5668789808917,0.904738514880494)
--(axis cs:22.9299363057325,0.904766896396285)
--(axis cs:22.2929936305732,0.903751874160826)
--(axis cs:21.656050955414,0.906026016620764)
--(axis cs:21.0191082802548,0.905140689851172)
--(axis cs:20.3821656050955,0.905638029838647)
--(axis cs:19.7452229299363,0.905398481725312)
--(axis cs:19.1082802547771,0.906583077586904)
--(axis cs:18.4713375796178,0.906908767046822)
--(axis cs:17.8343949044586,0.906254735473642)
--(axis cs:17.1974522292994,0.906430851051699)
--(axis cs:16.5605095541401,0.906512059111318)
--(axis cs:15.9235668789809,0.906809433545251)
--(axis cs:15.2866242038217,0.906423636082476)
--(axis cs:14.6496815286624,0.906949084537202)
--(axis cs:14.0127388535032,0.90632099013472)
--(axis cs:13.3757961783439,0.906826275521138)
--(axis cs:12.7388535031847,0.907448486397928)
--(axis cs:12.1019108280255,0.907324365931292)
--(axis cs:11.4649681528662,0.908283429119241)
--(axis cs:10.828025477707,0.908621735448949)
--(axis cs:10.1910828025478,0.910700524898445)
--(axis cs:9.55414012738853,0.911899186618101)
--(axis cs:8.9171974522293,0.911670503766539)
--(axis cs:8.28025477707006,0.912516462629255)
--(axis cs:7.64331210191083,0.913849270229571)
--(axis cs:7.00636942675159,0.914665083693335)
--(axis cs:6.36942675159236,0.915289368418084)
--(axis cs:5.73248407643312,0.915319852149434)
--(axis cs:5.09554140127389,0.915609330820757)
--(axis cs:4.45859872611465,0.915762819311185)
--(axis cs:3.82165605095541,0.915781461363565)
--(axis cs:3.18471337579618,0.915829450388726)
--(axis cs:2.54777070063694,0.915926510948444)
--(axis cs:1.91082802547771,0.915946992630796)
--(axis cs:1.27388535031847,0.916153645460102)
--(axis cs:0.636942675159236,0.916147690599442)
--(axis cs:0,0.916079383064668)
--cycle;


==> img/mnist/mnist_rate_distortion_lrp.tex <==
% lrp-a-flat
\addplot [line width=0.5, opacity=0.8, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table [row sep=\\]{%
0	0.915564971454442 \\
0.636942675159236	0.915249241957208 \\
1.27388535031847	0.914182096141158 \\
1.91082802547771	0.913384990103077 \\
2.54777070063694	0.912696832342772 \\
3.18471337579618	0.911705492149922 \\
3.82165605095541	0.911610428845743 \\
4.45859872611465	0.910597423146246 \\
5.09554140127389	0.909791541580344 \\
5.73248407643312	0.909369708862505 \\
6.36942675159236	0.909138373181922 \\
7.00636942675159	0.908375531422789 \\
7.64331210191083	0.906519337344216 \\
8.28025477707006	0.905690164521511 \\
8.9171974522293	0.905282773996587 \\
9.55414012738853	0.9054191856744 \\
10.1910828025478	0.904460609773523 \\
10.828025477707	0.903103243962978 \\
11.4649681528662	0.902260963952867 \\
12.1019108280255	0.901953587202006 \\
12.7388535031847	0.900898863503244 \\
13.3757961783439	0.899123547563504 \\
14.0127388535032	0.89750605907524 \\
14.6496815286624	0.896184821815987 \\
15.2866242038217	0.892546699359082 \\
15.9235668789809	0.889410775435972 \\
16.5605095541401	0.886875169998966 \\
17.1974522292994	0.881822417512012 \\
17.8343949044586	0.874493795077215 \\
18.4713375796178	0.868887333279708 \\
19.1082802547771	0.863764370550343 \\
19.7452229299363	0.857484827750159 \\
20.3821656050955	0.849647658307513 \\
21.0191082802548	0.843608460757678 \\
21.656050955414	0.827940664980488 \\
22.2929936305732	0.817012488915861 \\
22.9299363057325	0.812749606510988 \\
23.5668789808917	0.797875989739587 \\
24.203821656051	0.781661073988362 \\
24.8407643312102	0.767742146578421 \\
25.4777070063694	0.747512167933673 \\
26.1146496815287	0.733246414145178 \\
26.7515923566879	0.718510874167187 \\
27.3885350318471	0.696950631963373 \\
28.0254777070064	0.679469130793659 \\
28.6624203821656	0.663277497999479 \\
29.2993630573248	0.6461357247247 \\
29.9363057324841	0.63207092648845 \\
30.5732484076433	0.612669699960388 \\
31.2101910828025	0.592279611885096 \\
31.8471337579618	0.574711288037179 \\
32.484076433121	0.555349003288138 \\
33.1210191082803	0.538345414173455 \\
33.7579617834395	0.521898110978036 \\
34.3949044585987	0.505918641165554 \\
35.031847133758	0.48551525476847 \\
35.6687898089172	0.468329492285739 \\
36.3057324840764	0.447510030681296 \\
36.9426751592357	0.430036015477162 \\
37.5796178343949	0.408825479754269 \\
38.2165605095541	0.395901616680612 \\
38.8535031847134	0.38789101567887 \\
39.4904458598726	0.368596821763458 \\
40.1273885350318	0.351203641759012 \\
40.7643312101911	0.344321353502469 \\
41.4012738853503	0.331105996770966 \\
42.0382165605096	0.317738574900145 \\
42.6751592356688	0.306859044687438 \\
43.312101910828	0.297720884805415 \\
43.9490445859873	0.285753045337494 \\
44.5859872611465	0.272836896182697 \\
45.2229299363057	0.264143881363794 \\
45.859872611465	0.257768469916953 \\
46.4968152866242	0.253695068467144 \\
47.1337579617834	0.247523868887629 \\
47.7707006369427	0.240451336784018 \\
48.4076433121019	0.236707656645938 \\
49.0445859872611	0.216706395174625 \\
49.6815286624204	0.211256365341724 \\
50.3184713375796	0.19434927517216 \\
50.9554140127388	0.189626264188847 \\
51.5923566878981	0.17738066608231 \\
52.2292993630573	0.169422061597494 \\
52.8662420382166	0.157477472476161 \\
53.5031847133758	0.150141337029572 \\
54.140127388535	0.140068892002228 \\
54.7770700636943	0.137529361560668 \\
55.4140127388535	0.135063938105227 \\
56.0509554140127	0.127655643855027 \\
56.687898089172	0.124826757378225 \\
57.3248407643312	0.1173038936504 \\
57.9617834394904	0.115496774323102 \\
58.5987261146497	0.109850056118146 \\
59.2356687898089	0.107751102882251 \\
59.8726114649682	0.0974747186745921 \\
60.5095541401274	0.0912794000995374 \\
61.1464968152866	0.0870153778032115 \\
61.7834394904459	0.0836696877626941 \\
62.4203821656051	0.0788040796981376 \\
63.0573248407643	0.0756146849295008 \\
63.6942675159236	0.0729004501802038 \\
64.3312101910828	0.0686718259920316 \\
64.968152866242	0.0639418024870963 \\
65.6050955414013	0.0612573951105369 \\
66.2420382165605	0.0609042873507699 \\
66.8789808917197	0.0611003120626597 \\
67.515923566879	0.0602126713809356 \\
68.1528662420382	0.0567711007093105 \\
68.7898089171974	0.0564380243385208 \\
69.4267515923567	0.0548103594653956 \\
70.0636942675159	0.05316766861929 \\
70.7006369426752	0.0513099785447827 \\
71.3375796178344	0.0505450061681438 \\
71.9745222929936	0.0485567727194318 \\
72.6114649681529	0.0456268149646077 \\
73.2484076433121	0.0420307675196621 \\
73.8853503184713	0.0427707334669037 \\
74.5222929936306	0.045323355671726 \\
75.1592356687898	0.0455018684895622 \\
75.796178343949	0.0481263241523093 \\
76.4331210191083	0.0467338156094918 \\
77.0700636942675	0.0438497170077891 \\
77.7070063694268	0.0424094352688396 \\
78.343949044586	0.0389564687285314 \\
78.9808917197452	0.0378327443803056 \\
79.6178343949044	0.0355924633214438 \\
80.2547770700637	0.0359513183845675 \\
80.8917197452229	0.0353927122384706 \\
81.5286624203822	0.0361806111854356 \\
82.1656050955414	0.0329105919571784 \\
82.8025477707006	0.0333143587253737 \\
83.4394904458599	0.0303698098871828 \\
84.0764331210191	0.0292867926035305 \\
84.7133757961783	0.027863588639464 \\
85.3503184713376	0.0276722165300559 \\
85.9872611464968	0.0264658749433791 \\
86.6242038216561	0.0236178079489236 \\
87.2611464968153	0.0220086002116911 \\
87.8980891719745	0.020823577277475 \\
88.5350318471338	0.0179405827819884 \\
89.171974522293	0.016012131542241 \\
89.8089171974522	0.0119573991377804 \\
90.4458598726115	0.00804850425234559 \\
91.0828025477707	0.00509652472752826 \\
91.7197452229299	0.00344001865073023 \\
92.3566878980892	0.00207183151504865 \\
92.9936305732484	0.00162004072997316 \\
93.6305732484076	0.00103290714665773 \\
94.2675159235669	0.00086310290151534 \\
94.9044585987261	0.000796828518222246 \\
95.5414012738853	0.000720283981157556 \\
96.1783439490446	0.000274189714006541 \\
96.8152866242038	0.000155984506550722 \\
97.4522292993631	5.17217384751223e-05 \\
98.0891719745223	6.93125339556344e-06 \\
98.7261146496815	2.13038506507113e-06 \\
99.3630573248408	1.84760827045882e-06 \\
100	9.07070329958515e-11 \\
};
\path [fill=color1, fill opacity=0.5] (axis cs:0,0.9160976908346)
--(axis cs:0,0.915032252074283)
--(axis cs:0.636942675159236,0.914543994288819)
--(axis cs:1.27388535031847,0.9132690039486)
--(axis cs:1.91082802547771,0.912473682130933)
--(axis cs:2.54777070063694,0.91171668532972)
--(axis cs:3.18471337579618,0.910513174346484)
--(axis cs:3.82165605095541,0.910486745956676)
--(axis cs:4.45859872611465,0.909330638031585)
--(axis cs:5.09554140127389,0.908380108122003)
--(axis cs:5.73248407643312,0.907876331361229)
--(axis cs:6.36942675159236,0.907608631039617)
--(axis cs:7.00636942675159,0.90675229820739)
--(axis cs:7.64331210191083,0.904702918636459)
--(axis cs:8.28025477707006,0.903761950698985)
--(axis cs:8.9171974522293,0.903332337757373)
--(axis cs:9.55414012738853,0.903413556978852)
--(axis cs:10.1910828025478,0.902376745079955)
--(axis cs:10.828025477707,0.900917792815855)
--(axis cs:11.4649681528662,0.899992118187001)
--(axis cs:12.1019108280255,0.89965127555431)
--(axis cs:12.7388535031847,0.898530093609735)
--(axis cs:13.3757961783439,0.896489815970958)
--(axis cs:14.0127388535032,0.894678675284888)
--(axis cs:14.6496815286624,0.893262070210661)
--(axis cs:15.2866242038217,0.8893930206937)
--(axis cs:15.9235668789809,0.88603942231277)
--(axis cs:16.5605095541401,0.883319558514811)
--(axis cs:17.1974522292994,0.877981809748973)
--(axis cs:17.8343949044586,0.870229757946633)
--(axis cs:18.4713375796178,0.86437049425213)
--(axis cs:19.1082802547771,0.859020887475112)
--(axis cs:19.7452229299363,0.852412417724496)
--(axis cs:20.3821656050955,0.844305748123818)
--(axis cs:21.0191082802548,0.838098163647876)
--(axis cs:21.656050955414,0.821923640186742)
--(axis cs:22.2929936305732,0.810649576414521)
--(axis cs:22.9299363057325,0.806366797517342)
--(axis cs:23.5668789808917,0.791160353588481)
--(axis cs:24.203821656051,0.774712867969632)
--(axis cs:24.8407643312102,0.760582767227399)
--(axis cs:25.4777070063694,0.740326131879431)
--(axis cs:26.1146496815287,0.725880566279895)
--(axis cs:26.7515923566879,0.710909497697245)
--(axis cs:27.3885350318471,0.689262253059715)
--(axis cs:28.0254777070064,0.671665496276066)
--(axis cs:28.6624203821656,0.655561288308494)
--(axis cs:29.2993630573248,0.638552813332677)
--(axis cs:29.9363057324841,0.624449954364922)
--(axis cs:30.5732484076433,0.605080444283221)
--(axis cs:31.2101910828025,0.584658665873681)
--(axis cs:31.8471337579618,0.566970311672754)
--(axis cs:32.484076433121,0.547789075710641)
--(axis cs:33.1210191082803,0.530722898939385)
--(axis cs:33.7579617834395,0.514134060205166)
--(axis cs:34.3949044585987,0.498182240513866)
--(axis cs:35.031847133758,0.477754992264131)
--(axis cs:35.6687898089172,0.460637637873117)
--(axis cs:36.3057324840764,0.439997789935816)
--(axis cs:36.9426751592357,0.422701546775303)
--(axis cs:37.5796178343949,0.401669521941418)
--(axis cs:38.2165605095541,0.388861770363421)
--(axis cs:38.8535031847134,0.380940183543737)
--(axis cs:39.4904458598726,0.361904441363895)
--(axis cs:40.1273885350318,0.344917672432254)
--(axis cs:40.7643312101911,0.338176539769249)
--(axis cs:41.4012738853503,0.325081849023366)
--(axis cs:42.0382165605096,0.311853907787774)
--(axis cs:42.6751592356688,0.301177947363744)
--(axis cs:43.312101910828,0.292138777764443)
--(axis cs:43.9490445859873,0.280363498070856)
--(axis cs:44.5859872611465,0.267569579229341)
--(axis cs:45.2229299363057,0.258806178363873)
--(axis cs:45.859872611465,0.252460829206715)
--(axis cs:46.4968152866242,0.248346111961959)
--(axis cs:47.1337579617834,0.241959203728679)
--(axis cs:47.7707006369427,0.235029511766632)
--(axis cs:48.4076433121019,0.231192171072909)
--(axis cs:49.0445859872611,0.211103899885307)
--(axis cs:49.6815286624204,0.205714275196961)
--(axis cs:50.3184713375796,0.188860587241594)
--(axis cs:50.9554140127388,0.184227105230753)
--(axis cs:51.5923566878981,0.172072095420027)
--(axis cs:52.2292993630573,0.16401803297552)
--(axis cs:52.8662420382166,0.152238397199268)
--(axis cs:53.5031847133758,0.144907361888934)
--(axis cs:54.140127388535,0.135089015426867)
--(axis cs:54.7770700636943,0.132746250772309)
--(axis cs:55.4140127388535,0.130448729598192)
--(axis cs:56.0509554140127,0.123244359519474)
--(axis cs:56.687898089172,0.120326444043019)
--(axis cs:57.3248407643312,0.112997697467456)
--(axis cs:57.9617834394904,0.111439678221811)
--(axis cs:58.5987261146497,0.105769322607969)
--(axis cs:59.2356687898089,0.103709527500994)
--(axis cs:59.8726114649682,0.0934893803229263)
--(axis cs:60.5095541401274,0.0875845362062194)
--(axis cs:61.1464968152866,0.0834553532987249)
--(axis cs:61.7834394904459,0.080201052080455)
--(axis cs:62.4203821656051,0.0754196752371952)
--(axis cs:63.0573248407643,0.0721316198111625)
--(axis cs:63.6942675159236,0.0695380824251963)
--(axis cs:64.3312101910828,0.0653249327763468)
--(axis cs:64.968152866242,0.0608949066445679)
--(axis cs:65.6050955414013,0.0583225624388976)
--(axis cs:66.2420382165605,0.0579958071739419)
--(axis cs:66.8789808917197,0.0581831222015338)
--(axis cs:67.515923566879,0.0574551777396659)
--(axis cs:68.1528662420382,0.0539877703869462)
--(axis cs:68.7898089171974,0.0538910554410246)
--(axis cs:69.4267515923567,0.0522773922459212)
--(axis cs:70.0636942675159,0.0507434560886616)
--(axis cs:70.7006369426752,0.0488883803978708)
--(axis cs:71.3375796178344,0.0482414295798046)
--(axis cs:71.9745222929936,0.0463304868387551)
--(axis cs:72.6114649681529,0.0433099156112432)
--(axis cs:73.2484076433121,0.039737751302345)
--(axis cs:73.8853503184713,0.0405630247963521)
--(axis cs:74.5222929936306,0.043057101132107)
--(axis cs:75.1592356687898,0.0432182396424681)
--(axis cs:75.796178343949,0.0459109183075957)
--(axis cs:76.4331210191083,0.0444247352972516)
--(axis cs:77.0700636942675,0.0415348940712358)
--(axis cs:77.7070063694268,0.0400491335826109)
--(axis cs:78.343949044586,0.0365923801974233)
--(axis cs:78.9808917197452,0.0355843591247854)
--(axis cs:79.6178343949044,0.033418313671992)
--(axis cs:80.2547770700637,0.0339925853095864)
--(axis cs:80.8917197452229,0.0335927580937441)
--(axis cs:81.5286624203822,0.0343280715014677)
--(axis cs:82.1656050955414,0.0311211566736634)
--(axis cs:82.8025477707006,0.0314876307118129)
--(axis cs:83.4394904458599,0.0285214087019133)
--(axis cs:84.0764331210191,0.0274199094133885)
--(axis cs:84.7133757961783,0.0260766998016568)
--(axis cs:85.3503184713376,0.0259044835093717)
--(axis cs:85.9872611464968,0.0247242160499218)
--(axis cs:86.6242038216561,0.0218737789720994)
--(axis cs:87.2611464968153,0.02032431060392)
--(axis cs:87.8980891719745,0.0191600473395907)
--(axis cs:88.5350318471338,0.0163583954537618)
--(axis cs:89.171974522293,0.0143626138236286)
--(axis cs:89.8089171974522,0.0104940431864245)
--(axis cs:90.4458598726115,0.0068945421066566)
--(axis cs:91.0828025477707,0.00435315541521597)
--(axis cs:91.7197452229299,0.00290150521064544)
--(axis cs:92.3566878980892,0.00170887615892349)
--(axis cs:92.9936305732484,0.00134615546693801)
--(axis cs:93.6305732484076,0.000858612187058996)
--(axis cs:94.2675159235669,0.000704443740269983)
--(axis cs:94.9044585987261,0.000646055436557592)
--(axis cs:95.5414012738853,0.000578520005700683)
--(axis cs:96.1783439490446,0.000217360550125136)
--(axis cs:96.8152866242038,0.000110601808702567)
--(axis cs:97.4522292993631,3.52491275116366e-05)
--(axis cs:98.0891719745223,5.17423331208429e-06)
--(axis cs:98.7261146496815,1.76890884050212e-06)
--(axis cs:99.3630573248408,1.66315267071957e-06)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,2.03206387019808e-06)
--(axis cs:98.7261146496815,2.49186128964014e-06)
--(axis cs:98.0891719745223,8.68827347904259e-06)
--(axis cs:97.4522292993631,6.8194349438608e-05)
--(axis cs:96.8152866242038,0.000201367204398877)
--(axis cs:96.1783439490446,0.000331018877887947)
--(axis cs:95.5414012738853,0.000862047956614428)
--(axis cs:94.9044585987261,0.0009476015998869)
--(axis cs:94.2675159235669,0.0010217620627607)
--(axis cs:93.6305732484076,0.00120720210625645)
--(axis cs:92.9936305732484,0.00189392599300831)
--(axis cs:92.3566878980892,0.00243478687117381)
--(axis cs:91.7197452229299,0.00397853209081503)
--(axis cs:91.0828025477707,0.00583989403984054)
--(axis cs:90.4458598726115,0.00920246639803458)
--(axis cs:89.8089171974522,0.0134207550891362)
--(axis cs:89.171974522293,0.0176616492608535)
--(axis cs:88.5350318471338,0.019522770110215)
--(axis cs:87.8980891719745,0.0224871072153592)
--(axis cs:87.2611464968153,0.0236928898194622)
--(axis cs:86.6242038216561,0.0253618369257478)
--(axis cs:85.9872611464968,0.0282075338368364)
--(axis cs:85.3503184713376,0.02943994955074)
--(axis cs:84.7133757961783,0.0296504774772713)
--(axis cs:84.0764331210191,0.0311536757936726)
--(axis cs:83.4394904458599,0.0322182110724523)
--(axis cs:82.8025477707006,0.0351410867389345)
--(axis cs:82.1656050955414,0.0347000272406934)
--(axis cs:81.5286624203822,0.0380331508694035)
--(axis cs:80.8917197452229,0.037192666383197)
--(axis cs:80.2547770700637,0.0379100514595486)
--(axis cs:79.6178343949044,0.0377666129708955)
--(axis cs:78.9808917197452,0.0400811296358259)
--(axis cs:78.343949044586,0.0413205572596395)
--(axis cs:77.7070063694268,0.0447697369550683)
--(axis cs:77.0700636942675,0.0461645399443425)
--(axis cs:76.4331210191083,0.049042895921732)
--(axis cs:75.796178343949,0.0503417299970229)
--(axis cs:75.1592356687898,0.0477854973366562)
--(axis cs:74.5222929936306,0.0475896102113449)
--(axis cs:73.8853503184713,0.0449784421374552)
--(axis cs:73.2484076433121,0.0443237837369792)
--(axis cs:72.6114649681529,0.0479437143179722)
--(axis cs:71.9745222929936,0.0507830586001085)
--(axis cs:71.3375796178344,0.0528485827564829)
--(axis cs:70.7006369426752,0.0537315766916947)
--(axis cs:70.0636942675159,0.0555918811499184)
--(axis cs:69.4267515923567,0.0573433266848699)
--(axis cs:68.7898089171974,0.058984993236017)
--(axis cs:68.1528662420382,0.0595544310316747)
--(axis cs:67.515923566879,0.0629701650222053)
--(axis cs:66.8789808917197,0.0640175019237857)
--(axis cs:66.2420382165605,0.0638127675275979)
--(axis cs:65.6050955414013,0.0641922277821761)
--(axis cs:64.968152866242,0.0669886983296247)
--(axis cs:64.3312101910828,0.0720187192077165)
--(axis cs:63.6942675159236,0.0762628179352113)
--(axis cs:63.0573248407643,0.079097750047839)
--(axis cs:62.4203821656051,0.08218848415908)
--(axis cs:61.7834394904459,0.0871383234449331)
--(axis cs:61.1464968152866,0.0905754023076981)
--(axis cs:60.5095541401274,0.0949742639928554)
--(axis cs:59.8726114649682,0.101460057026258)
--(axis cs:59.2356687898089,0.111792678263509)
--(axis cs:58.5987261146497,0.113930789628323)
--(axis cs:57.9617834394904,0.119553870424394)
--(axis cs:57.3248407643312,0.121610089833344)
--(axis cs:56.687898089172,0.129327070713431)
--(axis cs:56.0509554140127,0.13206692819058)
--(axis cs:55.4140127388535,0.139679146612261)
--(axis cs:54.7770700636943,0.142312472349027)
--(axis cs:54.140127388535,0.145048768577589)
--(axis cs:53.5031847133758,0.15537531217021)
--(axis cs:52.8662420382166,0.162716547753055)
--(axis cs:52.2292993630573,0.174826090219468)
--(axis cs:51.5923566878981,0.182689236744593)
--(axis cs:50.9554140127388,0.195025423146942)
--(axis cs:50.3184713375796,0.199837963102727)
--(axis cs:49.6815286624204,0.216798455486487)
--(axis cs:49.0445859872611,0.222308890463943)
--(axis cs:48.4076433121019,0.242223142218968)
--(axis cs:47.7707006369427,0.245873161801404)
--(axis cs:47.1337579617834,0.253088534046579)
--(axis cs:46.4968152866242,0.259044024972329)
--(axis cs:45.859872611465,0.263076110627192)
--(axis cs:45.2229299363057,0.269481584363714)
--(axis cs:44.5859872611465,0.278104213136052)
--(axis cs:43.9490445859873,0.291142592604132)
--(axis cs:43.312101910828,0.303302991846387)
--(axis cs:42.6751592356688,0.312540142011133)
--(axis cs:42.0382165605096,0.323623242012516)
--(axis cs:41.4012738853503,0.337130144518566)
--(axis cs:40.7643312101911,0.350466167235689)
--(axis cs:40.1273885350318,0.357489611085769)
--(axis cs:39.4904458598726,0.375289202163022)
--(axis cs:38.8535031847134,0.394841847814002)
--(axis cs:38.2165605095541,0.402941462997804)
--(axis cs:37.5796178343949,0.415981437567119)
--(axis cs:36.9426751592357,0.437370484179022)
--(axis cs:36.3057324840764,0.455022271426777)
--(axis cs:35.6687898089172,0.47602134669836)
--(axis cs:35.031847133758,0.493275517272809)
--(axis cs:34.3949044585987,0.513655041817242)
--(axis cs:33.7579617834395,0.529662161750906)
--(axis cs:33.1210191082803,0.545967929407524)
--(axis cs:32.484076433121,0.562908930865636)
--(axis cs:31.8471337579618,0.582452264401604)
--(axis cs:31.2101910828025,0.599900557896512)
--(axis cs:30.5732484076433,0.620258955637556)
--(axis cs:29.9363057324841,0.639691898611978)
--(axis cs:29.2993630573248,0.653718636116722)
--(axis cs:28.6624203821656,0.670993707690465)
--(axis cs:28.0254777070064,0.687272765311252)
--(axis cs:27.3885350318471,0.704639010867031)
--(axis cs:26.7515923566879,0.726112250637128)
--(axis cs:26.1146496815287,0.740612262010462)
--(axis cs:25.4777070063694,0.754698203987916)
--(axis cs:24.8407643312102,0.774901525929443)
--(axis cs:24.203821656051,0.788609280007091)
--(axis cs:23.5668789808917,0.804591625890693)
--(axis cs:22.9299363057325,0.819132415504634)
--(axis cs:22.2929936305732,0.823375401417202)
--(axis cs:21.656050955414,0.833957689774234)
--(axis cs:21.0191082802548,0.84911875786748)
--(axis cs:20.3821656050955,0.854989568491207)
--(axis cs:19.7452229299363,0.862557237775822)
--(axis cs:19.1082802547771,0.868507853625575)
--(axis cs:18.4713375796178,0.873404172307286)
--(axis cs:17.8343949044586,0.878757832207797)
--(axis cs:17.1974522292994,0.885663025275052)
--(axis cs:16.5605095541401,0.890430781483121)
--(axis cs:15.9235668789809,0.892782128559174)
--(axis cs:15.2866242038217,0.895700378024463)
--(axis cs:14.6496815286624,0.899107573421312)
--(axis cs:14.0127388535032,0.900333442865592)
--(axis cs:13.3757961783439,0.90175727915605)
--(axis cs:12.7388535031847,0.903267633396753)
--(axis cs:12.1019108280255,0.904255898849702)
--(axis cs:11.4649681528662,0.904529809718734)
--(axis cs:10.828025477707,0.905288695110101)
--(axis cs:10.1910828025478,0.906544474467091)
--(axis cs:9.55414012738853,0.907424814369948)
--(axis cs:8.9171974522293,0.907233210235801)
--(axis cs:8.28025477707006,0.907618378344037)
--(axis cs:7.64331210191083,0.908335756051973)
--(axis cs:7.00636942675159,0.909998764638188)
--(axis cs:6.36942675159236,0.910668115324228)
--(axis cs:5.73248407643312,0.910863086363781)
--(axis cs:5.09554140127389,0.911202975038684)
--(axis cs:4.45859872611465,0.911864208260907)
--(axis cs:3.82165605095541,0.91273411173481)
--(axis cs:3.18471337579618,0.91289780995336)
--(axis cs:2.54777070063694,0.913676979355824)
--(axis cs:1.91082802547771,0.914296298075221)
--(axis cs:1.27388535031847,0.915095188333716)
--(axis cs:0.636942675159236,0.915954489625598)
--(axis cs:0,0.9160976908346)
--cycle;


==> img/mnist/mnist_rate_distortion_pgd_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color9, mark=square*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color9, thin}]
table {%
0 0.915482513338793
0.636942675159236 0.915586642201524
1.27388535031847 0.915294179137563
1.91082802547771 0.914735921618994
2.54777070063694 0.913794182377169
3.18471337579618 0.912586117306491
3.82165605095541 0.909745753251627
4.45859872611465 0.905855460936436
5.09554140127389 0.901529539054027
5.73248407643312 0.895467470416625
6.36942675159236 0.888858944697131
7.00636942675159 0.882854461850366
7.64331210191083 0.872795478440239
8.28025477707006 0.858735994305462
8.9171974522293 0.838762952770048
9.55414012738853 0.822531280145049
10.1910828025478 0.807314713741362
10.828025477707 0.787232169253402
11.4649681528662 0.763327411150094
12.1019108280255 0.744848195545492
12.7388535031847 0.728581657366594
13.3757961783439 0.710163011935074
14.0127388535032 0.687064077956602
14.6496815286624 0.670478002284653
15.2866242038217 0.654361410850543
15.9235668789809 0.635557308627758
16.5605095541401 0.616465349419159
17.1974522292994 0.598718126174063
17.8343949044586 0.584575162442634
18.4713375796178 0.558218109721201
19.1082802547771 0.53626074974658
19.7452229299363 0.521600556536578
20.3821656050955 0.506623270209529
21.0191082802548 0.488217324225116
21.656050955414 0.471992501065251
22.2929936305732 0.45623582569795
22.9299363057325 0.445017878560757
23.5668789808917 0.436989047564275
24.203821656051 0.42127372790128
24.8407643312102 0.406637684964226
25.4777070063694 0.388358115697629
26.1146496815287 0.375820760131464
26.7515923566879 0.366969451077166
27.3885350318471 0.353228710231488
28.0254777070064 0.339971710923273
28.6624203821656 0.329527526286256
29.2993630573248 0.31386782873742
29.9363057324841 0.30411914357639
30.5732484076433 0.295936265189084
31.2101910828025 0.289060278560064
31.8471337579618 0.285323642795411
32.484076433121 0.269161402113459
33.1210191082803 0.266974187642991
33.7579617834395 0.26425965217768
34.3949044585987 0.263419135485165
35.031847133758 0.263870467198067
35.6687898089172 0.26369845991263
36.3057324840764 0.2579008781429
36.9426751592357 0.262218924120552
37.5796178343949 0.256817193929646
38.2165605095541 0.258892705163253
38.8535031847134 0.255323780794115
39.4904458598726 0.254196584276326
40.1273885350318 0.24995889753994
40.7643312101911 0.247319702073081
41.4012738853503 0.240057659425895
42.0382165605096 0.233912247084041
42.6751592356688 0.220692077238985
43.312101910828 0.221522986942864
43.9490445859873 0.218216678345215
44.5859872611465 0.217442011512528
45.2229299363057 0.20626845861374
45.859872611465 0.198995294961352
46.4968152866242 0.191015850242249
47.1337579617834 0.186150592497125
47.7707006369427 0.180921542657696
48.4076433121019 0.177969582138766
49.0445859872611 0.172439874701878
49.6815286624204 0.165753372129065
50.3184713375796 0.158302534971162
50.9554140127388 0.152416410302121
51.5923566878981 0.146545215681198
52.2292993630573 0.140682072428732
52.8662420382166 0.138600029832735
53.5031847133758 0.141821693279471
54.140127388535 0.134146231609513
54.7770700636943 0.130969474100268
55.4140127388535 0.125498263761859
56.0509554140127 0.120405579546196
56.687898089172 0.118137432157618
57.3248407643312 0.113403830641765
57.9617834394904 0.11395529789365
58.5987261146497 0.107524318220223
59.2356687898089 0.102847247179133
59.8726114649682 0.102017982405311
60.5095541401274 0.103026618358668
61.1464968152866 0.102705522381246
61.7834394904459 0.0998280493884619
62.4203821656051 0.0934649508230455
63.0573248407643 0.0917858629702335
63.6942675159236 0.0864928142124522
64.3312101910828 0.0798606653044757
64.968152866242 0.0763222968255561
65.6050955414013 0.0728350011416434
66.2420382165605 0.0681443309633137
66.8789808917197 0.0664915802255105
67.515923566879 0.0675657788888098
68.1528662420382 0.0617191869262139
68.7898089171974 0.0622338650898481
69.4267515923567 0.0609489680022129
70.0636942675159 0.0570527658754357
70.7006369426752 0.056055974886472
71.3375796178344 0.0560857334854768
71.9745222929936 0.0588424303381008
72.6114649681529 0.0566597547769199
73.2484076433121 0.0580100022886666
73.8853503184713 0.056134877877694
74.5222929936306 0.0541330622055567
75.1592356687898 0.0532492492191251
75.796178343949 0.0529574819092667
76.4331210191083 0.0518833455867302
77.0700636942675 0.0485912724327337
77.7070063694268 0.04752527579368
78.343949044586 0.0428991272454436
78.9808917197452 0.0403285482184698
79.6178343949044 0.0357231178159255
80.2547770700637 0.0369004641787533
80.8917197452229 0.035370630107109
81.5286624203822 0.035492791334929
82.1656050955414 0.0347111438607796
82.8025477707006 0.0318726643896026
83.4394904458599 0.0293023191873842
84.0764331210191 0.0289043436513567
84.7133757961783 0.0249077153775263
85.3503184713376 0.0215289707390896
85.9872611464968 0.0210553256911013
86.6242038216561 0.0187925301175501
87.2611464968153 0.0159959206017738
87.8980891719745 0.0145069014823283
88.5350318471338 0.0118649496677694
89.171974522293 0.00765326859801469
89.8089171974522 0.00760667379617917
90.4458598726115 0.00879949929314842
91.0828025477707 0.00809623446842139
91.7197452229299 0.00711897660301668
92.3566878980892 0.00581638360374099
92.9936305732484 0.00617510068369739
93.6305732484076 0.00291071519102507
94.2675159235669 0.00227805753903512
94.9044585987261 0.00243322976337433
95.5414012738853 0.00167722714744456
96.1783439490446 0.00118154507081371
96.8152866242038 0.00119126895916742
97.4522292993631 0.00070973187072471
98.0891719745223 0.000274161314355554
98.7261146496815 4.8667736923243e-05
99.3630573248408 1.2464693247114e-05
100 0
};
\path [fill=color9, fill opacity=0.25] 
(axis cs:0,0.916088066468976)
--(axis cs:0,0.91487696020861)
--(axis cs:0.636942675159236,0.915052575635463)
--(axis cs:1.27388535031847,0.914668656193886)
--(axis cs:1.91082802547771,0.914010063450101)
--(axis cs:2.54777070063694,0.912875431062388)
--(axis cs:3.18471337579618,0.911534284101732)
--(axis cs:3.82165605095541,0.908242523324137)
--(axis cs:4.45859872611465,0.903855771345825)
--(axis cs:5.09554140127389,0.899103480739103)
--(axis cs:5.73248407643312,0.892483517294353)
--(axis cs:6.36942675159236,0.885379034307951)
--(axis cs:7.00636942675159,0.878992477869113)
--(axis cs:7.64331210191083,0.868211664001693)
--(axis cs:8.28025477707006,0.853517573452925)
--(axis cs:8.9171974522293,0.832846664569517)
--(axis cs:9.55414012738853,0.816105993113187)
--(axis cs:10.1910828025478,0.800533687836779)
--(axis cs:10.828025477707,0.780176517014705)
--(axis cs:11.4649681528662,0.755845306822456)
--(axis cs:12.1019108280255,0.737216682736715)
--(axis cs:12.7388535031847,0.720760995836924)
--(axis cs:13.3757961783439,0.702285907436768)
--(axis cs:14.0127388535032,0.679048874072619)
--(axis cs:14.6496815286624,0.662353912332345)
--(axis cs:15.2866242038217,0.646006612354327)
--(axis cs:15.9235668789809,0.627120450814049)
--(axis cs:16.5605095541401,0.607959177739695)
--(axis cs:17.1974522292994,0.590063653889828)
--(axis cs:17.8343949044586,0.575845280774586)
--(axis cs:18.4713375796178,0.549492723746134)
--(axis cs:19.1082802547771,0.527545086264449)
--(axis cs:19.7452229299363,0.512994293085073)
--(axis cs:20.3821656050955,0.498066507792912)
--(axis cs:21.0191082802548,0.479661715630864)
--(axis cs:21.656050955414,0.463428593172386)
--(axis cs:22.2929936305732,0.447799655348)
--(axis cs:22.9299363057325,0.436487996481193)
--(axis cs:23.5668789808917,0.428500612182125)
--(axis cs:24.203821656051,0.412898133146532)
--(axis cs:24.8407643312102,0.398387250391193)
--(axis cs:25.4777070063694,0.380145268523541)
--(axis cs:26.1146496815287,0.367644783007162)
--(axis cs:26.7515923566879,0.358888474752299)
--(axis cs:27.3885350318471,0.345242277712078)
--(axis cs:28.0254777070064,0.331729410309785)
--(axis cs:28.6624203821656,0.321434455366168)
--(axis cs:29.2993630573248,0.305916042939301)
--(axis cs:29.9363057324841,0.29613769830049)
--(axis cs:30.5732484076433,0.287865911603484)
--(axis cs:31.2101910828025,0.281069878517971)
--(axis cs:31.8471337579618,0.277367589964591)
--(axis cs:32.484076433121,0.261327613708001)
--(axis cs:33.1210191082803,0.258968816405065)
--(axis cs:33.7579617834395,0.256321616371059)
--(axis cs:34.3949044585987,0.255548175024695)
--(axis cs:35.031847133758,0.25623783168778)
--(axis cs:35.6687898089172,0.255999973778828)
--(axis cs:36.3057324840764,0.250465051204078)
--(axis cs:36.9426751592357,0.255034476407007)
--(axis cs:37.5796178343949,0.249615551385916)
--(axis cs:38.2165605095541,0.251567338741937)
--(axis cs:38.8535031847134,0.248086827749136)
--(axis cs:39.4904458598726,0.246948895854602)
--(axis cs:40.1273885350318,0.242888869811826)
--(axis cs:40.7643312101911,0.240537753590459)
--(axis cs:41.4012738853503,0.233421514796125)
--(axis cs:42.0382165605096,0.227391294090537)
--(axis cs:42.6751592356688,0.214211426938394)
--(axis cs:43.312101910828,0.215210134931261)
--(axis cs:43.9490445859873,0.211970973753572)
--(axis cs:44.5859872611465,0.211505501661426)
--(axis cs:45.2229299363057,0.200479839042317)
--(axis cs:45.859872611465,0.193336203783612)
--(axis cs:46.4968152866242,0.185349914328194)
--(axis cs:47.1337579617834,0.180592298894265)
--(axis cs:47.7707006369427,0.175466533316254)
--(axis cs:48.4076433121019,0.172443002089404)
--(axis cs:49.0445859872611,0.16689136100862)
--(axis cs:49.6815286624204,0.160138759693268)
--(axis cs:50.3184713375796,0.152749512771246)
--(axis cs:50.9554140127388,0.14703917258573)
--(axis cs:51.5923566878981,0.141370269883243)
--(axis cs:52.2292993630573,0.135708935951022)
--(axis cs:52.8662420382166,0.133678845070813)
--(axis cs:53.5031847133758,0.136756948774132)
--(axis cs:54.140127388535,0.129346579016447)
--(axis cs:54.7770700636943,0.126086087440685)
--(axis cs:55.4140127388535,0.121027124351838)
--(axis cs:56.0509554140127,0.115839403017767)
--(axis cs:56.687898089172,0.113648080031904)
--(axis cs:57.3248407643312,0.109064195323431)
--(axis cs:57.9617834394904,0.109863224314464)
--(axis cs:58.5987261146497,0.103492233424255)
--(axis cs:59.2356687898089,0.0990647814401302)
--(axis cs:59.8726114649682,0.0983040439089021)
--(axis cs:60.5095541401274,0.0992057481109778)
--(axis cs:61.1464968152866,0.0989562221621501)
--(axis cs:61.7834394904459,0.0960909309726599)
--(axis cs:62.4203821656051,0.0895958512696366)
--(axis cs:63.0573248407643,0.0878212524752601)
--(axis cs:63.6942675159236,0.0825256281939323)
--(axis cs:64.3312101910828,0.0760875175251426)
--(axis cs:64.968152866242,0.0725187267940142)
--(axis cs:65.6050955414013,0.0690080639387384)
--(axis cs:66.2420382165605,0.0643409213202921)
--(axis cs:66.8789808917197,0.0626303955916724)
--(axis cs:67.515923566879,0.0638025031082058)
--(axis cs:68.1528662420382,0.0583466469694426)
--(axis cs:68.7898089171974,0.0589463197878816)
--(axis cs:69.4267515923567,0.0576322639349331)
--(axis cs:70.0636942675159,0.0539332578626167)
--(axis cs:70.7006369426752,0.0529738482791591)
--(axis cs:71.3375796178344,0.0530327637502723)
--(axis cs:71.9745222929936,0.0558949845036446)
--(axis cs:72.6114649681529,0.0536920883010951)
--(axis cs:73.2484076433121,0.055261536819102)
--(axis cs:73.8853503184713,0.0533183002510465)
--(axis cs:74.5222929936306,0.0513382728733133)
--(axis cs:75.1592356687898,0.0505770821786796)
--(axis cs:75.796178343949,0.0502953216358439)
--(axis cs:76.4331210191083,0.0492320639406553)
--(axis cs:77.0700636942675,0.0461307485891904)
--(axis cs:77.7070063694268,0.0450587418937209)
--(axis cs:78.343949044586,0.040494479476199)
--(axis cs:78.9808917197452,0.0381454227476615)
--(axis cs:79.6178343949044,0.0335601439499008)
--(axis cs:80.2547770700637,0.0347945438996169)
--(axis cs:80.8917197452229,0.033183396439486)
--(axis cs:81.5286624203822,0.033356996100987)
--(axis cs:82.1656050955414,0.0324824210213833)
--(axis cs:82.8025477707006,0.0298161249986936)
--(axis cs:83.4394904458599,0.0273040580619067)
--(axis cs:84.0764331210191,0.0267386340123544)
--(axis cs:84.7133757961783,0.0229732821748858)
--(axis cs:85.3503184713376,0.0195220736531206)
--(axis cs:85.9872611464968,0.0189045678443521)
--(axis cs:86.6242038216561,0.0168792106210767)
--(axis cs:87.2611464968153,0.0141296716296724)
--(axis cs:87.8980891719745,0.0129155618627851)
--(axis cs:88.5350318471338,0.0104227700093417)
--(axis cs:89.171974522293,0.00632955957423608)
--(axis cs:89.8089171974522,0.00636494873087046)
--(axis cs:90.4458598726115,0.00759684664386832)
--(axis cs:91.0828025477707,0.00693880735275275)
--(axis cs:91.7197452229299,0.00598708227223686)
--(axis cs:92.3566878980892,0.0047662759283486)
--(axis cs:92.9936305732484,0.00510388820898321)
--(axis cs:93.6305732484076,0.00230985412094884)
--(axis cs:94.2675159235669,0.00171312533002055)
--(axis cs:94.9044585987261,0.00190136679782179)
--(axis cs:95.5414012738853,0.00122232980517897)
--(axis cs:96.1783439490446,0.000831995537076516)
--(axis cs:96.8152866242038,0.00084975035413301)
--(axis cs:97.4522292993631,0.000473246980261375)
--(axis cs:98.0891719745223,0.000182408297602458)
--(axis cs:98.7261146496815,3.31460496041338e-05)
--(axis cs:99.3630573248408,8.4452838234844e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,1.64841026707435e-05)
--(axis cs:98.7261146496815,6.41894242423522e-05)
--(axis cs:98.0891719745223,0.000365914331108651)
--(axis cs:97.4522292993631,0.000946216761188045)
--(axis cs:96.8152866242038,0.00153278756420183)
--(axis cs:96.1783439490446,0.00153109460455091)
--(axis cs:95.5414012738853,0.00213212448971015)
--(axis cs:94.9044585987261,0.00296509272892687)
--(axis cs:94.2675159235669,0.00284298974804969)
--(axis cs:93.6305732484076,0.00351157626110129)
--(axis cs:92.9936305732484,0.00724631315841156)
--(axis cs:92.3566878980892,0.00686649127913337)
--(axis cs:91.7197452229299,0.0082508709337965)
--(axis cs:91.0828025477707,0.00925366158409003)
--(axis cs:90.4458598726115,0.0100021519424285)
--(axis cs:89.8089171974522,0.00884839886148788)
--(axis cs:89.171974522293,0.0089769776217933)
--(axis cs:88.5350318471338,0.013307129326197)
--(axis cs:87.8980891719745,0.0160982411018715)
--(axis cs:87.2611464968153,0.0178621695738752)
--(axis cs:86.6242038216561,0.0207058496140234)
--(axis cs:85.9872611464968,0.0232060835378505)
--(axis cs:85.3503184713376,0.0235358678250585)
--(axis cs:84.7133757961783,0.0268421485801668)
--(axis cs:84.0764331210191,0.031070053290359)
--(axis cs:83.4394904458599,0.0313005803128617)
--(axis cs:82.8025477707006,0.0339292037805115)
--(axis cs:82.1656050955414,0.036939866700176)
--(axis cs:81.5286624203822,0.0376285865688711)
--(axis cs:80.8917197452229,0.0375578637747319)
--(axis cs:80.2547770700637,0.0390063844578897)
--(axis cs:79.6178343949044,0.0378860916819503)
--(axis cs:78.9808917197452,0.0425116736892781)
--(axis cs:78.343949044586,0.0453037750146881)
--(axis cs:77.7070063694268,0.0499918096936391)
--(axis cs:77.0700636942675,0.0510517962762769)
--(axis cs:76.4331210191083,0.0545346272328051)
--(axis cs:75.796178343949,0.0556196421826895)
--(axis cs:75.1592356687898,0.0559214162595707)
--(axis cs:74.5222929936306,0.0569278515378)
--(axis cs:73.8853503184713,0.0589514555043415)
--(axis cs:73.2484076433121,0.0607584677582312)
--(axis cs:72.6114649681529,0.0596274212527446)
--(axis cs:71.9745222929936,0.061789876172557)
--(axis cs:71.3375796178344,0.0591387032206812)
--(axis cs:70.7006369426752,0.0591381014937849)
--(axis cs:70.0636942675159,0.0601722738882548)
--(axis cs:69.4267515923567,0.0642656720694927)
--(axis cs:68.7898089171974,0.0655214103918147)
--(axis cs:68.1528662420382,0.0650917268829853)
--(axis cs:67.515923566879,0.0713290546694137)
--(axis cs:66.8789808917197,0.0703527648593486)
--(axis cs:66.2420382165605,0.0719477406063353)
--(axis cs:65.6050955414013,0.0766619383445483)
--(axis cs:64.968152866242,0.0801258668570981)
--(axis cs:64.3312101910828,0.0836338130838087)
--(axis cs:63.6942675159236,0.090460000230972)
--(axis cs:63.0573248407643,0.0957504734652069)
--(axis cs:62.4203821656051,0.0973340503764544)
--(axis cs:61.7834394904459,0.103565167804264)
--(axis cs:61.1464968152866,0.106454822600342)
--(axis cs:60.5095541401274,0.106847488606358)
--(axis cs:59.8726114649682,0.10573192090172)
--(axis cs:59.2356687898089,0.106629712918136)
--(axis cs:58.5987261146497,0.111556403016191)
--(axis cs:57.9617834394904,0.118047371472836)
--(axis cs:57.3248407643312,0.117743465960099)
--(axis cs:56.687898089172,0.122626784283333)
--(axis cs:56.0509554140127,0.124971756074626)
--(axis cs:55.4140127388535,0.129969403171879)
--(axis cs:54.7770700636943,0.13585286075985)
--(axis cs:54.140127388535,0.138945884202578)
--(axis cs:53.5031847133758,0.146886437784809)
--(axis cs:52.8662420382166,0.143521214594657)
--(axis cs:52.2292993630573,0.145655208906442)
--(axis cs:51.5923566878981,0.151720161479153)
--(axis cs:50.9554140127388,0.157793648018511)
--(axis cs:50.3184713375796,0.163855557171078)
--(axis cs:49.6815286624204,0.171367984564863)
--(axis cs:49.0445859872611,0.177988388395136)
--(axis cs:48.4076433121019,0.183496162188128)
--(axis cs:47.7707006369427,0.186376551999138)
--(axis cs:47.1337579617834,0.191708886099984)
--(axis cs:46.4968152866242,0.196681786156304)
--(axis cs:45.859872611465,0.204654386139093)
--(axis cs:45.2229299363057,0.212057078185164)
--(axis cs:44.5859872611465,0.223378521363629)
--(axis cs:43.9490445859873,0.224462382936859)
--(axis cs:43.312101910828,0.227835838954466)
--(axis cs:42.6751592356688,0.227172727539576)
--(axis cs:42.0382165605096,0.240433200077545)
--(axis cs:41.4012738853503,0.246693804055664)
--(axis cs:40.7643312101911,0.254101650555703)
--(axis cs:40.1273885350318,0.257028925268055)
--(axis cs:39.4904458598726,0.261444272698049)
--(axis cs:38.8535031847134,0.262560733839094)
--(axis cs:38.2165605095541,0.266218071584568)
--(axis cs:37.5796178343949,0.264018836473376)
--(axis cs:36.9426751592357,0.269403371834098)
--(axis cs:36.3057324840764,0.265336705081723)
--(axis cs:35.6687898089172,0.271396946046432)
--(axis cs:35.031847133758,0.271503102708354)
--(axis cs:34.3949044585987,0.271290095945634)
--(axis cs:33.7579617834395,0.2721976879843)
--(axis cs:33.1210191082803,0.274979558880916)
--(axis cs:32.484076433121,0.276995190518917)
--(axis cs:31.8471337579618,0.293279695626231)
--(axis cs:31.2101910828025,0.297050678602157)
--(axis cs:30.5732484076433,0.304006618774685)
--(axis cs:29.9363057324841,0.312100588852291)
--(axis cs:29.2993630573248,0.32181961453554)
--(axis cs:28.6624203821656,0.337620597206344)
--(axis cs:28.0254777070064,0.348214011536762)
--(axis cs:27.3885350318471,0.361215142750897)
--(axis cs:26.7515923566879,0.375050427402033)
--(axis cs:26.1146496815287,0.383996737255766)
--(axis cs:25.4777070063694,0.396570962871716)
--(axis cs:24.8407643312102,0.414888119537259)
--(axis cs:24.203821656051,0.429649322656028)
--(axis cs:23.5668789808917,0.445477482946425)
--(axis cs:22.9299363057325,0.453547760640321)
--(axis cs:22.2929936305732,0.464671996047899)
--(axis cs:21.656050955414,0.480556408958117)
--(axis cs:21.0191082802548,0.496772932819367)
--(axis cs:20.3821656050955,0.515180032626147)
--(axis cs:19.7452229299363,0.530206819988083)
--(axis cs:19.1082802547771,0.54497641322871)
--(axis cs:18.4713375796178,0.566943495696269)
--(axis cs:17.8343949044586,0.593305044110682)
--(axis cs:17.1974522292994,0.607372598458297)
--(axis cs:16.5605095541401,0.624971521098623)
--(axis cs:15.9235668789809,0.643994166441467)
--(axis cs:15.2866242038217,0.662716209346758)
--(axis cs:14.6496815286624,0.678602092236962)
--(axis cs:14.0127388535032,0.695079281840585)
--(axis cs:13.3757961783439,0.71804011643338)
--(axis cs:12.7388535031847,0.736402318896264)
--(axis cs:12.1019108280255,0.752479708354268)
--(axis cs:11.4649681528662,0.770809515477732)
--(axis cs:10.828025477707,0.7942878214921)
--(axis cs:10.1910828025478,0.814095739645944)
--(axis cs:9.55414012738853,0.828956567176911)
--(axis cs:8.9171974522293,0.84467924097058)
--(axis cs:8.28025477707006,0.863954415157998)
--(axis cs:7.64331210191083,0.877379292878785)
--(axis cs:7.00636942675159,0.886716445831618)
--(axis cs:6.36942675159236,0.892338855086311)
--(axis cs:5.73248407643312,0.898451423538897)
--(axis cs:5.09554140127389,0.903955597368951)
--(axis cs:4.45859872611465,0.907855150527048)
--(axis cs:3.82165605095541,0.911248983179118)
--(axis cs:3.18471337579618,0.91363795051125)
--(axis cs:2.54777070063694,0.91471293369195)
--(axis cs:1.91082802547771,0.915461779787887)
--(axis cs:1.27388535031847,0.91591970208124)
--(axis cs:0.636942675159236,0.916120708767585)
--(axis cs:0,0.916088066468976)
--cycle;


==> img/mnist/mnist_rate_distortion_sensitivity.tex <==
\addplot [line width=0.5, opacity=0.7, color6, mark=square, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color6, thin}]
table [row sep=\\]{%
0	0.915386432704981 \\
0.636942675159236	0.915466319646221 \\
1.27388535031847	0.91549818058731 \\
1.91082802547771	0.915555029558018 \\
2.54777070063694	0.915076629936229 \\
3.18471337579618	0.915278368736617 \\
3.82165605095541	0.915005862211692 \\
4.45859872611465	0.914483152933535 \\
5.09554140127389	0.914100724450545 \\
5.73248407643312	0.913761115182424 \\
6.36942675159236	0.91344562877086 \\
7.00636942675159	0.913338116555242 \\
7.64331210191083	0.912652540892595 \\
8.28025477707006	0.912225347377826 \\
8.9171974522293	0.911799258133979 \\
9.55414012738853	0.910638000442414 \\
10.1910828025478	0.909425395313883 \\
10.828025477707	0.909257432196755 \\
11.4649681528662	0.908682941277511 \\
12.1019108280255	0.908899197051069 \\
12.7388535031847	0.908554548194516 \\
13.3757961783439	0.908262228908716 \\
14.0127388535032	0.90582827428123 \\
14.6496815286624	0.905798189942725 \\
15.2866242038217	0.904927678613458 \\
15.9235668789809	0.904403088998515 \\
16.5605095541401	0.901595406763372 \\
17.1974522292994	0.901428864886984 \\
17.8343949044586	0.898817445544992 \\
18.4713375796178	0.898889780250611 \\
19.1082802547771	0.896749260385986 \\
19.7452229299363	0.894918381987372 \\
20.3821656050955	0.893950137851061 \\
21.0191082802548	0.890967610251246 \\
21.656050955414	0.887147798075166 \\
22.2929936305732	0.885304074952437 \\
22.9299363057325	0.883106769704609 \\
23.5668789808917	0.881922416862508 \\
24.203821656051	0.881011985723744 \\
24.8407643312102	0.881238057668961 \\
25.4777070063694	0.880745374709368 \\
26.1146496815287	0.877905310931965 \\
26.7515923566879	0.874024061953824 \\
27.3885350318471	0.867598244003893 \\
28.0254777070064	0.865775969330934 \\
28.6624203821656	0.86244084664766 \\
29.2993630573248	0.859343958915852 \\
29.9363057324841	0.857392861582048 \\
30.5732484076433	0.851136082220764 \\
31.2101910828025	0.846299592205396 \\
31.8471337579618	0.841446217759658 \\
32.484076433121	0.840058428849297 \\
33.1210191082803	0.835568735457055 \\
33.7579617834395	0.829392373417941 \\
34.3949044585987	0.823987642071006 \\
35.031847133758	0.820336939377012 \\
35.6687898089172	0.815725860441016 \\
36.3057324840764	0.809963920412556 \\
36.9426751592357	0.807752653463977 \\
37.5796178343949	0.802806472606317 \\
38.2165605095541	0.795967407597345 \\
38.8535031847134	0.788448351820989 \\
39.4904458598726	0.778853720513725 \\
40.1273885350318	0.773964728133178 \\
40.7643312101911	0.768326821368537 \\
41.4012738853503	0.759749110558842 \\
42.0382165605096	0.752544532035354 \\
42.6751592356688	0.744237631713368 \\
43.312101910828	0.736878169940956 \\
43.9490445859873	0.732240374619441 \\
44.5859872611465	0.727253433867245 \\
45.2229299363057	0.713394516589205 \\
45.859872611465	0.70254343819528 \\
46.4968152866242	0.699498279631425 \\
47.1337579617834	0.694387494108651 \\
47.7707006369427	0.689731387166375 \\
48.4076433121019	0.680647887570158 \\
49.0445859872611	0.673526439220113 \\
49.6815286624204	0.66038671536995 \\
50.3184713375796	0.654243150142174 \\
50.9554140127388	0.648636952024754 \\
51.5923566878981	0.640899885162562 \\
52.2292993630573	0.637690674478672 \\
52.8662420382166	0.62719499698409 \\
53.5031847133758	0.61978485327626 \\
54.140127388535	0.610478158480723 \\
54.7770700636943	0.605165536457171 \\
55.4140127388535	0.600073247727423 \\
56.0509554140127	0.589707402973481 \\
56.687898089172	0.58030597992245 \\
57.3248407643312	0.568950393085015 \\
57.9617834394904	0.566554158041126 \\
58.5987261146497	0.55560384068518 \\
59.2356687898089	0.544793832806326 \\
59.8726114649682	0.533672458653555 \\
60.5095541401274	0.519904293131331 \\
61.1464968152866	0.507404534536336 \\
61.7834394904459	0.507574468118528 \\
62.4203821656051	0.497410290953735 \\
63.0573248407643	0.486470042673398 \\
63.6942675159236	0.474487674405109 \\
64.3312101910828	0.473348184735876 \\
64.968152866242	0.462881473488189 \\
65.6050955414013	0.447879434750607 \\
66.2420382165605	0.439476074292508 \\
66.8789808917197	0.430954396572054 \\
67.515923566879	0.42079879030696 \\
68.1528662420382	0.41316523514465 \\
68.7898089171974	0.404829624336338 \\
69.4267515923567	0.391445683710103 \\
70.0636942675159	0.383234655048614 \\
70.7006369426752	0.364751958417772 \\
71.3375796178344	0.35818274494073 \\
71.9745222929936	0.345579177343736 \\
72.6114649681529	0.331290565038775 \\
73.2484076433121	0.324438026684188 \\
73.8853503184713	0.314678772400885 \\
74.5222929936306	0.307722076967067 \\
75.1592356687898	0.292941159668358 \\
75.796178343949	0.283757854875919 \\
76.4331210191083	0.277636622529328 \\
77.0700636942675	0.259995795097337 \\
77.7070063694268	0.249945584100104 \\
78.343949044586	0.239902768590935 \\
78.9808917197452	0.22853810598469 \\
79.6178343949044	0.222285293231939 \\
80.2547770700637	0.207850043071947 \\
80.8917197452229	0.197860383109345 \\
81.5286624203822	0.186255231656908 \\
82.1656050955414	0.173910134321573 \\
82.8025477707006	0.167148792558706 \\
83.4394904458599	0.157778153382171 \\
84.0764331210191	0.150309839883052 \\
84.7133757961783	0.139869533604922 \\
85.3503184713376	0.129008992221556 \\
85.9872611464968	0.121885412247714 \\
86.6242038216561	0.115105890896202 \\
87.2611464968153	0.104761055312438 \\
87.8980891719745	0.0948198631971152 \\
88.5350318471338	0.0835827011708389 \\
89.171974522293	0.0786235834552854 \\
89.8089171974522	0.0684405304792315 \\
90.4458598726115	0.0651775475146376 \\
91.0828025477707	0.051222296468068 \\
91.7197452229299	0.0471657979311255 \\
92.3566878980892	0.0456996013545271 \\
92.9936305732484	0.0336256066764318 \\
93.6305732484076	0.035131783257962 \\
94.2675159235669	0.0215883920240076 \\
94.9044585987261	0.0186964052989437 \\
95.5414012738853	0.0139848917079212 \\
96.1783439490446	0.0102982451778508 \\
96.8152866242038	0.00605672543752205 \\
97.4522292993631	0.00147221804357657 \\
98.0891719745223	0.000671652594258102 \\
98.7261146496815	0.000232330630867493 \\
99.3630573248408	0.000101805731075713 \\
100	9.07070329958515e-11 \\
};
\path [fill=color6, fill opacity=0.25]
(axis cs:0,0.916037575265186)
--(axis cs:0,0.914735290144777)
--(axis cs:0.636942675159236,0.914830835133611)
--(axis cs:1.27388535031847,0.914823972168775)
--(axis cs:1.91082802547771,0.914964921296186)
--(axis cs:2.54777070063694,0.914292039718179)
--(axis cs:3.18471337579618,0.914579784870212)
--(axis cs:3.82165605095541,0.914203244311096)
--(axis cs:4.45859872611465,0.91360699457558)
--(axis cs:5.09554140127389,0.913198981076606)
--(axis cs:5.73248407643312,0.912756852356703)
--(axis cs:6.36942675159236,0.912306295415899)
--(axis cs:7.00636942675159,0.912247950811205)
--(axis cs:7.64331210191083,0.911421018600268)
--(axis cs:8.28025477707006,0.910931263712697)
--(axis cs:8.9171974522293,0.910409462969798)
--(axis cs:9.55414012738853,0.909151598106383)
--(axis cs:10.1910828025478,0.90769844603983)
--(axis cs:10.828025477707,0.907605893263369)
--(axis cs:11.4649681528662,0.90692707350812)
--(axis cs:12.1019108280255,0.907168070341514)
--(axis cs:12.7388535031847,0.906790115997068)
--(axis cs:13.3757961783439,0.906485447313205)
--(axis cs:14.0127388535032,0.903671544584293)
--(axis cs:14.6496815286624,0.903668811573817)
--(axis cs:15.2866242038217,0.902686490980194)
--(axis cs:15.9235668789809,0.902131528326776)
--(axis cs:16.5605095541401,0.89900004081169)
--(axis cs:17.1974522292994,0.898868989425513)
--(axis cs:17.8343949044586,0.895980419486951)
--(axis cs:18.4713375796178,0.896150936652303)
--(axis cs:19.1082802547771,0.893864171861407)
--(axis cs:19.7452229299363,0.891909895489192)
--(axis cs:20.3821656050955,0.890755118429893)
--(axis cs:21.0191082802548,0.887648835647689)
--(axis cs:21.656050955414,0.883657815491951)
--(axis cs:22.2929936305732,0.881669968295954)
--(axis cs:22.9299363057325,0.879275672063918)
--(axis cs:23.5668789808917,0.878025511341013)
--(axis cs:24.203821656051,0.877067680988982)
--(axis cs:24.8407643312102,0.877299166178143)
--(axis cs:25.4777070063694,0.876725671302692)
--(axis cs:26.1146496815287,0.873795723187261)
--(axis cs:26.7515923566879,0.869740366202825)
--(axis cs:27.3885350318471,0.863014642122042)
--(axis cs:28.0254777070064,0.861113041653426)
--(axis cs:28.6624203821656,0.857746204870719)
--(axis cs:29.2993630573248,0.854433898125845)
--(axis cs:29.9363057324841,0.85242655844987)
--(axis cs:30.5732484076433,0.845965629814601)
--(axis cs:31.2101910828025,0.840942054272669)
--(axis cs:31.8471337579618,0.836099816815593)
--(axis cs:32.484076433121,0.834773055074414)
--(axis cs:33.1210191082803,0.830265284100231)
--(axis cs:33.7579617834395,0.823906738307351)
--(axis cs:34.3949044585987,0.818380908496642)
--(axis cs:35.031847133758,0.814812917819355)
--(axis cs:35.6687898089172,0.810123695778858)
--(axis cs:36.3057324840764,0.80443945002803)
--(axis cs:36.9426751592357,0.801927269474544)
--(axis cs:37.5796178343949,0.796873219305356)
--(axis cs:38.2165605095541,0.78986388334222)
--(axis cs:38.8535031847134,0.782122424259507)
--(axis cs:39.4904458598726,0.772477584385489)
--(axis cs:40.1273885350318,0.767454466518547)
--(axis cs:40.7643312101911,0.76166627718608)
--(axis cs:41.4012738853503,0.753095339588761)
--(axis cs:42.0382165605096,0.745778334618791)
--(axis cs:42.6751592356688,0.737401183579068)
--(axis cs:43.312101910828,0.729886935754616)
--(axis cs:43.9490445859873,0.725350866171379)
--(axis cs:44.5859872611465,0.720248941564597)
--(axis cs:45.2229299363057,0.706199566142659)
--(axis cs:45.859872611465,0.695193366858319)
--(axis cs:46.4968152866242,0.692089075681604)
--(axis cs:47.1337579617834,0.686978980970104)
--(axis cs:47.7707006369427,0.682432324082998)
--(axis cs:48.4076433121019,0.673262832937218)
--(axis cs:49.0445859872611,0.666006771368407)
--(axis cs:49.6815286624204,0.6528805620466)
--(axis cs:50.3184713375796,0.646704986521384)
--(axis cs:50.9554140127388,0.641225103242518)
--(axis cs:51.5923566878981,0.633601212529107)
--(axis cs:52.2292993630573,0.630389660025916)
--(axis cs:52.8662420382166,0.619953348782847)
--(axis cs:53.5031847133758,0.61258597445788)
--(axis cs:54.140127388535,0.603357359196594)
--(axis cs:54.7770700636943,0.59801855857788)
--(axis cs:55.4140127388535,0.592759773680777)
--(axis cs:56.0509554140127,0.582524929100219)
--(axis cs:56.687898089172,0.573159017849904)
--(axis cs:57.3248407643312,0.561878441128099)
--(axis cs:57.9617834394904,0.559612382972017)
--(axis cs:58.5987261146497,0.548483965418401)
--(axis cs:59.2356687898089,0.537730942716929)
--(axis cs:59.8726114649682,0.526625085341325)
--(axis cs:60.5095541401274,0.51289377771758)
--(axis cs:61.1464968152866,0.500355505405516)
--(axis cs:61.7834394904459,0.500603628604354)
--(axis cs:62.4203821656051,0.490333752246402)
--(axis cs:63.0573248407643,0.479529783981788)
--(axis cs:63.6942675159236,0.467689711742542)
--(axis cs:64.3312101910828,0.466541658767917)
--(axis cs:64.968152866242,0.456128144096899)
--(axis cs:65.6050955414013,0.441141736397505)
--(axis cs:66.2420382165605,0.432882462457271)
--(axis cs:66.8789808917197,0.424203594201423)
--(axis cs:67.515923566879,0.414438168592997)
--(axis cs:68.1528662420382,0.40686165069037)
--(axis cs:68.7898089171974,0.398480231113332)
--(axis cs:69.4267515923567,0.38508748200968)
--(axis cs:70.0636942675159,0.376812496111429)
--(axis cs:70.7006369426752,0.358457778657894)
--(axis cs:71.3375796178344,0.351991200033924)
--(axis cs:71.9745222929936,0.339678642543864)
--(axis cs:72.6114649681529,0.325423719268148)
--(axis cs:73.2484076433121,0.318561024374643)
--(axis cs:73.8853503184713,0.308811848894049)
--(axis cs:74.5222929936306,0.301917538814862)
--(axis cs:75.1592356687898,0.287300551427076)
--(axis cs:75.796178343949,0.278440847752315)
--(axis cs:76.4331210191083,0.272456168450855)
--(axis cs:77.0700636942675,0.25467389965973)
--(axis cs:77.7070063694268,0.244774194413306)
--(axis cs:78.343949044586,0.234730664000507)
--(axis cs:78.9808917197452,0.223186962329352)
--(axis cs:79.6178343949044,0.217036032584718)
--(axis cs:80.2547770700637,0.202614393444064)
--(axis cs:80.8917197452229,0.192773261289167)
--(axis cs:81.5286624203822,0.181340111249578)
--(axis cs:82.1656050955414,0.169230077509175)
--(axis cs:82.8025477707006,0.16269866166191)
--(axis cs:83.4394904458599,0.153544648489639)
--(axis cs:84.0764331210191,0.146244181456489)
--(axis cs:84.7133757961783,0.135726085783272)
--(axis cs:85.3503184713376,0.125023233790918)
--(axis cs:85.9872611464968,0.1181354942756)
--(axis cs:86.6242038216561,0.111420235396349)
--(axis cs:87.2611464968153,0.100822963113739)
--(axis cs:87.8980891719745,0.0908087276287166)
--(axis cs:88.5350318471338,0.0794998110445871)
--(axis cs:89.171974522293,0.0744904996194717)
--(axis cs:89.8089171974522,0.0645229350972808)
--(axis cs:90.4458598726115,0.061520566124424)
--(axis cs:91.0828025477707,0.0475827814146225)
--(axis cs:91.7197452229299,0.0437798265182492)
--(axis cs:92.3566878980892,0.0423870961398249)
--(axis cs:92.9936305732484,0.0305428301162781)
--(axis cs:93.6305732484076,0.0322531063279043)
--(axis cs:94.2675159235669,0.0191522031801066)
--(axis cs:94.9044585987261,0.0163152943627409)
--(axis cs:95.5414012738853,0.011778334862944)
--(axis cs:96.1783439490446,0.00859803957154015)
--(axis cs:96.8152866242038,0.00460820667347295)
--(axis cs:97.4522292993631,0.000943238081197)
--(axis cs:98.0891719745223,0.000368371963854871)
--(axis cs:98.7261146496815,0.000127688005038482)
--(axis cs:99.3630573248408,5.90233121690767e-05)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,0.000144588149982348)
--(axis cs:98.7261146496815,0.000336973256696504)
--(axis cs:98.0891719745223,0.000974933224661333)
--(axis cs:97.4522292993631,0.00200119800595614)
--(axis cs:96.8152866242038,0.00750524420157116)
--(axis cs:96.1783439490446,0.0119984507841615)
--(axis cs:95.5414012738853,0.0161914485528984)
--(axis cs:94.9044585987261,0.0210775162351465)
--(axis cs:94.2675159235669,0.0240245808679086)
--(axis cs:93.6305732484076,0.0380104601880197)
--(axis cs:92.9936305732484,0.0367083832365854)
--(axis cs:92.3566878980892,0.0490121065692293)
--(axis cs:91.7197452229299,0.0505517693440018)
--(axis cs:91.0828025477707,0.0548618115215135)
--(axis cs:90.4458598726115,0.0688345289048512)
--(axis cs:89.8089171974522,0.0723581258611822)
--(axis cs:89.171974522293,0.0827566672910992)
--(axis cs:88.5350318471338,0.0876655912970908)
--(axis cs:87.8980891719745,0.0988309987655137)
--(axis cs:87.2611464968153,0.108699147511137)
--(axis cs:86.6242038216561,0.118791546396056)
--(axis cs:85.9872611464968,0.125635330219829)
--(axis cs:85.3503184713376,0.132994750652195)
--(axis cs:84.7133757961783,0.144012981426572)
--(axis cs:84.0764331210191,0.154375498309615)
--(axis cs:83.4394904458599,0.162011658274702)
--(axis cs:82.8025477707006,0.171598923455501)
--(axis cs:82.1656050955414,0.178590191133972)
--(axis cs:81.5286624203822,0.191170352064238)
--(axis cs:80.8917197452229,0.202947504929524)
--(axis cs:80.2547770700637,0.21308569269983)
--(axis cs:79.6178343949044,0.22753455387916)
--(axis cs:78.9808917197452,0.233889249640028)
--(axis cs:78.343949044586,0.245074873181363)
--(axis cs:77.7070063694268,0.255116973786902)
--(axis cs:77.0700636942675,0.265317690534944)
--(axis cs:76.4331210191083,0.282817076607801)
--(axis cs:75.796178343949,0.289074861999523)
--(axis cs:75.1592356687898,0.29858176790964)
--(axis cs:74.5222929936306,0.313526615119272)
--(axis cs:73.8853503184713,0.320545695907721)
--(axis cs:73.2484076433121,0.330315028993733)
--(axis cs:72.6114649681529,0.337157410809401)
--(axis cs:71.9745222929936,0.351479712143608)
--(axis cs:71.3375796178344,0.364374289847537)
--(axis cs:70.7006369426752,0.37104613817765)
--(axis cs:70.0636942675159,0.389656813985798)
--(axis cs:69.4267515923567,0.397803885410526)
--(axis cs:68.7898089171974,0.411179017559345)
--(axis cs:68.1528662420382,0.41946881959893)
--(axis cs:67.515923566879,0.427159412020923)
--(axis cs:66.8789808917197,0.437705198942685)
--(axis cs:66.2420382165605,0.446069686127745)
--(axis cs:65.6050955414013,0.454617133103709)
--(axis cs:64.968152866242,0.469634802879479)
--(axis cs:64.3312101910828,0.480154710703836)
--(axis cs:63.6942675159236,0.481285637067676)
--(axis cs:63.0573248407643,0.493410301365007)
--(axis cs:62.4203821656051,0.504486829661068)
--(axis cs:61.7834394904459,0.514545307632702)
--(axis cs:61.1464968152866,0.514453563667156)
--(axis cs:60.5095541401274,0.526914808545082)
--(axis cs:59.8726114649682,0.540719831965785)
--(axis cs:59.2356687898089,0.551856722895724)
--(axis cs:58.5987261146497,0.56272371595196)
--(axis cs:57.9617834394904,0.573495933110236)
--(axis cs:57.3248407643312,0.576022345041931)
--(axis cs:56.687898089172,0.587452941994997)
--(axis cs:56.0509554140127,0.596889876846744)
--(axis cs:55.4140127388535,0.60738672177407)
--(axis cs:54.7770700636943,0.612312514336461)
--(axis cs:54.140127388535,0.617598957764853)
--(axis cs:53.5031847133758,0.62698373209464)
--(axis cs:52.8662420382166,0.634436645185332)
--(axis cs:52.2292993630573,0.644991688931428)
--(axis cs:51.5923566878981,0.648198557796017)
--(axis cs:50.9554140127388,0.656048800806989)
--(axis cs:50.3184713375796,0.661781313762964)
--(axis cs:49.6815286624204,0.667892868693301)
--(axis cs:49.0445859872611,0.68104610707182)
--(axis cs:48.4076433121019,0.688032942203098)
--(axis cs:47.7707006369427,0.697030450249753)
--(axis cs:47.1337579617834,0.701796007247197)
--(axis cs:46.4968152866242,0.706907483581247)
--(axis cs:45.859872611465,0.709893509532241)
--(axis cs:45.2229299363057,0.720589467035752)
--(axis cs:44.5859872611465,0.734257926169893)
--(axis cs:43.9490445859873,0.739129883067504)
--(axis cs:43.312101910828,0.743869404127295)
--(axis cs:42.6751592356688,0.751074079847667)
--(axis cs:42.0382165605096,0.759310729451917)
--(axis cs:41.4012738853503,0.766402881528922)
--(axis cs:40.7643312101911,0.774987365550994)
--(axis cs:40.1273885350318,0.780474989747809)
--(axis cs:39.4904458598726,0.785229856641962)
--(axis cs:38.8535031847134,0.794774279382471)
--(axis cs:38.2165605095541,0.80207093185247)
--(axis cs:37.5796178343949,0.808739725907277)
--(axis cs:36.9426751592357,0.813578037453409)
--(axis cs:36.3057324840764,0.815488390797082)
--(axis cs:35.6687898089172,0.821328025103175)
--(axis cs:35.031847133758,0.825860960934668)
--(axis cs:34.3949044585987,0.829594375645371)
--(axis cs:33.7579617834395,0.83487800852853)
--(axis cs:33.1210191082803,0.840872186813878)
--(axis cs:32.484076433121,0.84534380262418)
--(axis cs:31.8471337579618,0.846792618703723)
--(axis cs:31.2101910828025,0.851657130138123)
--(axis cs:30.5732484076433,0.856306534626928)
--(axis cs:29.9363057324841,0.862359164714225)
--(axis cs:29.2993630573248,0.864254019705859)
--(axis cs:28.6624203821656,0.867135488424601)
--(axis cs:28.0254777070064,0.870438897008443)
--(axis cs:27.3885350318471,0.872181845885744)
--(axis cs:26.7515923566879,0.878307757704822)
--(axis cs:26.1146496815287,0.882014898676668)
--(axis cs:25.4777070063694,0.884765078116043)
--(axis cs:24.8407643312102,0.885176949159779)
--(axis cs:24.203821656051,0.884956290458506)
--(axis cs:23.5668789808917,0.885819322384003)
--(axis cs:22.9299363057325,0.8869378673453)
--(axis cs:22.2929936305732,0.88893818160892)
--(axis cs:21.656050955414,0.890637780658381)
--(axis cs:21.0191082802548,0.894286384854802)
--(axis cs:20.3821656050955,0.897145157272229)
--(axis cs:19.7452229299363,0.897926868485552)
--(axis cs:19.1082802547771,0.899634348910566)
--(axis cs:18.4713375796178,0.901628623848918)
--(axis cs:17.8343949044586,0.901654471603033)
--(axis cs:17.1974522292994,0.903988740348456)
--(axis cs:16.5605095541401,0.904190772715054)
--(axis cs:15.9235668789809,0.906674649670254)
--(axis cs:15.2866242038217,0.907168866246722)
--(axis cs:14.6496815286624,0.907927568311633)
--(axis cs:14.0127388535032,0.907985003978167)
--(axis cs:13.3757961783439,0.910039010504227)
--(axis cs:12.7388535031847,0.910318980391963)
--(axis cs:12.1019108280255,0.910630323760624)
--(axis cs:11.4649681528662,0.910438809046903)
--(axis cs:10.828025477707,0.910908971130141)
--(axis cs:10.1910828025478,0.911152344587937)
--(axis cs:9.55414012738853,0.912124402778445)
--(axis cs:8.9171974522293,0.913189053298159)
--(axis cs:8.28025477707006,0.913519431042955)
--(axis cs:7.64331210191083,0.913884063184923)
--(axis cs:7.00636942675159,0.914428282299279)
--(axis cs:6.36942675159236,0.914584962125821)
--(axis cs:5.73248407643312,0.914765378008145)
--(axis cs:5.09554140127389,0.915002467824485)
--(axis cs:4.45859872611465,0.91535931129149)
--(axis cs:3.82165605095541,0.915808480112288)
--(axis cs:3.18471337579618,0.915976952603022)
--(axis cs:2.54777070063694,0.91586122015428)
--(axis cs:1.91082802547771,0.916145137819849)
--(axis cs:1.27388535031847,0.916172389005846)
--(axis cs:0.636942675159236,0.91610180415883)
--(axis cs:0,0.916037575265186)
--cycle;


==> img/mnist/mnist_rate_distortion_sfw_order_var_a.tex <==
\addplot [line width=0.5, opacity=0.7, color10, mark=triangle*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color10, thin}]
table {%
0 0.915408363250317
0.636942675159236 0.915214846556773
1.27388535031847 0.914489119341597
1.91082802547771 0.913979433112545
2.54777070063694 0.912600856485078
3.18471337579618 0.911819118536077
3.82165605095541 0.909570908478927
4.45859872611465 0.906714898761129
5.09554140127389 0.902716319013853
5.73248407643312 0.898503961331444
6.36942675159236 0.891712522363523
7.00636942675159 0.884026525545632
7.64331210191083 0.874321167427115
8.28025477707006 0.863311083047884
8.9171974522293 0.852213631487102
9.55414012738853 0.836024062927754
10.1910828025478 0.819387674474274
10.828025477707 0.80280440002156
11.4649681528662 0.781794309018005
12.1019108280255 0.762269675746211
12.7388535031847 0.739598661763594
13.3757961783439 0.720916958183516
14.0127388535032 0.706264043979463
14.6496815286624 0.690221426035278
15.2866242038217 0.677163881791057
15.9235668789809 0.652813398996368
16.5605095541401 0.636679598032497
17.1974522292994 0.612213618395617
17.8343949044586 0.581480763084837
18.4713375796178 0.558693173879292
19.1082802547771 0.537010845998157
19.7452229299363 0.524907662965343
20.3821656050955 0.502254857661028
21.0191082802548 0.475345463211634
21.656050955414 0.454708484722723
22.2929936305732 0.435194254254639
22.9299363057325 0.416960878373357
23.5668789808917 0.399584767013039
24.203821656051 0.385132999926354
24.8407643312102 0.365081473686623
25.4777070063694 0.3519208301853
26.1146496815287 0.339379845647927
26.7515923566879 0.33242421710298
27.3885350318471 0.320329797510194
28.0254777070064 0.312630047996445
28.6624203821656 0.298628380531773
29.2993630573248 0.286737360169573
29.9363057324841 0.273350504551451
30.5732484076433 0.267736433485156
31.2101910828025 0.25805336425004
31.8471337579618 0.240460278299458
32.484076433121 0.228484076071518
33.1210191082803 0.2184020992499
33.7579617834395 0.21373995439693
34.3949044585987 0.211075344918528
35.031847133758 0.200257584204415
35.6687898089172 0.196336810069289
36.3057324840764 0.187472735668602
36.9426751592357 0.177625221587081
37.5796178343949 0.169525885821886
38.2165605095541 0.162823793545678
38.8535031847134 0.155283837637255
39.4904458598726 0.153468382045672
40.1273885350318 0.150357872471022
40.7643312101911 0.144231850512106
41.4012738853503 0.140301655075886
42.0382165605096 0.131877458730797
42.6751592356688 0.127532347983099
43.312101910828 0.126189243353467
43.9490445859873 0.124545746715039
44.5859872611465 0.122020771806418
45.2229299363057 0.116269608905055
45.859872611465 0.109973391056262
46.4968152866242 0.109177835345766
47.1337579617834 0.105565505275214
47.7707006369427 0.0992745313977585
48.4076433121019 0.0926934569083651
49.0445859872611 0.0898969810119632
49.6815286624204 0.0848480725854928
50.3184713375796 0.0814269740627748
50.9554140127388 0.0782054029381177
51.5923566878981 0.0763183959086652
52.2292993630573 0.075478683769385
52.8662420382166 0.0713389561933222
53.5031847133758 0.0671094841721704
54.140127388535 0.062033450784812
54.7770700636943 0.0598027716077174
55.4140127388535 0.0537179044821708
56.0509554140127 0.0496112073136698
56.687898089172 0.0484689084093095
57.3248407643312 0.0452612851642483
57.9617834394904 0.0422962291482452
58.5987261146497 0.0396955129335302
59.2356687898089 0.0360385198255223
59.8726114649682 0.0355197039091089
60.5095541401274 0.0320555652758262
61.1464968152866 0.0296180243293569
61.7834394904459 0.0300130431513939
62.4203821656051 0.0305727252081784
63.0573248407643 0.0275725691004729
63.6942675159236 0.0260270850694834
64.3312101910828 0.0239057613234671
64.968152866242 0.0240379893480425
65.6050955414013 0.0206028489350342
66.2420382165605 0.0186384850806371
66.8789808917197 0.0153261583103165
67.515923566879 0.0141655280275829
68.1528662420382 0.0117043860686528
68.7898089171974 0.0117698971454759
69.4267515923567 0.010521624095729
70.0636942675159 0.00789420462971387
70.7006369426752 0.00697871359654069
71.3375796178344 0.00760384273415043
71.9745222929936 0.00722136436289715
72.6114649681529 0.00652669003529794
73.2484076433121 0.00628936050061611
73.8853503184713 0.00484281522100607
74.5222929936306 0.00382392563208142
75.1592356687898 0.00339515696297203
75.796178343949 0.00351269573396356
76.4331210191083 0.00400129506600583
77.0700636942675 0.00268456280424388
77.7070063694268 0.002903576453118
78.343949044586 0.00358901193001742
78.9808917197452 0.00230705061248283
79.6178343949044 0.00203365798396848
80.2547770700637 0.00141699541328674
80.8917197452229 0.000869865186300476
81.5286624203822 0.00102672494882719
82.1656050955414 0.000620370907204137
82.8025477707006 0.00039895760518029
83.4394904458599 0.000439410806362232
84.0764331210191 0.00055173759073514
84.7133757961783 0.000455310001852546
85.3503184713376 0.000339039690408099
85.9872611464968 0.000195095499055419
86.6242038216561 0.000224893732157747
87.2611464968153 0.00016419916914972
87.8980891719745 0.000164527858364196
88.5350318471338 4.93021562087181e-05
89.171974522293 3.54473336184935e-05
89.8089171974522 2.95517235172199e-05
90.4458598726115 2.95247309230473e-05
91.0828025477707 1.74300322260457e-05
91.7197452229299 1.25115230549305e-05
92.3566878980892 8.55397612186837e-06
92.9936305732484 8.40674427860344e-06
93.6305732484076 7.44655420197526e-06
94.2675159235669 7.15441811458606e-06
94.9044585987261 7.01026969549767e-06
95.5414012738853 6.84471230506356e-06
96.1783439490446 5.50775881909049e-06
96.8152866242038 1.02095308333028e-05
97.4522292993631 3.56678827735962e-05
98.0891719745223 6.25728622155775e-05
98.7261146496815 7.21039694409786e-05
99.3630573248408 4.90879812487188e-06
100 9.06140229517405e-11
};
\path [fill=color10, fill opacity=0.25] 
(axis cs:0,0.916036674747957)
--(axis cs:0,0.914780051752677)
--(axis cs:0.636942675159236,0.914504561815803)
--(axis cs:1.27388535031847,0.913742027735358)
--(axis cs:1.91082802547771,0.913074620487323)
--(axis cs:2.54777070063694,0.911455435306687)
--(axis cs:3.18471337579618,0.910590551928887)
--(axis cs:3.82165605095541,0.907971855312227)
--(axis cs:4.45859872611465,0.904797024443555)
--(axis cs:5.09554140127389,0.900379795715475)
--(axis cs:5.73248407643312,0.895801210490797)
--(axis cs:6.36942675159236,0.888333248434583)
--(axis cs:7.00636942675159,0.880146702175899)
--(axis cs:7.64331210191083,0.869909596473065)
--(axis cs:8.28025477707006,0.858253921129068)
--(axis cs:8.9171974522293,0.846808735386283)
--(axis cs:9.55414012738853,0.829999567474244)
--(axis cs:10.1910828025478,0.813061850379617)
--(axis cs:10.828025477707,0.796112805460833)
--(axis cs:11.4649681528662,0.774989197024542)
--(axis cs:12.1019108280255,0.755043896422146)
--(axis cs:12.7388535031847,0.732163775676051)
--(axis cs:13.3757961783439,0.713356697468489)
--(axis cs:14.0127388535032,0.698578106902737)
--(axis cs:14.6496815286624,0.682559933463207)
--(axis cs:15.2866242038217,0.669281660632354)
--(axis cs:15.9235668789809,0.644672414371352)
--(axis cs:16.5605095541401,0.628398359061509)
--(axis cs:17.1974522292994,0.603633936173771)
--(axis cs:17.8343949044586,0.572815384540114)
--(axis cs:18.4713375796178,0.549965695828003)
--(axis cs:19.1082802547771,0.528386934368605)
--(axis cs:19.7452229299363,0.516065577330539)
--(axis cs:20.3821656050955,0.493481403472317)
--(axis cs:21.0191082802548,0.466779051809535)
--(axis cs:21.656050955414,0.44619099957747)
--(axis cs:22.2929936305732,0.426748597699051)
--(axis cs:22.9299363057325,0.408611153395181)
--(axis cs:23.5668789808917,0.391336605947603)
--(axis cs:24.203821656051,0.377002784558196)
--(axis cs:24.8407643312102,0.357012143653428)
--(axis cs:25.4777070063694,0.344025813658225)
--(axis cs:26.1146496815287,0.331616477462596)
--(axis cs:26.7515923566879,0.324615038844859)
--(axis cs:27.3885350318471,0.312673264954783)
--(axis cs:28.0254777070064,0.305183907901933)
--(axis cs:28.6624203821656,0.291218511901835)
--(axis cs:29.2993630573248,0.279445835398697)
--(axis cs:29.9363057324841,0.266096056495462)
--(axis cs:30.5732484076433,0.260727407302451)
--(axis cs:31.2101910828025,0.251112698350347)
--(axis cs:31.8471337579618,0.233704366681303)
--(axis cs:32.484076433121,0.221759514732932)
--(axis cs:33.1210191082803,0.21174267694811)
--(axis cs:33.7579617834395,0.207093030427866)
--(axis cs:34.3949044585987,0.204507620368855)
--(axis cs:35.031847133758,0.193777410256666)
--(axis cs:35.6687898089172,0.1898306294941)
--(axis cs:36.3057324840764,0.181004658939572)
--(axis cs:36.9426751592357,0.171326932245335)
--(axis cs:37.5796178343949,0.163371937089912)
--(axis cs:38.2165605095541,0.156645449725288)
--(axis cs:38.8535031847134,0.149364487052986)
--(axis cs:39.4904458598726,0.147673281653932)
--(axis cs:40.1273885350318,0.144581678800115)
--(axis cs:40.7643312101911,0.138704660519712)
--(axis cs:41.4012738853503,0.134940582882612)
--(axis cs:42.0382165605096,0.126861139170964)
--(axis cs:42.6751592356688,0.122613534741667)
--(axis cs:43.312101910828,0.121335522642977)
--(axis cs:43.9490445859873,0.119631048382489)
--(axis cs:44.5859872611465,0.117086629131692)
--(axis cs:45.2229299363057,0.111241741242673)
--(axis cs:45.859872611465,0.105080972403397)
--(axis cs:46.4968152866242,0.104241653251849)
--(axis cs:47.1337579617834,0.100708664686344)
--(axis cs:47.7707006369427,0.0944419756246164)
--(axis cs:48.4076433121019,0.0879926047931121)
--(axis cs:49.0445859872611,0.0851744823953191)
--(axis cs:49.6815286624204,0.0803844831001741)
--(axis cs:50.3184713375796,0.0769717946675439)
--(axis cs:50.9554140127388,0.0735852134655118)
--(axis cs:51.5923566878981,0.0716734124166313)
--(axis cs:52.2292993630573,0.0709735742137636)
--(axis cs:52.8662420382166,0.0669634918980197)
--(axis cs:53.5031847133758,0.062858643440703)
--(axis cs:54.140127388535,0.0579336738223885)
--(axis cs:54.7770700636943,0.0555843312959675)
--(axis cs:55.4140127388535,0.0499008134892861)
--(axis cs:56.0509554140127,0.0456560361595353)
--(axis cs:56.687898089172,0.0446229535672703)
--(axis cs:57.3248407643312,0.0414668057493644)
--(axis cs:57.9617834394904,0.038512244200118)
--(axis cs:58.5987261146497,0.0361156884856879)
--(axis cs:59.2356687898089,0.0326033248031945)
--(axis cs:59.8726114649682,0.0321349512377212)
--(axis cs:60.5095541401274,0.0286509038321956)
--(axis cs:61.1464968152866,0.026413342410818)
--(axis cs:61.7834394904459,0.0267177129412567)
--(axis cs:62.4203821656051,0.0273303472578288)
--(axis cs:63.0573248407643,0.0243616688834669)
--(axis cs:63.6942675159236,0.0228537917439984)
--(axis cs:64.3312101910828,0.0208618507202265)
--(axis cs:64.968152866242,0.020973164571437)
--(axis cs:65.6050955414013,0.0177831465485157)
--(axis cs:66.2420382165605,0.0159794141096929)
--(axis cs:66.8789808917197,0.0128441099032852)
--(axis cs:67.515923566879,0.011801330586386)
--(axis cs:68.1528662420382,0.00957614038900566)
--(axis cs:68.7898089171974,0.00964830957747582)
--(axis cs:69.4267515923567,0.00847216553079757)
--(axis cs:70.0636942675159,0.00623745481932182)
--(axis cs:70.7006369426752,0.00533383241264935)
--(axis cs:71.3375796178344,0.00597834253661376)
--(axis cs:71.9745222929936,0.00558691052370309)
--(axis cs:72.6114649681529,0.00500079729209657)
--(axis cs:73.2484076433121,0.00476892538159322)
--(axis cs:73.8853503184713,0.00348591075495561)
--(axis cs:74.5222929936306,0.00268319765061457)
--(axis cs:75.1592356687898,0.0023530579898664)
--(axis cs:75.796178343949,0.00246539814083089)
--(axis cs:76.4331210191083,0.00282865980494878)
--(axis cs:77.0700636942675,0.00181835166058547)
--(axis cs:77.7070063694268,0.00199372453782383)
--(axis cs:78.343949044586,0.00264686735323969)
--(axis cs:78.9808917197452,0.0015678283602585)
--(axis cs:79.6178343949044,0.00135875605641068)
--(axis cs:80.2547770700637,0.000886892520458261)
--(axis cs:80.8917197452229,0.000516658217813581)
--(axis cs:81.5286624203822,0.000577587699375074)
--(axis cs:82.1656050955414,0.000315791293753635)
--(axis cs:82.8025477707006,0.000211192861989264)
--(axis cs:83.4394904458599,0.000237010789738598)
--(axis cs:84.0764331210191,0.000257145993167552)
--(axis cs:84.7133757961783,0.000219131979795208)
--(axis cs:85.3503184713376,0.000163604459195608)
--(axis cs:85.9872611464968,7.84536186803471e-05)
--(axis cs:86.6242038216561,8.745778022907e-05)
--(axis cs:87.2611464968153,3.11761801313794e-05)
--(axis cs:87.8980891719745,5.84089845532008e-05)
--(axis cs:88.5350318471338,2.7983337404934e-05)
--(axis cs:89.171974522293,1.31968021156628e-05)
--(axis cs:89.8089171974522,5.24145081726462e-06)
--(axis cs:90.4458598726115,1.02879775668779e-05)
--(axis cs:91.0828025477707,9.86423060407603e-06)
--(axis cs:91.7197452229299,7.07451032551946e-06)
--(axis cs:92.3566878980892,7.33118217498698e-06)
--(axis cs:92.9936305732484,7.41348465091459e-06)
--(axis cs:93.6305732484076,6.94459863634627e-06)
--(axis cs:94.2675159235669,6.79378191522743e-06)
--(axis cs:94.9044585987261,6.66840283675412e-06)
--(axis cs:95.5414012738853,6.47161406147514e-06)
--(axis cs:96.1783439490446,4.67805422808188e-06)
--(axis cs:96.8152866242038,2.55976613323261e-06)
--(axis cs:97.4522292993631,1.41039521632432e-05)
--(axis cs:98.0891719745223,2.5269883384876e-05)
--(axis cs:98.7261146496815,3.44806078697656e-05)
--(axis cs:99.3630573248408,2.9427385797349e-06)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:100,9.06140229517405e-11)
--(axis cs:99.3630573248408,6.87485767000887e-06)
--(axis cs:98.7261146496815,0.000109727331012192)
--(axis cs:98.0891719745223,9.98758410462789e-05)
--(axis cs:97.4522292993631,5.72318133839492e-05)
--(axis cs:96.8152866242038,1.7859295533373e-05)
--(axis cs:96.1783439490446,6.3374634100991e-06)
--(axis cs:95.5414012738853,7.21781054865198e-06)
--(axis cs:94.9044585987261,7.35213655424123e-06)
--(axis cs:94.2675159235669,7.51505431394469e-06)
--(axis cs:93.6305732484076,7.94850976760426e-06)
--(axis cs:92.9936305732484,9.40000390629229e-06)
--(axis cs:92.3566878980892,9.77677006874975e-06)
--(axis cs:91.7197452229299,1.79485357843416e-05)
--(axis cs:91.0828025477707,2.49958338480153e-05)
--(axis cs:90.4458598726115,4.87614842792167e-05)
--(axis cs:89.8089171974522,5.38619962171752e-05)
--(axis cs:89.171974522293,5.76978651213242e-05)
--(axis cs:88.5350318471338,7.06209750125023e-05)
--(axis cs:87.8980891719745,0.000270646732175191)
--(axis cs:87.2611464968153,0.000297222158168061)
--(axis cs:86.6242038216561,0.000362329684086424)
--(axis cs:85.9872611464968,0.000311737379430492)
--(axis cs:85.3503184713376,0.00051447492162059)
--(axis cs:84.7133757961783,0.000691488023909885)
--(axis cs:84.0764331210191,0.000846329188302728)
--(axis cs:83.4394904458599,0.000641810822985866)
--(axis cs:82.8025477707006,0.000586722348371317)
--(axis cs:82.1656050955414,0.000924950520654639)
--(axis cs:81.5286624203822,0.0014758621982793)
--(axis cs:80.8917197452229,0.00122307215478737)
--(axis cs:80.2547770700637,0.00194709830611522)
--(axis cs:79.6178343949044,0.00270855991152628)
--(axis cs:78.9808917197452,0.00304627286470715)
--(axis cs:78.343949044586,0.00453115650679515)
--(axis cs:77.7070063694268,0.00381342836841217)
--(axis cs:77.0700636942675,0.00355077394790228)
--(axis cs:76.4331210191083,0.00517393032706288)
--(axis cs:75.796178343949,0.00455999332709623)
--(axis cs:75.1592356687898,0.00443725593607765)
--(axis cs:74.5222929936306,0.00496465361354826)
--(axis cs:73.8853503184713,0.00619971968705653)
--(axis cs:73.2484076433121,0.007809795619639)
--(axis cs:72.6114649681529,0.0080525827784993)
--(axis cs:71.9745222929936,0.00885581820209122)
--(axis cs:71.3375796178344,0.00922934293168709)
--(axis cs:70.7006369426752,0.00862359478043203)
--(axis cs:70.0636942675159,0.00955095444010593)
--(axis cs:69.4267515923567,0.0125710826606605)
--(axis cs:68.7898089171974,0.0138914847134759)
--(axis cs:68.1528662420382,0.0138326317482999)
--(axis cs:67.515923566879,0.0165297254687799)
--(axis cs:66.8789808917197,0.0178082067173479)
--(axis cs:66.2420382165605,0.0212975560515813)
--(axis cs:65.6050955414013,0.0234225513215527)
--(axis cs:64.968152866242,0.0271028141246479)
--(axis cs:64.3312101910828,0.0269496719267078)
--(axis cs:63.6942675159236,0.0292003783949685)
--(axis cs:63.0573248407643,0.0307834693174789)
--(axis cs:62.4203821656051,0.033815103158528)
--(axis cs:61.7834394904459,0.0333083733615311)
--(axis cs:61.1464968152866,0.0328227062478958)
--(axis cs:60.5095541401274,0.0354602267194567)
--(axis cs:59.8726114649682,0.0389044565804966)
--(axis cs:59.2356687898089,0.0394737148478501)
--(axis cs:58.5987261146497,0.0432753373813725)
--(axis cs:57.9617834394904,0.0460802140963724)
--(axis cs:57.3248407643312,0.0490557645791322)
--(axis cs:56.687898089172,0.0523148632513487)
--(axis cs:56.0509554140127,0.0535663784678044)
--(axis cs:55.4140127388535,0.0575349954750556)
--(axis cs:54.7770700636943,0.0640212119194674)
--(axis cs:54.140127388535,0.0661332277472355)
--(axis cs:53.5031847133758,0.0713603249036378)
--(axis cs:52.8662420382166,0.0757144204886246)
--(axis cs:52.2292993630573,0.0799837933250064)
--(axis cs:51.5923566878981,0.080963379400699)
--(axis cs:50.9554140127388,0.0828255924107236)
--(axis cs:50.3184713375796,0.0858821534580057)
--(axis cs:49.6815286624204,0.0893116620708116)
--(axis cs:49.0445859872611,0.0946194796286073)
--(axis cs:48.4076433121019,0.0973943090236181)
--(axis cs:47.7707006369427,0.104107087170901)
--(axis cs:47.1337579617834,0.110422345864084)
--(axis cs:46.4968152866242,0.114114017439684)
--(axis cs:45.859872611465,0.114865809709126)
--(axis cs:45.2229299363057,0.121297476567436)
--(axis cs:44.5859872611465,0.126954914481145)
--(axis cs:43.9490445859873,0.129460445047589)
--(axis cs:43.312101910828,0.131042964063956)
--(axis cs:42.6751592356688,0.132451161224531)
--(axis cs:42.0382165605096,0.13689377829063)
--(axis cs:41.4012738853503,0.14566272726916)
--(axis cs:40.7643312101911,0.1497590405045)
--(axis cs:40.1273885350318,0.156134066141928)
--(axis cs:39.4904458598726,0.159263482437412)
--(axis cs:38.8535031847134,0.161203188221525)
--(axis cs:38.2165605095541,0.169002137366067)
--(axis cs:37.5796178343949,0.175679834553859)
--(axis cs:36.9426751592357,0.183923510928826)
--(axis cs:36.3057324840764,0.193940812397631)
--(axis cs:35.6687898089172,0.202842990644479)
--(axis cs:35.031847133758,0.206737758152165)
--(axis cs:34.3949044585987,0.217643069468201)
--(axis cs:33.7579617834395,0.220386878365995)
--(axis cs:33.1210191082803,0.22506152155169)
--(axis cs:32.484076433121,0.235208637410103)
--(axis cs:31.8471337579618,0.247216189917612)
--(axis cs:31.2101910828025,0.264994030149733)
--(axis cs:30.5732484076433,0.274745459667862)
--(axis cs:29.9363057324841,0.28060495260744)
--(axis cs:29.2993630573248,0.294028884940448)
--(axis cs:28.6624203821656,0.30603824916171)
--(axis cs:28.0254777070064,0.320076188090957)
--(axis cs:27.3885350318471,0.327986330065605)
--(axis cs:26.7515923566879,0.340233395361101)
--(axis cs:26.1146496815287,0.347143213833259)
--(axis cs:25.4777070063694,0.359815846712374)
--(axis cs:24.8407643312102,0.373150803719819)
--(axis cs:24.203821656051,0.393263215294513)
--(axis cs:23.5668789808917,0.407832928078475)
--(axis cs:22.9299363057325,0.425310603351532)
--(axis cs:22.2929936305732,0.443639910810226)
--(axis cs:21.656050955414,0.463225969867977)
--(axis cs:21.0191082802548,0.483911874613732)
--(axis cs:20.3821656050955,0.511028311849739)
--(axis cs:19.7452229299363,0.533749748600146)
--(axis cs:19.1082802547771,0.545634757627708)
--(axis cs:18.4713375796178,0.56742065193058)
--(axis cs:17.8343949044586,0.59014614162956)
--(axis cs:17.1974522292994,0.620793300617463)
--(axis cs:16.5605095541401,0.644960837003485)
--(axis cs:15.9235668789809,0.660954383621384)
--(axis cs:15.2866242038217,0.685046102949761)
--(axis cs:14.6496815286624,0.697882918607348)
--(axis cs:14.0127388535032,0.713949981056189)
--(axis cs:13.3757961783439,0.728477218898543)
--(axis cs:12.7388535031847,0.747033547851136)
--(axis cs:12.1019108280255,0.769495455070276)
--(axis cs:11.4649681528662,0.788599421011469)
--(axis cs:10.828025477707,0.809495994582286)
--(axis cs:10.1910828025478,0.825713498568931)
--(axis cs:9.55414012738853,0.842048558381264)
--(axis cs:8.9171974522293,0.857618527587922)
--(axis cs:8.28025477707006,0.868368244966699)
--(axis cs:7.64331210191083,0.878732738381165)
--(axis cs:7.00636942675159,0.887906348915366)
--(axis cs:6.36942675159236,0.895091796292464)
--(axis cs:5.73248407643312,0.901206712172091)
--(axis cs:5.09554140127389,0.90505284231223)
--(axis cs:4.45859872611465,0.908632773078703)
--(axis cs:3.82165605095541,0.911169961645627)
--(axis cs:3.18471337579618,0.913047685143268)
--(axis cs:2.54777070063694,0.913746277663469)
--(axis cs:1.91082802547771,0.914884245737766)
--(axis cs:1.27388535031847,0.915236210947836)
--(axis cs:0.636942675159236,0.915925131297744)
--(axis cs:0,0.916036674747957)
--cycle;


==> img/mnist/mnist_rate_distortion_sfw_order_var_b.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.915515506975353
0.636942675159236 0.915291130807018
1.27388535031847 0.914610721995123
1.91082802547771 0.913968700898113
2.54777070063694 0.913278063565958
3.18471337579618 0.911566871852847
3.82165605095541 0.909045555838384
4.45859872611465 0.9061207701487
5.09554140127389 0.902986996376421
5.73248407643312 0.896979984858772
6.36942675159236 0.891292300488567
7.00636942675159 0.883909361392725
7.64331210191083 0.874118765690364
8.28025477707006 0.860875287575182
8.9171974522293 0.849542131815106
9.55414012738853 0.83819488979876
10.1910828025478 0.819142400963465
10.828025477707 0.799906278424896
11.4649681528662 0.783906305114506
12.1019108280255 0.770254769342719
12.7388535031847 0.745393566618441
13.3757961783439 0.726009110044106
14.0127388535032 0.711451979747508
14.6496815286624 0.691596523672051
15.2866242038217 0.669794172981055
15.9235668789809 0.652617117378977
16.5605095541401 0.625948955215281
17.1974522292994 0.604185574197327
17.8343949044586 0.583505890988745
18.4713375796178 0.563118747053668
19.1082802547771 0.539961678393884
19.7452229299363 0.525330018711975
20.3821656050955 0.498833596089389
21.0191082802548 0.474622265309299
21.656050955414 0.454955571094033
22.2929936305732 0.436370195729542
22.9299363057325 0.421439845320492
23.5668789808917 0.404704255864417
24.203821656051 0.396171100917272
24.8407643312102 0.382650574015279
25.4777070063694 0.365225246625487
26.1146496815287 0.34804563597776
26.7515923566879 0.332593755530534
27.3885350318471 0.328221528293093
28.0254777070064 0.313248760890649
28.6624203821656 0.300340954657405
29.2993630573248 0.290636036881842
29.9363057324841 0.275794949770955
30.5732484076433 0.262429187381866
31.2101910828025 0.252397748400278
31.8471337579618 0.246224349660174
32.484076433121 0.23137986838768
33.1210191082803 0.218307591992915
33.7579617834395 0.212992557244184
34.3949044585987 0.198935438675432
35.031847133758 0.192778947108619
35.6687898089172 0.188906885004072
36.3057324840764 0.176824342499357
36.9426751592357 0.169138188364398
37.5796178343949 0.159485098029523
38.2165605095541 0.158545154153228
38.8535031847134 0.153834523310863
39.4904458598726 0.145573285027933
40.1273885350318 0.141124897134187
40.7643312101911 0.138525937105359
41.4012738853503 0.138483225165246
42.0382165605096 0.133191477924997
42.6751592356688 0.128765954131079
43.312101910828 0.124792630792011
43.9490445859873 0.123126714913403
44.5859872611465 0.118704031777947
45.2229299363057 0.116501407778391
45.859872611465 0.110307892875636
46.4968152866242 0.10270152864946
47.1337579617834 0.0947132513346082
47.7707006369427 0.0939434017210897
48.4076433121019 0.093431803641167
49.0445859872611 0.0887264073425121
49.6815286624204 0.0803602511666803
50.3184713375796 0.0790253162800587
50.9554140127388 0.0749829026084019
51.5923566878981 0.0693398577090171
52.2292993630573 0.0717814715180009
52.8662420382166 0.0697079134719667
53.5031847133758 0.0644458268611214
54.140127388535 0.0648622218732247
54.7770700636943 0.0624101705322018
55.4140127388535 0.0599157281823885
56.0509554140127 0.0598766682692429
56.687898089172 0.0546325231108434
57.3248407643312 0.0524818531759413
57.9617834394904 0.0480977058029989
58.5987261146497 0.0439300285024914
59.2356687898089 0.0421726216463079
59.8726114649682 0.0389694326872814
60.5095541401274 0.0369034675931852
61.1464968152866 0.0335927363490565
61.7834394904459 0.0340809992385781
62.4203821656051 0.0313772137542854
63.0573248407643 0.0295125158801798
63.6942675159236 0.0289313618617426
64.3312101910828 0.025323248282162
64.968152866242 0.0229263654039886
65.6050955414013 0.0217245476156789
66.2420382165605 0.0193483210903419
66.8789808917197 0.0187612086424341
67.515923566879 0.0189841724217542
68.1528662420382 0.0199444382595105
68.7898089171974 0.0169039488660667
69.4267515923567 0.0165095603310091
70.0636942675159 0.0170860213930992
70.7006369426752 0.013318507248957
71.3375796178344 0.0124654478903215
71.9745222929936 0.0125370567455003
72.6114649681529 0.0117941051206867
73.2484076433121 0.0123456729487164
73.8853503184713 0.0113449304557583
74.5222929936306 0.0123036909722337
75.1592356687898 0.0106037691082614
75.796178343949 0.00828264705976556
76.4331210191083 0.00597501834991025
77.0700636942675 0.00357003187025133
77.7070063694268 0.0033265953915086
78.343949044586 0.00130976848432675
78.9808917197452 0.000916467445418984
79.6178343949044 0.000773480905644669
80.2547770700637 0.00101159810522818
80.8917197452229 0.00102587806685192
81.5286624203822 0.000711718709052193
82.1656050955414 0.000456619887234714
82.8025477707006 0.000713163580755887
83.4394904458599 0.00106583017776917
84.0764331210191 0.000705895672702355
84.7133757961783 0.000559179788165455
85.3503184713376 0.000598806074874183
85.9872611464968 0.000589529007150282
86.6242038216561 0.00043221315858353
87.2611464968153 0.000358666396587488
87.8980891719745 0.000129406830056237
88.5350318471338 0.000148086778342936
89.171974522293 6.41118347528785e-05
89.8089171974522 4.31714728894944e-05
90.4458598726115 0.000118268334876893
91.0828025477707 8.21446018277122e-05
91.7197452229299 2.74500312472525e-05
92.3566878980892 2.95276120547422e-05
92.9936305732484 1.29721163201296e-05
93.6305732484076 1.12496133724249e-05
94.2675159235669 8.29544702576179e-06
94.9044585987261 8.27878212903699e-06
95.5414012738853 7.81313617392865e-06
96.1783439490446 8.03140951947889e-06
96.8152866242038 7.84679473103456e-06
97.4522292993631 7.61884722859596e-06
98.0891719745223 7.33944535439845e-06
98.7261146496815 5.25554244962811e-06
99.3630573248408 2.24389552520798e-06
100 0
};
\path [fill=color0, fill opacity=0.25] 
(axis cs:0,0.916100204106519)
--(axis cs:0,0.914930809844187)
--(axis cs:0.636942675159236,0.914715571938752)
--(axis cs:1.27388535031847,0.913797252903839)
--(axis cs:1.91082802547771,0.913114040287844)
--(axis cs:2.54777070063694,0.912283957784271)
--(axis cs:3.18471337579618,0.91027648651513)
--(axis cs:3.82165605095541,0.907428927729367)
--(axis cs:4.45859872611465,0.904115849185193)
--(axis cs:5.09554140127389,0.900675634668446)
--(axis cs:5.73248407643312,0.894060817662883)
--(axis cs:6.36942675159236,0.887950098634238)
--(axis cs:7.00636942675159,0.880016361604445)
--(axis cs:7.64331210191083,0.869588359966957)
--(axis cs:8.28025477707006,0.855802804614117)
--(axis cs:8.9171974522293,0.844083292039519)
--(axis cs:9.55414012738853,0.832354324400403)
--(axis cs:10.1910828025478,0.812839098460872)
--(axis cs:10.828025477707,0.793309504304936)
--(axis cs:11.4649681528662,0.777271499274278)
--(axis cs:12.1019108280255,0.763425486292506)
--(axis cs:12.7388535031847,0.73819124696875)
--(axis cs:13.3757961783439,0.71881540432338)
--(axis cs:14.0127388535032,0.704099615940779)
--(axis cs:14.6496815286624,0.684126979181611)
--(axis cs:15.2866242038217,0.662061305581432)
--(axis cs:15.9235668789809,0.644674522163649)
--(axis cs:16.5605095541401,0.617678379758528)
--(axis cs:17.1974522292994,0.595713550627389)
--(axis cs:17.8343949044586,0.574967354542988)
--(axis cs:18.4713375796178,0.554381373846378)
--(axis cs:19.1082802547771,0.531280226988909)
--(axis cs:19.7452229299363,0.516689271982769)
--(axis cs:20.3821656050955,0.490198160022371)
--(axis cs:21.0191082802548,0.465879669040335)
--(axis cs:21.656050955414,0.44635938925141)
--(axis cs:22.2929936305732,0.427985347961947)
--(axis cs:22.9299363057325,0.413109545896699)
--(axis cs:23.5668789808917,0.39647869587954)
--(axis cs:24.203821656051,0.3880582181643)
--(axis cs:24.8407643312102,0.374683704829022)
--(axis cs:25.4777070063694,0.357337770501582)
--(axis cs:26.1146496815287,0.340369333997812)
--(axis cs:26.7515923566879,0.325111765084446)
--(axis cs:27.3885350318471,0.320676948250096)
--(axis cs:28.0254777070064,0.305873598421239)
--(axis cs:28.6624203821656,0.293140670286526)
--(axis cs:29.2993630573248,0.283611372684083)
--(axis cs:29.9363057324841,0.268849183081031)
--(axis cs:30.5732484076433,0.255521684156947)
--(axis cs:31.2101910828025,0.245428514284999)
--(axis cs:31.8471337579618,0.239231911540809)
--(axis cs:32.484076433121,0.224688176235706)
--(axis cs:33.1210191082803,0.211623462423511)
--(axis cs:33.7579617834395,0.206392645959491)
--(axis cs:34.3949044585987,0.192480375185512)
--(axis cs:35.031847133758,0.186428282914231)
--(axis cs:35.6687898089172,0.182600832680947)
--(axis cs:36.3057324840764,0.170722467487498)
--(axis cs:36.9426751592357,0.163121781416614)
--(axis cs:37.5796178343949,0.1536948361144)
--(axis cs:38.2165605095541,0.152812315841888)
--(axis cs:38.8535031847134,0.148106723447037)
--(axis cs:39.4904458598726,0.140001395127548)
--(axis cs:40.1273885350318,0.135806580629974)
--(axis cs:40.7643312101911,0.133245827548986)
--(axis cs:41.4012738853503,0.133198794335178)
--(axis cs:42.0382165605096,0.128060262920711)
--(axis cs:42.6751592356688,0.123699088023671)
--(axis cs:43.312101910828,0.11974084130157)
--(axis cs:43.9490445859873,0.118143636893188)
--(axis cs:44.5859872611465,0.113586900527348)
--(axis cs:45.2229299363057,0.11154773868721)
--(axis cs:45.859872611465,0.105497622193996)
--(axis cs:46.4968152866242,0.0979403913839694)
--(axis cs:47.1337579617834,0.0901219376754009)
--(axis cs:47.7707006369427,0.0892255441948402)
--(axis cs:48.4076433121019,0.0884869979300282)
--(axis cs:49.0445859872611,0.0838759139791583)
--(axis cs:49.6815286624204,0.0756393035649507)
--(axis cs:50.3184713375796,0.0742698736594444)
--(axis cs:50.9554140127388,0.0702725785427777)
--(axis cs:51.5923566878981,0.0647758473259365)
--(axis cs:52.2292993630573,0.0670652602092943)
--(axis cs:52.8662420382166,0.065114946067583)
--(axis cs:53.5031847133758,0.0599167561920425)
--(axis cs:54.140127388535,0.0604553342078063)
--(axis cs:54.7770700636943,0.0579811844749541)
--(axis cs:55.4140127388535,0.0555141309458273)
--(axis cs:56.0509554140127,0.0556686954904333)
--(axis cs:56.687898089172,0.0504969759712964)
--(axis cs:57.3248407643312,0.048470519956803)
--(axis cs:57.9617834394904,0.0441293370957033)
--(axis cs:58.5987261146497,0.040123763724066)
--(axis cs:59.2356687898089,0.0383550514167907)
--(axis cs:59.8726114649682,0.0353147762948378)
--(axis cs:60.5095541401274,0.0332538454526795)
--(axis cs:61.1464968152866,0.0300005611168516)
--(axis cs:61.7834394904459,0.03056125763571)
--(axis cs:62.4203821656051,0.0279020806851372)
--(axis cs:63.0573248407643,0.026163636709634)
--(axis cs:63.6942675159236,0.0256003240612405)
--(axis cs:64.3312101910828,0.0222813851599047)
--(axis cs:64.968152866242,0.0200172886384762)
--(axis cs:65.6050955414013,0.0188173573481031)
--(axis cs:66.2420382165605,0.016586270341011)
--(axis cs:66.8789808917197,0.016103823247747)
--(axis cs:67.515923566879,0.0163071268333231)
--(axis cs:68.1528662420382,0.0172396366987298)
--(axis cs:68.7898089171974,0.0143923903083574)
--(axis cs:69.4267515923567,0.0140198809493863)
--(axis cs:70.0636942675159,0.0146682563577118)
--(axis cs:70.7006369426752,0.0112021930047146)
--(axis cs:71.3375796178344,0.0104543532709671)
--(axis cs:71.9745222929936,0.0105176887483959)
--(axis cs:72.6114649681529,0.00982295638261012)
--(axis cs:73.2484076433121,0.0102703309912608)
--(axis cs:73.8853503184713,0.00941221520642582)
--(axis cs:74.5222929936306,0.0103096330964381)
--(axis cs:75.1592356687898,0.00875954784103856)
--(axis cs:75.796178343949,0.00656079000912262)
--(axis cs:76.4331210191083,0.00446237135323777)
--(axis cs:77.0700636942675,0.00248463651299912)
--(axis cs:77.7070063694268,0.00219717214950018)
--(axis cs:78.343949044586,0.000722890577560107)
--(axis cs:78.9808917197452,0.000497663601256194)
--(axis cs:79.6178343949044,0.00039625199090585)
--(axis cs:80.2547770700637,0.000565566313518918)
--(axis cs:80.8917197452229,0.000599458348764193)
--(axis cs:81.5286624203822,0.000369774796623572)
--(axis cs:82.1656050955414,0.000188130577673781)
--(axis cs:82.8025477707006,0.000277648696433037)
--(axis cs:83.4394904458599,0.000435934716613415)
--(axis cs:84.0764331210191,0.000295623066078855)
--(axis cs:84.7133757961783,0.000132183498710475)
--(axis cs:85.3503184713376,0.000182778522458399)
--(axis cs:85.9872611464968,0.00021585494142825)
--(axis cs:86.6242038216561,0.000120230646841658)
--(axis cs:87.2611464968153,7.08581266860264e-05)
--(axis cs:87.8980891719745,4.54329550048309e-05)
--(axis cs:88.5350318471338,-1.17845006431699e-05)
--(axis cs:89.171974522293,5.85136893402518e-06)
--(axis cs:89.8089171974522,3.74588374308811e-06)
--(axis cs:90.4458598726115,1.60364924423079e-05)
--(axis cs:91.0828025477707,-1.02564261663147e-05)
--(axis cs:91.7197452229299,5.48295289972377e-07)
--(axis cs:92.3566878980892,-2.43600211803029e-05)
--(axis cs:92.9936305732484,8.51868520803065e-06)
--(axis cs:93.6305732484076,7.46165385401359e-06)
--(axis cs:94.2675159235669,7.08154968494277e-06)
--(axis cs:94.9044585987261,5.94474265502767e-06)
--(axis cs:95.5414012738853,6.99295692941528e-06)
--(axis cs:96.1783439490446,6.91815130001578e-06)
--(axis cs:96.8152866242038,7.38905454548214e-06)
--(axis cs:97.4522292993631,7.1171295624296e-06)
--(axis cs:98.0891719745223,7.06742668613312e-06)
--(axis cs:98.7261146496815,4.7336270038791e-06)
--(axis cs:99.3630573248408,1.92327047525471e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,2.56452057516126e-06)
--(axis cs:98.7261146496815,5.77745789537713e-06)
--(axis cs:98.0891719745223,7.61146402266379e-06)
--(axis cs:97.4522292993631,8.12056489476232e-06)
--(axis cs:96.8152866242038,8.30453491658697e-06)
--(axis cs:96.1783439490446,9.14466773894201e-06)
--(axis cs:95.5414012738853,8.63331541844202e-06)
--(axis cs:94.9044585987261,1.06128216030463e-05)
--(axis cs:94.2675159235669,9.50934436658082e-06)
--(axis cs:93.6305732484076,1.50375728908362e-05)
--(axis cs:92.9936305732484,1.74255474322286e-05)
--(axis cs:92.3566878980892,8.34152452897873e-05)
--(axis cs:91.7197452229299,5.43517672045327e-05)
--(axis cs:91.0828025477707,0.000174545629821739)
--(axis cs:90.4458598726115,0.000220500177311478)
--(axis cs:89.8089171974522,8.25970620359007e-05)
--(axis cs:89.171974522293,0.000122372300571732)
--(axis cs:88.5350318471338,0.000307958057329042)
--(axis cs:87.8980891719745,0.000213380705107644)
--(axis cs:87.2611464968153,0.000646474666488949)
--(axis cs:86.6242038216561,0.000744195670325402)
--(axis cs:85.9872611464968,0.000963203072872314)
--(axis cs:85.3503184713376,0.00101483362728997)
--(axis cs:84.7133757961783,0.000986176077620435)
--(axis cs:84.0764331210191,0.00111616827932586)
--(axis cs:83.4394904458599,0.00169572563892493)
--(axis cs:82.8025477707006,0.00114867846507874)
--(axis cs:82.1656050955414,0.000725109196795647)
--(axis cs:81.5286624203822,0.00105366262148081)
--(axis cs:80.8917197452229,0.00145229778493964)
--(axis cs:80.2547770700637,0.00145762989693744)
--(axis cs:79.6178343949044,0.00115070982038349)
--(axis cs:78.9808917197452,0.00133527128958177)
--(axis cs:78.343949044586,0.00189664639109339)
--(axis cs:77.7070063694268,0.00445601863351702)
--(axis cs:77.0700636942675,0.00465542722750355)
--(axis cs:76.4331210191083,0.00748766534658274)
--(axis cs:75.796178343949,0.0100045041104085)
--(axis cs:75.1592356687898,0.0124479903754842)
--(axis cs:74.5222929936306,0.0142977488480294)
--(axis cs:73.8853503184713,0.0132776457050907)
--(axis cs:73.2484076433121,0.0144210149061719)
--(axis cs:72.6114649681529,0.0137652538587634)
--(axis cs:71.9745222929936,0.0145564247426046)
--(axis cs:71.3375796178344,0.0144765425096758)
--(axis cs:70.7006369426752,0.0154348214931994)
--(axis cs:70.0636942675159,0.0195037864284866)
--(axis cs:69.4267515923567,0.0189992397126319)
--(axis cs:68.7898089171974,0.0194155074237759)
--(axis cs:68.1528662420382,0.0226492398202913)
--(axis cs:67.515923566879,0.0216612180101853)
--(axis cs:66.8789808917197,0.0214185940371213)
--(axis cs:66.2420382165605,0.0221103718396729)
--(axis cs:65.6050955414013,0.0246317378832548)
--(axis cs:64.968152866242,0.0258354421695011)
--(axis cs:64.3312101910828,0.0283651114044194)
--(axis cs:63.6942675159236,0.0322623996622446)
--(axis cs:63.0573248407643,0.0328613950507256)
--(axis cs:62.4203821656051,0.0348523468234337)
--(axis cs:61.7834394904459,0.0376007408414463)
--(axis cs:61.1464968152866,0.0371849115812614)
--(axis cs:60.5095541401274,0.0405530897336908)
--(axis cs:59.8726114649682,0.042624089079725)
--(axis cs:59.2356687898089,0.0459901918758251)
--(axis cs:58.5987261146497,0.0477362932809168)
--(axis cs:57.9617834394904,0.0520660745102945)
--(axis cs:57.3248407643312,0.0564931863950797)
--(axis cs:56.687898089172,0.0587680702503905)
--(axis cs:56.0509554140127,0.0640846410480524)
--(axis cs:55.4140127388535,0.0643173254189496)
--(axis cs:54.7770700636943,0.0668391565894495)
--(axis cs:54.140127388535,0.0692691095386432)
--(axis cs:53.5031847133758,0.0689748975302003)
--(axis cs:52.8662420382166,0.0743008808763503)
--(axis cs:52.2292993630573,0.0764976828267074)
--(axis cs:51.5923566878981,0.0739038680920976)
--(axis cs:50.9554140127388,0.0796932266740261)
--(axis cs:50.3184713375796,0.083780758900673)
--(axis cs:49.6815286624204,0.0850811987684099)
--(axis cs:49.0445859872611,0.0935769007058658)
--(axis cs:48.4076433121019,0.0983766093523057)
--(axis cs:47.7707006369427,0.0986612592473391)
--(axis cs:47.1337579617834,0.0993045649938156)
--(axis cs:46.4968152866242,0.10746266591495)
--(axis cs:45.859872611465,0.115118163557276)
--(axis cs:45.2229299363057,0.121455076869572)
--(axis cs:44.5859872611465,0.123821163028547)
--(axis cs:43.9490445859873,0.128109792933618)
--(axis cs:43.312101910828,0.129844420282452)
--(axis cs:42.6751592356688,0.133832820238487)
--(axis cs:42.0382165605096,0.138322692929284)
--(axis cs:41.4012738853503,0.143767655995315)
--(axis cs:40.7643312101911,0.143806046661733)
--(axis cs:40.1273885350318,0.146443213638399)
--(axis cs:39.4904458598726,0.151145174928318)
--(axis cs:38.8535031847134,0.159562323174688)
--(axis cs:38.2165605095541,0.164277992464567)
--(axis cs:37.5796178343949,0.165275359944646)
--(axis cs:36.9426751592357,0.175154595312181)
--(axis cs:36.3057324840764,0.182926217511216)
--(axis cs:35.6687898089172,0.195212937327197)
--(axis cs:35.031847133758,0.199129611303007)
--(axis cs:34.3949044585987,0.205390502165352)
--(axis cs:33.7579617834395,0.219592468528877)
--(axis cs:33.1210191082803,0.224991721562319)
--(axis cs:32.484076433121,0.238071560539655)
--(axis cs:31.8471337579618,0.253216787779538)
--(axis cs:31.2101910828025,0.259366982515557)
--(axis cs:30.5732484076433,0.269336690606786)
--(axis cs:29.9363057324841,0.282740716460878)
--(axis cs:29.2993630573248,0.297660701079602)
--(axis cs:28.6624203821656,0.307541239028284)
--(axis cs:28.0254777070064,0.320623923360059)
--(axis cs:27.3885350318471,0.335766108336089)
--(axis cs:26.7515923566879,0.340075745976621)
--(axis cs:26.1146496815287,0.355721937957708)
--(axis cs:25.4777070063694,0.373112722749391)
--(axis cs:24.8407643312102,0.390617443201535)
--(axis cs:24.203821656051,0.404283983670245)
--(axis cs:23.5668789808917,0.412929815849294)
--(axis cs:22.9299363057325,0.429770144744285)
--(axis cs:22.2929936305732,0.444755043497136)
--(axis cs:21.656050955414,0.463551752936656)
--(axis cs:21.0191082802548,0.483364861578263)
--(axis cs:20.3821656050955,0.507469032156407)
--(axis cs:19.7452229299363,0.533970765441181)
--(axis cs:19.1082802547771,0.548643129798858)
--(axis cs:18.4713375796178,0.571856120260958)
--(axis cs:17.8343949044586,0.592044427434502)
--(axis cs:17.1974522292994,0.612657597767265)
--(axis cs:16.5605095541401,0.634219530672033)
--(axis cs:15.9235668789809,0.660559712594305)
--(axis cs:15.2866242038217,0.677527040380679)
--(axis cs:14.6496815286624,0.699066068162492)
--(axis cs:14.0127388535032,0.718804343554237)
--(axis cs:13.3757961783439,0.733202815764832)
--(axis cs:12.7388535031847,0.752595886268131)
--(axis cs:12.1019108280255,0.777084052392931)
--(axis cs:11.4649681528662,0.790541110954733)
--(axis cs:10.828025477707,0.806503052544856)
--(axis cs:10.1910828025478,0.825445703466058)
--(axis cs:9.55414012738853,0.844035455197118)
--(axis cs:8.9171974522293,0.855000971590692)
--(axis cs:8.28025477707006,0.865947770536246)
--(axis cs:7.64331210191083,0.878649171413771)
--(axis cs:7.00636942675159,0.887802361181005)
--(axis cs:6.36942675159236,0.894634502342896)
--(axis cs:5.73248407643312,0.899899152054661)
--(axis cs:5.09554140127389,0.905298358084396)
--(axis cs:4.45859872611465,0.908125691112207)
--(axis cs:3.82165605095541,0.910662183947401)
--(axis cs:3.18471337579618,0.912857257190564)
--(axis cs:2.54777070063694,0.914272169347646)
--(axis cs:1.91082802547771,0.914823361508382)
--(axis cs:1.27388535031847,0.915424191086407)
--(axis cs:0.636942675159236,0.915866689675284)
--(axis cs:0,0.916100204106519)
--cycle;


==> img/mnist/mnist_rate_distortion_sfw_order_var_c.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.915533622518415
0.636942675159236 0.915216629240895
1.27388535031847 0.914852436120855
1.91082802547771 0.913848142977804
2.54777070063694 0.912805236661807
3.18471337579618 0.910642956383526
3.82165605095541 0.90819951237645
4.45859872611465 0.906264711478725
5.09554140127389 0.901651042914018
5.73248407643312 0.895875334460288
6.36942675159236 0.891025217741262
7.00636942675159 0.882639986159047
7.64331210191083 0.871856895346427
8.28025477707006 0.858422579172766
8.9171974522293 0.841620970856165
9.55414012738853 0.82629980121972
10.1910828025478 0.811000777943991
10.828025477707 0.794253139944049
11.4649681528662 0.772226762246573
12.1019108280255 0.751880480269902
12.7388535031847 0.733356558619998
13.3757961783439 0.713772723994916
14.0127388535032 0.699341398440301
14.6496815286624 0.682881770210806
15.2866242038217 0.663359494855395
15.9235668789809 0.643602287654066
16.5605095541401 0.625392557596788
17.1974522292994 0.61358642189065
17.8343949044586 0.591002705292776
18.4713375796178 0.568670407494064
19.1082802547771 0.552752569788136
19.7452229299363 0.532435087715276
20.3821656050955 0.513139311620034
21.0191082802548 0.493321174851153
21.656050955414 0.470009315506322
22.2929936305732 0.461631678030826
22.9299363057325 0.438674655349459
23.5668789808917 0.424483320419677
24.203821656051 0.408897705967538
24.8407643312102 0.399823740668362
25.4777070063694 0.39469262769795
26.1146496815287 0.382062000461738
26.7515923566879 0.371762510728149
27.3885350318471 0.36067994269979
28.0254777070064 0.351099519467862
28.6624203821656 0.341111075097506
29.2993630573248 0.331034429492574
29.9363057324841 0.321158117230116
30.5732484076433 0.31543965375211
31.2101910828025 0.297268373926054
31.8471337579618 0.290349764012835
32.484076433121 0.283082903002705
33.1210191082803 0.275213184868612
33.7579617834395 0.265222703067707
34.3949044585987 0.254260917420916
35.031847133758 0.249990099414836
35.6687898089172 0.239414868208701
36.3057324840764 0.226467341405881
36.9426751592357 0.221328515321149
37.5796178343949 0.210052850920171
38.2165605095541 0.199918682966887
38.8535031847134 0.195369573186773
39.4904458598726 0.189702624965278
40.1273885350318 0.183921363139828
40.7643312101911 0.176496909781578
41.4012738853503 0.172531189359132
42.0382165605096 0.168123732327527
42.6751592356688 0.16734255395532
43.312101910828 0.152256214091912
43.9490445859873 0.152787629992841
44.5859872611465 0.148673288264021
45.2229299363057 0.148547341046634
45.859872611465 0.146671408367549
46.4968152866242 0.145588004963394
47.1337579617834 0.133070213190256
47.7707006369427 0.12768154695641
48.4076433121019 0.123473785355372
49.0445859872611 0.118114556675049
49.6815286624204 0.111485894172005
50.3184713375796 0.109037148149852
50.9554140127388 0.104301870774725
51.5923566878981 0.0996213651309988
52.2292993630573 0.0996434471917869
52.8662420382166 0.0944132084746329
53.5031847133758 0.0951949803886941
54.140127388535 0.0967076074755589
54.7770700636943 0.0901489561600242
55.4140127388535 0.091773472993515
56.0509554140127 0.0854756113653705
56.687898089172 0.0858188014163321
57.3248407643312 0.0869270538487275
57.9617834394904 0.0829195231916092
58.5987261146497 0.0764383891636854
59.2356687898089 0.076298275588048
59.8726114649682 0.0708809756929044
60.5095541401274 0.0643563619674639
61.1464968152866 0.0636175437198572
61.7834394904459 0.0605805774076963
62.4203821656051 0.0608623595341473
63.0573248407643 0.0606164629904616
63.6942675159236 0.0585968427825993
64.3312101910828 0.0545675831085274
64.968152866242 0.0531595909216789
65.6050955414013 0.0481934022733792
66.2420382165605 0.0456070098342904
66.8789808917197 0.042299434984539
67.515923566879 0.0413167071770357
68.1528662420382 0.0417387974472639
68.7898089171974 0.0366657525185878
69.4267515923567 0.0322248989369867
70.0636942675159 0.0292280717496279
70.7006369426752 0.0236978682387493
71.3375796178344 0.0196203219580634
71.9745222929936 0.017569275208996
72.6114649681529 0.016219347734527
73.2484076433121 0.017376315692959
73.8853503184713 0.0155358970459101
74.5222929936306 0.0133575634233673
75.1592356687898 0.0127438484666063
75.796178343949 0.0140774955454799
76.4331210191083 0.0170205283600912
77.0700636942675 0.0140971931758961
77.7070063694268 0.0148755222594156
78.343949044586 0.0167520366788315
78.9808917197452 0.016918486831895
79.6178343949044 0.0156248553519913
80.2547770700637 0.0135916439476378
80.8917197452229 0.0146711093342738
81.5286624203822 0.013845758266204
82.1656050955414 0.015075071423308
82.8025477707006 0.0119500971131197
83.4394904458599 0.0104622078354255
84.0764331210191 0.0117047070635601
84.7133757961783 0.0132785411624004
85.3503184713376 0.0133989631459661
85.9872611464968 0.0119533870482632
86.6242038216561 0.0105117077759466
87.2611464968153 0.00603811207041584
87.8980891719745 0.00860201425475665
88.5350318471338 0.00729488650405663
89.171974522293 0.00656193315127005
89.8089171974522 0.00572011431835272
90.4458598726115 0.00557226016808746
91.0828025477707 0.00412212285688138
91.7197452229299 0.00325473751672884
92.3566878980892 0.00105952822102944
92.9936305732484 0.000948714666765559
93.6305732484076 0.000590272265237939
94.2675159235669 0.000209871222510302
94.9044585987261 5.61496439273651e-05
95.5414012738853 5.33374931823116e-05
96.1783439490446 4.20373769886423e-05
96.8152866242038 2.26858457851087e-05
97.4522292993631 4.58569915183227e-05
98.0891719745223 3.79960387870287e-05
98.7261146496815 1.05034151570671e-05
99.3630573248408 3.28706204181406e-06
100 2.9135449608475e-11
};
\path [fill=color1, fill opacity=0.25] 
(axis cs:0,0.91611892509782)
--(axis cs:0,0.91494831993901)
--(axis cs:0.636942675159236,0.91459002319611)
--(axis cs:1.27388535031847,0.914142207878221)
--(axis cs:1.91082802547771,0.912966552359848)
--(axis cs:2.54777070063694,0.911695038006893)
--(axis cs:3.18471337579618,0.909159194489714)
--(axis cs:3.82165605095541,0.906462577227334)
--(axis cs:4.45859872611465,0.904363840492754)
--(axis cs:5.09554140127389,0.899216889551194)
--(axis cs:5.73248407643312,0.89286183378278)
--(axis cs:6.36942675159236,0.887710703929483)
--(axis cs:7.00636942675159,0.878705595606517)
--(axis cs:7.64331210191083,0.86727088579871)
--(axis cs:8.28025477707006,0.85316240650855)
--(axis cs:8.9171974522293,0.835762783249664)
--(axis cs:9.55414012738853,0.820034933202351)
--(axis cs:10.1910828025478,0.804362498484446)
--(axis cs:10.828025477707,0.787361715162042)
--(axis cs:11.4649681528662,0.765120364740191)
--(axis cs:12.1019108280255,0.744822635103801)
--(axis cs:12.7388535031847,0.726065542317129)
--(axis cs:13.3757961783439,0.706463340224061)
--(axis cs:14.0127388535032,0.691814296802156)
--(axis cs:14.6496815286624,0.675239898270429)
--(axis cs:15.2866242038217,0.655516398297201)
--(axis cs:15.9235668789809,0.635746835232494)
--(axis cs:16.5605095541401,0.617284111890893)
--(axis cs:17.1974522292994,0.605440344554614)
--(axis cs:17.8343949044586,0.582748222202822)
--(axis cs:18.4713375796178,0.560294849553481)
--(axis cs:19.1082802547771,0.544417129910431)
--(axis cs:19.7452229299363,0.523812991113478)
--(axis cs:20.3821656050955,0.504660121784425)
--(axis cs:21.0191082802548,0.484803420346542)
--(axis cs:21.656050955414,0.461614544450972)
--(axis cs:22.2929936305732,0.453282766232357)
--(axis cs:22.9299363057325,0.430340533253324)
--(axis cs:23.5668789808917,0.416310276047389)
--(axis cs:24.203821656051,0.400875595978034)
--(axis cs:24.8407643312102,0.391993946008907)
--(axis cs:25.4777070063694,0.386784589539061)
--(axis cs:26.1146496815287,0.374243818603239)
--(axis cs:26.7515923566879,0.364030015958715)
--(axis cs:27.3885350318471,0.352953630799222)
--(axis cs:28.0254777070064,0.343392371716515)
--(axis cs:28.6624203821656,0.333532642571078)
--(axis cs:29.2993630573248,0.32355230085953)
--(axis cs:29.9363057324841,0.313643023853629)
--(axis cs:30.5732484076433,0.30780765496487)
--(axis cs:31.2101910828025,0.289832926003118)
--(axis cs:31.8471337579618,0.283104904868101)
--(axis cs:32.484076433121,0.275902412022337)
--(axis cs:33.1210191082803,0.268042331820633)
--(axis cs:33.7579617834395,0.258130390486935)
--(axis cs:34.3949044585987,0.247268612279911)
--(axis cs:35.031847133758,0.243015041914204)
--(axis cs:35.6687898089172,0.232619492345863)
--(axis cs:36.3057324840764,0.219822408500039)
--(axis cs:36.9426751592357,0.214786761990631)
--(axis cs:37.5796178343949,0.203607007462839)
--(axis cs:38.2165605095541,0.19337027750926)
--(axis cs:38.8535031847134,0.188773462214056)
--(axis cs:39.4904458598726,0.183225107705744)
--(axis cs:40.1273885350318,0.177532722695641)
--(axis cs:40.7643312101911,0.170142698194182)
--(axis cs:41.4012738853503,0.166214315730536)
--(axis cs:42.0382165605096,0.161914738211509)
--(axis cs:42.6751592356688,0.1611525712237)
--(axis cs:43.312101910828,0.14634411098654)
--(axis cs:43.9490445859873,0.146996676739327)
--(axis cs:44.5859872611465,0.142947410273865)
--(axis cs:45.2229299363057,0.142697199210086)
--(axis cs:45.859872611465,0.141033818638292)
--(axis cs:46.4968152866242,0.139953855204814)
--(axis cs:47.1337579617834,0.127828871698743)
--(axis cs:47.7707006369427,0.122465098990557)
--(axis cs:48.4076433121019,0.118234224883799)
--(axis cs:49.0445859872611,0.113052884161018)
--(axis cs:49.6815286624204,0.106625903853408)
--(axis cs:50.3184713375796,0.104425272233276)
--(axis cs:50.9554140127388,0.0997719764116755)
--(axis cs:51.5923566878981,0.0951461889741575)
--(axis cs:52.2292993630573,0.0950884922656722)
--(axis cs:52.8662420382166,0.089865428861757)
--(axis cs:53.5031847133758,0.0904307574815059)
--(axis cs:54.140127388535,0.0920060109079061)
--(axis cs:54.7770700636943,0.0854532830345037)
--(axis cs:55.4140127388535,0.0869902317292895)
--(axis cs:56.0509554140127,0.0807041960562749)
--(axis cs:56.687898089172,0.080989868546255)
--(axis cs:57.3248407643312,0.0821411300843397)
--(axis cs:57.9617834394904,0.0781677700053875)
--(axis cs:58.5987261146497,0.0718194261740387)
--(axis cs:59.2356687898089,0.0717511183163665)
--(axis cs:59.8726114649682,0.0662914658536524)
--(axis cs:60.5095541401274,0.0600279996134492)
--(axis cs:61.1464968152866,0.0593341398031965)
--(axis cs:61.7834394904459,0.0563378486269006)
--(axis cs:62.4203821656051,0.0567842449794234)
--(axis cs:63.0573248407643,0.0566946790555302)
--(axis cs:63.6942675159236,0.0548166703837829)
--(axis cs:64.3312101910828,0.0508580720571847)
--(axis cs:64.968152866242,0.0495008230435482)
--(axis cs:65.6050955414013,0.0447231227465476)
--(axis cs:66.2420382165605,0.0422250255796786)
--(axis cs:66.8789808917197,0.0388975298226837)
--(axis cs:67.515923566879,0.038093203739343)
--(axis cs:68.1528662420382,0.0385440918286079)
--(axis cs:68.7898089171974,0.0334691757603729)
--(axis cs:69.4267515923567,0.0292500870266174)
--(axis cs:70.0636942675159,0.0264139756023685)
--(axis cs:70.7006369426752,0.0210373206389086)
--(axis cs:71.3375796178344,0.0171527075628321)
--(axis cs:71.9745222929936,0.0154926749643221)
--(axis cs:72.6114649681529,0.0141092579649914)
--(axis cs:73.2484076433121,0.0152594529168747)
--(axis cs:73.8853503184713,0.0136242190338702)
--(axis cs:74.5222929936306,0.0114482407878081)
--(axis cs:75.1592356687898,0.0108620000730461)
--(axis cs:75.796178343949,0.0122136054985082)
--(axis cs:76.4331210191083,0.0150331551092136)
--(axis cs:77.0700636942675,0.0122146123622423)
--(axis cs:77.7070063694268,0.0129773101146902)
--(axis cs:78.343949044586,0.0147703959328814)
--(axis cs:78.9808917197452,0.0149465491704185)
--(axis cs:79.6178343949044,0.0136563840933332)
--(axis cs:80.2547770700637,0.0116697590837193)
--(axis cs:80.8917197452229,0.0128030603256895)
--(axis cs:81.5286624203822,0.0120432039559219)
--(axis cs:82.1656050955414,0.0132884352239765)
--(axis cs:82.8025477707006,0.0103045341810375)
--(axis cs:83.4394904458599,0.00890232604996648)
--(axis cs:84.0764331210191,0.0100271206976644)
--(axis cs:84.7133757961783,0.0115142758886039)
--(axis cs:85.3503184713376,0.011671901046953)
--(axis cs:85.9872611464968,0.0103046573315181)
--(axis cs:86.6242038216561,0.00897614731789797)
--(axis cs:87.2611464968153,0.00481310016386909)
--(axis cs:87.8980891719745,0.00729471736329136)
--(axis cs:88.5350318471338,0.00610022961597168)
--(axis cs:89.171974522293,0.00534287514507939)
--(axis cs:89.8089171974522,0.00460650370051432)
--(axis cs:90.4458598726115,0.00450253783905918)
--(axis cs:91.0828025477707,0.00316508903232457)
--(axis cs:91.7197452229299,0.0024019258544299)
--(axis cs:92.3566878980892,0.000688872001772621)
--(axis cs:92.9936305732484,0.000567374189867294)
--(axis cs:93.6305732484076,0.000313211280499794)
--(axis cs:94.2675159235669,0.000103830381936905)
--(axis cs:94.9044585987261,2.15450929612326e-05)
--(axis cs:95.5414012738853,1.98157393534125e-05)
--(axis cs:96.1783439490446,1.46894932709149e-05)
--(axis cs:96.8152866242038,1.11617579270527e-05)
--(axis cs:97.4522292993631,2.86627943191164e-05)
--(axis cs:98.0891719745223,2.30089275627621e-05)
--(axis cs:98.7261146496815,6.4189208955279e-06)
--(axis cs:99.3630573248408,2.82552132741158e-06)
--(axis cs:100,2.9135449608475e-11)
--(axis cs:100,2.9135449608475e-11)
--(axis cs:100,2.9135449608475e-11)
--(axis cs:99.3630573248408,3.74860275621654e-06)
--(axis cs:98.7261146496815,1.45879094186063e-05)
--(axis cs:98.0891719745223,5.29831500112953e-05)
--(axis cs:97.4522292993631,6.3051188717529e-05)
--(axis cs:96.8152866242038,3.42099336431647e-05)
--(axis cs:96.1783439490446,6.93852607063697e-05)
--(axis cs:95.5414012738853,8.68592470112107e-05)
--(axis cs:94.9044585987261,9.07541948934976e-05)
--(axis cs:94.2675159235669,0.000315912063083698)
--(axis cs:93.6305732484076,0.000867333249976084)
--(axis cs:92.9936305732484,0.00133005514366382)
--(axis cs:92.3566878980892,0.00143018444028626)
--(axis cs:91.7197452229299,0.00410754917902779)
--(axis cs:91.0828025477707,0.00507915668143818)
--(axis cs:90.4458598726115,0.00664198249711574)
--(axis cs:89.8089171974522,0.00683372493619112)
--(axis cs:89.171974522293,0.00778099115746071)
--(axis cs:88.5350318471338,0.00848954339214159)
--(axis cs:87.8980891719745,0.00990931114622193)
--(axis cs:87.2611464968153,0.00726312397696258)
--(axis cs:86.6242038216561,0.0120472682339953)
--(axis cs:85.9872611464968,0.0136021167650084)
--(axis cs:85.3503184713376,0.0151260252449792)
--(axis cs:84.7133757961783,0.0150428064361969)
--(axis cs:84.0764331210191,0.0133822934294558)
--(axis cs:83.4394904458599,0.0120220896208845)
--(axis cs:82.8025477707006,0.0135956600452019)
--(axis cs:82.1656050955414,0.0168617076226395)
--(axis cs:81.5286624203822,0.0156483125764861)
--(axis cs:80.8917197452229,0.0165391583428582)
--(axis cs:80.2547770700637,0.0155135288115564)
--(axis cs:79.6178343949044,0.0175933266106494)
--(axis cs:78.9808917197452,0.0188904244933715)
--(axis cs:78.343949044586,0.0187336774247815)
--(axis cs:77.7070063694268,0.0167737344041411)
--(axis cs:77.0700636942675,0.0159797739895498)
--(axis cs:76.4331210191083,0.0190079016109687)
--(axis cs:75.796178343949,0.0159413855924515)
--(axis cs:75.1592356687898,0.0146256968601665)
--(axis cs:74.5222929936306,0.0152668860589265)
--(axis cs:73.8853503184713,0.0174475750579501)
--(axis cs:73.2484076433121,0.0194931784690433)
--(axis cs:72.6114649681529,0.0183294375040626)
--(axis cs:71.9745222929936,0.0196458754536698)
--(axis cs:71.3375796178344,0.0220879363532947)
--(axis cs:70.7006369426752,0.02635841583859)
--(axis cs:70.0636942675159,0.0320421678968872)
--(axis cs:69.4267515923567,0.0351997108473559)
--(axis cs:68.7898089171974,0.0398623292768027)
--(axis cs:68.1528662420382,0.04493350306592)
--(axis cs:67.515923566879,0.0445402106147283)
--(axis cs:66.8789808917197,0.0457013401463943)
--(axis cs:66.2420382165605,0.0489889940889021)
--(axis cs:65.6050955414013,0.0516636818002107)
--(axis cs:64.968152866242,0.0568183587998096)
--(axis cs:64.3312101910828,0.05827709415987)
--(axis cs:63.6942675159236,0.0623770151814156)
--(axis cs:63.0573248407643,0.064538246925393)
--(axis cs:62.4203821656051,0.0649404740888712)
--(axis cs:61.7834394904459,0.064823306188492)
--(axis cs:61.1464968152866,0.0679009476365179)
--(axis cs:60.5095541401274,0.0686847243214787)
--(axis cs:59.8726114649682,0.0754704855321565)
--(axis cs:59.2356687898089,0.0808454328597296)
--(axis cs:58.5987261146497,0.0810573521533321)
--(axis cs:57.9617834394904,0.0876712763778308)
--(axis cs:57.3248407643312,0.0917129776131154)
--(axis cs:56.687898089172,0.0906477342864092)
--(axis cs:56.0509554140127,0.0902470266744661)
--(axis cs:55.4140127388535,0.0965567142577406)
--(axis cs:54.7770700636943,0.0948446292855447)
--(axis cs:54.140127388535,0.101409204043212)
--(axis cs:53.5031847133758,0.0999592032958822)
--(axis cs:52.8662420382166,0.0989609880875088)
--(axis cs:52.2292993630573,0.104198402117902)
--(axis cs:51.5923566878981,0.10409654128784)
--(axis cs:50.9554140127388,0.108831765137774)
--(axis cs:50.3184713375796,0.113649024066428)
--(axis cs:49.6815286624204,0.116345884490602)
--(axis cs:49.0445859872611,0.123176229189081)
--(axis cs:48.4076433121019,0.128713345826946)
--(axis cs:47.7707006369427,0.132897994922262)
--(axis cs:47.1337579617834,0.138311554681769)
--(axis cs:46.4968152866242,0.151222154721975)
--(axis cs:45.859872611465,0.152308998096806)
--(axis cs:45.2229299363057,0.154397482883182)
--(axis cs:44.5859872611465,0.154399166254177)
--(axis cs:43.9490445859873,0.158578583246355)
--(axis cs:43.312101910828,0.158168317197284)
--(axis cs:42.6751592356688,0.173532536686939)
--(axis cs:42.0382165605096,0.174332726443544)
--(axis cs:41.4012738853503,0.178848062987728)
--(axis cs:40.7643312101911,0.182851121368974)
--(axis cs:40.1273885350318,0.190310003584014)
--(axis cs:39.4904458598726,0.196180142224812)
--(axis cs:38.8535031847134,0.20196568415949)
--(axis cs:38.2165605095541,0.206467088424513)
--(axis cs:37.5796178343949,0.216498694377502)
--(axis cs:36.9426751592357,0.227870268651667)
--(axis cs:36.3057324840764,0.233112274311723)
--(axis cs:35.6687898089172,0.246210244071539)
--(axis cs:35.031847133758,0.256965156915467)
--(axis cs:34.3949044585987,0.26125322256192)
--(axis cs:33.7579617834395,0.272315015648479)
--(axis cs:33.1210191082803,0.282384037916591)
--(axis cs:32.484076433121,0.290263393983073)
--(axis cs:31.8471337579618,0.297594623157569)
--(axis cs:31.2101910828025,0.304703821848989)
--(axis cs:30.5732484076433,0.32307165253935)
--(axis cs:29.9363057324841,0.328673210606603)
--(axis cs:29.2993630573248,0.338516558125619)
--(axis cs:28.6624203821656,0.348689507623934)
--(axis cs:28.0254777070064,0.358806667219208)
--(axis cs:27.3885350318471,0.368406254600357)
--(axis cs:26.7515923566879,0.379495005497583)
--(axis cs:26.1146496815287,0.389880182320236)
--(axis cs:25.4777070063694,0.402600665856839)
--(axis cs:24.8407643312102,0.407653535327817)
--(axis cs:24.203821656051,0.416919815957042)
--(axis cs:23.5668789808917,0.432656364791964)
--(axis cs:22.9299363057325,0.447008777445595)
--(axis cs:22.2929936305732,0.469980589829296)
--(axis cs:21.656050955414,0.478404086561672)
--(axis cs:21.0191082802548,0.501838929355764)
--(axis cs:20.3821656050955,0.521618501455643)
--(axis cs:19.7452229299363,0.541057184317073)
--(axis cs:19.1082802547771,0.56108800966584)
--(axis cs:18.4713375796178,0.577045965434647)
--(axis cs:17.8343949044586,0.599257188382731)
--(axis cs:17.1974522292994,0.621732499226685)
--(axis cs:16.5605095541401,0.633501003302682)
--(axis cs:15.9235668789809,0.651457740075639)
--(axis cs:15.2866242038217,0.671202591413588)
--(axis cs:14.6496815286624,0.690523642151184)
--(axis cs:14.0127388535032,0.706868500078447)
--(axis cs:13.3757961783439,0.721082107765772)
--(axis cs:12.7388535031847,0.740647574922868)
--(axis cs:12.1019108280255,0.758938325436002)
--(axis cs:11.4649681528662,0.779333159752956)
--(axis cs:10.828025477707,0.801144564726055)
--(axis cs:10.1910828025478,0.817639057403537)
--(axis cs:9.55414012738853,0.83256466923709)
--(axis cs:8.9171974522293,0.847479158462667)
--(axis cs:8.28025477707006,0.863682751836982)
--(axis cs:7.64331210191083,0.876442904894144)
--(axis cs:7.00636942675159,0.886574376711577)
--(axis cs:6.36942675159236,0.894339731553042)
--(axis cs:5.73248407643312,0.898888835137797)
--(axis cs:5.09554140127389,0.904085196276842)
--(axis cs:4.45859872611465,0.908165582464696)
--(axis cs:3.82165605095541,0.909936447525566)
--(axis cs:3.18471337579618,0.912126718277339)
--(axis cs:2.54777070063694,0.913915435316721)
--(axis cs:1.91082802547771,0.91472973359576)
--(axis cs:1.27388535031847,0.915562664363489)
--(axis cs:0.636942675159236,0.915843235285679)
--(axis cs:0,0.91611892509782)
--cycle;



==> img/mnist/mnist_rate_distortion_sfw_order_var_d.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.915463412238751
0.636942675159236 0.915249786601635
1.27388535031847 0.9148494111537
1.91082802547771 0.914150328706019
2.54777070063694 0.913250223268988
3.18471337579618 0.911209362689406
3.82165605095541 0.908752526571043
4.45859872611465 0.905458561767591
5.09554140127389 0.900819537361967
5.73248407643312 0.894747238381533
6.36942675159236 0.889301288051065
7.00636942675159 0.881389770070091
7.64331210191083 0.869510568379774
8.28025477707006 0.855693476812448
8.9171974522293 0.844225098426687
9.55414012738853 0.827577435167623
10.1910828025478 0.812775752173038
10.828025477707 0.787498083594255
11.4649681528662 0.771917516151443
12.1019108280255 0.754227760592476
12.7388535031847 0.73798156177043
13.3757961783439 0.718231366885011
14.0127388535032 0.697390856088605
14.6496815286624 0.67472047055955
15.2866242038217 0.663128405456664
15.9235668789809 0.644366064902861
16.5605095541401 0.628848755587824
17.1974522292994 0.609820116035407
17.8343949044586 0.594020391103113
18.4713375796178 0.573622045837692
19.1082802547771 0.554163470168132
19.7452229299363 0.528461211157846
20.3821656050955 0.513305909985211
21.0191082802548 0.490597823542776
21.656050955414 0.471201759799151
22.2929936305732 0.457380540601444
22.9299363057325 0.444681945886696
23.5668789808917 0.42452654160923
24.203821656051 0.412583470899553
24.8407643312102 0.402659694352187
25.4777070063694 0.390103940285335
26.1146496815287 0.373981101342652
26.7515923566879 0.363216804647964
27.3885350318471 0.35004143155089
28.0254777070064 0.341146918583254
28.6624203821656 0.33305857337582
29.2993630573248 0.323198976768035
29.9363057324841 0.311926903249514
30.5732484076433 0.299828838966223
31.2101910828025 0.292240771559336
31.8471337579618 0.272840151806549
32.484076433121 0.267103292753127
33.1210191082803 0.256106787913567
33.7579617834395 0.249556746049702
34.3949044585987 0.238406419424212
35.031847133758 0.22859168468842
35.6687898089172 0.220817694370275
36.3057324840764 0.214728336006518
36.9426751592357 0.207178326446345
37.5796178343949 0.200902869987538
38.2165605095541 0.197367151055536
38.8535031847134 0.194719563672139
39.4904458598726 0.184238638642332
40.1273885350318 0.172847329667044
40.7643312101911 0.165254880360415
41.4012738853503 0.164989490973791
42.0382165605096 0.16431186819545
42.6751592356688 0.15994704514262
43.312101910828 0.151937624925475
43.9490445859873 0.145148952958722
44.5859872611465 0.141510661363987
45.2229299363057 0.133548247810246
45.859872611465 0.132084216357889
46.4968152866242 0.126397477360294
47.1337579617834 0.121241525130747
47.7707006369427 0.117739619183915
48.4076433121019 0.111133733888211
49.0445859872611 0.102843227198566
49.6815286624204 0.0951913836386527
50.3184713375796 0.0948929655342624
50.9554140127388 0.0913075348715234
51.5923566878981 0.093964634215223
52.2292993630573 0.0979311931323761
52.8662420382166 0.0971403095989766
53.5031847133758 0.0908352420237982
54.140127388535 0.0935736727079712
54.7770700636943 0.0961954745764865
55.4140127388535 0.0920135237728838
56.0509554140127 0.0913042504958316
56.687898089172 0.0906923882414409
57.3248407643312 0.0820352656470754
57.9617834394904 0.0792080859794863
58.5987261146497 0.0754506220455919
59.2356687898089 0.07283703366304
59.8726114649682 0.0732102878618979
60.5095541401274 0.0668523000844387
61.1464968152866 0.0620744390382069
61.7834394904459 0.0621987520819969
62.4203821656051 0.05691752420802
63.0573248407643 0.0501435071832819
63.6942675159236 0.0503966856086216
64.3312101910828 0.0489334991770904
64.968152866242 0.0459123874924324
65.6050955414013 0.0450855477558216
66.2420382165605 0.0391145391178347
66.8789808917197 0.0380030374022345
67.515923566879 0.0388745187438522
68.1528662420382 0.0335024770283287
68.7898089171974 0.0307510049692032
69.4267515923567 0.0297345365954342
70.0636942675159 0.0273429838235495
70.7006369426752 0.0281456557370833
71.3375796178344 0.0283637750347115
71.9745222929936 0.0275973990338576
72.6114649681529 0.026119697375489
73.2484076433121 0.0247528277923777
73.8853503184713 0.0246534547037881
74.5222929936306 0.0226003050165013
75.1592356687898 0.0228769850755287
75.796178343949 0.0196660847565604
76.4331210191083 0.0208076569795796
77.0700636942675 0.0212487043493654
77.7070063694268 0.0177547588685727
78.343949044586 0.01493890867423
78.9808917197452 0.0152036899389748
79.6178343949044 0.0131131450888364
80.2547770700637 0.0140406678222821
80.8917197452229 0.0121898384330989
81.5286624203822 0.0122485337275554
82.1656050955414 0.0128670249105041
82.8025477707006 0.0104418083535386
83.4394904458599 0.0111009397989638
84.0764331210191 0.0121267234211909
84.7133757961783 0.0103049667165136
85.3503184713376 0.0100086816021149
85.9872611464968 0.00824389546730728
86.6242038216561 0.00592967073947376
87.2611464968153 0.00547346695960827
87.8980891719745 0.00482060179460982
88.5350318471338 0.00431654756863766
89.171974522293 0.0034132057071682
89.8089171974522 0.00331645258261298
90.4458598726115 0.00364276904798838
91.0828025477707 0.00400091790447323
91.7197452229299 0.00359339325041592
92.3566878980892 0.00387563231622059
92.9936305732484 0.0025049491337727
93.6305732484076 0.00156863291804824
94.2675159235669 0.000832716738124931
94.9044585987261 0.000523199684818357
95.5414012738853 0.000192439300060108
96.1783439490446 6.14175350763557e-05
96.8152866242038 2.3827286706824e-05
97.4522292993631 2.8812739266284e-05
98.0891719745223 6.23756801280184e-06
98.7261146496815 2.62598242793788e-06
99.3630573248408 2.2991587002813e-06
100 0
};
\path [fill=color3, fill opacity=0.25] 
(axis cs:0,0.916080512546139)
--(axis cs:0,0.914846311931362)
--(axis cs:0.636942675159236,0.914579767648358)
--(axis cs:1.27388535031847,0.914186175515196)
--(axis cs:1.91082802547771,0.913272940681085)
--(axis cs:2.54777070063694,0.912284909636952)
--(axis cs:3.18471337579618,0.90988883404421)
--(axis cs:3.82165605095541,0.907133474356439)
--(axis cs:4.45859872611465,0.903483423536461)
--(axis cs:5.09554140127389,0.898282855381818)
--(axis cs:5.73248407643312,0.891594449286287)
--(axis cs:6.36942675159236,0.885767682802942)
--(axis cs:7.00636942675159,0.877257168138007)
--(axis cs:7.64331210191083,0.864852065591331)
--(axis cs:8.28025477707006,0.850297021983724)
--(axis cs:8.9171974522293,0.838363200579368)
--(axis cs:9.55414012738853,0.821301588687304)
--(axis cs:10.1910828025478,0.806219423285649)
--(axis cs:10.828025477707,0.780462170929935)
--(axis cs:11.4649681528662,0.764767090372918)
--(axis cs:12.1019108280255,0.74696397482435)
--(axis cs:12.7388535031847,0.730567022765083)
--(axis cs:13.3757961783439,0.710813853122863)
--(axis cs:14.0127388535032,0.689895864723445)
--(axis cs:14.6496815286624,0.667059803812277)
--(axis cs:15.2866242038217,0.655228988006651)
--(axis cs:15.9235668789809,0.63634541723079)
--(axis cs:16.5605095541401,0.620703630987506)
--(axis cs:17.1974522292994,0.601454558936245)
--(axis cs:17.8343949044586,0.585489107428701)
--(axis cs:18.4713375796178,0.565078269802634)
--(axis cs:19.1082802547771,0.5456551431523)
--(axis cs:19.7452229299363,0.519790970143205)
--(axis cs:20.3821656050955,0.504743800155775)
--(axis cs:21.0191082802548,0.482154388440522)
--(axis cs:21.656050955414,0.462722849525903)
--(axis cs:22.2929936305732,0.449045969162155)
--(axis cs:22.9299363057325,0.436523443817999)
--(axis cs:23.5668789808917,0.416646961022873)
--(axis cs:24.203821656051,0.404692427331682)
--(axis cs:24.8407643312102,0.394776084715579)
--(axis cs:25.4777070063694,0.382241219221458)
--(axis cs:26.1146496815287,0.366250680677917)
--(axis cs:26.7515923566879,0.355374677558818)
--(axis cs:27.3885350318471,0.342338109311952)
--(axis cs:28.0254777070064,0.333403246159955)
--(axis cs:28.6624203821656,0.325327361644444)
--(axis cs:29.2993630573248,0.315394704495741)
--(axis cs:29.9363057324841,0.304217178263659)
--(axis cs:30.5732484076433,0.292180402129701)
--(axis cs:31.2101910828025,0.284694496234429)
--(axis cs:31.8471337579618,0.26550952026965)
--(axis cs:32.484076433121,0.259780293904623)
--(axis cs:33.1210191082803,0.249025623718019)
--(axis cs:33.7579617834395,0.242410695029621)
--(axis cs:34.3949044585987,0.231459615149722)
--(axis cs:35.031847133758,0.22181135336819)
--(axis cs:35.6687898089172,0.214146603683424)
--(axis cs:36.3057324840764,0.208113138472887)
--(axis cs:36.9426751592357,0.200544294697957)
--(axis cs:37.5796178343949,0.194250327544594)
--(axis cs:38.2165605095541,0.190705182834505)
--(axis cs:38.8535031847134,0.188074582629319)
--(axis cs:39.4904458598726,0.177751011625945)
--(axis cs:40.1273885350318,0.166488926165287)
--(axis cs:40.7643312101911,0.158885935978486)
--(axis cs:41.4012738853503,0.158751282930915)
--(axis cs:42.0382165605096,0.157997152345018)
--(axis cs:42.6751592356688,0.153739003015684)
--(axis cs:43.312101910828,0.145802206790368)
--(axis cs:43.9490445859873,0.139151967574091)
--(axis cs:44.5859872611465,0.135511467507065)
--(axis cs:45.2229299363057,0.127752902146476)
--(axis cs:45.859872611465,0.126377895949351)
--(axis cs:46.4968152866242,0.120762025907562)
--(axis cs:47.1337579617834,0.115786981991332)
--(axis cs:47.7707006369427,0.112324368971142)
--(axis cs:48.4076433121019,0.105817499681805)
--(axis cs:49.0445859872611,0.0977749912549518)
--(axis cs:49.6815286624204,0.0904633430750446)
--(axis cs:50.3184713375796,0.0901621214179444)
--(axis cs:50.9554140127388,0.0867747251299824)
--(axis cs:51.5923566878981,0.0893976315154927)
--(axis cs:52.2292993630573,0.0933104023806207)
--(axis cs:52.8662420382166,0.0925190418021129)
--(axis cs:53.5031847133758,0.086236469860345)
--(axis cs:54.140127388535,0.0889771879085797)
--(axis cs:54.7770700636943,0.0916166531517943)
--(axis cs:55.4140127388535,0.08751559306282)
--(axis cs:56.0509554140127,0.0867730325467957)
--(axis cs:56.687898089172,0.0862458997225251)
--(axis cs:57.3248407643312,0.0774931215820661)
--(axis cs:57.9617834394904,0.0749030095668441)
--(axis cs:58.5987261146497,0.0711777041904386)
--(axis cs:59.2356687898089,0.068467107397227)
--(axis cs:59.8726114649682,0.0689326066522148)
--(axis cs:60.5095541401274,0.0625106155792354)
--(axis cs:61.1464968152866,0.0577352743346193)
--(axis cs:61.7834394904459,0.0579160955741648)
--(axis cs:62.4203821656051,0.0526224524726255)
--(axis cs:63.0573248407643,0.046068518669313)
--(axis cs:63.6942675159236,0.0464404865406926)
--(axis cs:64.3312101910828,0.0451910992778957)
--(axis cs:64.968152866242,0.042228799031516)
--(axis cs:65.6050955414013,0.0415613540905783)
--(axis cs:66.2420382165605,0.035757662652697)
--(axis cs:66.8789808917197,0.034540585621026)
--(axis cs:67.515923566879,0.0354763971107871)
--(axis cs:68.1528662420382,0.0303825393130732)
--(axis cs:68.7898089171974,0.0278968543378776)
--(axis cs:69.4267515923567,0.0269306702347691)
--(axis cs:70.0636942675159,0.0247351995642663)
--(axis cs:70.7006369426752,0.0255569100215131)
--(axis cs:71.3375796178344,0.0257733217825398)
--(axis cs:71.9745222929936,0.0250768941294238)
--(axis cs:72.6114649681529,0.0236742519222253)
--(axis cs:73.2484076433121,0.0224928158137006)
--(axis cs:73.8853503184713,0.0225534773632058)
--(axis cs:74.5222929936306,0.0204883399141297)
--(axis cs:75.1592356687898,0.020831071339969)
--(axis cs:75.796178343949,0.0176118764662155)
--(axis cs:76.4331210191083,0.0185760919940436)
--(axis cs:77.0700636942675,0.0190456556107787)
--(axis cs:77.7070063694268,0.0155830568371195)
--(axis cs:78.343949044586,0.0128912636075061)
--(axis cs:78.9808917197452,0.0130953648198494)
--(axis cs:79.6178343949044,0.0111241458099474)
--(axis cs:80.2547770700637,0.0120141867231458)
--(axis cs:80.8917197452229,0.0103284897035514)
--(axis cs:81.5286624203822,0.0104273223473078)
--(axis cs:82.1656050955414,0.0109670372266417)
--(axis cs:82.8025477707006,0.00874639214765354)
--(axis cs:83.4394904458599,0.00922714686715129)
--(axis cs:84.0764331210191,0.0101647334404282)
--(axis cs:84.7133757961783,0.00857135931110966)
--(axis cs:85.3503184713376,0.00821032235309744)
--(axis cs:85.9872611464968,0.00663176430207143)
--(axis cs:86.6242038216561,0.0045440418702105)
--(axis cs:87.2611464968153,0.00416112782541036)
--(axis cs:87.8980891719745,0.00362612279732005)
--(axis cs:88.5350318471338,0.00330091788670568)
--(axis cs:89.171974522293,0.00248629597427653)
--(axis cs:89.8089171974522,0.00239100449736042)
--(axis cs:90.4458598726115,0.00270052344606382)
--(axis cs:91.0828025477707,0.00301197125021494)
--(axis cs:91.7197452229299,0.00262816481660561)
--(axis cs:92.3566878980892,0.00288756676244264)
--(axis cs:92.9936305732484,0.00171937039974242)
--(axis cs:93.6305732484076,0.000964574612815377)
--(axis cs:94.2675159235669,0.000492991734086699)
--(axis cs:94.9044585987261,0.0002945450177399)
--(axis cs:95.5414012738853,9.28275061369359e-05)
--(axis cs:96.1783439490446,3.56476461424341e-05)
--(axis cs:96.8152866242038,1.05510998878644e-05)
--(axis cs:97.4522292993631,1.57174484387531e-05)
--(axis cs:98.0891719745223,3.42433755239964e-06)
--(axis cs:98.7261146496815,1.46642607849723e-06)
--(axis cs:99.3630573248408,1.01523898360081e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,3.58307841696179e-06)
--(axis cs:98.7261146496815,3.78553877737853e-06)
--(axis cs:98.0891719745223,9.05079847320405e-06)
--(axis cs:97.4522292993631,4.1908030093815e-05)
--(axis cs:96.8152866242038,3.71034735257836e-05)
--(axis cs:96.1783439490446,8.71874240102774e-05)
--(axis cs:95.5414012738853,0.000292051093983279)
--(axis cs:94.9044585987261,0.000751854351896814)
--(axis cs:94.2675159235669,0.00117244174216316)
--(axis cs:93.6305732484076,0.00217269122328109)
--(axis cs:92.9936305732484,0.00329052786780298)
--(axis cs:92.3566878980892,0.00486369786999854)
--(axis cs:91.7197452229299,0.00455862168422624)
--(axis cs:91.0828025477707,0.00498986455873153)
--(axis cs:90.4458598726115,0.00458501464991293)
--(axis cs:89.8089171974522,0.00424190066786554)
--(axis cs:89.171974522293,0.00434011544005988)
--(axis cs:88.5350318471338,0.00533217725056965)
--(axis cs:87.8980891719745,0.0060150807918996)
--(axis cs:87.2611464968153,0.00678580609380618)
--(axis cs:86.6242038216561,0.00731529960873702)
--(axis cs:85.9872611464968,0.00985602663254313)
--(axis cs:85.3503184713376,0.0118070408511324)
--(axis cs:84.7133757961783,0.0120385741219174)
--(axis cs:84.0764331210191,0.0140887134019536)
--(axis cs:83.4394904458599,0.0129747327307762)
--(axis cs:82.8025477707006,0.0121372245594236)
--(axis cs:82.1656050955414,0.0147670125943665)
--(axis cs:81.5286624203822,0.014069745107803)
--(axis cs:80.8917197452229,0.0140511871626464)
--(axis cs:80.2547770700637,0.0160671489214184)
--(axis cs:79.6178343949044,0.0151021443677255)
--(axis cs:78.9808917197452,0.0173120150581002)
--(axis cs:78.343949044586,0.0169865537409539)
--(axis cs:77.7070063694268,0.0199264609000259)
--(axis cs:77.0700636942675,0.0234517530879522)
--(axis cs:76.4331210191083,0.0230392219651156)
--(axis cs:75.796178343949,0.0217202930469053)
--(axis cs:75.1592356687898,0.0249228988110884)
--(axis cs:74.5222929936306,0.0247122701188729)
--(axis cs:73.8853503184713,0.0267534320443704)
--(axis cs:73.2484076433121,0.0270128397710548)
--(axis cs:72.6114649681529,0.0285651428287528)
--(axis cs:71.9745222929936,0.0301179039382915)
--(axis cs:71.3375796178344,0.0309542282868832)
--(axis cs:70.7006369426752,0.0307344014526535)
--(axis cs:70.0636942675159,0.0299507680828327)
--(axis cs:69.4267515923567,0.0325384029560993)
--(axis cs:68.7898089171974,0.0336051556005288)
--(axis cs:68.1528662420382,0.0366224147435841)
--(axis cs:67.515923566879,0.0422726403769172)
--(axis cs:66.8789808917197,0.041465489183443)
--(axis cs:66.2420382165605,0.0424714155829725)
--(axis cs:65.6050955414013,0.0486097414210649)
--(axis cs:64.968152866242,0.0495959759533488)
--(axis cs:64.3312101910828,0.0526758990762852)
--(axis cs:63.6942675159236,0.0543528846765505)
--(axis cs:63.0573248407643,0.0542184956972508)
--(axis cs:62.4203821656051,0.0612125959434145)
--(axis cs:61.7834394904459,0.0664814085898291)
--(axis cs:61.1464968152866,0.0664136037417945)
--(axis cs:60.5095541401274,0.071193984589642)
--(axis cs:59.8726114649682,0.0774879690715811)
--(axis cs:59.2356687898089,0.0772069599288529)
--(axis cs:58.5987261146497,0.0797235399007452)
--(axis cs:57.9617834394904,0.0835131623921285)
--(axis cs:57.3248407643312,0.0865774097120848)
--(axis cs:56.687898089172,0.0951388767603567)
--(axis cs:56.0509554140127,0.0958354684448674)
--(axis cs:55.4140127388535,0.0965114544829476)
--(axis cs:54.7770700636943,0.100774296001179)
--(axis cs:54.140127388535,0.0981701575073626)
--(axis cs:53.5031847133758,0.0954340141872513)
--(axis cs:52.8662420382166,0.10176157739584)
--(axis cs:52.2292993630573,0.102551983884131)
--(axis cs:51.5923566878981,0.0985316369149534)
--(axis cs:50.9554140127388,0.0958403446130643)
--(axis cs:50.3184713375796,0.0996238096505803)
--(axis cs:49.6815286624204,0.0999194242022608)
--(axis cs:49.0445859872611,0.10791146314218)
--(axis cs:48.4076433121019,0.116449968094616)
--(axis cs:47.7707006369427,0.123154869396687)
--(axis cs:47.1337579617834,0.126696068270163)
--(axis cs:46.4968152866242,0.132032928813026)
--(axis cs:45.859872611465,0.137790536766428)
--(axis cs:45.2229299363057,0.139343593474015)
--(axis cs:44.5859872611465,0.147509855220909)
--(axis cs:43.9490445859873,0.151145938343352)
--(axis cs:43.312101910828,0.158073043060583)
--(axis cs:42.6751592356688,0.166155087269555)
--(axis cs:42.0382165605096,0.170626584045882)
--(axis cs:41.4012738853503,0.171227699016667)
--(axis cs:40.7643312101911,0.171623824742345)
--(axis cs:40.1273885350318,0.179205733168802)
--(axis cs:39.4904458598726,0.19072626565872)
--(axis cs:38.8535031847134,0.20136454471496)
--(axis cs:38.2165605095541,0.204029119276568)
--(axis cs:37.5796178343949,0.207555412430482)
--(axis cs:36.9426751592357,0.213812358194734)
--(axis cs:36.3057324840764,0.221343533540148)
--(axis cs:35.6687898089172,0.227488785057127)
--(axis cs:35.031847133758,0.23537201600865)
--(axis cs:34.3949044585987,0.245353223698703)
--(axis cs:33.7579617834395,0.256702797069783)
--(axis cs:33.1210191082803,0.263187952109114)
--(axis cs:32.484076433121,0.274426291601631)
--(axis cs:31.8471337579618,0.280170783343449)
--(axis cs:31.2101910828025,0.299787046884244)
--(axis cs:30.5732484076433,0.307477275802744)
--(axis cs:29.9363057324841,0.319636628235369)
--(axis cs:29.2993630573248,0.33100324904033)
--(axis cs:28.6624203821656,0.340789785107195)
--(axis cs:28.0254777070064,0.348890591006553)
--(axis cs:27.3885350318471,0.357744753789827)
--(axis cs:26.7515923566879,0.37105893173711)
--(axis cs:26.1146496815287,0.381711522007386)
--(axis cs:25.4777070063694,0.397966661349211)
--(axis cs:24.8407643312102,0.410543303988796)
--(axis cs:24.203821656051,0.420474514467425)
--(axis cs:23.5668789808917,0.432406122195586)
--(axis cs:22.9299363057325,0.452840447955392)
--(axis cs:22.2929936305732,0.465715112040732)
--(axis cs:21.656050955414,0.479680670072399)
--(axis cs:21.0191082802548,0.499041258645029)
--(axis cs:20.3821656050955,0.521868019814646)
--(axis cs:19.7452229299363,0.537131452172487)
--(axis cs:19.1082802547771,0.562671797183965)
--(axis cs:18.4713375796178,0.58216582187275)
--(axis cs:17.8343949044586,0.602551674777525)
--(axis cs:17.1974522292994,0.61818567313457)
--(axis cs:16.5605095541401,0.636993880188141)
--(axis cs:15.9235668789809,0.652386712574932)
--(axis cs:15.2866242038217,0.671027822906678)
--(axis cs:14.6496815286624,0.682381137306824)
--(axis cs:14.0127388535032,0.704885847453765)
--(axis cs:13.3757961783439,0.725648880647159)
--(axis cs:12.7388535031847,0.745396100775776)
--(axis cs:12.1019108280255,0.761491546360601)
--(axis cs:11.4649681528662,0.779067941929968)
--(axis cs:10.828025477707,0.794533996258576)
--(axis cs:10.1910828025478,0.819332081060427)
--(axis cs:9.55414012738853,0.833853281647941)
--(axis cs:8.9171974522293,0.850086996274005)
--(axis cs:8.28025477707006,0.861089931641173)
--(axis cs:7.64331210191083,0.874169071168217)
--(axis cs:7.00636942675159,0.885522372002174)
--(axis cs:6.36942675159236,0.892834893299188)
--(axis cs:5.73248407643312,0.897900027476779)
--(axis cs:5.09554140127389,0.903356219342117)
--(axis cs:4.45859872611465,0.907433699998722)
--(axis cs:3.82165605095541,0.910371578785647)
--(axis cs:3.18471337579618,0.912529891334602)
--(axis cs:2.54777070063694,0.914215536901023)
--(axis cs:1.91082802547771,0.915027716730953)
--(axis cs:1.27388535031847,0.915512646792204)
--(axis cs:0.636942675159236,0.915919805554912)
--(axis cs:0,0.916080512546139)
--cycle;


==> img/mnist/mnist_rate_distortion_sfw_order_var_e.tex <==
\addplot [line width=0.5, opacity=0.7, color4, mark=o, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color4, thin}]
table {%
0 0.915530670499429
0.636942675159236 0.915181452180841
1.27388535031847 0.914622080968111
1.91082802547771 0.91434749882319
2.54777070063694 0.912940151605289
3.18471337579618 0.9116221823456
3.82165605095541 0.908981365073705
4.45859872611465 0.904293626327999
5.09554140127389 0.900301982808742
5.73248407643312 0.893708241512068
6.36942675159236 0.884648138292832
7.00636942675159 0.876984965424053
7.64331210191083 0.866015738322167
8.28025477707006 0.854092673495179
8.9171974522293 0.840642470815219
9.55414012738853 0.8228887162311
10.1910828025478 0.804732798573677
10.828025477707 0.787508943648427
11.4649681528662 0.765032519215601
12.1019108280255 0.740175382933521
12.7388535031847 0.725246244012378
13.3757961783439 0.70630681224633
14.0127388535032 0.687289428388176
14.6496815286624 0.671841476592235
15.2866242038217 0.656192534506554
15.9235668789809 0.639749838815769
16.5605095541401 0.626491518768889
17.1974522292994 0.615383608377306
17.8343949044586 0.595960774164996
18.4713375796178 0.576401513388846
19.1082802547771 0.55867531984346
19.7452229299363 0.540521789526101
20.3821656050955 0.519878936277237
21.0191082802548 0.508267271877267
21.656050955414 0.493706757051405
22.2929936305732 0.475355701390654
22.9299363057325 0.465389415582176
23.5668789808917 0.454499633291271
24.203821656051 0.437009010222973
24.8407643312102 0.430674436155241
25.4777070063694 0.415301037391182
26.1146496815287 0.404722309891367
26.7515923566879 0.394860849059769
27.3885350318471 0.382779555899906
28.0254777070064 0.371258565727621
28.6624203821656 0.366141823873331
29.2993630573248 0.358257999120833
29.9363057324841 0.344984942356823
30.5732484076433 0.334203229738778
31.2101910828025 0.321355929185811
31.8471337579618 0.301133473416121
32.484076433121 0.295354128139006
33.1210191082803 0.283866303537925
33.7579617834395 0.278716130235371
34.3949044585987 0.266998774097478
35.031847133758 0.257604977184219
35.6687898089172 0.24787505135806
36.3057324840764 0.240280776493412
36.9426751592357 0.230814434270003
37.5796178343949 0.223920172737812
38.2165605095541 0.222464281045823
38.8535031847134 0.218226431490899
39.4904458598726 0.215039589484568
40.1273885350318 0.217837599939332
40.7643312101911 0.220267577062622
41.4012738853503 0.224355776263485
42.0382165605096 0.218019280902066
42.6751592356688 0.210921447678501
43.312101910828 0.204504925981056
43.9490445859873 0.19654841432775
44.5859872611465 0.189736224193642
45.2229299363057 0.186856607117902
45.859872611465 0.179902788409524
46.4968152866242 0.175408176785527
47.1337579617834 0.170832004490484
47.7707006369427 0.163144663025771
48.4076433121019 0.161843420328557
49.0445859872611 0.15671313951739
49.6815286624204 0.150702090863437
50.3184713375796 0.149970730677806
50.9554140127388 0.144886011136644
51.5923566878981 0.1459885307676
52.2292993630573 0.142392057905319
52.8662420382166 0.133590482347599
53.5031847133758 0.132451961695494
54.140127388535 0.129726182725838
54.7770700636943 0.12619310557013
55.4140127388535 0.121085182148703
56.0509554140127 0.116816692600185
56.687898089172 0.108793878701105
57.3248407643312 0.104268809093967
57.9617834394904 0.0946568643087344
58.5987261146497 0.0888855736844681
59.2356687898089 0.0903790019561544
59.8726114649682 0.0924402029796437
60.5095541401274 0.0889208085565209
61.1464968152866 0.0787171075442353
61.7834394904459 0.0760861822161961
62.4203821656051 0.0692321215890179
63.0573248407643 0.0653387454104101
63.6942675159236 0.0657060414386169
64.3312101910828 0.0608172682649052
64.968152866242 0.0572993655469406
65.6050955414013 0.0510363152854214
66.2420382165605 0.0500153766482652
66.8789808917197 0.0463942006209196
67.515923566879 0.045128795952904
68.1528662420382 0.0453566944480248
68.7898089171974 0.0432915056658522
69.4267515923567 0.0423498495637228
70.0636942675159 0.0383894876501915
70.7006369426752 0.0373277418857221
71.3375796178344 0.0346721533700441
71.9745222929936 0.0318179522317651
72.6114649681529 0.0294126470781592
73.2484076433121 0.028693695820807
73.8853503184713 0.0301449474592988
74.5222929936306 0.0251421563728964
75.1592356687898 0.0227785558233269
75.796178343949 0.0224910590145627
76.4331210191083 0.02284349464162
77.0700636942675 0.0222841978896751
77.7070063694268 0.0220452250862836
78.343949044586 0.0205657309969648
78.9808917197452 0.0187730985457923
79.6178343949044 0.017400688833464
80.2547770700637 0.0163934091090481
80.8917197452229 0.0154385167109734
81.5286624203822 0.0155698291792823
82.1656050955414 0.0161879816498921
82.8025477707006 0.0159762669624519
83.4394904458599 0.0148302907351978
84.0764331210191 0.0140611101283965
84.7133757961783 0.0135856302257949
85.3503184713376 0.0115195346245023
85.9872611464968 0.0107456905407963
86.6242038216561 0.0105079100774502
87.2611464968153 0.0111031366291411
87.8980891719745 0.00889688002553482
88.5350318471338 0.00847837592803148
89.171974522293 0.00671338018413314
89.8089171974522 0.00457380580303001
90.4458598726115 0.00325176116689849
91.0828025477707 0.00250355897162774
91.7197452229299 0.0017347587551244
92.3566878980892 0.00193990961212031
92.9936305732484 0.00238669768786164
93.6305732484076 0.00189830514607346
94.2675159235669 0.000612769367704597
94.9044585987261 0.000273717752380241
95.5414012738853 8.75559500164957e-05
96.1783439490446 3.9696666686535e-05
96.8152866242038 1.86173450174371e-05
97.4522292993631 4.79424940834305e-06
98.0891719745223 3.11515829814146e-06
98.7261146496815 3.5244925816641e-06
99.3630573248408 2.47549040231054e-06
100 0
};
\path [fill=color4, fill opacity=0.25] 
(axis cs:0,0.916142183774977)
--(axis cs:0,0.914919157223881)
--(axis cs:0.636942675159236,0.914449544619737)
--(axis cs:1.27388535031847,0.913851245347366)
--(axis cs:1.91082802547771,0.913554393153861)
--(axis cs:2.54777070063694,0.911885388927118)
--(axis cs:3.18471337579618,0.910364689457223)
--(axis cs:3.82165605095541,0.907425479886014)
--(axis cs:4.45859872611465,0.902083756151297)
--(axis cs:5.09554140127389,0.897700572723529)
--(axis cs:5.73248407643312,0.890568290402535)
--(axis cs:6.36942675159236,0.880843292444371)
--(axis cs:7.00636942675159,0.872727511167396)
--(axis cs:7.64331210191083,0.861168935005153)
--(axis cs:8.28025477707006,0.848815825952106)
--(axis cs:8.9171974522293,0.834839637656991)
--(axis cs:9.55414012738853,0.816612003753515)
--(axis cs:10.1910828025478,0.798078641405991)
--(axis cs:10.828025477707,0.780727529909596)
--(axis cs:11.4649681528662,0.758034610039285)
--(axis cs:12.1019108280255,0.733114842246476)
--(axis cs:12.7388535031847,0.718175194490782)
--(axis cs:13.3757961783439,0.698966520258595)
--(axis cs:14.0127388535032,0.679939582162061)
--(axis cs:14.6496815286624,0.66419377804665)
--(axis cs:15.2866242038217,0.648619715579751)
--(axis cs:15.9235668789809,0.631867301993084)
--(axis cs:16.5605095541401,0.618694325356339)
--(axis cs:17.1974522292994,0.607397567336497)
--(axis cs:17.8343949044586,0.587787140327621)
--(axis cs:18.4713375796178,0.567963440396486)
--(axis cs:19.1082802547771,0.55012810649936)
--(axis cs:19.7452229299363,0.531753116083719)
--(axis cs:20.3821656050955,0.511313693373793)
--(axis cs:21.0191082802548,0.499908404723256)
--(axis cs:21.656050955414,0.485341638544869)
--(axis cs:22.2929936305732,0.467006775796252)
--(axis cs:22.9299363057325,0.456999153773642)
--(axis cs:23.5668789808917,0.446054989033261)
--(axis cs:24.203821656051,0.428810037612651)
--(axis cs:24.8407643312102,0.422352769512031)
--(axis cs:25.4777070063694,0.407040927286669)
--(axis cs:26.1146496815287,0.396459045082697)
--(axis cs:26.7515923566879,0.386613215322074)
--(axis cs:27.3885350318471,0.374511708203009)
--(axis cs:28.0254777070064,0.363248531767956)
--(axis cs:28.6624203821656,0.35811101098656)
--(axis cs:29.2993630573248,0.350357687823325)
--(axis cs:29.9363057324841,0.33708752724028)
--(axis cs:30.5732484076433,0.326272753311611)
--(axis cs:31.2101910828025,0.313725231826606)
--(axis cs:31.8471337579618,0.293508033988364)
--(axis cs:32.484076433121,0.287800130885438)
--(axis cs:33.1210191082803,0.276320922394866)
--(axis cs:33.7579617834395,0.271157116170453)
--(axis cs:34.3949044585987,0.259445972484538)
--(axis cs:35.031847133758,0.25027089655597)
--(axis cs:35.6687898089172,0.240778423200052)
--(axis cs:36.3057324840764,0.233154326264969)
--(axis cs:36.9426751592357,0.223835023912864)
--(axis cs:37.5796178343949,0.217049214992923)
--(axis cs:38.2165605095541,0.215712392273334)
--(axis cs:38.8535031847134,0.211517091909643)
--(axis cs:39.4904458598726,0.208403576175208)
--(axis cs:40.1273885350318,0.211350133148761)
--(axis cs:40.7643312101911,0.213787344972796)
--(axis cs:41.4012738853503,0.218030047047189)
--(axis cs:42.0382165605096,0.211850354124685)
--(axis cs:42.6751592356688,0.204795419946885)
--(axis cs:43.312101910828,0.198553514908749)
--(axis cs:43.9490445859873,0.19074451050245)
--(axis cs:44.5859872611465,0.183787563306886)
--(axis cs:45.2229299363057,0.181035523537068)
--(axis cs:45.859872611465,0.174448469253221)
--(axis cs:46.4968152866242,0.170096355324508)
--(axis cs:47.1337579617834,0.165668126962418)
--(axis cs:47.7707006369427,0.158194324435008)
--(axis cs:48.4076433121019,0.156950674628407)
--(axis cs:49.0445859872611,0.151872093789888)
--(axis cs:49.6815286624204,0.145838252252697)
--(axis cs:50.3184713375796,0.145019742925315)
--(axis cs:50.9554140127388,0.14000817809001)
--(axis cs:51.5923566878981,0.141070103421718)
--(axis cs:52.2292993630573,0.137297261600941)
--(axis cs:52.8662420382166,0.128451235944786)
--(axis cs:53.5031847133758,0.127448158618339)
--(axis cs:54.140127388535,0.124727972975696)
--(axis cs:54.7770700636943,0.121111074617964)
--(axis cs:55.4140127388535,0.115942581164573)
--(axis cs:56.0509554140127,0.111845540352706)
--(axis cs:56.687898089172,0.103926399151224)
--(axis cs:57.3248407643312,0.099465504843776)
--(axis cs:57.9617834394904,0.0901282782354334)
--(axis cs:58.5987261146497,0.0844616728154355)
--(axis cs:59.2356687898089,0.0859028456458909)
--(axis cs:59.8726114649682,0.0878224614927418)
--(axis cs:60.5095541401274,0.0844188733358426)
--(axis cs:61.1464968152866,0.0744102754712424)
--(axis cs:61.7834394904459,0.0718968817491266)
--(axis cs:62.4203821656051,0.0650988061212489)
--(axis cs:63.0573248407643,0.0610706462660711)
--(axis cs:63.6942675159236,0.061504812569084)
--(axis cs:64.3312101910828,0.0566582053875421)
--(axis cs:64.968152866242,0.0532632424877577)
--(axis cs:65.6050955414013,0.0471416040937738)
--(axis cs:66.2420382165605,0.0461869646691342)
--(axis cs:66.8789808917197,0.0426111831314552)
--(axis cs:67.515923566879,0.0415233604047957)
--(axis cs:68.1528662420382,0.0418930167711257)
--(axis cs:68.7898089171974,0.0399023004792145)
--(axis cs:69.4267515923567,0.0390365828456563)
--(axis cs:70.0636942675159,0.0352758645787982)
--(axis cs:70.7006369426752,0.0343468800780933)
--(axis cs:71.3375796178344,0.0316541054261699)
--(axis cs:71.9745222929936,0.0290673373006209)
--(axis cs:72.6114649681529,0.0270487853111733)
--(axis cs:73.2484076433121,0.0265594851207062)
--(axis cs:73.8853503184713,0.0279244118918188)
--(axis cs:74.5222929936306,0.0233258988708356)
--(axis cs:75.1592356687898,0.0211967993864714)
--(axis cs:75.796178343949,0.0209518592572176)
--(axis cs:76.4331210191083,0.0212085817872827)
--(axis cs:77.0700636942675,0.0207147460303289)
--(axis cs:77.7070063694268,0.0206651473553302)
--(axis cs:78.343949044586,0.019198707925063)
--(axis cs:78.9808917197452,0.0177826666025841)
--(axis cs:79.6178343949044,0.0164379172424086)
--(axis cs:80.2547770700637,0.0153915251638807)
--(axis cs:80.8917197452229,0.014328351995066)
--(axis cs:81.5286624203822,0.0144795934272664)
--(axis cs:82.1656050955414,0.0150777534695741)
--(axis cs:82.8025477707006,0.0149825295363792)
--(axis cs:83.4394904458599,0.0138265846349736)
--(axis cs:84.0764331210191,0.012850408949883)
--(axis cs:84.7133757961783,0.0123913487758278)
--(axis cs:85.3503184713376,0.0102491634167757)
--(axis cs:85.9872611464968,0.00955453465544304)
--(axis cs:86.6242038216561,0.00932433403440318)
--(axis cs:87.2611464968153,0.00991015505152481)
--(axis cs:87.8980891719745,0.0075880877858457)
--(axis cs:88.5350318471338,0.00722078786211817)
--(axis cs:89.171974522293,0.00551164383952376)
--(axis cs:89.8089171974522,0.00353208850335139)
--(axis cs:90.4458598726115,0.00241873592580575)
--(axis cs:91.0828025477707,0.0018409213339019)
--(axis cs:91.7197452229299,0.00121537434228298)
--(axis cs:92.3566878980892,0.00134560744429577)
--(axis cs:92.9936305732484,0.00175377753391981)
--(axis cs:93.6305732484076,0.00131662465429392)
--(axis cs:94.2675159235669,0.000395501558672011)
--(axis cs:94.9044585987261,0.000151608398117366)
--(axis cs:95.5414012738853,5.14516827460907e-05)
--(axis cs:96.1783439490446,2.5967194446568e-05)
--(axis cs:96.8152866242038,1.26468436933369e-05)
--(axis cs:97.4522292993631,3.90962606102618e-06)
--(axis cs:98.0891719745223,2.79503309380871e-06)
--(axis cs:98.7261146496815,3.30648082149475e-06)
--(axis cs:99.3630573248408,2.28225631938801e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,2.66872448523308e-06)
--(axis cs:98.7261146496815,3.74250434183345e-06)
--(axis cs:98.0891719745223,3.43528350247422e-06)
--(axis cs:97.4522292993631,5.67887275565993e-06)
--(axis cs:96.8152866242038,2.45878463415373e-05)
--(axis cs:96.1783439490446,5.34261389265021e-05)
--(axis cs:95.5414012738853,0.000123660217286901)
--(axis cs:94.9044585987261,0.000395827106643117)
--(axis cs:94.2675159235669,0.000830037176737183)
--(axis cs:93.6305732484076,0.002479985637853)
--(axis cs:92.9936305732484,0.00301961784180347)
--(axis cs:92.3566878980892,0.00253421177994485)
--(axis cs:91.7197452229299,0.00225414316796583)
--(axis cs:91.0828025477707,0.00316619660935357)
--(axis cs:90.4458598726115,0.00408478640799123)
--(axis cs:89.8089171974522,0.00561552310270863)
--(axis cs:89.171974522293,0.00791511652874252)
--(axis cs:88.5350318471338,0.00973596399394479)
--(axis cs:87.8980891719745,0.0102056722652239)
--(axis cs:87.2611464968153,0.0122961182067573)
--(axis cs:86.6242038216561,0.0116914861204972)
--(axis cs:85.9872611464968,0.0119368464261495)
--(axis cs:85.3503184713376,0.0127899058322289)
--(axis cs:84.7133757961783,0.0147799116757621)
--(axis cs:84.0764331210191,0.0152718113069101)
--(axis cs:83.4394904458599,0.0158339968354219)
--(axis cs:82.8025477707006,0.0169700043885247)
--(axis cs:82.1656050955414,0.0172982098302102)
--(axis cs:81.5286624203822,0.0166600649312982)
--(axis cs:80.8917197452229,0.0165486814268808)
--(axis cs:80.2547770700637,0.0173952930542156)
--(axis cs:79.6178343949044,0.0183634604245194)
--(axis cs:78.9808917197452,0.0197635304890006)
--(axis cs:78.343949044586,0.0219327540688667)
--(axis cs:77.7070063694268,0.023425302817237)
--(axis cs:77.0700636942675,0.0238536497490213)
--(axis cs:76.4331210191083,0.0244784074959573)
--(axis cs:75.796178343949,0.0240302587719077)
--(axis cs:75.1592356687898,0.0243603122601825)
--(axis cs:74.5222929936306,0.0269584138749572)
--(axis cs:73.8853503184713,0.0323654830267787)
--(axis cs:73.2484076433121,0.0308279065209078)
--(axis cs:72.6114649681529,0.0317765088451451)
--(axis cs:71.9745222929936,0.0345685671629093)
--(axis cs:71.3375796178344,0.0376902013139183)
--(axis cs:70.7006369426752,0.040308603693351)
--(axis cs:70.0636942675159,0.0415031107215848)
--(axis cs:69.4267515923567,0.0456631162817893)
--(axis cs:68.7898089171974,0.0466807108524899)
--(axis cs:68.1528662420382,0.048820372124924)
--(axis cs:67.515923566879,0.0487342315010123)
--(axis cs:66.8789808917197,0.050177218110384)
--(axis cs:66.2420382165605,0.0538437886273963)
--(axis cs:65.6050955414013,0.054931026477069)
--(axis cs:64.968152866242,0.0613354886061235)
--(axis cs:64.3312101910828,0.0649763311422684)
--(axis cs:63.6942675159236,0.0699072703081499)
--(axis cs:63.0573248407643,0.0696068445547492)
--(axis cs:62.4203821656051,0.0733654370567869)
--(axis cs:61.7834394904459,0.0802754826832657)
--(axis cs:61.1464968152866,0.0830239396172282)
--(axis cs:60.5095541401274,0.0934227437771993)
--(axis cs:59.8726114649682,0.0970579444665455)
--(axis cs:59.2356687898089,0.094855158266418)
--(axis cs:58.5987261146497,0.0933094745535007)
--(axis cs:57.9617834394904,0.0991854503820355)
--(axis cs:57.3248407643312,0.109072113344158)
--(axis cs:56.687898089172,0.113661358250987)
--(axis cs:56.0509554140127,0.121787844847663)
--(axis cs:55.4140127388535,0.126227783132834)
--(axis cs:54.7770700636943,0.131275136522297)
--(axis cs:54.140127388535,0.134724392475981)
--(axis cs:53.5031847133758,0.137455764772649)
--(axis cs:52.8662420382166,0.138729728750412)
--(axis cs:52.2292993630573,0.147486854209696)
--(axis cs:51.5923566878981,0.150906958113483)
--(axis cs:50.9554140127388,0.149763844183277)
--(axis cs:50.3184713375796,0.154921718430296)
--(axis cs:49.6815286624204,0.155565929474178)
--(axis cs:49.0445859872611,0.161554185244892)
--(axis cs:48.4076433121019,0.166736166028707)
--(axis cs:47.7707006369427,0.168095001616533)
--(axis cs:47.1337579617834,0.175995882018549)
--(axis cs:46.4968152866242,0.180719998246546)
--(axis cs:45.859872611465,0.185357107565826)
--(axis cs:45.2229299363057,0.192677690698736)
--(axis cs:44.5859872611465,0.195684885080398)
--(axis cs:43.9490445859873,0.202352318153051)
--(axis cs:43.312101910828,0.210456337053364)
--(axis cs:42.6751592356688,0.217047475410117)
--(axis cs:42.0382165605096,0.224188207679448)
--(axis cs:41.4012738853503,0.230681505479781)
--(axis cs:40.7643312101911,0.226747809152447)
--(axis cs:40.1273885350318,0.224325066729902)
--(axis cs:39.4904458598726,0.221675602793928)
--(axis cs:38.8535031847134,0.224935771072156)
--(axis cs:38.2165605095541,0.229216169818313)
--(axis cs:37.5796178343949,0.230791130482702)
--(axis cs:36.9426751592357,0.237793844627142)
--(axis cs:36.3057324840764,0.247407226721854)
--(axis cs:35.6687898089172,0.254971679516067)
--(axis cs:35.031847133758,0.264939057812468)
--(axis cs:34.3949044585987,0.274551575710419)
--(axis cs:33.7579617834395,0.286275144300288)
--(axis cs:33.1210191082803,0.291411684680984)
--(axis cs:32.484076433121,0.302908125392575)
--(axis cs:31.8471337579618,0.308758912843878)
--(axis cs:31.2101910828025,0.328986626545016)
--(axis cs:30.5732484076433,0.342133706165945)
--(axis cs:29.9363057324841,0.352882357473366)
--(axis cs:29.2993630573248,0.366158310418341)
--(axis cs:28.6624203821656,0.374172636760103)
--(axis cs:28.0254777070064,0.379268599687286)
--(axis cs:27.3885350318471,0.391047403596803)
--(axis cs:26.7515923566879,0.403108482797463)
--(axis cs:26.1146496815287,0.412985574700037)
--(axis cs:25.4777070063694,0.423561147495695)
--(axis cs:24.8407643312102,0.438996102798451)
--(axis cs:24.203821656051,0.445207982833295)
--(axis cs:23.5668789808917,0.46294427754928)
--(axis cs:22.9299363057325,0.47377967739071)
--(axis cs:22.2929936305732,0.483704626985055)
--(axis cs:21.656050955414,0.50207187555794)
--(axis cs:21.0191082802548,0.516626139031277)
--(axis cs:20.3821656050955,0.528444179180681)
--(axis cs:19.7452229299363,0.549290462968484)
--(axis cs:19.1082802547771,0.56722253318756)
--(axis cs:18.4713375796178,0.584839586381206)
--(axis cs:17.8343949044586,0.604134408002371)
--(axis cs:17.1974522292994,0.623369649418114)
--(axis cs:16.5605095541401,0.63428871218144)
--(axis cs:15.9235668789809,0.647632375638454)
--(axis cs:15.2866242038217,0.663765353433357)
--(axis cs:14.6496815286624,0.67948917513782)
--(axis cs:14.0127388535032,0.694639274614291)
--(axis cs:13.3757961783439,0.713647104234065)
--(axis cs:12.7388535031847,0.732317293533974)
--(axis cs:12.1019108280255,0.747235923620567)
--(axis cs:11.4649681528662,0.772030428391918)
--(axis cs:10.828025477707,0.794290357387258)
--(axis cs:10.1910828025478,0.811386955741364)
--(axis cs:9.55414012738853,0.829165428708686)
--(axis cs:8.9171974522293,0.846445303973447)
--(axis cs:8.28025477707006,0.859369521038252)
--(axis cs:7.64331210191083,0.87086254163918)
--(axis cs:7.00636942675159,0.881242419680711)
--(axis cs:6.36942675159236,0.888452984141293)
--(axis cs:5.73248407643312,0.8968481926216)
--(axis cs:5.09554140127389,0.902903392893955)
--(axis cs:4.45859872611465,0.906503496504701)
--(axis cs:3.82165605095541,0.910537250261396)
--(axis cs:3.18471337579618,0.912879675233976)
--(axis cs:2.54777070063694,0.913994914283461)
--(axis cs:1.91082802547771,0.91514060449252)
--(axis cs:1.27388535031847,0.915392916588855)
--(axis cs:0.636942675159236,0.915913359741945)
--(axis cs:0,0.916142183774977)
--cycle;


==> img/mnist/mnist_rate_distortion_sfw_order_var_f.tex <==
\addplot [line width=0.5, opacity=0.7, color5, mark=x, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color5, thin}]
table {%
0 0.915438967957161
0.636942675159236 0.915152466247091
1.27388535031847 0.915005342165241
1.91082802547771 0.914356085225008
2.54777070063694 0.912942909061676
3.18471337579618 0.91104458867223
3.82165605095541 0.909000597766135
4.45859872611465 0.904833188354969
5.09554140127389 0.899966735439375
5.73248407643312 0.895188111874741
6.36942675159236 0.885105890298728
7.00636942675159 0.877052595465211
7.64331210191083 0.86707592622377
8.28025477707006 0.850863233839627
8.9171974522293 0.83957365963608
9.55414012738853 0.823682044168236
10.1910828025478 0.802719476521015
10.828025477707 0.789612274621613
11.4649681528662 0.765620587414596
12.1019108280255 0.749476104334462
12.7388535031847 0.72554143979447
13.3757961783439 0.707607440717984
14.0127388535032 0.690369699095609
14.6496815286624 0.672728779345052
15.2866242038217 0.660298789052758
15.9235668789809 0.64210504419636
16.5605095541401 0.629201363595203
17.1974522292994 0.611634391564876
17.8343949044586 0.600542532494292
18.4713375796178 0.577495416230522
19.1082802547771 0.555535079189576
19.7452229299363 0.542164692603983
20.3821656050955 0.526228888533078
21.0191082802548 0.505613941291813
21.656050955414 0.489506614567945
22.2929936305732 0.474652031990699
22.9299363057325 0.453278179590125
23.5668789808917 0.442504231123021
24.203821656051 0.430244263286004
24.8407643312102 0.426020263435785
25.4777070063694 0.410449874681653
26.1146496815287 0.398085589433031
26.7515923566879 0.392073559791897
27.3885350318471 0.376311651902361
28.0254777070064 0.368826144089107
28.6624203821656 0.358682240628987
29.2993630573248 0.351631663508015
29.9363057324841 0.336644792587686
30.5732484076433 0.330760311351041
31.2101910828025 0.319448383054805
31.8471337579618 0.311578065027934
32.484076433121 0.293125347819478
33.1210191082803 0.281221562852224
33.7579617834395 0.270984799799371
34.3949044585987 0.26426847053076
35.031847133758 0.250505759274024
35.6687898089172 0.244612898829241
36.3057324840764 0.243307489182554
36.9426751592357 0.235350554112691
37.5796178343949 0.224034093527038
38.2165605095541 0.223773993770624
38.8535031847134 0.220450127297793
39.4904458598726 0.215490409628786
40.1273885350318 0.213012273116337
40.7643312101911 0.215323030446487
41.4012738853503 0.21359310538663
42.0382165605096 0.205912388204648
42.6751592356688 0.201057453492686
43.312101910828 0.189303730771928
43.9490445859873 0.18551268563038
44.5859872611465 0.182643113533054
45.2229299363057 0.181525884931995
45.859872611465 0.176875025126437
46.4968152866242 0.169813996006151
47.1337579617834 0.16376904475496
47.7707006369427 0.167140394848215
48.4076433121019 0.166782709246575
49.0445859872611 0.160739309753415
49.6815286624204 0.157163541193988
50.3184713375796 0.151519602285132
50.9554140127388 0.148005157585522
51.5923566878981 0.14009586346378
52.2292993630573 0.136591280258215
52.8662420382166 0.13183151940428
53.5031847133758 0.12620120690257
54.140127388535 0.122553768701673
54.7770700636943 0.123559846205247
55.4140127388535 0.119994567195715
56.0509554140127 0.121701946347364
56.687898089172 0.115868464718185
57.3248407643312 0.111259850363554
57.9617834394904 0.107614276247336
58.5987261146497 0.0969137247645981
59.2356687898089 0.0902730095545994
59.8726114649682 0.0853308105842792
60.5095541401274 0.0832315659621758
61.1464968152866 0.0756633236930963
61.7834394904459 0.0740225999718392
62.4203821656051 0.0733104598939776
63.0573248407643 0.0664317508989978
63.6942675159236 0.0687647453740767
64.3312101910828 0.0564822634125526
64.968152866242 0.0559525865782149
65.6050955414013 0.0513649048503463
66.2420382165605 0.0472004918746319
66.8789808917197 0.0482292773239358
67.515923566879 0.042142266044668
68.1528662420382 0.0404467594315586
68.7898089171974 0.0382047239937243
69.4267515923567 0.0341318712332352
70.0636942675159 0.0294716059604349
70.7006369426752 0.0310220506724666
71.3375796178344 0.0308368693658364
71.9745222929936 0.0286454627253067
72.6114649681529 0.0249114975673024
73.2484076433121 0.0233205851709307
73.8853503184713 0.0226844474456451
74.5222929936306 0.0205450580955949
75.1592356687898 0.0191303296507661
75.796178343949 0.0178087293096685
76.4331210191083 0.0169769793785115
77.0700636942675 0.0156105333615946
77.7070063694268 0.0128104029585396
78.343949044586 0.013257981165934
78.9808917197452 0.0135917425703708
79.6178343949044 0.0109867260994426
80.2547770700637 0.0115731852004101
80.8917197452229 0.0106530947816219
81.5286624203822 0.00896293313721344
82.1656050955414 0.00842430212183325
82.8025477707006 0.00787330161094774
83.4394904458599 0.00935098872648436
84.0764331210191 0.00951093298881888
84.7133757961783 0.00874627342990475
85.3503184713376 0.00601222280748292
85.9872611464968 0.00391927681518939
86.6242038216561 0.00350371899391684
87.2611464968153 0.00379180090578037
87.8980891719745 0.00381879443105342
88.5350318471338 0.00367383652900379
89.171974522293 0.0032823546470753
89.8089171974522 0.00240861028821584
90.4458598726115 0.00265650826771495
91.0828025477707 0.00259768931854976
91.7197452229299 0.00202566487013698
92.3566878980892 0.000790611612143095
92.9936305732484 0.000533651110186313
93.6305732484076 0.000250277858363416
94.2675159235669 6.55125350705721e-05
94.9044585987261 9.68963838788506e-05
95.5414012738853 6.62664214708802e-05
96.1783439490446 1.27538175415032e-05
96.8152866242038 8.98526588982707e-06
97.4522292993631 9.58684563111822e-06
98.0891719745223 8.58704408882138e-06
98.7261146496815 3.35795993948285e-06
99.3630573248408 1.98256521088402e-06
100 0
};
\path [fill=color5, fill opacity=0.25] 
(axis cs:0,0.916030337935273)
--(axis cs:0,0.914847597979049)
--(axis cs:0.636942675159236,0.914459272881957)
--(axis cs:1.27388535031847,0.91436525666635)
--(axis cs:1.91082802547771,0.913526443061803)
--(axis cs:2.54777070063694,0.911838125324149)
--(axis cs:3.18471337579618,0.909711167648223)
--(axis cs:3.82165605095541,0.907444668256636)
--(axis cs:4.45859872611465,0.902621219873282)
--(axis cs:5.09554140127389,0.89734574475703)
--(axis cs:5.73248407643312,0.892145839416567)
--(axis cs:6.36942675159236,0.881306505825049)
--(axis cs:7.00636942675159,0.872699781206956)
--(axis cs:7.64331210191083,0.862333813765737)
--(axis cs:8.28025477707006,0.845391307460339)
--(axis cs:8.9171974522293,0.833852097358298)
--(axis cs:9.55414012738853,0.817310069725151)
--(axis cs:10.1910828025478,0.795909271380482)
--(axis cs:10.828025477707,0.78249741361393)
--(axis cs:11.4649681528662,0.758330211608487)
--(axis cs:12.1019108280255,0.742058794770637)
--(axis cs:12.7388535031847,0.718199128021972)
--(axis cs:13.3757961783439,0.700068702706575)
--(axis cs:14.0127388535032,0.68278269257875)
--(axis cs:14.6496815286624,0.665123758410889)
--(axis cs:15.2866242038217,0.652669469335123)
--(axis cs:15.9235668789809,0.634360250997386)
--(axis cs:16.5605095541401,0.621304465038549)
--(axis cs:17.1974522292994,0.603396073514437)
--(axis cs:17.8343949044586,0.592397897416777)
--(axis cs:18.4713375796178,0.569149925801812)
--(axis cs:19.1082802547771,0.547032285805952)
--(axis cs:19.7452229299363,0.533676767445857)
--(axis cs:20.3821656050955,0.517800983512579)
--(axis cs:21.0191082802548,0.497348634326794)
--(axis cs:21.656050955414,0.481312961140805)
--(axis cs:22.2929936305732,0.46649642610799)
--(axis cs:22.9299363057325,0.445256278004063)
--(axis cs:23.5668789808917,0.434458377142462)
--(axis cs:24.203821656051,0.422196865985733)
--(axis cs:24.8407643312102,0.418046684034036)
--(axis cs:25.4777070063694,0.40249739066027)
--(axis cs:26.1146496815287,0.390099753826543)
--(axis cs:26.7515923566879,0.38406894939563)
--(axis cs:27.3885350318471,0.368195390308077)
--(axis cs:28.0254777070064,0.360630192065841)
--(axis cs:28.6624203821656,0.3505715766833)
--(axis cs:29.2993630573248,0.343473821476756)
--(axis cs:29.9363057324841,0.328564080403039)
--(axis cs:30.5732484076433,0.32277266053095)
--(axis cs:31.2101910828025,0.311512555913537)
--(axis cs:31.8471337579618,0.303522722292021)
--(axis cs:32.484076433121,0.285318060318396)
--(axis cs:33.1210191082803,0.273563654987072)
--(axis cs:33.7579617834395,0.26353455136914)
--(axis cs:34.3949044585987,0.256969487039752)
--(axis cs:35.031847133758,0.243311283563317)
--(axis cs:35.6687898089172,0.237514073967118)
--(axis cs:36.3057324840764,0.236356975983084)
--(axis cs:36.9426751592357,0.228568656907831)
--(axis cs:37.5796178343949,0.217364532142954)
--(axis cs:38.2165605095541,0.21713828866239)
--(axis cs:38.8535031847134,0.213701078828791)
--(axis cs:39.4904458598726,0.208794941951123)
--(axis cs:40.1273885350318,0.206455908622113)
--(axis cs:40.7643312101911,0.20873772534688)
--(axis cs:41.4012738853503,0.207266278839378)
--(axis cs:42.0382165605096,0.199732997230266)
--(axis cs:42.6751592356688,0.195032465348367)
--(axis cs:43.312101910828,0.18352752577371)
--(axis cs:43.9490445859873,0.179900178399757)
--(axis cs:44.5859872611465,0.177050695802099)
--(axis cs:45.2229299363057,0.176093333673918)
--(axis cs:45.859872611465,0.171295609803258)
--(axis cs:46.4968152866242,0.164457991206325)
--(axis cs:47.1337579617834,0.158571397512146)
--(axis cs:47.7707006369427,0.161965274828294)
--(axis cs:48.4076433121019,0.161455857509688)
--(axis cs:49.0445859872611,0.15551704262403)
--(axis cs:49.6815286624204,0.151891319033721)
--(axis cs:50.3184713375796,0.146304115926046)
--(axis cs:50.9554140127388,0.142813731664724)
--(axis cs:51.5923566878981,0.134935624403432)
--(axis cs:52.2292993630573,0.131312169105051)
--(axis cs:52.8662420382166,0.12676635059715)
--(axis cs:53.5031847133758,0.121237931726606)
--(axis cs:54.140127388535,0.117749296031556)
--(axis cs:54.7770700636943,0.118749001394678)
--(axis cs:55.4140127388535,0.115159563861666)
--(axis cs:56.0509554140127,0.117119875245558)
--(axis cs:56.687898089172,0.111193158257923)
--(axis cs:57.3248407643312,0.106574479050483)
--(axis cs:57.9617834394904,0.102698828801462)
--(axis cs:58.5987261146497,0.0919857202557939)
--(axis cs:59.2356687898089,0.0855466688461837)
--(axis cs:59.8726114649682,0.0806458105385217)
--(axis cs:60.5095541401274,0.0786124725919159)
--(axis cs:61.1464968152866,0.0711658007258922)
--(axis cs:61.7834394904459,0.0696617633339108)
--(axis cs:62.4203821656051,0.0689225370493797)
--(axis cs:63.0573248407643,0.0621926462723631)
--(axis cs:63.6942675159236,0.064349647232737)
--(axis cs:64.3312101910828,0.0524443775841065)
--(axis cs:64.968152866242,0.0518476558219809)
--(axis cs:65.6050955414013,0.0474388679810551)
--(axis cs:66.2420382165605,0.0434346203131024)
--(axis cs:66.8789808917197,0.0444344915456232)
--(axis cs:67.515923566879,0.038586629864748)
--(axis cs:68.1528662420382,0.0372087150286499)
--(axis cs:68.7898089171974,0.0349767343748005)
--(axis cs:69.4267515923567,0.0310724089603542)
--(axis cs:70.0636942675159,0.0267523092530794)
--(axis cs:70.7006369426752,0.0284143265845407)
--(axis cs:71.3375796178344,0.0281517441940435)
--(axis cs:71.9745222929936,0.0261381086923109)
--(axis cs:72.6114649681529,0.0225376214511982)
--(axis cs:73.2484076433121,0.0210950569016702)
--(axis cs:73.8853503184713,0.0205868940894449)
--(axis cs:74.5222929936306,0.018691640119402)
--(axis cs:75.1592356687898,0.0176465623028053)
--(axis cs:75.796178343949,0.0164921276726826)
--(axis cs:76.4331210191083,0.0156485223814779)
--(axis cs:77.0700636942675,0.0141966949675974)
--(axis cs:77.7070063694268,0.0112323448255735)
--(axis cs:78.343949044586,0.0117464345638156)
--(axis cs:78.9808917197452,0.012210824621402)
--(axis cs:79.6178343949044,0.00954916822758318)
--(axis cs:80.2547770700637,0.0101047007139354)
--(axis cs:80.8917197452229,0.00917698856986116)
--(axis cs:81.5286624203822,0.00753731741921305)
--(axis cs:82.1656050955414,0.00704608735272896)
--(axis cs:82.8025477707006,0.00650721742724567)
--(axis cs:83.4394904458599,0.00793717742117991)
--(axis cs:84.0764331210191,0.00810527442340175)
--(axis cs:84.7133757961783,0.0073168925981248)
--(axis cs:85.3503184713376,0.00475453670879459)
--(axis cs:85.9872611464968,0.00295505755059431)
--(axis cs:86.6242038216561,0.0026625665281629)
--(axis cs:87.2611464968153,0.00283845802853072)
--(axis cs:87.8980891719745,0.00288691548038814)
--(axis cs:88.5350318471338,0.00278531863301713)
--(axis cs:89.171974522293,0.00248338498676612)
--(axis cs:89.8089171974522,0.00173731132069798)
--(axis cs:90.4458598726115,0.00194751869166625)
--(axis cs:91.0828025477707,0.00190568768294877)
--(axis cs:91.7197452229299,0.00146466454206043)
--(axis cs:92.3566878980892,0.000496744157095181)
--(axis cs:92.9936305732484,0.000324528552294767)
--(axis cs:93.6305732484076,0.000146130391257753)
--(axis cs:94.2675159235669,3.48608221631672e-05)
--(axis cs:94.9044585987261,5.5340726735837e-05)
--(axis cs:95.5414012738853,3.30752558357518e-05)
--(axis cs:96.1783439490446,6.91545494854949e-06)
--(axis cs:96.8152866242038,5.33987286215781e-06)
--(axis cs:97.4522292993631,4.03717428579361e-06)
--(axis cs:98.0891719745223,4.52332802519322e-06)
--(axis cs:98.7261146496815,3.11281701933926e-06)
--(axis cs:99.3630573248408,1.66908068379098e-06)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:100,0)
--(axis cs:99.3630573248408,2.29604973797707e-06)
--(axis cs:98.7261146496815,3.60310285962643e-06)
--(axis cs:98.0891719745223,1.26507601524495e-05)
--(axis cs:97.4522292993631,1.51365169764428e-05)
--(axis cs:96.8152866242038,1.26306589174963e-05)
--(axis cs:96.1783439490446,1.85921801344569e-05)
--(axis cs:95.5414012738853,9.94575871060087e-05)
--(axis cs:94.9044585987261,0.000138452041021864)
--(axis cs:94.2675159235669,9.6164247977977e-05)
--(axis cs:93.6305732484076,0.000354425325469079)
--(axis cs:92.9936305732484,0.00074277366807786)
--(axis cs:92.3566878980892,0.00108447906719101)
--(axis cs:91.7197452229299,0.00258666519821352)
--(axis cs:91.0828025477707,0.00328969095415076)
--(axis cs:90.4458598726115,0.00336549784376365)
--(axis cs:89.8089171974522,0.0030799092557337)
--(axis cs:89.171974522293,0.00408132430738447)
--(axis cs:88.5350318471338,0.00456235442499045)
--(axis cs:87.8980891719745,0.00475067338171869)
--(axis cs:87.2611464968153,0.00474514378303002)
--(axis cs:86.6242038216561,0.00434487145967079)
--(axis cs:85.9872611464968,0.00488349607978447)
--(axis cs:85.3503184713376,0.00726990890617125)
--(axis cs:84.7133757961783,0.0101756542616847)
--(axis cs:84.0764331210191,0.010916591554236)
--(axis cs:83.4394904458599,0.0107648000317888)
--(axis cs:82.8025477707006,0.00923938579464982)
--(axis cs:82.1656050955414,0.00980251689093755)
--(axis cs:81.5286624203822,0.0103885488552138)
--(axis cs:80.8917197452229,0.0121292009933826)
--(axis cs:80.2547770700637,0.0130416696868847)
--(axis cs:79.6178343949044,0.012424283971302)
--(axis cs:78.9808917197452,0.0149726605193395)
--(axis cs:78.343949044586,0.0147695277680524)
--(axis cs:77.7070063694268,0.0143884610915058)
--(axis cs:77.0700636942675,0.0170243717555919)
--(axis cs:76.4331210191083,0.0183054363755451)
--(axis cs:75.796178343949,0.0191253309466543)
--(axis cs:75.1592356687898,0.0206140969987268)
--(axis cs:74.5222929936306,0.0223984760717879)
--(axis cs:73.8853503184713,0.0247820008018454)
--(axis cs:73.2484076433121,0.0255461134401912)
--(axis cs:72.6114649681529,0.0272853736834067)
--(axis cs:71.9745222929936,0.0311528167583025)
--(axis cs:71.3375796178344,0.0335219945376294)
--(axis cs:70.7006369426752,0.0336297747603926)
--(axis cs:70.0636942675159,0.0321909026677904)
--(axis cs:69.4267515923567,0.0371913335061161)
--(axis cs:68.7898089171974,0.0414327136126482)
--(axis cs:68.1528662420382,0.0436848038344674)
--(axis cs:67.515923566879,0.0456979022245879)
--(axis cs:66.8789808917197,0.0520240631022484)
--(axis cs:66.2420382165605,0.0509663634361614)
--(axis cs:65.6050955414013,0.0552909417196375)
--(axis cs:64.968152866242,0.060057517334449)
--(axis cs:64.3312101910828,0.0605201492409988)
--(axis cs:63.6942675159236,0.0731798435154164)
--(axis cs:63.0573248407643,0.0706708555256324)
--(axis cs:62.4203821656051,0.0776983827385755)
--(axis cs:61.7834394904459,0.0783834366097676)
--(axis cs:61.1464968152866,0.0801608466603004)
--(axis cs:60.5095541401274,0.0878506593324356)
--(axis cs:59.8726114649682,0.0900158106300368)
--(axis cs:59.2356687898089,0.0949993502630151)
--(axis cs:58.5987261146497,0.101841729273402)
--(axis cs:57.9617834394904,0.11252972369321)
--(axis cs:57.3248407643312,0.115945221676625)
--(axis cs:56.687898089172,0.120543771178447)
--(axis cs:56.0509554140127,0.126284017449171)
--(axis cs:55.4140127388535,0.124829570529763)
--(axis cs:54.7770700636943,0.128370691015815)
--(axis cs:54.140127388535,0.127358241371791)
--(axis cs:53.5031847133758,0.131164482078535)
--(axis cs:52.8662420382166,0.136896688211411)
--(axis cs:52.2292993630573,0.141870391411379)
--(axis cs:51.5923566878981,0.145256102524128)
--(axis cs:50.9554140127388,0.153196583506319)
--(axis cs:50.3184713375796,0.156735088644217)
--(axis cs:49.6815286624204,0.162435763354255)
--(axis cs:49.0445859872611,0.1659615768828)
--(axis cs:48.4076433121019,0.172109560983462)
--(axis cs:47.7707006369427,0.172315514868137)
--(axis cs:47.1337579617834,0.168966691997774)
--(axis cs:46.4968152866242,0.175170000805977)
--(axis cs:45.859872611465,0.182454440449616)
--(axis cs:45.2229299363057,0.186958436190073)
--(axis cs:44.5859872611465,0.188235531264009)
--(axis cs:43.9490445859873,0.191125192861003)
--(axis cs:43.312101910828,0.195079935770146)
--(axis cs:42.6751592356688,0.207082441637005)
--(axis cs:42.0382165605096,0.212091779179029)
--(axis cs:41.4012738853503,0.219919931933882)
--(axis cs:40.7643312101911,0.221908335546094)
--(axis cs:40.1273885350318,0.219568637610562)
--(axis cs:39.4904458598726,0.22218587730645)
--(axis cs:38.8535031847134,0.227199175766795)
--(axis cs:38.2165605095541,0.230409698878858)
--(axis cs:37.5796178343949,0.230703654911122)
--(axis cs:36.9426751592357,0.242132451317552)
--(axis cs:36.3057324840764,0.250258002382023)
--(axis cs:35.6687898089172,0.251711723691365)
--(axis cs:35.031847133758,0.257700234984731)
--(axis cs:34.3949044585987,0.271567454021768)
--(axis cs:33.7579617834395,0.278435048229602)
--(axis cs:33.1210191082803,0.288879470717377)
--(axis cs:32.484076433121,0.300932635320559)
--(axis cs:31.8471337579618,0.319633407763846)
--(axis cs:31.2101910828025,0.327384210196073)
--(axis cs:30.5732484076433,0.338747962171133)
--(axis cs:29.9363057324841,0.344725504772332)
--(axis cs:29.2993630573248,0.359789505539274)
--(axis cs:28.6624203821656,0.366792904574673)
--(axis cs:28.0254777070064,0.377022096112374)
--(axis cs:27.3885350318471,0.384427913496644)
--(axis cs:26.7515923566879,0.400078170188165)
--(axis cs:26.1146496815287,0.406071425039519)
--(axis cs:25.4777070063694,0.418402358703037)
--(axis cs:24.8407643312102,0.433993842837533)
--(axis cs:24.203821656051,0.438291660586274)
--(axis cs:23.5668789808917,0.45055008510358)
--(axis cs:22.9299363057325,0.461300081176186)
--(axis cs:22.2929936305732,0.482807637873409)
--(axis cs:21.656050955414,0.497700267995084)
--(axis cs:21.0191082802548,0.513879248256832)
--(axis cs:20.3821656050955,0.534656793553578)
--(axis cs:19.7452229299363,0.550652617762109)
--(axis cs:19.1082802547771,0.5640378725732)
--(axis cs:18.4713375796178,0.585840906659232)
--(axis cs:17.8343949044586,0.608687167571806)
--(axis cs:17.1974522292994,0.619872709615314)
--(axis cs:16.5605095541401,0.637098262151856)
--(axis cs:15.9235668789809,0.649849837395333)
--(axis cs:15.2866242038217,0.667928108770394)
--(axis cs:14.6496815286624,0.680333800279216)
--(axis cs:14.0127388535032,0.697956705612467)
--(axis cs:13.3757961783439,0.715146178729393)
--(axis cs:12.7388535031847,0.732883751566967)
--(axis cs:12.1019108280255,0.756893413898288)
--(axis cs:11.4649681528662,0.772910963220706)
--(axis cs:10.828025477707,0.796727135629296)
--(axis cs:10.1910828025478,0.809529681661548)
--(axis cs:9.55414012738853,0.830054018611321)
--(axis cs:8.9171974522293,0.845295221913862)
--(axis cs:8.28025477707006,0.856335160218916)
--(axis cs:7.64331210191083,0.871818038681802)
--(axis cs:7.00636942675159,0.881405409723466)
--(axis cs:6.36942675159236,0.888905274772407)
--(axis cs:5.73248407643312,0.898230384332914)
--(axis cs:5.09554140127389,0.90258772612172)
--(axis cs:4.45859872611465,0.907045156836656)
--(axis cs:3.82165605095541,0.910556527275633)
--(axis cs:3.18471337579618,0.912378009696237)
--(axis cs:2.54777070063694,0.914047692799203)
--(axis cs:1.91082802547771,0.915185727388214)
--(axis cs:1.27388535031847,0.915645427664132)
--(axis cs:0.636942675159236,0.915845659612225)
--(axis cs:0,0.916030337935273)
--cycle;



==> img/mnist/mnist_rate_distortion_shap.tex <==
% shap
\addplot [line width=0.5, opacity=0.8, color2, mark=diamond*, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color2, thin}]
table [row sep=\\]{%
0	0.915477395675844 \\
0.636942675159236	0.915511147875804 \\
1.27388535031847	0.91523094269447 \\
1.91082802547771	0.915310140494257 \\
2.54777070063694	0.915032456025947 \\
3.18471337579618	0.914434120451333 \\
3.82165605095541	0.914099645855604 \\
4.45859872611465	0.913779714424163 \\
5.09554140127389	0.91361902019009 \\
5.73248407643312	0.913372550164349 \\
6.36942675159236	0.913010667869821 \\
7.00636942675159	0.912039429533761 \\
7.64331210191083	0.909894335959107 \\
8.28025477707006	0.908838596958667 \\
8.9171974522293	0.907883301239926 \\
9.55414012738853	0.907296717767604 \\
10.1910828025478	0.905396919499617 \\
10.828025477707	0.901142768035643 \\
11.4649681528662	0.898582000848837 \\
12.1019108280255	0.895096784201451 \\
12.7388535031847	0.892796833626926 \\
13.3757961783439	0.89149837047793 \\
14.0127388535032	0.884343902743421 \\
14.6496815286624	0.879194337511435 \\
15.2866242038217	0.874038779623806 \\
15.9235668789809	0.868558812570991 \\
16.5605095541401	0.862101169141242 \\
17.1974522292994	0.856509993218351 \\
17.8343949044586	0.851266257190146 \\
18.4713375796178	0.843952705818228 \\
19.1082802547771	0.841076957141049 \\
19.7452229299363	0.837394347586669 \\
20.3821656050955	0.82807102666935 \\
21.0191082802548	0.822319729411975 \\
21.656050955414	0.812132446151227 \\
22.2929936305732	0.804173510354012 \\
22.9299363057325	0.79759049186483 \\
23.5668789808917	0.79047057193704 \\
24.203821656051	0.780370560614392 \\
24.8407643312102	0.774947629636154 \\
25.4777070063694	0.772054685857147 \\
26.1146496815287	0.769325117454864 \\
26.7515923566879	0.764819280067459 \\
27.3885350318471	0.761887535266578 \\
28.0254777070064	0.7548429362569 \\
28.6624203821656	0.748287306893617 \\
29.2993630573248	0.743654732573777 \\
29.9363057324841	0.733861412405968 \\
30.5732484076433	0.730378737822175 \\
31.2101910828025	0.722686512209475 \\
31.8471337579618	0.72194671548903 \\
32.484076433121	0.71801952585578 \\
33.1210191082803	0.714731817133725 \\
33.7579617834395	0.711754213836975 \\
34.3949044585987	0.705650139031932 \\
35.031847133758	0.705868469001725 \\
35.6687898089172	0.703618133598939 \\
36.3057324840764	0.697479651141912 \\
36.9426751592357	0.690944092925638 \\
37.5796178343949	0.694175007613376 \\
38.2165605095541	0.692502810917795 \\
38.8535031847134	0.687400265466422 \\
39.4904458598726	0.689671418783255 \\
40.1273885350318	0.687663124892861 \\
40.7643312101911	0.678960220878944 \\
41.4012738853503	0.669229168836027 \\
42.0382165605096	0.668338434440084 \\
42.6751592356688	0.669889817857183 \\
43.312101910828	0.669701692247763 \\
43.9490445859873	0.664348899368197 \\
44.5859872611465	0.665642134672962 \\
45.2229299363057	0.663670832196949 \\
45.859872611465	0.661964732459746 \\
46.4968152866242	0.65365864052088 \\
47.1337579617834	0.655439198247623 \\
47.7707006369427	0.652553067980334 \\
48.4076433121019	0.64408131641103 \\
49.0445859872611	0.639602767397882 \\
49.6815286624204	0.639637372879079 \\
50.3184713375796	0.641376153710298 \\
50.9554140127388	0.638386122397787 \\
51.5923566878981	0.635676244386123 \\
52.2292993630573	0.629696358237416 \\
52.8662420382166	0.633338759868784 \\
53.5031847133758	0.629449003195041 \\
54.140127388535	0.626316953974419 \\
54.7770700636943	0.620768784034153 \\
55.4140127388535	0.614643598369403 \\
56.0509554140127	0.613201194615067 \\
56.687898089172	0.610676424894982 \\
57.3248407643312	0.609995668041192 \\
57.9617834394904	0.609247906311766 \\
58.5987261146497	0.607384794002619 \\
59.2356687898089	0.604885708196612 \\
59.8726114649682	0.59919165239792 \\
60.5095541401274	0.598062005765395 \\
61.1464968152866	0.590166698190842 \\
61.7834394904459	0.588356541625099 \\
62.4203821656051	0.58755636946834 \\
63.0573248407643	0.588520232785617 \\
63.6942675159236	0.587103485856085 \\
64.3312101910828	0.582748551361539 \\
64.968152866242	0.588874187678941 \\
65.6050955414013	0.584686306763619 \\
66.2420382165605	0.587002407784243 \\
66.8789808917197	0.584073000435255 \\
67.515923566879	0.584844367509618 \\
68.1528662420382	0.583766357564741 \\
68.7898089171974	0.582345600171041 \\
69.4267515923567	0.587047143775225 \\
70.0636942675159	0.590470428790828 \\
70.7006369426752	0.582507245470885 \\
71.3375796178344	0.583191083987384 \\
71.9745222929936	0.579457557982214 \\
72.6114649681529	0.569434075110019 \\
73.2484076433121	0.556308685765768 \\
73.8853503184713	0.552028885662143 \\
74.5222929936306	0.552408839710031 \\
75.1592356687898	0.547264606718391 \\
75.796178343949	0.539718238278779 \\
76.4331210191083	0.535806615671316 \\
77.0700636942675	0.528482525372026 \\
77.7070063694268	0.522452853562301 \\
78.343949044586	0.523023076725744 \\
78.9808917197452	0.52368097078342 \\
79.6178343949044	0.520890309987194 \\
80.2547770700637	0.513692979783816 \\
80.8917197452229	0.505992818632442 \\
81.5286624203822	0.505030490039406 \\
82.1656050955414	0.510376583280526 \\
82.8025477707006	0.490542813220752 \\
83.4394904458599	0.477308900030246 \\
84.0764331210191	0.464180434307764 \\
84.7133757961783	0.454794038475045 \\
85.3503184713376	0.445885110331197 \\
85.9872611464968	0.430105680548189 \\
86.6242038216561	0.411076853237216 \\
87.2611464968153	0.387449200892372 \\
87.8980891719745	0.381118794276689 \\
88.5350318471338	0.372779634876447 \\
89.171974522293	0.363113671293456 \\
89.8089171974522	0.352633310552169 \\
90.4458598726115	0.336953488375537 \\
91.0828025477707	0.30955926877549 \\
91.7197452229299	0.280732427353365 \\
92.3566878980892	0.254482224605332 \\
92.9936305732484	0.223798617336351 \\
93.6305732484076	0.18470277938108 \\
94.2675159235669	0.148494441216895 \\
94.9044585987261	0.123165624817437 \\
95.5414012738853	0.0971234421808641 \\
96.1783439490446	0.0709743985113931 \\
96.8152866242038	0.053121124989227 \\
97.4522292993631	0.0333780459052717 \\
98.0891719745223	0.0183998673348846 \\
98.7261146496815	0.00683993043484116 \\
99.3630573248408	0.000543539782451649 \\
100	9.07070329958515e-11 \\
};
\path [fill=color2, fill opacity=0.5] (axis cs:0,0.916049506892377)
--(axis cs:0,0.914905284459311)
--(axis cs:0.636942675159236,0.91493122425783)
--(axis cs:1.27388535031847,0.914576144287567)
--(axis cs:1.91082802547771,0.914672379973805)
--(axis cs:2.54777070063694,0.914332043803053)
--(axis cs:3.18471337579618,0.913654411933798)
--(axis cs:3.82165605095541,0.913194594169858)
--(axis cs:4.45859872611465,0.912738959795478)
--(axis cs:5.09554140127389,0.912648657087667)
--(axis cs:5.73248407643312,0.912357116182845)
--(axis cs:6.36942675159236,0.91199440454898)
--(axis cs:7.00636942675159,0.910890400552742)
--(axis cs:7.64331210191083,0.908432630106539)
--(axis cs:8.28025477707006,0.907206935050909)
--(axis cs:8.9171974522293,0.906098065643346)
--(axis cs:9.55414012738853,0.905393707114881)
--(axis cs:10.1910828025478,0.903371881988777)
--(axis cs:10.828025477707,0.898666668893119)
--(axis cs:11.4649681528662,0.895822819992567)
--(axis cs:12.1019108280255,0.891986604416472)
--(axis cs:12.7388535031847,0.889436788160117)
--(axis cs:13.3757961783439,0.888146608142128)
--(axis cs:14.0127388535032,0.880482807805517)
--(axis cs:14.6496815286624,0.87491773572741)
--(axis cs:15.2866242038217,0.869479379056286)
--(axis cs:15.9235668789809,0.863730411549977)
--(axis cs:16.5605095541401,0.856967964900791)
--(axis cs:17.1974522292994,0.85115954410907)
--(axis cs:17.8343949044586,0.845638350003838)
--(axis cs:18.4713375796178,0.838093090998757)
--(axis cs:19.1082802547771,0.835081275388442)
--(axis cs:19.7452229299363,0.831090465253887)
--(axis cs:20.3821656050955,0.821690679023874)
--(axis cs:21.0191082802548,0.815750824875489)
--(axis cs:21.656050955414,0.805431220291406)
--(axis cs:22.2929936305732,0.797438405197756)
--(axis cs:22.9299363057325,0.790750662169463)
--(axis cs:23.5668789808917,0.78364973812222)
--(axis cs:24.203821656051,0.773471456120089)
--(axis cs:24.8407643312102,0.768065441658717)
--(axis cs:25.4777070063694,0.765094273178371)
--(axis cs:26.1146496815287,0.762339186825006)
--(axis cs:26.7515923566879,0.757914208517391)
--(axis cs:27.3885350318471,0.755042316819805)
--(axis cs:28.0254777070064,0.747858182339109)
--(axis cs:28.6624203821656,0.741331373614849)
--(axis cs:29.2993630573248,0.736617172309584)
--(axis cs:29.9363057324841,0.726586893027568)
--(axis cs:30.5732484076433,0.723283167843198)
--(axis cs:31.2101910828025,0.715574061314778)
--(axis cs:31.8471337579618,0.71472836452909)
--(axis cs:32.484076433121,0.710832207332703)
--(axis cs:33.1210191082803,0.70744664956009)
--(axis cs:33.7579617834395,0.704443340829568)
--(axis cs:34.3949044585987,0.698378898713345)
--(axis cs:35.031847133758,0.698406695715921)
--(axis cs:35.6687898089172,0.696358073407005)
--(axis cs:36.3057324840764,0.69004554155067)
--(axis cs:36.9426751592357,0.683488468739222)
--(axis cs:37.5796178343949,0.686608940420753)
--(axis cs:38.2165605095541,0.684953001038339)
--(axis cs:38.8535031847134,0.679886874271344)
--(axis cs:39.4904458598726,0.682226701479848)
--(axis cs:40.1273885350318,0.680281594355497)
--(axis cs:40.7643312101911,0.671577612482737)
--(axis cs:41.4012738853503,0.661778623348505)
--(axis cs:42.0382165605096,0.66079548600873)
--(axis cs:42.6751592356688,0.662271926664028)
--(axis cs:43.312101910828,0.662168046541245)
--(axis cs:43.9490445859873,0.656784850605555)
--(axis cs:44.5859872611465,0.65813220031326)
--(axis cs:45.2229299363057,0.656207690322488)
--(axis cs:45.859872611465,0.654495401566054)
--(axis cs:46.4968152866242,0.64619468531643)
--(axis cs:47.1337579617834,0.648119408002557)
--(axis cs:47.7707006369427,0.645106045416762)
--(axis cs:48.4076433121019,0.636630778910066)
--(axis cs:49.0445859872611,0.632125481396388)
--(axis cs:49.6815286624204,0.632270395751125)
--(axis cs:50.3184713375796,0.633919682257004)
--(axis cs:50.9554140127388,0.630996452821997)
--(axis cs:51.5923566878981,0.628343694432084)
--(axis cs:52.2292993630573,0.622424317006504)
--(axis cs:52.8662420382166,0.62609626215595)
--(axis cs:53.5031847133758,0.622322403949618)
--(axis cs:54.140127388535,0.619136621470383)
--(axis cs:54.7770700636943,0.613597802611038)
--(axis cs:55.4140127388535,0.6075131981624)
--(axis cs:56.0509554140127,0.606091386043714)
--(axis cs:56.687898089172,0.603620516371788)
--(axis cs:57.3248407643312,0.603016394418606)
--(axis cs:57.9617834394904,0.602459783240978)
--(axis cs:58.5987261146497,0.600566038926534)
--(axis cs:59.2356687898089,0.598164958462699)
--(axis cs:59.8726114649682,0.592418235480014)
--(axis cs:60.5095541401274,0.591251183214568)
--(axis cs:61.1464968152866,0.5833421110539)
--(axis cs:61.7834394904459,0.581689728928597)
--(axis cs:62.4203821656051,0.580982309465094)
--(axis cs:63.0573248407643,0.58206844592957)
--(axis cs:63.6942675159236,0.580712204086444)
--(axis cs:64.3312101910828,0.576213666724949)
--(axis cs:64.968152866242,0.582225122254452)
--(axis cs:65.6050955414013,0.578023979414449)
--(axis cs:66.2420382165605,0.580558972907406)
--(axis cs:66.8789808917197,0.577534928844322)
--(axis cs:67.515923566879,0.578379676801768)
--(axis cs:68.1528662420382,0.577354207948176)
--(axis cs:68.7898089171974,0.576116712771462)
--(axis cs:69.4267515923567,0.580878334073675)
--(axis cs:70.0636942675159,0.58431379199394)
--(axis cs:70.7006369426752,0.576230672929248)
--(axis cs:71.3375796178344,0.577075338612604)
--(axis cs:71.9745222929936,0.573342261562168)
--(axis cs:72.6114649681529,0.563049147396053)
--(axis cs:73.2484076433121,0.549844526643871)
--(axis cs:73.8853503184713,0.545669495036954)
--(axis cs:74.5222929936306,0.546113522823173)
--(axis cs:75.1592356687898,0.540988254881627)
--(axis cs:75.796178343949,0.533218503011879)
--(axis cs:76.4331210191083,0.529460579779123)
--(axis cs:77.0700636942675,0.522041631320834)
--(axis cs:77.7070063694268,0.516111487112685)
--(axis cs:78.343949044586,0.516664757124845)
--(axis cs:78.9808917197452,0.517287439638091)
--(axis cs:79.6178343949044,0.514539776998758)
--(axis cs:80.2547770700637,0.507331161531243)
--(axis cs:80.8917197452229,0.499624673139667)
--(axis cs:81.5286624203822,0.498456325906857)
--(axis cs:82.1656050955414,0.503989189827973)
--(axis cs:82.8025477707006,0.483980197196473)
--(axis cs:83.4394904458599,0.470946520486814)
--(axis cs:84.0764331210191,0.45794923527021)
--(axis cs:84.7133757961783,0.448672954452318)
--(axis cs:85.3503184713376,0.43980659182689)
--(axis cs:85.9872611464968,0.424004450933117)
--(axis cs:86.6242038216561,0.405095859349822)
--(axis cs:87.2611464968153,0.381555593303609)
--(axis cs:87.8980891719745,0.37523304899751)
--(axis cs:88.5350318471338,0.36692749146349)
--(axis cs:89.171974522293,0.357378629302664)
--(axis cs:89.8089171974522,0.346798782519285)
--(axis cs:90.4458598726115,0.331375416387423)
--(axis cs:91.0828025477707,0.303710370799496)
--(axis cs:91.7197452229299,0.274564863915845)
--(axis cs:92.3566878980892,0.248469829005981)
--(axis cs:92.9936305732484,0.21761878812895)
--(axis cs:93.6305732484076,0.179182580772701)
--(axis cs:94.2675159235669,0.143808109690262)
--(axis cs:94.9044585987261,0.1191798490947)
--(axis cs:95.5414012738853,0.09288018561793)
--(axis cs:96.1783439490446,0.0673181064983714)
--(axis cs:96.8152866242038,0.0497619988042344)
--(axis cs:97.4522292993631,0.0303187099508092)
--(axis cs:98.0891719745223,0.0156867875812114)
--(axis cs:98.7261146496815,0.00528604920913444)
--(axis cs:99.3630573248408,0.000285738430164731)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,0.000801341134738566)
--(axis cs:98.7261146496815,0.00839381166054789)
--(axis cs:98.0891719745223,0.0211129470885578)
--(axis cs:97.4522292993631,0.0364373818597343)
--(axis cs:96.8152866242038,0.0564802511742197)
--(axis cs:96.1783439490446,0.0746306905244148)
--(axis cs:95.5414012738853,0.101366698743798)
--(axis cs:94.9044585987261,0.127151400540174)
--(axis cs:94.2675159235669,0.153180772743527)
--(axis cs:93.6305732484076,0.190222977989458)
--(axis cs:92.9936305732484,0.229978446543751)
--(axis cs:92.3566878980892,0.260494620204684)
--(axis cs:91.7197452229299,0.286899990790885)
--(axis cs:91.0828025477707,0.315408166751484)
--(axis cs:90.4458598726115,0.34253156036365)
--(axis cs:89.8089171974522,0.358467838585053)
--(axis cs:89.171974522293,0.368848713284247)
--(axis cs:88.5350318471338,0.378631778289405)
--(axis cs:87.8980891719745,0.387004539555868)
--(axis cs:87.2611464968153,0.393342808481134)
--(axis cs:86.6242038216561,0.417057847124611)
--(axis cs:85.9872611464968,0.436206910163261)
--(axis cs:85.3503184713376,0.451963628835504)
--(axis cs:84.7133757961783,0.460915122497773)
--(axis cs:84.0764331210191,0.470411633345318)
--(axis cs:83.4394904458599,0.483671279573677)
--(axis cs:82.8025477707006,0.497105429245031)
--(axis cs:82.1656050955414,0.516763976733079)
--(axis cs:81.5286624203822,0.511604654171955)
--(axis cs:80.8917197452229,0.512360964125216)
--(axis cs:80.2547770700637,0.520054798036389)
--(axis cs:79.6178343949044,0.52724084297563)
--(axis cs:78.9808917197452,0.53007450192875)
--(axis cs:78.343949044586,0.529381396326642)
--(axis cs:77.7070063694268,0.528794220011918)
--(axis cs:77.0700636942675,0.534923419423218)
--(axis cs:76.4331210191083,0.542152651563509)
--(axis cs:75.796178343949,0.54621797354568)
--(axis cs:75.1592356687898,0.553540958555154)
--(axis cs:74.5222929936306,0.558704156596888)
--(axis cs:73.8853503184713,0.558388276287333)
--(axis cs:73.2484076433121,0.562772844887665)
--(axis cs:72.6114649681529,0.575819002823985)
--(axis cs:71.9745222929936,0.58557285440226)
--(axis cs:71.3375796178344,0.589306829362165)
--(axis cs:70.7006369426752,0.588783818012521)
--(axis cs:70.0636942675159,0.596627065587717)
--(axis cs:69.4267515923567,0.593215953476774)
--(axis cs:68.7898089171974,0.588574487570619)
--(axis cs:68.1528662420382,0.590178507181307)
--(axis cs:67.515923566879,0.591309058217469)
--(axis cs:66.8789808917197,0.590611072026188)
--(axis cs:66.2420382165605,0.59344584266108)
--(axis cs:65.6050955414013,0.591348634112789)
--(axis cs:64.968152866242,0.595523253103431)
--(axis cs:64.3312101910828,0.589283435998129)
--(axis cs:63.6942675159236,0.593494767625725)
--(axis cs:63.0573248407643,0.594972019641665)
--(axis cs:62.4203821656051,0.594130429471586)
--(axis cs:61.7834394904459,0.595023354321601)
--(axis cs:61.1464968152866,0.596991285327784)
--(axis cs:60.5095541401274,0.604872828316221)
--(axis cs:59.8726114649682,0.605965069315827)
--(axis cs:59.2356687898089,0.611606457930524)
--(axis cs:58.5987261146497,0.614203549078703)
--(axis cs:57.9617834394904,0.616036029382555)
--(axis cs:57.3248407643312,0.616974941663779)
--(axis cs:56.687898089172,0.617732333418176)
--(axis cs:56.0509554140127,0.62031100318642)
--(axis cs:55.4140127388535,0.621773998576405)
--(axis cs:54.7770700636943,0.627939765457268)
--(axis cs:54.140127388535,0.633497286478456)
--(axis cs:53.5031847133758,0.636575602440463)
--(axis cs:52.8662420382166,0.640581257581618)
--(axis cs:52.2292993630573,0.636968399468327)
--(axis cs:51.5923566878981,0.643008794340161)
--(axis cs:50.9554140127388,0.645775791973578)
--(axis cs:50.3184713375796,0.648832625163592)
--(axis cs:49.6815286624204,0.647004350007032)
--(axis cs:49.0445859872611,0.647080053399377)
--(axis cs:48.4076433121019,0.651531853911993)
--(axis cs:47.7707006369427,0.660000090543907)
--(axis cs:47.1337579617834,0.662758988492689)
--(axis cs:46.4968152866242,0.66112259572533)
--(axis cs:45.859872611465,0.669434063353439)
--(axis cs:45.2229299363057,0.67113397407141)
--(axis cs:44.5859872611465,0.673152069032665)
--(axis cs:43.9490445859873,0.671912948130838)
--(axis cs:43.312101910828,0.677235337954281)
--(axis cs:42.6751592356688,0.677507709050339)
--(axis cs:42.0382165605096,0.675881382871437)
--(axis cs:41.4012738853503,0.67667971432355)
--(axis cs:40.7643312101911,0.68634282927515)
--(axis cs:40.1273885350318,0.695044655430225)
--(axis cs:39.4904458598726,0.697116136086662)
--(axis cs:38.8535031847134,0.6949136566615)
--(axis cs:38.2165605095541,0.700052620797251)
--(axis cs:37.5796178343949,0.701741074805999)
--(axis cs:36.9426751592357,0.698399717112054)
--(axis cs:36.3057324840764,0.704913760733153)
--(axis cs:35.6687898089172,0.710878193790873)
--(axis cs:35.031847133758,0.713330242287529)
--(axis cs:34.3949044585987,0.712921379350519)
--(axis cs:33.7579617834395,0.719065086844383)
--(axis cs:33.1210191082803,0.72201698470736)
--(axis cs:32.484076433121,0.725206844378856)
--(axis cs:31.8471337579618,0.72916506644897)
--(axis cs:31.2101910828025,0.729798963104172)
--(axis cs:30.5732484076433,0.737474307801152)
--(axis cs:29.9363057324841,0.741135931784367)
--(axis cs:29.2993630573248,0.750692292837971)
--(axis cs:28.6624203821656,0.755243240172385)
--(axis cs:28.0254777070064,0.761827690174692)
--(axis cs:27.3885350318471,0.768732753713351)
--(axis cs:26.7515923566879,0.771724351617527)
--(axis cs:26.1146496815287,0.776311048084722)
--(axis cs:25.4777070063694,0.779015098535923)
--(axis cs:24.8407643312102,0.78182981761359)
--(axis cs:24.203821656051,0.787269665108695)
--(axis cs:23.5668789808917,0.797291405751859)
--(axis cs:22.9299363057325,0.804430321560197)
--(axis cs:22.2929936305732,0.810908615510268)
--(axis cs:21.656050955414,0.818833672011047)
--(axis cs:21.0191082802548,0.82888863394846)
--(axis cs:20.3821656050955,0.834451374314825)
--(axis cs:19.7452229299363,0.843698229919451)
--(axis cs:19.1082802547771,0.847072638893656)
--(axis cs:18.4713375796178,0.8498123206377)
--(axis cs:17.8343949044586,0.856894164376453)
--(axis cs:17.1974522292994,0.861860442327632)
--(axis cs:16.5605095541401,0.867234373381693)
--(axis cs:15.9235668789809,0.873387213592005)
--(axis cs:15.2866242038217,0.878598180191327)
--(axis cs:14.6496815286624,0.88347093929546)
--(axis cs:14.0127388535032,0.888204997681326)
--(axis cs:13.3757961783439,0.894850132813732)
--(axis cs:12.7388535031847,0.896156879093735)
--(axis cs:12.1019108280255,0.898206963986429)
--(axis cs:11.4649681528662,0.901341181705108)
--(axis cs:10.828025477707,0.903618867178167)
--(axis cs:10.1910828025478,0.907421957010457)
--(axis cs:9.55414012738853,0.909199728420326)
--(axis cs:8.9171974522293,0.909668536836507)
--(axis cs:8.28025477707006,0.910470258866425)
--(axis cs:7.64331210191083,0.911356041811675)
--(axis cs:7.00636942675159,0.913188458514781)
--(axis cs:6.36942675159236,0.914026931190663)
--(axis cs:5.73248407643312,0.914387984145854)
--(axis cs:5.09554140127389,0.914589383292513)
--(axis cs:4.45859872611465,0.914820469052848)
--(axis cs:3.82165605095541,0.915004697541349)
--(axis cs:3.18471337579618,0.915213828968868)
--(axis cs:2.54777070063694,0.915732868248841)
--(axis cs:1.91082802547771,0.915947901014709)
--(axis cs:1.27388535031847,0.915885741101374)
--(axis cs:0.636942675159236,0.916091071493778)
--(axis cs:0,0.916049506892377)
--cycle;


==> img/mnist/mnist_rate_distortion_smoothgrad.tex <==
% smoothgrad
\addplot [line width=0.5, opacity=0.8, color7, mark=triangle, mark repeat=20, mark phase=10, mark size=1.5pt, mark options={draw=black, fill=color7, thin}]
table [row sep=\\]{%
0	0.915548319260124 \\
0.636942675159236	0.915171982130269 \\
1.27388535031847	0.915038617666578 \\
1.91082802547771	0.914700869612861 \\
2.54777070063694	0.914298562963959 \\
3.18471337579618	0.913855284634628 \\
3.82165605095541	0.912718879120657 \\
4.45859872611465	0.911349633976934 \\
5.09554140127389	0.909097694897209 \\
5.73248407643312	0.90859016098897 \\
6.36942675159236	0.906170846892637 \\
7.00636942675159	0.903564057935146 \\
7.64331210191083	0.902077189748525 \\
8.28025477707006	0.899125805594085 \\
8.9171974522293	0.895226777284988 \\
9.55414012738853	0.887664138909895 \\
10.1910828025478	0.880519168484607 \\
10.828025477707	0.87552590994339 \\
11.4649681528662	0.869787369828555 \\
12.1019108280255	0.862547248329502 \\
12.7388535031847	0.853292671858799 \\
13.3757961783439	0.849090406504692 \\
14.0127388535032	0.844862067342619 \\
14.6496815286624	0.836162992336322 \\
15.2866242038217	0.823834617678658 \\
15.9235668789809	0.81534067234039 \\
16.5605095541401	0.807871376618423 \\
17.1974522292994	0.799451330687152 \\
17.8343949044586	0.787160825538958 \\
18.4713375796178	0.779690156191791 \\
19.1082802547771	0.771200923174183 \\
19.7452229299363	0.765836350212539 \\
20.3821656050955	0.750102324257368 \\
21.0191082802548	0.735125034519047 \\
21.656050955414	0.71698605577948 \\
22.2929936305732	0.707465713879446 \\
22.9299363057325	0.701557020635446 \\
23.5668789808917	0.691701590258931 \\
24.203821656051	0.672647613002291 \\
24.8407643312102	0.669045361314147 \\
25.4777070063694	0.659056682099349 \\
26.1146496815287	0.641729672780921 \\
26.7515923566879	0.622820742374715 \\
27.3885350318471	0.600878171432873 \\
28.0254777070064	0.584892231732792 \\
28.6624203821656	0.55858234365523 \\
29.2993630573248	0.546688075433108 \\
29.9363057324841	0.528168575528323 \\
30.5732484076433	0.512802786937264 \\
31.2101910828025	0.501407549749689 \\
31.8471337579618	0.488254731939057 \\
32.484076433121	0.477132084544292 \\
33.1210191082803	0.464078271127951 \\
33.7579617834395	0.448309542187637 \\
34.3949044585987	0.433001433394828 \\
35.031847133758	0.422232441148073 \\
35.6687898089172	0.412905611556168 \\
36.3057324840764	0.405796217073886 \\
36.9426751592357	0.395862676544198 \\
37.5796178343949	0.382151176454124 \\
38.2165605095541	0.373622062082363 \\
38.8535031847134	0.366753755678283 \\
39.4904458598726	0.355851053848983 \\
40.1273885350318	0.349756826130668 \\
40.7643312101911	0.341489212745028 \\
41.4012738853503	0.326613617371395 \\
42.0382165605096	0.317903518000035 \\
42.6751592356688	0.308147125598432 \\
43.312101910828	0.30244940984307 \\
43.9490445859873	0.302449958133721 \\
44.5859872611465	0.292875370200985 \\
45.2229299363057	0.283480001668341 \\
45.859872611465	0.271096247157408 \\
46.4968152866242	0.263794278523674 \\
47.1337579617834	0.258868711767662 \\
47.7707006369427	0.256079296295146 \\
48.4076433121019	0.254924728294814 \\
49.0445859872611	0.247390020537095 \\
49.6815286624204	0.236952797568578 \\
50.3184713375796	0.231571096177195 \\
50.9554140127388	0.22662146964038 \\
51.5923566878981	0.221800119236386 \\
52.2292993630573	0.220676179748046 \\
52.8662420382166	0.209074525768559 \\
53.5031847133758	0.20446425775382 \\
54.140127388535	0.203309502303233 \\
54.7770700636943	0.192739504636472 \\
55.4140127388535	0.186463500333954 \\
56.0509554140127	0.180746152584015 \\
56.687898089172	0.173052631745766 \\
57.3248407643312	0.171802178094495 \\
57.9617834394904	0.1633261811268 \\
58.5987261146497	0.161481285319814 \\
59.2356687898089	0.157091005606333 \\
59.8726114649682	0.148291302013851 \\
60.5095541401274	0.143194661993106 \\
61.1464968152866	0.134788952621715 \\
61.7834394904459	0.121760886746796 \\
62.4203821656051	0.114476947346763 \\
63.0573248407643	0.106735088948157 \\
63.6942675159236	0.102414049240841 \\
64.3312101910828	0.0978141496785556 \\
64.968152866242	0.0932311381531104 \\
65.6050955414013	0.0878025750846855 \\
66.2420382165605	0.083016762393921 \\
66.8789808917197	0.0743302308509893 \\
67.515923566879	0.0642906906511343 \\
68.1528662420382	0.0604646205972699 \\
68.7898089171974	0.0578283535317375 \\
69.4267515923567	0.052241622749101 \\
70.0636942675159	0.0478253369889368 \\
70.7006369426752	0.043199329178766 \\
71.3375796178344	0.0412938849170779 \\
71.9745222929936	0.0388606651783205 \\
72.6114649681529	0.0365893143961392 \\
73.2484076433121	0.0336129334863974 \\
73.8853503184713	0.0324173533937438 \\
74.5222929936306	0.0287610979147503 \\
75.1592356687898	0.0317321561973456 \\
75.796178343949	0.0286106820669881 \\
76.4331210191083	0.0257506934451008 \\
77.0700636942675	0.0249696072705588 \\
77.7070063694268	0.0213451186273806 \\
78.343949044586	0.0205571043451851 \\
78.9808917197452	0.0187367023775371 \\
79.6178343949044	0.0184144352279469 \\
80.2547770700637	0.0184326776558432 \\
80.8917197452229	0.0170658452363367 \\
81.5286624203822	0.0169420460111906 \\
82.1656050955414	0.0157302293595799 \\
82.8025477707006	0.0144793081813506 \\
83.4394904458599	0.0129969323392936 \\
84.0764331210191	0.0114055335478904 \\
84.7133757961783	0.0105340527202031 \\
85.3503184713376	0.0110144795934019 \\
85.9872611464968	0.0102502504185508 \\
86.6242038216561	0.00983413775311703 \\
87.2611464968153	0.0095420103088521 \\
87.8980891719745	0.00959457315907328 \\
88.5350318471338	0.00835511795107301 \\
89.171974522293	0.00567125054934159 \\
89.8089171974522	0.00383167604715794 \\
90.4458598726115	0.00363860960405992 \\
91.0828025477707	0.00226380080881014 \\
91.7197452229299	0.00130711927068274 \\
92.3566878980892	0.000809743309033392 \\
92.9936305732484	0.000466057790288343 \\
93.6305732484076	0.000387540354186377 \\
94.2675159235669	0.000421898761728718 \\
94.9044585987261	0.000214228085741016 \\
95.5414012738853	0.000158440616742472 \\
96.1783439490446	0.000104630232337766 \\
96.8152866242038	9.7171442476256e-05 \\
97.4522292993631	1.89061607410806e-05 \\
98.0891719745223	1.29386225744038e-05 \\
98.7261146496815	7.61015668580944e-06 \\
99.3630573248408	5.48163179737104e-06 \\
100	9.07070329958515e-11 \\
};
\path [fill=color7, fill opacity=0.5] (axis cs:0,0.916091534306726)
--(axis cs:0,0.915005104213522)
--(axis cs:0.636942675159236,0.914414090756443)
--(axis cs:1.27388535031847,0.914333873753915)
--(axis cs:1.91082802547771,0.913902704334155)
--(axis cs:2.54777070063694,0.913427459421885)
--(axis cs:3.18471337579618,0.91303311824268)
--(axis cs:3.82165605095541,0.911630217308796)
--(axis cs:4.45859872611465,0.910038183521594)
--(axis cs:5.09554140127389,0.907444531009921)
--(axis cs:5.73248407643312,0.907039966996113)
--(axis cs:6.36942675159236,0.904226829981087)
--(axis cs:7.00636942675159,0.90124516241494)
--(axis cs:7.64331210191083,0.899622407215749)
--(axis cs:8.28025477707006,0.896440229543823)
--(axis cs:8.9171974522293,0.892119259188254)
--(axis cs:9.55414012738853,0.883880373766519)
--(axis cs:10.1910828025478,0.876258046092272)
--(axis cs:10.828025477707,0.871020035435149)
--(axis cs:11.4649681528662,0.864893498992026)
--(axis cs:12.1019108280255,0.85731146185188)
--(axis cs:12.7388535031847,0.847869880969096)
--(axis cs:13.3757961783439,0.843551812430515)
--(axis cs:14.0127388535032,0.839135917875801)
--(axis cs:14.6496815286624,0.830247980002262)
--(axis cs:15.2866242038217,0.817676521770035)
--(axis cs:15.9235668789809,0.808981257432119)
--(axis cs:16.5605095541401,0.801392689095046)
--(axis cs:17.1974522292994,0.792786874501677)
--(axis cs:17.8343949044586,0.780329959327916)
--(axis cs:18.4713375796178,0.772853937042671)
--(axis cs:19.1082802547771,0.764236433218288)
--(axis cs:19.7452229299363,0.758803913189166)
--(axis cs:20.3821656050955,0.743013746941756)
--(axis cs:21.0191082802548,0.728073993297925)
--(axis cs:21.656050955414,0.709597542183841)
--(axis cs:22.2929936305732,0.699944027800336)
--(axis cs:22.9299363057325,0.69412137645934)
--(axis cs:23.5668789808917,0.684071491693712)
--(axis cs:24.203821656051,0.664903566748913)
--(axis cs:24.8407643312102,0.661300392881805)
--(axis cs:25.4777070063694,0.651287700609569)
--(axis cs:26.1146496815287,0.63382233955062)
--(axis cs:26.7515923566879,0.614961170909632)
--(axis cs:27.3885350318471,0.592888379922575)
--(axis cs:28.0254777070064,0.577074480060881)
--(axis cs:28.6624203821656,0.550741451443259)
--(axis cs:29.2993630573248,0.538856703511126)
--(axis cs:29.9363057324841,0.520403730675486)
--(axis cs:30.5732484076433,0.505198437834888)
--(axis cs:31.2101910828025,0.493943547881126)
--(axis cs:31.8471337579618,0.480903569348127)
--(axis cs:32.484076433121,0.469782378576395)
--(axis cs:33.1210191082803,0.456856142677966)
--(axis cs:33.7579617834395,0.441174525874732)
--(axis cs:34.3949044585987,0.425977201955135)
--(axis cs:35.031847133758,0.415174655376535)
--(axis cs:35.6687898089172,0.405927133009009)
--(axis cs:36.3057324840764,0.398957704494765)
--(axis cs:36.9426751592357,0.388957071546243)
--(axis cs:37.5796178343949,0.375345003288452)
--(axis cs:38.2165605095541,0.367002614024783)
--(axis cs:38.8535031847134,0.360283632211999)
--(axis cs:39.4904458598726,0.349558932985947)
--(axis cs:40.1273885350318,0.343558804526588)
--(axis cs:40.7643312101911,0.335365137022887)
--(axis cs:41.4012738853503,0.320370100330097)
--(axis cs:42.0382165605096,0.311595969001228)
--(axis cs:42.6751592356688,0.301951539922686)
--(axis cs:43.312101910828,0.296525894976989)
--(axis cs:43.9490445859873,0.29654813678997)
--(axis cs:44.5859872611465,0.287203348344833)
--(axis cs:45.2229299363057,0.277775550851335)
--(axis cs:45.859872611465,0.26563191728701)
--(axis cs:46.4968152866242,0.258327539246967)
--(axis cs:47.1337579617834,0.253486396270756)
--(axis cs:47.7707006369427,0.25082772973555)
--(axis cs:48.4076433121019,0.24974120955849)
--(axis cs:49.0445859872611,0.242077398773777)
--(axis cs:49.6815286624204,0.231719210109115)
--(axis cs:50.3184713375796,0.22653405346936)
--(axis cs:50.9554140127388,0.221371564423923)
--(axis cs:51.5923566878981,0.216551999224063)
--(axis cs:52.2292993630573,0.215535549334334)
--(axis cs:52.8662420382166,0.203855238130339)
--(axis cs:53.5031847133758,0.199242220904615)
--(axis cs:54.140127388535,0.198270581245824)
--(axis cs:54.7770700636943,0.187523433001506)
--(axis cs:55.4140127388535,0.181147481327996)
--(axis cs:56.0509554140127,0.175664795453873)
--(axis cs:56.687898089172,0.167946718182159)
--(axis cs:57.3248407643312,0.166476554809116)
--(axis cs:57.9617834394904,0.158174992665921)
--(axis cs:58.5987261146497,0.15639453116261)
--(axis cs:59.2356687898089,0.151981884972665)
--(axis cs:59.8726114649682,0.143010952467949)
--(axis cs:60.5095541401274,0.138003150317902)
--(axis cs:61.1464968152866,0.129780861822316)
--(axis cs:61.7834394904459,0.116764974925881)
--(axis cs:62.4203821656051,0.109511208810388)
--(axis cs:63.0573248407643,0.102011075365715)
--(axis cs:63.6942675159236,0.0979943997943306)
--(axis cs:64.3312101910828,0.0936458562986396)
--(axis cs:64.968152866242,0.089002328553386)
--(axis cs:65.6050955414013,0.0835177764770641)
--(axis cs:66.2420382165605,0.0788582942423908)
--(axis cs:66.8789808917197,0.0702414860390352)
--(axis cs:67.515923566879,0.0604734597505451)
--(axis cs:68.1528662420382,0.0568083584029274)
--(axis cs:68.7898089171974,0.054296767476495)
--(axis cs:69.4267515923567,0.0489094422491725)
--(axis cs:70.0636942675159,0.0447499482338638)
--(axis cs:70.7006369426752,0.0403104038544412)
--(axis cs:71.3375796178344,0.0385445702461776)
--(axis cs:71.9745222929936,0.0362652949651145)
--(axis cs:72.6114649681529,0.0341804025237288)
--(axis cs:73.2484076433121,0.0312559495644112)
--(axis cs:73.8853503184713,0.0300519303859577)
--(axis cs:74.5222929936306,0.0266574646705576)
--(axis cs:75.1592356687898,0.0296718263724337)
--(axis cs:75.796178343949,0.0266782705073306)
--(axis cs:76.4331210191083,0.0238989925764492)
--(axis cs:77.0700636942675,0.0231617421662713)
--(axis cs:77.7070063694268,0.0198758812310026)
--(axis cs:78.343949044586,0.0190394737190456)
--(axis cs:78.9808917197452,0.0173656345574637)
--(axis cs:79.6178343949044,0.0173542529481085)
--(axis cs:80.2547770700637,0.0174929456441982)
--(axis cs:80.8917197452229,0.0162017662395278)
--(axis cs:81.5286624203822,0.0160068409306228)
--(axis cs:82.1656050955414,0.0148421393219428)
--(axis cs:82.8025477707006,0.0135176862951891)
--(axis cs:83.4394904458599,0.0119236138476768)
--(axis cs:84.0764331210191,0.0103331287751207)
--(axis cs:84.7133757961783,0.00937336684997738)
--(axis cs:85.3503184713376,0.00989748561044462)
--(axis cs:85.9872611464968,0.0091359230252608)
--(axis cs:86.6242038216561,0.00867140748555454)
--(axis cs:87.2611464968153,0.00839926308411913)
--(axis cs:87.8980891719745,0.00850986105943967)
--(axis cs:88.5350318471338,0.00731047627696169)
--(axis cs:89.171974522293,0.00473082604709788)
--(axis cs:89.8089171974522,0.0030405975676126)
--(axis cs:90.4458598726115,0.00290963821283143)
--(axis cs:91.0828025477707,0.00170219849982208)
--(axis cs:91.7197452229299,0.00099138682047675)
--(axis cs:92.3566878980892,0.000602011775720148)
--(axis cs:92.9936305732484,0.000326996461332621)
--(axis cs:93.6305732484076,0.000276081929886373)
--(axis cs:94.2675159235669,0.000318276098534966)
--(axis cs:94.9044585987261,0.000161604129204653)
--(axis cs:95.5414012738853,0.000115917471189582)
--(axis cs:96.1783439490446,8.05447051990523e-05)
--(axis cs:96.8152866242038,7.60481005435881e-05)
--(axis cs:97.4522292993631,1.49845488417404e-05)
--(axis cs:98.0891719745223,9.92888937487878e-06)
--(axis cs:98.7261146496815,6.07215631752239e-06)
--(axis cs:99.3630573248408,4.20711174931723e-06)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:100,9.07070329958515e-11)
--(axis cs:99.3630573248408,6.75615184542486e-06)
--(axis cs:98.7261146496815,9.1481570540965e-06)
--(axis cs:98.0891719745223,1.59483557739288e-05)
--(axis cs:97.4522292993631,2.28277726404209e-05)
--(axis cs:96.8152866242038,0.000118294784408924)
--(axis cs:96.1783439490446,0.000128715759476479)
--(axis cs:95.5414012738853,0.000200963762295362)
--(axis cs:94.9044585987261,0.000266852042277378)
--(axis cs:94.2675159235669,0.00052552142492247)
--(axis cs:93.6305732484076,0.000498998778486381)
--(axis cs:92.9936305732484,0.000605119119244066)
--(axis cs:92.3566878980892,0.00101747484234664)
--(axis cs:91.7197452229299,0.00162285172088872)
--(axis cs:91.0828025477707,0.00282540311779819)
--(axis cs:90.4458598726115,0.00436758099528842)
--(axis cs:89.8089171974522,0.00462275452670327)
--(axis cs:89.171974522293,0.00661167505158529)
--(axis cs:88.5350318471338,0.00939975962518433)
--(axis cs:87.8980891719745,0.0106792852587069)
--(axis cs:87.2611464968153,0.0106847575335851)
--(axis cs:86.6242038216561,0.0109968680206795)
--(axis cs:85.9872611464968,0.0113645778118408)
--(axis cs:85.3503184713376,0.0121314735763591)
--(axis cs:84.7133757961783,0.0116947385904289)
--(axis cs:84.0764331210191,0.0124779383206601)
--(axis cs:83.4394904458599,0.0140702508309104)
--(axis cs:82.8025477707006,0.015440930067512)
--(axis cs:82.1656050955414,0.016618319397217)
--(axis cs:81.5286624203822,0.0178772510917584)
--(axis cs:80.8917197452229,0.0179299242331455)
--(axis cs:80.2547770700637,0.0193724096674882)
--(axis cs:79.6178343949044,0.0194746175077853)
--(axis cs:78.9808917197452,0.0201077701976105)
--(axis cs:78.343949044586,0.0220747349713245)
--(axis cs:77.7070063694268,0.0228143560237586)
--(axis cs:77.0700636942675,0.0267774723748464)
--(axis cs:76.4331210191083,0.0276023943137525)
--(axis cs:75.796178343949,0.0305430936266457)
--(axis cs:75.1592356687898,0.0337924860222574)
--(axis cs:74.5222929936306,0.030864731158943)
--(axis cs:73.8853503184713,0.0347827764015299)
--(axis cs:73.2484076433121,0.0359699174083836)
--(axis cs:72.6114649681529,0.0389982262685495)
--(axis cs:71.9745222929936,0.0414560353915266)
--(axis cs:71.3375796178344,0.0440431995879782)
--(axis cs:70.7006369426752,0.0460882545030908)
--(axis cs:70.0636942675159,0.0509007257440099)
--(axis cs:69.4267515923567,0.0555738032490295)
--(axis cs:68.7898089171974,0.06135993958698)
--(axis cs:68.1528662420382,0.0641208827916125)
--(axis cs:67.515923566879,0.0681079215517234)
--(axis cs:66.8789808917197,0.0784189756629434)
--(axis cs:66.2420382165605,0.0871752305454512)
--(axis cs:65.6050955414013,0.0920873736923068)
--(axis cs:64.968152866242,0.0974599477528348)
--(axis cs:64.3312101910828,0.101982443058472)
--(axis cs:63.6942675159236,0.106833698687352)
--(axis cs:63.0573248407643,0.111459102530599)
--(axis cs:62.4203821656051,0.119442685883138)
--(axis cs:61.7834394904459,0.126756798567711)
--(axis cs:61.1464968152866,0.139797043421114)
--(axis cs:60.5095541401274,0.14838617366831)
--(axis cs:59.8726114649682,0.153571651559754)
--(axis cs:59.2356687898089,0.16220012624)
--(axis cs:58.5987261146497,0.166568039477019)
--(axis cs:57.9617834394904,0.168477369587679)
--(axis cs:57.3248407643312,0.177127801379874)
--(axis cs:56.687898089172,0.178158545309372)
--(axis cs:56.0509554140127,0.185827509714158)
--(axis cs:55.4140127388535,0.191779519339913)
--(axis cs:54.7770700636943,0.197955576271438)
--(axis cs:54.140127388535,0.208348423360641)
--(axis cs:53.5031847133758,0.209686294603026)
--(axis cs:52.8662420382166,0.214293813406778)
--(axis cs:52.2292993630573,0.225816810161759)
--(axis cs:51.5923566878981,0.227048239248709)
--(axis cs:50.9554140127388,0.231871374856838)
--(axis cs:50.3184713375796,0.23660813888503)
--(axis cs:49.6815286624204,0.24218638502804)
--(axis cs:49.0445859872611,0.252702642300413)
--(axis cs:48.4076433121019,0.260108247031138)
--(axis cs:47.7707006369427,0.261330862854741)
--(axis cs:47.1337579617834,0.264251027264567)
--(axis cs:46.4968152866242,0.269261017800381)
--(axis cs:45.859872611465,0.276560577027805)
--(axis cs:45.2229299363057,0.289184452485347)
--(axis cs:44.5859872611465,0.298547392057138)
--(axis cs:43.9490445859873,0.308351779477473)
--(axis cs:43.312101910828,0.308372924709151)
--(axis cs:42.6751592356688,0.314342711274177)
--(axis cs:42.0382165605096,0.324211066998842)
--(axis cs:41.4012738853503,0.332857134412694)
--(axis cs:40.7643312101911,0.347613288467168)
--(axis cs:40.1273885350318,0.355954847734749)
--(axis cs:39.4904458598726,0.362143174712018)
--(axis cs:38.8535031847134,0.373223879144567)
--(axis cs:38.2165605095541,0.380241510139944)
--(axis cs:37.5796178343949,0.388957349619796)
--(axis cs:36.9426751592357,0.402768281542152)
--(axis cs:36.3057324840764,0.412634729653006)
--(axis cs:35.6687898089172,0.419884090103328)
--(axis cs:35.031847133758,0.429290226919611)
--(axis cs:34.3949044585987,0.440025664834521)
--(axis cs:33.7579617834395,0.455444558500542)
--(axis cs:33.1210191082803,0.471300399577936)
--(axis cs:32.484076433121,0.484481790512188)
--(axis cs:31.8471337579618,0.495605894529987)
--(axis cs:31.2101910828025,0.508871551618252)
--(axis cs:30.5732484076433,0.520407136039639)
--(axis cs:29.9363057324841,0.53593342038116)
--(axis cs:29.2993630573248,0.554519447355089)
--(axis cs:28.6624203821656,0.566423235867201)
--(axis cs:28.0254777070064,0.592709983404704)
--(axis cs:27.3885350318471,0.608867962943172)
--(axis cs:26.7515923566879,0.630680313839799)
--(axis cs:26.1146496815287,0.649637006011222)
--(axis cs:25.4777070063694,0.666825663589129)
--(axis cs:24.8407643312102,0.676790329746489)
--(axis cs:24.203821656051,0.680391659255669)
--(axis cs:23.5668789808917,0.69933168882415)
--(axis cs:22.9299363057325,0.708992664811552)
--(axis cs:22.2929936305732,0.714987399958557)
--(axis cs:21.656050955414,0.724374569375119)
--(axis cs:21.0191082802548,0.742176075740169)
--(axis cs:20.3821656050955,0.757190901572981)
--(axis cs:19.7452229299363,0.772868787235912)
--(axis cs:19.1082802547771,0.778165413130078)
--(axis cs:18.4713375796178,0.786526375340912)
--(axis cs:17.8343949044586,0.793991691750001)
--(axis cs:17.1974522292994,0.806115786872628)
--(axis cs:16.5605095541401,0.8143500641418)
--(axis cs:15.9235668789809,0.82170008724866)
--(axis cs:15.2866242038217,0.829992713587281)
--(axis cs:14.6496815286624,0.842078004670381)
--(axis cs:14.0127388535032,0.850588216809437)
--(axis cs:13.3757961783439,0.85462900057887)
--(axis cs:12.7388535031847,0.858715462748502)
--(axis cs:12.1019108280255,0.867783034807123)
--(axis cs:11.4649681528662,0.874681240665083)
--(axis cs:10.828025477707,0.88003178445163)
--(axis cs:10.1910828025478,0.884780290876941)
--(axis cs:9.55414012738853,0.891447904053271)
--(axis cs:8.9171974522293,0.898334295381722)
--(axis cs:8.28025477707006,0.901811381644347)
--(axis cs:7.64331210191083,0.904531972281301)
--(axis cs:7.00636942675159,0.905882953455352)
--(axis cs:6.36942675159236,0.908114863804188)
--(axis cs:5.73248407643312,0.910140354981826)
--(axis cs:5.09554140127389,0.910750858784497)
--(axis cs:4.45859872611465,0.912661084432273)
--(axis cs:3.82165605095541,0.913807540932518)
--(axis cs:3.18471337579618,0.914677451026577)
--(axis cs:2.54777070063694,0.915169666506032)
--(axis cs:1.91082802547771,0.915499034891568)
--(axis cs:1.27388535031847,0.915743361579241)
--(axis cs:0.636942675159236,0.915929873504095)
--(axis cs:0,0.916091534306726)
--cycle;


==> img/stl10/stl10_examples.tex <==
\begin{tabular}{c@{\;\;\;\;}c@{\;\;\;\;}c}
    image & L-RDE & sensitivity  \\
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_input.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_l_rde.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_sensitivity.png}
\end{tabular}
\\[2ex]
\begin{tabular}{@{}l@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{}}
    \toprule
    & $k=2000$ & $k=4000$ & $k=6000$ & $k=8000$ & multi-rate \\
    \midrule
    FW &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_fw_rc_rde_2000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_fw_rc_rde_4000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_fw_rc_rde_6000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_fw_rc_rde_8000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_fw_rc_rde_multi_cmap.png} \\

    AFW &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_afw_rc_rde_2000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_afw_rc_rde_4000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_afw_rc_rde_6000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_afw_rc_rde_8000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_afw_rc_rde_multi_cmap.png} \\

    LCG &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lcg_rc_rde_2000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lcg_rc_rde_4000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lcg_rc_rde_6000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lcg_rc_rde_8000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lcg_rc_rde_multi_cmap.png} \\

    LAFW &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lafw_rc_rde_2000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lafw_rc_rde_4000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lafw_rc_rde_6000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lafw_rc_rde_8000.png} &
    \includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_lafw_rc_rde_multi_cmap.png} \\

    %SFW &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_sfw_rc_rde_2000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_sfw_rc_rde_4000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_sfw_rc_rde_6000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_sfw_rc_rde_8000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_sfw_rc_rde_multi_cmap.png} \\

    %PGD &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_pgd_rc_rde_2000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_pgd_rc_rde_4000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_pgd_rc_rde_6000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_pgd_rc_rde_8000.png} &
    %\includegraphics[width=1.25cm, valign=c]{./img/stl10/5253/stl10_testing_5253_pgd_rc_rde_multi_cmap.png} \\
    \bottomrule
\end{tabular}




==> img/stl10/stl10_rate_accuracy_afw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.076875
0.340136054421769 0.0859375
0.680272108843537 0.14671875
1.02040816326531 0.21203125
1.36054421768707 0.24859375
1.70068027210884 0.32578125
2.04081632653061 0.370625
2.38095238095238 0.41
2.72108843537415 0.44171875
3.06122448979592 0.4834375
3.40136054421769 0.540625
3.74149659863946 0.594375
4.08163265306122 0.64125
4.42176870748299 0.67328125
4.76190476190476 0.6978125
5.10204081632653 0.725625
5.4421768707483 0.7440625
5.78231292517007 0.7571875
6.12244897959184 0.77078125
6.46258503401361 0.781875
6.80272108843537 0.79421875
7.14285714285714 0.8015625
7.48299319727891 0.811875
7.82312925170068 0.8128125
8.16326530612245 0.8234375
8.50340136054422 0.8290625
8.84353741496599 0.835
9.18367346938775 0.83953125
9.52380952380952 0.84609375
9.86394557823129 0.84859375
10.2040816326531 0.85328125
10.5442176870748 0.86421875
10.8843537414966 0.86671875
11.2244897959184 0.87515625
11.5646258503401 0.87125
11.9047619047619 0.875
12.2448979591837 0.881875
12.5850340136054 0.88453125
12.9251700680272 0.88546875
13.265306122449 0.8875
13.6054421768707 0.8865625
13.9455782312925 0.890625
14.2857142857143 0.8915625
14.6258503401361 0.8940625
14.9659863945578 0.89265625
15.3061224489796 0.89328125
15.6462585034014 0.89546875
15.9863945578231 0.8959375
16.3265306122449 0.8975
16.6666666666667 0.8965625
17.0068027210884 0.89546875
17.3469387755102 0.89828125
17.687074829932 0.8978125
18.0272108843537 0.89890625
18.3673469387755 0.8975
18.7074829931973 0.8975
19.047619047619 0.89703125
19.3877551020408 0.8953125
19.7278911564626 0.89609375
20.0680272108844 0.894375
20.4081632653061 0.89515625
20.7482993197279 0.89625
21.0884353741497 0.89765625
21.4285714285714 0.89546875
21.7687074829932 0.90015625
22.108843537415 0.90109375
22.4489795918367 0.89984375
22.7891156462585 0.89765625
23.1292517006803 0.90015625
23.469387755102 0.899375
23.8095238095238 0.898125
24.1496598639456 0.89890625
24.4897959183673 0.8978125
24.8299319727891 0.89984375
25.1700680272109 0.89765625
25.5102040816327 0.89640625
25.8503401360544 0.89125
26.1904761904762 0.88953125
26.530612244898 0.88546875
26.8707482993197 0.88171875
27.2108843537415 0.88203125
27.5510204081633 0.8834375
27.891156462585 0.8834375
28.2312925170068 0.88265625
28.5714285714286 0.8809375
28.9115646258503 0.87921875
29.2517006802721 0.87828125
29.5918367346939 0.876875
29.9319727891156 0.87171875
30.2721088435374 0.87109375
30.6122448979592 0.87359375
30.952380952381 0.87125
31.2925170068027 0.87390625
31.6326530612245 0.873125
31.9727891156463 0.8725
32.312925170068 0.87359375
32.6530612244898 0.875625
32.9931972789116 0.8809375
33.3333333333333 0.880625
33.6734693877551 0.881875
34.0136054421769 0.880625
34.3537414965986 0.88140625
34.6938775510204 0.876875
35.0340136054422 0.879375
35.3741496598639 0.8784375
35.7142857142857 0.87875
36.0544217687075 0.8778125
36.3945578231292 0.88
36.734693877551 0.87734375
37.0748299319728 0.87765625
37.4149659863946 0.8778125
37.7551020408163 0.874375
38.0952380952381 0.87421875
38.4353741496599 0.87484375
38.7755102040816 0.87265625
39.1156462585034 0.87203125
39.4557823129252 0.87015625
39.7959183673469 0.86828125
40.1360544217687 0.86953125
40.4761904761905 0.8703125
40.8163265306122 0.86875
41.156462585034 0.8709375
41.4965986394558 0.86875
41.8367346938776 0.8728125
42.1768707482993 0.86703125
42.5170068027211 0.8703125
42.8571428571429 0.86390625
43.1972789115646 0.868125
43.5374149659864 0.86515625
43.8775510204082 0.861875
44.2176870748299 0.85921875
44.5578231292517 0.8603125
44.8979591836735 0.85546875
45.2380952380952 0.8575
45.578231292517 0.858125
45.9183673469388 0.8553125
46.2585034013605 0.84921875
46.5986394557823 0.84515625
46.9387755102041 0.84390625
47.2789115646259 0.84125
47.6190476190476 0.84265625
47.9591836734694 0.84203125
48.2993197278912 0.83875
48.6394557823129 0.84140625
48.9795918367347 0.83953125
49.3197278911565 0.844375
49.6598639455782 0.84578125
50 0.84578125
50.3401360544218 0.84796875
50.6802721088435 0.851875
51.0204081632653 0.85203125
51.3605442176871 0.85703125
51.7006802721088 0.86078125
52.0408163265306 0.8659375
52.3809523809524 0.86828125
52.7210884353741 0.87015625
53.0612244897959 0.864375
53.4013605442177 0.865625
53.7414965986395 0.865625
54.0816326530612 0.8659375
54.421768707483 0.87078125
54.7619047619048 0.87234375
55.1020408163265 0.87359375
55.4421768707483 0.87546875
55.7823129251701 0.87375
56.1224489795918 0.86984375
56.4625850340136 0.87171875
56.8027210884354 0.87453125
57.1428571428571 0.8775
57.4829931972789 0.88125
57.8231292517007 0.88046875
58.1632653061224 0.87890625
58.5034013605442 0.87703125
58.843537414966 0.88078125
59.1836734693878 0.8784375
59.5238095238095 0.88390625
59.8639455782313 0.8853125
60.2040816326531 0.883125
60.5442176870748 0.8834375
60.8843537414966 0.8834375
61.2244897959184 0.8775
61.5646258503401 0.8796875
61.9047619047619 0.87609375
62.2448979591837 0.87734375
62.5850340136054 0.87890625
62.9251700680272 0.87984375
63.265306122449 0.88
63.6054421768707 0.8771875
63.9455782312925 0.87671875
64.2857142857143 0.87828125
64.6258503401361 0.87796875
64.9659863945578 0.8740625
65.3061224489796 0.8778125
65.6462585034014 0.87546875
65.9863945578231 0.874375
66.3265306122449 0.87359375
66.6666666666667 0.87078125
67.0068027210884 0.86921875
67.3469387755102 0.86765625
67.687074829932 0.86671875
68.0272108843537 0.86640625
68.3673469387755 0.86515625
68.7074829931973 0.860625
69.0476190476191 0.86109375
69.3877551020408 0.86703125
69.7278911564626 0.86359375
70.0680272108844 0.86671875
70.4081632653061 0.86515625
70.7482993197279 0.86
71.0884353741497 0.86171875
71.4285714285714 0.860625
71.7687074829932 0.86109375
72.108843537415 0.8628125
72.4489795918367 0.86203125
72.7891156462585 0.864375
73.1292517006803 0.86375
73.469387755102 0.86
73.8095238095238 0.85703125
74.1496598639456 0.85640625
74.4897959183673 0.85765625
74.8299319727891 0.8590625
75.1700680272109 0.8584375
75.5102040816327 0.8590625
75.8503401360544 0.86125
76.1904761904762 0.86484375
76.530612244898 0.87453125
76.8707482993197 0.8809375
77.2108843537415 0.88390625
77.5510204081633 0.8921875
77.891156462585 0.89203125
78.2312925170068 0.89875
78.5714285714286 0.90046875
78.9115646258503 0.9059375
79.2517006802721 0.90953125
79.5918367346939 0.915
79.9319727891156 0.916875
80.2721088435374 0.9190625
80.6122448979592 0.918125
80.9523809523809 0.92578125
81.2925170068027 0.9259375
81.6326530612245 0.928125
81.9727891156463 0.93109375
82.312925170068 0.92984375
82.6530612244898 0.9315625
82.9931972789116 0.9365625
83.3333333333333 0.936875
83.6734693877551 0.93890625
84.0136054421769 0.94
84.3537414965986 0.93765625
84.6938775510204 0.940625
85.0340136054422 0.9421875
85.3741496598639 0.94328125
85.7142857142857 0.94390625
86.0544217687075 0.9446875
86.3945578231292 0.9459375
86.734693877551 0.94828125
87.0748299319728 0.9478125
87.4149659863945 0.9465625
87.7551020408163 0.94796875
88.0952380952381 0.95140625
88.4353741496599 0.95
88.7755102040816 0.95109375
89.1156462585034 0.95
89.4557823129252 0.9521875
89.7959183673469 0.95359375
90.1360544217687 0.9528125
90.4761904761905 0.95203125
90.8163265306122 0.954375
91.156462585034 0.95171875
91.4965986394558 0.95171875
91.8367346938775 0.9490625
92.1768707482993 0.95125
92.5170068027211 0.95125
92.8571428571429 0.95453125
93.1972789115646 0.9540625
93.5374149659864 0.9546875
93.8775510204082 0.9559375
94.2176870748299 0.9553125
94.5578231292517 0.9575
94.8979591836735 0.95984375
95.2380952380952 0.9571875
95.578231292517 0.96015625
95.9183673469388 0.96078125
96.2585034013605 0.9596875
96.5986394557823 0.95890625
96.9387755102041 0.96015625
97.2789115646258 0.9603125
97.6190476190476 0.96015625
97.9591836734694 0.96
98.2993197278912 0.96015625
98.6394557823129 0.96125
98.9795918367347 0.9615625
99.3197278911565 0.95890625
99.6598639455782 0.959375
100 0.98
};
\path [fill=color3, fill opacity=0.25]
(axis cs:0,0.083621060952801)
--(axis cs:0,0.070128939047199)
--(axis cs:0.340136054421769,0.0776418903978143)
--(axis cs:0.680272108843537,0.131557479588738)
--(axis cs:1.02040816326531,0.198598988689227)
--(axis cs:1.36054421768707,0.234822833624632)
--(axis cs:1.70068027210884,0.310676066114982)
--(axis cs:2.04081632653061,0.357513580081647)
--(axis cs:2.38095238095238,0.394917878201353)
--(axis cs:2.72108843537415,0.425298264639404)
--(axis cs:3.06122448979592,0.465528291583832)
--(axis cs:3.40136054421769,0.519796957051925)
--(axis cs:3.74149659863946,0.572832996324314)
--(axis cs:4.08163265306122,0.62057729977318)
--(axis cs:4.42176870748299,0.653594127840307)
--(axis cs:4.76190476190476,0.679519735196925)
--(axis cs:5.10204081632653,0.709329568840925)
--(axis cs:5.4421768707483,0.727969058141603)
--(axis cs:5.78231292517007,0.742232377109044)
--(axis cs:6.12244897959184,0.756063639885401)
--(axis cs:6.46258503401361,0.768822629338591)
--(axis cs:6.80272108843537,0.780913466712731)
--(axis cs:7.14285714285714,0.788532799243396)
--(axis cs:7.48299319727891,0.7993879767065)
--(axis cs:7.82312925170068,0.801584154412653)
--(axis cs:8.16326530612245,0.812437400124743)
--(axis cs:8.50340136054422,0.817712507636119)
--(axis cs:8.84353741496599,0.82360807299108)
--(axis cs:9.18367346938775,0.827869196395995)
--(axis cs:9.52380952380952,0.834127372160052)
--(axis cs:9.86394557823129,0.836052238727235)
--(axis cs:10.2040816326531,0.840357007023386)
--(axis cs:10.5442176870748,0.851085890443831)
--(axis cs:10.8843537414966,0.853862572660823)
--(axis cs:11.2244897959184,0.862331266204666)
--(axis cs:11.5646258503401,0.858400129528179)
--(axis cs:11.9047619047619,0.862044434412674)
--(axis cs:12.2448979591837,0.869002142927122)
--(axis cs:12.5850340136054,0.871565750713319)
--(axis cs:12.9251700680272,0.872514288627252)
--(axis cs:13.265306122449,0.874252541839844)
--(axis cs:13.6054421768707,0.87323394225131)
--(axis cs:13.9455782312925,0.87793795341212)
--(axis cs:14.2857142857143,0.879787731547111)
--(axis cs:14.6258503401361,0.882612122494453)
--(axis cs:14.9659863945578,0.882628041951448)
--(axis cs:15.3061224489796,0.883780446136755)
--(axis cs:15.6462585034014,0.885839328740953)
--(axis cs:15.9863945578231,0.88591737864189)
--(axis cs:16.3265306122449,0.887771555152022)
--(axis cs:16.6666666666667,0.886189769579472)
--(axis cs:17.0068027210884,0.885803740983347)
--(axis cs:17.3469387755102,0.888381294974998)
--(axis cs:17.687074829932,0.88759539714871)
--(axis cs:18.0272108843537,0.888100772381791)
--(axis cs:18.3673469387755,0.887828579372547)
--(axis cs:18.7074829931973,0.887640103458228)
--(axis cs:19.047619047619,0.88608111430213)
--(axis cs:19.3877551020408,0.884926905881918)
--(axis cs:19.7278911564626,0.885552754098071)
--(axis cs:20.0680272108844,0.884162565263749)
--(axis cs:20.4081632653061,0.885040929075421)
--(axis cs:20.7482993197279,0.886007726092088)
--(axis cs:21.0884353741497,0.887250931881768)
--(axis cs:21.4285714285714,0.884797374731457)
--(axis cs:21.7687074829932,0.89061537931117)
--(axis cs:22.108843537415,0.890717802159966)
--(axis cs:22.4489795918367,0.889627113864233)
--(axis cs:22.7891156462585,0.887334672703591)
--(axis cs:23.1292517006803,0.890195791218611)
--(axis cs:23.469387755102,0.889012387972748)
--(axis cs:23.8095238095238,0.88672637776452)
--(axis cs:24.1496598639456,0.887608050707592)
--(axis cs:24.4897959183673,0.886062054581664)
--(axis cs:24.8299319727891,0.887977410513141)
--(axis cs:25.1700680272109,0.886182160084896)
--(axis cs:25.5102040816327,0.884687906908106)
--(axis cs:25.8503401360544,0.878620966280994)
--(axis cs:26.1904761904762,0.87692073088853)
--(axis cs:26.530612244898,0.872472394427044)
--(axis cs:26.8707482993197,0.869176478336094)
--(axis cs:27.2108843537415,0.870041782550947)
--(axis cs:27.5510204081633,0.872033022665572)
--(axis cs:27.891156462585,0.872417477883363)
--(axis cs:28.2312925170068,0.871065559729263)
--(axis cs:28.5714285714286,0.869856204724606)
--(axis cs:28.9115646258503,0.867906210209195)
--(axis cs:29.2517006802721,0.866984739021901)
--(axis cs:29.5918367346939,0.866270412530861)
--(axis cs:29.9319727891156,0.860678409680069)
--(axis cs:30.2721088435374,0.860975601065229)
--(axis cs:30.6122448979592,0.863987134383737)
--(axis cs:30.952380952381,0.861447335866149)
--(axis cs:31.2925170068027,0.864754134659274)
--(axis cs:31.6326530612245,0.863568648575996)
--(axis cs:31.9727891156463,0.86368493429969)
--(axis cs:32.312925170068,0.864969536416344)
--(axis cs:32.6530612244898,0.866418340820787)
--(axis cs:32.9931972789116,0.872105141363598)
--(axis cs:33.3333333333333,0.871401782067877)
--(axis cs:33.6734693877551,0.872817678944784)
--(axis cs:34.0136054421769,0.871464031719095)
--(axis cs:34.3537414965986,0.87261339057709)
--(axis cs:34.6938775510204,0.868766590330216)
--(axis cs:35.0340136054422,0.871064458862737)
--(axis cs:35.3741496598639,0.869656036270951)
--(axis cs:35.7142857142857,0.869352647090844)
--(axis cs:36.0544217687075,0.868108593466961)
--(axis cs:36.3945578231292,0.870901707266522)
--(axis cs:36.734693877551,0.867897305918435)
--(axis cs:37.0748299319728,0.86816749917537)
--(axis cs:37.4149659863946,0.86836656071145)
--(axis cs:37.7551020408163,0.865255767554743)
--(axis cs:38.0952380952381,0.864380640101647)
--(axis cs:38.4353741496599,0.865621049078888)
--(axis cs:38.7755102040816,0.862370770335981)
--(axis cs:39.1156462585034,0.861417224043886)
--(axis cs:39.4557823129252,0.85981067758808)
--(axis cs:39.7959183673469,0.858505376471406)
--(axis cs:40.1360544217687,0.859365145255854)
--(axis cs:40.4761904761905,0.860073019820533)
--(axis cs:40.8163265306122,0.858523567311271)
--(axis cs:41.156462585034,0.86048326274135)
--(axis cs:41.4965986394558,0.857910596151944)
--(axis cs:41.8367346938776,0.861806333016444)
--(axis cs:42.1768707482993,0.85630905624859)
--(axis cs:42.5170068027211,0.859614793798727)
--(axis cs:42.8571428571429,0.852893586252415)
--(axis cs:43.1972789115646,0.856586675400202)
--(axis cs:43.5374149659864,0.852960943130406)
--(axis cs:43.8775510204082,0.849470734031835)
--(axis cs:44.2176870748299,0.847021879228519)
--(axis cs:44.5578231292517,0.847572943682529)
--(axis cs:44.8979591836735,0.842927999164482)
--(axis cs:45.2380952380952,0.844085144670707)
--(axis cs:45.578231292517,0.844462894115217)
--(axis cs:45.9183673469388,0.841391773686558)
--(axis cs:46.2585034013605,0.835053206843628)
--(axis cs:46.5986394557823,0.831316254102234)
--(axis cs:46.9387755102041,0.829562079275812)
--(axis cs:47.2789115646259,0.828179375797575)
--(axis cs:47.6190476190476,0.828897111634906)
--(axis cs:47.9591836734694,0.828866477555309)
--(axis cs:48.2993197278912,0.825815799267679)
--(axis cs:48.6394557823129,0.829097300465313)
--(axis cs:48.9795918367347,0.827419906284027)
--(axis cs:49.3197278911565,0.832344637816848)
--(axis cs:49.6598639455782,0.833317542309292)
--(axis cs:50,0.834010937007376)
--(axis cs:50.3401360544218,0.836191147131789)
--(axis cs:50.6802721088435,0.839651183415376)
--(axis cs:51.0204081632653,0.840726299971734)
--(axis cs:51.3605442176871,0.845406053770347)
--(axis cs:51.7006802721088,0.849243338671378)
--(axis cs:52.0408163265306,0.853591030758376)
--(axis cs:52.3809523809524,0.857351163924574)
--(axis cs:52.7210884353741,0.85872045711062)
--(axis cs:53.0612244897959,0.852044762389902)
--(axis cs:53.4013605442177,0.854187122455429)
--(axis cs:53.7414965986395,0.854736437605651)
--(axis cs:54.0816326530612,0.854704908488664)
--(axis cs:54.421768707483,0.859579690742041)
--(axis cs:54.7619047619048,0.860927153798713)
--(axis cs:55.1020408163265,0.862028594450852)
--(axis cs:55.4421768707483,0.863986351546577)
--(axis cs:55.7823129251701,0.862236497927196)
--(axis cs:56.1224489795918,0.858361351546577)
--(axis cs:56.4625850340136,0.860050156162124)
--(axis cs:56.8027210884354,0.863062148096977)
--(axis cs:57.1428571428571,0.866226728983818)
--(axis cs:57.4829931972789,0.869845522665572)
--(axis cs:57.8231292517007,0.869009630634797)
--(axis cs:58.1632653061224,0.866781527492906)
--(axis cs:58.5034013605442,0.863943490681854)
--(axis cs:58.843537414966,0.868342818251962)
--(axis cs:59.1836734693878,0.865535043308661)
--(axis cs:59.5238095238095,0.871844615908063)
--(axis cs:59.8639455782313,0.873631244879449)
--(axis cs:60.2040816326531,0.870802499253066)
--(axis cs:60.5442176870748,0.871110356552462)
--(axis cs:60.8843537414966,0.871136688358445)
--(axis cs:61.2244897959184,0.865247350862419)
--(axis cs:61.5646258503401,0.867404533059742)
--(axis cs:61.9047619047619,0.86363080749379)
--(axis cs:62.2448979591837,0.865203306614333)
--(axis cs:62.5850340136054,0.866937481514171)
--(axis cs:62.9251700680272,0.86832238167412)
--(axis cs:63.265306122449,0.868876614462739)
--(axis cs:63.6054421768707,0.867074536354688)
--(axis cs:63.9455782312925,0.866009906152607)
--(axis cs:64.2857142857143,0.86855035472382)
--(axis cs:64.6258503401361,0.868700662512351)
--(axis cs:64.9659863945578,0.864062385559737)
--(axis cs:65.3061224489796,0.868157857195341)
--(axis cs:65.6462585034014,0.866127890124806)
--(axis cs:65.9863945578231,0.86503158804698)
--(axis cs:66.3265306122449,0.864751139683914)
--(axis cs:66.6666666666667,0.862309886927296)
--(axis cs:67.0068027210884,0.860227478020922)
--(axis cs:67.3469387755102,0.859295939560225)
--(axis cs:67.687074829932,0.857932400592363)
--(axis cs:68.0272108843537,0.857778719623611)
--(axis cs:68.3673469387755,0.855446939716733)
--(axis cs:68.7074829931973,0.85071878542741)
--(axis cs:69.0476190476191,0.851317876471406)
--(axis cs:69.3877551020408,0.858470299631272)
--(axis cs:69.7278911564626,0.854636483662592)
--(axis cs:70.0680272108844,0.858932539349501)
--(axis cs:70.4081632653061,0.85716691823839)
--(axis cs:70.7482993197279,0.851789902516803)
--(axis cs:71.0884353741497,0.854102188527328)
--(axis cs:71.4285714285714,0.854129574551439)
--(axis cs:71.7687074829932,0.854157405915203)
--(axis cs:72.108843537415,0.854722930691823)
--(axis cs:72.4489795918367,0.853662958355124)
--(axis cs:72.7891156462585,0.855736974848634)
--(axis cs:73.1292517006803,0.854790072324227)
--(axis cs:73.469387755102,0.850020888209909)
--(axis cs:73.8095238095238,0.847928241631744)
--(axis cs:74.1496598639456,0.847357883293048)
--(axis cs:74.4897959183673,0.847772684842149)
--(axis cs:74.8299319727891,0.849945359361731)
--(axis cs:75.1700680272109,0.849162726507356)
--(axis cs:75.5102040816327,0.849524128556973)
--(axis cs:75.8503401360544,0.851596345034174)
--(axis cs:76.1904761904762,0.854149164418193)
--(axis cs:76.530612244898,0.86320607190809)
--(axis cs:76.8707482993197,0.870367141306457)
--(axis cs:77.2108843537415,0.873306609854419)
--(axis cs:77.5510204081633,0.881830411262842)
--(axis cs:77.891156462585,0.881381344533274)
--(axis cs:78.2312925170068,0.887759440918861)
--(axis cs:78.5714285714286,0.889726118617126)
--(axis cs:78.9115646258503,0.895851921058368)
--(axis cs:79.2517006802721,0.898735485172624)
--(axis cs:79.5918367346939,0.904090437465806)
--(axis cs:79.9319727891156,0.905813516609653)
--(axis cs:80.2721088435374,0.90802259159292)
--(axis cs:80.6122448979592,0.9066388646651)
--(axis cs:80.9523809523809,0.91533476963452)
--(axis cs:81.2925170068027,0.91514924650028)
--(axis cs:81.6326530612245,0.917879002305778)
--(axis cs:81.9727891156463,0.920421481093699)
--(axis cs:82.312925170068,0.919602872861044)
--(axis cs:82.6530612244898,0.9210863919282)
--(axis cs:82.9931972789116,0.926392174717226)
--(axis cs:83.3333333333333,0.926736606743558)
--(axis cs:83.6734693877551,0.929130376471406)
--(axis cs:84.0136054421769,0.930181782244096)
--(axis cs:84.3537414965986,0.927452690566054)
--(axis cs:84.6938775510204,0.930893614712224)
--(axis cs:85.0340136054422,0.932470825809506)
--(axis cs:85.3741496598639,0.933955717258484)
--(axis cs:85.7142857142857,0.934845244432216)
--(axis cs:86.0544217687075,0.936562640851581)
--(axis cs:86.3945578231292,0.937933261087013)
--(axis cs:86.734693877551,0.940919367672676)
--(axis cs:87.0748299319728,0.940412501402159)
--(axis cs:87.4149659863945,0.939427576383747)
--(axis cs:87.7551020408163,0.940765318903941)
--(axis cs:88.0952380952381,0.944979459615714)
--(axis cs:88.4353741496599,0.943006830550794)
--(axis cs:88.7755102040816,0.944386677799339)
--(axis cs:89.1156462585034,0.943159878512563)
--(axis cs:89.4557823129252,0.945872228041318)
--(axis cs:89.7959183673469,0.947635118042931)
--(axis cs:90.1360544217687,0.946613058496834)
--(axis cs:90.4761904761905,0.945760684470047)
--(axis cs:90.8163265306122,0.948155592449965)
--(axis cs:91.156462585034,0.944859832153261)
--(axis cs:91.4965986394558,0.944928304271018)
--(axis cs:91.8367346938775,0.941824070132732)
--(axis cs:92.1768707482993,0.943930339960374)
--(axis cs:92.5170068027211,0.943504929664493)
--(axis cs:92.8571428571429,0.947302708252462)
--(axis cs:93.1972789115646,0.946652198579769)
--(axis cs:93.5374149659864,0.947223342072648)
--(axis cs:93.8775510204082,0.947483604254754)
--(axis cs:94.2176870748299,0.946057283789689)
--(axis cs:94.5578231292517,0.947620777887859)
--(axis cs:94.8979591836735,0.950692676744713)
--(axis cs:95.2380952380952,0.94800469634008)
--(axis cs:95.578231292517,0.951664647379559)
--(axis cs:95.9183673469388,0.953521113674298)
--(axis cs:96.2585034013605,0.95492531822647)
--(axis cs:96.5986394557823,0.953780459581246)
--(axis cs:96.9387755102041,0.955982087837273)
--(axis cs:97.2789115646258,0.957627397053737)
--(axis cs:97.6190476190476,0.959055719954142)
--(axis cs:97.9591836734694,0.958443615483349)
--(axis cs:98.2993197278912,0.95771094062001)
--(axis cs:98.6394557823129,0.958224231760776)
--(axis cs:98.9795918367347,0.957890313344343)
--(axis cs:99.3197278911565,0.954531293596757)
--(axis cs:99.6598639455782,0.954042217600986)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:99.6598639455782,0.964707782399014)
--(axis cs:99.3197278911565,0.963281206403243)
--(axis cs:98.9795918367347,0.965234686655657)
--(axis cs:98.6394557823129,0.964275768239225)
--(axis cs:98.2993197278912,0.96260155937999)
--(axis cs:97.9591836734694,0.961556384516651)
--(axis cs:97.6190476190476,0.961256780045858)
--(axis cs:97.2789115646258,0.962997602946263)
--(axis cs:96.9387755102041,0.964330412162727)
--(axis cs:96.5986394557823,0.964032040418754)
--(axis cs:96.2585034013605,0.96444968177353)
--(axis cs:95.9183673469388,0.968041386325702)
--(axis cs:95.578231292517,0.968647852620441)
--(axis cs:95.2380952380952,0.96637030365992)
--(axis cs:94.8979591836735,0.968994823255287)
--(axis cs:94.5578231292517,0.967379222112141)
--(axis cs:94.2176870748299,0.964567716210311)
--(axis cs:93.8775510204082,0.964391395745246)
--(axis cs:93.5374149659864,0.962151657927352)
--(axis cs:93.1972789115646,0.961472801420231)
--(axis cs:92.8571428571429,0.961759791747538)
--(axis cs:92.5170068027211,0.958995070335507)
--(axis cs:92.1768707482993,0.958569660039626)
--(axis cs:91.8367346938775,0.956300929867268)
--(axis cs:91.4965986394558,0.958509195728981)
--(axis cs:91.156462585034,0.958577667846739)
--(axis cs:90.8163265306122,0.960594407550035)
--(axis cs:90.4761904761905,0.958301815529953)
--(axis cs:90.1360544217687,0.959011941503165)
--(axis cs:89.7959183673469,0.959552381957069)
--(axis cs:89.4557823129252,0.958502771958681)
--(axis cs:89.1156462585034,0.956840121487436)
--(axis cs:88.7755102040816,0.957800822200661)
--(axis cs:88.4353741496599,0.956993169449206)
--(axis cs:88.0952380952381,0.957833040384286)
--(axis cs:87.7551020408163,0.955172181096059)
--(axis cs:87.4149659863945,0.953697423616253)
--(axis cs:87.0748299319728,0.955212498597841)
--(axis cs:86.734693877551,0.955643132327324)
--(axis cs:86.3945578231292,0.953941738912987)
--(axis cs:86.0544217687075,0.952812359148419)
--(axis cs:85.7142857142857,0.952967255567784)
--(axis cs:85.3741496598639,0.952606782741516)
--(axis cs:85.0340136054422,0.951904174190494)
--(axis cs:84.6938775510204,0.950356385287776)
--(axis cs:84.3537414965986,0.947859809433946)
--(axis cs:84.0136054421769,0.949818217755904)
--(axis cs:83.6734693877551,0.948682123528594)
--(axis cs:83.3333333333333,0.947013393256442)
--(axis cs:82.9931972789116,0.946732825282773)
--(axis cs:82.6530612244898,0.9420386080718)
--(axis cs:82.312925170068,0.940084627138956)
--(axis cs:81.9727891156463,0.941766018906301)
--(axis cs:81.6326530612245,0.938370997694222)
--(axis cs:81.2925170068027,0.93672575349972)
--(axis cs:80.9523809523809,0.93622773036548)
--(axis cs:80.6122448979592,0.9296111353349)
--(axis cs:80.2721088435374,0.93010240840708)
--(axis cs:79.9319727891156,0.927936483390347)
--(axis cs:79.5918367346939,0.925909562534195)
--(axis cs:79.2517006802721,0.920327014827376)
--(axis cs:78.9115646258503,0.916023078941632)
--(axis cs:78.5714285714286,0.911211381382874)
--(axis cs:78.2312925170068,0.909740559081139)
--(axis cs:77.891156462585,0.902681155466726)
--(axis cs:77.5510204081633,0.902544588737158)
--(axis cs:77.2108843537415,0.894505890145581)
--(axis cs:76.8707482993197,0.891507858693543)
--(axis cs:76.530612244898,0.88585642809191)
--(axis cs:76.1904761904762,0.875538335581807)
--(axis cs:75.8503401360544,0.870903654965826)
--(axis cs:75.5102040816327,0.868600871443027)
--(axis cs:75.1700680272109,0.867712273492644)
--(axis cs:74.8299319727891,0.868179640638269)
--(axis cs:74.4897959183673,0.867539815157851)
--(axis cs:74.1496598639456,0.865454616706952)
--(axis cs:73.8095238095238,0.866134258368256)
--(axis cs:73.469387755102,0.869979111790091)
--(axis cs:73.1292517006803,0.872709927675773)
--(axis cs:72.7891156462585,0.873013025151366)
--(axis cs:72.4489795918367,0.870399541644877)
--(axis cs:72.108843537415,0.870902069308177)
--(axis cs:71.7687074829932,0.868030094084797)
--(axis cs:71.4285714285714,0.867120425448561)
--(axis cs:71.0884353741497,0.869335311472672)
--(axis cs:70.7482993197279,0.868210097483197)
--(axis cs:70.4081632653061,0.87314558176161)
--(axis cs:70.0680272108844,0.874504960650499)
--(axis cs:69.7278911564626,0.872551016337408)
--(axis cs:69.3877551020408,0.875592200368728)
--(axis cs:69.0476190476191,0.870869623528594)
--(axis cs:68.7074829931973,0.87053121457259)
--(axis cs:68.3673469387755,0.874865560283267)
--(axis cs:68.0272108843537,0.875033780376389)
--(axis cs:67.687074829932,0.875505099407637)
--(axis cs:67.3469387755102,0.876016560439775)
--(axis cs:67.0068027210884,0.878210021979078)
--(axis cs:66.6666666666667,0.879252613072704)
--(axis cs:66.3265306122449,0.882436360316086)
--(axis cs:65.9863945578231,0.88371841195302)
--(axis cs:65.6462585034014,0.884809609875194)
--(axis cs:65.3061224489796,0.887467142804659)
--(axis cs:64.9659863945578,0.884062614440263)
--(axis cs:64.6258503401361,0.887236837487649)
--(axis cs:64.2857142857143,0.88801214527618)
--(axis cs:63.9455782312925,0.887427593847393)
--(axis cs:63.6054421768707,0.887300463645312)
--(axis cs:63.265306122449,0.891123385537261)
--(axis cs:62.9251700680272,0.89136511832588)
--(axis cs:62.5850340136054,0.890875018485829)
--(axis cs:62.2448979591837,0.889484193385667)
--(axis cs:61.9047619047619,0.88855669250621)
--(axis cs:61.5646258503401,0.891970466940258)
--(axis cs:61.2244897959184,0.889752649137581)
--(axis cs:60.8843537414966,0.895738311641555)
--(axis cs:60.5442176870748,0.895764643447538)
--(axis cs:60.2040816326531,0.895447500746935)
--(axis cs:59.8639455782313,0.896993755120551)
--(axis cs:59.5238095238095,0.895967884091937)
--(axis cs:59.1836734693878,0.891339956691339)
--(axis cs:58.843537414966,0.893219681748037)
--(axis cs:58.5034013605442,0.890119009318146)
--(axis cs:58.1632653061224,0.891030972507094)
--(axis cs:57.8231292517007,0.891927869365203)
--(axis cs:57.4829931972789,0.892654477334428)
--(axis cs:57.1428571428571,0.888773271016182)
--(axis cs:56.8027210884354,0.886000351903023)
--(axis cs:56.4625850340136,0.883387343837876)
--(axis cs:56.1224489795918,0.881326148453423)
--(axis cs:55.7823129251701,0.885263502072804)
--(axis cs:55.4421768707483,0.886951148453423)
--(axis cs:55.1020408163265,0.885158905549147)
--(axis cs:54.7619047619048,0.883760346201287)
--(axis cs:54.421768707483,0.881982809257959)
--(axis cs:54.0816326530612,0.877170091511336)
--(axis cs:53.7414965986395,0.876513562394349)
--(axis cs:53.4013605442177,0.877062877544571)
--(axis cs:53.0612244897959,0.876705237610098)
--(axis cs:52.7210884353741,0.88159204288938)
--(axis cs:52.3809523809524,0.879211336075426)
--(axis cs:52.0408163265306,0.878283969241624)
--(axis cs:51.7006802721088,0.872319161328622)
--(axis cs:51.3605442176871,0.868656446229653)
--(axis cs:51.0204081632653,0.863336200028266)
--(axis cs:50.6802721088435,0.864098816584624)
--(axis cs:50.3401360544218,0.859746352868211)
--(axis cs:50,0.857551562992624)
--(axis cs:49.6598639455782,0.858244957690708)
--(axis cs:49.3197278911565,0.856405362183152)
--(axis cs:48.9795918367347,0.851642593715973)
--(axis cs:48.6394557823129,0.853715199534687)
--(axis cs:48.2993197278912,0.851684200732321)
--(axis cs:47.9591836734694,0.855196022444692)
--(axis cs:47.6190476190476,0.856415388365094)
--(axis cs:47.2789115646259,0.854320624202425)
--(axis cs:46.9387755102041,0.858250420724188)
--(axis cs:46.5986394557823,0.858996245897767)
--(axis cs:46.2585034013605,0.863384293156372)
--(axis cs:45.9183673469388,0.869233226313442)
--(axis cs:45.578231292517,0.871787105884783)
--(axis cs:45.2380952380952,0.870914855329293)
--(axis cs:44.8979591836735,0.868009500835518)
--(axis cs:44.5578231292517,0.873052056317471)
--(axis cs:44.2176870748299,0.871415620771481)
--(axis cs:43.8775510204082,0.874279265968165)
--(axis cs:43.5374149659864,0.877351556869593)
--(axis cs:43.1972789115646,0.879663324599798)
--(axis cs:42.8571428571429,0.874918913747585)
--(axis cs:42.5170068027211,0.881010206201273)
--(axis cs:42.1768707482993,0.87775344375141)
--(axis cs:41.8367346938776,0.883818666983556)
--(axis cs:41.4965986394558,0.879589403848056)
--(axis cs:41.156462585034,0.88139173725865)
--(axis cs:40.8163265306122,0.878976432688729)
--(axis cs:40.4761904761905,0.880551980179467)
--(axis cs:40.1360544217687,0.879697354744146)
--(axis cs:39.7959183673469,0.878057123528594)
--(axis cs:39.4557823129252,0.88050182241192)
--(axis cs:39.1156462585034,0.882645275956114)
--(axis cs:38.7755102040816,0.882941729664019)
--(axis cs:38.4353741496599,0.884066450921112)
--(axis cs:38.0952380952381,0.884056859898353)
--(axis cs:37.7551020408163,0.883494232445257)
--(axis cs:37.4149659863946,0.88725843928855)
--(axis cs:37.0748299319728,0.88714500082463)
--(axis cs:36.734693877551,0.886790194081565)
--(axis cs:36.3945578231292,0.889098292733478)
--(axis cs:36.0544217687075,0.887516406533039)
--(axis cs:35.7142857142857,0.888147352909156)
--(axis cs:35.3741496598639,0.887218963729049)
--(axis cs:35.0340136054422,0.887685541137263)
--(axis cs:34.6938775510204,0.884983409669784)
--(axis cs:34.3537414965986,0.89019910942291)
--(axis cs:34.0136054421769,0.889785968280905)
--(axis cs:33.6734693877551,0.890932321055216)
--(axis cs:33.3333333333333,0.889848217932123)
--(axis cs:32.9931972789116,0.889769858636402)
--(axis cs:32.6530612244898,0.884831659179213)
--(axis cs:32.312925170068,0.882217963583656)
--(axis cs:31.9727891156463,0.88131506570031)
--(axis cs:31.6326530612245,0.882681351424004)
--(axis cs:31.2925170068027,0.883058365340726)
--(axis cs:30.952380952381,0.881052664133851)
--(axis cs:30.6122448979592,0.883200365616263)
--(axis cs:30.2721088435374,0.881211898934771)
--(axis cs:29.9319727891156,0.88275909031993)
--(axis cs:29.5918367346939,0.887479587469139)
--(axis cs:29.2517006802721,0.889577760978099)
--(axis cs:28.9115646258503,0.890531289790805)
--(axis cs:28.5714285714286,0.892018795275394)
--(axis cs:28.2312925170068,0.894246940270737)
--(axis cs:27.891156462585,0.894457522116637)
--(axis cs:27.5510204081633,0.894841977334428)
--(axis cs:27.2108843537415,0.894020717449054)
--(axis cs:26.8707482993197,0.894261021663906)
--(axis cs:26.530612244898,0.898465105572956)
--(axis cs:26.1904761904762,0.90214176911147)
--(axis cs:25.8503401360544,0.903879033719006)
--(axis cs:25.5102040816327,0.908124593091894)
--(axis cs:25.1700680272109,0.909130339915104)
--(axis cs:24.8299319727891,0.911710089486859)
--(axis cs:24.4897959183673,0.909562945418336)
--(axis cs:24.1496598639456,0.910204449292408)
--(axis cs:23.8095238095238,0.90952362223548)
--(axis cs:23.469387755102,0.909737612027252)
--(axis cs:23.1292517006803,0.910116708781389)
--(axis cs:22.7891156462585,0.907977827296409)
--(axis cs:22.4489795918367,0.910060386135767)
--(axis cs:22.108843537415,0.911469697840034)
--(axis cs:21.7687074829932,0.90969712068883)
--(axis cs:21.4285714285714,0.906140125268543)
--(axis cs:21.0884353741497,0.908061568118232)
--(axis cs:20.7482993197279,0.906492273907912)
--(axis cs:20.4081632653061,0.905271570924579)
--(axis cs:20.0680272108844,0.904587434736251)
--(axis cs:19.7278911564626,0.906634745901929)
--(axis cs:19.3877551020408,0.905698094118082)
--(axis cs:19.047619047619,0.90798138569787)
--(axis cs:18.7074829931973,0.907359896541772)
--(axis cs:18.3673469387755,0.907171420627453)
--(axis cs:18.0272108843537,0.909711727618209)
--(axis cs:17.687074829932,0.90802960285129)
--(axis cs:17.3469387755102,0.908181205025002)
--(axis cs:17.0068027210884,0.905133759016653)
--(axis cs:16.6666666666667,0.906935230420528)
--(axis cs:16.3265306122449,0.907228444847978)
--(axis cs:15.9863945578231,0.90595762135811)
--(axis cs:15.6462585034014,0.905098171259047)
--(axis cs:15.3061224489796,0.902782053863245)
--(axis cs:14.9659863945578,0.902684458048552)
--(axis cs:14.6258503401361,0.905512877505547)
--(axis cs:14.2857142857143,0.903337268452889)
--(axis cs:13.9455782312925,0.90331204658788)
--(axis cs:13.6054421768707,0.89989105774869)
--(axis cs:13.265306122449,0.900747458160156)
--(axis cs:12.9251700680272,0.898423211372748)
--(axis cs:12.5850340136054,0.897496749286681)
--(axis cs:12.2448979591837,0.894747857072878)
--(axis cs:11.9047619047619,0.887955565587326)
--(axis cs:11.5646258503401,0.884099870471821)
--(axis cs:11.2244897959184,0.887981233795334)
--(axis cs:10.8843537414966,0.879574927339177)
--(axis cs:10.5442176870748,0.877351609556169)
--(axis cs:10.2040816326531,0.866205492976614)
--(axis cs:9.86394557823129,0.861135261272765)
--(axis cs:9.52380952380952,0.858060127839948)
--(axis cs:9.18367346938775,0.851193303604005)
--(axis cs:8.84353741496599,0.84639192700892)
--(axis cs:8.50340136054422,0.840412492363881)
--(axis cs:8.16326530612245,0.834437599875257)
--(axis cs:7.82312925170068,0.824040845587348)
--(axis cs:7.48299319727891,0.8243620232935)
--(axis cs:7.14285714285714,0.814592200756604)
--(axis cs:6.80272108843537,0.807524033287269)
--(axis cs:6.46258503401361,0.794927370661409)
--(axis cs:6.12244897959184,0.785498860114599)
--(axis cs:5.78231292517007,0.772142622890956)
--(axis cs:5.4421768707483,0.760155941858397)
--(axis cs:5.10204081632653,0.741920431159075)
--(axis cs:4.76190476190476,0.716105264803075)
--(axis cs:4.42176870748299,0.692968372159693)
--(axis cs:4.08163265306122,0.66192270022682)
--(axis cs:3.74149659863946,0.615917003675686)
--(axis cs:3.40136054421769,0.561453042948075)
--(axis cs:3.06122448979592,0.501346708416168)
--(axis cs:2.72108843537415,0.458139235360596)
--(axis cs:2.38095238095238,0.425082121798647)
--(axis cs:2.04081632653061,0.383736419918353)
--(axis cs:1.70068027210884,0.340886433885018)
--(axis cs:1.36054421768707,0.262364666375368)
--(axis cs:1.02040816326531,0.225463511310773)
--(axis cs:0.680272108843537,0.161880020411262)
--(axis cs:0.340136054421769,0.0942331096021857)
--(axis cs:0,0.083621060952801)
--cycle;


==> img/stl10/stl10_rate_accuracy_deeptaylor.tex <==
% deep taylor
\addplot [line width=0.5, opacity=0.8, color5, mark=x, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color5, thin}]
table [row sep=\\]{%
0	0.0771875 \\
0.340136054421769	0.0684375 \\
0.680272108843537	0.05546875 \\
1.02040816326531	0.05984375 \\
1.36054421768707	0.0796875 \\
1.70068027210884	0.11234375 \\
2.04081632653061	0.14234375 \\
2.38095238095238	0.16984375 \\
2.72108843537415	0.1934375 \\
3.06122448979592	0.21609375 \\
3.40136054421769	0.243125 \\
3.74149659863946	0.2653125 \\
4.08163265306122	0.27703125 \\
4.42176870748299	0.29203125 \\
4.76190476190476	0.301875 \\
5.10204081632653	0.3125 \\
5.4421768707483	0.326875 \\
5.78231292517007	0.34125 \\
6.12244897959184	0.35265625 \\
6.46258503401361	0.35875 \\
6.80272108843537	0.37390625 \\
7.14285714285714	0.396875 \\
7.48299319727891	0.40609375 \\
7.82312925170068	0.41640625 \\
8.16326530612245	0.42890625 \\
8.50340136054422	0.4325 \\
8.84353741496599	0.450625 \\
9.18367346938775	0.47078125 \\
9.52380952380952	0.49078125 \\
9.86394557823129	0.5040625 \\
10.2040816326531	0.5165625 \\
10.5442176870748	0.53078125 \\
10.8843537414966	0.529375 \\
11.2244897959184	0.53265625 \\
11.5646258503401	0.53765625 \\
11.9047619047619	0.54375 \\
12.2448979591837	0.54625 \\
12.5850340136054	0.55359375 \\
12.9251700680272	0.55109375 \\
13.265306122449	0.55609375 \\
13.6054421768707	0.56421875 \\
13.9455782312925	0.56875 \\
14.2857142857143	0.569375 \\
14.6258503401361	0.576875 \\
14.9659863945578	0.58234375 \\
15.3061224489796	0.58625 \\
15.6462585034014	0.59171875 \\
15.9863945578231	0.59640625 \\
16.3265306122449	0.60046875 \\
16.6666666666667	0.5990625 \\
17.0068027210884	0.603125 \\
17.3469387755102	0.59875 \\
17.687074829932	0.60125 \\
18.0272108843537	0.60203125 \\
18.3673469387755	0.60171875 \\
18.7074829931973	0.59515625 \\
19.047619047619	0.59875 \\
19.3877551020408	0.60015625 \\
19.7278911564626	0.6015625 \\
20.0680272108844	0.604375 \\
20.4081632653061	0.608125 \\
20.7482993197279	0.60875 \\
21.0884353741497	0.60984375 \\
21.4285714285714	0.61421875 \\
21.7687074829932	0.61765625 \\
22.108843537415	0.63171875 \\
22.4489795918367	0.63484375 \\
22.7891156462585	0.6396875 \\
23.1292517006803	0.64 \\
23.469387755102	0.64796875 \\
23.8095238095238	0.65 \\
24.1496598639456	0.65875 \\
24.4897959183673	0.66078125 \\
24.8299319727891	0.66328125 \\
25.1700680272109	0.6678125 \\
25.5102040816327	0.67078125 \\
25.8503401360544	0.673125 \\
26.1904761904762	0.67890625 \\
26.530612244898	0.6821875 \\
26.8707482993197	0.68640625 \\
27.2108843537415	0.6925 \\
27.5510204081633	0.70015625 \\
27.891156462585	0.69828125 \\
28.2312925170068	0.7025 \\
28.5714285714286	0.70578125 \\
28.9115646258503	0.70875 \\
29.2517006802721	0.71171875 \\
29.5918367346939	0.71203125 \\
29.9319727891156	0.71984375 \\
30.2721088435374	0.7190625 \\
30.6122448979592	0.7265625 \\
30.952380952381	0.7290625 \\
31.2925170068027	0.7309375 \\
31.6326530612245	0.7346875 \\
31.9727891156463	0.74171875 \\
32.312925170068	0.74375 \\
32.6530612244898	0.7403125 \\
32.9931972789116	0.74390625 \\
33.3333333333333	0.75 \\
33.6734693877551	0.7478125 \\
34.0136054421769	0.74734375 \\
34.3537414965986	0.74375 \\
34.6938775510204	0.7471875 \\
35.0340136054422	0.74890625 \\
35.3741496598639	0.74734375 \\
35.7142857142857	0.754375 \\
36.0544217687075	0.755625 \\
36.3945578231292	0.75328125 \\
36.734693877551	0.7571875 \\
37.0748299319728	0.7634375 \\
37.4149659863946	0.7634375 \\
37.7551020408163	0.764375 \\
38.0952380952381	0.77578125 \\
38.4353741496599	0.775625 \\
38.7755102040816	0.78484375 \\
39.1156462585034	0.78875 \\
39.4557823129252	0.7925 \\
39.7959183673469	0.80296875 \\
40.1360544217687	0.80703125 \\
40.4761904761905	0.81390625 \\
40.8163265306122	0.81609375 \\
41.156462585034	0.82234375 \\
41.4965986394558	0.8296875 \\
41.8367346938776	0.831875 \\
42.1768707482993	0.83359375 \\
42.5170068027211	0.83859375 \\
42.8571428571429	0.84609375 \\
43.1972789115646	0.84734375 \\
43.5374149659864	0.85484375 \\
43.8775510204082	0.8565625 \\
44.2176870748299	0.8625 \\
44.5578231292517	0.863125 \\
44.8979591836735	0.8665625 \\
45.2380952380952	0.868125 \\
45.578231292517	0.87296875 \\
45.9183673469388	0.8725 \\
46.2585034013605	0.8796875 \\
46.5986394557823	0.87890625 \\
46.9387755102041	0.87984375 \\
47.2789115646259	0.87765625 \\
47.6190476190476	0.8803125 \\
47.9591836734694	0.87703125 \\
48.2993197278912	0.8790625 \\
48.6394557823129	0.885 \\
48.9795918367347	0.88390625 \\
49.3197278911565	0.88546875 \\
49.6598639455782	0.8875 \\
50	0.885 \\
50.3401360544218	0.88421875 \\
50.6802721088435	0.8834375 \\
51.0204081632653	0.88609375 \\
51.3605442176871	0.8853125 \\
51.7006802721088	0.888125 \\
52.0408163265306	0.88984375 \\
52.3809523809524	0.88984375 \\
52.7210884353741	0.8903125 \\
53.0612244897959	0.895 \\
53.4013605442177	0.89015625 \\
53.7414965986395	0.89046875 \\
54.0816326530612	0.89609375 \\
54.421768707483	0.89515625 \\
54.7619047619048	0.89328125 \\
55.1020408163265	0.89671875 \\
55.4421768707483	0.89875 \\
55.7823129251701	0.8996875 \\
56.1224489795918	0.90234375 \\
56.4625850340136	0.905625 \\
56.8027210884354	0.91046875 \\
57.1428571428571	0.90859375 \\
57.4829931972789	0.9134375 \\
57.8231292517007	0.91078125 \\
58.1632653061224	0.915 \\
58.5034013605442	0.92015625 \\
58.843537414966	0.92109375 \\
59.1836734693878	0.9228125 \\
59.5238095238095	0.923125 \\
59.8639455782313	0.92328125 \\
60.2040816326531	0.9271875 \\
60.5442176870748	0.92546875 \\
60.8843537414966	0.92859375 \\
61.2244897959184	0.9271875 \\
61.5646258503401	0.92453125 \\
61.9047619047619	0.92296875 \\
62.2448979591837	0.919375 \\
62.5850340136054	0.923125 \\
62.9251700680272	0.9203125 \\
63.265306122449	0.9165625 \\
63.6054421768707	0.91703125 \\
63.9455782312925	0.9175 \\
64.2857142857143	0.91765625 \\
64.6258503401361	0.9171875 \\
64.9659863945578	0.91625 \\
65.3061224489796	0.91671875 \\
65.6462585034014	0.9175 \\
65.9863945578231	0.918125 \\
66.3265306122449	0.9178125 \\
66.6666666666667	0.91796875 \\
67.0068027210884	0.918125 \\
67.3469387755102	0.91890625 \\
67.687074829932	0.91890625 \\
68.0272108843537	0.9215625 \\
68.3673469387755	0.92421875 \\
68.7074829931973	0.92578125 \\
69.0476190476191	0.92703125 \\
69.3877551020408	0.92890625 \\
69.7278911564626	0.93046875 \\
70.0680272108844	0.93375 \\
70.4081632653061	0.9321875 \\
70.7482993197279	0.93421875 \\
71.0884353741497	0.93421875 \\
71.4285714285714	0.9340625 \\
71.7687074829932	0.93171875 \\
72.108843537415	0.93109375 \\
72.4489795918367	0.93375 \\
72.7891156462585	0.93765625 \\
73.1292517006803	0.93234375 \\
73.469387755102	0.93078125 \\
73.8095238095238	0.92609375 \\
74.1496598639456	0.92484375 \\
74.4897959183673	0.9246875 \\
74.8299319727891	0.92671875 \\
75.1700680272109	0.92953125 \\
75.5102040816327	0.93046875 \\
75.8503401360544	0.93046875 \\
76.1904761904762	0.9353125 \\
76.530612244898	0.938125 \\
76.8707482993197	0.93984375 \\
77.2108843537415	0.94046875 \\
77.5510204081633	0.94140625 \\
77.891156462585	0.94234375 \\
78.2312925170068	0.94234375 \\
78.5714285714286	0.94375 \\
78.9115646258503	0.9471875 \\
79.2517006802721	0.948125 \\
79.5918367346939	0.9525 \\
79.9319727891156	0.95375 \\
80.2721088435374	0.95640625 \\
80.6122448979592	0.9571875 \\
80.9523809523809	0.95859375 \\
81.2925170068027	0.95984375 \\
81.6326530612245	0.95984375 \\
81.9727891156463	0.9596875 \\
82.312925170068	0.96015625 \\
82.6530612244898	0.9603125 \\
82.9931972789116	0.9596875 \\
83.3333333333333	0.9590625 \\
83.6734693877551	0.96 \\
84.0136054421769	0.95859375 \\
84.3537414965986	0.95359375 \\
84.6938775510204	0.95078125 \\
85.0340136054422	0.945625 \\
85.3741496598639	0.943125 \\
85.7142857142857	0.94140625 \\
86.0544217687075	0.940625 \\
86.3945578231292	0.94046875 \\
86.734693877551	0.94015625 \\
87.0748299319728	0.94015625 \\
87.4149659863945	0.94 \\
87.7551020408163	0.940625 \\
88.0952380952381	0.94 \\
88.4353741496599	0.94046875 \\
88.7755102040816	0.94109375 \\
89.1156462585034	0.94265625 \\
89.4557823129252	0.9425 \\
89.7959183673469	0.9425 \\
90.1360544217687	0.94265625 \\
90.4761904761905	0.94265625 \\
90.8163265306122	0.94296875 \\
91.156462585034	0.9446875 \\
91.4965986394558	0.94390625 \\
91.8367346938775	0.9459375 \\
92.1768707482993	0.94671875 \\
92.5170068027211	0.94671875 \\
92.8571428571429	0.94515625 \\
93.1972789115646	0.94984375 \\
93.5374149659864	0.95328125 \\
93.8775510204082	0.95234375 \\
94.2176870748299	0.95515625 \\
94.5578231292517	0.95296875 \\
94.8979591836735	0.956875 \\
95.2380952380952	0.9571875 \\
95.578231292517	0.9590625 \\
95.9183673469388	0.959375 \\
96.2585034013605	0.96 \\
96.5986394557823	0.96 \\
96.9387755102041	0.96 \\
97.2789115646258	0.96 \\
97.6190476190476	0.95984375 \\
97.9591836734694	0.96 \\
98.2993197278912	0.96 \\
98.6394557823129	0.96 \\
98.9795918367347	0.96 \\
99.3197278911565	0.96 \\
99.6598639455782	0.96078125 \\
100	1 \\
};
\path [fill=color5, fill opacity=0.5] (axis cs:0,0.0838952831097947)
--(axis cs:0,0.0704797168902053)
--(axis cs:0.340136054421769,0.0593759681955765)
--(axis cs:0.680272108843537,0.0461801055668616)
--(axis cs:1.02040816326531,0.0493471794279315)
--(axis cs:1.36054421768707,0.0658492268875638)
--(axis cs:1.70068027210884,0.0970877932316113)
--(axis cs:2.04081632653061,0.125480294114293)
--(axis cs:2.38095238095238,0.15314681576299)
--(axis cs:2.72108843537415,0.176951227523307)
--(axis cs:3.06122448979592,0.199550596776412)
--(axis cs:3.40136054421769,0.226922300662534)
--(axis cs:3.74149659863946,0.249511489398296)
--(axis cs:4.08163265306122,0.261166692368513)
--(axis cs:4.42176870748299,0.276198584587399)
--(axis cs:4.76190476190476,0.286003530819879)
--(axis cs:5.10204081632653,0.296714085427922)
--(axis cs:5.4421768707483,0.310770895131877)
--(axis cs:5.78231292517007,0.325544033023031)
--(axis cs:6.12244897959184,0.336764064209056)
--(axis cs:6.46258503401361,0.34244286823544)
--(axis cs:6.80272108843537,0.357345235639301)
--(axis cs:7.14285714285714,0.381425546679246)
--(axis cs:7.48299319727891,0.390738721467134)
--(axis cs:7.82312925170068,0.401004710702913)
--(axis cs:8.16326530612245,0.412985884957976)
--(axis cs:8.50340136054422,0.415310280683056)
--(axis cs:8.84353741496599,0.432954884799713)
--(axis cs:9.18367346938775,0.452539386629619)
--(axis cs:9.52380952380952,0.471883567039789)
--(axis cs:9.86394557823129,0.485921027992696)
--(axis cs:10.2040816326531,0.499951748866392)
--(axis cs:10.5442176870748,0.514668560616931)
--(axis cs:10.8843537414966,0.513910122209718)
--(axis cs:11.2244897959184,0.51756496233125)
--(axis cs:11.5646258503401,0.522503788428532)
--(axis cs:11.9047619047619,0.528890838592492)
--(axis cs:12.2448979591837,0.530833297592067)
--(axis cs:12.5850340136054,0.538300332262338)
--(axis cs:12.9251700680272,0.535301493337844)
--(axis cs:13.265306122449,0.539853718220408)
--(axis cs:13.6054421768707,0.547950555276986)
--(axis cs:13.9455782312925,0.552399648799643)
--(axis cs:14.2857142857143,0.552946675936269)
--(axis cs:14.6258503401361,0.560678776444161)
--(axis cs:14.9659863945578,0.566386886093289)
--(axis cs:15.3061224489796,0.570007913021896)
--(axis cs:15.6462585034014,0.575779227590787)
--(axis cs:15.9863945578231,0.58039926157029)
--(axis cs:16.3265306122449,0.584523245633657)
--(axis cs:16.6666666666667,0.583639612851413)
--(axis cs:17.0068027210884,0.587745458265765)
--(axis cs:17.3469387755102,0.583043425829674)
--(axis cs:17.687074829932,0.586475154788446)
--(axis cs:18.0272108843537,0.5879183168895)
--(axis cs:18.3673469387755,0.587206032377917)
--(axis cs:18.7074829931973,0.581025758443583)
--(axis cs:19.047619047619,0.583869033086875)
--(axis cs:19.3877551020408,0.586501475538275)
--(axis cs:19.7278911564626,0.588384332714008)
--(axis cs:20.0680272108844,0.591028566438244)
--(axis cs:20.4081632653061,0.594246126183017)
--(axis cs:20.7482993197279,0.595450810599112)
--(axis cs:21.0884353741497,0.595164420594609)
--(axis cs:21.4285714285714,0.598510657948965)
--(axis cs:21.7687074829932,0.601447371648098)
--(axis cs:22.108843537415,0.615822964076308)
--(axis cs:22.4489795918367,0.618573796711656)
--(axis cs:22.7891156462585,0.624346452193454)
--(axis cs:23.1292517006803,0.624751859184155)
--(axis cs:23.469387755102,0.632051380379373)
--(axis cs:23.8095238095238,0.63449509040079)
--(axis cs:24.1496598639456,0.643282039161544)
--(axis cs:24.4897959183673,0.646201005081957)
--(axis cs:24.8299319727891,0.64872915798689)
--(axis cs:25.1700680272109,0.65300412830307)
--(axis cs:25.5102040816327,0.656288259687836)
--(axis cs:25.8503401360544,0.658435604136654)
--(axis cs:26.1904761904762,0.663803591748722)
--(axis cs:26.530612244898,0.667976586122202)
--(axis cs:26.8707482993197,0.672595915951249)
--(axis cs:27.2108843537415,0.678814878069383)
--(axis cs:27.5510204081633,0.686374257633196)
--(axis cs:27.891156462585,0.68448127810716)
--(axis cs:28.2312925170068,0.688898058323062)
--(axis cs:28.5714285714286,0.692489592198422)
--(axis cs:28.9115646258503,0.695622587879761)
--(axis cs:29.2517006802721,0.699086318588579)
--(axis cs:29.5918367346939,0.699135817066137)
--(axis cs:29.9319727891156,0.706724695008049)
--(axis cs:30.2721088435374,0.706413093816047)
--(axis cs:30.6122448979592,0.713978856509496)
--(axis cs:30.952380952381,0.715864085298424)
--(axis cs:31.2925170068027,0.718251956883902)
--(axis cs:31.6326530612245,0.722203532009529)
--(axis cs:31.9727891156463,0.72899379961964)
--(axis cs:32.312925170068,0.730832768934542)
--(axis cs:32.6530612244898,0.727399699471824)
--(axis cs:32.9931972789116,0.731049330879826)
--(axis cs:33.3333333333333,0.737025309624811)
--(axis cs:33.6734693877551,0.734068965698103)
--(axis cs:34.0136054421769,0.734078666203803)
--(axis cs:34.3537414965986,0.729655662125966)
--(axis cs:34.6938775510204,0.733426628942337)
--(axis cs:35.0340136054422,0.735263353814329)
--(axis cs:35.3741496598639,0.734306366312577)
--(axis cs:35.7142857142857,0.741324821479235)
--(axis cs:36.0544217687075,0.742217255646732)
--(axis cs:36.3945578231292,0.739934459166188)
--(axis cs:36.734693877551,0.744277654008078)
--(axis cs:37.0748299319728,0.750551314684995)
--(axis cs:37.4149659863946,0.750363228147516)
--(axis cs:37.7551020408163,0.751800454216547)
--(axis cs:38.0952380952381,0.762604168274971)
--(axis cs:38.4353741496599,0.76177570476466)
--(axis cs:38.7755102040816,0.770891887589494)
--(axis cs:39.1156462585034,0.77411915118455)
--(axis cs:39.4557823129252,0.77775164286824)
--(axis cs:39.7959183673469,0.787823842940567)
--(axis cs:40.1360544217687,0.79193996233125)
--(axis cs:40.4761904761905,0.799278986657674)
--(axis cs:40.8163265306122,0.801341190366259)
--(axis cs:41.156462585034,0.807162992490588)
--(axis cs:41.4965986394558,0.814952081161047)
--(axis cs:41.8367346938776,0.818049827071818)
--(axis cs:42.1768707482993,0.81946528330446)
--(axis cs:42.5170068027211,0.82480483965647)
--(axis cs:42.8571428571429,0.832806397886193)
--(axis cs:43.1972789115646,0.833734448438595)
--(axis cs:43.5374149659864,0.841528435803065)
--(axis cs:43.8775510204082,0.843317201692823)
--(axis cs:44.2176870748299,0.849475423715055)
--(axis cs:44.5578231292517,0.850331658521651)
--(axis cs:44.8979591836735,0.854309072545814)
--(axis cs:45.2380952380952,0.855757692820778)
--(axis cs:45.578231292517,0.860957825229493)
--(axis cs:45.9183673469388,0.860305084137216)
--(axis cs:46.2585034013605,0.868027490971407)
--(axis cs:46.5986394557823,0.867136747272272)
--(axis cs:46.9387755102041,0.868730228473599)
--(axis cs:47.2789115646259,0.866267253390359)
--(axis cs:47.6190476190476,0.869135231306387)
--(axis cs:47.9591836734694,0.865789747268292)
--(axis cs:48.2993197278912,0.867644650856981)
--(axis cs:48.6394557823129,0.874496617453321)
--(axis cs:48.9795918367347,0.872518928242811)
--(axis cs:49.3197278911565,0.87447602182944)
--(axis cs:49.6598639455782,0.87712635021493)
--(axis cs:50,0.874435958703893)
--(axis cs:50.3401360544218,0.872958599007841)
--(axis cs:50.6802721088435,0.872750496859137)
--(axis cs:51.0204081632653,0.875327176117879)
--(axis cs:51.3605442176871,0.874690839506892)
--(axis cs:51.7006802721088,0.877855759234091)
--(axis cs:52.0408163265306,0.879691726390196)
--(axis cs:52.3809523809524,0.880702060859219)
--(axis cs:52.7210884353741,0.880424593704026)
--(axis cs:53.0612244897959,0.886189262837)
--(axis cs:53.4013605442177,0.87990234375)
--(axis cs:53.7414965986395,0.879532557974413)
--(axis cs:54.0816326530612,0.885619007516171)
--(axis cs:54.421768707483,0.884238386069376)
--(axis cs:54.7619047619048,0.882481952237955)
--(axis cs:55.1020408163265,0.885318872847299)
--(axis cs:55.4421768707483,0.887068744879449)
--(axis cs:55.7823129251701,0.888227964522105)
--(axis cs:56.1224489795918,0.890675973490871)
--(axis cs:56.4625850340136,0.893995292714228)
--(axis cs:56.8027210884354,0.898878882551844)
--(axis cs:57.1428571428571,0.897335293027859)
--(axis cs:57.4829931972789,0.90251308679127)
--(axis cs:57.8231292517007,0.900452283654021)
--(axis cs:58.1632653061224,0.904463981281827)
--(axis cs:58.5034013605442,0.91009765625)
--(axis cs:58.843537414966,0.911253701557806)
--(axis cs:59.1836734693878,0.914419742109428)
--(axis cs:59.5238095238095,0.915072059324965)
--(axis cs:59.8639455782313,0.915825401563818)
--(axis cs:60.2040816326531,0.920032555045307)
--(axis cs:60.5442176870748,0.918010343811277)
--(axis cs:60.8843537414966,0.920906149764055)
--(axis cs:61.2244897959184,0.919342110246721)
--(axis cs:61.5646258503401,0.916275397324864)
--(axis cs:61.9047619047619,0.914568609366005)
--(axis cs:62.2448979591837,0.910403371814175)
--(axis cs:62.5850340136054,0.914679004566235)
--(axis cs:62.9251700680272,0.912299925196576)
--(axis cs:63.265306122449,0.909060109837239)
--(axis cs:63.6054421768707,0.910815677093371)
--(axis cs:63.9455782312925,0.912670209758251)
--(axis cs:64.2857142857143,0.912445577510955)
--(axis cs:64.6258503401361,0.912609098371199)
--(axis cs:64.9659863945578,0.911326342708611)
--(axis cs:65.3061224489796,0.912048575312024)
--(axis cs:65.6462585034014,0.913366013576462)
--(axis cs:65.9863945578231,0.914191986217656)
--(axis cs:66.3265306122449,0.913337328422895)
--(axis cs:66.6666666666667,0.913659685259197)
--(axis cs:67.0068027210884,0.912998279395154)
--(axis cs:67.3469387755102,0.91475959497157)
--(axis cs:67.687074829932,0.914297744057032)
--(axis cs:68.0272108843537,0.917095860692957)
--(axis cs:68.3673469387755,0.918761346872012)
--(axis cs:68.7074829931973,0.919686529774754)
--(axis cs:69.0476190476191,0.920691110219481)
--(axis cs:69.3877551020408,0.922485397977235)
--(axis cs:69.7278911564626,0.923886544883602)
--(axis cs:70.0680272108844,0.927629515775003)
--(axis cs:70.4081632653061,0.925635063985462)
--(axis cs:70.7482993197279,0.928288996881539)
--(axis cs:71.0884353741497,0.928067956544531)
--(axis cs:71.4285714285714,0.927815552503235)
--(axis cs:71.7687074829932,0.924652998060973)
--(axis cs:72.108843537415,0.923778651511698)
--(axis cs:72.4489795918367,0.927337322203366)
--(axis cs:72.7891156462585,0.933518804655407)
--(axis cs:73.1292517006803,0.926267835847538)
--(axis cs:73.469387755102,0.924550352679317)
--(axis cs:73.8095238095238,0.920196250333248)
--(axis cs:74.1496598639456,0.919488660206697)
--(axis cs:74.4897959183673,0.919392405581357)
--(axis cs:74.8299319727891,0.92068062370816)
--(axis cs:75.1700680272109,0.923288120231084)
--(axis cs:75.5102040816327,0.924225620231084)
--(axis cs:75.8503401360544,0.924225620231084)
--(axis cs:76.1904761904762,0.929845494139735)
--(axis cs:76.530612244898,0.934481492557387)
--(axis cs:76.8707482993197,0.938743219954142)
--(axis cs:77.2108843537415,0.938577644850485)
--(axis cs:77.5510204081633,0.938210338247665)
--(axis cs:77.891156462585,0.938323205302688)
--(axis cs:78.2312925170068,0.938323205302688)
--(axis cs:78.5714285714286,0.938871095313751)
--(axis cs:78.9115646258503,0.941189784166881)
--(axis cs:79.2517006802721,0.941985846232226)
--(axis cs:79.5918367346939,0.946448463521551)
--(axis cs:79.9319727891156,0.947956094931957)
--(axis cs:80.2721088435374,0.951404762489335)
--(axis cs:80.6122448979592,0.952842071198967)
--(axis cs:80.9523809523809,0.955063236819819)
--(axis cs:81.2925170068027,0.958743219954142)
--(axis cs:81.6326530612245,0.958743219954142)
--(axis cs:81.9727891156463,0.958137255091173)
--(axis cs:82.312925170068,0.959055719954142)
--(axis cs:82.6530612244898,0.958124476904062)
--(axis cs:82.9931972789116,0.956265348541419)
--(axis cs:83.3333333333333,0.955348993487924)
--(axis cs:83.6734693877551,0.955045448869545)
--(axis cs:84.0136054421769,0.952702722214119)
--(axis cs:84.3537414965986,0.94643947152055)
--(axis cs:84.6938775510204,0.943579142942386)
--(axis cs:85.0340136054422,0.939636832141892)
--(axis cs:85.3741496598639,0.938453804397226)
--(axis cs:85.7142857142857,0.938151204431153)
--(axis cs:86.0544217687075,0.93845009204577)
--(axis cs:86.3945578231292,0.938577644850485)
--(axis cs:86.734693877551,0.939055719954142)
--(axis cs:87.0748299319728,0.939055719954142)
--(axis cs:87.4149659863945,0.94)
--(axis cs:87.7551020408163,0.93845009204577)
--(axis cs:88.0952380952381,0.94)
--(axis cs:88.4353741496599,0.938577644850485)
--(axis cs:88.7755102040816,0.938251634333817)
--(axis cs:89.1156462585034,0.938414100267779)
--(axis cs:89.4557823129252,0.938366013576462)
--(axis cs:89.7959183673469,0.938366013576462)
--(axis cs:90.1360544217687,0.938414100267779)
--(axis cs:90.4761904761905,0.938414100267779)
--(axis cs:90.8163265306122,0.938486126008778)
--(axis cs:91.156462585034,0.939292489329323)
--(axis cs:91.4965986394558,0.938950736540482)
--(axis cs:91.8367346938775,0.940226487688589)
--(axis cs:92.1768707482993,0.9408147855468)
--(axis cs:92.5170068027211,0.940747327833512)
--(axis cs:92.8571428571429,0.939688372000325)
--(axis cs:93.1972789115646,0.943500602562869)
--(axis cs:93.5374149659864,0.9473772855468)
--(axis cs:93.8775510204082,0.946267835847538)
--(axis cs:94.2176870748299,0.949801160206697)
--(axis cs:94.5578231292517,0.946406860379948)
--(axis cs:94.8979591836735,0.951359366700608)
--(axis cs:95.2380952380952,0.952391394860231)
--(axis cs:95.578231292517,0.956014748723764)
--(axis cs:95.9183673469388,0.95720009204577)
--(axis cs:96.2585034013605,0.96)
--(axis cs:96.5986394557823,0.96)
--(axis cs:96.9387755102041,0.96)
--(axis cs:97.2789115646258,0.96)
--(axis cs:97.6190476190476,0.958743219954142)
--(axis cs:97.9591836734694,0.96)
--(axis cs:98.2993197278912,0.96)
--(axis cs:98.6394557823129,0.96)
--(axis cs:98.9795918367347,0.96)
--(axis cs:99.3197278911565,0.96)
--(axis cs:99.6598639455782,0.958359453756321)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,0.963203046243679)
--(axis cs:99.3197278911565,0.96)
--(axis cs:98.9795918367347,0.96)
--(axis cs:98.6394557823129,0.96)
--(axis cs:98.2993197278912,0.96)
--(axis cs:97.9591836734694,0.96)
--(axis cs:97.6190476190476,0.960944280045858)
--(axis cs:97.2789115646258,0.96)
--(axis cs:96.9387755102041,0.96)
--(axis cs:96.5986394557823,0.96)
--(axis cs:96.2585034013605,0.96)
--(axis cs:95.9183673469388,0.96154990795423)
--(axis cs:95.578231292517,0.962110251276236)
--(axis cs:95.2380952380952,0.961983605139769)
--(axis cs:94.8979591836735,0.962390633299392)
--(axis cs:94.5578231292517,0.959530639620052)
--(axis cs:94.2176870748299,0.960511339793303)
--(axis cs:93.8775510204082,0.958419664152462)
--(axis cs:93.5374149659864,0.9591852144532)
--(axis cs:93.1972789115646,0.956186897437131)
--(axis cs:92.8571428571429,0.950624127999676)
--(axis cs:92.5170068027211,0.952690172166489)
--(axis cs:92.1768707482993,0.9526227144532)
--(axis cs:91.8367346938775,0.951648512311411)
--(axis cs:91.4965986394558,0.948861763459518)
--(axis cs:91.156462585034,0.950082510670677)
--(axis cs:90.8163265306122,0.947451373991222)
--(axis cs:90.4761904761905,0.946898399732221)
--(axis cs:90.1360544217687,0.946898399732221)
--(axis cs:89.7959183673469,0.946633986423538)
--(axis cs:89.4557823129252,0.946633986423538)
--(axis cs:89.1156462585034,0.946898399732221)
--(axis cs:88.7755102040816,0.943935865666183)
--(axis cs:88.4353741496599,0.942359855149515)
--(axis cs:88.0952380952381,0.94)
--(axis cs:87.7551020408163,0.942799907954231)
--(axis cs:87.4149659863945,0.94)
--(axis cs:87.0748299319728,0.941256780045858)
--(axis cs:86.734693877551,0.941256780045858)
--(axis cs:86.3945578231292,0.942359855149515)
--(axis cs:86.0544217687075,0.942799907954231)
--(axis cs:85.7142857142857,0.944661295568847)
--(axis cs:85.3741496598639,0.947796195602774)
--(axis cs:85.0340136054422,0.951613167858108)
--(axis cs:84.6938775510204,0.957983357057614)
--(axis cs:84.3537414965986,0.96074802847945)
--(axis cs:84.0136054421769,0.964484777785881)
--(axis cs:83.6734693877551,0.964954551130455)
--(axis cs:83.3333333333333,0.962776006512077)
--(axis cs:82.9931972789116,0.963109651458581)
--(axis cs:82.6530612244898,0.962500523095938)
--(axis cs:82.312925170068,0.961256780045858)
--(axis cs:81.9727891156463,0.961237744908827)
--(axis cs:81.6326530612245,0.960944280045858)
--(axis cs:81.2925170068027,0.960944280045858)
--(axis cs:80.9523809523809,0.962124263180181)
--(axis cs:80.6122448979592,0.961532928801033)
--(axis cs:80.2721088435374,0.961407737510665)
--(axis cs:79.9319727891156,0.959543905068043)
--(axis cs:79.5918367346939,0.958551536478449)
--(axis cs:79.2517006802721,0.954264153767774)
--(axis cs:78.9115646258503,0.953185215833119)
--(axis cs:78.5714285714286,0.948628904686249)
--(axis cs:78.2312925170068,0.946364294697312)
--(axis cs:77.891156462585,0.946364294697312)
--(axis cs:77.5510204081633,0.944602161752335)
--(axis cs:77.2108843537415,0.942359855149515)
--(axis cs:76.8707482993197,0.940944280045858)
--(axis cs:76.530612244898,0.941768507442613)
--(axis cs:76.1904761904762,0.940779505860265)
--(axis cs:75.8503401360544,0.936711879768916)
--(axis cs:75.5102040816327,0.936711879768916)
--(axis cs:75.1700680272109,0.935774379768916)
--(axis cs:74.8299319727891,0.93275687629184)
--(axis cs:74.4897959183673,0.929982594418643)
--(axis cs:74.1496598639456,0.930198839793303)
--(axis cs:73.8095238095238,0.931991249666752)
--(axis cs:73.469387755102,0.937012147320683)
--(axis cs:73.1292517006803,0.938419664152462)
--(axis cs:72.7891156462585,0.941793695344593)
--(axis cs:72.4489795918367,0.940162677796634)
--(axis cs:72.108843537415,0.938408848488302)
--(axis cs:71.7687074829932,0.938784501939027)
--(axis cs:71.4285714285714,0.940309447496765)
--(axis cs:71.0884353741497,0.940369543455469)
--(axis cs:70.7482993197279,0.940148503118461)
--(axis cs:70.4081632653061,0.938739936014538)
--(axis cs:70.0680272108844,0.939870484224997)
--(axis cs:69.7278911564626,0.937050955116398)
--(axis cs:69.3877551020408,0.935327102022765)
--(axis cs:69.0476190476191,0.933371389780519)
--(axis cs:68.7074829931973,0.931875970225246)
--(axis cs:68.3673469387755,0.929676153127987)
--(axis cs:68.0272108843537,0.926029139307043)
--(axis cs:67.687074829932,0.923514755942968)
--(axis cs:67.3469387755102,0.92305290502843)
--(axis cs:67.0068027210884,0.923251720604846)
--(axis cs:66.6666666666667,0.922277814740803)
--(axis cs:66.3265306122449,0.922287671577105)
--(axis cs:65.9863945578231,0.922058013782344)
--(axis cs:65.6462585034014,0.921633986423538)
--(axis cs:65.3061224489796,0.921388924687976)
--(axis cs:64.9659863945578,0.921173657291389)
--(axis cs:64.6258503401361,0.921765901628801)
--(axis cs:64.2857142857143,0.922866922489045)
--(axis cs:63.9455782312925,0.922329790241749)
--(axis cs:63.6054421768707,0.923246822906629)
--(axis cs:63.265306122449,0.924064890162761)
--(axis cs:62.9251700680272,0.928325074803424)
--(axis cs:62.5850340136054,0.931570995433765)
--(axis cs:62.2448979591837,0.928346628185825)
--(axis cs:61.9047619047619,0.931368890633995)
--(axis cs:61.5646258503401,0.932787102675136)
--(axis cs:61.2244897959184,0.935032889753279)
--(axis cs:60.8843537414966,0.936281350235945)
--(axis cs:60.5442176870748,0.932927156188723)
--(axis cs:60.2040816326531,0.934342444954693)
--(axis cs:59.8639455782313,0.930737098436182)
--(axis cs:59.5238095238095,0.931177940675034)
--(axis cs:59.1836734693878,0.931205257890572)
--(axis cs:58.843537414966,0.930933798442194)
--(axis cs:58.5034013605442,0.93021484375)
--(axis cs:58.1632653061224,0.925536018718173)
--(axis cs:57.8231292517007,0.921110216345979)
--(axis cs:57.4829931972789,0.92436191320873)
--(axis cs:57.1428571428571,0.919852206972141)
--(axis cs:56.8027210884354,0.922058617448156)
--(axis cs:56.4625850340136,0.917254707285772)
--(axis cs:56.1224489795918,0.914011526509129)
--(axis cs:55.7823129251701,0.911147035477895)
--(axis cs:55.4421768707483,0.910431255120551)
--(axis cs:55.1020408163265,0.908118627152701)
--(axis cs:54.7619047619048,0.904080547762045)
--(axis cs:54.421768707483,0.906074113930624)
--(axis cs:54.0816326530612,0.906568492483829)
--(axis cs:53.7414965986395,0.901404942025587)
--(axis cs:53.4013605442177,0.90041015625)
--(axis cs:53.0612244897959,0.903810737163)
--(axis cs:52.7210884353741,0.900200406295974)
--(axis cs:52.3809523809524,0.898985439140781)
--(axis cs:52.0408163265306,0.899995773609804)
--(axis cs:51.7006802721088,0.898394240765909)
--(axis cs:51.3605442176871,0.895934160493108)
--(axis cs:51.0204081632653,0.896860323882121)
--(axis cs:50.6802721088435,0.894124503140863)
--(axis cs:50.3401360544218,0.895478900992159)
--(axis cs:50,0.895564041296107)
--(axis cs:49.6598639455782,0.89787364978507)
--(axis cs:49.3197278911565,0.896461478170561)
--(axis cs:48.9795918367347,0.895293571757189)
--(axis cs:48.6394557823129,0.895503382546679)
--(axis cs:48.2993197278912,0.890480349143019)
--(axis cs:47.9591836734694,0.888272752731708)
--(axis cs:47.6190476190476,0.891489768693613)
--(axis cs:47.2789115646259,0.889045246609641)
--(axis cs:46.9387755102041,0.890957271526401)
--(axis cs:46.5986394557823,0.890675752727728)
--(axis cs:46.2585034013605,0.891347509028593)
--(axis cs:45.9183673469388,0.884694915862784)
--(axis cs:45.578231292517,0.884979674770507)
--(axis cs:45.2380952380952,0.880492307179222)
--(axis cs:44.8979591836735,0.878815927454186)
--(axis cs:44.5578231292517,0.875918341478349)
--(axis cs:44.2176870748299,0.875524576284945)
--(axis cs:43.8775510204082,0.869807798307177)
--(axis cs:43.5374149659864,0.868159064196935)
--(axis cs:43.1972789115646,0.860953051561405)
--(axis cs:42.8571428571429,0.859381102113807)
--(axis cs:42.5170068027211,0.85238266034353)
--(axis cs:42.1768707482993,0.84772221669554)
--(axis cs:41.8367346938776,0.845700172928182)
--(axis cs:41.4965986394558,0.844422918838953)
--(axis cs:41.156462585034,0.837524507509412)
--(axis cs:40.8163265306122,0.830846309633741)
--(axis cs:40.4761904761905,0.828533513342326)
--(axis cs:40.1360544217687,0.82212253766875)
--(axis cs:39.7959183673469,0.818113657059433)
--(axis cs:39.4557823129252,0.80724835713176)
--(axis cs:39.1156462585034,0.80338084881545)
--(axis cs:38.7755102040816,0.798795612410506)
--(axis cs:38.4353741496599,0.789474295235341)
--(axis cs:38.0952380952381,0.788958331725029)
--(axis cs:37.7551020408163,0.776949545783453)
--(axis cs:37.4149659863946,0.776511771852484)
--(axis cs:37.0748299319728,0.776323685315005)
--(axis cs:36.734693877551,0.770097345991922)
--(axis cs:36.3945578231292,0.766628040833812)
--(axis cs:36.0544217687075,0.769032744353268)
--(axis cs:35.7142857142857,0.767425178520765)
--(axis cs:35.3741496598639,0.760381133687423)
--(axis cs:35.0340136054422,0.762549146185671)
--(axis cs:34.6938775510204,0.760948371057663)
--(axis cs:34.3537414965986,0.757844337874034)
--(axis cs:34.0136054421769,0.760608833796197)
--(axis cs:33.6734693877551,0.761556034301897)
--(axis cs:33.3333333333333,0.762974690375189)
--(axis cs:32.9931972789116,0.756763169120174)
--(axis cs:32.6530612244898,0.753225300528176)
--(axis cs:32.312925170068,0.756667231065458)
--(axis cs:31.9727891156463,0.75444370038036)
--(axis cs:31.6326530612245,0.747171467990471)
--(axis cs:31.2925170068027,0.743623043116098)
--(axis cs:30.952380952381,0.742260914701576)
--(axis cs:30.6122448979592,0.739146143490504)
--(axis cs:30.2721088435374,0.731711906183954)
--(axis cs:29.9319727891156,0.732962804991951)
--(axis cs:29.5918367346939,0.724926682933863)
--(axis cs:29.2517006802721,0.724351181411421)
--(axis cs:28.9115646258503,0.721877412120239)
--(axis cs:28.5714285714286,0.719072907801578)
--(axis cs:28.2312925170068,0.716101941676938)
--(axis cs:27.891156462585,0.71208122189284)
--(axis cs:27.5510204081633,0.713938242366804)
--(axis cs:27.2108843537415,0.706185121930617)
--(axis cs:26.8707482993197,0.700216584048751)
--(axis cs:26.530612244898,0.696398413877798)
--(axis cs:26.1904761904762,0.694008908251278)
--(axis cs:25.8503401360544,0.687814395863346)
--(axis cs:25.5102040816327,0.685274240312164)
--(axis cs:25.1700680272109,0.682620871696931)
--(axis cs:24.8299319727891,0.67783334201311)
--(axis cs:24.4897959183673,0.675361494918043)
--(axis cs:24.1496598639456,0.674217960838456)
--(axis cs:23.8095238095238,0.66550490959921)
--(axis cs:23.469387755102,0.663886119620627)
--(axis cs:23.1292517006803,0.655248140815845)
--(axis cs:22.7891156462585,0.655028547806546)
--(axis cs:22.4489795918367,0.651113703288344)
--(axis cs:22.108843537415,0.647614535923692)
--(axis cs:21.7687074829932,0.633865128351902)
--(axis cs:21.4285714285714,0.629926842051035)
--(axis cs:21.0884353741497,0.624523079405392)
--(axis cs:20.7482993197279,0.622049189400888)
--(axis cs:20.4081632653061,0.622003873816983)
--(axis cs:20.0680272108844,0.617721433561756)
--(axis cs:19.7278911564626,0.614740667285992)
--(axis cs:19.3877551020408,0.613811024461725)
--(axis cs:19.047619047619,0.613630966913125)
--(axis cs:18.7074829931973,0.609286741556417)
--(axis cs:18.3673469387755,0.616231467622083)
--(axis cs:18.0272108843537,0.6161441831105)
--(axis cs:17.687074829932,0.616024845211554)
--(axis cs:17.3469387755102,0.614456574170327)
--(axis cs:17.0068027210884,0.618504541734235)
--(axis cs:16.6666666666667,0.614485387148587)
--(axis cs:16.3265306122449,0.616414254366343)
--(axis cs:15.9863945578231,0.61241323842971)
--(axis cs:15.6462585034014,0.607658272409213)
--(axis cs:15.3061224489796,0.602492086978104)
--(axis cs:14.9659863945578,0.598300613906711)
--(axis cs:14.6258503401361,0.593071223555839)
--(axis cs:14.2857142857143,0.585803324063731)
--(axis cs:13.9455782312925,0.585100351200357)
--(axis cs:13.6054421768707,0.580486944723014)
--(axis cs:13.265306122449,0.572333781779592)
--(axis cs:12.9251700680272,0.566886006662156)
--(axis cs:12.5850340136054,0.568887167737662)
--(axis cs:12.2448979591837,0.561666702407933)
--(axis cs:11.9047619047619,0.558609161407508)
--(axis cs:11.5646258503401,0.552808711571468)
--(axis cs:11.2244897959184,0.54774753766875)
--(axis cs:10.8843537414966,0.544839877790282)
--(axis cs:10.5442176870748,0.546893939383069)
--(axis cs:10.2040816326531,0.533173251133608)
--(axis cs:9.86394557823129,0.522203972007304)
--(axis cs:9.52380952380952,0.509678932960211)
--(axis cs:9.18367346938775,0.489023113370381)
--(axis cs:8.84353741496599,0.468295115200287)
--(axis cs:8.50340136054422,0.449689719316944)
--(axis cs:8.16326530612245,0.444826615042024)
--(axis cs:7.82312925170068,0.431807789297087)
--(axis cs:7.48299319727891,0.421448778532866)
--(axis cs:7.14285714285714,0.412324453320754)
--(axis cs:6.80272108843537,0.390467264360699)
--(axis cs:6.46258503401361,0.37505713176456)
--(axis cs:6.12244897959184,0.368548435790944)
--(axis cs:5.78231292517007,0.356955966976969)
--(axis cs:5.4421768707483,0.342979104868123)
--(axis cs:5.10204081632653,0.328285914572078)
--(axis cs:4.76190476190476,0.317746469180122)
--(axis cs:4.42176870748299,0.307863915412601)
--(axis cs:4.08163265306122,0.292895807631487)
--(axis cs:3.74149659863946,0.281113510601704)
--(axis cs:3.40136054421769,0.259327699337466)
--(axis cs:3.06122448979592,0.232636903223588)
--(axis cs:2.72108843537415,0.209923772476693)
--(axis cs:2.38095238095238,0.18654068423701)
--(axis cs:2.04081632653061,0.159207205885707)
--(axis cs:1.70068027210884,0.127599706768389)
--(axis cs:1.36054421768707,0.0935257731124362)
--(axis cs:1.02040816326531,0.0703403205720685)
--(axis cs:0.680272108843537,0.0647573944331384)
--(axis cs:0.340136054421769,0.0774990318044235)
--(axis cs:0,0.0838952831097947)
--cycle;


==> img/stl10/stl10_rate_accuracy_fw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.07640625
0.340136054421769 0.08609375
0.680272108843537 0.1315625
1.02040816326531 0.18328125
1.36054421768707 0.23859375
1.70068027210884 0.299375
2.04081632653061 0.35265625
2.38095238095238 0.39375
2.72108843537415 0.42859375
3.06122448979592 0.4709375
3.40136054421769 0.51296875
3.74149659863946 0.55140625
4.08163265306122 0.5871875
4.42176870748299 0.62375
4.76190476190476 0.6653125
5.10204081632653 0.69265625
5.4421768707483 0.71953125
5.78231292517007 0.75078125
6.12244897959184 0.760625
6.46258503401361 0.77859375
6.80272108843537 0.79234375
7.14285714285714 0.79953125
7.48299319727891 0.81
7.82312925170068 0.82546875
8.16326530612245 0.8309375
8.50340136054422 0.8396875
8.84353741496599 0.840625
9.18367346938775 0.8446875
9.52380952380952 0.85609375
9.86394557823129 0.855
10.2040816326531 0.85828125
10.5442176870748 0.85890625
10.8843537414966 0.8565625
11.2244897959184 0.86484375
11.5646258503401 0.859375
11.9047619047619 0.86359375
12.2448979591837 0.8628125
12.5850340136054 0.8678125
12.9251700680272 0.865
13.265306122449 0.86703125
13.6054421768707 0.86703125
13.9455782312925 0.86796875
14.2857142857143 0.87125
14.6258503401361 0.87421875
14.9659863945578 0.8775
15.3061224489796 0.88
15.6462585034014 0.88328125
15.9863945578231 0.8853125
16.3265306122449 0.8875
16.6666666666667 0.8903125
17.0068027210884 0.8915625
17.3469387755102 0.89375
17.687074829932 0.895625
18.0272108843537 0.8984375
18.3673469387755 0.89734375
18.7074829931973 0.89875
19.047619047619 0.898125
19.3877551020408 0.8996875
19.7278911564626 0.89765625
20.0680272108844 0.90140625
20.4081632653061 0.90203125
20.7482993197279 0.8984375
21.0884353741497 0.899375
21.4285714285714 0.89953125
21.7687074829932 0.900625
22.108843537415 0.90453125
22.4489795918367 0.90421875
22.7891156462585 0.9009375
23.1292517006803 0.9009375
23.469387755102 0.8984375
23.8095238095238 0.89578125
24.1496598639456 0.899375
24.4897959183673 0.89296875
24.8299319727891 0.89171875
25.1700680272109 0.89171875
25.5102040816327 0.89296875
25.8503401360544 0.8853125
26.1904761904762 0.88484375
26.530612244898 0.8828125
26.8707482993197 0.8815625
27.2108843537415 0.88265625
27.5510204081633 0.8778125
27.891156462585 0.87625
28.2312925170068 0.87203125
28.5714285714286 0.87078125
28.9115646258503 0.8759375
29.2517006802721 0.870625
29.5918367346939 0.87078125
29.9319727891156 0.8728125
30.2721088435374 0.87359375
30.6122448979592 0.8725
30.952380952381 0.87125
31.2925170068027 0.86609375
31.6326530612245 0.870625
31.9727891156463 0.865625
32.312925170068 0.86265625
32.6530612244898 0.8625
32.9931972789116 0.8671875
33.3333333333333 0.86671875
33.6734693877551 0.86640625
34.0136054421769 0.86921875
34.3537414965986 0.86828125
34.6938775510204 0.8665625
35.0340136054422 0.86203125
35.3741496598639 0.86453125
35.7142857142857 0.85859375
36.0544217687075 0.8603125
36.3945578231292 0.85890625
36.734693877551 0.856875
37.0748299319728 0.85515625
37.4149659863946 0.85640625
37.7551020408163 0.85875
38.0952380952381 0.8575
38.4353741496599 0.8565625
38.7755102040816 0.855625
39.1156462585034 0.85828125
39.4557823129252 0.8578125
39.7959183673469 0.85609375
40.1360544217687 0.85859375
40.4761904761905 0.85765625
40.8163265306122 0.8590625
41.156462585034 0.85859375
41.4965986394558 0.85703125
41.8367346938776 0.85875
42.1768707482993 0.8578125
42.5170068027211 0.85671875
42.8571428571429 0.8571875
43.1972789115646 0.8565625
43.5374149659864 0.856875
43.8775510204082 0.85625
44.2176870748299 0.85859375
44.5578231292517 0.85828125
44.8979591836735 0.855
45.2380952380952 0.85765625
45.578231292517 0.85796875
45.9183673469388 0.86078125
46.2585034013605 0.86078125
46.5986394557823 0.858125
46.9387755102041 0.86046875
47.2789115646259 0.85890625
47.6190476190476 0.8609375
47.9591836734694 0.8628125
48.2993197278912 0.86296875
48.6394557823129 0.86375
48.9795918367347 0.86328125
49.3197278911565 0.8621875
49.6598639455782 0.863125
50 0.86359375
50.3401360544218 0.8634375
50.6802721088435 0.8615625
51.0204081632653 0.86609375
51.3605442176871 0.8684375
51.7006802721088 0.86625
52.0408163265306 0.8684375
52.3809523809524 0.86921875
52.7210884353741 0.87046875
53.0612244897959 0.87234375
53.4013605442177 0.8715625
53.7414965986395 0.87140625
54.0816326530612 0.87171875
54.421768707483 0.8721875
54.7619047619048 0.8690625
55.1020408163265 0.87421875
55.4421768707483 0.870625
55.7823129251701 0.87203125
56.1224489795918 0.8675
56.4625850340136 0.8678125
56.8027210884354 0.86734375
57.1428571428571 0.866875
57.4829931972789 0.865625
57.8231292517007 0.86546875
58.1632653061224 0.86421875
58.5034013605442 0.86421875
58.843537414966 0.86265625
59.1836734693878 0.86515625
59.5238095238095 0.86125
59.8639455782313 0.8653125
60.2040816326531 0.86484375
60.5442176870748 0.86453125
60.8843537414966 0.8615625
61.2244897959184 0.868125
61.5646258503401 0.8665625
61.9047619047619 0.86875
62.2448979591837 0.8646875
62.5850340136054 0.87015625
62.9251700680272 0.87078125
63.265306122449 0.8715625
63.6054421768707 0.86890625
63.9455782312925 0.87328125
64.2857142857143 0.87140625
64.6258503401361 0.8728125
64.9659863945578 0.86921875
65.3061224489796 0.87203125
65.6462585034014 0.87140625
65.9863945578231 0.8696875
66.3265306122449 0.8715625
66.6666666666667 0.8709375
67.0068027210884 0.87078125
67.3469387755102 0.87046875
67.687074829932 0.8715625
68.0272108843537 0.8721875
68.3673469387755 0.86953125
68.7074829931973 0.87453125
69.0476190476191 0.87375
69.3877551020408 0.87671875
69.7278911564626 0.87390625
70.0680272108844 0.876875
70.4081632653061 0.87625
70.7482993197279 0.8746875
71.0884353741497 0.87390625
71.4285714285714 0.87140625
71.7687074829932 0.87328125
72.108843537415 0.8721875
72.4489795918367 0.8721875
72.7891156462585 0.8675
73.1292517006803 0.86625
73.469387755102 0.86328125
73.8095238095238 0.8678125
74.1496598639456 0.869375
74.4897959183673 0.8690625
74.8299319727891 0.86890625
75.1700680272109 0.87171875
75.5102040816327 0.871875
75.8503401360544 0.873125
76.1904761904762 0.87625
76.530612244898 0.885
76.8707482993197 0.890625
77.2108843537415 0.89328125
77.5510204081633 0.893125
77.891156462585 0.8965625
78.2312925170068 0.89515625
78.5714285714286 0.890625
78.9115646258503 0.8909375
79.2517006802721 0.89484375
79.5918367346939 0.9040625
79.9319727891156 0.90765625
80.2721088435374 0.9115625
80.6122448979592 0.91796875
80.9523809523809 0.9209375
81.2925170068027 0.92328125
81.6326530612245 0.9228125
81.9727891156463 0.926875
82.312925170068 0.9309375
82.6530612244898 0.93171875
82.9931972789116 0.93078125
83.3333333333333 0.9371875
83.6734693877551 0.94078125
84.0136054421769 0.93625
84.3537414965986 0.9396875
84.6938775510204 0.94078125
85.0340136054422 0.9465625
85.3741496598639 0.94921875
85.7142857142857 0.9503125
86.0544217687075 0.95
86.3945578231292 0.95109375
86.734693877551 0.95203125
87.0748299319728 0.95234375
87.4149659863945 0.9525
87.7551020408163 0.94984375
88.0952380952381 0.9528125
88.4353741496599 0.9515625
88.7755102040816 0.95078125
89.1156462585034 0.95015625
89.4557823129252 0.94703125
89.7959183673469 0.94640625
90.1360544217687 0.94796875
90.4761904761905 0.94578125
90.8163265306122 0.94796875
91.156462585034 0.9465625
91.4965986394558 0.944375
91.8367346938775 0.94125
92.1768707482993 0.9428125
92.5170068027211 0.9421875
92.8571428571429 0.94265625
93.1972789115646 0.94234375
93.5374149659864 0.94140625
93.8775510204082 0.94328125
94.2176870748299 0.9465625
94.5578231292517 0.9440625
94.8979591836735 0.9465625
95.2380952380952 0.94953125
95.578231292517 0.9515625
95.9183673469388 0.95234375
96.2585034013605 0.95609375
96.5986394557823 0.9571875
96.9387755102041 0.95921875
97.2789115646258 0.95984375
97.6190476190476 0.96
97.9591836734694 0.9615625
98.2993197278912 0.9621875
98.6394557823129 0.96234375
98.9795918367347 0.963125
99.3197278911565 0.9653125
99.6598639455782 0.965
100 0.98
};
\path [fill=color0, fill opacity=0.25]
(axis cs:0,0.0826294898306073)
--(axis cs:0,0.0701830101693926)
--(axis cs:0.340136054421769,0.0776246387516508)
--(axis cs:0.680272108843537,0.120256284657495)
--(axis cs:1.02040816326531,0.168452605856526)
--(axis cs:1.36054421768707,0.222274049440775)
--(axis cs:1.70068027210884,0.282953643487609)
--(axis cs:2.04081632653061,0.336934806917922)
--(axis cs:2.38095238095238,0.37867863149274)
--(axis cs:2.72108843537415,0.414526164656471)
--(axis cs:3.06122448979592,0.454728915833467)
--(axis cs:3.40136054421769,0.497344055178762)
--(axis cs:3.74149659863946,0.534094630955824)
--(axis cs:4.08163265306122,0.568712651209231)
--(axis cs:4.42176870748299,0.603433744337585)
--(axis cs:4.76190476190476,0.644467064875557)
--(axis cs:5.10204081632653,0.672654829075744)
--(axis cs:5.4421768707483,0.700721581352106)
--(axis cs:5.78231292517007,0.7328802973143)
--(axis cs:6.12244897959184,0.742705676844981)
--(axis cs:6.46258503401361,0.760964430019535)
--(axis cs:6.80272108843537,0.774713889068615)
--(axis cs:7.14285714285714,0.782555627237094)
--(axis cs:7.48299319727891,0.793226988244807)
--(axis cs:7.82312925170068,0.80883877660812)
--(axis cs:8.16326530612245,0.8155914798093)
--(axis cs:8.50340136054422,0.824474423943348)
--(axis cs:8.84353741496599,0.825587205816469)
--(axis cs:9.18367346938775,0.830043620500799)
--(axis cs:9.52380952380952,0.841921476090062)
--(axis cs:9.86394557823129,0.841288422602183)
--(axis cs:10.2040816326531,0.844251679722793)
--(axis cs:10.5442176870748,0.845713255666366)
--(axis cs:10.8843537414966,0.843380714823127)
--(axis cs:11.2244897959184,0.851668115828719)
--(axis cs:11.5646258503401,0.847212973586831)
--(axis cs:11.9047619047619,0.851258486031093)
--(axis cs:12.2448979591837,0.850368319211453)
--(axis cs:12.5850340136054,0.854518331191217)
--(axis cs:12.9251700680272,0.852403479338973)
--(axis cs:13.265306122449,0.854033426907214)
--(axis cs:13.6054421768707,0.854328803086402)
--(axis cs:13.9455782312925,0.855588725792041)
--(axis cs:14.2857142857143,0.858696707840452)
--(axis cs:14.6258503401361,0.862318703813402)
--(axis cs:14.9659863945578,0.865908898339877)
--(axis cs:15.3061224489796,0.867977567658975)
--(axis cs:15.6462585034014,0.8719619680259)
--(axis cs:15.9863945578231,0.873964188245052)
--(axis cs:16.3265306122449,0.877700254918514)
--(axis cs:16.6666666666667,0.880498168338749)
--(axis cs:17.0068027210884,0.882171238062366)
--(axis cs:17.3469387755102,0.884796460865272)
--(axis cs:17.687074829932,0.887586282958103)
--(axis cs:18.0272108843537,0.890860482522941)
--(axis cs:18.3673469387755,0.889461372077452)
--(axis cs:18.7074829931973,0.889810318366136)
--(axis cs:19.047619047619,0.890115996658667)
--(axis cs:19.3877551020408,0.89059759665764)
--(axis cs:19.7278911564626,0.888484357531693)
--(axis cs:20.0680272108844,0.892437279680679)
--(axis cs:20.4081632653061,0.894265889285496)
--(axis cs:20.7482993197279,0.890098319515543)
--(axis cs:21.0884353741497,0.889993898469904)
--(axis cs:21.4285714285714,0.890950271386245)
--(axis cs:21.7687074829932,0.890239405881918)
--(axis cs:22.108843537415,0.895497650979959)
--(axis cs:22.4489795918367,0.895018826327433)
--(axis cs:22.7891156462585,0.890549151447678)
--(axis cs:23.1292517006803,0.890129816146674)
--(axis cs:23.469387755102,0.886935600105988)
--(axis cs:23.8095238095238,0.884284740811958)
--(axis cs:24.1496598639456,0.887324836041945)
--(axis cs:24.4897959183673,0.88099440519656)
--(axis cs:24.8299319727891,0.878864798260656)
--(axis cs:25.1700680272109,0.878575727937679)
--(axis cs:25.5102040816327,0.879542169793921)
--(axis cs:25.8503401360544,0.872060003551807)
--(axis cs:26.1904761904762,0.871247067822522)
--(axis cs:26.530612244898,0.869463208529526)
--(axis cs:26.8707482993197,0.868668916059298)
--(axis cs:27.2108843537415,0.869695900569964)
--(axis cs:27.5510204081633,0.865203115319087)
--(axis cs:27.891156462585,0.862950810599111)
--(axis cs:28.2312925170068,0.858614617515592)
--(axis cs:28.5714285714286,0.857740209364961)
--(axis cs:28.9115646258503,0.862754991364101)
--(axis cs:29.2517006802721,0.857405647453892)
--(axis cs:29.5918367346939,0.857150242441297)
--(axis cs:29.9319727891156,0.859590262077334)
--(axis cs:30.2721088435374,0.860392806555044)
--(axis cs:30.6122448979592,0.859628624694847)
--(axis cs:30.952380952381,0.85829664293596)
--(axis cs:31.2925170068027,0.8533231648588)
--(axis cs:31.6326530612245,0.858300951491865)
--(axis cs:31.9727891156463,0.853358348719289)
--(axis cs:32.312925170068,0.850467200744503)
--(axis cs:32.6530612244898,0.850868652763958)
--(axis cs:32.9931972789116,0.855089944023866)
--(axis cs:33.3333333333333,0.855053425820707)
--(axis cs:33.6734693877551,0.854197656349987)
--(axis cs:34.0136054421769,0.857110556383232)
--(axis cs:34.3537414965986,0.856353187656742)
--(axis cs:34.6938775510204,0.854291184888711)
--(axis cs:35.0340136054422,0.849911247732836)
--(axis cs:35.3741496598639,0.852366479403036)
--(axis cs:35.7142857142857,0.84592965075094)
--(axis cs:36.0544217687075,0.847621695511919)
--(axis cs:36.3945578231292,0.846391381523528)
--(axis cs:36.734693877551,0.845529209625217)
--(axis cs:37.0748299319728,0.843911354375215)
--(axis cs:37.4149659863946,0.845910588025256)
--(axis cs:37.7551020408163,0.849028419636918)
--(axis cs:38.0952380952381,0.849393942980685)
--(axis cs:38.4353741496599,0.849024601368983)
--(axis cs:38.7755102040816,0.847101449717176)
--(axis cs:39.1156462585034,0.850920663208511)
--(axis cs:39.4557823129252,0.850283462786173)
--(axis cs:39.7959183673469,0.849202926811594)
--(axis cs:40.1360544217687,0.851902336908935)
--(axis cs:40.4761904761905,0.850177413281818)
--(axis cs:40.8163265306122,0.85209118425876)
--(axis cs:41.156462585034,0.852250602562869)
--(axis cs:41.4965986394558,0.849612588072145)
--(axis cs:41.8367346938776,0.850543388017908)
--(axis cs:42.1768707482993,0.850084687522115)
--(axis cs:42.5170068027211,0.848519695020097)
--(axis cs:42.8571428571429,0.84812807332554)
--(axis cs:43.1972789115646,0.847345488114065)
--(axis cs:43.5374149659864,0.84769219634008)
--(axis cs:43.8775510204082,0.846749698041394)
--(axis cs:44.2176870748299,0.848098088025256)
--(axis cs:44.5578231292517,0.847809239226345)
--(axis cs:44.8979591836735,0.844794104211884)
--(axis cs:45.2380952380952,0.84789697472058)
--(axis cs:45.578231292517,0.847861917853859)
--(axis cs:45.9183673469388,0.851003425588623)
--(axis cs:46.2585034013605,0.850924739328758)
--(axis cs:46.5986394557823,0.848064984172128)
--(axis cs:46.9387755102041,0.850699707629185)
--(axis cs:47.2789115646259,0.849348401771002)
--(axis cs:47.6190476190476,0.85183606323853)
--(axis cs:47.9591836734694,0.853470108794452)
--(axis cs:48.2993197278912,0.853758466049744)
--(axis cs:48.6394557823129,0.854921961421883)
--(axis cs:48.9795918367347,0.85499772013252)
--(axis cs:49.3197278911565,0.854147596694237)
--(axis cs:49.6598639455782,0.853921448903646)
--(axis cs:50,0.854705958169183)
--(axis cs:50.3401360544218,0.855622558975101)
--(axis cs:50.6802721088435,0.853123282148255)
--(axis cs:51.0204081632653,0.857899348946954)
--(axis cs:51.3605442176871,0.860048151720736)
--(axis cs:51.7006802721088,0.85747396799271)
--(axis cs:52.0408163265306,0.860094889400713)
--(axis cs:52.3809523809524,0.860386931255321)
--(axis cs:52.7210884353741,0.862140440865954)
--(axis cs:53.0612244897959,0.864293770509355)
--(axis cs:53.4013605442177,0.863772003642508)
--(axis cs:53.7414965986395,0.863372873313251)
--(axis cs:54.0816326530612,0.863870321870962)
--(axis cs:54.421768707483,0.864406803012874)
--(axis cs:54.7619047619048,0.860242026615174)
--(axis cs:55.1020408163265,0.867330695322429)
--(axis cs:55.4421768707483,0.862447491634587)
--(axis cs:55.7823129251701,0.86431640625)
--(axis cs:56.1224489795918,0.858819023990217)
--(axis cs:56.4625850340136,0.859193263998587)
--(axis cs:56.8027210884354,0.858554144982022)
--(axis cs:57.1428571428571,0.857937452196369)
--(axis cs:57.4829931972789,0.856595096675338)
--(axis cs:57.8231292517007,0.856337498963948)
--(axis cs:58.1632653061224,0.855049977399962)
--(axis cs:58.5034013605442,0.855093767558076)
--(axis cs:58.843537414966,0.852868677007526)
--(axis cs:59.1836734693878,0.855242817783776)
--(axis cs:59.5238095238095,0.85021009159292)
--(axis cs:59.8639455782313,0.855973171706246)
--(axis cs:60.2040816326531,0.855056177007526)
--(axis cs:60.5442176870748,0.854071084880783)
--(axis cs:60.8843537414966,0.851257104720099)
--(axis cs:61.2244897959184,0.857760547530139)
--(axis cs:61.5646258503401,0.856031913619759)
--(axis cs:61.9047619047619,0.858228473749097)
--(axis cs:62.2448979591837,0.854393215661637)
--(axis cs:62.5850340136054,0.860267861472989)
--(axis cs:62.9251700680272,0.860475392024161)
--(axis cs:63.265306122449,0.861377182521459)
--(axis cs:63.6054421768707,0.858636544909231)
--(axis cs:63.9455782312925,0.863054351042825)
--(axis cs:64.2857142857143,0.861463040438604)
--(axis cs:64.6258503401361,0.862576745977927)
--(axis cs:64.9659863945578,0.858946259400815)
--(axis cs:65.3061224489796,0.862808549078888)
--(axis cs:65.6462585034014,0.861628425588623)
--(axis cs:65.9863945578231,0.860026932283581)
--(axis cs:66.3265306122449,0.861818383059948)
--(axis cs:66.6666666666667,0.861171875)
--(axis cs:67.0068027210884,0.861198489441228)
--(axis cs:67.3469387755102,0.860984020258642)
--(axis cs:67.687074829932,0.862699959918329)
--(axis cs:68.0272108843537,0.863925296445962)
--(axis cs:68.3673469387755,0.861056510312638)
--(axis cs:68.7074829931973,0.86755788256428)
--(axis cs:69.0476190476191,0.865927740470898)
--(axis cs:69.3877551020408,0.870577266529871)
--(axis cs:69.7278911564626,0.86696578245655)
--(axis cs:70.0680272108844,0.871945535365577)
--(axis cs:70.4081632653061,0.870327488593728)
--(axis cs:70.7482993197279,0.868283751441111)
--(axis cs:71.0884353741497,0.866831056372391)
--(axis cs:71.4285714285714,0.863642117495976)
--(axis cs:71.7687074829932,0.865730078741319)
--(axis cs:72.108843537415,0.86443750590663)
--(axis cs:72.4489795918367,0.863642717635067)
--(axis cs:72.7891156462585,0.85847537886551)
--(axis cs:73.1292517006803,0.856698639620063)
--(axis cs:73.469387755102,0.852334598555086)
--(axis cs:73.8095238095238,0.857983603406183)
--(axis cs:74.1496598639456,0.860059187486163)
--(axis cs:74.4897959183673,0.860667469804556)
--(axis cs:74.8299319727891,0.860032418341372)
--(axis cs:75.1700680272109,0.862905307252056)
--(axis cs:75.5102040816327,0.863050202853451)
--(axis cs:75.8503401360544,0.864281850451038)
--(axis cs:76.1904761904762,0.866475589889023)
--(axis cs:76.530612244898,0.874058141214508)
--(axis cs:76.8707482993197,0.879626634198984)
--(axis cs:77.2108843537415,0.882852129433714)
--(axis cs:77.5510204081633,0.8835546875)
--(axis cs:77.891156462585,0.887357912759416)
--(axis cs:78.2312925170068,0.885019267826159)
--(axis cs:78.5714285714286,0.881782928949676)
--(axis cs:78.9115646258503,0.881606344386257)
--(axis cs:79.2517006802721,0.884623380736809)
--(axis cs:79.5918367346939,0.893314987115471)
--(axis cs:79.9319727891156,0.897058409453777)
--(axis cs:80.2721088435374,0.900558066134632)
--(axis cs:80.6122448979592,0.907488546231919)
--(axis cs:80.9523809523809,0.910674761987953)
--(axis cs:81.2925170068027,0.913109518260177)
--(axis cs:81.6326530612245,0.91249693020359)
--(axis cs:81.9727891156463,0.917170110743121)
--(axis cs:82.312925170068,0.92199141992922)
--(axis cs:82.6530612244898,0.923258652042749)
--(axis cs:82.9931972789116,0.921504934267483)
--(axis cs:83.3333333333333,0.927879880814497)
--(axis cs:83.6734693877551,0.93167300490096)
--(axis cs:84.0136054421769,0.925887387972748)
--(axis cs:84.3537414965986,0.930527572797373)
--(axis cs:84.6938775510204,0.931345917603284)
--(axis cs:85.0340136054422,0.938125542552166)
--(axis cs:85.3741496598639,0.94110975227425)
--(axis cs:85.7142857142857,0.94246954179482)
--(axis cs:86.0544217687075,0.942174083785293)
--(axis cs:86.3945578231292,0.943677659532163)
--(axis cs:86.734693877551,0.944734426233116)
--(axis cs:87.0748299319728,0.94518947152055)
--(axis cs:87.4149659863945,0.945565718564032)
--(axis cs:87.7551020408163,0.941904711294257)
--(axis cs:88.0952380952381,0.945938998298919)
--(axis cs:88.4353741496599,0.944304334306226)
--(axis cs:88.7755102040816,0.943335641360493)
--(axis cs:89.1156462585034,0.942482307790282)
--(axis cs:89.4557823129252,0.938662958355123)
--(axis cs:89.7959183673469,0.937984566147519)
--(axis cs:90.1360544217687,0.939762719078693)
--(axis cs:90.4761904761905,0.937491965682457)
--(axis cs:90.8163265306122,0.940100904050953)
--(axis cs:91.156462585034,0.938583321009447)
--(axis cs:91.4965986394558,0.936061016932112)
--(axis cs:91.8367346938775,0.933811439397445)
--(axis cs:92.1768707482993,0.93490174095661)
--(axis cs:92.5170068027211,0.935264229736419)
--(axis cs:92.8571428571429,0.935079861869466)
--(axis cs:93.1972789115646,0.93462890625)
--(axis cs:93.5374149659864,0.93535077500081)
--(axis cs:93.8775510204082,0.936373839048724)
--(axis cs:94.2176870748299,0.939943451873894)
--(axis cs:94.5578231292517,0.937306550563895)
--(axis cs:94.8979591836735,0.940294216196921)
--(axis cs:95.2380952380952,0.943091118322735)
--(axis cs:95.578231292517,0.945307924038435)
--(axis cs:95.9183673469388,0.945690929167871)
--(axis cs:96.2585034013605,0.951009056231662)
--(axis cs:96.5986394557823,0.952740118149713)
--(axis cs:96.9387755102041,0.95560546875)
--(axis cs:97.2789115646258,0.957937576045318)
--(axis cs:97.6190476190476,0.957318451129346)
--(axis cs:97.9591836734694,0.957890313344343)
--(axis cs:98.2993197278912,0.958286135868078)
--(axis cs:98.6394557823129,0.958323205302688)
--(axis cs:98.9795918367347,0.958586347641163)
--(axis cs:99.3197278911565,0.959791682021444)
--(axis cs:99.6598639455782,0.958239817070361)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:99.6598639455782,0.971760182929639)
--(axis cs:99.3197278911565,0.970833317978556)
--(axis cs:98.9795918367347,0.967663652358837)
--(axis cs:98.6394557823129,0.966364294697312)
--(axis cs:98.2993197278912,0.966088864131922)
--(axis cs:97.9591836734694,0.965234686655657)
--(axis cs:97.6190476190476,0.962681548870653)
--(axis cs:97.2789115646258,0.961749923954682)
--(axis cs:96.9387755102041,0.96283203125)
--(axis cs:96.5986394557823,0.961634881850287)
--(axis cs:96.2585034013605,0.961178443768338)
--(axis cs:95.9183673469388,0.958996570832129)
--(axis cs:95.578231292517,0.957817075961565)
--(axis cs:95.2380952380952,0.955971381677265)
--(axis cs:94.8979591836735,0.952830783803079)
--(axis cs:94.5578231292517,0.950818449436105)
--(axis cs:94.2176870748299,0.953181548126106)
--(axis cs:93.8775510204082,0.950188660951276)
--(axis cs:93.5374149659864,0.94746172499919)
--(axis cs:93.1972789115646,0.95005859375)
--(axis cs:92.8571428571429,0.950232638130534)
--(axis cs:92.5170068027211,0.94911077026358)
--(axis cs:92.1768707482993,0.95072325904339)
--(axis cs:91.8367346938775,0.948688560602555)
--(axis cs:91.4965986394558,0.952688983067888)
--(axis cs:91.156462585034,0.954541678990553)
--(axis cs:90.8163265306122,0.955836595949047)
--(axis cs:90.4761904761905,0.954070534317543)
--(axis cs:90.1360544217687,0.956174780921307)
--(axis cs:89.7959183673469,0.954827933852481)
--(axis cs:89.4557823129252,0.955399541644877)
--(axis cs:89.1156462585034,0.957830192209718)
--(axis cs:88.7755102040816,0.958226858639507)
--(axis cs:88.4353741496599,0.958820665693774)
--(axis cs:88.0952380952381,0.959686001701081)
--(axis cs:87.7551020408163,0.957782788705743)
--(axis cs:87.4149659863945,0.959434281435968)
--(axis cs:87.0748299319728,0.95949802847945)
--(axis cs:86.734693877551,0.959328073766884)
--(axis cs:86.3945578231292,0.958509840467837)
--(axis cs:86.0544217687075,0.957825916214707)
--(axis cs:85.7142857142857,0.95815545820518)
--(axis cs:85.3741496598639,0.95732774772575)
--(axis cs:85.0340136054422,0.954999457447834)
--(axis cs:84.6938775510204,0.950216582396716)
--(axis cs:84.3537414965986,0.948847427202627)
--(axis cs:84.0136054421769,0.946612612027252)
--(axis cs:83.6734693877551,0.94988949509904)
--(axis cs:83.3333333333333,0.946495119185503)
--(axis cs:82.9931972789116,0.940057565732517)
--(axis cs:82.6530612244898,0.940178847957251)
--(axis cs:82.312925170068,0.93988358007078)
--(axis cs:81.9727891156463,0.936579889256879)
--(axis cs:81.6326530612245,0.93312806979641)
--(axis cs:81.2925170068027,0.933452981739823)
--(axis cs:80.9523809523809,0.931200238012047)
--(axis cs:80.6122448979592,0.928448953768081)
--(axis cs:80.2721088435374,0.922566933865368)
--(axis cs:79.9319727891156,0.918254090546223)
--(axis cs:79.5918367346939,0.914810012884529)
--(axis cs:79.2517006802721,0.905064119263191)
--(axis cs:78.9115646258503,0.900268655613743)
--(axis cs:78.5714285714286,0.899467071050324)
--(axis cs:78.2312925170068,0.905293232173841)
--(axis cs:77.891156462585,0.905767087240585)
--(axis cs:77.5510204081633,0.9026953125)
--(axis cs:77.2108843537415,0.903710370566286)
--(axis cs:76.8707482993197,0.901623365801016)
--(axis cs:76.530612244898,0.895941858785492)
--(axis cs:76.1904761904762,0.886024410110977)
--(axis cs:75.8503401360544,0.881968149548962)
--(axis cs:75.5102040816327,0.880699797146549)
--(axis cs:75.1700680272109,0.880532192747944)
--(axis cs:74.8299319727891,0.877780081658628)
--(axis cs:74.4897959183673,0.877457530195444)
--(axis cs:74.1496598639456,0.878690812513837)
--(axis cs:73.8095238095238,0.877641396593817)
--(axis cs:73.469387755102,0.874227901444914)
--(axis cs:73.1292517006803,0.875801360379936)
--(axis cs:72.7891156462585,0.876524621134491)
--(axis cs:72.4489795918367,0.880732282364933)
--(axis cs:72.108843537415,0.87993749409337)
--(axis cs:71.7687074829932,0.880832421258681)
--(axis cs:71.4285714285714,0.879170382504024)
--(axis cs:71.0884353741497,0.880981443627609)
--(axis cs:70.7482993197279,0.881091248558889)
--(axis cs:70.4081632653061,0.882172511406272)
--(axis cs:70.0680272108844,0.881804464634423)
--(axis cs:69.7278911564626,0.88084671754345)
--(axis cs:69.3877551020408,0.882860233470129)
--(axis cs:69.0476190476191,0.881572259529102)
--(axis cs:68.7074829931973,0.88150461743572)
--(axis cs:68.3673469387755,0.878005989687362)
--(axis cs:68.0272108843537,0.880449703554038)
--(axis cs:67.687074829932,0.880425040081671)
--(axis cs:67.3469387755102,0.879953479741358)
--(axis cs:67.0068027210884,0.880364010558772)
--(axis cs:66.6666666666667,0.880703125)
--(axis cs:66.3265306122449,0.881306616940052)
--(axis cs:65.9863945578231,0.879348067716419)
--(axis cs:65.6462585034014,0.881184074411377)
--(axis cs:65.3061224489796,0.881253950921112)
--(axis cs:64.9659863945578,0.879491240599185)
--(axis cs:64.6258503401361,0.883048254022073)
--(axis cs:64.2857142857143,0.881349459561396)
--(axis cs:63.9455782312925,0.883508148957175)
--(axis cs:63.6054421768707,0.879175955090769)
--(axis cs:63.265306122449,0.881747817478541)
--(axis cs:62.9251700680272,0.881087107975839)
--(axis cs:62.5850340136054,0.880044638527011)
--(axis cs:62.2448979591837,0.874981784338363)
--(axis cs:61.9047619047619,0.879271526250903)
--(axis cs:61.5646258503401,0.877093086380241)
--(axis cs:61.2244897959184,0.878489452469861)
--(axis cs:60.8843537414966,0.871867895279901)
--(axis cs:60.5442176870748,0.874991415119217)
--(axis cs:60.2040816326531,0.874631322992474)
--(axis cs:59.8639455782313,0.874651828293754)
--(axis cs:59.5238095238095,0.87228990840708)
--(axis cs:59.1836734693878,0.875069682216224)
--(axis cs:58.843537414966,0.872443822992474)
--(axis cs:58.5034013605442,0.873343732441925)
--(axis cs:58.1632653061224,0.873387522600038)
--(axis cs:57.8231292517007,0.874600001036052)
--(axis cs:57.4829931972789,0.874654903324662)
--(axis cs:57.1428571428571,0.875812547803631)
--(axis cs:56.8027210884354,0.876133355017978)
--(axis cs:56.4625850340136,0.876431736001413)
--(axis cs:56.1224489795918,0.876180976009783)
--(axis cs:55.7823129251701,0.87974609375)
--(axis cs:55.4421768707483,0.878802508365413)
--(axis cs:55.1020408163265,0.881106804677571)
--(axis cs:54.7619047619048,0.877882973384826)
--(axis cs:54.421768707483,0.879968196987126)
--(axis cs:54.0816326530612,0.879567178129038)
--(axis cs:53.7414965986395,0.87943962668675)
--(axis cs:53.4013605442177,0.879352996357492)
--(axis cs:53.0612244897959,0.880393729490645)
--(axis cs:52.7210884353741,0.878797059134046)
--(axis cs:52.3809523809524,0.878050568744679)
--(axis cs:52.0408163265306,0.876780110599287)
--(axis cs:51.7006802721088,0.875026032007289)
--(axis cs:51.3605442176871,0.876826848279263)
--(axis cs:51.0204081632653,0.874288151053046)
--(axis cs:50.6802721088435,0.870001717851745)
--(axis cs:50.3401360544218,0.871252441024899)
--(axis cs:50,0.872481541830817)
--(axis cs:49.6598639455782,0.872328551096354)
--(axis cs:49.3197278911565,0.870227403305763)
--(axis cs:48.9795918367347,0.87156477986748)
--(axis cs:48.6394557823129,0.872578038578117)
--(axis cs:48.2993197278912,0.872179033950256)
--(axis cs:47.9591836734694,0.872154891205548)
--(axis cs:47.6190476190476,0.87003893676147)
--(axis cs:47.2789115646259,0.868464098228998)
--(axis cs:46.9387755102041,0.870237792370815)
--(axis cs:46.5986394557823,0.868185015827872)
--(axis cs:46.2585034013605,0.870637760671242)
--(axis cs:45.9183673469388,0.870559074411377)
--(axis cs:45.578231292517,0.868075582146141)
--(axis cs:45.2380952380952,0.86741552527942)
--(axis cs:44.8979591836735,0.865205895788116)
--(axis cs:44.5578231292517,0.868753260773655)
--(axis cs:44.2176870748299,0.869089411974744)
--(axis cs:43.8775510204082,0.865750301958606)
--(axis cs:43.5374149659864,0.86605780365992)
--(axis cs:43.1972789115646,0.865779511885935)
--(axis cs:42.8571428571429,0.86624692667446)
--(axis cs:42.5170068027211,0.864917804979903)
--(axis cs:42.1768707482993,0.865540312477885)
--(axis cs:41.8367346938776,0.866956611982092)
--(axis cs:41.4965986394558,0.864449911927855)
--(axis cs:41.156462585034,0.864936897437131)
--(axis cs:40.8163265306122,0.86603381574124)
--(axis cs:40.4761904761905,0.865135086718182)
--(axis cs:40.1360544217687,0.865285163091065)
--(axis cs:39.7959183673469,0.862984573188405)
--(axis cs:39.4557823129252,0.865341537213827)
--(axis cs:39.1156462585034,0.865641836791489)
--(axis cs:38.7755102040816,0.864148550282824)
--(axis cs:38.4353741496599,0.864100398631017)
--(axis cs:38.0952380952381,0.865606057019315)
--(axis cs:37.7551020408163,0.868471580363082)
--(axis cs:37.4149659863946,0.866901911974744)
--(axis cs:37.0748299319728,0.866401145624785)
--(axis cs:36.734693877551,0.868220790374783)
--(axis cs:36.3945578231292,0.871421118476472)
--(axis cs:36.0544217687075,0.873003304488081)
--(axis cs:35.7142857142857,0.87125784924906)
--(axis cs:35.3741496598639,0.876696020596964)
--(axis cs:35.0340136054422,0.874151252267164)
--(axis cs:34.6938775510204,0.878833815111289)
--(axis cs:34.3537414965986,0.880209312343258)
--(axis cs:34.0136054421769,0.881326943616768)
--(axis cs:33.6734693877551,0.878614843650013)
--(axis cs:33.3333333333333,0.878384074179293)
--(axis cs:32.9931972789116,0.879285055976134)
--(axis cs:32.6530612244898,0.874131347236042)
--(axis cs:32.312925170068,0.874845299255497)
--(axis cs:31.9727891156463,0.877891651280711)
--(axis cs:31.6326530612245,0.882949048508135)
--(axis cs:31.2925170068027,0.8788643351412)
--(axis cs:30.952380952381,0.88420335706404)
--(axis cs:30.6122448979592,0.885371375305153)
--(axis cs:30.2721088435374,0.886794693444955)
--(axis cs:29.9319727891156,0.886034737922666)
--(axis cs:29.5918367346939,0.884412257558703)
--(axis cs:29.2517006802721,0.883844352546108)
--(axis cs:28.9115646258503,0.889120008635899)
--(axis cs:28.5714285714286,0.883822290635038)
--(axis cs:28.2312925170068,0.885447882484408)
--(axis cs:27.891156462585,0.889549189400888)
--(axis cs:27.5510204081633,0.890421884680913)
--(axis cs:27.2108843537415,0.895616599430036)
--(axis cs:26.8707482993197,0.894456083940702)
--(axis cs:26.530612244898,0.896161791470474)
--(axis cs:26.1904761904762,0.898440432177478)
--(axis cs:25.8503401360544,0.898564996448193)
--(axis cs:25.5102040816327,0.906395330206079)
--(axis cs:25.1700680272109,0.904861772062321)
--(axis cs:24.8299319727891,0.904572701739344)
--(axis cs:24.4897959183673,0.90494309480344)
--(axis cs:24.1496598639456,0.911425163958055)
--(axis cs:23.8095238095238,0.907277759188042)
--(axis cs:23.469387755102,0.909939399894012)
--(axis cs:23.1292517006803,0.911745183853326)
--(axis cs:22.7891156462585,0.911325848552322)
--(axis cs:22.4489795918367,0.913418673672567)
--(axis cs:22.108843537415,0.913564849020041)
--(axis cs:21.7687074829932,0.911010594118082)
--(axis cs:21.4285714285714,0.908112228613755)
--(axis cs:21.0884353741497,0.908756101530096)
--(axis cs:20.7482993197279,0.906776680484457)
--(axis cs:20.4081632653061,0.909796610714504)
--(axis cs:20.0680272108844,0.910375220319321)
--(axis cs:19.7278911564626,0.906828142468308)
--(axis cs:19.3877551020408,0.908777403342359)
--(axis cs:19.047619047619,0.906134003341333)
--(axis cs:18.7074829931973,0.907689681633864)
--(axis cs:18.3673469387755,0.905226127922548)
--(axis cs:18.0272108843537,0.906014517477059)
--(axis cs:17.687074829932,0.903663717041897)
--(axis cs:17.3469387755102,0.902703539134728)
--(axis cs:17.0068027210884,0.900953761937634)
--(axis cs:16.6666666666667,0.900126831661251)
--(axis cs:16.3265306122449,0.897299745081486)
--(axis cs:15.9863945578231,0.896660811754948)
--(axis cs:15.6462585034014,0.8946005319741)
--(axis cs:15.3061224489796,0.892022432341025)
--(axis cs:14.9659863945578,0.889091101660123)
--(axis cs:14.6258503401361,0.886118796186598)
--(axis cs:14.2857142857143,0.883803292159548)
--(axis cs:13.9455782312925,0.880348774207959)
--(axis cs:13.6054421768707,0.879733696913598)
--(axis cs:13.265306122449,0.880029073092786)
--(axis cs:12.9251700680272,0.877596520661027)
--(axis cs:12.5850340136054,0.881106668808783)
--(axis cs:12.2448979591837,0.875256680788547)
--(axis cs:11.9047619047619,0.875929013968907)
--(axis cs:11.5646258503401,0.871537026413169)
--(axis cs:11.2244897959184,0.878019384171281)
--(axis cs:10.8843537414966,0.869744285176873)
--(axis cs:10.5442176870748,0.872099244333634)
--(axis cs:10.2040816326531,0.872310820277207)
--(axis cs:9.86394557823129,0.868711577397817)
--(axis cs:9.52380952380952,0.870266023909938)
--(axis cs:9.18367346938775,0.859331379499201)
--(axis cs:8.84353741496599,0.855662794183531)
--(axis cs:8.50340136054422,0.854900576056652)
--(axis cs:8.16326530612245,0.8462835201907)
--(axis cs:7.82312925170068,0.84209872339188)
--(axis cs:7.48299319727891,0.826773011755193)
--(axis cs:7.14285714285714,0.816506872762906)
--(axis cs:6.80272108843537,0.809973610931385)
--(axis cs:6.46258503401361,0.796223069980465)
--(axis cs:6.12244897959184,0.778544323155019)
--(axis cs:5.78231292517007,0.7686822026857)
--(axis cs:5.4421768707483,0.738340918647894)
--(axis cs:5.10204081632653,0.712657670924256)
--(axis cs:4.76190476190476,0.686157935124443)
--(axis cs:4.42176870748299,0.644066255662415)
--(axis cs:4.08163265306122,0.605662348790769)
--(axis cs:3.74149659863946,0.568717869044176)
--(axis cs:3.40136054421769,0.528593444821238)
--(axis cs:3.06122448979592,0.487146084166533)
--(axis cs:2.72108843537415,0.442661335343529)
--(axis cs:2.38095238095238,0.40882136850726)
--(axis cs:2.04081632653061,0.368377693082078)
--(axis cs:1.70068027210884,0.315796356512391)
--(axis cs:1.36054421768707,0.254913450559225)
--(axis cs:1.02040816326531,0.198109894143474)
--(axis cs:0.680272108843537,0.142868715342505)
--(axis cs:0.340136054421769,0.0945628612483491)
--(axis cs:0,0.0826294898306073)
--cycle;


==> img/stl10/stl10_rate_accuracy_guidedbackprop.tex <==
% guided backprop
\addplot [line width=0.5, opacity=0.8, color8, mark=oplus*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table [row sep=\\]{%
0	0.07515625 \\
0.340136054421769	0.0765625 \\
0.680272108843537	0.07609375 \\
1.02040816326531	0.07515625 \\
1.36054421768707	0.0753125 \\
1.70068027210884	0.07953125 \\
2.04081632653061	0.086875 \\
2.38095238095238	0.09625 \\
2.72108843537415	0.10234375 \\
3.06122448979592	0.1040625 \\
3.40136054421769	0.11515625 \\
3.74149659863946	0.11390625 \\
4.08163265306122	0.1184375 \\
4.42176870748299	0.12265625 \\
4.76190476190476	0.123125 \\
5.10204081632653	0.12375 \\
5.4421768707483	0.12625 \\
5.78231292517007	0.128125 \\
6.12244897959184	0.12875 \\
6.46258503401361	0.12890625 \\
6.80272108843537	0.13109375 \\
7.14285714285714	0.13109375 \\
7.48299319727891	0.13421875 \\
7.82312925170068	0.13234375 \\
8.16326530612245	0.1328125 \\
8.50340136054422	0.12984375 \\
8.84353741496599	0.12984375 \\
9.18367346938775	0.12859375 \\
9.52380952380952	0.1296875 \\
9.86394557823129	0.1265625 \\
10.2040816326531	0.126875 \\
10.5442176870748	0.12796875 \\
10.8843537414966	0.12765625 \\
11.2244897959184	0.13140625 \\
11.5646258503401	0.130625 \\
11.9047619047619	0.128125 \\
12.2448979591837	0.13 \\
12.5850340136054	0.13171875 \\
12.9251700680272	0.131875 \\
13.265306122449	0.13234375 \\
13.6054421768707	0.13671875 \\
13.9455782312925	0.13828125 \\
14.2857142857143	0.13625 \\
14.6258503401361	0.13828125 \\
14.9659863945578	0.1375 \\
15.3061224489796	0.1396875 \\
15.6462585034014	0.1403125 \\
15.9863945578231	0.14125 \\
16.3265306122449	0.14265625 \\
16.6666666666667	0.14421875 \\
17.0068027210884	0.1484375 \\
17.3469387755102	0.14828125 \\
17.687074829932	0.15140625 \\
18.0272108843537	0.15109375 \\
18.3673469387755	0.1515625 \\
18.7074829931973	0.15390625 \\
19.047619047619	0.1496875 \\
19.3877551020408	0.14859375 \\
19.7278911564626	0.1515625 \\
20.0680272108844	0.153125 \\
20.4081632653061	0.15296875 \\
20.7482993197279	0.15328125 \\
21.0884353741497	0.15296875 \\
21.4285714285714	0.15328125 \\
21.7687074829932	0.1546875 \\
22.108843537415	0.15859375 \\
22.4489795918367	0.15171875 \\
22.7891156462585	0.15296875 \\
23.1292517006803	0.15125 \\
23.469387755102	0.1509375 \\
23.8095238095238	0.14890625 \\
24.1496598639456	0.154375 \\
24.4897959183673	0.1515625 \\
24.8299319727891	0.14734375 \\
25.1700680272109	0.15203125 \\
25.5102040816327	0.15265625 \\
25.8503401360544	0.15015625 \\
26.1904761904762	0.15015625 \\
26.530612244898	0.14734375 \\
26.8707482993197	0.15390625 \\
27.2108843537415	0.1565625 \\
27.5510204081633	0.15546875 \\
27.891156462585	0.1534375 \\
28.2312925170068	0.15703125 \\
28.5714285714286	0.15671875 \\
28.9115646258503	0.158125 \\
29.2517006802721	0.15921875 \\
29.5918367346939	0.15890625 \\
29.9319727891156	0.16 \\
30.2721088435374	0.16421875 \\
30.6122448979592	0.16296875 \\
30.952380952381	0.16328125 \\
31.2925170068027	0.163125 \\
31.6326530612245	0.16578125 \\
31.9727891156463	0.16515625 \\
32.312925170068	0.161875 \\
32.6530612244898	0.16859375 \\
32.9931972789116	0.164375 \\
33.3333333333333	0.17 \\
33.6734693877551	0.1646875 \\
34.0136054421769	0.17015625 \\
34.3537414965986	0.1665625 \\
34.6938775510204	0.16765625 \\
35.0340136054422	0.16578125 \\
35.3741496598639	0.1596875 \\
35.7142857142857	0.16734375 \\
36.0544217687075	0.17140625 \\
36.3945578231292	0.175 \\
36.734693877551	0.17578125 \\
37.0748299319728	0.17671875 \\
37.4149659863946	0.1803125 \\
37.7551020408163	0.17671875 \\
38.0952380952381	0.1771875 \\
38.4353741496599	0.1771875 \\
38.7755102040816	0.179375 \\
39.1156462585034	0.1778125 \\
39.4557823129252	0.1753125 \\
39.7959183673469	0.173125 \\
40.1360544217687	0.17859375 \\
40.4761904761905	0.180625 \\
40.8163265306122	0.17734375 \\
41.156462585034	0.18578125 \\
41.4965986394558	0.18359375 \\
41.8367346938776	0.183125 \\
42.1768707482993	0.18796875 \\
42.5170068027211	0.186875 \\
42.8571428571429	0.1865625 \\
43.1972789115646	0.18734375 \\
43.5374149659864	0.1846875 \\
43.8775510204082	0.183125 \\
44.2176870748299	0.1865625 \\
44.5578231292517	0.2009375 \\
44.8979591836735	0.1975 \\
45.2380952380952	0.2009375 \\
45.578231292517	0.2084375 \\
45.9183673469388	0.205 \\
46.2585034013605	0.21203125 \\
46.5986394557823	0.21203125 \\
46.9387755102041	0.213125 \\
47.2789115646259	0.205 \\
47.6190476190476	0.21484375 \\
47.9591836734694	0.2084375 \\
48.2993197278912	0.20734375 \\
48.6394557823129	0.204375 \\
48.9795918367347	0.2059375 \\
49.3197278911565	0.20703125 \\
49.6598639455782	0.2071875 \\
50	0.20703125 \\
50.3401360544218	0.2046875 \\
50.6802721088435	0.2009375 \\
51.0204081632653	0.20578125 \\
51.3605442176871	0.20359375 \\
51.7006802721088	0.205 \\
52.0408163265306	0.205625 \\
52.3809523809524	0.21109375 \\
52.7210884353741	0.2109375 \\
53.0612244897959	0.216875 \\
53.4013605442177	0.21359375 \\
53.7414965986395	0.21546875 \\
54.0816326530612	0.21703125 \\
54.421768707483	0.21796875 \\
54.7619047619048	0.22296875 \\
55.1020408163265	0.22828125 \\
55.4421768707483	0.225625 \\
55.7823129251701	0.2340625 \\
56.1224489795918	0.23984375 \\
56.4625850340136	0.238125 \\
56.8027210884354	0.236875 \\
57.1428571428571	0.23984375 \\
57.4829931972789	0.239375 \\
57.8231292517007	0.24609375 \\
58.1632653061224	0.248125 \\
58.5034013605442	0.25359375 \\
58.843537414966	0.24828125 \\
59.1836734693878	0.24953125 \\
59.5238095238095	0.25296875 \\
59.8639455782313	0.25375 \\
60.2040816326531	0.255625 \\
60.5442176870748	0.25828125 \\
60.8843537414966	0.25359375 \\
61.2244897959184	0.26625 \\
61.5646258503401	0.2721875 \\
61.9047619047619	0.2709375 \\
62.2448979591837	0.2821875 \\
62.5850340136054	0.27578125 \\
62.9251700680272	0.28171875 \\
63.265306122449	0.28265625 \\
63.6054421768707	0.29046875 \\
63.9455782312925	0.2896875 \\
64.2857142857143	0.2890625 \\
64.6258503401361	0.286875 \\
64.9659863945578	0.28765625 \\
65.3061224489796	0.290625 \\
65.6462585034014	0.2896875 \\
65.9863945578231	0.289375 \\
66.3265306122449	0.2809375 \\
66.6666666666667	0.28421875 \\
67.0068027210884	0.28296875 \\
67.3469387755102	0.28359375 \\
67.687074829932	0.27875 \\
68.0272108843537	0.27984375 \\
68.3673469387755	0.276875 \\
68.7074829931973	0.27953125 \\
69.0476190476191	0.281875 \\
69.3877551020408	0.28140625 \\
69.7278911564626	0.29046875 \\
70.0680272108844	0.285 \\
70.4081632653061	0.28484375 \\
70.7482993197279	0.29296875 \\
71.0884353741497	0.295 \\
71.4285714285714	0.29609375 \\
71.7687074829932	0.29625 \\
72.108843537415	0.30109375 \\
72.4489795918367	0.30109375 \\
72.7891156462585	0.30046875 \\
73.1292517006803	0.29828125 \\
73.469387755102	0.29796875 \\
73.8095238095238	0.29890625 \\
74.1496598639456	0.3009375 \\
74.4897959183673	0.3015625 \\
74.8299319727891	0.2959375 \\
75.1700680272109	0.29796875 \\
75.5102040816327	0.30109375 \\
75.8503401360544	0.30203125 \\
76.1904761904762	0.30265625 \\
76.530612244898	0.30328125 \\
76.8707482993197	0.3015625 \\
77.2108843537415	0.304375 \\
77.5510204081633	0.3084375 \\
77.891156462585	0.3078125 \\
78.2312925170068	0.30953125 \\
78.5714285714286	0.31046875 \\
78.9115646258503	0.31 \\
79.2517006802721	0.31 \\
79.5918367346939	0.31234375 \\
79.9319727891156	0.30953125 \\
80.2721088435374	0.31 \\
80.6122448979592	0.30890625 \\
80.9523809523809	0.31140625 \\
81.2925170068027	0.3125 \\
81.6326530612245	0.31484375 \\
81.9727891156463	0.3175 \\
82.312925170068	0.31828125 \\
82.6530612244898	0.32 \\
82.9931972789116	0.3228125 \\
83.3333333333333	0.323125 \\
83.6734693877551	0.32671875 \\
84.0136054421769	0.33015625 \\
84.3537414965986	0.335625 \\
84.6938775510204	0.34328125 \\
85.0340136054422	0.3440625 \\
85.3741496598639	0.34859375 \\
85.7142857142857	0.3509375 \\
86.0544217687075	0.3571875 \\
86.3945578231292	0.36296875 \\
86.734693877551	0.36171875 \\
87.0748299319728	0.37109375 \\
87.4149659863945	0.37734375 \\
87.7551020408163	0.379375 \\
88.0952380952381	0.38765625 \\
88.4353741496599	0.3934375 \\
88.7755102040816	0.40671875 \\
89.1156462585034	0.41328125 \\
89.4557823129252	0.4215625 \\
89.7959183673469	0.42953125 \\
90.1360544217687	0.445 \\
90.4761904761905	0.4540625 \\
90.8163265306122	0.46640625 \\
91.156462585034	0.47921875 \\
91.4965986394558	0.4884375 \\
91.8367346938775	0.50171875 \\
92.1768707482993	0.5146875 \\
92.5170068027211	0.5284375 \\
92.8571428571429	0.5596875 \\
93.1972789115646	0.5796875 \\
93.5374149659864	0.59796875 \\
93.8775510204082	0.6165625 \\
94.2176870748299	0.62546875 \\
94.5578231292517	0.6503125 \\
94.8979591836735	0.67578125 \\
95.2380952380952	0.6990625 \\
95.578231292517	0.71 \\
95.9183673469388	0.72890625 \\
96.2585034013605	0.74265625 \\
96.5986394557823	0.76296875 \\
96.9387755102041	0.774375 \\
97.2789115646258	0.7853125 \\
97.6190476190476	0.7903125 \\
97.9591836734694	0.81125 \\
98.2993197278912	0.8178125 \\
98.6394557823129	0.8309375 \\
98.9795918367347	0.83609375 \\
99.3197278911565	0.8571875 \\
99.6598639455782	0.885625 \\
100	1 \\
};
\path [fill=color8, fill opacity=0.5] (axis cs:0,0.0818846168003316)
--(axis cs:0,0.0684278831996684)
--(axis cs:0.340136054421769,0.0694275763837469)
--(axis cs:0.680272108843537,0.0685881826083821)
--(axis cs:1.02040816326531,0.0681542219647487)
--(axis cs:1.36054421768707,0.0674452601323739)
--(axis cs:1.70068027210884,0.0704156785319857)
--(axis cs:2.04081632653061,0.0763046413064572)
--(axis cs:2.38095238095238,0.0844202844840016)
--(axis cs:2.72108843537415,0.0902805346765288)
--(axis cs:3.06122448979592,0.0917671166128616)
--(axis cs:3.40136054421769,0.103979407927838)
--(axis cs:3.74149659863946,0.102127837424121)
--(axis cs:4.08163265306122,0.107881586627444)
--(axis cs:4.42176870748299,0.11188701912597)
--(axis cs:4.76190476190476,0.112636155013986)
--(axis cs:5.10204081632653,0.1132266610992)
--(axis cs:5.4421768707483,0.11585064100627)
--(axis cs:5.78231292517007,0.117121432796091)
--(axis cs:6.12244897959184,0.117864065471599)
--(axis cs:6.46258503401361,0.11788233426467)
--(axis cs:6.80272108843537,0.119927151732393)
--(axis cs:7.14285714285714,0.119832752093396)
--(axis cs:7.48299319727891,0.122532189391654)
--(axis cs:7.82312925170068,0.120958103341637)
--(axis cs:8.16326530612245,0.121053941313129)
--(axis cs:8.50340136054422,0.118181696395995)
--(axis cs:8.84353741496599,0.118650707743925)
--(axis cs:9.18367346938775,0.117326825474787)
--(axis cs:9.52380952380952,0.118056152763958)
--(axis cs:9.86394557823129,0.115630232836596)
--(axis cs:10.2040816326531,0.115739617895234)
--(axis cs:10.5442176870748,0.11644738167412)
--(axis cs:10.8843537414966,0.115757005244267)
--(axis cs:11.2244897959184,0.120390122878244)
--(axis cs:11.5646258503401,0.118680558709828)
--(axis cs:11.9047619047619,0.11662973518003)
--(axis cs:12.2448979591837,0.118414659120638)
--(axis cs:12.5850340136054,0.12009437415045)
--(axis cs:12.9251700680272,0.120410472347841)
--(axis cs:13.265306122449,0.120297147959278)
--(axis cs:13.6054421768707,0.124535961572784)
--(axis cs:13.9455782312925,0.125415432843728)
--(axis cs:14.2857142857143,0.123645910678397)
--(axis cs:14.6258503401361,0.124680360060245)
--(axis cs:14.9659863945578,0.123475528850769)
--(axis cs:15.3061224489796,0.126423494651289)
--(axis cs:15.6462585034014,0.126880593687874)
--(axis cs:15.9863945578231,0.127776976234536)
--(axis cs:16.3265306122449,0.128511592533703)
--(axis cs:16.6666666666667,0.129951242059336)
--(axis cs:17.0068027210884,0.134264889636292)
--(axis cs:17.3469387755102,0.134373203350787)
--(axis cs:17.687074829932,0.137679726962742)
--(axis cs:18.0272108843537,0.137295851472174)
--(axis cs:18.3673469387755,0.137615081347771)
--(axis cs:18.7074829931973,0.1402047614245)
--(axis cs:19.047619047619,0.13627691080385)
--(axis cs:19.3877551020408,0.134475411964945)
--(axis cs:19.7278911564626,0.138122076308253)
--(axis cs:20.0680272108844,0.13939604549157)
--(axis cs:20.4081632653061,0.139242226962742)
--(axis cs:20.7482993197279,0.139392416212403)
--(axis cs:21.0884353741497,0.139186065679268)
--(axis cs:21.4285714285714,0.139060608706657)
--(axis cs:21.7687074829932,0.140154753731269)
--(axis cs:22.108843537415,0.144308873609865)
--(axis cs:22.4489795918367,0.136811210768049)
--(axis cs:22.7891156462585,0.138185193489782)
--(axis cs:23.1292517006803,0.135922634567431)
--(axis cs:23.469387755102,0.136052047683264)
--(axis cs:23.8095238095238,0.134098844349956)
--(axis cs:24.1496598639456,0.1393905720478)
--(axis cs:24.4897959183673,0.13686401777772)
--(axis cs:24.8299319727891,0.132839577584586)
--(axis cs:25.1700680272109,0.136922278455975)
--(axis cs:25.5102040816327,0.137298116367401)
--(axis cs:25.8503401360544,0.135391412988123)
--(axis cs:26.1904761904762,0.135409509534049)
--(axis cs:26.530612244898,0.131876714011469)
--(axis cs:26.8707482993197,0.137890327270298)
--(axis cs:27.2108843537415,0.140199904619441)
--(axis cs:27.5510204081633,0.139253989061582)
--(axis cs:27.891156462585,0.137737606248182)
--(axis cs:28.2312925170068,0.141103698245031)
--(axis cs:28.5714285714286,0.140974272712282)
--(axis cs:28.9115646258503,0.141733288621858)
--(axis cs:29.2517006802721,0.142909571492519)
--(axis cs:29.5918367346939,0.143637796029623)
--(axis cs:29.9319727891156,0.144185113777814)
--(axis cs:30.2721088435374,0.148049929994927)
--(axis cs:30.6122448979592,0.147194015790515)
--(axis cs:30.952380952381,0.147728744836197)
--(axis cs:31.2925170068027,0.147289022030762)
--(axis cs:31.6326530612245,0.14983634372838)
--(axis cs:31.9727891156463,0.149053033446341)
--(axis cs:32.312925170068,0.146447785008228)
--(axis cs:32.6530612244898,0.152690766255816)
--(axis cs:32.9931972789116,0.148836297884709)
--(axis cs:33.3333333333333,0.154296462031239)
--(axis cs:33.6734693877551,0.14912120402721)
--(axis cs:34.0136054421769,0.154463343362746)
--(axis cs:34.3537414965986,0.150969882188208)
--(axis cs:34.6938775510204,0.152019962573086)
--(axis cs:35.0340136054422,0.149804078652341)
--(axis cs:35.3741496598639,0.144423106497984)
--(axis cs:35.7142857142857,0.15158897883914)
--(axis cs:36.0544217687075,0.155267539005819)
--(axis cs:36.3945578231292,0.158895895131877)
--(axis cs:36.734693877551,0.159523610663614)
--(axis cs:37.0748299319728,0.160440006734631)
--(axis cs:37.4149659863946,0.163643862522936)
--(axis cs:37.7551020408163,0.159747622155986)
--(axis cs:38.0952380952381,0.160280836635714)
--(axis cs:38.4353741496599,0.159973387080835)
--(axis cs:38.7755102040816,0.161790908130778)
--(axis cs:39.1156462585034,0.159968909910688)
--(axis cs:39.4557823129252,0.157451281331493)
--(axis cs:39.7959183673469,0.155583806156783)
--(axis cs:40.1360544217687,0.16035868422273)
--(axis cs:40.4761904761905,0.162246934380941)
--(axis cs:40.8163265306122,0.158723645335163)
--(axis cs:41.156462585034,0.166651838823797)
--(axis cs:41.4965986394558,0.164476307485993)
--(axis cs:41.8367346938776,0.16373931195126)
--(axis cs:42.1768707482993,0.168215857222706)
--(axis cs:42.5170068027211,0.166958391474299)
--(axis cs:42.8571428571429,0.166391814913339)
--(axis cs:43.1972789115646,0.16706955045688)
--(axis cs:43.5374149659864,0.164571260641275)
--(axis cs:43.8775510204082,0.162954314913339)
--(axis cs:44.2176870748299,0.166551783571729)
--(axis cs:44.5578231292517,0.179479330612858)
--(axis cs:44.8979591836735,0.176119302003298)
--(axis cs:45.2380952380952,0.179999398766795)
--(axis cs:45.578231292517,0.186910996560245)
--(axis cs:45.9183673469388,0.183464195079944)
--(axis cs:46.2585034013605,0.190664607025334)
--(axis cs:46.5986394557823,0.190431550642622)
--(axis cs:46.9387755102041,0.192134584706831)
--(axis cs:47.2789115646259,0.183678708455055)
--(axis cs:47.6190476190476,0.193316139030419)
--(axis cs:47.9591836734694,0.187117550359216)
--(axis cs:48.2993197278912,0.18560717100106)
--(axis cs:48.6394557823129,0.182981816402336)
--(axis cs:48.9795918367347,0.18498892550345)
--(axis cs:49.3197278911565,0.18634586734601)
--(axis cs:49.6598639455782,0.186482071914658)
--(axis cs:50,0.186632310947257)
--(axis cs:50.3401360544218,0.184106343949501)
--(axis cs:50.6802721088435,0.180938224805614)
--(axis cs:51.0204081632653,0.185655294310711)
--(axis cs:51.3605442176871,0.183914864623458)
--(axis cs:51.7006802721088,0.185303918196054)
--(axis cs:52.0408163265306,0.186024050147826)
--(axis cs:52.3809523809524,0.191731936111933)
--(axis cs:52.7210884353741,0.19140283233027)
--(axis cs:53.0612244897959,0.197370135009419)
--(axis cs:53.4013605442177,0.19381480307826)
--(axis cs:53.7414965986395,0.195697519245397)
--(axis cs:54.0816326530612,0.197763248686065)
--(axis cs:54.421768707483,0.19931333876663)
--(axis cs:54.7619047619048,0.204017649482736)
--(axis cs:55.1020408163265,0.20891746599528)
--(axis cs:55.4421768707483,0.206752819145497)
--(axis cs:55.7823129251701,0.215342533004659)
--(axis cs:56.1224489795918,0.221327908674128)
--(axis cs:56.4625850340136,0.219588310538255)
--(axis cs:56.8027210884354,0.219021792164171)
--(axis cs:57.1428571428571,0.222428872183594)
--(axis cs:57.4829931972789,0.221598343354714)
--(axis cs:57.8231292517007,0.228296986889207)
--(axis cs:58.1632653061224,0.230455964253283)
--(axis cs:58.5034013605442,0.236202435804453)
--(axis cs:58.843537414966,0.23061896233278)
--(axis cs:59.1836734693878,0.232042599680017)
--(axis cs:59.5238095238095,0.235358915319748)
--(axis cs:59.8639455782313,0.23648057522016)
--(axis cs:60.2040816326531,0.238418090682186)
--(axis cs:60.5442176870748,0.241261863991037)
--(axis cs:60.8843537414966,0.235849579814795)
--(axis cs:61.2244897959184,0.248793825803512)
--(axis cs:61.5646258503401,0.255371331937662)
--(axis cs:61.9047619047619,0.253939139950137)
--(axis cs:62.2448979591837,0.266156400387523)
--(axis cs:62.5850340136054,0.259462718222597)
--(axis cs:62.9251700680272,0.266443426926653)
--(axis cs:63.265306122449,0.266630802840403)
--(axis cs:63.6054421768707,0.275757621130261)
--(axis cs:63.9455782312925,0.275141635163632)
--(axis cs:64.2857142857143,0.274497634228514)
--(axis cs:64.6258503401361,0.272083382046919)
--(axis cs:64.9659863945578,0.272999676738473)
--(axis cs:65.3061224489796,0.276608691314055)
--(axis cs:65.6462585034014,0.275578959915345)
--(axis cs:65.9863945578231,0.275230679652394)
--(axis cs:66.3265306122449,0.267225227094947)
--(axis cs:66.6666666666667,0.270820611451039)
--(axis cs:67.0068027210884,0.269618386971484)
--(axis cs:67.3469387755102,0.269839464335324)
--(axis cs:67.687074829932,0.265235983883693)
--(axis cs:68.0272108843537,0.265945992652077)
--(axis cs:68.3673469387755,0.264370423201165)
--(axis cs:68.7074829931973,0.266365028807374)
--(axis cs:69.0476190476191,0.268364512808187)
--(axis cs:69.3877551020408,0.268322863471591)
--(axis cs:69.7278911564626,0.276999619916362)
--(axis cs:70.0680272108844,0.271771993212346)
--(axis cs:70.4081632653061,0.271168039042597)
--(axis cs:70.7482993197279,0.279524424312615)
--(axis cs:71.0884353741497,0.281779926050713)
--(axis cs:71.4285714285714,0.283527929033291)
--(axis cs:71.7687074829932,0.284050392882623)
--(axis cs:72.108843537415,0.289023421698028)
--(axis cs:72.4489795918367,0.289724867904449)
--(axis cs:72.7891156462585,0.289048812926244)
--(axis cs:73.1292517006803,0.286817138279333)
--(axis cs:73.469387755102,0.287036919019379)
--(axis cs:73.8095238095238,0.287566765528427)
--(axis cs:74.1496598639456,0.290531723628928)
--(axis cs:74.4897959183673,0.290511367344974)
--(axis cs:74.8299319727891,0.284922671515943)
--(axis cs:75.1700680272109,0.286609098959896)
--(axis cs:75.5102040816327,0.290695766673846)
--(axis cs:75.8503401360544,0.292079412091413)
--(axis cs:76.1904761904762,0.292640412474222)
--(axis cs:76.530612244898,0.29276561701918)
--(axis cs:76.8707482993197,0.291614975329495)
--(axis cs:77.2108843537415,0.294413105131792)
--(axis cs:77.5510204081633,0.29840026159568)
--(axis cs:77.891156462585,0.297897624885549)
--(axis cs:78.2312925170068,0.300329253338747)
--(axis cs:78.5714285714286,0.301029375477192)
--(axis cs:78.9115646258503,0.299272026449329)
--(axis cs:79.2517006802721,0.300109200670474)
--(axis cs:79.5918367346939,0.301637578130986)
--(axis cs:79.9319727891156,0.298858087530763)
--(axis cs:80.2721088435374,0.299411612368414)
--(axis cs:80.6122448979592,0.298438793660855)
--(axis cs:80.9523809523809,0.300895152552271)
--(axis cs:81.2925170068027,0.302240979697915)
--(axis cs:81.6326530612245,0.304045335363259)
--(axis cs:81.9727891156463,0.305588339125255)
--(axis cs:82.312925170068,0.30712405014876)
--(axis cs:82.6530612244898,0.308475734934377)
--(axis cs:82.9931972789116,0.310256928945605)
--(axis cs:83.3333333333333,0.310604417580206)
--(axis cs:83.6734693877551,0.314296429720048)
--(axis cs:84.0136054421769,0.317302298260656)
--(axis cs:84.3537414965986,0.322680480797164)
--(axis cs:84.6938775510204,0.330878137326986)
--(axis cs:85.0340136054422,0.331317704608535)
--(axis cs:85.3741496598639,0.335184227549204)
--(axis cs:85.7142857142857,0.337631141610719)
--(axis cs:86.0544217687075,0.343148755959719)
--(axis cs:86.3945578231292,0.348357795351944)
--(axis cs:86.734693877551,0.346509749196386)
--(axis cs:87.0748299319728,0.356387159701165)
--(axis cs:87.4149659863945,0.361963278154684)
--(axis cs:87.7551020408163,0.364299835337562)
--(axis cs:88.0952380952381,0.37252457241204)
--(axis cs:88.4353741496599,0.378605319064325)
--(axis cs:88.7755102040816,0.390129542740901)
--(axis cs:89.1156462585034,0.396611754339624)
--(axis cs:89.4557823129252,0.404314625746639)
--(axis cs:89.7959183673469,0.411997397332093)
--(axis cs:90.1360544217687,0.428460017702419)
--(axis cs:90.4761904761905,0.437852150801337)
--(axis cs:90.8163265306122,0.449539966715268)
--(axis cs:91.156462585034,0.461452020926045)
--(axis cs:91.4965986394558,0.47075389718978)
--(axis cs:91.8367346938775,0.484169674611334)
--(axis cs:92.1768707482993,0.496596037223579)
--(axis cs:92.5170068027211,0.509760885800185)
--(axis cs:92.8571428571429,0.541362961075196)
--(axis cs:93.1972789115646,0.561284024873587)
--(axis cs:93.5374149659864,0.580022039246219)
--(axis cs:93.8775510204082,0.599032183068502)
--(axis cs:94.2176870748299,0.608714796390543)
--(axis cs:94.5578231292517,0.634188864595652)
--(axis cs:94.8979591836735,0.659736770942469)
--(axis cs:95.2380952380952,0.684498289020511)
--(axis cs:95.578231292517,0.695442993676395)
--(axis cs:95.9183673469388,0.715857167687656)
--(axis cs:96.2585034013605,0.731190474643898)
--(axis cs:96.5986394557823,0.750844027492906)
--(axis cs:96.9387755102041,0.764364400758797)
--(axis cs:97.2789115646258,0.775034904596154)
--(axis cs:97.6190476190476,0.777362824645117)
--(axis cs:97.9591836734694,0.798808118508881)
--(axis cs:98.2993197278912,0.807784767458599)
--(axis cs:98.6394557823129,0.821853893785755)
--(axis cs:98.9795918367347,0.827104599604712)
--(axis cs:99.3197278911565,0.846359539875444)
--(axis cs:99.6598639455782,0.879056573546562)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,0.892193426453438)
--(axis cs:99.3197278911565,0.868015460124556)
--(axis cs:98.9795918367347,0.845082900395288)
--(axis cs:98.6394557823129,0.840021106214245)
--(axis cs:98.2993197278912,0.827840232541401)
--(axis cs:97.9591836734694,0.823691881491119)
--(axis cs:97.6190476190476,0.803262175354883)
--(axis cs:97.2789115646258,0.795590095403846)
--(axis cs:96.9387755102041,0.784385599241203)
--(axis cs:96.5986394557823,0.775093472507094)
--(axis cs:96.2585034013605,0.754122025356102)
--(axis cs:95.9183673469388,0.741955332312344)
--(axis cs:95.578231292517,0.724557006323605)
--(axis cs:95.2380952380952,0.713626710979489)
--(axis cs:94.8979591836735,0.691825729057531)
--(axis cs:94.5578231292517,0.666436135404348)
--(axis cs:94.2176870748299,0.642222703609457)
--(axis cs:93.8775510204082,0.634092816931498)
--(axis cs:93.5374149659864,0.615915460753781)
--(axis cs:93.1972789115646,0.598090975126413)
--(axis cs:92.8571428571429,0.578012038924804)
--(axis cs:92.5170068027211,0.547114114199815)
--(axis cs:92.1768707482993,0.532778962776421)
--(axis cs:91.8367346938775,0.519267825388666)
--(axis cs:91.4965986394558,0.50612110281022)
--(axis cs:91.156462585034,0.496985479073955)
--(axis cs:90.8163265306122,0.483272533284732)
--(axis cs:90.4761904761905,0.470272849198662)
--(axis cs:90.1360544217687,0.461539982297581)
--(axis cs:89.7959183673469,0.447065102667907)
--(axis cs:89.4557823129252,0.438810374253361)
--(axis cs:89.1156462585034,0.429950745660376)
--(axis cs:88.7755102040816,0.423307957259099)
--(axis cs:88.4353741496599,0.408269680935675)
--(axis cs:88.0952380952381,0.40278792758796)
--(axis cs:87.7551020408163,0.394450164662438)
--(axis cs:87.4149659863945,0.392724221845316)
--(axis cs:87.0748299319728,0.385800340298835)
--(axis cs:86.734693877551,0.376927750803614)
--(axis cs:86.3945578231292,0.377579704648056)
--(axis cs:86.0544217687075,0.371226244040281)
--(axis cs:85.7142857142857,0.364243858389281)
--(axis cs:85.3741496598639,0.362003272450796)
--(axis cs:85.0340136054422,0.356807295391465)
--(axis cs:84.6938775510204,0.355684362673014)
--(axis cs:84.3537414965986,0.348569519202836)
--(axis cs:84.0136054421769,0.343010201739344)
--(axis cs:83.6734693877551,0.339141070279952)
--(axis cs:83.3333333333333,0.335645582419794)
--(axis cs:82.9931972789116,0.335368071054395)
--(axis cs:82.6530612244898,0.331524265065623)
--(axis cs:82.312925170068,0.32943844985124)
--(axis cs:81.9727891156463,0.329411660874745)
--(axis cs:81.6326530612245,0.325642164636741)
--(axis cs:81.2925170068027,0.322759020302085)
--(axis cs:80.9523809523809,0.321917347447729)
--(axis cs:80.6122448979592,0.319373706339145)
--(axis cs:80.2721088435374,0.320588387631586)
--(axis cs:79.9319727891156,0.320204412469237)
--(axis cs:79.5918367346939,0.323049921869014)
--(axis cs:79.2517006802721,0.319890799329526)
--(axis cs:78.9115646258503,0.320727973550671)
--(axis cs:78.5714285714286,0.319908124522808)
--(axis cs:78.2312925170068,0.318733246661253)
--(axis cs:77.891156462585,0.317727375114451)
--(axis cs:77.5510204081633,0.31847473840432)
--(axis cs:77.2108843537415,0.314336894868208)
--(axis cs:76.8707482993197,0.311510024670505)
--(axis cs:76.530612244898,0.31379688298082)
--(axis cs:76.1904761904762,0.312672087525778)
--(axis cs:75.8503401360544,0.311983087908587)
--(axis cs:75.5102040816327,0.311491733326154)
--(axis cs:75.1700680272109,0.309328401040104)
--(axis cs:74.8299319727891,0.306952328484057)
--(axis cs:74.4897959183673,0.312613632655026)
--(axis cs:74.1496598639456,0.311343276371072)
--(axis cs:73.8095238095238,0.310245734471573)
--(axis cs:73.469387755102,0.308900580980621)
--(axis cs:73.1292517006803,0.309745361720667)
--(axis cs:72.7891156462585,0.311888687073756)
--(axis cs:72.4489795918367,0.312462632095551)
--(axis cs:72.108843537415,0.313164078301972)
--(axis cs:71.7687074829932,0.308449607117377)
--(axis cs:71.4285714285714,0.308659570966709)
--(axis cs:71.0884353741497,0.308220073949287)
--(axis cs:70.7482993197279,0.306413075687385)
--(axis cs:70.4081632653061,0.298519460957403)
--(axis cs:70.0680272108844,0.298228006787654)
--(axis cs:69.7278911564626,0.303937880083638)
--(axis cs:69.3877551020408,0.294489636528409)
--(axis cs:69.0476190476191,0.295385487191813)
--(axis cs:68.7074829931973,0.292697471192626)
--(axis cs:68.3673469387755,0.289379576798835)
--(axis cs:68.0272108843537,0.293741507347923)
--(axis cs:67.687074829932,0.292264016116307)
--(axis cs:67.3469387755102,0.297348035664676)
--(axis cs:67.0068027210884,0.296319113028516)
--(axis cs:66.6666666666667,0.297616888548961)
--(axis cs:66.3265306122449,0.294649772905053)
--(axis cs:65.9863945578231,0.303519320347606)
--(axis cs:65.6462585034014,0.303796040084655)
--(axis cs:65.3061224489796,0.304641308685945)
--(axis cs:64.9659863945578,0.302312823261527)
--(axis cs:64.6258503401361,0.301666617953081)
--(axis cs:64.2857142857143,0.303627365771486)
--(axis cs:63.9455782312925,0.304233364836368)
--(axis cs:63.6054421768707,0.305179878869739)
--(axis cs:63.265306122449,0.298681697159597)
--(axis cs:62.9251700680272,0.296994073073347)
--(axis cs:62.5850340136054,0.292099781777403)
--(axis cs:62.2448979591837,0.298218599612477)
--(axis cs:61.9047619047619,0.287935860049863)
--(axis cs:61.5646258503401,0.289003668062338)
--(axis cs:61.2244897959184,0.283706174196488)
--(axis cs:60.8843537414966,0.271337920185205)
--(axis cs:60.5442176870748,0.275300636008963)
--(axis cs:60.2040816326531,0.272831909317814)
--(axis cs:59.8639455782313,0.27101942477984)
--(axis cs:59.5238095238095,0.270578584680252)
--(axis cs:59.1836734693878,0.267019900319983)
--(axis cs:58.843537414966,0.265943537667221)
--(axis cs:58.5034013605442,0.270985064195547)
--(axis cs:58.1632653061224,0.265794035746717)
--(axis cs:57.8231292517007,0.263890513110793)
--(axis cs:57.4829931972789,0.257151656645286)
--(axis cs:57.1428571428571,0.257258627816406)
--(axis cs:56.8027210884354,0.254728207835829)
--(axis cs:56.4625850340136,0.256661689461745)
--(axis cs:56.1224489795918,0.258359591325872)
--(axis cs:55.7823129251701,0.252782466995341)
--(axis cs:55.4421768707483,0.244497180854503)
--(axis cs:55.1020408163265,0.24764503400472)
--(axis cs:54.7619047619048,0.241919850517264)
--(axis cs:54.421768707483,0.23662416123337)
--(axis cs:54.0816326530612,0.236299251313935)
--(axis cs:53.7414965986395,0.235239980754603)
--(axis cs:53.4013605442177,0.23337269692174)
--(axis cs:53.0612244897959,0.236379864990581)
--(axis cs:52.7210884353741,0.23047216766973)
--(axis cs:52.3809523809524,0.230455563888067)
--(axis cs:52.0408163265306,0.225225949852174)
--(axis cs:51.7006802721088,0.224696081803946)
--(axis cs:51.3605442176871,0.223272635376542)
--(axis cs:51.0204081632653,0.225907205689289)
--(axis cs:50.6802721088435,0.220936775194386)
--(axis cs:50.3401360544218,0.225268656050499)
--(axis cs:50,0.227430189052743)
--(axis cs:49.6598639455782,0.227892928085342)
--(axis cs:49.3197278911565,0.22771663265399)
--(axis cs:48.9795918367347,0.22688607449655)
--(axis cs:48.6394557823129,0.225768183597664)
--(axis cs:48.2993197278912,0.22908032899894)
--(axis cs:47.9591836734694,0.229757449640784)
--(axis cs:47.6190476190476,0.236371360969581)
--(axis cs:47.2789115646259,0.226321291544945)
--(axis cs:46.9387755102041,0.234115415293169)
--(axis cs:46.5986394557823,0.233630949357378)
--(axis cs:46.2585034013605,0.233397892974666)
--(axis cs:45.9183673469388,0.226535804920056)
--(axis cs:45.578231292517,0.229964003439755)
--(axis cs:45.2380952380952,0.221875601233205)
--(axis cs:44.8979591836735,0.218880697996702)
--(axis cs:44.5578231292517,0.222395669387142)
--(axis cs:44.2176870748299,0.206573216428271)
--(axis cs:43.8775510204082,0.203295685086661)
--(axis cs:43.5374149659864,0.204803739358725)
--(axis cs:43.1972789115646,0.20761794954312)
--(axis cs:42.8571428571429,0.206733185086661)
--(axis cs:42.5170068027211,0.206791608525701)
--(axis cs:42.1768707482993,0.207721642777294)
--(axis cs:41.8367346938776,0.20251068804874)
--(axis cs:41.4965986394558,0.202711192514007)
--(axis cs:41.156462585034,0.204910661176203)
--(axis cs:40.8163265306122,0.195963854664837)
--(axis cs:40.4761904761905,0.199003065619059)
--(axis cs:40.1360544217687,0.19682881577727)
--(axis cs:39.7959183673469,0.190666193843217)
--(axis cs:39.4557823129252,0.193173718668507)
--(axis cs:39.1156462585034,0.195656090089312)
--(axis cs:38.7755102040816,0.196959091869222)
--(axis cs:38.4353741496599,0.194401612919165)
--(axis cs:38.0952380952381,0.194094163364286)
--(axis cs:37.7551020408163,0.193689877844014)
--(axis cs:37.4149659863946,0.196981137477064)
--(axis cs:37.0748299319728,0.192997493265369)
--(axis cs:36.734693877551,0.192038889336386)
--(axis cs:36.3945578231292,0.191104104868123)
--(axis cs:36.0544217687075,0.187544960994181)
--(axis cs:35.7142857142857,0.18309852116086)
--(axis cs:35.3741496598639,0.174951893502016)
--(axis cs:35.0340136054422,0.181758421347659)
--(axis cs:34.6938775510204,0.183292537426914)
--(axis cs:34.3537414965986,0.182155117811792)
--(axis cs:34.0136054421769,0.185849156637254)
--(axis cs:33.6734693877551,0.18025379597279)
--(axis cs:33.3333333333333,0.185703537968761)
--(axis cs:32.9931972789116,0.179913702115291)
--(axis cs:32.6530612244898,0.184496733744184)
--(axis cs:32.312925170068,0.177302214991772)
--(axis cs:31.9727891156463,0.181259466553659)
--(axis cs:31.6326530612245,0.18172615627162)
--(axis cs:31.2925170068027,0.178960977969238)
--(axis cs:30.952380952381,0.178833755163803)
--(axis cs:30.6122448979592,0.178743484209485)
--(axis cs:30.2721088435374,0.180387570005073)
--(axis cs:29.9319727891156,0.175814886222186)
--(axis cs:29.5918367346939,0.174174703970377)
--(axis cs:29.2517006802721,0.175527928507481)
--(axis cs:28.9115646258503,0.174516711378142)
--(axis cs:28.5714285714286,0.172463227287718)
--(axis cs:28.2312925170068,0.172958801754969)
--(axis cs:27.891156462585,0.169137393751818)
--(axis cs:27.5510204081633,0.171683510938418)
--(axis cs:27.2108843537415,0.172925095380559)
--(axis cs:26.8707482993197,0.169922172729702)
--(axis cs:26.530612244898,0.162810785988531)
--(axis cs:26.1904761904762,0.164902990465951)
--(axis cs:25.8503401360544,0.164921087011877)
--(axis cs:25.5102040816327,0.168014383632599)
--(axis cs:25.1700680272109,0.167140221544025)
--(axis cs:24.8299319727891,0.161847922415414)
--(axis cs:24.4897959183673,0.16626098222228)
--(axis cs:24.1496598639456,0.1693594279522)
--(axis cs:23.8095238095238,0.163713655650044)
--(axis cs:23.469387755102,0.165822952316736)
--(axis cs:23.1292517006803,0.166577365432569)
--(axis cs:22.7891156462585,0.167752306510218)
--(axis cs:22.4489795918367,0.166626289231951)
--(axis cs:22.108843537415,0.172878626390135)
--(axis cs:21.7687074829932,0.169220246268731)
--(axis cs:21.4285714285714,0.167501891293343)
--(axis cs:21.0884353741497,0.166751434320732)
--(axis cs:20.7482993197279,0.167170083787597)
--(axis cs:20.4081632653061,0.166695273037258)
--(axis cs:20.0680272108844,0.16685395450843)
--(axis cs:19.7278911564626,0.165002923691747)
--(axis cs:19.3877551020408,0.162712088035055)
--(axis cs:19.047619047619,0.16309808919615)
--(axis cs:18.7074829931973,0.1676077385755)
--(axis cs:18.3673469387755,0.165509918652229)
--(axis cs:18.0272108843537,0.164891648527826)
--(axis cs:17.687074829932,0.165132773037258)
--(axis cs:17.3469387755102,0.162189296649213)
--(axis cs:17.0068027210884,0.162610110363708)
--(axis cs:16.6666666666667,0.158486257940664)
--(axis cs:16.3265306122449,0.156800907466297)
--(axis cs:15.9863945578231,0.154723023765464)
--(axis cs:15.6462585034014,0.153744406312126)
--(axis cs:15.3061224489796,0.152951505348711)
--(axis cs:14.9659863945578,0.151524471149231)
--(axis cs:14.6258503401361,0.151882139939755)
--(axis cs:14.2857142857143,0.148854089321603)
--(axis cs:13.9455782312925,0.151147067156272)
--(axis cs:13.6054421768707,0.148901538427216)
--(axis cs:13.265306122449,0.144390352040722)
--(axis cs:12.9251700680272,0.143339527652159)
--(axis cs:12.5850340136054,0.14334312584955)
--(axis cs:12.2448979591837,0.141585340879362)
--(axis cs:11.9047619047619,0.13962026481997)
--(axis cs:11.5646258503401,0.142569441290172)
--(axis cs:11.2244897959184,0.142422377121756)
--(axis cs:10.8843537414966,0.139555494755733)
--(axis cs:10.5442176870748,0.13949011832588)
--(axis cs:10.2040816326531,0.138010382104766)
--(axis cs:9.86394557823129,0.137494767163404)
--(axis cs:9.52380952380952,0.141318847236042)
--(axis cs:9.18367346938775,0.139860674525213)
--(axis cs:8.84353741496599,0.141036792256075)
--(axis cs:8.50340136054422,0.141505803604005)
--(axis cs:8.16326530612245,0.144571058686871)
--(axis cs:7.82312925170068,0.143729396658363)
--(axis cs:7.48299319727891,0.145905310608346)
--(axis cs:7.14285714285714,0.142354747906604)
--(axis cs:6.80272108843537,0.142260348267607)
--(axis cs:6.46258503401361,0.13993016573533)
--(axis cs:6.12244897959184,0.139635934528401)
--(axis cs:5.78231292517007,0.139128567203909)
--(axis cs:5.4421768707483,0.13664935899373)
--(axis cs:5.10204081632653,0.1342733389008)
--(axis cs:4.76190476190476,0.133613844986014)
--(axis cs:4.42176870748299,0.13342548087403)
--(axis cs:4.08163265306122,0.128993413372556)
--(axis cs:3.74149659863946,0.125684662575879)
--(axis cs:3.40136054421769,0.126333092072162)
--(axis cs:3.06122448979592,0.116357883387138)
--(axis cs:2.72108843537415,0.114406965323471)
--(axis cs:2.38095238095238,0.108079715515998)
--(axis cs:2.04081632653061,0.0974453586935428)
--(axis cs:1.70068027210884,0.0886468214680143)
--(axis cs:1.36054421768707,0.0831797398676261)
--(axis cs:1.02040816326531,0.0821582780352513)
--(axis cs:0.680272108843537,0.0835993173916179)
--(axis cs:0.340136054421769,0.0836974236162531)
--(axis cs:0,0.0818846168003316)
--cycle;


==> img/stl10/stl10_rate_accuracy_lafw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.07703125
0.340136054421769 0.0803125
0.680272108843537 0.1003125
1.02040816326531 0.1765625
1.36054421768707 0.22703125
1.70068027210884 0.27453125
2.04081632653061 0.3346875
2.38095238095238 0.3828125
2.72108843537415 0.43484375
3.06122448979592 0.474375
3.40136054421769 0.51734375
3.74149659863946 0.56765625
4.08163265306122 0.604375
4.42176870748299 0.63546875
4.76190476190476 0.65671875
5.10204081632653 0.6803125
5.4421768707483 0.70078125
5.78231292517007 0.72453125
6.12244897959184 0.74578125
6.46258503401361 0.76078125
6.80272108843537 0.7696875
7.14285714285714 0.779375
7.48299319727891 0.78234375
7.82312925170068 0.79125
8.16326530612245 0.8034375
8.50340136054422 0.81828125
8.84353741496599 0.83328125
9.18367346938775 0.8415625
9.52380952380952 0.85015625
9.86394557823129 0.86
10.2040816326531 0.87015625
10.5442176870748 0.86734375
10.8843537414966 0.87359375
11.2244897959184 0.87640625
11.5646258503401 0.88203125
11.9047619047619 0.884375
12.2448979591837 0.886875
12.5850340136054 0.88703125
12.9251700680272 0.89015625
13.265306122449 0.89265625
13.6054421768707 0.8925
13.9455782312925 0.90015625
14.2857142857143 0.8996875
14.6258503401361 0.90671875
14.9659863945578 0.91265625
15.3061224489796 0.91484375
15.6462585034014 0.91640625
15.9863945578231 0.91703125
16.3265306122449 0.91921875
16.6666666666667 0.92015625
17.0068027210884 0.92078125
17.3469387755102 0.9165625
17.687074829932 0.915625
18.0272108843537 0.91546875
18.3673469387755 0.91953125
18.7074829931973 0.9165625
19.047619047619 0.91578125
19.3877551020408 0.9146875
19.7278911564626 0.91390625
20.0680272108844 0.91234375
20.4081632653061 0.9134375
20.7482993197279 0.913125
21.0884353741497 0.9159375
21.4285714285714 0.91734375
21.7687074829932 0.91578125
22.108843537415 0.91453125
22.4489795918367 0.915
22.7891156462585 0.91046875
23.1292517006803 0.9115625
23.469387755102 0.91546875
23.8095238095238 0.91375
24.1496598639456 0.9128125
24.4897959183673 0.91359375
24.8299319727891 0.915625
25.1700680272109 0.91625
25.5102040816327 0.9175
25.8503401360544 0.9134375
26.1904761904762 0.9071875
26.530612244898 0.90890625
26.8707482993197 0.91
27.2108843537415 0.90109375
27.5510204081633 0.899375
27.891156462585 0.89765625
28.2312925170068 0.89171875
28.5714285714286 0.88421875
28.9115646258503 0.890625
29.2517006802721 0.8878125
29.5918367346939 0.88484375
29.9319727891156 0.886875
30.2721088435374 0.8840625
30.6122448979592 0.881875
30.952380952381 0.8796875
31.2925170068027 0.8815625
31.6326530612245 0.8828125
31.9727891156463 0.88203125
32.312925170068 0.8815625
32.6530612244898 0.88390625
32.9931972789116 0.8859375
33.3333333333333 0.8821875
33.6734693877551 0.87859375
34.0136054421769 0.879375
34.3537414965986 0.88140625
34.6938775510204 0.87765625
35.0340136054422 0.87484375
35.3741496598639 0.87765625
35.7142857142857 0.8784375
36.0544217687075 0.87765625
36.3945578231292 0.87609375
36.734693877551 0.8759375
37.0748299319728 0.87734375
37.4149659863946 0.87296875
37.7551020408163 0.868125
38.0952380952381 0.87015625
38.4353741496599 0.87078125
38.7755102040816 0.86828125
39.1156462585034 0.87109375
39.4557823129252 0.8678125
39.7959183673469 0.8675
40.1360544217687 0.86421875
40.4761904761905 0.86265625
40.8163265306122 0.861875
41.156462585034 0.86125
41.4965986394558 0.8590625
41.8367346938776 0.8609375
42.1768707482993 0.85875
42.5170068027211 0.8609375
42.8571428571429 0.8625
43.1972789115646 0.85875
43.5374149659864 0.85859375
43.8775510204082 0.86
44.2176870748299 0.8609375
44.5578231292517 0.85984375
44.8979591836735 0.85875
45.2380952380952 0.86328125
45.578231292517 0.86109375
45.9183673469388 0.86140625
46.2585034013605 0.8609375
46.5986394557823 0.85984375
46.9387755102041 0.85578125
47.2789115646259 0.856875
47.6190476190476 0.85609375
47.9591836734694 0.8534375
48.2993197278912 0.8525
48.6394557823129 0.8534375
48.9795918367347 0.85375
49.3197278911565 0.8559375
49.6598639455782 0.85625
50 0.8540625
50.3401360544218 0.8559375
50.6802721088435 0.85671875
51.0204081632653 0.8575
51.3605442176871 0.8571875
51.7006802721088 0.85796875
52.0408163265306 0.8559375
52.3809523809524 0.85328125
52.7210884353741 0.85234375
53.0612244897959 0.85390625
53.4013605442177 0.8534375
53.7414965986395 0.85109375
54.0816326530612 0.855
54.421768707483 0.85171875
54.7619047619048 0.8553125
55.1020408163265 0.85390625
55.4421768707483 0.85453125
55.7823129251701 0.85625
56.1224489795918 0.85359375
56.4625850340136 0.85671875
56.8027210884354 0.8525
57.1428571428571 0.85859375
57.4829931972789 0.8584375
57.8231292517007 0.866875
58.1632653061224 0.861875
58.5034013605442 0.85828125
58.843537414966 0.86125
59.1836734693878 0.86328125
59.5238095238095 0.86078125
59.8639455782313 0.8584375
60.2040816326531 0.86359375
60.5442176870748 0.86609375
60.8843537414966 0.86359375
61.2244897959184 0.86421875
61.5646258503401 0.86375
61.9047619047619 0.8675
62.2448979591837 0.86390625
62.5850340136054 0.861875
62.9251700680272 0.865
63.265306122449 0.8590625
63.6054421768707 0.85953125
63.9455782312925 0.85828125
64.2857142857143 0.86046875
64.6258503401361 0.85828125
64.9659863945578 0.8571875
65.3061224489796 0.8596875
65.6462585034014 0.85953125
65.9863945578231 0.8603125
66.3265306122449 0.86078125
66.6666666666667 0.85671875
67.0068027210884 0.859375
67.3469387755102 0.8565625
67.687074829932 0.85703125
68.0272108843537 0.8575
68.3673469387755 0.85640625
68.7074829931973 0.85390625
69.0476190476191 0.853125
69.3877551020408 0.8584375
69.7278911564626 0.85765625
70.0680272108844 0.858125
70.4081632653061 0.8584375
70.7482993197279 0.8625
71.0884353741497 0.8628125
71.4285714285714 0.86625
71.7687074829932 0.86734375
72.108843537415 0.86984375
72.4489795918367 0.86703125
72.7891156462585 0.87140625
73.1292517006803 0.87359375
73.469387755102 0.87140625
73.8095238095238 0.87078125
74.1496598639456 0.87625
74.4897959183673 0.87453125
74.8299319727891 0.87640625
75.1700680272109 0.87703125
75.5102040816327 0.87828125
75.8503401360544 0.87375
76.1904761904762 0.88140625
76.530612244898 0.8871875
76.8707482993197 0.88421875
77.2108843537415 0.88421875
77.5510204081633 0.8834375
77.891156462585 0.88421875
78.2312925170068 0.8884375
78.5714285714286 0.88671875
78.9115646258503 0.89546875
79.2517006802721 0.8940625
79.5918367346939 0.895625
79.9319727891156 0.89984375
80.2721088435374 0.90390625
80.6122448979592 0.9075
80.9523809523809 0.91
81.2925170068027 0.9109375
81.6326530612245 0.91
81.9727891156463 0.90765625
82.312925170068 0.90890625
82.6530612244898 0.9146875
82.9931972789116 0.9171875
83.3333333333333 0.91234375
83.6734693877551 0.91796875
84.0136054421769 0.9175
84.3537414965986 0.92203125
84.6938775510204 0.92421875
85.0340136054422 0.9296875
85.3741496598639 0.9396875
85.7142857142857 0.9428125
86.0544217687075 0.93953125
86.3945578231292 0.94234375
86.734693877551 0.9409375
87.0748299319728 0.9446875
87.4149659863945 0.94328125
87.7551020408163 0.94765625
88.0952380952381 0.94625
88.4353741496599 0.9465625
88.7755102040816 0.94796875
89.1156462585034 0.94859375
89.4557823129252 0.95140625
89.7959183673469 0.9509375
90.1360544217687 0.95296875
90.4761904761905 0.9534375
90.8163265306122 0.95109375
91.156462585034 0.95390625
91.4965986394558 0.95484375
91.8367346938775 0.95375
92.1768707482993 0.95453125
92.5170068027211 0.9553125
92.8571428571429 0.95828125
93.1972789115646 0.9559375
93.5374149659864 0.9559375
93.8775510204082 0.96109375
94.2176870748299 0.95875
94.5578231292517 0.96171875
94.8979591836735 0.9596875
95.2380952380952 0.9621875
95.578231292517 0.9628125
95.9183673469388 0.96203125
96.2585034013605 0.96046875
96.5986394557823 0.9615625
96.9387755102041 0.960625
97.2789115646258 0.9590625
97.6190476190476 0.95984375
97.9591836734694 0.95984375
98.2993197278912 0.96078125
98.6394557823129 0.9609375
98.9795918367347 0.96109375
99.3197278911565 0.963125
99.6598639455782 0.96765625
100 0.98
};
\path [fill=color1, fill opacity=0.25]
(axis cs:0,0.0841895264001195)
--(axis cs:0,0.0698729735998805)
--(axis cs:0.340136054421769,0.0718102348204379)
--(axis cs:0.680272108843537,0.0862086923965187)
--(axis cs:1.02040816326531,0.160016752834412)
--(axis cs:1.36054421768707,0.212374026072638)
--(axis cs:1.70068027210884,0.258654073549017)
--(axis cs:2.04081632653061,0.317404826714352)
--(axis cs:2.38095238095238,0.36469364665108)
--(axis cs:2.72108843537415,0.415898689193038)
--(axis cs:3.06122448979592,0.456778980462489)
--(axis cs:3.40136054421769,0.499074199540314)
--(axis cs:3.74149659863946,0.548779774300366)
--(axis cs:4.08163265306122,0.58644290848769)
--(axis cs:4.42176870748299,0.618753548401529)
--(axis cs:4.76190476190476,0.641482184151923)
--(axis cs:5.10204081632653,0.665425125781125)
--(axis cs:5.4421768707483,0.684778432617284)
--(axis cs:5.78231292517007,0.708536181733115)
--(axis cs:6.12244897959184,0.730612433226127)
--(axis cs:6.46258503401361,0.746929544844396)
--(axis cs:6.80272108843537,0.75593910920283)
--(axis cs:7.14285714285714,0.766076527710508)
--(axis cs:7.48299319727891,0.768420626130124)
--(axis cs:7.82312925170068,0.776198260213335)
--(axis cs:8.16326530612245,0.787817383575678)
--(axis cs:8.50340136054422,0.802798191099542)
--(axis cs:8.84353741496599,0.817353099498653)
--(axis cs:9.18367346938775,0.825443597098074)
--(axis cs:9.52380952380952,0.834188631877963)
--(axis cs:9.86394557823129,0.844703152930312)
--(axis cs:10.2040816326531,0.855505534031367)
--(axis cs:10.5442176870748,0.853053533718499)
--(axis cs:10.8843537414966,0.859349656107603)
--(axis cs:11.2244897959184,0.86231360381869)
--(axis cs:11.5646258503401,0.869015096869771)
--(axis cs:11.9047619047619,0.871468109220659)
--(axis cs:12.2448979591837,0.874750670776045)
--(axis cs:12.5850340136054,0.874251706710642)
--(axis cs:12.9251700680272,0.877677248472395)
--(axis cs:13.265306122449,0.880202493374903)
--(axis cs:13.6054421768707,0.880329351092722)
--(axis cs:13.9455782312925,0.887335728620874)
--(axis cs:14.2857142857143,0.887126613132177)
--(axis cs:14.6258503401361,0.894407476341014)
--(axis cs:14.9659863945578,0.899920062796699)
--(axis cs:15.3061224489796,0.902551857470847)
--(axis cs:15.6462585034014,0.904288608542312)
--(axis cs:15.9863945578231,0.905031446458517)
--(axis cs:16.3265306122449,0.907059468389952)
--(axis cs:16.6666666666667,0.907477098627901)
--(axis cs:17.0068027210884,0.908068296511476)
--(axis cs:17.3469387755102,0.904161309723915)
--(axis cs:17.687074829932,0.902854041477172)
--(axis cs:18.0272108843537,0.90241601401761)
--(axis cs:18.3673469387755,0.906948743363141)
--(axis cs:18.7074829931973,0.903781091220042)
--(axis cs:19.047619047619,0.903122423222382)
--(axis cs:19.3877551020408,0.902501972064598)
--(axis cs:19.7278911564626,0.901384525104429)
--(axis cs:20.0680272108844,0.89976730831819)
--(axis cs:20.4081632653061,0.900314447456607)
--(axis cs:20.7482993197279,0.899785713888852)
--(axis cs:21.0884353741497,0.903288093816046)
--(axis cs:21.4285714285714,0.904971431521785)
--(axis cs:21.7687074829932,0.903108869870772)
--(axis cs:22.108843537415,0.902141215508042)
--(axis cs:22.4489795918367,0.90315658755016)
--(axis cs:22.7891156462585,0.899030455569982)
--(axis cs:23.1292517006803,0.899277204020071)
--(axis cs:23.469387755102,0.903007338003744)
--(axis cs:23.8095238095238,0.901493459773643)
--(axis cs:24.1496598639456,0.900148024229831)
--(axis cs:24.4897959183673,0.901399225156562)
--(axis cs:24.8299319727891,0.90263341501134)
--(axis cs:25.1700680272109,0.903092111286365)
--(axis cs:25.5102040816327,0.904803936320301)
--(axis cs:25.8503401360544,0.899900216053779)
--(axis cs:26.1904761904762,0.893475227094947)
--(axis cs:26.530612244898,0.894570724950586)
--(axis cs:26.8707482993197,0.895599096665636)
--(axis cs:27.2108843537415,0.886566582709797)
--(axis cs:27.5510204081633,0.885236749163395)
--(axis cs:27.891156462585,0.883664798076461)
--(axis cs:28.2312925170068,0.877216550270405)
--(axis cs:28.5714285714286,0.87014099948039)
--(axis cs:28.9115646258503,0.876519163995885)
--(axis cs:29.2517006802721,0.874554247852752)
--(axis cs:29.5918367346939,0.871885608277915)
--(axis cs:29.9319727891156,0.873672250606304)
--(axis cs:30.2721088435374,0.871432711159243)
--(axis cs:30.6122448979592,0.868860678711752)
--(axis cs:30.952380952381,0.867267866996745)
--(axis cs:31.2925170068027,0.868945554375383)
--(axis cs:31.6326530612245,0.869879774006949)
--(axis cs:31.9727891156463,0.868825972692996)
--(axis cs:32.312925170068,0.868601046857002)
--(axis cs:32.6530612244898,0.871367780752936)
--(axis cs:32.9931972789116,0.873985875043061)
--(axis cs:33.3333333333333,0.86961826425331)
--(axis cs:33.6734693877551,0.865076558639356)
--(axis cs:34.0136054421769,0.866155647453892)
--(axis cs:34.3537414965986,0.86795412371684)
--(axis cs:34.6938775510204,0.864187119916362)
--(axis cs:35.0340136054422,0.860713933364967)
--(axis cs:35.3741496598639,0.863725593639099)
--(axis cs:35.7142857142857,0.863999559285339)
--(axis cs:36.0544217687075,0.863019861726442)
--(axis cs:36.3945578231292,0.862260646530897)
--(axis cs:36.734693877551,0.862045576638998)
--(axis cs:37.0748299319728,0.863253810949518)
--(axis cs:37.4149659863946,0.858650531961506)
--(axis cs:37.7551020408163,0.853617211690583)
--(axis cs:38.0952380952381,0.855896765401987)
--(axis cs:38.4353741496599,0.856769364633692)
--(axis cs:38.7755102040816,0.854189280552642)
--(axis cs:39.1156462585034,0.857487251734688)
--(axis cs:39.4557823129252,0.85406410920283)
--(axis cs:39.7959183673469,0.853319989673096)
--(axis cs:40.1360544217687,0.851290818071412)
--(axis cs:40.4761904761905,0.849323042234376)
--(axis cs:40.8163265306122,0.849718463812816)
--(axis cs:41.156462585034,0.84980295448274)
--(axis cs:41.4965986394558,0.848080621560829)
--(axis cs:41.8367346938776,0.848900005425348)
--(axis cs:42.1768707482993,0.847485191766345)
--(axis cs:42.5170068027211,0.849322562686401)
--(axis cs:42.8571428571429,0.850445088455987)
--(axis cs:43.1972789115646,0.847294626329207)
--(axis cs:43.5374149659864,0.847501702237771)
--(axis cs:43.8775510204082,0.848073136999397)
--(axis cs:44.2176870748299,0.849252979678792)
--(axis cs:44.5578231292517,0.847720600702009)
--(axis cs:44.8979591836735,0.846837538529706)
--(axis cs:45.2380952380952,0.851222778993174)
--(axis cs:45.578231292517,0.847508294893376)
--(axis cs:45.9183673469388,0.848621484022914)
--(axis cs:46.2585034013605,0.847464476234536)
--(axis cs:46.5986394557823,0.845892571152485)
--(axis cs:46.9387755102041,0.842420889907482)
--(axis cs:47.2789115646259,0.843798540045883)
--(axis cs:47.6190476190476,0.842765550012117)
--(axis cs:47.9591836734694,0.840139744860577)
--(axis cs:48.2993197278912,0.839465176786357)
--(axis cs:48.6394557823129,0.839477095876165)
--(axis cs:48.9795918367347,0.839624571140014)
--(axis cs:49.3197278911565,0.842124058820245)
--(axis cs:49.6598639455782,0.8429429249243)
--(axis cs:50,0.840457053119634)
--(axis cs:50.3401360544218,0.842482183867461)
--(axis cs:50.6802721088435,0.843058389335244)
--(axis cs:51.0204081632653,0.843620439059031)
--(axis cs:51.3605442176871,0.845117566753531)
--(axis cs:51.7006802721088,0.845930067104257)
--(axis cs:52.0408163265306,0.843896044811095)
--(axis cs:52.3809523809524,0.840586313106518)
--(axis cs:52.7210884353741,0.83990378491471)
--(axis cs:53.0612244897959,0.841518524855611)
--(axis cs:53.4013605442177,0.841413481272171)
--(axis cs:53.7414965986395,0.838460563669917)
--(axis cs:54.0816326530612,0.84254892386679)
--(axis cs:54.421768707483,0.839171156888351)
--(axis cs:54.7619047619048,0.842976076392969)
--(axis cs:55.1020408163265,0.841225594398287)
--(axis cs:55.4421768707483,0.842448286741816)
--(axis cs:55.7823129251701,0.844235502734977)
--(axis cs:56.1224489795918,0.841521051636487)
--(axis cs:56.4625850340136,0.845365817169127)
--(axis cs:56.8027210884354,0.840539600865317)
--(axis cs:57.1428571428571,0.846964452737931)
--(axis cs:57.4829931972789,0.846771767063267)
--(axis cs:57.8231292517007,0.856437195925088)
--(axis cs:58.1632653061224,0.850624593106317)
--(axis cs:58.5034013605442,0.847164296520603)
--(axis cs:58.843537414966,0.851263245772035)
--(axis cs:59.1836734693878,0.85200163606371)
--(axis cs:59.5238095238095,0.850303776518214)
--(axis cs:59.8639455782313,0.848573735315065)
--(axis cs:60.2040816326531,0.853235280164215)
--(axis cs:60.5442176870748,0.855508515215898)
--(axis cs:60.8843537414966,0.853783792035332)
--(axis cs:61.2244897959184,0.854092121773233)
--(axis cs:61.5646258503401,0.853457568651363)
--(axis cs:61.9047619047619,0.858076298373582)
--(axis cs:62.2448979591837,0.853598541448104)
--(axis cs:62.5850340136054,0.850848921737287)
--(axis cs:62.9251700680272,0.854384626373671)
--(axis cs:63.265306122449,0.84828220537521)
--(axis cs:63.6054421768707,0.848503874424417)
--(axis cs:63.9455782312925,0.847540394258689)
--(axis cs:64.2857142857143,0.850317665826982)
--(axis cs:64.6258503401361,0.847466068313721)
--(axis cs:64.9659863945578,0.847022802491493)
--(axis cs:65.3061224489796,0.850350214205624)
--(axis cs:65.6462585034014,0.850121220229679)
--(axis cs:65.9863945578231,0.850560556458735)
--(axis cs:66.3265306122449,0.850901545232944)
--(axis cs:66.6666666666667,0.847339173480323)
--(axis cs:67.0068027210884,0.850440653897279)
--(axis cs:67.3469387755102,0.847348592704694)
--(axis cs:67.687074829932,0.849022842057199)
--(axis cs:68.0272108843537,0.84904497624144)
--(axis cs:68.3673469387755,0.848128478582898)
--(axis cs:68.7074829931973,0.845539098061175)
--(axis cs:69.0476190476191,0.845409538197225)
--(axis cs:69.3877551020408,0.850879385714496)
--(axis cs:69.7278911564626,0.850002217516607)
--(axis cs:70.0680272108844,0.850357797333926)
--(axis cs:70.4081632653061,0.850736885154798)
--(axis cs:70.7482993197279,0.854550757255872)
--(axis cs:71.0884353741497,0.855689616199683)
--(axis cs:71.4285714285714,0.859587868007496)
--(axis cs:71.7687074829932,0.859864913281818)
--(axis cs:72.108843537415,0.8618317703297)
--(axis cs:72.4489795918367,0.859866315356045)
--(axis cs:72.7891156462585,0.863075650981629)
--(axis cs:73.1292517006803,0.864686664821232)
--(axis cs:73.469387755102,0.863037958355124)
--(axis cs:73.8095238095238,0.862204718065447)
--(axis cs:74.1496598639456,0.866651826269292)
--(axis cs:74.4897959183673,0.865278610193772)
--(axis cs:74.8299319727891,0.866652839670196)
--(axis cs:75.1700680272109,0.867025891785865)
--(axis cs:75.5102040816327,0.868378405461381)
--(axis cs:75.8503401360544,0.864021555152022)
--(axis cs:76.1904761904762,0.871952741646461)
--(axis cs:76.530612244898,0.878680749320163)
--(axis cs:76.8707482993197,0.875083322290872)
--(axis cs:77.2108843537415,0.874571518452137)
--(axis cs:77.5510204081633,0.873333027113478)
--(axis cs:77.891156462585,0.87402921994081)
--(axis cs:78.2312925170068,0.877593697935554)
--(axis cs:78.5714285714286,0.875037086679455)
--(axis cs:78.9115646258503,0.884146098439765)
--(axis cs:79.2517006802721,0.882823118346583)
--(axis cs:79.5918367346939,0.884630970581205)
--(axis cs:79.9319727891156,0.888395454873488)
--(axis cs:80.2721088435374,0.892996250392729)
--(axis cs:80.6122448979592,0.896676444529299)
--(axis cs:80.9523809523809,0.898856912636253)
--(axis cs:81.2925170068027,0.900057699627183)
--(axis cs:81.6326530612245,0.899092185933248)
--(axis cs:81.9727891156463,0.897114349408037)
--(axis cs:82.312925170068,0.89818405624859)
--(axis cs:82.6530612244898,0.90438025406097)
--(axis cs:82.9931972789116,0.90649336029531)
--(axis cs:83.3333333333333,0.900673521676356)
--(axis cs:83.6734693877551,0.906646940742281)
--(axis cs:84.0136054421769,0.90648690327108)
--(axis cs:84.3537414965986,0.910220494636318)
--(axis cs:84.6938775510204,0.912599297647431)
--(axis cs:85.0340136054422,0.918496588007206)
--(axis cs:85.3741496598639,0.930415811756705)
--(axis cs:85.7142857142857,0.933572752990223)
--(axis cs:86.0544217687075,0.92970186828012)
--(axis cs:86.3945578231292,0.932660011283356)
--(axis cs:86.734693877551,0.931129000367586)
--(axis cs:87.0748299319728,0.935186194258629)
--(axis cs:87.4149659863945,0.934157312742483)
--(axis cs:87.7551020408163,0.939577887946237)
--(axis cs:88.0952380952381,0.937603147022977)
--(axis cs:88.4353741496599,0.938640898519268)
--(axis cs:88.7755102040816,0.940292322705305)
--(axis cs:89.1156462585034,0.94090987227266)
--(axis cs:89.4557823129252,0.943785933134805)
--(axis cs:89.7959183673469,0.943488689911904)
--(axis cs:90.1360544217687,0.945712555473336)
--(axis cs:90.4761904761905,0.946318633996638)
--(axis cs:90.8163265306122,0.943253832290458)
--(axis cs:91.156462585034,0.945970815852311)
--(axis cs:91.4965986394558,0.947535172952317)
--(axis cs:91.8367346938775,0.945631011839521)
--(axis cs:92.1768707482993,0.945597437625653)
--(axis cs:92.5170068027211,0.946342998044371)
--(axis cs:92.8571428571429,0.948917955712879)
--(axis cs:93.1972789115646,0.946640132628584)
--(axis cs:93.5374149659864,0.946396129540567)
--(axis cs:93.8775510204082,0.951943718948834)
--(axis cs:94.2176870748299,0.949118103120361)
--(axis cs:94.5578231292517,0.952401402039209)
--(axis cs:94.8979591836735,0.950349192900092)
--(axis cs:95.2380952380952,0.954152342800498)
--(axis cs:95.578231292517,0.954587315746388)
--(axis cs:95.9183673469388,0.954534582242535)
--(axis cs:96.2585034013605,0.95261424864547)
--(axis cs:96.5986394557823,0.955381545938107)
--(axis cs:96.9387755102041,0.955840840346127)
--(axis cs:97.2789115646258,0.955615358868218)
--(axis cs:97.6190476190476,0.955948501821254)
--(axis cs:97.9591836734694,0.956951739668953)
--(axis cs:98.2993197278912,0.95834375313001)
--(axis cs:98.6394557823129,0.958295361472955)
--(axis cs:98.9795918367347,0.958251634333817)
--(axis cs:99.3197278911565,0.958586347641163)
--(axis cs:99.6598639455782,0.961459116410857)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:99.6598639455782,0.973853383589143)
--(axis cs:99.3197278911565,0.967663652358837)
--(axis cs:98.9795918367347,0.963935865666183)
--(axis cs:98.6394557823129,0.963579638527045)
--(axis cs:98.2993197278912,0.96321874686999)
--(axis cs:97.9591836734694,0.962735760331047)
--(axis cs:97.6190476190476,0.963738998178746)
--(axis cs:97.2789115646258,0.962509641131782)
--(axis cs:96.9387755102041,0.965409159653873)
--(axis cs:96.5986394557823,0.967743454061893)
--(axis cs:96.2585034013605,0.96832325135453)
--(axis cs:95.9183673469388,0.969527917757465)
--(axis cs:95.578231292517,0.971037684253611)
--(axis cs:95.2380952380952,0.970222657199502)
--(axis cs:94.8979591836735,0.969025807099908)
--(axis cs:94.5578231292517,0.971036097960791)
--(axis cs:94.2176870748299,0.968381896879639)
--(axis cs:93.8775510204082,0.970243781051166)
--(axis cs:93.5374149659864,0.965478870459433)
--(axis cs:93.1972789115646,0.965234867371416)
--(axis cs:92.8571428571429,0.967644544287121)
--(axis cs:92.5170068027211,0.964282001955629)
--(axis cs:92.1768707482993,0.963465062374347)
--(axis cs:91.8367346938775,0.961868988160479)
--(axis cs:91.4965986394558,0.962152327047683)
--(axis cs:91.156462585034,0.961841684147689)
--(axis cs:90.8163265306122,0.958933667709541)
--(axis cs:90.4761904761905,0.960556366003362)
--(axis cs:90.1360544217687,0.960224944526664)
--(axis cs:89.7959183673469,0.958386310088096)
--(axis cs:89.4557823129252,0.959026566865195)
--(axis cs:89.1156462585034,0.95627762772734)
--(axis cs:88.7755102040816,0.955645177294695)
--(axis cs:88.4353741496599,0.954484101480732)
--(axis cs:88.0952380952381,0.954896852977023)
--(axis cs:87.7551020408163,0.955734612053763)
--(axis cs:87.4149659863945,0.952405187257517)
--(axis cs:87.0748299319728,0.954188805741371)
--(axis cs:86.734693877551,0.950745999632414)
--(axis cs:86.3945578231292,0.952027488716644)
--(axis cs:86.0544217687075,0.94936063171988)
--(axis cs:85.7142857142857,0.952052247009777)
--(axis cs:85.3741496598639,0.948959188243295)
--(axis cs:85.0340136054422,0.940878411992794)
--(axis cs:84.6938775510204,0.935838202352569)
--(axis cs:84.3537414965986,0.933842005363682)
--(axis cs:84.0136054421769,0.92851309672892)
--(axis cs:83.6734693877551,0.929290559257719)
--(axis cs:83.3333333333333,0.924013978323644)
--(axis cs:82.9931972789116,0.927881639704691)
--(axis cs:82.6530612244898,0.92499474593903)
--(axis cs:82.312925170068,0.91962844375141)
--(axis cs:81.9727891156463,0.918198150591963)
--(axis cs:81.6326530612245,0.920907814066752)
--(axis cs:81.2925170068027,0.921817300372817)
--(axis cs:80.9523809523809,0.921143087363747)
--(axis cs:80.6122448979592,0.918323555470701)
--(axis cs:80.2721088435374,0.914816249607271)
--(axis cs:79.9319727891156,0.911292045126512)
--(axis cs:79.5918367346939,0.906619029418795)
--(axis cs:79.2517006802721,0.905301881653417)
--(axis cs:78.9115646258503,0.906791401560235)
--(axis cs:78.5714285714286,0.898400413320545)
--(axis cs:78.2312925170068,0.899281302064446)
--(axis cs:77.891156462585,0.894408280059191)
--(axis cs:77.5510204081633,0.893541972886522)
--(axis cs:77.2108843537415,0.893865981547863)
--(axis cs:76.8707482993197,0.893354177709129)
--(axis cs:76.530612244898,0.895694250679837)
--(axis cs:76.1904761904762,0.890859758353539)
--(axis cs:75.8503401360544,0.883478444847978)
--(axis cs:75.5102040816327,0.888184094538619)
--(axis cs:75.1700680272109,0.887036608214135)
--(axis cs:74.8299319727891,0.886159660329804)
--(axis cs:74.4897959183673,0.883783889806228)
--(axis cs:74.1496598639456,0.885848173730707)
--(axis cs:73.8095238095238,0.879357781934553)
--(axis cs:73.469387755102,0.879774541644877)
--(axis cs:73.1292517006803,0.882500835178768)
--(axis cs:72.7891156462585,0.879736849018371)
--(axis cs:72.4489795918367,0.874196184643955)
--(axis cs:72.108843537415,0.8778557296703)
--(axis cs:71.7687074829932,0.874822586718182)
--(axis cs:71.4285714285714,0.872912131992504)
--(axis cs:71.0884353741497,0.869935383800317)
--(axis cs:70.7482993197279,0.870449242744128)
--(axis cs:70.4081632653061,0.866138114845202)
--(axis cs:70.0680272108844,0.865892202666074)
--(axis cs:69.7278911564626,0.865310282483393)
--(axis cs:69.3877551020408,0.865995614285504)
--(axis cs:69.0476190476191,0.860840461802775)
--(axis cs:68.7074829931973,0.862273401938825)
--(axis cs:68.3673469387755,0.864684021417102)
--(axis cs:68.0272108843537,0.86595502375856)
--(axis cs:67.687074829932,0.865039657942801)
--(axis cs:67.3469387755102,0.865776407295306)
--(axis cs:67.0068027210884,0.868309346102721)
--(axis cs:66.6666666666667,0.866098326519677)
--(axis cs:66.3265306122449,0.870660954767056)
--(axis cs:65.9863945578231,0.870064443541266)
--(axis cs:65.6462585034014,0.868941279770321)
--(axis cs:65.3061224489796,0.869024785794376)
--(axis cs:64.9659863945578,0.867352197508507)
--(axis cs:64.6258503401361,0.869096431686279)
--(axis cs:64.2857142857143,0.870619834173018)
--(axis cs:63.9455782312925,0.869022105741311)
--(axis cs:63.6054421768707,0.870558625575583)
--(axis cs:63.265306122449,0.869842794624789)
--(axis cs:62.9251700680272,0.875615373626329)
--(axis cs:62.5850340136054,0.872901078262713)
--(axis cs:62.2448979591837,0.874213958551896)
--(axis cs:61.9047619047619,0.876923701626418)
--(axis cs:61.5646258503401,0.874042431348637)
--(axis cs:61.2244897959184,0.874345378226768)
--(axis cs:60.8843537414966,0.873403707964668)
--(axis cs:60.5442176870748,0.876678984784102)
--(axis cs:60.2040816326531,0.873952219835785)
--(axis cs:59.8639455782313,0.868301264684935)
--(axis cs:59.5238095238095,0.871258723481786)
--(axis cs:59.1836734693878,0.87456086393629)
--(axis cs:58.843537414966,0.871236754227964)
--(axis cs:58.5034013605442,0.869398203479397)
--(axis cs:58.1632653061224,0.873125406893683)
--(axis cs:57.8231292517007,0.877312804074912)
--(axis cs:57.4829931972789,0.870103232936733)
--(axis cs:57.1428571428571,0.870223047262069)
--(axis cs:56.8027210884354,0.864460399134684)
--(axis cs:56.4625850340136,0.868071682830873)
--(axis cs:56.1224489795918,0.865666448363513)
--(axis cs:55.7823129251701,0.868264497265023)
--(axis cs:55.4421768707483,0.866614213258184)
--(axis cs:55.1020408163265,0.866586905601713)
--(axis cs:54.7619047619048,0.867648923607031)
--(axis cs:54.421768707483,0.864266343111649)
--(axis cs:54.0816326530612,0.86745107613321)
--(axis cs:53.7414965986395,0.863726936330083)
--(axis cs:53.4013605442177,0.865461518727829)
--(axis cs:53.0612244897959,0.866293975144389)
--(axis cs:52.7210884353741,0.86478371508529)
--(axis cs:52.3809523809524,0.865976186893482)
--(axis cs:52.0408163265306,0.867978955188905)
--(axis cs:51.7006802721088,0.870007432895743)
--(axis cs:51.3605442176871,0.869257433246469)
--(axis cs:51.0204081632653,0.871379560940969)
--(axis cs:50.6802721088435,0.870379110664756)
--(axis cs:50.3401360544218,0.869392816132539)
--(axis cs:50,0.867667946880366)
--(axis cs:49.6598639455782,0.8695570750757)
--(axis cs:49.3197278911565,0.869750941179755)
--(axis cs:48.9795918367347,0.867875428859986)
--(axis cs:48.6394557823129,0.867397904123835)
--(axis cs:48.2993197278912,0.865534823213644)
--(axis cs:47.9591836734694,0.866735255139423)
--(axis cs:47.6190476190476,0.869421949987883)
--(axis cs:47.2789115646259,0.869951459954118)
--(axis cs:46.9387755102041,0.869141610092518)
--(axis cs:46.5986394557823,0.873794928847515)
--(axis cs:46.2585034013605,0.874410523765464)
--(axis cs:45.9183673469388,0.874191015977086)
--(axis cs:45.578231292517,0.874679205106624)
--(axis cs:45.2380952380952,0.875339721006826)
--(axis cs:44.8979591836735,0.870662461470294)
--(axis cs:44.5578231292517,0.871966899297991)
--(axis cs:44.2176870748299,0.872622020321208)
--(axis cs:43.8775510204082,0.871926863000603)
--(axis cs:43.5374149659864,0.869685797762229)
--(axis cs:43.1972789115646,0.870205373670793)
--(axis cs:42.8571428571429,0.874554911544013)
--(axis cs:42.5170068027211,0.872552437313599)
--(axis cs:42.1768707482993,0.870014808233655)
--(axis cs:41.8367346938776,0.872974994574652)
--(axis cs:41.4965986394558,0.870044378439171)
--(axis cs:41.156462585034,0.87269704551726)
--(axis cs:40.8163265306122,0.874031536187184)
--(axis cs:40.4761904761905,0.875989457765624)
--(axis cs:40.1360544217687,0.877146681928588)
--(axis cs:39.7959183673469,0.881680010326904)
--(axis cs:39.4557823129252,0.88156089079717)
--(axis cs:39.1156462585034,0.884700248265312)
--(axis cs:38.7755102040816,0.882373219447358)
--(axis cs:38.4353741496599,0.884793135366308)
--(axis cs:38.0952380952381,0.884415734598013)
--(axis cs:37.7551020408163,0.882632788309417)
--(axis cs:37.4149659863946,0.887286968038494)
--(axis cs:37.0748299319728,0.891433689050482)
--(axis cs:36.734693877551,0.889829423361003)
--(axis cs:36.3945578231292,0.889926853469103)
--(axis cs:36.0544217687075,0.892292638273558)
--(axis cs:35.7142857142857,0.892875440714661)
--(axis cs:35.3741496598639,0.891586906360901)
--(axis cs:35.0340136054422,0.888973566635033)
--(axis cs:34.6938775510204,0.891125380083638)
--(axis cs:34.3537414965986,0.89485837628316)
--(axis cs:34.0136054421769,0.892594352546108)
--(axis cs:33.6734693877551,0.892110941360644)
--(axis cs:33.3333333333333,0.89475673574669)
--(axis cs:32.9931972789116,0.897889124956939)
--(axis cs:32.6530612244898,0.896444719247064)
--(axis cs:32.312925170068,0.894523953142998)
--(axis cs:31.9727891156463,0.895236527307004)
--(axis cs:31.6326530612245,0.895745225993051)
--(axis cs:31.2925170068027,0.894179445624617)
--(axis cs:30.952380952381,0.892107133003255)
--(axis cs:30.6122448979592,0.894889321288248)
--(axis cs:30.2721088435374,0.896692288840757)
--(axis cs:29.9319727891156,0.900077749393696)
--(axis cs:29.5918367346939,0.897801891722085)
--(axis cs:29.2517006802721,0.901070752147248)
--(axis cs:28.9115646258503,0.904730836004115)
--(axis cs:28.5714285714286,0.89829650051961)
--(axis cs:28.2312925170068,0.906220949729595)
--(axis cs:27.891156462585,0.911647701923539)
--(axis cs:27.5510204081633,0.913513250836605)
--(axis cs:27.2108843537415,0.915620917290203)
--(axis cs:26.8707482993197,0.924400903334364)
--(axis cs:26.530612244898,0.923241775049414)
--(axis cs:26.1904761904762,0.920899772905053)
--(axis cs:25.8503401360544,0.926974783946221)
--(axis cs:25.5102040816327,0.930196063679699)
--(axis cs:25.1700680272109,0.929407888713635)
--(axis cs:24.8299319727891,0.92861658498866)
--(axis cs:24.4897959183673,0.925788274843438)
--(axis cs:24.1496598639456,0.925476975770169)
--(axis cs:23.8095238095238,0.926006540226357)
--(axis cs:23.469387755102,0.927930161996256)
--(axis cs:23.1292517006803,0.923847795979929)
--(axis cs:22.7891156462585,0.921907044430018)
--(axis cs:22.4489795918367,0.92684341244984)
--(axis cs:22.108843537415,0.926921284491958)
--(axis cs:21.7687074829932,0.928453630129228)
--(axis cs:21.4285714285714,0.929716068478215)
--(axis cs:21.0884353741497,0.928586906183953)
--(axis cs:20.7482993197279,0.926464286111148)
--(axis cs:20.4081632653061,0.926560552543393)
--(axis cs:20.0680272108844,0.92492019168181)
--(axis cs:19.7278911564626,0.926427974895571)
--(axis cs:19.3877551020408,0.926873027935402)
--(axis cs:19.047619047619,0.928440076777618)
--(axis cs:18.7074829931973,0.929343908779958)
--(axis cs:18.3673469387755,0.932113756636859)
--(axis cs:18.0272108843537,0.92852148598239)
--(axis cs:17.687074829932,0.928395958522828)
--(axis cs:17.3469387755102,0.928963690276085)
--(axis cs:17.0068027210884,0.933494203488524)
--(axis cs:16.6666666666667,0.932835401372099)
--(axis cs:16.3265306122449,0.931378031610048)
--(axis cs:15.9863945578231,0.929031053541483)
--(axis cs:15.6462585034014,0.928523891457688)
--(axis cs:15.3061224489796,0.927135642529153)
--(axis cs:14.9659863945578,0.925392437203301)
--(axis cs:14.6258503401361,0.919030023658986)
--(axis cs:14.2857142857143,0.912248386867823)
--(axis cs:13.9455782312925,0.912976771379126)
--(axis cs:13.6054421768707,0.904670648907278)
--(axis cs:13.265306122449,0.905110006625097)
--(axis cs:12.9251700680272,0.902635251527605)
--(axis cs:12.5850340136054,0.899810793289358)
--(axis cs:12.2448979591837,0.898999329223955)
--(axis cs:11.9047619047619,0.897281890779341)
--(axis cs:11.5646258503401,0.895047403130229)
--(axis cs:11.2244897959184,0.89049889618131)
--(axis cs:10.8843537414966,0.887837843892397)
--(axis cs:10.5442176870748,0.881633966281501)
--(axis cs:10.2040816326531,0.884806965968633)
--(axis cs:9.86394557823129,0.875296847069688)
--(axis cs:9.52380952380952,0.866123868122037)
--(axis cs:9.18367346938775,0.857681402901926)
--(axis cs:8.84353741496599,0.849209400501347)
--(axis cs:8.50340136054422,0.833764308900458)
--(axis cs:8.16326530612245,0.819057616424322)
--(axis cs:7.82312925170068,0.806301739786665)
--(axis cs:7.48299319727891,0.796266873869876)
--(axis cs:7.14285714285714,0.792673472289492)
--(axis cs:6.80272108843537,0.78343589079717)
--(axis cs:6.46258503401361,0.774632955155603)
--(axis cs:6.12244897959184,0.760950066773873)
--(axis cs:5.78231292517007,0.740526318266885)
--(axis cs:5.4421768707483,0.716784067382716)
--(axis cs:5.10204081632653,0.695199874218875)
--(axis cs:4.76190476190476,0.671955315848077)
--(axis cs:4.42176870748299,0.652183951598471)
--(axis cs:4.08163265306122,0.62230709151231)
--(axis cs:3.74149659863946,0.586532725699634)
--(axis cs:3.40136054421769,0.535613300459686)
--(axis cs:3.06122448979592,0.491971019537511)
--(axis cs:2.72108843537415,0.453788810806962)
--(axis cs:2.38095238095238,0.40093135334892)
--(axis cs:2.04081632653061,0.351970173285648)
--(axis cs:1.70068027210884,0.290408426450983)
--(axis cs:1.36054421768707,0.241688473927362)
--(axis cs:1.02040816326531,0.193108247165588)
--(axis cs:0.680272108843537,0.114416307603481)
--(axis cs:0.340136054421769,0.0888147651795621)
--(axis cs:0,0.0841895264001195)
--cycle;


==> img/stl10/stl10_rate_accuracy_lagrange.tex <==
\addplot [line width=0.5, opacity=0.7, color4, mark=o, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color4, thin}]
table [row sep=\\]{%
0	0.07671875 \\
0.340136054421769	0.07734375 \\
0.680272108843537	0.07921875 \\
1.02040816326531	0.08375 \\
1.36054421768707	0.116875 \\
1.70068027210884	0.14625 \\
2.04081632653061	0.17140625 \\
2.38095238095238	0.22 \\
2.72108843537415	0.30140625 \\
3.06122448979592	0.36 \\
3.40136054421769	0.39703125 \\
3.74149659863946	0.43609375 \\
4.08163265306122	0.46546875 \\
4.42176870748299	0.4925 \\
4.76190476190476	0.51953125 \\
5.10204081632653	0.5490625 \\
5.4421768707483	0.56953125 \\
5.78231292517007	0.5890625 \\
6.12244897959184	0.60140625 \\
6.46258503401361	0.621875 \\
6.80272108843537	0.6328125 \\
7.14285714285714	0.649375 \\
7.48299319727891	0.66234375 \\
7.82312925170068	0.6715625 \\
8.16326530612245	0.6771875 \\
8.50340136054422	0.67921875 \\
8.84353741496599	0.68125 \\
9.18367346938775	0.67703125 \\
9.52380952380952	0.68234375 \\
9.86394557823129	0.688125 \\
10.2040816326531	0.69203125 \\
10.5442176870748	0.690625 \\
10.8843537414966	0.68765625 \\
11.2244897959184	0.69359375 \\
11.5646258503401	0.6990625 \\
11.9047619047619	0.696875 \\
12.2448979591837	0.7034375 \\
12.5850340136054	0.7003125 \\
12.9251700680272	0.70421875 \\
13.265306122449	0.7125 \\
13.6054421768707	0.7121875 \\
13.9455782312925	0.7046875 \\
14.2857142857143	0.70359375 \\
14.6258503401361	0.70109375 \\
14.9659863945578	0.701875 \\
15.3061224489796	0.70609375 \\
15.6462585034014	0.710625 \\
15.9863945578231	0.7103125 \\
16.3265306122449	0.7096875 \\
16.6666666666667	0.70859375 \\
17.0068027210884	0.70234375 \\
17.3469387755102	0.70703125 \\
17.687074829932	0.7034375 \\
18.0272108843537	0.7021875 \\
18.3673469387755	0.6978125 \\
18.7074829931973	0.704375 \\
19.047619047619	0.700625 \\
19.3877551020408	0.70234375 \\
19.7278911564626	0.70234375 \\
20.0680272108844	0.70078125 \\
20.4081632653061	0.7046875 \\
20.7482993197279	0.70453125 \\
21.0884353741497	0.70359375 \\
21.4285714285714	0.7021875 \\
21.7687074829932	0.705 \\
22.108843537415	0.708125 \\
22.4489795918367	0.70109375 \\
22.7891156462585	0.69859375 \\
23.1292517006803	0.69734375 \\
23.469387755102	0.70015625 \\
23.8095238095238	0.69796875 \\
24.1496598639456	0.69953125 \\
24.4897959183673	0.69625 \\
24.8299319727891	0.6915625 \\
25.1700680272109	0.698125 \\
25.5102040816327	0.69 \\
25.8503401360544	0.69546875 \\
26.1904761904762	0.69421875 \\
26.530612244898	0.69640625 \\
26.8707482993197	0.69109375 \\
27.2108843537415	0.69515625 \\
27.5510204081633	0.6903125 \\
27.891156462585	0.6878125 \\
28.2312925170068	0.686875 \\
28.5714285714286	0.6953125 \\
28.9115646258503	0.68984375 \\
29.2517006802721	0.6940625 \\
29.5918367346939	0.68953125 \\
29.9319727891156	0.696875 \\
30.2721088435374	0.700625 \\
30.6122448979592	0.69609375 \\
30.952380952381	0.69203125 \\
31.2925170068027	0.69171875 \\
31.6326530612245	0.69015625 \\
31.9727891156463	0.69234375 \\
32.312925170068	0.68953125 \\
32.6530612244898	0.6875 \\
32.9931972789116	0.68828125 \\
33.3333333333333	0.69140625 \\
33.6734693877551	0.69421875 \\
34.0136054421769	0.6909375 \\
34.3537414965986	0.6984375 \\
34.6938775510204	0.6884375 \\
35.0340136054422	0.69171875 \\
35.3741496598639	0.69609375 \\
35.7142857142857	0.6965625 \\
36.0544217687075	0.689375 \\
36.3945578231292	0.69921875 \\
36.734693877551	0.69484375 \\
37.0748299319728	0.69484375 \\
37.4149659863946	0.6934375 \\
37.7551020408163	0.695 \\
38.0952380952381	0.6946875 \\
38.4353741496599	0.68875 \\
38.7755102040816	0.6903125 \\
39.1156462585034	0.695 \\
39.4557823129252	0.69140625 \\
39.7959183673469	0.69296875 \\
40.1360544217687	0.6946875 \\
40.4761904761905	0.69078125 \\
40.8163265306122	0.69421875 \\
41.156462585034	0.69265625 \\
41.4965986394558	0.68734375 \\
41.8367346938776	0.69265625 \\
42.1768707482993	0.6909375 \\
42.5170068027211	0.6959375 \\
42.8571428571429	0.6965625 \\
43.1972789115646	0.69234375 \\
43.5374149659864	0.6984375 \\
43.8775510204082	0.69296875 \\
44.2176870748299	0.696875 \\
44.5578231292517	0.6959375 \\
44.8979591836735	0.69890625 \\
45.2380952380952	0.69625 \\
45.578231292517	0.70703125 \\
45.9183673469388	0.69703125 \\
46.2585034013605	0.70171875 \\
46.5986394557823	0.70390625 \\
46.9387755102041	0.70734375 \\
47.2789115646259	0.7028125 \\
47.6190476190476	0.70625 \\
47.9591836734694	0.70859375 \\
48.2993197278912	0.71265625 \\
48.6394557823129	0.71265625 \\
48.9795918367347	0.7121875 \\
49.3197278911565	0.7125 \\
49.6598639455782	0.71203125 \\
50	0.7134375 \\
50.3401360544218	0.7134375 \\
50.6802721088435	0.71703125 \\
51.0204081632653	0.7178125 \\
51.3605442176871	0.723125 \\
51.7006802721088	0.72390625 \\
52.0408163265306	0.72015625 \\
52.3809523809524	0.7228125 \\
52.7210884353741	0.72046875 \\
53.0612244897959	0.721875 \\
53.4013605442177	0.7259375 \\
53.7414965986395	0.723125 \\
54.0816326530612	0.73140625 \\
54.421768707483	0.72859375 \\
54.7619047619048	0.73359375 \\
55.1020408163265	0.73265625 \\
55.4421768707483	0.73265625 \\
55.7823129251701	0.73265625 \\
56.1224489795918	0.73515625 \\
56.4625850340136	0.73328125 \\
56.8027210884354	0.73609375 \\
57.1428571428571	0.74109375 \\
57.4829931972789	0.7396875 \\
57.8231292517007	0.74625 \\
58.1632653061224	0.743125 \\
58.5034013605442	0.7409375 \\
58.843537414966	0.74125 \\
59.1836734693878	0.7471875 \\
59.5238095238095	0.74328125 \\
59.8639455782313	0.74734375 \\
60.2040816326531	0.74984375 \\
60.5442176870748	0.75171875 \\
60.8843537414966	0.761875 \\
61.2244897959184	0.75859375 \\
61.5646258503401	0.75765625 \\
61.9047619047619	0.7578125 \\
62.2448979591837	0.75875 \\
62.5850340136054	0.7596875 \\
62.9251700680272	0.766875 \\
63.265306122449	0.7671875 \\
63.6054421768707	0.76359375 \\
63.9455782312925	0.7675 \\
64.2857142857143	0.769375 \\
64.6258503401361	0.77234375 \\
64.9659863945578	0.7725 \\
65.3061224489796	0.7703125 \\
65.6462585034014	0.76875 \\
65.9863945578231	0.77609375 \\
66.3265306122449	0.773125 \\
66.6666666666667	0.77359375 \\
67.0068027210884	0.77421875 \\
67.3469387755102	0.775 \\
67.687074829932	0.7771875 \\
68.0272108843537	0.78125 \\
68.3673469387755	0.78203125 \\
68.7074829931973	0.785 \\
69.0476190476191	0.78625 \\
69.3877551020408	0.78265625 \\
69.7278911564626	0.7846875 \\
70.0680272108844	0.7790625 \\
70.4081632653061	0.7809375 \\
70.7482993197279	0.78078125 \\
71.0884353741497	0.77921875 \\
71.4285714285714	0.78453125 \\
71.7687074829932	0.783125 \\
72.108843537415	0.7825 \\
72.4489795918367	0.78453125 \\
72.7891156462585	0.77875 \\
73.1292517006803	0.7771875 \\
73.469387755102	0.7765625 \\
73.8095238095238	0.78015625 \\
74.1496598639456	0.7796875 \\
74.4897959183673	0.78390625 \\
74.8299319727891	0.77984375 \\
75.1700680272109	0.7815625 \\
75.5102040816327	0.775 \\
75.8503401360544	0.775625 \\
76.1904761904762	0.77359375 \\
76.530612244898	0.7759375 \\
76.8707482993197	0.77203125 \\
77.2108843537415	0.77640625 \\
77.5510204081633	0.77265625 \\
77.891156462585	0.77515625 \\
78.2312925170068	0.77734375 \\
78.5714285714286	0.77734375 \\
78.9115646258503	0.77453125 \\
79.2517006802721	0.77296875 \\
79.5918367346939	0.775625 \\
79.9319727891156	0.7709375 \\
80.2721088435374	0.7746875 \\
80.6122448979592	0.77375 \\
80.9523809523809	0.77484375 \\
81.2925170068027	0.77859375 \\
81.6326530612245	0.7871875 \\
81.9727891156463	0.784375 \\
82.312925170068	0.7890625 \\
82.6530612244898	0.79328125 \\
82.9931972789116	0.79765625 \\
83.3333333333333	0.8015625 \\
83.6734693877551	0.8065625 \\
84.0136054421769	0.814375 \\
84.3537414965986	0.81203125 \\
84.6938775510204	0.82125 \\
85.0340136054422	0.82890625 \\
85.3741496598639	0.82828125 \\
85.7142857142857	0.835625 \\
86.0544217687075	0.83859375 \\
86.3945578231292	0.84359375 \\
86.734693877551	0.849375 \\
87.0748299319728	0.84953125 \\
87.4149659863945	0.85515625 \\
87.7551020408163	0.86015625 \\
88.0952380952381	0.859375 \\
88.4353741496599	0.86265625 \\
88.7755102040816	0.86484375 \\
89.1156462585034	0.86828125 \\
89.4557823129252	0.8653125 \\
89.7959183673469	0.86984375 \\
90.1360544217687	0.87234375 \\
90.4761904761905	0.878125 \\
90.8163265306122	0.87671875 \\
91.156462585034	0.8796875 \\
91.4965986394558	0.88359375 \\
91.8367346938775	0.889375 \\
92.1768707482993	0.89734375 \\
92.5170068027211	0.9078125 \\
92.8571428571429	0.91140625 \\
93.1972789115646	0.91546875 \\
93.5374149659864	0.91984375 \\
93.8775510204082	0.92421875 \\
94.2176870748299	0.9290625 \\
94.5578231292517	0.92953125 \\
94.8979591836735	0.93140625 \\
95.2380952380952	0.93375 \\
95.578231292517	0.9315625 \\
95.9183673469388	0.9365625 \\
96.2585034013605	0.9384375 \\
96.5986394557823	0.94234375 \\
96.9387755102041	0.9434375 \\
97.2789115646258	0.9565625 \\
97.6190476190476	0.96 \\
97.9591836734694	0.965625 \\
98.2993197278912	0.96625 \\
98.6394557823129	0.96234375 \\
98.9795918367347	0.9565625 \\
99.3197278911565	0.958125 \\
99.6598639455782	0.9603125 \\
100	0.98 \\
};
\path [fill=color4, fill opacity=0.25]
(axis cs:0,0.0837452512175585)
--(axis cs:0,0.0696922487824415)
--(axis cs:0.340136054421769,0.0711466164108574)
--(axis cs:0.680272108843537,0.0750720949715699)
--(axis cs:1.02040816326531,0.0784765625)
--(axis cs:1.36054421768707,0.105909633712798)
--(axis cs:1.70068027210884,0.13471415524934)
--(axis cs:2.04081632653061,0.156454634819399)
--(axis cs:2.38095238095238,0.20080017525435)
--(axis cs:2.72108843537415,0.28116688911271)
--(axis cs:3.06122448979592,0.342192254952089)
--(axis cs:3.40136054421769,0.379327435041441)
--(axis cs:3.74149659863946,0.417664124182092)
--(axis cs:4.08163265306122,0.448828457401354)
--(axis cs:4.42176870748299,0.475826214085615)
--(axis cs:4.76190476190476,0.500880440180875)
--(axis cs:5.10204081632653,0.530045340005206)
--(axis cs:5.4421768707483,0.550550482193908)
--(axis cs:5.78231292517007,0.570155483292922)
--(axis cs:6.12244897959184,0.58299008326684)
--(axis cs:6.46258503401361,0.602172140632986)
--(axis cs:6.80272108843537,0.612299107901883)
--(axis cs:7.14285714285714,0.62958858091086)
--(axis cs:7.48299319727891,0.643065357488002)
--(axis cs:7.82312925170068,0.652821148641776)
--(axis cs:8.16326530612245,0.65909287465686)
--(axis cs:8.50340136054422,0.660791711704158)
--(axis cs:8.84353741496599,0.662988020138899)
--(axis cs:9.18367346938775,0.658211443827509)
--(axis cs:9.52380952380952,0.662852335545765)
--(axis cs:9.86394557823129,0.668254412679075)
--(axis cs:10.2040816326531,0.672278840030962)
--(axis cs:10.5442176870748,0.670439190914711)
--(axis cs:10.8843537414966,0.667189634012125)
--(axis cs:11.2244897959184,0.673190603775594)
--(axis cs:11.5646258503401,0.678856857846049)
--(axis cs:11.9047619047619,0.676358353837057)
--(axis cs:12.2448979591837,0.683082320229095)
--(axis cs:12.5850340136054,0.679383510212497)
--(axis cs:12.9251700680272,0.684026563875334)
--(axis cs:13.265306122449,0.692096152664657)
--(axis cs:13.6054421768707,0.691529567308042)
--(axis cs:13.9455782312925,0.684061908152431)
--(axis cs:14.2857142857143,0.682889934047497)
--(axis cs:14.6258503401361,0.68089164803743)
--(axis cs:14.9659863945578,0.681330482995332)
--(axis cs:15.3061224489796,0.685606641775715)
--(axis cs:15.6462585034014,0.690768816180125)
--(axis cs:15.9863945578231,0.690317516956151)
--(axis cs:16.3265306122449,0.689309375838637)
--(axis cs:16.6666666666667,0.688227094802818)
--(axis cs:17.0068027210884,0.682389588432979)
--(axis cs:17.3469387755102,0.687237843372467)
--(axis cs:17.687074829932,0.683989434957772)
--(axis cs:18.0272108843537,0.682999102983101)
--(axis cs:18.3673469387755,0.678152766355997)
--(axis cs:18.7074829931973,0.684743421745919)
--(axis cs:19.047619047619,0.681074228505872)
--(axis cs:19.3877551020408,0.682084137737223)
--(axis cs:19.7278911564626,0.681823153166351)
--(axis cs:20.0680272108844,0.680732681120009)
--(axis cs:20.4081632653061,0.684607323183633)
--(axis cs:20.7482993197279,0.684389189754276)
--(axis cs:21.0884353741497,0.683112694166101)
--(axis cs:21.4285714285714,0.682019651925719)
--(axis cs:21.7687074829932,0.684727917314055)
--(axis cs:22.108843537415,0.687351516224431)
--(axis cs:22.4489795918367,0.680153599237877)
--(axis cs:22.7891156462585,0.678055964983029)
--(axis cs:23.1292517006803,0.676493511700791)
--(axis cs:23.469387755102,0.679190610749674)
--(axis cs:23.8095238095238,0.676866185652369)
--(axis cs:24.1496598639456,0.678442247713119)
--(axis cs:24.4897959183673,0.674896974671634)
--(axis cs:24.8299319727891,0.670273885469163)
--(axis cs:25.1700680272109,0.677030345794843)
--(axis cs:25.5102040816327,0.66859834817862)
--(axis cs:25.8503401360544,0.673820097170978)
--(axis cs:26.1904761904762,0.67341613491065)
--(axis cs:26.530612244898,0.675352549956481)
--(axis cs:26.8707482993197,0.669487870218383)
--(axis cs:27.2108843537415,0.67416061047003)
--(axis cs:27.5510204081633,0.669288036971083)
--(axis cs:27.891156462585,0.666570525843523)
--(axis cs:28.2312925170068,0.665842827146919)
--(axis cs:28.5714285714286,0.673782895620307)
--(axis cs:28.9115646258503,0.668245375249336)
--(axis cs:29.2517006802721,0.67245419267822)
--(axis cs:29.5918367346939,0.668526527935687)
--(axis cs:29.9319727891156,0.676224916856393)
--(axis cs:30.2721088435374,0.679494660640324)
--(axis cs:30.6122448979592,0.675483653511373)
--(axis cs:30.952380952381,0.670556420799642)
--(axis cs:31.2925170068027,0.670270138075421)
--(axis cs:31.6326530612245,0.669398610613608)
--(axis cs:31.9727891156463,0.671133001338893)
--(axis cs:32.312925170068,0.668700231044894)
--(axis cs:32.6530612244898,0.666719172202362)
--(axis cs:32.9931972789116,0.667654502249123)
--(axis cs:33.3333333333333,0.670077579491294)
--(axis cs:33.6734693877551,0.673253565629514)
--(axis cs:34.0136054421769,0.67034337360454)
--(axis cs:34.3537414965986,0.676612256643772)
--(axis cs:34.6938775510204,0.667365009990391)
--(axis cs:35.0340136054422,0.670874458651731)
--(axis cs:35.3741496598639,0.674560380793583)
--(axis cs:35.7142857142857,0.676068177800141)
--(axis cs:36.0544217687075,0.667865781409475)
--(axis cs:36.3945578231292,0.678159162139723)
--(axis cs:36.734693877551,0.673623112039188)
--(axis cs:37.0748299319728,0.673164722349569)
--(axis cs:37.4149659863946,0.672164122033456)
--(axis cs:37.7551020408163,0.673719450526627)
--(axis cs:38.0952380952381,0.673775376852618)
--(axis cs:38.4353741496599,0.667423341682756)
--(axis cs:38.7755102040816,0.669240009990391)
--(axis cs:39.1156462585034,0.67432360953748)
--(axis cs:39.4557823129252,0.670937770233773)
--(axis cs:39.7959183673469,0.671748561452828)
--(axis cs:40.1360544217687,0.673529196721915)
--(axis cs:40.4761904761905,0.670652451393894)
--(axis cs:40.8163265306122,0.674423416209731)
--(axis cs:41.156462585034,0.67180326752622)
--(axis cs:41.4965986394558,0.667058734414603)
--(axis cs:41.8367346938776,0.672109644206255)
--(axis cs:42.1768707482993,0.671348230706952)
--(axis cs:42.5170068027211,0.675917730565441)
--(axis cs:42.8571428571429,0.676624355601617)
--(axis cs:43.1972789115646,0.672767386087162)
--(axis cs:43.5374149659864,0.679068545392487)
--(axis cs:43.8775510204082,0.673603981012116)
--(axis cs:44.2176870748299,0.678184093773015)
--(axis cs:44.5578231292517,0.676875760453181)
--(axis cs:44.8979591836735,0.680236530508178)
--(axis cs:45.2380952380952,0.677626566498343)
--(axis cs:45.578231292517,0.688604729252173)
--(axis cs:45.9183673469388,0.678316123332341)
--(axis cs:46.2585034013605,0.683721097887366)
--(axis cs:46.5986394557823,0.685716216902802)
--(axis cs:46.9387755102041,0.689284207384868)
--(axis cs:47.2789115646259,0.684775414417822)
--(axis cs:47.6190476190476,0.688437435752583)
--(axis cs:47.9591836734694,0.690376474535041)
--(axis cs:48.2993197278912,0.694594595219413)
--(axis cs:48.6394557823129,0.69495297373258)
--(axis cs:48.9795918367347,0.69447802977378)
--(axis cs:49.3197278911565,0.695075541461179)
--(axis cs:49.6598639455782,0.693648774091347)
--(axis cs:50,0.694791037003619)
--(axis cs:50.3401360544218,0.695319173002361)
--(axis cs:50.6802721088435,0.699205573421441)
--(axis cs:51.0204081632653,0.69939711005262)
--(axis cs:51.3605442176871,0.705241903364806)
--(axis cs:51.7006802721088,0.705902770060916)
--(axis cs:52.0408163265306,0.702170789444823)
--(axis cs:52.3809523809524,0.7044832777529)
--(axis cs:52.7210884353741,0.702165300854816)
--(axis cs:53.0612244897959,0.703539535183979)
--(axis cs:53.4013605442177,0.707310994253924)
--(axis cs:53.7414965986395,0.704983002312917)
--(axis cs:54.0816326530612,0.713189498042533)
--(axis cs:54.421768707483,0.710645445140241)
--(axis cs:54.7619047619048,0.715825947407671)
--(axis cs:55.1020408163265,0.715377163848316)
--(axis cs:55.4421768707483,0.715119134208119)
--(axis cs:55.7823129251701,0.714927135020838)
--(axis cs:56.1224489795918,0.717534505076042)
--(axis cs:56.4625850340136,0.715760455905325)
--(axis cs:56.8027210884354,0.71872877714933)
--(axis cs:57.1428571428571,0.724156935139117)
--(axis cs:57.4829931972789,0.722472833082511)
--(axis cs:57.8231292517007,0.729173833598129)
--(axis cs:58.1632653061224,0.726639305999156)
--(axis cs:58.5034013605442,0.724278591690203)
--(axis cs:58.843537414966,0.725135830990365)
--(axis cs:59.1836734693878,0.73072785845455)
--(axis cs:59.5238095238095,0.726194754792338)
--(axis cs:59.8639455782313,0.730033783695247)
--(axis cs:60.2040816326531,0.732665962882934)
--(axis cs:60.5442176870748,0.735379192941195)
--(axis cs:60.8843537414966,0.7448592566292)
--(axis cs:61.2244897959184,0.741733687619)
--(axis cs:61.5646258503401,0.740446292636709)
--(axis cs:61.9047619047619,0.741050294682691)
--(axis cs:62.2448979591837,0.742061349744114)
--(axis cs:62.5850340136054,0.742603516629809)
--(axis cs:62.9251700680272,0.749388803749066)
--(axis cs:63.265306122449,0.749892691166201)
--(axis cs:63.6054421768707,0.746684548457592)
--(axis cs:63.9455782312925,0.74997838945937)
--(axis cs:64.2857142857143,0.751653686493587)
--(axis cs:64.6258503401361,0.755300845712648)
--(axis cs:64.9659863945578,0.755774246684391)
--(axis cs:65.3061224489796,0.752943408680879)
--(axis cs:65.6462585034014,0.751451331640789)
--(axis cs:65.9863945578231,0.75949534726761)
--(axis cs:66.3265306122449,0.756325854077932)
--(axis cs:66.6666666666667,0.757018345515841)
--(axis cs:67.0068027210884,0.757896127852366)
--(axis cs:67.3469387755102,0.759289783162351)
--(axis cs:67.687074829932,0.761212417932282)
--(axis cs:68.0272108843537,0.765664723345777)
--(axis cs:68.3673469387755,0.766284955657442)
--(axis cs:68.7074829931973,0.769747481757292)
--(axis cs:69.0476190476191,0.771556709294782)
--(axis cs:69.3877551020408,0.767556749384972)
--(axis cs:69.7278911564626,0.769606642896488)
--(axis cs:70.0680272108844,0.763521956769896)
--(axis cs:70.4081632653061,0.766071280370115)
--(axis cs:70.7482993197279,0.766635918320425)
--(axis cs:71.0884353741497,0.764892541512274)
--(axis cs:71.4285714285714,0.77002444775411)
--(axis cs:71.7687074829932,0.768929529488015)
--(axis cs:72.108843537415,0.768383350781568)
--(axis cs:72.4489795918367,0.771485822380995)
--(axis cs:72.7891156462585,0.765330169229452)
--(axis cs:73.1292517006803,0.763301756473238)
--(axis cs:73.469387755102,0.76298863253602)
--(axis cs:73.8095238095238,0.766737485240132)
--(axis cs:74.1496598639456,0.766030979604365)
--(axis cs:74.4897959183673,0.770348903246266)
--(axis cs:74.8299319727891,0.766232346345408)
--(axis cs:75.1700680272109,0.767501356402222)
--(axis cs:75.5102040816327,0.761223890644858)
--(axis cs:75.8503401360544,0.76237610213347)
--(axis cs:76.1904761904762,0.759908279639102)
--(axis cs:76.530612244898,0.762000341582101)
--(axis cs:76.8707482993197,0.758998256004178)
--(axis cs:77.2108843537415,0.763028769464651)
--(axis cs:77.5510204081633,0.758927642818229)
--(axis cs:77.891156462585,0.762417067984547)
--(axis cs:78.2312925170068,0.764035599967039)
--(axis cs:78.5714285714286,0.763893041670494)
--(axis cs:78.9115646258503,0.761138807030679)
--(axis cs:79.2517006802721,0.759916744669797)
--(axis cs:79.5918367346939,0.761958008684742)
--(axis cs:79.9319727891156,0.757864687085405)
--(axis cs:80.2721088435374,0.761442921722087)
--(axis cs:80.6122448979592,0.76057617549458)
--(axis cs:80.9523809523809,0.761432805240922)
--(axis cs:81.2925170068027,0.764966241070126)
--(axis cs:81.6326530612245,0.773218218034808)
--(axis cs:81.9727891156463,0.77078147449898)
--(axis cs:82.312925170068,0.774791984468829)
--(axis cs:82.6530612244898,0.779164263002081)
--(axis cs:82.9931972789116,0.783449698849877)
--(axis cs:83.3333333333333,0.787227972863994)
--(axis cs:83.6734693877551,0.792419528207514)
--(axis cs:84.0136054421769,0.800238098297502)
--(axis cs:84.3537414965986,0.7976042122044)
--(axis cs:84.6938775510204,0.806597005917025)
--(axis cs:85.0340136054422,0.815137411364937)
--(axis cs:85.3741496598639,0.813991701095792)
--(axis cs:85.7142857142857,0.822132171275009)
--(axis cs:86.0544217687075,0.825090676551569)
--(axis cs:86.3945578231292,0.830697577543101)
--(axis cs:86.734693877551,0.838146654412652)
--(axis cs:87.0748299319728,0.838185039356279)
--(axis cs:87.4149659863945,0.844899553950941)
--(axis cs:87.7551020408163,0.850227437679943)
--(axis cs:88.0952380952381,0.848777609401367)
--(axis cs:88.4353741496599,0.852208856759928)
--(axis cs:88.7755102040816,0.854956325958582)
--(axis cs:89.1156462585034,0.858538601247637)
--(axis cs:89.4557823129252,0.855031193602928)
--(axis cs:89.7959183673469,0.860347966376928)
--(axis cs:90.1360544217687,0.863286955426085)
--(axis cs:90.4761904761905,0.869462719975962)
--(axis cs:90.8163265306122,0.867803103401325)
--(axis cs:91.156462585034,0.870674510580752)
--(axis cs:91.4965986394558,0.874250848406776)
--(axis cs:91.8367346938775,0.879249784495445)
--(axis cs:92.1768707482993,0.886692949094128)
--(axis cs:92.5170068027211,0.897676929105212)
--(axis cs:92.8571428571429,0.901131902814752)
--(axis cs:93.1972789115646,0.907705845900779)
--(axis cs:93.5374149659864,0.912518229282387)
--(axis cs:93.8775510204082,0.9163037726883)
--(axis cs:94.2176870748299,0.92099417868526)
--(axis cs:94.5578231292517,0.920759022199104)
--(axis cs:94.8979591836735,0.922000274966384)
--(axis cs:95.2380952380952,0.924697945135737)
--(axis cs:95.578231292517,0.921901932283581)
--(axis cs:95.9183673469388,0.926570017779464)
--(axis cs:96.2585034013605,0.928368955922827)
--(axis cs:96.5986394557823,0.93158781064896)
--(axis cs:96.9387755102041,0.932697976182522)
--(axis cs:97.2789115646258,0.945485508641837)
--(axis cs:97.6190476190476,0.94964475301421)
--(axis cs:97.9591836734694,0.956407988114065)
--(axis cs:98.2993197278912,0.956770802033305)
--(axis cs:98.6394557823129,0.95287109375)
--(axis cs:98.9795918367347,0.946007490116415)
--(axis cs:99.3197278911565,0.948419128118782)
--(axis cs:99.6598639455782,0.955570386506961)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:99.6598639455782,0.965054613493039)
--(axis cs:99.3197278911565,0.967830871881218)
--(axis cs:98.9795918367347,0.967117509883585)
--(axis cs:98.6394557823129,0.97181640625)
--(axis cs:98.2993197278912,0.975729197966695)
--(axis cs:97.9591836734694,0.974842011885935)
--(axis cs:97.6190476190476,0.97035524698579)
--(axis cs:97.2789115646258,0.967639491358163)
--(axis cs:96.9387755102041,0.954177023817478)
--(axis cs:96.5986394557823,0.95309968935104)
--(axis cs:96.2585034013605,0.948506044077173)
--(axis cs:95.9183673469388,0.946554982220536)
--(axis cs:95.578231292517,0.941223067716419)
--(axis cs:95.2380952380952,0.942802054864263)
--(axis cs:94.8979591836735,0.940812225033616)
--(axis cs:94.5578231292517,0.938303477800897)
--(axis cs:94.2176870748299,0.93713082131474)
--(axis cs:93.8775510204082,0.9321337273117)
--(axis cs:93.5374149659864,0.927169270717613)
--(axis cs:93.1972789115646,0.923231654099222)
--(axis cs:92.8571428571429,0.921680597185248)
--(axis cs:92.5170068027211,0.917948070894788)
--(axis cs:92.1768707482993,0.907994550905872)
--(axis cs:91.8367346938775,0.899500215504555)
--(axis cs:91.4965986394558,0.892936651593224)
--(axis cs:91.156462585034,0.888700489419248)
--(axis cs:90.8163265306122,0.885634396598675)
--(axis cs:90.4761904761905,0.886787280024038)
--(axis cs:90.1360544217687,0.881400544573915)
--(axis cs:89.7959183673469,0.879339533623072)
--(axis cs:89.4557823129252,0.875593806397072)
--(axis cs:89.1156462585034,0.878023898752363)
--(axis cs:88.7755102040816,0.874731174041418)
--(axis cs:88.4353741496599,0.873103643240072)
--(axis cs:88.0952380952381,0.869972390598633)
--(axis cs:87.7551020408163,0.870085062320057)
--(axis cs:87.4149659863945,0.865412946049058)
--(axis cs:87.0748299319728,0.860877460643721)
--(axis cs:86.734693877551,0.860603345587348)
--(axis cs:86.3945578231292,0.856489922456899)
--(axis cs:86.0544217687075,0.852096823448431)
--(axis cs:85.7142857142857,0.849117828724991)
--(axis cs:85.3741496598639,0.842570798904208)
--(axis cs:85.0340136054422,0.842675088635063)
--(axis cs:84.6938775510204,0.835902994082975)
--(axis cs:84.3537414965986,0.8264582877956)
--(axis cs:84.0136054421769,0.828511901702498)
--(axis cs:83.6734693877551,0.820705471792486)
--(axis cs:83.3333333333333,0.815897027136006)
--(axis cs:82.9931972789116,0.811862801150123)
--(axis cs:82.6530612244898,0.807398236997919)
--(axis cs:82.312925170068,0.803333015531171)
--(axis cs:81.9727891156463,0.79796852550102)
--(axis cs:81.6326530612245,0.801156781965192)
--(axis cs:81.2925170068027,0.792221258929874)
--(axis cs:80.9523809523809,0.788254694759079)
--(axis cs:80.6122448979592,0.78692382450542)
--(axis cs:80.2721088435374,0.787932078277913)
--(axis cs:79.9319727891156,0.784010312914595)
--(axis cs:79.5918367346939,0.789291991315258)
--(axis cs:79.2517006802721,0.786020755330203)
--(axis cs:78.9115646258503,0.787923692969321)
--(axis cs:78.5714285714286,0.790794458329506)
--(axis cs:78.2312925170068,0.790651900032961)
--(axis cs:77.891156462585,0.787895432015453)
--(axis cs:77.5510204081633,0.786384857181771)
--(axis cs:77.2108843537415,0.789783730535349)
--(axis cs:76.8707482993197,0.785064243995821)
--(axis cs:76.530612244898,0.789874658417899)
--(axis cs:76.1904761904762,0.787279220360898)
--(axis cs:75.8503401360544,0.78887389786653)
--(axis cs:75.5102040816327,0.788776109355143)
--(axis cs:75.1700680272109,0.795623643597778)
--(axis cs:74.8299319727891,0.793455153654592)
--(axis cs:74.4897959183673,0.797463596753734)
--(axis cs:74.1496598639456,0.793344020395635)
--(axis cs:73.8095238095238,0.793575014759868)
--(axis cs:73.469387755102,0.79013636746398)
--(axis cs:73.1292517006803,0.791073243526762)
--(axis cs:72.7891156462585,0.792169830770548)
--(axis cs:72.4489795918367,0.797576677619005)
--(axis cs:72.108843537415,0.796616649218432)
--(axis cs:71.7687074829932,0.797320470511985)
--(axis cs:71.4285714285714,0.79903805224589)
--(axis cs:71.0884353741497,0.793544958487726)
--(axis cs:70.7482993197279,0.794926581679575)
--(axis cs:70.4081632653061,0.795803719629885)
--(axis cs:70.0680272108844,0.794603043230104)
--(axis cs:69.7278911564626,0.799768357103512)
--(axis cs:69.3877551020408,0.797755750615028)
--(axis cs:69.0476190476191,0.800943290705218)
--(axis cs:68.7074829931973,0.800252518242708)
--(axis cs:68.3673469387755,0.797777544342558)
--(axis cs:68.0272108843537,0.796835276654223)
--(axis cs:67.687074829932,0.793162582067718)
--(axis cs:67.3469387755102,0.790710216837649)
--(axis cs:67.0068027210884,0.790541372147633)
--(axis cs:66.6666666666667,0.790169154484159)
--(axis cs:66.3265306122449,0.789924145922068)
--(axis cs:65.9863945578231,0.79269215273239)
--(axis cs:65.6462585034014,0.786048668359211)
--(axis cs:65.3061224489796,0.787681591319121)
--(axis cs:64.9659863945578,0.789225753315609)
--(axis cs:64.6258503401361,0.789386654287352)
--(axis cs:64.2857142857143,0.787096313506413)
--(axis cs:63.9455782312925,0.785021610540629)
--(axis cs:63.6054421768707,0.780502951542408)
--(axis cs:63.265306122449,0.784482308833799)
--(axis cs:62.9251700680272,0.784361196250934)
--(axis cs:62.5850340136054,0.776771483370191)
--(axis cs:62.2448979591837,0.775438650255886)
--(axis cs:61.9047619047619,0.774574705317309)
--(axis cs:61.5646258503401,0.774866207363291)
--(axis cs:61.2244897959184,0.775453812381)
--(axis cs:60.8843537414966,0.7788907433708)
--(axis cs:60.5442176870748,0.768058307058805)
--(axis cs:60.2040816326531,0.767021537117067)
--(axis cs:59.8639455782313,0.764653716304753)
--(axis cs:59.5238095238095,0.760367745207662)
--(axis cs:59.1836734693878,0.76364714154545)
--(axis cs:58.843537414966,0.757364169009635)
--(axis cs:58.5034013605442,0.757596408309797)
--(axis cs:58.1632653061224,0.759610694000844)
--(axis cs:57.8231292517007,0.763326166401871)
--(axis cs:57.4829931972789,0.756902166917489)
--(axis cs:57.1428571428571,0.758030564860883)
--(axis cs:56.8027210884354,0.75345872285067)
--(axis cs:56.4625850340136,0.750802044094675)
--(axis cs:56.1224489795918,0.752777994923958)
--(axis cs:55.7823129251701,0.750385364979162)
--(axis cs:55.4421768707483,0.750193365791881)
--(axis cs:55.1020408163265,0.749935336151684)
--(axis cs:54.7619047619048,0.751361552592329)
--(axis cs:54.421768707483,0.74654205485976)
--(axis cs:54.0816326530612,0.749623001957467)
--(axis cs:53.7414965986395,0.741266997687083)
--(axis cs:53.4013605442177,0.744564005746076)
--(axis cs:53.0612244897959,0.740210464816021)
--(axis cs:52.7210884353741,0.738772199145184)
--(axis cs:52.3809523809524,0.7411417222471)
--(axis cs:52.0408163265306,0.738141710555177)
--(axis cs:51.7006802721088,0.741909729939084)
--(axis cs:51.3605442176871,0.741008096635194)
--(axis cs:51.0204081632653,0.73622788994738)
--(axis cs:50.6802721088435,0.734856926578559)
--(axis cs:50.3401360544218,0.731555826997639)
--(axis cs:50,0.732083962996381)
--(axis cs:49.6598639455782,0.730413725908653)
--(axis cs:49.3197278911565,0.729924458538821)
--(axis cs:48.9795918367347,0.72989697022622)
--(axis cs:48.6394557823129,0.73035952626742)
--(axis cs:48.2993197278912,0.730717904780587)
--(axis cs:47.9591836734694,0.726811025464959)
--(axis cs:47.6190476190476,0.724062564247417)
--(axis cs:47.2789115646259,0.720849585582178)
--(axis cs:46.9387755102041,0.725403292615132)
--(axis cs:46.5986394557823,0.722096283097198)
--(axis cs:46.2585034013605,0.719716402112634)
--(axis cs:45.9183673469388,0.715746376667659)
--(axis cs:45.578231292517,0.725457770747827)
--(axis cs:45.2380952380952,0.714873433501657)
--(axis cs:44.8979591836735,0.717575969491822)
--(axis cs:44.5578231292517,0.714999239546819)
--(axis cs:44.2176870748299,0.715565906226985)
--(axis cs:43.8775510204082,0.712333518987884)
--(axis cs:43.5374149659864,0.717806454607513)
--(axis cs:43.1972789115646,0.711920113912838)
--(axis cs:42.8571428571429,0.716500644398383)
--(axis cs:42.5170068027211,0.715957269434559)
--(axis cs:42.1768707482993,0.710526769293048)
--(axis cs:41.8367346938776,0.713202855793745)
--(axis cs:41.4965986394558,0.707628765585397)
--(axis cs:41.156462585034,0.71350923247378)
--(axis cs:40.8163265306122,0.714014083790269)
--(axis cs:40.4761904761905,0.710910048606107)
--(axis cs:40.1360544217687,0.715845803278085)
--(axis cs:39.7959183673469,0.714188938547172)
--(axis cs:39.4557823129252,0.711874729766227)
--(axis cs:39.1156462585034,0.71567639046252)
--(axis cs:38.7755102040816,0.711384990009609)
--(axis cs:38.4353741496599,0.710076658317244)
--(axis cs:38.0952380952381,0.715599623147382)
--(axis cs:37.7551020408163,0.716280549473373)
--(axis cs:37.4149659863946,0.714710877966544)
--(axis cs:37.0748299319728,0.716522777650431)
--(axis cs:36.734693877551,0.716064387960812)
--(axis cs:36.3945578231292,0.720278337860277)
--(axis cs:36.0544217687075,0.710884218590525)
--(axis cs:35.7142857142857,0.717056822199859)
--(axis cs:35.3741496598639,0.717627119206417)
--(axis cs:35.0340136054422,0.712563041348269)
--(axis cs:34.6938775510204,0.709509990009609)
--(axis cs:34.3537414965986,0.720262743356229)
--(axis cs:34.0136054421769,0.71153162639546)
--(axis cs:33.6734693877551,0.715183934370486)
--(axis cs:33.3333333333333,0.712734920508706)
--(axis cs:32.9931972789116,0.708907997750877)
--(axis cs:32.6530612244898,0.708280827797638)
--(axis cs:32.312925170068,0.710362268955107)
--(axis cs:31.9727891156463,0.713554498661107)
--(axis cs:31.6326530612245,0.710913889386392)
--(axis cs:31.2925170068027,0.71316736192458)
--(axis cs:30.952380952381,0.713506079200358)
--(axis cs:30.6122448979592,0.716703846488627)
--(axis cs:30.2721088435374,0.721755339359676)
--(axis cs:29.9319727891156,0.717525083143607)
--(axis cs:29.5918367346939,0.710535972064313)
--(axis cs:29.2517006802721,0.71567080732178)
--(axis cs:28.9115646258503,0.711442124750664)
--(axis cs:28.5714285714286,0.716842104379693)
--(axis cs:28.2312925170068,0.707907172853081)
--(axis cs:27.891156462585,0.709054474156477)
--(axis cs:27.5510204081633,0.711336963028917)
--(axis cs:27.2108843537415,0.716151889529971)
--(axis cs:26.8707482993197,0.712699629781617)
--(axis cs:26.530612244898,0.717459950043519)
--(axis cs:26.1904761904762,0.71502136508935)
--(axis cs:25.8503401360544,0.717117402829022)
--(axis cs:25.5102040816327,0.71140165182138)
--(axis cs:25.1700680272109,0.719219654205157)
--(axis cs:24.8299319727891,0.712851114530837)
--(axis cs:24.4897959183673,0.717603025328366)
--(axis cs:24.1496598639456,0.720620252286881)
--(axis cs:23.8095238095238,0.719071314347631)
--(axis cs:23.469387755102,0.721121889250326)
--(axis cs:23.1292517006803,0.718193988299209)
--(axis cs:22.7891156462585,0.719131535016971)
--(axis cs:22.4489795918367,0.722033900762123)
--(axis cs:22.108843537415,0.728898483775569)
--(axis cs:21.7687074829932,0.725272082685945)
--(axis cs:21.4285714285714,0.722355348074281)
--(axis cs:21.0884353741497,0.724074805833899)
--(axis cs:20.7482993197279,0.724673310245724)
--(axis cs:20.4081632653061,0.724767676816367)
--(axis cs:20.0680272108844,0.720829818879991)
--(axis cs:19.7278911564626,0.722864346833649)
--(axis cs:19.3877551020408,0.722603362262778)
--(axis cs:19.047619047619,0.720175771494128)
--(axis cs:18.7074829931973,0.724006578254081)
--(axis cs:18.3673469387755,0.717472233644002)
--(axis cs:18.0272108843537,0.721375897016899)
--(axis cs:17.687074829932,0.722885565042228)
--(axis cs:17.3469387755102,0.726824656627533)
--(axis cs:17.0068027210884,0.722297911567021)
--(axis cs:16.6666666666667,0.728960405197182)
--(axis cs:16.3265306122449,0.730065624161363)
--(axis cs:15.9863945578231,0.73030748304385)
--(axis cs:15.6462585034014,0.730481183819875)
--(axis cs:15.3061224489796,0.726580858224285)
--(axis cs:14.9659863945578,0.722419517004668)
--(axis cs:14.6258503401361,0.72129585196257)
--(axis cs:14.2857142857143,0.724297565952503)
--(axis cs:13.9455782312925,0.725313091847569)
--(axis cs:13.6054421768707,0.732845432691958)
--(axis cs:13.265306122449,0.732903847335343)
--(axis cs:12.9251700680272,0.724410936124666)
--(axis cs:12.5850340136054,0.721241489787503)
--(axis cs:12.2448979591837,0.723792679770905)
--(axis cs:11.9047619047619,0.717391646162943)
--(axis cs:11.5646258503401,0.719268142153951)
--(axis cs:11.2244897959184,0.713996896224406)
--(axis cs:10.8843537414966,0.708122865987874)
--(axis cs:10.5442176870748,0.710810809085289)
--(axis cs:10.2040816326531,0.711783659969038)
--(axis cs:9.86394557823129,0.707995587320925)
--(axis cs:9.52380952380952,0.701835164454235)
--(axis cs:9.18367346938775,0.695851056172491)
--(axis cs:8.84353741496599,0.699511979861101)
--(axis cs:8.50340136054422,0.697645788295842)
--(axis cs:8.16326530612245,0.69528212534314)
--(axis cs:7.82312925170068,0.690303851358224)
--(axis cs:7.48299319727891,0.681622142511998)
--(axis cs:7.14285714285714,0.66916141908914)
--(axis cs:6.80272108843537,0.653325892098117)
--(axis cs:6.46258503401361,0.641577859367014)
--(axis cs:6.12244897959184,0.61982241673316)
--(axis cs:5.78231292517007,0.607969516707078)
--(axis cs:5.4421768707483,0.588512017806092)
--(axis cs:5.10204081632653,0.568079659994794)
--(axis cs:4.76190476190476,0.538182059819125)
--(axis cs:4.42176870748299,0.509173785914385)
--(axis cs:4.08163265306122,0.482109042598646)
--(axis cs:3.74149659863946,0.454523375817908)
--(axis cs:3.40136054421769,0.414735064958559)
--(axis cs:3.06122448979592,0.377807745047911)
--(axis cs:2.72108843537415,0.32164561088729)
--(axis cs:2.38095238095238,0.23919982474565)
--(axis cs:2.04081632653061,0.186357865180601)
--(axis cs:1.70068027210884,0.15778584475066)
--(axis cs:1.36054421768707,0.127840366287202)
--(axis cs:1.02040816326531,0.0890234375)
--(axis cs:0.680272108843537,0.0833654050284301)
--(axis cs:0.340136054421769,0.0835408835891426)
--(axis cs:0,0.0837452512175585)
--cycle;


==> img/stl10/stl10_rate_accuracy_lcg_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color8, mark=oplus*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table {%
0 0.07765625
0.340136054421769 0.0871875
0.680272108843537 0.12109375
1.02040816326531 0.19203125
1.36054421768707 0.24640625
1.70068027210884 0.30953125
2.04081632653061 0.36640625
2.38095238095238 0.4234375
2.72108843537415 0.4659375
3.06122448979592 0.49203125
3.40136054421769 0.5284375
3.74149659863946 0.5696875
4.08163265306122 0.61625
4.42176870748299 0.65234375
4.76190476190476 0.67625
5.10204081632653 0.698125
5.4421768707483 0.71734375
5.78231292517007 0.745
6.12244897959184 0.768125
6.46258503401361 0.78203125
6.80272108843537 0.80203125
7.14285714285714 0.81375
7.48299319727891 0.8271875
7.82312925170068 0.8403125
8.16326530612245 0.84734375
8.50340136054422 0.85625
8.84353741496599 0.85953125
9.18367346938775 0.8625
9.52380952380952 0.861875
9.86394557823129 0.875625
10.2040816326531 0.8734375
10.5442176870748 0.87828125
10.8843537414966 0.8828125
11.2244897959184 0.8859375
11.5646258503401 0.88703125
11.9047619047619 0.8925
12.2448979591837 0.89078125
12.5850340136054 0.89984375
12.9251700680272 0.89828125
13.265306122449 0.8984375
13.6054421768707 0.9003125
13.9455782312925 0.9025
14.2857142857143 0.9009375
14.6258503401361 0.90578125
14.9659863945578 0.904375
15.3061224489796 0.90640625
15.6462585034014 0.90875
15.9863945578231 0.910625
16.3265306122449 0.9109375
16.6666666666667 0.91265625
17.0068027210884 0.91203125
17.3469387755102 0.91046875
17.687074829932 0.90984375
18.0272108843537 0.91015625
18.3673469387755 0.90890625
18.7074829931973 0.905625
19.047619047619 0.90375
19.3877551020408 0.9040625
19.7278911564626 0.9025
20.0680272108844 0.903125
20.4081632653061 0.90375
20.7482993197279 0.90140625
21.0884353741497 0.89953125
21.4285714285714 0.8990625
21.7687074829932 0.89703125
22.108843537415 0.89359375
22.4489795918367 0.89515625
22.7891156462585 0.89796875
23.1292517006803 0.89625
23.469387755102 0.8965625
23.8095238095238 0.8971875
24.1496598639456 0.8925
24.4897959183673 0.89421875
24.8299319727891 0.895625
25.1700680272109 0.8971875
25.5102040816327 0.89609375
25.8503401360544 0.898125
26.1904761904762 0.8978125
26.530612244898 0.8940625
26.8707482993197 0.89015625
27.2108843537415 0.888125
27.5510204081633 0.89125
27.891156462585 0.88921875
28.2312925170068 0.88484375
28.5714285714286 0.8875
28.9115646258503 0.88171875
29.2517006802721 0.88359375
29.5918367346939 0.88078125
29.9319727891156 0.87703125
30.2721088435374 0.8784375
30.6122448979592 0.87734375
30.952380952381 0.87390625
31.2925170068027 0.8740625
31.6326530612245 0.86734375
31.9727891156463 0.86765625
32.312925170068 0.8659375
32.6530612244898 0.86578125
32.9931972789116 0.86546875
33.3333333333333 0.86515625
33.6734693877551 0.86625
34.0136054421769 0.86453125
34.3537414965986 0.86390625
34.6938775510204 0.8609375
35.0340136054422 0.8646875
35.3741496598639 0.86625
35.7142857142857 0.86375
36.0544217687075 0.8665625
36.3945578231292 0.86203125
36.734693877551 0.86515625
37.0748299319728 0.86421875
37.4149659863946 0.8684375
37.7551020408163 0.8675
38.0952380952381 0.86625
38.4353741496599 0.86515625
38.7755102040816 0.8653125
39.1156462585034 0.86296875
39.4557823129252 0.86109375
39.7959183673469 0.85734375
40.1360544217687 0.85078125
40.4761904761905 0.848125
40.8163265306122 0.84671875
41.156462585034 0.84890625
41.4965986394558 0.850625
41.8367346938776 0.8484375
42.1768707482993 0.84640625
42.5170068027211 0.84234375
42.8571428571429 0.84265625
43.1972789115646 0.84953125
43.5374149659864 0.84609375
43.8775510204082 0.8546875
44.2176870748299 0.845
44.5578231292517 0.854375
44.8979591836735 0.8521875
45.2380952380952 0.853125
45.578231292517 0.84515625
45.9183673469388 0.84484375
46.2585034013605 0.84671875
46.5986394557823 0.84703125
46.9387755102041 0.85375
47.2789115646259 0.85296875
47.6190476190476 0.84328125
47.9591836734694 0.84390625
48.2993197278912 0.84140625
48.6394557823129 0.840625
48.9795918367347 0.84453125
49.3197278911565 0.84546875
49.6598639455782 0.84828125
50 0.84640625
50.3401360544218 0.85265625
50.6802721088435 0.85015625
51.0204081632653 0.858125
51.3605442176871 0.86
51.7006802721088 0.86109375
52.0408163265306 0.86
52.3809523809524 0.86296875
52.7210884353741 0.86265625
53.0612244897959 0.85671875
53.4013605442177 0.85859375
53.7414965986395 0.8615625
54.0816326530612 0.8603125
54.421768707483 0.8609375
54.7619047619048 0.8659375
55.1020408163265 0.8634375
55.4421768707483 0.863125
55.7823129251701 0.8659375
56.1224489795918 0.86671875
56.4625850340136 0.87015625
56.8027210884354 0.8759375
57.1428571428571 0.8775
57.4829931972789 0.8796875
57.8231292517007 0.87546875
58.1632653061224 0.87921875
58.5034013605442 0.87796875
58.843537414966 0.88078125
59.1836734693878 0.8784375
59.5238095238095 0.8765625
59.8639455782313 0.883125
60.2040816326531 0.8775
60.5442176870748 0.87765625
60.8843537414966 0.88015625
61.2244897959184 0.8784375
61.5646258503401 0.8759375
61.9047619047619 0.88140625
62.2448979591837 0.87828125
62.5850340136054 0.88
62.9251700680272 0.8834375
63.265306122449 0.88453125
63.6054421768707 0.8815625
63.9455782312925 0.88234375
64.2857142857143 0.88515625
64.6258503401361 0.884375
64.9659863945578 0.88125
65.3061224489796 0.881875
65.6462585034014 0.8828125
65.9863945578231 0.8884375
66.3265306122449 0.88390625
66.6666666666667 0.88296875
67.0068027210884 0.8834375
67.3469387755102 0.88546875
67.687074829932 0.8884375
68.0272108843537 0.885625
68.3673469387755 0.886875
68.7074829931973 0.88515625
69.0476190476191 0.88515625
69.3877551020408 0.885
69.7278911564626 0.8790625
70.0680272108844 0.87953125
70.4081632653061 0.8734375
70.7482993197279 0.874375
71.0884353741497 0.87171875
71.4285714285714 0.87328125
71.7687074829932 0.8740625
72.108843537415 0.87796875
72.4489795918367 0.88171875
72.7891156462585 0.885
73.1292517006803 0.88359375
73.469387755102 0.88375
73.8095238095238 0.8834375
74.1496598639456 0.88640625
74.4897959183673 0.88640625
74.8299319727891 0.884375
75.1700680272109 0.88671875
75.5102040816327 0.88703125
75.8503401360544 0.88765625
76.1904761904762 0.88359375
76.530612244898 0.8871875
76.8707482993197 0.88703125
77.2108843537415 0.88296875
77.5510204081633 0.88421875
77.891156462585 0.8809375
78.2312925170068 0.88484375
78.5714285714286 0.88515625
78.9115646258503 0.8915625
79.2517006802721 0.8896875
79.5918367346939 0.8865625
79.9319727891156 0.88796875
80.2721088435374 0.89
80.6122448979592 0.888125
80.9523809523809 0.89171875
81.2925170068027 0.8946875
81.6326530612245 0.89765625
81.9727891156463 0.9028125
82.312925170068 0.90921875
82.6530612244898 0.9109375
82.9931972789116 0.913125
83.3333333333333 0.915625
83.6734693877551 0.91671875
84.0136054421769 0.92015625
84.3537414965986 0.926875
84.6938775510204 0.93265625
85.0340136054422 0.933125
85.3741496598639 0.9375
85.7142857142857 0.93875
86.0544217687075 0.9403125
86.3945578231292 0.93953125
86.734693877551 0.9396875
87.0748299319728 0.9434375
87.4149659863945 0.94375
87.7551020408163 0.945625
88.0952380952381 0.9471875
88.4353741496599 0.9459375
88.7755102040816 0.94671875
89.1156462585034 0.94671875
89.4557823129252 0.94609375
89.7959183673469 0.94734375
90.1360544217687 0.9478125
90.4761904761905 0.94796875
90.8163265306122 0.94859375
91.156462585034 0.94734375
91.4965986394558 0.9440625
91.8367346938775 0.94484375
92.1768707482993 0.94421875
92.5170068027211 0.945625
92.8571428571429 0.945
93.1972789115646 0.94390625
93.5374149659864 0.94375
93.8775510204082 0.94234375
94.2176870748299 0.94703125
94.5578231292517 0.9484375
94.8979591836735 0.9478125
95.2380952380952 0.94578125
95.578231292517 0.95328125
95.9183673469388 0.95046875
96.2585034013605 0.95453125
96.5986394557823 0.9559375
96.9387755102041 0.9571875
97.2789115646258 0.9584375
97.6190476190476 0.9584375
97.9591836734694 0.95953125
98.2993197278912 0.96078125
98.6394557823129 0.96078125
98.9795918367347 0.9603125
99.3197278911565 0.95921875
99.6598639455782 0.963125
100 0.98
};
\path [fill=color8, fill opacity=0.25]
(axis cs:0,0.0840652087927851)
--(axis cs:0,0.0712472912072149)
--(axis cs:0.340136054421769,0.0772899535474063)
--(axis cs:0.680272108843537,0.10810546875)
--(axis cs:1.02040816326531,0.176885083593562)
--(axis cs:1.36054421768707,0.231571175952424)
--(axis cs:1.70068027210884,0.292105970501507)
--(axis cs:2.04081632653061,0.349468309021106)
--(axis cs:2.38095238095238,0.407594297038537)
--(axis cs:2.72108843537415,0.449844058141603)
--(axis cs:3.06122448979592,0.475489249770087)
--(axis cs:3.40136054421769,0.510054764695498)
--(axis cs:3.74149659863946,0.550189481395737)
--(axis cs:4.08163265306122,0.597242872270093)
--(axis cs:4.42176870748299,0.63381709560106)
--(axis cs:4.76190476190476,0.658433153114005)
--(axis cs:5.10204081632653,0.681167645256915)
--(axis cs:5.4421768707483,0.700922103113948)
--(axis cs:5.78231292517007,0.728039833511594)
--(axis cs:6.12244897959184,0.751384428485887)
--(axis cs:6.46258503401361,0.765693444014527)
--(axis cs:6.80272108843537,0.7867984400844)
--(axis cs:7.14285714285714,0.798744584107613)
--(axis cs:7.48299319727891,0.813316874325871)
--(axis cs:7.82312925170068,0.827654049911518)
--(axis cs:8.16326530612245,0.833861173782889)
--(axis cs:8.50340136054422,0.843092836099141)
--(axis cs:8.84353741496599,0.845888353814329)
--(axis cs:9.18367346938775,0.848907877701616)
--(axis cs:9.52380952380952,0.847714507008314)
--(axis cs:9.86394557823129,0.862420083793839)
--(axis cs:10.2040816326531,0.860235472956155)
--(axis cs:10.5442176870748,0.864973099967039)
--(axis cs:10.8843537414966,0.869936679903243)
--(axis cs:11.2244897959184,0.874137650416412)
--(axis cs:11.5646258503401,0.875130402436507)
--(axis cs:11.9047619047619,0.881392916243662)
--(axis cs:12.2448979591837,0.879479674835613)
--(axis cs:12.5850340136054,0.888521940742281)
--(axis cs:12.9251700680272,0.887751116441087)
--(axis cs:13.265306122449,0.887099277129922)
--(axis cs:13.6054421768707,0.889156582364457)
--(axis cs:13.9455782312925,0.891812104528059)
--(axis cs:14.2857142857143,0.890064714328346)
--(axis cs:14.6258503401361,0.895323820398884)
--(axis cs:14.9659863945578,0.893862541686877)
--(axis cs:15.3061224489796,0.896017442446306)
--(axis cs:15.6462585034014,0.898253883716762)
--(axis cs:15.9863945578231,0.900722636988431)
--(axis cs:16.3265306122449,0.90020241712214)
--(axis cs:16.6666666666667,0.903188628915534)
--(axis cs:17.0068027210884,0.901859518260177)
--(axis cs:17.3469387755102,0.899833181812595)
--(axis cs:17.687074829932,0.898938996425861)
--(axis cs:18.0272108843537,0.899802384542731)
--(axis cs:18.3673469387755,0.897423851546577)
--(axis cs:18.7074829931973,0.894128905586349)
--(axis cs:19.047619047619,0.891682437358139)
--(axis cs:19.3877551020408,0.891997308428531)
--(axis cs:19.7278911564626,0.890769862303831)
--(axis cs:20.0680272108844,0.891177365435799)
--(axis cs:20.4081632653061,0.892205065073335)
--(axis cs:20.7482993197279,0.890715231955806)
--(axis cs:21.0884353741497,0.888471922213959)
--(axis cs:21.4285714285714,0.888509297326407)
--(axis cs:21.7687074829932,0.886395681812595)
--(axis cs:22.108843537415,0.883743046385824)
--(axis cs:22.4489795918367,0.885568514742996)
--(axis cs:22.7891156462585,0.888943600507373)
--(axis cs:23.1292517006803,0.887544888789818)
--(axis cs:23.469387755102,0.887601508010192)
--(axis cs:23.8095238095238,0.888288448632895)
--(axis cs:24.1496598639456,0.883484894607153)
--(axis cs:24.4897959183673,0.884915742732784)
--(axis cs:24.8299319727891,0.887298408692464)
--(axis cs:25.1700680272109,0.889001832191525)
--(axis cs:25.5102040816327,0.886903160562749)
--(axis cs:25.8503401360544,0.889277537771167)
--(axis cs:26.1904761904762,0.889333822628458)
--(axis cs:26.530612244898,0.883601879030648)
--(axis cs:26.8707482993197,0.88022647721442)
--(axis cs:27.2108843537415,0.878593629931597)
--(axis cs:27.5510204081633,0.882138090980133)
--(axis cs:27.891156462585,0.880682342411523)
--(axis cs:28.2312925170068,0.875840818246878)
--(axis cs:28.5714285714286,0.878461651592057)
--(axis cs:28.9115646258503,0.87302734375)
--(axis cs:29.2517006802721,0.874524328310055)
--(axis cs:29.5918367346939,0.871809090335357)
--(axis cs:29.9319727891156,0.867833399783325)
--(axis cs:30.2721088435374,0.869088985981426)
--(axis cs:30.6122448979592,0.86779089203304)
--(axis cs:30.952380952381,0.863120206709785)
--(axis cs:31.2925170068027,0.864444474802933)
--(axis cs:31.6326530612245,0.857261481138987)
--(axis cs:31.9727891156463,0.857306990969732)
--(axis cs:32.312925170068,0.854836428197421)
--(axis cs:32.6530612244898,0.855467991712301)
--(axis cs:32.9931972789116,0.854371544744732)
--(axis cs:33.3333333333333,0.853916444098903)
--(axis cs:33.6734693877551,0.854538576509)
--(axis cs:34.0136054421769,0.852456182040135)
--(axis cs:34.3537414965986,0.851677363314955)
--(axis cs:34.6938775510204,0.848843097714216)
--(axis cs:35.0340136054422,0.850061214666524)
--(axis cs:35.3741496598639,0.85238418800836)
--(axis cs:35.7142857142857,0.849617146472558)
--(axis cs:36.0544217687075,0.852600729686983)
--(axis cs:36.3945578231292,0.847234152774405)
--(axis cs:36.734693877551,0.849787563720934)
--(axis cs:37.0748299319728,0.848538610475344)
--(axis cs:37.4149659863946,0.852654002132555)
--(axis cs:37.7551020408163,0.851352132289624)
--(axis cs:38.0952380952381,0.849292645256915)
--(axis cs:38.4353741496599,0.847888205857401)
--(axis cs:38.7755102040816,0.84842389690351)
--(axis cs:39.1156462585034,0.845495375042727)
--(axis cs:39.4557823129252,0.843343668763253)
--(axis cs:39.7959183673469,0.839868192030574)
--(axis cs:40.1360544217687,0.832630055381219)
--(axis cs:40.4761904761905,0.830064137252512)
--(axis cs:40.8163265306122,0.828212697374855)
--(axis cs:41.156462585034,0.830742975067477)
--(axis cs:41.4965986394558,0.832290055316876)
--(axis cs:41.8367346938776,0.830820355806594)
--(axis cs:42.1768707482993,0.827616365256427)
--(axis cs:42.5170068027211,0.8240950915686)
--(axis cs:42.8571428571429,0.824178562319541)
--(axis cs:43.1972789115646,0.831066986370706)
--(axis cs:43.5374149659864,0.827749185245548)
--(axis cs:43.8775510204082,0.836513989352417)
--(axis cs:44.2176870748299,0.826370934437277)
--(axis cs:44.5578231292517,0.836591370538986)
--(axis cs:44.8979591836735,0.834263387645104)
--(axis cs:45.2380952380952,0.83574987002634)
--(axis cs:45.578231292517,0.827677963648804)
--(axis cs:45.9183673469388,0.82750405848794)
--(axis cs:46.2585034013605,0.829117040561116)
--(axis cs:46.5986394557823,0.829126035816799)
--(axis cs:46.9387755102041,0.836355121813897)
--(axis cs:47.2789115646259,0.835588406513127)
--(axis cs:47.6190476190476,0.826238345712648)
--(axis cs:47.9591836734694,0.826150259679527)
--(axis cs:48.2993197278912,0.824343212988505)
--(axis cs:48.6394557823129,0.823067503423462)
--(axis cs:48.9795918367347,0.82707043265911)
--(axis cs:49.3197278911565,0.828109819337229)
--(axis cs:49.6598639455782,0.831321364665149)
--(axis cs:50,0.829318080439148)
--(axis cs:50.3401360544218,0.835788270503338)
--(axis cs:50.6802721088435,0.833936196557826)
--(axis cs:51.0204081632653,0.84202622575391)
--(axis cs:51.3605442176871,0.844124325263478)
--(axis cs:51.7006802721088,0.845786619543972)
--(axis cs:52.0408163265306,0.844710636100952)
--(axis cs:52.3809523809524,0.848181323448744)
--(axis cs:52.7210884353741,0.848402116806068)
--(axis cs:53.0612244897959,0.842081710163316)
--(axis cs:53.4013605442177,0.843926119344775)
--(axis cs:53.7414965986395,0.847449229021073)
--(axis cs:54.0816326530612,0.846010609657013)
--(axis cs:54.421768707483,0.84679655128133)
--(axis cs:54.7619047619048,0.851982561970394)
--(axis cs:55.1020408163265,0.849746107680998)
--(axis cs:55.4421768707483,0.849556754349251)
--(axis cs:55.7823129251701,0.85269652245572)
--(axis cs:56.1224489795918,0.853810750936654)
--(axis cs:56.4625850340136,0.857204733659714)
--(axis cs:56.8027210884354,0.863434448614626)
--(axis cs:57.1428571428571,0.865504568333762)
--(axis cs:57.4829931972789,0.868140913082924)
--(axis cs:57.8231292517007,0.863703299433771)
--(axis cs:58.1632653061224,0.866891219739671)
--(axis cs:58.5034013605442,0.867496739226345)
--(axis cs:58.843537414966,0.868981804527769)
--(axis cs:59.1836734693878,0.865388052274617)
--(axis cs:59.5238095238095,0.863094432024954)
--(axis cs:59.8639455782313,0.870165754376927)
--(axis cs:60.2040816326531,0.863858851492004)
--(axis cs:60.5442176870748,0.863967992516144)
--(axis cs:60.8843537414966,0.866502173974349)
--(axis cs:61.2244897959184,0.86526367549458)
--(axis cs:61.5646258503401,0.861903511977196)
--(axis cs:61.9047619047619,0.867920844726316)
--(axis cs:62.2448979591837,0.864764764184747)
--(axis cs:62.5850340136054,0.866845735749623)
--(axis cs:62.9251700680272,0.870768506849352)
--(axis cs:63.265306122449,0.872120450717006)
--(axis cs:63.6054421768707,0.869475985540194)
--(axis cs:63.9455782312925,0.87040529840078)
--(axis cs:64.2857142857143,0.873683822514623)
--(axis cs:64.6258503401361,0.872629425232824)
--(axis cs:64.9659863945578,0.869678661528439)
--(axis cs:65.3061224489796,0.86987638863015)
--(axis cs:65.6462585034014,0.871398827864307)
--(axis cs:65.9863945578231,0.878470819670177)
--(axis cs:66.3265306122449,0.873291325578065)
--(axis cs:66.6666666666667,0.871278925672926)
--(axis cs:67.0068027210884,0.872619232481151)
--(axis cs:67.3469387755102,0.875442444115359)
--(axis cs:67.687074829932,0.878788785745366)
--(axis cs:68.0272108843537,0.875721673957744)
--(axis cs:68.3673469387755,0.877475617644128)
--(axis cs:68.7074829931973,0.875475466195305)
--(axis cs:69.0476190476191,0.875384279405398)
--(axis cs:69.3877551020408,0.875115952399313)
--(axis cs:69.7278911564626,0.867802772488952)
--(axis cs:70.0680272108844,0.868357821485853)
--(axis cs:70.4081632653061,0.862053947561799)
--(axis cs:70.7482993197279,0.862325627488135)
--(axis cs:71.0884353741497,0.859608981231201)
--(axis cs:71.4285714285714,0.860193490681854)
--(axis cs:71.7687074829932,0.860253201816943)
--(axis cs:72.108843537415,0.864687140974522)
--(axis cs:72.4489795918367,0.86892578125)
--(axis cs:72.7891156462585,0.873098751768295)
--(axis cs:73.1292517006803,0.872302305479464)
--(axis cs:73.469387755102,0.872554827885999)
--(axis cs:73.8095238095238,0.87242613529857)
--(axis cs:74.1496598639456,0.876212041337294)
--(axis cs:74.4897959183673,0.877588480042885)
--(axis cs:74.8299319727891,0.874109474589049)
--(axis cs:75.1700680272109,0.876994717478886)
--(axis cs:75.5102040816327,0.877970244432216)
--(axis cs:75.8503401360544,0.87816548927261)
--(axis cs:76.1904761904762,0.873969281892487)
--(axis cs:76.530612244898,0.878501032828931)
--(axis cs:76.8707482993197,0.878659540167911)
--(axis cs:77.2108843537415,0.875027309164487)
--(axis cs:77.5510204081633,0.877029896739149)
--(axis cs:77.891156462585,0.875470494139735)
--(axis cs:78.2312925170068,0.878574705529022)
--(axis cs:78.5714285714286,0.87868214881095)
--(axis cs:78.9115646258503,0.883802667763547)
--(axis cs:79.2517006802721,0.881491353414704)
--(axis cs:79.5918367346939,0.878672261766905)
--(axis cs:79.9319727891156,0.879586793969953)
--(axis cs:80.2721088435374,0.881842341402165)
--(axis cs:80.6122448979592,0.880057860770288)
--(axis cs:80.9523809523809,0.882818091290451)
--(axis cs:81.2925170068027,0.88521333372216)
--(axis cs:81.6326530612245,0.887535273845241)
--(axis cs:81.9727891156463,0.892048140778785)
--(axis cs:82.312925170068,0.899117581002686)
--(axis cs:82.6530612244898,0.901175782031563)
--(axis cs:82.9931972789116,0.903683100027131)
--(axis cs:83.3333333333333,0.90600003646263)
--(axis cs:83.6734693877551,0.907042893053889)
--(axis cs:84.0136054421769,0.909853168511475)
--(axis cs:84.3537414965986,0.916388883050355)
--(axis cs:84.6938775510204,0.92233097751783)
--(axis cs:85.0340136054422,0.923010150487325)
--(axis cs:85.3741496598639,0.927924706334566)
--(axis cs:85.7142857142857,0.929332372303718)
--(axis cs:86.0544217687075,0.93096908804698)
--(axis cs:86.3945578231292,0.930741644982022)
--(axis cs:86.734693877551,0.931588505032572)
--(axis cs:87.0748299319728,0.935506273240529)
--(axis cs:87.4149659863945,0.93640692531363)
--(axis cs:87.7551020408163,0.938307946212918)
--(axis cs:88.0952380952381,0.940108937392805)
--(axis cs:88.4353741496599,0.938823994589268)
--(axis cs:88.7755102040816,0.939510025182047)
--(axis cs:89.1156462585034,0.939694963813925)
--(axis cs:89.4557823129252,0.938804772282446)
--(axis cs:89.7959183673469,0.940202814088073)
--(axis cs:90.1360544217687,0.94014663988016)
--(axis cs:90.4761904761905,0.940383555769871)
--(axis cs:90.8163265306122,0.940896231875415)
--(axis cs:91.156462585034,0.939040671273828)
--(axis cs:91.4965986394558,0.935309318031134)
--(axis cs:91.8367346938775,0.935929173129159)
--(axis cs:92.1768707482993,0.934799603453987)
--(axis cs:92.5170068027211,0.936019873589112)
--(axis cs:92.8571428571429,0.935071667947548)
--(axis cs:93.1972789115646,0.933911382084737)
--(axis cs:93.5374149659864,0.93372987864189)
--(axis cs:93.8775510204082,0.932468872843674)
--(axis cs:94.2176870748299,0.936806216244182)
--(axis cs:94.5578231292517,0.938353812399958)
--(axis cs:94.8979591836735,0.937748692946884)
--(axis cs:95.2380952380952,0.936190531162635)
--(axis cs:95.578231292517,0.944196069094539)
--(axis cs:95.9183673469388,0.941557383083126)
--(axis cs:96.2585034013605,0.947315913491381)
--(axis cs:96.5986394557823,0.949001843396654)
--(axis cs:96.9387755102041,0.951627093419732)
--(axis cs:97.2789115646258,0.953655334161447)
--(axis cs:97.6190476190476,0.954413398871477)
--(axis cs:97.9591836734694,0.956261588077581)
--(axis cs:98.2993197278912,0.958359453756321)
--(axis cs:98.6394557823129,0.957213119940147)
--(axis cs:98.9795918367347,0.958124476904062)
--(axis cs:99.3197278911565,0.955081304655407)
--(axis cs:99.6598639455782,0.95744412516709)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:99.6598639455782,0.96880587483291)
--(axis cs:99.3197278911565,0.963356195344593)
--(axis cs:98.9795918367347,0.962500523095938)
--(axis cs:98.6394557823129,0.964349380059853)
--(axis cs:98.2993197278912,0.963203046243679)
--(axis cs:97.9591836734694,0.962800911922419)
--(axis cs:97.6190476190476,0.962461601128523)
--(axis cs:97.2789115646258,0.963219665838553)
--(axis cs:96.9387755102041,0.962747906580268)
--(axis cs:96.5986394557823,0.962873156603346)
--(axis cs:96.2585034013605,0.96174658650862)
--(axis cs:95.9183673469388,0.959380116916874)
--(axis cs:95.578231292517,0.962366430905461)
--(axis cs:95.2380952380952,0.955371968837365)
--(axis cs:94.8979591836735,0.957876307053116)
--(axis cs:94.5578231292517,0.958521187600042)
--(axis cs:94.2176870748299,0.957256283755818)
--(axis cs:93.8775510204082,0.952218627156327)
--(axis cs:93.5374149659864,0.95377012135811)
--(axis cs:93.1972789115646,0.953901117915263)
--(axis cs:92.8571428571429,0.954928332052452)
--(axis cs:92.5170068027211,0.955230126410888)
--(axis cs:92.1768707482993,0.953637896546013)
--(axis cs:91.8367346938775,0.953758326870841)
--(axis cs:91.4965986394558,0.952815681968866)
--(axis cs:91.156462585034,0.955646828726172)
--(axis cs:90.8163265306122,0.956291268124585)
--(axis cs:90.4761904761905,0.95555394423013)
--(axis cs:90.1360544217687,0.95547836011984)
--(axis cs:89.7959183673469,0.954484685911927)
--(axis cs:89.4557823129252,0.953382727717554)
--(axis cs:89.1156462585034,0.953742536186075)
--(axis cs:88.7755102040816,0.953927474817953)
--(axis cs:88.4353741496599,0.953051005410732)
--(axis cs:88.0952380952381,0.954266062607195)
--(axis cs:87.7551020408163,0.952942053787082)
--(axis cs:87.4149659863945,0.95109307468637)
--(axis cs:87.0748299319728,0.951368726759471)
--(axis cs:86.734693877551,0.947786494967428)
--(axis cs:86.3945578231292,0.948320855017978)
--(axis cs:86.0544217687075,0.94965591195302)
--(axis cs:85.7142857142857,0.948167627696282)
--(axis cs:85.3741496598639,0.947075293665434)
--(axis cs:85.0340136054422,0.943239849512675)
--(axis cs:84.6938775510204,0.94298152248217)
--(axis cs:84.3537414965986,0.937361116949645)
--(axis cs:84.0136054421769,0.930459331488525)
--(axis cs:83.6734693877551,0.926394606946111)
--(axis cs:83.3333333333333,0.92524996353737)
--(axis cs:82.9931972789116,0.922566899972869)
--(axis cs:82.6530612244898,0.920699217968437)
--(axis cs:82.312925170068,0.919319918997314)
--(axis cs:81.9727891156463,0.913576859221215)
--(axis cs:81.6326530612245,0.907777226154759)
--(axis cs:81.2925170068027,0.90416166627784)
--(axis cs:80.9523809523809,0.900619408709549)
--(axis cs:80.6122448979592,0.896192139229712)
--(axis cs:80.2721088435374,0.898157658597835)
--(axis cs:79.9319727891156,0.896350706030047)
--(axis cs:79.5918367346939,0.894452738233095)
--(axis cs:79.2517006802721,0.897883646585296)
--(axis cs:78.9115646258503,0.899322332236453)
--(axis cs:78.5714285714286,0.89163035118905)
--(axis cs:78.2312925170068,0.891112794470978)
--(axis cs:77.891156462585,0.886404505860265)
--(axis cs:77.5510204081633,0.891407603260852)
--(axis cs:77.2108843537415,0.890910190835512)
--(axis cs:76.8707482993197,0.895402959832089)
--(axis cs:76.530612244898,0.895873967171069)
--(axis cs:76.1904761904762,0.893218218107513)
--(axis cs:75.8503401360544,0.89714701072739)
--(axis cs:75.5102040816327,0.896092255567784)
--(axis cs:75.1700680272109,0.896442782521114)
--(axis cs:74.8299319727891,0.894640525410952)
--(axis cs:74.4897959183673,0.895224019957115)
--(axis cs:74.1496598639456,0.896600458662706)
--(axis cs:73.8095238095238,0.89444886470143)
--(axis cs:73.469387755102,0.894945172114001)
--(axis cs:73.1292517006803,0.894885194520536)
--(axis cs:72.7891156462585,0.896901248231705)
--(axis cs:72.4489795918367,0.89451171875)
--(axis cs:72.108843537415,0.891250359025478)
--(axis cs:71.7687074829932,0.887871798183057)
--(axis cs:71.4285714285714,0.886369009318146)
--(axis cs:71.0884353741497,0.883828518768799)
--(axis cs:70.7482993197279,0.886424372511865)
--(axis cs:70.4081632653061,0.884821052438201)
--(axis cs:70.0680272108844,0.890704678514146)
--(axis cs:69.7278911564626,0.890322227511048)
--(axis cs:69.3877551020408,0.894884047600688)
--(axis cs:69.0476190476191,0.894928220594602)
--(axis cs:68.7074829931973,0.894837033804695)
--(axis cs:68.3673469387755,0.896274382355872)
--(axis cs:68.0272108843537,0.895528326042256)
--(axis cs:67.687074829932,0.898086214254634)
--(axis cs:67.3469387755102,0.895495055884641)
--(axis cs:67.0068027210884,0.894255767518849)
--(axis cs:66.6666666666667,0.894658574327074)
--(axis cs:66.3265306122449,0.894521174421935)
--(axis cs:65.9863945578231,0.898404180329823)
--(axis cs:65.6462585034014,0.894226172135693)
--(axis cs:65.3061224489796,0.89387361136985)
--(axis cs:64.9659863945578,0.892821338471561)
--(axis cs:64.6258503401361,0.896120574767176)
--(axis cs:64.2857142857143,0.896628677485377)
--(axis cs:63.9455782312925,0.89428220159922)
--(axis cs:63.6054421768707,0.893649014459806)
--(axis cs:63.265306122449,0.896942049282994)
--(axis cs:62.9251700680272,0.896106493150648)
--(axis cs:62.5850340136054,0.893154264250377)
--(axis cs:62.2448979591837,0.891797735815253)
--(axis cs:61.9047619047619,0.894891655273684)
--(axis cs:61.5646258503401,0.889971488022804)
--(axis cs:61.2244897959184,0.89161132450542)
--(axis cs:60.8843537414966,0.893810326025651)
--(axis cs:60.5442176870748,0.891344507483856)
--(axis cs:60.2040816326531,0.891141148507995)
--(axis cs:59.8639455782313,0.896084245623073)
--(axis cs:59.5238095238095,0.890030567975046)
--(axis cs:59.1836734693878,0.891486947725383)
--(axis cs:58.843537414966,0.892580695472231)
--(axis cs:58.5034013605442,0.888440760773655)
--(axis cs:58.1632653061224,0.891546280260329)
--(axis cs:57.8231292517007,0.887234200566229)
--(axis cs:57.4829931972789,0.891234086917076)
--(axis cs:57.1428571428571,0.889495431666238)
--(axis cs:56.8027210884354,0.888440551385374)
--(axis cs:56.4625850340136,0.883107766340286)
--(axis cs:56.1224489795918,0.879626749063346)
--(axis cs:55.7823129251701,0.87917847754428)
--(axis cs:55.4421768707483,0.876693245650749)
--(axis cs:55.1020408163265,0.877128892319001)
--(axis cs:54.7619047619048,0.879892438029606)
--(axis cs:54.421768707483,0.87507844871867)
--(axis cs:54.0816326530612,0.874614390342987)
--(axis cs:53.7414965986395,0.875675770978927)
--(axis cs:53.4013605442177,0.873261380655225)
--(axis cs:53.0612244897959,0.871355789836684)
--(axis cs:52.7210884353741,0.876910383193932)
--(axis cs:52.3809523809524,0.877756176551256)
--(axis cs:52.0408163265306,0.875289363899048)
--(axis cs:51.7006802721088,0.876400880456028)
--(axis cs:51.3605442176871,0.875875674736522)
--(axis cs:51.0204081632653,0.87422377424609)
--(axis cs:50.6802721088435,0.866376303442174)
--(axis cs:50.3401360544218,0.869524229496662)
--(axis cs:50,0.863494419560852)
--(axis cs:49.6598639455782,0.865241135334851)
--(axis cs:49.3197278911565,0.862827680662771)
--(axis cs:48.9795918367347,0.86199206734089)
--(axis cs:48.6394557823129,0.858182496576538)
--(axis cs:48.2993197278912,0.858469287011495)
--(axis cs:47.9591836734694,0.861662240320473)
--(axis cs:47.6190476190476,0.860324154287352)
--(axis cs:47.2789115646259,0.870349093486873)
--(axis cs:46.9387755102041,0.871144878186103)
--(axis cs:46.5986394557823,0.864936464183201)
--(axis cs:46.2585034013605,0.864320459438884)
--(axis cs:45.9183673469388,0.86218344151206)
--(axis cs:45.578231292517,0.862634536351196)
--(axis cs:45.2380952380952,0.87050012997366)
--(axis cs:44.8979591836735,0.870111612354896)
--(axis cs:44.5578231292517,0.872158629461014)
--(axis cs:44.2176870748299,0.863629065562723)
--(axis cs:43.8775510204082,0.872861010647583)
--(axis cs:43.5374149659864,0.864438314754452)
--(axis cs:43.1972789115646,0.867995513629294)
--(axis cs:42.8571428571429,0.861133937680459)
--(axis cs:42.5170068027211,0.8605924084314)
--(axis cs:42.1768707482993,0.865196134743573)
--(axis cs:41.8367346938776,0.866054644193406)
--(axis cs:41.4965986394558,0.868959944683124)
--(axis cs:41.156462585034,0.867069524932523)
--(axis cs:40.8163265306122,0.865224802625145)
--(axis cs:40.4761904761905,0.866185862747488)
--(axis cs:40.1360544217687,0.868932444618781)
--(axis cs:39.7959183673469,0.874819307969426)
--(axis cs:39.4557823129252,0.878843831236747)
--(axis cs:39.1156462585034,0.880442124957273)
--(axis cs:38.7755102040816,0.88220110309649)
--(axis cs:38.4353741496599,0.882424294142599)
--(axis cs:38.0952380952381,0.883207354743085)
--(axis cs:37.7551020408163,0.883647867710376)
--(axis cs:37.4149659863946,0.884220997867445)
--(axis cs:37.0748299319728,0.879898889524657)
--(axis cs:36.734693877551,0.880524936279065)
--(axis cs:36.3945578231292,0.876828347225595)
--(axis cs:36.0544217687075,0.880524270313017)
--(axis cs:35.7142857142857,0.877882853527442)
--(axis cs:35.3741496598639,0.88011581199164)
--(axis cs:35.0340136054422,0.879313785333476)
--(axis cs:34.6938775510204,0.873031902285785)
--(axis cs:34.3537414965986,0.876135136685045)
--(axis cs:34.0136054421769,0.876606317959865)
--(axis cs:33.6734693877551,0.877961423491)
--(axis cs:33.3333333333333,0.876396055901097)
--(axis cs:32.9931972789116,0.876565955255268)
--(axis cs:32.6530612244898,0.876094508287699)
--(axis cs:32.312925170068,0.877038571802579)
--(axis cs:31.9727891156463,0.878005509030268)
--(axis cs:31.6326530612245,0.877426018861012)
--(axis cs:31.2925170068027,0.883680525197067)
--(axis cs:30.952380952381,0.884692293290215)
--(axis cs:30.6122448979592,0.88689660796696)
--(axis cs:30.2721088435374,0.887786014018574)
--(axis cs:29.9319727891156,0.886229100216676)
--(axis cs:29.5918367346939,0.889753409664643)
--(axis cs:29.2517006802721,0.892663171689945)
--(axis cs:28.9115646258503,0.89041015625)
--(axis cs:28.5714285714286,0.896538348407943)
--(axis cs:28.2312925170068,0.893846681753122)
--(axis cs:27.891156462585,0.897755157588477)
--(axis cs:27.5510204081633,0.900361909019867)
--(axis cs:27.2108843537415,0.897656370068404)
--(axis cs:26.8707482993197,0.90008602278558)
--(axis cs:26.530612244898,0.904523120969352)
--(axis cs:26.1904761904762,0.906291177371542)
--(axis cs:25.8503401360544,0.906972462228833)
--(axis cs:25.5102040816327,0.905284339437251)
--(axis cs:25.1700680272109,0.905373167808475)
--(axis cs:24.8299319727891,0.903951591307536)
--(axis cs:24.4897959183673,0.903521757267216)
--(axis cs:24.1496598639456,0.901515105392847)
--(axis cs:23.8095238095238,0.906086551367105)
--(axis cs:23.469387755102,0.905523491989808)
--(axis cs:23.1292517006803,0.904955111210182)
--(axis cs:22.7891156462585,0.906993899492627)
--(axis cs:22.4489795918367,0.904743985257004)
--(axis cs:22.108843537415,0.903444453614176)
--(axis cs:21.7687074829932,0.907666818187405)
--(axis cs:21.4285714285714,0.909615702673593)
--(axis cs:21.0884353741497,0.910590577786041)
--(axis cs:20.7482993197279,0.912097268044194)
--(axis cs:20.4081632653061,0.915294934926665)
--(axis cs:20.0680272108844,0.915072634564201)
--(axis cs:19.7278911564626,0.914230137696169)
--(axis cs:19.3877551020408,0.916127691571469)
--(axis cs:19.047619047619,0.915817562641861)
--(axis cs:18.7074829931973,0.917121094413651)
--(axis cs:18.3673469387755,0.920388648453423)
--(axis cs:18.0272108843537,0.920510115457269)
--(axis cs:17.687074829932,0.920748503574139)
--(axis cs:17.3469387755102,0.921104318187405)
--(axis cs:17.0068027210884,0.922202981739823)
--(axis cs:16.6666666666667,0.922123871084466)
--(axis cs:16.3265306122449,0.92167258287786)
--(axis cs:15.9863945578231,0.920527363011569)
--(axis cs:15.6462585034014,0.919246116283238)
--(axis cs:15.3061224489796,0.916795057553694)
--(axis cs:14.9659863945578,0.914887458313123)
--(axis cs:14.6258503401361,0.916238679601116)
--(axis cs:14.2857142857143,0.911810285671654)
--(axis cs:13.9455782312925,0.913187895471941)
--(axis cs:13.6054421768707,0.911468417635543)
--(axis cs:13.265306122449,0.909775722870078)
--(axis cs:12.9251700680272,0.908811383558913)
--(axis cs:12.5850340136054,0.911165559257719)
--(axis cs:12.2448979591837,0.902082825164387)
--(axis cs:11.9047619047619,0.903607083756338)
--(axis cs:11.5646258503401,0.898932097563493)
--(axis cs:11.2244897959184,0.897737349583589)
--(axis cs:10.8843537414966,0.895688320096757)
--(axis cs:10.5442176870748,0.891589400032961)
--(axis cs:10.2040816326531,0.886639527043845)
--(axis cs:9.86394557823129,0.88882991620616)
--(axis cs:9.52380952380952,0.876035492991686)
--(axis cs:9.18367346938775,0.876092122298384)
--(axis cs:8.84353741496599,0.873174146185671)
--(axis cs:8.50340136054422,0.869407163900859)
--(axis cs:8.16326530612245,0.860826326217111)
--(axis cs:7.82312925170068,0.852970950088482)
--(axis cs:7.48299319727891,0.841058125674129)
--(axis cs:7.14285714285714,0.828755415892387)
--(axis cs:6.80272108843537,0.8172640599156)
--(axis cs:6.46258503401361,0.798369055985473)
--(axis cs:6.12244897959184,0.784865571514113)
--(axis cs:5.78231292517007,0.761960166488406)
--(axis cs:5.4421768707483,0.733765396886052)
--(axis cs:5.10204081632653,0.715082354743085)
--(axis cs:4.76190476190476,0.694066846885995)
--(axis cs:4.42176870748299,0.67087040439894)
--(axis cs:4.08163265306122,0.635257127729907)
--(axis cs:3.74149659863946,0.589185518604263)
--(axis cs:3.40136054421769,0.546820235304502)
--(axis cs:3.06122448979592,0.508573250229913)
--(axis cs:2.72108843537415,0.482030941858397)
--(axis cs:2.38095238095238,0.439280702961463)
--(axis cs:2.04081632653061,0.383344190978894)
--(axis cs:1.70068027210884,0.326956529498493)
--(axis cs:1.36054421768707,0.261241324047576)
--(axis cs:1.02040816326531,0.207177416406438)
--(axis cs:0.680272108843537,0.13408203125)
--(axis cs:0.340136054421769,0.0970850464525937)
--(axis cs:0,0.0840652087927851)
--cycle;


==> img/stl10/stl10_rate_accuracy_lime.tex <==
% lime
\addplot [line width=0.5, opacity=0.8, color3, mark=diamond, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table [row sep=\\]{%
0	0.07640625 \\
0.340136054421769	0.073125 \\
0.680272108843537	0.07671875 \\
1.02040816326531	0.07484375 \\
1.36054421768707	0.0665625 \\
1.70068027210884	0.06765625 \\
2.04081632653061	0.05828125 \\
2.38095238095238	0.05453125 \\
2.72108843537415	0.05078125 \\
3.06122448979592	0.0640625 \\
3.40136054421769	0.05515625 \\
3.74149659863946	0.04609375 \\
4.08163265306122	0.0484375 \\
4.42176870748299	0.051875 \\
4.76190476190476	0.06171875 \\
5.10204081632653	0.0634375 \\
5.4421768707483	0.0690625 \\
5.78231292517007	0.0684375 \\
6.12244897959184	0.06421875 \\
6.46258503401361	0.0646875 \\
6.80272108843537	0.05734375 \\
7.14285714285714	0.05328125 \\
7.48299319727891	0.0528125 \\
7.82312925170068	0.0815625 \\
8.16326530612245	0.10125 \\
8.50340136054422	0.10625 \\
8.84353741496599	0.10109375 \\
9.18367346938775	0.11015625 \\
9.52380952380952	0.11109375 \\
9.86394557823129	0.1096875 \\
10.2040816326531	0.110625 \\
10.5442176870748	0.11046875 \\
10.8843537414966	0.10234375 \\
11.2244897959184	0.1184375 \\
11.5646258503401	0.1178125 \\
11.9047619047619	0.12265625 \\
12.2448979591837	0.119375 \\
12.5850340136054	0.12421875 \\
12.9251700680272	0.12921875 \\
13.265306122449	0.14015625 \\
13.6054421768707	0.1434375 \\
13.9455782312925	0.14375 \\
14.2857142857143	0.1696875 \\
14.6258503401361	0.17375 \\
14.9659863945578	0.17 \\
15.3061224489796	0.17421875 \\
15.6462585034014	0.18828125 \\
15.9863945578231	0.195 \\
16.3265306122449	0.20265625 \\
16.6666666666667	0.2078125 \\
17.0068027210884	0.22828125 \\
17.3469387755102	0.23640625 \\
17.687074829932	0.24875 \\
18.0272108843537	0.25375 \\
18.3673469387755	0.26453125 \\
18.7074829931973	0.2834375 \\
19.047619047619	0.3065625 \\
19.3877551020408	0.31109375 \\
19.7278911564626	0.3134375 \\
20.0680272108844	0.32140625 \\
20.4081632653061	0.32890625 \\
20.7482993197279	0.33203125 \\
21.0884353741497	0.33484375 \\
21.4285714285714	0.34046875 \\
21.7687074829932	0.33375 \\
22.108843537415	0.34109375 \\
22.4489795918367	0.34328125 \\
22.7891156462585	0.3453125 \\
23.1292517006803	0.34984375 \\
23.469387755102	0.35703125 \\
23.8095238095238	0.36921875 \\
24.1496598639456	0.374375 \\
24.4897959183673	0.3890625 \\
24.8299319727891	0.38828125 \\
25.1700680272109	0.3915625 \\
25.5102040816327	0.39609375 \\
25.8503401360544	0.4 \\
26.1904761904762	0.40015625 \\
26.530612244898	0.4003125 \\
26.8707482993197	0.40125 \\
27.2108843537415	0.4 \\
27.5510204081633	0.393125 \\
27.891156462585	0.399375 \\
28.2312925170068	0.39796875 \\
28.5714285714286	0.3975 \\
28.9115646258503	0.40234375 \\
29.2517006802721	0.40453125 \\
29.5918367346939	0.41359375 \\
29.9319727891156	0.40421875 \\
30.2721088435374	0.4128125 \\
30.6122448979592	0.41421875 \\
30.952380952381	0.423125 \\
31.2925170068027	0.43171875 \\
31.6326530612245	0.42984375 \\
31.9727891156463	0.4315625 \\
32.312925170068	0.43265625 \\
32.6530612244898	0.4428125 \\
32.9931972789116	0.4421875 \\
33.3333333333333	0.43359375 \\
33.6734693877551	0.43625 \\
34.0136054421769	0.44 \\
34.3537414965986	0.4396875 \\
34.6938775510204	0.4434375 \\
35.0340136054422	0.468125 \\
35.3741496598639	0.465625 \\
35.7142857142857	0.46015625 \\
36.0544217687075	0.46078125 \\
36.3945578231292	0.4615625 \\
36.734693877551	0.4621875 \\
37.0748299319728	0.46625 \\
37.4149659863946	0.4765625 \\
37.7551020408163	0.47484375 \\
38.0952380952381	0.488125 \\
38.4353741496599	0.49078125 \\
38.7755102040816	0.49359375 \\
39.1156462585034	0.49375 \\
39.4557823129252	0.4946875 \\
39.7959183673469	0.494375 \\
40.1360544217687	0.49234375 \\
40.4761904761905	0.49296875 \\
40.8163265306122	0.494375 \\
41.156462585034	0.49703125 \\
41.4965986394558	0.4978125 \\
41.8367346938776	0.484375 \\
42.1768707482993	0.48703125 \\
42.5170068027211	0.48578125 \\
42.8571428571429	0.48453125 \\
43.1972789115646	0.48421875 \\
43.5374149659864	0.48390625 \\
43.8775510204082	0.483125 \\
44.2176870748299	0.4846875 \\
44.5578231292517	0.484375 \\
44.8979591836735	0.48390625 \\
45.2380952380952	0.49609375 \\
45.578231292517	0.49859375 \\
45.9183673469388	0.49984375 \\
46.2585034013605	0.50921875 \\
46.5986394557823	0.51125 \\
46.9387755102041	0.5178125 \\
47.2789115646259	0.523125 \\
47.6190476190476	0.5225 \\
47.9591836734694	0.52390625 \\
48.2993197278912	0.52171875 \\
48.6394557823129	0.5225 \\
48.9795918367347	0.53234375 \\
49.3197278911565	0.53734375 \\
49.6598639455782	0.53421875 \\
50	0.5403125 \\
50.3401360544218	0.5434375 \\
50.6802721088435	0.54234375 \\
51.0204081632653	0.540625 \\
51.3605442176871	0.545 \\
51.7006802721088	0.54515625 \\
52.0408163265306	0.54609375 \\
52.3809523809524	0.54484375 \\
52.7210884353741	0.55328125 \\
53.0612244897959	0.55234375 \\
53.4013605442177	0.5528125 \\
53.7414965986395	0.54875 \\
54.0816326530612	0.55046875 \\
54.421768707483	0.55078125 \\
54.7619047619048	0.55203125 \\
55.1020408163265	0.5496875 \\
55.4421768707483	0.553125 \\
55.7823129251701	0.5571875 \\
56.1224489795918	0.56109375 \\
56.4625850340136	0.5690625 \\
56.8027210884354	0.5778125 \\
57.1428571428571	0.57828125 \\
57.4829931972789	0.58375 \\
57.8231292517007	0.5875 \\
58.1632653061224	0.593125 \\
58.5034013605442	0.60140625 \\
58.843537414966	0.601875 \\
59.1836734693878	0.600625 \\
59.5238095238095	0.60734375 \\
59.8639455782313	0.59921875 \\
60.2040816326531	0.6059375 \\
60.5442176870748	0.60203125 \\
60.8843537414966	0.60171875 \\
61.2244897959184	0.59828125 \\
61.5646258503401	0.6021875 \\
61.9047619047619	0.6046875 \\
62.2448979591837	0.605 \\
62.5850340136054	0.5971875 \\
62.9251700680272	0.6003125 \\
63.265306122449	0.60265625 \\
63.6054421768707	0.6046875 \\
63.9455782312925	0.60828125 \\
64.2857142857143	0.60609375 \\
64.6258503401361	0.60828125 \\
64.9659863945578	0.6146875 \\
65.3061224489796	0.6178125 \\
65.6462585034014	0.61953125 \\
65.9863945578231	0.625 \\
66.3265306122449	0.618125 \\
66.6666666666667	0.62234375 \\
67.0068027210884	0.62875 \\
67.3469387755102	0.6396875 \\
67.687074829932	0.6490625 \\
68.0272108843537	0.653125 \\
68.3673469387755	0.664375 \\
68.7074829931973	0.66890625 \\
69.0476190476191	0.6671875 \\
69.3877551020408	0.66484375 \\
69.7278911564626	0.6796875 \\
70.0680272108844	0.6753125 \\
70.4081632653061	0.6815625 \\
70.7482993197279	0.68984375 \\
71.0884353741497	0.69671875 \\
71.4285714285714	0.69859375 \\
71.7687074829932	0.70109375 \\
72.108843537415	0.70453125 \\
72.4489795918367	0.715625 \\
72.7891156462585	0.725625 \\
73.1292517006803	0.7296875 \\
73.469387755102	0.724375 \\
73.8095238095238	0.7334375 \\
74.1496598639456	0.74484375 \\
74.4897959183673	0.77390625 \\
74.8299319727891	0.7865625 \\
75.1700680272109	0.78984375 \\
75.5102040816327	0.78765625 \\
75.8503401360544	0.78640625 \\
76.1904761904762	0.79953125 \\
76.530612244898	0.81015625 \\
76.8707482993197	0.80546875 \\
77.2108843537415	0.8115625 \\
77.5510204081633	0.8109375 \\
77.891156462585	0.825 \\
78.2312925170068	0.83359375 \\
78.5714285714286	0.845 \\
78.9115646258503	0.8475 \\
79.2517006802721	0.84609375 \\
79.5918367346939	0.844375 \\
79.9319727891156	0.84765625 \\
80.2721088435374	0.85578125 \\
80.6122448979592	0.863125 \\
80.9523809523809	0.86734375 \\
81.2925170068027	0.873125 \\
81.6326530612245	0.87171875 \\
81.9727891156463	0.8715625 \\
82.312925170068	0.87484375 \\
82.6530612244898	0.8740625 \\
82.9931972789116	0.876875 \\
83.3333333333333	0.8778125 \\
83.6734693877551	0.87921875 \\
84.0136054421769	0.87859375 \\
84.3537414965986	0.88109375 \\
84.6938775510204	0.8796875 \\
85.0340136054422	0.88359375 \\
85.3741496598639	0.88890625 \\
85.7142857142857	0.89859375 \\
86.0544217687075	0.90109375 \\
86.3945578231292	0.90375 \\
86.734693877551	0.91359375 \\
87.0748299319728	0.9103125 \\
87.4149659863945	0.91015625 \\
87.7551020408163	0.9178125 \\
88.0952380952381	0.920625 \\
88.4353741496599	0.92140625 \\
88.7755102040816	0.92390625 \\
89.1156462585034	0.92484375 \\
89.4557823129252	0.921875 \\
89.7959183673469	0.9246875 \\
90.1360544217687	0.9228125 \\
90.4761904761905	0.92234375 \\
90.8163265306122	0.92046875 \\
91.156462585034	0.924375 \\
91.4965986394558	0.92296875 \\
91.8367346938775	0.940625 \\
92.1768707482993	0.94015625 \\
92.5170068027211	0.9484375 \\
92.8571428571429	0.9546875 \\
93.1972789115646	0.95265625 \\
93.5374149659864	0.94875 \\
93.8775510204082	0.94859375 \\
94.2176870748299	0.94515625 \\
94.5578231292517	0.94859375 \\
94.8979591836735	0.9478125 \\
95.2380952380952	0.94328125 \\
95.578231292517	0.9453125 \\
95.9183673469388	0.94125 \\
96.2585034013605	0.94328125 \\
96.5986394557823	0.95109375 \\
96.9387755102041	0.9621875 \\
97.2789115646258	0.9625 \\
97.6190476190476	0.96359375 \\
97.9591836734694	0.96171875 \\
98.2993197278912	0.96265625 \\
98.6394557823129	0.96234375 \\
98.9795918367347	0.9628125 \\
99.3197278911565	0.9609375 \\
99.6598639455782	0.96203125 \\
100	1 \\
};
\path [fill=color3, fill opacity=0.5] (axis cs:0,0.0831104778102871)
--(axis cs:0,0.0697020221897129)
--(axis cs:0.340136054421769,0.0664271764845772)
--(axis cs:0.680272108843537,0.0704238975119206)
--(axis cs:1.02040816326531,0.0672171782565744)
--(axis cs:1.36054421768707,0.0573423845688108)
--(axis cs:1.70068027210884,0.0558899888898302)
--(axis cs:2.04081632653061,0.0464882721927825)
--(axis cs:2.38095238095238,0.0430688021562238)
--(axis cs:2.72108843537415,0.0401546524351317)
--(axis cs:3.06122448979592,0.0507927439441695)
--(axis cs:3.40136054421769,0.0412701630769615)
--(axis cs:3.74149659863946,0.032228969729184)
--(axis cs:4.08163265306122,0.0338922908110071)
--(axis cs:4.42176870748299,0.036807428604328)
--(axis cs:4.76190476190476,0.0461932489300931)
--(axis cs:5.10204081632653,0.047322739177778)
--(axis cs:5.4421768707483,0.0522803934837997)
--(axis cs:5.78231292517007,0.0516037604755523)
--(axis cs:6.12244897959184,0.0479008026449008)
--(axis cs:6.46258503401361,0.0497330148133657)
--(axis cs:6.80272108843537,0.0432450146748528)
--(axis cs:7.14285714285714,0.0383296348193986)
--(axis cs:7.48299319727891,0.0384089479800635)
--(axis cs:7.82312925170068,0.0664759526032788)
--(axis cs:8.16326530612245,0.085061432980389)
--(axis cs:8.50340136054422,0.0897019474495368)
--(axis cs:8.84353741496599,0.0852484403696938)
--(axis cs:9.18367346938775,0.0936986364851996)
--(axis cs:9.52380952380952,0.0949461775865184)
--(axis cs:9.86394557823129,0.0939402972086484)
--(axis cs:10.2040816326531,0.094571310478098)
--(axis cs:10.5442176870748,0.0937102432216955)
--(axis cs:10.8843537414966,0.0852896579316894)
--(axis cs:11.2244897959184,0.100386672679809)
--(axis cs:11.5646258503401,0.0991936758154906)
--(axis cs:11.9047619047619,0.103907521608875)
--(axis cs:12.2448979591837,0.100772061094077)
--(axis cs:12.5850340136054,0.104865311345111)
--(axis cs:12.9251700680272,0.109884538823907)
--(axis cs:13.265306122449,0.120318085262521)
--(axis cs:13.6054421768707,0.122966923685961)
--(axis cs:13.9455782312925,0.122905937414497)
--(axis cs:14.2857142857143,0.148464390434277)
--(axis cs:14.6258503401361,0.152266068896631)
--(axis cs:14.9659863945578,0.148849811470024)
--(axis cs:15.3061224489796,0.152913343071713)
--(axis cs:15.6462585034014,0.165661439932382)
--(axis cs:15.9863945578231,0.172030220314322)
--(axis cs:16.3265306122449,0.18074226583403)
--(axis cs:16.6666666666667,0.18595930914183)
--(axis cs:17.0068027210884,0.205881750126019)
--(axis cs:17.3469387755102,0.214285654280063)
--(axis cs:17.687074829932,0.227349239412793)
--(axis cs:18.0272108843537,0.232941196895999)
--(axis cs:18.3673469387755,0.244159444673262)
--(axis cs:18.7074829931973,0.264346764635488)
--(axis cs:19.047619047619,0.287365655745131)
--(axis cs:19.3877551020408,0.29308126712882)
--(axis cs:19.7278911564626,0.296370830444495)
--(axis cs:20.0680272108844,0.304740759573163)
--(axis cs:20.4081632653061,0.312957157536319)
--(axis cs:20.7482993197279,0.315032048412447)
--(axis cs:21.0884353741497,0.318561492072496)
--(axis cs:21.4285714285714,0.324652959268892)
--(axis cs:21.7687074829932,0.319044382434312)
--(axis cs:22.108843537415,0.324806807036129)
--(axis cs:22.4489795918367,0.32758105253113)
--(axis cs:22.7891156462585,0.330173576269472)
--(axis cs:23.1292517006803,0.335541526252415)
--(axis cs:23.469387755102,0.341033796989986)
--(axis cs:23.8095238095238,0.353205209262909)
--(axis cs:24.1496598639456,0.357569610624548)
--(axis cs:24.4897959183673,0.372272439609111)
--(axis cs:24.8299319727891,0.371185826803638)
--(axis cs:25.1700680272109,0.375824990032705)
--(axis cs:25.5102040816327,0.380899178098864)
--(axis cs:25.8503401360544,0.384023127104177)
--(axis cs:26.1904761904762,0.384563938000766)
--(axis cs:26.530612244898,0.38435055681093)
--(axis cs:26.8707482993197,0.385785122209718)
--(axis cs:27.2108843537415,0.384649009035766)
--(axis cs:27.5510204081633,0.377877484633439)
--(axis cs:27.891156462585,0.38397810545687)
--(axis cs:28.2312925170068,0.382793019023571)
--(axis cs:28.5714285714286,0.382210636100952)
--(axis cs:28.9115646258503,0.387328486261337)
--(axis cs:29.2517006802721,0.388675110493986)
--(axis cs:29.5918367346939,0.396978119471596)
--(axis cs:29.9319727891156,0.387133371118957)
--(axis cs:30.2721088435374,0.395933499280668)
--(axis cs:30.6122448979592,0.397407970417224)
--(axis cs:30.952380952381,0.405753712563622)
--(axis cs:31.2925170068027,0.414010626102265)
--(axis cs:31.6326530612245,0.412656527434768)
--(axis cs:31.9727891156463,0.414773575646218)
--(axis cs:32.312925170068,0.415495126329057)
--(axis cs:32.6530612244898,0.425996331937662)
--(axis cs:32.9931972789116,0.425539472193861)
--(axis cs:33.3333333333333,0.416813064215287)
--(axis cs:33.6734693877551,0.419678335745848)
--(axis cs:34.0136054421769,0.423604216508242)
--(axis cs:34.3537414965986,0.423254532543281)
--(axis cs:34.6938775510204,0.428166860070788)
--(axis cs:35.0340136054422,0.453564063422175)
--(axis cs:35.3741496598639,0.452256433626057)
--(axis cs:35.7142857142857,0.446066310949518)
--(axis cs:36.0544217687075,0.447157940610728)
--(axis cs:36.3945578231292,0.4476260258663)
--(axis cs:36.734693877551,0.449253299267679)
--(axis cs:37.0748299319728,0.452463510553453)
--(axis cs:37.4149659863946,0.464302847791816)
--(axis cs:37.7551020408163,0.461909180609133)
--(axis cs:38.0952380952381,0.474834418489593)
--(axis cs:38.4353741496599,0.477355380101035)
--(axis cs:38.7755102040816,0.480598862112602)
--(axis cs:39.1156462585034,0.480296810349676)
--(axis cs:39.4557823129252,0.480959934850933)
--(axis cs:39.7959183673469,0.480456329063637)
--(axis cs:40.1360544217687,0.479119709036686)
--(axis cs:40.4761904761905,0.479664183495669)
--(axis cs:40.8163265306122,0.481632449662202)
--(axis cs:41.156462585034,0.483846209570115)
--(axis cs:41.4965986394558,0.483651333548965)
--(axis cs:41.8367346938776,0.470345089846822)
--(axis cs:42.1768707482993,0.473304032212746)
--(axis cs:42.5170068027211,0.472411613612872)
--(axis cs:42.8571428571429,0.471055749022785)
--(axis cs:43.1972789115646,0.470000120729393)
--(axis cs:43.5374149659864,0.470458378026334)
--(axis cs:43.8775510204082,0.469604634140721)
--(axis cs:44.2176870748299,0.47115373891119)
--(axis cs:44.5578231292517,0.470891362817115)
--(axis cs:44.8979591836735,0.470540180656607)
--(axis cs:45.2380952380952,0.481757559713571)
--(axis cs:45.578231292517,0.484661040030131)
--(axis cs:45.9183673469388,0.486168736409363)
--(axis cs:46.2585034013605,0.495472093468469)
--(axis cs:46.5986394557823,0.496902837756088)
--(axis cs:46.9387755102041,0.503824797445474)
--(axis cs:47.2789115646259,0.509850932548792)
--(axis cs:47.6190476190476,0.509002931135986)
--(axis cs:47.9591836734694,0.510518080305506)
--(axis cs:48.2993197278912,0.508710658904072)
--(axis cs:48.6394557823129,0.508285060177399)
--(axis cs:48.9795918367347,0.51744324941772)
--(axis cs:49.3197278911565,0.523276842596056)
--(axis cs:49.6598639455782,0.519881229332138)
--(axis cs:50,0.526360979366803)
--(axis cs:50.3401360544218,0.52937974798036)
--(axis cs:50.6802721088435,0.529633797503784)
--(axis cs:51.0204081632653,0.527346622553294)
--(axis cs:51.3605442176871,0.532483226585928)
--(axis cs:51.7006802721088,0.53276929473381)
--(axis cs:52.0408163265306,0.533766219739671)
--(axis cs:52.3809523809524,0.532833619261476)
--(axis cs:52.7210884353741,0.54001544728752)
--(axis cs:53.0612244897959,0.539486830879826)
--(axis cs:53.4013605442177,0.539659685814584)
--(axis cs:53.7414965986395,0.535461571333458)
--(axis cs:54.0816326530612,0.53632274413928)
--(axis cs:54.421768707483,0.537295137554902)
--(axis cs:54.7619047619048,0.538396744710219)
--(axis cs:55.1020408163265,0.536941956345191)
--(axis cs:55.4421768707483,0.539592648310943)
--(axis cs:55.7823129251701,0.542758148775575)
--(axis cs:56.1224489795918,0.546506311903483)
--(axis cs:56.4625850340136,0.555270477699032)
--(axis cs:56.8027210884354,0.563859612307799)
--(axis cs:57.1428571428571,0.563997041236645)
--(axis cs:57.4829931972789,0.570303901052562)
--(axis cs:57.8231292517007,0.574636777468438)
--(axis cs:58.1632653061224,0.580128277531551)
--(axis cs:58.5034013605442,0.589329602567537)
--(axis cs:58.843537414966,0.589691820176757)
--(axis cs:59.1836734693878,0.588251525356398)
--(axis cs:59.5238095238095,0.595958940983474)
--(axis cs:59.8639455782313,0.587041442438063)
--(axis cs:60.2040816326531,0.595069100815664)
--(axis cs:60.5442176870748,0.591200207683531)
--(axis cs:60.8843537414966,0.59104469404263)
--(axis cs:61.2244897959184,0.587298937365773)
--(axis cs:61.5646258503401,0.590707178117433)
--(axis cs:61.9047619047619,0.594091909382798)
--(axis cs:62.2448979591837,0.59432728430288)
--(axis cs:62.5850340136054,0.587149311504485)
--(axis cs:62.9251700680272,0.59001080703575)
--(axis cs:63.265306122449,0.591468321057237)
--(axis cs:63.6054421768707,0.593702148480907)
--(axis cs:63.9455782312925,0.597755645725807)
--(axis cs:64.2857142857143,0.594412086679455)
--(axis cs:64.6258503401361,0.597221059921822)
--(axis cs:64.9659863945578,0.604358072013924)
--(axis cs:65.3061224489796,0.608409060064679)
--(axis cs:65.6462585034014,0.6086518879135)
--(axis cs:65.9863945578231,0.613086737987957)
--(axis cs:66.3265306122449,0.605776986001505)
--(axis cs:66.6666666666667,0.608944899673816)
--(axis cs:67.0068027210884,0.615712982063757)
--(axis cs:67.3469387755102,0.626210229864593)
--(axis cs:67.687074829932,0.634193073194786)
--(axis cs:68.0272108843537,0.639299827071818)
--(axis cs:68.3673469387755,0.649565984306822)
--(axis cs:68.7074829931973,0.654205497065513)
--(axis cs:69.0476190476191,0.653424549999197)
--(axis cs:69.3877551020408,0.651455580305506)
--(axis cs:69.7278911564626,0.666145989834638)
--(axis cs:70.0680272108844,0.661100244013886)
--(axis cs:70.4081632653061,0.668893506849352)
--(axis cs:70.7482993197279,0.676551374719389)
--(axis cs:71.0884353741497,0.684562606066698)
--(axis cs:71.4285714285714,0.685409432890215)
--(axis cs:71.7687074829932,0.686908696456973)
--(axis cs:72.108843537415,0.689770935044586)
--(axis cs:72.4489795918367,0.70181432067995)
--(axis cs:72.7891156462585,0.710720339813881)
--(axis cs:73.1292517006803,0.715370281081217)
--(axis cs:73.469387755102,0.709846191611376)
--(axis cs:73.8095238095238,0.718015231213867)
--(axis cs:74.1496598639456,0.728809378825552)
--(axis cs:74.4897959183673,0.757518902723615)
--(axis cs:74.8299319727891,0.770910058277228)
--(axis cs:75.1700680272109,0.774542851074297)
--(axis cs:75.5102040816327,0.772336664087698)
--(axis cs:75.8503401360544,0.771335830680945)
--(axis cs:76.1904761904762,0.785812371534806)
--(axis cs:76.530612244898,0.795604813353686)
--(axis cs:76.8707482993197,0.79091796875)
--(axis cs:77.2108843537415,0.797332137940456)
--(axis cs:77.5510204081633,0.797400216053779)
--(axis cs:77.891156462585,0.81079109952237)
--(axis cs:78.2312925170068,0.819233631705344)
--(axis cs:78.5714285714286,0.831880581543948)
--(axis cs:78.9115646258503,0.835398503066672)
--(axis cs:79.2517006802721,0.833778603775205)
--(axis cs:79.5918367346939,0.831010000955373)
--(axis cs:79.9319727891156,0.834435815363886)
--(axis cs:80.2721088435374,0.843917321799004)
--(axis cs:80.6122448979592,0.852637064280599)
--(axis cs:80.9523809523809,0.858113813560101)
--(axis cs:81.2925170068027,0.865425623693583)
--(axis cs:81.6326530612245,0.863905639672278)
--(axis cs:81.9727891156463,0.86381619843162)
--(axis cs:82.312925170068,0.86770815810073)
--(axis cs:82.6530612244898,0.86714887889827)
--(axis cs:82.9931972789116,0.870938014002511)
--(axis cs:83.3333333333333,0.872861800056392)
--(axis cs:83.6734693877551,0.873428961383679)
--(axis cs:84.0136054421769,0.873408764081071)
--(axis cs:84.3537414965986,0.87537356068531)
--(axis cs:84.6938775510204,0.873670733671582)
--(axis cs:85.0340136054422,0.875630722604728)
--(axis cs:85.3741496598639,0.880652707946984)
--(axis cs:85.7142857142857,0.889236568854524)
--(axis cs:86.0544217687075,0.891580908369667)
--(axis cs:86.3945578231292,0.894110185406834)
--(axis cs:86.734693877551,0.902551682197612)
--(axis cs:87.0748299319728,0.899739435005915)
--(axis cs:87.4149659863945,0.900936651753802)
--(axis cs:87.7551020408163,0.91181796513546)
--(axis cs:88.0952380952381,0.916092655708644)
--(axis cs:88.4353741496599,0.916164555898313)
--(axis cs:88.7755102040816,0.917100373014052)
--(axis cs:89.1156462585034,0.918340254329776)
--(axis cs:89.4557823129252,0.916374950062372)
--(axis cs:89.7959183673469,0.918279285266983)
--(axis cs:90.1360544217687,0.918016394860231)
--(axis cs:90.4761904761905,0.916321438628697)
--(axis cs:90.8163265306122,0.911635851504874)
--(axis cs:91.156462585034,0.917432471645634)
--(axis cs:91.4965986394558,0.916537509442958)
--(axis cs:91.8367346938775,0.935836855206199)
--(axis cs:92.1768707482993,0.933913120231084)
--(axis cs:92.5170068027211,0.939310950005894)
--(axis cs:92.8571428571429,0.945880010636028)
--(axis cs:93.1972789115646,0.945271086890408)
--(axis cs:93.5374149659864,0.941261605659109)
--(axis cs:93.8775510204082,0.940772100084703)
--(axis cs:94.2176870748299,0.936936284956438)
--(axis cs:94.5578231292517,0.940987211971674)
--(axis cs:94.8979591836735,0.940363689911904)
--(axis cs:95.2380952380952,0.935134704985166)
--(axis cs:95.578231292517,0.93720526657011)
--(axis cs:95.9183673469388,0.932584417753329)
--(axis cs:96.2585034013605,0.933976192709122)
--(axis cs:96.5986394557823,0.94103041677193)
--(axis cs:96.9387755102041,0.953145986719451)
--(axis cs:97.2789115646258,0.956699514685579)
--(axis cs:97.6190476190476,0.958548597127699)
--(axis cs:97.9591836734694,0.95821535329792)
--(axis cs:98.2993197278912,0.958173626008778)
--(axis cs:98.6394557823129,0.958065782009022)
--(axis cs:98.9795918367347,0.958234098371199)
--(axis cs:99.3197278911565,0.958277375298462)
--(axis cs:99.6598639455782,0.958255348646644)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,0.965807151353356)
--(axis cs:99.3197278911565,0.963597624701538)
--(axis cs:98.9795918367347,0.967390901628801)
--(axis cs:98.6394557823129,0.966621717990979)
--(axis cs:98.2993197278912,0.967138873991222)
--(axis cs:97.9591836734694,0.96522214670208)
--(axis cs:97.6190476190476,0.968638902872301)
--(axis cs:97.2789115646258,0.968300485314421)
--(axis cs:96.9387755102041,0.971229013280549)
--(axis cs:96.5986394557823,0.96115708322807)
--(axis cs:96.2585034013605,0.952586307290878)
--(axis cs:95.9183673469388,0.949915582246671)
--(axis cs:95.578231292517,0.95341973342989)
--(axis cs:95.2380952380952,0.951427795014834)
--(axis cs:94.8979591836735,0.955261310088096)
--(axis cs:94.5578231292517,0.956200288028326)
--(axis cs:94.2176870748299,0.953376215043562)
--(axis cs:93.8775510204082,0.956415399915297)
--(axis cs:93.5374149659864,0.956238394340891)
--(axis cs:93.1972789115646,0.960041413109592)
--(axis cs:92.8571428571429,0.963494989363972)
--(axis cs:92.5170068027211,0.957564049994106)
--(axis cs:92.1768707482993,0.946399379768916)
--(axis cs:91.8367346938775,0.945413144793801)
--(axis cs:91.4965986394558,0.929399990557042)
--(axis cs:91.156462585034,0.931317528354366)
--(axis cs:90.8163265306122,0.929301648495126)
--(axis cs:90.4761904761905,0.928366061371303)
--(axis cs:90.1360544217687,0.927608605139769)
--(axis cs:89.7959183673469,0.931095714733017)
--(axis cs:89.4557823129252,0.927375049937628)
--(axis cs:89.1156462585034,0.931347245670224)
--(axis cs:88.7755102040816,0.930712126985948)
--(axis cs:88.4353741496599,0.926647944101687)
--(axis cs:88.0952380952381,0.925157344291356)
--(axis cs:87.7551020408163,0.92380703486454)
--(axis cs:87.4149659863945,0.919375848246198)
--(axis cs:87.0748299319728,0.920885564994085)
--(axis cs:86.734693877551,0.924635817802388)
--(axis cs:86.3945578231292,0.913389814593166)
--(axis cs:86.0544217687075,0.910606591630333)
--(axis cs:85.7142857142857,0.907950931145476)
--(axis cs:85.3741496598639,0.897159792053016)
--(axis cs:85.0340136054422,0.891556777395272)
--(axis cs:84.6938775510204,0.885704266328418)
--(axis cs:84.3537414965986,0.88681393931469)
--(axis cs:84.0136054421769,0.883778735918929)
--(axis cs:83.6734693877551,0.885008538616321)
--(axis cs:83.3333333333333,0.882763199943608)
--(axis cs:82.9931972789116,0.882811985997488)
--(axis cs:82.6530612244898,0.88097612110173)
--(axis cs:82.312925170068,0.88197934189927)
--(axis cs:81.9727891156463,0.87930880156838)
--(axis cs:81.6326530612245,0.879531860327722)
--(axis cs:81.2925170068027,0.880824376306417)
--(axis cs:80.9523809523809,0.876573686439899)
--(axis cs:80.6122448979592,0.873612935719401)
--(axis cs:80.2721088435374,0.867645178200997)
--(axis cs:79.9319727891156,0.860876684636114)
--(axis cs:79.5918367346939,0.857739999044627)
--(axis cs:79.2517006802721,0.858408896224795)
--(axis cs:78.9115646258503,0.859601496933328)
--(axis cs:78.5714285714286,0.858119418456052)
--(axis cs:78.2312925170068,0.847953868294656)
--(axis cs:77.891156462585,0.83920890047763)
--(axis cs:77.5510204081633,0.824474783946221)
--(axis cs:77.2108843537415,0.825792862059544)
--(axis cs:76.8707482993197,0.82001953125)
--(axis cs:76.530612244898,0.824707686646314)
--(axis cs:76.1904761904762,0.813250128465194)
--(axis cs:75.8503401360544,0.801476669319055)
--(axis cs:75.5102040816327,0.802975835912302)
--(axis cs:75.1700680272109,0.805144648925703)
--(axis cs:74.8299319727891,0.802214941722772)
--(axis cs:74.4897959183673,0.790293597276385)
--(axis cs:74.1496598639456,0.760878121174448)
--(axis cs:73.8095238095238,0.748859768786132)
--(axis cs:73.469387755102,0.738903808388624)
--(axis cs:73.1292517006803,0.744004718918783)
--(axis cs:72.7891156462585,0.740529660186119)
--(axis cs:72.4489795918367,0.72943567932005)
--(axis cs:72.108843537415,0.719291564955414)
--(axis cs:71.7687074829932,0.715278803543027)
--(axis cs:71.4285714285714,0.711778067109785)
--(axis cs:71.0884353741497,0.708874893933302)
--(axis cs:70.7482993197279,0.703136125280611)
--(axis cs:70.4081632653061,0.694231493150648)
--(axis cs:70.0680272108844,0.689524755986114)
--(axis cs:69.7278911564626,0.693229010165362)
--(axis cs:69.3877551020408,0.678231919694493)
--(axis cs:69.0476190476191,0.680950450000803)
--(axis cs:68.7074829931973,0.683607002934487)
--(axis cs:68.3673469387755,0.679184015693178)
--(axis cs:68.0272108843537,0.666950172928182)
--(axis cs:67.687074829932,0.663931926805214)
--(axis cs:67.3469387755102,0.653164770135407)
--(axis cs:67.0068027210884,0.641787017936243)
--(axis cs:66.6666666666667,0.635742600326184)
--(axis cs:66.3265306122449,0.630473013998495)
--(axis cs:65.9863945578231,0.636913262012043)
--(axis cs:65.6462585034014,0.6304106120865)
--(axis cs:65.3061224489796,0.627215939935321)
--(axis cs:64.9659863945578,0.625016927986076)
--(axis cs:64.6258503401361,0.619341440078178)
--(axis cs:64.2857142857143,0.617775413320545)
--(axis cs:63.9455782312925,0.618806854274193)
--(axis cs:63.6054421768707,0.615672851519093)
--(axis cs:63.265306122449,0.613844178942763)
--(axis cs:62.9251700680272,0.61061419296425)
--(axis cs:62.5850340136054,0.607225688495515)
--(axis cs:62.2448979591837,0.61567271569712)
--(axis cs:61.9047619047619,0.615283090617202)
--(axis cs:61.5646258503401,0.613667821882567)
--(axis cs:61.2244897959184,0.609263562634227)
--(axis cs:60.8843537414966,0.612392805957369)
--(axis cs:60.5442176870748,0.612862292316469)
--(axis cs:60.2040816326531,0.616805899184336)
--(axis cs:59.8639455782313,0.611396057561937)
--(axis cs:59.5238095238095,0.618728559016526)
--(axis cs:59.1836734693878,0.612998474643602)
--(axis cs:58.843537414966,0.614058179823243)
--(axis cs:58.5034013605442,0.613482897432463)
--(axis cs:58.1632653061224,0.606121722468449)
--(axis cs:57.8231292517007,0.600363222531562)
--(axis cs:57.4829931972789,0.597196098947438)
--(axis cs:57.1428571428571,0.592565458763355)
--(axis cs:56.8027210884354,0.591765387692201)
--(axis cs:56.4625850340136,0.582854522300968)
--(axis cs:56.1224489795918,0.575681188096517)
--(axis cs:55.7823129251701,0.571616851224425)
--(axis cs:55.4421768707483,0.566657351689057)
--(axis cs:55.1020408163265,0.562433043654809)
--(axis cs:54.7619047619048,0.565665755289781)
--(axis cs:54.421768707483,0.564267362445098)
--(axis cs:54.0816326530612,0.56461475586072)
--(axis cs:53.7414965986395,0.562038428666542)
--(axis cs:53.4013605442177,0.565965314185417)
--(axis cs:53.0612244897959,0.565200669120174)
--(axis cs:52.7210884353741,0.56654705271248)
--(axis cs:52.3809523809524,0.556853880738524)
--(axis cs:52.0408163265306,0.558421280260329)
--(axis cs:51.7006802721088,0.55754320526619)
--(axis cs:51.3605442176871,0.557516773414072)
--(axis cs:51.0204081632653,0.553903377446706)
--(axis cs:50.6802721088435,0.555053702496216)
--(axis cs:50.3401360544218,0.55749525201964)
--(axis cs:50,0.554264020633197)
--(axis cs:49.6598639455782,0.548556270667862)
--(axis cs:49.3197278911565,0.551410657403944)
--(axis cs:48.9795918367347,0.54724425058228)
--(axis cs:48.6394557823129,0.536714939822601)
--(axis cs:48.2993197278912,0.534726841095928)
--(axis cs:47.9591836734694,0.537294419694494)
--(axis cs:47.6190476190476,0.535997068864013)
--(axis cs:47.2789115646259,0.536399067451208)
--(axis cs:46.9387755102041,0.531800202554526)
--(axis cs:46.5986394557823,0.525597162243912)
--(axis cs:46.2585034013605,0.522965406531532)
--(axis cs:45.9183673469388,0.513518763590637)
--(axis cs:45.578231292517,0.512526459969869)
--(axis cs:45.2380952380952,0.510429940286429)
--(axis cs:44.8979591836735,0.497272319343393)
--(axis cs:44.5578231292517,0.497858637182885)
--(axis cs:44.2176870748299,0.49822126108881)
--(axis cs:43.8775510204082,0.496645365859279)
--(axis cs:43.5374149659864,0.497354121973666)
--(axis cs:43.1972789115646,0.498437379270607)
--(axis cs:42.8571428571429,0.498006750977215)
--(axis cs:42.5170068027211,0.499150886387128)
--(axis cs:42.1768707482993,0.500758467787254)
--(axis cs:41.8367346938776,0.498404910153178)
--(axis cs:41.4965986394558,0.511973666451034)
--(axis cs:41.156462585034,0.510216290429885)
--(axis cs:40.8163265306122,0.507117550337798)
--(axis cs:40.4761904761905,0.506273316504331)
--(axis cs:40.1360544217687,0.505567790963314)
--(axis cs:39.7959183673469,0.508293670936363)
--(axis cs:39.4557823129252,0.508415065149067)
--(axis cs:39.1156462585034,0.507203189650324)
--(axis cs:38.7755102040816,0.506588637887398)
--(axis cs:38.4353741496599,0.504207119898965)
--(axis cs:38.0952380952381,0.501415581510407)
--(axis cs:37.7551020408163,0.487778319390867)
--(axis cs:37.4149659863946,0.488822152208184)
--(axis cs:37.0748299319728,0.480036489446547)
--(axis cs:36.734693877551,0.475121700732321)
--(axis cs:36.3945578231292,0.4754989741337)
--(axis cs:36.0544217687075,0.474404559389272)
--(axis cs:35.7142857142857,0.474246189050482)
--(axis cs:35.3741496598639,0.478993566373943)
--(axis cs:35.0340136054422,0.482685936577825)
--(axis cs:34.6938775510204,0.458708139929212)
--(axis cs:34.3537414965986,0.456120467456719)
--(axis cs:34.0136054421769,0.456395783491758)
--(axis cs:33.6734693877551,0.452821664254152)
--(axis cs:33.3333333333333,0.450374435784713)
--(axis cs:32.9931972789116,0.458835527806139)
--(axis cs:32.6530612244898,0.459628668062338)
--(axis cs:32.312925170068,0.449817373670943)
--(axis cs:31.9727891156463,0.448351424353783)
--(axis cs:31.6326530612245,0.447030972565232)
--(axis cs:31.2925170068027,0.449426873897735)
--(axis cs:30.952380952381,0.440496287436378)
--(axis cs:30.6122448979592,0.431029529582776)
--(axis cs:30.2721088435374,0.429691500719332)
--(axis cs:29.9319727891156,0.421304128881043)
--(axis cs:29.5918367346939,0.430209380528404)
--(axis cs:29.2517006802721,0.420387389506014)
--(axis cs:28.9115646258503,0.417359013738663)
--(axis cs:28.5714285714286,0.412789363899048)
--(axis cs:28.2312925170068,0.413144480976429)
--(axis cs:27.891156462585,0.41477189454313)
--(axis cs:27.5510204081633,0.408372515366561)
--(axis cs:27.2108843537415,0.415350990964234)
--(axis cs:26.8707482993197,0.416714877790282)
--(axis cs:26.530612244898,0.41627444318907)
--(axis cs:26.1904761904762,0.415748561999234)
--(axis cs:25.8503401360544,0.415976872895823)
--(axis cs:25.5102040816327,0.411288321901136)
--(axis cs:25.1700680272109,0.407300009967295)
--(axis cs:24.8299319727891,0.405376673196362)
--(axis cs:24.4897959183673,0.405852560390889)
--(axis cs:24.1496598639456,0.391180389375452)
--(axis cs:23.8095238095238,0.385232290737091)
--(axis cs:23.469387755102,0.373028703010014)
--(axis cs:23.1292517006803,0.364145973747585)
--(axis cs:22.7891156462585,0.360451423730528)
--(axis cs:22.4489795918367,0.35898144746887)
--(axis cs:22.108843537415,0.357380692963871)
--(axis cs:21.7687074829932,0.348455617565688)
--(axis cs:21.4285714285714,0.356284540731108)
--(axis cs:21.0884353741497,0.351126007927504)
--(axis cs:20.7482993197279,0.349030451587553)
--(axis cs:20.4081632653061,0.344855342463681)
--(axis cs:20.0680272108844,0.338071740426837)
--(axis cs:19.7278911564626,0.330504169555505)
--(axis cs:19.3877551020408,0.32910623287118)
--(axis cs:19.047619047619,0.325759344254869)
--(axis cs:18.7074829931973,0.302528235364512)
--(axis cs:18.3673469387755,0.284903055326738)
--(axis cs:18.0272108843537,0.274558803104001)
--(axis cs:17.687074829932,0.270150760587207)
--(axis cs:17.3469387755102,0.258526845719937)
--(axis cs:17.0068027210884,0.250680749873981)
--(axis cs:16.6666666666667,0.22966569085817)
--(axis cs:16.3265306122449,0.22457023416597)
--(axis cs:15.9863945578231,0.217969779685678)
--(axis cs:15.6462585034014,0.210901060067618)
--(axis cs:15.3061224489796,0.195524156928287)
--(axis cs:14.9659863945578,0.191150188529976)
--(axis cs:14.6258503401361,0.195233931103369)
--(axis cs:14.2857142857143,0.190910609565723)
--(axis cs:13.9455782312925,0.164594062585503)
--(axis cs:13.6054421768707,0.163908076314039)
--(axis cs:13.265306122449,0.159994414737479)
--(axis cs:12.9251700680272,0.148552961176093)
--(axis cs:12.5850340136054,0.143572188654889)
--(axis cs:12.2448979591837,0.137977938905923)
--(axis cs:11.9047619047619,0.141404978391125)
--(axis cs:11.5646258503401,0.136431324184509)
--(axis cs:11.2244897959184,0.136488327320191)
--(axis cs:10.8843537414966,0.119397842068311)
--(axis cs:10.5442176870748,0.127227256778304)
--(axis cs:10.2040816326531,0.126678689521902)
--(axis cs:9.86394557823129,0.125434702791352)
--(axis cs:9.52380952380952,0.127241322413482)
--(axis cs:9.18367346938775,0.1266138635148)
--(axis cs:8.84353741496599,0.116939059630306)
--(axis cs:8.50340136054422,0.122798052550463)
--(axis cs:8.16326530612245,0.117438567019611)
--(axis cs:7.82312925170068,0.0966490473967212)
--(axis cs:7.48299319727891,0.0672160520199365)
--(axis cs:7.14285714285714,0.0682328651806014)
--(axis cs:6.80272108843537,0.0714424853251472)
--(axis cs:6.46258503401361,0.0796419851866343)
--(axis cs:6.12244897959184,0.0805366973550992)
--(axis cs:5.78231292517007,0.0852712395244477)
--(axis cs:5.4421768707483,0.0858446065162003)
--(axis cs:5.10204081632653,0.079552260822222)
--(axis cs:4.76190476190476,0.0772442510699069)
--(axis cs:4.42176870748299,0.066942571395672)
--(axis cs:4.08163265306122,0.0629827091889929)
--(axis cs:3.74149659863946,0.059958530270816)
--(axis cs:3.40136054421769,0.0690423369230385)
--(axis cs:3.06122448979592,0.0773322560558305)
--(axis cs:2.72108843537415,0.0614078475648683)
--(axis cs:2.38095238095238,0.0659936978437762)
--(axis cs:2.04081632653061,0.0700742278072174)
--(axis cs:1.70068027210884,0.0794225111101698)
--(axis cs:1.36054421768707,0.0757826154311892)
--(axis cs:1.02040816326531,0.0824703217434256)
--(axis cs:0.680272108843537,0.0830136024880794)
--(axis cs:0.340136054421769,0.0798228235154227)
--(axis cs:0,0.0831104778102871)
--cycle;


==> img/stl10/stl10_rate_accuracy_lrp.tex <==
% lrp-a-flat
\addplot [line width=0.5, opacity=0.8, color1, mark=otimes*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table [row sep=\\]{%
0	0.0759375 \\
0.340136054421769	0.0590625 \\
0.680272108843537	0.048125 \\
1.02040816326531	0.0490625 \\
1.36054421768707	0.073125 \\
1.70068027210884	0.1059375 \\
2.04081632653061	0.1546875 \\
2.38095238095238	0.1684375 \\
2.72108843537415	0.17875 \\
3.06122448979592	0.2034375 \\
3.40136054421769	0.22109375 \\
3.74149659863946	0.25515625 \\
4.08163265306122	0.2746875 \\
4.42176870748299	0.28875 \\
4.76190476190476	0.3209375 \\
5.10204081632653	0.3440625 \\
5.4421768707483	0.36484375 \\
5.78231292517007	0.3871875 \\
6.12244897959184	0.3965625 \\
6.46258503401361	0.40140625 \\
6.80272108843537	0.4340625 \\
7.14285714285714	0.46671875 \\
7.48299319727891	0.48734375 \\
7.82312925170068	0.49953125 \\
8.16326530612245	0.51203125 \\
8.50340136054422	0.5246875 \\
8.84353741496599	0.528125 \\
9.18367346938775	0.5378125 \\
9.52380952380952	0.553125 \\
9.86394557823129	0.5640625 \\
10.2040816326531	0.5728125 \\
10.5442176870748	0.5846875 \\
10.8843537414966	0.5953125 \\
11.2244897959184	0.60375 \\
11.5646258503401	0.6078125 \\
11.9047619047619	0.6084375 \\
12.2448979591837	0.6096875 \\
12.5850340136054	0.60875 \\
12.9251700680272	0.6171875 \\
13.265306122449	0.61921875 \\
13.6054421768707	0.620625 \\
13.9455782312925	0.6184375 \\
14.2857142857143	0.62421875 \\
14.6258503401361	0.63296875 \\
14.9659863945578	0.63828125 \\
15.3061224489796	0.64359375 \\
15.6462585034014	0.65578125 \\
15.9863945578231	0.6571875 \\
16.3265306122449	0.66609375 \\
16.6666666666667	0.6728125 \\
17.0068027210884	0.67390625 \\
17.3469387755102	0.67546875 \\
17.687074829932	0.6915625 \\
18.0272108843537	0.70203125 \\
18.3673469387755	0.7125 \\
18.7074829931973	0.70921875 \\
19.047619047619	0.7175 \\
19.3877551020408	0.71453125 \\
19.7278911564626	0.718125 \\
20.0680272108844	0.72171875 \\
20.4081632653061	0.7228125 \\
20.7482993197279	0.7203125 \\
21.0884353741497	0.7228125 \\
21.4285714285714	0.7234375 \\
21.7687074829932	0.7234375 \\
22.108843537415	0.72984375 \\
22.4489795918367	0.73171875 \\
22.7891156462585	0.73765625 \\
23.1292517006803	0.74203125 \\
23.469387755102	0.75453125 \\
23.8095238095238	0.76125 \\
24.1496598639456	0.7728125 \\
24.4897959183673	0.77375 \\
24.8299319727891	0.778125 \\
25.1700680272109	0.784375 \\
25.5102040816327	0.78359375 \\
25.8503401360544	0.78984375 \\
26.1904761904762	0.79375 \\
26.530612244898	0.79203125 \\
26.8707482993197	0.7971875 \\
27.2108843537415	0.8 \\
27.5510204081633	0.805 \\
27.891156462585	0.81046875 \\
28.2312925170068	0.81046875 \\
28.5714285714286	0.81078125 \\
28.9115646258503	0.81046875 \\
29.2517006802721	0.8103125 \\
29.5918367346939	0.8153125 \\
29.9319727891156	0.8190625 \\
30.2721088435374	0.81921875 \\
30.6122448979592	0.8203125 \\
30.952380952381	0.82109375 \\
31.2925170068027	0.82109375 \\
31.6326530612245	0.820625 \\
31.9727891156463	0.82171875 \\
32.312925170068	0.8228125 \\
32.6530612244898	0.83015625 \\
32.9931972789116	0.83078125 \\
33.3333333333333	0.831875 \\
33.6734693877551	0.83875 \\
34.0136054421769	0.84328125 \\
34.3537414965986	0.8546875 \\
34.6938775510204	0.8553125 \\
35.0340136054422	0.85921875 \\
35.3741496598639	0.86375 \\
35.7142857142857	0.86546875 \\
36.0544217687075	0.86546875 \\
36.3945578231292	0.86484375 \\
36.734693877551	0.8615625 \\
37.0748299319728	0.860625 \\
37.4149659863946	0.86 \\
37.7551020408163	0.85671875 \\
38.0952380952381	0.86390625 \\
38.4353741496599	0.86453125 \\
38.7755102040816	0.8696875 \\
39.1156462585034	0.871875 \\
39.4557823129252	0.8740625 \\
39.7959183673469	0.87328125 \\
40.1360544217687	0.87734375 \\
40.4761904761905	0.88625 \\
40.8163265306122	0.88859375 \\
41.156462585034	0.8975 \\
41.4965986394558	0.89859375 \\
41.8367346938776	0.909375 \\
42.1768707482993	0.9109375 \\
42.5170068027211	0.921875 \\
42.8571428571429	0.91765625 \\
43.1972789115646	0.9196875 \\
43.5374149659864	0.92265625 \\
43.8775510204082	0.9259375 \\
44.2176870748299	0.9225 \\
44.5578231292517	0.925 \\
44.8979591836735	0.9321875 \\
45.2380952380952	0.93421875 \\
45.578231292517	0.9359375 \\
45.9183673469388	0.93671875 \\
46.2585034013605	0.9396875 \\
46.5986394557823	0.94046875 \\
46.9387755102041	0.9396875 \\
47.2789115646259	0.94 \\
47.6190476190476	0.94109375 \\
47.9591836734694	0.9415625 \\
48.2993197278912	0.94296875 \\
48.6394557823129	0.94328125 \\
48.9795918367347	0.945625 \\
49.3197278911565	0.945 \\
49.6598639455782	0.94484375 \\
50	0.94390625 \\
50.3401360544218	0.9459375 \\
50.6802721088435	0.9453125 \\
51.0204081632653	0.9475 \\
51.3605442176871	0.94953125 \\
51.7006802721088	0.94890625 \\
52.0408163265306	0.95140625 \\
52.3809523809524	0.95109375 \\
52.7210884353741	0.95203125 \\
53.0612244897959	0.9525 \\
53.4013605442177	0.95484375 \\
53.7414965986395	0.9534375 \\
54.0816326530612	0.95515625 \\
54.421768707483	0.956875 \\
54.7619047619048	0.95578125 \\
55.1020408163265	0.95921875 \\
55.4421768707483	0.9634375 \\
55.7823129251701	0.96109375 \\
56.1224489795918	0.96484375 \\
56.4625850340136	0.9665625 \\
56.8027210884354	0.96671875 \\
57.1428571428571	0.9675 \\
57.4829931972789	0.96765625 \\
57.8231292517007	0.96984375 \\
58.1632653061224	0.9721875 \\
58.5034013605442	0.97140625 \\
58.843537414966	0.97640625 \\
59.1836734693878	0.97609375 \\
59.5238095238095	0.98 \\
59.8639455782313	0.98703125 \\
60.2040816326531	0.98421875 \\
60.5442176870748	0.9846875 \\
60.8843537414966	0.98375 \\
61.2244897959184	0.9890625 \\
61.5646258503401	0.98515625 \\
61.9047619047619	0.98984375 \\
62.2448979591837	0.986875 \\
62.5850340136054	0.9878125 \\
62.9251700680272	0.9903125 \\
63.265306122449	0.989375 \\
63.6054421768707	0.99265625 \\
63.9455782312925	0.9896875 \\
64.2857142857143	0.98640625 \\
64.6258503401361	0.98390625 \\
64.9659863945578	0.97625 \\
65.3061224489796	0.97375 \\
65.6462585034014	0.97296875 \\
65.9863945578231	0.975625 \\
66.3265306122449	0.975625 \\
66.6666666666667	0.97328125 \\
67.0068027210884	0.9746875 \\
67.3469387755102	0.9803125 \\
67.687074829932	0.9815625 \\
68.0272108843537	0.98296875 \\
68.3673469387755	0.9828125 \\
68.7074829931973	0.9878125 \\
69.0476190476191	0.9875 \\
69.3877551020408	0.98578125 \\
69.7278911564626	0.98875 \\
70.0680272108844	0.988125 \\
70.4081632653061	0.98578125 \\
70.7482993197279	0.98828125 \\
71.0884353741497	0.99015625 \\
71.4285714285714	0.99046875 \\
71.7687074829932	0.9865625 \\
72.108843537415	0.9846875 \\
72.4489795918367	0.98171875 \\
72.7891156462585	0.983125 \\
73.1292517006803	0.985 \\
73.469387755102	0.98203125 \\
73.8095238095238	0.986875 \\
74.1496598639456	0.98703125 \\
74.4897959183673	0.9871875 \\
74.8299319727891	0.99078125 \\
75.1700680272109	0.99203125 \\
75.5102040816327	0.99328125 \\
75.8503401360544	0.9925 \\
76.1904761904762	0.98953125 \\
76.530612244898	0.9825 \\
76.8707482993197	0.9784375 \\
77.2108843537415	0.97890625 \\
77.5510204081633	0.97953125 \\
77.891156462585	0.97625 \\
78.2312925170068	0.975625 \\
78.5714285714286	0.97375 \\
78.9115646258503	0.97546875 \\
79.2517006802721	0.97578125 \\
79.5918367346939	0.97171875 \\
79.9319727891156	0.974375 \\
80.2721088435374	0.9740625 \\
80.6122448979592	0.97328125 \\
80.9523809523809	0.97453125 \\
81.2925170068027	0.969375 \\
81.6326530612245	0.9728125 \\
81.9727891156463	0.97765625 \\
82.312925170068	0.9734375 \\
82.6530612244898	0.9759375 \\
82.9931972789116	0.97546875 \\
83.3333333333333	0.9771875 \\
83.6734693877551	0.97671875 \\
84.0136054421769	0.97375 \\
84.3537414965986	0.9746875 \\
84.6938775510204	0.9775 \\
85.0340136054422	0.98828125 \\
85.3741496598639	0.98765625 \\
85.7142857142857	0.98609375 \\
86.0544217687075	0.9884375 \\
86.3945578231292	0.98890625 \\
86.734693877551	0.9878125 \\
87.0748299319728	0.9896875 \\
87.4149659863945	0.98765625 \\
87.7551020408163	0.98453125 \\
88.0952380952381	0.9846875 \\
88.4353741496599	0.984375 \\
88.7755102040816	0.9796875 \\
89.1156462585034	0.97875 \\
89.4557823129252	0.9790625 \\
89.7959183673469	0.9803125 \\
90.1360544217687	0.9790625 \\
90.4761904761905	0.98140625 \\
90.8163265306122	0.979375 \\
91.156462585034	0.97734375 \\
91.4965986394558	0.976875 \\
91.8367346938775	0.980625 \\
92.1768707482993	0.98234375 \\
92.5170068027211	0.9896875 \\
92.8571428571429	0.995 \\
93.1972789115646	0.998125 \\
93.5374149659864	0.998125 \\
93.8775510204082	0.9971875 \\
94.2176870748299	0.9978125 \\
94.5578231292517	0.99875 \\
94.8979591836735	0.99875 \\
95.2380952380952	0.99859375 \\
95.578231292517	0.99921875 \\
95.9183673469388	0.99828125 \\
96.2585034013605	0.99859375 \\
96.5986394557823	0.99703125 \\
96.9387755102041	0.99796875 \\
97.2789115646258	0.99921875 \\
97.6190476190476	0.99984375 \\
97.9591836734694	0.99796875 \\
98.2993197278912	0.99765625 \\
98.6394557823129	0.99875 \\
98.9795918367347	0.99828125 \\
99.3197278911565	0.9990625 \\
99.6598639455782	0.995625 \\
100	1 \\
};
\path [fill=color1, fill opacity=0.5] (axis cs:0,0.0827971130190766)
--(axis cs:0,0.0690778869809235)
--(axis cs:0.340136054421769,0.0499600154705226)
--(axis cs:0.680272108843537,0.040495302740381)
--(axis cs:1.02040816326531,0.040552386746471)
--(axis cs:1.36054421768707,0.0588819104269496)
--(axis cs:1.70068027210884,0.0896327076848122)
--(axis cs:2.04081632653061,0.139253486563698)
--(axis cs:2.38095238095238,0.153394633192211)
--(axis cs:2.72108843537415,0.161976988244807)
--(axis cs:3.06122448979592,0.184347763758104)
--(axis cs:3.40136054421769,0.200306727701929)
--(axis cs:3.74149659863946,0.234808333534972)
--(axis cs:4.08163265306122,0.253917230050634)
--(axis cs:4.42176870748299,0.268191561743534)
--(axis cs:4.76190476190476,0.300642378979029)
--(axis cs:5.10204081632653,0.324583566160454)
--(axis cs:5.4421768707483,0.346428101120386)
--(axis cs:5.78231292517007,0.369525482309586)
--(axis cs:6.12244897959184,0.377802330231937)
--(axis cs:6.46258503401361,0.383523420008063)
--(axis cs:6.80272108843537,0.414666975494341)
--(axis cs:7.14285714285714,0.447525632009474)
--(axis cs:7.48299319727891,0.469418839569528)
--(axis cs:7.82312925170068,0.481317639403473)
--(axis cs:8.16326530612245,0.493806647009131)
--(axis cs:8.50340136054422,0.505746214989948)
--(axis cs:8.84353741496599,0.509426951856022)
--(axis cs:9.18367346938775,0.519636365738572)
--(axis cs:9.52380952380952,0.535681395802685)
--(axis cs:9.86394557823129,0.546095342292018)
--(axis cs:10.2040816326531,0.554180874972325)
--(axis cs:10.5442176870748,0.567157183068502)
--(axis cs:10.8843537414966,0.578483293290047)
--(axis cs:11.2244897959184,0.586764548749026)
--(axis cs:11.5646258503401,0.590676680147379)
--(axis cs:11.9047619047619,0.592627438699357)
--(axis cs:12.2448979591837,0.592850928086199)
--(axis cs:12.5850340136054,0.592101399358495)
--(axis cs:12.9251700680272,0.600577323007074)
--(axis cs:13.265306122449,0.602907232672229)
--(axis cs:13.6054421768707,0.604998169052588)
--(axis cs:13.9455782312925,0.602455255823845)
--(axis cs:14.2857142857143,0.609169861671722)
--(axis cs:14.6258503401361,0.618950060104655)
--(axis cs:14.9659863945578,0.625517387595866)
--(axis cs:15.3061224489796,0.630491425256036)
--(axis cs:15.6462585034014,0.641702144678104)
--(axis cs:15.9863945578231,0.642539713556135)
--(axis cs:16.3265306122449,0.651548868645778)
--(axis cs:16.6666666666667,0.657851001560777)
--(axis cs:17.0068027210884,0.660031155973186)
--(axis cs:17.3469387755102,0.661195895669925)
--(axis cs:17.687074829932,0.677056026456847)
--(axis cs:18.0272108843537,0.687916289800253)
--(axis cs:18.3673469387755,0.699740995108922)
--(axis cs:18.7074829931973,0.69676422762604)
--(axis cs:19.047619047619,0.706157572337317)
--(axis cs:19.3877551020408,0.702792578781436)
--(axis cs:19.7278911564626,0.706591635631684)
--(axis cs:20.0680272108844,0.709684821092686)
--(axis cs:20.4081632653061,0.709653161780582)
--(axis cs:20.7482993197279,0.70719380848222)
--(axis cs:21.0884353741497,0.710787688157251)
--(axis cs:21.4285714285714,0.711061713349656)
--(axis cs:21.7687074829932,0.711948874086052)
--(axis cs:22.108843537415,0.71845391605649)
--(axis cs:22.4489795918367,0.719761141950779)
--(axis cs:22.7891156462585,0.725149004175274)
--(axis cs:23.1292517006803,0.729411659115321)
--(axis cs:23.469387755102,0.741464639388743)
--(axis cs:23.8095238095238,0.747626340599568)
--(axis cs:24.1496598639456,0.759290723491663)
--(axis cs:24.4897959183673,0.759735052186789)
--(axis cs:24.8299319727891,0.764671810349676)
--(axis cs:25.1700680272109,0.770754140940687)
--(axis cs:25.5102040816327,0.770521301845318)
--(axis cs:25.8503401360544,0.777207544446279)
--(axis cs:26.1904761904762,0.781763316867883)
--(axis cs:26.530612244898,0.780320233671671)
--(axis cs:26.8707482993197,0.784997277197179)
--(axis cs:27.2108843537415,0.787935598888883)
--(axis cs:27.5510204081633,0.794306752105319)
--(axis cs:27.891156462585,0.799387024424818)
--(axis cs:28.2312925170068,0.798946553959882)
--(axis cs:28.5714285714286,0.798940656211896)
--(axis cs:28.9115646258503,0.798826339141813)
--(axis cs:29.2517006802721,0.797796488526176)
--(axis cs:29.5918367346939,0.802788109732905)
--(axis cs:29.9319727891156,0.806546488526176)
--(axis cs:30.2721088435374,0.805945760266344)
--(axis cs:30.6122448979592,0.807546022777452)
--(axis cs:30.952380952381,0.808499879444785)
--(axis cs:31.2925170068027,0.809070127849249)
--(axis cs:31.6326530612245,0.808452000563411)
--(axis cs:31.9727891156463,0.809841164318306)
--(axis cs:32.312925170068,0.81073861678018)
--(axis cs:32.6530612244898,0.818216999601703)
--(axis cs:32.9931972789116,0.81877270748295)
--(axis cs:33.3333333333333,0.821303739129296)
--(axis cs:33.6734693877551,0.827050797553225)
--(axis cs:34.0136054421769,0.831480188165368)
--(axis cs:34.3537414965986,0.843997820089367)
--(axis cs:34.6938775510204,0.844249292428614)
--(axis cs:35.0340136054422,0.84872581428929)
--(axis cs:35.3741496598639,0.852809884520309)
--(axis cs:35.7142857142857,0.854930468634165)
--(axis cs:36.0544217687075,0.854535174392655)
--(axis cs:36.3945578231292,0.855011458026401)
--(axis cs:36.734693877551,0.851229379635616)
--(axis cs:37.0748299319728,0.8495540369369)
--(axis cs:37.4149659863946,0.849525712751725)
--(axis cs:37.7551020408163,0.845701757204821)
--(axis cs:38.0952380952381,0.853053217482803)
--(axis cs:38.4353741496599,0.853232206645038)
--(axis cs:38.7755102040816,0.858737799773117)
--(axis cs:39.1156462585034,0.860754186839463)
--(axis cs:39.4557823129252,0.863081490002445)
--(axis cs:39.7959183673469,0.862337212472768)
--(axis cs:40.1360544217687,0.865294773230725)
--(axis cs:40.4761904761905,0.873282661974455)
--(axis cs:40.8163265306122,0.875144459773643)
--(axis cs:41.156462585034,0.883438856402222)
--(axis cs:41.4965986394558,0.884636420290765)
--(axis cs:41.8367346938776,0.896325552274617)
--(axis cs:42.1768707482993,0.898029870354082)
--(axis cs:42.5170068027211,0.910148928068639)
--(axis cs:42.8571428571429,0.904855083733285)
--(axis cs:43.1972789115646,0.908099689863913)
--(axis cs:43.5374149659864,0.910716200856066)
--(axis cs:43.8775510204082,0.913328871662829)
--(axis cs:44.2176870748299,0.909624179903243)
--(axis cs:44.5578231292517,0.912491610481377)
--(axis cs:44.8979591836735,0.919067354645953)
--(axis cs:45.2380952380952,0.921485558313222)
--(axis cs:45.578231292517,0.923213673847733)
--(axis cs:45.9183673469388,0.924895888901448)
--(axis cs:46.2585034013605,0.928401546708442)
--(axis cs:46.5986394557823,0.930343063566141)
--(axis cs:46.9387755102041,0.930967064804998)
--(axis cs:47.2789115646259,0.932306819378425)
--(axis cs:47.6190476190476,0.934638827004039)
--(axis cs:47.9591836734694,0.934798086226348)
--(axis cs:48.2993197278912,0.936684511506564)
--(axis cs:48.6394557823129,0.935542954947009)
--(axis cs:48.9795918367347,0.938833852089565)
--(axis cs:49.3197278911565,0.938639586137526)
--(axis cs:49.6598639455782,0.938098395922137)
--(axis cs:50,0.937497291207215)
--(axis cs:50.3401360544218,0.93942594411009)
--(axis cs:50.6802721088435,0.938858315764899)
--(axis cs:51.0204081632653,0.941115640965359)
--(axis cs:51.3605442176871,0.942453361060435)
--(axis cs:51.7006802721088,0.941705467224287)
--(axis cs:52.0408163265306,0.944001742153411)
--(axis cs:52.3809523809524,0.943894291749779)
--(axis cs:52.7210884353741,0.944839744025678)
--(axis cs:53.0612244897959,0.945480967646068)
--(axis cs:53.4013605442177,0.948382919958194)
--(axis cs:53.7414965986395,0.946687199352037)
--(axis cs:54.0816326530612,0.949114965692101)
--(axis cs:54.421768707483,0.951527930147655)
--(axis cs:54.7619047619048,0.94994715740967)
--(axis cs:55.1020408163265,0.95267578125)
--(axis cs:55.4421768707483,0.957381237604018)
--(axis cs:55.7823129251701,0.955417073582292)
--(axis cs:56.1224489795918,0.957203435549192)
--(axis cs:56.4625850340136,0.960001337096781)
--(axis cs:56.8027210884354,0.959444178684975)
--(axis cs:57.1428571428571,0.960443026654242)
--(axis cs:57.4829931972789,0.960843370360707)
--(axis cs:57.8231292517007,0.962428945596591)
--(axis cs:58.1632653061224,0.964996657112303)
--(axis cs:58.5034013605442,0.963928688554522)
--(axis cs:58.843537414966,0.968256193795427)
--(axis cs:59.1836734693878,0.967639290229284)
--(axis cs:59.5238095238095,0.971240283366567)
--(axis cs:59.8639455782313,0.978818249062498)
--(axis cs:60.2040816326531,0.976011556998262)
--(axis cs:60.5442176870748,0.9764692754297)
--(axis cs:60.8843537414966,0.975322090230316)
--(axis cs:61.2244897959184,0.980909518959085)
--(axis cs:61.5646258503401,0.975871713314739)
--(axis cs:61.9047619047619,0.981698375718091)
--(axis cs:62.2448979591837,0.977859894607153)
--(axis cs:62.5850340136054,0.978917736299425)
--(axis cs:62.9251700680272,0.982292787043888)
--(axis cs:63.265306122449,0.981078240864157)
--(axis cs:63.6054421768707,0.9855487800887)
--(axis cs:63.9455782312925,0.981717888373788)
--(axis cs:64.2857142857143,0.97799476395209)
--(axis cs:64.6258503401361,0.974765604133304)
--(axis cs:64.9659863945578,0.966867881934004)
--(axis cs:65.3061224489796,0.965015359462891)
--(axis cs:65.6462585034014,0.965654955334628)
--(axis cs:65.9863945578231,0.968646847623066)
--(axis cs:66.3265306122449,0.968044207540986)
--(axis cs:66.6666666666667,0.964396677800454)
--(axis cs:67.0068027210884,0.965175159639152)
--(axis cs:67.3469387755102,0.970596807341322)
--(axis cs:67.687074829932,0.971503432201705)
--(axis cs:68.0272108843537,0.973654473186233)
--(axis cs:68.3673469387755,0.973895249050186)
--(axis cs:68.7074829931973,0.979444778188745)
--(axis cs:69.0476190476191,0.979030325739435)
--(axis cs:69.3877551020408,0.976924630299211)
--(axis cs:69.7278911564626,0.98064629631417)
--(axis cs:70.0680272108844,0.979962666525794)
--(axis cs:70.4081632653061,0.977373165968831)
--(axis cs:70.7482993197279,0.980931035715749)
--(axis cs:71.0884353741497,0.983052806603938)
--(axis cs:71.4285714285714,0.982983540177365)
--(axis cs:71.7687074829932,0.978388491032093)
--(axis cs:72.108843537415,0.97693750590663)
--(axis cs:72.4489795918367,0.974351687807601)
--(axis cs:72.7891156462585,0.976331044089482)
--(axis cs:73.1292517006803,0.978349329748445)
--(axis cs:73.469387755102,0.975591118322735)
--(axis cs:73.8095238095238,0.980678635906556)
--(axis cs:74.1496598639456,0.980457743836896)
--(axis cs:74.4897959183673,0.980939026065216)
--(axis cs:74.8299319727891,0.984550352679317)
--(axis cs:75.1700680272109,0.985691110219481)
--(axis cs:75.5102040816327,0.987186529774754)
--(axis cs:75.8503401360544,0.985812150910834)
--(axis cs:76.1904761904762,0.981705943114232)
--(axis cs:76.530612244898,0.973656850451038)
--(axis cs:76.8707482993197,0.969741157476214)
--(axis cs:77.2108843537415,0.970310835566013)
--(axis cs:77.5510204081633,0.970594235733534)
--(axis cs:77.891156462585,0.966506861827159)
--(axis cs:78.2312925170068,0.966084629107953)
--(axis cs:78.5714285714286,0.964457762777058)
--(axis cs:78.9115646258503,0.966383569094539)
--(axis cs:79.2517006802721,0.96706902073059)
--(axis cs:79.5918367346939,0.962558302243444)
--(axis cs:79.9319727891156,0.96665089065106)
--(axis cs:80.2721088435374,0.964890087656818)
--(axis cs:80.6122448979592,0.964084436686571)
--(axis cs:80.9523809523809,0.967318557440355)
--(axis cs:81.2925170068027,0.961489597953833)
--(axis cs:81.6326530612245,0.966349456207901)
--(axis cs:81.9727891156463,0.97350959497157)
--(axis cs:82.312925170068,0.966755357267752)
--(axis cs:82.6530612244898,0.97021314418369)
--(axis cs:82.9931972789116,0.968788748408335)
--(axis cs:83.3333333333333,0.968125968195577)
--(axis cs:83.6734693877551,0.967618885116742)
--(axis cs:84.0136054421769,0.963204029263302)
--(axis cs:84.3537414965986,0.965356344386257)
--(axis cs:84.6938775510204,0.967715837906041)
--(axis cs:85.0340136054422,0.980437683837127)
--(axis cs:85.3741496598639,0.979379630753746)
--(axis cs:85.7142857142857,0.97753391368559)
--(axis cs:86.0544217687075,0.980058388879253)
--(axis cs:86.3945578231292,0.980581376873445)
--(axis cs:86.734693877551,0.979324829067328)
--(axis cs:87.0748299319728,0.982396559978543)
--(axis cs:87.4149659863945,0.980413210296567)
--(axis cs:87.7551020408163,0.976579008559947)
--(axis cs:88.0952380952381,0.97776422973642)
--(axis cs:88.4353741496599,0.977599316891132)
--(axis cs:88.7755102040816,0.974897363879519)
--(axis cs:89.1156462585034,0.975674215674214)
--(axis cs:89.4557823129252,0.976402375298462)
--(axis cs:89.7959183673469,0.978124476904062)
--(axis cs:90.1360544217687,0.975348993487923)
--(axis cs:90.4761904761905,0.977301201258402)
--(axis cs:90.8163265306122,0.976714875298462)
--(axis cs:91.156462585034,0.973101600267779)
--(axis cs:91.4965986394558,0.971716752872561)
--(axis cs:91.8367346938775,0.973289721891323)
--(axis cs:92.1768707482993,0.975062626786579)
--(axis cs:92.5170068027211,0.982134434555598)
--(axis cs:92.8571428571429,0.989106544425932)
--(axis cs:93.1972789115646,0.994398674994465)
--(axis cs:93.5374149659864,0.99442693433032)
--(axis cs:93.8775510204082,0.992842071198967)
--(axis cs:94.2176870748299,0.993850495551738)
--(axis cs:94.5578231292517,0.9956711166464)
--(axis cs:94.8979591836735,0.995724231760776)
--(axis cs:95.2380952380952,0.995353386714251)
--(axis cs:95.578231292517,0.99677344062001)
--(axis cs:95.9183673469388,0.994702444882459)
--(axis cs:96.2585034013605,0.995344569382888)
--(axis cs:96.5986394557823,0.992422744057032)
--(axis cs:96.9387755102041,0.994135197963596)
--(axis cs:97.2789115646258,0.99677344062001)
--(axis cs:97.6190476190476,0.998743219954142)
--(axis cs:97.9591836734694,0.994192848646644)
--(axis cs:98.2993197278912,0.993574499112499)
--(axis cs:98.6394557823129,0.995702248723764)
--(axis cs:98.9795918367347,0.994750736819819)
--(axis cs:99.3197278911565,0.996402375298462)
--(axis cs:99.6598639455782,0.990362424380739)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,1.00088757561926)
--(axis cs:99.3197278911565,1.00172262470154)
--(axis cs:98.9795918367347,1.00181176318018)
--(axis cs:98.6394557823129,1.00179775127624)
--(axis cs:98.2993197278912,1.0017380008875)
--(axis cs:97.9591836734694,1.00174465135336)
--(axis cs:97.6190476190476,1.00094428004586)
--(axis cs:97.2789115646258,1.00166405937999)
--(axis cs:96.9387755102041,1.0018023020364)
--(axis cs:96.5986394557823,1.00163975594297)
--(axis cs:96.2585034013605,1.00184293061711)
--(axis cs:95.9183673469388,1.00186005511754)
--(axis cs:95.578231292517,1.00166405937999)
--(axis cs:95.2380952380952,1.00183411328575)
--(axis cs:94.8979591836735,1.00177576823922)
--(axis cs:94.5578231292517,1.0018288833536)
--(axis cs:94.2176870748299,1.00177450444826)
--(axis cs:93.8775510204082,1.00153292880103)
--(axis cs:93.5374149659864,1.00182306566968)
--(axis cs:93.1972789115646,1.00185132500553)
--(axis cs:92.8571428571429,1.00089345557407)
--(axis cs:92.5170068027211,0.997240565444402)
--(axis cs:92.1768707482993,0.989624873213421)
--(axis cs:91.8367346938775,0.987960278108677)
--(axis cs:91.4965986394558,0.982033247127439)
--(axis cs:91.156462585034,0.981585899732221)
--(axis cs:90.8163265306122,0.982035124701538)
--(axis cs:90.4761904761905,0.985511298741598)
--(axis cs:90.1360544217687,0.982776006512076)
--(axis cs:89.7959183673469,0.982500523095938)
--(axis cs:89.4557823129252,0.981722624701538)
--(axis cs:89.1156462585034,0.981825784325786)
--(axis cs:88.7755102040816,0.984477636120481)
--(axis cs:88.4353741496599,0.991150683108868)
--(axis cs:88.0952380952381,0.991610770263581)
--(axis cs:87.7551020408163,0.992483491440053)
--(axis cs:87.4149659863945,0.994899289703433)
--(axis cs:87.0748299319728,0.996978440021457)
--(axis cs:86.734693877551,0.996300170932672)
--(axis cs:86.3945578231292,0.997231123126555)
--(axis cs:86.0544217687075,0.996816611120747)
--(axis cs:85.7142857142857,0.99465358631441)
--(axis cs:85.3741496598639,0.995932869246254)
--(axis cs:85.0340136054422,0.996124816162873)
--(axis cs:84.6938775510204,0.987284162093959)
--(axis cs:84.3537414965986,0.984018655613743)
--(axis cs:84.0136054421769,0.984295970736698)
--(axis cs:83.6734693877551,0.985818614883258)
--(axis cs:83.3333333333333,0.986249031804423)
--(axis cs:82.9931972789116,0.982148751591665)
--(axis cs:82.6530612244898,0.98166185581631)
--(axis cs:82.312925170068,0.980119642732248)
--(axis cs:81.9727891156463,0.98180290502843)
--(axis cs:81.6326530612245,0.979275543792099)
--(axis cs:81.2925170068027,0.977260402046166)
--(axis cs:80.9523809523809,0.981743942559645)
--(axis cs:80.6122448979592,0.982478063313429)
--(axis cs:80.2721088435374,0.983234912343182)
--(axis cs:79.9319727891156,0.98209910934894)
--(axis cs:79.5918367346939,0.980879197756556)
--(axis cs:79.2517006802721,0.984493479269411)
--(axis cs:78.9115646258503,0.984553930905461)
--(axis cs:78.5714285714286,0.983042237222942)
--(axis cs:78.2312925170068,0.985165370892047)
--(axis cs:77.891156462585,0.985993138172841)
--(axis cs:77.5510204081633,0.988468264266466)
--(axis cs:77.2108843537415,0.987501664433987)
--(axis cs:76.8707482993197,0.987133842523786)
--(axis cs:76.530612244898,0.991343149548962)
--(axis cs:76.1904761904762,0.997356556885768)
--(axis cs:75.8503401360544,0.999187849089166)
--(axis cs:75.5102040816327,0.999375970225246)
--(axis cs:75.1700680272109,0.998371389780519)
--(axis cs:74.8299319727891,0.997012147320683)
--(axis cs:74.4897959183673,0.993435973934784)
--(axis cs:74.1496598639456,0.993604756163104)
--(axis cs:73.8095238095238,0.993071364093443)
--(axis cs:73.469387755102,0.988471381677265)
--(axis cs:73.1292517006803,0.991650670251555)
--(axis cs:72.7891156462585,0.989918955910518)
--(axis cs:72.4489795918367,0.989085812192399)
--(axis cs:72.108843537415,0.99243749409337)
--(axis cs:71.7687074829932,0.994736508967907)
--(axis cs:71.4285714285714,0.997953959822635)
--(axis cs:71.0884353741497,0.997259693396062)
--(axis cs:70.7482993197279,0.995631464284251)
--(axis cs:70.4081632653061,0.994189334031169)
--(axis cs:70.0680272108844,0.996287333474206)
--(axis cs:69.7278911564626,0.99685370368583)
--(axis cs:69.3877551020408,0.99463786970079)
--(axis cs:69.0476190476191,0.995969674260565)
--(axis cs:68.7074829931973,0.996180221811255)
--(axis cs:68.3673469387755,0.991729750949814)
--(axis cs:68.0272108843537,0.992283026813767)
--(axis cs:67.687074829932,0.991621567798295)
--(axis cs:67.3469387755102,0.990028192658678)
--(axis cs:67.0068027210884,0.984199840360848)
--(axis cs:66.6666666666667,0.982165822199546)
--(axis cs:66.3265306122449,0.983205792459014)
--(axis cs:65.9863945578231,0.982603152376934)
--(axis cs:65.6462585034014,0.980282544665372)
--(axis cs:65.3061224489796,0.982484640537109)
--(axis cs:64.9659863945578,0.985632118065996)
--(axis cs:64.6258503401361,0.993046895866696)
--(axis cs:64.2857142857143,0.99481773604791)
--(axis cs:63.9455782312925,0.997657111626212)
--(axis cs:63.6054421768707,0.9997637199113)
--(axis cs:63.265306122449,0.997671759135843)
--(axis cs:62.9251700680272,0.998332212956113)
--(axis cs:62.5850340136054,0.996707263700575)
--(axis cs:62.2448979591837,0.995890105392847)
--(axis cs:61.9047619047619,0.997989124281909)
--(axis cs:61.5646258503401,0.994440786685261)
--(axis cs:61.2244897959184,0.997215481040915)
--(axis cs:60.8843537414966,0.992177909769684)
--(axis cs:60.5442176870748,0.992905724570301)
--(axis cs:60.2040816326531,0.992425943001738)
--(axis cs:59.8639455782313,0.995244250937502)
--(axis cs:59.5238095238095,0.988759716633433)
--(axis cs:59.1836734693878,0.984548209770716)
--(axis cs:58.843537414966,0.984556306204573)
--(axis cs:58.5034013605442,0.978883811445478)
--(axis cs:58.1632653061224,0.979378342887697)
--(axis cs:57.8231292517007,0.977258554403409)
--(axis cs:57.4829931972789,0.974469129639293)
--(axis cs:57.1428571428571,0.974556973345758)
--(axis cs:56.8027210884354,0.973993321315025)
--(axis cs:56.4625850340136,0.973123662903219)
--(axis cs:56.1224489795918,0.972484064450808)
--(axis cs:55.7823129251701,0.966770426417708)
--(axis cs:55.4421768707483,0.969493762395982)
--(axis cs:55.1020408163265,0.96576171875)
--(axis cs:54.7619047619048,0.96161534259033)
--(axis cs:54.421768707483,0.962222069852345)
--(axis cs:54.0816326530612,0.961197534307899)
--(axis cs:53.7414965986395,0.960187800647963)
--(axis cs:53.4013605442177,0.961304580041806)
--(axis cs:53.0612244897959,0.959519032353932)
--(axis cs:52.7210884353741,0.959222755974322)
--(axis cs:52.3809523809524,0.958293208250221)
--(axis cs:52.0408163265306,0.958810757846589)
--(axis cs:51.7006802721088,0.956107032775713)
--(axis cs:51.3605442176871,0.956609138939565)
--(axis cs:51.0204081632653,0.953884359034641)
--(axis cs:50.6802721088435,0.951766684235101)
--(axis cs:50.3401360544218,0.95244905588991)
--(axis cs:50,0.950315208792785)
--(axis cs:49.6598639455782,0.951589104077863)
--(axis cs:49.3197278911565,0.951360413862474)
--(axis cs:48.9795918367347,0.952416147910435)
--(axis cs:48.6394557823129,0.951019545052991)
--(axis cs:48.2993197278912,0.949252988493436)
--(axis cs:47.9591836734694,0.948326913773652)
--(axis cs:47.6190476190476,0.947548672995961)
--(axis cs:47.2789115646259,0.947693180621575)
--(axis cs:46.9387755102041,0.948407935195002)
--(axis cs:46.5986394557823,0.950594436433859)
--(axis cs:46.2585034013605,0.950973453291558)
--(axis cs:45.9183673469388,0.948541611098553)
--(axis cs:45.578231292517,0.948661326152267)
--(axis cs:45.2380952380952,0.946951941686778)
--(axis cs:44.8979591836735,0.945307645354047)
--(axis cs:44.5578231292517,0.937508389518623)
--(axis cs:44.2176870748299,0.935375820096757)
--(axis cs:43.8775510204082,0.938546128337171)
--(axis cs:43.5374149659864,0.934596299143934)
--(axis cs:43.1972789115646,0.931275310136087)
--(axis cs:42.8571428571429,0.930457416266715)
--(axis cs:42.5170068027211,0.933601071931361)
--(axis cs:42.1768707482993,0.923845129645918)
--(axis cs:41.8367346938776,0.922424447725383)
--(axis cs:41.4965986394558,0.912551079709235)
--(axis cs:41.156462585034,0.911561143597778)
--(axis cs:40.8163265306122,0.902043040226357)
--(axis cs:40.4761904761905,0.899217338025545)
--(axis cs:40.1360544217687,0.889392726769275)
--(axis cs:39.7959183673469,0.884225287527232)
--(axis cs:39.4557823129252,0.885043509997555)
--(axis cs:39.1156462585034,0.882995813160536)
--(axis cs:38.7755102040816,0.880637200226883)
--(axis cs:38.4353741496599,0.875830293354962)
--(axis cs:38.0952380952381,0.874759282517197)
--(axis cs:37.7551020408163,0.867735742795179)
--(axis cs:37.4149659863946,0.870474287248275)
--(axis cs:37.0748299319728,0.8716959630631)
--(axis cs:36.734693877551,0.871895620364384)
--(axis cs:36.3945578231292,0.874676041973599)
--(axis cs:36.0544217687075,0.876402325607345)
--(axis cs:35.7142857142857,0.876007031365835)
--(axis cs:35.3741496598639,0.874690115479691)
--(axis cs:35.0340136054422,0.86971168571071)
--(axis cs:34.6938775510204,0.866375707571386)
--(axis cs:34.3537414965986,0.865377179910633)
--(axis cs:34.0136054421769,0.855082311834632)
--(axis cs:33.6734693877551,0.850449202446775)
--(axis cs:33.3333333333333,0.842446260870704)
--(axis cs:32.9931972789116,0.84278979251705)
--(axis cs:32.6530612244898,0.842095500398297)
--(axis cs:32.312925170068,0.83488638321982)
--(axis cs:31.9727891156463,0.833596335681694)
--(axis cs:31.6326530612245,0.832797999436589)
--(axis cs:31.2925170068027,0.833117372150751)
--(axis cs:30.952380952381,0.833687620555215)
--(axis cs:30.6122448979592,0.833078977222548)
--(axis cs:30.2721088435374,0.832491739733656)
--(axis cs:29.9319727891156,0.831578511473824)
--(axis cs:29.5918367346939,0.827836890267095)
--(axis cs:29.2517006802721,0.822828511473824)
--(axis cs:28.9115646258503,0.822111160858186)
--(axis cs:28.5714285714286,0.822621843788104)
--(axis cs:28.2312925170068,0.821990946040118)
--(axis cs:27.891156462585,0.821550475575181)
--(axis cs:27.5510204081633,0.815693247894681)
--(axis cs:27.2108843537415,0.812064401111117)
--(axis cs:26.8707482993197,0.809377722802821)
--(axis cs:26.530612244898,0.803742266328329)
--(axis cs:26.1904761904762,0.805736683132116)
--(axis cs:25.8503401360544,0.802479955553721)
--(axis cs:25.5102040816327,0.796666198154682)
--(axis cs:25.1700680272109,0.797995859059313)
--(axis cs:24.8299319727891,0.791578189650324)
--(axis cs:24.4897959183673,0.787764947813211)
--(axis cs:24.1496598639456,0.786334276508337)
--(axis cs:23.8095238095238,0.774873659400432)
--(axis cs:23.469387755102,0.767597860611257)
--(axis cs:23.1292517006803,0.754650840884679)
--(axis cs:22.7891156462585,0.750163495824726)
--(axis cs:22.4489795918367,0.743676358049221)
--(axis cs:22.108843537415,0.74123358394351)
--(axis cs:21.7687074829932,0.734926125913947)
--(axis cs:21.4285714285714,0.735813286650344)
--(axis cs:21.0884353741497,0.734837311842749)
--(axis cs:20.7482993197279,0.73343119151778)
--(axis cs:20.4081632653061,0.735971838219418)
--(axis cs:20.0680272108844,0.733752678907314)
--(axis cs:19.7278911564626,0.729658364368316)
--(axis cs:19.3877551020408,0.726269921218564)
--(axis cs:19.047619047619,0.728842427662683)
--(axis cs:18.7074829931973,0.72167327237396)
--(axis cs:18.3673469387755,0.725259004891078)
--(axis cs:18.0272108843537,0.716146210199747)
--(axis cs:17.687074829932,0.706068973543153)
--(axis cs:17.3469387755102,0.689741604330075)
--(axis cs:17.0068027210884,0.687781344026814)
--(axis cs:16.6666666666667,0.687773998439223)
--(axis cs:16.3265306122449,0.680638631354222)
--(axis cs:15.9863945578231,0.671835286443865)
--(axis cs:15.6462585034014,0.669860355321896)
--(axis cs:15.3061224489796,0.656696074743964)
--(axis cs:14.9659863945578,0.651045112404135)
--(axis cs:14.6258503401361,0.646987439895345)
--(axis cs:14.2857142857143,0.639267638328278)
--(axis cs:13.9455782312925,0.634419744176155)
--(axis cs:13.6054421768707,0.636251830947412)
--(axis cs:13.265306122449,0.635530267327771)
--(axis cs:12.9251700680272,0.633797676992926)
--(axis cs:12.5850340136054,0.625398600641505)
--(axis cs:12.2448979591837,0.626524071913801)
--(axis cs:11.9047619047619,0.624247561300643)
--(axis cs:11.5646258503401,0.624948319852621)
--(axis cs:11.2244897959184,0.620735451250974)
--(axis cs:10.8843537414966,0.612141706709953)
--(axis cs:10.5442176870748,0.602217816931498)
--(axis cs:10.2040816326531,0.591444125027675)
--(axis cs:9.86394557823129,0.582029657707983)
--(axis cs:9.52380952380952,0.570568604197315)
--(axis cs:9.18367346938775,0.555988634261428)
--(axis cs:8.84353741496599,0.546823048143978)
--(axis cs:8.50340136054422,0.543628785010052)
--(axis cs:8.16326530612245,0.530255852990869)
--(axis cs:7.82312925170068,0.517744860596527)
--(axis cs:7.48299319727891,0.505268660430472)
--(axis cs:7.14285714285714,0.485911867990526)
--(axis cs:6.80272108843537,0.453458024505659)
--(axis cs:6.46258503401361,0.419289079991937)
--(axis cs:6.12244897959184,0.415322669768063)
--(axis cs:5.78231292517007,0.404849517690414)
--(axis cs:5.4421768707483,0.383259398879614)
--(axis cs:5.10204081632653,0.363541433839546)
--(axis cs:4.76190476190476,0.341232621020971)
--(axis cs:4.42176870748299,0.309308438256466)
--(axis cs:4.08163265306122,0.295457769949366)
--(axis cs:3.74149659863946,0.275504166465028)
--(axis cs:3.40136054421769,0.241880772298071)
--(axis cs:3.06122448979592,0.222527236241896)
--(axis cs:2.72108843537415,0.195523011755193)
--(axis cs:2.38095238095238,0.183480366807789)
--(axis cs:2.04081632653061,0.170121513436302)
--(axis cs:1.70068027210884,0.122242292315188)
--(axis cs:1.36054421768707,0.0873680895730504)
--(axis cs:1.02040816326531,0.057572613253529)
--(axis cs:0.680272108843537,0.055754697259619)
--(axis cs:0.340136054421769,0.0681649845294774)
--(axis cs:0,0.0827971130190766)
--cycle;


==> img/stl10/stl10_rate_accuracy_pgd_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color9, mark=square*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color9, thin}]
table {%
0 0.0778125
0.340136054421769 0.0775
0.680272108843537 0.08234375
1.02040816326531 0.0903125
1.36054421768707 0.1065625
1.70068027210884 0.1178125
2.04081632653061 0.12703125
2.38095238095238 0.14046875
2.72108843537415 0.16140625
3.06122448979592 0.1803125
3.40136054421769 0.20453125
3.74149659863946 0.216875
4.08163265306122 0.23921875
4.42176870748299 0.2540625
4.76190476190476 0.26796875
5.10204081632653 0.28203125
5.4421768707483 0.29796875
5.78231292517007 0.31484375
6.12244897959184 0.32421875
6.46258503401361 0.34125
6.80272108843537 0.34609375
7.14285714285714 0.35328125
7.48299319727891 0.3671875
7.82312925170068 0.38484375
8.16326530612245 0.3928125
8.50340136054422 0.4
8.84353741496599 0.4190625
9.18367346938775 0.42859375
9.52380952380952 0.43625
9.86394557823129 0.44859375
10.2040816326531 0.4625
10.5442176870748 0.475
10.8843537414966 0.49046875
11.2244897959184 0.50265625
11.5646258503401 0.51796875
11.9047619047619 0.5325
12.2448979591837 0.54921875
12.5850340136054 0.5571875
12.9251700680272 0.555625
13.265306122449 0.5771875
13.6054421768707 0.580625
13.9455782312925 0.59203125
14.2857142857143 0.59390625
14.6258503401361 0.60578125
14.9659863945578 0.61328125
15.3061224489796 0.62265625
15.6462585034014 0.62609375
15.9863945578231 0.63421875
16.3265306122449 0.64125
16.6666666666667 0.64578125
17.0068027210884 0.6496875
17.3469387755102 0.64734375
17.687074829932 0.65671875
18.0272108843537 0.65890625
18.3673469387755 0.6715625
18.7074829931973 0.6759375
19.047619047619 0.67765625
19.3877551020408 0.68671875
19.7278911564626 0.694375
20.0680272108844 0.69671875
20.4081632653061 0.70609375
20.7482993197279 0.71046875
21.0884353741497 0.72265625
21.4285714285714 0.7184375
21.7687074829932 0.72625
22.108843537415 0.73171875
22.4489795918367 0.73203125
22.7891156462585 0.744375
23.1292517006803 0.7425
23.469387755102 0.7428125
23.8095238095238 0.753125
24.1496598639456 0.75296875
24.4897959183673 0.75234375
24.8299319727891 0.7575
25.1700680272109 0.76359375
25.5102040816327 0.76984375
25.8503401360544 0.77140625
26.1904761904762 0.77734375
26.530612244898 0.7765625
26.8707482993197 0.78578125
27.2108843537415 0.79125
27.5510204081633 0.79546875
27.891156462585 0.7965625
28.2312925170068 0.80125
28.5714285714286 0.80015625
28.9115646258503 0.81
29.2517006802721 0.80671875
29.5918367346939 0.8165625
29.9319727891156 0.82015625
30.2721088435374 0.8203125
30.6122448979592 0.82328125
30.952380952381 0.829375
31.2925170068027 0.8325
31.6326530612245 0.835625
31.9727891156463 0.8375
32.312925170068 0.8403125
32.6530612244898 0.8428125
32.9931972789116 0.84609375
33.3333333333333 0.84765625
33.6734693877551 0.85078125
34.0136054421769 0.854375
34.3537414965986 0.85421875
34.6938775510204 0.854375
35.0340136054422 0.8565625
35.3741496598639 0.85921875
35.7142857142857 0.859375
36.0544217687075 0.86046875
36.3945578231292 0.86421875
36.734693877551 0.86515625
37.0748299319728 0.8665625
37.4149659863946 0.86578125
37.7551020408163 0.87171875
38.0952380952381 0.869375
38.4353741496599 0.870625
38.7755102040816 0.87328125
39.1156462585034 0.873125
39.4557823129252 0.875625
39.7959183673469 0.87671875
40.1360544217687 0.87984375
40.4761904761905 0.88078125
40.8163265306122 0.88140625
41.156462585034 0.8828125
41.4965986394558 0.8834375
41.8367346938776 0.8803125
42.1768707482993 0.8853125
42.5170068027211 0.88296875
42.8571428571429 0.88625
43.1972789115646 0.8846875
43.5374149659864 0.890625
43.8775510204082 0.89
44.2176870748299 0.8884375
44.5578231292517 0.89328125
44.8979591836735 0.89359375
45.2380952380952 0.89296875
45.578231292517 0.89625
45.9183673469388 0.8925
46.2585034013605 0.89796875
46.5986394557823 0.8928125
46.9387755102041 0.8959375
47.2789115646259 0.894375
47.6190476190476 0.89453125
47.9591836734694 0.895625
48.2993197278912 0.89359375
48.6394557823129 0.89484375
48.9795918367347 0.8940625
49.3197278911565 0.89
49.6598639455782 0.8925
50 0.8896875
50.3401360544218 0.88609375
50.6802721088435 0.89078125
51.0204081632653 0.8834375
51.3605442176871 0.880625
51.7006802721088 0.88796875
52.0408163265306 0.88609375
52.3809523809524 0.885
52.7210884353741 0.8871875
53.0612244897959 0.88984375
53.4013605442177 0.8821875
53.7414965986395 0.88625
54.0816326530612 0.88984375
54.421768707483 0.8934375
54.7619047619048 0.88921875
55.1020408163265 0.88984375
55.4421768707483 0.88984375
55.7823129251701 0.88453125
56.1224489795918 0.8884375
56.4625850340136 0.88609375
56.8027210884354 0.884375
57.1428571428571 0.87890625
57.4829931972789 0.88078125
57.8231292517007 0.87875
58.1632653061224 0.88328125
58.5034013605442 0.88265625
58.843537414966 0.88375
59.1836734693878 0.88484375
59.5238095238095 0.88859375
59.8639455782313 0.88875
60.2040816326531 0.8871875
60.5442176870748 0.88890625
60.8843537414966 0.89109375
61.2244897959184 0.89359375
61.5646258503401 0.89203125
61.9047619047619 0.89078125
62.2448979591837 0.8971875
62.5850340136054 0.893125
62.9251700680272 0.89453125
63.265306122449 0.89640625
63.6054421768707 0.8946875
63.9455782312925 0.8940625
64.2857142857143 0.896875
64.6258503401361 0.8971875
64.9659863945578 0.89921875
65.3061224489796 0.9
65.6462585034014 0.900625
65.9863945578231 0.90375
66.3265306122449 0.905625
66.6666666666667 0.904375
67.0068027210884 0.90484375
67.3469387755102 0.9053125
67.687074829932 0.906875
68.0272108843537 0.90828125
68.3673469387755 0.9065625
68.7074829931973 0.90359375
69.0476190476191 0.90359375
69.3877551020408 0.906875
69.7278911564626 0.90578125
70.0680272108844 0.90859375
70.4081632653061 0.9065625
70.7482993197279 0.90890625
71.0884353741497 0.91
71.4285714285714 0.91046875
71.7687074829932 0.9121875
72.108843537415 0.91203125
72.4489795918367 0.913125
72.7891156462585 0.91140625
73.1292517006803 0.913125
73.469387755102 0.9140625
73.8095238095238 0.91359375
74.1496598639456 0.91640625
74.4897959183673 0.915625
74.8299319727891 0.91765625
75.1700680272109 0.9184375
75.5102040816327 0.91953125
75.8503401360544 0.92078125
76.1904761904762 0.92296875
76.530612244898 0.9221875
76.8707482993197 0.923125
77.2108843537415 0.9234375
77.5510204081633 0.92359375
77.891156462585 0.92359375
78.2312925170068 0.92359375
78.5714285714286 0.924375
78.9115646258503 0.92546875
79.2517006802721 0.928125
79.5918367346939 0.92796875
79.9319727891156 0.92984375
80.2721088435374 0.93203125
80.6122448979592 0.933125
80.9523809523809 0.93421875
81.2925170068027 0.936875
81.6326530612245 0.93953125
81.9727891156463 0.94125
82.312925170068 0.9415625
82.6530612244898 0.9428125
82.9931972789116 0.94984375
83.3333333333333 0.9515625
83.6734693877551 0.95734375
84.0136054421769 0.9578125
84.3537414965986 0.95640625
84.6938775510204 0.96578125
85.0340136054422 0.969375
85.3741496598639 0.97515625
85.7142857142857 0.9746875
86.0544217687075 0.9759375
86.3945578231292 0.976875
86.734693877551 0.97640625
87.0748299319728 0.9771875
87.4149659863945 0.97484375
87.7551020408163 0.97609375
88.0952380952381 0.973125
88.4353741496599 0.9740625
88.7755102040816 0.9746875
89.1156462585034 0.97296875
89.4557823129252 0.97609375
89.7959183673469 0.97484375
90.1360544217687 0.97359375
90.4761904761905 0.9728125
90.8163265306122 0.96984375
91.156462585034 0.9728125
91.4965986394558 0.9725
91.8367346938775 0.96828125
92.1768707482993 0.9646875
92.5170068027211 0.9621875
92.8571428571429 0.96125
93.1972789115646 0.96203125
93.5374149659864 0.95546875
93.8775510204082 0.954375
94.2176870748299 0.955625
94.5578231292517 0.9534375
94.8979591836735 0.956875
95.2380952380952 0.956875
95.578231292517 0.95875
95.9183673469388 0.959375
96.2585034013605 0.95921875
96.5986394557823 0.95953125
96.9387755102041 0.9571875
97.2789115646258 0.95234375
97.6190476190476 0.9478125
97.9591836734694 0.9446875
98.2993197278912 0.94546875
98.6394557823129 0.94875
98.9795918367347 0.9503125
99.3197278911565 0.95703125
99.6598639455782 0.95765625
100 0.98
};
\path [fill=color9, fill opacity=0.25]
(axis cs:0,0.0850218862598796)
--(axis cs:0,0.0706031137401204)
--(axis cs:0.340136054421769,0.070917070489706)
--(axis cs:0.680272108843537,0.074604222636299)
--(axis cs:1.02040816326531,0.0801985933770509)
--(axis cs:1.36054421768707,0.0956835762174737)
--(axis cs:1.70068027210884,0.107722194255399)
--(axis cs:2.04081632653061,0.115692606580493)
--(axis cs:2.38095238095238,0.12760886418371)
--(axis cs:2.72108843537415,0.14595401913845)
--(axis cs:3.06122448979592,0.16429806597416)
--(axis cs:3.40136054421769,0.187839457060412)
--(axis cs:3.74149659863946,0.1999019054825)
--(axis cs:4.08163265306122,0.223090087833344)
--(axis cs:4.42176870748299,0.237554260461629)
--(axis cs:4.76190476190476,0.251332469665615)
--(axis cs:5.10204081632653,0.265549895215214)
--(axis cs:5.4421768707483,0.2819504456319)
--(axis cs:5.78231292517007,0.298509446724348)
--(axis cs:6.12244897959184,0.307517818070334)
--(axis cs:6.46258503401361,0.324865853803691)
--(axis cs:6.80272108843537,0.329432265769515)
--(axis cs:7.14285714285714,0.337890240824116)
--(axis cs:7.48299319727891,0.350322630355529)
--(axis cs:7.82312925170068,0.367167429220941)
--(axis cs:8.16326530612245,0.374624826333787)
--(axis cs:8.50340136054422,0.381130345981618)
--(axis cs:8.84353741496599,0.3990484477772)
--(axis cs:9.18367346938775,0.408361458314898)
--(axis cs:9.52380952380952,0.415414174546842)
--(axis cs:9.86394557823129,0.42774625623658)
--(axis cs:10.2040816326531,0.442220391714655)
--(axis cs:10.5442176870748,0.454206326405075)
--(axis cs:10.8843537414966,0.470555733050814)
--(axis cs:11.2244897959184,0.48283203125)
--(axis cs:11.5646258503401,0.498334500105469)
--(axis cs:11.9047619047619,0.512671211656584)
--(axis cs:12.2448979591837,0.529425343372467)
--(axis cs:12.5850340136054,0.537112548128901)
--(axis cs:12.9251700680272,0.536179386961192)
--(axis cs:13.265306122449,0.557282386800268)
--(axis cs:13.6054421768707,0.561341413988754)
--(axis cs:13.9455782312925,0.573081155967442)
--(axis cs:14.2857142857143,0.57469028896316)
--(axis cs:14.6258503401361,0.587663186183737)
--(axis cs:14.9659863945578,0.59531701186061)
--(axis cs:15.3061224489796,0.604740386507752)
--(axis cs:15.6462585034014,0.60889543353491)
--(axis cs:15.9863945578231,0.617059293563667)
--(axis cs:16.3265306122449,0.624477556831114)
--(axis cs:16.6666666666667,0.629202968990042)
--(axis cs:17.0068027210884,0.63279268650886)
--(axis cs:17.3469387755102,0.630386114061404)
--(axis cs:17.687074829932,0.639503806090035)
--(axis cs:18.0272108843537,0.642192189526707)
--(axis cs:18.3673469387755,0.654132021988175)
--(axis cs:18.7074829931973,0.658505927761864)
--(axis cs:19.047619047619,0.658967639968822)
--(axis cs:19.3877551020408,0.66885085838114)
--(axis cs:19.7278911564626,0.676187326333787)
--(axis cs:20.0680272108844,0.678499380655494)
--(axis cs:20.4081632653061,0.68841688970835)
--(axis cs:20.7482993197279,0.692719743353473)
--(axis cs:21.0884353741497,0.705573662254663)
--(axis cs:21.4285714285714,0.700812237680642)
--(axis cs:21.7687074829932,0.709071380134925)
--(axis cs:22.108843537415,0.715133567363651)
--(axis cs:22.4489795918367,0.715647976934079)
--(axis cs:22.7891156462585,0.729536390692795)
--(axis cs:23.1292517006803,0.727270633836236)
--(axis cs:23.469387755102,0.72734947233368)
--(axis cs:23.8095238095238,0.738294105072993)
--(axis cs:24.1496598639456,0.737041198245031)
--(axis cs:24.4897959183673,0.736989342562434)
--(axis cs:24.8299319727891,0.742467280152427)
--(axis cs:25.1700680272109,0.748093454179203)
--(axis cs:25.5102040816327,0.754780926339869)
--(axis cs:25.8503401360544,0.755595887098623)
--(axis cs:26.1904761904762,0.762708664939718)
--(axis cs:26.530612244898,0.760852890214916)
--(axis cs:26.8707482993197,0.770500309048211)
--(axis cs:27.2108843537415,0.776390196797376)
--(axis cs:27.5510204081633,0.780481458325279)
--(axis cs:27.891156462585,0.781698846608634)
--(axis cs:28.2312925170068,0.787092201166062)
--(axis cs:28.5714285714286,0.785258949903308)
--(axis cs:28.9115646258503,0.795425970229549)
--(axis cs:29.2517006802721,0.791209842903082)
--(axis cs:29.5918367346939,0.802873894165676)
--(axis cs:29.9319727891156,0.806477052742044)
--(axis cs:30.2721088435374,0.806471470533964)
--(axis cs:30.6122448979592,0.810090424437196)
--(axis cs:30.952380952381,0.816486594651329)
--(axis cs:31.2925170068027,0.819561376058407)
--(axis cs:31.6326530612245,0.823157084633981)
--(axis cs:31.9727891156463,0.824613074631279)
--(axis cs:32.312925170068,0.828248098888883)
--(axis cs:32.6530612244898,0.830922475581856)
--(axis cs:32.9931972789116,0.83447840215579)
--(axis cs:33.3333333333333,0.835645325229493)
--(axis cs:33.6734693877551,0.839862512605322)
--(axis cs:34.0136054421769,0.843800131190327)
--(axis cs:34.3537414965986,0.84274382896035)
--(axis cs:34.6938775510204,0.843740776923562)
--(axis cs:35.0340136054422,0.844970575604903)
--(axis cs:35.3741496598639,0.847480891230565)
--(axis cs:35.7142857142857,0.848015768731566)
--(axis cs:36.0544217687075,0.848930012143827)
--(axis cs:36.3945578231292,0.852199887794864)
--(axis cs:36.734693877551,0.852803216875776)
--(axis cs:37.0748299319728,0.85478368259116)
--(axis cs:37.4149659863946,0.853935824630987)
--(axis cs:37.7551020408163,0.859693541619407)
--(axis cs:38.0952380952381,0.857225526320315)
--(axis cs:38.4353741496599,0.858678961966115)
--(axis cs:38.7755102040816,0.86126794344844)
--(axis cs:39.1156462585034,0.861573458529202)
--(axis cs:39.4557823129252,0.863855092132851)
--(axis cs:39.7959183673469,0.865165970222775)
--(axis cs:40.1360544217687,0.86828519321356)
--(axis cs:40.4761904761905,0.869646296121515)
--(axis cs:40.8163265306122,0.869696862463936)
--(axis cs:41.156462585034,0.871609663750234)
--(axis cs:41.4965986394558,0.872199815497465)
--(axis cs:41.8367346938776,0.869370641214508)
--(axis cs:42.1768707482993,0.874046845202016)
--(axis cs:42.5170068027211,0.872581778573495)
--(axis cs:42.8571428571429,0.875734820484455)
--(axis cs:43.1972789115646,0.874315689025506)
--(axis cs:43.5374149659864,0.879852670130361)
--(axis cs:43.8775510204082,0.879316566928768)
--(axis cs:44.2176870748299,0.877754959632598)
--(axis cs:44.5578231292517,0.882136878944369)
--(axis cs:44.8979591836735,0.882484519905789)
--(axis cs:45.2380952380952,0.881995124531058)
--(axis cs:45.578231292517,0.885221327264151)
--(axis cs:45.9183673469388,0.881879237402873)
--(axis cs:46.2585034013605,0.887387119620457)
--(axis cs:46.5986394557823,0.882041940875811)
--(axis cs:46.9387755102041,0.884639722762516)
--(axis cs:47.2789115646259,0.883287682047277)
--(axis cs:47.6190476190476,0.88330672711747)
--(axis cs:47.9591836734694,0.883749421786281)
--(axis cs:48.2993197278912,0.882186346243069)
--(axis cs:48.6394557823129,0.882435256200034)
--(axis cs:48.9795918367347,0.881171135201153)
--(axis cs:49.3197278911565,0.87723277578484)
--(axis cs:49.6598639455782,0.879078748013586)
--(axis cs:50,0.876093272951977)
--(axis cs:50.3401360544218,0.872749817610475)
--(axis cs:50.6802721088435,0.877331250703379)
--(axis cs:51.0204081632653,0.870385129338591)
--(axis cs:51.3605442176871,0.867017450430976)
--(axis cs:51.7006802721088,0.874607676117707)
--(axis cs:52.0408163265306,0.873014008579769)
--(axis cs:52.3809523809524,0.871560995496652)
--(axis cs:52.7210884353741,0.873735019251779)
--(axis cs:53.0612244897959,0.876105420990984)
--(axis cs:53.4013605442177,0.868891179276755)
--(axis cs:53.7414965986395,0.872149573712672)
--(axis cs:54.0816326530612,0.875988602828302)
--(axis cs:54.421768707483,0.879577191406867)
--(axis cs:54.7619047619048,0.875731930420567)
--(axis cs:55.1020408163265,0.876556397886193)
--(axis cs:55.4421768707483,0.876229544059382)
--(axis cs:55.7823129251701,0.871637296239454)
--(axis cs:56.1224489795918,0.875132575099373)
--(axis cs:56.4625850340136,0.872746959166188)
--(axis cs:56.8027210884354,0.870953748013586)
--(axis cs:57.1428571428571,0.866840663217775)
--(axis cs:57.4829931972789,0.867745329378869)
--(axis cs:57.8231292517007,0.866495794278643)
--(axis cs:58.1632653061224,0.871001000830976)
--(axis cs:58.5034013605442,0.870574076039478)
--(axis cs:58.843537414966,0.871470915774219)
--(axis cs:59.1836734693878,0.873483259463088)
--(axis cs:59.5238095238095,0.876983329481172)
--(axis cs:59.8639455782313,0.876752978376612)
--(axis cs:60.2040816326531,0.875495636311363)
--(axis cs:60.5442176870748,0.877308156952904)
--(axis cs:60.8843537414966,0.879157695118762)
--(axis cs:61.2244897959184,0.88187622076671)
--(axis cs:61.5646258503401,0.880690924538736)
--(axis cs:61.9047619047619,0.879630890336299)
--(axis cs:62.2448979591837,0.88638334633911)
--(axis cs:62.5850340136054,0.882441566928768)
--(axis cs:62.9251700680272,0.884494486675004)
--(axis cs:63.265306122449,0.886560388216352)
--(axis cs:63.6054421768707,0.884819868688227)
--(axis cs:63.9455782312925,0.883781193602928)
--(axis cs:64.2857142857143,0.886824468491978)
--(axis cs:64.6258503401361,0.8876801737876)
--(axis cs:64.9659863945578,0.889422411578939)
--(axis cs:65.3061224489796,0.890737573670797)
--(axis cs:65.6462585034014,0.891698128998417)
--(axis cs:65.9863945578231,0.894372965715502)
--(axis cs:66.3265306122449,0.896555052561718)
--(axis cs:66.6666666666667,0.895762405249864)
--(axis cs:67.0068027210884,0.895873716439572)
--(axis cs:67.3469387755102,0.896812478458207)
--(axis cs:67.687074829932,0.897502034726014)
--(axis cs:68.0272108843537,0.899458074015796)
--(axis cs:68.3673469387755,0.897238501357594)
--(axis cs:68.7074829931973,0.89480089057709)
--(axis cs:69.0476190476191,0.893295297653771)
--(axis cs:69.3877551020408,0.896319990116415)
--(axis cs:69.7278911564626,0.89526471014729)
--(axis cs:70.0680272108844,0.897655814043287)
--(axis cs:70.4081632653061,0.895948923305318)
--(axis cs:70.7482993197279,0.898758924443856)
--(axis cs:71.0884353741497,0.899121076217474)
--(axis cs:71.4285714285714,0.900030489098422)
--(axis cs:71.7687074829932,0.901727790750784)
--(axis cs:72.108843537415,0.900997822314586)
--(axis cs:72.4489795918367,0.902919104211884)
--(axis cs:72.7891156462585,0.900655631859387)
--(axis cs:73.1292517006803,0.902516815926562)
--(axis cs:73.469387755102,0.903664058097766)
--(axis cs:73.8095238095238,0.903106268943467)
--(axis cs:74.1496598639456,0.9062354558766)
--(axis cs:74.4897959183673,0.905481904552657)
--(axis cs:74.8299319727891,0.907580604562538)
--(axis cs:75.1700680272109,0.908389815533678)
--(axis cs:75.5102040816327,0.90938956498101)
--(axis cs:75.8503401360544,0.910848596375101)
--(axis cs:76.1904761904762,0.913484020258642)
--(axis cs:76.530612244898,0.912774936906233)
--(axis cs:76.8707482993197,0.914057155737964)
--(axis cs:77.2108843537415,0.914667990499749)
--(axis cs:77.5510204081633,0.914704885217911)
--(axis cs:77.891156462585,0.91475006125104)
--(axis cs:78.2312925170068,0.914809571669591)
--(axis cs:78.5714285714286,0.91533454155388)
--(axis cs:78.9115646258503,0.916727015448229)
--(axis cs:79.2517006802721,0.919959162124857)
--(axis cs:79.5918367346939,0.91958565627656)
--(axis cs:79.9319727891156,0.920431693516373)
--(axis cs:80.2721088435374,0.922909403470572)
--(axis cs:80.6122448979592,0.923774445934699)
--(axis cs:80.9523809523809,0.924748107494974)
--(axis cs:81.2925170068027,0.926777135972882)
--(axis cs:81.6326530612245,0.929692170781984)
--(axis cs:81.9727891156463,0.931399780461778)
--(axis cs:82.312925170068,0.930967809488191)
--(axis cs:82.6530612244898,0.9320703125)
--(axis cs:82.9931972789116,0.940050332516763)
--(axis cs:83.3333333333333,0.941725844260239)
--(axis cs:83.6734693877551,0.947454397081459)
--(axis cs:84.0136054421769,0.947721249160492)
--(axis cs:84.3537414965986,0.946721526513057)
--(axis cs:84.6938775510204,0.956628092692476)
--(axis cs:85.0340136054422,0.961052991296723)
--(axis cs:85.3741496598639,0.969312357695165)
--(axis cs:85.7142857142857,0.968543687710927)
--(axis cs:86.0544217687075,0.970608295449359)
--(axis cs:86.3945578231292,0.972144968344409)
--(axis cs:86.734693877551,0.971368663915418)
--(axis cs:87.0748299319728,0.972663580147695)
--(axis cs:87.4149659863945,0.968938170455961)
--(axis cs:87.7551020408163,0.970859338561228)
--(axis cs:88.0952380952381,0.966876526065216)
--(axis cs:88.4353741496599,0.967667693146975)
--(axis cs:88.7755102040816,0.968875517181107)
--(axis cs:89.1156462585034,0.966474058705208)
--(axis cs:89.4557823129252,0.970826645874937)
--(axis cs:89.7959183673469,0.969130233407691)
--(axis cs:90.1360544217687,0.967131444040404)
--(axis cs:90.4761904761905,0.966036816891132)
--(axis cs:90.8163265306122,0.962580986996815)
--(axis cs:91.156462585034,0.966053727940235)
--(axis cs:91.4965986394558,0.96546197158331)
--(axis cs:91.8367346938775,0.960039270774255)
--(axis cs:92.1768707482993,0.955880010636028)
--(axis cs:92.5170068027211,0.953304538053698)
--(axis cs:92.8571428571429,0.952533940337233)
--(axis cs:93.1972789115646,0.953422531679139)
--(axis cs:93.5374149659864,0.947044801645233)
--(axis cs:93.8775510204082,0.947098462496017)
--(axis cs:94.2176870748299,0.949373474307313)
--(axis cs:94.5578231292517,0.947038220732263)
--(axis cs:94.8979591836735,0.952181400452852)
--(axis cs:95.2380952380952,0.952203804397226)
--(axis cs:95.578231292517,0.95536990853518)
--(axis cs:95.9183673469388,0.956714875298462)
--(axis cs:96.2585034013605,0.956796953756321)
--(axis cs:96.5986394557823,0.955655637727933)
--(axis cs:96.9387755102041,0.952186965970901)
--(axis cs:97.2789115646258,0.945813912430311)
--(axis cs:97.6190476190476,0.941076342046492)
--(axis cs:97.9591836734694,0.939008304160723)
--(axis cs:98.2993197278912,0.939538996881539)
--(axis cs:98.6394557823129,0.942309127950062)
--(axis cs:98.9795918367347,0.943616100492995)
--(axis cs:99.3197278911565,0.949372235232933)
--(axis cs:99.6598639455782,0.95019656526388)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:100,0.98)
--(axis cs:99.6598639455782,0.96511593473612)
--(axis cs:99.3197278911565,0.964690264767067)
--(axis cs:98.9795918367347,0.957008899507005)
--(axis cs:98.6394557823129,0.955190872049938)
--(axis cs:98.2993197278912,0.951398503118461)
--(axis cs:97.9591836734694,0.950366695839277)
--(axis cs:97.6190476190476,0.954548657953508)
--(axis cs:97.2789115646258,0.958873587569689)
--(axis cs:96.9387755102041,0.962188034029098)
--(axis cs:96.5986394557823,0.963406862272067)
--(axis cs:96.2585034013605,0.961640546243679)
--(axis cs:95.9183673469388,0.962035124701538)
--(axis cs:95.578231292517,0.96213009146482)
--(axis cs:95.2380952380952,0.961546195602774)
--(axis cs:94.8979591836735,0.961568599547148)
--(axis cs:94.5578231292517,0.959836779267737)
--(axis cs:94.2176870748299,0.961876525692687)
--(axis cs:93.8775510204082,0.961651537503983)
--(axis cs:93.5374149659864,0.963892698354767)
--(axis cs:93.1972789115646,0.970639968320861)
--(axis cs:92.8571428571429,0.969966059662767)
--(axis cs:92.5170068027211,0.971070461946302)
--(axis cs:92.1768707482993,0.973494989363972)
--(axis cs:91.8367346938775,0.976523229225745)
--(axis cs:91.4965986394558,0.97953802841669)
--(axis cs:91.156462585034,0.979571272059765)
--(axis cs:90.8163265306122,0.977106513003185)
--(axis cs:90.4761904761905,0.979588183108868)
--(axis cs:90.1360544217687,0.980056055959596)
--(axis cs:89.7959183673469,0.980557266592309)
--(axis cs:89.4557823129252,0.981360854125063)
--(axis cs:89.1156462585034,0.979463441294792)
--(axis cs:88.7755102040816,0.980499482818893)
--(axis cs:88.4353741496599,0.980457306853025)
--(axis cs:88.0952380952381,0.979373473934784)
--(axis cs:87.7551020408163,0.981328161438772)
--(axis cs:87.4149659863945,0.980749329544039)
--(axis cs:87.0748299319728,0.981711419852305)
--(axis cs:86.734693877551,0.981443836084582)
--(axis cs:86.3945578231292,0.981605031655591)
--(axis cs:86.0544217687075,0.981266704550641)
--(axis cs:85.7142857142857,0.980831312289073)
--(axis cs:85.3741496598639,0.981000142304835)
--(axis cs:85.0340136054422,0.977697008703277)
--(axis cs:84.6938775510204,0.974934407307525)
--(axis cs:84.3537414965986,0.966090973486944)
--(axis cs:84.0136054421769,0.967903750839507)
--(axis cs:83.6734693877551,0.967233102918541)
--(axis cs:83.3333333333333,0.961399155739761)
--(axis cs:82.9931972789116,0.959637167483237)
--(axis cs:82.6530612244898,0.9535546875)
--(axis cs:82.312925170068,0.952157190511809)
--(axis cs:81.9727891156463,0.951100219538222)
--(axis cs:81.6326530612245,0.949370329218016)
--(axis cs:81.2925170068027,0.946972864027118)
--(axis cs:80.9523809523809,0.943689392505026)
--(axis cs:80.6122448979592,0.942475554065301)
--(axis cs:80.2721088435374,0.941153096529428)
--(axis cs:79.9319727891156,0.939255806483626)
--(axis cs:79.5918367346939,0.93635184372344)
--(axis cs:79.2517006802721,0.936290837875143)
--(axis cs:78.9115646258503,0.934210484551771)
--(axis cs:78.5714285714286,0.93341545844612)
--(axis cs:78.2312925170068,0.932377928330409)
--(axis cs:77.891156462585,0.93243743874896)
--(axis cs:77.5510204081633,0.932482614782089)
--(axis cs:77.2108843537415,0.932207009500251)
--(axis cs:76.8707482993197,0.932192844262036)
--(axis cs:76.530612244898,0.931600063093767)
--(axis cs:76.1904761904762,0.932453479741358)
--(axis cs:75.8503401360544,0.930713903624899)
--(axis cs:75.5102040816327,0.92967293501899)
--(axis cs:75.1700680272109,0.928485184466322)
--(axis cs:74.8299319727891,0.927731895437462)
--(axis cs:74.4897959183673,0.925768095447343)
--(axis cs:74.1496598639456,0.9265770441234)
--(axis cs:73.8095238095238,0.924081231056533)
--(axis cs:73.469387755102,0.924460941902234)
--(axis cs:73.1292517006803,0.923733184073438)
--(axis cs:72.7891156462585,0.922156868140613)
--(axis cs:72.4489795918367,0.923330895788116)
--(axis cs:72.108843537415,0.923064677685414)
--(axis cs:71.7687074829932,0.922647209249216)
--(axis cs:71.4285714285714,0.920907010901578)
--(axis cs:71.0884353741497,0.920878923782526)
--(axis cs:70.7482993197279,0.919053575556145)
--(axis cs:70.4081632653061,0.917176076694682)
--(axis cs:70.0680272108844,0.919531685956713)
--(axis cs:69.7278911564626,0.91629778985271)
--(axis cs:69.3877551020408,0.917430009883585)
--(axis cs:69.0476190476191,0.913892202346228)
--(axis cs:68.7074829931973,0.91238660942291)
--(axis cs:68.3673469387755,0.915886498642406)
--(axis cs:68.0272108843537,0.917104425984204)
--(axis cs:67.687074829932,0.916247965273986)
--(axis cs:67.3469387755102,0.913812521541792)
--(axis cs:67.0068027210884,0.913813783560427)
--(axis cs:66.6666666666667,0.912987594750136)
--(axis cs:66.3265306122449,0.914694947438282)
--(axis cs:65.9863945578231,0.913127034284498)
--(axis cs:65.6462585034014,0.909551871001583)
--(axis cs:65.3061224489796,0.909262426329203)
--(axis cs:64.9659863945578,0.909015088421061)
--(axis cs:64.6258503401361,0.9066948262124)
--(axis cs:64.2857142857143,0.906925531508022)
--(axis cs:63.9455782312925,0.904343806397072)
--(axis cs:63.6054421768707,0.904555131311773)
--(axis cs:63.265306122449,0.906252111783648)
--(axis cs:62.9251700680272,0.904568013324996)
--(axis cs:62.5850340136054,0.903808433071232)
--(axis cs:62.2448979591837,0.90799165366089)
--(axis cs:61.9047619047619,0.901931609663701)
--(axis cs:61.5646258503401,0.903371575461264)
--(axis cs:61.2244897959184,0.90531127923329)
--(axis cs:60.8843537414966,0.903029804881238)
--(axis cs:60.5442176870748,0.900504343047096)
--(axis cs:60.2040816326531,0.898879363688637)
--(axis cs:59.8639455782313,0.900747021623388)
--(axis cs:59.5238095238095,0.900204170518828)
--(axis cs:59.1836734693878,0.896204240536912)
--(axis cs:58.843537414966,0.896029084225781)
--(axis cs:58.5034013605442,0.894738423960522)
--(axis cs:58.1632653061224,0.895561499169024)
--(axis cs:57.8231292517007,0.891004205721357)
--(axis cs:57.4829931972789,0.893817170621131)
--(axis cs:57.1428571428571,0.890971836782225)
--(axis cs:56.8027210884354,0.897796251986414)
--(axis cs:56.4625850340136,0.899440540833812)
--(axis cs:56.1224489795918,0.901742424900627)
--(axis cs:55.7823129251701,0.897425203760546)
--(axis cs:55.4421768707483,0.903457955940618)
--(axis cs:55.1020408163265,0.903131102113807)
--(axis cs:54.7619047619048,0.902705569579432)
--(axis cs:54.421768707483,0.907297808593133)
--(axis cs:54.0816326530612,0.903698897171698)
--(axis cs:53.7414965986395,0.900350426287328)
--(axis cs:53.4013605442177,0.895483820723245)
--(axis cs:53.0612244897959,0.903582079009016)
--(axis cs:52.7210884353741,0.900639980748221)
--(axis cs:52.3809523809524,0.898439004503348)
--(axis cs:52.0408163265306,0.899173491420231)
--(axis cs:51.7006802721088,0.901329823882293)
--(axis cs:51.3605442176871,0.894232549569024)
--(axis cs:51.0204081632653,0.896489870661409)
--(axis cs:50.6802721088435,0.904231249296621)
--(axis cs:50.3401360544218,0.899437682389525)
--(axis cs:50,0.903281727048023)
--(axis cs:49.6598639455782,0.905921251986414)
--(axis cs:49.3197278911565,0.90276722421516)
--(axis cs:48.9795918367347,0.906953864798847)
--(axis cs:48.6394557823129,0.907252243799966)
--(axis cs:48.2993197278912,0.90500115375693)
--(axis cs:47.9591836734694,0.907500578213719)
--(axis cs:47.6190476190476,0.90575577288253)
--(axis cs:47.2789115646259,0.905462317952723)
--(axis cs:46.9387755102041,0.907235277237484)
--(axis cs:46.5986394557823,0.903583059124189)
--(axis cs:46.2585034013605,0.908550380379542)
--(axis cs:45.9183673469388,0.903120762597127)
--(axis cs:45.578231292517,0.907278672735849)
--(axis cs:45.2380952380952,0.903942375468942)
--(axis cs:44.8979591836735,0.904702980094211)
--(axis cs:44.5578231292517,0.904425621055631)
--(axis cs:44.2176870748299,0.899120040367402)
--(axis cs:43.8775510204082,0.900683433071232)
--(axis cs:43.5374149659864,0.901397329869639)
--(axis cs:43.1972789115646,0.895059310974494)
--(axis cs:42.8571428571429,0.896765179515545)
--(axis cs:42.5170068027211,0.893355721426505)
--(axis cs:42.1768707482993,0.896578154797984)
--(axis cs:41.8367346938776,0.891254358785492)
--(axis cs:41.4965986394558,0.894675184502535)
--(axis cs:41.156462585034,0.894015336249766)
--(axis cs:40.8163265306122,0.893115637536064)
--(axis cs:40.4761904761905,0.891916203878484)
--(axis cs:40.1360544217687,0.89140230678644)
--(axis cs:39.7959183673469,0.888271529777225)
--(axis cs:39.4557823129252,0.887394907867149)
--(axis cs:39.1156462585034,0.884676541470798)
--(axis cs:38.7755102040816,0.88529455655156)
--(axis cs:38.4353741496599,0.882571038033885)
--(axis cs:38.0952380952381,0.881524473679685)
--(axis cs:37.7551020408163,0.883743958380593)
--(axis cs:37.4149659863946,0.877626675369013)
--(axis cs:37.0748299319728,0.87834131740884)
--(axis cs:36.734693877551,0.877509283124223)
--(axis cs:36.3945578231292,0.876237612205136)
--(axis cs:36.0544217687075,0.872007487856173)
--(axis cs:35.7142857142857,0.870734231268434)
--(axis cs:35.3741496598639,0.870956608769435)
--(axis cs:35.0340136054422,0.868154424395097)
--(axis cs:34.6938775510204,0.865009223076438)
--(axis cs:34.3537414965986,0.86569367103965)
--(axis cs:34.0136054421769,0.864949868809673)
--(axis cs:33.6734693877551,0.861699987394678)
--(axis cs:33.3333333333333,0.859667174770507)
--(axis cs:32.9931972789116,0.85770909784421)
--(axis cs:32.6530612244898,0.854702524418144)
--(axis cs:32.312925170068,0.852376901111117)
--(axis cs:31.9727891156463,0.850386925368721)
--(axis cs:31.6326530612245,0.848092915366019)
--(axis cs:31.2925170068027,0.845438623941593)
--(axis cs:30.952380952381,0.842263405348671)
--(axis cs:30.6122448979592,0.836472075562804)
--(axis cs:30.2721088435374,0.834153529466036)
--(axis cs:29.9319727891156,0.833835447257956)
--(axis cs:29.5918367346939,0.830251105834324)
--(axis cs:29.2517006802721,0.822227657096918)
--(axis cs:28.9115646258503,0.824574029770451)
--(axis cs:28.5714285714286,0.815053550096692)
--(axis cs:28.2312925170068,0.815407798833938)
--(axis cs:27.891156462585,0.811426153391366)
--(axis cs:27.5510204081633,0.810456041674721)
--(axis cs:27.2108843537415,0.806109803202624)
--(axis cs:26.8707482993197,0.801062190951789)
--(axis cs:26.530612244898,0.792272109785084)
--(axis cs:26.1904761904762,0.791978835060282)
--(axis cs:25.8503401360544,0.787216612901377)
--(axis cs:25.5102040816327,0.784906573660131)
--(axis cs:25.1700680272109,0.779094045820797)
--(axis cs:24.8299319727891,0.772532719847573)
--(axis cs:24.4897959183673,0.767698157437566)
--(axis cs:24.1496598639456,0.768896301754969)
--(axis cs:23.8095238095238,0.767955894927008)
--(axis cs:23.469387755102,0.75827552766632)
--(axis cs:23.1292517006803,0.757729366163764)
--(axis cs:22.7891156462585,0.759213609307205)
--(axis cs:22.4489795918367,0.748414523065921)
--(axis cs:22.108843537415,0.748303932636349)
--(axis cs:21.7687074829932,0.743428619865075)
--(axis cs:21.4285714285714,0.736062762319358)
--(axis cs:21.0884353741497,0.739738837745337)
--(axis cs:20.7482993197279,0.728217756646527)
--(axis cs:20.4081632653061,0.72377061029165)
--(axis cs:20.0680272108844,0.714938119344506)
--(axis cs:19.7278911564626,0.712562673666213)
--(axis cs:19.3877551020408,0.70458664161886)
--(axis cs:19.047619047619,0.696344860031178)
--(axis cs:18.7074829931973,0.693369072238136)
--(axis cs:18.3673469387755,0.688992978011825)
--(axis cs:18.0272108843537,0.675620310473293)
--(axis cs:17.687074829932,0.673933693909965)
--(axis cs:17.3469387755102,0.664301385938596)
--(axis cs:17.0068027210884,0.666582313491139)
--(axis cs:16.6666666666667,0.662359531009957)
--(axis cs:16.3265306122449,0.658022443168886)
--(axis cs:15.9863945578231,0.651378206436334)
--(axis cs:15.6462585034014,0.64329206646509)
--(axis cs:15.3061224489796,0.640572113492248)
--(axis cs:14.9659863945578,0.63124548813939)
--(axis cs:14.6258503401361,0.623899313816264)
--(axis cs:14.2857142857143,0.61312221103684)
--(axis cs:13.9455782312925,0.610981344032558)
--(axis cs:13.6054421768707,0.599908586011246)
--(axis cs:13.265306122449,0.597092613199732)
--(axis cs:12.9251700680272,0.575070613038808)
--(axis cs:12.5850340136054,0.577262451871099)
--(axis cs:12.2448979591837,0.569012156627533)
--(axis cs:11.9047619047619,0.552328788343415)
--(axis cs:11.5646258503401,0.537602999894531)
--(axis cs:11.2244897959184,0.52248046875)
--(axis cs:10.8843537414966,0.510381766949186)
--(axis cs:10.5442176870748,0.495793673594925)
--(axis cs:10.2040816326531,0.482779608285345)
--(axis cs:9.86394557823129,0.46944124376342)
--(axis cs:9.52380952380952,0.457085825453158)
--(axis cs:9.18367346938775,0.448826041685102)
--(axis cs:8.84353741496599,0.4390765522228)
--(axis cs:8.50340136054422,0.418869654018382)
--(axis cs:8.16326530612245,0.411000173666213)
--(axis cs:7.82312925170068,0.402520070779059)
--(axis cs:7.48299319727891,0.384052369644471)
--(axis cs:7.14285714285714,0.368672259175884)
--(axis cs:6.80272108843537,0.362755234230485)
--(axis cs:6.46258503401361,0.357634146196309)
--(axis cs:6.12244897959184,0.340919681929666)
--(axis cs:5.78231292517007,0.331178053275652)
--(axis cs:5.4421768707483,0.3139870543681)
--(axis cs:5.10204081632653,0.298512604784786)
--(axis cs:4.76190476190476,0.284605030334385)
--(axis cs:4.42176870748299,0.270570739538371)
--(axis cs:4.08163265306122,0.255347412166656)
--(axis cs:3.74149659863946,0.2338480945175)
--(axis cs:3.40136054421769,0.221223042939588)
--(axis cs:3.06122448979592,0.19632693402584)
--(axis cs:2.72108843537415,0.17685848086155)
--(axis cs:2.38095238095238,0.15332863581629)
--(axis cs:2.04081632653061,0.138369893419507)
--(axis cs:1.70068027210884,0.127902805744601)
--(axis cs:1.36054421768707,0.117441423782526)
--(axis cs:1.02040816326531,0.100426406622949)
--(axis cs:0.680272108843537,0.090083277363701)
--(axis cs:0.340136054421769,0.084082929510294)
--(axis cs:0,0.0850218862598796)
--cycle;


==> img/stl10/stl10_rate_accuracy_sensitivity.tex <==
\addplot [line width=0.5, opacity=0.7, color6, mark=square, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color6, thin}]
table [row sep=\\]{%
0	0.0771875 \\
0.340136054421769	0.07484375 \\
0.680272108843537	0.0728125 \\
1.02040816326531	0.073125 \\
1.36054421768707	0.0734375 \\
1.70068027210884	0.0703125 \\
2.04081632653061	0.0684375 \\
2.38095238095238	0.0721875 \\
2.72108843537415	0.0753125 \\
3.06122448979592	0.0725 \\
3.40136054421769	0.0728125 \\
3.74149659863946	0.07515625 \\
4.08163265306122	0.075 \\
4.42176870748299	0.07328125 \\
4.76190476190476	0.07453125 \\
5.10204081632653	0.0765625 \\
5.4421768707483	0.07640625 \\
5.78231292517007	0.07796875 \\
6.12244897959184	0.07484375 \\
6.46258503401361	0.0778125 \\
6.80272108843537	0.07890625 \\
7.14285714285714	0.08171875 \\
7.48299319727891	0.08390625 \\
7.82312925170068	0.08 \\
8.16326530612245	0.08578125 \\
8.50340136054422	0.08609375 \\
8.84353741496599	0.09046875 \\
9.18367346938775	0.0875 \\
9.52380952380952	0.095 \\
9.86394557823129	0.091875 \\
10.2040816326531	0.09453125 \\
10.5442176870748	0.09390625 \\
10.8843537414966	0.0953125 \\
11.2244897959184	0.0975 \\
11.5646258503401	0.09984375 \\
11.9047619047619	0.103125 \\
12.2448979591837	0.10484375 \\
12.5850340136054	0.1084375 \\
12.9251700680272	0.10796875 \\
13.265306122449	0.10953125 \\
13.6054421768707	0.11109375 \\
13.9455782312925	0.11078125 \\
14.2857142857143	0.11640625 \\
14.6258503401361	0.11921875 \\
14.9659863945578	0.1171875 \\
15.3061224489796	0.1228125 \\
15.6462585034014	0.12609375 \\
15.9863945578231	0.12734375 \\
16.3265306122449	0.13 \\
16.6666666666667	0.13171875 \\
17.0068027210884	0.13515625 \\
17.3469387755102	0.13640625 \\
17.687074829932	0.1465625 \\
18.0272108843537	0.14375 \\
18.3673469387755	0.144375 \\
18.7074829931973	0.15015625 \\
19.047619047619	0.1528125 \\
19.3877551020408	0.155625 \\
19.7278911564626	0.15703125 \\
20.0680272108844	0.16171875 \\
20.4081632653061	0.168125 \\
20.7482993197279	0.16890625 \\
21.0884353741497	0.171875 \\
21.4285714285714	0.17375 \\
21.7687074829932	0.174375 \\
22.108843537415	0.17328125 \\
22.4489795918367	0.17703125 \\
22.7891156462585	0.1809375 \\
23.1292517006803	0.183125 \\
23.469387755102	0.1834375 \\
23.8095238095238	0.18515625 \\
24.1496598639456	0.1840625 \\
24.4897959183673	0.18859375 \\
24.8299319727891	0.1925 \\
25.1700680272109	0.19625 \\
25.5102040816327	0.19265625 \\
25.8503401360544	0.195625 \\
26.1904761904762	0.19296875 \\
26.530612244898	0.1928125 \\
26.8707482993197	0.1925 \\
27.2108843537415	0.1921875 \\
27.5510204081633	0.19453125 \\
27.891156462585	0.191875 \\
28.2312925170068	0.1953125 \\
28.5714285714286	0.195625 \\
28.9115646258503	0.1946875 \\
29.2517006802721	0.198125 \\
29.5918367346939	0.1971875 \\
29.9319727891156	0.20109375 \\
30.2721088435374	0.20171875 \\
30.6122448979592	0.20421875 \\
30.952380952381	0.204375 \\
31.2925170068027	0.20375 \\
31.6326530612245	0.20546875 \\
31.9727891156463	0.2096875 \\
32.312925170068	0.21484375 \\
32.6530612244898	0.2165625 \\
32.9931972789116	0.2175 \\
33.3333333333333	0.21953125 \\
33.6734693877551	0.2234375 \\
34.0136054421769	0.2246875 \\
34.3537414965986	0.2234375 \\
34.6938775510204	0.22953125 \\
35.0340136054422	0.230625 \\
35.3741496598639	0.2359375 \\
35.7142857142857	0.23296875 \\
36.0544217687075	0.2403125 \\
36.3945578231292	0.245 \\
36.734693877551	0.245 \\
37.0748299319728	0.25 \\
37.4149659863946	0.2521875 \\
37.7551020408163	0.25640625 \\
38.0952380952381	0.255625 \\
38.4353741496599	0.2590625 \\
38.7755102040816	0.2646875 \\
39.1156462585034	0.2675 \\
39.4557823129252	0.27203125 \\
39.7959183673469	0.27296875 \\
40.1360544217687	0.27734375 \\
40.4761904761905	0.2809375 \\
40.8163265306122	0.27890625 \\
41.156462585034	0.28828125 \\
41.4965986394558	0.29078125 \\
41.8367346938776	0.2928125 \\
42.1768707482993	0.2959375 \\
42.5170068027211	0.300625 \\
42.8571428571429	0.30671875 \\
43.1972789115646	0.31 \\
43.5374149659864	0.31359375 \\
43.8775510204082	0.31359375 \\
44.2176870748299	0.3196875 \\
44.5578231292517	0.325 \\
44.8979591836735	0.3240625 \\
45.2380952380952	0.326875 \\
45.578231292517	0.3265625 \\
45.9183673469388	0.33171875 \\
46.2585034013605	0.33625 \\
46.5986394557823	0.3378125 \\
46.9387755102041	0.3453125 \\
47.2789115646259	0.348125 \\
47.6190476190476	0.35421875 \\
47.9591836734694	0.35859375 \\
48.2993197278912	0.3628125 \\
48.6394557823129	0.37046875 \\
48.9795918367347	0.3734375 \\
49.3197278911565	0.37890625 \\
49.6598639455782	0.3728125 \\
50	0.38359375 \\
50.3401360544218	0.38609375 \\
50.6802721088435	0.391875 \\
51.0204081632653	0.3909375 \\
51.3605442176871	0.3996875 \\
51.7006802721088	0.4003125 \\
52.0408163265306	0.40359375 \\
52.3809523809524	0.41046875 \\
52.7210884353741	0.42203125 \\
53.0612244897959	0.428125 \\
53.4013605442177	0.433125 \\
53.7414965986395	0.435625 \\
54.0816326530612	0.44125 \\
54.421768707483	0.44875 \\
54.7619047619048	0.45359375 \\
55.1020408163265	0.461875 \\
55.4421768707483	0.470625 \\
55.7823129251701	0.46890625 \\
56.1224489795918	0.4834375 \\
56.4625850340136	0.4884375 \\
56.8027210884354	0.49625 \\
57.1428571428571	0.498125 \\
57.4829931972789	0.5021875 \\
57.8231292517007	0.508125 \\
58.1632653061224	0.511875 \\
58.5034013605442	0.52171875 \\
58.843537414966	0.520625 \\
59.1836734693878	0.5325 \\
59.5238095238095	0.54328125 \\
59.8639455782313	0.5421875 \\
60.2040816326531	0.54953125 \\
60.5442176870748	0.55578125 \\
60.8843537414966	0.56359375 \\
61.2244897959184	0.5696875 \\
61.5646258503401	0.57140625 \\
61.9047619047619	0.5796875 \\
62.2448979591837	0.5853125 \\
62.5850340136054	0.5928125 \\
62.9251700680272	0.59421875 \\
63.265306122449	0.5975 \\
63.6054421768707	0.5990625 \\
63.9455782312925	0.605625 \\
64.2857142857143	0.60546875 \\
64.6258503401361	0.61015625 \\
64.9659863945578	0.614375 \\
65.3061224489796	0.61796875 \\
65.6462585034014	0.6225 \\
65.9863945578231	0.62921875 \\
66.3265306122449	0.63390625 \\
66.6666666666667	0.63609375 \\
67.0068027210884	0.6409375 \\
67.3469387755102	0.64359375 \\
67.687074829932	0.65390625 \\
68.0272108843537	0.65484375 \\
68.3673469387755	0.65890625 \\
68.7074829931973	0.6671875 \\
69.0476190476191	0.6746875 \\
69.3877551020408	0.67859375 \\
69.7278911564626	0.6846875 \\
70.0680272108844	0.68421875 \\
70.4081632653061	0.6959375 \\
70.7482993197279	0.69953125 \\
71.0884353741497	0.70546875 \\
71.4285714285714	0.70890625 \\
71.7687074829932	0.70953125 \\
72.108843537415	0.7209375 \\
72.4489795918367	0.72609375 \\
72.7891156462585	0.7315625 \\
73.1292517006803	0.7359375 \\
73.469387755102	0.73765625 \\
73.8095238095238	0.74109375 \\
74.1496598639456	0.7528125 \\
74.4897959183673	0.7578125 \\
74.8299319727891	0.763125 \\
75.1700680272109	0.76875 \\
75.5102040816327	0.77328125 \\
75.8503401360544	0.7753125 \\
76.1904761904762	0.780625 \\
76.530612244898	0.78140625 \\
76.8707482993197	0.7853125 \\
77.2108843537415	0.78640625 \\
77.5510204081633	0.790625 \\
77.891156462585	0.7921875 \\
78.2312925170068	0.79546875 \\
78.5714285714286	0.79890625 \\
78.9115646258503	0.79578125 \\
79.2517006802721	0.79875 \\
79.5918367346939	0.8003125 \\
79.9319727891156	0.80109375 \\
80.2721088435374	0.80421875 \\
80.6122448979592	0.8109375 \\
80.9523809523809	0.8109375 \\
81.2925170068027	0.8125 \\
81.6326530612245	0.8159375 \\
81.9727891156463	0.81453125 \\
82.312925170068	0.81515625 \\
82.6530612244898	0.8215625 \\
82.9931972789116	0.82515625 \\
83.3333333333333	0.825 \\
83.6734693877551	0.8278125 \\
84.0136054421769	0.8265625 \\
84.3537414965986	0.8303125 \\
84.6938775510204	0.833125 \\
85.0340136054422	0.83421875 \\
85.3741496598639	0.83734375 \\
85.7142857142857	0.84 \\
86.0544217687075	0.8396875 \\
86.3945578231292	0.84171875 \\
86.734693877551	0.84359375 \\
87.0748299319728	0.84359375 \\
87.4149659863945	0.8440625 \\
87.7551020408163	0.84765625 \\
88.0952380952381	0.84921875 \\
88.4353741496599	0.85203125 \\
88.7755102040816	0.8571875 \\
89.1156462585034	0.86375 \\
89.4557823129252	0.86859375 \\
89.7959183673469	0.8715625 \\
90.1360544217687	0.879375 \\
90.4761904761905	0.88578125 \\
90.8163265306122	0.88671875 \\
91.156462585034	0.89015625 \\
91.4965986394558	0.89765625 \\
91.8367346938775	0.899375 \\
92.1768707482993	0.90171875 \\
92.5170068027211	0.90296875 \\
92.8571428571429	0.90640625 \\
93.1972789115646	0.90828125 \\
93.5374149659864	0.9134375 \\
93.8775510204082	0.91359375 \\
94.2176870748299	0.91515625 \\
94.5578231292517	0.91734375 \\
94.8979591836735	0.9175 \\
95.2380952380952	0.91859375 \\
95.578231292517	0.9184375 \\
95.9183673469388	0.9259375 \\
96.2585034013605	0.93140625 \\
96.5986394557823	0.9346875 \\
96.9387755102041	0.94125 \\
97.2789115646258	0.94796875 \\
97.6190476190476	0.954375 \\
97.9591836734694	0.9590625 \\
98.2993197278912	0.95875 \\
98.6394557823129	0.9596875 \\
98.9795918367347	0.9596875 \\
99.3197278911565	0.96125 \\
99.6598639455782	0.96796875 \\
100	1 \\
};
\path [fill=color6, fill opacity=0.25]
(axis cs:0,0.0840707071041821)
--(axis cs:0,0.0703042928958179)
--(axis cs:0.340136054421769,0.0677470225394437)
--(axis cs:0.680272108843537,0.0653012169831916)
--(axis cs:1.02040816326531,0.0661769791381657)
--(axis cs:1.36054421768707,0.0656998211759608)
--(axis cs:1.70068027210884,0.0626118851547983)
--(axis cs:2.04081632653061,0.0608290815700069)
--(axis cs:2.38095238095238,0.0637595902303159)
--(axis cs:2.72108843537415,0.066546253573164)
--(axis cs:3.06122448979592,0.0637131079068734)
--(axis cs:3.40136054421769,0.0637794288438694)
--(axis cs:3.74149659863946,0.0658593955160415)
--(axis cs:4.08163265306122,0.0654316806922532)
--(axis cs:4.42176870748299,0.0636984894412279)
--(axis cs:4.76190476190476,0.0649008384163496)
--(axis cs:5.10204081632653,0.0662635846459104)
--(axis cs:5.4421768707483,0.0663628376094681)
--(axis cs:5.78231292517007,0.0672839780128684)
--(axis cs:6.12244897959184,0.0650493587740327)
--(axis cs:6.46258503401361,0.0671112284907791)
--(axis cs:6.80272108843537,0.0680831350932747)
--(axis cs:7.14285714285714,0.0705223001657176)
--(axis cs:7.48299319727891,0.0724022774301572)
--(axis cs:7.82312925170068,0.0687157368549576)
--(axis cs:8.16326530612245,0.0740816399794143)
--(axis cs:8.50340136054422,0.0743120991499311)
--(axis cs:8.84353741496599,0.0785374899990629)
--(axis cs:9.18367346938775,0.0769386673167221)
--(axis cs:9.52380952380952,0.0832576734559962)
--(axis cs:9.86394557823129,0.0803581851657769)
--(axis cs:10.2040816326531,0.0831255183925591)
--(axis cs:10.5442176870748,0.0828667735226685)
--(axis cs:10.8843537414966,0.0843037338507485)
--(axis cs:11.2244897959184,0.0858629147579951)
--(axis cs:11.5646258503401,0.0883256931258882)
--(axis cs:11.9047619047619,0.09134132568047)
--(axis cs:12.2448979591837,0.0934715130147868)
--(axis cs:12.5850340136054,0.0959268234072416)
--(axis cs:12.9251700680272,0.0958558315416308)
--(axis cs:13.265306122449,0.0973047031000499)
--(axis cs:13.6054421768707,0.0987623522791017)
--(axis cs:13.9455782312925,0.0977819595530555)
--(axis cs:14.2857142857143,0.103700800321296)
--(axis cs:14.6258503401361,0.106719131475548)
--(axis cs:14.9659863945578,0.104149019120596)
--(axis cs:15.3061224489796,0.110218250824099)
--(axis cs:15.6462585034014,0.113301526739278)
--(axis cs:15.9863945578231,0.114513562014047)
--(axis cs:16.3265306122449,0.117445188531259)
--(axis cs:16.6666666666667,0.118326307030679)
--(axis cs:17.0068027210884,0.122079425397873)
--(axis cs:17.3469387755102,0.12380405241739)
--(axis cs:17.687074829932,0.132522397393496)
--(axis cs:18.0272108843537,0.129212004883687)
--(axis cs:18.3673469387755,0.129556971298132)
--(axis cs:18.7074829931973,0.134852234991963)
--(axis cs:19.047619047619,0.138166015755226)
--(axis cs:19.3877551020408,0.139932397220906)
--(axis cs:19.7278911564626,0.14172661185163)
--(axis cs:20.0680272108844,0.146551190692495)
--(axis cs:20.4081632653061,0.152633628047185)
--(axis cs:20.7482993197279,0.153526398222488)
--(axis cs:21.0884353741497,0.156539548052771)
--(axis cs:21.4285714285714,0.159567972171439)
--(axis cs:21.7687074829932,0.159578225028387)
--(axis cs:22.108843537415,0.158406372583718)
--(axis cs:22.4489795918367,0.162468676129312)
--(axis cs:22.7891156462585,0.166211792340792)
--(axis cs:23.1292517006803,0.168268406050206)
--(axis cs:23.469387755102,0.16873836896701)
--(axis cs:23.8095238095238,0.170449011248144)
--(axis cs:24.1496598639456,0.169975607093549)
--(axis cs:24.4897959183673,0.174513290006175)
--(axis cs:24.8299319727891,0.179042557721263)
--(axis cs:25.1700680272109,0.182603958558561)
--(axis cs:25.5102040816327,0.178672979814068)
--(axis cs:25.8503401360544,0.182250727878305)
--(axis cs:26.1904761904762,0.178865280491654)
--(axis cs:26.530612244898,0.17886166294654)
--(axis cs:26.8707482993197,0.178659659570901)
--(axis cs:27.2108843537415,0.178163028850769)
--(axis cs:27.5510204081633,0.180969683279339)
--(axis cs:27.891156462585,0.178515710663652)
--(axis cs:28.2312925170068,0.182009725621986)
--(axis cs:28.5714285714286,0.182468560951848)
--(axis cs:28.9115646258503,0.181554277361773)
--(axis cs:29.2517006802721,0.184203588628301)
--(axis cs:29.5918367346939,0.183093838778689)
--(axis cs:29.9319727891156,0.18654165798689)
--(axis cs:30.2721088435374,0.188029795824072)
--(axis cs:30.6122448979592,0.189192692818917)
--(axis cs:30.952380952381,0.189254986536749)
--(axis cs:31.2925170068027,0.18891846205472)
--(axis cs:31.6326530612245,0.190481458325279)
--(axis cs:31.9727891156463,0.194786679406969)
--(axis cs:32.312925170068,0.199859003829382)
--(axis cs:32.6530612244898,0.201639934775453)
--(axis cs:32.9931972789116,0.202040056365635)
--(axis cs:33.3333333333333,0.204509636238327)
--(axis cs:33.6734693877551,0.207535415805207)
--(axis cs:34.0136054421769,0.209892658699683)
--(axis cs:34.3537414965986,0.208504712964014)
--(axis cs:34.6938775510204,0.21528648660071)
--(axis cs:35.0340136054422,0.215749802021735)
--(axis cs:35.3741496598639,0.220774028178364)
--(axis cs:35.7142857142857,0.217749719767243)
--(axis cs:36.0544217687075,0.22591557060767)
--(axis cs:36.3945578231292,0.230260698480683)
--(axis cs:36.734693877551,0.230081269760369)
--(axis cs:37.0748299319728,0.235270407100588)
--(axis cs:37.4149659863946,0.237981955823462)
--(axis cs:37.7551020408163,0.241824696967392)
--(axis cs:38.0952380952381,0.239985968214575)
--(axis cs:38.4353741496599,0.244030414564862)
--(axis cs:38.7755102040816,0.249718991594134)
--(axis cs:39.1156462585034,0.252078968013163)
--(axis cs:39.4557823129252,0.256476905355204)
--(axis cs:39.7959183673469,0.257566591508215)
--(axis cs:40.1360544217687,0.261249419287631)
--(axis cs:40.4761904761905,0.265085270428957)
--(axis cs:40.8163265306122,0.262540449324118)
--(axis cs:41.156462585034,0.272058844888171)
--(axis cs:41.4965986394558,0.273383904863519)
--(axis cs:41.8367346938776,0.276037782601521)
--(axis cs:42.1768707482993,0.279265430054736)
--(axis cs:42.5170068027211,0.28361374094694)
--(axis cs:42.8571428571429,0.289905701373235)
--(axis cs:43.1972789115646,0.294216502132555)
--(axis cs:43.5374149659864,0.297642265919816)
--(axis cs:43.8775510204082,0.29749586436253)
--(axis cs:44.2176870748299,0.303364001477811)
--(axis cs:44.5578231292517,0.308995692832853)
--(axis cs:44.8979591836735,0.306846171194501)
--(axis cs:45.2380952380952,0.310124177412048)
--(axis cs:45.578231292517,0.309886426401456)
--(axis cs:45.9183673469388,0.315284331752024)
--(axis cs:46.2585034013605,0.319771828033207)
--(axis cs:46.5986394557823,0.321693597098074)
--(axis cs:46.9387755102041,0.32937926106288)
--(axis cs:47.2789115646259,0.331837764266102)
--(axis cs:47.6190476190476,0.338084767086191)
--(axis cs:47.9591836734694,0.342755062272456)
--(axis cs:48.2993197278912,0.346677039412248)
--(axis cs:48.6394557823129,0.354022730029321)
--(axis cs:48.9795918367347,0.356631543152891)
--(axis cs:49.3197278911565,0.362879612684652)
--(axis cs:49.6598639455782,0.356738625364406)
--(axis cs:50,0.367227366610594)
--(axis cs:50.3401360544218,0.369372273605042)
--(axis cs:50.6802721088435,0.37486990881469)
--(axis cs:51.0204081632653,0.374055109582729)
--(axis cs:51.3605442176871,0.382735207573727)
--(axis cs:51.7006802721088,0.383412606974382)
--(axis cs:52.0408163265306,0.387125130177963)
--(axis cs:52.3809523809524,0.39310872060119)
--(axis cs:52.7210884353741,0.404027240352054)
--(axis cs:53.0612244897959,0.409894380173248)
--(axis cs:53.4013605442177,0.414390774050582)
--(axis cs:53.7414965986395,0.416944301248096)
--(axis cs:54.0816326530612,0.422702509619518)
--(axis cs:54.421768707483,0.42997153852856)
--(axis cs:54.7619047619048,0.434556791813947)
--(axis cs:55.1020408163265,0.442626063784974)
--(axis cs:55.4421768707483,0.451002653848078)
--(axis cs:55.7823129251701,0.44933183480816)
--(axis cs:56.1224489795918,0.463562593664234)
--(axis cs:56.4625850340136,0.469373259076679)
--(axis cs:56.8027210884354,0.476990662300509)
--(axis cs:57.1428571428571,0.479190765158754)
--(axis cs:57.4829931972789,0.483375549932768)
--(axis cs:57.8231292517007,0.489801501976042)
--(axis cs:58.1632653061224,0.49379672054004)
--(axis cs:58.5034013605442,0.503629132309499)
--(axis cs:58.843537414966,0.502468814712088)
--(axis cs:59.1836734693878,0.514996360067441)
--(axis cs:59.5238095238095,0.526061874816392)
--(axis cs:59.8639455782313,0.525293250995855)
--(axis cs:60.2040816326531,0.533132849254895)
--(axis cs:60.5442176870748,0.539450450185447)
--(axis cs:60.8843537414966,0.547362529161529)
--(axis cs:61.2244897959184,0.553469504548501)
--(axis cs:61.5646258503401,0.555395687252025)
--(axis cs:61.9047619047619,0.563846705003132)
--(axis cs:62.2448979591837,0.569629015703215)
--(axis cs:62.5850340136054,0.577744928604328)
--(axis cs:62.9251700680272,0.57853800228189)
--(axis cs:63.265306122449,0.581894543472314)
--(axis cs:63.6054421768707,0.584229676101803)
--(axis cs:63.9455782312925,0.590755573194786)
--(axis cs:64.2857142857143,0.590086418101242)
--(axis cs:64.6258503401361,0.59445423035218)
--(axis cs:64.9659863945578,0.598525778727603)
--(axis cs:65.3061224489796,0.60266411185163)
--(axis cs:65.6462585034014,0.607186329166255)
--(axis cs:65.9863945578231,0.612801168812569)
--(axis cs:66.3265306122449,0.617609941004106)
--(axis cs:66.6666666666667,0.620053432240578)
--(axis cs:67.0068027210884,0.62435317990988)
--(axis cs:67.3469387755102,0.627278140543456)
--(axis cs:67.687074829932,0.637712676373952)
--(axis cs:68.0272108843537,0.638578486641718)
--(axis cs:68.3673469387755,0.642692665408141)
--(axis cs:68.7074829931973,0.650840065432357)
--(axis cs:69.0476190476191,0.658898565067314)
--(axis cs:69.3877551020408,0.662782180753214)
--(axis cs:69.7278911564626,0.669198590708666)
--(axis cs:70.0680272108844,0.668434345824956)
--(axis cs:70.4081632653061,0.679921875)
--(axis cs:70.7482993197279,0.68432663915197)
--(axis cs:71.0884353741497,0.690374302976918)
--(axis cs:71.4285714285714,0.69354377028216)
--(axis cs:71.7687074829932,0.694614117961734)
--(axis cs:72.108843537415,0.705459677534251)
--(axis cs:72.4489795918367,0.710412394112024)
--(axis cs:72.7891156462585,0.717125219833925)
--(axis cs:73.1292517006803,0.721311214666524)
--(axis cs:73.469387755102,0.723128426248183)
--(axis cs:73.8095238095238,0.72629149766482)
--(axis cs:74.1496598639456,0.739080072708142)
--(axis cs:74.4897959183673,0.743825479256912)
--(axis cs:74.8299319727891,0.750596041843774)
--(axis cs:75.1700680272109,0.756483348719289)
--(axis cs:75.5102040816327,0.761653592977327)
--(axis cs:75.8503401360544,0.763562866216644)
--(axis cs:76.1904761904762,0.768854281895844)
--(axis cs:76.530612244898,0.77006844769495)
--(axis cs:76.8707482993197,0.774846410377681)
--(axis cs:77.2108843537415,0.775295303134013)
--(axis cs:77.5510204081633,0.780417235513564)
--(axis cs:77.891156462585,0.781906193602928)
--(axis cs:78.2312925170068,0.786235714359239)
--(axis cs:78.5714285714286,0.789614525947691)
--(axis cs:78.9115646258503,0.786266403555814)
--(axis cs:79.2517006802721,0.790127445291155)
--(axis cs:79.5918367346939,0.790825256881874)
--(axis cs:79.9319727891156,0.792201667140892)
--(axis cs:80.2721088435374,0.794342907132737)
--(axis cs:80.6122448979592,0.800983266655608)
--(axis cs:80.9523809523809,0.802083572690123)
--(axis cs:81.2925170068027,0.802915746760636)
--(axis cs:81.6326530612245,0.806041880827427)
--(axis cs:81.9727891156463,0.805278610193772)
--(axis cs:82.312925170068,0.805727995493877)
--(axis cs:82.6530612244898,0.812210926078223)
--(axis cs:82.9931972789116,0.816412333832384)
--(axis cs:83.3333333333333,0.815885997972406)
--(axis cs:83.6734693877551,0.818728893785755)
--(axis cs:84.0136054421769,0.818113117813936)
--(axis cs:84.3537414965986,0.821683311705322)
--(axis cs:84.6938775510204,0.825266250180183)
--(axis cs:85.0340136054422,0.826204390062365)
--(axis cs:85.3741496598639,0.829621492881457)
--(axis cs:85.7142857142857,0.831622027113466)
--(axis cs:86.0544217687075,0.832965514496346)
--(axis cs:86.3945578231292,0.83517578125)
--(axis cs:86.734693877551,0.837373575804963)
--(axis cs:87.0748299319728,0.837438306832297)
--(axis cs:87.4149659863945,0.837250320302111)
--(axis cs:87.7551020408163,0.839769034036228)
--(axis cs:88.0952380952381,0.841064014560821)
--(axis cs:88.4353741496599,0.843161718199485)
--(axis cs:88.7755102040816,0.84749244246407)
--(axis cs:89.1156462585034,0.853741306269282)
--(axis cs:89.4557823129252,0.858913951366407)
--(axis cs:89.7959183673469,0.862543164149204)
--(axis cs:90.1360544217687,0.871058723103108)
--(axis cs:90.4761904761905,0.878162184726645)
--(axis cs:90.8163265306122,0.879511348248006)
--(axis cs:91.156462585034,0.882679964044757)
--(axis cs:91.4965986394558,0.89052466873818)
--(axis cs:91.8367346938775,0.893160194305978)
--(axis cs:92.1768707482993,0.895183073093066)
--(axis cs:92.5170068027211,0.897452252249024)
--(axis cs:92.8571428571429,0.899773528370396)
--(axis cs:93.1972789115646,0.900490141591098)
--(axis cs:93.5374149659864,0.904409709180532)
--(axis cs:93.8775510204082,0.904836755550862)
--(axis cs:94.2176870748299,0.906190470160528)
--(axis cs:94.5578231292517,0.907816883532353)
--(axis cs:94.8979591836735,0.908430052561718)
--(axis cs:95.2380952380952,0.909435384636687)
--(axis cs:95.578231292517,0.909197752990223)
--(axis cs:95.9183673469388,0.916632955172693)
--(axis cs:96.2585034013605,0.921839425858964)
--(axis cs:96.5986394557823,0.925105237053097)
--(axis cs:96.9387755102041,0.931760746659769)
--(axis cs:97.2789115646258,0.940162966754534)
--(axis cs:97.6190476190476,0.948306153149106)
--(axis cs:97.9591836734694,0.955977427929896)
--(axis cs:98.2993197278912,0.955686643136453)
--(axis cs:98.6394557823129,0.958137255091173)
--(axis cs:98.9795918367347,0.958131115483349)
--(axis cs:99.3197278911565,0.958224231760776)
--(axis cs:99.6598639455782,0.961849044908635)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,0.974088455091365)
--(axis cs:99.3197278911565,0.964275768239225)
--(axis cs:98.9795918367347,0.961243884516651)
--(axis cs:98.6394557823129,0.961237744908827)
--(axis cs:98.2993197278912,0.961813356863547)
--(axis cs:97.9591836734694,0.962147572070104)
--(axis cs:97.6190476190476,0.960443846850894)
--(axis cs:97.2789115646258,0.955774533245466)
--(axis cs:96.9387755102041,0.950739253340231)
--(axis cs:96.5986394557823,0.944269762946903)
--(axis cs:96.2585034013605,0.940973074141036)
--(axis cs:95.9183673469388,0.935242044827307)
--(axis cs:95.578231292517,0.927677247009777)
--(axis cs:95.2380952380952,0.927752115363313)
--(axis cs:94.8979591836735,0.926569947438282)
--(axis cs:94.5578231292517,0.926870616467647)
--(axis cs:94.2176870748299,0.924122029839472)
--(axis cs:93.8775510204082,0.922350744449138)
--(axis cs:93.5374149659864,0.922465290819468)
--(axis cs:93.1972789115646,0.916072358408902)
--(axis cs:92.8571428571429,0.913038971629604)
--(axis cs:92.5170068027211,0.908485247750976)
--(axis cs:92.1768707482993,0.908254426906934)
--(axis cs:91.8367346938775,0.905589805694022)
--(axis cs:91.4965986394558,0.90478783126182)
--(axis cs:91.156462585034,0.897632535955243)
--(axis cs:90.8163265306122,0.893926151751994)
--(axis cs:90.4761904761905,0.893400315273355)
--(axis cs:90.1360544217687,0.887691276896892)
--(axis cs:89.7959183673469,0.880581835850796)
--(axis cs:89.4557823129252,0.878273548633593)
--(axis cs:89.1156462585034,0.873758693730718)
--(axis cs:88.7755102040816,0.86688255753593)
--(axis cs:88.4353741496599,0.860900781800515)
--(axis cs:88.0952380952381,0.857373485439179)
--(axis cs:87.7551020408163,0.855543465963772)
--(axis cs:87.4149659863945,0.850874679697889)
--(axis cs:87.0748299319728,0.849749193167703)
--(axis cs:86.734693877551,0.849813924195037)
--(axis cs:86.3945578231292,0.84826171875)
--(axis cs:86.0544217687075,0.846409485503654)
--(axis cs:85.7142857142857,0.848377972886534)
--(axis cs:85.3741496598639,0.845066007118543)
--(axis cs:85.0340136054422,0.842233109937635)
--(axis cs:84.6938775510204,0.840983749819817)
--(axis cs:84.3537414965986,0.838941688294678)
--(axis cs:84.0136054421769,0.835011882186064)
--(axis cs:83.6734693877551,0.836896106214245)
--(axis cs:83.3333333333333,0.834114002027594)
--(axis cs:82.9931972789116,0.833900166167616)
--(axis cs:82.6530612244898,0.830914073921777)
--(axis cs:82.312925170068,0.824584504506123)
--(axis cs:81.9727891156463,0.823783889806228)
--(axis cs:81.6326530612245,0.825833119172573)
--(axis cs:81.2925170068027,0.822084253239364)
--(axis cs:80.9523809523809,0.819791427309877)
--(axis cs:80.6122448979592,0.820891733344392)
--(axis cs:80.2721088435374,0.814094592867263)
--(axis cs:79.9319727891156,0.809985832859108)
--(axis cs:79.5918367346939,0.809799743118126)
--(axis cs:79.2517006802721,0.807372554708845)
--(axis cs:78.9115646258503,0.805296096444186)
--(axis cs:78.5714285714286,0.808197974052309)
--(axis cs:78.2312925170068,0.804701785640761)
--(axis cs:77.891156462585,0.802468806397072)
--(axis cs:77.5510204081633,0.800832764486436)
--(axis cs:77.2108843537415,0.797517196865987)
--(axis cs:76.8707482993197,0.795778589622319)
--(axis cs:76.530612244898,0.79274405230505)
--(axis cs:76.1904761904762,0.792395718104156)
--(axis cs:75.8503401360544,0.787062133783355)
--(axis cs:75.5102040816327,0.784908907022673)
--(axis cs:75.1700680272109,0.781016651280711)
--(axis cs:74.8299319727891,0.775653958156226)
--(axis cs:74.4897959183673,0.771799520743088)
--(axis cs:74.1496598639456,0.766544927291858)
--(axis cs:73.8095238095238,0.75589600233518)
--(axis cs:73.469387755102,0.752184073751817)
--(axis cs:73.1292517006803,0.750563785333476)
--(axis cs:72.7891156462585,0.745999780166075)
--(axis cs:72.4489795918367,0.741775105887976)
--(axis cs:72.108843537415,0.736415322465749)
--(axis cs:71.7687074829932,0.724448382038266)
--(axis cs:71.4285714285714,0.72426872971784)
--(axis cs:71.0884353741497,0.720563197023082)
--(axis cs:70.7482993197279,0.71473586084803)
--(axis cs:70.4081632653061,0.711953125)
--(axis cs:70.0680272108844,0.700003154175044)
--(axis cs:69.7278911564626,0.700176409291334)
--(axis cs:69.3877551020408,0.694405319246786)
--(axis cs:69.0476190476191,0.690476434932686)
--(axis cs:68.7074829931973,0.683534934567643)
--(axis cs:68.3673469387755,0.67511983459186)
--(axis cs:68.0272108843537,0.671109013358282)
--(axis cs:67.687074829932,0.670099823626048)
--(axis cs:67.3469387755102,0.659909359456544)
--(axis cs:67.0068027210884,0.65752182009012)
--(axis cs:66.6666666666667,0.652134067759422)
--(axis cs:66.3265306122449,0.650202558995894)
--(axis cs:65.9863945578231,0.645636331187431)
--(axis cs:65.6462585034014,0.637813670833745)
--(axis cs:65.3061224489796,0.63327338814837)
--(axis cs:64.9659863945578,0.630224221272397)
--(axis cs:64.6258503401361,0.625858269647819)
--(axis cs:64.2857142857143,0.620851081898758)
--(axis cs:63.9455782312925,0.620494426805214)
--(axis cs:63.6054421768707,0.613895323898197)
--(axis cs:63.265306122449,0.613105456527686)
--(axis cs:62.9251700680272,0.60989949771811)
--(axis cs:62.5850340136054,0.607880071395672)
--(axis cs:62.2448979591837,0.600995984296785)
--(axis cs:61.9047619047619,0.595528294996868)
--(axis cs:61.5646258503401,0.587416812747975)
--(axis cs:61.2244897959184,0.585905495451499)
--(axis cs:60.8843537414966,0.579824970838471)
--(axis cs:60.5442176870748,0.572112049814553)
--(axis cs:60.2040816326531,0.565929650745105)
--(axis cs:59.8639455782313,0.559081749004145)
--(axis cs:59.5238095238095,0.560500625183608)
--(axis cs:59.1836734693878,0.550003639932559)
--(axis cs:58.843537414966,0.538781185287912)
--(axis cs:58.5034013605442,0.539808367690501)
--(axis cs:58.1632653061224,0.52995327945996)
--(axis cs:57.8231292517007,0.526448498023958)
--(axis cs:57.4829931972789,0.520999450067232)
--(axis cs:57.1428571428571,0.517059234841245)
--(axis cs:56.8027210884354,0.515509337699491)
--(axis cs:56.4625850340136,0.507501740923321)
--(axis cs:56.1224489795918,0.503312406335766)
--(axis cs:55.7823129251701,0.48848066519184)
--(axis cs:55.4421768707483,0.490247346151922)
--(axis cs:55.1020408163265,0.481123936215026)
--(axis cs:54.7619047619048,0.472630708186053)
--(axis cs:54.421768707483,0.46752846147144)
--(axis cs:54.0816326530612,0.459797490380482)
--(axis cs:53.7414965986395,0.454305698751904)
--(axis cs:53.4013605442177,0.451859225949417)
--(axis cs:53.0612244897959,0.446355619826752)
--(axis cs:52.7210884353741,0.440035259647946)
--(axis cs:52.3809523809524,0.42782877939881)
--(axis cs:52.0408163265306,0.420062369822036)
--(axis cs:51.7006802721088,0.417212393025618)
--(axis cs:51.3605442176871,0.416639792426273)
--(axis cs:51.0204081632653,0.407819890417271)
--(axis cs:50.6802721088435,0.40888009118531)
--(axis cs:50.3401360544218,0.402815226394958)
--(axis cs:50,0.399960133389406)
--(axis cs:49.6598639455782,0.388886374635594)
--(axis cs:49.3197278911565,0.394932887315348)
--(axis cs:48.9795918367347,0.390243456847109)
--(axis cs:48.6394557823129,0.386914769970679)
--(axis cs:48.2993197278912,0.378947960587752)
--(axis cs:47.9591836734694,0.374432437727544)
--(axis cs:47.6190476190476,0.370352732913809)
--(axis cs:47.2789115646259,0.364412235733898)
--(axis cs:46.9387755102041,0.36124573893712)
--(axis cs:46.5986394557823,0.353931402901926)
--(axis cs:46.2585034013605,0.352728171966793)
--(axis cs:45.9183673469388,0.348153168247976)
--(axis cs:45.578231292517,0.343238573598544)
--(axis cs:45.2380952380952,0.343625822587952)
--(axis cs:44.8979591836735,0.341278828805499)
--(axis cs:44.5578231292517,0.341004307167147)
--(axis cs:44.2176870748299,0.336010998522189)
--(axis cs:43.8775510204082,0.32969163563747)
--(axis cs:43.5374149659864,0.329545234080184)
--(axis cs:43.1972789115646,0.325783497867445)
--(axis cs:42.8571428571429,0.323531798626765)
--(axis cs:42.5170068027211,0.31763625905306)
--(axis cs:42.1768707482993,0.312609569945264)
--(axis cs:41.8367346938776,0.309587217398479)
--(axis cs:41.4965986394558,0.308178595136481)
--(axis cs:41.156462585034,0.304503655111829)
--(axis cs:40.8163265306122,0.295272050675882)
--(axis cs:40.4761904761905,0.296789729571043)
--(axis cs:40.1360544217687,0.293438080712369)
--(axis cs:39.7959183673469,0.288370908491785)
--(axis cs:39.4557823129252,0.287585594644796)
--(axis cs:39.1156462585034,0.282921031986837)
--(axis cs:38.7755102040816,0.279656008405866)
--(axis cs:38.4353741496599,0.274094585435138)
--(axis cs:38.0952380952381,0.271264031785425)
--(axis cs:37.7551020408163,0.270987803032608)
--(axis cs:37.4149659863946,0.266393044176538)
--(axis cs:37.0748299319728,0.264729592899412)
--(axis cs:36.734693877551,0.259918730239631)
--(axis cs:36.3945578231292,0.259739301519317)
--(axis cs:36.0544217687075,0.25470942939233)
--(axis cs:35.7142857142857,0.248187780232757)
--(axis cs:35.3741496598639,0.251100971821636)
--(axis cs:35.0340136054422,0.245500197978265)
--(axis cs:34.6938775510204,0.24377601339929)
--(axis cs:34.3537414965986,0.238370287035986)
--(axis cs:34.0136054421769,0.239482341300317)
--(axis cs:33.6734693877551,0.239339584194793)
--(axis cs:33.3333333333333,0.234552863761673)
--(axis cs:32.9931972789116,0.232959943634365)
--(axis cs:32.6530612244898,0.231485065224547)
--(axis cs:32.312925170068,0.229828496170618)
--(axis cs:31.9727891156463,0.224588320593031)
--(axis cs:31.6326530612245,0.220456041674721)
--(axis cs:31.2925170068027,0.218581537945279)
--(axis cs:30.952380952381,0.219495013463251)
--(axis cs:30.6122448979592,0.219244807181083)
--(axis cs:30.2721088435374,0.215407704175928)
--(axis cs:29.9319727891156,0.21564584201311)
--(axis cs:29.5918367346939,0.211281161221311)
--(axis cs:29.2517006802721,0.212046411371699)
--(axis cs:28.9115646258503,0.207820722638227)
--(axis cs:28.5714285714286,0.208781439048152)
--(axis cs:28.2312925170068,0.208615274378014)
--(axis cs:27.891156462585,0.205234289336348)
--(axis cs:27.5510204081633,0.208092816720661)
--(axis cs:27.2108843537415,0.206211971149231)
--(axis cs:26.8707482993197,0.206340340429099)
--(axis cs:26.530612244898,0.20676333705346)
--(axis cs:26.1904761904762,0.207072219508346)
--(axis cs:25.8503401360544,0.208999272121695)
--(axis cs:25.5102040816327,0.206639520185932)
--(axis cs:25.1700680272109,0.20989604144144)
--(axis cs:24.8299319727891,0.205957442278737)
--(axis cs:24.4897959183673,0.202674209993825)
--(axis cs:24.1496598639456,0.198149392906451)
--(axis cs:23.8095238095238,0.199863488751856)
--(axis cs:23.469387755102,0.19813663103299)
--(axis cs:23.1292517006803,0.197981593949794)
--(axis cs:22.7891156462585,0.195663207659208)
--(axis cs:22.4489795918367,0.191593823870688)
--(axis cs:22.108843537415,0.188156127416282)
--(axis cs:21.7687074829932,0.189171774971613)
--(axis cs:21.4285714285714,0.187932027828561)
--(axis cs:21.0884353741497,0.187210451947229)
--(axis cs:20.7482993197279,0.184286101777512)
--(axis cs:20.4081632653061,0.183616371952815)
--(axis cs:20.0680272108844,0.176886309307505)
--(axis cs:19.7278911564626,0.17233588814837)
--(axis cs:19.3877551020408,0.171317602779094)
--(axis cs:19.047619047619,0.167458984244774)
--(axis cs:18.7074829931973,0.165460265008037)
--(axis cs:18.3673469387755,0.159193028701868)
--(axis cs:18.0272108843537,0.158287995116313)
--(axis cs:17.687074829932,0.160602602606504)
--(axis cs:17.3469387755102,0.14900844758261)
--(axis cs:17.0068027210884,0.148233074602127)
--(axis cs:16.6666666666667,0.145111192969321)
--(axis cs:16.3265306122449,0.142554811468741)
--(axis cs:15.9863945578231,0.140173937985953)
--(axis cs:15.6462585034014,0.138885973260722)
--(axis cs:15.3061224489796,0.135406749175901)
--(axis cs:14.9659863945578,0.130225980879404)
--(axis cs:14.6258503401361,0.131718368524452)
--(axis cs:14.2857142857143,0.129111699678704)
--(axis cs:13.9455782312925,0.123780540446945)
--(axis cs:13.6054421768707,0.123425147720898)
--(axis cs:13.265306122449,0.12175779689995)
--(axis cs:12.9251700680272,0.120081668458369)
--(axis cs:12.5850340136054,0.120948176592758)
--(axis cs:12.2448979591837,0.116215986985213)
--(axis cs:11.9047619047619,0.11490867431953)
--(axis cs:11.5646258503401,0.111361806874112)
--(axis cs:11.2244897959184,0.109137085242005)
--(axis cs:10.8843537414966,0.106321266149252)
--(axis cs:10.5442176870748,0.104945726477331)
--(axis cs:10.2040816326531,0.105936981607441)
--(axis cs:9.86394557823129,0.103391814834223)
--(axis cs:9.52380952380952,0.106742326544004)
--(axis cs:9.18367346938775,0.0980613326832779)
--(axis cs:8.84353741496599,0.102400010000937)
--(axis cs:8.50340136054422,0.0978754008500689)
--(axis cs:8.16326530612245,0.0974808600205857)
--(axis cs:7.82312925170068,0.0912842631450424)
--(axis cs:7.48299319727891,0.0954102225698428)
--(axis cs:7.14285714285714,0.0929151998342824)
--(axis cs:6.80272108843537,0.0897293649067253)
--(axis cs:6.46258503401361,0.0885137715092209)
--(axis cs:6.12244897959184,0.0846381412259673)
--(axis cs:5.78231292517007,0.0886535219871316)
--(axis cs:5.4421768707483,0.0864496623905319)
--(axis cs:5.10204081632653,0.0868614153540896)
--(axis cs:4.76190476190476,0.0841616615836504)
--(axis cs:4.42176870748299,0.0828640105587721)
--(axis cs:4.08163265306122,0.0845683193077468)
--(axis cs:3.74149659863946,0.0844531044839584)
--(axis cs:3.40136054421769,0.0818455711561306)
--(axis cs:3.06122448979592,0.0812868920931265)
--(axis cs:2.72108843537415,0.084078746426836)
--(axis cs:2.38095238095238,0.0806154097696841)
--(axis cs:2.04081632653061,0.0760459184299931)
--(axis cs:1.70068027210884,0.0780131148452017)
--(axis cs:1.36054421768707,0.0811751788240392)
--(axis cs:1.02040816326531,0.0800730208618343)
--(axis cs:0.680272108843537,0.0803237830168084)
--(axis cs:0.340136054421769,0.0819404774605563)
--(axis cs:0,0.0840707071041821)
--cycle;


==> img/stl10/stl10_rate_accuracy_shap.tex <==
% shap
\addplot [line width=0.5, opacity=0.8, color2, mark=diamond*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color2, thin}]
table [row sep=\\]{%
0	0.0765625 \\
0.340136054421769	0.07453125 \\
0.680272108843537	0.07203125 \\
1.02040816326531	0.07203125 \\
1.36054421768707	0.07328125 \\
1.70068027210884	0.07 \\
2.04081632653061	0.0721875 \\
2.38095238095238	0.0703125 \\
2.72108843537415	0.0728125 \\
3.06122448979592	0.07046875 \\
3.40136054421769	0.07734375 \\
3.74149659863946	0.0759375 \\
4.08163265306122	0.07328125 \\
4.42176870748299	0.07421875 \\
4.76190476190476	0.0790625 \\
5.10204081632653	0.075625 \\
5.4421768707483	0.07421875 \\
5.78231292517007	0.07828125 \\
6.12244897959184	0.07890625 \\
6.46258503401361	0.08359375 \\
6.80272108843537	0.08171875 \\
7.14285714285714	0.08078125 \\
7.48299319727891	0.0884375 \\
7.82312925170068	0.08796875 \\
8.16326530612245	0.09296875 \\
8.50340136054422	0.09546875 \\
8.84353741496599	0.0946875 \\
9.18367346938775	0.10015625 \\
9.52380952380952	0.09625 \\
9.86394557823129	0.10328125 \\
10.2040816326531	0.1075 \\
10.5442176870748	0.10546875 \\
10.8843537414966	0.1109375 \\
11.2244897959184	0.1096875 \\
11.5646258503401	0.10890625 \\
11.9047619047619	0.1096875 \\
12.2448979591837	0.11265625 \\
12.5850340136054	0.1165625 \\
12.9251700680272	0.1159375 \\
13.265306122449	0.11390625 \\
13.6054421768707	0.10890625 \\
13.9455782312925	0.10921875 \\
14.2857142857143	0.116875 \\
14.6258503401361	0.114375 \\
14.9659863945578	0.1184375 \\
15.3061224489796	0.11078125 \\
15.6462585034014	0.11453125 \\
15.9863945578231	0.116875 \\
16.3265306122449	0.1165625 \\
16.6666666666667	0.1221875 \\
17.0068027210884	0.123125 \\
17.3469387755102	0.11953125 \\
17.687074829932	0.1178125 \\
18.0272108843537	0.11984375 \\
18.3673469387755	0.123125 \\
18.7074829931973	0.12171875 \\
19.047619047619	0.1234375 \\
19.3877551020408	0.124375 \\
19.7278911564626	0.12078125 \\
20.0680272108844	0.12421875 \\
20.4081632653061	0.12515625 \\
20.7482993197279	0.12296875 \\
21.0884353741497	0.12203125 \\
21.4285714285714	0.1184375 \\
21.7687074829932	0.12296875 \\
22.108843537415	0.1259375 \\
22.4489795918367	0.12328125 \\
22.7891156462585	0.12234375 \\
23.1292517006803	0.1265625 \\
23.469387755102	0.12625 \\
23.8095238095238	0.13109375 \\
24.1496598639456	0.13046875 \\
24.4897959183673	0.12921875 \\
24.8299319727891	0.133125 \\
25.1700680272109	0.13078125 \\
25.5102040816327	0.1378125 \\
25.8503401360544	0.1321875 \\
26.1904761904762	0.14109375 \\
26.530612244898	0.14 \\
26.8707482993197	0.14046875 \\
27.2108843537415	0.143125 \\
27.5510204081633	0.14140625 \\
27.891156462585	0.14375 \\
28.2312925170068	0.14671875 \\
28.5714285714286	0.1475 \\
28.9115646258503	0.14703125 \\
29.2517006802721	0.14828125 \\
29.5918367346939	0.14984375 \\
29.9319727891156	0.151875 \\
30.2721088435374	0.15515625 \\
30.6122448979592	0.1553125 \\
30.952380952381	0.16015625 \\
31.2925170068027	0.16078125 \\
31.6326530612245	0.16390625 \\
31.9727891156463	0.1659375 \\
32.312925170068	0.1684375 \\
32.6530612244898	0.1690625 \\
32.9931972789116	0.17171875 \\
33.3333333333333	0.17109375 \\
33.6734693877551	0.1753125 \\
34.0136054421769	0.1771875 \\
34.3537414965986	0.17375 \\
34.6938775510204	0.17390625 \\
35.0340136054422	0.1771875 \\
35.3741496598639	0.17875 \\
35.7142857142857	0.18109375 \\
36.0544217687075	0.1809375 \\
36.3945578231292	0.18296875 \\
36.734693877551	0.18828125 \\
37.0748299319728	0.18421875 \\
37.4149659863946	0.1821875 \\
37.7551020408163	0.18578125 \\
38.0952380952381	0.19015625 \\
38.4353741496599	0.1896875 \\
38.7755102040816	0.189375 \\
39.1156462585034	0.19 \\
39.4557823129252	0.195625 \\
39.7959183673469	0.19140625 \\
40.1360544217687	0.19875 \\
40.4761904761905	0.1975 \\
40.8163265306122	0.19890625 \\
41.156462585034	0.20015625 \\
41.4965986394558	0.20203125 \\
41.8367346938776	0.2040625 \\
42.1768707482993	0.20578125 \\
42.5170068027211	0.2071875 \\
42.8571428571429	0.20359375 \\
43.1972789115646	0.20609375 \\
43.5374149659864	0.2071875 \\
43.8775510204082	0.20671875 \\
44.2176870748299	0.21390625 \\
44.5578231292517	0.20734375 \\
44.8979591836735	0.20953125 \\
45.2380952380952	0.21328125 \\
45.578231292517	0.216875 \\
45.9183673469388	0.21578125 \\
46.2585034013605	0.216875 \\
46.5986394557823	0.21703125 \\
46.9387755102041	0.22 \\
47.2789115646259	0.22171875 \\
47.6190476190476	0.21625 \\
47.9591836734694	0.21828125 \\
48.2993197278912	0.2159375 \\
48.6394557823129	0.22328125 \\
48.9795918367347	0.22140625 \\
49.3197278911565	0.22171875 \\
49.6598639455782	0.2253125 \\
50	0.22359375 \\
50.3401360544218	0.2234375 \\
50.6802721088435	0.22546875 \\
51.0204081632653	0.23234375 \\
51.3605442176871	0.2271875 \\
51.7006802721088	0.2290625 \\
52.0408163265306	0.23078125 \\
52.3809523809524	0.23359375 \\
52.7210884353741	0.236875 \\
53.0612244897959	0.2315625 \\
53.4013605442177	0.23875 \\
53.7414965986395	0.23625 \\
54.0816326530612	0.24 \\
54.421768707483	0.2409375 \\
54.7619047619048	0.24296875 \\
55.1020408163265	0.24390625 \\
55.4421768707483	0.2478125 \\
55.7823129251701	0.24609375 \\
56.1224489795918	0.250625 \\
56.4625850340136	0.25359375 \\
56.8027210884354	0.255625 \\
57.1428571428571	0.25625 \\
57.4829931972789	0.25765625 \\
57.8231292517007	0.25671875 \\
58.1632653061224	0.2596875 \\
58.5034013605442	0.2671875 \\
58.843537414966	0.26203125 \\
59.1836734693878	0.26734375 \\
59.5238095238095	0.27171875 \\
59.8639455782313	0.269375 \\
60.2040816326531	0.26734375 \\
60.5442176870748	0.2759375 \\
60.8843537414966	0.27453125 \\
61.2244897959184	0.27890625 \\
61.5646258503401	0.28421875 \\
61.9047619047619	0.28609375 \\
62.2448979591837	0.28609375 \\
62.5850340136054	0.288125 \\
62.9251700680272	0.29109375 \\
63.265306122449	0.29609375 \\
63.6054421768707	0.2940625 \\
63.9455782312925	0.29609375 \\
64.2857142857143	0.2984375 \\
64.6258503401361	0.304375 \\
64.9659863945578	0.30375 \\
65.3061224489796	0.303125 \\
65.6462585034014	0.31203125 \\
65.9863945578231	0.308125 \\
66.3265306122449	0.31140625 \\
66.6666666666667	0.31265625 \\
67.0068027210884	0.31390625 \\
67.3469387755102	0.31203125 \\
67.687074829932	0.31359375 \\
68.0272108843537	0.3203125 \\
68.3673469387755	0.31875 \\
68.7074829931973	0.32046875 \\
69.0476190476191	0.32265625 \\
69.3877551020408	0.32515625 \\
69.7278911564626	0.33171875 \\
70.0680272108844	0.3340625 \\
70.4081632653061	0.33234375 \\
70.7482993197279	0.3325 \\
71.0884353741497	0.3321875 \\
71.4285714285714	0.3346875 \\
71.7687074829932	0.34265625 \\
72.108843537415	0.34421875 \\
72.4489795918367	0.34671875 \\
72.7891156462585	0.35046875 \\
73.1292517006803	0.35109375 \\
73.469387755102	0.35 \\
73.8095238095238	0.35125 \\
74.1496598639456	0.3578125 \\
74.4897959183673	0.35921875 \\
74.8299319727891	0.3590625 \\
75.1700680272109	0.3596875 \\
75.5102040816327	0.36375 \\
75.8503401360544	0.36578125 \\
76.1904761904762	0.36859375 \\
76.530612244898	0.36734375 \\
76.8707482993197	0.37375 \\
77.2108843537415	0.3778125 \\
77.5510204081633	0.36984375 \\
77.891156462585	0.3784375 \\
78.2312925170068	0.37953125 \\
78.5714285714286	0.383125 \\
78.9115646258503	0.38453125 \\
79.2517006802721	0.3846875 \\
79.5918367346939	0.3909375 \\
79.9319727891156	0.3884375 \\
80.2721088435374	0.39359375 \\
80.6122448979592	0.39515625 \\
80.9523809523809	0.39984375 \\
81.2925170068027	0.40203125 \\
81.6326530612245	0.40640625 \\
81.9727891156463	0.4046875 \\
82.312925170068	0.40546875 \\
82.6530612244898	0.4025 \\
82.9931972789116	0.409375 \\
83.3333333333333	0.40984375 \\
83.6734693877551	0.40890625 \\
84.0136054421769	0.416875 \\
84.3537414965986	0.416875 \\
84.6938775510204	0.42140625 \\
85.0340136054422	0.425 \\
85.3741496598639	0.42671875 \\
85.7142857142857	0.43171875 \\
86.0544217687075	0.4434375 \\
86.3945578231292	0.43953125 \\
86.734693877551	0.4475 \\
87.0748299319728	0.4571875 \\
87.4149659863945	0.46390625 \\
87.7551020408163	0.468125 \\
88.0952380952381	0.47578125 \\
88.4353741496599	0.488125 \\
88.7755102040816	0.50421875 \\
89.1156462585034	0.51578125 \\
89.4557823129252	0.53015625 \\
89.7959183673469	0.55921875 \\
90.1360544217687	0.57359375 \\
90.4761904761905	0.5978125 \\
90.8163265306122	0.62671875 \\
91.156462585034	0.64109375 \\
91.4965986394558	0.6553125 \\
91.8367346938775	0.665625 \\
92.1768707482993	0.6834375 \\
92.5170068027211	0.6915625 \\
92.8571428571429	0.71359375 \\
93.1972789115646	0.7265625 \\
93.5374149659864	0.73984375 \\
93.8775510204082	0.74890625 \\
94.2176870748299	0.75171875 \\
94.5578231292517	0.7525 \\
94.8979591836735	0.76078125 \\
95.2380952380952	0.76546875 \\
95.578231292517	0.77859375 \\
95.9183673469388	0.799375 \\
96.2585034013605	0.81234375 \\
96.5986394557823	0.8340625 \\
96.9387755102041	0.84921875 \\
97.2789115646258	0.87 \\
97.6190476190476	0.875 \\
97.9591836734694	0.89046875 \\
98.2993197278912	0.9103125 \\
98.6394557823129	0.9275 \\
98.9795918367347	0.95078125 \\
99.3197278911565	0.96625 \\
99.6598639455782	0.9934375 \\
100	1 \\
};
\path [fill=color2, fill opacity=0.5] (axis cs:0,0.083714778681094)
--(axis cs:0,0.069410221318906)
--(axis cs:0.340136054421769,0.0672987513823103)
--(axis cs:0.680272108843537,0.0643040545870319)
--(axis cs:1.02040816326531,0.0636926413385278)
--(axis cs:1.36054421768707,0.0659284412171558)
--(axis cs:1.70068027210884,0.0608421553089842)
--(axis cs:2.04081632653061,0.0637437631557745)
--(axis cs:2.38095238095238,0.0609354657155017)
--(axis cs:2.72108843537415,0.0626412370575847)
--(axis cs:3.06122448979592,0.0599277540980706)
--(axis cs:3.40136054421769,0.0658846306347967)
--(axis cs:3.74149659863946,0.0640611187583724)
--(axis cs:4.08163265306122,0.0608796752206893)
--(axis cs:4.42176870748299,0.0611477609867623)
--(axis cs:4.76190476190476,0.0648993133630567)
--(axis cs:5.10204081632653,0.060647574563528)
--(axis cs:5.4421768707483,0.0591287262581923)
--(axis cs:5.78231292517007,0.0627281316516929)
--(axis cs:6.12244897959184,0.0625842121282119)
--(axis cs:6.46258503401361,0.066916246758211)
--(axis cs:6.80272108843537,0.0648796293431168)
--(axis cs:7.14285714285714,0.0637820484124472)
--(axis cs:7.48299319727891,0.0706201178565617)
--(axis cs:7.82312925170068,0.0701072643656138)
--(axis cs:8.16326530612245,0.0751195489287521)
--(axis cs:8.50340136054422,0.077630238034164)
--(axis cs:8.84353741496599,0.0771958507298639)
--(axis cs:9.18367346938775,0.0825420833902383)
--(axis cs:9.52380952380952,0.0787719864678148)
--(axis cs:9.86394557823129,0.0859911288910006)
--(axis cs:10.2040816326531,0.091257913021896)
--(axis cs:10.5442176870748,0.0892751763739523)
--(axis cs:10.8843537414966,0.0946572921998635)
--(axis cs:11.2244897959184,0.093658780124731)
--(axis cs:11.5646258503401,0.0934478486123431)
--(axis cs:11.9047619047619,0.0952508804127344)
--(axis cs:12.2448979591837,0.0975997589827367)
--(axis cs:12.5850340136054,0.10166423968544)
--(axis cs:12.9251700680272,0.101343852466232)
--(axis cs:13.265306122449,0.0987305190235711)
--(axis cs:13.6054421768707,0.0937160722243947)
--(axis cs:13.9455782312925,0.0947547417453688)
--(axis cs:14.2857142857143,0.101527736964982)
--(axis cs:14.6258503401361,0.0995982185004861)
--(axis cs:14.9659863945578,0.103743560254841)
--(axis cs:15.3061224489796,0.0961019205946085)
--(axis cs:15.6462585034014,0.100536390430846)
--(axis cs:15.9863945578231,0.102260455877711)
--(axis cs:16.3265306122449,0.101306230676797)
--(axis cs:16.6666666666667,0.107500051944906)
--(axis cs:17.0068027210884,0.108552279019437)
--(axis cs:17.3469387755102,0.104924212148007)
--(axis cs:17.687074829932,0.103517279381922)
--(axis cs:18.0272108843537,0.105726087467352)
--(axis cs:18.3673469387755,0.10872807060767)
--(axis cs:18.7074829931973,0.107674912014037)
--(axis cs:19.047619047619,0.109466170103314)
--(axis cs:19.3877551020408,0.110885705742319)
--(axis cs:19.7278911564626,0.10724079626576)
--(axis cs:20.0680272108844,0.110517957479192)
--(axis cs:20.4081632653061,0.110767603178682)
--(axis cs:20.7482993197279,0.109246396201383)
--(axis cs:21.0884353741497,0.108445794893376)
--(axis cs:21.4285714285714,0.105222476699971)
--(axis cs:21.7687074829932,0.109750479632483)
--(axis cs:22.108843537415,0.111746060956032)
--(axis cs:22.4489795918367,0.109474369139123)
--(axis cs:22.7891156462585,0.108249750448267)
--(axis cs:23.1292517006803,0.112372405033228)
--(axis cs:23.469387755102,0.11267542997307)
--(axis cs:23.8095238095238,0.117057383767019)
--(axis cs:24.1496598639456,0.116147202065873)
--(axis cs:24.4897959183673,0.115613653599339)
--(axis cs:24.8299319727891,0.118296034295105)
--(axis cs:25.1700680272109,0.116687927117233)
--(axis cs:25.5102040816327,0.123255493676395)
--(axis cs:25.8503401360544,0.11753255352945)
--(axis cs:26.1904761904762,0.126098188421138)
--(axis cs:26.530612244898,0.124492630280251)
--(axis cs:26.8707482993197,0.125379358261365)
--(axis cs:27.2108843537415,0.127697785008228)
--(axis cs:27.5510204081633,0.125966367588787)
--(axis cs:27.891156462585,0.128049498819952)
--(axis cs:28.2312925170068,0.131286281401745)
--(axis cs:28.5714285714286,0.131633338535)
--(axis cs:28.9115646258503,0.130726750139586)
--(axis cs:29.2517006802721,0.13218810443717)
--(axis cs:29.5918367346939,0.134212342622337)
--(axis cs:29.9319727891156,0.136334456769896)
--(axis cs:30.2721088435374,0.139417831076862)
--(axis cs:30.6122448979592,0.139238625364406)
--(axis cs:30.952380952381,0.144320573143641)
--(axis cs:31.2925170068027,0.145190773002087)
--(axis cs:31.6326530612245,0.148736175863992)
--(axis cs:31.9727891156463,0.150310669052588)
--(axis cs:32.312925170068,0.152860792402434)
--(axis cs:32.6530612244898,0.153524411638126)
--(axis cs:32.9931972789116,0.156614828879061)
--(axis cs:33.3333333333333,0.155970267884306)
--(axis cs:33.6734693877551,0.160150286088012)
--(axis cs:34.0136054421769,0.161931230676797)
--(axis cs:34.3537414965986,0.15914590043443)
--(axis cs:34.6938775510204,0.15893169017286)
--(axis cs:35.0340136054422,0.162799184580693)
--(axis cs:35.3741496598639,0.163735053832982)
--(axis cs:35.7142857142857,0.165830293682544)
--(axis cs:36.0544217687075,0.166662975333891)
--(axis cs:36.3945578231292,0.168194227527777)
--(axis cs:36.734693877551,0.17327615188768)
--(axis cs:37.0748299319728,0.169842038463813)
--(axis cs:37.4149659863946,0.167194800564043)
--(axis cs:37.7551020408163,0.171187275726931)
--(axis cs:38.0952380952381,0.175122578583971)
--(axis cs:38.4353741496599,0.174614233295645)
--(axis cs:38.7755102040816,0.173944694434847)
--(axis cs:39.1156462585034,0.174774391544768)
--(axis cs:39.4557823129252,0.180456497582946)
--(axis cs:39.7959183673469,0.176444432854678)
--(axis cs:40.1360544217687,0.183865188372455)
--(axis cs:40.4761904761905,0.182769112248236)
--(axis cs:40.8163265306122,0.18397889242981)
--(axis cs:41.156462585034,0.185198257776039)
--(axis cs:41.4965986394558,0.187386393666918)
--(axis cs:41.8367346938776,0.188803730468763)
--(axis cs:42.1768707482993,0.190573503340101)
--(axis cs:42.5170068027211,0.192185262211194)
--(axis cs:42.8571428571429,0.188870309204374)
--(axis cs:43.1972789115646,0.19092556194628)
--(axis cs:43.5374149659864,0.191912489091593)
--(axis cs:43.8775510204082,0.191723188421138)
--(axis cs:44.2176870748299,0.198373379521315)
--(axis cs:44.5578231292517,0.192852075796658)
--(axis cs:44.8979591836735,0.194412182670981)
--(axis cs:45.2380952380952,0.197972873542305)
--(axis cs:45.578231292517,0.201254883575678)
--(axis cs:45.9183673469388,0.200599864290985)
--(axis cs:46.2585034013605,0.201834035225828)
--(axis cs:46.5986394557823,0.201833540215614)
--(axis cs:46.9387755102041,0.204562897351394)
--(axis cs:47.2789115646259,0.206350063720935)
--(axis cs:47.6190476190476,0.201050094082772)
--(axis cs:47.9591836734694,0.203094211663878)
--(axis cs:48.2993197278912,0.201068714574509)
--(axis cs:48.6394557823129,0.207607802160961)
--(axis cs:48.9795918367347,0.205822503188888)
--(axis cs:49.3197278911565,0.206276397108767)
--(axis cs:49.6598639455782,0.209423615047334)
--(axis cs:50,0.20794892614974)
--(axis cs:50.3401360544218,0.208067882952922)
--(axis cs:50.6802721088435,0.209842224195592)
--(axis cs:51.0204081632653,0.216644767434596)
--(axis cs:51.3605442176871,0.211448172173511)
--(axis cs:51.7006802721088,0.213260282338931)
--(axis cs:52.0408163265306,0.214544154669538)
--(axis cs:52.3809523809524,0.217225618594491)
--(axis cs:52.7210884353741,0.220480379866068)
--(axis cs:53.0612244897959,0.2157156857777)
--(axis cs:53.4013605442177,0.222292096751235)
--(axis cs:53.7414965986395,0.220134647386925)
--(axis cs:54.0816326530612,0.223629246920301)
--(axis cs:54.421768707483,0.224576070337063)
--(axis cs:54.7619047619048,0.22655000708166)
--(axis cs:55.1020408163265,0.227644504976901)
--(axis cs:55.4421768707483,0.230839967365956)
--(axis cs:55.7823129251701,0.229513168128714)
--(axis cs:56.1224489795918,0.234025735453157)
--(axis cs:56.4625850340136,0.236324601338778)
--(axis cs:56.8027210884354,0.238397596038125)
--(axis cs:57.1428571428571,0.239397575503039)
--(axis cs:57.4829931972789,0.240422481046042)
--(axis cs:57.8231292517007,0.239375208950442)
--(axis cs:58.1632653061224,0.242231872136993)
--(axis cs:58.5034013605442,0.249945708970349)
--(axis cs:58.843537414966,0.244673967571696)
--(axis cs:59.1836734693878,0.250159857001355)
--(axis cs:59.5238095238095,0.254555403601505)
--(axis cs:59.8639455782313,0.252127125746639)
--(axis cs:60.2040816326531,0.249766981389137)
--(axis cs:60.5442176870748,0.258386522699598)
--(axis cs:60.8843537414966,0.25734069851307)
--(axis cs:61.2244897959184,0.261729018070701)
--(axis cs:61.5646258503401,0.267272928290414)
--(axis cs:61.9047619047619,0.269577713407594)
--(axis cs:62.2448979591837,0.26889543353491)
--(axis cs:62.5850340136054,0.271514248866392)
--(axis cs:62.9251700680272,0.274436845459478)
--(axis cs:63.265306122449,0.280261686944888)
--(axis cs:63.6054421768707,0.278518275194475)
--(axis cs:63.9455782312925,0.280381408663074)
--(axis cs:64.2857142857143,0.282849164109973)
--(axis cs:64.6258503401361,0.288818509568953)
--(axis cs:64.9659863945578,0.288975800274158)
--(axis cs:65.3061224489796,0.286941735781324)
--(axis cs:65.6462585034014,0.296742197979213)
--(axis cs:65.9863945578231,0.293240829089225)
--(axis cs:66.3265306122449,0.296595624438715)
--(axis cs:66.6666666666667,0.29750819476936)
--(axis cs:67.0068027210884,0.299073104630993)
--(axis cs:67.3469387755102,0.29743466207582)
--(axis cs:67.687074829932,0.298397922867809)
--(axis cs:68.0272108843537,0.305257592559663)
--(axis cs:68.3673469387755,0.303508114831932)
--(axis cs:68.7074829931973,0.305919279631196)
--(axis cs:69.0476190476191,0.307708462351294)
--(axis cs:69.3877551020408,0.309594549605601)
--(axis cs:69.7278911564626,0.316797782566049)
--(axis cs:70.0680272108844,0.318744470465866)
--(axis cs:70.4081632653061,0.317324675925358)
--(axis cs:70.7482993197279,0.317314531627012)
--(axis cs:71.0884353741497,0.317279001209658)
--(axis cs:71.4285714285714,0.319488221516919)
--(axis cs:71.7687074829932,0.327811536318289)
--(axis cs:72.108843537415,0.329099051908248)
--(axis cs:72.4489795918367,0.332258698344765)
--(axis cs:72.7891156462585,0.335695518555608)
--(axis cs:73.1292517006803,0.336501736272484)
--(axis cs:73.469387755102,0.33595718065535)
--(axis cs:73.8095238095238,0.337712011592302)
--(axis cs:74.1496598639456,0.34413574305912)
--(axis cs:74.4897959183673,0.345393921981143)
--(axis cs:74.8299319727891,0.34507138888667)
--(axis cs:75.1700680272109,0.34550950746184)
--(axis cs:75.5102040816327,0.349873875019213)
--(axis cs:75.8503401360544,0.351711631033715)
--(axis cs:76.1904761904762,0.355003381908649)
--(axis cs:76.530612244898,0.353738653599339)
--(axis cs:76.8707482993197,0.359962127131699)
--(axis cs:77.2108843537415,0.364148300145416)
--(axis cs:77.5510204081633,0.355705836434852)
--(axis cs:77.891156462585,0.364896694112895)
--(axis cs:78.2312925170068,0.365475194076311)
--(axis cs:78.5714285714286,0.369271573729449)
--(axis cs:78.9115646258503,0.370520725936072)
--(axis cs:79.2517006802721,0.371240691814017)
--(axis cs:79.5918367346939,0.377040772001213)
--(axis cs:79.9319727891156,0.374717578842345)
--(axis cs:80.2721088435374,0.380792583733285)
--(axis cs:80.6122448979592,0.382110091360422)
--(axis cs:80.9523809523809,0.387140552328583)
--(axis cs:81.2925170068027,0.389533920573364)
--(axis cs:81.6326530612245,0.394191408748401)
--(axis cs:81.9727891156463,0.392568678080087)
--(axis cs:82.312925170068,0.393132712926898)
--(axis cs:82.6530612244898,0.390661419952585)
--(axis cs:82.9931972789116,0.396960743295257)
--(axis cs:83.3333333333333,0.397361691953697)
--(axis cs:83.6734693877551,0.396574852279102)
--(axis cs:84.0136054421769,0.403468678294554)
--(axis cs:84.3537414965986,0.40346938967508)
--(axis cs:84.6938775510204,0.408033760662957)
--(axis cs:85.0340136054422,0.411090239207215)
--(axis cs:85.3741496598639,0.412411859403848)
--(axis cs:85.7142857142857,0.417101269690767)
--(axis cs:86.0544217687075,0.428534119568332)
--(axis cs:86.3945578231292,0.424872724827613)
--(axis cs:86.734693877551,0.432422937618402)
--(axis cs:87.0748299319728,0.441634075068506)
--(axis cs:87.4149659863945,0.448431200481734)
--(axis cs:87.7551020408163,0.452028595485909)
--(axis cs:88.0952380952381,0.459846514773359)
--(axis cs:88.4353741496599,0.470988067106564)
--(axis cs:88.7755102040816,0.486471892729115)
--(axis cs:89.1156462585034,0.497922968219565)
--(axis cs:89.4557823129252,0.511905501289571)
--(axis cs:89.7959183673469,0.540788089274981)
--(axis cs:90.1360544217687,0.554422009904585)
--(axis cs:90.4761904761905,0.578800355475925)
--(axis cs:90.8163265306122,0.608200333560236)
--(axis cs:91.156462585034,0.623796459943863)
--(axis cs:91.4965986394558,0.639173493546786)
--(axis cs:91.8367346938775,0.64977457533963)
--(axis cs:92.1768707482993,0.668079676849124)
--(axis cs:92.5170068027211,0.675552235081402)
--(axis cs:92.8571428571429,0.698208318511894)
--(axis cs:93.1972789115646,0.711467737077854)
--(axis cs:93.5374149659864,0.726273044519399)
--(axis cs:93.8775510204082,0.737161081211593)
--(axis cs:94.2176870748299,0.740325567336404)
--(axis cs:94.5578231292517,0.74157558679127)
--(axis cs:94.8979591836735,0.748003199299212)
--(axis cs:95.2380952380952,0.752040039098009)
--(axis cs:95.578231292517,0.764008273327613)
--(axis cs:95.9183673469388,0.784703793736952)
--(axis cs:96.2585034013605,0.79802153617965)
--(axis cs:96.5986394557823,0.820026473486659)
--(axis cs:96.9387755102041,0.836858770681849)
--(axis cs:97.2789115646258,0.861103092207867)
--(axis cs:97.6190476190476,0.865314784165455)
--(axis cs:97.9591836734694,0.878517524022379)
--(axis cs:98.2993197278912,0.897437420595284)
--(axis cs:98.6394557823129,0.914024145172566)
--(axis cs:98.9795918367347,0.940503190648726)
--(axis cs:99.3197278911565,0.956297682958127)
--(axis cs:99.6598639455782,0.986795439033933)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,1.00007956096607)
--(axis cs:99.3197278911565,0.976202317041873)
--(axis cs:98.9795918367347,0.961059309351274)
--(axis cs:98.6394557823129,0.940975854827434)
--(axis cs:98.2993197278912,0.923187579404716)
--(axis cs:97.9591836734694,0.902419975977621)
--(axis cs:97.6190476190476,0.884685215834545)
--(axis cs:97.2789115646258,0.878896907792133)
--(axis cs:96.9387755102041,0.861578729318151)
--(axis cs:96.5986394557823,0.848098526513341)
--(axis cs:96.2585034013605,0.82666596382035)
--(axis cs:95.9183673469388,0.814046206263048)
--(axis cs:95.578231292517,0.793179226672387)
--(axis cs:95.2380952380952,0.778897460901991)
--(axis cs:94.8979591836735,0.773559300700788)
--(axis cs:94.5578231292517,0.76342441320873)
--(axis cs:94.2176870748299,0.763111932663596)
--(axis cs:93.8775510204082,0.760651418788407)
--(axis cs:93.5374149659864,0.753414455480601)
--(axis cs:93.1972789115646,0.741657262922146)
--(axis cs:92.8571428571429,0.728979181488106)
--(axis cs:92.5170068027211,0.707572764918597)
--(axis cs:92.1768707482993,0.698795323150876)
--(axis cs:91.8367346938775,0.68147542466037)
--(axis cs:91.4965986394558,0.671451506453214)
--(axis cs:91.156462585034,0.658391040056137)
--(axis cs:90.8163265306122,0.645237166439764)
--(axis cs:90.4761904761905,0.616824644524074)
--(axis cs:90.1360544217687,0.592765490095415)
--(axis cs:89.7959183673469,0.577649410725019)
--(axis cs:89.4557823129252,0.548406998710429)
--(axis cs:89.1156462585034,0.533639531780435)
--(axis cs:88.7755102040816,0.521965607270885)
--(axis cs:88.4353741496599,0.505261932893436)
--(axis cs:88.0952380952381,0.491715985226641)
--(axis cs:87.7551020408163,0.484221404514091)
--(axis cs:87.4149659863945,0.479381299518266)
--(axis cs:87.0748299319728,0.472740924931494)
--(axis cs:86.734693877551,0.462577062381598)
--(axis cs:86.3945578231292,0.454189775172387)
--(axis cs:86.0544217687075,0.458340880431668)
--(axis cs:85.7142857142857,0.446336230309233)
--(axis cs:85.3741496598639,0.441025640596152)
--(axis cs:85.0340136054422,0.438909760792785)
--(axis cs:84.6938775510204,0.434778739337043)
--(axis cs:84.3537414965986,0.43028061032492)
--(axis cs:84.0136054421769,0.430281321705446)
--(axis cs:83.6734693877551,0.421237647720898)
--(axis cs:83.3333333333333,0.422325808046303)
--(axis cs:82.9931972789116,0.421789256704743)
--(axis cs:82.6530612244898,0.414338580047415)
--(axis cs:82.312925170068,0.417804787073102)
--(axis cs:81.9727891156463,0.416806321919913)
--(axis cs:81.6326530612245,0.418621091251599)
--(axis cs:81.2925170068027,0.414528579426636)
--(axis cs:80.9523809523809,0.412546947671417)
--(axis cs:80.6122448979592,0.408202408639578)
--(axis cs:80.2721088435374,0.406394916266715)
--(axis cs:79.9319727891156,0.402157421157655)
--(axis cs:79.5918367346939,0.404834227998787)
--(axis cs:79.2517006802721,0.398134308185983)
--(axis cs:78.9115646258503,0.398541774063928)
--(axis cs:78.5714285714286,0.396978426270551)
--(axis cs:78.2312925170068,0.393587305923689)
--(axis cs:77.891156462585,0.391978305887105)
--(axis cs:77.5510204081633,0.383981663565148)
--(axis cs:77.2108843537415,0.391476699854584)
--(axis cs:76.8707482993197,0.387537872868301)
--(axis cs:76.530612244898,0.380948846400661)
--(axis cs:76.1904761904762,0.38218411809135)
--(axis cs:75.8503401360544,0.379850868966285)
--(axis cs:75.5102040816327,0.377626124980787)
--(axis cs:75.1700680272109,0.37386549253816)
--(axis cs:74.8299319727891,0.37305361111333)
--(axis cs:74.4897959183673,0.373043578018857)
--(axis cs:74.1496598639456,0.37148925694088)
--(axis cs:73.8095238095238,0.364787988407698)
--(axis cs:73.469387755102,0.36404281934465)
--(axis cs:73.1292517006803,0.365685763727516)
--(axis cs:72.7891156462585,0.365241981444392)
--(axis cs:72.4489795918367,0.361178801655235)
--(axis cs:72.108843537415,0.359338448091752)
--(axis cs:71.7687074829932,0.357500963681711)
--(axis cs:71.4285714285714,0.349886778483081)
--(axis cs:71.0884353741497,0.347095998790342)
--(axis cs:70.7482993197279,0.347685468372988)
--(axis cs:70.4081632653061,0.347362824074642)
--(axis cs:70.0680272108844,0.349380529534134)
--(axis cs:69.7278911564626,0.346639717433951)
--(axis cs:69.3877551020408,0.340717950394399)
--(axis cs:69.0476190476191,0.337604037648706)
--(axis cs:68.7074829931973,0.335018220368804)
--(axis cs:68.3673469387755,0.333991885168068)
--(axis cs:68.0272108843537,0.335367407440337)
--(axis cs:67.687074829932,0.328789577132191)
--(axis cs:67.3469387755102,0.32662783792418)
--(axis cs:67.0068027210884,0.328739395369007)
--(axis cs:66.6666666666667,0.32780430523064)
--(axis cs:66.3265306122449,0.326216875561285)
--(axis cs:65.9863945578231,0.323009170910775)
--(axis cs:65.6462585034014,0.327320302020787)
--(axis cs:65.3061224489796,0.319308264218676)
--(axis cs:64.9659863945578,0.318524199725842)
--(axis cs:64.6258503401361,0.319931490431047)
--(axis cs:64.2857142857143,0.314025835890027)
--(axis cs:63.9455782312925,0.311806091336926)
--(axis cs:63.6054421768707,0.309606724805525)
--(axis cs:63.265306122449,0.311925813055112)
--(axis cs:62.9251700680272,0.307750654540522)
--(axis cs:62.5850340136054,0.304735751133608)
--(axis cs:62.2448979591837,0.30329206646509)
--(axis cs:61.9047619047619,0.302609786592406)
--(axis cs:61.5646258503401,0.301164571709586)
--(axis cs:61.2244897959184,0.296083481929299)
--(axis cs:60.8843537414966,0.29172180148693)
--(axis cs:60.5442176870748,0.293488477300402)
--(axis cs:60.2040816326531,0.284920518610863)
--(axis cs:59.8639455782313,0.286622874253361)
--(axis cs:59.5238095238095,0.288882096398495)
--(axis cs:59.1836734693878,0.284527642998645)
--(axis cs:58.843537414966,0.279388532428304)
--(axis cs:58.5034013605442,0.284429291029651)
--(axis cs:58.1632653061224,0.277143127863007)
--(axis cs:57.8231292517007,0.274062291049558)
--(axis cs:57.4829931972789,0.274890018953958)
--(axis cs:57.1428571428571,0.273102424496961)
--(axis cs:56.8027210884354,0.272852403961875)
--(axis cs:56.4625850340136,0.270862898661222)
--(axis cs:56.1224489795918,0.267224264546843)
--(axis cs:55.7823129251701,0.262674331871286)
--(axis cs:55.4421768707483,0.264785032634044)
--(axis cs:55.1020408163265,0.260167995023099)
--(axis cs:54.7619047619048,0.25938749291834)
--(axis cs:54.421768707483,0.257298929662937)
--(axis cs:54.0816326530612,0.256370753079699)
--(axis cs:53.7414965986395,0.252365352613075)
--(axis cs:53.4013605442177,0.255207903248765)
--(axis cs:53.0612244897959,0.2474093142223)
--(axis cs:52.7210884353741,0.253269620133932)
--(axis cs:52.3809523809524,0.249961881405509)
--(axis cs:52.0408163265306,0.247018345330462)
--(axis cs:51.7006802721088,0.244864717661069)
--(axis cs:51.3605442176871,0.242926827826489)
--(axis cs:51.0204081632653,0.248042732565404)
--(axis cs:50.6802721088435,0.241095275804408)
--(axis cs:50.3401360544218,0.238807117047078)
--(axis cs:50,0.23923857385026)
--(axis cs:49.6598639455782,0.241201384952666)
--(axis cs:49.3197278911565,0.237161102891233)
--(axis cs:48.9795918367347,0.236989996811112)
--(axis cs:48.6394557823129,0.238954697839039)
--(axis cs:48.2993197278912,0.230806285425491)
--(axis cs:47.9591836734694,0.233468288336122)
--(axis cs:47.6190476190476,0.231449905917228)
--(axis cs:47.2789115646259,0.237087436279065)
--(axis cs:46.9387755102041,0.235437102648606)
--(axis cs:46.5986394557823,0.232228959784386)
--(axis cs:46.2585034013605,0.231915964774172)
--(axis cs:45.9183673469388,0.230962635709015)
--(axis cs:45.578231292517,0.232495116424322)
--(axis cs:45.2380952380952,0.228589626457695)
--(axis cs:44.8979591836735,0.224650317329019)
--(axis cs:44.5578231292517,0.221835424203342)
--(axis cs:44.2176870748299,0.229439120478685)
--(axis cs:43.8775510204082,0.221714311578862)
--(axis cs:43.5374149659864,0.222462510908407)
--(axis cs:43.1972789115646,0.22126193805372)
--(axis cs:42.8571428571429,0.218317190795626)
--(axis cs:42.5170068027211,0.222189737788806)
--(axis cs:42.1768707482993,0.220988996659899)
--(axis cs:41.8367346938776,0.219321269531238)
--(axis cs:41.4965986394558,0.216676106333082)
--(axis cs:41.156462585034,0.215114242223961)
--(axis cs:40.8163265306122,0.21383360757019)
--(axis cs:40.4761904761905,0.212230887751764)
--(axis cs:40.1360544217687,0.213634811627545)
--(axis cs:39.7959183673469,0.206368067145322)
--(axis cs:39.4557823129252,0.210793502417054)
--(axis cs:39.1156462585034,0.205225608455232)
--(axis cs:38.7755102040816,0.204805305565153)
--(axis cs:38.4353741496599,0.204760766704355)
--(axis cs:38.0952380952381,0.205189921416029)
--(axis cs:37.7551020408163,0.200375224273069)
--(axis cs:37.4149659863946,0.197180199435957)
--(axis cs:37.0748299319728,0.198595461536187)
--(axis cs:36.734693877551,0.20328634811232)
--(axis cs:36.3945578231292,0.197743272472223)
--(axis cs:36.0544217687075,0.195212024666109)
--(axis cs:35.7142857142857,0.196357206317456)
--(axis cs:35.3741496598639,0.193764946167018)
--(axis cs:35.0340136054422,0.191575815419307)
--(axis cs:34.6938775510204,0.18888080982714)
--(axis cs:34.3537414965986,0.18835409956557)
--(axis cs:34.0136054421769,0.192443769323203)
--(axis cs:33.6734693877551,0.190474713911988)
--(axis cs:33.3333333333333,0.186217232115694)
--(axis cs:32.9931972789116,0.186822671120939)
--(axis cs:32.6530612244898,0.184600588361874)
--(axis cs:32.312925170068,0.184014207597566)
--(axis cs:31.9727891156463,0.181564330947412)
--(axis cs:31.6326530612245,0.179076324136008)
--(axis cs:31.2925170068027,0.176371726997913)
--(axis cs:30.952380952381,0.175991926856359)
--(axis cs:30.6122448979592,0.171386374635594)
--(axis cs:30.2721088435374,0.170894668923138)
--(axis cs:29.9319727891156,0.167415543230104)
--(axis cs:29.5918367346939,0.165475157377663)
--(axis cs:29.2517006802721,0.16437439556283)
--(axis cs:28.9115646258503,0.163335749860414)
--(axis cs:28.5714285714286,0.163366661465)
--(axis cs:28.2312925170068,0.162151218598255)
--(axis cs:27.891156462585,0.159450501180048)
--(axis cs:27.5510204081633,0.156846132411213)
--(axis cs:27.2108843537415,0.158552214991772)
--(axis cs:26.8707482993197,0.155558141738635)
--(axis cs:26.530612244898,0.155507369719749)
--(axis cs:26.1904761904762,0.156089311578862)
--(axis cs:25.8503401360544,0.14684244647055)
--(axis cs:25.5102040816327,0.152369506323605)
--(axis cs:25.1700680272109,0.144874572882767)
--(axis cs:24.8299319727891,0.147953965704895)
--(axis cs:24.4897959183673,0.142823846400661)
--(axis cs:24.1496598639456,0.144790297934127)
--(axis cs:23.8095238095238,0.145130116232981)
--(axis cs:23.469387755102,0.13982457002693)
--(axis cs:23.1292517006803,0.140752594966772)
--(axis cs:22.7891156462585,0.136437749551733)
--(axis cs:22.4489795918367,0.137088130860877)
--(axis cs:22.108843537415,0.140128939043968)
--(axis cs:21.7687074829932,0.136187020367517)
--(axis cs:21.4285714285714,0.131652523300029)
--(axis cs:21.0884353741497,0.135616705106624)
--(axis cs:20.7482993197279,0.136691103798617)
--(axis cs:20.4081632653061,0.139544896821318)
--(axis cs:20.0680272108844,0.137919542520809)
--(axis cs:19.7278911564626,0.13432170373424)
--(axis cs:19.3877551020408,0.137864294257681)
--(axis cs:19.047619047619,0.137408829896686)
--(axis cs:18.7074829931973,0.135762587985963)
--(axis cs:18.3673469387755,0.13752192939233)
--(axis cs:18.0272108843537,0.133961412532648)
--(axis cs:17.687074829932,0.132107720618078)
--(axis cs:17.3469387755102,0.134138287851993)
--(axis cs:17.0068027210884,0.137697720980563)
--(axis cs:16.6666666666667,0.136874948055094)
--(axis cs:16.3265306122449,0.131818769323203)
--(axis cs:15.9863945578231,0.131489544122289)
--(axis cs:15.6462585034014,0.128526109569154)
--(axis cs:15.3061224489796,0.125460579405392)
--(axis cs:14.9659863945578,0.133131439745159)
--(axis cs:14.6258503401361,0.129151781499514)
--(axis cs:14.2857142857143,0.132222263035018)
--(axis cs:13.9455782312925,0.123682758254631)
--(axis cs:13.6054421768707,0.124096427775605)
--(axis cs:13.265306122449,0.129081980976429)
--(axis cs:12.9251700680272,0.130531147533768)
--(axis cs:12.5850340136054,0.13146076031456)
--(axis cs:12.2448979591837,0.127712741017263)
--(axis cs:11.9047619047619,0.124124119587266)
--(axis cs:11.5646258503401,0.124364651387657)
--(axis cs:11.2244897959184,0.125716219875269)
--(axis cs:10.8843537414966,0.127217707800136)
--(axis cs:10.5442176870748,0.121662323626048)
--(axis cs:10.2040816326531,0.123742086978104)
--(axis cs:9.86394557823129,0.120571371108999)
--(axis cs:9.52380952380952,0.113728013532185)
--(axis cs:9.18367346938775,0.117770416609762)
--(axis cs:8.84353741496599,0.112179149270136)
--(axis cs:8.50340136054422,0.113307261965836)
--(axis cs:8.16326530612245,0.110817951071248)
--(axis cs:7.82312925170068,0.105830235634386)
--(axis cs:7.48299319727891,0.106254882143438)
--(axis cs:7.14285714285714,0.0977804515875528)
--(axis cs:6.80272108843537,0.0985578706568832)
--(axis cs:6.46258503401361,0.100271253241789)
--(axis cs:6.12244897959184,0.0952282878717881)
--(axis cs:5.78231292517007,0.0938343683483071)
--(axis cs:5.4421768707483,0.0893087737418077)
--(axis cs:5.10204081632653,0.090602425436472)
--(axis cs:4.76190476190476,0.0932256866369433)
--(axis cs:4.42176870748299,0.0872897390132377)
--(axis cs:4.08163265306122,0.0856828247793107)
--(axis cs:3.74149659863946,0.0878138812416276)
--(axis cs:3.40136054421769,0.0888028693652033)
--(axis cs:3.06122448979592,0.0810097459019294)
--(axis cs:2.72108843537415,0.0829837629424153)
--(axis cs:2.38095238095238,0.0796895342844983)
--(axis cs:2.04081632653061,0.0806312368442255)
--(axis cs:1.70068027210884,0.0791578446910158)
--(axis cs:1.36054421768707,0.0806340587828442)
--(axis cs:1.02040816326531,0.0803698586614722)
--(axis cs:0.680272108843537,0.0797584454129681)
--(axis cs:0.340136054421769,0.0817637486176896)
--(axis cs:0,0.083714778681094)
--cycle;


==> img/stl10/stl10_rate_accuracy_smoothgrad.tex <==
% smoothgrad
\addplot [line width=0.5, opacity=0.8, color7, mark=triangle, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color7, thin}]
table [row sep=\\]{%
0	0.07703125 \\
0.340136054421769	0.0740625 \\
0.680272108843537	0.08359375 \\
1.02040816326531	0.08453125 \\
1.36054421768707	0.081875 \\
1.70068027210884	0.0878125 \\
2.04081632653061	0.09640625 \\
2.38095238095238	0.10546875 \\
2.72108843537415	0.11328125 \\
3.06122448979592	0.12390625 \\
3.40136054421769	0.13515625 \\
3.74149659863946	0.1428125 \\
4.08163265306122	0.16578125 \\
4.42176870748299	0.1790625 \\
4.76190476190476	0.18921875 \\
5.10204081632653	0.1884375 \\
5.4421768707483	0.19453125 \\
5.78231292517007	0.1978125 \\
6.12244897959184	0.2015625 \\
6.46258503401361	0.2096875 \\
6.80272108843537	0.21875 \\
7.14285714285714	0.21734375 \\
7.48299319727891	0.2190625 \\
7.82312925170068	0.220625 \\
8.16326530612245	0.22109375 \\
8.50340136054422	0.21546875 \\
8.84353741496599	0.218125 \\
9.18367346938775	0.2234375 \\
9.52380952380952	0.223125 \\
9.86394557823129	0.2278125 \\
10.2040816326531	0.230625 \\
10.5442176870748	0.23953125 \\
10.8843537414966	0.25234375 \\
11.2244897959184	0.25859375 \\
11.5646258503401	0.26390625 \\
11.9047619047619	0.2765625 \\
12.2448979591837	0.276875 \\
12.5850340136054	0.29171875 \\
12.9251700680272	0.29765625 \\
13.265306122449	0.316875 \\
13.6054421768707	0.3221875 \\
13.9455782312925	0.33078125 \\
14.2857142857143	0.33375 \\
14.6258503401361	0.33734375 \\
14.9659863945578	0.3421875 \\
15.3061224489796	0.35796875 \\
15.6462585034014	0.35625 \\
15.9863945578231	0.35578125 \\
16.3265306122449	0.35484375 \\
16.6666666666667	0.35890625 \\
17.0068027210884	0.36359375 \\
17.3469387755102	0.36390625 \\
17.687074829932	0.37625 \\
18.0272108843537	0.38140625 \\
18.3673469387755	0.39140625 \\
18.7074829931973	0.39609375 \\
19.047619047619	0.4071875 \\
19.3877551020408	0.413125 \\
19.7278911564626	0.41984375 \\
20.0680272108844	0.42140625 \\
20.4081632653061	0.423125 \\
20.7482993197279	0.42796875 \\
21.0884353741497	0.42921875 \\
21.4285714285714	0.43390625 \\
21.7687074829932	0.43375 \\
22.108843537415	0.4440625 \\
22.4489795918367	0.4515625 \\
22.7891156462585	0.4496875 \\
23.1292517006803	0.45265625 \\
23.469387755102	0.45484375 \\
23.8095238095238	0.46140625 \\
24.1496598639456	0.46109375 \\
24.4897959183673	0.46875 \\
24.8299319727891	0.46765625 \\
25.1700680272109	0.47640625 \\
25.5102040816327	0.47734375 \\
25.8503401360544	0.48640625 \\
26.1904761904762	0.495 \\
26.530612244898	0.49890625 \\
26.8707482993197	0.5071875 \\
27.2108843537415	0.51 \\
27.5510204081633	0.51140625 \\
27.891156462585	0.51796875 \\
28.2312925170068	0.5215625 \\
28.5714285714286	0.52484375 \\
28.9115646258503	0.52484375 \\
29.2517006802721	0.53125 \\
29.5918367346939	0.53390625 \\
29.9319727891156	0.5415625 \\
30.2721088435374	0.5415625 \\
30.6122448979592	0.545 \\
30.952380952381	0.5484375 \\
31.2925170068027	0.5465625 \\
31.6326530612245	0.5484375 \\
31.9727891156463	0.55046875 \\
32.312925170068	0.55109375 \\
32.6530612244898	0.55265625 \\
32.9931972789116	0.556875 \\
33.3333333333333	0.56140625 \\
33.6734693877551	0.55875 \\
34.0136054421769	0.56328125 \\
34.3537414965986	0.5653125 \\
34.6938775510204	0.56640625 \\
35.0340136054422	0.57203125 \\
35.3741496598639	0.57453125 \\
35.7142857142857	0.57625 \\
36.0544217687075	0.5790625 \\
36.3945578231292	0.58078125 \\
36.734693877551	0.58875 \\
37.0748299319728	0.58640625 \\
37.4149659863946	0.58984375 \\
37.7551020408163	0.59703125 \\
38.0952380952381	0.60265625 \\
38.4353741496599	0.5990625 \\
38.7755102040816	0.6115625 \\
39.1156462585034	0.61390625 \\
39.4557823129252	0.611875 \\
39.7959183673469	0.623125 \\
40.1360544217687	0.62890625 \\
40.4761904761905	0.6428125 \\
40.8163265306122	0.645625 \\
41.156462585034	0.65625 \\
41.4965986394558	0.66015625 \\
41.8367346938776	0.6728125 \\
42.1768707482993	0.68484375 \\
42.5170068027211	0.685 \\
42.8571428571429	0.69453125 \\
43.1972789115646	0.6978125 \\
43.5374149659864	0.69875 \\
43.8775510204082	0.7115625 \\
44.2176870748299	0.7178125 \\
44.5578231292517	0.72765625 \\
44.8979591836735	0.73484375 \\
45.2380952380952	0.73828125 \\
45.578231292517	0.74 \\
45.9183673469388	0.74765625 \\
46.2585034013605	0.7521875 \\
46.5986394557823	0.7565625 \\
46.9387755102041	0.75921875 \\
47.2789115646259	0.75828125 \\
47.6190476190476	0.76171875 \\
47.9591836734694	0.7634375 \\
48.2993197278912	0.7628125 \\
48.6394557823129	0.76609375 \\
48.9795918367347	0.76609375 \\
49.3197278911565	0.769375 \\
49.6598639455782	0.77234375 \\
50	0.7746875 \\
50.3401360544218	0.77546875 \\
50.6802721088435	0.78046875 \\
51.0204081632653	0.78078125 \\
51.3605442176871	0.78515625 \\
51.7006802721088	0.79328125 \\
52.0408163265306	0.795625 \\
52.3809523809524	0.79859375 \\
52.7210884353741	0.80234375 \\
53.0612244897959	0.810625 \\
53.4013605442177	0.816875 \\
53.7414965986395	0.82484375 \\
54.0816326530612	0.82328125 \\
54.421768707483	0.8290625 \\
54.7619047619048	0.835625 \\
55.1020408163265	0.8428125 \\
55.4421768707483	0.84796875 \\
55.7823129251701	0.85453125 \\
56.1224489795918	0.86234375 \\
56.4625850340136	0.86640625 \\
56.8027210884354	0.875625 \\
57.1428571428571	0.8784375 \\
57.4829931972789	0.8840625 \\
57.8231292517007	0.8884375 \\
58.1632653061224	0.88828125 \\
58.5034013605442	0.89390625 \\
58.843537414966	0.89546875 \\
59.1836734693878	0.8928125 \\
59.5238095238095	0.90125 \\
59.8639455782313	0.90609375 \\
60.2040816326531	0.9046875 \\
60.5442176870748	0.910625 \\
60.8843537414966	0.90546875 \\
61.2244897959184	0.9078125 \\
61.5646258503401	0.91375 \\
61.9047619047619	0.9140625 \\
62.2448979591837	0.91890625 \\
62.5850340136054	0.92421875 \\
62.9251700680272	0.91875 \\
63.265306122449	0.92125 \\
63.6054421768707	0.92046875 \\
63.9455782312925	0.9240625 \\
64.2857142857143	0.92546875 \\
64.6258503401361	0.9278125 \\
64.9659863945578	0.92765625 \\
65.3061224489796	0.93140625 \\
65.6462585034014	0.93671875 \\
65.9863945578231	0.93671875 \\
66.3265306122449	0.94171875 \\
66.6666666666667	0.9434375 \\
67.0068027210884	0.9434375 \\
67.3469387755102	0.953125 \\
67.687074829932	0.95203125 \\
68.0272108843537	0.95265625 \\
68.3673469387755	0.95390625 \\
68.7074829931973	0.95421875 \\
69.0476190476191	0.9540625 \\
69.3877551020408	0.95234375 \\
69.7278911564626	0.9496875 \\
70.0680272108844	0.95203125 \\
70.4081632653061	0.94984375 \\
70.7482993197279	0.94765625 \\
71.0884353741497	0.94828125 \\
71.4285714285714	0.943125 \\
71.7687074829932	0.948125 \\
72.108843537415	0.94125 \\
72.4489795918367	0.941875 \\
72.7891156462585	0.93875 \\
73.1292517006803	0.935 \\
73.469387755102	0.926875 \\
73.8095238095238	0.93328125 \\
74.1496598639456	0.93265625 \\
74.4897959183673	0.9309375 \\
74.8299319727891	0.93078125 \\
75.1700680272109	0.93265625 \\
75.5102040816327	0.93609375 \\
75.8503401360544	0.9340625 \\
76.1904761904762	0.93359375 \\
76.530612244898	0.935625 \\
76.8707482993197	0.9371875 \\
77.2108843537415	0.935 \\
77.5510204081633	0.93625 \\
77.891156462585	0.941875 \\
78.2312925170068	0.94078125 \\
78.5714285714286	0.9428125 \\
78.9115646258503	0.94546875 \\
79.2517006802721	0.9440625 \\
79.5918367346939	0.94921875 \\
79.9319727891156	0.95125 \\
80.2721088435374	0.9475 \\
80.6122448979592	0.95140625 \\
80.9523809523809	0.95296875 \\
81.2925170068027	0.96046875 \\
81.6326530612245	0.9625 \\
81.9727891156463	0.9578125 \\
82.312925170068	0.96203125 \\
82.6530612244898	0.9625 \\
82.9931972789116	0.96328125 \\
83.3333333333333	0.96359375 \\
83.6734693877551	0.9621875 \\
84.0136054421769	0.96125 \\
84.3537414965986	0.96234375 \\
84.6938775510204	0.96140625 \\
85.0340136054422	0.9590625 \\
85.3741496598639	0.955625 \\
85.7142857142857	0.955 \\
86.0544217687075	0.95421875 \\
86.3945578231292	0.9565625 \\
86.734693877551	0.95640625 \\
87.0748299319728	0.951875 \\
87.4149659863945	0.9540625 \\
87.7551020408163	0.95125 \\
88.0952380952381	0.948125 \\
88.4353741496599	0.95015625 \\
88.7755102040816	0.94859375 \\
89.1156462585034	0.94875 \\
89.4557823129252	0.946875 \\
89.7959183673469	0.94671875 \\
90.1360544217687	0.94671875 \\
90.4761904761905	0.94859375 \\
90.8163265306122	0.946875 \\
91.156462585034	0.9434375 \\
91.4965986394558	0.9421875 \\
91.8367346938775	0.94265625 \\
92.1768707482993	0.943125 \\
92.5170068027211	0.94296875 \\
92.8571428571429	0.940625 \\
93.1972789115646	0.94140625 \\
93.5374149659864	0.94296875 \\
93.8775510204082	0.94625 \\
94.2176870748299	0.94625 \\
94.5578231292517	0.95171875 \\
94.8979591836735	0.95359375 \\
95.2380952380952	0.9534375 \\
95.578231292517	0.95515625 \\
95.9183673469388	0.95859375 \\
96.2585034013605	0.9584375 \\
96.5986394557823	0.96 \\
96.9387755102041	0.96 \\
97.2789115646258	0.96 \\
97.6190476190476	0.96 \\
97.9591836734694	0.96 \\
98.2993197278912	0.96 \\
98.6394557823129	0.96 \\
98.9795918367347	0.96 \\
99.3197278911565	0.96 \\
99.6598639455782	0.9665625 \\
100	1 \\
};
\path [fill=color7, fill opacity=0.5] (axis cs:0,0.0832299222939681)
--(axis cs:0,0.0708325777060319)
--(axis cs:0.340136054421769,0.0665436029082343)
--(axis cs:0.680272108843537,0.0736294621137005)
--(axis cs:1.02040816326531,0.0743895649810096)
--(axis cs:1.36054421768707,0.0703797351800296)
--(axis cs:1.70068027210884,0.0744268236791559)
--(axis cs:2.04081632653061,0.0813662363328387)
--(axis cs:2.38095238095238,0.0897630866285127)
--(axis cs:2.72108843537415,0.0960220445510376)
--(axis cs:3.06122448979592,0.105838260204535)
--(axis cs:3.40136054421769,0.116990349975337)
--(axis cs:3.74149659863946,0.125259349338522)
--(axis cs:4.08163265306122,0.148750660760381)
--(axis cs:4.42176870748299,0.16280104820586)
--(axis cs:4.76190476190476,0.17393905728714)
--(axis cs:5.10204081632653,0.174535969024005)
--(axis cs:5.4421768707483,0.181354892031967)
--(axis cs:5.78231292517007,0.185235679172814)
--(axis cs:6.12244897959184,0.189869005078193)
--(axis cs:6.46258503401361,0.196887451267335)
--(axis cs:6.80272108843537,0.205868255900124)
--(axis cs:7.14285714285714,0.204909152422316)
--(axis cs:7.48299319727891,0.207211842641272)
--(axis cs:7.82312925170068,0.20767164293596)
--(axis cs:8.16326530612245,0.208815054113194)
--(axis cs:8.50340136054422,0.203392892278013)
--(axis cs:8.84353741496599,0.204814342071034)
--(axis cs:9.18367346938775,0.209213170737474)
--(axis cs:9.52380952380952,0.209270885343339)
--(axis cs:9.86394557823129,0.213002840338579)
--(axis cs:10.2040816326531,0.215282087360552)
--(axis cs:10.5442176870748,0.223915713314957)
--(axis cs:10.8843537414966,0.235417636996962)
--(axis cs:11.2244897959184,0.241957469665615)
--(axis cs:11.5646258503401,0.246889665951184)
--(axis cs:11.9047619047619,0.259255564127441)
--(axis cs:12.2448979591837,0.259334893544432)
--(axis cs:12.5850340136054,0.274406580077746)
--(axis cs:12.9251700680272,0.280005845218794)
--(axis cs:13.265306122449,0.298733002312917)
--(axis cs:13.6054421768707,0.304530882712614)
--(axis cs:13.9455782312925,0.314134081483868)
--(axis cs:14.2857142857143,0.317294994320449)
--(axis cs:14.6258503401361,0.321719055178762)
--(axis cs:14.9659863945578,0.326972543425482)
--(axis cs:15.3061224489796,0.342613100396957)
--(axis cs:15.6462585034014,0.341759312956718)
--(axis cs:15.9863945578231,0.341354873252204)
--(axis cs:16.3265306122449,0.340900776522315)
--(axis cs:16.6666666666667,0.345779927638229)
--(axis cs:17.0068027210884,0.348898836748678)
--(axis cs:17.3469387755102,0.349069890306001)
--(axis cs:17.687074829932,0.36047194107139)
--(axis cs:18.0272108843537,0.365464334538579)
--(axis cs:18.3673469387755,0.375339199844231)
--(axis cs:18.7074829931973,0.379852543789413)
--(axis cs:19.047619047619,0.391593047438798)
--(axis cs:19.3877551020408,0.398122762211194)
--(axis cs:19.7278911564626,0.406629809233112)
--(axis cs:20.0680272108844,0.407941368853403)
--(axis cs:20.4081632653061,0.40976214181008)
--(axis cs:20.7482993197279,0.414663466712731)
--(axis cs:21.0884353741497,0.415470706038456)
--(axis cs:21.4285714285714,0.421025616443175)
--(axis cs:21.7687074829932,0.420101163384127)
--(axis cs:22.108843537415,0.430427644986461)
--(axis cs:22.4489795918367,0.439604493184399)
--(axis cs:22.7891156462585,0.436462377330289)
--(axis cs:23.1292517006803,0.439315891527134)
--(axis cs:23.469387755102,0.441723968089916)
--(axis cs:23.8095238095238,0.448897479273315)
--(axis cs:24.1496598639456,0.44849836503033)
--(axis cs:24.4897959183673,0.455508302230663)
--(axis cs:24.8299319727891,0.454223278720077)
--(axis cs:25.1700680272109,0.46263394863857)
--(axis cs:25.5102040816327,0.46338847027678)
--(axis cs:25.8503401360544,0.471782899085529)
--(axis cs:26.1904761904762,0.480481697846783)
--(axis cs:26.530612244898,0.485048349830973)
--(axis cs:26.8707482993197,0.494842575708547)
--(axis cs:27.2108843537415,0.4972111319788)
--(axis cs:27.5510204081633,0.498865499164482)
--(axis cs:27.891156462585,0.506043086462667)
--(axis cs:28.2312925170068,0.508816208125774)
--(axis cs:28.5714285714286,0.513400454129241)
--(axis cs:28.9115646258503,0.513785284573334)
--(axis cs:29.2517006802721,0.520442316146674)
--(axis cs:29.5918367346939,0.523225941718618)
--(axis cs:29.9319727891156,0.530973211727267)
--(axis cs:30.2721088435374,0.531759835866149)
--(axis cs:30.6122448979592,0.536072060743641)
--(axis cs:30.952380952381,0.539221522861403)
--(axis cs:31.2925170068027,0.538021066560285)
--(axis cs:31.6326530612245,0.540417787043888)
--(axis cs:31.9727891156463,0.542310506896121)
--(axis cs:32.312925170068,0.54241881828225)
--(axis cs:32.6530612244898,0.544182635701354)
--(axis cs:32.9931972789116,0.547442194811685)
--(axis cs:33.3333333333333,0.551451537637617)
--(axis cs:33.6734693877551,0.548984375)
--(axis cs:34.0136054421769,0.552914497436356)
--(axis cs:34.3537414965986,0.554287286697341)
--(axis cs:34.6938775510204,0.554780233448134)
--(axis cs:35.0340136054422,0.560565474643898)
--(axis cs:35.3741496598639,0.562830824874385)
--(axis cs:35.7142857142857,0.563731702844561)
--(axis cs:36.0544217687075,0.566199277468438)
--(axis cs:36.3945578231292,0.567492462501927)
--(axis cs:36.734693877551,0.575251518052293)
--(axis cs:37.0748299319728,0.573412096017546)
--(axis cs:37.4149659863946,0.576131824844155)
--(axis cs:37.7551020408163,0.583344386006679)
--(axis cs:38.0952380952381,0.588131052272652)
--(axis cs:38.4353741496599,0.583791860070788)
--(axis cs:38.7755102040816,0.59633062921223)
--(axis cs:39.1156462585034,0.597895091609891)
--(axis cs:39.4557823129252,0.595532233127382)
--(axis cs:39.7959183673469,0.606922300662534)
--(axis cs:40.1360544217687,0.611569308680905)
--(axis cs:40.4761904761905,0.625534793713531)
--(axis cs:40.8163265306122,0.628573983839677)
--(axis cs:41.156462585034,0.639193391692283)
--(axis cs:41.4965986394558,0.643814358468624)
--(axis cs:41.8367346938776,0.656235081895373)
--(axis cs:42.1768707482993,0.669683108621844)
--(axis cs:42.5170068027211,0.670108142307385)
--(axis cs:42.8571428571429,0.68056299211315)
--(axis cs:43.1972789115646,0.68354131620146)
--(axis cs:43.5374149659864,0.684580754533503)
--(axis cs:43.8775510204082,0.698616507401314)
--(axis cs:44.2176870748299,0.704056481031515)
--(axis cs:44.5578231292517,0.715081325014008)
--(axis cs:44.8979591836735,0.721868692116692)
--(axis cs:45.2380952380952,0.725995565889719)
--(axis cs:45.578231292517,0.727888262579233)
--(axis cs:45.9183673469388,0.735800362960427)
--(axis cs:46.2585034013605,0.741717766195947)
--(axis cs:46.5986394557823,0.747488347671627)
--(axis cs:46.9387755102041,0.75077783724256)
--(axis cs:47.2789115646259,0.749480801645777)
--(axis cs:47.6190476190476,0.7525343886566)
--(axis cs:47.9591836734694,0.755313814709732)
--(axis cs:48.2993197278912,0.755303756723929)
--(axis cs:48.6394557823129,0.757886556998262)
--(axis cs:48.9795918367347,0.757439731045353)
--(axis cs:49.3197278911565,0.760605490499749)
--(axis cs:49.6598639455782,0.762755020113058)
--(axis cs:50,0.764651211776816)
--(axis cs:50.3401360544218,0.765398785250137)
--(axis cs:50.6802721088435,0.769359519905789)
--(axis cs:51.0204081632653,0.769825019525697)
--(axis cs:51.3605442176871,0.77363488167412)
--(axis cs:51.7006802721088,0.780908160732857)
--(axis cs:52.0408163265306,0.783550326940567)
--(axis cs:52.3809523809524,0.786609851831724)
--(axis cs:52.7210884353741,0.790617271428723)
--(axis cs:53.0612244897959,0.799677912962819)
--(axis cs:53.4013605442177,0.806129261950407)
--(axis cs:53.7414965986395,0.813356369308078)
--(axis cs:54.0816326530612,0.811288601265995)
--(axis cs:54.421768707483,0.816879320176757)
--(axis cs:54.7619047619048,0.823128052130432)
--(axis cs:55.1020408163265,0.829035006180821)
--(axis cs:55.4421768707483,0.835016497338821)
--(axis cs:55.7823129251701,0.841626206572176)
--(axis cs:56.1224489795918,0.849712828561261)
--(axis cs:56.4625850340136,0.854289395581021)
--(axis cs:56.8027210884354,0.863622415185206)
--(axis cs:57.1428571428571,0.867221051550499)
--(axis cs:57.4829931972789,0.872436073308732)
--(axis cs:57.8231292517007,0.876505041098355)
--(axis cs:58.1632653061224,0.877267720306768)
--(axis cs:58.5034013605442,0.881886594339692)
--(axis cs:58.843537414966,0.882731065302607)
--(axis cs:59.1836734693878,0.879935198646971)
--(axis cs:59.5238095238095,0.888431338419445)
--(axis cs:59.8639455782313,0.89379797880093)
--(axis cs:60.2040816326531,0.892657137816848)
--(axis cs:60.5442176870748,0.898770319605083)
--(axis cs:60.8843537414966,0.893735767106752)
--(axis cs:61.2244897959184,0.896527391750059)
--(axis cs:61.5646258503401,0.902602634238183)
--(axis cs:61.9047619047619,0.903666809857679)
--(axis cs:62.2448979591837,0.909431580433027)
--(axis cs:62.5850340136054,0.915202057952823)
--(axis cs:62.9251700680272,0.910045984392517)
--(axis cs:63.265306122449,0.912000968365194)
--(axis cs:63.6054421768707,0.911251220783955)
--(axis cs:63.9455782312925,0.915148458041216)
--(axis cs:64.2857142857143,0.917269695020097)
--(axis cs:64.6258503401361,0.919397046670777)
--(axis cs:64.9659863945578,0.919450219078693)
--(axis cs:65.3061224489796,0.922661243228555)
--(axis cs:65.6462585034014,0.927436267870348)
--(axis cs:65.9863945578231,0.92707646245469)
--(axis cs:66.3265306122449,0.932175880385799)
--(axis cs:66.6666666666667,0.934228769348339)
--(axis cs:67.0068027210884,0.933820466403039)
--(axis cs:67.3469387755102,0.946092393793989)
--(axis cs:67.687074829932,0.94487563863214)
--(axis cs:68.0272108843537,0.945633821723302)
--(axis cs:68.3673469387755,0.947315357411564)
--(axis cs:68.7074829931973,0.947293413808011)
--(axis cs:69.0476190476191,0.947391784625806)
--(axis cs:69.3877551020408,0.944733451632961)
--(axis cs:69.7278911564626,0.94210167715393)
--(axis cs:70.0680272108844,0.944809307853717)
--(axis cs:70.4081632653061,0.942074705819063)
--(axis cs:70.7482993197279,0.938603668378783)
--(axis cs:71.0884353741497,0.939612916862098)
--(axis cs:71.4285714285714,0.933112495610956)
--(axis cs:71.7687074829932,0.939682392677128)
--(axis cs:72.108843537415,0.931271843926215)
--(axis cs:72.4489795918367,0.931719689045816)
--(axis cs:72.7891156462585,0.927881600815664)
--(axis cs:73.1292517006803,0.924278250977587)
--(axis cs:73.469387755102,0.9153515625)
--(axis cs:73.8095238095238,0.922313709640908)
--(axis cs:74.1496598639456,0.921610728043214)
--(axis cs:74.4897959183673,0.919990412962819)
--(axis cs:74.8299319727891,0.919516018476228)
--(axis cs:75.1700680272109,0.922782338649061)
--(axis cs:75.5102040816327,0.925824044909231)
--(axis cs:75.8503401360544,0.92307628038248)
--(axis cs:76.1904761904762,0.922416054701219)
--(axis cs:76.530612244898,0.924400901942817)
--(axis cs:76.8707482993197,0.926379816146674)
--(axis cs:77.2108843537415,0.923838954385498)
--(axis cs:77.5510204081633,0.925395649487472)
--(axis cs:77.891156462585,0.931613191289174)
--(axis cs:78.2312925170068,0.930590784048265)
--(axis cs:78.5714285714286,0.932517289291841)
--(axis cs:78.9115646258503,0.934888020913452)
--(axis cs:79.2517006802721,0.933366576898365)
--(axis cs:79.5918367346939,0.938282557974413)
--(axis cs:79.9319727891156,0.941249885559737)
--(axis cs:80.2721088435374,0.936375757136017)
--(axis cs:80.6122448979592,0.940039045720588)
--(axis cs:80.9523809523809,0.941209785796647)
--(axis cs:81.2925170068027,0.949894332115377)
--(axis cs:81.6326530612245,0.952416312399958)
--(axis cs:81.9727891156463,0.947255683215797)
--(axis cs:82.312925170068,0.953183248833986)
--(axis cs:82.6530612244898,0.95334423829427)
--(axis cs:82.9931972789116,0.954673639551008)
--(axis cs:83.3333333333333,0.955480049360864)
--(axis cs:83.6734693877551,0.953838033398516)
--(axis cs:84.0136054421769,0.953051526616478)
--(axis cs:84.3537414965986,0.9533971369327)
--(axis cs:84.6938775510204,0.953053928391901)
--(axis cs:85.0340136054422,0.950117486017536)
--(axis cs:85.3741496598639,0.946833767628963)
--(axis cs:85.7142857142857,0.946219622346489)
--(axis cs:86.0544217687075,0.945601173831578)
--(axis cs:86.3945578231292,0.947796253573164)
--(axis cs:86.734693877551,0.94769402073059)
--(axis cs:87.0748299319728,0.943877913051729)
--(axis cs:87.4149659863945,0.945595078012912)
--(axis cs:87.7551020408163,0.943905626688686)
--(axis cs:88.0952380952381,0.941321225215488)
--(axis cs:88.4353741496599,0.942627846143669)
--(axis cs:88.7755102040816,0.942099058705208)
--(axis cs:89.1156462585034,0.942236979687292)
--(axis cs:89.4557823129252,0.940492134906887)
--(axis cs:89.7959183673469,0.940515463881579)
--(axis cs:90.1360544217687,0.940420868227584)
--(axis cs:90.4761904761905,0.941428815356045)
--(axis cs:90.8163265306122,0.940451920448279)
--(axis cs:91.156462585034,0.938552734765469)
--(axis cs:91.4965986394558,0.938206285720578)
--(axis cs:91.8367346938775,0.938378282009022)
--(axis cs:92.1768707482993,0.938511323511321)
--(axis cs:92.5170068027211,0.938376828927536)
--(axis cs:92.8571428571429,0.938436976904062)
--(axis cs:93.1972789115646,0.938151204431153)
--(axis cs:93.5374149659864,0.938397644633411)
--(axis cs:93.8775510204082,0.940332321325179)
--(axis cs:94.2176870748299,0.940456094931957)
--(axis cs:94.5578231292517,0.945448184470047)
--(axis cs:94.8979591836735,0.947761292296235)
--(axis cs:95.2380952380952,0.947568367499486)
--(axis cs:95.578231292517,0.949801160206697)
--(axis cs:95.9183673469388,0.955397838247665)
--(axis cs:96.2585034013605,0.955082897648961)
--(axis cs:96.5986394557823,0.96)
--(axis cs:96.9387755102041,0.96)
--(axis cs:97.2789115646258,0.96)
--(axis cs:97.6190476190476,0.96)
--(axis cs:97.9591836734694,0.96)
--(axis cs:98.2993197278912,0.96)
--(axis cs:98.6394557823129,0.96)
--(axis cs:98.9795918367347,0.96)
--(axis cs:99.3197278911565,0.96)
--(axis cs:99.6598639455782,0.960693367499486)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:100,1)
--(axis cs:99.6598639455782,0.972431632500514)
--(axis cs:99.3197278911565,0.96)
--(axis cs:98.9795918367347,0.96)
--(axis cs:98.6394557823129,0.96)
--(axis cs:98.2993197278912,0.96)
--(axis cs:97.9591836734694,0.96)
--(axis cs:97.6190476190476,0.96)
--(axis cs:97.2789115646258,0.96)
--(axis cs:96.9387755102041,0.96)
--(axis cs:96.5986394557823,0.96)
--(axis cs:96.2585034013605,0.961792102351039)
--(axis cs:95.9183673469388,0.961789661752335)
--(axis cs:95.578231292517,0.960511339793303)
--(axis cs:95.2380952380952,0.959306632500514)
--(axis cs:94.8979591836735,0.959426207703765)
--(axis cs:94.5578231292517,0.957989315529953)
--(axis cs:94.2176870748299,0.952043905068043)
--(axis cs:93.8775510204082,0.952167678674822)
--(axis cs:93.5374149659864,0.947539855366589)
--(axis cs:93.1972789115646,0.944661295568847)
--(axis cs:92.8571428571429,0.942813023095938)
--(axis cs:92.5170068027211,0.947560671072464)
--(axis cs:92.1768707482993,0.947738676488679)
--(axis cs:91.8367346938775,0.946934217990978)
--(axis cs:91.4965986394558,0.946168714279422)
--(axis cs:91.156462585034,0.948322265234531)
--(axis cs:90.8163265306122,0.953298079551721)
--(axis cs:90.4761904761905,0.955758684643955)
--(axis cs:90.1360544217687,0.953016631772417)
--(axis cs:89.7959183673469,0.952922036118421)
--(axis cs:89.4557823129252,0.953257865093113)
--(axis cs:89.1156462585034,0.955263020312708)
--(axis cs:88.7755102040816,0.955088441294792)
--(axis cs:88.4353741496599,0.957684653856331)
--(axis cs:88.0952380952381,0.954928774784512)
--(axis cs:87.7551020408163,0.958594373311314)
--(axis cs:87.4149659863945,0.962529921987088)
--(axis cs:87.0748299319728,0.959872086948271)
--(axis cs:86.734693877551,0.965118479269411)
--(axis cs:86.3945578231292,0.965328746426836)
--(axis cs:86.0544217687075,0.962836326168422)
--(axis cs:85.7142857142857,0.963780377653511)
--(axis cs:85.3741496598639,0.964416232371037)
--(axis cs:85.0340136054422,0.968007513982464)
--(axis cs:84.6938775510204,0.969758571608099)
--(axis cs:84.3537414965986,0.9712903630673)
--(axis cs:84.0136054421769,0.969448473383522)
--(axis cs:83.6734693877551,0.970536966601484)
--(axis cs:83.3333333333333,0.971707450639136)
--(axis cs:82.9931972789116,0.971888860448992)
--(axis cs:82.6530612244898,0.97165576170573)
--(axis cs:82.312925170068,0.970879251166014)
--(axis cs:81.9727891156463,0.968369316784203)
--(axis cs:81.6326530612245,0.972583687600042)
--(axis cs:81.2925170068027,0.971043167884623)
--(axis cs:80.9523809523809,0.964727714203353)
--(axis cs:80.6122448979592,0.962773454279412)
--(axis cs:80.2721088435374,0.958624242863983)
--(axis cs:79.9319727891156,0.961250114440263)
--(axis cs:79.5918367346939,0.960154942025587)
--(axis cs:79.2517006802721,0.954758423101635)
--(axis cs:78.9115646258503,0.956049479086548)
--(axis cs:78.5714285714286,0.953107710708159)
--(axis cs:78.2312925170068,0.950971715951735)
--(axis cs:77.891156462585,0.952136808710826)
--(axis cs:77.5510204081633,0.947104350512529)
--(axis cs:77.2108843537415,0.946161045614502)
--(axis cs:76.8707482993197,0.947995183853326)
--(axis cs:76.530612244898,0.946849098057183)
--(axis cs:76.1904761904762,0.944771445298781)
--(axis cs:75.8503401360544,0.94504871961752)
--(axis cs:75.5102040816327,0.946363455090769)
--(axis cs:75.1700680272109,0.942530161350939)
--(axis cs:74.8299319727891,0.942046481523772)
--(axis cs:74.4897959183673,0.941884587037181)
--(axis cs:74.1496598639456,0.943701771956786)
--(axis cs:73.8095238095238,0.944248790359092)
--(axis cs:73.469387755102,0.9383984375)
--(axis cs:73.1292517006803,0.945721749022413)
--(axis cs:72.7891156462585,0.949618399184336)
--(axis cs:72.4489795918367,0.952030310954184)
--(axis cs:72.108843537415,0.951228156073785)
--(axis cs:71.7687074829932,0.956567607322871)
--(axis cs:71.4285714285714,0.953137504389044)
--(axis cs:71.0884353741497,0.956949583137902)
--(axis cs:70.7482993197279,0.956708831621217)
--(axis cs:70.4081632653061,0.957612794180937)
--(axis cs:70.0680272108844,0.959253192146283)
--(axis cs:69.7278911564626,0.95727332284607)
--(axis cs:69.3877551020408,0.959954048367039)
--(axis cs:69.0476190476191,0.960733215374195)
--(axis cs:68.7074829931973,0.961144086191989)
--(axis cs:68.3673469387755,0.960497142588436)
--(axis cs:68.0272108843537,0.959678678276698)
--(axis cs:67.687074829932,0.95918686136786)
--(axis cs:67.3469387755102,0.960157606206011)
--(axis cs:67.0068027210884,0.953054533596961)
--(axis cs:66.6666666666667,0.952646230651661)
--(axis cs:66.3265306122449,0.951261619614201)
--(axis cs:65.9863945578231,0.94636103754531)
--(axis cs:65.6462585034014,0.946001232129652)
--(axis cs:65.3061224489796,0.940151256771445)
--(axis cs:64.9659863945578,0.935862280921307)
--(axis cs:64.6258503401361,0.936227953329223)
--(axis cs:64.2857142857143,0.933667804979903)
--(axis cs:63.9455782312925,0.932976541958784)
--(axis cs:63.6054421768707,0.929686279216044)
--(axis cs:63.265306122449,0.930499031634806)
--(axis cs:62.9251700680272,0.927454015607483)
--(axis cs:62.5850340136054,0.933235442047177)
--(axis cs:62.2448979591837,0.928380919566973)
--(axis cs:61.9047619047619,0.924458190142321)
--(axis cs:61.5646258503401,0.924897365761817)
--(axis cs:61.2244897959184,0.919097608249941)
--(axis cs:60.8843537414966,0.917201732893248)
--(axis cs:60.5442176870748,0.922479680394917)
--(axis cs:60.2040816326531,0.916717862183152)
--(axis cs:59.8639455782313,0.91838952119907)
--(axis cs:59.5238095238095,0.914068661580555)
--(axis cs:59.1836734693878,0.905689801353029)
--(axis cs:58.843537414966,0.908206434697393)
--(axis cs:58.5034013605442,0.905925905660308)
--(axis cs:58.1632653061224,0.899294779693232)
--(axis cs:57.8231292517007,0.900369958901645)
--(axis cs:57.4829931972789,0.895688926691268)
--(axis cs:57.1428571428571,0.889653948449501)
--(axis cs:56.8027210884354,0.887627584814794)
--(axis cs:56.4625850340136,0.87852310441898)
--(axis cs:56.1224489795918,0.874974671438739)
--(axis cs:55.7823129251701,0.867436293427824)
--(axis cs:55.4421768707483,0.860921002661179)
--(axis cs:55.1020408163265,0.856589993819178)
--(axis cs:54.7619047619048,0.848121947869567)
--(axis cs:54.421768707483,0.841245679823243)
--(axis cs:54.0816326530612,0.835273898734005)
--(axis cs:53.7414965986395,0.836331130691922)
--(axis cs:53.4013605442177,0.827620738049593)
--(axis cs:53.0612244897959,0.821572087037181)
--(axis cs:52.7210884353741,0.814070228571277)
--(axis cs:52.3809523809524,0.810577648168276)
--(axis cs:52.0408163265306,0.807699673059433)
--(axis cs:51.7006802721088,0.805654339267143)
--(axis cs:51.3605442176871,0.79667761832588)
--(axis cs:51.0204081632653,0.791737480474303)
--(axis cs:50.6802721088435,0.791577980094211)
--(axis cs:50.3401360544218,0.785538714749863)
--(axis cs:50,0.784723788223184)
--(axis cs:49.6598639455782,0.781932479886942)
--(axis cs:49.3197278911565,0.778144509500251)
--(axis cs:48.9795918367347,0.774747768954647)
--(axis cs:48.6394557823129,0.774300943001738)
--(axis cs:48.2993197278912,0.770321243276071)
--(axis cs:47.9591836734694,0.771561185290268)
--(axis cs:47.6190476190476,0.7709031113434)
--(axis cs:47.2789115646259,0.767081698354223)
--(axis cs:46.9387755102041,0.76765966275744)
--(axis cs:46.5986394557823,0.765636652328373)
--(axis cs:46.2585034013605,0.762657233804053)
--(axis cs:45.9183673469388,0.759512137039573)
--(axis cs:45.578231292517,0.752111737420767)
--(axis cs:45.2380952380952,0.750566934110281)
--(axis cs:44.8979591836735,0.747818807883308)
--(axis cs:44.5578231292517,0.740231174985992)
--(axis cs:44.2176870748299,0.731568518968485)
--(axis cs:43.8775510204082,0.724508492598686)
--(axis cs:43.5374149659864,0.712919245466497)
--(axis cs:43.1972789115646,0.71208368379854)
--(axis cs:42.8571428571429,0.70849950788685)
--(axis cs:42.5170068027211,0.699891857692616)
--(axis cs:42.1768707482993,0.700004391378156)
--(axis cs:41.8367346938776,0.689389918104627)
--(axis cs:41.4965986394558,0.676498141531376)
--(axis cs:41.156462585034,0.673306608307717)
--(axis cs:40.8163265306122,0.662676016160323)
--(axis cs:40.4761904761905,0.660090206286469)
--(axis cs:40.1360544217687,0.646243191319095)
--(axis cs:39.7959183673469,0.639327699337466)
--(axis cs:39.4557823129252,0.628217766872618)
--(axis cs:39.1156462585034,0.629917408390109)
--(axis cs:38.7755102040816,0.62679437078777)
--(axis cs:38.4353741496599,0.614333139929212)
--(axis cs:38.0952380952381,0.617181447727348)
--(axis cs:37.7551020408163,0.610718113993321)
--(axis cs:37.4149659863946,0.603555675155845)
--(axis cs:37.0748299319728,0.599400403982454)
--(axis cs:36.734693877551,0.602248481947707)
--(axis cs:36.3945578231292,0.594070037498073)
--(axis cs:36.0544217687075,0.591925722531562)
--(axis cs:35.7142857142857,0.588768297155439)
--(axis cs:35.3741496598639,0.586231675125615)
--(axis cs:35.0340136054422,0.583497025356102)
--(axis cs:34.6938775510204,0.578032266551866)
--(axis cs:34.3537414965986,0.576337713302659)
--(axis cs:34.0136054421769,0.573648002563644)
--(axis cs:33.6734693877551,0.568515625)
--(axis cs:33.3333333333333,0.571360962362383)
--(axis cs:32.9931972789116,0.566307805188315)
--(axis cs:32.6530612244898,0.561129864298646)
--(axis cs:32.312925170068,0.55976868171775)
--(axis cs:31.9727891156463,0.558626993103879)
--(axis cs:31.6326530612245,0.556457212956113)
--(axis cs:31.2925170068027,0.555103933439715)
--(axis cs:30.952380952381,0.557653477138597)
--(axis cs:30.6122448979592,0.553927939256359)
--(axis cs:30.2721088435374,0.551365164133851)
--(axis cs:29.9319727891156,0.552151788272733)
--(axis cs:29.5918367346939,0.544586558281382)
--(axis cs:29.2517006802721,0.542057683853326)
--(axis cs:28.9115646258503,0.535902215426666)
--(axis cs:28.5714285714286,0.53628704587076)
--(axis cs:28.2312925170068,0.534308791874226)
--(axis cs:27.891156462585,0.529894413537333)
--(axis cs:27.5510204081633,0.523947000835518)
--(axis cs:27.2108843537415,0.5227888680212)
--(axis cs:26.8707482993197,0.519532424291454)
--(axis cs:26.530612244898,0.512764150169027)
--(axis cs:26.1904761904762,0.509518302153217)
--(axis cs:25.8503401360544,0.501029600914471)
--(axis cs:25.5102040816327,0.49129902972322)
--(axis cs:25.1700680272109,0.49017855136143)
--(axis cs:24.8299319727891,0.481089221279923)
--(axis cs:24.4897959183673,0.481991697769337)
--(axis cs:24.1496598639456,0.47368913496967)
--(axis cs:23.8095238095238,0.473915020726685)
--(axis cs:23.469387755102,0.467963531910084)
--(axis cs:23.1292517006803,0.465996608472866)
--(axis cs:22.7891156462585,0.462912622669711)
--(axis cs:22.4489795918367,0.463520506815601)
--(axis cs:22.108843537415,0.457697355013539)
--(axis cs:21.7687074829932,0.447398836615873)
--(axis cs:21.4285714285714,0.446786883556825)
--(axis cs:21.0884353741497,0.442966793961544)
--(axis cs:20.7482993197279,0.441274033287269)
--(axis cs:20.4081632653061,0.43648785818992)
--(axis cs:20.0680272108844,0.434871131146597)
--(axis cs:19.7278911564626,0.433057690766888)
--(axis cs:19.3877551020408,0.428127237788806)
--(axis cs:19.047619047619,0.422781952561202)
--(axis cs:18.7074829931973,0.412334956210587)
--(axis cs:18.3673469387755,0.407473300155769)
--(axis cs:18.0272108843537,0.397348165461421)
--(axis cs:17.687074829932,0.39202805892861)
--(axis cs:17.3469387755102,0.378742609693999)
--(axis cs:17.0068027210884,0.378288663251322)
--(axis cs:16.6666666666667,0.372032572361771)
--(axis cs:16.3265306122449,0.368786723477685)
--(axis cs:15.9863945578231,0.370207626747796)
--(axis cs:15.6462585034014,0.370740687043282)
--(axis cs:15.3061224489796,0.373324399603043)
--(axis cs:14.9659863945578,0.357402456574517)
--(axis cs:14.6258503401361,0.352968444821238)
--(axis cs:14.2857142857143,0.350205005679551)
--(axis cs:13.9455782312925,0.347428418516132)
--(axis cs:13.6054421768707,0.339844117287386)
--(axis cs:13.265306122449,0.335016997687083)
--(axis cs:12.9251700680272,0.315306654781206)
--(axis cs:12.5850340136054,0.309030919922254)
--(axis cs:12.2448979591837,0.294415106455568)
--(axis cs:11.9047619047619,0.293869435872559)
--(axis cs:11.5646258503401,0.280922834048816)
--(axis cs:11.2244897959184,0.275230030334385)
--(axis cs:10.8843537414966,0.269269863003038)
--(axis cs:10.5442176870748,0.255146786685043)
--(axis cs:10.2040816326531,0.245967912639448)
--(axis cs:9.86394557823129,0.242622159661421)
--(axis cs:9.52380952380952,0.236979114656661)
--(axis cs:9.18367346938775,0.237661829262526)
--(axis cs:8.84353741496599,0.231435657928966)
--(axis cs:8.50340136054422,0.227544607721987)
--(axis cs:8.16326530612245,0.233372445886806)
--(axis cs:7.82312925170068,0.23357835706404)
--(axis cs:7.48299319727891,0.230913157358728)
--(axis cs:7.14285714285714,0.229778347577684)
--(axis cs:6.80272108843537,0.231631744099876)
--(axis cs:6.46258503401361,0.222487548732665)
--(axis cs:6.12244897959184,0.213255994921807)
--(axis cs:5.78231292517007,0.210389320827186)
--(axis cs:5.4421768707483,0.207707607968033)
--(axis cs:5.10204081632653,0.202339030975996)
--(axis cs:4.76190476190476,0.20449844271286)
--(axis cs:4.42176870748299,0.19532395179414)
--(axis cs:4.08163265306122,0.182811839239619)
--(axis cs:3.74149659863946,0.160365650661478)
--(axis cs:3.40136054421769,0.153322150024663)
--(axis cs:3.06122448979592,0.141974239795465)
--(axis cs:2.72108843537415,0.130540455448962)
--(axis cs:2.38095238095238,0.121174413371487)
--(axis cs:2.04081632653061,0.111446263667161)
--(axis cs:1.70068027210884,0.101198176320844)
--(axis cs:1.36054421768707,0.0933702648199704)
--(axis cs:1.02040816326531,0.0946729350189904)
--(axis cs:0.680272108843537,0.0935580378862995)
--(axis cs:0.340136054421769,0.0815813970917657)
--(axis cs:0,0.0832299222939681)
--cycle;


==> img/stl10/stl10_rate_distortion_afw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color3, mark=diamond, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table {%
0 0.718670983910561
0.340136054421769 0.711473882645369
0.680272108843537 0.686118887811899
1.02040816326531 0.642163221091032
1.36054421768707 0.587262811660767
1.70068027210884 0.527474558588583
2.04081632653061 0.479074528269412
2.38095238095238 0.438210982724631
2.72108843537415 0.404767129916436
3.06122448979592 0.370111898170634
3.40136054421769 0.334137044261219
3.74149659863946 0.301615391497495
4.08163265306122 0.271873825949983
4.42176870748299 0.248057530278058
4.76190476190476 0.227627642115151
5.10204081632653 0.207011031369506
5.4421768707483 0.188759972221121
5.78231292517007 0.17473539665167
6.12244897959184 0.160383890279229
6.46258503401361 0.149385902586537
6.80272108843537 0.137799529776679
7.14285714285714 0.126836621390904
7.48299319727891 0.115816594856429
7.82312925170068 0.111869036160917
8.16326530612245 0.10370374695669
8.50340136054422 0.0988663417603579
8.84353741496599 0.0934550065522524
9.18367346938775 0.0882714789345151
9.52380952380952 0.0840443165168133
9.86394557823129 0.0820082230485116
10.2040816326531 0.0795760714839034
10.5442176870748 0.0761567731407586
10.8843537414966 0.0728373919745509
11.2244897959184 0.0682229637082768
11.5646258503401 0.0688033647051262
11.9047619047619 0.0649637239599772
12.2448979591837 0.0618912101072555
12.5850340136054 0.0603132132758491
12.9251700680272 0.0591393106944259
13.265306122449 0.0580105412099664
13.6054421768707 0.0546507988164861
13.9455782312925 0.0529721265635929
14.2857142857143 0.0520940791373828
14.6258503401361 0.0506302540074342
14.9659863945578 0.0511931340511821
15.3061224489796 0.0503906657735752
15.6462585034014 0.0483840539615918
15.9863945578231 0.0474983360002085
16.3265306122449 0.0480406822053328
16.6666666666667 0.0476538003003958
17.0068027210884 0.0485886253276163
17.3469387755102 0.0491474115113154
17.687074829932 0.0499372283744657
18.0272108843537 0.0498618137525777
18.3673469387755 0.0506711478583808
18.7074829931973 0.0514458428584223
19.047619047619 0.0506897272302468
19.3877551020408 0.0510817303724313
19.7278911564626 0.0522903523164245
20.0680272108844 0.0532479089195635
20.4081632653061 0.0531648652252802
20.7482993197279 0.0529298994352947
21.0884353741497 0.0525936221080037
21.4285714285714 0.0538103531962811
21.7687074829932 0.0530729580464249
22.108843537415 0.0528414649805543
22.4489795918367 0.0532406594986698
22.7891156462585 0.0548413023839083
23.1292517006803 0.0549048284460279
23.469387755102 0.0547565981746204
23.8095238095238 0.0550943013178783
24.1496598639456 0.0567688250944164
24.4897959183673 0.0564069681592851
24.8299319727891 0.0575715375432205
25.1700680272109 0.056713307504298
25.5102040816327 0.0580689522244902
25.8503401360544 0.0594974391137214
26.1904761904762 0.0606163298936799
26.530612244898 0.0612290498216893
26.8707482993197 0.0623650806541517
27.2108843537415 0.0638100613769122
27.5510204081633 0.064773844674478
27.891156462585 0.0663827834614266
28.2312925170068 0.0681618766013262
28.5714285714286 0.067668224398452
28.9115646258503 0.0668570339215481
29.2517006802721 0.0692998992345984
29.5918367346939 0.0711369936264333
29.9319727891156 0.0715401792343736
30.2721088435374 0.0720719693017796
30.6122448979592 0.0719836458606296
30.952380952381 0.070028828058217
31.2925170068027 0.0711114609819037
31.6326530612245 0.070685933567225
31.9727891156463 0.0698094080973788
32.312925170068 0.0703293793422088
32.6530612244898 0.0701675901261587
32.9931972789116 0.0700209995192182
33.3333333333333 0.0702408746948115
33.6734693877551 0.0700870813725123
34.0136054421769 0.0711136954419529
34.3537414965986 0.0717758646754669
34.6938775510204 0.0725212045848299
35.0340136054422 0.0737023604483949
35.3741496598639 0.073811474058147
35.7142857142857 0.0747611040834267
36.0544217687075 0.0739129403400581
36.3945578231292 0.0737349733506942
36.734693877551 0.073510746299604
37.0748299319728 0.0746751616490315
37.4149659863946 0.0760387753222419
37.7551020408163 0.0755910395236914
38.0952380952381 0.0767319800109788
38.4353741496599 0.0776435108077048
38.7755102040816 0.0791810224379147
39.1156462585034 0.0784417507337265
39.4557823129252 0.0798692651602941
39.7959183673469 0.080451004831233
40.1360544217687 0.0805861093318451
40.4761904761905 0.0820963216136403
40.8163265306122 0.0815528579399882
41.156462585034 0.0829597354499767
41.4965986394558 0.083371227213381
41.8367346938776 0.0823545494933729
42.1768707482993 0.0841413537287046
42.5170068027211 0.0844273868906363
42.8571428571429 0.0855421095868604
43.1972789115646 0.0855668964755483
43.5374149659864 0.085966865013871
43.8775510204082 0.0860439335259356
44.2176870748299 0.0873090124339748
44.5578231292517 0.0874175518288399
44.8979591836735 0.0878898953044511
45.2380952380952 0.0874949945326055
45.578231292517 0.0875934419331594
45.9183673469388 0.0884353133303515
46.2585034013605 0.088296159909561
46.5986394557823 0.0890604489452755
46.9387755102041 0.0899311931627096
47.2789115646259 0.0894242130855673
47.6190476190476 0.0897530626936673
47.9591836734694 0.0902516287278658
48.2993197278912 0.0905777905451987
48.6394557823129 0.0891654843221724
48.9795918367347 0.0907795233446729
49.3197278911565 0.0902309313486739
49.6598639455782 0.0903217065128613
50 0.0902439630631551
50.3401360544218 0.0895281316826624
50.6802721088435 0.0897950950921913
51.0204081632653 0.089772144421403
51.3605442176871 0.088962379056896
51.7006802721088 0.0892676266256492
52.0408163265306 0.088684590193246
52.3809523809524 0.0891749017646858
52.7210884353741 0.0892120414347714
53.0612244897959 0.0900691326364211
53.4013605442177 0.0906002062321085
53.7414965986395 0.0898484535686518
54.0816326530612 0.0894590695968744
54.421768707483 0.0887786291829575
54.7619047619048 0.0883921146436842
55.1020408163265 0.0880686530734077
55.4421768707483 0.0875302890473154
55.7823129251701 0.0883881130162688
56.1224489795918 0.0881877549958634
56.4625850340136 0.0873536988666532
56.8027210884354 0.0875660178095836
57.1428571428571 0.0857481533936894
57.4829931972789 0.0859045312502593
57.8231292517007 0.0851412686512335
58.1632653061224 0.084980581045899
58.5034013605442 0.083778936761384
58.843537414966 0.0836187103002046
59.1836734693878 0.0826497506837425
59.5238095238095 0.0807605399318451
59.8639455782313 0.0807992963848757
60.2040816326531 0.0804272457557709
60.5442176870748 0.0802033600348675
60.8843537414966 0.0809865084617994
61.2244897959184 0.080329855198999
61.5646258503401 0.0809908603788271
61.9047619047619 0.0802861855049627
62.2448979591837 0.0790793191715431
62.5850340136054 0.0780172575167074
62.9251700680272 0.0772484924058806
63.265306122449 0.0784047394873859
63.6054421768707 0.076565618325495
63.9455782312925 0.0773421378458267
64.2857142857143 0.0776559826082322
64.6258503401361 0.0764359671936753
64.9659863945578 0.0764904950304667
65.3061224489796 0.0754894117596605
65.6462585034014 0.0761573887191569
65.9863945578231 0.0769075459503796
66.3265306122449 0.0770867968280064
66.6666666666667 0.0764684703133204
67.0068027210884 0.0773428571910676
67.3469387755102 0.0767441830957422
67.687074829932 0.0775577981530673
68.0272108843537 0.0764332728793513
68.3673469387755 0.076927587826472
68.7074829931973 0.0764344279719168
69.0476190476191 0.0772348218171935
69.3877551020408 0.0786540767955072
69.7278911564626 0.0805937739854379
70.0680272108844 0.0796592244332388
70.4081632653061 0.0792664137784868
70.7482993197279 0.0801183537134179
71.0884353741497 0.0798979153034329
71.4285714285714 0.0798971882874225
71.7687074829932 0.0792866453916039
72.108843537415 0.0773363174123906
72.4489795918367 0.0775397057540132
72.7891156462585 0.0758260843353861
73.1292517006803 0.0738350386918957
73.469387755102 0.0738007400842488
73.8095238095238 0.0737775069649079
74.1496598639456 0.0724459178209946
74.4897959183673 0.0703521985907136
74.8299319727891 0.0699716167027583
75.1700680272109 0.0691533556021987
75.5102040816327 0.0674199337224214
75.8503401360544 0.0639453714050025
76.1904761904762 0.0612050386152487
76.530612244898 0.0599551152861485
76.8707482993197 0.0585693850389951
77.2108843537415 0.0573726309707807
77.5510204081633 0.0543438109577248
77.891156462585 0.053216988777881
78.2312925170068 0.0506146647512331
78.5714285714286 0.0493606983805269
78.9115646258503 0.048697268523748
79.2517006802721 0.0472552127044633
79.5918367346939 0.0444131468742003
79.9319727891156 0.0425197665389153
80.2721088435374 0.0425009253034284
80.6122448979592 0.0416468470588106
80.9523809523809 0.0394957955621825
81.2925170068027 0.0395690321563383
81.6326530612245 0.0370360170536505
81.9727891156463 0.0356241832897
82.312925170068 0.0352638903750599
82.6530612244898 0.0345419265530459
82.9931972789116 0.0331066442740722
83.3333333333333 0.032319038744183
83.6734693877551 0.030884862125226
84.0136054421769 0.0301880240905985
84.3537414965986 0.0292170035115401
84.6938775510204 0.0280553705646427
85.0340136054422 0.0272452452478393
85.3741496598639 0.0262966892407129
85.7142857142857 0.0260627282012465
86.0544217687075 0.0242316645027277
86.3945578231292 0.0242352575290177
86.734693877551 0.0234899150060938
87.0748299319728 0.0227164646408912
87.4149659863945 0.0211681086925307
87.7551020408163 0.0204402402663727
88.0952380952381 0.0190730361200659
88.4353741496599 0.0183180256332629
88.7755102040816 0.0168562027605225
89.1156462585034 0.0160029070091941
89.4557823129252 0.0158436683830462
89.7959183673469 0.0148355194609879
90.1360544217687 0.0141895312423154
90.4761904761905 0.0138965618521936
90.8163265306122 0.0132670937996589
91.156462585034 0.0126543652461207
91.4965986394558 0.0125566992654689
91.8367346938775 0.0120384723628656
92.1768707482993 0.0115745086643154
92.5170068027211 0.0106733490031857
92.8571428571429 0.00999919295337978
93.1972789115646 0.00954824337081132
93.5374149659864 0.00902128996328277
93.8775510204082 0.00795707181510225
94.2176870748299 0.00743996515959214
94.5578231292517 0.00661529251367073
94.8979591836735 0.00607217721951198
95.2380952380952 0.00541200648988911
95.578231292517 0.00493212838054201
95.9183673469388 0.00439118884924129
96.2585034013605 0.00390784331008357
96.5986394557823 0.00356423959176207
96.9387755102041 0.00277582130471936
97.2789115646258 0.0024189932120796
97.6190476190476 0.00195730666898419
97.9591836734694 0.00173238490657096
98.2993197278912 0.00134987719980834
98.6394557823129 0.00107146039724775
98.9795918367347 0.000669813774945502
99.3197278911565 0.000306820894005391
99.6598639455782 0.000140114102259303
100 1.46300749293005e-13
};
\path [fill=color3, fill opacity=0.25]
(axis cs:0,0.720538036392947)
--(axis cs:0,0.716803931428174)
--(axis cs:0.340136054421769,0.709374044169042)
--(axis cs:0.680272108843537,0.682859395479514)
--(axis cs:1.02040816326531,0.637710460486514)
--(axis cs:1.36054421768707,0.582193859741076)
--(axis cs:1.70068027210884,0.522029884674568)
--(axis cs:2.04081632653061,0.474008832519362)
--(axis cs:2.38095238095238,0.433302292186015)
--(axis cs:2.72108843537415,0.399704536458859)
--(axis cs:3.06122448979592,0.364550479705698)
--(axis cs:3.40136054421769,0.328151321598237)
--(axis cs:3.74149659863946,0.295450810361)
--(axis cs:4.08163265306122,0.265797350112481)
--(axis cs:4.42176870748299,0.242085164682461)
--(axis cs:4.76190476190476,0.221575975737695)
--(axis cs:5.10204081632653,0.201176692836083)
--(axis cs:5.4421768707483,0.182925448705998)
--(axis cs:5.78231292517007,0.169060253062223)
--(axis cs:6.12244897959184,0.1545359812381)
--(axis cs:6.46258503401361,0.143881143402082)
--(axis cs:6.80272108843537,0.132423741256948)
--(axis cs:7.14285714285714,0.121784371241002)
--(axis cs:7.48299319727891,0.110937323942493)
--(axis cs:7.82312925170068,0.107203086583703)
--(axis cs:8.16326530612245,0.0991149793433584)
--(axis cs:8.50340136054422,0.0945737157330915)
--(axis cs:8.84353741496599,0.0890185590190976)
--(axis cs:9.18367346938775,0.0837577332677467)
--(axis cs:9.52380952380952,0.0796049597782858)
--(axis cs:9.86394557823129,0.0776514280149612)
--(axis cs:10.2040816326531,0.0750005372777849)
--(axis cs:10.5442176870748,0.0716376319664789)
--(axis cs:10.8843537414966,0.0685186731263353)
--(axis cs:11.2244897959184,0.063742778367849)
--(axis cs:11.5646258503401,0.0641494579545138)
--(axis cs:11.9047619047619,0.0605803654597811)
--(axis cs:12.2448979591837,0.0575360108000879)
--(axis cs:12.5850340136054,0.055773456443944)
--(axis cs:12.9251700680272,0.0547239448023695)
--(axis cs:13.265306122449,0.0534788238517565)
--(axis cs:13.6054421768707,0.0502345322446561)
--(axis cs:13.9455782312925,0.0488454069255346)
--(axis cs:14.2857142857143,0.0480603520818855)
--(axis cs:14.6258503401361,0.0466189815082851)
--(axis cs:14.9659863945578,0.0473016985568757)
--(axis cs:15.3061224489796,0.0467282550654761)
--(axis cs:15.6462585034014,0.0446824703988602)
--(axis cs:15.9863945578231,0.0438525634965042)
--(axis cs:16.3265306122449,0.0443038356728874)
--(axis cs:16.6666666666667,0.0440764600689215)
--(axis cs:17.0068027210884,0.0451995683235397)
--(axis cs:17.3469387755102,0.0459091297328011)
--(axis cs:17.687074829932,0.0464037574325445)
--(axis cs:18.0272108843537,0.0462752547132298)
--(axis cs:18.3673469387755,0.0472577711917278)
--(axis cs:18.7074829931973,0.0480908670886891)
--(axis cs:19.047619047619,0.0471637910228708)
--(axis cs:19.3877551020408,0.0477116289751617)
--(axis cs:19.7278911564626,0.0488021576589244)
--(axis cs:20.0680272108844,0.049921093302224)
--(axis cs:20.4081632653061,0.0498468020590196)
--(axis cs:20.7482993197279,0.0493966750033027)
--(axis cs:21.0884353741497,0.0491135037431173)
--(axis cs:21.4285714285714,0.0502834230573977)
--(axis cs:21.7687074829932,0.0495238996608808)
--(axis cs:22.108843537415,0.0493699964412087)
--(axis cs:22.4489795918367,0.0497348563892678)
--(axis cs:22.7891156462585,0.0514045960539809)
--(axis cs:23.1292517006803,0.0514370034203726)
--(axis cs:23.469387755102,0.0513510461736353)
--(axis cs:23.8095238095238,0.0516538432932307)
--(axis cs:24.1496598639456,0.0531611087044179)
--(axis cs:24.4897959183673,0.0529773342349305)
--(axis cs:24.8299319727891,0.0540753112331443)
--(axis cs:25.1700680272109,0.0532946700124639)
--(axis cs:25.5102040816327,0.0545937173879822)
--(axis cs:25.8503401360544,0.0559808129232109)
--(axis cs:26.1904761904762,0.05701771571708)
--(axis cs:26.530612244898,0.0575927599396446)
--(axis cs:26.8707482993197,0.0587001779392819)
--(axis cs:27.2108843537415,0.060336071928597)
--(axis cs:27.5510204081633,0.061340200962104)
--(axis cs:27.891156462585,0.0632187890458779)
--(axis cs:28.2312925170068,0.0647317050141062)
--(axis cs:28.5714285714286,0.0644645657810405)
--(axis cs:28.9115646258503,0.0635579806351805)
--(axis cs:29.2517006802721,0.0660634679696942)
--(axis cs:29.5918367346939,0.0678491258780661)
--(axis cs:29.9319727891156,0.0682372690635672)
--(axis cs:30.2721088435374,0.0687603814425488)
--(axis cs:30.6122448979592,0.0688831291381419)
--(axis cs:30.952380952381,0.0668980970532781)
--(axis cs:31.2925170068027,0.0681693558373469)
--(axis cs:31.6326530612245,0.0677060456624687)
--(axis cs:31.9727891156463,0.066848432840276)
--(axis cs:32.312925170068,0.0672750760269479)
--(axis cs:32.6530612244898,0.067203380281714)
--(axis cs:32.9931972789116,0.0672160853269292)
--(axis cs:33.3333333333333,0.0673169393701705)
--(axis cs:33.6734693877551,0.0672340302834534)
--(axis cs:34.0136054421769,0.0684300979300542)
--(axis cs:34.3537414965986,0.0688809960331241)
--(axis cs:34.6938775510204,0.0695063554037478)
--(axis cs:35.0340136054422,0.0708765467903735)
--(axis cs:35.3741496598639,0.0710515557937382)
--(axis cs:35.7142857142857,0.0719102484206649)
--(axis cs:36.0544217687075,0.0711932273063364)
--(axis cs:36.3945578231292,0.0710138976971833)
--(axis cs:36.734693877551,0.0705911987211121)
--(axis cs:37.0748299319728,0.0718002721534131)
--(axis cs:37.4149659863946,0.0730895712956779)
--(axis cs:37.7551020408163,0.0726722103291621)
--(axis cs:38.0952380952381,0.0737859935906768)
--(axis cs:38.4353741496599,0.0748685751267454)
--(axis cs:38.7755102040816,0.076286373470019)
--(axis cs:39.1156462585034,0.0754861171485443)
--(axis cs:39.4557823129252,0.0768086007217795)
--(axis cs:39.7959183673469,0.077373368173879)
--(axis cs:40.1360544217687,0.0777691066555796)
--(axis cs:40.4761904761905,0.0790578372245335)
--(axis cs:40.8163265306122,0.0786622517187759)
--(axis cs:41.156462585034,0.0799294960912246)
--(axis cs:41.4965986394558,0.0804415375407198)
--(axis cs:41.8367346938776,0.0793443857399761)
--(axis cs:42.1768707482993,0.0811791875808655)
--(axis cs:42.5170068027211,0.0815389618812198)
--(axis cs:42.8571428571429,0.0826656460795094)
--(axis cs:43.1972789115646,0.082592002999198)
--(axis cs:43.5374149659864,0.0829035459679863)
--(axis cs:43.8775510204082,0.0830065006319012)
--(axis cs:44.2176870748299,0.0842288641111805)
--(axis cs:44.5578231292517,0.0843953243313058)
--(axis cs:44.8979591836735,0.0848808416944975)
--(axis cs:45.2380952380952,0.084455052262245)
--(axis cs:45.578231292517,0.0846130376337175)
--(axis cs:45.9183673469388,0.0853606688217385)
--(axis cs:46.2585034013605,0.0852104190907794)
--(axis cs:46.5986394557823,0.0859352372188351)
--(axis cs:46.9387755102041,0.0867722414867484)
--(axis cs:47.2789115646259,0.0863809555831129)
--(axis cs:47.6190476190476,0.0865108389550247)
--(axis cs:47.9591836734694,0.087141121473071)
--(axis cs:48.2993197278912,0.087364494441925)
--(axis cs:48.6394557823129,0.0860923065000073)
--(axis cs:48.9795918367347,0.0875890941675685)
--(axis cs:49.3197278911565,0.0871470120411094)
--(axis cs:49.6598639455782,0.0872436080938662)
--(axis cs:50,0.0869800109494151)
--(axis cs:50.3401360544218,0.0864701491673063)
--(axis cs:50.6802721088435,0.0865844838843077)
--(axis cs:51.0204081632653,0.0866329173792325)
--(axis cs:51.3605442176871,0.0856737794979032)
--(axis cs:51.7006802721088,0.0859802568283621)
--(axis cs:52.0408163265306,0.0854623743317642)
--(axis cs:52.3809523809524,0.0859713761570419)
--(axis cs:52.7210884353741,0.0860671967294336)
--(axis cs:53.0612244897959,0.0865803366253829)
--(axis cs:53.4013605442177,0.0873393963904043)
--(axis cs:53.7414965986395,0.0865806908008222)
--(axis cs:54.0816326530612,0.0862477481000738)
--(axis cs:54.421768707483,0.0854483013510602)
--(axis cs:54.7619047619048,0.0851367810505602)
--(axis cs:55.1020408163265,0.0848154512533392)
--(axis cs:55.4421768707483,0.0842905639936916)
--(axis cs:55.7823129251701,0.0849996080704352)
--(axis cs:56.1224489795918,0.0849336873770957)
--(axis cs:56.4625850340136,0.0841835155853638)
--(axis cs:56.8027210884354,0.0842427459382866)
--(axis cs:57.1428571428571,0.0826439043239925)
--(axis cs:57.4829931972789,0.0826675770336131)
--(axis cs:57.8231292517007,0.0817711661472696)
--(axis cs:58.1632653061224,0.0816331603061288)
--(axis cs:58.5034013605442,0.0803689277351196)
--(axis cs:58.843537414966,0.0800220471475167)
--(axis cs:59.1836734693878,0.0792202604403957)
--(axis cs:59.5238095238095,0.0777842402236577)
--(axis cs:59.8639455782313,0.0777704893989374)
--(axis cs:60.2040816326531,0.0772466820878607)
--(axis cs:60.5442176870748,0.0771422539388538)
--(axis cs:60.8843537414966,0.0779069407241205)
--(axis cs:61.2244897959184,0.0771861672264275)
--(axis cs:61.5646258503401,0.0776951717465114)
--(axis cs:61.9047619047619,0.0769543248426967)
--(axis cs:62.2448979591837,0.0760347761192563)
--(axis cs:62.5850340136054,0.0749196944452507)
--(axis cs:62.9251700680272,0.0742798296181956)
--(axis cs:63.265306122449,0.0752483035247769)
--(axis cs:63.6054421768707,0.0739132759753423)
--(axis cs:63.9455782312925,0.0746414181603254)
--(axis cs:64.2857142857143,0.0750154467594809)
--(axis cs:64.6258503401361,0.0739958934974985)
--(axis cs:64.9659863945578,0.0739282252635655)
--(axis cs:65.3061224489796,0.0732441195861741)
--(axis cs:65.6462585034014,0.0735009784636719)
--(axis cs:65.9863945578231,0.0743763782692051)
--(axis cs:66.3265306122449,0.0748132421870497)
--(axis cs:66.6666666666667,0.0742312908429877)
--(axis cs:67.0068027210884,0.0748464527717712)
--(axis cs:67.3469387755102,0.0744725189540461)
--(axis cs:67.687074829932,0.0750256638725401)
--(axis cs:68.0272108843537,0.0740321940677583)
--(axis cs:68.3673469387755,0.0744272254915328)
--(axis cs:68.7074829931973,0.0738313722793454)
--(axis cs:69.0476190476191,0.0745228101848168)
--(axis cs:69.3877551020408,0.0758098244891343)
--(axis cs:69.7278911564626,0.0777028245073874)
--(axis cs:70.0680272108844,0.0768447069047592)
--(axis cs:70.4081632653061,0.0762871659647722)
--(axis cs:70.7482993197279,0.07712994256189)
--(axis cs:71.0884353741497,0.076784711881883)
--(axis cs:71.4285714285714,0.0768294398770105)
--(axis cs:71.7687074829932,0.0761833815678859)
--(axis cs:72.108843537415,0.0740466125108198)
--(axis cs:72.4489795918367,0.0743092787594783)
--(axis cs:72.7891156462585,0.0726720989637505)
--(axis cs:73.1292517006803,0.0707179125550727)
--(axis cs:73.469387755102,0.0705304442546703)
--(axis cs:73.8095238095238,0.0707084386670457)
--(axis cs:74.1496598639456,0.0694069227370268)
--(axis cs:74.4897959183673,0.0672253975595991)
--(axis cs:74.8299319727891,0.0670640810231434)
--(axis cs:75.1700680272109,0.0661672581430292)
--(axis cs:75.5102040816327,0.0645030419474868)
--(axis cs:75.8503401360544,0.0610279073501293)
--(axis cs:76.1904761904762,0.0582518371830168)
--(axis cs:76.530612244898,0.0571171087092818)
--(axis cs:76.8707482993197,0.0557392236629494)
--(axis cs:77.2108843537415,0.0544009994118612)
--(axis cs:77.5510204081633,0.0514261263060732)
--(axis cs:77.891156462585,0.0504530418124732)
--(axis cs:78.2312925170068,0.0479990952911457)
--(axis cs:78.5714285714286,0.0466583285983559)
--(axis cs:78.9115646258503,0.0457885886697657)
--(axis cs:79.2517006802721,0.0445160585887523)
--(axis cs:79.5918367346939,0.0417573337050238)
--(axis cs:79.9319727891156,0.0400714148039727)
--(axis cs:80.2721088435374,0.040032692934947)
--(axis cs:80.6122448979592,0.0389983359630654)
--(axis cs:80.9523809523809,0.0371386448905033)
--(axis cs:81.2925170068027,0.0372608619947837)
--(axis cs:81.6326530612245,0.0348312889321255)
--(axis cs:81.9727891156463,0.0334647616599668)
--(axis cs:82.312925170068,0.0330868756571709)
--(axis cs:82.6530612244898,0.0325052239017587)
--(axis cs:82.9931972789116,0.0310975698422091)
--(axis cs:83.3333333333333,0.0304462282795543)
--(axis cs:83.6734693877551,0.0289952665526173)
--(axis cs:84.0136054421769,0.028434454254361)
--(axis cs:84.3537414965986,0.027519829014709)
--(axis cs:84.6938775510204,0.0264555206056342)
--(axis cs:85.0340136054422,0.0256509961563505)
--(axis cs:85.3741496598639,0.024635888211981)
--(axis cs:85.7142857142857,0.0244381010712088)
--(axis cs:86.0544217687075,0.0226640057072263)
--(axis cs:86.3945578231292,0.0227612557309323)
--(axis cs:86.734693877551,0.0220412105200894)
--(axis cs:87.0748299319728,0.021186626580711)
--(axis cs:87.4149659863945,0.0197392587022657)
--(axis cs:87.7551020408163,0.0190009637718143)
--(axis cs:88.0952380952381,0.0177570980623368)
--(axis cs:88.4353741496599,0.0169518841805151)
--(axis cs:88.7755102040816,0.0156460420587022)
--(axis cs:89.1156462585034,0.0147951893803246)
--(axis cs:89.4557823129252,0.0145966269556959)
--(axis cs:89.7959183673469,0.0137600773523087)
--(axis cs:90.1360544217687,0.0131625050684816)
--(axis cs:90.4761904761905,0.0128733383096692)
--(axis cs:90.8163265306122,0.0121963586263146)
--(axis cs:91.156462585034,0.0115507209406451)
--(axis cs:91.4965986394558,0.0114596665792919)
--(axis cs:91.8367346938775,0.0109919236170916)
--(axis cs:92.1768707482993,0.0105988822988171)
--(axis cs:92.5170068027211,0.00968310679106684)
--(axis cs:92.8571428571429,0.00908153547968216)
--(axis cs:93.1972789115646,0.00861145628841966)
--(axis cs:93.5374149659864,0.00816300669797086)
--(axis cs:93.8775510204082,0.00705859971604542)
--(axis cs:94.2176870748299,0.00654765640096965)
--(axis cs:94.5578231292517,0.00576924806959645)
--(axis cs:94.8979591836735,0.00523695131018201)
--(axis cs:95.2380952380952,0.00472113236021906)
--(axis cs:95.578231292517,0.00418091986101551)
--(axis cs:95.9183673469388,0.00371639645608884)
--(axis cs:96.2585034013605,0.00332149355030544)
--(axis cs:96.5986394557823,0.00294717753991291)
--(axis cs:96.9387755102041,0.00230074595056338)
--(axis cs:97.2789115646258,0.00198424335002018)
--(axis cs:97.6190476190476,0.00160527554070608)
--(axis cs:97.9591836734694,0.00138534915828667)
--(axis cs:98.2993197278912,0.00107440095217596)
--(axis cs:98.6394557823129,0.00083066719509725)
--(axis cs:98.9795918367347,0.000499140156497934)
--(axis cs:99.3197278911565,0.00020780892789528)
--(axis cs:99.6598639455782,8.79816930877488e-05)
--(axis cs:100,1.46300749293005e-13)
--(axis cs:100,1.46300749293005e-13)
--(axis cs:100,1.46300749293005e-13)
--(axis cs:99.6598639455782,0.000192246511430858)
--(axis cs:99.3197278911565,0.000405832860115501)
--(axis cs:98.9795918367347,0.000840487393393071)
--(axis cs:98.6394557823129,0.00131225359939825)
--(axis cs:98.2993197278912,0.00162535344744072)
--(axis cs:97.9591836734694,0.00207942065485525)
--(axis cs:97.6190476190476,0.00230933779726231)
--(axis cs:97.2789115646258,0.00285374307413903)
--(axis cs:96.9387755102041,0.00325089665887534)
--(axis cs:96.5986394557823,0.00418130164361122)
--(axis cs:96.2585034013605,0.00449419306986171)
--(axis cs:95.9183673469388,0.00506598124239373)
--(axis cs:95.578231292517,0.0056833369000685)
--(axis cs:95.2380952380952,0.00610288061955916)
--(axis cs:94.8979591836735,0.00690740312884195)
--(axis cs:94.5578231292517,0.007461336957745)
--(axis cs:94.2176870748299,0.00833227391821463)
--(axis cs:93.8775510204082,0.00885554391415908)
--(axis cs:93.5374149659864,0.00987957322859468)
--(axis cs:93.1972789115646,0.010485030453203)
--(axis cs:92.8571428571429,0.0109168504270774)
--(axis cs:92.5170068027211,0.0116635912153046)
--(axis cs:92.1768707482993,0.0125501350298137)
--(axis cs:91.8367346938775,0.0130850211086396)
--(axis cs:91.4965986394558,0.0136537319516458)
--(axis cs:91.156462585034,0.0137580095515963)
--(axis cs:90.8163265306122,0.0143378289730031)
--(axis cs:90.4761904761905,0.014919785394718)
--(axis cs:90.1360544217687,0.0152165574161493)
--(axis cs:89.7959183673469,0.0159109615696672)
--(axis cs:89.4557823129252,0.0170907098103965)
--(axis cs:89.1156462585034,0.0172106246380637)
--(axis cs:88.7755102040816,0.0180663634623429)
--(axis cs:88.4353741496599,0.0196841670860106)
--(axis cs:88.0952380952381,0.020388974177795)
--(axis cs:87.7551020408163,0.0218795167609311)
--(axis cs:87.4149659863945,0.0225969586827956)
--(axis cs:87.0748299319728,0.0242463027010714)
--(axis cs:86.734693877551,0.0249386194920983)
--(axis cs:86.3945578231292,0.0257092593271031)
--(axis cs:86.0544217687075,0.025799323298229)
--(axis cs:85.7142857142857,0.0276873553312843)
--(axis cs:85.3741496598639,0.0279574902694448)
--(axis cs:85.0340136054422,0.0288394943393281)
--(axis cs:84.6938775510204,0.0296552205236512)
--(axis cs:84.3537414965986,0.0309141780083713)
--(axis cs:84.0136054421769,0.0319415939268361)
--(axis cs:83.6734693877551,0.0327744576978347)
--(axis cs:83.3333333333333,0.0341918492088117)
--(axis cs:82.9931972789116,0.0351157187059353)
--(axis cs:82.6530612244898,0.0365786292043331)
--(axis cs:82.312925170068,0.0374409050929489)
--(axis cs:81.9727891156463,0.0377836049194332)
--(axis cs:81.6326530612245,0.0392407451751754)
--(axis cs:81.2925170068027,0.0418772023178928)
--(axis cs:80.9523809523809,0.0418529462338617)
--(axis cs:80.6122448979592,0.0442953581545557)
--(axis cs:80.2721088435374,0.0449691576719098)
--(axis cs:79.9319727891156,0.0449681182738579)
--(axis cs:79.5918367346939,0.0470689600433769)
--(axis cs:79.2517006802721,0.0499943668201742)
--(axis cs:78.9115646258503,0.0516059483777304)
--(axis cs:78.5714285714286,0.0520630681626978)
--(axis cs:78.2312925170068,0.0532302342113206)
--(axis cs:77.891156462585,0.0559809357432888)
--(axis cs:77.5510204081633,0.0572614956093763)
--(axis cs:77.2108843537415,0.0603442625297001)
--(axis cs:76.8707482993197,0.0613995464150408)
--(axis cs:76.530612244898,0.0627931218630153)
--(axis cs:76.1904761904762,0.0641582400474805)
--(axis cs:75.8503401360544,0.0668628354598757)
--(axis cs:75.5102040816327,0.0703368254973559)
--(axis cs:75.1700680272109,0.0721394530613681)
--(axis cs:74.8299319727891,0.0728791523823733)
--(axis cs:74.4897959183673,0.0734789996218282)
--(axis cs:74.1496598639456,0.0754849129049625)
--(axis cs:73.8095238095238,0.07684657526277)
--(axis cs:73.469387755102,0.0770710359138274)
--(axis cs:73.1292517006803,0.0769521648287188)
--(axis cs:72.7891156462585,0.0789800697070217)
--(axis cs:72.4489795918367,0.0807701327485481)
--(axis cs:72.108843537415,0.0806260223139613)
--(axis cs:71.7687074829932,0.0823899092153219)
--(axis cs:71.4285714285714,0.0829649366978344)
--(axis cs:71.0884353741497,0.0830111187249827)
--(axis cs:70.7482993197279,0.0831067648649457)
--(axis cs:70.4081632653061,0.0822456615922014)
--(axis cs:70.0680272108844,0.0824737419617185)
--(axis cs:69.7278911564626,0.0834847234634883)
--(axis cs:69.3877551020408,0.0814983291018802)
--(axis cs:69.0476190476191,0.0799468334495701)
--(axis cs:68.7074829931973,0.0790374836644882)
--(axis cs:68.3673469387755,0.0794279501614113)
--(axis cs:68.0272108843537,0.0788343516909443)
--(axis cs:67.687074829932,0.0800899324335945)
--(axis cs:67.3469387755102,0.0790158472374384)
--(axis cs:67.0068027210884,0.079839261610364)
--(axis cs:66.6666666666667,0.0787056497836531)
--(axis cs:66.3265306122449,0.0793603514689631)
--(axis cs:65.9863945578231,0.0794387136315542)
--(axis cs:65.6462585034014,0.0788137989746418)
--(axis cs:65.3061224489796,0.0777347039331469)
--(axis cs:64.9659863945578,0.0790527647973679)
--(axis cs:64.6258503401361,0.0788760408898522)
--(axis cs:64.2857142857143,0.0802965184569835)
--(axis cs:63.9455782312925,0.080042857531328)
--(axis cs:63.6054421768707,0.0792179606756478)
--(axis cs:63.265306122449,0.0815611754499948)
--(axis cs:62.9251700680272,0.0802171551935656)
--(axis cs:62.5850340136054,0.0811148205881641)
--(axis cs:62.2448979591837,0.0821238622238299)
--(axis cs:61.9047619047619,0.0836180461672286)
--(axis cs:61.5646258503401,0.0842865490111427)
--(axis cs:61.2244897959184,0.0834735431715705)
--(axis cs:60.8843537414966,0.0840660761994783)
--(axis cs:60.5442176870748,0.0832644661308812)
--(axis cs:60.2040816326531,0.0836078094236812)
--(axis cs:59.8639455782313,0.0838281033708141)
--(axis cs:59.5238095238095,0.0837368396400326)
--(axis cs:59.1836734693878,0.0860792409270893)
--(axis cs:58.843537414966,0.0872153734528924)
--(axis cs:58.5034013605442,0.0871889457876484)
--(axis cs:58.1632653061224,0.0883280017856691)
--(axis cs:57.8231292517007,0.0885113711551975)
--(axis cs:57.4829931972789,0.0891414854669054)
--(axis cs:57.1428571428571,0.0888524024633863)
--(axis cs:56.8027210884354,0.0908892896808806)
--(axis cs:56.4625850340136,0.0905238821479426)
--(axis cs:56.1224489795918,0.0914418226146311)
--(axis cs:55.7823129251701,0.0917766179621023)
--(axis cs:55.4421768707483,0.0907700141009393)
--(axis cs:55.1020408163265,0.0913218548934761)
--(axis cs:54.7619047619048,0.0916474482368082)
--(axis cs:54.421768707483,0.0921089570148549)
--(axis cs:54.0816326530612,0.092670391093675)
--(axis cs:53.7414965986395,0.0931162163364814)
--(axis cs:53.4013605442177,0.0938610160738126)
--(axis cs:53.0612244897959,0.0935579286474593)
--(axis cs:52.7210884353741,0.0923568861401093)
--(axis cs:52.3809523809524,0.0923784273723298)
--(axis cs:52.0408163265306,0.0919068060547278)
--(axis cs:51.7006802721088,0.0925549964229363)
--(axis cs:51.3605442176871,0.0922509786158888)
--(axis cs:51.0204081632653,0.0929113714635735)
--(axis cs:50.6802721088435,0.0930057063000748)
--(axis cs:50.3401360544218,0.0925861141980184)
--(axis cs:50,0.0935079151768951)
--(axis cs:49.6598639455782,0.0933998049318565)
--(axis cs:49.3197278911565,0.0933148506562384)
--(axis cs:48.9795918367347,0.0939699525217773)
--(axis cs:48.6394557823129,0.0922386621443375)
--(axis cs:48.2993197278912,0.0937910866484725)
--(axis cs:47.9591836734694,0.0933621359826606)
--(axis cs:47.6190476190476,0.0929952864323099)
--(axis cs:47.2789115646259,0.0924674705880217)
--(axis cs:46.9387755102041,0.0930901448386708)
--(axis cs:46.5986394557823,0.0921856606717158)
--(axis cs:46.2585034013605,0.0913819007283427)
--(axis cs:45.9183673469388,0.0915099578389646)
--(axis cs:45.578231292517,0.0905738462326014)
--(axis cs:45.2380952380952,0.0905349368029661)
--(axis cs:44.8979591836735,0.0908989489144046)
--(axis cs:44.5578231292517,0.090439779326374)
--(axis cs:44.2176870748299,0.0903891607567692)
--(axis cs:43.8775510204082,0.0890813664199699)
--(axis cs:43.5374149659864,0.0890301840597558)
--(axis cs:43.1972789115646,0.0885417899518986)
--(axis cs:42.8571428571429,0.0884185730942114)
--(axis cs:42.5170068027211,0.0873158119000529)
--(axis cs:42.1768707482993,0.0871035198765436)
--(axis cs:41.8367346938776,0.0853647132467696)
--(axis cs:41.4965986394558,0.0863009168860422)
--(axis cs:41.156462585034,0.0859899748087287)
--(axis cs:40.8163265306122,0.0844434641612005)
--(axis cs:40.4761904761905,0.085134806002747)
--(axis cs:40.1360544217687,0.0834031120081107)
--(axis cs:39.7959183673469,0.083528641488587)
--(axis cs:39.4557823129252,0.0829299295988088)
--(axis cs:39.1156462585034,0.0813973843189087)
--(axis cs:38.7755102040816,0.0820756714058105)
--(axis cs:38.4353741496599,0.0804184464886643)
--(axis cs:38.0952380952381,0.0796779664312808)
--(axis cs:37.7551020408163,0.0785098687182208)
--(axis cs:37.4149659863946,0.0789879793488058)
--(axis cs:37.0748299319728,0.0775500511446499)
--(axis cs:36.734693877551,0.076430293878096)
--(axis cs:36.3945578231292,0.0764560490042051)
--(axis cs:36.0544217687075,0.0766326533737798)
--(axis cs:35.7142857142857,0.0776119597461884)
--(axis cs:35.3741496598639,0.0765713923225558)
--(axis cs:35.0340136054422,0.0765281741064163)
--(axis cs:34.6938775510204,0.0755360537659121)
--(axis cs:34.3537414965986,0.0746707333178097)
--(axis cs:34.0136054421769,0.0737972929538515)
--(axis cs:33.6734693877551,0.0729401324615713)
--(axis cs:33.3333333333333,0.0731648100194525)
--(axis cs:32.9931972789116,0.0728259137115072)
--(axis cs:32.6530612244898,0.0731317999706034)
--(axis cs:32.312925170068,0.0733836826574698)
--(axis cs:31.9727891156463,0.0727703833544816)
--(axis cs:31.6326530612245,0.0736658214719813)
--(axis cs:31.2925170068027,0.0740535661264604)
--(axis cs:30.952380952381,0.0731595590631559)
--(axis cs:30.6122448979592,0.0750841625831173)
--(axis cs:30.2721088435374,0.0753835571610105)
--(axis cs:29.9319727891156,0.07484308940518)
--(axis cs:29.5918367346939,0.0744248613748004)
--(axis cs:29.2517006802721,0.0725363304995025)
--(axis cs:28.9115646258503,0.0701560872079158)
--(axis cs:28.5714285714286,0.0708718830158636)
--(axis cs:28.2312925170068,0.0715920481885463)
--(axis cs:27.891156462585,0.0695467778769754)
--(axis cs:27.5510204081633,0.0682074883868519)
--(axis cs:27.2108843537415,0.0672840508252275)
--(axis cs:26.8707482993197,0.0660299833690215)
--(axis cs:26.530612244898,0.0648653397037339)
--(axis cs:26.1904761904762,0.0642149440702798)
--(axis cs:25.8503401360544,0.0630140653042319)
--(axis cs:25.5102040816327,0.0615441870609983)
--(axis cs:25.1700680272109,0.060131944996132)
--(axis cs:24.8299319727891,0.0610677638532968)
--(axis cs:24.4897959183673,0.0598366020836396)
--(axis cs:24.1496598639456,0.0603765414844149)
--(axis cs:23.8095238095238,0.0585347593425259)
--(axis cs:23.469387755102,0.0581621501756054)
--(axis cs:23.1292517006803,0.0583726534716832)
--(axis cs:22.7891156462585,0.0582780087138356)
--(axis cs:22.4489795918367,0.0567464626080718)
--(axis cs:22.108843537415,0.0563129335198999)
--(axis cs:21.7687074829932,0.0566220164319691)
--(axis cs:21.4285714285714,0.0573372833351644)
--(axis cs:21.0884353741497,0.05607374047289)
--(axis cs:20.7482993197279,0.0564631238672868)
--(axis cs:20.4081632653061,0.0564829283915409)
--(axis cs:20.0680272108844,0.0565747245369029)
--(axis cs:19.7278911564626,0.0557785469739246)
--(axis cs:19.3877551020408,0.0544518317697009)
--(axis cs:19.047619047619,0.0542156634376227)
--(axis cs:18.7074829931973,0.0548008186281556)
--(axis cs:18.3673469387755,0.0540845245250337)
--(axis cs:18.0272108843537,0.0534483727919256)
--(axis cs:17.687074829932,0.0534706993163869)
--(axis cs:17.3469387755102,0.0523856932898296)
--(axis cs:17.0068027210884,0.0519776823316929)
--(axis cs:16.6666666666667,0.0512311405318701)
--(axis cs:16.3265306122449,0.0517775287377782)
--(axis cs:15.9863945578231,0.0511441085039129)
--(axis cs:15.6462585034014,0.0520856375243234)
--(axis cs:15.3061224489796,0.0540530764816743)
--(axis cs:14.9659863945578,0.0550845695454886)
--(axis cs:14.6258503401361,0.0546415265065832)
--(axis cs:14.2857142857143,0.05612780619288)
--(axis cs:13.9455782312925,0.0570988462016511)
--(axis cs:13.6054421768707,0.0590670653883162)
--(axis cs:13.265306122449,0.0625422585681764)
--(axis cs:12.9251700680272,0.0635546765864823)
--(axis cs:12.5850340136054,0.0648529701077542)
--(axis cs:12.2448979591837,0.0662464094144232)
--(axis cs:11.9047619047619,0.0693470824601733)
--(axis cs:11.5646258503401,0.0734572714557385)
--(axis cs:11.2244897959184,0.0727031490487045)
--(axis cs:10.8843537414966,0.0771561108227665)
--(axis cs:10.5442176870748,0.0806759143150383)
--(axis cs:10.2040816326531,0.0841516056900219)
--(axis cs:9.86394557823129,0.086365018082062)
--(axis cs:9.52380952380952,0.0884836732553407)
--(axis cs:9.18367346938775,0.0927852246012835)
--(axis cs:8.84353741496599,0.0978914540854072)
--(axis cs:8.50340136054422,0.103158967787624)
--(axis cs:8.16326530612245,0.108292514570022)
--(axis cs:7.82312925170068,0.11653498573813)
--(axis cs:7.48299319727891,0.120695865770365)
--(axis cs:7.14285714285714,0.131888871540807)
--(axis cs:6.80272108843537,0.14317531829641)
--(axis cs:6.46258503401361,0.154890661770992)
--(axis cs:6.12244897959184,0.166231799320358)
--(axis cs:5.78231292517007,0.180410540241117)
--(axis cs:5.4421768707483,0.194594495736244)
--(axis cs:5.10204081632653,0.212845369902929)
--(axis cs:4.76190476190476,0.233679308492607)
--(axis cs:4.42176870748299,0.254029895873654)
--(axis cs:4.08163265306122,0.277950301787486)
--(axis cs:3.74149659863946,0.307779972633989)
--(axis cs:3.40136054421769,0.340122766924202)
--(axis cs:3.06122448979592,0.375673316635569)
--(axis cs:2.72108843537415,0.409829723374012)
--(axis cs:2.38095238095238,0.443119673263248)
--(axis cs:2.04081632653061,0.484140224019461)
--(axis cs:1.70068027210884,0.532919232502598)
--(axis cs:1.36054421768707,0.592331763580458)
--(axis cs:1.02040816326531,0.64661598169555)
--(axis cs:0.680272108843537,0.689378380144284)
--(axis cs:0.340136054421769,0.713573721121695)
--(axis cs:0,0.720538036392947)
--cycle;


==> img/stl10/stl10_rate_distortion_deeptaylor.tex <==
% deep taylor
\addplot [line width=0.5, opacity=0.8, color5, mark=x, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color5, thin}]
table [row sep=\\]{%
0	0.718709116876125 \\
0.340136054421769	0.721584549844265 \\
0.680272108843537	0.716515600532293 \\
1.02040816326531	0.708872469961643 \\
1.36054421768707	0.695491641759872 \\
1.70068027210884	0.679935432672501 \\
2.04081632653061	0.663438960313797 \\
2.38095238095238	0.648496651947498 \\
2.72108843537415	0.632322228774428 \\
3.06122448979592	0.612712177354842 \\
3.40136054421769	0.596337399575859 \\
3.74149659863946	0.582979703056626 \\
4.08163265306122	0.569534293464385 \\
4.42176870748299	0.557669462631457 \\
4.76190476190476	0.548784368946217 \\
5.10204081632653	0.540615187324584 \\
5.4421768707483	0.530820775837638 \\
5.78231292517007	0.520970110758208 \\
6.12244897959184	0.512339565390721 \\
6.46258503401361	0.50357594181085 \\
6.80272108843537	0.492668363044504 \\
7.14285714285714	0.478136880075035 \\
7.48299319727891	0.4689855364908 \\
7.82312925170068	0.459726879600785 \\
8.16326530612245	0.449005307935877 \\
8.50340136054422	0.440473086135462 \\
8.84353741496599	0.429852619681769 \\
9.18367346938775	0.419816940478631 \\
9.52380952380952	0.410728930535988 \\
9.86394557823129	0.401948026021964 \\
10.2040816326531	0.393910140393591 \\
10.5442176870748	0.381556897605024 \\
10.8843537414966	0.377336940736932 \\
11.2244897959184	0.370769011372322 \\
11.5646258503401	0.363656560117779 \\
11.9047619047619	0.358942168624199 \\
12.2448979591837	0.352870531634399 \\
12.5850340136054	0.344638112936682 \\
12.9251700680272	0.339838095207715 \\
13.265306122449	0.336172443421747 \\
13.6054421768707	0.328666946524008 \\
13.9455782312925	0.325446931629685 \\
14.2857142857143	0.320247302334119 \\
14.6258503401361	0.313771207019954 \\
14.9659863945578	0.309830238429395 \\
15.3061224489796	0.302719018500784 \\
15.6462585034014	0.301069062698032 \\
15.9863945578231	0.295276926349979 \\
16.3265306122449	0.293136988822143 \\
16.6666666666667	0.289017570752894 \\
17.0068027210884	0.286909781572826 \\
17.3469387755102	0.286169723121884 \\
17.687074829932	0.284036719011842 \\
18.0272108843537	0.283490705016881 \\
18.3673469387755	0.281347848437214 \\
18.7074829931973	0.279821985595476 \\
19.047619047619	0.277254151591064 \\
19.3877551020408	0.271538263319501 \\
19.7278911564626	0.26902859706206 \\
20.0680272108844	0.265446934383666 \\
20.4081632653061	0.261694309143863 \\
20.7482993197279	0.259128944006517 \\
21.0884353741497	0.257138474351071 \\
21.4285714285714	0.25451611429978 \\
21.7687074829932	0.250771273188401 \\
22.108843537415	0.245322401097933 \\
22.4489795918367	0.243618272443835 \\
22.7891156462585	0.23994489391713 \\
23.1292517006803	0.235994095149861 \\
23.469387755102	0.232544599395394 \\
23.8095238095238	0.230020195992375 \\
24.1496598639456	0.226558045922163 \\
24.4897959183673	0.224230741407377 \\
24.8299319727891	0.222917651209628 \\
25.1700680272109	0.218852364002008 \\
25.5102040816327	0.216402512332897 \\
25.8503401360544	0.214743480113303 \\
26.1904761904762	0.212173316519688 \\
26.530612244898	0.208606845119472 \\
26.8707482993197	0.208227099231378 \\
27.2108843537415	0.204158769947967 \\
27.5510204081633	0.202700421569173 \\
27.891156462585	0.20304549330425 \\
28.2312925170068	0.200049371425999 \\
28.5714285714286	0.197026289891327 \\
28.9115646258503	0.19478219780106 \\
29.2517006802721	0.193021243666817 \\
29.5918367346939	0.189393522823262 \\
29.9319727891156	0.185612927095613 \\
30.2721088435374	0.183265942575569 \\
30.6122448979592	0.178300218014841 \\
30.952380952381	0.1750928559253 \\
31.2925170068027	0.172600167792562 \\
31.6326530612245	0.171271394846013 \\
31.9727891156463	0.168910355202394 \\
32.312925170068	0.165617946626004 \\
32.6530612244898	0.164923688304723 \\
32.9931972789116	0.162880235779702 \\
33.3333333333333	0.160922060652498 \\
33.6734693877551	0.161012781860939 \\
34.0136054421769	0.160295497087096 \\
34.3537414965986	0.160157363050179 \\
34.6938775510204	0.157615125788327 \\
35.0340136054422	0.155690706501798 \\
35.3741496598639	0.153393038911884 \\
35.7142857142857	0.150916474750461 \\
36.0544217687075	0.149222676322753 \\
36.3945578231292	0.145572521083098 \\
36.734693877551	0.144081672091303 \\
37.0748299319728	0.141597653392155 \\
37.4149659863946	0.139636070252305 \\
37.7551020408163	0.136902245938771 \\
38.0952380952381	0.13238716434966 \\
38.4353741496599	0.129309276673296 \\
38.7755102040816	0.125476978721606 \\
39.1156462585034	0.123487752162652 \\
39.4557823129252	0.120109906817452 \\
39.7959183673469	0.116354210543834 \\
40.1360544217687	0.114019437542618 \\
40.4761904761905	0.111379869751286 \\
40.8163265306122	0.108768349134118 \\
41.156462585034	0.107693821419669 \\
41.4965986394558	0.104486311213831 \\
41.8367346938776	0.103788014630221 \\
42.1768707482993	0.103210110738298 \\
42.5170068027211	0.0996413952826109 \\
42.8571428571429	0.0954361168259122 \\
43.1972789115646	0.094683985576771 \\
43.5374149659864	0.0913963143014342 \\
43.8775510204082	0.0895473473162373 \\
44.2176870748299	0.0881380871004874 \\
44.5578231292517	0.0874073452522095 \\
44.8979591836735	0.084976719749279 \\
45.2380952380952	0.0836313684792298 \\
45.578231292517	0.0817726321620687 \\
45.9183673469388	0.0811407417898967 \\
46.2585034013605	0.0789953215610973 \\
46.5986394557823	0.0771542676515572 \\
46.9387755102041	0.0757181153142307 \\
47.2789115646259	0.075483440373874 \\
47.6190476190476	0.0737574248404215 \\
47.9591836734694	0.0725441933594222 \\
48.2993197278912	0.0718029538255617 \\
48.6394557823129	0.0684054822589328 \\
48.9795918367347	0.0678630198647779 \\
49.3197278911565	0.0665391221547302 \\
49.6598639455782	0.0644853644133574 \\
50	0.0634273959758882 \\
50.3401360544218	0.0627585223215535 \\
50.6802721088435	0.0618360747059815 \\
51.0204081632653	0.0605053240063417 \\
51.3605442176871	0.0595899019151696 \\
51.7006802721088	0.0571088220199139 \\
52.0408163265306	0.0569339827556859 \\
52.3809523809524	0.0555591226255856 \\
52.7210884353741	0.0548195571929102 \\
53.0612244897959	0.053284141805819 \\
53.4013605442177	0.0528133247800574 \\
53.7414965986395	0.0518742535702025 \\
54.0816326530612	0.0505502805571485 \\
54.421768707483	0.049642026854922 \\
54.7619047619048	0.0484478630592264 \\
55.1020408163265	0.0473766045073566 \\
55.4421768707483	0.046574748557745 \\
55.7823129251701	0.0460360730727068 \\
56.1224489795918	0.0455550180854848 \\
56.4625850340136	0.044527170703989 \\
56.8027210884354	0.0433119690109432 \\
57.1428571428571	0.0427717351934375 \\
57.4829931972789	0.0409523281180375 \\
57.8231292517007	0.0402887185413129 \\
58.1632653061224	0.0391582500243622 \\
58.5034013605442	0.0384331815454695 \\
58.843537414966	0.0378184460225467 \\
59.1836734693878	0.0373256708285753 \\
59.5238095238095	0.0363839958077602 \\
59.8639455782313	0.035400757886393 \\
60.2040816326531	0.0343337100528584 \\
60.5442176870748	0.0337647365114677 \\
60.8843537414966	0.0331723325369373 \\
61.2244897959184	0.0317454324818598 \\
61.5646258503401	0.0312423789901818 \\
61.9047619047619	0.0312443008569686 \\
62.2448979591837	0.0314956231249373 \\
62.5850340136054	0.0303264739463191 \\
62.9251700680272	0.0294284756210986 \\
63.265306122449	0.0288580634303362 \\
63.6054421768707	0.0285315276573018 \\
63.9455782312925	0.0278710748773975 \\
64.2857142857143	0.0275012856089272 \\
64.6258503401361	0.026560898826255 \\
64.9659863945578	0.0261127635367819 \\
65.3061224489796	0.0250837766073517 \\
65.6462585034014	0.0244247229037872 \\
65.9863945578231	0.023655220985394 \\
66.3265306122449	0.0237177846022221 \\
66.6666666666667	0.0225928274986005 \\
67.0068027210884	0.0225727797298288 \\
67.3469387755102	0.0221645592451687 \\
67.687074829932	0.0215960953733993 \\
68.0272108843537	0.0207640413200639 \\
68.3673469387755	0.0201419077482443 \\
68.7074829931973	0.0196794418403408 \\
69.0476190476191	0.0193159553532751 \\
69.3877551020408	0.0188223594966692 \\
69.7278911564626	0.0181700405023898 \\
70.0680272108844	0.0177360886818407 \\
70.4081632653061	0.0178904351144147 \\
70.7482993197279	0.0171770952144993 \\
71.0884353741497	0.017200068908159 \\
71.4285714285714	0.0171276197013227 \\
71.7687074829932	0.0168077460699498 \\
72.108843537415	0.0167494671016724 \\
72.4489795918367	0.0165257341120723 \\
72.7891156462585	0.0163122208468511 \\
73.1292517006803	0.0164357825466713 \\
73.469387755102	0.016107329305834 \\
73.8095238095238	0.0163489642897647 \\
74.1496598639456	0.015790420102871 \\
74.4897959183673	0.0158060255027277 \\
74.8299319727891	0.0155171030741789 \\
75.1700680272109	0.0153386546225788 \\
75.5102040816327	0.0149255533896598 \\
75.8503401360544	0.0146213198990701 \\
76.1904761904762	0.0139941179276977 \\
76.530612244898	0.0135523211306966 \\
76.8707482993197	0.0131408135511479 \\
77.2108843537415	0.0130419863390752 \\
77.5510204081633	0.0122048847863763 \\
77.891156462585	0.0117982104460907 \\
78.2312925170068	0.0111709129004724 \\
78.5714285714286	0.0103925108510319 \\
78.9115646258503	0.0102826469985554 \\
79.2517006802721	0.00983586327212123 \\
79.5918367346939	0.00924617396471263 \\
79.9319727891156	0.00912067624839507 \\
80.2721088435374	0.00839853086851539 \\
80.6122448979592	0.00839979973803368 \\
80.9523809523809	0.0078338370443439 \\
81.2925170068027	0.00732599169702021 \\
81.6326530612245	0.00714085036792663 \\
81.9727891156463	0.0067617056605973 \\
82.312925170068	0.00614289975664826 \\
82.6530612244898	0.00589916690989853 \\
82.9931972789116	0.00560131242633721 \\
83.3333333333333	0.0054491650701035 \\
83.6734693877551	0.00504019701522659 \\
84.0136054421769	0.00492468511425622 \\
84.3537414965986	0.00473708205522448 \\
84.6938775510204	0.00475594353842739 \\
85.0340136054422	0.0049423471001264 \\
85.3741496598639	0.00487696186211623 \\
85.7142857142857	0.00508490491958115 \\
86.0544217687075	0.00527114525755254 \\
86.3945578231292	0.00511220558871075 \\
86.734693877551	0.00516342787039112 \\
87.0748299319728	0.00507115807012196 \\
87.4149659863945	0.00496061399478582 \\
87.7551020408163	0.00467194455220892 \\
88.0952380952381	0.00478250075649321 \\
88.4353741496599	0.00459989896510282 \\
88.7755102040816	0.00433735864623763 \\
89.1156462585034	0.00425786100832914 \\
89.4557823129252	0.00417461231506216 \\
89.7959183673469	0.00392089996544448 \\
90.1360544217687	0.00370182291885186 \\
90.4761904761905	0.00363851114194827 \\
90.8163265306122	0.00359952173822158 \\
91.156462585034	0.00338428545419609 \\
91.4965986394558	0.00327585099973992 \\
91.8367346938775	0.00322478953446625 \\
92.1768707482993	0.00313725229766808 \\
92.5170068027211	0.00306498683633422 \\
92.8571428571429	0.00310372606698049 \\
93.1972789115646	0.00298560357177841 \\
93.5374149659864	0.00289123416431327 \\
93.8775510204082	0.00288333203459891 \\
94.2176870748299	0.00268697138137026 \\
94.5578231292517	0.0026886256421205 \\
94.8979591836735	0.00249726552117603 \\
95.2380952380952	0.00249691817785924 \\
95.578231292517	0.00227356683868458 \\
95.9183673469388	0.00225274820247399 \\
96.2585034013605	0.00199703071507813 \\
96.5986394557823	0.00184669182147886 \\
96.9387755102041	0.0017506750768562 \\
97.2789115646258	0.00162823147641761 \\
97.6190476190476	0.00132817860529685 \\
97.9591836734694	0.00110743844924748 \\
98.2993197278912	0.000934253483174021 \\
98.6394557823129	0.000831285118241835 \\
98.9795918367347	0.000630858779471216 \\
99.3197278911565	0.000498075976967395 \\
99.6598639455782	0.000254487822980423 \\
100	1.49018575257287e-13 \\
};
\path [fill=color5, fill opacity=0.5] (axis cs:0,0.720499093376582)
--(axis cs:0,0.716919140375669)
--(axis cs:0.340136054421769,0.719562699338624)
--(axis cs:0.680272108843537,0.714119588039492)
--(axis cs:1.02040816326531,0.706131815354419)
--(axis cs:1.36054421768707,0.692219445946857)
--(axis cs:1.70068027210884,0.676271659004469)
--(axis cs:2.04081632653061,0.659448074437166)
--(axis cs:2.38095238095238,0.644467380646779)
--(axis cs:2.72108843537415,0.628137354571778)
--(axis cs:3.06122448979592,0.608323067860219)
--(axis cs:3.40136054421769,0.591686379382593)
--(axis cs:3.74149659863946,0.578424223490447)
--(axis cs:4.08163265306122,0.564890586544798)
--(axis cs:4.42176870748299,0.552983107126633)
--(axis cs:4.76190476190476,0.544143744111161)
--(axis cs:5.10204081632653,0.535943917129258)
--(axis cs:5.4421768707483,0.526086742653053)
--(axis cs:5.78231292517007,0.516021801015269)
--(axis cs:6.12244897959184,0.507447160181567)
--(axis cs:6.46258503401361,0.498533714978585)
--(axis cs:6.80272108843537,0.487556564733258)
--(axis cs:7.14285714285714,0.47302765483524)
--(axis cs:7.48299319727891,0.463839194503858)
--(axis cs:7.82312925170068,0.454722875760943)
--(axis cs:8.16326530612245,0.443858689777248)
--(axis cs:8.50340136054422,0.435256991554746)
--(axis cs:8.84353741496599,0.424802787693144)
--(axis cs:9.18367346938775,0.414429792119547)
--(axis cs:9.52380952380952,0.405221070174151)
--(axis cs:9.86394557823129,0.396264269402979)
--(axis cs:10.2040816326531,0.388355264627676)
--(axis cs:10.5442176870748,0.375848360209264)
--(axis cs:10.8843537414966,0.371533855875553)
--(axis cs:11.2244897959184,0.365235719028424)
--(axis cs:11.5646258503401,0.357962149118917)
--(axis cs:11.9047619047619,0.353320808113379)
--(axis cs:12.2448979591837,0.347314155260209)
--(axis cs:12.5850340136054,0.339252885441852)
--(axis cs:12.9251700680272,0.334293936696064)
--(axis cs:13.265306122449,0.330507902912728)
--(axis cs:13.6054421768707,0.323284026871112)
--(axis cs:13.9455782312925,0.320084729778303)
--(axis cs:14.2857142857143,0.314989799597903)
--(axis cs:14.6258503401361,0.308750188206267)
--(axis cs:14.9659863945578,0.304748377311055)
--(axis cs:15.3061224489796,0.2977133296087)
--(axis cs:15.6462585034014,0.296230390481429)
--(axis cs:15.9863945578231,0.29057237961224)
--(axis cs:16.3265306122449,0.288361540799066)
--(axis cs:16.6666666666667,0.284332092761573)
--(axis cs:17.0068027210884,0.282362475086476)
--(axis cs:17.3469387755102,0.281593776064614)
--(axis cs:17.687074829932,0.279603478724749)
--(axis cs:18.0272108843537,0.279026038747516)
--(axis cs:18.3673469387755,0.276722209984976)
--(axis cs:18.7074829931973,0.275244876184471)
--(axis cs:19.047619047619,0.272646071383094)
--(axis cs:19.3877551020408,0.267084302223097)
--(axis cs:19.7278911564626,0.264517808159)
--(axis cs:20.0680272108844,0.261004812074339)
--(axis cs:20.4081632653061,0.257275412883592)
--(axis cs:20.7482993197279,0.254670079182233)
--(axis cs:21.0884353741497,0.2525599294275)
--(axis cs:21.4285714285714,0.249909290228725)
--(axis cs:21.7687074829932,0.246176018813503)
--(axis cs:22.108843537415,0.240952547911358)
--(axis cs:22.4489795918367,0.239129664204911)
--(axis cs:22.7891156462585,0.235621786956305)
--(axis cs:23.1292517006803,0.231615856890512)
--(axis cs:23.469387755102,0.228124299063676)
--(axis cs:23.8095238095238,0.225555079526649)
--(axis cs:24.1496598639456,0.222245324408686)
--(axis cs:24.4897959183673,0.219920702462595)
--(axis cs:24.8299319727891,0.218722360764198)
--(axis cs:25.1700680272109,0.214477614314109)
--(axis cs:25.5102040816327,0.212330800806377)
--(axis cs:25.8503401360544,0.210425943382217)
--(axis cs:26.1904761904762,0.207805494725682)
--(axis cs:26.530612244898,0.204461654745545)
--(axis cs:26.8707482993197,0.204095203903935)
--(axis cs:27.2108843537415,0.200059380948693)
--(axis cs:27.5510204081633,0.198702600398619)
--(axis cs:27.891156462585,0.198959970970271)
--(axis cs:28.2312925170068,0.195956225348089)
--(axis cs:28.5714285714286,0.192956060110964)
--(axis cs:28.9115646258503,0.190895100103861)
--(axis cs:29.2517006802721,0.188917066847611)
--(axis cs:29.5918367346939,0.185343017961496)
--(axis cs:29.9319727891156,0.181664081747331)
--(axis cs:30.2721088435374,0.179292920562016)
--(axis cs:30.6122448979592,0.174497517102534)
--(axis cs:30.952380952381,0.171304542924337)
--(axis cs:31.2925170068027,0.168897316982369)
--(axis cs:31.6326530612245,0.167559673896511)
--(axis cs:31.9727891156463,0.165041388013564)
--(axis cs:32.312925170068,0.161722333044885)
--(axis cs:32.6530612244898,0.161191719814515)
--(axis cs:32.9931972789116,0.15910373459958)
--(axis cs:33.3333333333333,0.156942811477715)
--(axis cs:33.6734693877551,0.157031793592207)
--(axis cs:34.0136054421769,0.156387761283419)
--(axis cs:34.3537414965986,0.156071002014286)
--(axis cs:34.6938775510204,0.153765896021943)
--(axis cs:35.0340136054422,0.151789304807792)
--(axis cs:35.3741496598639,0.149430220068088)
--(axis cs:35.7142857142857,0.146980389068046)
--(axis cs:36.0544217687075,0.14542222805537)
--(axis cs:36.3945578231292,0.1417379795096)
--(axis cs:36.734693877551,0.140145162165823)
--(axis cs:37.0748299319728,0.137686061808899)
--(axis cs:37.4149659863946,0.135751814557761)
--(axis cs:37.7551020408163,0.133025487417116)
--(axis cs:38.0952380952381,0.128507831634229)
--(axis cs:38.4353741496599,0.125364008040305)
--(axis cs:38.7755102040816,0.121708299489908)
--(axis cs:39.1156462585034,0.119629154141309)
--(axis cs:39.4557823129252,0.11621040202224)
--(axis cs:39.7959183673469,0.112500751589111)
--(axis cs:40.1360544217687,0.110196680473021)
--(axis cs:40.4761904761905,0.107653220901852)
--(axis cs:40.8163265306122,0.105076182122744)
--(axis cs:41.156462585034,0.103956792176576)
--(axis cs:41.4965986394558,0.100753007875029)
--(axis cs:41.8367346938776,0.100197951682969)
--(axis cs:42.1768707482993,0.0994962193774496)
--(axis cs:42.5170068027211,0.0961704884890744)
--(axis cs:42.8571428571429,0.0918051591013975)
--(axis cs:43.1972789115646,0.090990751455215)
--(axis cs:43.5374149659864,0.0877097114626888)
--(axis cs:43.8775510204082,0.0861773418590011)
--(axis cs:44.2176870748299,0.084807037882237)
--(axis cs:44.5578231292517,0.083935149371645)
--(axis cs:44.8979591836735,0.081659734552392)
--(axis cs:45.2380952380952,0.0803769354847176)
--(axis cs:45.578231292517,0.0784887226831104)
--(axis cs:45.9183673469388,0.0779629997702879)
--(axis cs:46.2585034013605,0.0759404699384835)
--(axis cs:46.5986394557823,0.0739044772864086)
--(axis cs:46.9387755102041,0.0726748128737055)
--(axis cs:47.2789115646259,0.0726154112656923)
--(axis cs:47.6190476190476,0.070776343365298)
--(axis cs:47.9591836734694,0.0695143434409921)
--(axis cs:48.2993197278912,0.0687417876198271)
--(axis cs:48.6394557823129,0.0654202885833515)
--(axis cs:48.9795918367347,0.0650225006258121)
--(axis cs:49.3197278911565,0.0636746679928554)
--(axis cs:49.6598639455782,0.0617460927390162)
--(axis cs:50,0.0605308247707837)
--(axis cs:50.3401360544218,0.060132589755008)
--(axis cs:50.6802721088435,0.0591092295890879)
--(axis cs:51.0204081632653,0.057880721663563)
--(axis cs:51.3605442176871,0.0570723473823213)
--(axis cs:51.7006802721088,0.0547358358965325)
--(axis cs:52.0408163265306,0.0546873904813798)
--(axis cs:52.3809523809524,0.0533926642968669)
--(axis cs:52.7210884353741,0.052614893134662)
--(axis cs:53.0612244897959,0.0510609526512215)
--(axis cs:53.4013605442177,0.0505640958340193)
--(axis cs:53.7414965986395,0.0496773667217738)
--(axis cs:54.0816326530612,0.0483327021787209)
--(axis cs:54.421768707483,0.0474948463310854)
--(axis cs:54.7619047619048,0.0462844249112055)
--(axis cs:55.1020408163265,0.0453426575576432)
--(axis cs:55.4421768707483,0.0444481266143069)
--(axis cs:55.7823129251701,0.0439265039921356)
--(axis cs:56.1224489795918,0.0434841912399931)
--(axis cs:56.4625850340136,0.0424979893866909)
--(axis cs:56.8027210884354,0.0413906514738234)
--(axis cs:57.1428571428571,0.0408303675658621)
--(axis cs:57.4829931972789,0.0391262717712159)
--(axis cs:57.8231292517007,0.0384975959460897)
--(axis cs:58.1632653061224,0.037339590266066)
--(axis cs:58.5034013605442,0.0367043379319906)
--(axis cs:58.843537414966,0.0361174205057431)
--(axis cs:59.1836734693878,0.0357209082422402)
--(axis cs:59.5238095238095,0.0348860370495863)
--(axis cs:59.8639455782313,0.0338370504943344)
--(axis cs:60.2040816326531,0.0328485797492518)
--(axis cs:60.5442176870748,0.0322498999675014)
--(axis cs:60.8843537414966,0.0317422079868848)
--(axis cs:61.2244897959184,0.03035450545201)
--(axis cs:61.5646258503401,0.0298944754486377)
--(axis cs:61.9047619047619,0.0298828173355792)
--(axis cs:62.2448979591837,0.0300568517955999)
--(axis cs:62.5850340136054,0.0289739387916553)
--(axis cs:62.9251700680272,0.0280973376428348)
--(axis cs:63.265306122449,0.0275276387705062)
--(axis cs:63.6054421768707,0.0272162771532809)
--(axis cs:63.9455782312925,0.0265555546241096)
--(axis cs:64.2857142857143,0.02613428441453)
--(axis cs:64.6258503401361,0.0253145303639723)
--(axis cs:64.9659863945578,0.0248502171991721)
--(axis cs:65.3061224489796,0.0238606324231703)
--(axis cs:65.6462585034014,0.0232597124933209)
--(axis cs:65.9863945578231,0.0224272183346278)
--(axis cs:66.3265306122449,0.0226014603886875)
--(axis cs:66.6666666666667,0.0214516568269058)
--(axis cs:67.0068027210884,0.0214265348119985)
--(axis cs:67.3469387755102,0.0210379202712398)
--(axis cs:67.687074829932,0.0205209755140508)
--(axis cs:68.0272108843537,0.0197168764320546)
--(axis cs:68.3673469387755,0.019140472555376)
--(axis cs:68.7074829931973,0.0186800850102706)
--(axis cs:69.0476190476191,0.0183096830371391)
--(axis cs:69.3877551020408,0.0178273067980343)
--(axis cs:69.7278911564626,0.017176333135051)
--(axis cs:70.0680272108844,0.0167635445980979)
--(axis cs:70.4081632653061,0.0169243024045525)
--(axis cs:70.7482993197279,0.0162604402801869)
--(axis cs:71.0884353741497,0.01622665148766)
--(axis cs:71.4285714285714,0.0161966285493986)
--(axis cs:71.7687074829932,0.0158540504401475)
--(axis cs:72.108843537415,0.0158214504008148)
--(axis cs:72.4489795918367,0.0156241336854028)
--(axis cs:72.7891156462585,0.0154472484895037)
--(axis cs:73.1292517006803,0.0155625083697762)
--(axis cs:73.469387755102,0.0152124562417383)
--(axis cs:73.8095238095238,0.0154503709482832)
--(axis cs:74.1496598639456,0.0149453747891476)
--(axis cs:74.4897959183673,0.0149177897154278)
--(axis cs:74.8299319727891,0.0147223668437931)
--(axis cs:75.1700680272109,0.0145273805731093)
--(axis cs:75.5102040816327,0.0141135739923316)
--(axis cs:75.8503401360544,0.0138100362719923)
--(axis cs:76.1904761904762,0.013229902430437)
--(axis cs:76.530612244898,0.0128227963711229)
--(axis cs:76.8707482993197,0.0124064933633888)
--(axis cs:77.2108843537415,0.0122737548886936)
--(axis cs:77.5510204081633,0.0114860650106583)
--(axis cs:77.891156462585,0.0111091979196214)
--(axis cs:78.2312925170068,0.0105191953057382)
--(axis cs:78.5714285714286,0.00968696995156649)
--(axis cs:78.9115646258503,0.00965812616149405)
--(axis cs:79.2517006802721,0.00916764849336291)
--(axis cs:79.5918367346939,0.00861046026893211)
--(axis cs:79.9319727891156,0.00851455632471311)
--(axis cs:80.2721088435374,0.00771896780307818)
--(axis cs:80.6122448979592,0.00782703836092483)
--(axis cs:80.9523809523809,0.00725817363464785)
--(axis cs:81.2925170068027,0.0067595702631752)
--(axis cs:81.6326530612245,0.00661428783034177)
--(axis cs:81.9727891156463,0.00622632797333714)
--(axis cs:82.312925170068,0.00563234582088437)
--(axis cs:82.6530612244898,0.00537961967491755)
--(axis cs:82.9931972789116,0.00513628353688763)
--(axis cs:83.3333333333333,0.00499658105463761)
--(axis cs:83.6734693877551,0.00465321244458577)
--(axis cs:84.0136054421769,0.00454075171324509)
--(axis cs:84.3537414965986,0.004374889618021)
--(axis cs:84.6938775510204,0.00441806567823143)
--(axis cs:85.0340136054422,0.00456486730818331)
--(axis cs:85.3741496598639,0.00451909713216695)
--(axis cs:85.7142857142857,0.00467869512061157)
--(axis cs:86.0544217687075,0.00488084088939858)
--(axis cs:86.3945578231292,0.00470361194055015)
--(axis cs:86.734693877551,0.00477880793540934)
--(axis cs:87.0748299319728,0.00470389734236846)
--(axis cs:87.4149659863945,0.0045971764761912)
--(axis cs:87.7551020408163,0.00432060638794425)
--(axis cs:88.0952380952381,0.00440685837390131)
--(axis cs:88.4353741496599,0.00421358488308408)
--(axis cs:88.7755102040816,0.00400199754677052)
--(axis cs:89.1156462585034,0.00390196520290166)
--(axis cs:89.4557823129252,0.00385106772658659)
--(axis cs:89.7959183673469,0.00361673473266525)
--(axis cs:90.1360544217687,0.00343112102242516)
--(axis cs:90.4761904761905,0.00335506360442881)
--(axis cs:90.8163265306122,0.00332946490294995)
--(axis cs:91.156462585034,0.00309468118799471)
--(axis cs:91.4965986394558,0.00302226067825391)
--(axis cs:91.8367346938775,0.00295734584834777)
--(axis cs:92.1768707482993,0.00288532973467399)
--(axis cs:92.5170068027211,0.00280509200703292)
--(axis cs:92.8571428571429,0.00285367513303484)
--(axis cs:93.1972789115646,0.00273482337822683)
--(axis cs:93.5374149659864,0.00267083653671152)
--(axis cs:93.8775510204082,0.00267358004967812)
--(axis cs:94.2176870748299,0.00247253354001044)
--(axis cs:94.5578231292517,0.00247147001801272)
--(axis cs:94.8979591836735,0.00231048681476585)
--(axis cs:95.2380952380952,0.00229627249955532)
--(axis cs:95.578231292517,0.00210576252259461)
--(axis cs:95.9183673469388,0.00208094681564496)
--(axis cs:96.2585034013605,0.0018515611643677)
--(axis cs:96.5986394557823,0.00170777611286381)
--(axis cs:96.9387755102041,0.00162860866232101)
--(axis cs:97.2789115646258,0.00149885725117984)
--(axis cs:97.6190476190476,0.00120070958319892)
--(axis cs:97.9591836734694,0.00100124838087156)
--(axis cs:98.2993197278912,0.00084779134795758)
--(axis cs:98.6394557823129,0.000755917205024444)
--(axis cs:98.9795918367347,0.000577269270929676)
--(axis cs:99.3197278911565,0.000455356701924074)
--(axis cs:99.6598639455782,0.000220875033620356)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,0.000288100612340489)
--(axis cs:99.3197278911565,0.000540795252010717)
--(axis cs:98.9795918367347,0.000684448288012757)
--(axis cs:98.6394557823129,0.000906653031459225)
--(axis cs:98.2993197278912,0.00102071561839046)
--(axis cs:97.9591836734694,0.0012136285176234)
--(axis cs:97.6190476190476,0.00145564762739478)
--(axis cs:97.2789115646258,0.00175760570165539)
--(axis cs:96.9387755102041,0.00187274149139139)
--(axis cs:96.5986394557823,0.0019856075300939)
--(axis cs:96.2585034013605,0.00214250026578855)
--(axis cs:95.9183673469388,0.00242454958930301)
--(axis cs:95.578231292517,0.00244137115477456)
--(axis cs:95.2380952380952,0.00269756385616315)
--(axis cs:94.8979591836735,0.0026840442275862)
--(axis cs:94.5578231292517,0.00290578126622828)
--(axis cs:94.2176870748299,0.00290140922273007)
--(axis cs:93.8775510204082,0.0030930840195197)
--(axis cs:93.5374149659864,0.00311163179191503)
--(axis cs:93.1972789115646,0.00323638376532998)
--(axis cs:92.8571428571429,0.00335377700092615)
--(axis cs:92.5170068027211,0.00332488166563552)
--(axis cs:92.1768707482993,0.00338917486066218)
--(axis cs:91.8367346938775,0.00349223322058474)
--(axis cs:91.4965986394558,0.00352944132122593)
--(axis cs:91.156462585034,0.00367388972039748)
--(axis cs:90.8163265306122,0.00386957857349321)
--(axis cs:90.4761904761905,0.00392195867946773)
--(axis cs:90.1360544217687,0.00397252481527856)
--(axis cs:89.7959183673469,0.00422506519822371)
--(axis cs:89.4557823129252,0.00449815690353772)
--(axis cs:89.1156462585034,0.00461375681375661)
--(axis cs:88.7755102040816,0.00467271974570475)
--(axis cs:88.4353741496599,0.00498621304712157)
--(axis cs:88.0952380952381,0.00515814313908512)
--(axis cs:87.7551020408163,0.00502328271647358)
--(axis cs:87.4149659863945,0.00532405151338043)
--(axis cs:87.0748299319728,0.00543841879787547)
--(axis cs:86.734693877551,0.00554804780537289)
--(axis cs:86.3945578231292,0.00552079923687135)
--(axis cs:86.0544217687075,0.0056614496257065)
--(axis cs:85.7142857142857,0.00549111471855073)
--(axis cs:85.3741496598639,0.00523482659206551)
--(axis cs:85.0340136054422,0.00531982689206948)
--(axis cs:84.6938775510204,0.00509382139862336)
--(axis cs:84.3537414965986,0.00509927449242796)
--(axis cs:84.0136054421769,0.00530861851526734)
--(axis cs:83.6734693877551,0.00542718158586742)
--(axis cs:83.3333333333333,0.00590174908556939)
--(axis cs:82.9931972789116,0.00606634131578679)
--(axis cs:82.6530612244898,0.0064187141448795)
--(axis cs:82.312925170068,0.00665345369241215)
--(axis cs:81.9727891156463,0.00729708334785747)
--(axis cs:81.6326530612245,0.00766741290551149)
--(axis cs:81.2925170068027,0.00789241313086521)
--(axis cs:80.9523809523809,0.00840950045403994)
--(axis cs:80.6122448979592,0.00897256111514252)
--(axis cs:80.2721088435374,0.00907809393395261)
--(axis cs:79.9319727891156,0.00972679617207704)
--(axis cs:79.5918367346939,0.00988188766049315)
--(axis cs:79.2517006802721,0.0105040780508796)
--(axis cs:78.9115646258503,0.0109071678356168)
--(axis cs:78.5714285714286,0.0110980517504972)
--(axis cs:78.2312925170068,0.0118226304952066)
--(axis cs:77.891156462585,0.0124872229725601)
--(axis cs:77.5510204081633,0.0129237045620944)
--(axis cs:77.2108843537415,0.0138102177894568)
--(axis cs:76.8707482993197,0.013875133738907)
--(axis cs:76.530612244898,0.0142818458902704)
--(axis cs:76.1904761904762,0.0147583334249583)
--(axis cs:75.8503401360544,0.0154326035261479)
--(axis cs:75.5102040816327,0.015737532786988)
--(axis cs:75.1700680272109,0.0161499286720482)
--(axis cs:74.8299319727891,0.0163118393045647)
--(axis cs:74.4897959183673,0.0166942612900276)
--(axis cs:74.1496598639456,0.0166354654165945)
--(axis cs:73.8095238095238,0.0172475576312463)
--(axis cs:73.469387755102,0.0170022023699298)
--(axis cs:73.1292517006803,0.0173090567235663)
--(axis cs:72.7891156462585,0.0171771932041985)
--(axis cs:72.4489795918367,0.0174273345387418)
--(axis cs:72.108843537415,0.01767748380253)
--(axis cs:71.7687074829932,0.0177614416997521)
--(axis cs:71.4285714285714,0.0180586108532469)
--(axis cs:71.0884353741497,0.0181734863286581)
--(axis cs:70.7482993197279,0.0180937501488116)
--(axis cs:70.4081632653061,0.018856567824277)
--(axis cs:70.0680272108844,0.0187086327655835)
--(axis cs:69.7278911564626,0.0191637478697287)
--(axis cs:69.3877551020408,0.019817412195304)
--(axis cs:69.0476190476191,0.0203222276694111)
--(axis cs:68.7074829931973,0.020678798670411)
--(axis cs:68.3673469387755,0.0211433429411126)
--(axis cs:68.0272108843537,0.0218112062080731)
--(axis cs:67.687074829932,0.0226712152327477)
--(axis cs:67.3469387755102,0.0232911982190976)
--(axis cs:67.0068027210884,0.0237190246476591)
--(axis cs:66.6666666666667,0.0237339981702953)
--(axis cs:66.3265306122449,0.0248341088157566)
--(axis cs:65.9863945578231,0.0248832236361603)
--(axis cs:65.6462585034014,0.0255897333142534)
--(axis cs:65.3061224489796,0.0263069207915331)
--(axis cs:64.9659863945578,0.0273753098743917)
--(axis cs:64.6258503401361,0.0278072672885376)
--(axis cs:64.2857142857143,0.0288682868033243)
--(axis cs:63.9455782312925,0.0291865951306853)
--(axis cs:63.6054421768707,0.0298467781613227)
--(axis cs:63.265306122449,0.0301884880901663)
--(axis cs:62.9251700680272,0.0307596135993624)
--(axis cs:62.5850340136054,0.0316790091009829)
--(axis cs:62.2448979591837,0.0329343944542748)
--(axis cs:61.9047619047619,0.032605784378358)
--(axis cs:61.5646258503401,0.0325902825317259)
--(axis cs:61.2244897959184,0.0331363595117095)
--(axis cs:60.8843537414966,0.0346024570869898)
--(axis cs:60.5442176870748,0.0352795730554341)
--(axis cs:60.2040816326531,0.035818840356465)
--(axis cs:59.8639455782313,0.0369644652784516)
--(axis cs:59.5238095238095,0.0378819545659341)
--(axis cs:59.1836734693878,0.0389304334149105)
--(axis cs:58.843537414966,0.0395194715393502)
--(axis cs:58.5034013605442,0.0401620251589484)
--(axis cs:58.1632653061224,0.0409769097826584)
--(axis cs:57.8231292517007,0.0420798411365361)
--(axis cs:57.4829931972789,0.0427783844648591)
--(axis cs:57.1428571428571,0.044713102821013)
--(axis cs:56.8027210884354,0.0452332865480631)
--(axis cs:56.4625850340136,0.0465563520212871)
--(axis cs:56.1224489795918,0.0476258449309765)
--(axis cs:55.7823129251701,0.0481456421532779)
--(axis cs:55.4421768707483,0.0487013705011832)
--(axis cs:55.1020408163265,0.0494105514570699)
--(axis cs:54.7619047619048,0.0506113012072474)
--(axis cs:54.421768707483,0.0517892073787586)
--(axis cs:54.0816326530612,0.0527678589355761)
--(axis cs:53.7414965986395,0.0540711404186313)
--(axis cs:53.4013605442177,0.0550625537260955)
--(axis cs:53.0612244897959,0.0555073309604165)
--(axis cs:52.7210884353741,0.0570242212511585)
--(axis cs:52.3809523809524,0.0577255809543042)
--(axis cs:52.0408163265306,0.0591805750299919)
--(axis cs:51.7006802721088,0.0594818081432953)
--(axis cs:51.3605442176871,0.062107456448018)
--(axis cs:51.0204081632653,0.0631299263491205)
--(axis cs:50.6802721088435,0.064562919822875)
--(axis cs:50.3401360544218,0.065384454888099)
--(axis cs:50,0.0663239671809927)
--(axis cs:49.6598639455782,0.0672246360876986)
--(axis cs:49.3197278911565,0.0694035763166049)
--(axis cs:48.9795918367347,0.0707035391037437)
--(axis cs:48.6394557823129,0.0713906759345141)
--(axis cs:48.2993197278912,0.0748641200312962)
--(axis cs:47.9591836734694,0.0755740432778523)
--(axis cs:47.6190476190476,0.076738506315545)
--(axis cs:47.2789115646259,0.0783514694820557)
--(axis cs:46.9387755102041,0.078761417754756)
--(axis cs:46.5986394557823,0.0804040580167057)
--(axis cs:46.2585034013605,0.0820501731837111)
--(axis cs:45.9183673469388,0.0843184838095055)
--(axis cs:45.578231292517,0.0850565416410269)
--(axis cs:45.2380952380952,0.0868858014737421)
--(axis cs:44.8979591836735,0.0882937049461661)
--(axis cs:44.5578231292517,0.090879541132774)
--(axis cs:44.2176870748299,0.0914691363187378)
--(axis cs:43.8775510204082,0.0929173527734736)
--(axis cs:43.5374149659864,0.0950829171401796)
--(axis cs:43.1972789115646,0.0983772196983271)
--(axis cs:42.8571428571429,0.099067074550427)
--(axis cs:42.5170068027211,0.103112302076148)
--(axis cs:42.1768707482993,0.106924002099146)
--(axis cs:41.8367346938776,0.107378077577473)
--(axis cs:41.4965986394558,0.108219614552632)
--(axis cs:41.156462585034,0.111430850662762)
--(axis cs:40.8163265306122,0.112460516145492)
--(axis cs:40.4761904761905,0.11510651860072)
--(axis cs:40.1360544217687,0.117842194612216)
--(axis cs:39.7959183673469,0.120207669498556)
--(axis cs:39.4557823129252,0.124009411612664)
--(axis cs:39.1156462585034,0.127346350183994)
--(axis cs:38.7755102040816,0.129245657953305)
--(axis cs:38.4353741496599,0.133254545306286)
--(axis cs:38.0952380952381,0.136266497065092)
--(axis cs:37.7551020408163,0.140779004460425)
--(axis cs:37.4149659863946,0.143520325946849)
--(axis cs:37.0748299319728,0.14550924497541)
--(axis cs:36.734693877551,0.148018182016783)
--(axis cs:36.3945578231292,0.149407062656597)
--(axis cs:36.0544217687075,0.153023124590136)
--(axis cs:35.7142857142857,0.154852560432876)
--(axis cs:35.3741496598639,0.15735585775568)
--(axis cs:35.0340136054422,0.159592108195804)
--(axis cs:34.6938775510204,0.16146435555471)
--(axis cs:34.3537414965986,0.164243724086073)
--(axis cs:34.0136054421769,0.164203232890772)
--(axis cs:33.6734693877551,0.164993770129671)
--(axis cs:33.3333333333333,0.164901309827281)
--(axis cs:32.9931972789116,0.166656736959823)
--(axis cs:32.6530612244898,0.168655656794931)
--(axis cs:32.312925170068,0.169513560207123)
--(axis cs:31.9727891156463,0.172779322391223)
--(axis cs:31.6326530612245,0.174983115795515)
--(axis cs:31.2925170068027,0.176303018602756)
--(axis cs:30.952380952381,0.178881168926263)
--(axis cs:30.6122448979592,0.182102918927147)
--(axis cs:30.2721088435374,0.187238964589122)
--(axis cs:29.9319727891156,0.189561772443895)
--(axis cs:29.5918367346939,0.193444027685027)
--(axis cs:29.2517006802721,0.197125420486022)
--(axis cs:28.9115646258503,0.19866929549826)
--(axis cs:28.5714285714286,0.20109651967169)
--(axis cs:28.2312925170068,0.204142517503909)
--(axis cs:27.891156462585,0.207131015638229)
--(axis cs:27.5510204081633,0.206698242739727)
--(axis cs:27.2108843537415,0.20825815894724)
--(axis cs:26.8707482993197,0.212358994558822)
--(axis cs:26.530612244898,0.212752035493398)
--(axis cs:26.1904761904762,0.216541138313694)
--(axis cs:25.8503401360544,0.219061016844389)
--(axis cs:25.5102040816327,0.220474223859418)
--(axis cs:25.1700680272109,0.223227113689906)
--(axis cs:24.8299319727891,0.227112941655058)
--(axis cs:24.4897959183673,0.228540780352159)
--(axis cs:24.1496598639456,0.230870767435639)
--(axis cs:23.8095238095238,0.234485312458101)
--(axis cs:23.469387755102,0.236964899727113)
--(axis cs:23.1292517006803,0.24037233340921)
--(axis cs:22.7891156462585,0.244268000877955)
--(axis cs:22.4489795918367,0.24810688068276)
--(axis cs:22.108843537415,0.249692254284508)
--(axis cs:21.7687074829932,0.2553665275633)
--(axis cs:21.4285714285714,0.259122938370835)
--(axis cs:21.0884353741497,0.261717019274642)
--(axis cs:20.7482993197279,0.2635878088308)
--(axis cs:20.4081632653061,0.266113205404133)
--(axis cs:20.0680272108844,0.269889056692993)
--(axis cs:19.7278911564626,0.273539385965119)
--(axis cs:19.3877551020408,0.275992224415905)
--(axis cs:19.047619047619,0.281862231799033)
--(axis cs:18.7074829931973,0.28439909500648)
--(axis cs:18.3673469387755,0.285973486889452)
--(axis cs:18.0272108843537,0.287955371286245)
--(axis cs:17.687074829932,0.288469959298935)
--(axis cs:17.3469387755102,0.290745670179155)
--(axis cs:17.0068027210884,0.291457088059177)
--(axis cs:16.6666666666667,0.293703048744216)
--(axis cs:16.3265306122449,0.297912436845221)
--(axis cs:15.9863945578231,0.299981473087719)
--(axis cs:15.6462585034014,0.305907734914634)
--(axis cs:15.3061224489796,0.307724707392868)
--(axis cs:14.9659863945578,0.314912099547735)
--(axis cs:14.6258503401361,0.318792225833641)
--(axis cs:14.2857142857143,0.325504805070335)
--(axis cs:13.9455782312925,0.330809133481067)
--(axis cs:13.6054421768707,0.334049866176905)
--(axis cs:13.265306122449,0.341836983930766)
--(axis cs:12.9251700680272,0.345382253719366)
--(axis cs:12.5850340136054,0.350023340431512)
--(axis cs:12.2448979591837,0.358426908008588)
--(axis cs:11.9047619047619,0.364563529135018)
--(axis cs:11.5646258503401,0.369350971116641)
--(axis cs:11.2244897959184,0.37630230371622)
--(axis cs:10.8843537414966,0.383140025598311)
--(axis cs:10.5442176870748,0.387265435000783)
--(axis cs:10.2040816326531,0.399465016159506)
--(axis cs:9.86394557823129,0.40763178264095)
--(axis cs:9.52380952380952,0.416236790897825)
--(axis cs:9.18367346938775,0.425204088837716)
--(axis cs:8.84353741496599,0.434902451670395)
--(axis cs:8.50340136054422,0.445689180716178)
--(axis cs:8.16326530612245,0.454151926094505)
--(axis cs:7.82312925170068,0.464730883440626)
--(axis cs:7.48299319727891,0.474131878477742)
--(axis cs:7.14285714285714,0.48324610531483)
--(axis cs:6.80272108843537,0.49778016135575)
--(axis cs:6.46258503401361,0.508618168643115)
--(axis cs:6.12244897959184,0.517231970599875)
--(axis cs:5.78231292517007,0.525918420501146)
--(axis cs:5.4421768707483,0.535554809022223)
--(axis cs:5.10204081632653,0.545286457519909)
--(axis cs:4.76190476190476,0.553424993781273)
--(axis cs:4.42176870748299,0.56235581813628)
--(axis cs:4.08163265306122,0.574178000383972)
--(axis cs:3.74149659863946,0.587535182622805)
--(axis cs:3.40136054421769,0.600988419769125)
--(axis cs:3.06122448979592,0.617101286849466)
--(axis cs:2.72108843537415,0.636507102977078)
--(axis cs:2.38095238095238,0.652525923248217)
--(axis cs:2.04081632653061,0.667429846190428)
--(axis cs:1.70068027210884,0.683599206340532)
--(axis cs:1.36054421768707,0.698763837572887)
--(axis cs:1.02040816326531,0.711613124568868)
--(axis cs:0.680272108843537,0.718911613025094)
--(axis cs:0.340136054421769,0.723606400349906)
--(axis cs:0,0.720499093376582)
--cycle;


==> img/stl10/stl10_rate_distortion_fw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color0, mark=*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color0, thin}]
table {%
0 0.718636067509651
0.340136054421769 0.712396298795938
0.680272108843537 0.687354379594326
1.02040816326531 0.648709652870893
1.36054421768707 0.602634563948959
1.70068027210884 0.551961130667478
2.04081632653061 0.499133707217406
2.38095238095238 0.455875962974969
2.72108843537415 0.414941727598089
3.06122448979592 0.375139440922599
3.40136054421769 0.342052120033656
3.74149659863946 0.313365926619282
4.08163265306122 0.284980008603961
4.42176870748299 0.26049882455511
4.76190476190476 0.235224530055465
5.10204081632653 0.212331369829511
5.4421768707483 0.193027450054946
5.78231292517007 0.172360410085132
6.12244897959184 0.16199860278943
6.46258503401361 0.149569635052922
6.80272108843537 0.138511982875802
7.14285714285714 0.129712878930793
7.48299319727891 0.121679041112393
7.82312925170068 0.112578091133436
8.16326530612245 0.106060050373062
8.50340136054422 0.100678938015582
8.84353741496599 0.0971962687604599
9.18367346938775 0.0922406552221472
9.52380952380952 0.0856986667534157
9.86394557823129 0.0837206312219421
10.2040816326531 0.0809613972796337
10.5442176870748 0.0785116966504711
10.8843537414966 0.0778385125555286
11.2244897959184 0.0742604032335328
11.5646258503401 0.0753351301587551
11.9047619047619 0.0732794828162571
12.2448979591837 0.0721960056434973
12.5850340136054 0.070307846853807
12.9251700680272 0.0695319400677987
13.265306122449 0.06743388328135
13.6054421768707 0.0674183584595433
13.9455782312925 0.0658782005101931
14.2857142857143 0.0651666960853916
14.6258503401361 0.0639696400604825
14.9659863945578 0.0634200385440477
15.3061224489796 0.0644183169739823
15.6462585034014 0.0618934491121468
15.9863945578231 0.0618995917370237
16.3265306122449 0.0620448513577222
16.6666666666667 0.0630787495630293
17.0068027210884 0.0627446171903042
17.3469387755102 0.0633486629589783
17.687074829932 0.0633634767123901
18.0272108843537 0.0621853324624781
18.3673469387755 0.0629808456915279
18.7074829931973 0.0607720470572753
19.047619047619 0.0625000280414405
19.3877551020408 0.0618235961132604
19.7278911564626 0.0627575486141101
20.0680272108844 0.0614881111097675
20.4081632653061 0.0613484010471128
20.7482993197279 0.0626289389484345
21.0884353741497 0.0620879719267595
21.4285714285714 0.0624211129321391
21.7687074829932 0.0600728537917123
22.108843537415 0.0599878922920536
22.4489795918367 0.0611893191648146
22.7891156462585 0.0607576038603882
23.1292517006803 0.0612618028280248
23.469387755102 0.0638307112568723
23.8095238095238 0.0635325261251792
24.1496598639456 0.0640895036756545
24.4897959183673 0.0664276260406904
24.8299319727891 0.0661637520268255
25.1700680272109 0.0669244730042639
25.5102040816327 0.0660665380374551
25.8503401360544 0.068574850608249
26.1904761904762 0.069390889722358
26.530612244898 0.0683877632112292
26.8707482993197 0.0702158082508133
27.2108843537415 0.0690646164339526
27.5510204081633 0.0702783230542028
27.891156462585 0.0698149357094104
28.2312925170068 0.0703170855064591
28.5714285714286 0.0702507416875211
28.9115646258503 0.0695832555408689
29.2517006802721 0.0709811760631828
29.5918367346939 0.069967595456115
29.9319727891156 0.0703605913596736
30.2721088435374 0.0711837914181652
30.6122448979592 0.0718756783063683
30.952380952381 0.0714839920633992
31.2925170068027 0.0729034457404886
31.6326530612245 0.0738258454313428
31.9727891156463 0.0745934359810277
32.312925170068 0.0737570075639462
32.6530612244898 0.0754213847263006
32.9931972789116 0.0758146058465361
33.3333333333333 0.0761429157358903
33.6734693877551 0.0763403720822414
34.0136054421769 0.0760416964828526
34.3537414965986 0.0766912988065238
34.6938775510204 0.0779153338327473
35.0340136054422 0.0782743893406867
35.3741496598639 0.0774168109382532
35.7142857142857 0.0796787130242222
36.0544217687075 0.0785072600362031
36.3945578231292 0.0785898754177277
36.734693877551 0.077614240769016
37.0748299319728 0.0782886783905105
37.4149659863946 0.0784417298891397
37.7551020408163 0.0789577136136499
38.0952380952381 0.0789294848034452
38.4353741496599 0.0785534406560152
38.7755102040816 0.0797022199386864
39.1156462585034 0.0782290688567393
39.4557823129252 0.0790672337353539
39.7959183673469 0.0792583504566572
40.1360544217687 0.0787970252966301
40.4761904761905 0.080500653232056
40.8163265306122 0.079883479485076
41.156462585034 0.0790650399807657
41.4965986394558 0.0809306181484458
41.8367346938776 0.0811716008628085
42.1768707482993 0.0808834769534433
42.5170068027211 0.0818147567535564
42.8571428571429 0.081251998785538
43.1972789115646 0.0817137251817899
43.5374149659864 0.0821009319552116
43.8775510204082 0.0827303047339903
44.2176870748299 0.0833065876491868
44.5578231292517 0.0819167520895406
44.8979591836735 0.0835053747382155
45.2380952380952 0.0838687487071728
45.578231292517 0.0832096531741064
45.9183673469388 0.0835926584333717
46.2585034013605 0.0839792614701036
46.5986394557823 0.0855492655399867
46.9387755102041 0.0846964758678717
47.2789115646259 0.085240703602625
47.6190476190476 0.082541518196935
47.9591836734694 0.0831487457301605
48.2993197278912 0.0834494832465136
48.6394557823129 0.0836820009503624
48.9795918367347 0.0820839118602151
49.3197278911565 0.08217172798697
49.6598639455782 0.0826469600193446
50 0.0833080968299542
50.3401360544218 0.0818007633205283
50.6802721088435 0.0834476103771644
51.0204081632653 0.083091585716747
51.3605442176871 0.0816682301655496
51.7006802721088 0.0827340122145636
52.0408163265306 0.0823286339479662
52.3809523809524 0.0826649564426431
52.7210884353741 0.0827844753721858
53.0612244897959 0.0835248893196348
53.4013605442177 0.0829253155945841
53.7414965986395 0.084740152106215
54.0816326530612 0.0847768003142171
54.421768707483 0.0867330137286611
54.7619047619048 0.086479477040919
55.1020408163265 0.0854932530384777
55.4421768707483 0.0857513456316513
55.7823129251701 0.0847258514650304
56.1224489795918 0.0864806628407428
56.4625850340136 0.0857174578251347
56.8027210884354 0.0868961655783071
57.1428571428571 0.0864745314132242
57.4829931972789 0.0866323230476206
57.8231292517007 0.0858906865055339
58.1632653061224 0.0860994679976187
58.5034013605442 0.0856048990016599
58.843537414966 0.085682525666679
59.1836734693878 0.0851750967505489
59.5238095238095 0.0854541662089939
59.8639455782313 0.0841037075615277
60.2040816326531 0.0838144863506639
60.5442176870748 0.0836317801562457
60.8843537414966 0.0837209883442041
61.2244897959184 0.0822435208904601
61.5646258503401 0.0809267591111993
61.9047619047619 0.0805414015703837
62.2448979591837 0.0811291793846568
62.5850340136054 0.0795855099174678
62.9251700680272 0.0800070945517216
63.265306122449 0.080060381598865
63.6054421768707 0.0795419089114972
63.9455782312925 0.0792472989672028
64.2857142857143 0.0788727443232843
64.6258503401361 0.0788229119134291
64.9659863945578 0.0784528990952342
65.3061224489796 0.0777578663564955
65.6462585034014 0.077483016269974
65.9863945578231 0.076432200044898
66.3265306122449 0.0761500576232264
66.6666666666667 0.0767911330285995
67.0068027210884 0.0765734442972512
67.3469387755102 0.0758742029639049
67.687074829932 0.0754160790753278
68.0272108843537 0.0764097483978326
68.3673469387755 0.0765134406241555
68.7074829931973 0.0765751559101405
69.0476190476191 0.0760021570073434
69.3877551020408 0.0748436878297114
69.7278911564626 0.0742885675989246
70.0680272108844 0.0728301554441771
70.4081632653061 0.0732440342669185
70.7482993197279 0.072740492085834
71.0884353741497 0.0728408401719907
71.4285714285714 0.072001670948829
71.7687074829932 0.0716028401518039
72.108843537415 0.0718771085313658
72.4489795918367 0.0694763726908561
72.7891156462585 0.0692543850905969
73.1292517006803 0.06805047695781
73.469387755102 0.0677334093179566
73.8095238095238 0.0667801435881664
74.1496598639456 0.0662488141910519
74.4897959183673 0.0651385759902603
74.8299319727891 0.0651099919866831
75.1700680272109 0.0642380237898583
75.5102040816327 0.0612683854959135
75.8503401360544 0.0602450555819623
76.1904761904762 0.0593452438608501
76.530612244898 0.0570364918954832
76.8707482993197 0.0567217129316185
77.2108843537415 0.0557460124170088
77.5510204081633 0.0557245829189504
77.891156462585 0.0541868050777302
78.2312925170068 0.0534895359201764
78.5714285714286 0.0538349442098991
78.9115646258503 0.0523144330615179
79.2517006802721 0.0520567578661643
79.5918367346939 0.0498008813369659
79.9319727891156 0.0479679546682695
80.2721088435374 0.0456296260066242
80.6122448979592 0.0439567391202517
80.9523809523809 0.0424648925053921
81.2925170068027 0.0415327749050604
81.6326530612245 0.0408857193728679
81.9727891156463 0.0391238330797826
82.312925170068 0.0370636466070076
82.6530612244898 0.037083206415308
82.9931972789116 0.0360468097505561
83.3333333333333 0.0343340938271123
83.6734693877551 0.0334437620206152
84.0136054421769 0.0330286055121236
84.3537414965986 0.0310940518206849
84.6938775510204 0.0293671141334173
85.0340136054422 0.0274527416160246
85.3741496598639 0.0259763395129536
85.7142857142857 0.0245180928483648
86.0544217687075 0.0241198063885437
86.3945578231292 0.0232757421416928
86.734693877551 0.0217922307777251
87.0748299319728 0.0214939011857791
87.4149659863945 0.0203541276133337
87.7551020408163 0.0191323308382208
88.0952380952381 0.0183096948710899
88.4353741496599 0.0175242454801023
88.7755102040816 0.0168692918862887
89.1156462585034 0.016135733078515
89.4557823129252 0.0154403620789367
89.7959183673469 0.0146407307648264
90.1360544217687 0.0147465805082782
90.4761904761905 0.0142414288157223
90.8163265306122 0.0136481391572382
91.156462585034 0.0129802284414059
91.4965986394558 0.0128315428931437
91.8367346938775 0.0121126768232115
92.1768707482993 0.0115902152505021
92.5170068027211 0.0108013822929338
92.8571428571429 0.0102565175596128
93.1972789115646 0.00950008550756766
93.5374149659864 0.00867402842756354
93.8775510204082 0.0082611330555912
94.2176870748299 0.00737044371234486
94.5578231292517 0.00727470703133644
94.8979591836735 0.00679726508557658
95.2380952380952 0.00609000691984995
95.578231292517 0.00549596190691133
95.9183673469388 0.00525638607138037
96.2585034013605 0.00444661984561766
96.5986394557823 0.00410883312232222
96.9387755102041 0.00334354664924385
97.2789115646258 0.00290396525008603
97.6190476190476 0.00250800273139414
97.9591836734694 0.00208806460468535
98.2993197278912 0.00164134074195472
98.6394557823129 0.00127654108693174
98.9795918367347 0.000875150860356941
99.3197278911565 0.000678451544426379
99.6598639455782 0.000204841583348736
100 7.24220683423482e-14
};
\path [fill=color0, fill opacity=0.25]
(axis cs:0,0.720508539213816)
--(axis cs:0,0.716763595805486)
--(axis cs:0.340136054421769,0.710286745094899)
--(axis cs:0.680272108843537,0.684097271711785)
--(axis cs:1.02040816326531,0.644906947038631)
--(axis cs:1.36054421768707,0.597880692893055)
--(axis cs:1.70068027210884,0.546413827232982)
--(axis cs:2.04081632653061,0.493884408437315)
--(axis cs:2.38095238095238,0.45032624382908)
--(axis cs:2.72108843537415,0.409168506084383)
--(axis cs:3.06122448979592,0.369543294615956)
--(axis cs:3.40136054421769,0.336590092433712)
--(axis cs:3.74149659863946,0.307845083095231)
--(axis cs:4.08163265306122,0.279491489582593)
--(axis cs:4.42176870748299,0.254973133208853)
--(axis cs:4.76190476190476,0.229185810376176)
--(axis cs:5.10204081632653,0.20623371140542)
--(axis cs:5.4421768707483,0.187012236253441)
--(axis cs:5.78231292517007,0.166739289067987)
--(axis cs:6.12244897959184,0.156309488977069)
--(axis cs:6.46258503401361,0.143993319934865)
--(axis cs:6.80272108843537,0.13289876515917)
--(axis cs:7.14285714285714,0.124307021943939)
--(axis cs:7.48299319727891,0.11624252331314)
--(axis cs:7.82312925170068,0.107236071525035)
--(axis cs:8.16326530612245,0.101061522678347)
--(axis cs:8.50340136054422,0.0955449970126505)
--(axis cs:8.84353741496599,0.0921861657374216)
--(axis cs:9.18367346938775,0.087290438503562)
--(axis cs:9.52380952380952,0.0809678319873181)
--(axis cs:9.86394557823129,0.0790707388191138)
--(axis cs:10.2040816326531,0.0762913847899478)
--(axis cs:10.5442176870748,0.0738429243025933)
--(axis cs:10.8843537414966,0.0730802665252114)
--(axis cs:11.2244897959184,0.0697177224951199)
--(axis cs:11.5646258503401,0.0708973818433239)
--(axis cs:11.9047619047619,0.0688634911780939)
--(axis cs:12.2448979591837,0.0678374488383478)
--(axis cs:12.5850340136054,0.0659242385607617)
--(axis cs:12.9251700680272,0.0652453059574654)
--(axis cs:13.265306122449,0.0631101646728306)
--(axis cs:13.6054421768707,0.063258388309653)
--(axis cs:13.9455782312925,0.0618978146097232)
--(axis cs:14.2857142857143,0.0609849745361012)
--(axis cs:14.6258503401361,0.0600995454473358)
--(axis cs:14.9659863945578,0.059432583006559)
--(axis cs:15.3061224489796,0.0602887631653055)
--(axis cs:15.6462585034014,0.058017201660597)
--(axis cs:15.9863945578231,0.0578523437196485)
--(axis cs:16.3265306122449,0.0581309694128957)
--(axis cs:16.6666666666667,0.0592281443660274)
--(axis cs:17.0068027210884,0.0589693520764524)
--(axis cs:17.3469387755102,0.0592981131272621)
--(axis cs:17.687074829932,0.0595075558843411)
--(axis cs:18.0272108843537,0.0581708862913977)
--(axis cs:18.3673469387755,0.0591007963870798)
--(axis cs:18.7074829931973,0.0567930709917187)
--(axis cs:19.047619047619,0.0583572633701534)
--(axis cs:19.3877551020408,0.057869379229482)
--(axis cs:19.7278911564626,0.0587892285705219)
--(axis cs:20.0680272108844,0.0575623730063733)
--(axis cs:20.4081632653061,0.0574202607239409)
--(axis cs:20.7482993197279,0.0587783911514076)
--(axis cs:21.0884353741497,0.0582143810932012)
--(axis cs:21.4285714285714,0.0586977213866067)
--(axis cs:21.7687074829932,0.0562382604059246)
--(axis cs:22.108843537415,0.0562250705358941)
--(axis cs:22.4489795918367,0.0574149868927997)
--(axis cs:22.7891156462585,0.0566833080110839)
--(axis cs:23.1292517006803,0.0574547647419642)
--(axis cs:23.469387755102,0.0597474657175742)
--(axis cs:23.8095238095238,0.059450683535843)
--(axis cs:24.1496598639456,0.0602064515543534)
--(axis cs:24.4897959183673,0.0622965708286691)
--(axis cs:24.8299319727891,0.0620736593093814)
--(axis cs:25.1700680272109,0.0627648464157908)
--(axis cs:25.5102040816327,0.0620889757513377)
--(axis cs:25.8503401360544,0.0646482599455338)
--(axis cs:26.1904761904762,0.065532591734965)
--(axis cs:26.530612244898,0.0644009064910305)
--(axis cs:26.8707482993197,0.0662968080219469)
--(axis cs:27.2108843537415,0.0652989044500132)
--(axis cs:27.5510204081633,0.0665939147402234)
--(axis cs:27.891156462585,0.0660067491223072)
--(axis cs:28.2312925170068,0.0667514191052668)
--(axis cs:28.5714285714286,0.0666771696363307)
--(axis cs:28.9115646258503,0.0661770467629588)
--(axis cs:29.2517006802721,0.0676038680139224)
--(axis cs:29.5918367346939,0.0664505624750489)
--(axis cs:29.9319727891156,0.0667693192495695)
--(axis cs:30.2721088435374,0.0677571477138007)
--(axis cs:30.6122448979592,0.0683832252751397)
--(axis cs:30.952380952381,0.0680351456408517)
--(axis cs:31.2925170068027,0.069393941195676)
--(axis cs:31.6326530612245,0.0705493834366291)
--(axis cs:31.9727891156463,0.0709052272539075)
--(axis cs:32.312925170068,0.0703404200334959)
--(axis cs:32.6530612244898,0.0720212195757934)
--(axis cs:32.9931972789116,0.0723708251332742)
--(axis cs:33.3333333333333,0.0727359908314361)
--(axis cs:33.6734693877551,0.0729031142854985)
--(axis cs:34.0136054421769,0.0725688342355295)
--(axis cs:34.3537414965986,0.073316514017501)
--(axis cs:34.6938775510204,0.0743625420410708)
--(axis cs:35.0340136054422,0.0748393565154067)
--(axis cs:35.3741496598639,0.0739132656566703)
--(axis cs:35.7142857142857,0.076264693360489)
--(axis cs:36.0544217687075,0.0749592055154409)
--(axis cs:36.3945578231292,0.0749729964556333)
--(axis cs:36.734693877551,0.0741666765203926)
--(axis cs:37.0748299319728,0.0748341035874573)
--(axis cs:37.4149659863946,0.0750604994970842)
--(axis cs:37.7551020408163,0.075460710828629)
--(axis cs:38.0952380952381,0.0755937900015992)
--(axis cs:38.4353741496599,0.0752321280197729)
--(axis cs:38.7755102040816,0.0763373391910222)
--(axis cs:39.1156462585034,0.0747487421320591)
--(axis cs:39.4557823129252,0.0756680542524425)
--(axis cs:39.7959183673469,0.0758420097426882)
--(axis cs:40.1360544217687,0.0754189953926073)
--(axis cs:40.4761904761905,0.0770818400869965)
--(axis cs:40.8163265306122,0.0766085428457106)
--(axis cs:41.156462585034,0.0757289943996746)
--(axis cs:41.4965986394558,0.0774485081402339)
--(axis cs:41.8367346938776,0.0777893688267747)
--(axis cs:42.1768707482993,0.0775136150925039)
--(axis cs:42.5170068027211,0.0785409985997546)
--(axis cs:42.8571428571429,0.0779568347684715)
--(axis cs:43.1972789115646,0.0783307546598082)
--(axis cs:43.5374149659864,0.0788842271781215)
--(axis cs:43.8775510204082,0.0795589404450361)
--(axis cs:44.2176870748299,0.0799215855546978)
--(axis cs:44.5578231292517,0.0787498822345223)
--(axis cs:44.8979591836735,0.0801921756896253)
--(axis cs:45.2380952380952,0.0804410896786326)
--(axis cs:45.578231292517,0.0799850292480241)
--(axis cs:45.9183673469388,0.0803186465772883)
--(axis cs:46.2585034013605,0.0807585895319195)
--(axis cs:46.5986394557823,0.0821113433149856)
--(axis cs:46.9387755102041,0.0814708904446549)
--(axis cs:47.2789115646259,0.0819002881467747)
--(axis cs:47.6190476190476,0.0794305728711774)
--(axis cs:47.9591836734694,0.079924267325679)
--(axis cs:48.2993197278912,0.0802534150512635)
--(axis cs:48.6394557823129,0.0805420029847449)
--(axis cs:48.9795918367347,0.0788713193812929)
--(axis cs:49.3197278911565,0.0791307930975943)
--(axis cs:49.6598639455782,0.0794656401561034)
--(axis cs:50,0.0800044730782812)
--(axis cs:50.3401360544218,0.0788443272430667)
--(axis cs:50.6802721088435,0.0802391825525852)
--(axis cs:51.0204081632653,0.0800112702451424)
--(axis cs:51.3605442176871,0.0788819783138447)
--(axis cs:51.7006802721088,0.0796583555496836)
--(axis cs:52.0408163265306,0.0794564405300419)
--(axis cs:52.3809523809524,0.0796154096343913)
--(axis cs:52.7210884353741,0.0798704629733491)
--(axis cs:53.0612244897959,0.0805409240964957)
--(axis cs:53.4013605442177,0.0800489376867058)
--(axis cs:53.7414965986395,0.0815884298499042)
--(axis cs:54.0816326530612,0.0817336203804006)
--(axis cs:54.421768707483,0.0834860791577669)
--(axis cs:54.7619047619048,0.083215655569563)
--(axis cs:55.1020408163265,0.0825262500768759)
--(axis cs:55.4421768707483,0.0825151073345807)
--(axis cs:55.7823129251701,0.0816605903051538)
--(axis cs:56.1224489795918,0.0833583459615534)
--(axis cs:56.4625850340136,0.08261698285566)
--(axis cs:56.8027210884354,0.0837161514412268)
--(axis cs:57.1428571428571,0.083373929132801)
--(axis cs:57.4829931972789,0.0835058357599931)
--(axis cs:57.8231292517007,0.0827841051539036)
--(axis cs:58.1632653061224,0.0830779161262021)
--(axis cs:58.5034013605442,0.0827382872951991)
--(axis cs:58.843537414966,0.0827127803813047)
--(axis cs:59.1836734693878,0.0821282956084661)
--(axis cs:59.5238095238095,0.0823579722819815)
--(axis cs:59.8639455782313,0.0811764710999689)
--(axis cs:60.2040816326531,0.0808902345798962)
--(axis cs:60.5442176870748,0.0806792728396085)
--(axis cs:60.8843537414966,0.0808294262622552)
--(axis cs:61.2244897959184,0.079511959915891)
--(axis cs:61.5646258503401,0.0780866644492765)
--(axis cs:61.9047619047619,0.0776682188373103)
--(axis cs:62.2448979591837,0.0784002096452293)
--(axis cs:62.5850340136054,0.0769595363652097)
--(axis cs:62.9251700680272,0.0771967596249103)
--(axis cs:63.265306122449,0.0773611524533974)
--(axis cs:63.6054421768707,0.076816851697635)
--(axis cs:63.9455782312925,0.0766088888401866)
--(axis cs:64.2857142857143,0.0761165388891254)
--(axis cs:64.6258503401361,0.0760566965710115)
--(axis cs:64.9659863945578,0.0757042027127897)
--(axis cs:65.3061224489796,0.0751650831026144)
--(axis cs:65.6462585034014,0.0748419778355487)
--(axis cs:65.9863945578231,0.0738478779202926)
--(axis cs:66.3265306122449,0.0734682595155642)
--(axis cs:66.6666666666667,0.0741585652343975)
--(axis cs:67.0068027210884,0.0739156065750368)
--(axis cs:67.3469387755102,0.0731728843135462)
--(axis cs:67.687074829932,0.0727448176689232)
--(axis cs:68.0272108843537,0.0736906830104057)
--(axis cs:68.3673469387755,0.073809791958466)
--(axis cs:68.7074829931973,0.0738732819894291)
--(axis cs:69.0476190476191,0.073166562405441)
--(axis cs:69.3877551020408,0.0721410295873201)
--(axis cs:69.7278911564626,0.0717132809689734)
--(axis cs:70.0680272108844,0.0703825359322425)
--(axis cs:70.4081632653061,0.0707610637263791)
--(axis cs:70.7482993197279,0.070253044650708)
--(axis cs:71.0884353741497,0.070091953363378)
--(axis cs:71.4285714285714,0.0693818089414094)
--(axis cs:71.7687074829932,0.0688280322441891)
--(axis cs:72.108843537415,0.0690583884903238)
--(axis cs:72.4489795918367,0.0666660996594244)
--(axis cs:72.7891156462585,0.0664288249282499)
--(axis cs:73.1292517006803,0.0651311884461784)
--(axis cs:73.469387755102,0.0647683492092674)
--(axis cs:73.8095238095238,0.0638767125770203)
--(axis cs:74.1496598639456,0.0631755234199983)
--(axis cs:74.4897959183673,0.0621836608458399)
--(axis cs:74.8299319727891,0.0622172754693409)
--(axis cs:75.1700680272109,0.0612330836720347)
--(axis cs:75.5102040816327,0.0583440442347877)
--(axis cs:75.8503401360544,0.0572897945974147)
--(axis cs:76.1904761904762,0.0562932837020275)
--(axis cs:76.530612244898,0.0541356868035098)
--(axis cs:76.8707482993197,0.0537367308303173)
--(axis cs:77.2108843537415,0.0529140926770201)
--(axis cs:77.5510204081633,0.052889540368593)
--(axis cs:77.891156462585,0.0512245305638119)
--(axis cs:78.2312925170068,0.0507305660225743)
--(axis cs:78.5714285714286,0.0512604800496094)
--(axis cs:78.9115646258503,0.0497030304613108)
--(axis cs:79.2517006802721,0.0492641439268268)
--(axis cs:79.5918367346939,0.0471715656106921)
--(axis cs:79.9319727891156,0.0451034238211074)
--(axis cs:80.2721088435374,0.0431070148654009)
--(axis cs:80.6122448979592,0.0413722875842955)
--(axis cs:80.9523809523809,0.0400584793470858)
--(axis cs:81.2925170068027,0.0391334764036227)
--(axis cs:81.6326530612245,0.0385189901911741)
--(axis cs:81.9727891156463,0.0367899077311096)
--(axis cs:82.312925170068,0.0349934954632727)
--(axis cs:82.6530612244898,0.0351025893077623)
--(axis cs:82.9931972789116,0.034164355778498)
--(axis cs:83.3333333333333,0.0321370963919105)
--(axis cs:83.6734693877551,0.0313747356813912)
--(axis cs:84.0136054421769,0.0309425256151503)
--(axis cs:84.3537414965986,0.0291569467476082)
--(axis cs:84.6938775510204,0.027492358979987)
--(axis cs:85.0340136054422,0.025773998225792)
--(axis cs:85.3741496598639,0.0243186699533201)
--(axis cs:85.7142857142857,0.0229330441416496)
--(axis cs:86.0544217687075,0.0225182481990008)
--(axis cs:86.3945578231292,0.0217835422523223)
--(axis cs:86.734693877551,0.0202015602633619)
--(axis cs:87.0748299319728,0.0199677406163662)
--(axis cs:87.4149659863945,0.0188721518159912)
--(axis cs:87.7551020408163,0.0175787518839521)
--(axis cs:88.0952380952381,0.0168684190469914)
--(axis cs:88.4353741496599,0.0161391176281091)
--(axis cs:88.7755102040816,0.01557981829382)
--(axis cs:89.1156462585034,0.0148130845261268)
--(axis cs:89.4557823129252,0.0141272172032776)
--(axis cs:89.7959183673469,0.0133415289858696)
--(axis cs:90.1360544217687,0.0135568368112531)
--(axis cs:90.4761904761905,0.0130043956569163)
--(axis cs:90.8163265306122,0.0124485151570905)
--(axis cs:91.156462585034,0.0119057540581579)
--(axis cs:91.4965986394558,0.0117081619989849)
--(axis cs:91.8367346938775,0.0109718695546742)
--(axis cs:92.1768707482993,0.0104419177721027)
--(axis cs:92.5170068027211,0.00971453769292478)
--(axis cs:92.8571428571429,0.00918758854135606)
--(axis cs:93.1972789115646,0.00845791556789845)
--(axis cs:93.5374149659864,0.0077880047703811)
--(axis cs:93.8775510204082,0.00730539329644347)
--(axis cs:94.2176870748299,0.00646049249416497)
--(axis cs:94.5578231292517,0.00643486911022565)
--(axis cs:94.8979591836735,0.00591085032617362)
--(axis cs:95.2380952380952,0.00524764414527279)
--(axis cs:95.578231292517,0.00477233159972941)
--(axis cs:95.9183673469388,0.00446913757064001)
--(axis cs:96.2585034013605,0.0037745431911082)
--(axis cs:96.5986394557823,0.00346293739388382)
--(axis cs:96.9387755102041,0.00280994994923262)
--(axis cs:97.2789115646258,0.0023903133931778)
--(axis cs:97.6190476190476,0.00199518375428247)
--(axis cs:97.9591836734694,0.00168858486210012)
--(axis cs:98.2993197278912,0.00131924665000432)
--(axis cs:98.6394557823129,0.00104333951867497)
--(axis cs:98.9795918367347,0.000668813953415806)
--(axis cs:99.3197278911565,0.000502172488020551)
--(axis cs:99.6598639455782,0.000135481426609063)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:99.6598639455782,0.000274201740088409)
--(axis cs:99.3197278911565,0.000854730600832207)
--(axis cs:98.9795918367347,0.00108148776729808)
--(axis cs:98.6394557823129,0.0015097426551885)
--(axis cs:98.2993197278912,0.00196343483390511)
--(axis cs:97.9591836734694,0.00248754434727059)
--(axis cs:97.6190476190476,0.00302082170850581)
--(axis cs:97.2789115646258,0.00341761710699426)
--(axis cs:96.9387755102041,0.00387714334925508)
--(axis cs:96.5986394557823,0.00475472885076061)
--(axis cs:96.2585034013605,0.00511869650012712)
--(axis cs:95.9183673469388,0.00604363457212073)
--(axis cs:95.578231292517,0.00621959221409325)
--(axis cs:95.2380952380952,0.0069323696944271)
--(axis cs:94.8979591836735,0.00768367984497953)
--(axis cs:94.5578231292517,0.00811454495244722)
--(axis cs:94.2176870748299,0.00828039493052475)
--(axis cs:93.8775510204082,0.00921687281473894)
--(axis cs:93.5374149659864,0.00956005208474598)
--(axis cs:93.1972789115646,0.0105422554472369)
--(axis cs:92.8571428571429,0.0113254465778696)
--(axis cs:92.5170068027211,0.0118882268929429)
--(axis cs:92.1768707482993,0.0127385127289016)
--(axis cs:91.8367346938775,0.0132534840917489)
--(axis cs:91.4965986394558,0.0139549237873026)
--(axis cs:91.156462585034,0.0140547028246539)
--(axis cs:90.8163265306122,0.014847763157386)
--(axis cs:90.4761904761905,0.0154784619745283)
--(axis cs:90.1360544217687,0.0159363242053033)
--(axis cs:89.7959183673469,0.0159399325437832)
--(axis cs:89.4557823129252,0.0167535069545957)
--(axis cs:89.1156462585034,0.0174583816309032)
--(axis cs:88.7755102040816,0.0181587654787575)
--(axis cs:88.4353741496599,0.0189093733320954)
--(axis cs:88.0952380952381,0.0197509706951884)
--(axis cs:87.7551020408163,0.0206859097924896)
--(axis cs:87.4149659863945,0.0218361034106763)
--(axis cs:87.0748299319728,0.0230200617551921)
--(axis cs:86.734693877551,0.0233829012920882)
--(axis cs:86.3945578231292,0.0247679420310633)
--(axis cs:86.0544217687075,0.0257213645780866)
--(axis cs:85.7142857142857,0.0261031415550801)
--(axis cs:85.3741496598639,0.027634009072587)
--(axis cs:85.0340136054422,0.0291314850062572)
--(axis cs:84.6938775510204,0.0312418692868476)
--(axis cs:84.3537414965986,0.0330311568937617)
--(axis cs:84.0136054421769,0.035114685409097)
--(axis cs:83.6734693877551,0.0355127883598392)
--(axis cs:83.3333333333333,0.0365310912623141)
--(axis cs:82.9931972789116,0.0379292637226143)
--(axis cs:82.6530612244898,0.0390638235228537)
--(axis cs:82.312925170068,0.0391337977507425)
--(axis cs:81.9727891156463,0.0414577584284556)
--(axis cs:81.6326530612245,0.0432524485545617)
--(axis cs:81.2925170068027,0.043932073406498)
--(axis cs:80.9523809523809,0.0448713056636983)
--(axis cs:80.6122448979592,0.046541190656208)
--(axis cs:80.2721088435374,0.0481522371478474)
--(axis cs:79.9319727891156,0.0508324855154316)
--(axis cs:79.5918367346939,0.0524301970632397)
--(axis cs:79.2517006802721,0.0548493718055017)
--(axis cs:78.9115646258503,0.054925835661725)
--(axis cs:78.5714285714286,0.0564094083701887)
--(axis cs:78.2312925170068,0.0562485058177786)
--(axis cs:77.891156462585,0.0571490795916485)
--(axis cs:77.5510204081633,0.0585596254693079)
--(axis cs:77.2108843537415,0.0585779321569975)
--(axis cs:76.8707482993197,0.0597066950329197)
--(axis cs:76.530612244898,0.0599372969874566)
--(axis cs:76.1904761904762,0.0623972040196728)
--(axis cs:75.8503401360544,0.0632003165665099)
--(axis cs:75.5102040816327,0.0641927267570393)
--(axis cs:75.1700680272109,0.0672429639076819)
--(axis cs:74.8299319727891,0.0680027085040254)
--(axis cs:74.4897959183673,0.0680934911346807)
--(axis cs:74.1496598639456,0.0693221049621056)
--(axis cs:73.8095238095238,0.0696835745993125)
--(axis cs:73.469387755102,0.0706984694266459)
--(axis cs:73.1292517006803,0.0709697654694415)
--(axis cs:72.7891156462585,0.0720799452529439)
--(axis cs:72.4489795918367,0.0722866457222878)
--(axis cs:72.108843537415,0.0746958285724079)
--(axis cs:71.7687074829932,0.0743776480594187)
--(axis cs:71.4285714285714,0.0746215329562487)
--(axis cs:71.0884353741497,0.0755897269806034)
--(axis cs:70.7482993197279,0.07522793952096)
--(axis cs:70.4081632653061,0.075727004807458)
--(axis cs:70.0680272108844,0.0752777749561118)
--(axis cs:69.7278911564626,0.0768638542288758)
--(axis cs:69.3877551020408,0.0775463460721027)
--(axis cs:69.0476190476191,0.0788377516092459)
--(axis cs:68.7074829931973,0.0792770298308519)
--(axis cs:68.3673469387755,0.079217089289845)
--(axis cs:68.0272108843537,0.0791288137852596)
--(axis cs:67.687074829932,0.0780873404817324)
--(axis cs:67.3469387755102,0.0785755216142636)
--(axis cs:67.0068027210884,0.0792312820194656)
--(axis cs:66.6666666666667,0.0794237008228015)
--(axis cs:66.3265306122449,0.0788318557308887)
--(axis cs:65.9863945578231,0.0790165221695033)
--(axis cs:65.6462585034014,0.0801240547043992)
--(axis cs:65.3061224489796,0.0803506496103765)
--(axis cs:64.9659863945578,0.0812015954776788)
--(axis cs:64.6258503401361,0.0815891272558468)
--(axis cs:64.2857142857143,0.0816289497574432)
--(axis cs:63.9455782312925,0.0818857090942191)
--(axis cs:63.6054421768707,0.0822669661253595)
--(axis cs:63.265306122449,0.0827596107443327)
--(axis cs:62.9251700680272,0.082817429478533)
--(axis cs:62.5850340136054,0.0822114834697259)
--(axis cs:62.2448979591837,0.0838581491240842)
--(axis cs:61.9047619047619,0.0834145843034572)
--(axis cs:61.5646258503401,0.0837668537731221)
--(axis cs:61.2244897959184,0.0849750818650291)
--(axis cs:60.8843537414966,0.0866125504261531)
--(axis cs:60.5442176870748,0.0865842874728829)
--(axis cs:60.2040816326531,0.0867387381214316)
--(axis cs:59.8639455782313,0.0870309440230864)
--(axis cs:59.5238095238095,0.0885503601360063)
--(axis cs:59.1836734693878,0.0882218978926318)
--(axis cs:58.843537414966,0.0886522709520533)
--(axis cs:58.5034013605442,0.0884715107081208)
--(axis cs:58.1632653061224,0.0891210198690354)
--(axis cs:57.8231292517007,0.0889972678571643)
--(axis cs:57.4829931972789,0.0897588103352481)
--(axis cs:57.1428571428571,0.0895751336936475)
--(axis cs:56.8027210884354,0.0900761797153875)
--(axis cs:56.4625850340136,0.0888179327946095)
--(axis cs:56.1224489795918,0.0896029797199322)
--(axis cs:55.7823129251701,0.087791112624907)
--(axis cs:55.4421768707483,0.0889875839287219)
--(axis cs:55.1020408163265,0.0884602560000795)
--(axis cs:54.7619047619048,0.089743298512275)
--(axis cs:54.421768707483,0.0899799482995552)
--(axis cs:54.0816326530612,0.0878199802480337)
--(axis cs:53.7414965986395,0.0878918743625258)
--(axis cs:53.4013605442177,0.0858016935024623)
--(axis cs:53.0612244897959,0.0865088545427738)
--(axis cs:52.7210884353741,0.0856984877710225)
--(axis cs:52.3809523809524,0.085714503250895)
--(axis cs:52.0408163265306,0.0852008273658906)
--(axis cs:51.7006802721088,0.0858096688794437)
--(axis cs:51.3605442176871,0.0844544820172545)
--(axis cs:51.0204081632653,0.0861719011883516)
--(axis cs:50.6802721088435,0.0866560382017436)
--(axis cs:50.3401360544218,0.0847571993979899)
--(axis cs:50,0.0866117205816273)
--(axis cs:49.6598639455782,0.0858282798825859)
--(axis cs:49.3197278911565,0.0852126628763457)
--(axis cs:48.9795918367347,0.0852965043391374)
--(axis cs:48.6394557823129,0.08682199891598)
--(axis cs:48.2993197278912,0.0866455514417637)
--(axis cs:47.9591836734694,0.0863732241346419)
--(axis cs:47.6190476190476,0.0856524635226927)
--(axis cs:47.2789115646259,0.0885811190584752)
--(axis cs:46.9387755102041,0.0879220612910885)
--(axis cs:46.5986394557823,0.0889871877649878)
--(axis cs:46.2585034013605,0.0871999334082878)
--(axis cs:45.9183673469388,0.0868666702894552)
--(axis cs:45.578231292517,0.0864342771001886)
--(axis cs:45.2380952380952,0.0872964077357131)
--(axis cs:44.8979591836735,0.0868185737868058)
--(axis cs:44.5578231292517,0.085083621944559)
--(axis cs:44.2176870748299,0.0866915897436758)
--(axis cs:43.8775510204082,0.0859016690229445)
--(axis cs:43.5374149659864,0.0853176367323017)
--(axis cs:43.1972789115646,0.0850966957037717)
--(axis cs:42.8571428571429,0.0845471628026045)
--(axis cs:42.5170068027211,0.0850885149073582)
--(axis cs:42.1768707482993,0.0842533388143827)
--(axis cs:41.8367346938776,0.0845538328988423)
--(axis cs:41.4965986394558,0.0844127281566576)
--(axis cs:41.156462585034,0.0824010855618568)
--(axis cs:40.8163265306122,0.0831584161244413)
--(axis cs:40.4761904761905,0.0839194663771156)
--(axis cs:40.1360544217687,0.0821750552006529)
--(axis cs:39.7959183673469,0.0826746911706262)
--(axis cs:39.4557823129252,0.0824664132182654)
--(axis cs:39.1156462585034,0.0817093955814196)
--(axis cs:38.7755102040816,0.0830671006863506)
--(axis cs:38.4353741496599,0.0818747532922576)
--(axis cs:38.0952380952381,0.0822651796052912)
--(axis cs:37.7551020408163,0.0824547163986709)
--(axis cs:37.4149659863946,0.0818229602811952)
--(axis cs:37.0748299319728,0.0817432531935636)
--(axis cs:36.734693877551,0.0810618050176394)
--(axis cs:36.3945578231292,0.0822067543798222)
--(axis cs:36.0544217687075,0.0820553145569653)
--(axis cs:35.7142857142857,0.0830927326879554)
--(axis cs:35.3741496598639,0.0809203562198362)
--(axis cs:35.0340136054422,0.0817094221659667)
--(axis cs:34.6938775510204,0.0814681256244238)
--(axis cs:34.3537414965986,0.0800660835955465)
--(axis cs:34.0136054421769,0.0795145587301756)
--(axis cs:33.6734693877551,0.0797776298789842)
--(axis cs:33.3333333333333,0.0795498406403446)
--(axis cs:32.9931972789116,0.0792583865597979)
--(axis cs:32.6530612244898,0.0788215498768078)
--(axis cs:32.312925170068,0.0771735950943965)
--(axis cs:31.9727891156463,0.0782816447081479)
--(axis cs:31.6326530612245,0.0771023074260565)
--(axis cs:31.2925170068027,0.0764129502853011)
--(axis cs:30.952380952381,0.0749328384859467)
--(axis cs:30.6122448979592,0.0753681313375969)
--(axis cs:30.2721088435374,0.0746104351225296)
--(axis cs:29.9319727891156,0.0739518634697777)
--(axis cs:29.5918367346939,0.0734846284371811)
--(axis cs:29.2517006802721,0.0743584841124432)
--(axis cs:28.9115646258503,0.072989464318779)
--(axis cs:28.5714285714286,0.0738243137387114)
--(axis cs:28.2312925170068,0.0738827519076513)
--(axis cs:27.891156462585,0.0736231222965136)
--(axis cs:27.5510204081633,0.0739627313681823)
--(axis cs:27.2108843537415,0.0728303284178921)
--(axis cs:26.8707482993197,0.0741348084796797)
--(axis cs:26.530612244898,0.0723746199314278)
--(axis cs:26.1904761904762,0.073249187709751)
--(axis cs:25.8503401360544,0.0725014412709641)
--(axis cs:25.5102040816327,0.0700441003235726)
--(axis cs:25.1700680272109,0.071084099592737)
--(axis cs:24.8299319727891,0.0702538447442696)
--(axis cs:24.4897959183673,0.0705586812527118)
--(axis cs:24.1496598639456,0.0679725557969556)
--(axis cs:23.8095238095238,0.0676143687145154)
--(axis cs:23.469387755102,0.0679139567961703)
--(axis cs:23.1292517006803,0.0650688409140854)
--(axis cs:22.7891156462585,0.0648318997096926)
--(axis cs:22.4489795918367,0.0649636514368295)
--(axis cs:22.108843537415,0.0637507140482131)
--(axis cs:21.7687074829932,0.0639074471775)
--(axis cs:21.4285714285714,0.0661445044776715)
--(axis cs:21.0884353741497,0.0659615627603178)
--(axis cs:20.7482993197279,0.0664794867454614)
--(axis cs:20.4081632653061,0.0652765413702847)
--(axis cs:20.0680272108844,0.0654138492131617)
--(axis cs:19.7278911564626,0.0667258686576983)
--(axis cs:19.3877551020408,0.0657778129970388)
--(axis cs:19.047619047619,0.0666427927127277)
--(axis cs:18.7074829931973,0.064751023122832)
--(axis cs:18.3673469387755,0.0668608949959759)
--(axis cs:18.0272108843537,0.0661997786335585)
--(axis cs:17.687074829932,0.0672193975404391)
--(axis cs:17.3469387755102,0.0673992127906945)
--(axis cs:17.0068027210884,0.066519882304156)
--(axis cs:16.6666666666667,0.0669293547600311)
--(axis cs:16.3265306122449,0.0659587333025487)
--(axis cs:15.9863945578231,0.065946839754399)
--(axis cs:15.6462585034014,0.0657696965636965)
--(axis cs:15.3061224489796,0.0685478707826592)
--(axis cs:14.9659863945578,0.0674074940815364)
--(axis cs:14.6258503401361,0.0678397346736292)
--(axis cs:14.2857142857143,0.0693484176346819)
--(axis cs:13.9455782312925,0.069858586410663)
--(axis cs:13.6054421768707,0.0715783286094337)
--(axis cs:13.265306122449,0.0717576018898694)
--(axis cs:12.9251700680272,0.073818574178132)
--(axis cs:12.5850340136054,0.0746914551468524)
--(axis cs:12.2448979591837,0.0765545624486469)
--(axis cs:11.9047619047619,0.0776954744544202)
--(axis cs:11.5646258503401,0.0797728784741863)
--(axis cs:11.2244897959184,0.0788030839719456)
--(axis cs:10.8843537414966,0.0825967585858459)
--(axis cs:10.5442176870748,0.083180468998349)
--(axis cs:10.2040816326531,0.0856314097693196)
--(axis cs:9.86394557823129,0.0883705236247704)
--(axis cs:9.52380952380952,0.0904295015195132)
--(axis cs:9.18367346938775,0.0971908719407324)
--(axis cs:8.84353741496599,0.102206371783498)
--(axis cs:8.50340136054422,0.105812879018513)
--(axis cs:8.16326530612245,0.111058578067776)
--(axis cs:7.82312925170068,0.117920110741836)
--(axis cs:7.48299319727891,0.127115558911647)
--(axis cs:7.14285714285714,0.135118735917647)
--(axis cs:6.80272108843537,0.144125200592433)
--(axis cs:6.46258503401361,0.155145950170979)
--(axis cs:6.12244897959184,0.167687716601791)
--(axis cs:5.78231292517007,0.177981531102276)
--(axis cs:5.4421768707483,0.199042663856451)
--(axis cs:5.10204081632653,0.218429028253602)
--(axis cs:4.76190476190476,0.241263249734755)
--(axis cs:4.42176870748299,0.266024515901367)
--(axis cs:4.08163265306122,0.290468527625329)
--(axis cs:3.74149659863946,0.318886770143333)
--(axis cs:3.40136054421769,0.347514147633601)
--(axis cs:3.06122448979592,0.380735587229241)
--(axis cs:2.72108843537415,0.420714949111795)
--(axis cs:2.38095238095238,0.461425682120858)
--(axis cs:2.04081632653061,0.504383005997498)
--(axis cs:1.70068027210884,0.557508434101974)
--(axis cs:1.36054421768707,0.607388435004863)
--(axis cs:1.02040816326531,0.652512358703156)
--(axis cs:0.680272108843537,0.690611487476867)
--(axis cs:0.340136054421769,0.714505852496978)
--(axis cs:0,0.720508539213816)
--cycle;


==> img/stl10/stl10_rate_distortion_guidedbackprop.tex <==
% guided backprop
\addplot [line width=0.5, opacity=0.8, color8, mark=oplus*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table [row sep=\\]{%
0	0.71919958949089 \\
0.340136054421769	0.719297086000443 \\
0.680272108843537	0.717910318076611 \\
1.02040816326531	0.715532967299223 \\
1.36054421768707	0.713333299458027 \\
1.70068027210884	0.709677787721157 \\
2.04081632653061	0.7063898229599 \\
2.38095238095238	0.703008438944817 \\
2.72108843537415	0.700712354183197 \\
3.06122448979592	0.698655898869038 \\
3.40136054421769	0.69505034044385 \\
3.74149659863946	0.69350798279047 \\
4.08163265306122	0.691460852921009 \\
4.42176870748299	0.688976245075464 \\
4.76190476190476	0.686575120985508 \\
5.10204081632653	0.684261545389891 \\
5.4421768707483	0.681996056884527 \\
5.78231292517007	0.680575447529554 \\
6.12244897959184	0.679591497480869 \\
6.46258503401361	0.677804639190435 \\
6.80272108843537	0.678337739706039 \\
7.14285714285714	0.677686781734228 \\
7.48299319727891	0.676483900398016 \\
7.82312925170068	0.67508529856801 \\
8.16326530612245	0.675666658878326 \\
8.50340136054422	0.675346526503563 \\
8.84353741496599	0.674923767596483 \\
9.18367346938775	0.672905648499727 \\
9.52380952380952	0.671911405473948 \\
9.86394557823129	0.671493232995272 \\
10.2040816326531	0.670459589362144 \\
10.5442176870748	0.669993086755276 \\
10.8843537414966	0.669248265624046 \\
11.2244897959184	0.667659350633621 \\
11.5646258503401	0.666483979821205 \\
11.9047619047619	0.667202216535807 \\
12.2448979591837	0.66536040648818 \\
12.5850340136054	0.665361704230308 \\
12.9251700680272	0.664206799268723 \\
13.265306122449	0.663501915633678 \\
13.6054421768707	0.662548270821571 \\
13.9455782312925	0.661229673475027 \\
14.2857142857143	0.661086009442806 \\
14.6258503401361	0.661018484979868 \\
14.9659863945578	0.659074653089046 \\
15.3061224489796	0.658357953429222 \\
15.6462585034014	0.657135976999998 \\
15.9863945578231	0.657027393579483 \\
16.3265306122449	0.6565008251369 \\
16.6666666666667	0.65617324128747 \\
17.0068027210884	0.655483192056417 \\
17.3469387755102	0.653683451116085 \\
17.687074829932	0.652211887091398 \\
18.0272108843537	0.651373763531446 \\
18.3673469387755	0.651887029260397 \\
18.7074829931973	0.650903767049313 \\
19.047619047619	0.651440567225218 \\
19.3877551020408	0.650865698158741 \\
19.7278911564626	0.649387167841196 \\
20.0680272108844	0.649621710851789 \\
20.4081632653061	0.649251189678907 \\
20.7482993197279	0.649404215216637 \\
21.0884353741497	0.64843957066536 \\
21.4285714285714	0.646612114608288 \\
21.7687074829932	0.646927374228835 \\
22.108843537415	0.646386491060257 \\
22.4489795918367	0.646040374860168 \\
22.7891156462585	0.645380148887634 \\
23.1292517006803	0.644184715375304 \\
23.469387755102	0.643588361889124 \\
23.8095238095238	0.643729741498828 \\
24.1496598639456	0.641915521249175 \\
24.4897959183673	0.643151358962059 \\
24.8299319727891	0.64184575162828 \\
25.1700680272109	0.640543335676193 \\
25.5102040816327	0.640107493624091 \\
25.8503401360544	0.640196027755737 \\
26.1904761904762	0.638866190910339 \\
26.530612244898	0.639573933705687 \\
26.8707482993197	0.637477093599737 \\
27.2108843537415	0.636371101438999 \\
27.5510204081633	0.637358661964536 \\
27.891156462585	0.636746597364545 \\
28.2312925170068	0.635363701619208 \\
28.5714285714286	0.635930581986904 \\
28.9115646258503	0.634274502769113 \\
29.2517006802721	0.633650770131499 \\
29.5918367346939	0.633590260148048 \\
29.9319727891156	0.632337271478027 \\
30.2721088435374	0.630336899179965 \\
30.6122448979592	0.629425428546965 \\
30.952380952381	0.62716343132779 \\
31.2925170068027	0.627823964320123 \\
31.6326530612245	0.62556432871148 \\
31.9727891156463	0.62489052221179 \\
32.312925170068	0.626235937401652 \\
32.6530612244898	0.623579043895006 \\
32.9931972789116	0.622763868775219 \\
33.3333333333333	0.62181189853698 \\
33.6734693877551	0.623028809912503 \\
34.0136054421769	0.619691491611302 \\
34.3537414965986	0.621312702763826 \\
34.6938775510204	0.620162338241935 \\
35.0340136054422	0.620764526277781 \\
35.3741496598639	0.620134770944715 \\
35.7142857142857	0.617902448112145 \\
36.0544217687075	0.614362228568643 \\
36.3945578231292	0.613370087230578 \\
36.734693877551	0.613817484173924 \\
37.0748299319728	0.612588822003454 \\
37.4149659863946	0.609310099594295 \\
37.7551020408163	0.61092303417623 \\
38.0952380952381	0.60809267106466 \\
38.4353741496599	0.608582496438175 \\
38.7755102040816	0.607507015801966 \\
39.1156462585034	0.607142151705921 \\
39.4557823129252	0.607746000811458 \\
39.7959183673469	0.606917413491756 \\
40.1360544217687	0.605824982430786 \\
40.4761904761905	0.606571917701513 \\
40.8163265306122	0.605410185866058 \\
41.156462585034	0.603364628590643 \\
41.4965986394558	0.601769001297653 \\
41.8367346938776	0.602166271377355 \\
42.1768707482993	0.60162975916639 \\
42.5170068027211	0.601204771413468 \\
42.8571428571429	0.599412572626024 \\
43.1972789115646	0.599019362181425 \\
43.5374149659864	0.600789378071204 \\
43.8775510204082	0.598857005592436 \\
44.2176870748299	0.599267823947594 \\
44.5578231292517	0.595697562722489 \\
44.8979591836735	0.597780015226454 \\
45.2380952380952	0.596398275140673 \\
45.578231292517	0.595873942826875 \\
45.9183673469388	0.595583538394421 \\
46.2585034013605	0.594816240263171 \\
46.5986394557823	0.594156316528097 \\
46.9387755102041	0.593810920799151 \\
47.2789115646259	0.596301603857428 \\
47.6190476190476	0.593382381368428 \\
47.9591836734694	0.591750869099051 \\
48.2993197278912	0.594585620504804 \\
48.6394557823129	0.592832248965278 \\
48.9795918367347	0.592574763852172 \\
49.3197278911565	0.59062551336363 \\
49.6598639455782	0.590443490743637 \\
50	0.59014242223464 \\
50.3401360544218	0.591371180899441 \\
50.6802721088435	0.589880540650338 \\
51.0204081632653	0.587371188700199 \\
51.3605442176871	0.589910621531308 \\
51.7006802721088	0.588016122141853 \\
52.0408163265306	0.587723759487271 \\
52.3809523809524	0.585571693517268 \\
52.7210884353741	0.584118073321879 \\
53.0612244897959	0.580980404447764 \\
53.4013605442177	0.582122420119122 \\
53.7414965986395	0.582345459908247 \\
54.0816326530612	0.579674304369837 \\
54.421768707483	0.579938941691071 \\
54.7619047619048	0.575306932609528 \\
55.1020408163265	0.575941752120853 \\
55.4421768707483	0.576871954035014 \\
55.7823129251701	0.573120841421187 \\
56.1224489795918	0.572244240064174 \\
56.4625850340136	0.570733180977404 \\
56.8027210884354	0.571167637463659 \\
57.1428571428571	0.569014572426677 \\
57.4829931972789	0.569178451001644 \\
57.8231292517007	0.566414029961452 \\
58.1632653061224	0.564680683072656 \\
58.5034013605442	0.561519054379314 \\
58.843537414966	0.561310339700431 \\
59.1836734693878	0.560649736057967 \\
59.5238095238095	0.558316339012235 \\
59.8639455782313	0.556053439471871 \\
60.2040816326531	0.555020700190216 \\
60.5442176870748	0.553215305041522 \\
60.8843537414966	0.553651184951887 \\
61.2244897959184	0.548404763722792 \\
61.5646258503401	0.54838363292627 \\
61.9047619047619	0.545072364043444 \\
62.2448979591837	0.540994277689606 \\
62.5850340136054	0.541089479625225 \\
62.9251700680272	0.539204466091469 \\
63.265306122449	0.536245741294697 \\
63.6054421768707	0.534264653548598 \\
63.9455782312925	0.533629675917327 \\
64.2857142857143	0.532274372661486 \\
64.6258503401361	0.531356861637905 \\
64.9659863945578	0.529192088413984 \\
65.3061224489796	0.528373987730593 \\
65.6462585034014	0.526870567966253 \\
65.9863945578231	0.526716981157661 \\
66.3265306122449	0.526420267699286 \\
66.6666666666667	0.525362434871495 \\
67.0068027210884	0.525129364570603 \\
67.3469387755102	0.522733452748507 \\
67.687074829932	0.524635146902874 \\
68.0272108843537	0.524561641123146 \\
68.3673469387755	0.524852102268487 \\
68.7074829931973	0.523166933394969 \\
69.0476190476191	0.522955069269519 \\
69.3877551020408	0.522899627897423 \\
69.7278911564626	0.522218005078612 \\
70.0680272108844	0.521347280286718 \\
70.4081632653061	0.52335966410581 \\
70.7482993197279	0.521263119772193 \\
71.0884353741497	0.519707803900237 \\
71.4285714285714	0.518941654023365 \\
71.7687074829932	0.519091485751269 \\
72.108843537415	0.515533799910627 \\
72.4489795918367	0.516000089337613 \\
72.7891156462585	0.515289276064868 \\
73.1292517006803	0.514639442445914 \\
73.469387755102	0.51267115314291 \\
73.8095238095238	0.511234567628417 \\
74.1496598639456	0.511578023604816 \\
74.4897959183673	0.510129837043387 \\
74.8299319727891	0.509818712622673 \\
75.1700680272109	0.507464443476874 \\
75.5102040816327	0.505024371007785 \\
75.8503401360544	0.50430782631156 \\
76.1904761904762	0.501094158324668 \\
76.530612244898	0.500686246427085 \\
76.8707482993197	0.498395122029233 \\
77.2108843537415	0.498621514327974 \\
77.5510204081633	0.497528107461467 \\
77.891156462585	0.495747968932202 \\
78.2312925170068	0.495336592371032 \\
78.5714285714286	0.493273082188357 \\
78.9115646258503	0.492505138191882 \\
79.2517006802721	0.49031533281189 \\
79.5918367346939	0.488739700113536 \\
79.9319727891156	0.488039331318439 \\
80.2721088435374	0.487787305381296 \\
80.6122448979592	0.486581485871913 \\
80.9523809523809	0.486106929886267 \\
81.2925170068027	0.483087794431021 \\
81.6326530612245	0.48041871760404 \\
81.9727891156463	0.479849877868382 \\
82.312925170068	0.476916035698367 \\
82.6530612244898	0.47629157198199 \\
82.9931972789116	0.47468264512341 \\
83.3333333333333	0.473271322353068 \\
83.6734693877551	0.470816312058459 \\
84.0136054421769	0.467257468068919 \\
84.3537414965986	0.46617295000165 \\
84.6938775510204	0.462810325954965 \\
85.0340136054422	0.463413281368755 \\
85.3741496598639	0.460684175136448 \\
85.7142857142857	0.456680743121386 \\
86.0544217687075	0.452519070673012 \\
86.3945578231292	0.449960601086622 \\
86.734693877551	0.447795912468849 \\
87.0748299319728	0.445200358395167 \\
87.4149659863945	0.442093229846537 \\
87.7551020408163	0.438724778958478 \\
88.0952380952381	0.432819112769847 \\
88.4353741496599	0.427545692335652 \\
88.7755102040816	0.421814198343999 \\
89.1156462585034	0.414955648561332 \\
89.4557823129252	0.408992409887984 \\
89.7959183673469	0.401029604412417 \\
90.1360544217687	0.393569852080936 \\
90.4761904761905	0.382784221310708 \\
90.8163265306122	0.373967827854669 \\
91.156462585034	0.362545711989417 \\
91.4965986394558	0.354669985802881 \\
91.8367346938775	0.346217832870913 \\
92.1768707482993	0.334285209883384 \\
92.5170068027211	0.324802681881616 \\
92.8571428571429	0.311150566652672 \\
93.1972789115646	0.302435625942758 \\
93.5374149659864	0.289886499004032 \\
93.8775510204082	0.275840457626033 \\
94.2176870748299	0.267323111685764 \\
94.5578231292517	0.256859202324144 \\
94.8979591836735	0.240432868684512 \\
95.2380952380952	0.227360266948003 \\
95.578231292517	0.212352499159184 \\
95.9183673469388	0.194839346313403 \\
96.2585034013605	0.182830297655301 \\
96.5986394557823	0.167647689712992 \\
96.9387755102041	0.157289844226232 \\
97.2789115646258	0.145229100751733 \\
97.6190476190476	0.132743683284935 \\
97.9591836734694	0.123304327435464 \\
98.2993197278912	0.109787904041918 \\
98.6394557823129	0.0991781021241441 \\
98.9795918367347	0.0918950099826538 \\
99.3197278911565	0.0756430573178255 \\
99.6598639455782	0.0492156259513267 \\
100	1.49018575257287e-13 \\
};
\path [fill=color8, fill opacity=0.5] (axis cs:0,0.721035239063252)
--(axis cs:0,0.717363939918529)
--(axis cs:0.340136054421769,0.717409814806988)
--(axis cs:0.680272108843537,0.715967891795525)
--(axis cs:1.02040816326531,0.713504644207228)
--(axis cs:1.36054421768707,0.711188955860154)
--(axis cs:1.70068027210884,0.707364911823615)
--(axis cs:2.04081632653061,0.704006591332607)
--(axis cs:2.38095238095238,0.700482301271995)
--(axis cs:2.72108843537415,0.698030923718708)
--(axis cs:3.06122448979592,0.695906996720231)
--(axis cs:3.40136054421769,0.692243085764668)
--(axis cs:3.74149659863946,0.690588909558996)
--(axis cs:4.08163265306122,0.688571516618472)
--(axis cs:4.42176870748299,0.685950648678492)
--(axis cs:4.76190476190476,0.683581516580789)
--(axis cs:5.10204081632653,0.681172010965901)
--(axis cs:5.4421768707483,0.678896827080425)
--(axis cs:5.78231292517007,0.677488292179534)
--(axis cs:6.12244897959184,0.676454459005116)
--(axis cs:6.46258503401361,0.674583518335243)
--(axis cs:6.80272108843537,0.675120734408128)
--(axis cs:7.14285714285714,0.674353890158238)
--(axis cs:7.48299319727891,0.673169028261615)
--(axis cs:7.82312925170068,0.671719829921809)
--(axis cs:8.16326530612245,0.672418393022971)
--(axis cs:8.50340136054422,0.671835956440618)
--(axis cs:8.84353741496599,0.671468229040363)
--(axis cs:9.18367346938775,0.669392660557094)
--(axis cs:9.52380952380952,0.668298486003196)
--(axis cs:9.86394557823129,0.667965385665696)
--(axis cs:10.2040816326531,0.666803474167848)
--(axis cs:10.5442176870748,0.666391131506899)
--(axis cs:10.8843537414966,0.665564875673102)
--(axis cs:11.2244897959184,0.663909073015944)
--(axis cs:11.5646258503401,0.662811326874931)
--(axis cs:11.9047619047619,0.663427996777619)
--(axis cs:12.2448979591837,0.661496493977755)
--(axis cs:12.5850340136054,0.661452346879937)
--(axis cs:12.9251700680272,0.660274199130316)
--(axis cs:13.265306122449,0.659567932481054)
--(axis cs:13.6054421768707,0.658695173848286)
--(axis cs:13.9455782312925,0.657218731188327)
--(axis cs:14.2857142857143,0.657002109871747)
--(axis cs:14.6258503401361,0.656909822546706)
--(axis cs:14.9659863945578,0.654791019317209)
--(axis cs:15.3061224489796,0.654081034017495)
--(axis cs:15.6462585034014,0.652880007871746)
--(axis cs:15.9863945578231,0.652700054860306)
--(axis cs:16.3265306122449,0.652172664228316)
--(axis cs:16.6666666666667,0.651698788526345)
--(axis cs:17.0068027210884,0.651108972957934)
--(axis cs:17.3469387755102,0.649272208537301)
--(axis cs:17.687074829932,0.647590192483837)
--(axis cs:18.0272108843537,0.646978409640675)
--(axis cs:18.3673469387755,0.647389949912063)
--(axis cs:18.7074829931973,0.646371958113667)
--(axis cs:19.047619047619,0.646928729682255)
--(axis cs:19.3877551020408,0.64626693494753)
--(axis cs:19.7278911564626,0.644881841536353)
--(axis cs:20.0680272108844,0.645015518233188)
--(axis cs:20.4081632653061,0.644559669287114)
--(axis cs:20.7482993197279,0.644850606873902)
--(axis cs:21.0884353741497,0.643773527091949)
--(axis cs:21.4285714285714,0.642006155362889)
--(axis cs:21.7687074829932,0.642255776310259)
--(axis cs:22.108843537415,0.641648569926855)
--(axis cs:22.4489795918367,0.641159163902572)
--(axis cs:22.7891156462585,0.640302494704981)
--(axis cs:23.1292517006803,0.63901839990734)
--(axis cs:23.469387755102,0.638683324634979)
--(axis cs:23.8095238095238,0.638779078267141)
--(axis cs:24.1496598639456,0.636978649561)
--(axis cs:24.4897959183673,0.638267587620373)
--(axis cs:24.8299319727891,0.636873520307465)
--(axis cs:25.1700680272109,0.635485947326541)
--(axis cs:25.5102040816327,0.635066642900552)
--(axis cs:25.8503401360544,0.635135790591109)
--(axis cs:26.1904761904762,0.633792171818613)
--(axis cs:26.530612244898,0.634386424446233)
--(axis cs:26.8707482993197,0.632203305305649)
--(axis cs:27.2108843537415,0.63120022628481)
--(axis cs:27.5510204081633,0.632230056098237)
--(axis cs:27.891156462585,0.631514139148332)
--(axis cs:28.2312925170068,0.63010498195687)
--(axis cs:28.5714285714286,0.630771888237903)
--(axis cs:28.9115646258503,0.629094504015224)
--(axis cs:29.2517006802721,0.628245572413176)
--(axis cs:29.5918367346939,0.628472220163934)
--(axis cs:29.9319727891156,0.62706743315502)
--(axis cs:30.2721088435374,0.624804784004448)
--(axis cs:30.6122448979592,0.623971644650976)
--(axis cs:30.952380952381,0.621786986991506)
--(axis cs:31.2925170068027,0.622439033903523)
--(axis cs:31.6326530612245,0.620297934947569)
--(axis cs:31.9727891156463,0.619478182565006)
--(axis cs:32.312925170068,0.620798091838631)
--(axis cs:32.6530612244898,0.618099953644361)
--(axis cs:32.9931972789116,0.617419043608972)
--(axis cs:33.3333333333333,0.616431095676185)
--(axis cs:33.6734693877551,0.617541709782781)
--(axis cs:34.0136054421769,0.614307062067884)
--(axis cs:34.3537414965986,0.615776749654235)
--(axis cs:34.6938775510204,0.614807737955804)
--(axis cs:35.0340136054422,0.615335506595234)
--(axis cs:35.3741496598639,0.614775015914425)
--(axis cs:35.7142857142857,0.612471664868613)
--(axis cs:36.0544217687075,0.608745908614391)
--(axis cs:36.3945578231292,0.60773021882551)
--(axis cs:36.734693877551,0.608404317940954)
--(axis cs:37.0748299319728,0.607154856829804)
--(axis cs:37.4149659863946,0.603809974286662)
--(axis cs:37.7551020408163,0.605471951006975)
--(axis cs:38.0952380952381,0.602630000122498)
--(axis cs:38.4353741496599,0.603071248980745)
--(axis cs:38.7755102040816,0.601827550324985)
--(axis cs:39.1156462585034,0.601436488087403)
--(axis cs:39.4557823129252,0.602065730681575)
--(axis cs:39.7959183673469,0.601336894517607)
--(axis cs:40.1360544217687,0.600175266086662)
--(axis cs:40.4761904761905,0.600895515723396)
--(axis cs:40.8163265306122,0.599664522748065)
--(axis cs:41.156462585034,0.597554132538423)
--(axis cs:41.4965986394558,0.596023096607805)
--(axis cs:41.8367346938776,0.596433302016817)
--(axis cs:42.1768707482993,0.595722494861389)
--(axis cs:42.5170068027211,0.595380025197378)
--(axis cs:42.8571428571429,0.59355596574843)
--(axis cs:43.1972789115646,0.59314763595046)
--(axis cs:43.5374149659864,0.594740089093435)
--(axis cs:43.8775510204082,0.592897362035203)
--(axis cs:44.2176870748299,0.593292731244873)
--(axis cs:44.5578231292517,0.589558143545692)
--(axis cs:44.8979591836735,0.591664740536835)
--(axis cs:45.2380952380952,0.590527864264586)
--(axis cs:45.578231292517,0.589811237482745)
--(axis cs:45.9183673469388,0.589384934799519)
--(axis cs:46.2585034013605,0.588766914169962)
--(axis cs:46.5986394557823,0.58803420971778)
--(axis cs:46.9387755102041,0.587947704792703)
--(axis cs:47.2789115646259,0.590304896268838)
--(axis cs:47.6190476190476,0.587389166974022)
--(axis cs:47.9591836734694,0.585677083982263)
--(axis cs:48.2993197278912,0.588576861245793)
--(axis cs:48.6394557823129,0.58677548349199)
--(axis cs:48.9795918367347,0.58657568315274)
--(axis cs:49.3197278911565,0.584602154563625)
--(axis cs:49.6598639455782,0.584365687696082)
--(axis cs:50,0.584106920755551)
--(axis cs:50.3401360544218,0.58531580167483)
--(axis cs:50.6802721088435,0.583917579811626)
--(axis cs:51.0204081632653,0.581295602526229)
--(axis cs:51.3605442176871,0.58381025240608)
--(axis cs:51.7006802721088,0.581972919673906)
--(axis cs:52.0408163265306,0.58167305248127)
--(axis cs:52.3809523809524,0.579491683046445)
--(axis cs:52.7210884353741,0.577956639631659)
--(axis cs:53.0612244897959,0.574940123735356)
--(axis cs:53.4013605442177,0.576024800608888)
--(axis cs:53.7414965986395,0.576215893424557)
--(axis cs:54.0816326530612,0.573558636694698)
--(axis cs:54.421768707483,0.573869163049068)
--(axis cs:54.7619047619048,0.569413557318074)
--(axis cs:55.1020408163265,0.569903479205154)
--(axis cs:55.4421768707483,0.570960238331476)
--(axis cs:55.7823129251701,0.567119431072075)
--(axis cs:56.1224489795918,0.566351646398422)
--(axis cs:56.4625850340136,0.564818671011965)
--(axis cs:56.8027210884354,0.565380270881697)
--(axis cs:57.1428571428571,0.563078093252956)
--(axis cs:57.4829931972789,0.563300675235519)
--(axis cs:57.8231292517007,0.560716934839237)
--(axis cs:58.1632653061224,0.558838117218576)
--(axis cs:58.5034013605442,0.555752642412797)
--(axis cs:58.843537414966,0.555646059159468)
--(axis cs:59.1836734693878,0.554776807702418)
--(axis cs:59.5238095238095,0.552573915783482)
--(axis cs:59.8639455782313,0.550409753587636)
--(axis cs:60.2040816326531,0.549192914072159)
--(axis cs:60.5442176870748,0.547563277792629)
--(axis cs:60.8843537414966,0.54787611344488)
--(axis cs:61.2244897959184,0.542722222426188)
--(axis cs:61.5646258503401,0.542798882765983)
--(axis cs:61.9047619047619,0.539590747414292)
--(axis cs:62.2448979591837,0.5356080699117)
--(axis cs:62.5850340136054,0.535651869323966)
--(axis cs:62.9251700680272,0.533919644385211)
--(axis cs:63.265306122449,0.530874539406637)
--(axis cs:63.6054421768707,0.528920046963947)
--(axis cs:63.9455782312925,0.528433318442485)
--(axis cs:64.2857142857143,0.527136212638908)
--(axis cs:64.6258503401361,0.526176383578714)
--(axis cs:64.9659863945578,0.52412887553592)
--(axis cs:65.3061224489796,0.523376574880748)
--(axis cs:65.6462585034014,0.521728920684696)
--(axis cs:65.9863945578231,0.521695153282185)
--(axis cs:66.3265306122449,0.521272877287705)
--(axis cs:66.6666666666667,0.520319045155656)
--(axis cs:67.0068027210884,0.520146268878489)
--(axis cs:67.3469387755102,0.517719646847265)
--(axis cs:67.687074829932,0.519833420494332)
--(axis cs:68.0272108843537,0.519704646845451)
--(axis cs:68.3673469387755,0.519972143249638)
--(axis cs:68.7074829931973,0.518120539153078)
--(axis cs:69.0476190476191,0.518190207875724)
--(axis cs:69.3877551020408,0.518161265051486)
--(axis cs:69.7278911564626,0.517434327785275)
--(axis cs:70.0680272108844,0.516713843567309)
--(axis cs:70.4081632653061,0.518748568326727)
--(axis cs:70.7482993197279,0.51652023338873)
--(axis cs:71.0884353741497,0.515031220630754)
--(axis cs:71.4285714285714,0.51437060812515)
--(axis cs:71.7687074829932,0.514560337187605)
--(axis cs:72.108843537415,0.510971279374735)
--(axis cs:72.4489795918367,0.511544663989973)
--(axis cs:72.7891156462585,0.510872797263576)
--(axis cs:73.1292517006803,0.51025024405952)
--(axis cs:73.469387755102,0.508303697878946)
--(axis cs:73.8095238095238,0.506839551216167)
--(axis cs:74.1496598639456,0.507176349650547)
--(axis cs:74.4897959183673,0.505831356998768)
--(axis cs:74.8299319727891,0.505460755017887)
--(axis cs:75.1700680272109,0.503169223079155)
--(axis cs:75.5102040816327,0.500690684999927)
--(axis cs:75.8503401360544,0.499986792925881)
--(axis cs:76.1904761904762,0.496825562344267)
--(axis cs:76.530612244898,0.496333356479095)
--(axis cs:76.8707482993197,0.493961341860736)
--(axis cs:77.2108843537415,0.494285399453615)
--(axis cs:77.5510204081633,0.493244715798435)
--(axis cs:77.891156462585,0.491385228108681)
--(axis cs:78.2312925170068,0.490999059021145)
--(axis cs:78.5714285714286,0.489059149243418)
--(axis cs:78.9115646258503,0.488060362743462)
--(axis cs:79.2517006802721,0.485837438575016)
--(axis cs:79.5918367346939,0.484337142373248)
--(axis cs:79.9319727891156,0.483741328607239)
--(axis cs:80.2721088435374,0.483435251179797)
--(axis cs:80.6122448979592,0.482161647809534)
--(axis cs:80.9523809523809,0.481822348629871)
--(axis cs:81.2925170068027,0.478691236928556)
--(axis cs:81.6326530612245,0.475910803870121)
--(axis cs:81.9727891156463,0.475500562190102)
--(axis cs:82.312925170068,0.472554631423244)
--(axis cs:82.6530612244898,0.471970010812417)
--(axis cs:82.9931972789116,0.470357743427633)
--(axis cs:83.3333333333333,0.468920326131999)
--(axis cs:83.6734693877551,0.466318110924409)
--(axis cs:84.0136054421769,0.46279971447531)
--(axis cs:84.3537414965986,0.461757078604968)
--(axis cs:84.6938775510204,0.458608066631897)
--(axis cs:85.0340136054422,0.458971960156138)
--(axis cs:85.3741496598639,0.456119990233222)
--(axis cs:85.7142857142857,0.452327353294326)
--(axis cs:86.0544217687075,0.447996938700374)
--(axis cs:86.3945578231292,0.445399314655953)
--(axis cs:86.734693877551,0.443111629553934)
--(axis cs:87.0748299319728,0.440577024281806)
--(axis cs:87.4149659863945,0.437298431563566)
--(axis cs:87.7551020408163,0.434022341126056)
--(axis cs:88.0952380952381,0.427878386062604)
--(axis cs:88.4353741496599,0.422700711104465)
--(axis cs:88.7755102040816,0.416851596949176)
--(axis cs:89.1156462585034,0.40989894117633)
--(axis cs:89.4557823129252,0.40400141506313)
--(axis cs:89.7959183673469,0.395855536255621)
--(axis cs:90.1360544217687,0.38840588760744)
--(axis cs:90.4761904761905,0.377733603649177)
--(axis cs:90.8163265306122,0.368663416386424)
--(axis cs:91.156462585034,0.357250038798078)
--(axis cs:91.4965986394558,0.349271360108655)
--(axis cs:91.8367346938775,0.34095023716064)
--(axis cs:92.1768707482993,0.329001542673885)
--(axis cs:92.5170068027211,0.319538853932919)
--(axis cs:92.8571428571429,0.306150747537277)
--(axis cs:93.1972789115646,0.297602252831176)
--(axis cs:93.5374149659864,0.285131248285896)
--(axis cs:93.8775510204082,0.271122481681254)
--(axis cs:94.2176870748299,0.262759460064249)
--(axis cs:94.5578231292517,0.252330601142136)
--(axis cs:94.8979591836735,0.236007915886362)
--(axis cs:95.2380952380952,0.223190972709298)
--(axis cs:95.578231292517,0.208316709372761)
--(axis cs:95.9183673469388,0.191252958778784)
--(axis cs:96.2585034013605,0.179660970364354)
--(axis cs:96.5986394557823,0.164547550134514)
--(axis cs:96.9387755102041,0.154456899951668)
--(axis cs:97.2789115646258,0.14256588231525)
--(axis cs:97.6190476190476,0.13035507780948)
--(axis cs:97.9591836734694,0.121086414133913)
--(axis cs:98.2993197278912,0.107814859478575)
--(axis cs:98.6394557823129,0.0974115611444173)
--(axis cs:98.9795918367347,0.0902270129271446)
--(axis cs:99.3197278911565,0.0738813871585231)
--(axis cs:99.6598639455782,0.0478688964443034)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,0.0505623554583501)
--(axis cs:99.3197278911565,0.0774047274771279)
--(axis cs:98.9795918367347,0.093563007038163)
--(axis cs:98.6394557823129,0.100944643103871)
--(axis cs:98.2993197278912,0.11176094860526)
--(axis cs:97.9591836734694,0.125522240737016)
--(axis cs:97.6190476190476,0.13513228876039)
--(axis cs:97.2789115646258,0.147892319188215)
--(axis cs:96.9387755102041,0.160122788500796)
--(axis cs:96.5986394557823,0.170747829291471)
--(axis cs:96.2585034013605,0.185999624946248)
--(axis cs:95.9183673469388,0.198425733848021)
--(axis cs:95.578231292517,0.216388288945608)
--(axis cs:95.2380952380952,0.231529561186708)
--(axis cs:94.8979591836735,0.244857821482661)
--(axis cs:94.5578231292517,0.261387803506152)
--(axis cs:94.2176870748299,0.271886763307279)
--(axis cs:93.8775510204082,0.280558433570812)
--(axis cs:93.5374149659864,0.294641749722168)
--(axis cs:93.1972789115646,0.307268999054341)
--(axis cs:92.8571428571429,0.316150385768068)
--(axis cs:92.5170068027211,0.330066509830314)
--(axis cs:92.1768707482993,0.339568877092883)
--(axis cs:91.8367346938775,0.351485428581185)
--(axis cs:91.4965986394558,0.360068611497107)
--(axis cs:91.156462585034,0.367841385180756)
--(axis cs:90.8163265306122,0.379272239322914)
--(axis cs:90.4761904761905,0.387834838972239)
--(axis cs:90.1360544217687,0.398733816554433)
--(axis cs:89.7959183673469,0.406203672569213)
--(axis cs:89.4557823129252,0.413983404712838)
--(axis cs:89.1156462585034,0.420012355946335)
--(axis cs:88.7755102040816,0.426776799738822)
--(axis cs:88.4353741496599,0.432390673566839)
--(axis cs:88.0952380952381,0.437759839477089)
--(axis cs:87.7551020408163,0.443427216790899)
--(axis cs:87.4149659863945,0.446888028129509)
--(axis cs:87.0748299319728,0.449823692508527)
--(axis cs:86.734693877551,0.452480195383765)
--(axis cs:86.3945578231292,0.45452188751729)
--(axis cs:86.0544217687075,0.45704120264565)
--(axis cs:85.7142857142857,0.461034132948445)
--(axis cs:85.3741496598639,0.465248360039674)
--(axis cs:85.0340136054422,0.467854602581372)
--(axis cs:84.6938775510204,0.467012585278033)
--(axis cs:84.3537414965986,0.470588821398331)
--(axis cs:84.0136054421769,0.471715221662529)
--(axis cs:83.6734693877551,0.475314513192509)
--(axis cs:83.3333333333333,0.477622318574138)
--(axis cs:82.9931972789116,0.479007546819186)
--(axis cs:82.6530612244898,0.480613133151563)
--(axis cs:82.312925170068,0.48127743997349)
--(axis cs:81.9727891156463,0.484199193546663)
--(axis cs:81.6326530612245,0.484926631337959)
--(axis cs:81.2925170068027,0.487484351933487)
--(axis cs:80.9523809523809,0.490391511142663)
--(axis cs:80.6122448979592,0.491001323934292)
--(axis cs:80.2721088435374,0.492139359582795)
--(axis cs:79.9319727891156,0.492337334029638)
--(axis cs:79.5918367346939,0.493142257853823)
--(axis cs:79.2517006802721,0.494793227048765)
--(axis cs:78.9115646258503,0.496949913640302)
--(axis cs:78.5714285714286,0.497487015133296)
--(axis cs:78.2312925170068,0.499674125720919)
--(axis cs:77.891156462585,0.500110709755723)
--(axis cs:77.5510204081633,0.501811499124499)
--(axis cs:77.2108843537415,0.502957629202333)
--(axis cs:76.8707482993197,0.50282890219773)
--(axis cs:76.530612244898,0.505039136375075)
--(axis cs:76.1904761904762,0.505362754305068)
--(axis cs:75.8503401360544,0.508628859697239)
--(axis cs:75.5102040816327,0.509358057015642)
--(axis cs:75.1700680272109,0.511759663874594)
--(axis cs:74.8299319727891,0.514176670227459)
--(axis cs:74.4897959183673,0.514428317088006)
--(axis cs:74.1496598639456,0.515979697559084)
--(axis cs:73.8095238095238,0.515629584040666)
--(axis cs:73.469387755102,0.517038608406874)
--(axis cs:73.1292517006803,0.519028640832308)
--(axis cs:72.7891156462585,0.519705754866161)
--(axis cs:72.4489795918367,0.520455514685252)
--(axis cs:72.108843537415,0.520096320446519)
--(axis cs:71.7687074829932,0.523622634314933)
--(axis cs:71.4285714285714,0.52351269992158)
--(axis cs:71.0884353741497,0.52438438716972)
--(axis cs:70.7482993197279,0.526006006155656)
--(axis cs:70.4081632653061,0.527970759884893)
--(axis cs:70.0680272108844,0.525980717006128)
--(axis cs:69.7278911564626,0.527001682371949)
--(axis cs:69.3877551020408,0.52763799074336)
--(axis cs:69.0476190476191,0.527719930663314)
--(axis cs:68.7074829931973,0.528213327636859)
--(axis cs:68.3673469387755,0.529732061287336)
--(axis cs:68.0272108843537,0.52941863540084)
--(axis cs:67.687074829932,0.529436873311416)
--(axis cs:67.3469387755102,0.52774725864975)
--(axis cs:67.0068027210884,0.530112460262717)
--(axis cs:66.6666666666667,0.530405824587334)
--(axis cs:66.3265306122449,0.531567658110867)
--(axis cs:65.9863945578231,0.531738809033136)
--(axis cs:65.6462585034014,0.532012215247809)
--(axis cs:65.3061224489796,0.533371400580437)
--(axis cs:64.9659863945578,0.534255301292047)
--(axis cs:64.6258503401361,0.536537339697097)
--(axis cs:64.2857142857143,0.537412532684064)
--(axis cs:63.9455782312925,0.53882603339217)
--(axis cs:63.6054421768707,0.539609260133249)
--(axis cs:63.265306122449,0.541616943182757)
--(axis cs:62.9251700680272,0.544489287797727)
--(axis cs:62.5850340136054,0.546527089926484)
--(axis cs:62.2448979591837,0.546380485467512)
--(axis cs:61.9047619047619,0.550553980672597)
--(axis cs:61.5646258503401,0.553968383086557)
--(axis cs:61.2244897959184,0.554087305019396)
--(axis cs:60.8843537414966,0.559426256458893)
--(axis cs:60.5442176870748,0.558867332290414)
--(axis cs:60.2040816326531,0.560848486308274)
--(axis cs:59.8639455782313,0.561697125356106)
--(axis cs:59.5238095238095,0.564058762240989)
--(axis cs:59.1836734693878,0.566522664413516)
--(axis cs:58.843537414966,0.566974620241393)
--(axis cs:58.5034013605442,0.567285466345831)
--(axis cs:58.1632653061224,0.570523248926737)
--(axis cs:57.8231292517007,0.572111125083667)
--(axis cs:57.4829931972789,0.575056226767769)
--(axis cs:57.1428571428571,0.574951051600398)
--(axis cs:56.8027210884354,0.576955004045621)
--(axis cs:56.4625850340136,0.576647690942844)
--(axis cs:56.1224489795918,0.578136833729926)
--(axis cs:55.7823129251701,0.579122251770299)
--(axis cs:55.4421768707483,0.582783669738552)
--(axis cs:55.1020408163265,0.581980025036551)
--(axis cs:54.7619047619048,0.581200307900982)
--(axis cs:54.421768707483,0.586008720333073)
--(axis cs:54.0816326530612,0.585789972044976)
--(axis cs:53.7414965986395,0.588475026391937)
--(axis cs:53.4013605442177,0.588220039629355)
--(axis cs:53.0612244897959,0.587020685160173)
--(axis cs:52.7210884353741,0.590279507012099)
--(axis cs:52.3809523809524,0.59165170398809)
--(axis cs:52.0408163265306,0.593774466493272)
--(axis cs:51.7006802721088,0.5940593246098)
--(axis cs:51.3605442176871,0.596010990656536)
--(axis cs:51.0204081632653,0.593446774874169)
--(axis cs:50.6802721088435,0.59584350148905)
--(axis cs:50.3401360544218,0.597426560124052)
--(axis cs:50,0.596177923713728)
--(axis cs:49.6598639455782,0.596521293791192)
--(axis cs:49.3197278911565,0.596648872163634)
--(axis cs:48.9795918367347,0.598573844551603)
--(axis cs:48.6394557823129,0.598889014438567)
--(axis cs:48.2993197278912,0.600594379763815)
--(axis cs:47.9591836734694,0.597824654215839)
--(axis cs:47.6190476190476,0.599375595762835)
--(axis cs:47.2789115646259,0.602298311446018)
--(axis cs:46.9387755102041,0.599674136805599)
--(axis cs:46.5986394557823,0.600278423338414)
--(axis cs:46.2585034013605,0.600865566356381)
--(axis cs:45.9183673469388,0.601782141989323)
--(axis cs:45.578231292517,0.601936648171004)
--(axis cs:45.2380952380952,0.602268686016759)
--(axis cs:44.8979591836735,0.603895289916072)
--(axis cs:44.5578231292517,0.601836981899286)
--(axis cs:44.2176870748299,0.605242916650314)
--(axis cs:43.8775510204082,0.604816649149668)
--(axis cs:43.5374149659864,0.606838667048972)
--(axis cs:43.1972789115646,0.60489108841239)
--(axis cs:42.8571428571429,0.605269179503619)
--(axis cs:42.5170068027211,0.607029517629558)
--(axis cs:42.1768707482993,0.607537023471391)
--(axis cs:41.8367346938776,0.607899240737893)
--(axis cs:41.4965986394558,0.607514905987501)
--(axis cs:41.156462585034,0.609175124642864)
--(axis cs:40.8163265306122,0.611155848984051)
--(axis cs:40.4761904761905,0.612248319679629)
--(axis cs:40.1360544217687,0.611474698774909)
--(axis cs:39.7959183673469,0.612497932465904)
--(axis cs:39.4557823129252,0.613426270941341)
--(axis cs:39.1156462585034,0.612847815324439)
--(axis cs:38.7755102040816,0.613186481278947)
--(axis cs:38.4353741496599,0.614093743895606)
--(axis cs:38.0952380952381,0.613555342006822)
--(axis cs:37.7551020408163,0.616374117345485)
--(axis cs:37.4149659863946,0.614810224901928)
--(axis cs:37.0748299319728,0.618022787177104)
--(axis cs:36.734693877551,0.619230650406893)
--(axis cs:36.3945578231292,0.619009955635646)
--(axis cs:36.0544217687075,0.619978548522896)
--(axis cs:35.7142857142857,0.623333231355677)
--(axis cs:35.3741496598639,0.625494525975004)
--(axis cs:35.0340136054422,0.626193545960327)
--(axis cs:34.6938775510204,0.625516938528066)
--(axis cs:34.3537414965986,0.626848655873417)
--(axis cs:34.0136054421769,0.62507592115472)
--(axis cs:33.6734693877551,0.628515910042225)
--(axis cs:33.3333333333333,0.627192701397775)
--(axis cs:32.9931972789116,0.628108693941466)
--(axis cs:32.6530612244898,0.629058134145652)
--(axis cs:32.312925170068,0.631673782964674)
--(axis cs:31.9727891156463,0.630302861858574)
--(axis cs:31.6326530612245,0.630830722475391)
--(axis cs:31.2925170068027,0.633208894736724)
--(axis cs:30.952380952381,0.632539875664074)
--(axis cs:30.6122448979592,0.634879212442954)
--(axis cs:30.2721088435374,0.635869014355482)
--(axis cs:29.9319727891156,0.637607109801034)
--(axis cs:29.5918367346939,0.638708300132163)
--(axis cs:29.2517006802721,0.639055967849822)
--(axis cs:28.9115646258503,0.639454501523001)
--(axis cs:28.5714285714286,0.641089275735905)
--(axis cs:28.2312925170068,0.640622421281546)
--(axis cs:27.891156462585,0.641979055580758)
--(axis cs:27.5510204081633,0.642487267830834)
--(axis cs:27.2108843537415,0.641541976593189)
--(axis cs:26.8707482993197,0.642750881893825)
--(axis cs:26.530612244898,0.644761442965142)
--(axis cs:26.1904761904762,0.643940210002065)
--(axis cs:25.8503401360544,0.645256264920365)
--(axis cs:25.5102040816327,0.64514834434763)
--(axis cs:25.1700680272109,0.645600724025846)
--(axis cs:24.8299319727891,0.646817982949094)
--(axis cs:24.4897959183673,0.648035130303745)
--(axis cs:24.1496598639456,0.64685239293735)
--(axis cs:23.8095238095238,0.648680404730514)
--(axis cs:23.469387755102,0.648493399143269)
--(axis cs:23.1292517006803,0.649351030843269)
--(axis cs:22.7891156462585,0.650457803070288)
--(axis cs:22.4489795918367,0.650921585817763)
--(axis cs:22.108843537415,0.651124412193658)
--(axis cs:21.7687074829932,0.651598972147411)
--(axis cs:21.4285714285714,0.651218073853686)
--(axis cs:21.0884353741497,0.65310561423877)
--(axis cs:20.7482993197279,0.653957823559371)
--(axis cs:20.4081632653061,0.653942710070701)
--(axis cs:20.0680272108844,0.654227903470389)
--(axis cs:19.7278911564626,0.653892494146039)
--(axis cs:19.3877551020408,0.655464461369952)
--(axis cs:19.047619047619,0.655952404768181)
--(axis cs:18.7074829931973,0.655435575984958)
--(axis cs:18.3673469387755,0.656384108608731)
--(axis cs:18.0272108843537,0.655769117422218)
--(axis cs:17.687074829932,0.65683358169896)
--(axis cs:17.3469387755102,0.658094693694869)
--(axis cs:17.0068027210884,0.659857411154901)
--(axis cs:16.6666666666667,0.660647694048595)
--(axis cs:16.3265306122449,0.660828986045484)
--(axis cs:15.9863945578231,0.66135473229866)
--(axis cs:15.6462585034014,0.66139194612825)
--(axis cs:15.3061224489796,0.66263487284095)
--(axis cs:14.9659863945578,0.663358286860884)
--(axis cs:14.6258503401361,0.66512714741303)
--(axis cs:14.2857142857143,0.665169909013866)
--(axis cs:13.9455782312925,0.665240615761728)
--(axis cs:13.6054421768707,0.666401367794856)
--(axis cs:13.265306122449,0.667435898786303)
--(axis cs:12.9251700680272,0.668139399407129)
--(axis cs:12.5850340136054,0.66927106158068)
--(axis cs:12.2448979591837,0.669224318998606)
--(axis cs:11.9047619047619,0.670976436293995)
--(axis cs:11.5646258503401,0.670156632767479)
--(axis cs:11.2244897959184,0.671409628251298)
--(axis cs:10.8843537414966,0.67293165557499)
--(axis cs:10.5442176870748,0.673595042003652)
--(axis cs:10.2040816326531,0.674115704556441)
--(axis cs:9.86394557823129,0.675021080324847)
--(axis cs:9.52380952380952,0.675524324944699)
--(axis cs:9.18367346938775,0.67641863644236)
--(axis cs:8.84353741496599,0.678379306152603)
--(axis cs:8.50340136054422,0.678857096566508)
--(axis cs:8.16326530612245,0.678914924733682)
--(axis cs:7.82312925170068,0.678450767214212)
--(axis cs:7.48299319727891,0.679798772534417)
--(axis cs:7.14285714285714,0.681019673310218)
--(axis cs:6.80272108843537,0.681554745003951)
--(axis cs:6.46258503401361,0.681025760045628)
--(axis cs:6.12244897959184,0.682728535956622)
--(axis cs:5.78231292517007,0.683662602879575)
--(axis cs:5.4421768707483,0.68509528668863)
--(axis cs:5.10204081632653,0.68735107981388)
--(axis cs:4.76190476190476,0.689568725390227)
--(axis cs:4.42176870748299,0.692001841472437)
--(axis cs:4.08163265306122,0.694350189223547)
--(axis cs:3.74149659863946,0.696427056021945)
--(axis cs:3.40136054421769,0.697857595123032)
--(axis cs:3.06122448979592,0.701404801017844)
--(axis cs:2.72108843537415,0.703393784647686)
--(axis cs:2.38095238095238,0.705534576617639)
--(axis cs:2.04081632653061,0.708773054587193)
--(axis cs:1.70068027210884,0.711990663618699)
--(axis cs:1.36054421768707,0.7154776430559)
--(axis cs:1.02040816326531,0.717561290391218)
--(axis cs:0.680272108843537,0.719852744357697)
--(axis cs:0.340136054421769,0.721184357193897)
--(axis cs:0,0.721035239063252)
--cycle;


==> img/stl10/stl10_rate_distortion_lafw_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color1, mark=otimes*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table {%
0 0.719025175273418
0.340136054421769 0.712783443331718
0.680272108843537 0.695480742752552
1.02040816326531 0.659108461141586
1.36054421768707 0.605785822570324
1.70068027210884 0.552685045674443
2.04081632653061 0.506801089682849
2.38095238095238 0.466486513573295
2.72108843537415 0.427459942372555
3.06122448979592 0.39439923737783
3.40136054421769 0.358191874648751
3.74149659863946 0.325437809110184
4.08163265306122 0.297778366680877
4.42176870748299 0.272083671519221
4.76190476190476 0.248215816864727
5.10204081632653 0.227314209555904
5.4421768707483 0.203943248047783
5.78231292517007 0.186603904533572
6.12244897959184 0.166732454159706
6.46258503401361 0.148999077613895
6.80272108843537 0.138434105617719
7.14285714285714 0.129771083434283
7.48299319727891 0.122225550321237
7.82312925170068 0.115034473954424
8.16326530612245 0.107040153282187
8.50340136054422 0.0997801760205479
8.84353741496599 0.093332196396272
9.18367346938775 0.0875774279264614
9.52380952380952 0.084811488062073
9.86394557823129 0.0796434596521241
10.2040816326531 0.0743772205398245
10.5442176870748 0.074365210460202
10.8843537414966 0.0705648719212643
11.2244897959184 0.0699364371837624
11.5646258503401 0.0658950761144519
11.9047619047619 0.0636863040040053
12.2448979591837 0.0613074778208041
12.5850340136054 0.0613954435868087
12.9251700680272 0.0580943907002944
13.265306122449 0.0564895478551535
13.6054421768707 0.0556917206033966
13.9455782312925 0.0536737232773661
14.2857142857143 0.0531953679376989
14.6258503401361 0.0513935408815437
14.9659863945578 0.0482482742986342
15.3061224489796 0.0481242567039455
15.6462585034014 0.0481466576384959
15.9863945578231 0.0474504465553414
16.3265306122449 0.0465439474492328
16.6666666666667 0.0465624080760347
17.0068027210884 0.0458120970139892
17.3469387755102 0.0467177879188334
17.687074829932 0.0469226855214027
18.0272108843537 0.0470784445653325
18.3673469387755 0.0459046504643982
18.7074829931973 0.0471863887827026
19.047619047619 0.0474848139156531
19.3877551020408 0.0482687331732738
19.7278911564626 0.047742469969184
20.0680272108844 0.0480272080332096
20.4081632653061 0.046213345190757
20.7482993197279 0.0475989521205959
21.0884353741497 0.0471506253466806
21.4285714285714 0.0469065030485933
21.7687074829932 0.0467235659579401
22.108843537415 0.0476765273578554
22.4489795918367 0.0476692170381898
22.7891156462585 0.0482662085994174
23.1292517006803 0.0499738673440607
23.469387755102 0.0493207742522611
23.8095238095238 0.049340854233076
24.1496598639456 0.0498435426529249
24.4897959183673 0.0517565111809547
24.8299319727891 0.0519578313405624
25.1700680272109 0.0521413361303414
25.5102040816327 0.0534819789439905
25.8503401360544 0.0546092820766314
26.1904761904762 0.0563856473235376
26.530612244898 0.0568694830708553
26.8707482993197 0.0561233319826367
27.2108843537415 0.0596536595276419
27.5510204081633 0.0600072259846719
27.891156462585 0.0605647016081555
28.2312925170068 0.0615146698850515
28.5714285714286 0.0637102163673309
28.9115646258503 0.06287840568183
29.2517006802721 0.0627020676840398
29.5918367346939 0.0644306056366819
29.9319727891156 0.0649224349380878
30.2721088435374 0.0654147679567448
30.6122448979592 0.0671411044445101
30.952380952381 0.0672745831537912
31.2925170068027 0.0676851818695743
31.6326530612245 0.0688318009344078
31.9727891156463 0.0693015479498735
32.312925170068 0.0692481758967565
32.6530612244898 0.0704649161890933
32.9931972789116 0.0713646020946749
33.3333333333333 0.0723113197000937
33.6734693877551 0.0728605186335111
34.0136054421769 0.0746039989339687
34.3537414965986 0.0753928594477665
34.6938775510204 0.0756517329429291
35.0340136054422 0.0778583088387813
35.3741496598639 0.0781358754283642
35.7142857142857 0.0769776023505588
36.0544217687075 0.0779170446435172
36.3945578231292 0.0791380472452802
36.734693877551 0.0793230989836053
37.0748299319728 0.0793017321587451
37.4149659863946 0.082280223781161
37.7551020408163 0.0825330128823699
38.0952380952381 0.0837759956547365
38.4353741496599 0.0822825731841215
38.7755102040816 0.0844584868164663
39.1156462585034 0.082889779209258
39.4557823129252 0.083462842827726
39.7959183673469 0.0849646230444218
40.1360544217687 0.0845818373825196
40.4761904761905 0.0859983224966041
40.8163265306122 0.0856254528225485
41.156462585034 0.0866694465720006
41.4965986394558 0.087433479613467
41.8367346938776 0.0862972380205
42.1768707482993 0.0875193621915607
42.5170068027211 0.0883879035535289
42.8571428571429 0.0873103723022871
43.1972789115646 0.0889398362526361
43.5374149659864 0.089855684425392
43.8775510204082 0.0901258304467389
44.2176870748299 0.0905771435159846
44.5578231292517 0.0925658803283215
44.8979591836735 0.0936627276887265
45.2380952380952 0.0941074552914381
45.578231292517 0.0939024202020734
45.9183673469388 0.0947859941476583
46.2585034013605 0.0959205836472925
46.5986394557823 0.097388914104746
46.9387755102041 0.0973991100919607
47.2789115646259 0.0977110553604524
47.6190476190476 0.0979713015462158
47.9591836734694 0.0992729255793525
48.2993197278912 0.0996787760316099
48.6394557823129 0.0999698283804586
48.9795918367347 0.0994976466282357
49.3197278911565 0.0989918226211137
49.6598639455782 0.0972304008236852
50 0.098452946668456
50.3401360544218 0.097443885249583
50.6802721088435 0.0969335313235296
51.0204081632653 0.0985248089084404
51.3605442176871 0.0995225067421304
51.7006802721088 0.101738694068273
52.0408163265306 0.10394000130793
52.3809523809524 0.102899401047849
52.7210884353741 0.105063667178367
53.0612244897959 0.105491506063903
53.4013605442177 0.10523041817286
53.7414965986395 0.105780794774937
54.0816326530612 0.105110045055006
54.421768707483 0.105587778938197
54.7619047619048 0.105630304410002
55.1020408163265 0.104865678712942
55.4421768707483 0.104501417834556
55.7823129251701 0.103126205189983
56.1224489795918 0.102345947474577
56.4625850340136 0.100459346129163
56.8027210884354 0.100245533379485
57.1428571428571 0.0989361277100682
57.4829931972789 0.0983904663126852
57.8231292517007 0.0967427172367431
58.1632653061224 0.0984967969637495
58.5034013605442 0.0988795112551922
58.843537414966 0.0975727054238936
59.1836734693878 0.0971165485076946
59.5238095238095 0.0974676471349537
59.8639455782313 0.0980519742072326
60.2040816326531 0.0971601363536355
60.5442176870748 0.0956471621633134
60.8843537414966 0.0964670059073435
61.2244897959184 0.0957684378731635
61.5646258503401 0.0944204742068995
61.9047619047619 0.0946625922151863
62.2448979591837 0.0946041157185168
62.5850340136054 0.094861804270538
62.9251700680272 0.0936911002259462
63.265306122449 0.0940752219213989
63.6054421768707 0.0939733697070419
63.9455782312925 0.0940969039531257
64.2857142857143 0.0926147238730501
64.6258503401361 0.0928230846240337
64.9659863945578 0.0932470752313238
65.3061224489796 0.0927518830764511
65.6462585034014 0.0921761339266848
65.9863945578231 0.0914873939022194
66.3265306122449 0.0907099731591775
66.6666666666667 0.0898895641094905
67.0068027210884 0.089693480335038
67.3469387755102 0.0891681380863197
67.687074829932 0.088969559779688
68.0272108843537 0.0882061300612018
68.3673469387755 0.0865514759162457
68.7074829931973 0.0853814484809994
69.0476190476191 0.0861328918131176
69.3877551020408 0.0853572513372617
69.7278911564626 0.0840719275489948
70.0680272108844 0.0836720557909694
70.4081632653061 0.0817238586214928
70.7482993197279 0.0801335181438421
71.0884353741497 0.0806759218057772
71.4285714285714 0.0786733066634166
71.7687074829932 0.0783148498622582
72.108843537415 0.0773178891104234
72.4489795918367 0.0767298107531473
72.7891156462585 0.0758719908320335
73.1292517006803 0.074534966207091
73.469387755102 0.0747046355870394
73.8095238095238 0.0744690185137649
74.1496598639456 0.0736552154169351
74.4897959183673 0.0731326780708401
74.8299319727891 0.0722947544444853
75.1700680272109 0.0709696630965244
75.5102040816327 0.07053919140433
75.8503401360544 0.0690328796711278
76.1904761904762 0.0674091095041511
76.530612244898 0.0630310619107645
76.8707482993197 0.0639138437138213
77.2108843537415 0.0610243839621601
77.5510204081633 0.0599024293958678
77.891156462585 0.0571402733111486
78.2312925170068 0.0568470468999147
78.5714285714286 0.0530876591670066
78.9115646258503 0.051999950623092
79.2517006802721 0.0503447018814263
79.5918367346939 0.0497193074711335
79.9319727891156 0.048524658337523
80.2721088435374 0.0469782197324029
80.6122448979592 0.0455371279312404
80.9523809523809 0.0451080613488888
81.2925170068027 0.0441706774450414
81.6326530612245 0.0428788563408442
81.9727891156463 0.0423269845615204
82.312925170068 0.0418878468321621
82.6530612244898 0.0416400759988724
82.9931972789116 0.0390084050444635
83.3333333333333 0.0382147933428106
83.6734693877551 0.0379795635245366
84.0136054421769 0.0367979144996098
84.3537414965986 0.0346893858450095
84.6938775510204 0.0341894406060064
85.0340136054422 0.031686728471233
85.3741496598639 0.026164190666845
85.7142857142857 0.0252889750496366
86.0544217687075 0.0247987211121855
86.3945578231292 0.0235858168010437
86.734693877551 0.0232507316357421
87.0748299319728 0.0220051592494222
87.4149659863945 0.0213811787941803
87.7551020408163 0.0202908706775282
88.0952380952381 0.0200297425498273
88.4353741496599 0.0192641874170908
88.7755102040816 0.018002552392084
89.1156462585034 0.0171985496135985
89.4557823129252 0.016469968884207
89.7959183673469 0.0156646338882591
90.1360544217687 0.0153360733893193
90.4761904761905 0.015057580606038
90.8163265306122 0.0142945546422503
91.156462585034 0.0136673760796664
91.4965986394558 0.0127235925585605
91.8367346938775 0.0123330638863322
92.1768707482993 0.0116524829584107
92.5170068027211 0.0107858293511041
92.8571428571429 0.00990710986856372
93.1972789115646 0.00935397446786129
93.5374149659864 0.00895290555379656
93.8775510204082 0.00823912178134669
94.2176870748299 0.00746257589297925
94.5578231292517 0.00678897173537679
94.8979591836735 0.00608899144908296
95.2380952380952 0.00508578932226628
95.578231292517 0.00499316373898507
95.9183673469388 0.00432681530598175
96.2585034013605 0.00393498711647219
96.5986394557823 0.00343265747330569
96.9387755102041 0.00315459921549776
97.2789115646258 0.00289801813176948
97.6190476190476 0.00264217590486342
97.9591836734694 0.0021153647972105
98.2993197278912 0.00176957687059789
98.6394557823129 0.00147394842198397
98.9795918367347 0.0012143638604367
99.3197278911565 0.000795152580294694
99.6598639455782 0.000397327818725635
100 7.24220683423482e-14
};
\path [fill=color1, fill opacity=0.25]
(axis cs:0,0.720841397061232)
--(axis cs:0,0.717208953485605)
--(axis cs:0.340136054421769,0.710767281999437)
--(axis cs:0.680272108843537,0.692733125170136)
--(axis cs:1.02040816326531,0.655002240576951)
--(axis cs:1.36054421768707,0.600643566702241)
--(axis cs:1.70068027210884,0.547285889018398)
--(axis cs:2.04081632653061,0.501377765965775)
--(axis cs:2.38095238095238,0.46084828083815)
--(axis cs:2.72108843537415,0.421665141872414)
--(axis cs:3.06122448979592,0.388706803799781)
--(axis cs:3.40136054421769,0.352249832738631)
--(axis cs:3.74149659863946,0.31944596969328)
--(axis cs:4.08163265306122,0.291488066750122)
--(axis cs:4.42176870748299,0.265928405769739)
--(axis cs:4.76190476190476,0.241885113728161)
--(axis cs:5.10204081632653,0.221223891858612)
--(axis cs:5.4421768707483,0.197740193220151)
--(axis cs:5.78231292517007,0.180381636647312)
--(axis cs:6.12244897959184,0.160645214574032)
--(axis cs:6.46258503401361,0.143478182023138)
--(axis cs:6.80272108843537,0.133038169974933)
--(axis cs:7.14285714285714,0.124562295609197)
--(axis cs:7.48299319727891,0.117272437858615)
--(axis cs:7.82312925170068,0.109939392889391)
--(axis cs:8.16326530612245,0.1020368220109)
--(axis cs:8.50340136054422,0.0947922869884393)
--(axis cs:8.84353741496599,0.0882025176927495)
--(axis cs:9.18367346938775,0.0824705495346081)
--(axis cs:9.52380952380952,0.0798601136280617)
--(axis cs:9.86394557823129,0.074747740894298)
--(axis cs:10.2040816326531,0.0696278468747426)
--(axis cs:10.5442176870748,0.0694924582083283)
--(axis cs:10.8843537414966,0.0658557566274325)
--(axis cs:11.2244897959184,0.0651105394996906)
--(axis cs:11.5646258503401,0.0615261771457324)
--(axis cs:11.9047619047619,0.0592437423436027)
--(axis cs:12.2448979591837,0.0571317005752223)
--(axis cs:12.5850340136054,0.0571335523356545)
--(axis cs:12.9251700680272,0.0538788232545779)
--(axis cs:13.265306122449,0.0522862924800342)
--(axis cs:13.6054421768707,0.0517203789816954)
--(axis cs:13.9455782312925,0.0496394119204627)
--(axis cs:14.2857142857143,0.0492960412556189)
--(axis cs:14.6258503401361,0.0476701604840299)
--(axis cs:14.9659863945578,0.0444787591768419)
--(axis cs:15.3061224489796,0.0443021293646089)
--(axis cs:15.6462585034014,0.0443253600584542)
--(axis cs:15.9863945578231,0.0436334121504063)
--(axis cs:16.3265306122449,0.0427444788378393)
--(axis cs:16.6666666666667,0.0426459739729703)
--(axis cs:17.0068027210884,0.0422145403766163)
--(axis cs:17.3469387755102,0.0429899041874402)
--(axis cs:17.687074829932,0.0432308403257936)
--(axis cs:18.0272108843537,0.0433110614866494)
--(axis cs:18.3673469387755,0.0421318076413201)
--(axis cs:18.7074829931973,0.0434615604679068)
--(axis cs:19.047619047619,0.0436172327623684)
--(axis cs:19.3877551020408,0.0444934684499747)
--(axis cs:19.7278911564626,0.0438788862532174)
--(axis cs:20.0680272108844,0.0441993507608996)
--(axis cs:20.4081632653061,0.0423497056968551)
--(axis cs:20.7482993197279,0.0436352307906893)
--(axis cs:21.0884353741497,0.0434298170584859)
--(axis cs:21.4285714285714,0.0432408553408266)
--(axis cs:21.7687074829932,0.0430517597527162)
--(axis cs:22.108843537415,0.0440761360341106)
--(axis cs:22.4489795918367,0.0442303501886831)
--(axis cs:22.7891156462585,0.0450335061521507)
--(axis cs:23.1292517006803,0.0463814446368791)
--(axis cs:23.469387755102,0.0458101717471387)
--(axis cs:23.8095238095238,0.0457903318744682)
--(axis cs:24.1496598639456,0.0461567360852607)
--(axis cs:24.4897959183673,0.0480794512260434)
--(axis cs:24.8299319727891,0.0483203880526216)
--(axis cs:25.1700680272109,0.0484656958945539)
--(axis cs:25.5102040816327,0.0498286010079274)
--(axis cs:25.8503401360544,0.0507238668325648)
--(axis cs:26.1904761904762,0.0525321039992869)
--(axis cs:26.530612244898,0.0529887014642005)
--(axis cs:26.8707482993197,0.0525535640405714)
--(axis cs:27.2108843537415,0.055643849181271)
--(axis cs:27.5510204081633,0.0561816244635049)
--(axis cs:27.891156462585,0.0566347885066929)
--(axis cs:28.2312925170068,0.0575693236031264)
--(axis cs:28.5714285714286,0.059708570912047)
--(axis cs:28.9115646258503,0.0588840004676501)
--(axis cs:29.2517006802721,0.0586620337141087)
--(axis cs:29.5918367346939,0.0604836928803007)
--(axis cs:29.9319727891156,0.0611211114319213)
--(axis cs:30.2721088435374,0.0615888753666986)
--(axis cs:30.6122448979592,0.0632699757398248)
--(axis cs:30.952380952381,0.0633755530727979)
--(axis cs:31.2925170068027,0.0639765836769025)
--(axis cs:31.6326530612245,0.0650269566359253)
--(axis cs:31.9727891156463,0.0653569302087908)
--(axis cs:32.312925170068,0.0653894240592101)
--(axis cs:32.6530612244898,0.0663948027872615)
--(axis cs:32.9931972789116,0.0674137529166716)
--(axis cs:33.3333333333333,0.0683344436421846)
--(axis cs:33.6734693877551,0.0689343414286546)
--(axis cs:34.0136054421769,0.0706757313794914)
--(axis cs:34.3537414965986,0.0716231546248254)
--(axis cs:34.6938775510204,0.0719771867824232)
--(axis cs:35.0340136054422,0.0740400021949138)
--(axis cs:35.3741496598639,0.0744857375882331)
--(axis cs:35.7142857142857,0.0731449277042806)
--(axis cs:36.0544217687075,0.0742319762756089)
--(axis cs:36.3945578231292,0.0756262149428922)
--(axis cs:36.734693877551,0.0756391263569681)
--(axis cs:37.0748299319728,0.0757270916353223)
--(axis cs:37.4149659863946,0.0787191873424082)
--(axis cs:37.7551020408163,0.0789425315378561)
--(axis cs:38.0952380952381,0.0803305184453485)
--(axis cs:38.4353741496599,0.078697258493679)
--(axis cs:38.7755102040816,0.0809502863878307)
--(axis cs:39.1156462585034,0.0794968468638329)
--(axis cs:39.4557823129252,0.0800355312046106)
--(axis cs:39.7959183673469,0.081537978486161)
--(axis cs:40.1360544217687,0.0813285544182651)
--(axis cs:40.4761904761905,0.0826964377667013)
--(axis cs:40.8163265306122,0.0823463359333111)
--(axis cs:41.156462585034,0.0834349899588637)
--(axis cs:41.4965986394558,0.0844240110588569)
--(axis cs:41.8367346938776,0.0831464338565615)
--(axis cs:42.1768707482993,0.0845592207794695)
--(axis cs:42.5170068027211,0.0854481944211646)
--(axis cs:42.8571428571429,0.0841519764515067)
--(axis cs:43.1972789115646,0.0859010887222872)
--(axis cs:43.5374149659864,0.0869100471816985)
--(axis cs:43.8775510204082,0.0869924528370743)
--(axis cs:44.2176870748299,0.087524096523159)
--(axis cs:44.5578231292517,0.089335930031096)
--(axis cs:44.8979591836735,0.0904388683781696)
--(axis cs:45.2380952380952,0.0907871513269551)
--(axis cs:45.578231292517,0.0905098144089588)
--(axis cs:45.9183673469388,0.0914751569963618)
--(axis cs:46.2585034013605,0.0924402393937903)
--(axis cs:46.5986394557823,0.0938618686150311)
--(axis cs:46.9387755102041,0.0939234725683007)
--(axis cs:47.2789115646259,0.094318392921926)
--(axis cs:47.6190476190476,0.0944162315003282)
--(axis cs:47.9591836734694,0.0956698227237529)
--(axis cs:48.2993197278912,0.0961975038294372)
--(axis cs:48.6394557823129,0.0963323545983201)
--(axis cs:48.9795918367347,0.095780780716879)
--(axis cs:49.3197278911565,0.0953513324910981)
--(axis cs:49.6598639455782,0.0938038560253641)
--(axis cs:50,0.0949567002719554)
--(axis cs:50.3401360544218,0.0940593864628246)
--(axis cs:50.6802721088435,0.093527212264988)
--(axis cs:51.0204081632653,0.094946562458738)
--(axis cs:51.3605442176871,0.0962206076867815)
--(axis cs:51.7006802721088,0.098047563767376)
--(axis cs:52.0408163265306,0.100355952829618)
--(axis cs:52.3809523809524,0.0991771111362821)
--(axis cs:52.7210884353741,0.10160118179878)
--(axis cs:53.0612244897959,0.101815984653748)
--(axis cs:53.4013605442177,0.101497377119061)
--(axis cs:53.7414965986395,0.102242037772752)
--(axis cs:54.0816326530612,0.101615969306899)
--(axis cs:54.421768707483,0.102112351520837)
--(axis cs:54.7619047619048,0.102197557538781)
--(axis cs:55.1020408163265,0.101527002964591)
--(axis cs:55.4421768707483,0.10111054873131)
--(axis cs:55.7823129251701,0.0997354363685003)
--(axis cs:56.1224489795918,0.0990239175464541)
--(axis cs:56.4625850340136,0.097130245838467)
--(axis cs:56.8027210884354,0.0969279783852488)
--(axis cs:57.1428571428571,0.0958503903857582)
--(axis cs:57.4829931972789,0.0952538039436299)
--(axis cs:57.8231292517007,0.093923439579787)
--(axis cs:58.1632653061224,0.0955011716852439)
--(axis cs:58.5034013605442,0.0959541128609694)
--(axis cs:58.843537414966,0.0948072123494108)
--(axis cs:59.1836734693878,0.0942591816541882)
--(axis cs:59.5238095238095,0.0946718181805899)
--(axis cs:59.8639455782313,0.0953262064172785)
--(axis cs:60.2040816326531,0.0944137229699814)
--(axis cs:60.5442176870748,0.0930329787083277)
--(axis cs:60.8843537414966,0.0938266727762157)
--(axis cs:61.2244897959184,0.0930142678210365)
--(axis cs:61.5646258503401,0.0918271716169428)
--(axis cs:61.9047619047619,0.0920120407621615)
--(axis cs:62.2448979591837,0.0919489403058122)
--(axis cs:62.5850340136054,0.0921727990938813)
--(axis cs:62.9251700680272,0.0911957417418098)
--(axis cs:63.265306122449,0.0914780018688035)
--(axis cs:63.6054421768707,0.0913444066245934)
--(axis cs:63.9455782312925,0.091561469215906)
--(axis cs:64.2857142857143,0.0901445637215571)
--(axis cs:64.6258503401361,0.0902546248954202)
--(axis cs:64.9659863945578,0.0907375561160917)
--(axis cs:65.3061224489796,0.0903545665049663)
--(axis cs:65.6462585034014,0.0898383657610816)
--(axis cs:65.9863945578231,0.0891811312293306)
--(axis cs:66.3265306122449,0.0883754086593618)
--(axis cs:66.6666666666667,0.0875220517936125)
--(axis cs:67.0068027210884,0.0874623934959634)
--(axis cs:67.3469387755102,0.0869445788296397)
--(axis cs:67.687074829932,0.0868657016990372)
--(axis cs:68.0272108843537,0.0858464794193781)
--(axis cs:68.3673469387755,0.0843386784804215)
--(axis cs:68.7074829931973,0.0831536555840699)
--(axis cs:69.0476190476191,0.0839967743022899)
--(axis cs:69.3877551020408,0.0832419448589647)
--(axis cs:69.7278911564626,0.081966088182841)
--(axis cs:70.0680272108844,0.0815642205578019)
--(axis cs:70.4081632653061,0.0794853076471287)
--(axis cs:70.7482993197279,0.0779855403423387)
--(axis cs:71.0884353741497,0.0784977652348346)
--(axis cs:71.4285714285714,0.0764696796732193)
--(axis cs:71.7687074829932,0.0759500782053718)
--(axis cs:72.108843537415,0.0750671730526734)
--(axis cs:72.4489795918367,0.0744722650722571)
--(axis cs:72.7891156462585,0.0735981868486426)
--(axis cs:73.1292517006803,0.0721895423386227)
--(axis cs:73.469387755102,0.0724035283842147)
--(axis cs:73.8095238095238,0.0720785033312851)
--(axis cs:74.1496598639456,0.0713014895639622)
--(axis cs:74.4897959183673,0.0709021565922301)
--(axis cs:74.8299319727891,0.0699447760145406)
--(axis cs:75.1700680272109,0.0684839078311699)
--(axis cs:75.5102040816327,0.0680610034418235)
--(axis cs:75.8503401360544,0.0665044235797328)
--(axis cs:76.1904761904762,0.0647721423840145)
--(axis cs:76.530612244898,0.060507312009991)
--(axis cs:76.8707482993197,0.0612679120357161)
--(axis cs:77.2108843537415,0.0583302755953937)
--(axis cs:77.5510204081633,0.0571341714745327)
--(axis cs:77.891156462585,0.0543607802992603)
--(axis cs:78.2312925170068,0.0541103453933463)
--(axis cs:78.5714285714286,0.0505495438868179)
--(axis cs:78.9115646258503,0.0495171002049271)
--(axis cs:79.2517006802721,0.0480855324314593)
--(axis cs:79.5918367346939,0.0474307667357891)
--(axis cs:79.9319727891156,0.0461889101283203)
--(axis cs:80.2721088435374,0.0448634756609302)
--(axis cs:80.6122448979592,0.0432411700953211)
--(axis cs:80.9523809523809,0.0427621423057976)
--(axis cs:81.2925170068027,0.0418482297562499)
--(axis cs:81.6326530612245,0.0404912176634706)
--(axis cs:81.9727891156463,0.0398841667178307)
--(axis cs:82.312925170068,0.0394977539874375)
--(axis cs:82.6530612244898,0.0392637575222793)
--(axis cs:82.9931972789116,0.0367445654014958)
--(axis cs:83.3333333333333,0.036000340569762)
--(axis cs:83.6734693877551,0.0355207537486608)
--(axis cs:84.0136054421769,0.0343424241601315)
--(axis cs:84.3537414965986,0.0321823719542464)
--(axis cs:84.6938775510204,0.0316554530149417)
--(axis cs:85.0340136054422,0.0292281640147042)
--(axis cs:85.3741496598639,0.0244619805511871)
--(axis cs:85.7142857142857,0.0236647692943982)
--(axis cs:86.0544217687075,0.0231400229129898)
--(axis cs:86.3945578231292,0.021947315907773)
--(axis cs:86.734693877551,0.021629229805664)
--(axis cs:87.0748299319728,0.0204709489884881)
--(axis cs:87.4149659863945,0.0198708648445736)
--(axis cs:87.7551020408163,0.0188134513110168)
--(axis cs:88.0952380952381,0.0184947916279615)
--(axis cs:88.4353741496599,0.0178187665534622)
--(axis cs:88.7755102040816,0.0166362609595503)
--(axis cs:89.1156462585034,0.0158222345254533)
--(axis cs:89.4557823129252,0.0150519043147593)
--(axis cs:89.7959183673469,0.0144273758987245)
--(axis cs:90.1360544217687,0.0140488803430222)
--(axis cs:90.4761904761905,0.0138196157886986)
--(axis cs:90.8163265306122,0.0130110732136319)
--(axis cs:91.156462585034,0.0124599320243548)
--(axis cs:91.4965986394558,0.0115638445085778)
--(axis cs:91.8367346938775,0.0111244322156108)
--(axis cs:92.1768707482993,0.0105185886473942)
--(axis cs:92.5170068027211,0.00967408772534162)
--(axis cs:92.8571428571429,0.00884598219499057)
--(axis cs:93.1972789115646,0.00834354504310355)
--(axis cs:93.5374149659864,0.00793266310525786)
--(axis cs:93.8775510204082,0.00726918303658333)
--(axis cs:94.2176870748299,0.00653995493902409)
--(axis cs:94.5578231292517,0.00592500527704068)
--(axis cs:94.8979591836735,0.0052882305449678)
--(axis cs:95.2380952380952,0.00441851985824056)
--(axis cs:95.578231292517,0.00432397390663412)
--(axis cs:95.9183673469388,0.00370557686697785)
--(axis cs:96.2585034013605,0.00325994394612729)
--(axis cs:96.5986394557823,0.00279874353756718)
--(axis cs:96.9387755102041,0.0026074263862108)
--(axis cs:97.2789115646258,0.00236688689607325)
--(axis cs:97.6190476190476,0.00210547121688346)
--(axis cs:97.9591836734694,0.00165735660800684)
--(axis cs:98.2993197278912,0.00139837270974213)
--(axis cs:98.6394557823129,0.00114095942583384)
--(axis cs:98.9795918367347,0.000980436829323551)
--(axis cs:99.3197278911565,0.000610538536294002)
--(axis cs:99.6598639455782,0.000275273694685498)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:99.6598639455782,0.000519381942765772)
--(axis cs:99.3197278911565,0.000979766624295385)
--(axis cs:98.9795918367347,0.00144829089154984)
--(axis cs:98.6394557823129,0.0018069374181341)
--(axis cs:98.2993197278912,0.00214078103145364)
--(axis cs:97.9591836734694,0.00257337298641416)
--(axis cs:97.6190476190476,0.00317888059284338)
--(axis cs:97.2789115646258,0.0034291493674657)
--(axis cs:96.9387755102041,0.00370177204478472)
--(axis cs:96.5986394557823,0.0040665714090442)
--(axis cs:96.2585034013605,0.00461003028681709)
--(axis cs:95.9183673469388,0.00494805374498565)
--(axis cs:95.578231292517,0.00566235357133603)
--(axis cs:95.2380952380952,0.00575305878629201)
--(axis cs:94.8979591836735,0.00688975235319811)
--(axis cs:94.5578231292517,0.00765293819371289)
--(axis cs:94.2176870748299,0.00838519684693441)
--(axis cs:93.8775510204082,0.00920906052611006)
--(axis cs:93.5374149659864,0.00997314800233527)
--(axis cs:93.1972789115646,0.010364403892619)
--(axis cs:92.8571428571429,0.0109682375421369)
--(axis cs:92.5170068027211,0.0118975709768665)
--(axis cs:92.1768707482993,0.0127863772694272)
--(axis cs:91.8367346938775,0.0135416955570535)
--(axis cs:91.4965986394558,0.0138833406085432)
--(axis cs:91.156462585034,0.014874820134978)
--(axis cs:90.8163265306122,0.0155780360708687)
--(axis cs:90.4761904761905,0.0162955454233775)
--(axis cs:90.1360544217687,0.0166232664356164)
--(axis cs:89.7959183673469,0.0169018918777936)
--(axis cs:89.4557823129252,0.0178880334536547)
--(axis cs:89.1156462585034,0.0185748647017437)
--(axis cs:88.7755102040816,0.0193688438246178)
--(axis cs:88.4353741496599,0.0207096082807194)
--(axis cs:88.0952380952381,0.0215646934716931)
--(axis cs:87.7551020408163,0.0217682900440396)
--(axis cs:87.4149659863945,0.022891492743787)
--(axis cs:87.0748299319728,0.0235393695103562)
--(axis cs:86.734693877551,0.0248722334658201)
--(axis cs:86.3945578231292,0.0252243176943144)
--(axis cs:86.0544217687075,0.0264574193113813)
--(axis cs:85.7142857142857,0.0269131808048751)
--(axis cs:85.3741496598639,0.0278664007825029)
--(axis cs:85.0340136054422,0.0341452929277618)
--(axis cs:84.6938775510204,0.0367234281970712)
--(axis cs:84.3537414965986,0.0371963997357725)
--(axis cs:84.0136054421769,0.0392534048390882)
--(axis cs:83.6734693877551,0.0404383733004124)
--(axis cs:83.3333333333333,0.0404292461158592)
--(axis cs:82.9931972789116,0.0412722446874313)
--(axis cs:82.6530612244898,0.0440163944754654)
--(axis cs:82.312925170068,0.0442779396768868)
--(axis cs:81.9727891156463,0.0447698024052101)
--(axis cs:81.6326530612245,0.0452664950182179)
--(axis cs:81.2925170068027,0.0464931251338329)
--(axis cs:80.9523809523809,0.0474539803919801)
--(axis cs:80.6122448979592,0.0478330857671598)
--(axis cs:80.2721088435374,0.0490929638038756)
--(axis cs:79.9319727891156,0.0508604065467257)
--(axis cs:79.5918367346939,0.0520078482064779)
--(axis cs:79.2517006802721,0.0526038713313932)
--(axis cs:78.9115646258503,0.054482801041257)
--(axis cs:78.5714285714286,0.0556257744471954)
--(axis cs:78.2312925170068,0.0595837484064831)
--(axis cs:77.891156462585,0.059919766323037)
--(axis cs:77.5510204081633,0.0626706873172028)
--(axis cs:77.2108843537415,0.0637184923289265)
--(axis cs:76.8707482993197,0.0665597753919265)
--(axis cs:76.530612244898,0.0655548118115379)
--(axis cs:76.1904761904762,0.0700460766242877)
--(axis cs:75.8503401360544,0.0715613357625228)
--(axis cs:75.5102040816327,0.0730173793668365)
--(axis cs:75.1700680272109,0.0734554183618788)
--(axis cs:74.8299319727891,0.07464473287443)
--(axis cs:74.4897959183673,0.0753631995494501)
--(axis cs:74.1496598639456,0.076008941269908)
--(axis cs:73.8095238095238,0.0768595336962448)
--(axis cs:73.469387755102,0.0770057427898641)
--(axis cs:73.1292517006803,0.0768803900755593)
--(axis cs:72.7891156462585,0.0781457948154243)
--(axis cs:72.4489795918367,0.0789873564340376)
--(axis cs:72.108843537415,0.0795686051681735)
--(axis cs:71.7687074829932,0.0806796215191447)
--(axis cs:71.4285714285714,0.0808769336536139)
--(axis cs:71.0884353741497,0.0828540783767197)
--(axis cs:70.7482993197279,0.0822814959453455)
--(axis cs:70.4081632653061,0.0839624095958569)
--(axis cs:70.0680272108844,0.0857798910241368)
--(axis cs:69.7278911564626,0.0861777669151486)
--(axis cs:69.3877551020408,0.0874725578155587)
--(axis cs:69.0476190476191,0.0882690093239453)
--(axis cs:68.7074829931973,0.0876092413779288)
--(axis cs:68.3673469387755,0.0887642733520699)
--(axis cs:68.0272108843537,0.0905657807030255)
--(axis cs:67.687074829932,0.0910734178603387)
--(axis cs:67.3469387755102,0.0913916973429996)
--(axis cs:67.0068027210884,0.0919245671741126)
--(axis cs:66.6666666666667,0.0922570764253684)
--(axis cs:66.3265306122449,0.0930445376589931)
--(axis cs:65.9863945578231,0.0937936565751082)
--(axis cs:65.6462585034014,0.0945139020922879)
--(axis cs:65.3061224489796,0.0951491996479359)
--(axis cs:64.9659863945578,0.095756594346556)
--(axis cs:64.6258503401361,0.0953915443526471)
--(axis cs:64.2857142857143,0.0950848840245431)
--(axis cs:63.9455782312925,0.0966323386903454)
--(axis cs:63.6054421768707,0.0966023327894904)
--(axis cs:63.265306122449,0.0966724419739943)
--(axis cs:62.9251700680272,0.0961864587100825)
--(axis cs:62.5850340136054,0.0975508094471946)
--(axis cs:62.2448979591837,0.0972592911312215)
--(axis cs:61.9047619047619,0.0973131436682111)
--(axis cs:61.5646258503401,0.0970137767968562)
--(axis cs:61.2244897959184,0.0985226079252906)
--(axis cs:60.8843537414966,0.0991073390384712)
--(axis cs:60.5442176870748,0.0982613456182992)
--(axis cs:60.2040816326531,0.0999065497372895)
--(axis cs:59.8639455782313,0.100777741997187)
--(axis cs:59.5238095238095,0.100263476089318)
--(axis cs:59.1836734693878,0.099973915361201)
--(axis cs:58.843537414966,0.100338198498376)
--(axis cs:58.5034013605442,0.101804909649415)
--(axis cs:58.1632653061224,0.101492422242255)
--(axis cs:57.8231292517007,0.0995619948936991)
--(axis cs:57.4829931972789,0.101527128681741)
--(axis cs:57.1428571428571,0.102021865034378)
--(axis cs:56.8027210884354,0.103563088373721)
--(axis cs:56.4625850340136,0.103788446419859)
--(axis cs:56.1224489795918,0.105667977402699)
--(axis cs:55.7823129251701,0.106516974011467)
--(axis cs:55.4421768707483,0.107892286937801)
--(axis cs:55.1020408163265,0.108204354461293)
--(axis cs:54.7619047619048,0.109063051281223)
--(axis cs:54.421768707483,0.109063206355557)
--(axis cs:54.0816326530612,0.108604120803113)
--(axis cs:53.7414965986395,0.109319551777123)
--(axis cs:53.4013605442177,0.10896345922666)
--(axis cs:53.0612244897959,0.109167027474058)
--(axis cs:52.7210884353741,0.108526152557953)
--(axis cs:52.3809523809524,0.106621690959416)
--(axis cs:52.0408163265306,0.107524049786243)
--(axis cs:51.7006802721088,0.10542982436917)
--(axis cs:51.3605442176871,0.102824405797479)
--(axis cs:51.0204081632653,0.102103055358143)
--(axis cs:50.6802721088435,0.100339850382071)
--(axis cs:50.3401360544218,0.100828384036341)
--(axis cs:50,0.101949193064957)
--(axis cs:49.6598639455782,0.100656945622006)
--(axis cs:49.3197278911565,0.102632312751129)
--(axis cs:48.9795918367347,0.103214512539592)
--(axis cs:48.6394557823129,0.103607302162597)
--(axis cs:48.2993197278912,0.103160048233783)
--(axis cs:47.9591836734694,0.102876028434952)
--(axis cs:47.6190476190476,0.101526371592103)
--(axis cs:47.2789115646259,0.101103717798979)
--(axis cs:46.9387755102041,0.100874747615621)
--(axis cs:46.5986394557823,0.100915959594461)
--(axis cs:46.2585034013605,0.0994009279007948)
--(axis cs:45.9183673469388,0.0980968312989549)
--(axis cs:45.578231292517,0.097295025995188)
--(axis cs:45.2380952380952,0.0974277592559212)
--(axis cs:44.8979591836735,0.0968865869992835)
--(axis cs:44.5578231292517,0.095795830625547)
--(axis cs:44.2176870748299,0.0936301905088103)
--(axis cs:43.8775510204082,0.0932592080564036)
--(axis cs:43.5374149659864,0.0928013216690855)
--(axis cs:43.1972789115646,0.091978583782985)
--(axis cs:42.8571428571429,0.0904687681530674)
--(axis cs:42.5170068027211,0.0913276126858933)
--(axis cs:42.1768707482993,0.0904795036036519)
--(axis cs:41.8367346938776,0.0894480421844385)
--(axis cs:41.4965986394558,0.0904429481680772)
--(axis cs:41.156462585034,0.0899039031851375)
--(axis cs:40.8163265306122,0.0889045697117859)
--(axis cs:40.4761904761905,0.0893002072265068)
--(axis cs:40.1360544217687,0.087835120346774)
--(axis cs:39.7959183673469,0.0883912676026827)
--(axis cs:39.4557823129252,0.0868901544508413)
--(axis cs:39.1156462585034,0.086282711554683)
--(axis cs:38.7755102040816,0.0879666872451019)
--(axis cs:38.4353741496599,0.0858678878745639)
--(axis cs:38.0952380952381,0.0872214728641245)
--(axis cs:37.7551020408163,0.0861234942268837)
--(axis cs:37.4149659863946,0.0858412602199138)
--(axis cs:37.0748299319728,0.0828763726821679)
--(axis cs:36.734693877551,0.0830070716102425)
--(axis cs:36.3945578231292,0.0826498795476682)
--(axis cs:36.0544217687075,0.0816021130114256)
--(axis cs:35.7142857142857,0.080810276996837)
--(axis cs:35.3741496598639,0.0817860132684952)
--(axis cs:35.0340136054422,0.0816766154826489)
--(axis cs:34.6938775510204,0.0793262791034351)
--(axis cs:34.3537414965986,0.0791625642707075)
--(axis cs:34.0136054421769,0.0785322664884461)
--(axis cs:33.6734693877551,0.0767866958383675)
--(axis cs:33.3333333333333,0.0762881957580029)
--(axis cs:32.9931972789116,0.0753154512726782)
--(axis cs:32.6530612244898,0.0745350295909251)
--(axis cs:32.312925170068,0.0731069277343029)
--(axis cs:31.9727891156463,0.0732461656909563)
--(axis cs:31.6326530612245,0.0726366452328902)
--(axis cs:31.2925170068027,0.0713937800622462)
--(axis cs:30.952380952381,0.0711736132347846)
--(axis cs:30.6122448979592,0.0710122331491955)
--(axis cs:30.2721088435374,0.069240660546791)
--(axis cs:29.9319727891156,0.0687237584442542)
--(axis cs:29.5918367346939,0.0683775183930631)
--(axis cs:29.2517006802721,0.0667421016539709)
--(axis cs:28.9115646258503,0.0668728108960098)
--(axis cs:28.5714285714286,0.0677118618226148)
--(axis cs:28.2312925170068,0.0654600161669766)
--(axis cs:27.891156462585,0.064494614709618)
--(axis cs:27.5510204081633,0.0638328275058389)
--(axis cs:27.2108843537415,0.0636634698740129)
--(axis cs:26.8707482993197,0.0596930999247021)
--(axis cs:26.530612244898,0.0607502646775101)
--(axis cs:26.1904761904762,0.0602391906477883)
--(axis cs:25.8503401360544,0.0584946973206981)
--(axis cs:25.5102040816327,0.0571353568800536)
--(axis cs:25.1700680272109,0.0558169763661289)
--(axis cs:24.8299319727891,0.0555952746285033)
--(axis cs:24.4897959183673,0.055433571135866)
--(axis cs:24.1496598639456,0.0535303492205892)
--(axis cs:23.8095238095238,0.0528913765916837)
--(axis cs:23.469387755102,0.0528313767573834)
--(axis cs:23.1292517006803,0.0535662900512422)
--(axis cs:22.7891156462585,0.0514989110466842)
--(axis cs:22.4489795918367,0.0511080838876966)
--(axis cs:22.108843537415,0.0512769186816003)
--(axis cs:21.7687074829932,0.050395372163164)
--(axis cs:21.4285714285714,0.05057215075636)
--(axis cs:21.0884353741497,0.0508714336348753)
--(axis cs:20.7482993197279,0.0515626734505024)
--(axis cs:20.4081632653061,0.050076984684659)
--(axis cs:20.0680272108844,0.0518550653055195)
--(axis cs:19.7278911564626,0.0516060536851506)
--(axis cs:19.3877551020408,0.0520439978965728)
--(axis cs:19.047619047619,0.0513523950689377)
--(axis cs:18.7074829931973,0.0509112170974985)
--(axis cs:18.3673469387755,0.0496774932874763)
--(axis cs:18.0272108843537,0.0508458276440155)
--(axis cs:17.687074829932,0.0506145307170118)
--(axis cs:17.3469387755102,0.0504456716502266)
--(axis cs:17.0068027210884,0.049409653651362)
--(axis cs:16.6666666666667,0.050478842179099)
--(axis cs:16.3265306122449,0.0503434160606263)
--(axis cs:15.9863945578231,0.0512674809602766)
--(axis cs:15.6462585034014,0.0519679552185375)
--(axis cs:15.3061224489796,0.0519463840432821)
--(axis cs:14.9659863945578,0.0520177894204265)
--(axis cs:14.6258503401361,0.0551169212790576)
--(axis cs:14.2857142857143,0.0570946946197789)
--(axis cs:13.9455782312925,0.0577080346342695)
--(axis cs:13.6054421768707,0.0596630622250977)
--(axis cs:13.265306122449,0.0606928032302728)
--(axis cs:12.9251700680272,0.0623099581460109)
--(axis cs:12.5850340136054,0.065657334837963)
--(axis cs:12.2448979591837,0.0654832550663859)
--(axis cs:11.9047619047619,0.0681288656644079)
--(axis cs:11.5646258503401,0.0702639750831714)
--(axis cs:11.2244897959184,0.0747623348678342)
--(axis cs:10.8843537414966,0.0752739872150962)
--(axis cs:10.5442176870748,0.0792379627120756)
--(axis cs:10.2040816326531,0.0791265942049063)
--(axis cs:9.86394557823129,0.0845391784099502)
--(axis cs:9.52380952380952,0.0897628624960843)
--(axis cs:9.18367346938775,0.0926843063183146)
--(axis cs:8.84353741496599,0.0984618750997945)
--(axis cs:8.50340136054422,0.104768065052656)
--(axis cs:8.16326530612245,0.112043484553473)
--(axis cs:7.82312925170068,0.120129555019456)
--(axis cs:7.48299319727891,0.127178662783859)
--(axis cs:7.14285714285714,0.13497987125937)
--(axis cs:6.80272108843537,0.143830041260505)
--(axis cs:6.46258503401361,0.154519973204653)
--(axis cs:6.12244897959184,0.172819693745381)
--(axis cs:5.78231292517007,0.192826172419832)
--(axis cs:5.4421768707483,0.210146302875415)
--(axis cs:5.10204081632653,0.233404527253197)
--(axis cs:4.76190476190476,0.254546520001293)
--(axis cs:4.42176870748299,0.278238937268703)
--(axis cs:4.08163265306122,0.304068666611633)
--(axis cs:3.74149659863946,0.331429648527088)
--(axis cs:3.40136054421769,0.364133916558871)
--(axis cs:3.06122448979592,0.400091670955879)
--(axis cs:2.72108843537415,0.433254742872695)
--(axis cs:2.38095238095238,0.472124746308441)
--(axis cs:2.04081632653061,0.512224413399923)
--(axis cs:1.70068027210884,0.558084202330489)
--(axis cs:1.36054421768707,0.610928078438407)
--(axis cs:1.02040816326531,0.663214681706221)
--(axis cs:0.680272108843537,0.698228360334968)
--(axis cs:0.340136054421769,0.714799604664)
--(axis cs:0,0.720841397061232)
--cycle;


==> img/stl10/stl10_rate_distortion_lagrange.tex <==
\addplot [line width=0.5, opacity=0.7, color4, mark=o, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color4, thin}]
table [row sep=\\]{%
0	0.718871769607067 \\
0.340136054421769	0.719493958055973 \\
0.680272108843537	0.71625630453229 \\
1.02040816326531	0.703948264271021 \\
1.36054421768707	0.679467786625028 \\
1.70068027210884	0.651674620322883 \\
2.04081632653061	0.625048905462027 \\
2.38095238095238	0.594636884648353 \\
2.72108843537415	0.551524647399783 \\
3.06122448979592	0.507992276260629 \\
3.40136054421769	0.472589885657653 \\
3.74149659863946	0.443636701933574 \\
4.08163265306122	0.41685531952302 \\
4.42176870748299	0.391176964360493 \\
4.76190476190476	0.36485285984071 \\
5.10204081632653	0.343034941912419 \\
5.4421768707483	0.326801316884475 \\
5.78231292517007	0.309553807616843 \\
6.12244897959184	0.293043122518471 \\
6.46258503401361	0.276852323598492 \\
6.80272108843537	0.264872683571605 \\
7.14285714285714	0.254581287870811 \\
7.48299319727891	0.242558151287228 \\
7.82312925170068	0.233411982766834 \\
8.16326530612245	0.225053182081419 \\
8.50340136054422	0.220237807829719 \\
8.84353741496599	0.213612035682004 \\
9.18367346938775	0.212830382328583 \\
9.52380952380952	0.206840390397487 \\
9.86394557823129	0.201886346174067 \\
10.2040816326531	0.199662873630417 \\
10.5442176870748	0.199495882260327 \\
10.8843537414966	0.197246874698445 \\
11.2244897959184	0.194597411097645 \\
11.5646258503401	0.19163765949284 \\
11.9047619047619	0.19235558668442 \\
12.2448979591837	0.190861670396027 \\
12.5850340136054	0.190388129852059 \\
12.9251700680272	0.189542625296039 \\
13.265306122449	0.186726153836661 \\
13.6054421768707	0.186752561260057 \\
13.9455782312925	0.189966004340263 \\
14.2857142857143	0.190208841769521 \\
14.6258503401361	0.191758768882684 \\
14.9659863945578	0.191971130983234 \\
15.3061224489796	0.190108257045957 \\
15.6462585034014	0.18911555271939 \\
15.9863945578231	0.189418712509593 \\
16.3265306122449	0.188830058346328 \\
16.6666666666667	0.189230619488394 \\
17.0068027210884	0.190968650428592 \\
17.3469387755102	0.189391626780057 \\
17.687074829932	0.190580307953554 \\
18.0272108843537	0.191191524477798 \\
18.3673469387755	0.192243675468106 \\
18.7074829931973	0.192663583600538 \\
19.047619047619	0.190823985428653 \\
19.3877551020408	0.192639507542495 \\
19.7278911564626	0.192057282981264 \\
20.0680272108844	0.193221058089396 \\
20.4081632653061	0.19201314870672 \\
20.7482993197279	0.190440101997912 \\
21.0884353741497	0.191829122927974 \\
21.4285714285714	0.192470140484643 \\
21.7687074829932	0.191487763160437 \\
22.108843537415	0.190918908671876 \\
22.4489795918367	0.19371621001026 \\
22.7891156462585	0.195015264662524 \\
23.1292517006803	0.194340096818594 \\
23.469387755102	0.196159889521615 \\
23.8095238095238	0.197859248228875 \\
24.1496598639456	0.19570130566213 \\
24.4897959183673	0.198669520462798 \\
24.8299319727891	0.20041022631437 \\
25.1700680272109	0.198944094680542 \\
25.5102040816327	0.201513675523802 \\
25.8503401360544	0.198052291039015 \\
26.1904761904762	0.200043921110332 \\
26.530612244898	0.19957145155418 \\
26.8707482993197	0.200134161784811 \\
27.2108843537415	0.199220631414469 \\
27.5510204081633	0.200668896015328 \\
27.891156462585	0.201584934774993 \\
28.2312925170068	0.204335535091226 \\
28.5714285714286	0.202727688930659 \\
28.9115646258503	0.203291754610767 \\
29.2517006802721	0.203003152821095 \\
29.5918367346939	0.204087386748748 \\
29.9319727891156	0.20332131802428 \\
30.2721088435374	0.203775866093163 \\
30.6122448979592	0.205697837412991 \\
30.952380952381	0.206659878879592 \\
31.2925170068027	0.206421201471166 \\
31.6326530612245	0.208341621035236 \\
31.9727891156463	0.208766998587533 \\
32.312925170068	0.209084415317997 \\
32.6530612244898	0.20907349705423 \\
32.9931972789116	0.210104700812582 \\
33.3333333333333	0.209408669691614 \\
33.6734693877551	0.208336058154734 \\
34.0136054421769	0.21026959549499 \\
34.3537414965986	0.210116782983285 \\
34.6938775510204	0.209938737760382 \\
35.0340136054422	0.21014798526926 \\
35.3741496598639	0.210143003668994 \\
35.7142857142857	0.209367773082203 \\
36.0544217687075	0.209669303803605 \\
36.3945578231292	0.208424923476718 \\
36.734693877551	0.210749818356267 \\
37.0748299319728	0.211042200979711 \\
37.4149659863946	0.212952055167416 \\
37.7551020408163	0.21096886948141 \\
38.0952380952381	0.210824753510072 \\
38.4353741496599	0.211717924878808 \\
38.7755102040816	0.211456320400694 \\
39.1156462585034	0.211612429770036 \\
39.4557823129252	0.213241768041949 \\
39.7959183673469	0.213431112467735 \\
40.1360544217687	0.21138945989469 \\
40.4761904761905	0.213822890625613 \\
40.8163265306122	0.213564323026269 \\
41.156462585034	0.213751923612512 \\
41.4965986394558	0.215192623017646 \\
41.8367346938776	0.214764329723938 \\
42.1768707482993	0.214083565065821 \\
42.5170068027211	0.213774928760108 \\
42.8571428571429	0.21362406563218 \\
43.1972789115646	0.216341758903996 \\
43.5374149659864	0.213288499312527 \\
43.8775510204082	0.215510298100127 \\
44.2176870748299	0.215216575771211 \\
44.5578231292517	0.214423390631723 \\
44.8979591836735	0.216803529865423 \\
45.2380952380952	0.214551238971569 \\
45.578231292517	0.210623697961449 \\
45.9183673469388	0.215339538076033 \\
46.2585034013605	0.213434535639389 \\
46.5986394557823	0.212858435867732 \\
46.9387755102041	0.212796795197958 \\
47.2789115646259	0.211993402224767 \\
47.6190476190476	0.210959895446908 \\
47.9591836734694	0.211392391141827 \\
48.2993197278912	0.210293723456546 \\
48.6394557823129	0.210110075325445 \\
48.9795918367347	0.21003769526879 \\
49.3197278911565	0.210914049828138 \\
49.6598639455782	0.209753733858132 \\
50	0.209960404039212 \\
50.3401360544218	0.20856292411246 \\
50.6802721088435	0.208596516903313 \\
51.0204081632653	0.207388661663562 \\
51.3605442176871	0.206247586848714 \\
51.7006802721088	0.205247603182707 \\
52.0408163265306	0.205732871364865 \\
52.3809523809524	0.205101053785068 \\
52.7210884353741	0.205540016622689 \\
53.0612244897959	0.205172392070486 \\
53.4013605442177	0.202766111296795 \\
53.7414965986395	0.202122205941834 \\
54.0816326530612	0.200757735555529 \\
54.421768707483	0.201818531947708 \\
54.7619047619048	0.199644080524872 \\
55.1020408163265	0.20118086736366 \\
55.4421768707483	0.200799099991257 \\
55.7823129251701	0.198943077892698 \\
56.1224489795918	0.199672569951083 \\
56.4625850340136	0.19818776265144 \\
56.8027210884354	0.197974067517657 \\
57.1428571428571	0.197139141966289 \\
57.4829931972789	0.195806082106207 \\
57.8231292517007	0.191611971058215 \\
58.1632653061224	0.194210443056401 \\
58.5034013605442	0.19454930284286 \\
58.843537414966	0.193561776732115 \\
59.1836734693878	0.191259653881901 \\
59.5238095238095	0.191561678042785 \\
59.8639455782313	0.190961401506501 \\
60.2040816326531	0.188930467938955 \\
60.5442176870748	0.187285718586117 \\
60.8843537414966	0.185574429058421 \\
61.2244897959184	0.186162300850221 \\
61.5646258503401	0.183939703886733 \\
61.9047619047619	0.185297886283111 \\
62.2448979591837	0.182603020852828 \\
62.5850340136054	0.18180903498515 \\
62.9251700680272	0.180784034909808 \\
63.265306122449	0.179410439796394 \\
63.6054421768707	0.180453196416351 \\
63.9455782312925	0.179403597780247 \\
64.2857142857143	0.177151644707808 \\
64.6258503401361	0.175407547801137 \\
64.9659863945578	0.174749818557872 \\
65.3061224489796	0.175752164269226 \\
65.6462585034014	0.174502622448453 \\
65.9863945578231	0.172290798675845 \\
66.3265306122449	0.173464723464347 \\
66.6666666666667	0.171332747017519 \\
67.0068027210884	0.171242935697088 \\
67.3469387755102	0.169568231641728 \\
67.687074829932	0.168912381146797 \\
68.0272108843537	0.167226061681689 \\
68.3673469387755	0.167167239003991 \\
68.7074829931973	0.164703436033478 \\
69.0476190476191	0.163162866908633 \\
69.3877551020408	0.161357386597589 \\
69.7278911564626	0.161852198110262 \\
70.0680272108844	0.160197591029571 \\
70.4081632653061	0.159470313951352 \\
70.7482993197279	0.158247172358859 \\
71.0884353741497	0.156375767516667 \\
71.4285714285714	0.154614768539718 \\
71.7687074829932	0.154245928458336 \\
72.108843537415	0.1545800050342 \\
72.4489795918367	0.151962514201544 \\
72.7891156462585	0.151270852438891 \\
73.1292517006803	0.150866468703784 \\
73.469387755102	0.150467320789434 \\
73.8095238095238	0.149803100657498 \\
74.1496598639456	0.148402951074292 \\
74.4897959183673	0.146028292545005 \\
74.8299319727891	0.147127741633614 \\
75.1700680272109	0.145872762598799 \\
75.5102040816327	0.145909962829911 \\
75.8503401360544	0.146156191215686 \\
76.1904761904762	0.143952134015648 \\
76.530612244898	0.144185837227293 \\
76.8707482993197	0.142495820495125 \\
77.2108843537415	0.139135853545135 \\
77.5510204081633	0.139181379046836 \\
77.891156462585	0.137176676423151 \\
78.2312925170068	0.134558275405907 \\
78.5714285714286	0.13485098987262 \\
78.9115646258503	0.134373892791803 \\
79.2517006802721	0.133456702357842 \\
79.5918367346939	0.130229067886362 \\
79.9319727891156	0.130874232779126 \\
80.2721088435374	0.129324863630278 \\
80.6122448979592	0.127432015397049 \\
80.9523809523809	0.126186040095911 \\
81.2925170068027	0.125071895723991 \\
81.6326530612245	0.121099864221426 \\
81.9727891156463	0.120583366950581 \\
82.312925170068	0.116681702549151 \\
82.6530612244898	0.11236944052435 \\
82.9931972789116	0.110176228769286 \\
83.3333333333333	0.10820397046709 \\
83.6734693877551	0.106402818292987 \\
84.0136054421769	0.103306889242865 \\
84.3537414965986	0.101971449480856 \\
84.6938775510204	0.0973899560634467 \\
85.0340136054422	0.0964954524655485 \\
85.3741496598639	0.0932731516526127 \\
85.7142857142857	0.0913370299461506 \\
86.0544217687075	0.0906226297503534 \\
86.3945578231292	0.0866405230132108 \\
86.734693877551	0.0829257785342185 \\
87.0748299319728	0.0812805510278229 \\
87.4149659863945	0.0760597816338647 \\
87.7551020408163	0.0728738687693393 \\
88.0952380952381	0.0694535178144292 \\
88.4353741496599	0.0670997457791962 \\
88.7755102040816	0.0645532485790146 \\
89.1156462585034	0.0620046758804533 \\
89.4557823129252	0.0575359203010932 \\
89.7959183673469	0.0534217791095718 \\
90.1360544217687	0.0512165087585755 \\
90.4761904761905	0.0487837431379411 \\
90.8163265306122	0.0465578788635209 \\
91.156462585034	0.0440654612293675 \\
91.4965986394558	0.0392034446144365 \\
91.8367346938775	0.0358899908037412 \\
92.1768707482993	0.0322611047383161 \\
92.5170068027211	0.0288096162052026 \\
92.8571428571429	0.0259361051167806 \\
93.1972789115646	0.0223972104006579 \\
93.5374149659864	0.019991902427052 \\
93.8775510204082	0.0174125375134112 \\
94.2176870748299	0.015486135643616 \\
94.5578231292517	0.0134860942168325 \\
94.8979591836735	0.0113569142898268 \\
95.2380952380952	0.0101589378347765 \\
95.578231292517	0.00940899329136733 \\
95.9183673469388	0.00861739414474353 \\
96.2585034013605	0.00803336223212473 \\
96.5986394557823	0.00682112096129608 \\
96.9387755102041	0.00660491014696158 \\
97.2789115646258	0.00676751475372576 \\
97.6190476190476	0.00584157495175208 \\
97.9591836734694	0.00547393520948956 \\
98.2993197278912	0.00590463093928514 \\
98.6394557823129	0.00486954408997656 \\
98.9795918367347	0.00494979036980584 \\
99.3197278911565	0.00330996255800981 \\
99.6598639455782	0.00206285012714246 \\
100	1.49018575257287e-13 \\
};
\path [fill=color4, fill opacity=0.25]
(axis cs:0,0.720704879878877)
--(axis cs:0,0.717038659335257)
--(axis cs:0.340136054421769,0.717639655439647)
--(axis cs:0.680272108843537,0.714210523873646)
--(axis cs:1.02040816326531,0.701448185813624)
--(axis cs:1.36054421768707,0.676037726942202)
--(axis cs:1.70068027210884,0.647619185106254)
--(axis cs:2.04081632653061,0.620381789784983)
--(axis cs:2.38095238095238,0.589034562360781)
--(axis cs:2.72108843537415,0.545007622872042)
--(axis cs:3.06122448979592,0.501676513447205)
--(axis cs:3.40136054421769,0.466592405540601)
--(axis cs:3.74149659863946,0.43740060803945)
--(axis cs:4.08163265306122,0.410608670658703)
--(axis cs:4.42176870748299,0.384619662206831)
--(axis cs:4.76190476190476,0.358023761296766)
--(axis cs:5.10204081632653,0.336015055627215)
--(axis cs:5.4421768707483,0.319817684838118)
--(axis cs:5.78231292517007,0.302351388006925)
--(axis cs:6.12244897959184,0.285928644801734)
--(axis cs:6.46258503401361,0.269620355650257)
--(axis cs:6.80272108843537,0.25758574318629)
--(axis cs:7.14285714285714,0.247601696271183)
--(axis cs:7.48299319727891,0.235435873120349)
--(axis cs:7.82312925170068,0.226315633462045)
--(axis cs:8.16326530612245,0.218068597403916)
--(axis cs:8.50340136054422,0.213278720242303)
--(axis cs:8.84353741496599,0.206641385326229)
--(axis cs:9.18367346938775,0.205900401396884)
--(axis cs:9.52380952380952,0.19985919068879)
--(axis cs:9.86394557823129,0.194967633985165)
--(axis cs:10.2040816326531,0.1927856841824)
--(axis cs:10.5442176870748,0.192545754495567)
--(axis cs:10.8843537414966,0.190308166828995)
--(axis cs:11.2244897959184,0.187846598713751)
--(axis cs:11.5646258503401,0.18494171876839)
--(axis cs:11.9047619047619,0.185664706881408)
--(axis cs:12.2448979591837,0.184069415304322)
--(axis cs:12.5850340136054,0.183507623457666)
--(axis cs:12.9251700680272,0.183057562525591)
--(axis cs:13.265306122449,0.180042803977011)
--(axis cs:13.6054421768707,0.180085133221454)
--(axis cs:13.9455782312925,0.183218880994914)
--(axis cs:14.2857142857143,0.18354373339944)
--(axis cs:14.6258503401361,0.185007332474334)
--(axis cs:14.9659863945578,0.185356289677586)
--(axis cs:15.3061224489796,0.183421099398451)
--(axis cs:15.6462585034014,0.182459890079852)
--(axis cs:15.9863945578231,0.182792448865622)
--(axis cs:16.3265306122449,0.182240750821487)
--(axis cs:16.6666666666667,0.182745275856646)
--(axis cs:17.0068027210884,0.184494141082882)
--(axis cs:17.3469387755102,0.182849949668085)
--(axis cs:17.687074829932,0.184050632205338)
--(axis cs:18.0272108843537,0.184660031369164)
--(axis cs:18.3673469387755,0.185583963286093)
--(axis cs:18.7074829931973,0.186023583112873)
--(axis cs:19.047619047619,0.184218154999229)
--(axis cs:19.3877551020408,0.18576996972628)
--(axis cs:19.7278911564626,0.185424234703073)
--(axis cs:20.0680272108844,0.186596496711686)
--(axis cs:20.4081632653061,0.185342388879745)
--(axis cs:20.7482993197279,0.183739967946961)
--(axis cs:21.0884353741497,0.18510238167797)
--(axis cs:21.4285714285714,0.185710188101962)
--(axis cs:21.7687074829932,0.184729919971302)
--(axis cs:22.108843537415,0.184089782093524)
--(axis cs:22.4489795918367,0.186880083188427)
--(axis cs:22.7891156462585,0.188303066073278)
--(axis cs:23.1292517006803,0.187593664367252)
--(axis cs:23.469387755102,0.189172143272802)
--(axis cs:23.8095238095238,0.190923345654529)
--(axis cs:24.1496598639456,0.188713621198213)
--(axis cs:24.4897959183673,0.191494727263383)
--(axis cs:24.8299319727891,0.193361689239924)
--(axis cs:25.1700680272109,0.191882785976791)
--(axis cs:25.5102040816327,0.194330069765723)
--(axis cs:25.8503401360544,0.190798694680151)
--(axis cs:26.1904761904762,0.192798755292075)
--(axis cs:26.530612244898,0.192587471923891)
--(axis cs:26.8707482993197,0.193030374033239)
--(axis cs:27.2108843537415,0.19228892312394)
--(axis cs:27.5510204081633,0.19355407887232)
--(axis cs:27.891156462585,0.194515116078789)
--(axis cs:28.2312925170068,0.197243636141403)
--(axis cs:28.5714285714286,0.195532075000157)
--(axis cs:28.9115646258503,0.19629039941245)
--(axis cs:29.2517006802721,0.195834724366814)
--(axis cs:29.5918367346939,0.197191030426128)
--(axis cs:29.9319727891156,0.196386488598612)
--(axis cs:30.2721088435374,0.196717559050709)
--(axis cs:30.6122448979592,0.198787364536353)
--(axis cs:30.952380952381,0.19962117530026)
--(axis cs:31.2925170068027,0.199338474672763)
--(axis cs:31.6326530612245,0.201381965684565)
--(axis cs:31.9727891156463,0.201877949794297)
--(axis cs:32.312925170068,0.202114211196242)
--(axis cs:32.6530612244898,0.202184072416962)
--(axis cs:32.9931972789116,0.203420182981887)
--(axis cs:33.3333333333333,0.202549370348186)
--(axis cs:33.6734693877551,0.201532970204604)
--(axis cs:34.0136054421769,0.203501442859158)
--(axis cs:34.3537414965986,0.203175841889999)
--(axis cs:34.6938775510204,0.203117027173433)
--(axis cs:35.0340136054422,0.203369243726851)
--(axis cs:35.3741496598639,0.203207737887071)
--(axis cs:35.7142857142857,0.202789213927138)
--(axis cs:36.0544217687075,0.202896634481425)
--(axis cs:36.3945578231292,0.201553320527508)
--(axis cs:36.734693877551,0.20396171510575)
--(axis cs:37.0748299319728,0.204228460832218)
--(axis cs:37.4149659863946,0.206128557375772)
--(axis cs:37.7551020408163,0.204192206402403)
--(axis cs:38.0952380952381,0.204066966940944)
--(axis cs:38.4353741496599,0.205022891390552)
--(axis cs:38.7755102040816,0.204958844113678)
--(axis cs:39.1156462585034,0.205063190566028)
--(axis cs:39.4557823129252,0.206594645892594)
--(axis cs:39.7959183673469,0.206634767889214)
--(axis cs:40.1360544217687,0.204789843494329)
--(axis cs:40.4761904761905,0.207377472489363)
--(axis cs:40.8163265306122,0.20691870068109)
--(axis cs:41.156462585034,0.207200303707762)
--(axis cs:41.4965986394558,0.208563122357937)
--(axis cs:41.8367346938776,0.208135517910893)
--(axis cs:42.1768707482993,0.207537436963132)
--(axis cs:42.5170068027211,0.207250890203144)
--(axis cs:42.8571428571429,0.207250856476936)
--(axis cs:43.1972789115646,0.209930579353726)
--(axis cs:43.5374149659864,0.20667181638867)
--(axis cs:43.8775510204082,0.209137209587249)
--(axis cs:44.2176870748299,0.208961871729278)
--(axis cs:44.5578231292517,0.208097983551894)
--(axis cs:44.8979591836735,0.210614345316515)
--(axis cs:45.2380952380952,0.208393392670088)
--(axis cs:45.578231292517,0.204298967182261)
--(axis cs:45.9183673469388,0.209186259247458)
--(axis cs:46.2585034013605,0.207226044101827)
--(axis cs:46.5986394557823,0.206606719456345)
--(axis cs:46.9387755102041,0.206600569417139)
--(axis cs:47.2789115646259,0.205863714224267)
--(axis cs:47.6190476190476,0.204978763622388)
--(axis cs:47.9591836734694,0.205126623855424)
--(axis cs:48.2993197278912,0.204023181473718)
--(axis cs:48.6394557823129,0.203919132148784)
--(axis cs:48.9795918367347,0.203771739606044)
--(axis cs:49.3197278911565,0.204793394334484)
--(axis cs:49.6598639455782,0.203398479056259)
--(axis cs:50,0.203854233774942)
--(axis cs:50.3401360544218,0.202425293896514)
--(axis cs:50.6802721088435,0.2025079625672)
--(axis cs:51.0204081632653,0.201084558046921)
--(axis cs:51.3605442176871,0.199927301676232)
--(axis cs:51.7006802721088,0.199156354604648)
--(axis cs:52.0408163265306,0.199585484217542)
--(axis cs:52.3809523809524,0.199018567377836)
--(axis cs:52.7210884353741,0.199412104358598)
--(axis cs:53.0612244897959,0.198928914975279)
--(axis cs:53.4013605442177,0.19661232512883)
--(axis cs:53.7414965986395,0.196108643839844)
--(axis cs:54.0816326530612,0.194774014146087)
--(axis cs:54.421768707483,0.195494960922011)
--(axis cs:54.7619047619048,0.193594586053579)
--(axis cs:55.1020408163265,0.195112056051425)
--(axis cs:55.4421768707483,0.194723589789907)
--(axis cs:55.7823129251701,0.193030124990588)
--(axis cs:56.1224489795918,0.193664711020694)
--(axis cs:56.4625850340136,0.192218832381842)
--(axis cs:56.8027210884354,0.191957718971315)
--(axis cs:57.1428571428571,0.191177595109061)
--(axis cs:57.4829931972789,0.18975606083558)
--(axis cs:57.8231292517007,0.185792009930193)
--(axis cs:58.1632653061224,0.188330923280089)
--(axis cs:58.5034013605442,0.18869498507941)
--(axis cs:58.843537414966,0.187705120695251)
--(axis cs:59.1836734693878,0.185411389060461)
--(axis cs:59.5238095238095,0.185697501112883)
--(axis cs:59.8639455782313,0.184937668329558)
--(axis cs:60.2040816326531,0.183086428191928)
--(axis cs:60.5442176870748,0.181382273795972)
--(axis cs:60.8843537414966,0.179629894676678)
--(axis cs:61.2244897959184,0.180188038293165)
--(axis cs:61.5646258503401,0.178054736201035)
--(axis cs:61.9047619047619,0.179404330004716)
--(axis cs:62.2448979591837,0.176898878501802)
--(axis cs:62.5850340136054,0.175885518548844)
--(axis cs:62.9251700680272,0.174921183422311)
--(axis cs:63.265306122449,0.173663200419537)
--(axis cs:63.6054421768707,0.174777422277842)
--(axis cs:63.9455782312925,0.173745546195216)
--(axis cs:64.2857142857143,0.171499891386789)
--(axis cs:64.6258503401361,0.169878215132168)
--(axis cs:64.9659863945578,0.169085834451749)
--(axis cs:65.3061224489796,0.169818373392323)
--(axis cs:65.6462585034014,0.168924497888104)
--(axis cs:65.9863945578231,0.166616899031966)
--(axis cs:66.3265306122449,0.167982531778214)
--(axis cs:66.6666666666667,0.165910234116766)
--(axis cs:67.0068027210884,0.165691108053226)
--(axis cs:67.3469387755102,0.164109578459673)
--(axis cs:67.687074829932,0.163335876911426)
--(axis cs:68.0272108843537,0.16194747873663)
--(axis cs:68.3673469387755,0.161878068752529)
--(axis cs:68.7074829931973,0.159399674423081)
--(axis cs:69.0476190476191,0.157941578287034)
--(axis cs:69.3877551020408,0.156295683104172)
--(axis cs:69.7278911564626,0.156704432977608)
--(axis cs:70.0680272108844,0.15516911249429)
--(axis cs:70.4081632653061,0.154591028079559)
--(axis cs:70.7482993197279,0.153403834819369)
--(axis cs:71.0884353741497,0.151701147973981)
--(axis cs:71.4285714285714,0.149779543003981)
--(axis cs:71.7687074829932,0.149479595651463)
--(axis cs:72.108843537415,0.149784219707423)
--(axis cs:72.4489795918367,0.147300252047379)
--(axis cs:72.7891156462585,0.14659651550803)
--(axis cs:73.1292517006803,0.14624289496172)
--(axis cs:73.469387755102,0.14573622226196)
--(axis cs:73.8095238095238,0.145314952194028)
--(axis cs:74.1496598639456,0.143625295062806)
--(axis cs:74.4897959183673,0.14141752375676)
--(axis cs:74.8299319727891,0.142539745019394)
--(axis cs:75.1700680272109,0.141099964294065)
--(axis cs:75.5102040816327,0.141287046154624)
--(axis cs:75.8503401360544,0.141512890696281)
--(axis cs:76.1904761904762,0.139336563953549)
--(axis cs:76.530612244898,0.139542669036027)
--(axis cs:76.8707482993197,0.13810167310478)
--(axis cs:77.2108843537415,0.134507528041671)
--(axis cs:77.5510204081633,0.134465855242649)
--(axis cs:77.891156462585,0.132542617330702)
--(axis cs:78.2312925170068,0.12991814704124)
--(axis cs:78.5714285714286,0.130067869420501)
--(axis cs:78.9115646258503,0.129640422185269)
--(axis cs:79.2517006802721,0.128792219820661)
--(axis cs:79.5918367346939,0.125317109019553)
--(axis cs:79.9319727891156,0.125974781254056)
--(axis cs:80.2721088435374,0.124445287067711)
--(axis cs:80.6122448979592,0.12258277366612)
--(axis cs:80.9523809523809,0.121268989297693)
--(axis cs:81.2925170068027,0.120036667213594)
--(axis cs:81.6326530612245,0.116349188371926)
--(axis cs:81.9727891156463,0.115774076993628)
--(axis cs:82.312925170068,0.111763635170949)
--(axis cs:82.6530612244898,0.10750725641221)
--(axis cs:82.9931972789116,0.105230617329616)
--(axis cs:83.3333333333333,0.10340975334223)
--(axis cs:83.6734693877551,0.101607736225466)
--(axis cs:84.0136054421769,0.0985104703596518)
--(axis cs:84.3537414965986,0.0970500265064678)
--(axis cs:84.6938775510204,0.092554757258062)
--(axis cs:85.0340136054422,0.0917460104787717)
--(axis cs:85.3741496598639,0.0883687108812268)
--(axis cs:85.7142857142857,0.0866303600446924)
--(axis cs:86.0544217687075,0.0858505232297052)
--(axis cs:86.3945578231292,0.0820270576485933)
--(axis cs:86.734693877551,0.0785449290700603)
--(axis cs:87.0748299319728,0.0769075807836092)
--(axis cs:87.4149659863945,0.0719526153237367)
--(axis cs:87.7551020408163,0.0689908849277155)
--(axis cs:88.0952380952381,0.065730376818071)
--(axis cs:88.4353741496599,0.063469704857032)
--(axis cs:88.7755102040816,0.0610593328690857)
--(axis cs:89.1156462585034,0.0584801325355428)
--(axis cs:89.4557823129252,0.0542224697396317)
--(axis cs:89.7959183673469,0.0505108415152917)
--(axis cs:90.1360544217687,0.048295123962886)
--(axis cs:90.4761904761905,0.0460262145961635)
--(axis cs:90.8163265306122,0.043828033673394)
--(axis cs:91.156462585034,0.0414713380897356)
--(axis cs:91.4965986394558,0.0366964858840632)
--(axis cs:91.8367346938775,0.0334900839376949)
--(axis cs:92.1768707482993,0.029782430972274)
--(axis cs:92.5170068027211,0.0266421907502295)
--(axis cs:92.8571428571429,0.0238132808746135)
--(axis cs:93.1972789115646,0.0204082029019106)
--(axis cs:93.5374149659864,0.0181740167300877)
--(axis cs:93.8775510204082,0.0158345916760642)
--(axis cs:94.2176870748299,0.0140625549031482)
--(axis cs:94.5578231292517,0.0122980848294393)
--(axis cs:94.8979591836735,0.0103510445859534)
--(axis cs:95.2380952380952,0.0092951850638625)
--(axis cs:95.578231292517,0.00854423155100626)
--(axis cs:95.9183673469388,0.00766108926953819)
--(axis cs:96.2585034013605,0.00713634575367337)
--(axis cs:96.5986394557823,0.00604134685706174)
--(axis cs:96.9387755102041,0.00579922031280064)
--(axis cs:97.2789115646258,0.00592622265637147)
--(axis cs:97.6190476190476,0.005069294264647)
--(axis cs:97.9591836734694,0.00473387847615131)
--(axis cs:98.2993197278912,0.0052047835894583)
--(axis cs:98.6394557823129,0.00422251822266863)
--(axis cs:98.9795918367347,0.00434579340204675)
--(axis cs:99.3197278911565,0.00288548871490289)
--(axis cs:99.6598639455782,0.00178412849090416)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,0.00234157176338077)
--(axis cs:99.3197278911565,0.00373443640111673)
--(axis cs:98.9795918367347,0.00555378733756492)
--(axis cs:98.6394557823129,0.00551656995728449)
--(axis cs:98.2993197278912,0.00660447828911198)
--(axis cs:97.9591836734694,0.00621399194282781)
--(axis cs:97.6190476190476,0.00661385563885716)
--(axis cs:97.2789115646258,0.00760880685108006)
--(axis cs:96.9387755102041,0.00741059998112251)
--(axis cs:96.5986394557823,0.00760089506553043)
--(axis cs:96.2585034013605,0.0089303787105761)
--(axis cs:95.9183673469388,0.00957369901994886)
--(axis cs:95.578231292517,0.0102737550317284)
--(axis cs:95.2380952380952,0.0110226906056904)
--(axis cs:94.8979591836735,0.0123627839937001)
--(axis cs:94.5578231292517,0.0146741036042257)
--(axis cs:94.2176870748299,0.0169097163840837)
--(axis cs:93.8775510204082,0.0189904833507581)
--(axis cs:93.5374149659864,0.0218097881240163)
--(axis cs:93.1972789115646,0.0243862178994053)
--(axis cs:92.8571428571429,0.0280589293589477)
--(axis cs:92.5170068027211,0.0309770416601757)
--(axis cs:92.1768707482993,0.0347397785043582)
--(axis cs:91.8367346938775,0.0382898976697874)
--(axis cs:91.4965986394558,0.0417104033448098)
--(axis cs:91.156462585034,0.0466595843689994)
--(axis cs:90.8163265306122,0.0492877240536478)
--(axis cs:90.4761904761905,0.0515412716797187)
--(axis cs:90.1360544217687,0.054137893554265)
--(axis cs:89.7959183673469,0.0563327167038519)
--(axis cs:89.4557823129252,0.0608493708625546)
--(axis cs:89.1156462585034,0.0655292192253638)
--(axis cs:88.7755102040816,0.0680471642889435)
--(axis cs:88.4353741496599,0.0707297867013604)
--(axis cs:88.0952380952381,0.0731766588107875)
--(axis cs:87.7551020408163,0.076756852610963)
--(axis cs:87.4149659863945,0.0801669479439927)
--(axis cs:87.0748299319728,0.0856535212720366)
--(axis cs:86.734693877551,0.0873066279983768)
--(axis cs:86.3945578231292,0.0912539883778284)
--(axis cs:86.0544217687075,0.0953947362710016)
--(axis cs:85.7142857142857,0.0960436998476087)
--(axis cs:85.3741496598639,0.0981775924239986)
--(axis cs:85.0340136054422,0.101244894452325)
--(axis cs:84.6938775510204,0.102225154868831)
--(axis cs:84.3537414965986,0.106892872455243)
--(axis cs:84.0136054421769,0.108103308126078)
--(axis cs:83.6734693877551,0.111197900360507)
--(axis cs:83.3333333333333,0.11299818759195)
--(axis cs:82.9931972789116,0.115121840208955)
--(axis cs:82.6530612244898,0.117231624636491)
--(axis cs:82.312925170068,0.121599769927353)
--(axis cs:81.9727891156463,0.125392656907535)
--(axis cs:81.6326530612245,0.125850540070925)
--(axis cs:81.2925170068027,0.130107124234389)
--(axis cs:80.9523809523809,0.131103090894129)
--(axis cs:80.6122448979592,0.132281257127979)
--(axis cs:80.2721088435374,0.134204440192844)
--(axis cs:79.9319727891156,0.135773684304197)
--(axis cs:79.5918367346939,0.135141026753172)
--(axis cs:79.2517006802721,0.138121184895022)
--(axis cs:78.9115646258503,0.139107363398338)
--(axis cs:78.5714285714286,0.139634110324739)
--(axis cs:78.2312925170068,0.139198403770574)
--(axis cs:77.891156462585,0.1418107355156)
--(axis cs:77.5510204081633,0.143896902851024)
--(axis cs:77.2108843537415,0.143764179048599)
--(axis cs:76.8707482993197,0.146889967885469)
--(axis cs:76.530612244898,0.14882900541856)
--(axis cs:76.1904761904762,0.148567704077748)
--(axis cs:75.8503401360544,0.15079949173509)
--(axis cs:75.5102040816327,0.150532879505197)
--(axis cs:75.1700680272109,0.150645560903533)
--(axis cs:74.8299319727891,0.151715738247833)
--(axis cs:74.4897959183673,0.150639061333249)
--(axis cs:74.1496598639456,0.153180607085779)
--(axis cs:73.8095238095238,0.154291249120969)
--(axis cs:73.469387755102,0.155198419316909)
--(axis cs:73.1292517006803,0.155490042445848)
--(axis cs:72.7891156462585,0.155945189369752)
--(axis cs:72.4489795918367,0.156624776355709)
--(axis cs:72.108843537415,0.159375790360977)
--(axis cs:71.7687074829932,0.159012261265209)
--(axis cs:71.4285714285714,0.159449994075455)
--(axis cs:71.0884353741497,0.161050387059353)
--(axis cs:70.7482993197279,0.163090509898349)
--(axis cs:70.4081632653061,0.164349599823145)
--(axis cs:70.0680272108844,0.165226069564852)
--(axis cs:69.7278911564626,0.166999963242915)
--(axis cs:69.3877551020408,0.166419090091006)
--(axis cs:69.0476190476191,0.168384155530231)
--(axis cs:68.7074829931973,0.170007197643876)
--(axis cs:68.3673469387755,0.172456409255454)
--(axis cs:68.0272108843537,0.172504644626749)
--(axis cs:67.687074829932,0.174488885382168)
--(axis cs:67.3469387755102,0.175026884823784)
--(axis cs:67.0068027210884,0.17679476334095)
--(axis cs:66.6666666666667,0.176755259918273)
--(axis cs:66.3265306122449,0.17894691515048)
--(axis cs:65.9863945578231,0.177964698319724)
--(axis cs:65.6462585034014,0.180080747008802)
--(axis cs:65.3061224489796,0.181685955146129)
--(axis cs:64.9659863945578,0.180413802663994)
--(axis cs:64.6258503401361,0.180936880470106)
--(axis cs:64.2857142857143,0.182803398028827)
--(axis cs:63.9455782312925,0.185061649365277)
--(axis cs:63.6054421768707,0.18612897055486)
--(axis cs:63.265306122449,0.185157679173251)
--(axis cs:62.9251700680272,0.186646886397304)
--(axis cs:62.5850340136054,0.187732551421457)
--(axis cs:62.2448979591837,0.188307163203853)
--(axis cs:61.9047619047619,0.191191442561506)
--(axis cs:61.5646258503401,0.189824671572431)
--(axis cs:61.2244897959184,0.192136563407277)
--(axis cs:60.8843537414966,0.191518963440165)
--(axis cs:60.5442176870748,0.193189163376261)
--(axis cs:60.2040816326531,0.194774507685982)
--(axis cs:59.8639455782313,0.196985134683445)
--(axis cs:59.5238095238095,0.197425854972687)
--(axis cs:59.1836734693878,0.19710791870334)
--(axis cs:58.843537414966,0.19941843276898)
--(axis cs:58.5034013605442,0.20040362060631)
--(axis cs:58.1632653061224,0.200089962832714)
--(axis cs:57.8231292517007,0.197431932186238)
--(axis cs:57.4829931972789,0.201856103376833)
--(axis cs:57.1428571428571,0.203100688823517)
--(axis cs:56.8027210884354,0.203990416063998)
--(axis cs:56.4625850340136,0.204156692921038)
--(axis cs:56.1224489795918,0.205680428881473)
--(axis cs:55.7823129251701,0.204856030794808)
--(axis cs:55.4421768707483,0.206874610192608)
--(axis cs:55.1020408163265,0.207249678675895)
--(axis cs:54.7619047619048,0.205693574996166)
--(axis cs:54.421768707483,0.208142102973405)
--(axis cs:54.0816326530612,0.206741456964972)
--(axis cs:53.7414965986395,0.208135768043825)
--(axis cs:53.4013605442177,0.208919897464759)
--(axis cs:53.0612244897959,0.211415869165693)
--(axis cs:52.7210884353741,0.21166792888678)
--(axis cs:52.3809523809524,0.2111835401923)
--(axis cs:52.0408163265306,0.211880258512188)
--(axis cs:51.7006802721088,0.211338851760765)
--(axis cs:51.3605442176871,0.212567872021195)
--(axis cs:51.0204081632653,0.213692765280203)
--(axis cs:50.6802721088435,0.214685071239426)
--(axis cs:50.3401360544218,0.214700554328406)
--(axis cs:50,0.216066574303482)
--(axis cs:49.6598639455782,0.216108988660005)
--(axis cs:49.3197278911565,0.217034705321793)
--(axis cs:48.9795918367347,0.216303650931535)
--(axis cs:48.6394557823129,0.216301018502106)
--(axis cs:48.2993197278912,0.216564265439375)
--(axis cs:47.9591836734694,0.217658158428229)
--(axis cs:47.6190476190476,0.216941027271427)
--(axis cs:47.2789115646259,0.218123090225267)
--(axis cs:46.9387755102041,0.218993020978778)
--(axis cs:46.5986394557823,0.21911015227912)
--(axis cs:46.2585034013605,0.219643027176952)
--(axis cs:45.9183673469388,0.221492816904608)
--(axis cs:45.578231292517,0.216948428740637)
--(axis cs:45.2380952380952,0.220709085273049)
--(axis cs:44.8979591836735,0.22299271441433)
--(axis cs:44.5578231292517,0.220748797711552)
--(axis cs:44.2176870748299,0.221471279813144)
--(axis cs:43.8775510204082,0.221883386613004)
--(axis cs:43.5374149659864,0.219905182236385)
--(axis cs:43.1972789115646,0.222752938454266)
--(axis cs:42.8571428571429,0.219997274787424)
--(axis cs:42.5170068027211,0.220298967317072)
--(axis cs:42.1768707482993,0.22062969316851)
--(axis cs:41.8367346938776,0.221393141536983)
--(axis cs:41.4965986394558,0.221822123677354)
--(axis cs:41.156462585034,0.220303543517261)
--(axis cs:40.8163265306122,0.220209945371449)
--(axis cs:40.4761904761905,0.220268308761863)
--(axis cs:40.1360544217687,0.217989076295052)
--(axis cs:39.7959183673469,0.220227457046256)
--(axis cs:39.4557823129252,0.219888890191305)
--(axis cs:39.1156462585034,0.218161668974043)
--(axis cs:38.7755102040816,0.217953796687711)
--(axis cs:38.4353741496599,0.218412958367063)
--(axis cs:38.0952380952381,0.217582540079199)
--(axis cs:37.7551020408163,0.217745532560418)
--(axis cs:37.4149659863946,0.219775552959059)
--(axis cs:37.0748299319728,0.217855941127203)
--(axis cs:36.734693877551,0.217537921606784)
--(axis cs:36.3945578231292,0.215296526425928)
--(axis cs:36.0544217687075,0.216441973125785)
--(axis cs:35.7142857142857,0.215946332237269)
--(axis cs:35.3741496598639,0.217078269450918)
--(axis cs:35.0340136054422,0.216926726811668)
--(axis cs:34.6938775510204,0.21676044834733)
--(axis cs:34.3537414965986,0.21705772407657)
--(axis cs:34.0136054421769,0.217037748130821)
--(axis cs:33.6734693877551,0.215139146104864)
--(axis cs:33.3333333333333,0.216267969035043)
--(axis cs:32.9931972789116,0.216789218643276)
--(axis cs:32.6530612244898,0.215962921691498)
--(axis cs:32.312925170068,0.216054619439751)
--(axis cs:31.9727891156463,0.215656047380769)
--(axis cs:31.6326530612245,0.215301276385906)
--(axis cs:31.2925170068027,0.213503928269569)
--(axis cs:30.952380952381,0.213698582458924)
--(axis cs:30.6122448979592,0.21260831028963)
--(axis cs:30.2721088435374,0.210834173135617)
--(axis cs:29.9319727891156,0.210256147449947)
--(axis cs:29.5918367346939,0.210983743071367)
--(axis cs:29.2517006802721,0.210171581275377)
--(axis cs:28.9115646258503,0.210293109809084)
--(axis cs:28.5714285714286,0.209923302861161)
--(axis cs:28.2312925170068,0.21142743404105)
--(axis cs:27.891156462585,0.208654753471197)
--(axis cs:27.5510204081633,0.207783713158337)
--(axis cs:27.2108843537415,0.206152339704997)
--(axis cs:26.8707482993197,0.207237949536384)
--(axis cs:26.530612244898,0.206555431184468)
--(axis cs:26.1904761904762,0.207289086928589)
--(axis cs:25.8503401360544,0.205305887397878)
--(axis cs:25.5102040816327,0.208697281281882)
--(axis cs:25.1700680272109,0.206005403384292)
--(axis cs:24.8299319727891,0.207458763388815)
--(axis cs:24.4897959183673,0.205844313662213)
--(axis cs:24.1496598639456,0.202688990126047)
--(axis cs:23.8095238095238,0.204795150803221)
--(axis cs:23.469387755102,0.203147635770428)
--(axis cs:23.1292517006803,0.201086529269937)
--(axis cs:22.7891156462585,0.201727463251771)
--(axis cs:22.4489795918367,0.200552336832093)
--(axis cs:22.108843537415,0.197748035250229)
--(axis cs:21.7687074829932,0.198245606349571)
--(axis cs:21.4285714285714,0.199230092867324)
--(axis cs:21.0884353741497,0.198555864177978)
--(axis cs:20.7482993197279,0.197140236048862)
--(axis cs:20.4081632653061,0.198683908533695)
--(axis cs:20.0680272108844,0.199845619467106)
--(axis cs:19.7278911564626,0.198690331259454)
--(axis cs:19.3877551020408,0.199509045358709)
--(axis cs:19.047619047619,0.197429815858078)
--(axis cs:18.7074829931973,0.199303584088203)
--(axis cs:18.3673469387755,0.198903387650119)
--(axis cs:18.0272108843537,0.197723017586432)
--(axis cs:17.687074829932,0.197109983701771)
--(axis cs:17.3469387755102,0.195933303892029)
--(axis cs:17.0068027210884,0.197443159774302)
--(axis cs:16.6666666666667,0.195715963120142)
--(axis cs:16.3265306122449,0.195419365871168)
--(axis cs:15.9863945578231,0.196044976153565)
--(axis cs:15.6462585034014,0.195771215358928)
--(axis cs:15.3061224489796,0.196795414693462)
--(axis cs:14.9659863945578,0.198585972288883)
--(axis cs:14.6258503401361,0.198510205291035)
--(axis cs:14.2857142857143,0.196873950139603)
--(axis cs:13.9455782312925,0.196713127685612)
--(axis cs:13.6054421768707,0.19341998929866)
--(axis cs:13.265306122449,0.193409503696311)
--(axis cs:12.9251700680272,0.196027688066487)
--(axis cs:12.5850340136054,0.197268636246453)
--(axis cs:12.2448979591837,0.197653925487732)
--(axis cs:11.9047619047619,0.199046466487432)
--(axis cs:11.5646258503401,0.19833360021729)
--(axis cs:11.2244897959184,0.201348223481539)
--(axis cs:10.8843537414966,0.204185582567895)
--(axis cs:10.5442176870748,0.206446010025088)
--(axis cs:10.2040816326531,0.206540063078435)
--(axis cs:9.86394557823129,0.208805058362969)
--(axis cs:9.52380952380952,0.213821590106184)
--(axis cs:9.18367346938775,0.219760363260282)
--(axis cs:8.84353741496599,0.22058268603778)
--(axis cs:8.50340136054422,0.227196895417135)
--(axis cs:8.16326530612245,0.232037766758921)
--(axis cs:7.82312925170068,0.240508332071623)
--(axis cs:7.48299319727891,0.249680429454106)
--(axis cs:7.14285714285714,0.261560879470439)
--(axis cs:6.80272108843537,0.27215962395692)
--(axis cs:6.46258503401361,0.284084291546727)
--(axis cs:6.12244897959184,0.300157600235208)
--(axis cs:5.78231292517007,0.316756227226761)
--(axis cs:5.4421768707483,0.333784948930833)
--(axis cs:5.10204081632653,0.350054828197623)
--(axis cs:4.76190476190476,0.371681958384654)
--(axis cs:4.42176870748299,0.397734266514155)
--(axis cs:4.08163265306122,0.423101968387336)
--(axis cs:3.74149659863946,0.449872795827698)
--(axis cs:3.40136054421769,0.478587365774705)
--(axis cs:3.06122448979592,0.514308039074054)
--(axis cs:2.72108843537415,0.558041671927525)
--(axis cs:2.38095238095238,0.600239206935924)
--(axis cs:2.04081632653061,0.629716021139071)
--(axis cs:1.70068027210884,0.655730055539512)
--(axis cs:1.36054421768707,0.682897846307853)
--(axis cs:1.02040816326531,0.706448342728418)
--(axis cs:0.680272108843537,0.718302085190933)
--(axis cs:0.340136054421769,0.721348260672299)
--(axis cs:0,0.720704879878877)
--cycle;


==> img/stl10/stl10_rate_distortion_lcg_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color8, mark=oplus*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color8, thin}]
table {%
0 0.718423196673393
0.340136054421769 0.711282981038094
0.680272108843537 0.691814600229263
1.02040816326531 0.651927649378777
1.36054421768707 0.597822504304349
1.70068027210884 0.539818885754794
2.04081632653061 0.487806377451634
2.38095238095238 0.441796071074277
2.72108843537415 0.404166484984586
3.06122448979592 0.366508140932464
3.40136054421769 0.333901684695151
3.74149659863946 0.306611155617608
4.08163265306122 0.277331097946877
4.42176870748299 0.248561734521039
4.76190476190476 0.223916248170928
5.10204081632653 0.202937509391387
5.4421768707483 0.183078848252542
5.78231292517007 0.166851402999753
6.12244897959184 0.150552343354119
6.46258503401361 0.137974104064249
6.80272108843537 0.126703350671645
7.14285714285714 0.118526687775712
7.48299319727891 0.10861305350079
7.82312925170068 0.100264901552747
8.16326530612245 0.0953854708612012
8.50340136054422 0.0909430433232957
8.84353741496599 0.0878289877450625
9.18367346938775 0.083780769663419
9.52380952380952 0.0823678809520458
9.86394557823129 0.0752819899069481
10.2040816326531 0.0750342985376755
10.5442176870748 0.0730268029818339
10.8843537414966 0.069043904366634
11.2244897959184 0.0680502384163947
11.5646258503401 0.0652181463675449
11.9047619047619 0.0628258260309977
12.2448979591837 0.0626449403642367
12.5850340136054 0.0598891146870039
12.9251700680272 0.0591923456193867
13.265306122449 0.0596035531308095
13.6054421768707 0.0598822944026778
13.9455782312925 0.0568986669955758
14.2857142857143 0.0571951144436922
14.6258503401361 0.0548489738487454
14.9659863945578 0.0558396479418084
15.3061224489796 0.0556101096866316
15.6462585034014 0.0540908148120642
15.9863945578231 0.0533344061595333
16.3265306122449 0.0552279728415309
16.6666666666667 0.0552101853000276
17.0068027210884 0.0556046957384971
17.3469387755102 0.0560887746548318
17.687074829932 0.0559505711286631
18.0272108843537 0.0553244518327513
18.3673469387755 0.0570030122388327
18.7074829931973 0.0580927678367809
19.047619047619 0.0592106955338696
19.3877551020408 0.0590099866310207
19.7278911564626 0.0612961661169924
20.0680272108844 0.06149942123146
20.4081632653061 0.0618327977792309
20.7482993197279 0.0624761616623402
21.0884353741497 0.0631757636290722
21.4285714285714 0.0641614706659279
21.7687074829932 0.0647021840787567
22.108843537415 0.0676401605341223
22.4489795918367 0.0654608529657838
22.7891156462585 0.0665291469980923
23.1292517006803 0.0663399881793663
23.469387755102 0.0658981348332053
23.8095238095238 0.0667147399359824
24.1496598639456 0.0700309099899456
24.4897959183673 0.0697801574738759
24.8299319727891 0.0702401704377228
25.1700680272109 0.0701209231709251
25.5102040816327 0.0699261801746179
25.8503401360544 0.0694129514885765
26.1904761904762 0.0701744509767157
26.530612244898 0.0709151525847932
26.8707482993197 0.0719656800999731
27.2108843537415 0.0736325952946646
27.5510204081633 0.0722451274379399
27.891156462585 0.0737438009250719
28.2312925170068 0.075142883304735
28.5714285714286 0.0759128063209693
28.9115646258503 0.0774979945278507
29.2517006802721 0.0772415796125551
29.5918367346939 0.0767630817819137
29.9319727891156 0.0775872439361157
30.2721088435374 0.0788817291901569
30.6122448979592 0.0778839181843307
30.952380952381 0.0806490527770815
31.2925170068027 0.0804879135668386
31.6326530612245 0.0805788185738959
31.9727891156463 0.0815778718454866
32.312925170068 0.0817480090088346
32.6530612244898 0.08258616144781
32.9931972789116 0.0815074644960066
33.3333333333333 0.0817910458124641
33.6734693877551 0.0819071596572818
34.0136054421769 0.0814218021910097
34.3537414965986 0.0826808290750794
34.6938775510204 0.0836067891878234
35.0340136054422 0.082152388283155
35.3741496598639 0.0820855592437381
35.7142857142857 0.0821724390326516
36.0544217687075 0.0815154040306786
36.3945578231292 0.0836194765526574
36.734693877551 0.0830625647516845
37.0748299319728 0.0838585590100265
37.4149659863946 0.0838458160943272
37.7551020408163 0.0845059966094766
38.0952380952381 0.085088058719734
38.4353741496599 0.0857763822338202
38.7755102040816 0.0868691979614259
39.1156462585034 0.0883927445355502
39.4557823129252 0.089123440005227
39.7959183673469 0.090213558999235
40.1360544217687 0.091144885658286
40.4761904761905 0.0935875979975906
40.8163265306122 0.093972030525387
41.156462585034 0.0934159252195829
41.4965986394558 0.0924648375940564
41.8367346938776 0.0935180263086471
42.1768707482993 0.0956147998912452
42.5170068027211 0.0961488759361243
42.8571428571429 0.0945686130494914
43.1972789115646 0.0926873437392614
43.5374149659864 0.0924673175180745
43.8775510204082 0.0908503532562483
44.2176870748299 0.0921145153665932
44.5578231292517 0.0922348816956583
44.8979591836735 0.0911463561712529
45.2380952380952 0.0906883690632751
45.578231292517 0.0911446658258035
45.9183673469388 0.0927129875828251
46.2585034013605 0.0919075771798055
46.5986394557823 0.092839160535624
46.9387755102041 0.0917445685223973
47.2789115646259 0.0919274229108183
47.6190476190476 0.0937317765034514
47.9591836734694 0.0944609202212047
48.2993197278912 0.0945293751551294
48.6394557823129 0.095853357737588
48.9795918367347 0.095168445593865
49.3197278911565 0.0931958316075809
49.6598639455782 0.0938234896158752
50 0.0935392527689444
50.3401360544218 0.0910079819984397
50.6802721088435 0.0909673674373332
51.0204081632653 0.0902436271726402
51.3605442176871 0.0894218590506785
51.7006802721088 0.0892054824963941
52.0408163265306 0.0888350605083928
52.3809523809524 0.0881231981582964
52.7210884353741 0.0879319384777919
53.0612244897959 0.089147972025457
53.4013605442177 0.0871222070180502
53.7414965986395 0.0881521893487963
54.0816326530612 0.0882252827843518
54.421768707483 0.090488921538682
54.7619047619048 0.0887656263165557
55.1020408163265 0.0884261015149516
55.4421768707483 0.0884312508011516
55.7823129251701 0.0881201912982959
56.1224489795918 0.0874764922358545
56.4625850340136 0.08631347644451
56.8027210884354 0.0842585640026969
57.1428571428571 0.0824635560735084
57.4829931972789 0.0812393822326728
57.8231292517007 0.0816377814663421
58.1632653061224 0.0815165922938957
58.5034013605442 0.0797078266332144
58.843537414966 0.0786132334906496
59.1836734693878 0.0780719688170203
59.5238095238095 0.0769814727309157
59.8639455782313 0.0759755711744483
60.2040816326531 0.0762325590797894
60.5442176870748 0.0753103091096902
60.8843537414966 0.0733607604565482
61.2244897959184 0.0720375187028638
61.5646258503401 0.0726783396880746
61.9047619047619 0.0716702874105273
62.2448979591837 0.0704173903202157
62.5850340136054 0.0687067744849931
62.9251700680272 0.0676476044237056
63.265306122449 0.0669325232788809
63.6054421768707 0.067820492730268
63.9455782312925 0.0657805727606109
64.2857142857143 0.0657035819184629
64.6258503401361 0.0650869924614133
64.9659863945578 0.0656092108779275
65.3061224489796 0.0638875786176773
65.6462585034014 0.0637206630898117
65.9863945578231 0.0618428662842459
66.3265306122449 0.0624967128389197
66.6666666666667 0.0621631959585855
67.0068027210884 0.0613815657961149
67.3469387755102 0.0596941288384315
67.687074829932 0.0597183537110224
68.0272108843537 0.060224491163
68.3673469387755 0.059469275907475
68.7074829931973 0.0598681733588079
69.0476190476191 0.0590061883922672
69.3877551020408 0.0584599243502905
69.7278911564626 0.0589833333604001
70.0680272108844 0.0605551210665977
70.4081632653061 0.0613947048417964
70.7482993197279 0.0591972150164167
71.0884353741497 0.0584786643448934
71.4285714285714 0.0596363462022925
71.7687074829932 0.0588113757082908
72.108843537415 0.0588833471013482
72.4489795918367 0.0584124644886018
72.7891156462585 0.0570551680284782
73.1292517006803 0.0575764226727164
73.469387755102 0.057717330371327
73.8095238095238 0.0577528714746096
74.1496598639456 0.0567774051516304
74.4897959183673 0.0556000100352933
74.8299319727891 0.0553865783495642
75.1700680272109 0.0547308648882607
75.5102040816327 0.0548827126570967
75.8503401360544 0.0550884426208581
76.1904761904762 0.0544378985977236
76.530612244898 0.0542191335803912
76.8707482993197 0.0535053640400397
77.2108843537415 0.0548963415391585
77.5510204081633 0.0545740827850965
77.891156462585 0.0534509143033271
78.2312925170068 0.052889952853184
78.5714285714286 0.0526262293062277
78.9115646258503 0.0511918729900309
79.2517006802721 0.0492730392424887
79.5918367346939 0.0489218419284392
79.9319727891156 0.0481807885200117
80.2721088435374 0.0478830762025757
80.6122448979592 0.0474544854546642
80.9523809523809 0.0458920953138605
81.2925170068027 0.0435099658299439
81.6326530612245 0.0427187510713864
81.9727891156463 0.0405836565949598
82.312925170068 0.0385510447722989
82.6530612244898 0.0363612707666251
82.9931972789116 0.035599668847282
83.3333333333333 0.0340600312942948
83.6734693877551 0.0330029485443844
84.0136054421769 0.0310393103271291
84.3537414965986 0.0297416497029229
84.6938775510204 0.0284333260446377
85.0340136054422 0.0277377352907692
85.3741496598639 0.0261020249360923
85.7142857142857 0.0252587713595733
86.0544217687075 0.0239302394923504
86.3945578231292 0.0229986699420646
86.734693877551 0.0220487376555179
87.0748299319728 0.0214775423499235
87.4149659863945 0.0200388793457818
87.7551020408163 0.019540431763317
88.0952380952381 0.019036138699973
88.4353741496599 0.0178112605053949
88.7755102040816 0.0165706561690117
89.1156462585034 0.0151341277603196
89.4557823129252 0.0144534516852335
89.7959183673469 0.0140534308670061
90.1360544217687 0.0133831738296939
90.4761904761905 0.0131585431060354
90.8163265306122 0.0121451762357427
91.156462585034 0.0114651684118947
91.4965986394558 0.0107545599040515
91.8367346938775 0.0103567209863529
92.1768707482993 0.00996639287759203
92.5170068027211 0.00908591023170114
92.8571428571429 0.00912100649562437
93.1972789115646 0.00834910994236559
93.5374149659864 0.00807092248597949
93.8775510204082 0.00763749940600774
94.2176870748299 0.00746262236758807
94.5578231292517 0.00697898226158684
94.8979591836735 0.00628395977601837
95.2380952380952 0.0060012387285145
95.578231292517 0.00531462428654277
95.9183673469388 0.00505889039339935
96.2585034013605 0.00450371632114833
96.5986394557823 0.00400804018511761
96.9387755102041 0.00358788857761786
97.2789115646258 0.00308858291413197
97.6190476190476 0.00272775304819966
97.9591836734694 0.00244595932837921
98.2993197278912 0.00188055384139257
98.6394557823129 0.00133834601365699
98.9795918367347 0.00100208191340839
99.3197278911565 0.000435599709026406
99.6598639455782 0.000206147311844773
100 1.46300749293005e-13
};
\path [fill=color8, fill opacity=0.25]
(axis cs:0,0.720290873122061)
--(axis cs:0,0.716555520224726)
--(axis cs:0.340136054421769,0.709163160637751)
--(axis cs:0.680272108843537,0.688911596674134)
--(axis cs:1.02040816326531,0.647761269429104)
--(axis cs:1.36054421768707,0.592585416775663)
--(axis cs:1.70068027210884,0.534167861276753)
--(axis cs:2.04081632653061,0.482396419013123)
--(axis cs:2.38095238095238,0.436101675371102)
--(axis cs:2.72108843537415,0.398591658241975)
--(axis cs:3.06122448979592,0.3611051178924)
--(axis cs:3.40136054421769,0.328424631507928)
--(axis cs:3.74149659863946,0.30092734649379)
--(axis cs:4.08163265306122,0.271493226942843)
--(axis cs:4.42176870748299,0.24240009665911)
--(axis cs:4.76190476190476,0.217853146725742)
--(axis cs:5.10204081632653,0.196975236553138)
--(axis cs:5.4421768707483,0.177390573616179)
--(axis cs:5.78231292517007,0.161209010910361)
--(axis cs:6.12244897959184,0.145081691188258)
--(axis cs:6.46258503401361,0.132600183750637)
--(axis cs:6.80272108843537,0.121567955369177)
--(axis cs:7.14285714285714,0.113425269903232)
--(axis cs:7.48299319727891,0.103789942470039)
--(axis cs:7.82312925170068,0.0955498582857099)
--(axis cs:8.16326530612245,0.0906274257051706)
--(axis cs:8.50340136054422,0.0862774730085239)
--(axis cs:8.84353741496599,0.0833124220630259)
--(axis cs:9.18367346938775,0.0792301831120177)
--(axis cs:9.52380952380952,0.0776451170744739)
--(axis cs:9.86394557823129,0.0709457126272215)
--(axis cs:10.2040816326531,0.0705898070085951)
--(axis cs:10.5442176870748,0.0684800953527836)
--(axis cs:10.8843537414966,0.0646979286719824)
--(axis cs:11.2244897959184,0.063890466485617)
--(axis cs:11.5646258503401,0.0610640170073178)
--(axis cs:11.9047619047619,0.0585515125127662)
--(axis cs:12.2448979591837,0.0584647419214381)
--(axis cs:12.5850340136054,0.0559250660300151)
--(axis cs:12.9251700680272,0.0552304075514117)
--(axis cs:13.265306122449,0.0557002178383497)
--(axis cs:13.6054421768707,0.0559662762407411)
--(axis cs:13.9455782312925,0.0529571879012045)
--(axis cs:14.2857142857143,0.0532822299813583)
--(axis cs:14.6258503401361,0.051082136316254)
--(axis cs:14.9659863945578,0.0518754929485548)
--(axis cs:15.3061224489796,0.0515182483188299)
--(axis cs:15.6462585034014,0.0501362421961226)
--(axis cs:15.9863945578231,0.049565803343536)
--(axis cs:16.3265306122449,0.0511272741363807)
--(axis cs:16.6666666666667,0.0513044884439638)
--(axis cs:17.0068027210884,0.0517302937643663)
--(axis cs:17.3469387755102,0.0521700624716856)
--(axis cs:17.687074829932,0.0520278719670454)
--(axis cs:18.0272108843537,0.0515679160868376)
--(axis cs:18.3673469387755,0.0531522589422069)
--(axis cs:18.7074829931973,0.0542323387133302)
--(axis cs:19.047619047619,0.0554530068411323)
--(axis cs:19.3877551020408,0.0552914200387568)
--(axis cs:19.7278911564626,0.0576931277818204)
--(axis cs:20.0680272108844,0.0579342961091504)
--(axis cs:20.4081632653061,0.0581982646318408)
--(axis cs:20.7482993197279,0.0590817597940763)
--(axis cs:21.0884353741497,0.0596506681168138)
--(axis cs:21.4285714285714,0.0606140790767762)
--(axis cs:21.7687074829932,0.061176032203199)
--(axis cs:22.108843537415,0.0642437036042549)
--(axis cs:22.4489795918367,0.062267897463108)
--(axis cs:22.7891156462585,0.0631948025228467)
--(axis cs:23.1292517006803,0.0633452892524517)
--(axis cs:23.469387755102,0.0626946005283489)
--(axis cs:23.8095238095238,0.0635905599057419)
--(axis cs:24.1496598639456,0.0668764598971411)
--(axis cs:24.4897959183673,0.0665642769518221)
--(axis cs:24.8299319727891,0.0670726267336562)
--(axis cs:25.1700680272109,0.0669677122423437)
--(axis cs:25.5102040816327,0.066694043640757)
--(axis cs:25.8503401360544,0.0664657294615576)
--(axis cs:26.1904761904762,0.0671281909774864)
--(axis cs:26.530612244898,0.0676564200369505)
--(axis cs:26.8707482993197,0.0687603294126887)
--(axis cs:27.2108843537415,0.0707070206858571)
--(axis cs:27.5510204081633,0.0689885246482073)
--(axis cs:27.891156462585,0.0706713135845165)
--(axis cs:28.2312925170068,0.0721147626716534)
--(axis cs:28.5714285714286,0.0729151071676134)
--(axis cs:28.9115646258503,0.074532060364895)
--(axis cs:29.2517006802721,0.0741754579282657)
--(axis cs:29.5918367346939,0.0736101489378123)
--(axis cs:29.9319727891156,0.0744863138376907)
--(axis cs:30.2721088435374,0.0756970852202838)
--(axis cs:30.6122448979592,0.0745178922254596)
--(axis cs:30.952380952381,0.0771405488170212)
--(axis cs:31.2925170068027,0.0771519532941558)
--(axis cs:31.6326530612245,0.0770714634409367)
--(axis cs:31.9727891156463,0.0777392268478869)
--(axis cs:32.312925170068,0.0779279187593482)
--(axis cs:32.6530612244898,0.0788519621514598)
--(axis cs:32.9931972789116,0.0775687303430535)
--(axis cs:33.3333333333333,0.0777984383321853)
--(axis cs:33.6734693877551,0.0778898287639116)
--(axis cs:34.0136054421769,0.0771995462310381)
--(axis cs:34.3537414965986,0.0786462609780752)
--(axis cs:34.6938775510204,0.0794271184569288)
--(axis cs:35.0340136054422,0.0780280466121225)
--(axis cs:35.3741496598639,0.0779356796812134)
--(axis cs:35.7142857142857,0.077856784527597)
--(axis cs:36.0544217687075,0.0773061224047551)
--(axis cs:36.3945578231292,0.079221096807336)
--(axis cs:36.734693877551,0.0785935896127512)
--(axis cs:37.0748299319728,0.0794245992321299)
--(axis cs:37.4149659863946,0.0794712771867571)
--(axis cs:37.7551020408163,0.0802151607688922)
--(axis cs:38.0952380952381,0.0806246822077254)
--(axis cs:38.4353741496599,0.0814270328975289)
--(axis cs:38.7755102040816,0.0823771775086788)
--(axis cs:39.1156462585034,0.0840004125905004)
--(axis cs:39.4557823129252,0.0846183750348277)
--(axis cs:39.7959183673469,0.0857690646166834)
--(axis cs:40.1360544217687,0.0864631397197189)
--(axis cs:40.4761904761905,0.0888466586064038)
--(axis cs:40.8163265306122,0.0890930084819195)
--(axis cs:41.156462585034,0.0887790733151865)
--(axis cs:41.4965986394558,0.0878167489636435)
--(axis cs:41.8367346938776,0.0887998276481747)
--(axis cs:42.1768707482993,0.0907007813889098)
--(axis cs:42.5170068027211,0.0912544650641877)
--(axis cs:42.8571428571429,0.0898068285566033)
--(axis cs:43.1972789115646,0.0880964750152467)
--(axis cs:43.5374149659864,0.087891234841582)
--(axis cs:43.8775510204082,0.0863069765313335)
--(axis cs:44.2176870748299,0.0876584762806664)
--(axis cs:44.5578231292517,0.0879356246442246)
--(axis cs:44.8979591836735,0.0866861930751087)
--(axis cs:45.2380952380952,0.0862550749334875)
--(axis cs:45.578231292517,0.0867895480748516)
--(axis cs:45.9183673469388,0.0883876389698014)
--(axis cs:46.2585034013605,0.0876503919265129)
--(axis cs:46.5986394557823,0.0884982904360073)
--(axis cs:46.9387755102041,0.0872633768546832)
--(axis cs:47.2789115646259,0.0875126656109386)
--(axis cs:47.6190476190476,0.0894919384864489)
--(axis cs:47.9591836734694,0.090079573381177)
--(axis cs:48.2993197278912,0.0902321585012687)
--(axis cs:48.6394557823129,0.0914108172716147)
--(axis cs:48.9795918367347,0.0907837456428348)
--(axis cs:49.3197278911565,0.0890918679820104)
--(axis cs:49.6598639455782,0.0896175261174361)
--(axis cs:50,0.0893742076886822)
--(axis cs:50.3401360544218,0.0867742166768058)
--(axis cs:50.6802721088435,0.0867998778492342)
--(axis cs:51.0204081632653,0.0860327715884896)
--(axis cs:51.3605442176871,0.0853590484149722)
--(axis cs:51.7006802721088,0.0852676020485613)
--(axis cs:52.0408163265306,0.0847948106093366)
--(axis cs:52.3809523809524,0.0841659101695165)
--(axis cs:52.7210884353741,0.0839273187787239)
--(axis cs:53.0612244897959,0.0851116129856453)
--(axis cs:53.4013605442177,0.0831459324610837)
--(axis cs:53.7414965986395,0.0842701496572493)
--(axis cs:54.0816326530612,0.0842714119086789)
--(axis cs:54.421768707483,0.0866243497963706)
--(axis cs:54.7619047619048,0.0848090792264233)
--(axis cs:55.1020408163265,0.0843292893525301)
--(axis cs:55.4421768707483,0.0844672860107615)
--(axis cs:55.7823129251701,0.0842517746237134)
--(axis cs:56.1224489795918,0.0835217248382173)
--(axis cs:56.4625850340136,0.0823425525698671)
--(axis cs:56.8027210884354,0.0801997425060744)
--(axis cs:57.1428571428571,0.0784982244141229)
--(axis cs:57.4829931972789,0.0773415238866905)
--(axis cs:57.8231292517007,0.0778175863876002)
--(axis cs:58.1632653061224,0.077468830076517)
--(axis cs:58.5034013605442,0.0761116094344404)
--(axis cs:58.843537414966,0.0748955792601535)
--(axis cs:59.1836734693878,0.0742236649250483)
--(axis cs:59.5238095238095,0.0732755557109488)
--(axis cs:59.8639455782313,0.0721225996640151)
--(axis cs:60.2040816326531,0.0723903329793189)
--(axis cs:60.5442176870748,0.0715200290467863)
--(axis cs:60.8843537414966,0.0697040450648548)
--(axis cs:61.2244897959184,0.0685176862681771)
--(axis cs:61.5646258503401,0.0689710283907865)
--(axis cs:61.9047619047619,0.0679920444969829)
--(axis cs:62.2448979591837,0.0668703629113097)
--(axis cs:62.5850340136054,0.0652976212587963)
--(axis cs:62.9251700680272,0.0643249514330921)
--(axis cs:63.265306122449,0.0636801208812332)
--(axis cs:63.6054421768707,0.0644185921198994)
--(axis cs:63.9455782312925,0.06262744307496)
--(axis cs:64.2857142857143,0.0625397473328012)
--(axis cs:64.6258503401361,0.0619517449476646)
--(axis cs:64.9659863945578,0.0623816634027978)
--(axis cs:65.3061224489796,0.060697040837127)
--(axis cs:65.6462585034014,0.0606548499589025)
--(axis cs:65.9863945578231,0.0591102239618237)
--(axis cs:66.3265306122449,0.0597377810410441)
--(axis cs:66.6666666666667,0.0594294110817492)
--(axis cs:67.0068027210884,0.0587575096055775)
--(axis cs:67.3469387755102,0.0571530141601506)
--(axis cs:67.687074829932,0.0572562246690757)
--(axis cs:68.0272108843537,0.0576339917028348)
--(axis cs:68.3673469387755,0.056907657446528)
--(axis cs:68.7074829931973,0.0572888080875007)
--(axis cs:69.0476190476191,0.0565994731107543)
--(axis cs:69.3877551020408,0.0559901802316799)
--(axis cs:69.7278911564626,0.0564520928107958)
--(axis cs:70.0680272108844,0.0577958450095499)
--(axis cs:70.4081632653061,0.058511717518169)
--(axis cs:70.7482993197279,0.0564456396963443)
--(axis cs:71.0884353741497,0.0558512283355998)
--(axis cs:71.4285714285714,0.0567928663261565)
--(axis cs:71.7687074829932,0.0559654869045707)
--(axis cs:72.108843537415,0.0561408906190178)
--(axis cs:72.4489795918367,0.0555126386379202)
--(axis cs:72.7891156462585,0.0543730884176872)
--(axis cs:73.1292517006803,0.0548507100314196)
--(axis cs:73.469387755102,0.0550113372302205)
--(axis cs:73.8095238095238,0.0552299762875978)
--(axis cs:74.1496598639456,0.0543516817983771)
--(axis cs:74.4897959183673,0.0531961193283028)
--(axis cs:74.8299319727891,0.0528883300032885)
--(axis cs:75.1700680272109,0.0521983818154654)
--(axis cs:75.5102040816327,0.0525753297727598)
--(axis cs:75.8503401360544,0.052488944040516)
--(axis cs:76.1904761904762,0.0519906891461479)
--(axis cs:76.530612244898,0.0517638721490972)
--(axis cs:76.8707482993197,0.0510904019606772)
--(axis cs:77.2108843537415,0.0524607241430204)
--(axis cs:77.5510204081633,0.052252170845203)
--(axis cs:77.891156462585,0.0512232198781002)
--(axis cs:78.2312925170068,0.050574444205027)
--(axis cs:78.5714285714286,0.0502377388189992)
--(axis cs:78.9115646258503,0.0487882597964888)
--(axis cs:79.2517006802721,0.0470719628014276)
--(axis cs:79.5918367346939,0.0467326556581157)
--(axis cs:79.9319727891156,0.0459108141346981)
--(axis cs:80.2721088435374,0.0455625474062237)
--(axis cs:80.6122448979592,0.0452546531832107)
--(axis cs:80.9523809523809,0.0436550005595977)
--(axis cs:81.2925170068027,0.0414559424885445)
--(axis cs:81.6326530612245,0.0407270286657384)
--(axis cs:81.9727891156463,0.0384919456880647)
--(axis cs:82.312925170068,0.0367159973057483)
--(axis cs:82.6530612244898,0.0345304254031461)
--(axis cs:82.9931972789116,0.0339819159749094)
--(axis cs:83.3333333333333,0.0323832258023453)
--(axis cs:83.6734693877551,0.0312384358482799)
--(axis cs:84.0136054421769,0.0293657255735484)
--(axis cs:84.3537414965986,0.0280058632166278)
--(axis cs:84.6938775510204,0.0268655531337757)
--(axis cs:85.0340136054422,0.0260757591897282)
--(axis cs:85.3741496598639,0.0243718218987869)
--(axis cs:85.7142857142857,0.0237140701096381)
--(axis cs:86.0544217687075,0.0222928229078367)
--(axis cs:86.3945578231292,0.0214292617661001)
--(axis cs:86.734693877551,0.0203224857639259)
--(axis cs:87.0748299319728,0.0200055504401751)
--(axis cs:87.4149659863945,0.0185238238043224)
--(axis cs:87.7551020408163,0.0180722025628117)
--(axis cs:88.0952380952381,0.0176090682761799)
--(axis cs:88.4353741496599,0.0164569428515476)
--(axis cs:88.7755102040816,0.0152756000855398)
--(axis cs:89.1156462585034,0.0139251230000556)
--(axis cs:89.4557823129252,0.0132864584144998)
--(axis cs:89.7959183673469,0.0129360717009288)
--(axis cs:90.1360544217687,0.0122547267219067)
--(axis cs:90.4761904761905,0.0120599326517767)
--(axis cs:90.8163265306122,0.0111024367892136)
--(axis cs:91.156462585034,0.0104624271863065)
--(axis cs:91.4965986394558,0.009798201400728)
--(axis cs:91.8367346938775,0.00940254938897125)
--(axis cs:92.1768707482993,0.00908790025880263)
--(axis cs:92.5170068027211,0.00822450651211927)
--(axis cs:92.8571428571429,0.00825922839227445)
--(axis cs:93.1972789115646,0.00747746829138221)
--(axis cs:93.5374149659864,0.00719289046580127)
--(axis cs:93.8775510204082,0.00681960881982437)
--(axis cs:94.2176870748299,0.00657811305389813)
--(axis cs:94.5578231292517,0.00607899489607658)
--(axis cs:94.8979591836735,0.00555137496982338)
--(axis cs:95.2380952380952,0.00517656827761099)
--(axis cs:95.578231292517,0.0045617266452784)
--(axis cs:95.9183673469388,0.00430402833083283)
--(axis cs:96.2585034013605,0.00374733655756494)
--(axis cs:96.5986394557823,0.00337255731649823)
--(axis cs:96.9387755102041,0.00294782670919026)
--(axis cs:97.2789115646258,0.00252970429373619)
--(axis cs:97.6190476190476,0.00216776796114661)
--(axis cs:97.9591836734694,0.00196810380850122)
--(axis cs:98.2993197278912,0.00150348114632873)
--(axis cs:98.6394557823129,0.00103988262966481)
--(axis cs:98.9795918367347,0.000810943267135708)
--(axis cs:99.3197278911565,0.000335966011205824)
--(axis cs:99.6598639455782,0.000127559220242654)
--(axis cs:100,1.46300749293005e-13)
--(axis cs:100,1.46300749293005e-13)
--(axis cs:100,1.46300749293005e-13)
--(axis cs:99.6598639455782,0.000284735403446893)
--(axis cs:99.3197278911565,0.000535233406846989)
--(axis cs:98.9795918367347,0.00119322055968108)
--(axis cs:98.6394557823129,0.00163680939764916)
--(axis cs:98.2993197278912,0.0022576265364564)
--(axis cs:97.9591836734694,0.00292381484825721)
--(axis cs:97.6190476190476,0.00328773813525272)
--(axis cs:97.2789115646258,0.00364746153452774)
--(axis cs:96.9387755102041,0.00422795044604546)
--(axis cs:96.5986394557823,0.00464352305373699)
--(axis cs:96.2585034013605,0.00526009608473172)
--(axis cs:95.9183673469388,0.00581375245596586)
--(axis cs:95.578231292517,0.00606752192780714)
--(axis cs:95.2380952380952,0.00682590917941801)
--(axis cs:94.8979591836735,0.00701654458221336)
--(axis cs:94.5578231292517,0.00787896962709711)
--(axis cs:94.2176870748299,0.00834713168127801)
--(axis cs:93.8775510204082,0.0084553899921911)
--(axis cs:93.5374149659864,0.00894895450615771)
--(axis cs:93.1972789115646,0.00922075159334897)
--(axis cs:92.8571428571429,0.00998278459897429)
--(axis cs:92.5170068027211,0.00994731395128301)
--(axis cs:92.1768707482993,0.0108448854963814)
--(axis cs:91.8367346938775,0.0113108925837346)
--(axis cs:91.4965986394558,0.011710918407375)
--(axis cs:91.156462585034,0.012467909637483)
--(axis cs:90.8163265306122,0.0131879156822718)
--(axis cs:90.4761904761905,0.014257153560294)
--(axis cs:90.1360544217687,0.0145116209374811)
--(axis cs:89.7959183673469,0.0151707900330833)
--(axis cs:89.4557823129252,0.0156204449559671)
--(axis cs:89.1156462585034,0.0163431325205837)
--(axis cs:88.7755102040816,0.0178657122524836)
--(axis cs:88.4353741496599,0.0191655781592423)
--(axis cs:88.0952380952381,0.0204632091237661)
--(axis cs:87.7551020408163,0.0210086609638224)
--(axis cs:87.4149659863945,0.0215539348872412)
--(axis cs:87.0748299319728,0.0229495342596719)
--(axis cs:86.734693877551,0.0237749895471099)
--(axis cs:86.3945578231292,0.0245680781180291)
--(axis cs:86.0544217687075,0.0255676560768642)
--(axis cs:85.7142857142857,0.0268034726095084)
--(axis cs:85.3741496598639,0.0278322279733976)
--(axis cs:85.0340136054422,0.0293997113918102)
--(axis cs:84.6938775510204,0.0300010989554998)
--(axis cs:84.3537414965986,0.031477436189218)
--(axis cs:84.0136054421769,0.0327128950807097)
--(axis cs:83.6734693877551,0.0347674612404889)
--(axis cs:83.3333333333333,0.0357368367862443)
--(axis cs:82.9931972789116,0.0372174217196546)
--(axis cs:82.6530612244898,0.0381921161301041)
--(axis cs:82.312925170068,0.0403860922388496)
--(axis cs:81.9727891156463,0.0426753675018549)
--(axis cs:81.6326530612245,0.0447104734770343)
--(axis cs:81.2925170068027,0.0455639891713433)
--(axis cs:80.9523809523809,0.0481291900681232)
--(axis cs:80.6122448979592,0.0496543177261177)
--(axis cs:80.2721088435374,0.0502036049989278)
--(axis cs:79.9319727891156,0.0504507629053253)
--(axis cs:79.5918367346939,0.0511110281987627)
--(axis cs:79.2517006802721,0.0514741156835499)
--(axis cs:78.9115646258503,0.0535954861835729)
--(axis cs:78.5714285714286,0.0550147197934562)
--(axis cs:78.2312925170068,0.055205461501341)
--(axis cs:77.891156462585,0.0556786087285541)
--(axis cs:77.5510204081633,0.05689599472499)
--(axis cs:77.2108843537415,0.0573319589352967)
--(axis cs:76.8707482993197,0.0559203261194022)
--(axis cs:76.530612244898,0.0566743950116852)
--(axis cs:76.1904761904762,0.0568851080492994)
--(axis cs:75.8503401360544,0.0576879412012003)
--(axis cs:75.5102040816327,0.0571900955414336)
--(axis cs:75.1700680272109,0.057263347961056)
--(axis cs:74.8299319727891,0.0578848266958398)
--(axis cs:74.4897959183673,0.0580039007422839)
--(axis cs:74.1496598639456,0.0592031285048838)
--(axis cs:73.8095238095238,0.0602757666616214)
--(axis cs:73.469387755102,0.0604233235124334)
--(axis cs:73.1292517006803,0.0603021353140133)
--(axis cs:72.7891156462585,0.0597372476392691)
--(axis cs:72.4489795918367,0.0613122903392833)
--(axis cs:72.108843537415,0.0616258035836787)
--(axis cs:71.7687074829932,0.061657264512011)
--(axis cs:71.4285714285714,0.0624798260784285)
--(axis cs:71.0884353741497,0.061106100354187)
--(axis cs:70.7482993197279,0.0619487903364891)
--(axis cs:70.4081632653061,0.0642776921654238)
--(axis cs:70.0680272108844,0.0633143971236456)
--(axis cs:69.7278911564626,0.0615145739100045)
--(axis cs:69.3877551020408,0.0609296684689011)
--(axis cs:69.0476190476191,0.0614129036737802)
--(axis cs:68.7074829931973,0.062447538630115)
--(axis cs:68.3673469387755,0.062030894368422)
--(axis cs:68.0272108843537,0.0628149906231652)
--(axis cs:67.687074829932,0.0621804827529692)
--(axis cs:67.3469387755102,0.0622352435167125)
--(axis cs:67.0068027210884,0.0640056219866523)
--(axis cs:66.6666666666667,0.0648969808354219)
--(axis cs:66.3265306122449,0.0652556446367953)
--(axis cs:65.9863945578231,0.064575508606668)
--(axis cs:65.6462585034014,0.0667864762207209)
--(axis cs:65.3061224489796,0.0670781163982275)
--(axis cs:64.9659863945578,0.0688367583530572)
--(axis cs:64.6258503401361,0.0682222399751619)
--(axis cs:64.2857142857143,0.0688674165041246)
--(axis cs:63.9455782312925,0.0689337024462618)
--(axis cs:63.6054421768707,0.0712223933406365)
--(axis cs:63.265306122449,0.0701849256765286)
--(axis cs:62.9251700680272,0.070970257414319)
--(axis cs:62.5850340136054,0.07211592771119)
--(axis cs:62.2448979591837,0.0739644177291217)
--(axis cs:61.9047619047619,0.0753485303240717)
--(axis cs:61.5646258503401,0.0763856509853627)
--(axis cs:61.2244897959184,0.0755573511375506)
--(axis cs:60.8843537414966,0.0770174758482416)
--(axis cs:60.5442176870748,0.0791005891725941)
--(axis cs:60.2040816326531,0.0800747851802599)
--(axis cs:59.8639455782313,0.0798285426848816)
--(axis cs:59.5238095238095,0.0806873897508827)
--(axis cs:59.1836734693878,0.0819202727089923)
--(axis cs:58.843537414966,0.0823308877211457)
--(axis cs:58.5034013605442,0.0833040438319884)
--(axis cs:58.1632653061224,0.0855643545112744)
--(axis cs:57.8231292517007,0.085457976545084)
--(axis cs:57.4829931972789,0.085137240578655)
--(axis cs:57.1428571428571,0.0864288877328938)
--(axis cs:56.8027210884354,0.0883173854993193)
--(axis cs:56.4625850340136,0.0902844003191529)
--(axis cs:56.1224489795918,0.0914312596334918)
--(axis cs:55.7823129251701,0.0919886079728783)
--(axis cs:55.4421768707483,0.0923952155915417)
--(axis cs:55.1020408163265,0.0925229136773732)
--(axis cs:54.7619047619048,0.0927221734066882)
--(axis cs:54.421768707483,0.0943534932809935)
--(axis cs:54.0816326530612,0.0921791536600247)
--(axis cs:53.7414965986395,0.0920342290403434)
--(axis cs:53.4013605442177,0.0910984815750168)
--(axis cs:53.0612244897959,0.0931843310652688)
--(axis cs:52.7210884353741,0.0919365581768599)
--(axis cs:52.3809523809524,0.0920804861470763)
--(axis cs:52.0408163265306,0.0928753104074489)
--(axis cs:51.7006802721088,0.0931433629442269)
--(axis cs:51.3605442176871,0.0934846696863848)
--(axis cs:51.0204081632653,0.0944544827567907)
--(axis cs:50.6802721088435,0.0951348570254321)
--(axis cs:50.3401360544218,0.0952417473200735)
--(axis cs:50,0.0977042978492067)
--(axis cs:49.6598639455782,0.0980294531143144)
--(axis cs:49.3197278911565,0.0972997952331513)
--(axis cs:48.9795918367347,0.0995531455448952)
--(axis cs:48.6394557823129,0.100295898203561)
--(axis cs:48.2993197278912,0.0988265918089901)
--(axis cs:47.9591836734694,0.0988422670612324)
--(axis cs:47.6190476190476,0.0979716145204539)
--(axis cs:47.2789115646259,0.096342180210698)
--(axis cs:46.9387755102041,0.0962257601901114)
--(axis cs:46.5986394557823,0.0971800306352406)
--(axis cs:46.2585034013605,0.096164762433098)
--(axis cs:45.9183673469388,0.0970383361958489)
--(axis cs:45.578231292517,0.0954997835767553)
--(axis cs:45.2380952380952,0.0951216631930627)
--(axis cs:44.8979591836735,0.095606519267397)
--(axis cs:44.5578231292517,0.0965341387470919)
--(axis cs:44.2176870748299,0.0965705544525201)
--(axis cs:43.8775510204082,0.0953937299811631)
--(axis cs:43.5374149659864,0.097043400194567)
--(axis cs:43.1972789115646,0.097278212463276)
--(axis cs:42.8571428571429,0.0993303975423796)
--(axis cs:42.5170068027211,0.101043286808061)
--(axis cs:42.1768707482993,0.100528818393581)
--(axis cs:41.8367346938776,0.0982362249691195)
--(axis cs:41.4965986394558,0.0971129262244693)
--(axis cs:41.156462585034,0.0980527771239793)
--(axis cs:40.8163265306122,0.0988510525688545)
--(axis cs:40.4761904761905,0.0983285373887775)
--(axis cs:40.1360544217687,0.0958266315968531)
--(axis cs:39.7959183673469,0.0946580533817866)
--(axis cs:39.4557823129252,0.0936285049756263)
--(axis cs:39.1156462585034,0.0927850764806)
--(axis cs:38.7755102040816,0.091361218414173)
--(axis cs:38.4353741496599,0.0901257315701116)
--(axis cs:38.0952380952381,0.0895514352317427)
--(axis cs:37.7551020408163,0.088796832450061)
--(axis cs:37.4149659863946,0.0882203550018973)
--(axis cs:37.0748299319728,0.0882925187879232)
--(axis cs:36.734693877551,0.0875315398906178)
--(axis cs:36.3945578231292,0.0880178562979788)
--(axis cs:36.0544217687075,0.0857246856566021)
--(axis cs:35.7142857142857,0.0864880935377062)
--(axis cs:35.3741496598639,0.0862354388062628)
--(axis cs:35.0340136054422,0.0862767299541874)
--(axis cs:34.6938775510204,0.087786459918718)
--(axis cs:34.3537414965986,0.0867153971720837)
--(axis cs:34.0136054421769,0.0856440581509812)
--(axis cs:33.6734693877551,0.0859244905506519)
--(axis cs:33.3333333333333,0.0857836532927429)
--(axis cs:32.9931972789116,0.0854461986489598)
--(axis cs:32.6530612244898,0.0863203607441602)
--(axis cs:32.312925170068,0.085568099258321)
--(axis cs:31.9727891156463,0.0854165168430864)
--(axis cs:31.6326530612245,0.0840861737068551)
--(axis cs:31.2925170068027,0.0838238738395214)
--(axis cs:30.952380952381,0.0841575567371419)
--(axis cs:30.6122448979592,0.0812499441432018)
--(axis cs:30.2721088435374,0.0820663731600301)
--(axis cs:29.9319727891156,0.0806881740345407)
--(axis cs:29.5918367346939,0.0799160146260152)
--(axis cs:29.2517006802721,0.0803077012968444)
--(axis cs:28.9115646258503,0.0804639286908063)
--(axis cs:28.5714285714286,0.0789105054743251)
--(axis cs:28.2312925170068,0.0781710039378166)
--(axis cs:27.891156462585,0.0768162882656274)
--(axis cs:27.5510204081633,0.0755017302276725)
--(axis cs:27.2108843537415,0.076558169903472)
--(axis cs:26.8707482993197,0.0751710307872575)
--(axis cs:26.530612244898,0.0741738851326359)
--(axis cs:26.1904761904762,0.073220710975945)
--(axis cs:25.8503401360544,0.0723601735155955)
--(axis cs:25.5102040816327,0.0731583167084788)
--(axis cs:25.1700680272109,0.0732741340995065)
--(axis cs:24.8299319727891,0.0734077141417895)
--(axis cs:24.4897959183673,0.0729960379959297)
--(axis cs:24.1496598639456,0.0731853600827502)
--(axis cs:23.8095238095238,0.0698389199662229)
--(axis cs:23.469387755102,0.0691016691380618)
--(axis cs:23.1292517006803,0.0693346871062809)
--(axis cs:22.7891156462585,0.069863491473338)
--(axis cs:22.4489795918367,0.0686538084684596)
--(axis cs:22.108843537415,0.0710366174639896)
--(axis cs:21.7687074829932,0.0682283359543143)
--(axis cs:21.4285714285714,0.0677088622550797)
--(axis cs:21.0884353741497,0.0667008591413307)
--(axis cs:20.7482993197279,0.0658705635306042)
--(axis cs:20.4081632653061,0.065467330926621)
--(axis cs:20.0680272108844,0.0650645463537696)
--(axis cs:19.7278911564626,0.0648992044521644)
--(axis cs:19.3877551020408,0.0627285532232846)
--(axis cs:19.047619047619,0.0629683842266069)
--(axis cs:18.7074829931973,0.0619531969602316)
--(axis cs:18.3673469387755,0.0608537655354585)
--(axis cs:18.0272108843537,0.059080987578665)
--(axis cs:17.687074829932,0.0598732702902808)
--(axis cs:17.3469387755102,0.0600074868379781)
--(axis cs:17.0068027210884,0.0594790977126279)
--(axis cs:16.6666666666667,0.0591158821560913)
--(axis cs:16.3265306122449,0.0593286715466812)
--(axis cs:15.9863945578231,0.0571030089755306)
--(axis cs:15.6462585034014,0.0580453874280057)
--(axis cs:15.3061224489796,0.0597019710544333)
--(axis cs:14.9659863945578,0.0598038029350621)
--(axis cs:14.6258503401361,0.0586158113812368)
--(axis cs:14.2857142857143,0.0611079989060261)
--(axis cs:13.9455782312925,0.0608401460899471)
--(axis cs:13.6054421768707,0.0637983125646146)
--(axis cs:13.265306122449,0.0635068884232693)
--(axis cs:12.9251700680272,0.0631542836873617)
--(axis cs:12.5850340136054,0.0638531633439927)
--(axis cs:12.2448979591837,0.0668251388070353)
--(axis cs:11.9047619047619,0.0671001395492293)
--(axis cs:11.5646258503401,0.0693722757277719)
--(axis cs:11.2244897959184,0.0722100103471723)
--(axis cs:10.8843537414966,0.0733898800612856)
--(axis cs:10.5442176870748,0.0775735106108842)
--(axis cs:10.2040816326531,0.079478790066756)
--(axis cs:9.86394557823129,0.0796182671866747)
--(axis cs:9.52380952380952,0.0870906448296177)
--(axis cs:9.18367346938775,0.0883313562148204)
--(axis cs:8.84353741496599,0.092345553427099)
--(axis cs:8.50340136054422,0.0956086136380674)
--(axis cs:8.16326530612245,0.100143516017232)
--(axis cs:7.82312925170068,0.104979944819784)
--(axis cs:7.48299319727891,0.11343616453154)
--(axis cs:7.14285714285714,0.123628105648191)
--(axis cs:6.80272108843537,0.131838745974113)
--(axis cs:6.46258503401361,0.14334802437786)
--(axis cs:6.12244897959184,0.15602299551998)
--(axis cs:5.78231292517007,0.172493795089146)
--(axis cs:5.4421768707483,0.188767122888905)
--(axis cs:5.10204081632653,0.208899782229636)
--(axis cs:4.76190476190476,0.229979349616114)
--(axis cs:4.42176870748299,0.254723372382968)
--(axis cs:4.08163265306122,0.283168968950911)
--(axis cs:3.74149659863946,0.312294964741425)
--(axis cs:3.40136054421769,0.339378737882373)
--(axis cs:3.06122448979592,0.371911163972528)
--(axis cs:2.72108843537415,0.409741311727196)
--(axis cs:2.38095238095238,0.447490466777452)
--(axis cs:2.04081632653061,0.493216335890145)
--(axis cs:1.70068027210884,0.545469910232835)
--(axis cs:1.36054421768707,0.603059591833035)
--(axis cs:1.02040816326531,0.65609402932845)
--(axis cs:0.680272108843537,0.694717603784393)
--(axis cs:0.340136054421769,0.713402801438436)
--(axis cs:0,0.720290873122061)
--cycle;


==> img/stl10/stl10_rate_distortion_lime.tex <==
% lime
\addplot [line width=0.5, opacity=0.8, color3, mark=diamond, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color3, thin}]
table [row sep=\\]{%
0	0.718766905963421 \\
0.340136054421769	0.719279825687408 \\
0.680272108843537	0.719054994285107 \\
1.02040816326531	0.719696340709925 \\
1.36054421768707	0.720801150798798 \\
1.70068027210884	0.719882019460201 \\
2.04081632653061	0.719227051138878 \\
2.38095238095238	0.721684906482697 \\
2.72108843537415	0.721767579317093 \\
3.06122448979592	0.719566322267056 \\
3.40136054421769	0.721828900575638 \\
3.74149659863946	0.720498013794422 \\
4.08163265306122	0.7190960252285 \\
4.42176870748299	0.716560619771481 \\
4.76190476190476	0.712873773872852 \\
5.10204081632653	0.711100943684578 \\
5.4421768707483	0.708536891937256 \\
5.78231292517007	0.707640231847763 \\
6.12244897959184	0.70704089730978 \\
6.46258503401361	0.706936928033829 \\
6.80272108843537	0.708689357042313 \\
7.14285714285714	0.706616966575384 \\
7.48299319727891	0.704294118881226 \\
7.82312925170068	0.693521218597889 \\
8.16326530612245	0.686528349518776 \\
8.50340136054422	0.681956080496311 \\
8.84353741496599	0.681016996204853 \\
9.18367346938775	0.677157157361507 \\
9.52380952380952	0.673107976615429 \\
9.86394557823129	0.669560510069132 \\
10.2040816326531	0.671066290140152 \\
10.5442176870748	0.671618112623692 \\
10.8843537414966	0.673285162746906 \\
11.2244897959184	0.667619900852442 \\
11.5646258503401	0.662521747350693 \\
11.9047619047619	0.658827974945307 \\
12.2448979591837	0.656783409565687 \\
12.5850340136054	0.651662666797638 \\
12.9251700680272	0.649301793575287 \\
13.265306122449	0.648591429591179 \\
13.6054421768707	0.645840649455786 \\
13.9455782312925	0.642577523142099 \\
14.2857142857143	0.637907748054713 \\
14.6258503401361	0.637374363616109 \\
14.9659863945578	0.636021920349449 \\
15.3061224489796	0.636433494202793 \\
15.6462585034014	0.62865327399224 \\
15.9863945578231	0.624190028831363 \\
16.3265306122449	0.621327185966075 \\
16.6666666666667	0.619676921721548 \\
17.0068027210884	0.607133836140856 \\
17.3469387755102	0.604488716190681 \\
17.687074829932	0.599910825099796 \\
18.0272108843537	0.598196739051491 \\
18.3673469387755	0.596328085614368 \\
18.7074829931973	0.587132567754015 \\
19.047619047619	0.58296027559787 \\
19.3877551020408	0.580949590033852 \\
19.7278911564626	0.577698293752037 \\
20.0680272108844	0.572714173896238 \\
20.4081632653061	0.567030665995553 \\
20.7482993197279	0.564303674846888 \\
21.0884353741497	0.563433628850617 \\
21.4285714285714	0.561713891904801 \\
21.7687074829932	0.557089810119942 \\
22.108843537415	0.553946159342304 \\
22.4489795918367	0.549810659531504 \\
22.7891156462585	0.548413011068478 \\
23.1292517006803	0.544420191366225 \\
23.469387755102	0.539619502881542 \\
23.8095238095238	0.534323109742254 \\
24.1496598639456	0.531078150910325 \\
24.4897959183673	0.521313174823299 \\
24.8299319727891	0.519619817612693 \\
25.1700680272109	0.517317020678893 \\
25.5102040816327	0.511089385147206 \\
25.8503401360544	0.513561960179359 \\
26.1904761904762	0.514649803069187 \\
26.530612244898	0.511425703024724 \\
26.8707482993197	0.510091383737745 \\
27.2108843537415	0.509503029626794 \\
27.5510204081633	0.509222693505581 \\
27.891156462585	0.505497542591765 \\
28.2312925170068	0.504347718622303 \\
28.5714285714286	0.502232480715029 \\
28.9115646258503	0.497846050842782 \\
29.2517006802721	0.4989822980389 \\
29.5918367346939	0.494185275160708 \\
29.9319727891156	0.494074035027297 \\
30.2721088435374	0.489268324940931 \\
30.6122448979592	0.486131021381589 \\
30.952380952381	0.480210300879553 \\
31.2925170068027	0.476398428889224 \\
31.6326530612245	0.474350926552433 \\
31.9727891156463	0.474700465073111 \\
32.312925170068	0.473683851483511 \\
32.6530612244898	0.47169523271441 \\
32.9931972789116	0.472663679048419 \\
33.3333333333333	0.470511640496843 \\
33.6734693877551	0.470530102690973 \\
34.0136054421769	0.467642966882267 \\
34.3537414965986	0.467758005578944 \\
34.6938775510204	0.465493011916697 \\
35.0340136054422	0.44944372332131 \\
35.3741496598639	0.447062889345689 \\
35.7142857142857	0.449148618920299 \\
36.0544217687075	0.446630763359717 \\
36.3945578231292	0.445005756374449 \\
36.734693877551	0.444814300968719 \\
37.0748299319728	0.442133684424916 \\
37.4149659863946	0.440244526537135 \\
37.7551020408163	0.439926825107541 \\
38.0952380952381	0.435342044933786 \\
38.4353741496599	0.432242688957194 \\
38.7755102040816	0.431105741824285 \\
39.1156462585034	0.429391851861437 \\
39.4557823129252	0.426307205805206 \\
39.7959183673469	0.425694020210503 \\
40.1360544217687	0.423975173806684 \\
40.4761904761905	0.420724264756136 \\
40.8163265306122	0.416569568184932 \\
41.156462585034	0.415011430253799 \\
41.4965986394558	0.414535583631732 \\
41.8367346938776	0.418981894778044 \\
42.1768707482993	0.418285832426336 \\
42.5170068027211	0.416812546875226 \\
42.8571428571429	0.41319245192637 \\
43.1972789115646	0.406728432354503 \\
43.5374149659864	0.404888649632339 \\
43.8775510204082	0.403297451817671 \\
44.2176870748299	0.401085718456015 \\
44.5578231292517	0.398713685148723 \\
44.8979591836735	0.394991091049596 \\
45.2380952380952	0.389211920707166 \\
45.578231292517	0.389419896028849 \\
45.9183673469388	0.385311902187823 \\
46.2585034013605	0.378901692040818 \\
46.5986394557823	0.37680839450084 \\
46.9387755102041	0.374423633427323 \\
47.2789115646259	0.371963301126743 \\
47.6190476190476	0.369641070243579 \\
47.9591836734694	0.368279079499443 \\
48.2993197278912	0.367585430431936 \\
48.6394557823129	0.362300970404358 \\
48.9795918367347	0.356044829497769 \\
49.3197278911565	0.355452820768223 \\
49.6598639455782	0.354889359391418 \\
50	0.352368318263143 \\
50.3401360544218	0.352543284716303 \\
50.6802721088435	0.351884388047729 \\
51.0204081632653	0.350288340625484 \\
51.3605442176871	0.346428295685437 \\
51.7006802721088	0.344521448071646 \\
52.0408163265306	0.341268048213533 \\
52.3809523809524	0.338950429044926 \\
52.7210884353741	0.336852741644616 \\
53.0612244897959	0.335716731234825 \\
53.4013605442177	0.335003985197327 \\
53.7414965986395	0.336086149773 \\
54.0816326530612	0.336905272075855 \\
54.421768707483	0.335782135430454 \\
54.7619047619048	0.333904677478458 \\
55.1020408163265	0.332471868148496 \\
55.4421768707483	0.328700187857139 \\
55.7823129251701	0.324632631729874 \\
56.1224489795918	0.320902927339775 \\
56.4625850340136	0.317063369373573 \\
56.8027210884354	0.316248184932156 \\
57.1428571428571	0.315983089048459 \\
57.4829931972789	0.314574448393869 \\
57.8231292517007	0.30878503854432 \\
58.1632653061224	0.305769965408326 \\
58.5034013605442	0.301546676890066 \\
58.843537414966	0.299411395808893 \\
59.1836734693878	0.298643212861462 \\
59.5238095238095	0.298123359624897 \\
59.8639455782313	0.298506002104914 \\
60.2040816326531	0.294474058378719 \\
60.5442176870748	0.293760763350438 \\
60.8843537414966	0.292845927401943 \\
61.2244897959184	0.290613708080864 \\
61.5646258503401	0.286613733137208 \\
61.9047619047619	0.284044203246262 \\
62.2448979591837	0.280589510316267 \\
62.5850340136054	0.284305568153943 \\
62.9251700680272	0.281886804248276 \\
63.265306122449	0.277832805060513 \\
63.6054421768707	0.275793534595305 \\
63.9455782312925	0.27120630000213 \\
64.2857142857143	0.271036895363618 \\
64.6258503401361	0.269775265163469 \\
64.9659863945578	0.260647339448416 \\
65.3061224489796	0.25441375989104 \\
65.6462585034014	0.247327479077354 \\
65.9863945578231	0.240417573298455 \\
66.3265306122449	0.239562700379633 \\
66.6666666666667	0.236871448656739 \\
67.0068027210884	0.231009768914298 \\
67.3469387755102	0.227938791365172 \\
67.687074829932	0.221974710505433 \\
68.0272108843537	0.222776990460565 \\
68.3673469387755	0.220018049584172 \\
68.7074829931973	0.218197285068915 \\
69.0476190476191	0.215122228909529 \\
69.3877551020408	0.212776383614257 \\
69.7278911564626	0.20441530630801 \\
70.0680272108844	0.20752940288621 \\
70.4081632653061	0.204275350381087 \\
70.7482993197279	0.195943603987184 \\
71.0884353741497	0.195824124805464 \\
71.4285714285714	0.189124272321944 \\
71.7687074829932	0.185251233082082 \\
72.108843537415	0.182325609032875 \\
72.4489795918367	0.178243113301068 \\
72.7891156462585	0.171842963834529 \\
73.1292517006803	0.170072727505929 \\
73.469387755102	0.168407609664062 \\
73.8095238095238	0.16285595940104 \\
74.1496598639456	0.155118957466878 \\
74.4897959183673	0.142872319807743 \\
74.8299319727891	0.133765248270632 \\
75.1700680272109	0.132214383959908 \\
75.5102040816327	0.129947754224917 \\
75.8503401360544	0.12971785186665 \\
76.1904761904762	0.124093903270311 \\
76.530612244898	0.119767440960892 \\
76.8707482993197	0.119514695552797 \\
77.2108843537415	0.116721101174801 \\
77.5510204081633	0.116949915907662 \\
77.891156462585	0.111308752072992 \\
78.2312925170068	0.106552469029788 \\
78.5714285714286	0.102909798393387 \\
78.9115646258503	0.102535148639735 \\
79.2517006802721	0.102572040870379 \\
79.5918367346939	0.10213150161494 \\
79.9319727891156	0.100547181629489 \\
80.2721088435374	0.0963246545695446 \\
80.6122448979592	0.0891249493599218 \\
80.9523809523809	0.0849436711798184 \\
81.2925170068027	0.081982359101299 \\
81.6326530612245	0.0810964876172346 \\
81.9727891156463	0.0826580446612353 \\
82.312925170068	0.0807928451900207 \\
82.6530612244898	0.0768604103074263 \\
82.9931972789116	0.0737039039309467 \\
83.3333333333333	0.0713909499503368 \\
83.6734693877551	0.0667028931811978 \\
84.0136054421769	0.0668227338980876 \\
84.3537414965986	0.0659566124852804 \\
84.6938775510204	0.0648160024906031 \\
85.0340136054422	0.0614516412776967 \\
85.3741496598639	0.0590644620232615 \\
85.7142857142857	0.0584699525052185 \\
86.0544217687075	0.0561515599984743 \\
86.3945578231292	0.052202621775808 \\
86.734693877551	0.0462837368134066 \\
87.0748299319728	0.0443386642920069 \\
87.4149659863945	0.0408792270427671 \\
87.7551020408163	0.0358225054373688 \\
88.0952380952381	0.0340916886313298 \\
88.4353741496599	0.0328822185375645 \\
88.7755102040816	0.0311439960068261 \\
89.1156462585034	0.0310292343189804 \\
89.4557823129252	0.0279554163546185 \\
89.7959183673469	0.0275087504116244 \\
90.1360544217687	0.0252053014578332 \\
90.4761904761905	0.0242898145581337 \\
90.8163265306122	0.0225028065489958 \\
91.156462585034	0.0215711923172732 \\
91.4965986394558	0.0203277728128074 \\
91.8367346938775	0.0160844141953163 \\
92.1768707482993	0.0157738113165527 \\
92.5170068027211	0.0139156329816801 \\
92.8571428571429	0.0121336626089185 \\
93.1972789115646	0.0111054765609815 \\
93.5374149659864	0.0111276058937087 \\
93.8775510204082	0.0100308662814028 \\
94.2176870748299	0.0106549886289124 \\
94.5578231292517	0.0098765692271226 \\
94.8979591836735	0.00936554567147994 \\
95.2380952380952	0.00896277384968498 \\
95.578231292517	0.00843253437002938 \\
95.9183673469388	0.0087294021038929 \\
96.2585034013605	0.00781062433810328 \\
96.5986394557823	0.00677849684189131 \\
96.9387755102041	0.0052576348980747 \\
97.2789115646258	0.00417981724814525 \\
97.6190476190476	0.00444393572260069 \\
97.9591836734694	0.00338361212399031 \\
98.2993197278912	0.00344171875651916 \\
98.6394557823129	0.00352960223258849 \\
98.9795918367347	0.00389471110310113 \\
99.3197278911565	0.0027356847982127 \\
99.6598639455782	0.00211802288449684 \\
100	1.49018575257287e-13 \\
};
\path [fill=color3, fill opacity=0.5] (axis cs:0,0.720594142942223)
--(axis cs:0,0.716939668984618)
--(axis cs:0.340136054421769,0.717437984165697)
--(axis cs:0.680272108843537,0.717180495816169)
--(axis cs:1.02040816326531,0.717733126187742)
--(axis cs:1.36054421768707,0.718760302229062)
--(axis cs:1.70068027210884,0.717856350980166)
--(axis cs:2.04081632653061,0.717081662401164)
--(axis cs:2.38095238095238,0.719548482962931)
--(axis cs:2.72108843537415,0.719577840757421)
--(axis cs:3.06122448979592,0.717264877045346)
--(axis cs:3.40136054421769,0.719534142056039)
--(axis cs:3.74149659863946,0.718162703351326)
--(axis cs:4.08163265306122,0.716758315136891)
--(axis cs:4.42176870748299,0.7141732208749)
--(axis cs:4.76190476190476,0.710424381015532)
--(axis cs:5.10204081632653,0.708589588780813)
--(axis cs:5.4421768707483,0.706033863534526)
--(axis cs:5.78231292517007,0.705057269859717)
--(axis cs:6.12244897959184,0.704409716368244)
--(axis cs:6.46258503401361,0.704284490571228)
--(axis cs:6.80272108843537,0.706089807707554)
--(axis cs:7.14285714285714,0.703928430236954)
--(axis cs:7.48299319727891,0.701552189153602)
--(axis cs:7.82312925170068,0.69047666446522)
--(axis cs:8.16326530612245,0.683405463609018)
--(axis cs:8.50340136054422,0.678759280458781)
--(axis cs:8.84353741496599,0.677874672855845)
--(axis cs:9.18367346938775,0.673931111757456)
--(axis cs:9.52380952380952,0.669864543901554)
--(axis cs:9.86394557823129,0.666298613905559)
--(axis cs:10.2040816326531,0.667827110759702)
--(axis cs:10.5442176870748,0.668363627076994)
--(axis cs:10.8843537414966,0.670079675713607)
--(axis cs:11.2244897959184,0.664298447774924)
--(axis cs:11.5646258503401,0.659248604467114)
--(axis cs:11.9047619047619,0.655386376604926)
--(axis cs:12.2448979591837,0.653258994449644)
--(axis cs:12.5850340136054,0.648107967213239)
--(axis cs:12.9251700680272,0.6458559695527)
--(axis cs:13.265306122449,0.645060018782077)
--(axis cs:13.6054421768707,0.64239064302433)
--(axis cs:13.9455782312925,0.638904086085133)
--(axis cs:14.2857142857143,0.634296183650277)
--(axis cs:14.6258503401361,0.633615371374429)
--(axis cs:14.9659863945578,0.632336478897796)
--(axis cs:15.3061224489796,0.632705257600737)
--(axis cs:15.6462585034014,0.624625034812496)
--(axis cs:15.9863945578231,0.620061929152459)
--(axis cs:16.3265306122449,0.617070532651477)
--(axis cs:16.6666666666667,0.6155429350569)
--(axis cs:17.0068027210884,0.602917557427408)
--(axis cs:17.3469387755102,0.60019342954406)
--(axis cs:17.687074829932,0.595589329837325)
--(axis cs:18.0272108843537,0.593899794049819)
--(axis cs:18.3673469387755,0.591899974914359)
--(axis cs:18.7074829931973,0.58255879642697)
--(axis cs:19.047619047619,0.578356577337889)
--(axis cs:19.3877551020408,0.576377414599476)
--(axis cs:19.7278911564626,0.573176850838666)
--(axis cs:20.0680272108844,0.568088050267231)
--(axis cs:20.4081632653061,0.562341417007614)
--(axis cs:20.7482993197279,0.55965410209121)
--(axis cs:21.0884353741497,0.558786410250021)
--(axis cs:21.4285714285714,0.557198108211161)
--(axis cs:21.7687074829932,0.552365948234291)
--(axis cs:22.108843537415,0.549247898922416)
--(axis cs:22.4489795918367,0.545009310935142)
--(axis cs:22.7891156462585,0.543645363460276)
--(axis cs:23.1292517006803,0.539737267768497)
--(axis cs:23.469387755102,0.53491799894887)
--(axis cs:23.8095238095238,0.529510109315418)
--(axis cs:24.1496598639456,0.52622720353833)
--(axis cs:24.4897959183673,0.516705981093581)
--(axis cs:24.8299319727891,0.51501532947664)
--(axis cs:25.1700680272109,0.512913207116057)
--(axis cs:25.5102040816327,0.506553182236278)
--(axis cs:25.8503401360544,0.509021659763276)
--(axis cs:26.1904761904762,0.510207333180382)
--(axis cs:26.530612244898,0.506911828675307)
--(axis cs:26.8707482993197,0.505723550299633)
--(axis cs:27.2108843537415,0.505161440558141)
--(axis cs:27.5510204081633,0.504690779174378)
--(axis cs:27.891156462585,0.501242415799509)
--(axis cs:28.2312925170068,0.500052156615502)
--(axis cs:28.5714285714286,0.497786125691004)
--(axis cs:28.9115646258503,0.49351757365661)
--(axis cs:29.2517006802721,0.494543316942371)
--(axis cs:29.5918367346939,0.489596621656908)
--(axis cs:29.9319727891156,0.489476205274871)
--(axis cs:30.2721088435374,0.484695363462697)
--(axis cs:30.6122448979592,0.48162550815772)
--(axis cs:30.952380952381,0.475561110352666)
--(axis cs:31.2925170068027,0.47161441465256)
--(axis cs:31.6326530612245,0.469821415764907)
--(axis cs:31.9727891156463,0.470185182323525)
--(axis cs:32.312925170068,0.469032705570073)
--(axis cs:32.6530612244898,0.46712516522425)
--(axis cs:32.9931972789116,0.468050634335241)
--(axis cs:33.3333333333333,0.466055688312484)
--(axis cs:33.6734693877551,0.466031508449967)
--(axis cs:34.0136054421769,0.463170196075041)
--(axis cs:34.3537414965986,0.463347847414062)
--(axis cs:34.6938775510204,0.460956605767799)
--(axis cs:35.0340136054422,0.44478676317037)
--(axis cs:35.3741496598639,0.442584014581266)
--(axis cs:35.7142857142857,0.444506117519195)
--(axis cs:36.0544217687075,0.441972793615971)
--(axis cs:36.3945578231292,0.440417583709151)
--(axis cs:36.734693877551,0.440371630241294)
--(axis cs:37.0748299319728,0.437656938411066)
--(axis cs:37.4149659863946,0.435799805573022)
--(axis cs:37.7551020408163,0.435434767298413)
--(axis cs:38.0952380952381,0.430792871170251)
--(axis cs:38.4353741496599,0.427855756818592)
--(axis cs:38.7755102040816,0.426681344777177)
--(axis cs:39.1156462585034,0.424888912657496)
--(axis cs:39.4557823129252,0.421946462459396)
--(axis cs:39.7959183673469,0.421409590700997)
--(axis cs:40.1360544217687,0.419702468474487)
--(axis cs:40.4761904761905,0.416506265134196)
--(axis cs:40.8163265306122,0.412172990013144)
--(axis cs:41.156462585034,0.410549184370515)
--(axis cs:41.4965986394558,0.41009899853879)
--(axis cs:41.8367346938776,0.414591383945313)
--(axis cs:42.1768707482993,0.413977887979809)
--(axis cs:42.5170068027211,0.412529233783587)
--(axis cs:42.8571428571429,0.408580982095096)
--(axis cs:43.1972789115646,0.402072419264918)
--(axis cs:43.5374149659864,0.400347425194075)
--(axis cs:43.8775510204082,0.398868874820484)
--(axis cs:44.2176870748299,0.396838351453048)
--(axis cs:44.5578231292517,0.394329634779206)
--(axis cs:44.8979591836735,0.390582630055705)
--(axis cs:45.2380952380952,0.384788288795462)
--(axis cs:45.578231292517,0.384924969876491)
--(axis cs:45.9183673469388,0.380971609717791)
--(axis cs:46.2585034013605,0.374559767144011)
--(axis cs:46.5986394557823,0.372419502373297)
--(axis cs:46.9387755102041,0.370026362440715)
--(axis cs:47.2789115646259,0.367553232508012)
--(axis cs:47.6190476190476,0.365173137939201)
--(axis cs:47.9591836734694,0.363961187909182)
--(axis cs:48.2993197278912,0.363128240543656)
--(axis cs:48.6394557823129,0.357897969324211)
--(axis cs:48.9795918367347,0.351540998973091)
--(axis cs:49.3197278911565,0.350959345158851)
--(axis cs:49.6598639455782,0.350278507402029)
--(axis cs:50,0.34783450619431)
--(axis cs:50.3401360544218,0.348100529013051)
--(axis cs:50.6802721088435,0.347378582307593)
--(axis cs:51.0204081632653,0.34580367367682)
--(axis cs:51.3605442176871,0.342181684825039)
--(axis cs:51.7006802721088,0.340377566553661)
--(axis cs:52.0408163265306,0.337064597185386)
--(axis cs:52.3809523809524,0.334911881782861)
--(axis cs:52.7210884353741,0.33265765790913)
--(axis cs:53.0612244897959,0.331504937362337)
--(axis cs:53.4013605442177,0.330813055873814)
--(axis cs:53.7414965986395,0.331853093607696)
--(axis cs:54.0816326530612,0.332612841105997)
--(axis cs:54.421768707483,0.331485268493384)
--(axis cs:54.7619047619048,0.32963867423934)
--(axis cs:55.1020408163265,0.328135427068783)
--(axis cs:55.4421768707483,0.324388464240887)
--(axis cs:55.7823129251701,0.32042962669729)
--(axis cs:56.1224489795918,0.316818666555536)
--(axis cs:56.4625850340136,0.312829736520844)
--(axis cs:56.8027210884354,0.311936213569218)
--(axis cs:57.1428571428571,0.311638837979229)
--(axis cs:57.4829931972789,0.310261432857393)
--(axis cs:57.8231292517007,0.304523190576395)
--(axis cs:58.1632653061224,0.301472329514683)
--(axis cs:58.5034013605442,0.297202985880764)
--(axis cs:58.843537414966,0.295077953897623)
--(axis cs:59.1836734693878,0.294382474518548)
--(axis cs:59.5238095238095,0.293797719696709)
--(axis cs:59.8639455782313,0.29413143556074)
--(axis cs:60.2040816326531,0.290152864940029)
--(axis cs:60.5442176870748,0.289422323891225)
--(axis cs:60.8843537414966,0.288423969493066)
--(axis cs:61.2244897959184,0.286064371900641)
--(axis cs:61.5646258503401,0.282124373455859)
--(axis cs:61.9047619047619,0.279405980177277)
--(axis cs:62.2448979591837,0.276073714573217)
--(axis cs:62.5850340136054,0.279507657373432)
--(axis cs:62.9251700680272,0.277097282148821)
--(axis cs:63.265306122449,0.273147983080419)
--(axis cs:63.6054421768707,0.271095421446169)
--(axis cs:63.9455782312925,0.266554571396084)
--(axis cs:64.2857142857143,0.266198053915858)
--(axis cs:64.6258503401361,0.265088472344574)
--(axis cs:64.9659863945578,0.255984046817651)
--(axis cs:65.3061224489796,0.249928692393857)
--(axis cs:65.6462585034014,0.242863552394958)
--(axis cs:65.9863945578231,0.235781703710449)
--(axis cs:66.3265306122449,0.234963133612053)
--(axis cs:66.6666666666667,0.232253366821412)
--(axis cs:67.0068027210884,0.226228214920367)
--(axis cs:67.3469387755102,0.223149767102412)
--(axis cs:67.687074829932,0.217107587991474)
--(axis cs:68.0272108843537,0.217947983517015)
--(axis cs:68.3673469387755,0.215419752543181)
--(axis cs:68.7074829931973,0.21349534768497)
--(axis cs:69.0476190476191,0.210437306185963)
--(axis cs:69.3877551020408,0.208013562461946)
--(axis cs:69.7278911564626,0.199686654558908)
--(axis cs:70.0680272108844,0.202712640448103)
--(axis cs:70.4081632653061,0.199652372993195)
--(axis cs:70.7482993197279,0.191585107205146)
--(axis cs:71.0884353741497,0.191468809071194)
--(axis cs:71.4285714285714,0.184788682968553)
--(axis cs:71.7687074829932,0.18094678396658)
--(axis cs:72.108843537415,0.177881079149126)
--(axis cs:72.4489795918367,0.173613869500764)
--(axis cs:72.7891156462585,0.167376207603079)
--(axis cs:73.1292517006803,0.16569769612718)
--(axis cs:73.469387755102,0.164054816248124)
--(axis cs:73.8095238095238,0.158289403844688)
--(axis cs:74.1496598639456,0.150594407858371)
--(axis cs:74.4897959183673,0.138529336775701)
--(axis cs:74.8299319727891,0.12960523019342)
--(axis cs:75.1700680272109,0.128204767708864)
--(axis cs:75.5102040816327,0.125884305968976)
--(axis cs:75.8503401360544,0.125804851331824)
--(axis cs:76.1904761904762,0.120130653305164)
--(axis cs:76.530612244898,0.115984115413814)
--(axis cs:76.8707482993197,0.115594963583808)
--(axis cs:77.2108843537415,0.113004875127433)
--(axis cs:77.5510204081633,0.11310650393625)
--(axis cs:77.891156462585,0.107620478014796)
--(axis cs:78.2312925170068,0.103089576083498)
--(axis cs:78.5714285714286,0.0991683961787423)
--(axis cs:78.9115646258503,0.0988206702603063)
--(axis cs:79.2517006802721,0.0988585989691787)
--(axis cs:79.5918367346939,0.0982823050011094)
--(axis cs:79.9319727891156,0.0966600675300525)
--(axis cs:80.2721088435374,0.0927359943258418)
--(axis cs:80.6122448979592,0.0857998323312688)
--(axis cs:80.9523809523809,0.0817941067021716)
--(axis cs:81.2925170068027,0.0789590327280396)
--(axis cs:81.6326530612245,0.0779726537903061)
--(axis cs:81.9727891156463,0.0795653405002099)
--(axis cs:82.312925170068,0.0777498055720461)
--(axis cs:82.6530612244898,0.0739698337777903)
--(axis cs:82.9931972789116,0.0709599037398884)
--(axis cs:83.3333333333333,0.0687092787482778)
--(axis cs:83.6734693877551,0.0640775409783246)
--(axis cs:84.0136054421769,0.0641557087138501)
--(axis cs:84.3537414965986,0.0633604038030062)
--(axis cs:84.6938775510204,0.0619965884008207)
--(axis cs:85.0340136054422,0.0589122881278352)
--(axis cs:85.3741496598639,0.056584395921428)
--(axis cs:85.7142857142857,0.0561697835329721)
--(axis cs:86.0544217687075,0.0538334996735845)
--(axis cs:86.3945578231292,0.0497291939375997)
--(axis cs:86.734693877551,0.0438690961707008)
--(axis cs:87.0748299319728,0.0420689250931629)
--(axis cs:87.4149659863945,0.0385700747237209)
--(axis cs:87.7551020408163,0.0337392251217408)
--(axis cs:88.0952380952381,0.0323102556127425)
--(axis cs:88.4353741496599,0.0310708079105684)
--(axis cs:88.7755102040816,0.0293760460531408)
--(axis cs:89.1156462585034,0.029281533974112)
--(axis cs:89.4557823129252,0.0263738539365834)
--(axis cs:89.7959183673469,0.0257043500451409)
--(axis cs:90.1360544217687,0.0235412883980481)
--(axis cs:90.4761904761905,0.0225907092525502)
--(axis cs:90.8163265306122,0.0207388273353557)
--(axis cs:91.156462585034,0.0198801381775156)
--(axis cs:91.4965986394558,0.0187087307679797)
--(axis cs:91.8367346938775,0.0146292503389463)
--(axis cs:92.1768707482993,0.0142241586310605)
--(axis cs:92.5170068027211,0.0124753331752837)
--(axis cs:92.8571428571429,0.0108445676069179)
--(axis cs:93.1972789115646,0.009998694778973)
--(axis cs:93.5374149659864,0.0100787513668439)
--(axis cs:93.8775510204082,0.0090286977461166)
--(axis cs:94.2176870748299,0.00967286660641557)
--(axis cs:94.5578231292517,0.00885208323334254)
--(axis cs:94.8979591836735,0.00840252456658058)
--(axis cs:95.2380952380952,0.00796738120842043)
--(axis cs:95.578231292517,0.0074722574024463)
--(axis cs:95.9183673469388,0.0078644429800907)
--(axis cs:96.2585034013605,0.00693276966780958)
--(axis cs:96.5986394557823,0.00605995010611649)
--(axis cs:96.9387755102041,0.00458236564871523)
--(axis cs:97.2789115646258,0.00358271684915446)
--(axis cs:97.6190476190476,0.00393054997749758)
--(axis cs:97.9591836734694,0.00296553299033607)
--(axis cs:98.2993197278912,0.0030197287868765)
--(axis cs:98.6394557823129,0.0030487272040376)
--(axis cs:98.9795918367347,0.00330016128653771)
--(axis cs:99.3197278911565,0.00248074102191435)
--(axis cs:99.6598639455782,0.00195561024863338)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,0.0022804355203603)
--(axis cs:99.3197278911565,0.00299062857451104)
--(axis cs:98.9795918367347,0.00448926091966455)
--(axis cs:98.6394557823129,0.00401047726113938)
--(axis cs:98.2993197278912,0.00386370872616181)
--(axis cs:97.9591836734694,0.00380169125764454)
--(axis cs:97.6190476190476,0.00495732146770381)
--(axis cs:97.2789115646258,0.00477691764713604)
--(axis cs:96.9387755102041,0.00593290414743417)
--(axis cs:96.5986394557823,0.00749704357766613)
--(axis cs:96.2585034013605,0.00868847900839698)
--(axis cs:95.9183673469388,0.0095943612276951)
--(axis cs:95.578231292517,0.00939281133761246)
--(axis cs:95.2380952380952,0.00995816649094954)
--(axis cs:94.8979591836735,0.0103285667763793)
--(axis cs:94.5578231292517,0.0109010552209027)
--(axis cs:94.2176870748299,0.0116371106514093)
--(axis cs:93.8775510204082,0.011033034816689)
--(axis cs:93.5374149659864,0.0121764604205734)
--(axis cs:93.1972789115646,0.0122122583429899)
--(axis cs:92.8571428571429,0.0134227576109191)
--(axis cs:92.5170068027211,0.0153559327880766)
--(axis cs:92.1768707482993,0.0173234640020449)
--(axis cs:91.8367346938775,0.0175395780516863)
--(axis cs:91.4965986394558,0.021946814857635)
--(axis cs:91.156462585034,0.0232622464570307)
--(axis cs:90.8163265306122,0.0242667857626358)
--(axis cs:90.4761904761905,0.0259889198637171)
--(axis cs:90.1360544217687,0.0268693145176183)
--(axis cs:89.7959183673469,0.0293131507781079)
--(axis cs:89.4557823129252,0.0295369787726536)
--(axis cs:89.1156462585034,0.0327769346638488)
--(axis cs:88.7755102040816,0.0329119459605115)
--(axis cs:88.4353741496599,0.0346936291645605)
--(axis cs:88.0952380952381,0.035873121649917)
--(axis cs:87.7551020408163,0.0379057857529969)
--(axis cs:87.4149659863945,0.0431883793618134)
--(axis cs:87.0748299319728,0.0466084034908508)
--(axis cs:86.734693877551,0.0486983774561125)
--(axis cs:86.3945578231292,0.0546760496140164)
--(axis cs:86.0544217687075,0.0584696203233641)
--(axis cs:85.7142857142857,0.060770121477465)
--(axis cs:85.3741496598639,0.061544528125095)
--(axis cs:85.0340136054422,0.0639909944275582)
--(axis cs:84.6938775510204,0.0676354165803855)
--(axis cs:84.3537414965986,0.0685528211675547)
--(axis cs:84.0136054421769,0.0694897590823251)
--(axis cs:83.6734693877551,0.0693282453840711)
--(axis cs:83.3333333333333,0.0740726211523958)
--(axis cs:82.9931972789116,0.0764479041220049)
--(axis cs:82.6530612244898,0.0797509868370622)
--(axis cs:82.312925170068,0.0838358848079953)
--(axis cs:81.9727891156463,0.0857507488222608)
--(axis cs:81.6326530612245,0.084220321444163)
--(axis cs:81.2925170068027,0.0850056854745584)
--(axis cs:80.9523809523809,0.0880932356574652)
--(axis cs:80.6122448979592,0.0924500663885749)
--(axis cs:80.2721088435374,0.0999133148132473)
--(axis cs:79.9319727891156,0.104434295728925)
--(axis cs:79.5918367346939,0.105980698228771)
--(axis cs:79.2517006802721,0.10628548277158)
--(axis cs:78.9115646258503,0.106249627019164)
--(axis cs:78.5714285714286,0.106651200608032)
--(axis cs:78.2312925170068,0.110015361976077)
--(axis cs:77.891156462585,0.114997026131188)
--(axis cs:77.5510204081633,0.120793327879073)
--(axis cs:77.2108843537415,0.120437327222169)
--(axis cs:76.8707482993197,0.123434427521786)
--(axis cs:76.530612244898,0.123550766507971)
--(axis cs:76.1904761904762,0.128057153235458)
--(axis cs:75.8503401360544,0.133630852401476)
--(axis cs:75.5102040816327,0.134011202480858)
--(axis cs:75.1700680272109,0.136224000210952)
--(axis cs:74.8299319727891,0.137925266347845)
--(axis cs:74.4897959183673,0.147215302839786)
--(axis cs:74.1496598639456,0.159643507075385)
--(axis cs:73.8095238095238,0.167422514957392)
--(axis cs:73.469387755102,0.17276040308)
--(axis cs:73.1292517006803,0.174447758884679)
--(axis cs:72.7891156462585,0.176309720065978)
--(axis cs:72.4489795918367,0.182872357101372)
--(axis cs:72.108843537415,0.186770138916625)
--(axis cs:71.7687074829932,0.189555682197584)
--(axis cs:71.4285714285714,0.193459861675336)
--(axis cs:71.0884353741497,0.200179440539734)
--(axis cs:70.7482993197279,0.200302100769221)
--(axis cs:70.4081632653061,0.208898327768978)
--(axis cs:70.0680272108844,0.212346165324316)
--(axis cs:69.7278911564626,0.209143958057113)
--(axis cs:69.3877551020408,0.217539204766567)
--(axis cs:69.0476190476191,0.219807151633095)
--(axis cs:68.7074829931973,0.22289922245286)
--(axis cs:68.3673469387755,0.224616346625163)
--(axis cs:68.0272108843537,0.227605997404116)
--(axis cs:67.687074829932,0.226841833019393)
--(axis cs:67.3469387755102,0.232727815627932)
--(axis cs:67.0068027210884,0.235791322908229)
--(axis cs:66.6666666666667,0.241489530492066)
--(axis cs:66.3265306122449,0.244162267147212)
--(axis cs:65.9863945578231,0.245053442886461)
--(axis cs:65.6462585034014,0.25179140575975)
--(axis cs:65.3061224489796,0.258898827388223)
--(axis cs:64.9659863945578,0.26531063207918)
--(axis cs:64.6258503401361,0.274462057982363)
--(axis cs:64.2857142857143,0.275875736811378)
--(axis cs:63.9455782312925,0.275858028608175)
--(axis cs:63.6054421768707,0.28049164774444)
--(axis cs:63.265306122449,0.282517627040606)
--(axis cs:62.9251700680272,0.286676326347731)
--(axis cs:62.5850340136054,0.289103478934454)
--(axis cs:62.2448979591837,0.285105306059318)
--(axis cs:61.9047619047619,0.288682426315248)
--(axis cs:61.5646258503401,0.291103092818557)
--(axis cs:61.2244897959184,0.295163044261087)
--(axis cs:60.8843537414966,0.29726788531082)
--(axis cs:60.5442176870748,0.29809920280965)
--(axis cs:60.2040816326531,0.298795251817409)
--(axis cs:59.8639455782313,0.302880568649088)
--(axis cs:59.5238095238095,0.302448999553084)
--(axis cs:59.1836734693878,0.302903951204375)
--(axis cs:58.843537414966,0.303744837720163)
--(axis cs:58.5034013605442,0.305890367899368)
--(axis cs:58.1632653061224,0.31006760130197)
--(axis cs:57.8231292517007,0.313046886512245)
--(axis cs:57.4829931972789,0.318887463930345)
--(axis cs:57.1428571428571,0.320327340117689)
--(axis cs:56.8027210884354,0.320560156295093)
--(axis cs:56.4625850340136,0.321297002226302)
--(axis cs:56.1224489795918,0.324987188124015)
--(axis cs:55.7823129251701,0.328835636762458)
--(axis cs:55.4421768707483,0.333011911473391)
--(axis cs:55.1020408163265,0.336808309228208)
--(axis cs:54.7619047619048,0.338170680717577)
--(axis cs:54.421768707483,0.340079002367525)
--(axis cs:54.0816326530612,0.341197703045714)
--(axis cs:53.7414965986395,0.340319205938305)
--(axis cs:53.4013605442177,0.33919491452084)
--(axis cs:53.0612244897959,0.339928525107312)
--(axis cs:52.7210884353741,0.341047825380102)
--(axis cs:52.3809523809524,0.342988976306991)
--(axis cs:52.0408163265306,0.34547149924168)
--(axis cs:51.7006802721088,0.348665329589631)
--(axis cs:51.3605442176871,0.350674906545835)
--(axis cs:51.0204081632653,0.354773007574148)
--(axis cs:50.6802721088435,0.356390193787864)
--(axis cs:50.3401360544218,0.356986040419554)
--(axis cs:50,0.356902130331976)
--(axis cs:49.6598639455782,0.359500211380808)
--(axis cs:49.3197278911565,0.359946296377595)
--(axis cs:48.9795918367347,0.360548660022446)
--(axis cs:48.6394557823129,0.366703971484505)
--(axis cs:48.2993197278912,0.372042620320217)
--(axis cs:47.9591836734694,0.372596971089705)
--(axis cs:47.6190476190476,0.374109002547956)
--(axis cs:47.2789115646259,0.376373369745475)
--(axis cs:46.9387755102041,0.378820904413931)
--(axis cs:46.5986394557823,0.381197286628384)
--(axis cs:46.2585034013605,0.383243616937624)
--(axis cs:45.9183673469388,0.389652194657855)
--(axis cs:45.578231292517,0.393914822181206)
--(axis cs:45.2380952380952,0.393635552618871)
--(axis cs:44.8979591836735,0.399399552043487)
--(axis cs:44.5578231292517,0.40309773551824)
--(axis cs:44.2176870748299,0.405333085458983)
--(axis cs:43.8775510204082,0.407726028814857)
--(axis cs:43.5374149659864,0.409429874070604)
--(axis cs:43.1972789115646,0.411384445444088)
--(axis cs:42.8571428571429,0.417803921757644)
--(axis cs:42.5170068027211,0.421095859966865)
--(axis cs:42.1768707482993,0.422593776872863)
--(axis cs:41.8367346938776,0.423372405610775)
--(axis cs:41.4965986394558,0.418972168724674)
--(axis cs:41.156462585034,0.419473676137082)
--(axis cs:40.8163265306122,0.42096614635672)
--(axis cs:40.4761904761905,0.424942264378076)
--(axis cs:40.1360544217687,0.428247879138882)
--(axis cs:39.7959183673469,0.42997844972001)
--(axis cs:39.4557823129252,0.430667949151015)
--(axis cs:39.1156462585034,0.433894791065379)
--(axis cs:38.7755102040816,0.435530138871394)
--(axis cs:38.4353741496599,0.436629621095797)
--(axis cs:38.0952380952381,0.439891218697322)
--(axis cs:37.7551020408163,0.444418882916669)
--(axis cs:37.4149659863946,0.444689247501249)
--(axis cs:37.0748299319728,0.446610430438767)
--(axis cs:36.734693877551,0.449256971696145)
--(axis cs:36.3945578231292,0.449593929039746)
--(axis cs:36.0544217687075,0.451288733103464)
--(axis cs:35.7142857142857,0.453791120321402)
--(axis cs:35.3741496598639,0.451541764110111)
--(axis cs:35.0340136054422,0.454100683472251)
--(axis cs:34.6938775510204,0.470029418065594)
--(axis cs:34.3537414965986,0.472168163743826)
--(axis cs:34.0136054421769,0.472115737689494)
--(axis cs:33.6734693877551,0.475028696931979)
--(axis cs:33.3333333333333,0.474967592681202)
--(axis cs:32.9931972789116,0.477276723761597)
--(axis cs:32.6530612244898,0.47626530020457)
--(axis cs:32.312925170068,0.478334997396948)
--(axis cs:31.9727891156463,0.479215747822696)
--(axis cs:31.6326530612245,0.47888043733996)
--(axis cs:31.2925170068027,0.481182443125889)
--(axis cs:30.952380952381,0.48485949140644)
--(axis cs:30.6122448979592,0.490636534605457)
--(axis cs:30.2721088435374,0.493841286419165)
--(axis cs:29.9319727891156,0.498671864779723)
--(axis cs:29.5918367346939,0.498773928664507)
--(axis cs:29.2517006802721,0.503421279135429)
--(axis cs:28.9115646258503,0.502174528028953)
--(axis cs:28.5714285714286,0.506678835739054)
--(axis cs:28.2312925170068,0.508643280629104)
--(axis cs:27.891156462585,0.509752669384022)
--(axis cs:27.5510204081633,0.513754607836783)
--(axis cs:27.2108843537415,0.513844618695447)
--(axis cs:26.8707482993197,0.514459217175856)
--(axis cs:26.530612244898,0.515939577374141)
--(axis cs:26.1904761904762,0.519092272957992)
--(axis cs:25.8503401360544,0.518102260595442)
--(axis cs:25.5102040816327,0.515625588058135)
--(axis cs:25.1700680272109,0.521720834241728)
--(axis cs:24.8299319727891,0.524224305748745)
--(axis cs:24.4897959183673,0.525920368553017)
--(axis cs:24.1496598639456,0.535929098282321)
--(axis cs:23.8095238095238,0.53913611016909)
--(axis cs:23.469387755102,0.544321006814214)
--(axis cs:23.1292517006803,0.549103114963954)
--(axis cs:22.7891156462585,0.55318065867668)
--(axis cs:22.4489795918367,0.554612008127866)
--(axis cs:22.108843537415,0.558644419762191)
--(axis cs:21.7687074829932,0.561813672005593)
--(axis cs:21.4285714285714,0.566229675598441)
--(axis cs:21.0884353741497,0.568080847451212)
--(axis cs:20.7482993197279,0.568953247602565)
--(axis cs:20.4081632653061,0.571719914983492)
--(axis cs:20.0680272108844,0.577340297525246)
--(axis cs:19.7278911564626,0.582219736665408)
--(axis cs:19.3877551020408,0.585521765468227)
--(axis cs:19.047619047619,0.587563973857852)
--(axis cs:18.7074829931973,0.591706339081061)
--(axis cs:18.3673469387755,0.600756196314377)
--(axis cs:18.0272108843537,0.602493684053163)
--(axis cs:17.687074829932,0.604232320362267)
--(axis cs:17.3469387755102,0.608784002837302)
--(axis cs:17.0068027210884,0.611350114854304)
--(axis cs:16.6666666666667,0.623810908386195)
--(axis cs:16.3265306122449,0.625583839280672)
--(axis cs:15.9863945578231,0.628318128510267)
--(axis cs:15.6462585034014,0.632681513171985)
--(axis cs:15.3061224489796,0.640161730804848)
--(axis cs:14.9659863945578,0.639707361801102)
--(axis cs:14.6258503401361,0.641133355857789)
--(axis cs:14.2857142857143,0.641519312459149)
--(axis cs:13.9455782312925,0.646250960199066)
--(axis cs:13.6054421768707,0.649290655887242)
--(axis cs:13.265306122449,0.652122840400281)
--(axis cs:12.9251700680272,0.652747617597874)
--(axis cs:12.5850340136054,0.655217366382037)
--(axis cs:12.2448979591837,0.660307824681731)
--(axis cs:11.9047619047619,0.662269573285687)
--(axis cs:11.5646258503401,0.665794890234272)
--(axis cs:11.2244897959184,0.670941353929959)
--(axis cs:10.8843537414966,0.676490649780205)
--(axis cs:10.5442176870748,0.674872598170389)
--(axis cs:10.2040816326531,0.674305469520602)
--(axis cs:9.86394557823129,0.672822406232705)
--(axis cs:9.52380952380952,0.676351409329303)
--(axis cs:9.18367346938775,0.680383202965558)
--(axis cs:8.84353741496599,0.684159319553861)
--(axis cs:8.50340136054422,0.685152880533841)
--(axis cs:8.16326530612245,0.689651235428534)
--(axis cs:7.82312925170068,0.696565772730558)
--(axis cs:7.48299319727891,0.70703604860885)
--(axis cs:7.14285714285714,0.709305502913814)
--(axis cs:6.80272108843537,0.711288906377071)
--(axis cs:6.46258503401361,0.709589365496429)
--(axis cs:6.12244897959184,0.709672078251316)
--(axis cs:5.78231292517007,0.710223193835809)
--(axis cs:5.4421768707483,0.711039920339985)
--(axis cs:5.10204081632653,0.713612298588343)
--(axis cs:4.76190476190476,0.715323166730173)
--(axis cs:4.42176870748299,0.718948018668062)
--(axis cs:4.08163265306122,0.72143373532011)
--(axis cs:3.74149659863946,0.722833324237519)
--(axis cs:3.40136054421769,0.724123659095237)
--(axis cs:3.06122448979592,0.721867767488765)
--(axis cs:2.72108843537415,0.723957317876764)
--(axis cs:2.38095238095238,0.723821330002462)
--(axis cs:2.04081632653061,0.721372439876591)
--(axis cs:1.70068027210884,0.721907687940236)
--(axis cs:1.36054421768707,0.722841999368533)
--(axis cs:1.02040816326531,0.721659555232107)
--(axis cs:0.680272108843537,0.720929492754044)
--(axis cs:0.340136054421769,0.72112166720912)
--(axis cs:0,0.720594142942223)
--cycle;


==> img/stl10/stl10_rate_distortion_lrp.tex <==
% lrp-a-flat
\addplot [line width=0.5, opacity=0.8, color1, mark=otimes*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color1, thin}]
table [row sep=\\]{%
0	0.718581347763538 \\
0.340136054421769	0.722781559228897 \\
0.680272108843537	0.719835877120495 \\
1.02040816326531	0.7154612159729 \\
1.36054421768707	0.701508499830961 \\
1.70068027210884	0.681923521161079 \\
2.04081632653061	0.6634206482023 \\
2.38095238095238	0.649270900422707 \\
2.72108843537415	0.633445140263066 \\
3.06122448979592	0.617503748484887 \\
3.40136054421769	0.604008373635588 \\
3.74149659863946	0.582857135559316 \\
4.08163265306122	0.571511800973967 \\
4.42176870748299	0.557647853311937 \\
4.76190476190476	0.536674577254307 \\
5.10204081632653	0.517604244036775 \\
5.4421768707483	0.502443106418068 \\
5.78231292517007	0.48698241355798 \\
6.12244897959184	0.475311955643756 \\
6.46258503401361	0.463223769892652 \\
6.80272108843537	0.445394996865998 \\
7.14285714285714	0.431506154333374 \\
7.48299319727891	0.417759523551392 \\
7.82312925170068	0.408657985948939 \\
8.16326530612245	0.401173973955763 \\
8.50340136054422	0.389658033523001 \\
8.84353741496599	0.382761239030669 \\
9.18367346938775	0.375353393593473 \\
9.52380952380952	0.363735419225695 \\
9.86394557823129	0.355536900763223 \\
10.2040816326531	0.346056232638816 \\
10.5442176870748	0.341541228915366 \\
10.8843537414966	0.332755282462579 \\
11.2244897959184	0.323974137333776 \\
11.5646258503401	0.316993336027856 \\
11.9047619047619	0.311373373473929 \\
12.2448979591837	0.304634379815202 \\
12.5850340136054	0.303064284305076 \\
12.9251700680272	0.29838725348766 \\
13.265306122449	0.293500826599426 \\
13.6054421768707	0.290035895246597 \\
13.9455782312925	0.289534284093255 \\
14.2857142857143	0.285448271508083 \\
14.6258503401361	0.281448610794587 \\
14.9659863945578	0.275071788834387 \\
15.3061224489796	0.270006301790141 \\
15.6462585034014	0.267180388635518 \\
15.9863945578231	0.263122932745737 \\
16.3265306122449	0.257429033452325 \\
16.6666666666667	0.253494289276241 \\
17.0068027210884	0.250217163356098 \\
17.3469387755102	0.245507567161591 \\
17.687074829932	0.237967102338837 \\
18.0272108843537	0.234040625459044 \\
18.3673469387755	0.227656136135168 \\
18.7074829931973	0.223651732351755 \\
19.047619047619	0.218509497349905 \\
19.3877551020408	0.21698099646487 \\
19.7278911564626	0.21284142712839 \\
20.0680272108844	0.208822800795393 \\
20.4081632653061	0.204215391737533 \\
20.7482993197279	0.200197406724542 \\
21.0884353741497	0.198583720839625 \\
21.4285714285714	0.195530947986628 \\
21.7687074829932	0.19352892648666 \\
22.108843537415	0.188709972901708 \\
22.4489795918367	0.186529954689293 \\
22.7891156462585	0.180831251833624 \\
23.1292517006803	0.176875471195712 \\
23.469387755102	0.171481753609305 \\
23.8095238095238	0.168667472408861 \\
24.1496598639456	0.16427428155744 \\
24.4897959183673	0.161429322696179 \\
24.8299319727891	0.159053509903285 \\
25.1700680272109	0.154577126673024 \\
25.5102040816327	0.152691170566442 \\
25.8503401360544	0.151069727540703 \\
26.1904761904762	0.147941174874518 \\
26.530612244898	0.146225159064673 \\
26.8707482993197	0.144532303408834 \\
27.2108843537415	0.140994491545631 \\
27.5510204081633	0.137878830823015 \\
27.891156462585	0.135539512237833 \\
28.2312925170068	0.135057877242673 \\
28.5714285714286	0.134265963328284 \\
28.9115646258503	0.133106091994749 \\
29.2517006802721	0.132518664686836 \\
29.5918367346939	0.12859027659083 \\
29.9319727891156	0.126421756703465 \\
30.2721088435374	0.125533809583936 \\
30.6122448979592	0.124619277891576 \\
30.952380952381	0.121851436760817 \\
31.2925170068027	0.120563475562818 \\
31.6326530612245	0.12093262890192 \\
31.9727891156463	0.119022222549263 \\
32.312925170068	0.116835008292357 \\
32.6530612244898	0.113394702468185 \\
32.9931972789116	0.111633691079592 \\
33.3333333333333	0.108133777274584 \\
33.6734693877551	0.105755129461158 \\
34.0136054421769	0.102824708404178 \\
34.3537414965986	0.100534247604248 \\
34.6938775510204	0.0966431460419433 \\
35.0340136054422	0.0944851137624845 \\
35.3741496598639	0.089390429771784 \\
35.7142857142857	0.08776181606686 \\
36.0544217687075	0.0876574418606637 \\
36.3945578231292	0.0858967945869734 \\
36.734693877551	0.0856846394215731 \\
37.0748299319728	0.0844462037370325 \\
37.4149659863946	0.0829515037829295 \\
37.7551020408163	0.0833684091681517 \\
38.0952380952381	0.0793068018107462 \\
38.4353741496599	0.0784240524465426 \\
38.7755102040816	0.0778660390820778 \\
39.1156462585034	0.075796397912747 \\
39.4557823129252	0.0749631733025805 \\
39.7959183673469	0.0732207921367572 \\
40.1360544217687	0.0716390739076618 \\
40.4761904761905	0.0690900583795674 \\
40.8163265306122	0.0665587131870335 \\
41.156462585034	0.0627732304665782 \\
41.4965986394558	0.0614326773867379 \\
41.8367346938776	0.0595399486371464 \\
42.1768707482993	0.0580478563296574 \\
42.5170068027211	0.0543002115411441 \\
42.8571428571429	0.0524684893780797 \\
43.1972789115646	0.0503039583135456 \\
43.5374149659864	0.0489445724542701 \\
43.8775510204082	0.0464974687936018 \\
44.2176870748299	0.0447772681698652 \\
44.5578231292517	0.0433375980832042 \\
44.8979591836735	0.0405641530502909 \\
45.2380952380952	0.0389941173401443 \\
45.578231292517	0.0384710302473315 \\
45.9183673469388	0.0373966073737134 \\
46.2585034013605	0.0365549484819609 \\
46.5986394557823	0.0354126263656346 \\
46.9387755102041	0.0351313715672182 \\
47.2789115646259	0.0340505550940442 \\
47.6190476190476	0.0332306321750389 \\
47.9591836734694	0.0317117839415127 \\
48.2993197278912	0.031238864995122 \\
48.6394557823129	0.0302836395706156 \\
48.9795918367347	0.0296236453256647 \\
49.3197278911565	0.0289301174237265 \\
49.6598639455782	0.0287761661602529 \\
50	0.0283444564327029 \\
50.3401360544218	0.0272555637837612 \\
50.6802721088435	0.0271265476963758 \\
51.0204081632653	0.0257266559431871 \\
51.3605442176871	0.0244548788339686 \\
51.7006802721088	0.0248429540532638 \\
52.0408163265306	0.0236152814447962 \\
52.3809523809524	0.0229661117418892 \\
52.7210884353741	0.0223246097567568 \\
53.0612244897959	0.0219672844389092 \\
53.4013605442177	0.0206545057945603 \\
53.7414965986395	0.0209179214379129 \\
54.0816326530612	0.0207214243370728 \\
54.421768707483	0.0204320911522032 \\
54.7619047619048	0.0202781128580713 \\
55.1020408163265	0.0196464614521271 \\
55.4421768707483	0.0193945879805192 \\
55.7823129251701	0.0173946992668865 \\
56.1224489795918	0.0168151073419706 \\
56.4625850340136	0.0163212902792566 \\
56.8027210884354	0.0155824769119145 \\
57.1428571428571	0.0152274157001989 \\
57.4829931972789	0.0144318400051729 \\
57.8231292517007	0.0142424253989103 \\
58.1632653061224	0.0145079520256444 \\
58.5034013605442	0.013550511104358 \\
58.843537414966	0.0126445525682312 \\
59.1836734693878	0.0119939739492353 \\
59.5238095238095	0.0107913605636783 \\
59.8639455782313	0.00955168191710884 \\
60.2040816326531	0.00965879180554436 \\
60.5442176870748	0.00946363899458264 \\
60.8843537414966	0.00941766507797659 \\
61.2244897959184	0.0083577717753168 \\
61.5646258503401	0.00879068335766955 \\
61.9047619047619	0.00793899893037477 \\
62.2448979591837	0.00746528377039014 \\
62.5850340136054	0.00652694498405975 \\
62.9251700680272	0.00641721462672788 \\
63.265306122449	0.00667693069101962 \\
63.6054421768707	0.00570696896877519 \\
63.9455782312925	0.00559627146964638 \\
64.2857142857143	0.00531015858785071 \\
64.6258503401361	0.00466421784753149 \\
64.9659863945578	0.0049491485891783 \\
65.3061224489796	0.00518012873918594 \\
65.6462585034014	0.00532122711167791 \\
65.9863945578231	0.00504763881778734 \\
66.3265306122449	0.00472316675975792 \\
66.6666666666667	0.00449316276858485 \\
67.0068027210884	0.00398653210154241 \\
67.3469387755102	0.00360803916795319 \\
67.687074829932	0.00331530584509705 \\
68.0272108843537	0.0031130734699462 \\
68.3673469387755	0.0030147933436383 \\
68.7074829931973	0.00274141695009134 \\
69.0476190476191	0.00262303347360308 \\
69.3877551020408	0.00242772872814882 \\
69.7278911564626	0.00229022903951545 \\
70.0680272108844	0.00215961522727256 \\
70.4081632653061	0.00210952060937807 \\
70.7482993197279	0.00235669217239145 \\
71.0884353741497	0.00222871416109375 \\
71.4285714285714	0.00237148529883419 \\
71.7687074829932	0.00266265337713841 \\
72.108843537415	0.00267857630239459 \\
72.4489795918367	0.0028978314803571 \\
72.7891156462585	0.00279231248295745 \\
73.1292517006803	0.00288799773458983 \\
73.469387755102	0.00306107105499677 \\
73.8095238095238	0.00332219977090583 \\
74.1496598639456	0.00322841250141242 \\
74.4897959183673	0.00318646496875987 \\
74.8299319727891	0.00317436604904182 \\
75.1700680272109	0.0032128363920112 \\
75.5102040816327	0.00310498741178219 \\
75.8503401360544	0.00331233592649538 \\
76.1904761904762	0.00327835979922347 \\
76.530612244898	0.00334515317501935 \\
76.8707482993197	0.00347922287298974 \\
77.2108843537415	0.00337662402484209 \\
77.5510204081633	0.00339487790972484 \\
77.891156462585	0.00338237775383038 \\
78.2312925170068	0.00334308509289683 \\
78.5714285714286	0.00326140190687466 \\
78.9115646258503	0.0032391108222791 \\
79.2517006802721	0.0031850501967123 \\
79.5918367346939	0.00304926632880263 \\
79.9319727891156	0.00309826979006398 \\
80.2721088435374	0.00289595184457994 \\
80.6122448979592	0.00295189872421433 \\
80.9523809523809	0.00318395019600736 \\
81.2925170068027	0.00326894628925242 \\
81.6326530612245	0.00358583738502142 \\
81.9727891156463	0.00346597591897895 \\
82.312925170068	0.00337402313802757 \\
82.6530612244898	0.0030014043112866 \\
82.9931972789116	0.00286274709627395 \\
83.3333333333333	0.0024692526000824 \\
83.6734693877551	0.00246765169687012 \\
84.0136054421769	0.00237424704018917 \\
84.3537414965986	0.00246386809955067 \\
84.6938775510204	0.00230674601899764 \\
85.0340136054422	0.00186682495866448 \\
85.3741496598639	0.00173104109094842 \\
85.7142857142857	0.00176606499514611 \\
86.0544217687075	0.00173705157231213 \\
86.3945578231292	0.00171219529971138 \\
86.734693877551	0.00176280777884208 \\
87.0748299319728	0.00181210704853102 \\
87.4149659863945	0.00179417327577552 \\
87.7551020408163	0.00180116762980246 \\
88.0952380952381	0.00184514895255695 \\
88.4353741496599	0.00172076002324081 \\
88.7755102040816	0.00191771258074259 \\
89.1156462585034	0.0020307729733542 \\
89.4557823129252	0.00202166323961088 \\
89.7959183673469	0.00195708057247313 \\
90.1360544217687	0.00208723571746064 \\
90.4761904761905	0.00201659819691725 \\
90.8163265306122	0.00222858728394307 \\
91.156462585034	0.00224133042698865 \\
91.4965986394558	0.00229269072107515 \\
91.8367346938775	0.00213343661856063 \\
92.1768707482993	0.00208990323271484 \\
92.5170068027211	0.00212010910531087 \\
92.8571428571429	0.00211338823621595 \\
93.1972789115646	0.00199623618150756 \\
93.5374149659864	0.00186885112084121 \\
93.8775510204082	0.00180545088616874 \\
94.2176870748299	0.00180732301500877 \\
94.5578231292517	0.00165392449086663 \\
94.8979591836735	0.00149443508357493 \\
95.2380952380952	0.00125991615998293 \\
95.578231292517	0.00113003874902164 \\
95.9183673469388	0.000880315050292868 \\
96.2585034013605	0.000877526102593911 \\
96.5986394557823	0.000893179454574182 \\
96.9387755102041	0.00089368628208055 \\
97.2789115646258	0.000844973898783359 \\
97.6190476190476	0.00070511006233446 \\
97.9591836734694	0.000574635353746116 \\
98.2993197278912	0.000443333467806939 \\
98.6394557823129	0.000331225613453687 \\
98.9795918367347	0.000297335186760759 \\
99.3197278911565	0.00016080666555188 \\
99.6598639455782	4.36321318590371e-05 \\
100	1.49018575257287e-13 \\
};
\path [fill=color1, fill opacity=0.5] (axis cs:0,0.720468087377886)
--(axis cs:0,0.716694608149191)
--(axis cs:0.340136054421769,0.720902294433428)
--(axis cs:0.680272108843537,0.71773166941655)
--(axis cs:1.02040816326531,0.71321057692811)
--(axis cs:1.36054421768707,0.698683785998627)
--(axis cs:1.70068027210884,0.678580796416726)
--(axis cs:2.04081632653061,0.659829792354404)
--(axis cs:2.38095238095238,0.645585611795098)
--(axis cs:2.72108843537415,0.629462671717288)
--(axis cs:3.06122448979592,0.612970421550694)
--(axis cs:3.40136054421769,0.599353905647548)
--(axis cs:3.74149659863946,0.578031304195733)
--(axis cs:4.08163265306122,0.566514822704971)
--(axis cs:4.42176870748299,0.552218466067708)
--(axis cs:4.76190476190476,0.53133802937242)
--(axis cs:5.10204081632653,0.51237379850697)
--(axis cs:5.4421768707483,0.497182050779916)
--(axis cs:5.78231292517007,0.48201101445345)
--(axis cs:6.12244897959184,0.470236230698593)
--(axis cs:6.46258503401361,0.458337442692819)
--(axis cs:6.80272108843537,0.440571614119872)
--(axis cs:7.14285714285714,0.426867775540201)
--(axis cs:7.48299319727891,0.413169191506399)
--(axis cs:7.82312925170068,0.404130967335811)
--(axis cs:8.16326530612245,0.396713491352104)
--(axis cs:8.50340136054422,0.385197893461261)
--(axis cs:8.84353741496599,0.378190655289832)
--(axis cs:9.18367346938775,0.370687309023556)
--(axis cs:9.52380952380952,0.359092822860935)
--(axis cs:9.86394557823129,0.350653825139628)
--(axis cs:10.2040816326531,0.341164413188144)
--(axis cs:10.5442176870748,0.336534461592088)
--(axis cs:10.8843537414966,0.327768617818466)
--(axis cs:11.2244897959184,0.319124676569184)
--(axis cs:11.5646258503401,0.312172297086261)
--(axis cs:11.9047619047619,0.306972444662757)
--(axis cs:12.2448979591837,0.300179544730519)
--(axis cs:12.5850340136054,0.29867007175719)
--(axis cs:12.9251700680272,0.294079019025468)
--(axis cs:13.265306122449,0.289214890947547)
--(axis cs:13.6054421768707,0.28590362785717)
--(axis cs:13.9455782312925,0.285334624574883)
--(axis cs:14.2857142857143,0.281300948323239)
--(axis cs:14.6258503401361,0.27741421760315)
--(axis cs:14.9659863945578,0.271212546121182)
--(axis cs:15.3061224489796,0.266029049209395)
--(axis cs:15.6462585034014,0.263261232657688)
--(axis cs:15.9863945578231,0.259271956676976)
--(axis cs:16.3265306122449,0.253718856967914)
--(axis cs:16.6666666666667,0.249575399826394)
--(axis cs:17.0068027210884,0.24647796936986)
--(axis cs:17.3469387755102,0.24177416720868)
--(axis cs:17.687074829932,0.234274224739898)
--(axis cs:18.0272108843537,0.230517042616161)
--(axis cs:18.3673469387755,0.224238427098259)
--(axis cs:18.7074829931973,0.220231945544845)
--(axis cs:19.047619047619,0.215220432991021)
--(axis cs:19.3877551020408,0.21366953848759)
--(axis cs:19.7278911564626,0.209534599282585)
--(axis cs:20.0680272108844,0.205561214144488)
--(axis cs:20.4081632653061,0.200982494487843)
--(axis cs:20.7482993197279,0.197004094110351)
--(axis cs:21.0884353741497,0.195280123491462)
--(axis cs:21.4285714285714,0.192338014630159)
--(axis cs:21.7687074829932,0.19028701322417)
--(axis cs:22.108843537415,0.185492661001624)
--(axis cs:22.4489795918367,0.183202663706006)
--(axis cs:22.7891156462585,0.177416649193837)
--(axis cs:23.1292517006803,0.173524749242619)
--(axis cs:23.469387755102,0.168042717211115)
--(axis cs:23.8095238095238,0.165350813039612)
--(axis cs:24.1496598639456,0.160864298835849)
--(axis cs:24.4897959183673,0.157989199628104)
--(axis cs:24.8299319727891,0.15548447281132)
--(axis cs:25.1700680272109,0.151045356060824)
--(axis cs:25.5102040816327,0.149466047193121)
--(axis cs:25.8503401360544,0.147481382489229)
--(axis cs:26.1904761904762,0.144598574113377)
--(axis cs:26.530612244898,0.142773398511395)
--(axis cs:26.8707482993197,0.141109391986409)
--(axis cs:27.2108843537415,0.137503432172052)
--(axis cs:27.5510204081633,0.134415701074651)
--(axis cs:27.891156462585,0.132007381452742)
--(axis cs:28.2312925170068,0.131597576743835)
--(axis cs:28.5714285714286,0.130877073762562)
--(axis cs:28.9115646258503,0.129660823897349)
--(axis cs:29.2517006802721,0.129009989364822)
--(axis cs:29.5918367346939,0.125067030083406)
--(axis cs:29.9319727891156,0.122930556270223)
--(axis cs:30.2721088435374,0.12198505770042)
--(axis cs:30.6122448979592,0.121186901716487)
--(axis cs:30.952380952381,0.1183049372921)
--(axis cs:31.2925170068027,0.11701782934124)
--(axis cs:31.6326530612245,0.117266328840989)
--(axis cs:31.9727891156463,0.115375321906322)
--(axis cs:32.312925170068,0.113171091884095)
--(axis cs:32.6530612244898,0.109844106780198)
--(axis cs:32.9931972789116,0.108138730398363)
--(axis cs:33.3333333333333,0.104814985232948)
--(axis cs:33.6734693877551,0.102325300374683)
--(axis cs:34.0136054421769,0.0993902036663385)
--(axis cs:34.3537414965986,0.0972483427408417)
--(axis cs:34.6938775510204,0.0935854820892428)
--(axis cs:35.0340136054422,0.0913802203770783)
--(axis cs:35.3741496598639,0.0863837274731769)
--(axis cs:35.7142857142857,0.0846419878864649)
--(axis cs:36.0544217687075,0.0846794665553156)
--(axis cs:36.3945578231292,0.0829795102425716)
--(axis cs:36.734693877551,0.0827609850454949)
--(axis cs:37.0748299319728,0.0813691802150712)
--(axis cs:37.4149659863946,0.0800382014891334)
--(axis cs:37.7551020408163,0.080431080407566)
--(axis cs:38.0952380952381,0.0765114609136317)
--(axis cs:38.4353741496599,0.0755336089375848)
--(axis cs:38.7755102040816,0.075064547430212)
--(axis cs:39.1156462585034,0.0730793995599832)
--(axis cs:39.4557823129252,0.0721749872522714)
--(axis cs:39.7959183673469,0.0704771635242228)
--(axis cs:40.1360544217687,0.06902967009306)
--(axis cs:40.4761904761905,0.0664527503281693)
--(axis cs:40.8163265306122,0.0639615997459993)
--(axis cs:41.156462585034,0.0603009077660417)
--(axis cs:41.4965986394558,0.0589895676398426)
--(axis cs:41.8367346938776,0.0571779203063773)
--(axis cs:42.1768707482993,0.0557961331851086)
--(axis cs:42.5170068027211,0.0521795471855629)
--(axis cs:42.8571428571429,0.0503628231618695)
--(axis cs:43.1972789115646,0.0483689239555905)
--(axis cs:43.5374149659864,0.0468978950214257)
--(axis cs:43.8775510204082,0.044466016877129)
--(axis cs:44.2176870748299,0.0428506454345719)
--(axis cs:44.5578231292517,0.0414677691738644)
--(axis cs:44.8979591836735,0.0387052884686316)
--(axis cs:45.2380952380952,0.0372416487724589)
--(axis cs:45.578231292517,0.0366787986976339)
--(axis cs:45.9183673469388,0.03567129015768)
--(axis cs:46.2585034013605,0.0348634280545578)
--(axis cs:46.5986394557823,0.033768414574966)
--(axis cs:46.9387755102041,0.0334463900091429)
--(axis cs:47.2789115646259,0.0323965081166736)
--(axis cs:47.6190476190476,0.0316018483397368)
--(axis cs:47.9591836734694,0.030068871001729)
--(axis cs:48.2993197278912,0.0296142887478346)
--(axis cs:48.6394557823129,0.0286252610114096)
--(axis cs:48.9795918367347,0.0280542941800932)
--(axis cs:49.3197278911565,0.0272625751738352)
--(axis cs:49.6598639455782,0.027241490112332)
--(axis cs:50,0.0268463698656114)
--(axis cs:50.3401360544218,0.0257634564908467)
--(axis cs:50.6802721088435,0.0255116539142331)
--(axis cs:51.0204081632653,0.0242262163787996)
--(axis cs:51.3605442176871,0.0228574093756732)
--(axis cs:51.7006802721088,0.0233755386597595)
--(axis cs:52.0408163265306,0.0220280861393119)
--(axis cs:52.3809523809524,0.0214296398089847)
--(axis cs:52.7210884353741,0.0206892492280177)
--(axis cs:53.0612244897959,0.0205071967293193)
--(axis cs:53.4013605442177,0.0190970047496294)
--(axis cs:53.7414965986395,0.0193997460278127)
--(axis cs:54.0816326530612,0.0192210599910451)
--(axis cs:54.421768707483,0.0189231381714817)
--(axis cs:54.7619047619048,0.0188017128203886)
--(axis cs:55.1020408163265,0.018145720340653)
--(axis cs:55.4421768707483,0.0179475782694438)
--(axis cs:55.7823129251701,0.015998362117263)
--(axis cs:56.1224489795918,0.0153420810878383)
--(axis cs:56.4625850340136,0.0149406645348553)
--(axis cs:56.8027210884354,0.0140373832047797)
--(axis cs:57.1428571428571,0.0138092023407151)
--(axis cs:57.4829931972789,0.0131608454977442)
--(axis cs:57.8231292517007,0.01293233571488)
--(axis cs:58.1632653061224,0.0130818887080284)
--(axis cs:58.5034013605442,0.0122801803959985)
--(axis cs:58.843537414966,0.0112873109868669)
--(axis cs:59.1836734693878,0.0107456079613927)
--(axis cs:59.5238095238095,0.00960628450159052)
--(axis cs:59.8639455782313,0.0083188448562946)
--(axis cs:60.2040816326531,0.00851787889659693)
--(axis cs:60.5442176870748,0.00836125364753115)
--(axis cs:60.8843537414966,0.00822218020146008)
--(axis cs:61.2244897959184,0.00717705971645267)
--(axis cs:61.5646258503401,0.00769537253142253)
--(axis cs:61.9047619047619,0.00684474771544505)
--(axis cs:62.2448979591837,0.00645016776548152)
--(axis cs:62.5850340136054,0.00563519100832926)
--(axis cs:62.9251700680272,0.00555305287186807)
--(axis cs:63.265306122449,0.00586215224138155)
--(axis cs:63.6054421768707,0.00485590586595909)
--(axis cs:63.9455782312925,0.00487408740155544)
--(axis cs:64.2857142857143,0.0045713161116901)
--(axis cs:64.6258503401361,0.00401182504336242)
--(axis cs:64.9659863945578,0.00425266877614662)
--(axis cs:65.3061224489796,0.00447541917302712)
--(axis cs:65.6462585034014,0.00466260894244572)
--(axis cs:65.9863945578231,0.00439705079505952)
--(axis cs:66.3265306122449,0.00412140936221168)
--(axis cs:66.6666666666667,0.00390264798217832)
--(axis cs:67.0068027210884,0.00344411554458921)
--(axis cs:67.3469387755102,0.00307073051637608)
--(axis cs:67.687074829932,0.00284538334812653)
--(axis cs:68.0272108843537,0.00266237706932805)
--(axis cs:68.3673469387755,0.00251890712069386)
--(axis cs:68.7074829931973,0.00234608632369558)
--(axis cs:69.0476190476191,0.002222836582435)
--(axis cs:69.3877551020408,0.00207023332028826)
--(axis cs:69.7278911564626,0.00194272202999954)
--(axis cs:70.0680272108844,0.00179709272097377)
--(axis cs:70.4081632653061,0.00177342325642118)
--(axis cs:70.7482993197279,0.00198292175408235)
--(axis cs:71.0884353741497,0.00188569353497244)
--(axis cs:71.4285714285714,0.00194085443606847)
--(axis cs:71.7687074829932,0.00223807319190225)
--(axis cs:72.108843537415,0.00227105945724535)
--(axis cs:72.4489795918367,0.00246334468774039)
--(axis cs:72.7891156462585,0.00241353944511421)
--(axis cs:73.1292517006803,0.00256200093025203)
--(axis cs:73.469387755102,0.00271772475809803)
--(axis cs:73.8095238095238,0.00296884109488124)
--(axis cs:74.1496598639456,0.00285753479245228)
--(axis cs:74.4897959183673,0.00285571787491868)
--(axis cs:74.8299319727891,0.00281675968995473)
--(axis cs:75.1700680272109,0.00289039991636763)
--(axis cs:75.5102040816327,0.00280865807202551)
--(axis cs:75.8503401360544,0.00301048681938747)
--(axis cs:76.1904761904762,0.00296662960162847)
--(axis cs:76.530612244898,0.003038379480551)
--(axis cs:76.8707482993197,0.00319328586383649)
--(axis cs:77.2108843537415,0.0030874376839982)
--(axis cs:77.5510204081633,0.00309191313839961)
--(axis cs:77.891156462585,0.0030804570163696)
--(axis cs:78.2312925170068,0.00304213676400345)
--(axis cs:78.5714285714286,0.00297558307071684)
--(axis cs:78.9115646258503,0.00294845369286447)
--(axis cs:79.2517006802721,0.00290958998963205)
--(axis cs:79.5918367346939,0.00279579942686094)
--(axis cs:79.9319727891156,0.00284409830993113)
--(axis cs:80.2721088435374,0.00266690034458566)
--(axis cs:80.6122448979592,0.00268150390695026)
--(axis cs:80.9523809523809,0.0028994329448692)
--(axis cs:81.2925170068027,0.00298877055618939)
--(axis cs:81.6326530612245,0.00325598241999559)
--(axis cs:81.9727891156463,0.00316932098700459)
--(axis cs:82.312925170068,0.00307945415526965)
--(axis cs:82.6530612244898,0.00276114414635229)
--(axis cs:82.9931972789116,0.00263262360559002)
--(axis cs:83.3333333333333,0.00224084492063622)
--(axis cs:83.6734693877551,0.00228685541093635)
--(axis cs:84.0136054421769,0.00220178014797768)
--(axis cs:84.3537414965986,0.00228490883876326)
--(axis cs:84.6938775510204,0.00214550884107364)
--(axis cs:85.0340136054422,0.00173485042169085)
--(axis cs:85.3741496598639,0.00159961718414744)
--(axis cs:85.7142857142857,0.0016389219302227)
--(axis cs:86.0544217687075,0.00161545318011919)
--(axis cs:86.3945578231292,0.00159110599571485)
--(axis cs:86.734693877551,0.00162998206202665)
--(axis cs:87.0748299319728,0.00165797660662732)
--(axis cs:87.4149659863945,0.0016434025007134)
--(axis cs:87.7551020408163,0.00164721354167901)
--(axis cs:88.0952380952381,0.00168526181595402)
--(axis cs:88.4353741496599,0.00157119682667857)
--(axis cs:88.7755102040816,0.0017609224641365)
--(axis cs:89.1156462585034,0.00188173451250867)
--(axis cs:89.4557823129252,0.00187264702741453)
--(axis cs:89.7959183673469,0.00180675184457499)
--(axis cs:90.1360544217687,0.00191358847045672)
--(axis cs:90.4761904761905,0.00184533598113991)
--(axis cs:90.8163265306122,0.00204220441768186)
--(axis cs:91.156462585034,0.00205807778852241)
--(axis cs:91.4965986394558,0.00207616058600618)
--(axis cs:91.8367346938775,0.00193372925184951)
--(axis cs:92.1768707482993,0.0018949452403809)
--(axis cs:92.5170068027211,0.00190352255488641)
--(axis cs:92.8571428571429,0.00187845671308322)
--(axis cs:93.1972789115646,0.00177702405066531)
--(axis cs:93.5374149659864,0.00165502597036836)
--(axis cs:93.8775510204082,0.00160139986524128)
--(axis cs:94.2176870748299,0.0016122900326402)
--(axis cs:94.5578231292517,0.00147155668288597)
--(axis cs:94.8979591836735,0.00131483806343531)
--(axis cs:95.2380952380952,0.00110920741975931)
--(axis cs:95.578231292517,0.000997202815189409)
--(axis cs:95.9183673469388,0.000786071336421478)
--(axis cs:96.2585034013605,0.000776257963992084)
--(axis cs:96.5986394557823,0.000804760181587743)
--(axis cs:96.9387755102041,0.000819406650214067)
--(axis cs:97.2789115646258,0.000761333241659368)
--(axis cs:97.6190476190476,0.000619599869064433)
--(axis cs:97.9591836734694,0.000510237979961982)
--(axis cs:98.2993197278912,0.000385886694021519)
--(axis cs:98.6394557823129,0.00028206856255203)
--(axis cs:98.9795918367347,0.000249989569538343)
--(axis cs:99.3197278911565,0.000135274507845721)
--(axis cs:99.6598639455782,3.7721891479757e-05)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,4.95423722383173e-05)
--(axis cs:99.3197278911565,0.00018633882325804)
--(axis cs:98.9795918367347,0.000344680803983175)
--(axis cs:98.6394557823129,0.000380382664355345)
--(axis cs:98.2993197278912,0.000500780241592359)
--(axis cs:97.9591836734694,0.000639032727530249)
--(axis cs:97.6190476190476,0.000790620255604487)
--(axis cs:97.2789115646258,0.00092861455590735)
--(axis cs:96.9387755102041,0.000967965913947033)
--(axis cs:96.5986394557823,0.000981598727560622)
--(axis cs:96.2585034013605,0.000978794241195737)
--(axis cs:95.9183673469388,0.000974558764164258)
--(axis cs:95.578231292517,0.00126287468285388)
--(axis cs:95.2380952380952,0.00141062490020654)
--(axis cs:94.8979591836735,0.00167403210371454)
--(axis cs:94.5578231292517,0.00183629229884728)
--(axis cs:94.2176870748299,0.00200235599737735)
--(axis cs:93.8775510204082,0.00200950190709619)
--(axis cs:93.5374149659864,0.00208267627131406)
--(axis cs:93.1972789115646,0.00221544831234982)
--(axis cs:92.8571428571429,0.00234831975934869)
--(axis cs:92.5170068027211,0.00233669565573534)
--(axis cs:92.1768707482993,0.00228486122504877)
--(axis cs:91.8367346938775,0.00233314398527175)
--(axis cs:91.4965986394558,0.00250922085614412)
--(axis cs:91.156462585034,0.00242458306545489)
--(axis cs:90.8163265306122,0.00241497015020428)
--(axis cs:90.4761904761905,0.00218786041269459)
--(axis cs:90.1360544217687,0.00226088296446456)
--(axis cs:89.7959183673469,0.00210740930037127)
--(axis cs:89.4557823129252,0.00217067945180723)
--(axis cs:89.1156462585034,0.00217981143419972)
--(axis cs:88.7755102040816,0.00207450269734867)
--(axis cs:88.4353741496599,0.00187032321980304)
--(axis cs:88.0952380952381,0.00200503608915987)
--(axis cs:87.7551020408163,0.0019551217179259)
--(axis cs:87.4149659863945,0.00194494405083764)
--(axis cs:87.0748299319728,0.00196623749043471)
--(axis cs:86.734693877551,0.00189563349565751)
--(axis cs:86.3945578231292,0.00183328460370791)
--(axis cs:86.0544217687075,0.00185864996450507)
--(axis cs:85.7142857142857,0.00189320806006952)
--(axis cs:85.3741496598639,0.00186246499774941)
--(axis cs:85.0340136054422,0.00199879949563811)
--(axis cs:84.6938775510204,0.00246798319692164)
--(axis cs:84.3537414965986,0.00264282736033809)
--(axis cs:84.0136054421769,0.00254671393240066)
--(axis cs:83.6734693877551,0.0026484479828039)
--(axis cs:83.3333333333333,0.00269766027952859)
--(axis cs:82.9931972789116,0.00309287058695788)
--(axis cs:82.6530612244898,0.00324166447622092)
--(axis cs:82.312925170068,0.0036685921207855)
--(axis cs:81.9727891156463,0.00376263085095332)
--(axis cs:81.6326530612245,0.00391569235004725)
--(axis cs:81.2925170068027,0.00354912202231545)
--(axis cs:80.9523809523809,0.00346846744714552)
--(axis cs:80.6122448979592,0.00322229354147839)
--(axis cs:80.2721088435374,0.00312500334457421)
--(axis cs:79.9319727891156,0.00335244127019682)
--(axis cs:79.5918367346939,0.00330273323074433)
--(axis cs:79.2517006802721,0.00346051040379255)
--(axis cs:78.9115646258503,0.00352976795169373)
--(axis cs:78.5714285714286,0.00354722074303247)
--(axis cs:78.2312925170068,0.00364403342179022)
--(axis cs:77.891156462585,0.00368429849129116)
--(axis cs:77.5510204081633,0.00369784268105006)
--(axis cs:77.2108843537415,0.00366581036568598)
--(axis cs:76.8707482993197,0.003765159882143)
--(axis cs:76.530612244898,0.00365192686948771)
--(axis cs:76.1904761904762,0.00359008999681847)
--(axis cs:75.8503401360544,0.00361418503360328)
--(axis cs:75.5102040816327,0.00340131675153886)
--(axis cs:75.1700680272109,0.00353527286765477)
--(axis cs:74.8299319727891,0.00353197240812892)
--(axis cs:74.4897959183673,0.00351721206260106)
--(axis cs:74.1496598639456,0.00359929021037256)
--(axis cs:73.8095238095238,0.00367555844693041)
--(axis cs:73.469387755102,0.00340441735189551)
--(axis cs:73.1292517006803,0.00321399453892763)
--(axis cs:72.7891156462585,0.00317108552080069)
--(axis cs:72.4489795918367,0.00333231827297381)
--(axis cs:72.108843537415,0.00308609314754384)
--(axis cs:71.7687074829932,0.00308723356237457)
--(axis cs:71.4285714285714,0.0028021161615999)
--(axis cs:71.0884353741497,0.00257173478721507)
--(axis cs:70.7482993197279,0.00273046259070056)
--(axis cs:70.4081632653061,0.00244561796233495)
--(axis cs:70.0680272108844,0.00252213773357135)
--(axis cs:69.7278911564626,0.00263773604903136)
--(axis cs:69.3877551020408,0.00278522413600939)
--(axis cs:69.0476190476191,0.00302323036477116)
--(axis cs:68.7074829931973,0.0031367475764871)
--(axis cs:68.3673469387755,0.00351067956658275)
--(axis cs:68.0272108843537,0.00356376987056435)
--(axis cs:67.687074829932,0.00378522834206758)
--(axis cs:67.3469387755102,0.00414534781953029)
--(axis cs:67.0068027210884,0.00452894865849561)
--(axis cs:66.6666666666667,0.00508367755499138)
--(axis cs:66.3265306122449,0.00532492415730415)
--(axis cs:65.9863945578231,0.00569822684051515)
--(axis cs:65.6462585034014,0.00597984528091011)
--(axis cs:65.3061224489796,0.00588483830534476)
--(axis cs:64.9659863945578,0.00564562840220998)
--(axis cs:64.6258503401361,0.00531661065170056)
--(axis cs:64.2857142857143,0.00604900106401132)
--(axis cs:63.9455782312925,0.00631845553773732)
--(axis cs:63.6054421768707,0.0065580320715913)
--(axis cs:63.265306122449,0.00749170914065768)
--(axis cs:62.9251700680272,0.0072813763815877)
--(axis cs:62.5850340136054,0.00741869895979024)
--(axis cs:62.2448979591837,0.00848039977529875)
--(axis cs:61.9047619047619,0.00903325014530449)
--(axis cs:61.5646258503401,0.00988599418391657)
--(axis cs:61.2244897959184,0.00953848383418092)
--(axis cs:60.8843537414966,0.0106131499544931)
--(axis cs:60.5442176870748,0.0105660243416341)
--(axis cs:60.2040816326531,0.0107997047144918)
--(axis cs:59.8639455782313,0.0107845189779231)
--(axis cs:59.5238095238095,0.011976436625766)
--(axis cs:59.1836734693878,0.0132423399370779)
--(axis cs:58.843537414966,0.0140017941495954)
--(axis cs:58.5034013605442,0.0148208418127174)
--(axis cs:58.1632653061224,0.0159340153432604)
--(axis cs:57.8231292517007,0.0155525150829405)
--(axis cs:57.4829931972789,0.0157028345126017)
--(axis cs:57.1428571428571,0.0166456290596828)
--(axis cs:56.8027210884354,0.0171275706190494)
--(axis cs:56.4625850340136,0.0177019160236579)
--(axis cs:56.1224489795918,0.0182881335961029)
--(axis cs:55.7823129251701,0.01879103641651)
--(axis cs:55.4421768707483,0.0208415976915946)
--(axis cs:55.1020408163265,0.0211472025636012)
--(axis cs:54.7619047619048,0.0217545128957539)
--(axis cs:54.421768707483,0.0219410441329247)
--(axis cs:54.0816326530612,0.0222217886831004)
--(axis cs:53.7414965986395,0.022436096848013)
--(axis cs:53.4013605442177,0.0222120068394913)
--(axis cs:53.0612244897959,0.0234273721484992)
--(axis cs:52.7210884353741,0.0239599702854959)
--(axis cs:52.3809523809524,0.0245025836747937)
--(axis cs:52.0408163265306,0.0252024767502806)
--(axis cs:51.7006802721088,0.026310369446768)
--(axis cs:51.3605442176871,0.026052348292264)
--(axis cs:51.0204081632653,0.0272270955075745)
--(axis cs:50.6802721088435,0.0287414414785185)
--(axis cs:50.3401360544218,0.0287476710766756)
--(axis cs:50,0.0298425429997945)
--(axis cs:49.6598639455782,0.0303108422081738)
--(axis cs:49.3197278911565,0.0305976596736178)
--(axis cs:48.9795918367347,0.0311929964712363)
--(axis cs:48.6394557823129,0.0319420181298217)
--(axis cs:48.2993197278912,0.0328634412424094)
--(axis cs:47.9591836734694,0.0333546968812965)
--(axis cs:47.6190476190476,0.0348594160103411)
--(axis cs:47.2789115646259,0.0357046020714148)
--(axis cs:46.9387755102041,0.0368163531252934)
--(axis cs:46.5986394557823,0.0370568381563031)
--(axis cs:46.2585034013605,0.0382464689093641)
--(axis cs:45.9183673469388,0.0391219245897467)
--(axis cs:45.578231292517,0.0402632617970292)
--(axis cs:45.2380952380952,0.0407465859078296)
--(axis cs:44.8979591836735,0.0424230176319501)
--(axis cs:44.5578231292517,0.0452074269925441)
--(axis cs:44.2176870748299,0.0467038909051584)
--(axis cs:43.8775510204082,0.0485289207100745)
--(axis cs:43.5374149659864,0.0509912498871146)
--(axis cs:43.1972789115646,0.0522389926715007)
--(axis cs:42.8571428571429,0.05457415559429)
--(axis cs:42.5170068027211,0.0564208758967254)
--(axis cs:42.1768707482993,0.0602995794742063)
--(axis cs:41.8367346938776,0.0619019769679156)
--(axis cs:41.4965986394558,0.0638757871336332)
--(axis cs:41.156462585034,0.0652455531671148)
--(axis cs:40.8163265306122,0.0691558266280677)
--(axis cs:40.4761904761905,0.0717273664309654)
--(axis cs:40.1360544217687,0.0742484777222636)
--(axis cs:39.7959183673469,0.0759644207492915)
--(axis cs:39.4557823129252,0.0777513593528896)
--(axis cs:39.1156462585034,0.0785133962655108)
--(axis cs:38.7755102040816,0.0806675307339436)
--(axis cs:38.4353741496599,0.0813144959555005)
--(axis cs:38.0952380952381,0.0821021427078607)
--(axis cs:37.7551020408163,0.0863057379287374)
--(axis cs:37.4149659863946,0.0858648060767256)
--(axis cs:37.0748299319728,0.0875232272589938)
--(axis cs:36.734693877551,0.0886082937976514)
--(axis cs:36.3945578231292,0.0888140789313752)
--(axis cs:36.0544217687075,0.0906354171660118)
--(axis cs:35.7142857142857,0.090881644247255)
--(axis cs:35.3741496598639,0.092397132070391)
--(axis cs:35.0340136054422,0.0975900071478908)
--(axis cs:34.6938775510204,0.0997008099946438)
--(axis cs:34.3537414965986,0.103820152467655)
--(axis cs:34.0136054421769,0.106259213142017)
--(axis cs:33.6734693877551,0.109184958547633)
--(axis cs:33.3333333333333,0.11145256931622)
--(axis cs:32.9931972789116,0.115128651760821)
--(axis cs:32.6530612244898,0.116945298156171)
--(axis cs:32.312925170068,0.12049892470062)
--(axis cs:31.9727891156463,0.122669123192204)
--(axis cs:31.6326530612245,0.12459892896285)
--(axis cs:31.2925170068027,0.124109121784395)
--(axis cs:30.952380952381,0.125397936229534)
--(axis cs:30.6122448979592,0.128051654066665)
--(axis cs:30.2721088435374,0.129082561467452)
--(axis cs:29.9319727891156,0.129912957136708)
--(axis cs:29.5918367346939,0.132113523098254)
--(axis cs:29.2517006802721,0.136027340008849)
--(axis cs:28.9115646258503,0.136551360092149)
--(axis cs:28.5714285714286,0.137654852894005)
--(axis cs:28.2312925170068,0.138518177741511)
--(axis cs:27.891156462585,0.139071643022924)
--(axis cs:27.5510204081633,0.141341960571378)
--(axis cs:27.2108843537415,0.144485550919209)
--(axis cs:26.8707482993197,0.14795521483126)
--(axis cs:26.530612244898,0.149676919617951)
--(axis cs:26.1904761904762,0.151283775635658)
--(axis cs:25.8503401360544,0.154658072592178)
--(axis cs:25.5102040816327,0.155916293939762)
--(axis cs:25.1700680272109,0.158108897285225)
--(axis cs:24.8299319727891,0.16262254699525)
--(axis cs:24.4897959183673,0.164869445764253)
--(axis cs:24.1496598639456,0.167684264279032)
--(axis cs:23.8095238095238,0.17198413177811)
--(axis cs:23.469387755102,0.174920790007495)
--(axis cs:23.1292517006803,0.180226193148804)
--(axis cs:22.7891156462585,0.184245854473411)
--(axis cs:22.4489795918367,0.18985724567258)
--(axis cs:22.108843537415,0.191927284801793)
--(axis cs:21.7687074829932,0.196770839749149)
--(axis cs:21.4285714285714,0.198723881343097)
--(axis cs:21.0884353741497,0.201887318187788)
--(axis cs:20.7482993197279,0.203390719338732)
--(axis cs:20.4081632653061,0.207448288987223)
--(axis cs:20.0680272108844,0.212084387446299)
--(axis cs:19.7278911564626,0.216148254974195)
--(axis cs:19.3877551020408,0.22029245444215)
--(axis cs:19.047619047619,0.221798561708789)
--(axis cs:18.7074829931973,0.227071519158664)
--(axis cs:18.3673469387755,0.231073845172076)
--(axis cs:18.0272108843537,0.237564208301926)
--(axis cs:17.687074829932,0.241659979937777)
--(axis cs:17.3469387755102,0.249240967114502)
--(axis cs:17.0068027210884,0.253956357342335)
--(axis cs:16.6666666666667,0.257413178726087)
--(axis cs:16.3265306122449,0.261139209936737)
--(axis cs:15.9863945578231,0.266973908814499)
--(axis cs:15.6462585034014,0.271099544613347)
--(axis cs:15.3061224489796,0.273983554370887)
--(axis cs:14.9659863945578,0.278931031547591)
--(axis cs:14.6258503401361,0.285483003986023)
--(axis cs:14.2857142857143,0.289595594692926)
--(axis cs:13.9455782312925,0.293733943611628)
--(axis cs:13.6054421768707,0.294168162636023)
--(axis cs:13.265306122449,0.297786762251304)
--(axis cs:12.9251700680272,0.302695487949853)
--(axis cs:12.5850340136054,0.307458496852962)
--(axis cs:12.2448979591837,0.309089214899885)
--(axis cs:11.9047619047619,0.3157743022851)
--(axis cs:11.5646258503401,0.321814374969451)
--(axis cs:11.2244897959184,0.328823598098367)
--(axis cs:10.8843537414966,0.337741947106691)
--(axis cs:10.5442176870748,0.346547996238645)
--(axis cs:10.2040816326531,0.350948052089488)
--(axis cs:9.86394557823129,0.360419976386817)
--(axis cs:9.52380952380952,0.368378015590456)
--(axis cs:9.18367346938775,0.38001947816339)
--(axis cs:8.84353741496599,0.387331822771507)
--(axis cs:8.50340136054422,0.394118173584741)
--(axis cs:8.16326530612245,0.405634456559421)
--(axis cs:7.82312925170068,0.413185004562068)
--(axis cs:7.48299319727891,0.422349855596386)
--(axis cs:7.14285714285714,0.436144533126547)
--(axis cs:6.80272108843537,0.450218379612125)
--(axis cs:6.46258503401361,0.468110097092485)
--(axis cs:6.12244897959184,0.480387680588919)
--(axis cs:5.78231292517007,0.49195381266251)
--(axis cs:5.4421768707483,0.50770416205622)
--(axis cs:5.10204081632653,0.522834689566579)
--(axis cs:4.76190476190476,0.542011125136195)
--(axis cs:4.42176870748299,0.563077240556167)
--(axis cs:4.08163265306122,0.576508779242963)
--(axis cs:3.74149659863946,0.587682966922898)
--(axis cs:3.40136054421769,0.608662841623629)
--(axis cs:3.06122448979592,0.62203707541908)
--(axis cs:2.72108843537415,0.637427608808843)
--(axis cs:2.38095238095238,0.652956189050317)
--(axis cs:2.04081632653061,0.667011504050196)
--(axis cs:1.70068027210884,0.685266245905433)
--(axis cs:1.36054421768707,0.704333213663295)
--(axis cs:1.02040816326531,0.717711855017691)
--(axis cs:0.680272108843537,0.72194008482444)
--(axis cs:0.340136054421769,0.724660824024366)
--(axis cs:0,0.720468087377886)
--cycle;


==> img/stl10/stl10_rate_distortion_pgd_multi.tex <==
\addplot [line width=0.5, opacity=0.7, color9, mark=square*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color9, thin}]
table {%
0 0.718719349205494
0.340136054421769 0.717906942069531
0.680272108843537 0.712355129271746
1.02040816326531 0.704150415956974
1.36054421768707 0.693303289413452
1.70068027210884 0.67984262958169
2.04081632653061 0.665851288288832
2.38095238095238 0.651718693673611
2.72108843537415 0.635616398900747
3.06122448979592 0.620707899779081
3.40136054421769 0.606160140559077
3.74149659863946 0.591195337194949
4.08163265306122 0.573868705555797
4.42176870748299 0.560495226429775
4.76190476190476 0.543933456558734
5.10204081632653 0.528830850692466
5.4421768707483 0.515360228609061
5.78231292517007 0.500060114085791
6.12244897959184 0.4908087161812
6.46258503401361 0.476592664453929
6.80272108843537 0.46598046633575
7.14285714285714 0.455481097482116
7.48299319727891 0.443658467417008
7.82312925170068 0.433169677325241
8.16326530612245 0.422373094526392
8.50340136054422 0.413469241589432
8.84353741496599 0.404489626096085
9.18367346938775 0.395894222105949
9.52380952380952 0.386805124243513
9.86394557823129 0.379738862765656
10.2040816326531 0.37323997130644
10.5442176870748 0.363988563061238
10.8843537414966 0.354347870795368
11.2244897959184 0.345876840576286
11.5646258503401 0.336916204420685
11.9047619047619 0.327694896039038
12.2448979591837 0.320942430300628
12.5850340136054 0.312798832709056
12.9251700680272 0.308362836953371
13.265306122449 0.299887082062555
13.6054421768707 0.292542141931685
13.9455782312925 0.287180464362592
14.2857142857143 0.282134889252198
14.6258503401361 0.274215103197531
14.9659863945578 0.268392080014593
15.3061224489796 0.263293320591407
15.6462585034014 0.258258550552458
15.9863945578231 0.251985557706996
16.3265306122449 0.245720568869361
16.6666666666667 0.242811056786233
17.0068027210884 0.239948964921386
17.3469387755102 0.235783817030096
17.687074829932 0.230046840929598
18.0272108843537 0.226273964115331
18.3673469387755 0.220466952593589
18.7074829931973 0.217699511129977
19.047619047619 0.213765086517946
19.3877551020408 0.20871605106491
19.7278911564626 0.206228017723702
20.0680272108844 0.202174855245615
20.4081632653061 0.197580575575805
20.7482993197279 0.195577790944428
21.0884353741497 0.189950629768446
21.4285714285714 0.188865119996607
21.7687074829932 0.183986157163259
22.108843537415 0.180770259290038
22.4489795918367 0.17577628483069
22.7891156462585 0.17320913313178
23.1292517006803 0.168865075459262
23.469387755102 0.166683885888339
23.8095238095238 0.161111096981786
24.1496598639456 0.158576949961372
24.4897959183673 0.157607884442336
24.8299319727891 0.152907992001332
25.1700680272109 0.150075468259135
25.5102040816327 0.145710243491929
25.8503401360544 0.144584545268851
26.1904761904762 0.141738736542156
26.530612244898 0.139516502297733
26.8707482993197 0.137053358722834
27.2108843537415 0.134063284892868
27.5510204081633 0.13237316282512
27.891156462585 0.131018197592545
28.2312925170068 0.128805484080217
28.5714285714286 0.127796514910261
28.9115646258503 0.125230683522032
29.2517006802721 0.125573478595449
29.5918367346939 0.120688693185207
29.9319727891156 0.119756353001114
30.2721088435374 0.118599684066074
30.6122448979592 0.119134797558355
30.952380952381 0.116406959691995
31.2925170068027 0.113811778888911
31.6326530612245 0.111620172595575
31.9727891156463 0.11120333707399
32.312925170068 0.109360849788224
32.6530612244898 0.107888055106425
32.9931972789116 0.105440075152987
33.3333333333333 0.10407342861133
33.6734693877551 0.102743420432284
34.0136054421769 0.101401413585866
34.3537414965986 0.101668190035535
34.6938775510204 0.100214387627733
35.0340136054422 0.0979265711920733
35.3741496598639 0.0984946034083257
35.7142857142857 0.0968624460992804
36.0544217687075 0.0939224627040677
36.3945578231292 0.0935291339044064
36.734693877551 0.0914136830615215
37.0748299319728 0.0908351391970519
37.4149659863946 0.0905587204995247
37.7551020408163 0.0877165016446942
38.0952380952381 0.0865256202177201
38.4353741496599 0.0857093250338412
38.7755102040816 0.0843065514527174
39.1156462585034 0.083736485648316
39.4557823129252 0.0818030062100594
39.7959183673469 0.0811562242648442
40.1360544217687 0.0800769083594857
40.4761904761905 0.0785089615309937
40.8163265306122 0.0770895428378061
41.156462585034 0.0749293412949551
41.4965986394558 0.0745649691746389
41.8367346938776 0.0751628406595166
42.1768707482993 0.0734115219570684
42.5170068027211 0.0719832586188523
42.8571428571429 0.0708680738596217
43.1972789115646 0.070360566864054
43.5374149659864 0.0689914600512964
43.8775510204082 0.0681147543421677
44.2176870748299 0.0668583368487079
44.5578231292517 0.0639968566523657
44.8979591836735 0.0641351196508057
45.2380952380952 0.0629801012525019
45.578231292517 0.0627049765302943
45.9183673469388 0.0613234136717718
46.2585034013605 0.0591038970815899
46.5986394557823 0.0591182867176359
46.9387755102041 0.0567057498098095
47.2789115646259 0.0560661528101029
47.6190476190476 0.0562649800228184
47.9591836734694 0.0561238426322814
48.2993197278912 0.0544499526220728
48.6394557823129 0.0541574119240512
48.9795918367347 0.0531569465517231
49.3197278911565 0.0533423489890803
49.6598639455782 0.0526983683306212
50 0.0523576776034957
50.3401360544218 0.051590165127156
50.6802721088435 0.0512154396744497
51.0204081632653 0.0528868017944988
51.3605442176871 0.0537934054765794
51.7006802721088 0.0523471540562474
52.0408163265306 0.0504001296707896
52.3809523809524 0.0504777597382308
52.7210884353741 0.0510122168152274
53.0612244897959 0.050665176753481
53.4013605442177 0.0512923441708308
53.7414965986395 0.0508950667259163
54.0816326530612 0.0504268317884811
54.421768707483 0.0502906409830603
54.7619047619048 0.0498065842788921
55.1020408163265 0.0500586383181851
55.4421768707483 0.0495730287873135
55.7823129251701 0.0509858680420266
56.1224489795918 0.0499924406962335
56.4625850340136 0.050378509260331
56.8027210884354 0.0505773273765221
57.1428571428571 0.0512745711081634
57.4829931972789 0.0518469342017457
57.8231292517007 0.0502899280517766
58.1632653061224 0.0501143726585715
58.5034013605442 0.0496938412241338
58.843537414966 0.0491955879607871
59.1836734693878 0.0487497294588851
59.5238095238095 0.0487823205725823
59.8639455782313 0.0488374147044852
60.2040816326531 0.0484210195501656
60.5442176870748 0.0478193584581135
60.8843537414966 0.0476286502746421
61.2244897959184 0.0466732030748183
61.5646258503401 0.0465312955997257
61.9047619047619 0.0468545597469955
62.2448979591837 0.0454610341005492
62.5850340136054 0.0460607633178796
62.9251700680272 0.0447073940389
63.265306122449 0.0451323194517248
63.6054421768707 0.0448593918406744
63.9455782312925 0.0450695598825121
64.2857142857143 0.0436646899893362
64.6258503401361 0.0433543626512798
64.9659863945578 0.042641260080367
65.3061224489796 0.042110384720046
65.6462585034014 0.0419040673519507
65.9863945578231 0.0412764975006186
66.3265306122449 0.0414262188324012
66.6666666666667 0.0406045808284265
67.0068027210884 0.0406064906970692
67.3469387755102 0.0404721214044617
67.687074829932 0.0406179145869474
68.0272108843537 0.0399192249742683
68.3673469387755 0.0403665159942116
68.7074829931973 0.0398634530826302
69.0476190476191 0.0401307852714108
69.3877551020408 0.0388587259469446
69.7278911564626 0.0403732643013967
70.0680272108844 0.0399561326813576
70.4081632653061 0.0403153904812287
70.7482993197279 0.0396391411758242
71.0884353741497 0.0403709222491229
71.4285714285714 0.0400432740296646
71.7687074829932 0.039363374442762
72.108843537415 0.0396488243148934
72.4489795918367 0.0384603519076901
72.7891156462585 0.03889953240672
73.1292517006803 0.0383755303431789
73.469387755102 0.0390416101086179
73.8095238095238 0.0383704738081818
74.1496598639456 0.0388821337324717
74.4897959183673 0.0383793473296104
74.8299319727891 0.0385692784709896
75.1700680272109 0.0369670788342124
75.5102040816327 0.0365505416290919
75.8503401360544 0.0363345184000733
76.1904761904762 0.0355748968390448
76.530612244898 0.0345135074909287
76.8707482993197 0.0339148403048544
77.2108843537415 0.0333697495539671
77.5510204081633 0.0325342791146948
77.891156462585 0.0313827294980333
78.2312925170068 0.0322230225538864
78.5714285714286 0.0307318724180513
78.9115646258503 0.0300115178085559
79.2517006802721 0.0294135692705506
79.5918367346939 0.0279348522268066
79.9319727891156 0.0267954223454749
80.2721088435374 0.0262737359572299
80.6122448979592 0.025561160566653
80.9523809523809 0.0252396161201305
81.2925170068027 0.0242108269896037
81.6326530612245 0.0237023396404085
81.9727891156463 0.0228848083556534
82.312925170068 0.0221898360368542
82.6530612244898 0.021094136172463
82.9931972789116 0.0197561620466577
83.3333333333333 0.0191971387781734
83.6734693877551 0.0180289121003557
84.0136054421769 0.0175141078056169
84.3537414965986 0.0170066466467766
84.6938775510204 0.0157794303998597
85.0340136054422 0.0149991306333303
85.3741496598639 0.0146421814755613
85.7142857142857 0.013567281086739
86.0544217687075 0.0129162050430678
86.3945578231292 0.0124090971977844
86.734693877551 0.0120096283162914
87.0748299319728 0.0116044890156316
87.4149659863945 0.0113635279118196
87.7551020408163 0.0109029360698353
88.0952380952381 0.0103237679400799
88.4353741496599 0.00971697140854724
88.7755102040816 0.00930166038685375
89.1156462585034 0.00927820628588173
89.4557823129252 0.00899149512728807
89.7959183673469 0.00850534086493282
90.1360544217687 0.00819065111574383
90.4761904761905 0.00793922747862037
90.8163265306122 0.00751927464053056
91.156462585034 0.00686901969638712
91.4965986394558 0.00658898764426647
91.8367346938775 0.00614451524690584
92.1768707482993 0.00573644386764256
92.5170068027211 0.00539781948848017
92.8571428571429 0.00504020355723902
93.1972789115646 0.00502646803683095
93.5374149659864 0.00493568562991956
93.8775510204082 0.00448201756876202
94.2176870748299 0.00402423785534286
94.5578231292517 0.00366299934113473
94.8979591836735 0.00335147537628609
95.2380952380952 0.00301699193274911
95.578231292517 0.00240320932052592
95.9183673469388 0.00217469398418369
96.2585034013605 0.00173138090059637
96.5986394557823 0.00139295435187404
96.9387755102041 0.00112214580103015
97.2789115646258 0.000947655275000003
97.6190476190476 0.000996217320077961
97.9591836734694 0.00095662364419056
98.2993197278912 0.000953185434098691
98.6394557823129 0.000812290215815041
98.9795918367347 0.000719173823195358
99.3197278911565 0.000521009695399599
99.6598639455782 0.000228390574171403
100 7.24220683423482e-14
};
\path [fill=color9, fill opacity=0.25]
(axis cs:0,0.720576053992269)
--(axis cs:0,0.716862644418718)
--(axis cs:0.340136054421769,0.715996732402005)
--(axis cs:0.680272108843537,0.710181163055059)
--(axis cs:1.02040816326531,0.701601651357825)
--(axis cs:1.36054421768707,0.690240446595273)
--(axis cs:1.70068027210884,0.676441251703566)
--(axis cs:2.04081632653061,0.662205822362047)
--(axis cs:2.38095238095238,0.647759296429341)
--(axis cs:2.72108843537415,0.631243862081851)
--(axis cs:3.06122448979592,0.615931400136724)
--(axis cs:3.40136054421769,0.601037314356608)
--(axis cs:3.74149659863946,0.585976061937312)
--(axis cs:4.08163265306122,0.568501929819981)
--(axis cs:4.42176870748299,0.55468220319685)
--(axis cs:4.76190476190476,0.538097398954469)
--(axis cs:5.10204081632653,0.522989492625879)
--(axis cs:5.4421768707483,0.50956541522182)
--(axis cs:5.78231292517007,0.494330442580835)
--(axis cs:6.12244897959184,0.484968385979794)
--(axis cs:6.46258503401361,0.470565279641725)
--(axis cs:6.80272108843537,0.460083103769388)
--(axis cs:7.14285714285714,0.449607526139625)
--(axis cs:7.48299319727891,0.437720104003327)
--(axis cs:7.82312925170068,0.427273406509518)
--(axis cs:8.16326530612245,0.416288518961304)
--(axis cs:8.50340136054422,0.407478771408947)
--(axis cs:8.84353741496599,0.398439485877179)
--(axis cs:9.18367346938775,0.389807430029873)
--(axis cs:9.52380952380952,0.380731377418281)
--(axis cs:9.86394557823129,0.373705926878944)
--(axis cs:10.2040816326531,0.367152940609771)
--(axis cs:10.5442176870748,0.357762644750217)
--(axis cs:10.8843537414966,0.348209395016487)
--(axis cs:11.2244897959184,0.339747442196933)
--(axis cs:11.5646258503401,0.330795384984347)
--(axis cs:11.9047619047619,0.321624811592288)
--(axis cs:12.2448979591837,0.314752163925812)
--(axis cs:12.5850340136054,0.306509538479691)
--(axis cs:12.9251700680272,0.302104566062788)
--(axis cs:13.265306122449,0.293645411932367)
--(axis cs:13.6054421768707,0.286451142980993)
--(axis cs:13.9455782312925,0.281055503417606)
--(axis cs:14.2857142857143,0.276026164254493)
--(axis cs:14.6258503401361,0.268358691648023)
--(axis cs:14.9659863945578,0.262573868058515)
--(axis cs:15.3061224489796,0.257620709956843)
--(axis cs:15.6462585034014,0.252506070099888)
--(axis cs:15.9863945578231,0.246307938648446)
--(axis cs:16.3265306122449,0.240175988321753)
--(axis cs:16.6666666666667,0.237379010816165)
--(axis cs:17.0068027210884,0.234301700966683)
--(axis cs:17.3469387755102,0.230272521291273)
--(axis cs:17.687074829932,0.224389548467831)
--(axis cs:18.0272108843537,0.22082093455703)
--(axis cs:18.3673469387755,0.215009652142587)
--(axis cs:18.7074829931973,0.212134031080181)
--(axis cs:19.047619047619,0.208161556986277)
--(axis cs:19.3877551020408,0.203126571198474)
--(axis cs:19.7278911564626,0.200614812045581)
--(axis cs:20.0680272108844,0.196745200259548)
--(axis cs:20.4081632653061,0.19201444677594)
--(axis cs:20.7482993197279,0.190052339768058)
--(axis cs:21.0884353741497,0.184411672068552)
--(axis cs:21.4285714285714,0.183233836745274)
--(axis cs:21.7687074829932,0.178338604302274)
--(axis cs:22.108843537415,0.175336806636039)
--(axis cs:22.4489795918367,0.170257338877266)
--(axis cs:22.7891156462585,0.167827083477363)
--(axis cs:23.1292517006803,0.163608103272431)
--(axis cs:23.469387755102,0.161375584064904)
--(axis cs:23.8095238095238,0.155967023435286)
--(axis cs:24.1496598639456,0.153445699926938)
--(axis cs:24.4897959183673,0.152351581597388)
--(axis cs:24.8299319727891,0.147813038886072)
--(axis cs:25.1700680272109,0.14495323908466)
--(axis cs:25.5102040816327,0.140642918543788)
--(axis cs:25.8503401360544,0.139436396001905)
--(axis cs:26.1904761904762,0.136794813807036)
--(axis cs:26.530612244898,0.134535449834156)
--(axis cs:26.8707482993197,0.132020197454201)
--(axis cs:27.2108843537415,0.129269504241859)
--(axis cs:27.5510204081633,0.127634711377734)
--(axis cs:27.891156462585,0.12636016323026)
--(axis cs:28.2312925170068,0.124167064358031)
--(axis cs:28.5714285714286,0.123059388639997)
--(axis cs:28.9115646258503,0.120751928422695)
--(axis cs:29.2517006802721,0.121038970688671)
--(axis cs:29.5918367346939,0.116338036779202)
--(axis cs:29.9319727891156,0.115468734482999)
--(axis cs:30.2721088435374,0.114141387715564)
--(axis cs:30.6122448979592,0.114741260724111)
--(axis cs:30.952380952381,0.112360015829821)
--(axis cs:31.2925170068027,0.109595241478932)
--(axis cs:31.6326530612245,0.107547163599289)
--(axis cs:31.9727891156463,0.107086187047876)
--(axis cs:32.312925170068,0.105283463891326)
--(axis cs:32.6530612244898,0.103798322366486)
--(axis cs:32.9931972789116,0.101280114822135)
--(axis cs:33.3333333333333,0.100019642500712)
--(axis cs:33.6734693877551,0.0989165751667209)
--(axis cs:34.0136054421769,0.0976411683449233)
--(axis cs:34.3537414965986,0.0977520004254892)
--(axis cs:34.6938775510204,0.0963413129617471)
--(axis cs:35.0340136054422,0.0939883200295998)
--(axis cs:35.3741496598639,0.0946151996676005)
--(axis cs:35.7142857142857,0.0928177046570589)
--(axis cs:36.0544217687075,0.089995084309235)
--(axis cs:36.3945578231292,0.0895636159395998)
--(axis cs:36.734693877551,0.0874992778301941)
--(axis cs:37.0748299319728,0.0871184270616479)
--(axis cs:37.4149659863946,0.0867036677398604)
--(axis cs:37.7551020408163,0.0839448726485045)
--(axis cs:38.0952380952381,0.0828394594144026)
--(axis cs:38.4353741496599,0.0821391537326933)
--(axis cs:38.7755102040816,0.0805920855393885)
--(axis cs:39.1156462585034,0.0802292650126418)
--(axis cs:39.4557823129252,0.0780939654549176)
--(axis cs:39.7959183673469,0.0774902369535546)
--(axis cs:40.1360544217687,0.0764934004041341)
--(axis cs:40.4761904761905,0.0750450616451493)
--(axis cs:40.8163265306122,0.0735635511122182)
--(axis cs:41.156462585034,0.0716331444452484)
--(axis cs:41.4965986394558,0.0710369724497645)
--(axis cs:41.8367346938776,0.0716912670054154)
--(axis cs:42.1768707482993,0.0699788164898516)
--(axis cs:42.5170068027211,0.0685540755616378)
--(axis cs:42.8571428571429,0.0674428510769928)
--(axis cs:43.1972789115646,0.0668328878498295)
--(axis cs:43.5374149659864,0.0655671792541095)
--(axis cs:43.8775510204082,0.0649072019553855)
--(axis cs:44.2176870748299,0.0635420599477577)
--(axis cs:44.5578231292517,0.0606775299592557)
--(axis cs:44.8979591836735,0.0610058346729884)
--(axis cs:45.2380952380952,0.0597856421618717)
--(axis cs:45.578231292517,0.0595981631825261)
--(axis cs:45.9183673469388,0.0581611088456787)
--(axis cs:46.2585034013605,0.05590638003485)
--(axis cs:46.5986394557823,0.055970290633515)
--(axis cs:46.9387755102041,0.0534648625290756)
--(axis cs:47.2789115646259,0.0527653911920483)
--(axis cs:47.6190476190476,0.0531809268292503)
--(axis cs:47.9591836734694,0.0528758149919343)
--(axis cs:48.2993197278912,0.0513620667630901)
--(axis cs:48.6394557823129,0.0510558139772872)
--(axis cs:48.9795918367347,0.0500787799596139)
--(axis cs:49.3197278911565,0.0502139367573472)
--(axis cs:49.6598639455782,0.0494471795833865)
--(axis cs:50,0.049157958770008)
--(axis cs:50.3401360544218,0.0484301547463378)
--(axis cs:50.6802721088435,0.0479859141504248)
--(axis cs:51.0204081632653,0.0496699499636773)
--(axis cs:51.3605442176871,0.0504746416387518)
--(axis cs:51.7006802721088,0.0492844656496702)
--(axis cs:52.0408163265306,0.0473070777364188)
--(axis cs:52.3809523809524,0.0470929285160053)
--(axis cs:52.7210884353741,0.0477999702141852)
--(axis cs:53.0612244897959,0.0475373447633037)
--(axis cs:53.4013605442177,0.0481329703204866)
--(axis cs:53.7414965986395,0.0476930606009137)
--(axis cs:54.0816326530612,0.0472131179232739)
--(axis cs:54.421768707483,0.0470437984982618)
--(axis cs:54.7619047619048,0.0466411171342127)
--(axis cs:55.1020408163265,0.0469451980257629)
--(axis cs:55.4421768707483,0.0465500574534685)
--(axis cs:55.7823129251701,0.0477894695133372)
--(axis cs:56.1224489795918,0.0468755690334234)
--(axis cs:56.4625850340136,0.0473600143342183)
--(axis cs:56.8027210884354,0.0475086822657812)
--(axis cs:57.1428571428571,0.0481934980691282)
--(axis cs:57.4829931972789,0.0487927157730278)
--(axis cs:57.8231292517007,0.0474095921113535)
--(axis cs:58.1632653061224,0.047219605938974)
--(axis cs:58.5034013605442,0.0468737575250554)
--(axis cs:58.843537414966,0.0463073183581941)
--(axis cs:59.1836734693878,0.0458763868782474)
--(axis cs:59.5238095238095,0.0457757308508763)
--(axis cs:59.8639455782313,0.0459490134847329)
--(axis cs:60.2040816326531,0.0453872092322091)
--(axis cs:60.5442176870748,0.0449069797935546)
--(axis cs:60.8843537414966,0.0447212670093672)
--(axis cs:61.2244897959184,0.0439223817114294)
--(axis cs:61.5646258503401,0.0436670591312137)
--(axis cs:61.9047619047619,0.0439909471333912)
--(axis cs:62.2448979591837,0.0426471750432498)
--(axis cs:62.5850340136054,0.043189619189854)
--(axis cs:62.9251700680272,0.0419276337099591)
--(axis cs:63.265306122449,0.0424629820288046)
--(axis cs:63.6054421768707,0.0422795123864622)
--(axis cs:63.9455782312925,0.0422939028100636)
--(axis cs:64.2857142857143,0.0410283103165485)
--(axis cs:64.6258503401361,0.0407033347341559)
--(axis cs:64.9659863945578,0.0400698950571715)
--(axis cs:65.3061224489796,0.0396458974934157)
--(axis cs:65.6462585034014,0.0393013705347533)
--(axis cs:65.9863945578231,0.0388739384955582)
--(axis cs:66.3265306122449,0.0390693861430328)
--(axis cs:66.6666666666667,0.0382630182282195)
--(axis cs:67.0068027210884,0.0380973408917582)
--(axis cs:67.3469387755102,0.0382004672266599)
--(axis cs:67.687074829932,0.0382968267576662)
--(axis cs:68.0272108843537,0.0375188281862676)
--(axis cs:68.3673469387755,0.0379604026394639)
--(axis cs:68.7074829931973,0.037459158361309)
--(axis cs:69.0476190476191,0.0376941904355507)
--(axis cs:69.3877551020408,0.0363647198866209)
--(axis cs:69.7278911564626,0.0379085504197664)
--(axis cs:70.0680272108844,0.0375730322209818)
--(axis cs:70.4081632653061,0.0378160517090639)
--(axis cs:70.7482993197279,0.0373459585007635)
--(axis cs:71.0884353741497,0.0379090194472675)
--(axis cs:71.4285714285714,0.0377029349514908)
--(axis cs:71.7687074829932,0.0369309726195718)
--(axis cs:72.108843537415,0.0373778745456543)
--(axis cs:72.4489795918367,0.0363197606399246)
--(axis cs:72.7891156462585,0.036489645246933)
--(axis cs:73.1292517006803,0.0361238603630487)
--(axis cs:73.469387755102,0.0367463207514486)
--(axis cs:73.8095238095238,0.0361967814558072)
--(axis cs:74.1496598639456,0.0365970257875825)
--(axis cs:74.4897959183673,0.0360953975137133)
--(axis cs:74.8299319727891,0.0362679397232047)
--(axis cs:75.1700680272109,0.0348712596494765)
--(axis cs:75.5102040816327,0.0343136152322883)
--(axis cs:75.8503401360544,0.0341243164447029)
--(axis cs:76.1904761904762,0.0334080575022182)
--(axis cs:76.530612244898,0.0323292767904696)
--(axis cs:76.8707482993197,0.0317502601966357)
--(axis cs:77.2108843537415,0.0313711745735045)
--(axis cs:77.5510204081633,0.0304526352703844)
--(axis cs:77.891156462585,0.0293381891933553)
--(axis cs:78.2312925170068,0.0300851875064397)
--(axis cs:78.5714285714286,0.0287418791512613)
--(axis cs:78.9115646258503,0.0280604177345836)
--(axis cs:79.2517006802721,0.0274927727994302)
--(axis cs:79.5918367346939,0.0260503911714964)
--(axis cs:79.9319727891156,0.02489462201553)
--(axis cs:80.2721088435374,0.0244026587422851)
--(axis cs:80.6122448979592,0.0237597031892029)
--(axis cs:80.9523809523809,0.0234833634499014)
--(axis cs:81.2925170068027,0.0224455487918128)
--(axis cs:81.6326530612245,0.0219626398540707)
--(axis cs:81.9727891156463,0.021230437699549)
--(axis cs:82.312925170068,0.0204592102883979)
--(axis cs:82.6530612244898,0.0194506662842406)
--(axis cs:82.9931972789116,0.0182370528243442)
--(axis cs:83.3333333333333,0.0177523293664162)
--(axis cs:83.6734693877551,0.0166123579926478)
--(axis cs:84.0136054421769,0.016075177439779)
--(axis cs:84.3537414965986,0.0156060307536217)
--(axis cs:84.6938775510204,0.0144958596988552)
--(axis cs:85.0340136054422,0.0137209303012397)
--(axis cs:85.3741496598639,0.0133964588718783)
--(axis cs:85.7142857142857,0.012437371208769)
--(axis cs:86.0544217687075,0.0117896939211857)
--(axis cs:86.3945578231292,0.0113302352731532)
--(axis cs:86.734693877551,0.0109937926473459)
--(axis cs:87.0748299319728,0.01063740392854)
--(axis cs:87.4149659863945,0.0103702829286618)
--(axis cs:87.7551020408163,0.00994075330378279)
--(axis cs:88.0952380952381,0.00941020906136272)
--(axis cs:88.4353741496599,0.00880225739647256)
--(axis cs:88.7755102040816,0.00848691624878337)
--(axis cs:89.1156462585034,0.00840738807096852)
--(axis cs:89.4557823129252,0.00814873858085187)
--(axis cs:89.7959183673469,0.00770819557739295)
--(axis cs:90.1360544217687,0.00734611501241231)
--(axis cs:90.4761904761905,0.00711267327585869)
--(axis cs:90.8163265306122,0.00671479928385391)
--(axis cs:91.156462585034,0.00612952094095341)
--(axis cs:91.4965986394558,0.00583109403994068)
--(axis cs:91.8367346938775,0.00545036028170105)
--(axis cs:92.1768707482993,0.00504324223530348)
--(axis cs:92.5170068027211,0.00466298939991087)
--(axis cs:92.8571428571429,0.0043819901390799)
--(axis cs:93.1972789115646,0.00434193005246013)
--(axis cs:93.5374149659864,0.00419637748060201)
--(axis cs:93.8775510204082,0.00378684577464182)
--(axis cs:94.2176870748299,0.00337084416167077)
--(axis cs:94.5578231292517,0.00307598202363232)
--(axis cs:94.8979591836735,0.00279390011555058)
--(axis cs:95.2380952380952,0.00248407714891246)
--(axis cs:95.578231292517,0.00196284858206052)
--(axis cs:95.9183673469388,0.00175817158198883)
--(axis cs:96.2585034013605,0.00140837781496181)
--(axis cs:96.5986394557823,0.00108607922284021)
--(axis cs:96.9387755102041,0.000869525643530179)
--(axis cs:97.2789115646258,0.000754320106740691)
--(axis cs:97.6190476190476,0.000810083615085317)
--(axis cs:97.9591836734694,0.00075463087812036)
--(axis cs:98.2993197278912,0.000771213737505154)
--(axis cs:98.6394557823129,0.000673198820473739)
--(axis cs:98.9795918367347,0.000601834898146379)
--(axis cs:99.3197278911565,0.000454126956690725)
--(axis cs:99.6598639455782,0.000199942883274735)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:100,7.24220683423482e-14)
--(axis cs:99.6598639455782,0.00025683826506807)
--(axis cs:99.3197278911565,0.000587892434108473)
--(axis cs:98.9795918367347,0.000836512748244337)
--(axis cs:98.6394557823129,0.000951381611156344)
--(axis cs:98.2993197278912,0.00113515713069223)
--(axis cs:97.9591836734694,0.00115861641026076)
--(axis cs:97.6190476190476,0.00118235102507061)
--(axis cs:97.2789115646258,0.00114099044325932)
--(axis cs:96.9387755102041,0.00137476595853012)
--(axis cs:96.5986394557823,0.00169982948090787)
--(axis cs:96.2585034013605,0.00205438398623093)
--(axis cs:95.9183673469388,0.00259121638637855)
--(axis cs:95.578231292517,0.00284357005899132)
--(axis cs:95.2380952380952,0.00354990671658576)
--(axis cs:94.8979591836735,0.0039090506370216)
--(axis cs:94.5578231292517,0.00425001665863715)
--(axis cs:94.2176870748299,0.00467763154901495)
--(axis cs:93.8775510204082,0.00517718936288222)
--(axis cs:93.5374149659864,0.0056749937792371)
--(axis cs:93.1972789115646,0.00571100602120178)
--(axis cs:92.8571428571429,0.00569841697539813)
--(axis cs:92.5170068027211,0.00613264957704947)
--(axis cs:92.1768707482993,0.00642964549998165)
--(axis cs:91.8367346938775,0.00683867021211063)
--(axis cs:91.4965986394558,0.00734688124859225)
--(axis cs:91.156462585034,0.00760851845182082)
--(axis cs:90.8163265306122,0.00832374999720721)
--(axis cs:90.4761904761905,0.00876578168138205)
--(axis cs:90.1360544217687,0.00903518721907535)
--(axis cs:89.7959183673469,0.00930248615247269)
--(axis cs:89.4557823129252,0.00983425167372428)
--(axis cs:89.1156462585034,0.0101490245007949)
--(axis cs:88.7755102040816,0.0101164045249241)
--(axis cs:88.4353741496599,0.0106316854206219)
--(axis cs:88.0952380952381,0.0112373268187971)
--(axis cs:87.7551020408163,0.0118651188358878)
--(axis cs:87.4149659863945,0.0123567728949774)
--(axis cs:87.0748299319728,0.0125715741027232)
--(axis cs:86.734693877551,0.013025463985237)
--(axis cs:86.3945578231292,0.0134879591224156)
--(axis cs:86.0544217687075,0.0140427161649499)
--(axis cs:85.7142857142857,0.014697190964709)
--(axis cs:85.3741496598639,0.0158879040792442)
--(axis cs:85.0340136054422,0.0162773309654209)
--(axis cs:84.6938775510204,0.0170630011008642)
--(axis cs:84.3537414965986,0.0184072625399316)
--(axis cs:84.0136054421769,0.0189530381714547)
--(axis cs:83.6734693877551,0.0194454662080637)
--(axis cs:83.3333333333333,0.0206419481899305)
--(axis cs:82.9931972789116,0.0212752712689712)
--(axis cs:82.6530612244898,0.0227376060606854)
--(axis cs:82.312925170068,0.0239204617853105)
--(axis cs:81.9727891156463,0.0245391790117577)
--(axis cs:81.6326530612245,0.0254420394267462)
--(axis cs:81.2925170068027,0.0259761051873946)
--(axis cs:80.9523809523809,0.0269958687903596)
--(axis cs:80.6122448979592,0.0273626179441032)
--(axis cs:80.2721088435374,0.0281448131721746)
--(axis cs:79.9319727891156,0.0286962226754197)
--(axis cs:79.5918367346939,0.0298193132821167)
--(axis cs:79.2517006802721,0.0313343657416709)
--(axis cs:78.9115646258503,0.0319626178825283)
--(axis cs:78.5714285714286,0.0327218656848412)
--(axis cs:78.2312925170068,0.0343608576013332)
--(axis cs:77.891156462585,0.0334272698027114)
--(axis cs:77.5510204081633,0.0346159229590053)
--(axis cs:77.2108843537415,0.0353683245344297)
--(axis cs:76.8707482993197,0.036079420413073)
--(axis cs:76.530612244898,0.0366977381913879)
--(axis cs:76.1904761904762,0.0377417361758714)
--(axis cs:75.8503401360544,0.0385447203554438)
--(axis cs:75.5102040816327,0.0387874680258955)
--(axis cs:75.1700680272109,0.0390628980189483)
--(axis cs:74.8299319727891,0.0408706172187745)
--(axis cs:74.4897959183673,0.0406632971455074)
--(axis cs:74.1496598639456,0.0411672416773609)
--(axis cs:73.8095238095238,0.0405441661605564)
--(axis cs:73.469387755102,0.0413368994657871)
--(axis cs:73.1292517006803,0.040627200323309)
--(axis cs:72.7891156462585,0.0413094195665069)
--(axis cs:72.4489795918367,0.0406009431754556)
--(axis cs:72.108843537415,0.0419197740841326)
--(axis cs:71.7687074829932,0.0417957762659521)
--(axis cs:71.4285714285714,0.0423836131078383)
--(axis cs:71.0884353741497,0.0428328250509784)
--(axis cs:70.7482993197279,0.041932323850885)
--(axis cs:70.4081632653061,0.0428147292533934)
--(axis cs:70.0680272108844,0.0423392331417334)
--(axis cs:69.7278911564626,0.042837978183027)
--(axis cs:69.3877551020408,0.0413527320072682)
--(axis cs:69.0476190476191,0.0425673801072708)
--(axis cs:68.7074829931973,0.0422677478039514)
--(axis cs:68.3673469387755,0.0427726293489592)
--(axis cs:68.0272108843537,0.0423196217622691)
--(axis cs:67.687074829932,0.0429390024162287)
--(axis cs:67.3469387755102,0.0427437755822636)
--(axis cs:67.0068027210884,0.0431156405023802)
--(axis cs:66.6666666666667,0.0429461434286336)
--(axis cs:66.3265306122449,0.0437830515217695)
--(axis cs:65.9863945578231,0.0436790565056791)
--(axis cs:65.6462585034014,0.0445067641691481)
--(axis cs:65.3061224489796,0.0445748719466764)
--(axis cs:64.9659863945578,0.0452126251035624)
--(axis cs:64.6258503401361,0.0460053905684038)
--(axis cs:64.2857142857143,0.0463010696621238)
--(axis cs:63.9455782312925,0.0478452169549606)
--(axis cs:63.6054421768707,0.0474392712948865)
--(axis cs:63.265306122449,0.047801656874645)
--(axis cs:62.9251700680272,0.0474871543678409)
--(axis cs:62.5850340136054,0.0489319074459051)
--(axis cs:62.2448979591837,0.0482748931578486)
--(axis cs:61.9047619047619,0.0497181723605999)
--(axis cs:61.5646258503401,0.0493955320682376)
--(axis cs:61.2244897959184,0.0494240244382072)
--(axis cs:60.8843537414966,0.050536033539917)
--(axis cs:60.5442176870748,0.0507317371226724)
--(axis cs:60.2040816326531,0.0514548298681221)
--(axis cs:59.8639455782313,0.0517258159242375)
--(axis cs:59.5238095238095,0.0517889102942883)
--(axis cs:59.1836734693878,0.0516230720395228)
--(axis cs:58.843537414966,0.0520838575633802)
--(axis cs:58.5034013605442,0.0525139249232121)
--(axis cs:58.1632653061224,0.0530091393781691)
--(axis cs:57.8231292517007,0.0531702639921997)
--(axis cs:57.4829931972789,0.0549011526304635)
--(axis cs:57.1428571428571,0.0543556441471986)
--(axis cs:56.8027210884354,0.0536459724872631)
--(axis cs:56.4625850340136,0.0533970041864437)
--(axis cs:56.1224489795918,0.0531093123590435)
--(axis cs:55.7823129251701,0.054182266570716)
--(axis cs:55.4421768707483,0.0525960001211585)
--(axis cs:55.1020408163265,0.0531720786106074)
--(axis cs:54.7619047619048,0.0529720514235714)
--(axis cs:54.421768707483,0.0535374834678588)
--(axis cs:54.0816326530612,0.0536405456536884)
--(axis cs:53.7414965986395,0.0540970728509189)
--(axis cs:53.4013605442177,0.054451718021175)
--(axis cs:53.0612244897959,0.0537930087436583)
--(axis cs:52.7210884353741,0.0542244634162696)
--(axis cs:52.3809523809524,0.0538625909604562)
--(axis cs:52.0408163265306,0.0534931816051604)
--(axis cs:51.7006802721088,0.0554098424628247)
--(axis cs:51.3605442176871,0.0571121693144071)
--(axis cs:51.0204081632653,0.0561036536253203)
--(axis cs:50.6802721088435,0.0544449651984747)
--(axis cs:50.3401360544218,0.0547501755079741)
--(axis cs:50,0.0555573964369835)
--(axis cs:49.6598639455782,0.0559495570778559)
--(axis cs:49.3197278911565,0.0564707612208133)
--(axis cs:48.9795918367347,0.0562351131438322)
--(axis cs:48.6394557823129,0.0572590098708153)
--(axis cs:48.2993197278912,0.0575378384810555)
--(axis cs:47.9591836734694,0.0593718702726284)
--(axis cs:47.6190476190476,0.0593490332163865)
--(axis cs:47.2789115646259,0.0593669144281576)
--(axis cs:46.9387755102041,0.0599466370905434)
--(axis cs:46.5986394557823,0.0622662828017569)
--(axis cs:46.2585034013605,0.0623014141283298)
--(axis cs:45.9183673469388,0.064485718497865)
--(axis cs:45.578231292517,0.0658117898780624)
--(axis cs:45.2380952380952,0.0661745603431322)
--(axis cs:44.8979591836735,0.067264404628623)
--(axis cs:44.5578231292517,0.0673161833454757)
--(axis cs:44.2176870748299,0.0701746137496582)
--(axis cs:43.8775510204082,0.07132230672895)
--(axis cs:43.5374149659864,0.0724157408484832)
--(axis cs:43.1972789115646,0.0738882458782784)
--(axis cs:42.8571428571429,0.0742932966422507)
--(axis cs:42.5170068027211,0.0754124416760668)
--(axis cs:42.1768707482993,0.0768442274242852)
--(axis cs:41.8367346938776,0.0786344143136179)
--(axis cs:41.4965986394558,0.0780929658995132)
--(axis cs:41.156462585034,0.0782255381446618)
--(axis cs:40.8163265306122,0.0806155345633941)
--(axis cs:40.4761904761905,0.0819728614168381)
--(axis cs:40.1360544217687,0.0836604163148373)
--(axis cs:39.7959183673469,0.0848222115761339)
--(axis cs:39.4557823129252,0.0855120469652013)
--(axis cs:39.1156462585034,0.0872437062839901)
--(axis cs:38.7755102040816,0.0880210173660463)
--(axis cs:38.4353741496599,0.0892794963349891)
--(axis cs:38.0952380952381,0.0902117810210376)
--(axis cs:37.7551020408163,0.0914881306408838)
--(axis cs:37.4149659863946,0.0944137732591891)
--(axis cs:37.0748299319728,0.0945518513324559)
--(axis cs:36.734693877551,0.0953280882928489)
--(axis cs:36.3945578231292,0.097494651869213)
--(axis cs:36.0544217687075,0.0978498410989004)
--(axis cs:35.7142857142857,0.100907187541502)
--(axis cs:35.3741496598639,0.102374007149051)
--(axis cs:35.0340136054422,0.101864822354547)
--(axis cs:34.6938775510204,0.104087462293718)
--(axis cs:34.3537414965986,0.10558437964558)
--(axis cs:34.0136054421769,0.105161658826809)
--(axis cs:33.6734693877551,0.106570265697846)
--(axis cs:33.3333333333333,0.108127214721948)
--(axis cs:32.9931972789116,0.109600035483839)
--(axis cs:32.6530612244898,0.111977787846364)
--(axis cs:32.312925170068,0.113438235685123)
--(axis cs:31.9727891156463,0.115320487100104)
--(axis cs:31.6326530612245,0.115693181591861)
--(axis cs:31.2925170068027,0.118028316298891)
--(axis cs:30.952380952381,0.12045390355417)
--(axis cs:30.6122448979592,0.123528334392599)
--(axis cs:30.2721088435374,0.123057980416584)
--(axis cs:29.9319727891156,0.124043971519229)
--(axis cs:29.5918367346939,0.125039349591212)
--(axis cs:29.2517006802721,0.130107986502227)
--(axis cs:28.9115646258503,0.12970943862137)
--(axis cs:28.5714285714286,0.132533641180525)
--(axis cs:28.2312925170068,0.133443903802404)
--(axis cs:27.891156462585,0.13567623195483)
--(axis cs:27.5510204081633,0.137111614272505)
--(axis cs:27.2108843537415,0.138857065543878)
--(axis cs:26.8707482993197,0.142086519991466)
--(axis cs:26.530612244898,0.14449755476131)
--(axis cs:26.1904761904762,0.146682659277275)
--(axis cs:25.8503401360544,0.149732694535798)
--(axis cs:25.5102040816327,0.15077756844007)
--(axis cs:25.1700680272109,0.15519769743361)
--(axis cs:24.8299319727891,0.158002945116592)
--(axis cs:24.4897959183673,0.162864187287285)
--(axis cs:24.1496598639456,0.163708199995805)
--(axis cs:23.8095238095238,0.166255170528286)
--(axis cs:23.469387755102,0.171992187711773)
--(axis cs:23.1292517006803,0.174122047646093)
--(axis cs:22.7891156462585,0.178591182786198)
--(axis cs:22.4489795918367,0.181295230784115)
--(axis cs:22.108843537415,0.186203711944037)
--(axis cs:21.7687074829932,0.189633710024243)
--(axis cs:21.4285714285714,0.19449640324794)
--(axis cs:21.0884353741497,0.19548958746834)
--(axis cs:20.7482993197279,0.201103242120797)
--(axis cs:20.4081632653061,0.20314670437567)
--(axis cs:20.0680272108844,0.207604510231681)
--(axis cs:19.7278911564626,0.211841223401823)
--(axis cs:19.3877551020408,0.214305530931346)
--(axis cs:19.047619047619,0.219368616049614)
--(axis cs:18.7074829931973,0.223264991179774)
--(axis cs:18.3673469387755,0.225924253044591)
--(axis cs:18.0272108843537,0.231726993673633)
--(axis cs:17.687074829932,0.235704133391365)
--(axis cs:17.3469387755102,0.241295112768918)
--(axis cs:17.0068027210884,0.245596228876089)
--(axis cs:16.6666666666667,0.248243102756301)
--(axis cs:16.3265306122449,0.251265149416969)
--(axis cs:15.9863945578231,0.257663176765547)
--(axis cs:15.6462585034014,0.264011031005029)
--(axis cs:15.3061224489796,0.268965931225971)
--(axis cs:14.9659863945578,0.27421029197067)
--(axis cs:14.6258503401361,0.280071514747039)
--(axis cs:14.2857142857143,0.288243614249903)
--(axis cs:13.9455782312925,0.293305425307578)
--(axis cs:13.6054421768707,0.298633140882378)
--(axis cs:13.265306122449,0.306128752192743)
--(axis cs:12.9251700680272,0.314621107843955)
--(axis cs:12.5850340136054,0.319088126938421)
--(axis cs:12.2448979591837,0.327132696675443)
--(axis cs:11.9047619047619,0.333764980485788)
--(axis cs:11.5646258503401,0.343037023857023)
--(axis cs:11.2244897959184,0.352006238955639)
--(axis cs:10.8843537414966,0.360486346574249)
--(axis cs:10.5442176870748,0.37021448137226)
--(axis cs:10.2040816326531,0.379327002003109)
--(axis cs:9.86394557823129,0.385771798652367)
--(axis cs:9.52380952380952,0.392878871068744)
--(axis cs:9.18367346938775,0.401981014182025)
--(axis cs:8.84353741496599,0.410539766314992)
--(axis cs:8.50340136054422,0.419459711769918)
--(axis cs:8.16326530612245,0.428457670091481)
--(axis cs:7.82312925170068,0.439065948140963)
--(axis cs:7.48299319727891,0.449596830830689)
--(axis cs:7.14285714285714,0.461354668824607)
--(axis cs:6.80272108843537,0.471877828902112)
--(axis cs:6.46258503401361,0.482620049266132)
--(axis cs:6.12244897959184,0.496649046382606)
--(axis cs:5.78231292517007,0.505789785590747)
--(axis cs:5.4421768707483,0.521155041996302)
--(axis cs:5.10204081632653,0.534672208759053)
--(axis cs:4.76190476190476,0.549769514162999)
--(axis cs:4.42176870748299,0.5663082496627)
--(axis cs:4.08163265306122,0.579235481291612)
--(axis cs:3.74149659863946,0.596414612452587)
--(axis cs:3.40136054421769,0.611282966761547)
--(axis cs:3.06122448979592,0.625484399421439)
--(axis cs:2.72108843537415,0.639988935719644)
--(axis cs:2.38095238095238,0.655678090917881)
--(axis cs:2.04081632653061,0.669496754215616)
--(axis cs:1.70068027210884,0.683244007459813)
--(axis cs:1.36054421768707,0.696366132231632)
--(axis cs:1.02040816326531,0.706699180556123)
--(axis cs:0.680272108843537,0.714529095488433)
--(axis cs:0.340136054421769,0.719817151737057)
--(axis cs:0,0.720576053992269)
--cycle;


==> img/stl10/stl10_rate_distortion_sensitivity.tex <==
\addplot [line width=0.5, opacity=0.7, color6, mark=square, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color6, thin}]
table [row sep=\\]{%
0	0.71875130802393 \\
0.340136054421769	0.719389234185219 \\
0.680272108843537	0.719352099001408 \\
1.02040816326531	0.719541145861149 \\
1.36054421768707	0.719617660492659 \\
1.70068027210884	0.719619219750166 \\
2.04081632653061	0.719605284929276 \\
2.38095238095238	0.719464400857687 \\
2.72108843537415	0.719755884110928 \\
3.06122448979592	0.720365351885557 \\
3.40136054421769	0.719899804592133 \\
3.74149659863946	0.719937762916088 \\
4.08163265306122	0.720883312225342 \\
4.42176870748299	0.721496275961399 \\
4.76190476190476	0.721585703939199 \\
5.10204081632653	0.721376703083515 \\
5.4421768707483	0.721707797795534 \\
5.78231292517007	0.722684831470251 \\
6.12244897959184	0.722616496682167 \\
6.46258503401361	0.72277795612812 \\
6.80272108843537	0.723111711144447 \\
7.14285714285714	0.722212074697018 \\
7.48299319727891	0.722400458306074 \\
7.82312925170068	0.722680221796036 \\
8.16326530612245	0.722466831803322 \\
8.50340136054422	0.721892826855183 \\
8.84353741496599	0.72127392873168 \\
9.18367346938775	0.722675722688436 \\
9.52380952380952	0.721946506202221 \\
9.86394557823129	0.723146450072527 \\
10.2040816326531	0.72148804217577 \\
10.5442176870748	0.721273558139801 \\
10.8843537414966	0.721109543442726 \\
11.2244897959184	0.720933212935924 \\
11.5646258503401	0.719002017229796 \\
11.9047619047619	0.718416908979416 \\
12.2448979591837	0.716659499853849 \\
12.5850340136054	0.715810381323099 \\
12.9251700680272	0.715102718770504 \\
13.265306122449	0.714548605829477 \\
13.6054421768707	0.713216628730297 \\
13.9455782312925	0.712836648523808 \\
14.2857142857143	0.710388991832733 \\
14.6258503401361	0.709525784403086 \\
14.9659863945578	0.708585997521877 \\
15.3061224489796	0.70722248852253 \\
15.6462585034014	0.70541137740016 \\
15.9863945578231	0.703625093251467 \\
16.3265306122449	0.702211262285709 \\
16.6666666666667	0.700518694669008 \\
17.0068027210884	0.698969467878342 \\
17.3469387755102	0.69550486177206 \\
17.687074829932	0.693203378468752 \\
18.0272108843537	0.692014507055283 \\
18.3673469387755	0.689097333997488 \\
18.7074829931973	0.687144755125046 \\
19.047619047619	0.68623220987618 \\
19.3877551020408	0.683548673018813 \\
19.7278911564626	0.682815558984876 \\
20.0680272108844	0.679360005632043 \\
20.4081632653061	0.676604211330414 \\
20.7482993197279	0.675396749228239 \\
21.0884353741497	0.672584816962481 \\
21.4285714285714	0.671548288688064 \\
21.7687074829932	0.670942369922996 \\
22.108843537415	0.66938334506005 \\
22.4489795918367	0.667547020986676 \\
22.7891156462585	0.665231375135481 \\
23.1292517006803	0.663795144371688 \\
23.469387755102	0.66183552691713 \\
23.8095238095238	0.66003238171339 \\
24.1496598639456	0.659306503999978 \\
24.4897959183673	0.656305985469371 \\
24.8299319727891	0.655060895020142 \\
25.1700680272109	0.653564087611157 \\
25.5102040816327	0.65342913857894 \\
25.8503401360544	0.651353622864117 \\
26.1904761904762	0.649769054880599 \\
26.530612244898	0.648370459404541 \\
26.8707482993197	0.64689889976813 \\
27.2108843537415	0.646209046285658 \\
27.5510204081633	0.644484756461316 \\
27.891156462585	0.643503759837186 \\
28.2312925170068	0.642465511379123 \\
28.5714285714286	0.640621536367689 \\
28.9115646258503	0.63856578382256 \\
29.2517006802721	0.636553158548777 \\
29.5918367346939	0.634955416965131 \\
29.9319727891156	0.633268079108275 \\
30.2721088435374	0.632218020689579 \\
30.6122448979592	0.630514471428323 \\
30.952380952381	0.628737529877417 \\
31.2925170068027	0.628290689725591 \\
31.6326530612245	0.62611059601023 \\
31.9727891156463	0.624437426592312 \\
32.312925170068	0.62109547088794 \\
32.6530612244898	0.619236991914377 \\
32.9931972789116	0.617059899174378 \\
33.3333333333333	0.615174428927371 \\
33.6734693877551	0.612900566296757 \\
34.0136054421769	0.611238969717529 \\
34.3537414965986	0.609983125242443 \\
34.6938775510204	0.607802518113467 \\
35.0340136054422	0.604408875973577 \\
35.3741496598639	0.602643325592649 \\
35.7142857142857	0.601325540659723 \\
36.0544217687075	0.597990869728401 \\
36.3945578231292	0.596600741191496 \\
36.734693877551	0.593339063223802 \\
37.0748299319728	0.590376773074545 \\
37.4149659863946	0.588895653723143 \\
37.7551020408163	0.586068131396351 \\
38.0952380952381	0.58339272606092 \\
38.4353741496599	0.582899743387452 \\
38.7755102040816	0.578520637157371 \\
39.1156462585034	0.575298031455968 \\
39.4557823129252	0.572824245888105 \\
39.7959183673469	0.570583217910625 \\
40.1360544217687	0.565465284003098 \\
40.4761904761905	0.563627334888342 \\
40.8163265306122	0.562980324125911 \\
41.156462585034	0.558019456278807 \\
41.4965986394558	0.554970981681654 \\
41.8367346938776	0.553154795611085 \\
42.1768707482993	0.549294094478155 \\
42.5170068027211	0.54746063588162 \\
42.8571428571429	0.54180853363854 \\
43.1972789115646	0.538268962163627 \\
43.5374149659864	0.535178063577325 \\
43.8775510204082	0.532435110855676 \\
44.2176870748299	0.528322815867218 \\
44.5578231292517	0.52428229922289 \\
44.8979591836735	0.52012111508173 \\
45.2380952380952	0.516870992973853 \\
45.578231292517	0.511838539770461 \\
45.9183673469388	0.509859782721291 \\
46.2585034013605	0.506795982160237 \\
46.5986394557823	0.502968141130689 \\
46.9387755102041	0.500034206994109 \\
47.2789115646259	0.49550120893657 \\
47.6190476190476	0.490372676281224 \\
47.9591836734694	0.484856269585264 \\
48.2993197278912	0.482378032237981 \\
48.6394557823129	0.47693821082125 \\
48.9795918367347	0.47248559750771 \\
49.3197278911565	0.469258066426581 \\
49.6598639455782	0.46662457735444 \\
50	0.460333384001327 \\
50.3401360544218	0.458854858390096 \\
50.6802721088435	0.453878445701817 \\
51.0204081632653	0.451958409400314 \\
51.3605442176871	0.446162120898263 \\
51.7006802721088	0.443135322265841 \\
52.0408163265306	0.440284963006352 \\
52.3809523809524	0.434457015806602 \\
52.7210884353741	0.429776695995267 \\
53.0612244897959	0.423140335930677 \\
53.4013605442177	0.418956834605302 \\
53.7414965986395	0.415603507386955 \\
54.0816326530612	0.413340401089163 \\
54.421768707483	0.407627198726388 \\
54.7619047619048	0.403630441902769 \\
55.1020408163265	0.399520309937271 \\
55.4421768707483	0.395474635392616 \\
55.7823129251701	0.392824953850065 \\
56.1224489795918	0.388577833988984 \\
56.4625850340136	0.38242147120702 \\
56.8027210884354	0.37784852625041 \\
57.1428571428571	0.375326868686411 \\
57.4829931972789	0.370742377042909 \\
57.8231292517007	0.368647268721563 \\
58.1632653061224	0.364167572992461 \\
58.5034013605442	0.359282123757876 \\
58.843537414966	0.355422230278188 \\
59.1836734693878	0.347395970084477 \\
59.5238095238095	0.343276355089467 \\
59.8639455782313	0.340022777527628 \\
60.2040816326531	0.336009382964339 \\
60.5442176870748	0.330275990240331 \\
60.8843537414966	0.324512828283365 \\
61.2244897959184	0.319650930041897 \\
61.5646258503401	0.315521145783313 \\
61.9047619047619	0.308393440685266 \\
62.2448979591837	0.304403594820953 \\
62.5850340136054	0.301175528285028 \\
62.9251700680272	0.297260433745578 \\
63.265306122449	0.293401482387707 \\
63.6054421768707	0.290064806929787 \\
63.9455782312925	0.283438257420667 \\
64.2857142857143	0.280380416439351 \\
64.6258503401361	0.276665457767941 \\
64.9659863945578	0.270065949748729 \\
65.3061224489796	0.267169501775804 \\
65.6462585034014	0.261398270268661 \\
65.9863945578231	0.258181693350376 \\
66.3265306122449	0.254697056765158 \\
66.6666666666667	0.2498791079005 \\
67.0068027210884	0.246288083059591 \\
67.3469387755102	0.240849229254541 \\
67.687074829932	0.236934537658012 \\
68.0272108843537	0.233525321844228 \\
68.3673469387755	0.230206291068225 \\
68.7074829931973	0.226030189279833 \\
69.0476190476191	0.22181557680262 \\
69.3877551020408	0.217948692511877 \\
69.7278911564626	0.213242209513381 \\
70.0680272108844	0.210592381587911 \\
70.4081632653061	0.205547006004554 \\
70.7482993197279	0.204241459663476 \\
71.0884353741497	0.200701793285051 \\
71.4285714285714	0.196872331909046 \\
71.7687074829932	0.194689926675679 \\
72.108843537415	0.189027531939788 \\
72.4489795918367	0.183506480059548 \\
72.7891156462585	0.181917438232538 \\
73.1292517006803	0.178326113515072 \\
73.469387755102	0.176675073212418 \\
73.8095238095238	0.172320575380159 \\
74.1496598639456	0.167311930175506 \\
74.4897959183673	0.162329160164971 \\
74.8299319727891	0.159799013462972 \\
75.1700680272109	0.154667130280087 \\
75.5102040816327	0.149839214646561 \\
75.8503401360544	0.148035321943724 \\
76.1904761904762	0.143671877599088 \\
76.530612244898	0.141722528497125 \\
76.8707482993197	0.136792752921433 \\
77.2108843537415	0.135348121592245 \\
77.5510204081633	0.130654311867547 \\
77.891156462585	0.127053804190315 \\
78.2312925170068	0.124284980520483 \\
78.5714285714286	0.120832506251246 \\
78.9115646258503	0.117569285670219 \\
79.2517006802721	0.116332695104038 \\
79.5918367346939	0.113340296339637 \\
79.9319727891156	0.109818373228702 \\
80.2721088435374	0.107220895144868 \\
80.6122448979592	0.102507434309257 \\
80.9523809523809	0.10145471346547 \\
81.2925170068027	0.0982271201409519 \\
81.6326530612245	0.096357457227698 \\
81.9727891156463	0.0943798587974793 \\
82.312925170068	0.093959378990136 \\
82.6530612244898	0.0909112564844954 \\
82.9931972789116	0.0877135541341514 \\
83.3333333333333	0.0861454561679768 \\
83.6734693877551	0.0823118539514892 \\
84.0136054421769	0.080047028613696 \\
84.3537414965986	0.0779420965372089 \\
84.6938775510204	0.0746950894354154 \\
85.0340136054422	0.0729863802781919 \\
85.3741496598639	0.0702500718621314 \\
85.7142857142857	0.0678884937593647 \\
86.0544217687075	0.0665239549833489 \\
86.3945578231292	0.0625741711648912 \\
86.734693877551	0.0602295927825615 \\
87.0748299319728	0.0584322052213372 \\
87.4149659863945	0.0565044196527321 \\
87.7551020408163	0.0531267361563656 \\
88.0952380952381	0.0504670325253685 \\
88.4353741496599	0.0478381573292533 \\
88.7755102040816	0.0447790935926944 \\
89.1156462585034	0.0428229266700043 \\
89.4557823129252	0.0407649007400626 \\
89.7959183673469	0.0387147107801749 \\
90.1360544217687	0.0346275297334473 \\
90.4761904761905	0.0323357991225597 \\
90.8163265306122	0.030340635789666 \\
91.156462585034	0.0277552929947666 \\
91.4965986394558	0.0259181121189084 \\
91.8367346938775	0.023303222378914 \\
92.1768707482993	0.021117002532871 \\
92.5170068027211	0.0183584506779519 \\
92.8571428571429	0.016504033313148 \\
93.1972789115646	0.0156001119208674 \\
93.5374149659864	0.0144277519472443 \\
93.8775510204082	0.0131613213989747 \\
94.2176870748299	0.0115318931044429 \\
94.5578231292517	0.0109072071447219 \\
94.8979591836735	0.010308755079111 \\
95.2380952380952	0.0096306122856529 \\
95.578231292517	0.00890676622076462 \\
95.9183673469388	0.00788299970990688 \\
96.2585034013605	0.00681294378979775 \\
96.5986394557823	0.00597586225261562 \\
96.9387755102041	0.00506256799205644 \\
97.2789115646258	0.00418549834535192 \\
97.6190476190476	0.00353797340162646 \\
97.9591836734694	0.00274505708747951 \\
98.2993197278912	0.00245441373824005 \\
98.6394557823129	0.00177003555990204 \\
98.9795918367347	0.00134087998801007 \\
99.3197278911565	0.000457793790495247 \\
99.6598639455782	0.000152409737608401 \\
100	1.49018575257287e-13 \\
};
\path [fill=color6, fill opacity=0.25]
(axis cs:0,0.720596884928692)
--(axis cs:0,0.716905731119167)
--(axis cs:0.340136054421769,0.717480100824838)
--(axis cs:0.680272108843537,0.717441579680756)
--(axis cs:1.02040816326531,0.717531705537532)
--(axis cs:1.36054421768707,0.71758547045863)
--(axis cs:1.70068027210884,0.717642400422701)
--(axis cs:2.04081632653061,0.717586111289493)
--(axis cs:2.38095238095238,0.717382064185261)
--(axis cs:2.72108843537415,0.717650700049257)
--(axis cs:3.06122448979592,0.718252757634498)
--(axis cs:3.40136054421769,0.717782482171803)
--(axis cs:3.74149659863946,0.717792327102847)
--(axis cs:4.08163265306122,0.718668519856785)
--(axis cs:4.42176870748299,0.719270679395936)
--(axis cs:4.76190476190476,0.719360764661653)
--(axis cs:5.10204081632653,0.719060996344178)
--(axis cs:5.4421768707483,0.719468078167461)
--(axis cs:5.78231292517007,0.72041736090745)
--(axis cs:6.12244897959184,0.720360152342228)
--(axis cs:6.46258503401361,0.720405120782344)
--(axis cs:6.80272108843537,0.72078127355647)
--(axis cs:7.14285714285714,0.71984677398842)
--(axis cs:7.48299319727891,0.720073875932533)
--(axis cs:7.82312925170068,0.7203273421747)
--(axis cs:8.16326530612245,0.719990509848624)
--(axis cs:8.50340136054422,0.719427363304169)
--(axis cs:8.84353741496599,0.718756264520765)
--(axis cs:9.18367346938775,0.720296085208582)
--(axis cs:9.52380952380952,0.719461979899372)
--(axis cs:9.86394557823129,0.720644096965263)
--(axis cs:10.2040816326531,0.718973624233767)
--(axis cs:10.5442176870748,0.718662082571439)
--(axis cs:10.8843537414966,0.718562011272932)
--(axis cs:11.2244897959184,0.718351697672417)
--(axis cs:11.5646258503401,0.716373401141946)
--(axis cs:11.9047619047619,0.715799063742399)
--(axis cs:12.2448979591837,0.713946166495385)
--(axis cs:12.5850340136054,0.713091401326106)
--(axis cs:12.9251700680272,0.712322697998395)
--(axis cs:13.265306122449,0.711760733737655)
--(axis cs:13.6054421768707,0.710369626031788)
--(axis cs:13.9455782312925,0.709909009064896)
--(axis cs:14.2857142857143,0.707463327454716)
--(axis cs:14.6258503401361,0.706460663186661)
--(axis cs:14.9659863945578,0.705544476392685)
--(axis cs:15.3061224489796,0.704233453094023)
--(axis cs:15.6462585034014,0.70222141763856)
--(axis cs:15.9863945578231,0.700350451214746)
--(axis cs:16.3265306122449,0.698908292598466)
--(axis cs:16.6666666666667,0.697152006887153)
--(axis cs:17.0068027210884,0.695602794208923)
--(axis cs:17.3469387755102,0.691914334444304)
--(axis cs:17.687074829932,0.689520220889238)
--(axis cs:18.0272108843537,0.688270257317798)
--(axis cs:18.3673469387755,0.685333568886941)
--(axis cs:18.7074829931973,0.683364291313118)
--(axis cs:19.047619047619,0.682366543789916)
--(axis cs:19.3877551020408,0.679566807685149)
--(axis cs:19.7278911564626,0.678912259248375)
--(axis cs:20.0680272108844,0.675471678065387)
--(axis cs:20.4081632653061,0.672776315849712)
--(axis cs:20.7482993197279,0.671731372320872)
--(axis cs:21.0884353741497,0.668884500540414)
--(axis cs:21.4285714285714,0.667815769875406)
--(axis cs:21.7687074829932,0.66717115238204)
--(axis cs:22.108843537415,0.665569572834154)
--(axis cs:22.4489795918367,0.663939998046729)
--(axis cs:22.7891156462585,0.661507220396416)
--(axis cs:23.1292517006803,0.660004151570067)
--(axis cs:23.469387755102,0.658160806467175)
--(axis cs:23.8095238095238,0.656352161689187)
--(axis cs:24.1496598639456,0.655637436326803)
--(axis cs:24.4897959183673,0.652759546714124)
--(axis cs:24.8299319727891,0.651341133465761)
--(axis cs:25.1700680272109,0.649734007672551)
--(axis cs:25.5102040816327,0.649717458740722)
--(axis cs:25.8503401360544,0.647553118637904)
--(axis cs:26.1904761904762,0.646000270628617)
--(axis cs:26.530612244898,0.644578389708304)
--(axis cs:26.8707482993197,0.643290359352627)
--(axis cs:27.2108843537415,0.642424359878598)
--(axis cs:27.5510204081633,0.640769466258743)
--(axis cs:27.891156462585,0.639697826740107)
--(axis cs:28.2312925170068,0.638577450053353)
--(axis cs:28.5714285714286,0.636816036476433)
--(axis cs:28.9115646258503,0.634644009260359)
--(axis cs:29.2517006802721,0.632559234338863)
--(axis cs:29.5918367346939,0.630968961275376)
--(axis cs:29.9319727891156,0.629223634180366)
--(axis cs:30.2721088435374,0.628111544356521)
--(axis cs:30.6122448979592,0.626332287669984)
--(axis cs:30.952380952381,0.624463616191221)
--(axis cs:31.2925170068027,0.623997141950896)
--(axis cs:31.6326530612245,0.621733273695212)
--(axis cs:31.9727891156463,0.62001948785195)
--(axis cs:32.312925170068,0.616548052923641)
--(axis cs:32.6530612244898,0.614834624269642)
--(axis cs:32.9931972789116,0.612440966024497)
--(axis cs:33.3333333333333,0.610442343508657)
--(axis cs:33.6734693877551,0.608141164294497)
--(axis cs:34.0136054421769,0.606531367738481)
--(axis cs:34.3537414965986,0.605130189809706)
--(axis cs:34.6938775510204,0.603197337236597)
--(axis cs:35.0340136054422,0.599572751665863)
--(axis cs:35.3741496598639,0.597672465980641)
--(axis cs:35.7142857142857,0.596422049292979)
--(axis cs:36.0544217687075,0.593113889361758)
--(axis cs:36.3945578231292,0.59162813509839)
--(axis cs:36.734693877551,0.588413375625744)
--(axis cs:37.0748299319728,0.585458423924758)
--(axis cs:37.4149659863946,0.583906374229717)
--(axis cs:37.7551020408163,0.581001839694983)
--(axis cs:38.0952380952381,0.578215448797451)
--(axis cs:38.4353741496599,0.577624169906056)
--(axis cs:38.7755102040816,0.573437302472213)
--(axis cs:39.1156462585034,0.570179323225721)
--(axis cs:39.4557823129252,0.567565698673384)
--(axis cs:39.7959183673469,0.565225932868853)
--(axis cs:40.1360544217687,0.560021944261053)
--(axis cs:40.4761904761905,0.55813236668741)
--(axis cs:40.8163265306122,0.557414049114105)
--(axis cs:41.156462585034,0.552634067973955)
--(axis cs:41.4965986394558,0.549594507875017)
--(axis cs:41.8367346938776,0.547586450430108)
--(axis cs:42.1768707482993,0.543587698476608)
--(axis cs:42.5170068027211,0.541771158041329)
--(axis cs:42.8571428571429,0.536066751629425)
--(axis cs:43.1972789115646,0.532452264144433)
--(axis cs:43.5374149659864,0.529333411878619)
--(axis cs:43.8775510204082,0.526796578501272)
--(axis cs:44.2176870748299,0.522661959833773)
--(axis cs:44.5578231292517,0.518647950109614)
--(axis cs:44.8979591836735,0.514231321650032)
--(axis cs:45.2380952380952,0.511074866819823)
--(axis cs:45.578231292517,0.506045163558241)
--(axis cs:45.9183673469388,0.504045504156689)
--(axis cs:46.2585034013605,0.501127818780633)
--(axis cs:46.5986394557823,0.497338043220004)
--(axis cs:46.9387755102041,0.494123022031104)
--(axis cs:47.2789115646259,0.489813368963088)
--(axis cs:47.6190476190476,0.484558566868426)
--(axis cs:47.9591836734694,0.479170908158225)
--(axis cs:48.2993197278912,0.476595497187535)
--(axis cs:48.6394557823129,0.471118620450114)
--(axis cs:48.9795918367347,0.466631975463396)
--(axis cs:49.3197278911565,0.463497004435132)
--(axis cs:49.6598639455782,0.461080256389848)
--(axis cs:50,0.454575872715266)
--(axis cs:50.3401360544218,0.453102855801776)
--(axis cs:50.6802721088435,0.448196011664789)
--(axis cs:51.0204081632653,0.446199218220114)
--(axis cs:51.3605442176871,0.440526927396278)
--(axis cs:51.7006802721088,0.437515453469078)
--(axis cs:52.0408163265306,0.434619898093832)
--(axis cs:52.3809523809524,0.428773537669479)
--(axis cs:52.7210884353741,0.424056284083419)
--(axis cs:53.0612244897959,0.417285834150055)
--(axis cs:53.4013605442177,0.413113579211547)
--(axis cs:53.7414965986395,0.40992683490605)
--(axis cs:54.0816326530612,0.407460022873281)
--(axis cs:54.421768707483,0.401922960998878)
--(axis cs:54.7619047619048,0.397791898338175)
--(axis cs:55.1020408163265,0.393735889021132)
--(axis cs:55.4421768707483,0.389348909000515)
--(axis cs:55.7823129251701,0.386946913888505)
--(axis cs:56.1224489795918,0.382588340259116)
--(axis cs:56.4625850340136,0.376453511562514)
--(axis cs:56.8027210884354,0.371834220179487)
--(axis cs:57.1428571428571,0.369253876191239)
--(axis cs:57.4829931972789,0.364583346244829)
--(axis cs:57.8231292517007,0.362683437933076)
--(axis cs:58.1632653061224,0.357995171232499)
--(axis cs:58.5034013605442,0.35296160768544)
--(axis cs:58.843537414966,0.349116740566489)
--(axis cs:59.1836734693878,0.341094416626324)
--(axis cs:59.5238095238095,0.336856122946804)
--(axis cs:59.8639455782313,0.333819271358801)
--(axis cs:60.2040816326531,0.329682354919954)
--(axis cs:60.5442176870748,0.324043312830544)
--(axis cs:60.8843537414966,0.318158560483366)
--(axis cs:61.2244897959184,0.313293335121382)
--(axis cs:61.5646258503401,0.3093430919967)
--(axis cs:61.9047619047619,0.301956644976379)
--(axis cs:62.2448979591837,0.298263220752411)
--(axis cs:62.5850340136054,0.294985828857725)
--(axis cs:62.9251700680272,0.291059018274883)
--(axis cs:63.265306122449,0.287521196840046)
--(axis cs:63.6054421768707,0.284085902614175)
--(axis cs:63.9455782312925,0.277584078889669)
--(axis cs:64.2857142857143,0.274494015077703)
--(axis cs:64.6258503401361,0.270733377821663)
--(axis cs:64.9659863945578,0.264142233682603)
--(axis cs:65.3061224489796,0.261537194432731)
--(axis cs:65.6462585034014,0.255802505136075)
--(axis cs:65.9863945578231,0.25253927527488)
--(axis cs:66.3265306122449,0.249209201824458)
--(axis cs:66.6666666666667,0.244585632669391)
--(axis cs:67.0068027210884,0.240825244397048)
--(axis cs:67.3469387755102,0.235282441612859)
--(axis cs:67.687074829932,0.231642929786057)
--(axis cs:68.0272108843537,0.228145823578536)
--(axis cs:68.3673469387755,0.224968276136572)
--(axis cs:68.7074829931973,0.220665095142306)
--(axis cs:69.0476190476191,0.216502825408298)
--(axis cs:69.3877551020408,0.212680421691753)
--(axis cs:69.7278911564626,0.208051965519368)
--(axis cs:70.0680272108844,0.20543506948193)
--(axis cs:70.4081632653061,0.200302793978175)
--(axis cs:70.7482993197279,0.199088801866623)
--(axis cs:71.0884353741497,0.195638224404419)
--(axis cs:71.4285714285714,0.191879977904161)
--(axis cs:71.7687074829932,0.18972068493333)
--(axis cs:72.108843537415,0.184063750127485)
--(axis cs:72.4489795918367,0.178561165844801)
--(axis cs:72.7891156462585,0.177010835181861)
--(axis cs:73.1292517006803,0.173286057745915)
--(axis cs:73.469387755102,0.171684359807166)
--(axis cs:73.8095238095238,0.167300595442971)
--(axis cs:74.1496598639456,0.162131162414944)
--(axis cs:74.4897959183673,0.157326768569536)
--(axis cs:74.8299319727891,0.154977567247238)
--(axis cs:75.1700680272109,0.149796371214885)
--(axis cs:75.5102040816327,0.145054108989757)
--(axis cs:75.8503401360544,0.143302139823647)
--(axis cs:76.1904761904762,0.138946391951471)
--(axis cs:76.530612244898,0.137004616422052)
--(axis cs:76.8707482993197,0.132161145393417)
--(axis cs:77.2108843537415,0.13071012752399)
--(axis cs:77.5510204081633,0.126240324435794)
--(axis cs:77.891156462585,0.122588590361852)
--(axis cs:78.2312925170068,0.12017485181648)
--(axis cs:78.5714285714286,0.116851274272336)
--(axis cs:78.9115646258503,0.113468399357507)
--(axis cs:79.2517006802721,0.112533395241416)
--(axis cs:79.5918367346939,0.10951938842305)
--(axis cs:79.9319727891156,0.106322634883754)
--(axis cs:80.2721088435374,0.103673394388418)
--(axis cs:80.6122448979592,0.0992460677928642)
--(axis cs:80.9523809523809,0.0983652125152644)
--(axis cs:81.2925170068027,0.0951421921657019)
--(axis cs:81.6326530612245,0.0932306471308741)
--(axis cs:81.9727891156463,0.0915417932170807)
--(axis cs:82.312925170068,0.0910813386819932)
--(axis cs:82.6530612244898,0.0881350390319436)
--(axis cs:82.9931972789116,0.0848375771419706)
--(axis cs:83.3333333333333,0.0833425890996144)
--(axis cs:83.6734693877551,0.0795978926417031)
--(axis cs:84.0136054421769,0.0773448767256262)
--(axis cs:84.3537414965986,0.0752665212572264)
--(axis cs:84.6938775510204,0.0720694370271861)
--(axis cs:85.0340136054422,0.070433121608266)
--(axis cs:85.3741496598639,0.0676775723549031)
--(axis cs:85.7142857142857,0.0653248245404191)
--(axis cs:86.0544217687075,0.0639231144809833)
--(axis cs:86.3945578231292,0.0600571137345106)
--(axis cs:86.734693877551,0.0577414439084053)
--(axis cs:87.0748299319728,0.0560273762223326)
--(axis cs:87.4149659863945,0.0539879816254979)
--(axis cs:87.7551020408163,0.0506471008516437)
--(axis cs:88.0952380952381,0.048180408483391)
--(axis cs:88.4353741496599,0.0455831559984223)
--(axis cs:88.7755102040816,0.0424839860281133)
--(axis cs:89.1156462585034,0.0405244216484664)
--(axis cs:89.4557823129252,0.0386092955903492)
--(axis cs:89.7959183673469,0.0365756440432999)
--(axis cs:90.1360544217687,0.0325350444987315)
--(axis cs:90.4761904761905,0.0303656354317774)
--(axis cs:90.8163265306122,0.0283835077605864)
--(axis cs:91.156462585034,0.0260080257129604)
--(axis cs:91.4965986394558,0.0242348879068011)
--(axis cs:91.8367346938775,0.0217989791392109)
--(axis cs:92.1768707482993,0.0196605746954194)
--(axis cs:92.5170068027211,0.0170563895588576)
--(axis cs:92.8571428571429,0.0153578981717512)
--(axis cs:93.1972789115646,0.0145131539037452)
--(axis cs:93.5374149659864,0.0133883364753205)
--(axis cs:93.8775510204082,0.0122120071601127)
--(axis cs:94.2176870748299,0.0107281525045129)
--(axis cs:94.5578231292517,0.0100969198540317)
--(axis cs:94.8979591836735,0.00956560910451285)
--(axis cs:95.2380952380952,0.00892034997012923)
--(axis cs:95.578231292517,0.00821175901599173)
--(axis cs:95.9183673469388,0.00724416339078197)
--(axis cs:96.2585034013605,0.00627296700222845)
--(axis cs:96.5986394557823,0.00540555919183369)
--(axis cs:96.9387755102041,0.00456524018368247)
--(axis cs:97.2789115646258,0.00375534251291412)
--(axis cs:97.6190476190476,0.00313852733533734)
--(axis cs:97.9591836734694,0.002394291036587)
--(axis cs:98.2993197278912,0.00212447419497923)
--(axis cs:98.6394557823129,0.00150207190477588)
--(axis cs:98.9795918367347,0.00114010273701402)
--(axis cs:99.3197278911565,0.000361291540244638)
--(axis cs:99.6598639455782,0.000118580304732732)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,0.00018623917048407)
--(axis cs:99.3197278911565,0.000554296040745856)
--(axis cs:98.9795918367347,0.00154165723900611)
--(axis cs:98.6394557823129,0.0020379992150282)
--(axis cs:98.2993197278912,0.00278435328150088)
--(axis cs:97.9591836734694,0.00309582313837203)
--(axis cs:97.6190476190476,0.00393741946791558)
--(axis cs:97.2789115646258,0.00461565417778973)
--(axis cs:96.9387755102041,0.0055598958004304)
--(axis cs:96.5986394557823,0.00654616531339755)
--(axis cs:96.2585034013605,0.00735292057736704)
--(axis cs:95.9183673469388,0.0085218360290318)
--(axis cs:95.578231292517,0.00960177342553751)
--(axis cs:95.2380952380952,0.0103408746011766)
--(axis cs:94.8979591836735,0.0110519010537092)
--(axis cs:94.5578231292517,0.0117174944354121)
--(axis cs:94.2176870748299,0.0123356337043728)
--(axis cs:93.8775510204082,0.0141106356378367)
--(axis cs:93.5374149659864,0.0154671674191681)
--(axis cs:93.1972789115646,0.0166870699379896)
--(axis cs:92.8571428571429,0.0176501684545449)
--(axis cs:92.5170068027211,0.0196605117970463)
--(axis cs:92.1768707482993,0.0225734303703225)
--(axis cs:91.8367346938775,0.0248074656186172)
--(axis cs:91.4965986394558,0.0276013363310156)
--(axis cs:91.156462585034,0.0295025602765728)
--(axis cs:90.8163265306122,0.0322977638187455)
--(axis cs:90.4761904761905,0.0343059628133419)
--(axis cs:90.1360544217687,0.0367200149681632)
--(axis cs:89.7959183673469,0.0408537775170499)
--(axis cs:89.4557823129252,0.0429205058897761)
--(axis cs:89.1156462585034,0.0451214316915423)
--(axis cs:88.7755102040816,0.0470742011572754)
--(axis cs:88.4353741496599,0.0500931586600842)
--(axis cs:88.0952380952381,0.0527536565673461)
--(axis cs:87.7551020408163,0.0556063714610874)
--(axis cs:87.4149659863945,0.0590208576799663)
--(axis cs:87.0748299319728,0.0608370342203417)
--(axis cs:86.734693877551,0.0627177416567177)
--(axis cs:86.3945578231292,0.0650912285952717)
--(axis cs:86.0544217687075,0.0691247954857146)
--(axis cs:85.7142857142857,0.0704521629783104)
--(axis cs:85.3741496598639,0.0728225713693597)
--(axis cs:85.0340136054422,0.0755396389481177)
--(axis cs:84.6938775510204,0.0773207418436447)
--(axis cs:84.3537414965986,0.0806176718171914)
--(axis cs:84.0136054421769,0.0827491805017659)
--(axis cs:83.6734693877551,0.0850258152612754)
--(axis cs:83.3333333333333,0.0889483232363392)
--(axis cs:82.9931972789116,0.0905895311263321)
--(axis cs:82.6530612244898,0.0936874739370472)
--(axis cs:82.312925170068,0.0968374192982788)
--(axis cs:81.9727891156463,0.097217924377878)
--(axis cs:81.6326530612245,0.0994842673245219)
--(axis cs:81.2925170068027,0.101312048116202)
--(axis cs:80.9523809523809,0.104544214415676)
--(axis cs:80.6122448979592,0.10576880082565)
--(axis cs:80.2721088435374,0.110768395901319)
--(axis cs:79.9319727891156,0.11331411157365)
--(axis cs:79.5918367346939,0.117161204256223)
--(axis cs:79.2517006802721,0.120131994966661)
--(axis cs:78.9115646258503,0.121670171982931)
--(axis cs:78.5714285714286,0.124813738230157)
--(axis cs:78.2312925170068,0.128395109224487)
--(axis cs:77.891156462585,0.131519018018777)
--(axis cs:77.5510204081633,0.135068299299301)
--(axis cs:77.2108843537415,0.1399861156605)
--(axis cs:76.8707482993197,0.141424360449448)
--(axis cs:76.530612244898,0.146440440572198)
--(axis cs:76.1904761904762,0.148397363246704)
--(axis cs:75.8503401360544,0.152768504063801)
--(axis cs:75.5102040816327,0.154624320303365)
--(axis cs:75.1700680272109,0.159537889345289)
--(axis cs:74.8299319727891,0.164620459678706)
--(axis cs:74.4897959183673,0.167331551760406)
--(axis cs:74.1496598639456,0.172492697936068)
--(axis cs:73.8095238095238,0.177340555317347)
--(axis cs:73.469387755102,0.181665786617669)
--(axis cs:73.1292517006803,0.18336616928423)
--(axis cs:72.7891156462585,0.186824041283214)
--(axis cs:72.4489795918367,0.188451794274296)
--(axis cs:72.108843537415,0.19399131375209)
--(axis cs:71.7687074829932,0.199659168418028)
--(axis cs:71.4285714285714,0.201864685913931)
--(axis cs:71.0884353741497,0.205765362165683)
--(axis cs:70.7482993197279,0.209394117460329)
--(axis cs:70.4081632653061,0.210791218030933)
--(axis cs:70.0680272108844,0.215749693693892)
--(axis cs:69.7278911564626,0.218432453507393)
--(axis cs:69.3877551020408,0.223216963332001)
--(axis cs:69.0476190476191,0.227128328196942)
--(axis cs:68.7074829931973,0.231395283417361)
--(axis cs:68.3673469387755,0.235444305999878)
--(axis cs:68.0272108843537,0.23890482010992)
--(axis cs:67.687074829932,0.242226145529967)
--(axis cs:67.3469387755102,0.246416016896223)
--(axis cs:67.0068027210884,0.251750921722133)
--(axis cs:66.6666666666667,0.255172583131608)
--(axis cs:66.3265306122449,0.260184911705857)
--(axis cs:65.9863945578231,0.263824111425872)
--(axis cs:65.6462585034014,0.266994035401246)
--(axis cs:65.3061224489796,0.272801809118877)
--(axis cs:64.9659863945578,0.275989665814855)
--(axis cs:64.6258503401361,0.28259753771422)
--(axis cs:64.2857142857143,0.286266817800998)
--(axis cs:63.9455782312925,0.289292435951666)
--(axis cs:63.6054421768707,0.296043711245399)
--(axis cs:63.265306122449,0.299281767935367)
--(axis cs:62.9251700680272,0.303461849216273)
--(axis cs:62.5850340136054,0.307365227712331)
--(axis cs:62.2448979591837,0.310543968889496)
--(axis cs:61.9047619047619,0.314830236394154)
--(axis cs:61.5646258503401,0.321699199569926)
--(axis cs:61.2244897959184,0.326008524962412)
--(axis cs:60.8843537414966,0.330867096083363)
--(axis cs:60.5442176870748,0.336508667650118)
--(axis cs:60.2040816326531,0.342336411008723)
--(axis cs:59.8639455782313,0.346226283696455)
--(axis cs:59.5238095238095,0.34969658723213)
--(axis cs:59.1836734693878,0.35369752354263)
--(axis cs:58.843537414966,0.361727719989887)
--(axis cs:58.5034013605442,0.365602639830311)
--(axis cs:58.1632653061224,0.370339974752424)
--(axis cs:57.8231292517007,0.37461109951005)
--(axis cs:57.4829931972789,0.376901407840988)
--(axis cs:57.1428571428571,0.381399861181584)
--(axis cs:56.8027210884354,0.383862832321333)
--(axis cs:56.4625850340136,0.388389430851525)
--(axis cs:56.1224489795918,0.394567327718853)
--(axis cs:55.7823129251701,0.398702993811626)
--(axis cs:55.4421768707483,0.401600361784718)
--(axis cs:55.1020408163265,0.40530473085341)
--(axis cs:54.7619047619048,0.409468985467363)
--(axis cs:54.421768707483,0.413331436453898)
--(axis cs:54.0816326530612,0.419220779305044)
--(axis cs:53.7414965986395,0.42128017986786)
--(axis cs:53.4013605442177,0.424800089999057)
--(axis cs:53.0612244897959,0.428994837711299)
--(axis cs:52.7210884353741,0.435497107907114)
--(axis cs:52.3809523809524,0.440140493943725)
--(axis cs:52.0408163265306,0.445950027918872)
--(axis cs:51.7006802721088,0.448755191062604)
--(axis cs:51.3605442176871,0.451797314400247)
--(axis cs:51.0204081632653,0.457717600580514)
--(axis cs:50.6802721088435,0.459560879738844)
--(axis cs:50.3401360544218,0.464606860978415)
--(axis cs:50,0.466090895287389)
--(axis cs:49.6598639455782,0.472168898319031)
--(axis cs:49.3197278911565,0.475019128418031)
--(axis cs:48.9795918367347,0.478339219552024)
--(axis cs:48.6394557823129,0.482757801192386)
--(axis cs:48.2993197278912,0.488160567288427)
--(axis cs:47.9591836734694,0.490541631012303)
--(axis cs:47.6190476190476,0.496186785694022)
--(axis cs:47.2789115646259,0.501189048910053)
--(axis cs:46.9387755102041,0.505945391957115)
--(axis cs:46.5986394557823,0.508598239041374)
--(axis cs:46.2585034013605,0.512464145539842)
--(axis cs:45.9183673469388,0.515674061285894)
--(axis cs:45.578231292517,0.51763191598268)
--(axis cs:45.2380952380952,0.522667119127882)
--(axis cs:44.8979591836735,0.526010908513428)
--(axis cs:44.5578231292517,0.529916648336166)
--(axis cs:44.2176870748299,0.533983671900664)
--(axis cs:43.8775510204082,0.538073643210079)
--(axis cs:43.5374149659864,0.541022715276031)
--(axis cs:43.1972789115646,0.54408566018282)
--(axis cs:42.8571428571429,0.547550315647655)
--(axis cs:42.5170068027211,0.553150113721911)
--(axis cs:42.1768707482993,0.555000490479702)
--(axis cs:41.8367346938776,0.558723140792063)
--(axis cs:41.4965986394558,0.560347455488291)
--(axis cs:41.156462585034,0.563404844583659)
--(axis cs:40.8163265306122,0.568546599137716)
--(axis cs:40.4761904761905,0.569122303089275)
--(axis cs:40.1360544217687,0.570908623745144)
--(axis cs:39.7959183673469,0.575940502952398)
--(axis cs:39.4557823129252,0.578082793102826)
--(axis cs:39.1156462585034,0.580416739686215)
--(axis cs:38.7755102040816,0.58360397184253)
--(axis cs:38.4353741496599,0.588175316868847)
--(axis cs:38.0952380952381,0.588570003324389)
--(axis cs:37.7551020408163,0.591134423097718)
--(axis cs:37.4149659863946,0.59388493321657)
--(axis cs:37.0748299319728,0.595295122224332)
--(axis cs:36.734693877551,0.598264750821861)
--(axis cs:36.3945578231292,0.601573347284603)
--(axis cs:36.0544217687075,0.602867850095044)
--(axis cs:35.7142857142857,0.606229032026466)
--(axis cs:35.3741496598639,0.607614185204656)
--(axis cs:35.0340136054422,0.60924500028129)
--(axis cs:34.6938775510204,0.612407698990338)
--(axis cs:34.3537414965986,0.614836060675179)
--(axis cs:34.0136054421769,0.615946571696576)
--(axis cs:33.6734693877551,0.617659968299018)
--(axis cs:33.3333333333333,0.619906514346085)
--(axis cs:32.9931972789116,0.621678832324259)
--(axis cs:32.6530612244898,0.623639359559112)
--(axis cs:32.312925170068,0.625642888852239)
--(axis cs:31.9727891156463,0.628855365332675)
--(axis cs:31.6326530612245,0.630487918325248)
--(axis cs:31.2925170068027,0.632584237500286)
--(axis cs:30.952380952381,0.633011443563612)
--(axis cs:30.6122448979592,0.634696655186663)
--(axis cs:30.2721088435374,0.636324497022637)
--(axis cs:29.9319727891156,0.637312524036183)
--(axis cs:29.5918367346939,0.638941872654886)
--(axis cs:29.2517006802721,0.640547082758691)
--(axis cs:28.9115646258503,0.642487558384761)
--(axis cs:28.5714285714286,0.644427036258945)
--(axis cs:28.2312925170068,0.646353572704893)
--(axis cs:27.891156462585,0.647309692934264)
--(axis cs:27.5510204081633,0.648200046663888)
--(axis cs:27.2108843537415,0.649993732692718)
--(axis cs:26.8707482993197,0.650507440183633)
--(axis cs:26.530612244898,0.652162529100778)
--(axis cs:26.1904761904762,0.65353783913258)
--(axis cs:25.8503401360544,0.65515412709033)
--(axis cs:25.5102040816327,0.657140818417159)
--(axis cs:25.1700680272109,0.657394167549764)
--(axis cs:24.8299319727891,0.658780656574524)
--(axis cs:24.4897959183673,0.659852424224618)
--(axis cs:24.1496598639456,0.662975571673153)
--(axis cs:23.8095238095238,0.663712601737594)
--(axis cs:23.469387755102,0.665510247367085)
--(axis cs:23.1292517006803,0.66758613717331)
--(axis cs:22.7891156462585,0.668955529874547)
--(axis cs:22.4489795918367,0.671154043926623)
--(axis cs:22.108843537415,0.673197117285947)
--(axis cs:21.7687074829932,0.674713587463951)
--(axis cs:21.4285714285714,0.675280807500721)
--(axis cs:21.0884353741497,0.676285133384547)
--(axis cs:20.7482993197279,0.679062126135606)
--(axis cs:20.4081632653061,0.680432106811116)
--(axis cs:20.0680272108844,0.683248333198699)
--(axis cs:19.7278911564626,0.686718858721377)
--(axis cs:19.3877551020408,0.687530538352477)
--(axis cs:19.047619047619,0.690097875962443)
--(axis cs:18.7074829931973,0.690925218936974)
--(axis cs:18.3673469387755,0.692861099108035)
--(axis cs:18.0272108843537,0.695758756792767)
--(axis cs:17.687074829932,0.696886536048266)
--(axis cs:17.3469387755102,0.699095389099817)
--(axis cs:17.0068027210884,0.70233614154776)
--(axis cs:16.6666666666667,0.703885382450863)
--(axis cs:16.3265306122449,0.705514231972953)
--(axis cs:15.9863945578231,0.706899735288187)
--(axis cs:15.6462585034014,0.708601337161759)
--(axis cs:15.3061224489796,0.710211523951037)
--(axis cs:14.9659863945578,0.71162751865107)
--(axis cs:14.6258503401361,0.71259090561951)
--(axis cs:14.2857142857143,0.71331465621075)
--(axis cs:13.9455782312925,0.71576428798272)
--(axis cs:13.6054421768707,0.716063631428806)
--(axis cs:13.265306122449,0.7173364779213)
--(axis cs:12.9251700680272,0.717882739542613)
--(axis cs:12.5850340136054,0.718529361320092)
--(axis cs:12.2448979591837,0.719372833212313)
--(axis cs:11.9047619047619,0.721034754216433)
--(axis cs:11.5646258503401,0.721630633317645)
--(axis cs:11.2244897959184,0.723514728199432)
--(axis cs:10.8843537414966,0.72365707561252)
--(axis cs:10.5442176870748,0.723885033708163)
--(axis cs:10.2040816326531,0.724002460117773)
--(axis cs:9.86394557823129,0.725648803179791)
--(axis cs:9.52380952380952,0.72443103250507)
--(axis cs:9.18367346938775,0.725055360168291)
--(axis cs:8.84353741496599,0.723791592942595)
--(axis cs:8.50340136054422,0.724358290406196)
--(axis cs:8.16326530612245,0.72494315375802)
--(axis cs:7.82312925170068,0.725033101417372)
--(axis cs:7.48299319727891,0.724727040679616)
--(axis cs:7.14285714285714,0.724577375405616)
--(axis cs:6.80272108843537,0.725442148732425)
--(axis cs:6.46258503401361,0.725150791473897)
--(axis cs:6.12244897959184,0.724872841022106)
--(axis cs:5.78231292517007,0.724952302033052)
--(axis cs:5.4421768707483,0.723947517423607)
--(axis cs:5.10204081632653,0.723692409822853)
--(axis cs:4.76190476190476,0.723810643216746)
--(axis cs:4.42176870748299,0.723721872526862)
--(axis cs:4.08163265306122,0.723098104593899)
--(axis cs:3.74149659863946,0.722083198729329)
--(axis cs:3.40136054421769,0.722017127012462)
--(axis cs:3.06122448979592,0.722477946136616)
--(axis cs:2.72108843537415,0.721861068172598)
--(axis cs:2.38095238095238,0.721546737530113)
--(axis cs:2.04081632653061,0.721624458569059)
--(axis cs:1.70068027210884,0.72159603907763)
--(axis cs:1.36054421768707,0.721649850526687)
--(axis cs:1.02040816326531,0.721550586184766)
--(axis cs:0.680272108843537,0.721262618322059)
--(axis cs:0.340136054421769,0.721298367545599)
--(axis cs:0,0.720596884928692)
--cycle;


==> img/stl10/stl10_rate_distortion_shap.tex <==
% shap
\addplot [line width=0.5, opacity=0.8, color2, mark=diamond*, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color2, thin}]
table [row sep=\\]{%
0	0.718559694588184 \\
0.340136054421769	0.720991169214249 \\
0.680272108843537	0.723022782951593 \\
1.02040816326531	0.723585052192211 \\
1.36054421768707	0.723535033166409 \\
1.70068027210884	0.723695349693298 \\
2.04081632653061	0.72178868919611 \\
2.38095238095238	0.721653796732426 \\
2.72108843537415	0.721107279658318 \\
3.06122448979592	0.720995935201645 \\
3.40136054421769	0.718378976881504 \\
3.74149659863946	0.718009462952614 \\
4.08163265306122	0.717127349972725 \\
4.42176870748299	0.7162643840909 \\
4.76190476190476	0.712786825299263 \\
5.10204081632653	0.71206836104393 \\
5.4421768707483	0.711077454984188 \\
5.78231292517007	0.70941801816225 \\
6.12244897959184	0.707339471280575 \\
6.46258503401361	0.704877364933491 \\
6.80272108843537	0.704335144013166 \\
7.14285714285714	0.702245104014874 \\
7.48299319727891	0.700076788961887 \\
7.82312925170068	0.699769083410501 \\
8.16326530612245	0.697076096087694 \\
8.50340136054422	0.695684382021427 \\
8.84353741496599	0.69463962584734 \\
9.18367346938775	0.692013326883316 \\
9.52380952380952	0.691877473890781 \\
9.86394557823129	0.689245402216911 \\
10.2040816326531	0.686363837867975 \\
10.5442176870748	0.686112463474274 \\
10.8843537414966	0.683835508078337 \\
11.2244897959184	0.682390794456005 \\
11.5646258503401	0.680857224911451 \\
11.9047619047619	0.679383646845818 \\
12.2448979591837	0.679001146405935 \\
12.5850340136054	0.677476494759321 \\
12.9251700680272	0.676355916112661 \\
13.265306122449	0.675174967348576 \\
13.6054421768707	0.675004115998745 \\
13.9455782312925	0.674778108596802 \\
14.2857142857143	0.673442701101303 \\
14.6258503401361	0.674166747331619 \\
14.9659863945578	0.672335609346628 \\
15.3061224489796	0.672319289147854 \\
15.6462585034014	0.672515113800764 \\
15.9863945578231	0.671279993057251 \\
16.3265306122449	0.670307406336069 \\
16.6666666666667	0.668747382164001 \\
17.0068027210884	0.668625494241714 \\
17.3469387755102	0.668185752630234 \\
17.687074829932	0.667472068667412 \\
18.0272108843537	0.666583871692419 \\
18.3673469387755	0.666199113428593 \\
18.7074829931973	0.664980872571468 \\
19.047619047619	0.664636908173561 \\
19.3877551020408	0.664065761119127 \\
19.7278911564626	0.663479780480266 \\
20.0680272108844	0.661539456322789 \\
20.4081632653061	0.662867039591074 \\
20.7482993197279	0.662041606232524 \\
21.0884353741497	0.661629022359848 \\
21.4285714285714	0.661596494913101 \\
21.7687074829932	0.660079896301031 \\
22.108843537415	0.659657060466707 \\
22.4489795918367	0.658361746966839 \\
22.7891156462585	0.658918049409986 \\
23.1292517006803	0.656737769246101 \\
23.469387755102	0.656425706893206 \\
23.8095238095238	0.655098212435842 \\
24.1496598639456	0.654394746683538 \\
24.4897959183673	0.65418120097369 \\
24.8299319727891	0.653000528626144 \\
25.1700680272109	0.65129389218986 \\
25.5102040816327	0.649407686516643 \\
25.8503401360544	0.649005069620907 \\
26.1904761904762	0.6465733153373 \\
26.530612244898	0.646467348709702 \\
26.8707482993197	0.645659059174359 \\
27.2108843537415	0.643797406684607 \\
27.5510204081633	0.643099542725831 \\
27.891156462585	0.643853562511504 \\
28.2312925170068	0.642378135528415 \\
28.5714285714286	0.641272455267608 \\
28.9115646258503	0.641383976377547 \\
29.2517006802721	0.641127799227834 \\
29.5918367346939	0.639748621275648 \\
29.9319727891156	0.639478558711708 \\
30.2721088435374	0.638594243321568 \\
30.6122448979592	0.637509988890961 \\
30.952380952381	0.63667931416072 \\
31.2925170068027	0.635020208042115 \\
31.6326530612245	0.634427774585783 \\
31.9727891156463	0.633552961852402 \\
32.312925170068	0.63147647542879 \\
32.6530612244898	0.632153407642618 \\
32.9931972789116	0.631714366786182 \\
33.3333333333333	0.629797367816791 \\
33.6734693877551	0.629233624748886 \\
34.0136054421769	0.628513042833656 \\
34.3537414965986	0.628599236570299 \\
34.6938775510204	0.627813480459154 \\
35.0340136054422	0.626007760558277 \\
35.3741496598639	0.625587605498731 \\
35.7142857142857	0.623797435052693 \\
36.0544217687075	0.623937089447863 \\
36.3945578231292	0.62418196643237 \\
36.734693877551	0.623216553642414 \\
37.0748299319728	0.62170825489331 \\
37.4149659863946	0.621931088780984 \\
37.7551020408163	0.619473029347137 \\
38.0952380952381	0.619192903493531 \\
38.4353741496599	0.617569787465036 \\
38.7755102040816	0.616751112635247 \\
39.1156462585034	0.618295597666874 \\
39.4557823129252	0.615490632718429 \\
39.7959183673469	0.615063146925531 \\
40.1360544217687	0.613769199927337 \\
40.4761904761905	0.614809612506069 \\
40.8163265306122	0.61355551202083 \\
41.156462585034	0.612347051464021 \\
41.4965986394558	0.611262736197095 \\
41.8367346938776	0.611028520893306 \\
42.1768707482993	0.609961816766299 \\
42.5170068027211	0.609287713291124 \\
42.8571428571429	0.608431811374612 \\
43.1972789115646	0.606498402475845 \\
43.5374149659864	0.607487944978056 \\
43.8775510204082	0.605086130924756 \\
44.2176870748299	0.604173060043249 \\
44.5578231292517	0.605441335233627 \\
44.8979591836735	0.604656228169333 \\
45.2380952380952	0.603292701073224 \\
45.578231292517	0.599937897099298 \\
45.9183673469388	0.599479999435716 \\
46.2585034013605	0.598765237532789 \\
46.5986394557823	0.597715685678413 \\
46.9387755102041	0.597689152505482 \\
47.2789115646259	0.596370346288895 \\
47.6190476190476	0.596372189352987 \\
47.9591836734694	0.595486457181396 \\
48.2993197278912	0.593668337968993 \\
48.6394557823129	0.59373859252315 \\
48.9795918367347	0.591934012646088 \\
49.3197278911565	0.591908301110088 \\
49.6598639455782	0.590981975696632 \\
50	0.590651764892973 \\
50.3401360544218	0.590731643784384 \\
50.6802721088435	0.590048775043106 \\
51.0204081632653	0.587638746490702 \\
51.3605442176871	0.586939477052074 \\
51.7006802721088	0.585700196846155 \\
52.0408163265306	0.585107595228765 \\
52.3809523809524	0.582844338477298 \\
52.7210884353741	0.581938458169752 \\
53.0612244897959	0.583341762328346 \\
53.4013605442177	0.580344735605613 \\
53.7414965986395	0.581007804140827 \\
54.0816326530612	0.578648515695968 \\
54.421768707483	0.577950191391574 \\
54.7619047619048	0.576398880329798 \\
55.1020408163265	0.575594016842224 \\
55.4421768707483	0.574458407196507 \\
55.7823129251701	0.574470180294011 \\
56.1224489795918	0.572059736170631 \\
56.4625850340136	0.572039909899904 \\
56.8027210884354	0.570693238423846 \\
57.1428571428571	0.569491093377183 \\
57.4829931972789	0.568645434095233 \\
57.8231292517007	0.56882910380562 \\
58.1632653061224	0.566655622021135 \\
58.5034013605442	0.56433558161094 \\
58.843537414966	0.565332992798612 \\
59.1836734693878	0.563255688504978 \\
59.5238095238095	0.561112261345334 \\
59.8639455782313	0.56035220474314 \\
60.2040816326531	0.559391268899744 \\
60.5442176870748	0.558139933349521 \\
60.8843537414966	0.556432424244958 \\
61.2244897959184	0.554605697528332 \\
61.5646258503401	0.55262028673149 \\
61.9047619047619	0.550978115792823 \\
62.2448979591837	0.550579526496986 \\
62.5850340136054	0.54860910617369 \\
62.9251700680272	0.547419280525937 \\
63.265306122449	0.545171905995685 \\
63.6054421768707	0.545589804954652 \\
63.9455782312925	0.542401295391605 \\
64.2857142857143	0.542111285158044 \\
64.6258503401361	0.539427033431784 \\
64.9659863945578	0.537935345509686 \\
65.3061224489796	0.536854968429507 \\
65.6462585034014	0.534092929360029 \\
65.9863945578231	0.532835078063449 \\
66.3265306122449	0.531699556293966 \\
66.6666666666667	0.529834354892111 \\
67.0068027210884	0.528741097092634 \\
67.3469387755102	0.526161451200151 \\
67.687074829932	0.52391772853996 \\
68.0272108843537	0.521247554687258 \\
68.3673469387755	0.52099826293187 \\
68.7074829931973	0.518906032008804 \\
69.0476190476191	0.517381288501396 \\
69.3877551020408	0.515124000835142 \\
69.7278911564626	0.512464173419545 \\
70.0680272108844	0.510808588619146 \\
70.4081632653061	0.509286775550925 \\
70.7482993197279	0.507927963948986 \\
71.0884353741497	0.506431196957491 \\
71.4285714285714	0.504025897548248 \\
71.7687074829932	0.50171398382172 \\
72.108843537415	0.499318161319049 \\
72.4489795918367	0.496133796294474 \\
72.7891156462585	0.494024357825287 \\
73.1292517006803	0.492601150235654 \\
73.469387755102	0.490185533412199 \\
73.8095238095238	0.489117766309544 \\
74.1496598639456	0.485433111117019 \\
74.4897959183673	0.483543084351303 \\
74.8299319727891	0.482915168689682 \\
75.1700680272109	0.480310951997949 \\
75.5102040816327	0.47834764901366 \\
75.8503401360544	0.475287721993189 \\
76.1904761904762	0.473273206930226 \\
76.530612244898	0.469438000257805 \\
76.8707482993197	0.466847345424541 \\
77.2108843537415	0.463390909084748 \\
77.5510204081633	0.46360938228422 \\
77.891156462585	0.459964212367092 \\
78.2312925170068	0.457454177881279 \\
78.5714285714286	0.455006401464511 \\
78.9115646258503	0.453580110738209 \\
79.2517006802721	0.451474843963409 \\
79.5918367346939	0.446551121087261 \\
79.9319727891156	0.445491513078161 \\
80.2721088435374	0.441544641429293 \\
80.6122448979592	0.438565659482919 \\
80.9523809523809	0.433956253340671 \\
81.2925170068027	0.430438032088101 \\
81.6326530612245	0.425731652228327 \\
81.9727891156463	0.422147679510597 \\
82.312925170068	0.417578910942621 \\
82.6530612244898	0.417686180220624 \\
82.9931972789116	0.412303313626895 \\
83.3333333333333	0.410528223603272 \\
83.6734693877551	0.407187924833285 \\
84.0136054421769	0.4027579395085 \\
84.3537414965986	0.399456256069075 \\
84.6938775510204	0.395537463650151 \\
85.0340136054422	0.391726504820907 \\
85.3741496598639	0.388048783109042 \\
85.7142857142857	0.383802939668759 \\
86.0544217687075	0.375462416669076 \\
86.3945578231292	0.371482936688106 \\
86.734693877551	0.36396905150232 \\
87.0748299319728	0.357969954225762 \\
87.4149659863945	0.349816747797515 \\
87.7551020408163	0.343990060889953 \\
88.0952380952381	0.337397654864785 \\
88.4353741496599	0.329290455211922 \\
88.7755102040816	0.319258891760524 \\
89.1156462585034	0.309613445675854 \\
89.4557823129252	0.301039923228554 \\
89.7959183673469	0.288676983145441 \\
90.1360544217687	0.280666857382381 \\
90.4761904761905	0.269360084183023 \\
90.8163265306122	0.257253591659179 \\
91.156462585034	0.249637840463692 \\
91.4965986394558	0.239552771060313 \\
91.8367346938775	0.230344090528734 \\
92.1768707482993	0.218305891191144 \\
92.5170068027211	0.206832419685127 \\
92.8571428571429	0.195387036364791 \\
93.1972789115646	0.184361056296607 \\
93.5374149659864	0.17613108813527 \\
93.8775510204082	0.167019865931299 \\
94.2176870748299	0.16014453914383 \\
94.5578231292517	0.154557663306521 \\
94.8979591836735	0.14583307947923 \\
95.2380952380952	0.140667536154648 \\
95.578231292517	0.131995306589213 \\
95.9183673469388	0.122369230854625 \\
96.2585034013605	0.114285971627648 \\
96.5986394557823	0.105761467431191 \\
96.9387755102041	0.0965644187395783 \\
97.2789115646258	0.085107593866844 \\
97.6190476190476	0.0756687295697953 \\
97.9591836734694	0.0666245076872797 \\
98.2993197278912	0.0587527510464245 \\
98.6394557823129	0.0490243814145298 \\
98.9795918367347	0.0417514685993025 \\
99.3197278911565	0.0251882160485456 \\
99.6598639455782	0.0109402570453639 \\
100	1.49018575257287e-13 \\
};
\path [fill=color2, fill opacity=0.5] (axis cs:0,0.720430770721294)
--(axis cs:0,0.716688618455075)
--(axis cs:0.340136054421769,0.719130536788148)
--(axis cs:0.680272108843537,0.72107225928733)
--(axis cs:1.02040816326531,0.721566952765931)
--(axis cs:1.36054421768707,0.721423250370411)
--(axis cs:1.70068027210884,0.72156745068669)
--(axis cs:2.04081632653061,0.719567047680701)
--(axis cs:2.38095238095238,0.719349244946172)
--(axis cs:2.72108843537415,0.718748151799896)
--(axis cs:3.06122448979592,0.718590790394427)
--(axis cs:3.40136054421769,0.715906345077125)
--(axis cs:3.74149659863946,0.715511714289541)
--(axis cs:4.08163265306122,0.714506899638651)
--(axis cs:4.42176870748299,0.713655825741879)
--(axis cs:4.76190476190476,0.710003120704394)
--(axis cs:5.10204081632653,0.709234568463691)
--(axis cs:5.4421768707483,0.708154283793194)
--(axis cs:5.78231292517007,0.706484720147221)
--(axis cs:6.12244897959184,0.704225131311251)
--(axis cs:6.46258503401361,0.701823657866226)
--(axis cs:6.80272108843537,0.701067489936489)
--(axis cs:7.14285714285714,0.69895181309474)
--(axis cs:7.48299319727891,0.696664850927741)
--(axis cs:7.82312925170068,0.696203924862812)
--(axis cs:8.16326530612245,0.693526700657356)
--(axis cs:8.50340136054422,0.692133246463937)
--(axis cs:8.84353741496599,0.690953906661116)
--(axis cs:9.18367346938775,0.688309344101899)
--(axis cs:9.52380952380952,0.688185937214059)
--(axis cs:9.86394557823129,0.685483930366285)
--(axis cs:10.2040816326531,0.682489115122805)
--(axis cs:10.5442176870748,0.682292993492039)
--(axis cs:10.8843537414966,0.679899402006389)
--(axis cs:11.2244897959184,0.678504015805153)
--(axis cs:11.5646258503401,0.676947186121407)
--(axis cs:11.9047619047619,0.675490610801932)
--(axis cs:12.2448979591837,0.675081350367877)
--(axis cs:12.5850340136054,0.67357006914658)
--(axis cs:12.9251700680272,0.67225435265648)
--(axis cs:13.265306122449,0.671080079162366)
--(axis cs:13.6054421768707,0.671137191981066)
--(axis cs:13.9455782312925,0.670825061111307)
--(axis cs:14.2857142857143,0.669254950729699)
--(axis cs:14.6258503401361,0.670135250986297)
--(axis cs:14.9659863945578,0.668225588791133)
--(axis cs:15.3061224489796,0.668329701511003)
--(axis cs:15.6462585034014,0.668598736682685)
--(axis cs:15.9863945578231,0.667350816726265)
--(axis cs:16.3265306122449,0.666207224711642)
--(axis cs:16.6666666666667,0.664751289292129)
--(axis cs:17.0068027210884,0.664459068090617)
--(axis cs:17.3469387755102,0.663873337798065)
--(axis cs:17.687074829932,0.663333521335322)
--(axis cs:18.0272108843537,0.662316829602854)
--(axis cs:18.3673469387755,0.662089751673432)
--(axis cs:18.7074829931973,0.660818888059852)
--(axis cs:19.047619047619,0.660351426798501)
--(axis cs:19.3877551020408,0.659714126184626)
--(axis cs:19.7278911564626,0.659371438396515)
--(axis cs:20.0680272108844,0.657362769160278)
--(axis cs:20.4081632653061,0.658578516421794)
--(axis cs:20.7482993197279,0.657933661352283)
--(axis cs:21.0884353741497,0.657383462494023)
--(axis cs:21.4285714285714,0.657279526554858)
--(axis cs:21.7687074829932,0.655798830342317)
--(axis cs:22.108843537415,0.655289241396651)
--(axis cs:22.4489795918367,0.654017228284948)
--(axis cs:22.7891156462585,0.654454897728753)
--(axis cs:23.1292517006803,0.652384013799895)
--(axis cs:23.469387755102,0.652087003765578)
--(axis cs:23.8095238095238,0.650687676514041)
--(axis cs:24.1496598639456,0.649955551051369)
--(axis cs:24.4897959183673,0.649817599451225)
--(axis cs:24.8299319727891,0.648445859822091)
--(axis cs:25.1700680272109,0.64687638420822)
--(axis cs:25.5102040816327,0.644972369452727)
--(axis cs:25.8503401360544,0.644417112943403)
--(axis cs:26.1904761904762,0.642134896483512)
--(axis cs:26.530612244898,0.641932346548417)
--(axis cs:26.8707482993197,0.641089377344687)
--(axis cs:27.2108843537415,0.639126467462191)
--(axis cs:27.5510204081633,0.638491774140526)
--(axis cs:27.891156462585,0.639170600363553)
--(axis cs:28.2312925170068,0.637757011545739)
--(axis cs:28.5714285714286,0.636543736671823)
--(axis cs:28.9115646258503,0.636609747648848)
--(axis cs:29.2517006802721,0.636305369346269)
--(axis cs:29.5918367346939,0.635128261847288)
--(axis cs:29.9319727891156,0.634782514017103)
--(axis cs:30.2721088435374,0.633876800924004)
--(axis cs:30.6122448979592,0.632792388783463)
--(axis cs:30.952380952381,0.63188663123334)
--(axis cs:31.2925170068027,0.63016940284781)
--(axis cs:31.6326530612245,0.629815912417951)
--(axis cs:31.9727891156463,0.628871829814691)
--(axis cs:32.312925170068,0.626601649587088)
--(axis cs:32.6530612244898,0.627289557924783)
--(axis cs:32.9931972789116,0.626948742340821)
--(axis cs:33.3333333333333,0.62487232712618)
--(axis cs:33.6734693877551,0.624307203631728)
--(axis cs:34.0136054421769,0.623772383745266)
--(axis cs:34.3537414965986,0.623856037374552)
--(axis cs:34.6938775510204,0.622915579568864)
--(axis cs:35.0340136054422,0.621308380870712)
--(axis cs:35.3741496598639,0.620667406340641)
--(axis cs:35.7142857142857,0.619062774296456)
--(axis cs:36.0544217687075,0.619150098086064)
--(axis cs:36.3945578231292,0.619431125906911)
--(axis cs:36.734693877551,0.61830721791341)
--(axis cs:37.0748299319728,0.616925342164632)
--(axis cs:37.4149659863946,0.617087642694037)
--(axis cs:37.7551020408163,0.614649995126778)
--(axis cs:38.0952380952381,0.614120033040441)
--(axis cs:38.4353741496599,0.612711579539836)
--(axis cs:38.7755102040816,0.611744586578641)
--(axis cs:39.1156462585034,0.613364508390927)
--(axis cs:39.4557823129252,0.610599023041432)
--(axis cs:39.7959183673469,0.610260946632609)
--(axis cs:40.1360544217687,0.608883391531886)
--(axis cs:40.4761904761905,0.609845671543713)
--(axis cs:40.8163265306122,0.608757460008075)
--(axis cs:41.156462585034,0.607453513266231)
--(axis cs:41.4965986394558,0.606503772732378)
--(axis cs:41.8367346938776,0.606124386713607)
--(axis cs:42.1768707482993,0.604912459670335)
--(axis cs:42.5170068027211,0.604363747864482)
--(axis cs:42.8571428571429,0.60342537080279)
--(axis cs:43.1972789115646,0.601581470345)
--(axis cs:43.5374149659864,0.602576113107939)
--(axis cs:43.8775510204082,0.600202347322668)
--(axis cs:44.2176870748299,0.599193703531359)
--(axis cs:44.5578231292517,0.600540118110416)
--(axis cs:44.8979591836735,0.599761741822732)
--(axis cs:45.2380952380952,0.598324285459796)
--(axis cs:45.578231292517,0.594909345540329)
--(axis cs:45.9183673469388,0.594582532714151)
--(axis cs:46.2585034013605,0.593797636584956)
--(axis cs:46.5986394557823,0.592828347402375)
--(axis cs:46.9387755102041,0.592727350114175)
--(axis cs:47.2789115646259,0.591407118419644)
--(axis cs:47.6190476190476,0.591431884513838)
--(axis cs:47.9591836734694,0.590556796930679)
--(axis cs:48.2993197278912,0.588788539987225)
--(axis cs:48.6394557823129,0.588788086435661)
--(axis cs:48.9795918367347,0.587129745469389)
--(axis cs:49.3197278911565,0.586854327887687)
--(axis cs:49.6598639455782,0.585981733162073)
--(axis cs:50,0.585611396153215)
--(axis cs:50.3401360544218,0.585659333677965)
--(axis cs:50.6802721088435,0.585073085132081)
--(axis cs:51.0204081632653,0.582554790002973)
--(axis cs:51.3605442176871,0.581993463536694)
--(axis cs:51.7006802721088,0.580625493049455)
--(axis cs:52.0408163265306,0.579978207145443)
--(axis cs:52.3809523809524,0.577685915826982)
--(axis cs:52.7210884353741,0.57673670654103)
--(axis cs:53.0612244897959,0.578477950981518)
--(axis cs:53.4013605442177,0.57516254715667)
--(axis cs:53.7414965986395,0.576031219163092)
--(axis cs:54.0816326530612,0.573526302238566)
--(axis cs:54.421768707483,0.572765257379478)
--(axis cs:54.7619047619048,0.571240518389189)
--(axis cs:55.1020408163265,0.570598611483249)
--(axis cs:55.4421768707483,0.569402324058735)
--(axis cs:55.7823129251701,0.569377839211288)
--(axis cs:56.1224489795918,0.56691142721139)
--(axis cs:56.4625850340136,0.567011034803268)
--(axis cs:56.8027210884354,0.565525586147587)
--(axis cs:57.1428571428571,0.564196555007455)
--(axis cs:57.4829931972789,0.563709208287295)
--(axis cs:57.8231292517007,0.563658504542495)
--(axis cs:58.1632653061224,0.56155731017799)
--(axis cs:58.5034013605442,0.559279021543202)
--(axis cs:58.843537414966,0.560153167743003)
--(axis cs:59.1836734693878,0.558072855947651)
--(axis cs:59.5238095238095,0.556060643343994)
--(axis cs:59.8639455782313,0.555272619074812)
--(axis cs:60.2040816326531,0.554153903760344)
--(axis cs:60.5442176870748,0.55285897350089)
--(axis cs:60.8843537414966,0.551189635083614)
--(axis cs:61.2244897959184,0.549454112353392)
--(axis cs:61.5646258503401,0.547514580592481)
--(axis cs:61.9047619047619,0.545821032739493)
--(axis cs:62.2448979591837,0.545406418224867)
--(axis cs:62.5850340136054,0.543331106381551)
--(axis cs:62.9251700680272,0.542248786531998)
--(axis cs:63.265306122449,0.54004609686339)
--(axis cs:63.6054421768707,0.540309725047243)
--(axis cs:63.9455782312925,0.537265119178449)
--(axis cs:64.2857142857143,0.536990931899217)
--(axis cs:64.6258503401361,0.534254976379675)
--(axis cs:64.9659863945578,0.532815466627175)
--(axis cs:65.3061224489796,0.531581447586784)
--(axis cs:65.6462585034014,0.528810902473177)
--(axis cs:65.9863945578231,0.527642422185018)
--(axis cs:66.3265306122449,0.526575279495906)
--(axis cs:66.6666666666667,0.524719771715312)
--(axis cs:67.0068027210884,0.523562410560075)
--(axis cs:67.3469387755102,0.521092199614642)
--(axis cs:67.687074829932,0.518728367783525)
--(axis cs:68.0272108843537,0.516215156926631)
--(axis cs:68.3673469387755,0.515766046172549)
--(axis cs:68.7074829931973,0.513826278547385)
--(axis cs:69.0476190476191,0.512118499518034)
--(axis cs:69.3877551020408,0.509961421122378)
--(axis cs:69.7278911564626,0.507362693835719)
--(axis cs:70.0680272108844,0.505718110983638)
--(axis cs:70.4081632653061,0.504121618805904)
--(axis cs:70.7482993197279,0.502763627267677)
--(axis cs:71.0884353741497,0.501122136597446)
--(axis cs:71.4285714285714,0.498755771904899)
--(axis cs:71.7687074829932,0.496586098511002)
--(axis cs:72.108843537415,0.494071311473195)
--(axis cs:72.4489795918367,0.490836756217577)
--(axis cs:72.7891156462585,0.48876052148849)
--(axis cs:73.1292517006803,0.487412351122473)
--(axis cs:73.469387755102,0.484873398614131)
--(axis cs:73.8095238095238,0.48394659659456)
--(axis cs:74.1496598639456,0.479890002622246)
--(axis cs:74.4897959183673,0.478278926448589)
--(axis cs:74.8299319727891,0.477641326220911)
--(axis cs:75.1700680272109,0.474992329549288)
--(axis cs:75.5102040816327,0.472843235309213)
--(axis cs:75.8503401360544,0.46987119783539)
--(axis cs:76.1904761904762,0.467797125671838)
--(axis cs:76.530612244898,0.464043248643748)
--(axis cs:76.8707482993197,0.461374876949293)
--(axis cs:77.2108843537415,0.457781999762448)
--(axis cs:77.5510204081633,0.458245397894083)
--(axis cs:77.891156462585,0.45440606826811)
--(axis cs:78.2312925170068,0.451765906935481)
--(axis cs:78.5714285714286,0.449424700598873)
--(axis cs:78.9115646258503,0.447745705506613)
--(axis cs:79.2517006802721,0.445853003368616)
--(axis cs:79.5918367346939,0.440935857987813)
--(axis cs:79.9319727891156,0.439751615785679)
--(axis cs:80.2721088435374,0.436088803516639)
--(axis cs:80.6122448979592,0.432870068676151)
--(axis cs:80.9523809523809,0.428345478044909)
--(axis cs:81.2925170068027,0.42485344890479)
--(axis cs:81.6326530612245,0.420264052953648)
--(axis cs:81.9727891156463,0.416559175732244)
--(axis cs:82.312925170068,0.412091478838543)
--(axis cs:82.6530612244898,0.412147344151348)
--(axis cs:82.9931972789116,0.406792833123282)
--(axis cs:83.3333333333333,0.404780913737302)
--(axis cs:83.6734693877551,0.401691419583294)
--(axis cs:84.0136054421769,0.396896063430282)
--(axis cs:84.3537414965986,0.393754363681484)
--(axis cs:84.6938775510204,0.389692019227528)
--(axis cs:85.0340136054422,0.385999709928824)
--(axis cs:85.3741496598639,0.382207303433806)
--(axis cs:85.7142857142857,0.377859141333908)
--(axis cs:86.0544217687075,0.369618053790068)
--(axis cs:86.3945578231292,0.365611808769839)
--(axis cs:86.734693877551,0.357992456341367)
--(axis cs:87.0748299319728,0.351899656511836)
--(axis cs:87.4149659863945,0.343742406835617)
--(axis cs:87.7551020408163,0.337970513806033)
--(axis cs:88.0952380952381,0.33132038596351)
--(axis cs:88.4353741496599,0.3231567233592)
--(axis cs:88.7755102040816,0.313172073795647)
--(axis cs:89.1156462585034,0.303579512253266)
--(axis cs:89.4557823129252,0.295019710888429)
--(axis cs:89.7959183673469,0.283008367031957)
--(axis cs:90.1360544217687,0.274966633479034)
--(axis cs:90.4761904761905,0.263810047090474)
--(axis cs:90.8163265306122,0.252094700751526)
--(axis cs:91.156462585034,0.244711630589143)
--(axis cs:91.4965986394558,0.234519440361541)
--(axis cs:91.8367346938775,0.2254569820035)
--(axis cs:92.1768707482993,0.213479576078836)
--(axis cs:92.5170068027211,0.202133168771415)
--(axis cs:92.8571428571429,0.190788571903117)
--(axis cs:93.1972789115646,0.180006242120924)
--(axis cs:93.5374149659864,0.171993900458006)
--(axis cs:93.8775510204082,0.163251856733322)
--(axis cs:94.2176870748299,0.156445913193768)
--(axis cs:94.5578231292517,0.150892419776378)
--(axis cs:94.8979591836735,0.142159063676496)
--(axis cs:95.2380952380952,0.137126189993948)
--(axis cs:95.578231292517,0.128432882865534)
--(axis cs:95.9183673469388,0.119037827348617)
--(axis cs:96.2585034013605,0.11127897488622)
--(axis cs:96.5986394557823,0.102852501558417)
--(axis cs:96.9387755102041,0.093921630770679)
--(axis cs:97.2789115646258,0.0827163010466295)
--(axis cs:97.6190476190476,0.0734271710584359)
--(axis cs:97.9591836734694,0.0643173018064577)
--(axis cs:98.2993197278912,0.0563655677969764)
--(axis cs:98.6394557823129,0.046373104899489)
--(axis cs:98.9795918367347,0.0392787407921252)
--(axis cs:99.3197278911565,0.0224613217652798)
--(axis cs:99.6598639455782,0.00952157796588592)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,0.0123589361248419)
--(axis cs:99.3197278911565,0.0279151103318115)
--(axis cs:98.9795918367347,0.0442241964064798)
--(axis cs:98.6394557823129,0.0516756579295706)
--(axis cs:98.2993197278912,0.0611399342958726)
--(axis cs:97.9591836734694,0.0689317135681018)
--(axis cs:97.6190476190476,0.0779102880811547)
--(axis cs:97.2789115646258,0.0874988866870584)
--(axis cs:96.9387755102041,0.0992072067084776)
--(axis cs:96.5986394557823,0.108670433303965)
--(axis cs:96.2585034013605,0.117292968369076)
--(axis cs:95.9183673469388,0.125700634360633)
--(axis cs:95.578231292517,0.135557730312892)
--(axis cs:95.2380952380952,0.144208882315348)
--(axis cs:94.8979591836735,0.149507095281964)
--(axis cs:94.5578231292517,0.158222906836665)
--(axis cs:94.2176870748299,0.163843165093892)
--(axis cs:93.8775510204082,0.170787875129275)
--(axis cs:93.5374149659864,0.180268275812534)
--(axis cs:93.1972789115646,0.18871587047229)
--(axis cs:92.8571428571429,0.199985500826465)
--(axis cs:92.5170068027211,0.211531670598838)
--(axis cs:92.1768707482993,0.223132206303452)
--(axis cs:91.8367346938775,0.235231199053969)
--(axis cs:91.4965986394558,0.244586101759086)
--(axis cs:91.156462585034,0.25456405033824)
--(axis cs:90.8163265306122,0.262412482566832)
--(axis cs:90.4761904761905,0.274910121275572)
--(axis cs:90.1360544217687,0.286367081285728)
--(axis cs:89.7959183673469,0.294345599258924)
--(axis cs:89.4557823129252,0.30706013556868)
--(axis cs:89.1156462585034,0.315647379098442)
--(axis cs:88.7755102040816,0.325345709725401)
--(axis cs:88.4353741496599,0.335424187064645)
--(axis cs:88.0952380952381,0.343474923766059)
--(axis cs:87.7551020408163,0.350009607973874)
--(axis cs:87.4149659863945,0.355891088759413)
--(axis cs:87.0748299319728,0.364040251939688)
--(axis cs:86.734693877551,0.369945646663273)
--(axis cs:86.3945578231292,0.377354064606373)
--(axis cs:86.0544217687075,0.381306779548085)
--(axis cs:85.7142857142857,0.389746738003609)
--(axis cs:85.3741496598639,0.393890262784278)
--(axis cs:85.0340136054422,0.39745329971299)
--(axis cs:84.6938775510204,0.401382908072775)
--(axis cs:84.3537414965986,0.405158148456665)
--(axis cs:84.0136054421769,0.408619815586717)
--(axis cs:83.6734693877551,0.412684430083275)
--(axis cs:83.3333333333333,0.416275533469242)
--(axis cs:82.9931972789116,0.417813794130509)
--(axis cs:82.6530612244898,0.423225016289899)
--(axis cs:82.312925170068,0.423066343046698)
--(axis cs:81.9727891156463,0.427736183288949)
--(axis cs:81.6326530612245,0.431199251503006)
--(axis cs:81.2925170068027,0.436022615271412)
--(axis cs:80.9523809523809,0.439567028636433)
--(axis cs:80.6122448979592,0.444261250289686)
--(axis cs:80.2721088435374,0.447000479341948)
--(axis cs:79.9319727891156,0.451231410370644)
--(axis cs:79.5918367346939,0.45216638418671)
--(axis cs:79.2517006802721,0.457096684558203)
--(axis cs:78.9115646258503,0.459414515969806)
--(axis cs:78.5714285714286,0.46058810233015)
--(axis cs:78.2312925170068,0.463142448827077)
--(axis cs:77.891156462585,0.465522356466074)
--(axis cs:77.5510204081633,0.468973366674356)
--(axis cs:77.2108843537415,0.468999818407048)
--(axis cs:76.8707482993197,0.472319813899788)
--(axis cs:76.530612244898,0.474832751871863)
--(axis cs:76.1904761904762,0.478749288188614)
--(axis cs:75.8503401360544,0.480704246150988)
--(axis cs:75.5102040816327,0.483852062718108)
--(axis cs:75.1700680272109,0.485629574446611)
--(axis cs:74.8299319727891,0.488189011158453)
--(axis cs:74.4897959183673,0.488807242254017)
--(axis cs:74.1496598639456,0.490976219611793)
--(axis cs:73.8095238095238,0.494288936024528)
--(axis cs:73.469387755102,0.495497668210267)
--(axis cs:73.1292517006803,0.497789949348836)
--(axis cs:72.7891156462585,0.499288194162085)
--(axis cs:72.4489795918367,0.501430836371371)
--(axis cs:72.108843537415,0.504565011164903)
--(axis cs:71.7687074829932,0.506841869132438)
--(axis cs:71.4285714285714,0.509296023191596)
--(axis cs:71.0884353741497,0.511740257317537)
--(axis cs:70.7482993197279,0.513092300630295)
--(axis cs:70.4081632653061,0.514451932295945)
--(axis cs:70.0680272108844,0.515899066254655)
--(axis cs:69.7278911564626,0.517565653003372)
--(axis cs:69.3877551020408,0.520286580547906)
--(axis cs:69.0476190476191,0.522644077484757)
--(axis cs:68.7074829931973,0.523985785470223)
--(axis cs:68.3673469387755,0.526230479691191)
--(axis cs:68.0272108843537,0.526279952447885)
--(axis cs:67.687074829932,0.529107089296395)
--(axis cs:67.3469387755102,0.531230702785659)
--(axis cs:67.0068027210884,0.533919783625192)
--(axis cs:66.6666666666667,0.534948938068909)
--(axis cs:66.3265306122449,0.536823833092025)
--(axis cs:65.9863945578231,0.53802773394188)
--(axis cs:65.6462585034014,0.53937495624688)
--(axis cs:65.3061224489796,0.542128489272229)
--(axis cs:64.9659863945578,0.543055224392197)
--(axis cs:64.6258503401361,0.544599090483894)
--(axis cs:64.2857142857143,0.547231638416871)
--(axis cs:63.9455782312925,0.547537471604761)
--(axis cs:63.6054421768707,0.550869884862061)
--(axis cs:63.265306122449,0.55029771512798)
--(axis cs:62.9251700680272,0.552589774519877)
--(axis cs:62.5850340136054,0.553887105965829)
--(axis cs:62.2448979591837,0.555752634769104)
--(axis cs:61.9047619047619,0.556135198846153)
--(axis cs:61.5646258503401,0.557725992870499)
--(axis cs:61.2244897959184,0.559757282703271)
--(axis cs:60.8843537414966,0.561675213406303)
--(axis cs:60.5442176870748,0.563420893198152)
--(axis cs:60.2040816326531,0.564628634039145)
--(axis cs:59.8639455782313,0.565431790411467)
--(axis cs:59.5238095238095,0.566163879346673)
--(axis cs:59.1836734693878,0.568438521062305)
--(axis cs:58.843537414966,0.570512817854222)
--(axis cs:58.5034013605442,0.569392141678678)
--(axis cs:58.1632653061224,0.57175393386428)
--(axis cs:57.8231292517007,0.573999703068744)
--(axis cs:57.4829931972789,0.573581659903171)
--(axis cs:57.1428571428571,0.57478563174691)
--(axis cs:56.8027210884354,0.575860890700106)
--(axis cs:56.4625850340136,0.57706878499654)
--(axis cs:56.1224489795918,0.577208045129873)
--(axis cs:55.7823129251701,0.579562521376733)
--(axis cs:55.4421768707483,0.57951449033428)
--(axis cs:55.1020408163265,0.580589422201199)
--(axis cs:54.7619047619048,0.581557242270407)
--(axis cs:54.421768707483,0.58313512540367)
--(axis cs:54.0816326530612,0.583770729153369)
--(axis cs:53.7414965986395,0.585984389118562)
--(axis cs:53.4013605442177,0.585526924054556)
--(axis cs:53.0612244897959,0.588205573675174)
--(axis cs:52.7210884353741,0.587140209798475)
--(axis cs:52.3809523809524,0.588002761127614)
--(axis cs:52.0408163265306,0.590236983312086)
--(axis cs:51.7006802721088,0.590774900642856)
--(axis cs:51.3605442176871,0.591885490567454)
--(axis cs:51.0204081632653,0.592722702978431)
--(axis cs:50.6802721088435,0.595024464954131)
--(axis cs:50.3401360544218,0.595803953890803)
--(axis cs:50,0.595692133632731)
--(axis cs:49.6598639455782,0.595982218231191)
--(axis cs:49.3197278911565,0.59696227433249)
--(axis cs:48.9795918367347,0.596738279822787)
--(axis cs:48.6394557823129,0.598689098610639)
--(axis cs:48.2993197278912,0.598548135950761)
--(axis cs:47.9591836734694,0.600416117432113)
--(axis cs:47.6190476190476,0.601312494192136)
--(axis cs:47.2789115646259,0.601333574158146)
--(axis cs:46.9387755102041,0.602650954896788)
--(axis cs:46.5986394557823,0.602603023954451)
--(axis cs:46.2585034013605,0.603732838480622)
--(axis cs:45.9183673469388,0.604377466157281)
--(axis cs:45.578231292517,0.604966448658268)
--(axis cs:45.2380952380952,0.608261116686652)
--(axis cs:44.8979591836735,0.609550714515934)
--(axis cs:44.5578231292517,0.610342552356837)
--(axis cs:44.2176870748299,0.60915241655514)
--(axis cs:43.8775510204082,0.609969914526844)
--(axis cs:43.5374149659864,0.612399776848174)
--(axis cs:43.1972789115646,0.61141533460669)
--(axis cs:42.8571428571429,0.613438251946434)
--(axis cs:42.5170068027211,0.614211678717765)
--(axis cs:42.1768707482993,0.615011173862264)
--(axis cs:41.8367346938776,0.615932655073004)
--(axis cs:41.4965986394558,0.616021699661813)
--(axis cs:41.156462585034,0.617240589661811)
--(axis cs:40.8163265306122,0.618353564033585)
--(axis cs:40.4761904761905,0.619773553468426)
--(axis cs:40.1360544217687,0.618655008322789)
--(axis cs:39.7959183673469,0.619865347218454)
--(axis cs:39.4557823129252,0.620382242395426)
--(axis cs:39.1156462585034,0.623226686942822)
--(axis cs:38.7755102040816,0.621757638691853)
--(axis cs:38.4353741496599,0.622427995390236)
--(axis cs:38.0952380952381,0.624265773946621)
--(axis cs:37.7551020408163,0.624296063567496)
--(axis cs:37.4149659863946,0.626774534867931)
--(axis cs:37.0748299319728,0.626491167621989)
--(axis cs:36.734693877551,0.628125889371419)
--(axis cs:36.3945578231292,0.628932806957829)
--(axis cs:36.0544217687075,0.628724080809663)
--(axis cs:35.7142857142857,0.62853209580893)
--(axis cs:35.3741496598639,0.630507804656821)
--(axis cs:35.0340136054422,0.630707140245843)
--(axis cs:34.6938775510204,0.632711381349443)
--(axis cs:34.3537414965986,0.633342435766046)
--(axis cs:34.0136054421769,0.633253701922046)
--(axis cs:33.6734693877551,0.634160045866044)
--(axis cs:33.3333333333333,0.634722408507402)
--(axis cs:32.9931972789116,0.636479991231543)
--(axis cs:32.6530612244898,0.637017257360453)
--(axis cs:32.312925170068,0.636351301270491)
--(axis cs:31.9727891156463,0.638234093890112)
--(axis cs:31.6326530612245,0.639039636753616)
--(axis cs:31.2925170068027,0.63987101323642)
--(axis cs:30.952380952381,0.641471997088099)
--(axis cs:30.6122448979592,0.642227588998459)
--(axis cs:30.2721088435374,0.643311685719131)
--(axis cs:29.9319727891156,0.644174603406312)
--(axis cs:29.5918367346939,0.644368980704009)
--(axis cs:29.2517006802721,0.645950229109398)
--(axis cs:28.9115646258503,0.646158205106246)
--(axis cs:28.5714285714286,0.646001173863394)
--(axis cs:28.2312925170068,0.646999259511092)
--(axis cs:27.891156462585,0.648536524659455)
--(axis cs:27.5510204081633,0.647707311311136)
--(axis cs:27.2108843537415,0.648468345907023)
--(axis cs:26.8707482993197,0.65022874100403)
--(axis cs:26.530612244898,0.651002350870988)
--(axis cs:26.1904761904762,0.651011734191088)
--(axis cs:25.8503401360544,0.653593026298412)
--(axis cs:25.5102040816327,0.653843003580558)
--(axis cs:25.1700680272109,0.655711400171501)
--(axis cs:24.8299319727891,0.657555197430197)
--(axis cs:24.4897959183673,0.658544802496154)
--(axis cs:24.1496598639456,0.658833942315707)
--(axis cs:23.8095238095238,0.659508748357642)
--(axis cs:23.469387755102,0.660764410020833)
--(axis cs:23.1292517006803,0.661091524692308)
--(axis cs:22.7891156462585,0.663381201091218)
--(axis cs:22.4489795918367,0.66270626564873)
--(axis cs:22.108843537415,0.664024879536762)
--(axis cs:21.7687074829932,0.664360962259746)
--(axis cs:21.4285714285714,0.665913463271344)
--(axis cs:21.0884353741497,0.665874582225673)
--(axis cs:20.7482993197279,0.666149551112765)
--(axis cs:20.4081632653061,0.667155562760354)
--(axis cs:20.0680272108844,0.665716143485301)
--(axis cs:19.7278911564626,0.667588122564016)
--(axis cs:19.3877551020408,0.668417396053629)
--(axis cs:19.047619047619,0.668922389548621)
--(axis cs:18.7074829931973,0.669142857083085)
--(axis cs:18.3673469387755,0.670308475183753)
--(axis cs:18.0272108843537,0.670850913781984)
--(axis cs:17.687074829932,0.671610615999501)
--(axis cs:17.3469387755102,0.672498167462403)
--(axis cs:17.0068027210884,0.672791920392812)
--(axis cs:16.6666666666667,0.672743475035874)
--(axis cs:16.3265306122449,0.674407587960496)
--(axis cs:15.9863945578231,0.675209169388237)
--(axis cs:15.6462585034014,0.676431490918843)
--(axis cs:15.3061224489796,0.676308876784705)
--(axis cs:14.9659863945578,0.676445629902124)
--(axis cs:14.6258503401361,0.678198243676942)
--(axis cs:14.2857142857143,0.677630451472907)
--(axis cs:13.9455782312925,0.678731156082296)
--(axis cs:13.6054421768707,0.678871040016424)
--(axis cs:13.265306122449,0.679269855534786)
--(axis cs:12.9251700680272,0.680457479568843)
--(axis cs:12.5850340136054,0.681382920372063)
--(axis cs:12.2448979591837,0.682920942443993)
--(axis cs:11.9047619047619,0.683276682889703)
--(axis cs:11.5646258503401,0.684767263701496)
--(axis cs:11.2244897959184,0.686277573106857)
--(axis cs:10.8843537414966,0.687771614150284)
--(axis cs:10.5442176870748,0.689931933456508)
--(axis cs:10.2040816326531,0.690238560613146)
--(axis cs:9.86394557823129,0.693006874067538)
--(axis cs:9.52380952380952,0.695569010567503)
--(axis cs:9.18367346938775,0.695717309664733)
--(axis cs:8.84353741496599,0.698325345033563)
--(axis cs:8.50340136054422,0.699235517578917)
--(axis cs:8.16326530612245,0.700625491518032)
--(axis cs:7.82312925170068,0.703334241958191)
--(axis cs:7.48299319727891,0.703488726996033)
--(axis cs:7.14285714285714,0.705538394935007)
--(axis cs:6.80272108843537,0.707602798089844)
--(axis cs:6.46258503401361,0.707931072000756)
--(axis cs:6.12244897959184,0.710453811249898)
--(axis cs:5.78231292517007,0.71235131617728)
--(axis cs:5.4421768707483,0.714000626175183)
--(axis cs:5.10204081632653,0.714902153624169)
--(axis cs:4.76190476190476,0.715570529894132)
--(axis cs:4.42176870748299,0.718872942439922)
--(axis cs:4.08163265306122,0.719747800306799)
--(axis cs:3.74149659863946,0.720507211615687)
--(axis cs:3.40136054421769,0.720851608685883)
--(axis cs:3.06122448979592,0.723401080008863)
--(axis cs:2.72108843537415,0.72346640751674)
--(axis cs:2.38095238095238,0.72395834851868)
--(axis cs:2.04081632653061,0.724010330711518)
--(axis cs:1.70068027210884,0.725823248699907)
--(axis cs:1.36054421768707,0.725646815962406)
--(axis cs:1.02040816326531,0.725603151618491)
--(axis cs:0.680272108843537,0.724973306615856)
--(axis cs:0.340136054421769,0.72285180164035)
--(axis cs:0,0.720430770721294)
--cycle;


==> img/stl10/stl10_rate_distortion_smoothgrad.tex <==
% smoothgrad
\addplot [line width=0.5, opacity=0.8, color7, mark=triangle, mark repeat=30, mark phase=15, mark size=1.5pt, mark options={draw=black, fill=color7, thin}]
table [row sep=\\]{%
0	0.718900465667248 \\
0.340136054421769	0.719145317524672 \\
0.680272108843537	0.71497792840004 \\
1.02040816326531	0.709987808167934 \\
1.36054421768707	0.704852434545755 \\
1.70068027210884	0.700445004999638 \\
2.04081632653061	0.692663285136223 \\
2.38095238095238	0.686526309400797 \\
2.72108843537415	0.680068671479821 \\
3.06122448979592	0.673457845617086 \\
3.40136054421769	0.666859435029328 \\
3.74149659863946	0.663582201264799 \\
4.08163265306122	0.653954192809761 \\
4.42176870748299	0.644336613956839 \\
4.76190476190476	0.640009053202812 \\
5.10204081632653	0.637089687499683 \\
5.4421768707483	0.630404411635827 \\
5.78231292517007	0.624121174528846 \\
6.12244897959184	0.620613348152256 \\
6.46258503401361	0.616399120832793 \\
6.80272108843537	0.612296531600878 \\
7.14285714285714	0.609034721810021 \\
7.48299319727891	0.604171476769261 \\
7.82312925170068	0.599596985151293 \\
8.16326530612245	0.595364325361443 \\
8.50340136054422	0.590051261311455 \\
8.84353741496599	0.583602874768549 \\
9.18367346938775	0.58038986113359 \\
9.52380952380952	0.575876093609404 \\
9.86394557823129	0.573468189919804 \\
10.2040816326531	0.566774537253368 \\
10.5442176870748	0.557835265978974 \\
10.8843537414966	0.549228597289621 \\
11.2244897959184	0.544142930914422 \\
11.5646258503401	0.541208886816676 \\
11.9047619047619	0.533505360340059 \\
12.2448979591837	0.529542049012789 \\
12.5850340136054	0.523968028735853 \\
12.9251700680272	0.520174566309779 \\
13.265306122449	0.510553382643538 \\
13.6054421768707	0.504941209687713 \\
13.9455782312925	0.497387195764766 \\
14.2857142857143	0.494686618330436 \\
14.6258503401361	0.487550428759732 \\
14.9659863945578	0.483098639426482 \\
15.3061224489796	0.47636799876218 \\
15.6462585034014	0.471479517435114 \\
15.9863945578231	0.465903405755913 \\
16.3265306122449	0.459456940693643 \\
16.6666666666667	0.455445277721641 \\
17.0068027210884	0.449242758260719 \\
17.3469387755102	0.443186127684033 \\
17.687074829932	0.437040922923388 \\
18.0272108843537	0.430716487253835 \\
18.3673469387755	0.423173497017442 \\
18.7074829931973	0.417359951858516 \\
19.047619047619	0.412266592559911 \\
19.3877551020408	0.407317552966615 \\
19.7278911564626	0.401623717511787 \\
20.0680272108844	0.400133093393875 \\
20.4081632653061	0.396297929501284 \\
20.7482993197279	0.392336874346414 \\
21.0884353741497	0.388436374357397 \\
21.4285714285714	0.386015433454309 \\
21.7687074829932	0.38248179459206 \\
22.108843537415	0.378119537363171 \\
22.4489795918367	0.375076211855151 \\
22.7891156462585	0.371706625334626 \\
23.1292517006803	0.370828548254916 \\
23.469387755102	0.370295340971632 \\
23.8095238095238	0.367414280457551 \\
24.1496598639456	0.36804195173291 \\
24.4897959183673	0.363615224981521 \\
24.8299319727891	0.362980681219217 \\
25.1700680272109	0.358812929990027 \\
25.5102040816327	0.358482467845897 \\
25.8503401360544	0.354243231253107 \\
26.1904761904762	0.351391387331265 \\
26.530612244898	0.350596313834566 \\
26.8707482993197	0.347715983809296 \\
27.2108843537415	0.344270262861896 \\
27.5510204081633	0.343100313331232 \\
27.891156462585	0.340056243433191 \\
28.2312925170068	0.336376572999279 \\
28.5714285714286	0.335152552646634 \\
28.9115646258503	0.333629821465282 \\
29.2517006802721	0.330331451111079 \\
29.5918367346939	0.328292197305546 \\
29.9319727891156	0.32509429203181 \\
30.2721088435374	0.324210454216872 \\
30.6122448979592	0.321793063793819 \\
30.952380952381	0.317117898279183 \\
31.2925170068027	0.314829697243344 \\
31.6326530612245	0.310732616023373 \\
31.9727891156463	0.308818476773385 \\
32.312925170068	0.307267151953002 \\
32.6530612244898	0.302858541974186 \\
32.9931972789116	0.30141086870481 \\
33.3333333333333	0.297825810740392 \\
33.6734693877551	0.294111494217237 \\
34.0136054421769	0.291475585293336 \\
34.3537414965986	0.288875997199544 \\
34.6938775510204	0.2869499277963 \\
35.0340136054422	0.284211300242232 \\
35.3741496598639	0.279981891015559 \\
35.7142857142857	0.277710335514226 \\
36.0544217687075	0.275591320034438 \\
36.3945578231292	0.274637848514559 \\
36.734693877551	0.270825703743064 \\
37.0748299319728	0.271212890229718 \\
37.4149659863946	0.268457070982325 \\
37.7551020408163	0.265224077518141 \\
38.0952380952381	0.263440861069353 \\
38.4353741496599	0.262051874684563 \\
38.7755102040816	0.256446695692244 \\
39.1156462585034	0.256212771261186 \\
39.4557823129252	0.253084994762552 \\
39.7959183673469	0.248225758273528 \\
40.1360544217687	0.245881531380645 \\
40.4761904761905	0.241272563393446 \\
40.8163265306122	0.238478130155589 \\
41.156462585034	0.234896068535972 \\
41.4965986394558	0.234293292531206 \\
41.8367346938776	0.228988709753696 \\
42.1768707482993	0.224128721660624 \\
42.5170068027211	0.221554391887355 \\
42.8571428571429	0.21798082375588 \\
43.1972789115646	0.215056487999798 \\
43.5374149659864	0.212895737849186 \\
43.8775510204082	0.208770579840731 \\
44.2176870748299	0.20371128495048 \\
44.5578231292517	0.197248280391508 \\
44.8979591836735	0.194340567761719 \\
45.2380952380952	0.192512139670817 \\
45.578231292517	0.188818476472195 \\
45.9183673469388	0.184459638423826 \\
46.2585034013605	0.181526438258315 \\
46.5986394557823	0.178692837980307 \\
46.9387755102041	0.174787892340747 \\
47.2789115646259	0.171388537179397 \\
47.6190476190476	0.166589387290354 \\
47.9591836734694	0.162986523311255 \\
48.2993197278912	0.159437615380081 \\
48.6394557823129	0.156011789862737 \\
48.9795918367347	0.153222979929358 \\
49.3197278911565	0.148255036635925 \\
49.6598639455782	0.144081993696087 \\
50	0.141940518826662 \\
50.3401360544218	0.138769536224828 \\
50.6802721088435	0.134680698136157 \\
51.0204081632653	0.132193922546612 \\
51.3605442176871	0.127754220518115 \\
51.7006802721088	0.123966312146547 \\
52.0408163265306	0.121790950655237 \\
52.3809523809524	0.118932113848152 \\
52.7210884353741	0.116561734048353 \\
53.0612244897959	0.111949978758687 \\
53.4013605442177	0.107557042463378 \\
53.7414965986395	0.101454415464886 \\
54.0816326530612	0.0999844240732469 \\
54.421768707483	0.0968439926445336 \\
54.7619047619048	0.0936695279276409 \\
55.1020408163265	0.0889741930755451 \\
55.4421768707483	0.0863127203316973 \\
55.7823129251701	0.0828382830548814 \\
56.1224489795918	0.0796042310745288 \\
56.4625850340136	0.074943277621568 \\
56.8027210884354	0.0717436903215285 \\
57.1428571428571	0.0675368759673018 \\
57.4829931972789	0.0654603661947535 \\
57.8231292517007	0.0623831685190335 \\
58.1632653061224	0.0609807429283379 \\
58.5034013605442	0.0582998563763949 \\
58.843537414966	0.0560087155827406 \\
59.1836734693878	0.0547660037126805 \\
59.5238095238095	0.0508188262826831 \\
59.8639455782313	0.048023056637245 \\
60.2040816326531	0.0466215619910055 \\
60.5442176870748	0.0440860731938801 \\
60.8843537414966	0.0428606911844317 \\
61.2244897959184	0.0407076174366851 \\
61.5646258503401	0.0389158902085934 \\
61.9047619047619	0.0367834132362918 \\
62.2448979591837	0.0352928835996802 \\
62.5850340136054	0.0326289038889853 \\
62.9251700680272	0.0321973810617518 \\
63.265306122449	0.0305384275771929 \\
63.6054421768707	0.0295885856229315 \\
63.9455782312925	0.0276754930962323 \\
64.2857142857143	0.0269658745703093 \\
64.6258503401361	0.0257011104702002 \\
64.9659863945578	0.0241919308837784 \\
65.3061224489796	0.0224861539520426 \\
65.6462585034014	0.0209775604533199 \\
65.9863945578231	0.0199315308282557 \\
66.3265306122449	0.0188974368027672 \\
66.6666666666667	0.0183301596225056 \\
67.0068027210884	0.0185115383105952 \\
67.3469387755102	0.0167934079428123 \\
67.687074829932	0.0160185622047272 \\
68.0272108843537	0.0154478444604219 \\
68.3673469387755	0.0143085245639273 \\
68.7074829931973	0.0142584417152387 \\
69.0476190476191	0.0134907136148296 \\
69.3877551020408	0.013314933543579 \\
69.7278911564626	0.0129295520810362 \\
70.0680272108844	0.0124309528186078 \\
70.4081632653061	0.0122885068287876 \\
70.7482993197279	0.0116808786462077 \\
71.0884353741497	0.0118538255314533 \\
71.4285714285714	0.0118243332573402 \\
71.7687074829932	0.011394864827183 \\
72.108843537415	0.0121398859533937 \\
72.4489795918367	0.0119011159819316 \\
72.7891156462585	0.0116389644679619 \\
73.1292517006803	0.0113379367562277 \\
73.469387755102	0.0113093285170741 \\
73.8095238095238	0.0111408995731328 \\
74.1496598639456	0.0106368038472357 \\
74.4897959183673	0.0100173209393072 \\
74.8299319727891	0.00988058634919786 \\
75.1700680272109	0.00930488929262729 \\
75.5102040816327	0.00903597506673935 \\
75.8503401360544	0.00890733955189546 \\
76.1904761904762	0.00877927171893136 \\
76.530612244898	0.00848066095592912 \\
76.8707482993197	0.00824519601314211 \\
77.2108843537415	0.00755669369903378 \\
77.5510204081633	0.00739669635656998 \\
77.891156462585	0.00726444359339622 \\
78.2312925170068	0.00698863291705267 \\
78.5714285714286	0.00666749702190153 \\
78.9115646258503	0.00641494149943627 \\
79.2517006802721	0.00641392356746298 \\
79.5918367346939	0.00597901728075695 \\
79.9319727891156	0.00594274920731205 \\
80.2721088435374	0.00582952889733312 \\
80.6122448979592	0.00556950030366116 \\
80.9523809523809	0.00551447230668242 \\
81.2925170068027	0.0053792383781622 \\
81.6326530612245	0.00511321671613108 \\
81.9727891156463	0.00526425594770595 \\
82.312925170068	0.00508868337075626 \\
82.6530612244898	0.00506383653452401 \\
82.9931972789116	0.00489398237341319 \\
83.3333333333333	0.00471322920452394 \\
83.6734693877551	0.00478447969887892 \\
84.0136054421769	0.0047534533450645 \\
84.3537414965986	0.00471546831317672 \\
84.6938775510204	0.00431693869912797 \\
85.0340136054422	0.0044830341902595 \\
85.3741496598639	0.00449583964215529 \\
85.7142857142857	0.00444524568851842 \\
86.0544217687075	0.0044441407269839 \\
86.3945578231292	0.00425449540053652 \\
86.734693877551	0.00409500109975678 \\
87.0748299319728	0.00407415545029549 \\
87.4149659863945	0.00399022447763316 \\
87.7551020408163	0.00407908677327343 \\
88.0952380952381	0.00391973110436323 \\
88.4353741496599	0.00373307146711868 \\
88.7755102040816	0.00380919413644576 \\
89.1156462585034	0.00373200429383445 \\
89.4557823129252	0.00369416695585566 \\
89.7959183673469	0.00366429777720025 \\
90.1360544217687	0.00353770926190786 \\
90.4761904761905	0.00315013431248193 \\
90.8163265306122	0.00317214938896871 \\
91.156462585034	0.00322815230013106 \\
91.4965986394558	0.00313939616912551 \\
91.8367346938775	0.00303598787733528 \\
92.1768707482993	0.00300541264886024 \\
92.5170068027211	0.00284915621683141 \\
92.8571428571429	0.00302241251259054 \\
93.1972789115646	0.002847412023002 \\
93.5374149659864	0.00259264198841821 \\
93.8775510204082	0.00243143165085499 \\
94.2176870748299	0.00247694802876014 \\
94.5578231292517	0.00228221971090147 \\
94.8979591836735	0.00224766921655788 \\
95.2380952380952	0.00215895498037556 \\
95.578231292517	0.00221364548471662 \\
95.9183673469388	0.00196863792935822 \\
96.2585034013605	0.00186866237726261 \\
96.5986394557823	0.00171597423321974 \\
96.9387755102041	0.00154276587322494 \\
97.2789115646258	0.00128598611707073 \\
97.6190476190476	0.000893144725102437 \\
97.9591836734694	0.00073134677588391 \\
98.2993197278912	0.000375229904108965 \\
98.6394557823129	0.000226585676466511 \\
98.9795918367347	9.98249726522793e-05 \\
99.3197278911565	5.51347568395999e-05 \\
99.6598639455782	1.49305222318596e-05 \\
100	1.49018575257287e-13 \\
};
\path [fill=color7, fill opacity=0.5] (axis cs:0,0.720762681985969)
--(axis cs:0,0.717038249348527)
--(axis cs:0.340136054421769,0.717268412214531)
--(axis cs:0.680272108843537,0.712776700848132)
--(axis cs:1.02040816326531,0.707608695991582)
--(axis cs:1.36054421768707,0.702231031020262)
--(axis cs:1.70068027210884,0.697779536932304)
--(axis cs:2.04081632653061,0.68967957378304)
--(axis cs:2.38095238095238,0.683317286761831)
--(axis cs:2.72108843537415,0.67646261765352)
--(axis cs:3.06122448979592,0.669614674129811)
--(axis cs:3.40136054421769,0.662638055941311)
--(axis cs:3.74149659863946,0.659249526996294)
--(axis cs:4.08163265306122,0.649444742479517)
--(axis cs:4.42176870748299,0.639707987789709)
--(axis cs:4.76190476190476,0.635226429750025)
--(axis cs:5.10204081632653,0.632141219876632)
--(axis cs:5.4421768707483,0.625644823423416)
--(axis cs:5.78231292517007,0.619423247254963)
--(axis cs:6.12244897959184,0.615954479800313)
--(axis cs:6.46258503401361,0.611471044864037)
--(axis cs:6.80272108843537,0.607547816428861)
--(axis cs:7.14285714285714,0.604248357258239)
--(axis cs:7.48299319727891,0.599405897489297)
--(axis cs:7.82312925170068,0.594571525913691)
--(axis cs:8.16326530612245,0.590373281200743)
--(axis cs:8.50340136054422,0.585086234098481)
--(axis cs:8.84353741496599,0.57844671775041)
--(axis cs:9.18367346938775,0.575049969408348)
--(axis cs:9.52380952380952,0.570577366854671)
--(axis cs:9.86394557823129,0.568016221090916)
--(axis cs:10.2040816326531,0.561142851216332)
--(axis cs:10.5442176870748,0.552112084381594)
--(axis cs:10.8843537414966,0.543404034625609)
--(axis cs:11.2244897959184,0.538373603515598)
--(axis cs:11.5646258503401,0.53561614943634)
--(axis cs:11.9047619047619,0.527748355173495)
--(axis cs:12.2448979591837,0.523626883311116)
--(axis cs:12.5850340136054,0.518124222881894)
--(axis cs:12.9251700680272,0.514294676075859)
--(axis cs:13.265306122449,0.504682277489117)
--(axis cs:13.6054421768707,0.498941725302009)
--(axis cs:13.9455782312925,0.491478728711352)
--(axis cs:14.2857142857143,0.488827047511667)
--(axis cs:14.6258503401361,0.481580539742311)
--(axis cs:14.9659863945578,0.47714493108024)
--(axis cs:15.3061224489796,0.470504571148552)
--(axis cs:15.6462585034014,0.465827420388179)
--(axis cs:15.9863945578231,0.460169274078945)
--(axis cs:16.3265306122449,0.453751134740707)
--(axis cs:16.6666666666667,0.449725986554117)
--(axis cs:17.0068027210884,0.443342195055327)
--(axis cs:17.3469387755102,0.437297284037794)
--(axis cs:17.687074829932,0.431178363876238)
--(axis cs:18.0272108843537,0.424917622113731)
--(axis cs:18.3673469387755,0.417266371292204)
--(axis cs:18.7074829931973,0.41146966358736)
--(axis cs:19.047619047619,0.406541192845793)
--(axis cs:19.3877551020408,0.401770644347314)
--(axis cs:19.7278911564626,0.396082684847419)
--(axis cs:20.0680272108844,0.394566654411227)
--(axis cs:20.4081632653061,0.390739462686557)
--(axis cs:20.7482993197279,0.386882423259267)
--(axis cs:21.0884353741497,0.383122775416065)
--(axis cs:21.4285714285714,0.380720559278967)
--(axis cs:21.7687074829932,0.37707546381226)
--(axis cs:22.108843537415,0.372937283536213)
--(axis cs:22.4489795918367,0.370102587326366)
--(axis cs:22.7891156462585,0.366502502995517)
--(axis cs:23.1292517006803,0.365837196814291)
--(axis cs:23.469387755102,0.365112682724868)
--(axis cs:23.8095238095238,0.362585461294726)
--(axis cs:24.1496598639456,0.363197347149358)
--(axis cs:24.4897959183673,0.358819876977106)
--(axis cs:24.8299319727891,0.358255396237132)
--(axis cs:25.1700680272109,0.353960011530575)
--(axis cs:25.5102040816327,0.353922741633618)
--(axis cs:25.8503401360544,0.34965705894779)
--(axis cs:26.1904761904762,0.346615351575794)
--(axis cs:26.530612244898,0.345935503456225)
--(axis cs:26.8707482993197,0.343100496816847)
--(axis cs:27.2108843537415,0.339435389875938)
--(axis cs:27.5510204081633,0.33815538419028)
--(axis cs:27.891156462585,0.335310690297684)
--(axis cs:28.2312925170068,0.331563916448153)
--(axis cs:28.5714285714286,0.330634152294066)
--(axis cs:28.9115646258503,0.329028190669409)
--(axis cs:29.2517006802721,0.325807179691281)
--(axis cs:29.5918367346939,0.323762942752267)
--(axis cs:29.9319727891156,0.320685931318579)
--(axis cs:30.2721088435374,0.319825861259414)
--(axis cs:30.6122448979592,0.31772628060218)
--(axis cs:30.952380952381,0.312745304244437)
--(axis cs:31.2925170068027,0.310543793407281)
--(axis cs:31.6326530612245,0.30635816027607)
--(axis cs:31.9727891156463,0.304392425935342)
--(axis cs:32.312925170068,0.302717493901116)
--(axis cs:32.6530612244898,0.298388410960483)
--(axis cs:32.9931972789116,0.296825064345541)
--(axis cs:33.3333333333333,0.29330983940441)
--(axis cs:33.6734693877551,0.289498866960487)
--(axis cs:34.0136054421769,0.286815921707243)
--(axis cs:34.3537414965986,0.284397401637604)
--(axis cs:34.6938775510204,0.282292482230692)
--(axis cs:35.0340136054422,0.279605073376786)
--(axis cs:35.3741496598639,0.275302157232689)
--(axis cs:35.7142857142857,0.273028229426299)
--(axis cs:36.0544217687075,0.271076284033299)
--(axis cs:36.3945578231292,0.269801653283819)
--(axis cs:36.734693877551,0.266059178199048)
--(axis cs:37.0748299319728,0.266501924424173)
--(axis cs:37.4149659863946,0.263628934724223)
--(axis cs:37.7551020408163,0.260572422376779)
--(axis cs:38.0952380952381,0.258818062093863)
--(axis cs:38.4353741496599,0.257411210684312)
--(axis cs:38.7755102040816,0.251611793623539)
--(axis cs:39.1156462585034,0.251489761961282)
--(axis cs:39.4557823129252,0.248252755659186)
--(axis cs:39.7959183673469,0.243665639478762)
--(axis cs:40.1360544217687,0.241213405561066)
--(axis cs:40.4761904761905,0.236639271779452)
--(axis cs:40.8163265306122,0.233919301999541)
--(axis cs:41.156462585034,0.230429800460302)
--(axis cs:41.4965986394558,0.229925100003623)
--(axis cs:41.8367346938776,0.224566323337022)
--(axis cs:42.1768707482993,0.21983409108998)
--(axis cs:42.5170068027211,0.217171488582731)
--(axis cs:42.8571428571429,0.213721309840936)
--(axis cs:43.1972789115646,0.210799791182685)
--(axis cs:43.5374149659864,0.208600545770316)
--(axis cs:43.8775510204082,0.204555113675534)
--(axis cs:44.2176870748299,0.199379940289471)
--(axis cs:44.5578231292517,0.193208375438295)
--(axis cs:44.8979591836735,0.190176103537752)
--(axis cs:45.2380952380952,0.188406672265799)
--(axis cs:45.578231292517,0.184890159661003)
--(axis cs:45.9183673469388,0.180460638501699)
--(axis cs:46.2585034013605,0.177682218934649)
--(axis cs:46.5986394557823,0.174864189604267)
--(axis cs:46.9387755102041,0.170993601135172)
--(axis cs:47.2789115646259,0.167529102304141)
--(axis cs:47.6190476190476,0.16289544874816)
--(axis cs:47.9591836734694,0.159349789219163)
--(axis cs:48.2993197278912,0.155741874770484)
--(axis cs:48.6394557823129,0.152270575360568)
--(axis cs:48.9795918367347,0.14972836896916)
--(axis cs:49.3197278911565,0.144593151124448)
--(axis cs:49.6598639455782,0.140417753964202)
--(axis cs:50,0.138220860250318)
--(axis cs:50.3401360544218,0.135058730901369)
--(axis cs:50.6802721088435,0.13102785437046)
--(axis cs:51.0204081632653,0.128368309056688)
--(axis cs:51.3605442176871,0.124092705109537)
--(axis cs:51.7006802721088,0.120337755267373)
--(axis cs:52.0408163265306,0.118083373062725)
--(axis cs:52.3809523809524,0.115412689943568)
--(axis cs:52.7210884353741,0.113073764772864)
--(axis cs:53.0612244897959,0.108415051226881)
--(axis cs:53.4013605442177,0.104040383852243)
--(axis cs:53.7414965986395,0.0979322495009298)
--(axis cs:54.0816326530612,0.0964186860032078)
--(axis cs:54.421768707483,0.093475321253961)
--(axis cs:54.7619047619048,0.0902457319038973)
--(axis cs:55.1020408163265,0.085572957217943)
--(axis cs:55.4421768707483,0.0830945889742438)
--(axis cs:55.7823129251701,0.0798961737905687)
--(axis cs:56.1224489795918,0.0766303654589796)
--(axis cs:56.4625850340136,0.0722542461882336)
--(axis cs:56.8027210884354,0.0690335385081838)
--(axis cs:57.1428571428571,0.0649172482057119)
--(axis cs:57.4829931972789,0.0628126128384748)
--(axis cs:57.8231292517007,0.0599046777921993)
--(axis cs:58.1632653061224,0.0585389891590515)
--(axis cs:58.5034013605442,0.0558601868470049)
--(axis cs:58.843537414966,0.0537280704377662)
--(axis cs:59.1836734693878,0.0523871513844946)
--(axis cs:59.5238095238095,0.0485901388863232)
--(axis cs:59.8639455782313,0.0459525773650281)
--(axis cs:60.2040816326531,0.0445775214619201)
--(axis cs:60.5442176870748,0.0420455708000144)
--(axis cs:60.8843537414966,0.0408075702851918)
--(axis cs:61.2244897959184,0.0387423467682772)
--(axis cs:61.5646258503401,0.0370147102065775)
--(axis cs:61.9047619047619,0.0349472780047637)
--(axis cs:62.2448979591837,0.0334905249093123)
--(axis cs:62.5850340136054,0.0309570593403744)
--(axis cs:62.9251700680272,0.0305059912146738)
--(axis cs:63.265306122449,0.0288907429709228)
--(axis cs:63.6054421768707,0.0279544883175918)
--(axis cs:63.9455782312925,0.026102027273125)
--(axis cs:64.2857142857143,0.0255046096213163)
--(axis cs:64.6258503401361,0.0241809065117679)
--(axis cs:64.9659863945578,0.0228147224506998)
--(axis cs:65.3061224489796,0.0211792997357838)
--(axis cs:65.6462585034014,0.0197257835411202)
--(axis cs:65.9863945578231,0.0186848347179446)
--(axis cs:66.3265306122449,0.0177072187670468)
--(axis cs:66.6666666666667,0.0172399518333685)
--(axis cs:67.0068027210884,0.0172872012343202)
--(axis cs:67.3469387755102,0.015704038399379)
--(axis cs:67.687074829932,0.015006907282883)
--(axis cs:68.0272108843537,0.0144190983555202)
--(axis cs:68.3673469387755,0.0133520654267038)
--(axis cs:68.7074829931973,0.0132809338724845)
--(axis cs:69.0476190476191,0.0125631974986505)
--(axis cs:69.3877551020408,0.0124042274582042)
--(axis cs:69.7278911564626,0.0120379979757025)
--(axis cs:70.0680272108844,0.0116057005273249)
--(axis cs:70.4081632653061,0.0114763904790286)
--(axis cs:70.7482993197279,0.010846792503938)
--(axis cs:71.0884353741497,0.0110322865645895)
--(axis cs:71.4285714285714,0.0110319966169082)
--(axis cs:71.7687074829932,0.0106277666237151)
--(axis cs:72.108843537415,0.0113448413693805)
--(axis cs:72.4489795918367,0.0111032497668433)
--(axis cs:72.7891156462585,0.0108622034831722)
--(axis cs:73.1292517006803,0.0105347095288468)
--(axis cs:73.469387755102,0.0105336127061169)
--(axis cs:73.8095238095238,0.0103673712833967)
--(axis cs:74.1496598639456,0.00985986632787608)
--(axis cs:74.4897959183673,0.00933203565585216)
--(axis cs:74.8299319727891,0.0091710947307704)
--(axis cs:75.1700680272109,0.00866476663841031)
--(axis cs:75.5102040816327,0.00838174658839062)
--(axis cs:75.8503401360544,0.00827790076401522)
--(axis cs:76.1904761904762,0.00814108495486284)
--(axis cs:76.530612244898,0.00786569470864261)
--(axis cs:76.8707482993197,0.00763950115200372)
--(axis cs:77.2108843537415,0.00698661592764804)
--(axis cs:77.5510204081633,0.006864004933603)
--(axis cs:77.891156462585,0.00672457125240981)
--(axis cs:78.2312925170068,0.0064916023397007)
--(axis cs:78.5714285714286,0.00615544315953307)
--(axis cs:78.9115646258503,0.00596437046391649)
--(axis cs:79.2517006802721,0.00596960578508725)
--(axis cs:79.5918367346939,0.00554098667558523)
--(axis cs:79.9319727891156,0.00550545311641247)
--(axis cs:80.2721088435374,0.00540753142148135)
--(axis cs:80.6122448979592,0.00514317239763673)
--(axis cs:80.9523809523809,0.0050937234893659)
--(axis cs:81.2925170068027,0.00497559980706996)
--(axis cs:81.6326530612245,0.00472318830471611)
--(axis cs:81.9727891156463,0.00484283216393561)
--(axis cs:82.312925170068,0.00470524438575228)
--(axis cs:82.6530612244898,0.00469908871852624)
--(axis cs:82.9931972789116,0.00453217746911738)
--(axis cs:83.3333333333333,0.00435327973946103)
--(axis cs:83.6734693877551,0.0044312953275742)
--(axis cs:84.0136054421769,0.00437770249910755)
--(axis cs:84.3537414965986,0.00436456344338528)
--(axis cs:84.6938775510204,0.00397425805912639)
--(axis cs:85.0340136054422,0.00415461284301812)
--(axis cs:85.3741496598639,0.00413611165235086)
--(axis cs:85.7142857142857,0.00411612519009937)
--(axis cs:86.0544217687075,0.00410475720751414)
--(axis cs:86.3945578231292,0.00392040114698528)
--(axis cs:86.734693877551,0.00379220987931312)
--(axis cs:87.0748299319728,0.003754004775265)
--(axis cs:87.4149659863945,0.00369156161915786)
--(axis cs:87.7551020408163,0.00377272257502155)
--(axis cs:88.0952380952381,0.00363129045652939)
--(axis cs:88.4353741496599,0.00346027569486514)
--(axis cs:88.7755102040816,0.00355423314318157)
--(axis cs:89.1156462585034,0.0034645048487924)
--(axis cs:89.4557823129252,0.00341765587332638)
--(axis cs:89.7959183673469,0.00337133419600769)
--(axis cs:90.1360544217687,0.00326289275499413)
--(axis cs:90.4761904761905,0.00291380675857454)
--(axis cs:90.8163265306122,0.00294706632856744)
--(axis cs:91.156462585034,0.00297636005110885)
--(axis cs:91.4965986394558,0.0028857445277457)
--(axis cs:91.8367346938775,0.00279659977004966)
--(axis cs:92.1768707482993,0.00276459975772709)
--(axis cs:92.5170068027211,0.00263068128867455)
--(axis cs:92.8571428571429,0.00278252471798479)
--(axis cs:93.1972789115646,0.00263450342936519)
--(axis cs:93.5374149659864,0.00237868789758559)
--(axis cs:93.8775510204082,0.00222173426126659)
--(axis cs:94.2176870748299,0.00228088480343586)
--(axis cs:94.5578231292517,0.00209319549549431)
--(axis cs:94.8979591836735,0.00206267913284789)
--(axis cs:95.2380952380952,0.00196789226002794)
--(axis cs:95.578231292517,0.00202511794299831)
--(axis cs:95.9183673469388,0.00180974766989371)
--(axis cs:96.2585034013605,0.0017170259400594)
--(axis cs:96.5986394557823,0.00158716693666992)
--(axis cs:96.9387755102041,0.00141827932987074)
--(axis cs:97.2789115646258,0.00117825462039392)
--(axis cs:97.6190476190476,0.000812478123340717)
--(axis cs:97.9591836734694,0.000659057836814182)
--(axis cs:98.2993197278912,0.000335641399880063)
--(axis cs:98.6394557823129,0.000203264915175385)
--(axis cs:98.9795918367347,8.59766249220186e-05)
--(axis cs:99.3197278911565,4.75501821468383e-05)
--(axis cs:99.6598639455782,1.24805870367413e-05)
--(axis cs:100,1.36833646162385e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:100,1.61203504352189e-13)
--(axis cs:99.6598639455782,1.7380457426978e-05)
--(axis cs:99.3197278911565,6.27193315323615e-05)
--(axis cs:98.9795918367347,0.00011367332038254)
--(axis cs:98.6394557823129,0.000249906437757636)
--(axis cs:98.2993197278912,0.000414818408337866)
--(axis cs:97.9591836734694,0.000803635714953638)
--(axis cs:97.6190476190476,0.000973811326864157)
--(axis cs:97.2789115646258,0.00139371761374754)
--(axis cs:96.9387755102041,0.00166725241657913)
--(axis cs:96.5986394557823,0.00184478152976956)
--(axis cs:96.2585034013605,0.00202029881446582)
--(axis cs:95.9183673469388,0.00212752818882273)
--(axis cs:95.578231292517,0.00240217302643492)
--(axis cs:95.2380952380952,0.00235001770072317)
--(axis cs:94.8979591836735,0.00243265930026788)
--(axis cs:94.5578231292517,0.00247124392630862)
--(axis cs:94.2176870748299,0.00267301125408443)
--(axis cs:93.8775510204082,0.00264112904044339)
--(axis cs:93.5374149659864,0.00280659607925082)
--(axis cs:93.1972789115646,0.00306032061663882)
--(axis cs:92.8571428571429,0.00326230030719628)
--(axis cs:92.5170068027211,0.00306763114498828)
--(axis cs:92.1768707482993,0.00324622553999338)
--(axis cs:91.8367346938775,0.0032753759846209)
--(axis cs:91.4965986394558,0.00339304781050532)
--(axis cs:91.156462585034,0.00347994454915327)
--(axis cs:90.8163265306122,0.00339723244936998)
--(axis cs:90.4761904761905,0.00338646186638932)
--(axis cs:90.1360544217687,0.00381252576882159)
--(axis cs:89.7959183673469,0.0039572613583928)
--(axis cs:89.4557823129252,0.00397067803838493)
--(axis cs:89.1156462585034,0.0039995037388765)
--(axis cs:88.7755102040816,0.00406415512970995)
--(axis cs:88.4353741496599,0.00400586723937222)
--(axis cs:88.0952380952381,0.00420817175219706)
--(axis cs:87.7551020408163,0.0043854509715253)
--(axis cs:87.4149659863945,0.00428888733610846)
--(axis cs:87.0748299319728,0.00439430612532599)
--(axis cs:86.734693877551,0.00439779232020044)
--(axis cs:86.3945578231292,0.00458858965408775)
--(axis cs:86.0544217687075,0.00478352424645367)
--(axis cs:85.7142857142857,0.00477436618693747)
--(axis cs:85.3741496598639,0.00485556763195973)
--(axis cs:85.0340136054422,0.00481145553750088)
--(axis cs:84.6938775510204,0.00465961933912955)
--(axis cs:84.3537414965986,0.00506637318296816)
--(axis cs:84.0136054421769,0.00512920419102144)
--(axis cs:83.6734693877551,0.00513766407018364)
--(axis cs:83.3333333333333,0.00507317866958685)
--(axis cs:82.9931972789116,0.00525578727770899)
--(axis cs:82.6530612244898,0.00542858435052179)
--(axis cs:82.312925170068,0.00547212235576024)
--(axis cs:81.9727891156463,0.00568567973147628)
--(axis cs:81.6326530612245,0.00550324512754605)
--(axis cs:81.2925170068027,0.00578287694925445)
--(axis cs:80.9523809523809,0.00593522112399894)
--(axis cs:80.6122448979592,0.00599582820968559)
--(axis cs:80.2721088435374,0.00625152637318488)
--(axis cs:79.9319727891156,0.00638004529821164)
--(axis cs:79.5918367346939,0.00641704788592866)
--(axis cs:79.2517006802721,0.0068582413498387)
--(axis cs:78.9115646258503,0.00686551253495605)
--(axis cs:78.5714285714286,0.00717955088426999)
--(axis cs:78.2312925170068,0.00748566349440465)
--(axis cs:77.891156462585,0.00780431593438263)
--(axis cs:77.5510204081633,0.00792938777953696)
--(axis cs:77.2108843537415,0.00812677147041952)
--(axis cs:76.8707482993197,0.0088508908742805)
--(axis cs:76.530612244898,0.00909562720321563)
--(axis cs:76.1904761904762,0.00941745848299988)
--(axis cs:75.8503401360544,0.0095367783397757)
--(axis cs:75.5102040816327,0.00969020354508808)
--(axis cs:75.1700680272109,0.00994501194684426)
--(axis cs:74.8299319727891,0.0105900779676253)
--(axis cs:74.4897959183673,0.0107026062227623)
--(axis cs:74.1496598639456,0.0114137413665953)
--(axis cs:73.8095238095238,0.0119144278628689)
--(axis cs:73.469387755102,0.0120850443280313)
--(axis cs:73.1292517006803,0.0121411639836085)
--(axis cs:72.7891156462585,0.0124157254527517)
--(axis cs:72.4489795918367,0.01269898219702)
--(axis cs:72.108843537415,0.0129349305374069)
--(axis cs:71.7687074829932,0.012161963030651)
--(axis cs:71.4285714285714,0.0126166698977722)
--(axis cs:71.0884353741497,0.0126753644983171)
--(axis cs:70.7482993197279,0.0125149647884775)
--(axis cs:70.4081632653061,0.0131006231785466)
--(axis cs:70.0680272108844,0.0132562051098907)
--(axis cs:69.7278911564626,0.0138211061863698)
--(axis cs:69.3877551020408,0.0142256396289538)
--(axis cs:69.0476190476191,0.0144182297310086)
--(axis cs:68.7074829931973,0.015235949557993)
--(axis cs:68.3673469387755,0.0152649837011509)
--(axis cs:68.0272108843537,0.0164765905653236)
--(axis cs:67.687074829932,0.0170302171265715)
--(axis cs:67.3469387755102,0.0178827774862455)
--(axis cs:67.0068027210884,0.0197358753868702)
--(axis cs:66.6666666666667,0.0194203674116428)
--(axis cs:66.3265306122449,0.0200876548384875)
--(axis cs:65.9863945578231,0.0211782269385667)
--(axis cs:65.6462585034014,0.0222293373655196)
--(axis cs:65.3061224489796,0.0237930081683014)
--(axis cs:64.9659863945578,0.025569139316857)
--(axis cs:64.6258503401361,0.0272213144286324)
--(axis cs:64.2857142857143,0.0284271395193024)
--(axis cs:63.9455782312925,0.0292489589193397)
--(axis cs:63.6054421768707,0.0312226829282713)
--(axis cs:63.265306122449,0.032186112183463)
--(axis cs:62.9251700680272,0.0338887709088299)
--(axis cs:62.5850340136054,0.0343007484375963)
--(axis cs:62.2448979591837,0.0370952422900481)
--(axis cs:61.9047619047619,0.03861954846782)
--(axis cs:61.5646258503401,0.0408170702106093)
--(axis cs:61.2244897959184,0.0426728881050929)
--(axis cs:60.8843537414966,0.0449138120836717)
--(axis cs:60.5442176870748,0.0461265755877457)
--(axis cs:60.2040816326531,0.0486656025200909)
--(axis cs:59.8639455782313,0.0500935359094618)
--(axis cs:59.5238095238095,0.053047513679043)
--(axis cs:59.1836734693878,0.0571448560408663)
--(axis cs:58.843537414966,0.0582893607277151)
--(axis cs:58.5034013605442,0.060739525905785)
--(axis cs:58.1632653061224,0.0634224966976244)
--(axis cs:57.8231292517007,0.0648616592458677)
--(axis cs:57.4829931972789,0.0681081195510322)
--(axis cs:57.1428571428571,0.0701565037288917)
--(axis cs:56.8027210884354,0.0744538421348733)
--(axis cs:56.4625850340136,0.0776323090549024)
--(axis cs:56.1224489795918,0.082578096690078)
--(axis cs:55.7823129251701,0.0857803923191941)
--(axis cs:55.4421768707483,0.0895308516891508)
--(axis cs:55.1020408163265,0.0923754289331472)
--(axis cs:54.7619047619048,0.0970933239513846)
--(axis cs:54.421768707483,0.100212664035106)
--(axis cs:54.0816326530612,0.103550162143286)
--(axis cs:53.7414965986395,0.104976581428843)
--(axis cs:53.4013605442177,0.111073701074513)
--(axis cs:53.0612244897959,0.115484906290493)
--(axis cs:52.7210884353741,0.120049703323842)
--(axis cs:52.3809523809524,0.122451537752737)
--(axis cs:52.0408163265306,0.12549852824775)
--(axis cs:51.7006802721088,0.127594869025721)
--(axis cs:51.3605442176871,0.131415735926693)
--(axis cs:51.0204081632653,0.136019536036536)
--(axis cs:50.6802721088435,0.138333541901853)
--(axis cs:50.3401360544218,0.142480341548286)
--(axis cs:50,0.145660177403007)
--(axis cs:49.6598639455782,0.147746233427972)
--(axis cs:49.3197278911565,0.151916922147403)
--(axis cs:48.9795918367347,0.156717590889555)
--(axis cs:48.6394557823129,0.159753004364905)
--(axis cs:48.2993197278912,0.163133355989677)
--(axis cs:47.9591836734694,0.166623257403346)
--(axis cs:47.6190476190476,0.170283325832547)
--(axis cs:47.2789115646259,0.175247972054653)
--(axis cs:46.9387755102041,0.178582183546323)
--(axis cs:46.5986394557823,0.182521486356347)
--(axis cs:46.2585034013605,0.185370657581981)
--(axis cs:45.9183673469388,0.188458638345953)
--(axis cs:45.578231292517,0.192746793283387)
--(axis cs:45.2380952380952,0.196617607075834)
--(axis cs:44.8979591836735,0.198505031985686)
--(axis cs:44.5578231292517,0.201288185344722)
--(axis cs:44.2176870748299,0.208042629611489)
--(axis cs:43.8775510204082,0.212986046005927)
--(axis cs:43.5374149659864,0.217190929928055)
--(axis cs:43.1972789115646,0.219313184816911)
--(axis cs:42.8571428571429,0.222240337670824)
--(axis cs:42.5170068027211,0.225937295191979)
--(axis cs:42.1768707482993,0.228423352231267)
--(axis cs:41.8367346938776,0.233411096170371)
--(axis cs:41.4965986394558,0.238661485058789)
--(axis cs:41.156462585034,0.239362336611641)
--(axis cs:40.8163265306122,0.243036958311638)
--(axis cs:40.4761904761905,0.24590585500744)
--(axis cs:40.1360544217687,0.250549657200225)
--(axis cs:39.7959183673469,0.252785877068294)
--(axis cs:39.4557823129252,0.257917233865918)
--(axis cs:39.1156462585034,0.26093578056109)
--(axis cs:38.7755102040816,0.261281597760949)
--(axis cs:38.4353741496599,0.266692538684813)
--(axis cs:38.0952380952381,0.268063660044844)
--(axis cs:37.7551020408163,0.269875732659504)
--(axis cs:37.4149659863946,0.273285207240426)
--(axis cs:37.0748299319728,0.275923856035263)
--(axis cs:36.734693877551,0.27559222928708)
--(axis cs:36.3945578231292,0.2794740437453)
--(axis cs:36.0544217687075,0.280106356035577)
--(axis cs:35.7142857142857,0.282392441602152)
--(axis cs:35.3741496598639,0.284661624798429)
--(axis cs:35.0340136054422,0.288817527107678)
--(axis cs:34.6938775510204,0.291607373361908)
--(axis cs:34.3537414965986,0.293354592761484)
--(axis cs:34.0136054421769,0.296135248879428)
--(axis cs:33.6734693877551,0.298724121473988)
--(axis cs:33.3333333333333,0.302341782076374)
--(axis cs:32.9931972789116,0.305996673064079)
--(axis cs:32.6530612244898,0.30732867298789)
--(axis cs:32.312925170068,0.311816810004887)
--(axis cs:31.9727891156463,0.313244527611429)
--(axis cs:31.6326530612245,0.315107071770676)
--(axis cs:31.2925170068027,0.319115601079406)
--(axis cs:30.952380952381,0.321490492313929)
--(axis cs:30.6122448979592,0.325859846985457)
--(axis cs:30.2721088435374,0.32859504717433)
--(axis cs:29.9319727891156,0.329502652745041)
--(axis cs:29.5918367346939,0.332821451858824)
--(axis cs:29.2517006802721,0.334855722530877)
--(axis cs:28.9115646258503,0.338231452261154)
--(axis cs:28.5714285714286,0.339670952999201)
--(axis cs:28.2312925170068,0.341189229550404)
--(axis cs:27.891156462585,0.344801796568698)
--(axis cs:27.5510204081633,0.348045242472183)
--(axis cs:27.2108843537415,0.349105135847855)
--(axis cs:26.8707482993197,0.352331470801745)
--(axis cs:26.530612244898,0.355257124212907)
--(axis cs:26.1904761904762,0.356167423086736)
--(axis cs:25.8503401360544,0.358829403558425)
--(axis cs:25.5102040816327,0.363042194058177)
--(axis cs:25.1700680272109,0.363665848449479)
--(axis cs:24.8299319727891,0.367705966201301)
--(axis cs:24.4897959183673,0.368410572985937)
--(axis cs:24.1496598639456,0.372886556316463)
--(axis cs:23.8095238095238,0.372243099620377)
--(axis cs:23.469387755102,0.375477999218396)
--(axis cs:23.1292517006803,0.375819899695542)
--(axis cs:22.7891156462585,0.376910747673735)
--(axis cs:22.4489795918367,0.380049836383936)
--(axis cs:22.108843537415,0.383301791190129)
--(axis cs:21.7687074829932,0.387888125371861)
--(axis cs:21.4285714285714,0.391310307629652)
--(axis cs:21.0884353741497,0.393749973298728)
--(axis cs:20.7482993197279,0.39779132543356)
--(axis cs:20.4081632653061,0.401856396316011)
--(axis cs:20.0680272108844,0.405699532376522)
--(axis cs:19.7278911564626,0.407164750176155)
--(axis cs:19.3877551020408,0.412864461585916)
--(axis cs:19.047619047619,0.417991992274028)
--(axis cs:18.7074829931973,0.423250240129672)
--(axis cs:18.3673469387755,0.42908062274268)
--(axis cs:18.0272108843537,0.436515352393939)
--(axis cs:17.687074829932,0.442903481970539)
--(axis cs:17.3469387755102,0.449074971330273)
--(axis cs:17.0068027210884,0.455143321466112)
--(axis cs:16.6666666666667,0.461164568889165)
--(axis cs:16.3265306122449,0.465162746646579)
--(axis cs:15.9863945578231,0.471637537432881)
--(axis cs:15.6462585034014,0.477131614482048)
--(axis cs:15.3061224489796,0.482231426375808)
--(axis cs:14.9659863945578,0.489052347772725)
--(axis cs:14.6258503401361,0.493520317777153)
--(axis cs:14.2857142857143,0.500546189149205)
--(axis cs:13.9455782312925,0.503295662818179)
--(axis cs:13.6054421768707,0.510940694073417)
--(axis cs:13.265306122449,0.51642448779796)
--(axis cs:12.9251700680272,0.526054456543699)
--(axis cs:12.5850340136054,0.529811834589813)
--(axis cs:12.2448979591837,0.535457214714462)
--(axis cs:11.9047619047619,0.539262365506624)
--(axis cs:11.5646258503401,0.546801624197012)
--(axis cs:11.2244897959184,0.549912258313246)
--(axis cs:10.8843537414966,0.555053159953633)
--(axis cs:10.5442176870748,0.563558447576355)
--(axis cs:10.2040816326531,0.572406223290404)
--(axis cs:9.86394557823129,0.578920158748692)
--(axis cs:9.52380952380952,0.581174820364137)
--(axis cs:9.18367346938775,0.585729752858832)
--(axis cs:8.84353741496599,0.588759031786688)
--(axis cs:8.50340136054422,0.595016288524429)
--(axis cs:8.16326530612245,0.600355369522143)
--(axis cs:7.82312925170068,0.604622444388895)
--(axis cs:7.48299319727891,0.608937056049226)
--(axis cs:7.14285714285714,0.613821086361804)
--(axis cs:6.80272108843537,0.617045246772894)
--(axis cs:6.46258503401361,0.62132719680155)
--(axis cs:6.12244897959184,0.625272216504198)
--(axis cs:5.78231292517007,0.628819101802728)
--(axis cs:5.4421768707483,0.635163999848239)
--(axis cs:5.10204081632653,0.642038155122735)
--(axis cs:4.76190476190476,0.644791676655598)
--(axis cs:4.42176870748299,0.648965240123969)
--(axis cs:4.08163265306122,0.658463643140004)
--(axis cs:3.74149659863946,0.667914875533303)
--(axis cs:3.40136054421769,0.671080814117345)
--(axis cs:3.06122448979592,0.677301017104361)
--(axis cs:2.72108843537415,0.683674725306122)
--(axis cs:2.38095238095238,0.689735332039763)
--(axis cs:2.04081632653061,0.695646996489406)
--(axis cs:1.70068027210884,0.703110473066972)
--(axis cs:1.36054421768707,0.707473838071249)
--(axis cs:1.02040816326531,0.712366920344287)
--(axis cs:0.680272108843537,0.717179155951947)
--(axis cs:0.340136054421769,0.721022222834812)
--(axis cs:0,0.720762681985969)
--cycle;


==> macros.tex <==
%==============================================================================
% ABBREVIATIONS
%------------------------------------------------------------------------------
\RequirePackage{amsmath,amsfonts,amssymb}
\RequirePackage{bbm}  
\RequirePackage{bm} 
\RequirePackage{mathtools}

% utility
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\renewcommand{\P}{\mathbb{P}}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\affspan}{aff}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\minimize}{minimize}
\DeclareMathOperator{\maximize}{maximize}
%\DeclareMathOperator{\subjectto}{subject~to}
\DeclareMathOperator{\subjectto}{s.t.}
\newcommand{\kron}{\otimes}
\newcommand{\hada}{\odot}

% mathbf
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}} 
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}} 
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}
\newcommand{\bfone}{\mathbf{1}}
\newcommand{\bfzero}{\mathbf{0}}

% mathcal
\newcommand{\CA}{\mathcal{A}}     
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CD}{\mathcal{D}}
\newcommand{\CE}{\mathcal{E}}     
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CI}{\mathcal{I}} 
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CM}{\mathcal{M}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CO}{\mathcal{O}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CQ}{\mathcal{Q}}
\newcommand{\CR}{\mathcal{R}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CW}{\mathcal{W}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\CZ}{\mathcal{Z}}

% bm
\newcommand{\bfmu}{\bm{\mu}}
\newcommand{\bfsigma}{\bm{\sigma}}
\newcommand{\bfSigma}{\bm{\Sigma}}
\newcommand{\bflambda}{\bm{\lambda}}
\newcommand{\bfLambda}{\bm{\Lambda}}
\newcommand{\bfeta}{\bm{\eta}}
\newcommand{\bftheta}{\bm{\theta}}
\newcommand{\bfTheta}{\bm{\Theta}}
\newcommand{\bfpi}{\bm{\pi}}
\newcommand{\bfPi}{\bm{\Pi}}

% algorithmic
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}
\algrenewcommand\algorithmiccomment[1]{\hfill\textcolor{gray}{$\triangleright$ #1}}

